Estimating the Adversarial Robustness of Attributions in Text with Transformers

Explanations are crucial parts of deep neural network (DNN) classifiers. In high stakes applications, faithful and robust explanations are important to understand and gain trust in DNN classifiers. However, recent work has shown that state-of-the-art attribution methods in text classifiers are susceptible to imperceptible adversarial perturbations that alter explanations significantly while maintaining the correct prediction outcome. If undetected, this can critically mislead the users of DNNs. Thus, it is crucial to understand the influence of such adversarial perturbations on the networks' explanations and their perceptibility. In this work, we establish a novel definition of attribution robustness (AR) in text classification, based on Lipschitz continuity. Crucially, it reflects both attribution change induced by adversarial input alterations and perceptibility of such alterations. Moreover, we introduce a wide set of text similarity measures to effectively capture locality between two text samples and imperceptibility of adversarial perturbations in text. We then propose our novel TransformerExplanationAttack (TEA), a strong adversary that provides a tight estimation for attribution robustness in text classification. TEA uses state-of-the-art language models to extract word substitutions that result in fluent, contextual adversarial samples. Finally, with experiments on several text classification architectures, we show that TEA consistently outperforms current state-of-the-art AR estimators, yielding perturbations that alter explanations to a greater extent while being more fluent and less perceptible.

==> data/mlm_plots/auc_files/agnews_aucs.tex <==
x	orig_pp	orig_ge	et_use	et_tse	et_p_l2	et_p_h	et_p	et_ce	attack	adv_pp	adv_ge
0	65.78	2.4	0.51	0.49	1.32	1.03	0.16	0.96	tef	142.07	2.61
0	66.31	2.39	0.69	0.64	2.3	1.85	0.34	1.34	tef	140.24	2.54
0	65.97	2.37	0.86	0.78	2.52	2.01	0.4	1.86	tef	145.71	2.54
0	66.33	2.38	0.92	0.81	2.92	2.36	0.42	1.94	tef	140.8	2.51
0	65.81	2.38	0.88	0.83	2.34	1.9	0.35	1.86	tef	145.25	2.54
0	66.12	2.38	0.96	0.9	2.92	2.37	0.44	2.07	tef	140.46	2.52
0	66.02	2.37	1.12	1.04	3.29	2.69	0.46	2.27	tef	144.78	2.52
0	70.95	2.24	0.79	0.77	2.09	1.7	0.33	1.51	tef	161.77	2.4
0	70.52	2.25	1.4	1.36	4.01	3.27	0.58	2.89	tef	151.17	2.38
0	70.82	2.25	0.9	0.85	2.47	2.02	0.4	1.8	tef	158.58	2.4
0	51.22	1.34	0.8	0.82	1.76	1.36	0.19	1.98	tef	119.42	1.48
0	51.53	1.34	1.68	1.69	4.22	3.3	0.72	4.33	tef	106.21	1.46
0	51.61	1.34	0.78	0.77	1.82	1.45	0.23	1.85	tef	112.66	1.48
0	55.96	1.23	0.7	0.7	2.22	1.65	0.34	1.6	tef	119.79	1.34
0	55.47	1.22	1.28	1.26	4.17	2.99	0.64	2.89	tef	112.15	1.33
0	55.97	1.23	0.74	0.71	2.52	1.87	0.34	1.67	tef	113.58	1.32
1	65.4	2.52	0.76	0.89	1.51	1.17	0.35	1.41	mlm	116.19	2.35
1	65.36	2.51	1.01	1.06	3.02	2.46	1.19	1.76	mlm	93.51	2.3
1	65.55	2.53	0.98	1.04	2.23	1.86	0.81	1.81	mlm	103.76	2.44
1	65.54	2.52	1.11	1.1	3.16	2.66	1.53	1.83	mlm	95.03	2.38
1	65.26	2.51	0.98	1.06	2.28	1.81	0.83	1.9	mlm	105.01	2.4
1	65.1	2.51	1.07	1.13	3.08	2.57	1.29	1.83	mlm	95.24	2.35
1	65.26	2.5	1.16	1.21	3.3	2.71	1.31	1.96	mlm	96.05	2.34
1	70.23	2.41	0.93	1.06	1.83	1.58	0.75	1.8	mlm	111.37	2.41
1	70.23	2.42	1.62	1.82	3.68	3.16	1.74	3.04	mlm	107.68	2.3
1	70.23	2.41	1.14	1.28	2.53	2.1	1.01	2.13	mlm	105.86	2.32
1	50.02	1.3	0.93	1.1	1.41	1.21	0.35	1.77	mlm	93.97	1.45
1	49.65	1.3	1.77	2.08	3.45	2.83	1.25	3.55	mlm	80.57	1.37
1	49.63	1.3	1.13	1.28	2.04	1.83	0.83	2.2	mlm	80.26	1.34
1	54.27	1.19	0.93	1.07	2.31	1.66	0.55	1.82	mlm	93.75	1.24
1	54.54	1.2	1.42	1.58	3.85	2.88	1.34	2.59	mlm	86.57	1.19
1	54.1	1.19	0.96	1.0	2.73	2.12	0.92	1.77	mlm	87.77	1.11
2	65.22	2.52	0.79	0.93	1.58	1.25	0.31	1.52	mlm_distil	125.47	2.38
2	65.37	2.51	0.99	1.03	3.01	2.47	1.05	1.67	mlm_distil	98.95	2.33
2	65.72	2.53	0.98	1.02	2.3	1.91	0.8	1.86	mlm_distil	111.01	2.45
2	65.43	2.52	1.12	1.09	3.21	2.72	1.46	1.86	mlm_distil	98.56	2.41
2	65.13	2.51	0.99	1.07	2.4	1.86	0.69	1.96	mlm_distil	112.95	2.42
2	64.91	2.51	1.08	1.12	3.15	2.6	1.15	1.82	mlm_distil	99.57	2.37
2	65.19	2.5	1.17	1.2	3.3	2.75	1.23	1.96	mlm_distil	101.24	2.36
2	70.43	2.41	0.89	1.01	1.86	1.59	0.66	1.68	mlm_distil	120.86	2.36
2	70.29	2.41	1.58	1.75	3.71	3.13	1.16	2.83	mlm_distil	113.91	2.3
2	70.02	2.41	1.11	1.23	2.6	2.11	1.02	2.03	mlm_distil	112.21	2.29
2	49.98	1.3	0.88	1.04	1.53	1.25	0.35	1.57	mlm_distil	99.84	1.39
2	49.43	1.29	1.74	2.04	3.59	2.92	1.41	3.4	mlm_distil	83.23	1.34
2	49.79	1.29	1.07	1.2	2.13	1.81	0.67	2.02	mlm_distil	85.43	1.32
2	54.2	1.19	0.88	1.0	2.09	1.59	0.59	1.72	mlm_distil	98.58	1.19
2	54.97	1.2	1.36	1.48	3.81	2.93	1.27	2.56	mlm_distil	89.82	1.16
2	53.84	1.19	0.93	0.97	2.56	2.05	0.97	1.7	mlm_distil	91.73	1.09
3	65.52	2.52	0.76	0.89	1.55	1.18	0.4	1.41	mlm_fast	119.38	2.39
3	65.47	2.51	1.0	1.06	3.02	2.39	1.23	1.76	mlm_fast	95.61	2.33
3	65.39	2.53	0.99	1.04	2.19	1.83	0.83	1.84	mlm_fast	106.51	2.47
3	65.57	2.52	1.12	1.11	3.15	2.62	1.32	1.94	mlm_fast	98.2	2.39
3	65.01	2.51	0.98	1.07	2.26	1.76	0.8	1.96	mlm_fast	106.59	2.45
3	65.17	2.51	1.07	1.13	3.06	2.54	1.0	1.87	mlm_fast	97.28	2.37
3	65.18	2.5	1.17	1.23	3.16	2.61	1.26	1.98	mlm_fast	98.42	2.37
3	70.43	2.41	0.94	1.06	1.8	1.55	0.76	1.77	mlm_fast	113.26	2.44
3	70.33	2.42	1.63	1.83	3.59	3.05	1.3	3.01	mlm_fast	112.26	2.33
3	69.71	2.41	1.15	1.29	2.53	2.08	1.03	2.18	mlm_fast	106.83	2.36
3	50.06	1.3	0.95	1.13	1.43	1.22	0.34	1.81	mlm_fast	98.99	1.48
3	49.53	1.3	1.79	2.13	3.32	2.78	1.26	3.64	mlm_fast	83.83	1.4
3	49.53	1.3	1.15	1.32	2.03	1.81	0.8	2.2	mlm_fast	82.96	1.35
3	54.18	1.2	0.95	1.1	2.31	1.6	0.63	1.84	mlm_fast	96.28	1.27
3	54.04	1.2	1.45	1.62	3.7	2.82	1.16	2.72	mlm_fast	88.08	1.19
3	54.08	1.19	0.98	1.02	2.73	2.14	0.94	1.83	mlm_fast	89.06	1.12
4	65.27	2.52	0.79	0.93	1.61	1.25	0.31	1.53	mlm_distil_fast	128.63	2.39
4	65.53	2.51	1.0	1.04	2.99	2.42	0.98	1.73	mlm_distil_fast	101.14	2.34
4	65.46	2.53	0.99	1.03	2.32	1.88	0.74	1.85	mlm_distil_fast	114.72	2.47
4	65.62	2.52	1.13	1.09	3.23	2.71	1.11	1.86	mlm_distil_fast	101.56	2.41
4	65.15	2.51	0.98	1.07	2.37	1.85	0.72	1.99	mlm_distil_fast	114.51	2.44
4	65.12	2.5	1.07	1.11	3.21	2.63	1.21	1.82	mlm_distil_fast	101.01	2.38
4	65.18	2.5	1.16	1.19	3.26	2.72	1.08	1.95	mlm_distil_fast	104.51	2.37
4	70.35	2.41	0.91	1.02	1.89	1.6	0.62	1.73	mlm_distil_fast	122.09	2.39
4	70.05	2.42	1.58	1.75	3.6	3.04	1.13	2.89	mlm_distil_fast	118.0	2.32
4	70.16	2.41	1.11	1.23	2.56	2.06	0.94	2.1	mlm_distil_fast	115.72	2.33
4	49.85	1.3	0.9	1.05	1.54	1.26	0.34	1.59	mlm_distil_fast	103.2	1.41
4	49.4	1.3	1.73	2.04	3.36	2.84	1.23	3.49	mlm_distil_fast	86.04	1.37
4	49.71	1.29	1.09	1.22	2.03	1.81	0.78	2.08	mlm_distil_fast	86.89	1.34
4	54.44	1.19	0.88	0.99	2.09	1.58	0.59	1.63	mlm_distil_fast	100.91	1.2
4	55.0	1.2	1.36	1.49	3.75	2.85	1.25	2.49	mlm_distil_fast	93.44	1.17
4	54.11	1.19	0.94	0.98	2.64	2.07	0.79	1.72	mlm_distil_fast	94.46	1.1


==> data/mlm_plots/auc_files/fakenews_aucs.tex <==
x	orig_pp	orig_ge	et_use	et_tse	et_p_l2	et_p_h	et_p	et_ce	attack	adv_pp	adv_ge
0	17.22	25.96	0.48	0.45	0.5	0.55	0.06	0.53	tef	46.6	28.16
0	17.16	25.87	0.58	0.55	0.57	0.64	0.08	0.57	tef	44.73	27.93
0	17.41	25.84	1.29	1.22	1.03	1.11	0.13	1.28	tef	48.61	27.93
0	17.06	25.78	1.07	1.01	0.77	0.9	0.11	0.94	tef	45.69	27.64
0	16.85	26.08	1.1	1.03	0.84	0.93	0.12	1.0	tef	45.7	28.2
0	16.73	26.11	0.9	0.85	0.63	0.73	0.09	0.77	tef	44.31	28.2
0	16.5	26.23	1.07	0.99	0.8	0.93	0.12	0.95	tef	44.76	28.64
0	17.52	24.46	1.21	1.18	1.06	1.22	0.16	1.39	tef	48.49	25.55
0	17.22	24.56	2.44	2.34	1.99	2.37	0.35	2.6	tef	48.52	25.78
0	18.3	24.56	1.01	0.96	0.84	0.97	0.13	1.05	tef	51.38	25.85
0	22.37	9.78	1.31	1.35	0.98	1.11	0.19	1.63	tef	54.4	10.61
0	17.37	11.14	2.31	2.41	1.75	2.05	0.3	2.72	tef	39.18	12.2
0	15.09	11.5	0.87	0.86	0.61	0.72	0.1	0.88	tef	37.02	12.54
0	30.4	7.39	1.41	1.48	1.53	1.5	0.26	2.03	tef	66.73	7.9
0	18.22	9.45	2.13	2.2	1.88	2.06	0.31	2.7	tef	40.68	10.38
0	15.82	10.58	1.25	1.23	0.96	1.11	0.14	1.44	tef	41.29	11.87
1	16.45	25.86	1.21	0.86	0.81	0.87	0.19	0.78	mlm	34.29	24.33
1	16.62	25.85	2.44	1.7	1.82	1.97	0.84	1.41	mlm	30.48	24.26
1	16.73	25.78	1.92	1.39	1.1	1.26	0.3	1.05	mlm	33.08	24.58
1	16.56	25.73	3.01	2.07	2.01	2.28	0.74	1.65	mlm	29.62	24.98
1	16.0	26.09	1.84	1.17	1.25	1.37	0.45	0.91	mlm	28.84	24.88
1	16.43	26.0	2.77	1.73	1.88	2.18	0.78	1.48	mlm	28.4	25.05
1	15.69	26.93	2.17	1.4	1.46	1.65	0.62	1.19	mlm	27.16	25.61
1	16.99	24.61	1.91	1.39	1.1	1.31	0.36	1.02	mlm	34.59	23.74
1	19.07	24.81	3.64	2.66	2.61	2.45	0.65	1.9	mlm	36.63	24.3
1	17.31	24.51	1.81	1.22	1.04	1.23	0.35	0.94	mlm	34.65	23.37
1	17.9	10.34	1.76	1.74	1.04	1.22	0.27	1.17	mlm	40.37	11.32
1	14.94	11.57	2.96	2.52	1.79	2.14	0.54	1.7	mlm	27.32	12.07
1	14.92	11.58	1.78	1.14	1.14	1.34	0.38	0.78	mlm	27.83	12.32
1	19.82	9.52	1.88	2.03	2.61	1.49	0.31	1.21	mlm	42.49	9.74
1	14.65	10.43	2.86	2.74	1.78	2.08	0.49	1.61	mlm	29.22	10.71
1	15.17	10.61	1.9	1.79	1.19	1.37	0.29	0.97	mlm	32.3	11.42
2	16.77	25.84	1.19	0.89	0.85	0.9	0.16	0.82	mlm_distil	39.05	24.2
2	16.74	25.93	2.32	1.66	1.72	1.92	0.58	1.4	mlm_distil	33.05	24.21
2	17.17	25.67	1.88	1.41	1.14	1.27	0.28	1.08	mlm_distil	36.96	24.26
2	16.95	25.8	3.03	2.15	2.04	2.29	0.73	1.73	mlm_distil	32.28	24.57
2	16.2	26.1	1.86	1.26	1.23	1.37	0.37	1.01	mlm_distil	31.23	24.9
2	16.02	26.02	2.81	1.91	1.94	2.19	0.66	1.63	mlm_distil	30.62	24.92
2	16.42	26.11	2.17	1.52	1.47	1.65	0.53	1.28	mlm_distil	30.82	25.26
2	16.95	24.67	1.84	1.38	1.08	1.29	0.31	1.05	mlm_distil	36.87	23.48
2	16.71	24.65	3.53	2.65	1.98	2.36	0.55	1.88	mlm_distil	37.23	23.54
2	17.26	24.53	1.75	1.21	1.06	1.23	0.28	0.95	mlm_distil	37.45	23.28
2	17.07	10.11	1.66	1.64	1.05	1.24	0.27	1.08	mlm_distil	36.52	10.82
2	14.5	11.63	2.9	2.54	1.78	2.12	0.51	1.87	mlm_distil	28.44	11.99
2	15.05	11.61	1.82	1.34	1.15	1.33	0.38	0.97	mlm_distil	28.86	12.19
2	18.6	9.22	1.77	1.81	1.11	1.34	0.3	1.23	mlm_distil	45.51	9.38
2	15.23	10.86	2.85	2.79	1.74	2.07	0.45	1.62	mlm_distil	31.33	11.06
2	15.51	10.57	1.86	1.83	1.18	1.34	0.3	1.02	mlm_distil	33.39	10.97
3	16.92	26.04	1.26	0.89	0.82	0.89	0.2	0.79	mlm_fast	36.19	24.96
3	16.76	26.0	2.36	1.66	1.68	1.83	0.63	1.4	mlm_fast	32.34	24.75
3	17.01	25.91	1.98	1.41	1.14	1.26	0.3	1.09	mlm_fast	34.53	25.82
3	16.88	25.89	3.0	1.99	1.97	2.19	0.65	1.7	mlm_fast	32.18	25.9
3	16.69	26.21	1.88	1.16	1.25	1.36	0.41	0.99	mlm_fast	31.11	26.27
3	17.07	26.0	2.79	1.73	1.88	2.06	0.71	1.55	mlm_fast	30.97	26.26
3	16.54	26.21	2.23	1.42	1.45	1.62	0.58	1.29	mlm_fast	28.79	25.98
3	17.1	24.63	1.88	1.42	1.07	1.28	0.36	1.02	mlm_fast	37.27	24.39
3	18.91	24.61	3.67	2.63	2.48	2.37	0.55	1.9	mlm_fast	39.17	24.79
3	18.09	24.55	1.86	1.24	1.1	1.24	0.31	0.96	mlm_fast	36.49	24.13
3	17.45	10.36	1.82	1.79	1.03	1.21	0.25	1.15	mlm_fast	37.34	11.77
3	15.13	11.53	3.07	2.56	1.75	2.06	0.52	1.71	mlm_fast	30.74	12.8
3	15.2	11.57	1.89	1.19	1.15	1.33	0.35	0.84	mlm_fast	30.27	12.75
3	23.6	8.98	1.91	2.03	2.72	1.48	0.31	1.28	mlm_fast	51.12	9.4
3	15.7	10.53	2.84	2.93	1.8	2.08	0.42	1.58	mlm_fast	32.1	10.88
3	15.36	10.61	1.92	1.84	1.17	1.35	0.28	0.97	mlm_fast	33.99	11.92
4	17.26	25.93	1.22	0.9	0.85	0.91	0.2	0.83	mlm_distil_fast	41.22	24.72
4	16.78	26.0	2.24	1.62	1.64	1.8	0.49	1.44	mlm_distil_fast	35.85	24.66
4	16.95	25.83	1.83	1.38	1.08	1.21	0.25	1.11	mlm_distil_fast	38.99	25.55
4	17.01	25.73	2.89	2.09	1.86	2.07	0.66	1.79	mlm_distil_fast	34.01	25.41
4	16.43	26.2	1.79	1.25	1.18	1.31	0.4	1.08	mlm_distil_fast	32.07	26.6
4	16.77	26.15	2.6	1.81	1.81	1.99	0.6	1.64	mlm_distil_fast	31.94	26.58
4	16.65	26.23	2.13	1.52	1.43	1.57	0.51	1.39	mlm_distil_fast	31.15	26.74
4	17.08	24.71	1.81	1.4	1.06	1.26	0.3	1.06	mlm_distil_fast	40.17	24.03
4	16.54	24.74	3.47	2.65	1.89	2.24	0.5	1.95	mlm_distil_fast	39.71	24.42
4	18.21	24.55	1.76	1.25	1.06	1.21	0.26	1.0	mlm_distil_fast	40.13	23.8
4	17.59	10.29	1.72	1.71	1.06	1.24	0.25	1.14	mlm_distil_fast	38.37	11.17
4	15.04	11.36	2.75	2.49	1.68	1.99	0.46	1.81	mlm_distil_fast	32.74	12.34
4	15.16	11.57	1.78	1.26	1.12	1.29	0.35	0.93	mlm_distil_fast	31.11	12.92
4	19.16	9.64	1.85	1.91	1.11	1.32	0.26	1.26	mlm_distil_fast	47.35	10.03
4	16.02	10.43	2.8	2.83	1.74	2.05	0.43	1.59	mlm_distil_fast	33.27	10.88
4	15.55	10.61	1.87	1.83	1.17	1.33	0.29	1.02	mlm_distil_fast	35.71	11.55


==> data/mlm_plots/auc_files/imdb_aucs.tex <==
x	orig_pp	orig_ge	et_use	et_tse	et_p_l2	et_p_h	et_p	et_ce	attack	adv_pp	adv_ge
0	23.07	11.73	0.54	0.51	0.82	0.89	0.1	0.68	tef	55.78	12.81
0	23.04	11.75	1.13	1.08	1.86	1.98	0.3	1.43	tef	54.77	12.61
0	22.97	11.68	0.8	0.77	1.2	1.3	0.16	1.0	tef	57.63	12.69
0	22.93	11.68	1.17	1.12	1.82	1.95	0.27	1.53	tef	56.77	12.62
0	23.07	11.74	0.89	0.84	1.31	1.42	0.18	1.07	tef	58.17	12.76
0	23.06	11.73	1.34	1.28	2.0	2.14	0.28	1.68	tef	56.49	12.64
0	23.08	11.74	0.95	0.89	1.45	1.56	0.19	1.11	tef	58.13	12.75
0	23.7	11.8	1.22	1.18	1.73	1.91	0.29	1.85	tef	58.95	12.32
0	21.85	12.07	1.57	1.5	2.27	2.52	0.39	2.36	tef	55.49	12.65
0	21.88	12.01	1.13	1.06	1.7	1.85	0.28	1.56	tef	56.74	12.6
0	18.66	5.74	0.94	0.97	1.15	1.3	0.15	1.47	tef	43.29	6.42
0	18.59	5.76	1.48	1.51	1.69	1.89	0.28	2.26	tef	44.15	6.46
0	18.57	5.75	0.76	0.75	0.97	1.09	0.12	1.04	tef	43.35	6.48
0	18.73	5.45	0.89	0.87	1.19	1.3	0.18	1.27	tef	43.4	6.14
0	18.73	5.47	1.62	1.6	2.17	2.38	0.32	2.26	tef	42.31	6.15
0	18.72	5.47	0.88	0.85	1.11	1.24	0.16	1.2	tef	44.93	6.21
1	23.13	11.76	0.82	0.79	0.83	0.89	0.16	0.81	mlm	48.58	10.96
1	23.07	11.77	1.55	1.55	1.9	2.03	0.55	1.31	mlm	42.25	10.96
1	23.01	11.71	1.14	1.16	1.17	1.27	0.29	1.04	mlm	44.92	11.06
1	23.01	11.69	1.7	1.67	2.22	2.4	0.87	1.24	mlm	39.86	11.18
1	23.06	11.76	1.23	1.19	1.28	1.36	0.29	1.06	mlm	44.5	11.13
1	23.12	11.74	1.8	1.76	2.29	2.46	0.81	1.36	mlm	39.75	11.25
1	23.06	11.75	1.22	1.19	1.5	1.59	0.46	1.0	mlm	41.41	11.21
1	21.82	12.02	1.54	1.48	1.47	1.64	0.58	1.67	mlm	42.99	11.38
1	21.72	12.11	2.07	1.95	2.11	2.35	0.88	1.96	mlm	41.56	11.47
1	21.72	12.11	1.38	1.31	1.48	1.63	0.61	1.3	mlm	42.15	11.49
1	18.57	5.76	1.21	1.29	1.11	1.25	0.26	1.14	mlm	37.48	5.99
1	18.63	5.76	1.92	1.77	1.81	1.99	0.5	1.55	mlm	33.85	6.08
1	18.65	5.75	1.25	1.17	1.29	1.43	0.3	0.99	mlm	36.13	5.86
1	18.85	5.45	1.2	1.1	1.23	1.35	0.31	1.07	mlm	37.59	5.57
1	18.64	5.48	1.97	1.79	2.13	2.34	0.58	1.63	mlm	35.65	5.47
1	18.79	5.47	1.47	1.23	1.57	1.73	0.51	1.13	mlm	35.69	5.38
2	23.05	11.76	0.83	0.8	0.87	0.93	0.14	0.83	mlm_distil	54.28	10.83
2	23.1	11.75	1.55	1.55	1.98	2.09	0.56	1.39	mlm_distil	45.47	10.87
2	22.96	11.7	1.14	1.15	1.21	1.29	0.25	1.03	mlm_distil	49.36	10.86
2	23.0	11.69	1.71	1.7	2.3	2.47	0.77	1.31	mlm_distil	42.95	11.03
2	23.09	11.74	1.22	1.2	1.3	1.36	0.23	1.1	mlm_distil	49.36	10.87
2	23.11	11.73	1.81	1.78	2.33	2.49	0.69	1.41	mlm_distil	43.01	11.13
2	23.12	11.74	1.2	1.18	1.49	1.58	0.4	1.02	mlm_distil	45.48	10.98
2	21.83	12.02	1.47	1.43	1.49	1.65	0.56	1.57	mlm_distil	45.09	11.25
2	21.66	12.12	2.02	1.88	2.12	2.35	0.77	1.89	mlm_distil	44.17	11.38
2	21.67	12.1	1.33	1.26	1.49	1.63	0.6	1.26	mlm_distil	45.1	11.4
2	18.58	5.75	1.17	1.24	1.1	1.24	0.24	1.11	mlm_distil	39.59	5.84
2	18.59	5.75	1.92	1.87	1.84	2.02	0.46	1.62	mlm_distil	35.81	5.9
2	18.59	5.75	1.22	1.13	1.27	1.41	0.26	0.96	mlm_distil	38.21	5.73
2	18.8	5.45	1.16	1.07	1.23	1.33	0.3	1.04	mlm_distil	40.17	5.43
2	18.82	5.46	1.96	1.79	2.14	2.35	0.52	1.66	mlm_distil	37.82	5.32
2	18.78	5.46	1.44	1.22	1.57	1.71	0.47	1.11	mlm_distil	38.13	5.24
3	23.15	11.76	0.83	0.8	0.82	0.89	0.15	0.81	mlm_fast	49.83	11.09
3	23.1	11.77	1.54	1.53	1.83	1.95	0.51	1.31	mlm_fast	44.36	11.25
3	23.0	11.73	1.16	1.16	1.16	1.25	0.28	1.01	mlm_fast	46.27	11.68
3	22.98	11.69	1.65	1.6	2.08	2.24	0.73	1.2	mlm_fast	42.23	11.64
3	23.09	11.76	1.26	1.19	1.26	1.34	0.27	1.08	mlm_fast	46.24	11.84
3	23.13	11.73	1.74	1.65	2.13	2.28	0.74	1.31	mlm_fast	42.2	11.72
3	23.1	11.76	1.25	1.2	1.45	1.55	0.41	1.0	mlm_fast	43.06	11.83
3	21.67	12.07	1.51	1.45	1.44	1.61	0.5	1.61	mlm_fast	45.05	11.63
3	21.7	12.1	2.03	1.9	2.01	2.23	0.79	1.9	mlm_fast	44.73	11.77
3	21.69	12.1	1.39	1.31	1.46	1.6	0.57	1.27	mlm_fast	44.47	11.63
3	18.59	5.75	1.24	1.29	1.11	1.24	0.24	1.13	mlm_fast	39.8	6.17
3	18.62	5.75	1.9	1.66	1.7	1.86	0.42	1.48	mlm_fast	37.12	6.72
3	18.62	5.75	1.27	1.17	1.26	1.4	0.26	1.0	mlm_fast	38.6	6.19
3	18.81	5.46	1.23	1.11	1.22	1.33	0.29	1.08	mlm_fast	39.82	5.84
3	18.78	5.49	1.98	1.78	2.1	2.28	0.52	1.65	mlm_fast	38.61	5.73
3	18.77	5.47	1.47	1.2	1.54	1.69	0.47	1.14	mlm_fast	38.35	5.73
4	23.09	11.76	0.84	0.8	0.87	0.93	0.13	0.84	mlm_distil_fast	56.51	10.96
4	23.09	11.75	1.55	1.54	1.93	2.03	0.48	1.36	mlm_distil_fast	48.53	11.08
4	23.03	11.7	1.13	1.13	1.19	1.27	0.25	1.02	mlm_distil_fast	52.05	11.31
4	22.99	11.7	1.65	1.6	2.17	2.32	0.63	1.24	mlm_distil_fast	46.77	11.47
4	23.09	11.74	1.22	1.18	1.28	1.34	0.23	1.11	mlm_distil_fast	51.81	11.43
4	23.12	11.73	1.74	1.67	2.19	2.34	0.59	1.37	mlm_distil_fast	46.65	11.51
4	23.11	11.74	1.21	1.18	1.45	1.54	0.4	1.02	mlm_distil_fast	48.03	11.42
4	21.74	12.03	1.46	1.41	1.45	1.61	0.48	1.53	mlm_distil_fast	48.9	11.44
4	21.7	12.11	2.0	1.87	2.05	2.26	0.7	1.85	mlm_distil_fast	48.16	11.58
4	21.66	12.1	1.33	1.25	1.46	1.6	0.52	1.25	mlm_distil_fast	48.16	11.56
4	18.59	5.74	1.18	1.24	1.1	1.24	0.21	1.11	mlm_distil_fast	42.32	6.0
4	18.62	5.75	1.9	1.81	1.76	1.94	0.42	1.6	mlm_distil_fast	39.76	6.44
4	18.61	5.75	1.22	1.12	1.26	1.38	0.25	0.97	mlm_distil_fast	40.83	6.06
4	18.79	5.45	1.18	1.07	1.22	1.32	0.28	1.07	mlm_distil_fast	42.94	5.63
4	18.77	5.48	1.94	1.77	2.11	2.28	0.46	1.64	mlm_distil_fast	40.59	5.54
4	18.73	5.47	1.45	1.21	1.53	1.67	0.42	1.13	mlm_distil_fast	41.37	5.55


==> data/mlm_plots/auc_files/mr_aucs.tex <==
x	orig_pp	orig_ge	et_use	et_tse	et_p_l2	et_p_h	et_p	et_ce	attack	adv_pp	adv_ge
0	70.8	1.15	0.72	0.75	8.5	3.96	0.69	2.43	tef	139.24	1.25
0	65.23	1.22	0.75	0.8	6.42	3.62	0.71	2.15	tef	128.85	1.34
0	68.73	1.23	0.79	0.83	8.09	3.96	0.86	2.66	tef	133.37	1.36
0	68.62	1.23	1.08	1.14	9.31	5.01	1.03	3.77	tef	130.02	1.34
0	61.0	1.1	0.47	0.49	4.1	1.9	0.32	1.44	tef	129.09	1.23
0	61.17	1.11	0.58	0.61	5.14	2.59	0.48	1.63	tef	123.78	1.21
0	60.44	1.1	0.41	0.42	2.97	1.82	0.29	1.09	tef	122.62	1.22
0	64.3	1.03	0.53	0.56	4.11	2.22	0.41	1.8	tef	132.48	1.14
0	61.89	1.03	0.84	0.89	6.58	3.64	0.58	2.84	tef	130.82	1.12
0	62.93	1.03	0.52	0.54	3.75	2.15	0.3	1.62	tef	136.43	1.15
0	32.19	0.45	0.53	0.6	2.76	1.67	0.26	1.76	tef	74.37	0.54
0	33.36	0.45	0.94	1.03	5.17	3.3	0.73	3.41	tef	67.38	0.54
0	33.03	0.45	0.44	0.48	2.41	1.4	0.19	1.42	tef	77.46	0.55
0	34.99	0.42	0.44	0.48	2.65	1.63	0.39	1.45	tef	79.06	0.5
0	34.63	0.42	0.75	0.79	4.74	2.94	0.49	2.41	tef	74.41	0.5
0	33.99	0.41	0.51	0.54	3.2	1.95	0.32	1.66	tef	74.73	0.51
1	83.12	1.1	0.83	1.0	9.85	4.12	1.03	2.37	mlm	124.45	1.09
1	66.83	1.24	0.85	1.02	5.59	3.11	1.7	2.24	mlm	100.46	1.2
1	70.86	1.27	0.82	1.04	5.57	2.93	1.1	2.62	mlm	118.45	1.2
1	69.3	1.26	1.15	1.43	7.38	4.24	2.38	3.2	mlm	97.57	1.23
1	61.51	1.15	0.6	0.76	2.91	1.53	0.36	1.8	mlm	119.94	1.11
1	61.29	1.15	0.71	0.86	5.34	2.67	0.95	1.5	mlm	94.32	1.12
1	61.15	1.15	0.62	0.68	3.66	2.3	0.96	1.22	mlm	92.07	1.14
1	64.01	1.07	0.71	0.86	3.19	1.81	0.59	2.25	mlm	111.43	1.07
1	63.38	1.07	0.97	1.16	5.27	2.89	1.06	2.63	mlm	101.44	1.06
1	62.77	1.07	0.94	1.14	4.84	2.6	0.76	3.44	mlm	109.45	0.92
1	33.18	0.46	0.72	0.92	2.21	1.35	0.16	2.25	mlm	85.44	0.58
1	34.18	0.48	1.08	1.29	3.99	3.24	0.79	2.86	mlm	63.65	0.53
1	33.23	0.46	0.67	0.81	2.28	1.52	0.33	1.82	mlm	68.03	0.55
1	33.65	0.42	0.6	0.7	2.06	1.34	0.39	1.5	mlm	70.58	0.48
1	33.68	0.42	0.87	1.0	3.77	2.49	0.77	2.08	mlm	60.56	0.46
1	35.46	0.41	0.62	0.69	2.37	1.59	0.54	1.65	mlm	61.63	0.47
2	78.54	1.08	0.85	1.03	11.18	4.39	0.83	2.12	mlm_distil	132.32	1.06
2	67.25	1.24	0.85	1.01	5.85	3.26	1.35	2.0	mlm_distil	111.17	1.19
2	70.16	1.28	0.85	1.07	5.61	3.01	1.08	2.52	mlm_distil	127.71	1.19
2	69.68	1.27	1.14	1.38	8.02	4.39	1.47	3.01	mlm_distil	105.11	1.22
2	60.48	1.15	0.61	0.77	3.53	1.69	0.39	1.77	mlm_distil	134.16	1.09
2	61.31	1.15	0.71	0.84	6.03	2.96	0.98	1.35	mlm_distil	100.81	1.11
2	61.73	1.14	0.6	0.67	3.51	2.25	0.61	1.21	mlm_distil	99.8	1.13
2	64.42	1.07	0.69	0.85	3.51	1.88	0.51	2.12	mlm_distil	124.13	1.02
2	62.8	1.07	0.95	1.14	6.39	3.14	0.97	2.42	mlm_distil	106.3	1.03
2	63.19	1.08	0.9	1.08	4.63	2.56	0.9	3.2	mlm_distil	117.08	0.89
2	32.63	0.46	0.71	0.88	1.89	1.31	0.16	2.08	mlm_distil	92.87	0.52
2	33.22	0.46	0.99	1.2	3.42	2.33	0.77	2.66	mlm_distil	66.46	0.48
2	33.0	0.46	0.61	0.74	2.15	1.46	0.47	1.67	mlm_distil	67.1	0.51
2	34.02	0.42	0.58	0.69	2.12	1.38	0.4	1.42	mlm_distil	77.62	0.45
2	34.27	0.41	0.93	1.07	3.84	2.59	0.86	2.08	mlm_distil	63.02	0.42
2	33.67	0.41	0.59	0.67	2.18	1.56	0.72	1.48	mlm_distil	62.13	0.43
3	82.18	1.04	0.85	1.02	9.9	4.07	0.99	2.32	mlm_fast	123.04	1.04
3	67.17	1.25	0.86	1.02	5.57	3.15	1.63	2.12	mlm_fast	103.66	1.22
3	70.65	1.27	0.83	1.04	5.63	2.88	1.01	2.53	mlm_fast	122.04	1.22
3	70.05	1.26	1.17	1.45	6.99	4.02	1.88	3.23	mlm_fast	102.04	1.26
3	61.6	1.15	0.6	0.75	3.08	1.55	0.36	1.71	mlm_fast	124.16	1.13
3	61.34	1.15	0.72	0.86	5.27	2.58	1.0	1.4	mlm_fast	95.93	1.13
3	60.95	1.15	0.62	0.68	3.69	2.22	0.88	1.28	mlm_fast	95.4	1.16
3	64.31	1.07	0.71	0.86	3.22	1.8	0.53	2.22	mlm_fast	115.58	1.07
3	63.53	1.07	0.96	1.14	5.25	2.84	1.02	2.46	mlm_fast	105.42	1.06
3	62.62	1.07	0.94	1.14	5.05	2.58	0.67	3.5	mlm_fast	112.68	0.93
3	33.42	0.47	0.73	0.93	2.16	1.35	0.16	2.28	mlm_fast	90.13	0.57
3	33.64	0.46	1.06	1.27	3.64	2.44	0.76	2.8	mlm_fast	66.85	0.52
3	32.68	0.46	0.67	0.82	2.36	1.54	0.33	1.82	mlm_fast	69.4	0.56
3	33.59	0.42	0.6	0.7	2.07	1.35	0.4	1.56	mlm_fast	71.63	0.48
3	34.41	0.43	0.9	1.04	3.73	2.5	0.63	2.2	mlm_fast	63.75	0.47
3	36.78	0.43	0.65	0.71	2.32	1.61	0.55	1.67	mlm_fast	65.38	0.48
4	77.8	1.08	0.85	1.05	11.28	4.42	1.01	2.18	mlm_distil_fast	133.13	1.05
4	67.57	1.24	0.85	1.02	6.02	3.27	1.43	2.02	mlm_distil_fast	113.31	1.21
4	71.77	1.27	0.85	1.04	5.84	2.95	0.86	2.51	mlm_distil_fast	133.39	1.19
4	70.62	1.27	1.14	1.39	8.17	4.29	1.4	3.15	mlm_distil_fast	110.47	1.22
4	60.21	1.14	0.61	0.76	3.38	1.64	0.37	1.76	mlm_distil_fast	139.33	1.1
4	61.26	1.15	0.71	0.84	5.47	2.8	0.87	1.43	mlm_distil_fast	103.96	1.11
4	61.62	1.14	0.59	0.65	3.39	2.18	0.66	1.13	mlm_distil_fast	102.4	1.13
4	64.29	1.07	0.7	0.85	3.47	1.84	0.46	1.99	mlm_distil_fast	130.62	1.03
4	62.6	1.07	0.96	1.14	6.21	3.06	0.88	2.44	mlm_distil_fast	111.01	1.04
4	63.49	1.07	0.9	1.09	4.45	2.47	0.86	3.23	mlm_distil_fast	119.26	0.89
4	32.59	0.46	0.73	0.91	1.88	1.32	0.15	2.17	mlm_distil_fast	95.37	0.53
4	33.32	0.46	1.01	1.21	3.47	2.4	0.63	2.61	mlm_distil_fast	68.25	0.49
4	33.01	0.46	0.62	0.76	2.18	1.46	0.45	1.72	mlm_distil_fast	68.34	0.51
4	34.06	0.42	0.6	0.7	2.08	1.37	0.37	1.44	mlm_distil_fast	78.45	0.45
4	34.04	0.41	0.9	1.05	3.82	2.54	0.67	2.06	mlm_distil_fast	65.21	0.43
4	34.96	0.42	0.59	0.67	2.15	1.57	0.57	1.46	mlm_distil_fast	64.45	0.44


==> data/mlm_plots/auc_files/relative_mlm_aucs.tex <==
x	model	explainer	et_use	et_tse	et_p	et_ce	dataset
0	cnn	s	0.4901960774702038	0.8163265289462724	1.1874999925781249	0.46874999951171875	agnews
1	cnn	s	0.15277777756558641	0.3333333328888889	0.4927536224742703	-0.024691358014530325	mr
2	cnn	s	0.5185185175582989	0.5490196067666283	0.599999994	0.19117647030709342	imdb
3	cnn	s	0.35937499943847656	0.4590163926901371	0.5714285673469387	0.23255813926446736	yelp
4	cnn	s	1.5208333301649304	0.9111111090864197	2.1666666305555564	0.4716981123175507	fakenews
0	cnn	ig	0.4637681152699014	0.6562499989746094	2.499999992647058	0.3134328355869903	agnews
1	cnn	ig	0.13333333315555554	0.27499999965624994	1.3943661952192026	0.04186046509680923	mr
2	cnn	ig	0.37168141560028206	0.43518518478223583	0.8333333305555557	-0.08391608385740126	imdb
3	cnn	ig	0.21641791028625512	0.2954545452307161	1.0999999963333333	-0.06010928958463978	yelp
4	cnn	ig	3.206896546195006	2.0909090871074376	9.499999881250002	1.473684207940905	fakenews
0	lstm	s	0.13953488355868038	0.33333333290598294	1.0249999974375	-0.02688172041565501	agnews
1	lstm	s	0.03797468349623447	0.2530120478879374	0.27906976711736087	-0.015037593979309188	mr
2	lstm	s	0.42499999946874983	0.5064935058357226	0.8124999949218749	0.03999999996000003	imdb
3	lstm	s	0.24786324765139897	0.2982456137734688	1.124999996484375	-0.052631578916589636	yelp
4	lstm	s	0.4883720926446727	0.1393442621808653	1.307692297633136	-0.1796874998596191	fakenews
0	lstm	ig	0.20652173890595468	0.3580246909160189	2.642857136564626	-0.05670103089860765	agnews
1	lstm	ig	0.06481481475480094	0.25438596468913516	1.3106796103779808	-0.15119363391215018	mr
2	lstm	ig	0.4529914526042808	0.4910714281329717	2.222222213991769	-0.18954248353624675	imdb
3	lstm	ig	0.2698412696984967	0.4444444442092887	1.0256410230111768	-0.10774410770783036	yelp
4	lstm	ig	1.813084110455061	1.0495049494559354	5.727272675206612	0.7553191481326392	fakenews
0	lstmatt	s	0.11363636350723139	0.2771084334010743	1.371428567510204	0.02150537633252389	agnews
1	lstmatt	s	0.2765957440923495	0.5510204070387339	0.12499999960937493	0.24999999982638896	mr
2	lstmatt	s	0.3820224714808736	0.4166666661706349	0.6111111077160494	-0.009345794383788984	imdb
3	lstmatt	s	0.44329896861515566	0.5161290317030869	1.8823529301038058	0.0	yelp
4	lstmatt	s	0.6727272721157024	0.13592232996512385	2.7499999770833337	-0.08999999990999996	fakenews
0	lstmatt	ig	0.1145833332139758	0.2555555552716048	1.9318181774276861	-0.1159420289294965	agnews
1	lstmatt	ig	0.22413793064803808	0.4098360649019081	0.9791666646267361	-0.0797546011780646	mr
2	lstmatt	ig	0.3432835818333704	0.3749999997070312	1.8928571360969386	-0.1904761903628117	imdb
3	lstmatt	ig	0.5123966937914077	0.5555555550807219	2.166666657638889	-0.050632911360358954	yelp
4	lstmatt	ig	2.077777775469136	1.0352941164290659	7.666666581481484	0.9220779208804183	fakenews
0	lstmatt	a	0.03571428568239779	0.16346153830436383	1.8478260829395086	-0.1365638765918221	agnews
1	lstmatt	a	0.5121951207019632	0.6190476175736963	2.3103448196195004	0.11926605493645305	mr
2	lstmatt	a	0.28421052601662056	0.33707865130665315	1.4210526240997232	-0.09909909900982071	imdb
3	lstmatt	a	0.4565217386342155	0.4886363630810951	1.789473674792244	-0.049999999958333374	yelp
4	lstmatt	a	1.0280373822167872	0.41414141372308944	4.1666666319444445	0.2526315786814404	fakenews
0	bert	s	0.17721518964909472	0.3766233761342554	1.2727272688705231	0.19205298000526294	agnews
1	bert	s	0.3396226408686364	0.5357142847576529	0.4390243891731112	0.24999999986111107	mr
2	bert	s	0.26229508175221716	0.25423728792013794	0.999999996551724	-0.09729729724470425	imdb
3	bert	s	0.2365591395305814	0.3076923073541842	0.937499994140625	-0.061224489754269106	yelp
4	bert	s	0.5785123962161054	0.17796610154409648	1.2499999921875	-0.26618705016821065	fakenews
0	bert	ig	0.1571428570306124	0.3382352938689446	1.9999999965517246	0.05190311416889162	agnews
1	bert	ig	0.15476190457766442	0.3033707861759878	0.8275862054696792	-0.07394366194579448	mr
2	bert	ig	0.3184713373767697	0.2999999998	1.2564102531886916	-0.16949152535191034	imdb
3	bert	ig	0.2965116277345863	0.3313609465494906	1.0999999972499996	-0.04230769229142007	yelp
4	bert	ig	0.4918032784869659	0.1367521366936958	0.8571428546938776	-0.269230769127219	fakenews
0	bert	a	0.26666666637037023	0.5058823523460209	1.5249999961874998	0.18333333323148138	agnews
1	bert	a	0.8076923061390532	1.1111111090534977	1.5333333282222221	1.1234567894299647	mr
2	bert	a	0.2212389378573107	0.23584905638127446	1.1785714243622445	-0.16666666655982906	imdb
3	bert	a	0.2456140348722684	0.33027522905479323	1.8499999907499995	-0.0993788819258517	yelp
4	bert	a	0.7920792071365552	0.2708333330512153	1.6923076792899407	-0.1047619046621316	fakenews
0	roberta	s	0.162499999796875	0.34146341421772775	0.8421052587257617	-0.10606060600704008	agnews
1	roberta	s	0.35849056536133844	0.5333333324444446	-0.38461538313609467	0.2784090907509039	mr
2	roberta	s	0.2872340422476234	0.329896906876395	0.7333333284444447	-0.22448979576565323	imdb
3	roberta	s	0.18867924510501952	0.2962962960219477	0.4999999968749999	-0.20588235282006911	yelp
4	roberta	s	0.34351145011945683	0.28888888867489704	0.42105262936288096	-0.2822085887839211	fakenews
0	roberta	ig	0.05357142853954086	0.230769230632681	0.7361111100887346	-0.18013856808772785	agnews
1	roberta	ig	0.14893617005432336	0.25242718422094446	0.08219178070932641	-0.16129032253334602	mr
2	roberta	ig	0.2972972970964207	0.17218543034954606	0.785714282908163	-0.3141592918963896	imdb
3	roberta	ig	0.1736842104349031	0.20103092773142742	0.777777775617284	-0.28571428561710394	yelp
4	roberta	ig	0.2813852812634695	0.04564315350803183	0.7999999973333335	-0.3749999998621324	fakenews
0	roberta	a	0.44871794814266913	0.6623376614774836	2.608695640831758	0.18918918908692478	agnews
1	roberta	a	0.5227272715392562	0.6874999985677085	0.7368421013850416	0.2816901406466972	mr
2	roberta	a	0.6447368412569252	0.5599999992533332	1.4999999875	-0.0480769230306953	imdb
3	roberta	a	0.30172413767092754	0.2758620687277052	1.4285714217687078	-0.20903954790449747	yelp
4	roberta	a	1.0459770102919805	0.3255813949702541	2.7999999720000006	-0.11363636350723139	fakenews
0	xlnet	s	0.328571428102041	0.5285714278163267	0.6176470570069204	0.13749999991406248	agnews
1	xlnet	s	0.3636363628099173	0.4583333323784722	0.0	0.03448275859690847	mr
2	xlnet	s	0.3483146063502082	0.2643678157880831	0.7222222182098766	-0.15748031483662964	imdb
3	xlnet	s	0.31168831128352165	0.2933333329422222	0.9230769159763313	-0.1651376145273967	yelp
4	xlnet	s	0.3333333330969267	0.3716216213705258	0.19230769156804728	-0.4039408865005217	fakenews
0	xlnet	ig	0.1093749999145507	0.2539682537666919	1.0937499982910157	-0.1038062283377834	agnews
1	xlnet	ig	0.15999999978666668	0.265822784473642	0.5714285702623907	-0.1369294605240957	mr
2	xlnet	ig	0.21604938258268547	0.11874999992578121	0.8124999974609373	-0.27876106182355703	imdb
3	xlnet	ig	0.23780487790377747	0.19135802457323567	1.1212121178145085	-0.319999999872	yelp
4	xlnet	ig	0.34272300453393284	0.2454545453429752	0.5806451594172736	-0.4037037035541838	fakenews
0	xlnet	a	0.2972972968955442	0.4084507036500695	1.7058823479238754	0.059880239485101704	agnews
1	xlnet	a	0.21568627408688965	0.2777777772633743	0.6874999978515626	-0.0060240963819132	mr
2	xlnet	a	0.6704545446926653	0.4470588230034602	2.187499986328125	-0.058333333284722275	imdb
3	xlnet	a	0.5999999993333333	0.516853932003535	2.333333317777778	-0.02325581393546063	yelp
4	xlnet	a	0.5199999995839999	0.4552845524753784	1.0714285637755099	-0.3263888886622299	fakenews


==> data/mlm_plots/auc_files/relative_mlm_distil_aucs.tex <==
x	model	explainer	et_use	et_tse	et_p	et_ce	dataset
0	cnn	s	0.5490196067666283	0.8979591818408997	0.937499994140625	0.5833333327256945	agnews
1	cnn	s	0.18055555530478398	0.3733333328355556	0.20289855043058186	-0.1275720164084066	mr
2	cnn	s	0.5370370360425238	0.5686274498654365	0.3999999960000001	0.22058823496972305	imdb
3	cnn	s	0.3749999994140625	0.4426229500940608	0.35714285459183664	0.24418604622769075	yelp
4	cnn	s	1.4791666635850693	0.9777777756049382	1.6666666388888896	0.5471698102883588	fakenews
0	cnn	ig	0.4347826080655326	0.6093749990478516	2.088235287975778	0.2462686565326352	agnews
1	cnn	ig	0.13333333315555554	0.26249999967187493	0.9014084494346363	-0.0697674418280151	mr
2	cnn	ig	0.37168141560028206	0.43518518478223583	0.8666666637777779	-0.027972027952467136	imdb
3	cnn	ig	0.23134328340944516	0.3106060603707529	0.6666666644444444	-0.06557377045597067	yelp
4	cnn	ig	2.9999999948275864	2.0181818145123964	6.249999921875	1.456140348322561	fakenews
0	lstm	s	0.13953488355868038	0.30769230729783037	0.9999999974999999	0.0	agnews
1	lstm	s	0.07594936699246908	0.28915662615764276	0.2558139531909141	-0.052631578927582155	mr
2	lstm	s	0.42499999946874983	0.49350649286557585	0.562499996484375	0.029999999970000024	imdb
3	lstm	s	0.21367521349258528	0.2631578945060019	1.1562499963867185	-0.08771929819431615	yelp
4	lstm	s	0.4573643407307252	0.15573770479037888	1.1538461449704145	-0.15624999987792965	fakenews
0	lstm	ig	0.21739130411153126	0.3456790119189148	2.476190470294785	-0.04123711338080553	agnews
1	lstm	ig	0.05555555550411506	0.21052631560480148	0.42718446560467516	-0.20159151188286703	mr
2	lstm	ig	0.4615384611439842	0.5178571423947702	1.851851844993141	-0.14379084957922164	imdb
3	lstm	ig	0.2486772485456734	0.4444444442092887	0.7692307672583824	-0.11111111107369998	yelp
4	lstm	ig	1.831775699222639	1.128712870169591	5.636363585123967	0.8404255310208241	fakenews
0	lstmatt	s	0.12499999985795453	0.28915662615764276	0.9714285686530612	0.0537634408313099	agnews
1	lstmatt	s	0.29787233979176103	0.5714285702623907	0.21874999931640626	0.22916666650752318	mr
2	lstmatt	s	0.37078651643731847	0.4285714280612245	0.277777776234568	0.028037383151366953	imdb
3	lstmatt	s	0.39175257691571913	0.44086021457972024	1.8235294010380618	-0.04477611936957009	yelp
4	lstmatt	s	0.6909090902809917	0.2233009706569893	2.0833333159722223	0.009999999990000008	fakenews
0	lstmatt	ig	0.12499999986979178	0.24444444417283961	1.613636359969008	-0.12077294680155887	agnews
1	lstmatt	ig	0.22413793064803808	0.37704917970975543	1.0416666644965278	-0.1717791409989084	mr
2	lstmatt	ig	0.3507462683949654	0.39062499969482417	1.4642857090561219	-0.16071428561862247	imdb
3	lstmatt	ig	0.4876033053821461	0.5299145294616115	1.708333326215278	-0.08227848096058331	yelp
4	lstmatt	ig	2.122222219864198	1.2470588220622838	6.333333262962965	1.116883115432619	fakenews
0	lstmatt	a	0.044642857102997285	0.15384615369822477	1.6739130398393194	-0.1365638765918221	agnews
1	lstmatt	a	0.4634146330160619	0.5952380938208618	1.1034482720570749	0.11009174301826434	mr
2	lstmatt	a	0.26315789445983384	0.32584269626309803	1.1052631520775624	-0.08108108100803513	imdb
3	lstmatt	a	0.41304347781190925	0.45454545402892566	1.4210526240997232	-0.09999999991666657	yelp
4	lstmatt	a	1.0280373822167872	0.5353535348127743	3.416666638194445	0.3473684206869807	fakenews
0	bert	s	0.1265822783207819	0.31168831128352165	0.9999999969696969	0.11258278138239546	agnews
1	bert	s	0.3018867918832323	0.5178571419323978	0.24390243842950632	0.17777777767901237	mr
2	bert	s	0.20491803261891964	0.2118644066001149	0.9310344795481572	-0.1513513512695398	imdb
3	bert	s	0.2043010750491387	0.2637362634464435	0.8124999949218749	-0.12244897950853806	yelp
4	bert	s	0.520661156594495	0.1694915252800919	0.937499994140625	-0.24460431637078817	fakenews
0	bert	ig	0.12857142847959196	0.2867647056714964	0.9999999982758622	-0.020761245667556678	agnews
1	bert	ig	0.13095238079648525	0.28089887608887754	0.6724137919441142	-0.14788732389158896	mr
2	bert	ig	0.2866242036390928	0.25333333316444434	0.9743589718606179	-0.1991525422884947	imdb
3	bert	ig	0.23255813939967557	0.26627218919155504	1.1999999969999997	-0.1346153845636095	yelp
4	bert	ig	0.4467213112923273	0.1324786324220177	0.5714285697959186	-0.2769230768165681	fakenews
0	bert	a	0.23333333307407417	0.4470588230034602	1.5499999961249997	0.12777777770678997	agnews
1	bert	a	0.7307692293639053	0.9999999981481482	1.9999999933333334	0.9753086413732662	mr
2	bert	a	0.1769911502858487	0.18867924510501952	1.1428571387755098	-0.19230769218441815	imdb
3	bert	a	0.1929824559710682	0.2752293575456609	1.599999992	-0.17391304337024036	yelp
4	bert	a	0.7326732666013135	0.26041666639539934	1.1538461449704145	-0.09523809514739236	fakenews
0	roberta	s	0.09999999987499995	0.2682926825996432	0.8421052587257617	-0.20707070696612587	agnews
1	roberta	s	0.3396226408686364	0.466666665888889	-0.38461538313609467	0.18181818171487607	mr
2	roberta	s	0.24468085080353102	0.27835051517695825	0.599999996	-0.24489795901707612	imdb
3	roberta	s	0.16981132059451753	0.2592592590192044	0.31249999804687495	-0.22352941163321793	yelp
4	roberta	s	0.267175572315133	0.21481481465569258	0.42105262936288096	-0.33742331267642733	fakenews
0	roberta	ig	0.035714285693027245	0.20710059159343164	0.9583333320023149	-0.21478060041229088	agnews
1	roberta	ig	0.05319148930511549	0.165048543529079	0.05479452047288427	-0.2199413489091081	mr
2	roberta	ig	0.2972972970964207	0.2384105958686023	0.6428571405612243	-0.283185840582661	imdb
3	roberta	ig	0.1421052630831025	0.18556701021362518	0.5277777763117285	-0.2959183672462863	yelp
4	roberta	ig	0.2554112553006877	0.05394190869131036	0.6999999976666667	-0.3124999998851103	fakenews
0	roberta	a	0.37179487131821176	0.5584415577163095	1.9130434699432894	0.09189189184222055	agnews
1	roberta	a	0.38636363548553715	0.5416666655381944	1.473684202770083	0.17605633790418568	mr
2	roberta	a	0.6052631570983379	0.506666665991111	1.1666666569444446	-0.07692307684911248	imdb
3	roberta	a	0.2758620687277052	0.2586206894322236	1.0476190426303855	-0.24858757048102392	yelp
4	roberta	a	1.0919540217333863	0.5581395342347216	2.7999999720000006	0.10227272715650823	fakenews
0	xlnet	s	0.2571428567755103	0.4285714279591838	0.7352941154844288	0.07499999995312492	agnews
1	xlnet	s	0.3181818174586776	0.4374999990885416	0.02564102557527944	-0.02068965515814508	mr
2	xlnet	s	0.3033707861759878	0.22988505720702876	0.666666662962963	-0.1811023620621241	imdb
3	xlnet	s	0.29870129831337494	0.2799999996266666	0.8461538396449704	-0.2844036694638499	yelp
4	xlnet	s	0.2553191487550929	0.2229729728223156	0.15384615325443776	-0.3940886697566065	fakenews
0	xlnet	ig	0.062499999951171926	0.1746031744646006	0.9843749984619141	-0.11418685117156166	agnews
1	xlnet	ig	0.23999999968000008	0.35443037929818944	0.755102039275302	-0.1369294605240957	mr
2	xlnet	ig	0.209876543080323	0.11874999992578121	0.624999998046875	-0.26548672554624475	imdb
3	xlnet	ig	0.20121951207242716	0.1419753085543362	0.7878787854912762	-0.33599999986560003	yelp
4	xlnet	ig	0.33802816885538595	0.26818181805991725	0.45161290176899066	-0.39999999985185186	fakenews
0	xlnet	a	0.25675675640978823	0.3661971825828209	1.8529411710207606	0.017964071845530512	agnews
1	xlnet	a	0.15686274479046514	0.24074074029492457	1.2499999960937498	-0.10843373487443747	mr
2	xlnet	a	0.6363636356404958	0.43529411713494814	1.9374999878906247	-0.07499999993749988	imdb
3	xlnet	a	0.5444444438395061	0.4494382017422043	1.6666666555555556	-0.08527131776335564	yelp
4	xlnet	a	0.48799999960960005	0.4878048776521912	1.1428571346938774	-0.2916666664641203	fakenews


==> data/mlm_plots/auc_files/relative_mlm_distil_fast_aucs.tex <==
x	model	explainer	et_use	et_tse	et_p	et_ce	dataset
0	cnn	s	0.5490196067666283	0.8979591818408997	0.937499994140625	0.5937499993815105	agnews
1	cnn	s	0.18055555530478398	0.39999999946666676	0.4637681152699014	-0.10288065839387626	mr
2	cnn	s	0.5555555545267489	0.5686274498654365	0.299999997	0.23529411730103794	imdb
3	cnn	s	0.35937499943847656	0.4426229500940608	0.28571428367346924	0.19767441837479724	yelp
4	cnn	s	1.541666663454861	0.9999999977777777	2.3333332944444454	0.5660377347810608	fakenews
0	cnn	ig	0.449275361667717	0.6249999990234375	1.8823529356401378	0.2910447759022053	agnews
1	cnn	ig	0.13333333315555554	0.27499999965624994	1.0140845056139656	-0.06046511625094641	mr
2	cnn	ig	0.37168141560028206	0.42592592553154995	0.5999999979999999	-0.048951048916817334	imdb
3	cnn	ig	0.18656716403987522	0.27272727252066103	0.49999999833333336	-0.09289617481262512	yelp
4	cnn	ig	2.8620689605826404	1.9454545419173555	5.124999935937501	1.5263157867959374	fakenews
0	lstm	s	0.15116279052190373	0.3205128201019066	0.8499999978749998	-0.005376344083131002	agnews
1	lstm	s	0.07594936699246908	0.2530120478879374	0.0	-0.05639097742240953	mr
2	lstm	s	0.4124999994843748	0.46753246692528233	0.562499996484375	0.019999999980000016	imdb
3	lstm	s	0.21367521349258528	0.2631578945060019	0.7187499977539062	-0.09356725140727057	yelp
4	lstm	s	0.41860465083829096	0.1311475408761085	0.9230769159763313	-0.13281249989624017	fakenews
0	lstm	ig	0.2282608693171076	0.3456790119189148	1.6428571389455786	-0.04123711338080553	agnews
1	lstm	ig	0.05555555550411506	0.2192982454216682	0.35922330062211316	-0.16445623337812834	mr
2	lstm	ig	0.41025640990576373	0.4285714281887754	1.3333333283950615	-0.18954248353624675	imdb
3	lstm	ig	0.22751322739285013	0.4021164019036421	0.5897435882314266	-0.14814814809826674	yelp
4	lstm	ig	1.7009345778495937	1.0693069296343494	4.999999954545455	0.9042553181869626	fakenews
0	lstmatt	s	0.11363636350723139	0.28915662615764276	1.057142854122449	0.06989247308070291	agnews
1	lstmatt	s	0.29787233979176103	0.5510204070387339	0.1562499995117187	0.22222222206790126	mr
2	lstmatt	s	0.37078651643731847	0.4047619042800453	0.277777776234568	0.03738317753515594	imdb
3	lstmatt	s	0.37113402023594444	0.4301075264192392	1.2941176394463667	-0.06716417905435514	yelp
4	lstmatt	s	0.6272727267024792	0.21359223280233758	2.333333313888889	0.07999999992000006	fakenews
0	lstmatt	ig	0.1145833332139758	0.23333333307407417	1.7499999960227273	-0.12077294680155887	agnews
1	lstmatt	ig	0.22413793064803808	0.37704917970975543	0.8124999983072917	-0.12269938642779177	mr
2	lstmatt	ig	0.2985074624638003	0.3046874997619628	1.107142853188775	-0.1845238094139738	imdb
3	lstmatt	ig	0.42148760295744825	0.435897435524874	1.4583333272569445	-0.09493670880067305	yelp
4	lstmatt	ig	1.8888888867901237	1.1294117633771628	5.666666603703705	1.129870128402766	fakenews
0	lstmatt	a	0.03571428568239779	0.1442307690920857	1.347826084026465	-0.1409691629334938	agnews
1	lstmatt	a	0.4390243891731112	0.5476190463151929	1.275862064565993	0.03669724767275464	mr
2	lstmatt	a	0.2736842102382272	0.32584269626309803	1.1052631520775624	-0.08108108100803513	imdb
3	lstmatt	a	0.4021739126063327	0.4431818176782025	1.3157894667590029	-0.09999999991666657	yelp
4	lstmatt	a	0.9906542046816313	0.5353535348127743	3.249999972916667	0.4631578942493075	fakenews
0	bert	s	0.1518987339849383	0.3246753242536684	0.8787878761248851	0.14569536414192358	agnews
1	bert	s	0.3207547163759344	0.5178571419323978	0.12195121921475323	0.10555555549691355	mr
2	bert	s	0.19672131131416284	0.1949152540721057	0.6551724115338883	-0.17297297287947408	imdb
3	bert	s	0.2043010750491387	0.2637362634464435	0.6874999957031251	-0.12244897950853806	yelp
4	bert	s	0.4958677681852333	0.18644067780810109	0.8749999945312499	-0.23741007177164733	fakenews
0	bert	ig	0.12857142847959196	0.2867647056714964	0.9482758604340071	0.0	agnews
1	bert	ig	0.14285714268707483	0.28089887608887754	0.5172413784185494	-0.14084507037294186	mr
2	bert	ig	0.273885350144022	0.24666666650222227	0.7948717928336618	-0.21610169482368563	imdb
3	bert	ig	0.21511627894469976	0.24260355015230567	0.9749999975624999	-0.11923076918491125	yelp
4	bert	ig	0.42213114736797913	0.1324786324220177	0.4285714273469388	-0.2499999999038462	fakenews
0	bert	a	0.23333333307407417	0.4470588230034602	1.3499999966249996	0.16666666657407408	agnews
1	bert	a	0.7307692293639053	1.0185185166323731	1.8666666604444446	0.9938271598803534	mr
2	bert	a	0.1769911502858487	0.17924528284976854	0.8571428540816325	-0.19871794859056544	imdb
3	bert	a	0.18421052615420147	0.2568807337092837	1.2999999935	-0.17391304337024036	yelp
4	bert	a	0.7425742566905205	0.30208333301866325	0.9999999923076923	-0.04761904757369618	fakenews
0	roberta	s	0.12499999984374997	0.28048780453599065	0.7894736800554017	-0.19696969687021726	agnews
1	roberta	s	0.3773584898540405	0.5166666658055556	-0.42307692144970416	0.23295454532218485	mr
2	roberta	s	0.25531914866455413	0.27835051517695825	0.39999999733333336	-0.24489795901707612	imdb
3	roberta	s	0.16037735833926656	0.24074074051783262	0.24999999843750007	-0.247058823384083	yelp
4	roberta	s	0.3129770989977273	0.26666666646913567	0.3157894720221607	-0.3006134967480899	fakenews
0	roberta	ig	0.02976190474418937	0.20710059159343164	0.7083333323495371	-0.19399538101755298	agnews
1	roberta	ig	0.07446808502716168	0.17475728138373073	-0.13698630118221053	-0.23460410550304872	mr
2	roberta	ig	0.28378378359203793	0.19867549655716857	0.4999999982142855	-0.2920353981008692	imdb
3	roberta	ig	0.12105263151523545	0.13917525766021896	0.388888887808642	-0.3231292515907723	yelp
4	roberta	ig	0.19047619039373323	0.033195020733114124	0.5333333315555556	-0.33455882340641224	fakenews
0	roberta	a	0.39743589692636433	0.5844155836566031	2.3913043374291116	0.12432432425712196	agnews
1	roberta	a	0.409090908161157	0.5833333321180556	1.368421045429363	0.21126760548502285	mr
2	roberta	a	0.6052631570983379	0.49333333267555574	1.0833333243055556	-0.06730769224297342	imdb
3	roberta	a	0.2758620687277052	0.241379310136742	0.8571428530612246	-0.2598870055028887	yelp
4	roberta	a	1.0459770102919805	0.4651162785289346	2.4999999749999997	0.056818181753615755	fakenews
0	xlnet	s	0.2571428567755103	0.4142857136938776	0.7352941154844288	0.018749999988281127	agnews
1	xlnet	s	0.3636363628099173	0.4583333323784722	-0.05128205115055888	-0.006896551719381695	mr
2	xlnet	s	0.32584269626309803	0.22988505720702876	0.555555552469136	-0.15748031483662964	imdb
3	xlnet	s	0.31168831128352165	0.2933333329422222	0.6923076869822485	-0.20183486220015154	yelp
4	xlnet	s	0.31205673736733575	0.2905405403442293	0.0	-0.37931034464073377	fakenews
0	xlnet	ig	0.062499999951171926	0.18253968239480975	0.9531249985107422	-0.13840830445037772	agnews
1	xlnet	ig	0.19999999973333338	0.329113923634033	0.3673469380258227	-0.1452282157073742	mr
2	xlnet	ig	0.1975308640755981	0.1062499999335937	0.4374999986328125	-0.27433628306445296	imdb
3	xlnet	ig	0.1890243901286437	0.1419753085543362	0.7272727250688702	-0.36399999985439996	yelp
4	xlnet	ig	0.3145539904626507	0.286363636233471	0.38709677294484907	-0.4111111109588477	fakenews
0	xlnet	a	0.2702702699050401	0.3802816896052371	1.3235294078719722	0.029940119742550852	agnews
1	xlnet	a	0.15686274479046514	0.24074074029492457	0.7812499975585935	-0.12048192763826387	mr
2	xlnet	a	0.6477272719912189	0.423529411266436	1.6249999898437502	-0.058333333284722275	imdb
3	xlnet	a	0.4333333328518519	0.3483146063502082	1.2666666582222226	-0.13178294563427673	yelp
4	xlnet	a	0.49599999960320007	0.4878048776521912	1.0714285637755099	-0.2916666664641203	fakenews


==> data/mlm_plots/auc_files/relative_mlm_fast_aucs.tex <==
x	model	explainer	et_use	et_tse	et_p	et_ce	dataset
0	cnn	s	0.4901960774702038	0.8163265289462724	1.4999999906250001	0.46874999951171875	agnews
1	cnn	s	0.18055555530478398	0.35999999952000006	0.4347826080655326	-0.045267489693305685	mr
2	cnn	s	0.5370370360425238	0.5686274498654365	0.4999999949999999	0.19117647030709342	imdb
3	cnn	s	0.35937499943847656	0.4754098352862135	0.5714285673469387	0.24418604622769075	yelp
4	cnn	s	1.6249999966145834	0.9777777756049382	2.3333332944444454	0.4905660368102528	fakenews
0	cnn	ig	0.449275361667717	0.6562499989746094	2.6176470511245666	0.3134328355869903	agnews
1	cnn	ig	0.1466666664711111	0.27499999965624994	1.2957746460622892	-0.013953488365602939	mr
2	cnn	ig	0.36283185808598967	0.4166666662808641	0.6999999976666667	-0.08391608385740126	imdb
3	cnn	ig	0.21641791028625512	0.2878787876606978	0.7666666641111112	-0.06557377045597067	yelp
4	cnn	ig	3.0689655119500596	2.0181818145123964	6.874999914062501	1.456140348322561	fakenews
0	lstm	s	0.15116279052190373	0.33333333290598294	1.0749999973124997	-0.010752688166262004	agnews
1	lstm	s	0.05063291132831267	0.2530120478879374	0.1744186044483505	-0.048872180432754944	mr
2	lstm	s	0.44999999943749985	0.5064935058357226	0.7499999953125002	0.009999999990000008	imdb
3	lstm	s	0.25641025619110236	0.2982456137734688	0.74999999765625	-0.02923976606477209	yelp
4	lstm	s	0.534883720515594	0.15573770479037888	1.307692297633136	-0.14843749988403315	fakenews
0	lstm	ig	0.21739130411153126	0.37037036991312305	2.1428571377551022	0.0	agnews
1	lstm	ig	0.08333333325617269	0.2719298243228686	0.8252427176453953	-0.14323607423256338	mr
2	lstm	ig	0.41025640990576373	0.4285714281887754	1.7037036973936897	-0.21568627436883253	imdb
3	lstm	ig	0.2804232802749083	0.44973544949749467	0.7692307672583824	-0.08080808078087276	yelp
4	lstm	ig	1.8037383160712723	0.9702970287422801	4.909090864462811	0.8085106374377548	fakenews
0	lstmatt	s	0.11363636350723139	0.28915662615764276	1.2857142820408165	0.0537634408313099	agnews
1	lstmatt	s	0.2765957440923495	0.5306122438150771	0.12499999960937493	0.18749999986979168	mr
2	lstmatt	s	0.41573033661153896	0.4166666661706349	0.4999999972222224	0.009345794383788984	imdb
3	lstmatt	s	0.46391752529493036	0.5376344080240489	1.4117646975778544	0.029850746246379897	yelp
4	lstmatt	s	0.7090909084462808	0.12621359211047212	2.4166666465277777	-0.009999999990000008	fakenews
0	lstmatt	ig	0.1145833332139758	0.2555555552716048	1.2727272698347107	-0.09661835744124704	agnews
1	lstmatt	ig	0.24137930992865642	0.4098360649019081	1.0833333310763889	-0.14110429439196054	mr
2	lstmatt	ig	0.2985074624638003	0.2890624997741698	1.6428571369897955	-0.22023809510700107	imdb
3	lstmatt	ig	0.4958677681852333	0.5042735038425014	1.5833333267361112	-0.056962025280403825	yelp
4	lstmatt	ig	2.099999997666667	1.0352941164290659	6.88888881234568	1.0129870116714454	fakenews
0	lstmatt	a	0.044642857102997285	0.18269230751664195	1.7391304310018902	-0.12775330390847872	agnews
1	lstmatt	a	0.5121951207019632	0.6190476175736963	2.034482751605232	0.17431192644558532	mr
2	lstmatt	a	0.31578947335180063	0.3483146063502082	1.1578947307479224	-0.09909909900982071	imdb
3	lstmatt	a	0.4782608690453687	0.5113636357825414	1.6315789387811634	-0.024999999979166687	yelp
4	lstmatt	a	1.084112148519521	0.43434343390470354	3.833333301388889	0.35789473646537406	fakenews
0	bert	s	0.18987341748117278	0.3766233761342554	1.3030302990817262	0.17218543034954606	agnews
1	bert	s	0.3396226408686364	0.5357142847576529	0.29268292611540764	0.23333333320370378	mr
2	bert	s	0.2377049178379468	0.22881355912812412	0.7241379285374555	-0.12972972965960552	imdb
3	bert	s	0.2365591395305814	0.28571428540031385	1.062499993359375	-0.06802721083807664	yelp
4	bert	s	0.5537190078068437	0.2033898303361103	1.2499999921875	-0.26618705016821065	fakenews
0	bert	ig	0.16428571416836735	0.3455882350400086	1.2413793082045188	0.0415224913351132	agnews
1	bert	ig	0.14285714268707483	0.28089887608887754	0.7586206883472059	-0.13380281685429474	mr
2	bert	ig	0.29299363038662807	0.2666666664888888	1.0256410230111768	-0.1949152541546969	imdb
3	bert	ig	0.27325581379461866	0.31360946727005373	1.0499999973749996	-0.06538461535946742	yelp
4	bert	ig	0.50409836044914	0.12393162387866172	0.5714285697959186	-0.269230769127219	fakenews
0	bert	a	0.2777777774691357	0.5176470582145329	1.5749999960624999	0.2111111109938272	agnews
1	bert	a	0.8076923061390532	1.1111111090534977	1.2333333292222224	1.1604938264441393	mr
2	bert	a	0.2300884953716031	0.23584905638127446	1.0357142820153056	-0.1858974357782709	imdb
3	bert	a	0.23684210505540168	0.3211009171366045	1.6999999915000001	-0.10559006204621743	yelp
4	bert	a	0.84158415758259	0.29166666636284727	1.384615373964497	-0.08571428563265313	fakenews
0	roberta	s	0.1874999997656249	0.3780487800267697	0.7894736800554017	-0.0858585858152229	agnews
1	roberta	s	0.3773584898540405	0.5499999990833335	-0.38461538313609467	0.2954545452866734	mr
2	roberta	s	0.3191489358306927	0.329896906876395	0.599999996	-0.23129251684946092	imdb
3	roberta	s	0.21698113187077248	0.30555555527263356	0.37499999765625	-0.1941176469446366	yelp
4	roberta	s	0.3893129768020511	0.32592592568449924	0.3157894720221607	-0.2944785274267003	fakenews
0	roberta	ig	0.06547619043721661	0.26035502943174255	0.7499999989583335	-0.15935334869298998	agnews
1	roberta	ig	0.12765957433227718	0.23300970851164102	0.041095890354663205	-0.17888563044607467	mr
2	roberta	ig	0.28378378359203793	0.09933774827858421	0.4999999982142855	-0.34513274321011816	imdb
3	roberta	ig	0.1736842104349031	0.17525773186842378	0.6111111094135802	-0.29251700670322545	yelp
4	roberta	ig	0.3290043288619028	0.062240663874588896	0.733333330888889	-0.37132352927524875	fakenews
0	roberta	a	0.4743589737508217	0.7142857133580706	2.47826085879017	0.18918918908692478	agnews
1	roberta	a	0.5227272715392562	0.7083333318576388	0.7368421013850416	0.2816901406466972	mr
2	roberta	a	0.6710526306959834	0.5599999992533332	1.1666666569444446	-0.03846153842455624	imdb
3	roberta	a	0.32758620661414994	0.31034482731866836	0.952380947845805	-0.19209039537170036	yelp
4	roberta	a	1.1724137917558464	0.38372092978637096	2.4999999749999997	-0.0454545454028926	fakenews
0	xlnet	s	0.3571428566326531	0.5714285706122452	0.8529411739619376	0.14999999990625	agnews
1	xlnet	s	0.3636363628099173	0.4583333323784722	0.02564102557527944	0.07586206891319863	mr
2	xlnet	s	0.3820224714808736	0.27586206864843454	0.6111111077160494	-0.14960629909479814	imdb
3	xlnet	s	0.33766233722381517	0.31999999957333336	0.7692307633136095	-0.155963302609208	yelp
4	xlnet	s	0.35460992882651776	0.3716216213705258	0.19230769156804728	-0.3694581278968186	fakenews
0	xlnet	ig	0.13281249989624017	0.2857142854875284	0.8124999987304686	-0.058823529391410515	agnews
1	xlnet	ig	0.19999999973333338	0.3164556958019548	0.28571428513119534	-0.08713692942442448	mr
2	xlnet	ig	0.2222222220850479	0.11249999992968746	0.624999998046875	-0.2699115043053488	imdb
3	xlnet	ig	0.2073170730443189	0.1543209875590611	0.7575757552800731	-0.3239999998704	yelp
4	xlnet	ig	0.3333333331768388	0.3318181816673553	0.35483870853277827	-0.4148148146611797	fakenews
0	xlnet	a	0.3243243238860482	0.43661971769490193	1.7647058771626292	0.09580838317616273	agnews
1	xlnet	a	0.27450980338331415	0.3148148142318243	0.7187499977539062	0.0060240963819132	mr
2	xlnet	a	0.6704545446926653	0.41176470539792387	1.9374999878906247	-0.049999999958333374	imdb
3	xlnet	a	0.5999999993333333	0.4943820219164248	1.9999999866666671	-0.038759689892434376	yelp
4	xlnet	a	0.5359999995711999	0.4959349589463944	0.9999999928571429	-0.3263888886622299	fakenews


==> data/mlm_plots/auc_files/yelp_aucs.tex <==
x	orig_pp	orig_ge	et_use	et_tse	et_p_l2	et_p_h	et_p	et_ce	attack	adv_pp	adv_ge
0	22.24	7.79	0.64	0.61	1.17	1.1	0.14	0.86	tef	59.19	8.67
0	22.02	7.84	1.34	1.32	2.65	2.42	0.3	1.83	tef	57.93	8.54
0	24.03	7.7	1.17	1.14	2.41	2.03	0.32	1.71	tef	62.82	8.38
0	27.99	6.29	1.89	1.89	3.63	3.12	0.39	2.97	tef	71.44	6.69
0	22.9	8.01	0.97	0.93	1.71	1.61	0.17	1.34	tef	60.42	8.75
0	22.77	8.0	1.21	1.17	2.15	2.03	0.24	1.58	tef	59.11	8.74
0	22.97	7.98	0.92	0.88	1.65	1.54	0.19	1.2	tef	61.37	8.75
0	21.74	8.63	0.93	0.91	1.51	1.47	0.16	1.47	tef	62.86	9.17
0	21.68	8.7	1.72	1.69	3.04	2.93	0.4	2.6	tef	56.15	9.19
0	21.45	8.71	1.14	1.09	1.95	1.87	0.2	1.61	tef	60.73	9.28
0	18.14	3.83	1.06	1.08	1.42	1.4	0.16	1.7	tef	46.79	4.29
0	18.06	3.98	1.9	1.94	2.66	2.56	0.36	2.94	tef	44.27	4.47
0	17.26	4.15	1.16	1.16	1.71	1.67	0.21	1.77	tef	43.51	4.68
0	17.01	4.01	0.77	0.75	1.09	1.08	0.13	1.09	tef	43.41	4.6
0	17.22	3.97	1.64	1.62	2.39	2.38	0.33	2.5	tef	42.35	4.52
0	17.1	3.93	0.9	0.89	1.31	1.33	0.15	1.29	tef	44.65	4.45
1	21.93	8.01	0.87	0.89	1.18	1.02	0.22	1.06	mlm	45.25	7.14
1	21.61	8.11	1.63	1.71	2.31	2.19	0.63	1.72	mlm	40.68	7.4
1	22.9	7.93	1.46	1.48	2.03	1.87	0.68	1.62	mlm	42.34	7.24
1	23.02	8.08	2.4	2.73	2.89	2.8	0.79	2.65	mlm	41.43	7.55
1	22.21	8.2	1.4	1.41	1.76	1.72	0.49	1.34	mlm	41.23	7.52
1	22.16	8.24	1.83	1.82	2.63	2.49	0.76	1.5	mlm	39.46	7.72
1	22.08	8.2	1.34	1.31	1.86	1.77	0.53	1.14	mlm	39.53	7.61
1	21.15	8.89	1.15	1.19	1.3	1.33	0.31	1.38	mlm	42.63	8.55
1	21.03	9.02	2.23	2.25	2.77	2.75	0.84	2.49	mlm	38.27	8.58
1	21.13	8.8	1.42	1.45	1.83	1.81	0.57	1.45	mlm	39.5	8.5
1	16.9	4.17	1.26	1.4	1.21	1.29	0.24	1.35	mlm	36.34	4.3
1	16.55	4.26	2.23	2.33	2.24	2.35	0.64	2.1	mlm	31.19	4.4
1	16.8	4.26	1.51	1.48	1.66	1.74	0.51	1.4	mlm	32.89	4.33
1	16.71	4.07	1.01	0.97	1.14	1.19	0.25	0.91	mlm	35.6	3.96
1	16.46	4.07	2.03	1.93	2.35	2.47	0.7	1.7	mlm	31.69	4.05
1	16.65	4.09	1.44	1.35	1.64	1.72	0.5	1.26	mlm	32.7	3.86
2	21.7	8.03	0.88	0.88	1.4	1.09	0.19	1.07	mlm_distil	51.69	7.07
2	21.94	8.03	1.65	1.73	2.59	2.31	0.5	1.71	mlm_distil	45.17	7.24
2	23.04	7.94	1.42	1.44	2.08	1.87	0.69	1.56	mlm_distil	46.78	7.15
2	23.01	8.04	2.36	2.73	2.85	2.77	0.69	2.64	mlm_distil	45.42	7.42
2	22.12	8.2	1.35	1.34	1.87	1.71	0.48	1.28	mlm_distil	45.23	7.37
2	22.14	8.22	1.8	1.79	2.6	2.46	0.65	1.45	mlm_distil	42.71	7.58
2	22.15	8.2	1.3	1.28	1.89	1.78	0.46	1.08	mlm_distil	43.54	7.45
2	21.08	8.84	1.12	1.15	1.32	1.35	0.29	1.29	mlm_distil	47.48	8.4
2	20.94	8.87	2.12	2.14	2.62	2.69	0.88	2.25	mlm_distil	40.76	8.35
2	20.99	8.83	1.36	1.39	1.82	1.81	0.52	1.33	mlm_distil	42.03	8.44
2	16.95	4.17	1.24	1.36	1.22	1.3	0.21	1.32	mlm_distil	39.56	4.18
2	16.83	4.25	2.17	2.3	2.2	2.34	0.55	2.07	mlm_distil	33.44	4.26
2	16.81	4.27	1.48	1.46	1.65	1.73	0.43	1.33	mlm_distil	34.92	4.2
2	16.52	4.1	1.0	0.96	1.13	1.19	0.24	0.78	mlm_distil	39.06	3.89
2	16.63	4.1	1.97	1.85	2.31	2.43	0.59	1.66	mlm_distil	33.08	3.95
2	16.68	4.1	1.39	1.29	1.6	1.69	0.4	1.18	mlm_distil	35.34	3.78
3	22.02	8.01	0.87	0.9	1.15	1.0	0.22	1.07	mlm_fast	46.6	7.24
3	21.67	8.11	1.63	1.7	2.21	2.07	0.53	1.71	mlm_fast	43.64	7.6
3	22.89	7.95	1.47	1.48	2.04	1.82	0.56	1.66	mlm_fast	45.69	7.5
3	23.16	8.04	2.42	2.74	2.84	2.68	0.69	2.73	mlm_fast	46.34	7.72
3	22.27	8.21	1.42	1.43	1.77	1.69	0.41	1.38	mlm_fast	43.49	7.87
3	22.22	8.24	1.81	1.76	2.48	2.35	0.62	1.49	mlm_fast	42.09	8.07
3	22.22	8.21	1.36	1.33	1.84	1.74	0.5	1.17	mlm_fast	41.17	7.98
3	21.02	8.85	1.15	1.17	1.26	1.31	0.33	1.37	mlm_fast	44.61	8.69
3	21.13	8.81	2.19	2.22	2.64	2.65	0.82	2.43	mlm_fast	41.4	8.58
3	21.07	8.8	1.41	1.44	1.78	1.77	0.54	1.44	mlm_fast	41.28	8.7
3	17.04	4.17	1.29	1.41	1.19	1.27	0.22	1.37	mlm_fast	38.98	4.4
3	16.83	4.25	2.23	2.28	2.17	2.27	0.58	2.08	mlm_fast	35.17	4.64
3	16.86	4.27	1.54	1.52	1.68	1.74	0.41	1.43	mlm_fast	35.06	4.5
3	16.63	4.08	1.03	0.99	1.13	1.18	0.23	0.92	mlm_fast	37.53	4.15
3	16.88	4.05	1.98	1.87	2.25	2.34	0.58	1.69	mlm_fast	34.38	4.16
3	16.56	4.1	1.44	1.33	1.61	1.69	0.45	1.24	mlm_fast	34.61	4.04
4	21.7	8.02	0.87	0.88	1.35	1.08	0.18	1.03	mlm_distil_fast	53.46	7.14
4	21.94	8.07	1.59	1.68	2.48	2.2	0.45	1.66	mlm_distil_fast	48.3	7.38
4	23.17	7.94	1.42	1.44	2.12	1.84	0.55	1.55	mlm_distil_fast	50.42	7.29
4	23.16	8.0	2.32	2.65	2.85	2.68	0.62	2.53	mlm_distil_fast	49.84	7.5
4	22.08	8.22	1.33	1.33	1.82	1.66	0.39	1.25	mlm_distil_fast	47.94	7.62
4	22.09	8.21	1.72	1.68	2.43	2.32	0.59	1.43	mlm_distil_fast	46.6	7.78
4	22.23	8.22	1.29	1.27	1.84	1.73	0.44	1.08	mlm_distil_fast	45.93	7.71
4	21.05	8.84	1.12	1.15	1.31	1.33	0.27	1.29	mlm_distil_fast	50.15	8.5
4	21.3	8.78	2.09	2.1	2.65	2.65	0.79	2.29	mlm_distil_fast	44.55	8.39
4	20.97	8.85	1.35	1.37	1.81	1.78	0.46	1.33	mlm_distil_fast	45.02	8.57
4	17.01	4.16	1.23	1.34	1.21	1.28	0.2	1.28	mlm_distil_fast	42.06	4.24
4	16.93	4.23	2.13	2.21	2.14	2.26	0.5	1.99	mlm_distil_fast	37.21	4.44
4	16.83	4.27	1.48	1.44	1.62	1.7	0.39	1.31	mlm_distil_fast	37.29	4.33
4	16.65	4.08	1.01	0.97	1.14	1.19	0.22	0.87	mlm_distil_fast	40.84	4.0
4	16.79	4.09	1.95	1.85	2.26	2.37	0.57	1.59	mlm_distil_fast	36.47	4.06
4	16.64	4.09	1.29	1.2	1.47	1.54	0.34	1.12	mlm_distil_fast	37.55	3.88


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	126.88	208.28	182.24	84.32	332.25	123.96	255.77	6.00	8.57	8.00	5.06	12.08	3.51	11.00	141.78	231.68	204.85	104.19	359.18	127.50	284.81	6.00	8.42	8.00	4.95	11.88	3.47	11.00	854
0.06	139.29	245.01	201.81	57.02	433.01	188.00	295.49	5.00	8.23	8.00	4.42	12.05	3.82	11.00	170.00	289.83	241.71	60.91	518.75	228.92	350.45	5.00	8.10	8.00	4.30	11.89	3.80	10.00	954
0.11	139.67	248.26	201.63	52.89	443.62	195.36	302.91	5.00	8.19	8.00	4.44	11.95	3.75	11.00	190.67	321.09	263.16	97.83	544.35	223.26	391.80	5.00	8.00	8.00	4.28	11.72	3.72	10.00	969
0.15	134.63	239.47	197.30	52.21	426.74	187.27	289.35	6.00	8.58	8.00	4.81	12.35	3.77	11.00	219.89	354.88	304.36	96.01	613.76	258.88	424.90	6.00	8.30	8.00	4.61	11.99	3.69	10.00	886
0.18	136.92	239.26	197.20	77.34	401.19	161.93	294.68	6.00	8.30	8.00	4.54	12.06	3.76	11.00	251.84	401.64	343.16	163.69	639.58	237.95	487.02	5.00	7.99	8.00	4.38	11.61	3.62	10.00	994
0.32	139.43	248.35	201.27	51.54	445.17	196.82	302.19	5.00	8.20	8.00	4.39	12.00	3.81	11.00	349.89	571.69	480.83	210.58	932.80	361.11	685.83	5.00	7.76	7.00	4.22	11.30	3.54	10.00	2633


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/comparison_vals_auc.tex <==
name	auc
orig_pp	70.16
orig_ge	2.41
adv_pp	115.72
adv_ge	2.33


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.19	0.36	0.36	0.13	0.58	0.23	0.52	0.78	0.83	0.85	0.72	0.94	0.11	0.91	0.63	0.69	0.71	0.58	0.81	0.12	0.78	854
0.06	0.05	0.22	0.20	0.01	0.44	0.22	0.37	0.70	0.77	0.79	0.64	0.90	0.13	0.86	0.55	0.63	0.64	0.50	0.75	0.12	0.72	954
0.11	-0.03	0.11	0.08	-0.06	0.28	0.17	0.21	0.59	0.68	0.70	0.54	0.83	0.14	0.80	0.46	0.54	0.55	0.41	0.67	0.13	0.64	969
0.15	-0.06	0.02	-0.01	-0.11	0.15	0.13	0.09	0.49	0.59	0.61	0.42	0.76	0.17	0.70	0.36	0.45	0.46	0.31	0.59	0.14	0.54	886
0.18	-0.10	-0.04	-0.06	-0.14	0.07	0.10	0.01	0.38	0.50	0.53	0.31	0.69	0.19	0.63	0.27	0.37	0.39	0.22	0.52	0.15	0.47	994
0.32	-0.18	-0.12	-0.12	-0.22	-0.02	0.10	-0.07	0.13	0.30	0.32	0.05	0.54	0.24	0.47	0.08	0.21	0.22	0.03	0.39	0.18	0.34	2633


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/correlations_auc.tex <==
name	auc
pcc	0.01
spearman	0.16
kendall	0.12


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	3.34	5.85	4.76	1.98	9.72	3.87	7.26	3.13	6.74	5.07	1.14	12.34	5.60	8.23	2.68	10.71	5.85	-0.26	21.68	10.97	15.48	854
0.06	3.22	5.18	4.43	2.14	8.23	3.05	6.29	3.09	6.12	4.59	1.38	10.87	4.74	7.48	2.81	11.33	5.82	-0.66	23.32	11.99	16.05	954
0.11	3.09	4.39	3.97	2.45	6.32	1.94	5.18	3.00	5.04	4.08	1.79	8.29	3.25	5.89	2.84	9.44	4.89	-1.34	20.22	10.78	10.69	969
0.15	2.88	3.86	3.56	2.38	5.33	1.47	4.48	2.82	4.28	3.56	1.87	6.69	2.41	5.05	2.64	7.50	4.08	-1.62	16.62	9.12	7.91	886
0.18	2.67	3.40	3.22	2.26	4.53	1.13	3.86	2.55	3.64	3.25	1.87	5.42	1.78	4.24	2.43	6.02	3.64	-0.95	12.98	6.96	6.16	994
0.32	2.28	2.78	2.67	2.01	3.56	0.77	3.14	2.20	2.91	2.67	1.82	4.00	1.09	3.31	2.14	4.11	2.99	0.10	8.12	4.01	4.51	2633


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/ets_sts_auc.tex <==
name	auc
et_use	1.11
et_tse	1.23
et_ce	2.10


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.24	7.03	2.46	-16.36	30.43	23.39	4.98	4.97	10.79	8.20	1.44	20.15	9.35	13.51	4.58	13.54	8.57	-4.88	31.97	18.43	15.77	854
0.06	1.02	5.64	1.90	-10.55	21.83	16.19	4.10	5.19	10.02	8.00	2.73	17.32	7.29	12.75	4.65	13.92	8.46	-7.43	35.27	21.35	15.37	954
0.11	0.79	4.93	1.35	-15.62	25.49	20.56	2.92	4.63	8.39	6.85	2.77	14.01	5.62	10.53	3.95	10.87	7.04	-5.63	27.37	16.50	12.40	969
0.15	0.56	2.69	0.92	-6.65	12.03	9.34	1.99	4.34	7.02	5.90	2.78	11.26	4.24	8.33	3.64	8.56	5.66	-5.83	22.94	14.39	9.49	886
0.18	0.42	2.36	0.72	-6.84	11.56	9.20	1.34	4.05	6.19	5.28	2.68	9.70	3.51	7.13	3.43	7.44	4.93	-5.62	20.49	13.06	7.95	994
0.32	0.25	1.37	0.42	-9.50	12.25	10.87	0.77	3.62	5.06	4.46	2.71	7.42	2.35	5.74	3.08	5.57	4.00	-2.11	13.26	7.68	5.84	2633


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.94
et_p_h	2.06
et_p_l2	2.56


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.07	0.16	0.13	0.03	0.30	0.13	0.23	0.02	0.05	0.04	0.01	0.08	0.04	0.07	0.02	0.04	0.04	0.02	0.07	0.03	0.06	854
0.06	0.10	0.25	0.20	0.03	0.48	0.23	0.35	0.03	0.06	0.04	0.01	0.10	0.04	0.08	0.03	0.05	0.05	0.02	0.09	0.03	0.07	954
0.11	0.15	0.40	0.32	0.04	0.76	0.36	0.56	0.04	0.08	0.06	0.03	0.13	0.05	0.11	0.04	0.07	0.07	0.04	0.10	0.03	0.09	969
0.15	0.26	0.61	0.53	0.16	1.05	0.44	0.86	0.05	0.09	0.08	0.04	0.15	0.05	0.13	0.06	0.09	0.08	0.05	0.12	0.04	0.11	886
0.18	0.37	0.88	0.73	-0.11	1.87	0.99	1.20	0.07	0.11	0.11	0.05	0.17	0.06	0.15	0.07	0.10	0.10	0.06	0.14	0.04	0.13	994
0.32	0.73	1.69	1.33	0.29	3.08	1.40	2.26	0.09	0.14	0.14	0.08	0.20	0.06	0.18	0.10	0.13	0.13	0.09	0.17	0.04	0.16	2633


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.24
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.93	0.94	0.90	0.96	0.03	0.95	0.91	0.93	0.94	0.89	0.97	0.04	0.96	0.89	0.93	0.95	0.86	0.99	0.07	0.98	854
0.06	0.89	0.91	0.91	0.88	0.95	0.03	0.93	0.89	0.91	0.92	0.87	0.96	0.05	0.95	0.87	0.91	0.93	0.83	0.99	0.08	0.98	954
0.11	0.86	0.89	0.89	0.85	0.92	0.04	0.91	0.86	0.89	0.89	0.84	0.94	0.05	0.92	0.85	0.89	0.91	0.81	0.98	0.09	0.96	969
0.15	0.84	0.86	0.86	0.82	0.90	0.04	0.89	0.83	0.86	0.87	0.81	0.92	0.05	0.90	0.82	0.87	0.88	0.77	0.96	0.10	0.94	886
0.18	0.81	0.84	0.84	0.79	0.88	0.04	0.86	0.80	0.84	0.84	0.78	0.89	0.06	0.88	0.79	0.84	0.86	0.74	0.95	0.10	0.92	994
0.32	0.75	0.79	0.79	0.73	0.84	0.05	0.82	0.75	0.79	0.79	0.73	0.85	0.06	0.83	0.74	0.79	0.81	0.68	0.91	0.11	0.87	2633


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	3.11	3.15	3.30	2.42	3.87	0.73	3.41	0.23	0.33	0.31	0.20	0.46	0.13	0.41	1.65	5.00	3.86	0.64	9.37	4.36	7.19	854
0.06	0.59	0.65	0.64	0.57	0.73	0.08	0.68	0.27	0.38	0.35	0.23	0.52	0.14	0.46	1.78	5.27	3.95	0.62	9.92	4.65	7.41	954
0.11	0.79	0.85	0.83	0.73	0.96	0.12	0.89	0.32	0.42	0.40	0.28	0.56	0.14	0.50	2.17	5.99	4.70	0.98	11.00	5.01	8.38	969
0.15	1.05	1.12	1.11	1.01	1.23	0.11	1.18	0.35	0.45	0.43	0.31	0.59	0.14	0.53	2.45	6.76	5.47	1.25	12.28	5.52	9.67	886
0.18	1.35	1.44	1.42	1.26	1.62	0.18	1.51	0.37	0.46	0.45	0.33	0.60	0.14	0.53	2.51	6.92	5.69	1.39	12.45	5.53	9.81	994
0.32	1.92	2.62	2.78	1.99	3.25	0.63	3.11	0.35	0.44	0.42	0.31	0.57	0.13	0.50	2.69	7.01	5.94	1.57	12.46	5.44	10.06	2633


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/time_misc_auc.tex <==
name	auc
attack_time	0.45
l2	0.12
lom	1.87


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.40	0.46	0.40	0.24	0.69	0.22	0.60	0.69	0.76	0.80	0.64	0.88	0.12	0.87	0.81	0.86	0.88	0.79	0.93	0.07	0.92	854
0.06	0.20	0.33	0.33	0.09	0.56	0.23	0.50	0.62	0.70	0.71	0.57	0.83	0.13	0.80	0.78	0.83	0.84	0.75	0.91	0.08	0.88	954
0.11	0.00	0.23	0.25	0.02	0.44	0.21	0.40	0.53	0.62	0.64	0.48	0.77	0.14	0.73	0.73	0.79	0.80	0.70	0.87	0.09	0.85	969
0.15	0.00	0.14	0.00	-0.04	0.32	0.18	0.25	0.47	0.56	0.57	0.41	0.70	0.14	0.67	0.69	0.75	0.75	0.65	0.84	0.09	0.81	886
0.18	0.00	0.08	0.00	-0.06	0.23	0.15	0.20	0.40	0.49	0.50	0.34	0.64	0.15	0.60	0.65	0.71	0.72	0.61	0.81	0.10	0.78	994
0.32	0.00	0.03	0.00	-0.06	0.12	0.09	0.00	0.23	0.36	0.36	0.19	0.53	0.17	0.47	0.56	0.63	0.64	0.52	0.74	0.11	0.71	2633


==> data/mlm_plots/mlm_distil_fast/agnews/bert/a/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.15
top50	0.21


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	125.40	205.95	181.10	85.80	326.10	120.15	253.98	6.00	8.63	8.00	5.16	12.11	3.47	11.00	142.85	231.29	203.79	103.99	358.59	127.30	283.84	6.00	8.54	8.00	5.05	12.02	3.48	11.00	892
0.06	139.63	251.53	201.49	29.86	473.21	221.68	298.41	6.00	8.31	8.00	4.49	12.13	3.82	11.00	173.13	298.06	244.85	45.84	550.29	252.23	347.80	5.00	8.15	8.00	4.37	11.93	3.78	10.00	965
0.11	140.06	249.58	201.89	54.90	444.26	194.68	306.47	6.00	8.33	8.00	4.47	12.18	3.86	11.00	195.02	329.00	271.45	74.79	583.20	254.20	390.43	5.00	8.09	8.00	4.31	11.87	3.78	10.00	994
0.15	133.58	234.44	195.78	65.22	403.65	169.21	286.77	6.00	8.61	8.00	4.89	12.34	3.73	11.00	224.54	355.51	304.07	94.48	616.54	261.03	420.19	6.00	8.24	8.00	4.59	11.89	3.65	10.00	887
0.18	137.66	239.76	198.62	78.34	401.17	161.42	295.72	6.00	8.25	8.00	4.49	12.02	3.76	11.00	258.34	411.24	354.47	160.08	662.41	251.17	491.56	5.00	7.87	8.00	4.22	11.52	3.65	10.00	998
0.32	138.78	245.02	200.48	61.22	428.82	183.80	298.35	5.00	8.22	8.00	4.45	12.00	3.77	11.00	363.64	583.35	502.92	225.54	941.15	357.81	701.10	5.00	7.76	7.00	4.16	11.36	3.60	10.00	2738


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	70.05
orig_ge	2.42
adv_pp	118.00
adv_ge	2.32


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	-0.17	0.07	0.06	-0.26	0.40	0.33	0.30	0.07	0.25	0.27	-0.02	0.52	0.27	0.43	0.06	0.19	0.20	-0.01	0.40	0.21	0.33	892
0.06	-0.33	-0.11	-0.14	-0.42	0.20	0.31	0.07	-0.11	0.07	0.07	-0.20	0.35	0.27	0.27	-0.08	0.06	0.05	-0.14	0.27	0.20	0.21	965
0.11	-0.46	-0.28	-0.29	-0.55	-0.00	0.27	-0.12	-0.25	-0.08	-0.10	-0.33	0.16	0.24	0.07	-0.17	-0.05	-0.06	-0.23	0.13	0.18	0.06	994
0.15	-0.58	-0.42	-0.44	-0.65	-0.19	0.23	-0.30	-0.37	-0.22	-0.23	-0.45	0.01	0.23	-0.08	-0.27	-0.15	-0.16	-0.32	0.02	0.17	-0.05	887
0.18	-0.66	-0.53	-0.55	-0.73	-0.33	0.20	-0.43	-0.48	-0.33	-0.35	-0.54	-0.12	0.21	-0.21	-0.34	-0.24	-0.24	-0.40	-0.08	0.16	-0.15	998
0.32	-0.79	-0.68	-0.71	-0.84	-0.53	0.16	-0.61	-0.64	-0.51	-0.53	-0.69	-0.33	0.18	-0.40	-0.47	-0.37	-0.39	-0.52	-0.23	0.14	-0.28	2738


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/correlations_auc.tex <==
name	auc
pcc	-0.12
spearman	-0.07
kendall	-0.05


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	4.73	8.21	6.73	2.88	13.53	5.33	10.09	4.58	9.67	7.31	2.32	17.02	7.35	12.90	3.95	14.42	8.54	-0.32	29.17	14.75	18.63	892
0.06	4.56	6.99	6.06	3.03	10.95	3.96	8.39	4.41	8.10	6.54	2.27	13.94	5.84	9.81	3.84	14.46	7.12	-1.37	30.29	15.83	19.15	965
0.11	4.37	6.14	5.58	3.31	8.97	2.83	7.20	4.12	6.86	5.72	2.87	10.85	3.99	8.39	3.95	13.12	6.65	-1.78	28.02	14.90	15.37	994
0.15	4.11	5.49	5.08	3.24	7.75	2.25	6.36	4.01	6.01	5.27	2.94	9.08	3.07	7.24	3.71	10.21	5.81	-1.58	22.00	11.79	10.74	887
0.18	3.88	4.94	4.68	3.27	6.61	1.67	5.70	3.78	5.29	4.74	3.03	7.56	2.26	6.19	3.62	8.69	5.34	-0.66	18.05	9.36	9.19	998
0.32	3.51	4.20	4.05	3.08	5.33	1.13	4.65	3.52	4.49	4.20	3.02	5.96	1.47	5.12	3.20	5.89	4.44	0.41	11.37	5.48	6.50	2738


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/ets_sts_auc.tex <==
name	auc
et_use	1.58
et_tse	1.75
et_ce	2.89


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.69	8.49	3.26	-14.94	31.92	23.43	6.59	6.93	16.77	12.73	2.83	30.70	13.94	21.74	6.56	21.16	13.50	-5.98	48.30	27.14	26.47	892
0.06	1.38	7.74	2.52	-18.20	33.67	25.94	5.23	7.21	15.12	11.61	3.89	26.34	11.23	19.97	6.32	19.31	12.04	-3.80	42.43	23.12	22.98	965
0.11	1.09	5.03	1.85	-13.33	23.39	18.36	3.86	6.72	12.71	9.48	3.44	21.98	9.27	15.70	5.84	16.69	9.78	-11.92	45.31	28.61	18.17	994
0.15	0.79	3.69	1.30	-11.65	19.04	15.34	2.52	6.29	9.93	8.34	4.48	15.38	5.45	12.26	5.25	11.32	7.86	-0.21	22.85	11.53	13.60	887
0.18	0.63	2.57	0.97	-5.99	11.12	8.56	1.81	6.01	8.81	7.53	4.28	13.35	4.54	10.21	5.07	9.58	6.64	1.09	18.08	8.50	10.96	998
0.32	0.37	1.71	0.59	-11.82	15.24	13.53	1.00	5.42	7.48	6.53	3.84	11.11	3.63	8.40	4.57	8.07	5.83	-0.80	16.94	8.87	8.55	2738


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/ets_time_misc_auc.tex <==
name	auc
et_p	1.13
et_p_h	3.04
et_p_l2	3.60


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.07	0.17	0.14	0.04	0.31	0.14	0.25	0.02	0.05	0.03	0.01	0.08	0.04	0.06	0.02	0.04	0.03	0.02	0.07	0.03	0.06	892
0.06	0.11	0.27	0.22	0.05	0.48	0.22	0.37	0.03	0.06	0.05	0.01	0.10	0.04	0.08	0.03	0.05	0.05	0.02	0.08	0.03	0.07	965
0.11	0.16	0.42	0.35	0.04	0.80	0.38	0.56	0.04	0.07	0.06	0.03	0.12	0.05	0.11	0.04	0.07	0.07	0.03	0.10	0.03	0.09	994
0.15	0.28	0.63	0.55	0.18	1.09	0.45	0.88	0.05	0.10	0.09	0.04	0.15	0.05	0.14	0.06	0.09	0.08	0.05	0.12	0.03	0.11	887
0.18	0.43	0.88	0.79	0.27	1.49	0.61	1.21	0.07	0.11	0.11	0.06	0.17	0.05	0.15	0.08	0.10	0.10	0.07	0.14	0.04	0.13	998
0.32	0.82	1.74	1.42	0.36	3.13	1.38	2.29	0.10	0.14	0.14	0.08	0.20	0.06	0.18	0.10	0.13	0.13	0.09	0.17	0.04	0.16	2738


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.25
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.91	0.93	0.93	0.90	0.96	0.03	0.95	0.91	0.93	0.94	0.89	0.97	0.04	0.96	0.89	0.92	0.95	0.85	1.00	0.07	0.98	892
0.06	0.89	0.91	0.91	0.87	0.94	0.03	0.93	0.88	0.91	0.92	0.86	0.96	0.05	0.94	0.86	0.91	0.92	0.83	0.98	0.08	0.97	965
0.11	0.86	0.88	0.89	0.84	0.92	0.04	0.91	0.85	0.88	0.89	0.83	0.94	0.05	0.92	0.84	0.89	0.91	0.80	0.98	0.09	0.96	994
0.15	0.83	0.86	0.86	0.81	0.90	0.04	0.88	0.83	0.86	0.87	0.81	0.91	0.05	0.90	0.81	0.86	0.88	0.77	0.96	0.09	0.93	887
0.18	0.81	0.83	0.84	0.79	0.88	0.04	0.86	0.80	0.84	0.84	0.78	0.89	0.05	0.88	0.79	0.84	0.86	0.74	0.95	0.10	0.92	998
0.32	0.76	0.79	0.79	0.74	0.84	0.05	0.82	0.76	0.80	0.80	0.74	0.85	0.06	0.84	0.74	0.79	0.81	0.68	0.91	0.11	0.87	2738


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	3.33	3.38	3.44	2.62	4.14	0.76	3.58	0.44	5.29	1.01	-4.31	14.90	9.60	4.99	3.32	10.11	7.83	1.41	18.80	8.69	14.39	892
0.06	0.91	1.07	0.98	0.79	1.35	0.28	1.15	0.50	6.80	1.27	-9.46	23.06	16.26	5.86	3.58	10.12	7.92	1.78	18.46	8.34	14.64	965
0.11	1.20	1.43	1.30	0.91	1.95	0.52	1.48	0.59	6.82	1.43	-9.02	22.66	15.84	6.34	3.90	10.88	8.97	2.14	19.61	8.74	15.68	994
0.15	1.66	1.87	1.77	1.45	2.28	0.41	1.95	0.57	6.61	1.33	-7.09	20.31	13.70	6.95	4.48	11.65	9.42	2.32	20.98	9.33	16.31	887
0.18	2.27	2.55	2.41	2.06	3.03	0.49	2.77	0.64	7.07	1.37	-7.46	21.60	14.53	7.70	4.37	11.59	9.32	2.30	20.88	9.29	16.66	998
0.32	3.57	4.59	4.74	3.44	5.73	1.14	5.51	0.63	6.56	1.36	-6.32	19.45	12.89	6.90	4.81	11.61	9.52	2.48	20.75	9.13	16.49	2738


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/time_misc_auc.tex <==
name	auc
attack_time	0.76
l2	1.95
lom	3.26


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.20	0.27	0.20	0.06	0.49	0.22	0.40	0.33	0.46	0.47	0.30	0.62	0.16	0.56	0.54	0.61	0.62	0.49	0.73	0.12	0.69	892
0.06	0.00	0.16	0.00	-0.04	0.36	0.20	0.25	0.27	0.37	0.36	0.21	0.53	0.16	0.47	0.47	0.55	0.55	0.43	0.66	0.12	0.63	965
0.11	0.00	0.09	0.00	-0.06	0.24	0.15	0.20	0.20	0.30	0.30	0.16	0.44	0.14	0.40	0.42	0.49	0.50	0.39	0.60	0.11	0.56	994
0.15	0.00	0.06	0.00	-0.06	0.18	0.12	0.00	0.15	0.25	0.25	0.12	0.38	0.13	0.33	0.38	0.44	0.44	0.34	0.55	0.10	0.51	887
0.18	0.00	0.03	0.00	-0.06	0.12	0.09	0.00	0.12	0.19	0.19	0.08	0.30	0.11	0.27	0.33	0.40	0.40	0.30	0.51	0.10	0.48	998
0.32	0.00	0.01	0.00	-0.04	0.06	0.05	0.00	0.06	0.12	0.11	0.02	0.21	0.10	0.18	0.27	0.34	0.33	0.24	0.43	0.09	0.40	2738


==> data/mlm_plots/mlm_distil_fast/agnews/bert/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.07
top50	0.13


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	128.26	209.88	182.83	85.67	334.09	124.21	261.99	6.00	8.58	8.00	5.10	12.05	3.48	11.00	146.35	235.01	207.99	108.36	361.65	126.65	287.27	6.00	8.54	8.00	5.02	12.07	3.52	10.50	895
0.06	137.93	251.15	199.93	29.87	472.43	221.28	296.65	6.00	8.29	8.00	4.50	12.07	3.78	11.00	177.06	306.80	250.37	72.64	540.95	234.15	359.76	6.00	8.25	8.00	4.48	12.03	3.77	10.00	975
0.11	139.25	247.81	201.59	53.69	441.93	194.12	303.21	5.50	8.24	8.00	4.46	12.01	3.78	11.00	197.52	337.85	284.56	100.68	575.02	237.17	402.88	5.00	8.18	8.00	4.48	11.88	3.70	10.00	983
0.15	136.51	238.28	196.90	52.94	423.62	185.34	287.28	6.00	8.55	8.00	4.82	12.28	3.73	11.00	230.98	371.61	315.94	145.41	597.82	226.20	453.52	6.00	8.47	8.00	4.80	12.14	3.67	11.00	908
0.18	134.72	239.38	197.58	77.73	401.02	161.65	298.30	5.25	8.23	8.00	4.48	11.98	3.75	11.00	272.43	428.46	366.80	186.60	670.31	241.85	530.55	5.00	8.18	8.00	4.52	11.85	3.67	10.00	1014
0.32	139.44	248.20	201.61	51.46	444.93	196.74	301.99	5.00	8.21	8.00	4.42	12.01	3.79	11.00	359.54	601.06	522.24	252.66	949.45	348.40	750.52	5.00	8.11	8.00	4.49	11.72	3.62	10.00	2630


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/comparison_vals_auc.tex <==
name	auc
orig_pp	70.35
orig_ge	2.41
adv_pp	122.09
adv_ge	2.39


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.42	0.54	0.56	0.33	0.75	0.21	0.69	0.66	0.74	0.78	0.58	0.90	0.16	0.85	0.50	0.58	0.60	0.44	0.73	0.14	0.69	895
0.06	0.29	0.44	0.46	0.22	0.67	0.22	0.61	0.56	0.65	0.68	0.46	0.84	0.19	0.79	0.41	0.50	0.52	0.34	0.66	0.16	0.61	975
0.11	0.16	0.31	0.31	0.10	0.52	0.21	0.46	0.43	0.55	0.58	0.34	0.76	0.21	0.70	0.31	0.41	0.43	0.25	0.57	0.16	0.53	983
0.15	0.03	0.18	0.17	-0.02	0.38	0.20	0.32	0.28	0.43	0.47	0.18	0.67	0.24	0.61	0.20	0.31	0.33	0.13	0.49	0.18	0.45	908
0.18	-0.06	0.08	0.07	-0.12	0.27	0.19	0.20	0.12	0.30	0.33	0.04	0.56	0.26	0.50	0.09	0.22	0.24	0.03	0.41	0.19	0.36	1014
0.32	-0.24	-0.10	-0.11	-0.29	0.10	0.20	0.03	-0.18	0.05	0.04	-0.26	0.35	0.30	0.27	-0.13	0.04	0.03	-0.18	0.25	0.21	0.19	2630


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/correlations_auc.tex <==
name	auc
pcc	0.05
spearman	0.11
kendall	0.08


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	2.06	3.94	3.25	1.12	6.76	2.82	4.93	2.07	4.72	3.48	0.43	9.01	4.29	5.82	2.03	6.82	3.99	-0.17	13.81	6.99	9.40	895
0.06	2.04	3.53	3.07	1.32	5.75	2.22	4.37	2.16	4.13	3.38	1.10	7.16	3.03	5.19	2.03	7.24	4.02	-0.56	15.04	7.80	9.40	975
0.11	2.21	3.35	3.05	1.68	5.02	1.67	4.01	2.15	3.88	3.15	1.29	6.46	2.58	4.81	2.24	7.32	3.88	-1.15	15.78	8.47	8.38	983
0.15	2.32	3.18	3.03	1.89	4.48	1.29	3.81	2.23	3.54	3.11	1.68	5.40	1.86	4.34	2.31	6.44	3.64	-1.22	14.10	7.66	6.92	908
0.18	2.27	3.05	2.91	1.89	4.22	1.16	3.62	2.26	3.34	2.99	1.75	4.93	1.59	4.03	2.29	5.80	3.54	-1.21	12.81	7.01	6.07	1014
0.32	2.16	2.72	2.64	1.92	3.53	0.81	3.19	2.15	2.89	2.71	1.84	3.93	1.04	3.44	2.13	4.14	3.01	-0.12	8.40	4.26	4.52	2630


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/ets_sts_auc.tex <==
name	auc
et_use	0.91
et_tse	1.02
et_ce	1.73


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.69	4.79	1.44	-10.65	20.24	15.44	3.29	2.88	7.28	5.22	-0.10	14.67	7.39	9.14	2.59	9.39	5.52	-4.00	22.79	13.39	10.56	895
0.06	0.58	3.30	1.05	-5.72	12.33	9.03	2.26	3.00	6.60	4.84	0.83	12.38	5.78	8.24	2.65	8.46	4.98	-4.14	21.05	12.59	9.53	975
0.11	0.49	2.96	0.86	-11.37	17.29	14.33	1.78	3.21	6.25	4.80	1.07	11.44	5.19	7.71	2.78	8.06	4.66	-5.04	21.15	13.09	8.92	983
0.15	0.40	2.13	0.66	-7.07	11.32	9.19	1.31	3.24	5.27	4.32	1.95	8.59	3.32	6.08	2.79	6.02	4.01	-0.51	12.56	6.54	6.70	908
0.18	0.33	1.43	0.54	-2.47	5.33	3.90	0.98	3.25	5.06	4.29	1.84	8.28	3.22	5.77	2.79	5.67	3.80	-1.52	12.87	7.20	6.04	1014
0.32	0.21	1.23	0.36	-6.19	8.65	7.42	0.63	3.27	4.70	4.12	2.19	7.21	2.51	5.27	2.82	5.19	3.71	-1.61	11.99	6.80	5.37	2630


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.62
et_p_h	1.60
et_p_l2	1.89


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.07	0.18	0.16	0.04	0.33	0.15	0.25	0.02	0.05	0.04	0.01	0.09	0.04	0.08	0.03	0.05	0.04	0.02	0.08	0.03	0.06	895
0.06	0.13	0.31	0.25	0.06	0.56	0.25	0.43	0.03	0.07	0.05	0.02	0.11	0.05	0.10	0.03	0.06	0.06	0.03	0.09	0.03	0.08	975
0.11	0.20	0.47	0.41	0.09	0.85	0.38	0.65	0.04	0.08	0.07	0.03	0.13	0.05	0.12	0.05	0.08	0.07	0.04	0.11	0.04	0.10	983
0.15	0.32	0.70	0.63	0.21	1.20	0.50	0.99	0.06	0.11	0.10	0.05	0.16	0.05	0.15	0.06	0.09	0.09	0.06	0.13	0.04	0.12	908
0.18	0.46	1.00	0.86	0.24	1.76	0.76	1.37	0.08	0.12	0.12	0.06	0.18	0.06	0.16	0.08	0.11	0.11	0.07	0.15	0.04	0.14	1014
0.32	0.83	1.86	1.51	0.34	3.39	1.52	2.47	0.10	0.15	0.15	0.08	0.21	0.06	0.19	0.10	0.13	0.13	0.09	0.18	0.04	0.16	2630


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.27
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.91	0.93	0.93	0.90	0.96	0.03	0.95	0.91	0.93	0.94	0.89	0.97	0.04	0.96	0.89	0.93	0.95	0.86	0.99	0.07	0.98	895
0.06	0.89	0.91	0.91	0.87	0.94	0.03	0.93	0.89	0.91	0.92	0.87	0.96	0.05	0.95	0.87	0.91	0.93	0.84	0.99	0.08	0.97	975
0.11	0.86	0.88	0.89	0.85	0.92	0.04	0.91	0.85	0.89	0.89	0.84	0.94	0.05	0.93	0.85	0.89	0.91	0.81	0.98	0.08	0.96	983
0.15	0.84	0.86	0.86	0.82	0.90	0.04	0.89	0.83	0.86	0.87	0.81	0.92	0.05	0.90	0.83	0.87	0.89	0.78	0.96	0.09	0.94	908
0.18	0.81	0.84	0.84	0.79	0.88	0.04	0.86	0.81	0.84	0.85	0.78	0.90	0.06	0.88	0.80	0.85	0.87	0.75	0.95	0.10	0.93	1014
0.32	0.76	0.79	0.79	0.73	0.84	0.05	0.82	0.75	0.79	0.80	0.73	0.85	0.06	0.84	0.75	0.80	0.82	0.69	0.91	0.11	0.88	2630


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	3.01	2.99	3.09	2.32	3.66	0.67	3.19	1.73	25.57	4.32	-30.89	82.03	56.46	17.45	1.02	2.74	2.19	0.55	4.92	2.18	3.91	895
0.06	0.70	0.81	0.75	0.56	1.06	0.25	0.85	2.01	27.79	5.30	-40.03	95.60	67.81	19.47	0.97	2.56	2.07	0.49	4.63	2.07	3.55	975
0.11	1.12	1.27	1.23	0.91	1.64	0.36	1.35	2.94	35.15	7.01	-28.96	99.25	64.10	28.74	1.26	3.04	2.55	0.68	5.40	2.36	4.26	983
0.15	1.33	1.65	1.46	0.92	2.38	0.73	1.71	3.58	44.09	8.13	-42.86	131.05	86.96	39.33	1.52	3.61	2.99	0.92	6.31	2.70	5.27	908
0.18	4.12	5.12	4.78	3.93	6.31	1.19	6.04	4.33	45.52	11.03	-33.01	124.06	78.53	44.39	1.72	3.90	3.40	1.10	6.70	2.80	5.44	1014
0.32	3.10	3.61	3.46	2.86	4.36	0.75	4.15	4.83	55.02	12.88	-43.34	153.39	98.37	55.74	1.98	4.36	3.91	1.31	7.41	3.05	6.27	2630


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/time_misc_auc.tex <==
name	auc
attack_time	0.88
l2	12.35
lom	1.04


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.20	0.38	0.40	0.16	0.60	0.22	0.60	0.60	0.67	0.67	0.53	0.80	0.14	0.75	0.75	0.80	0.81	0.71	0.89	0.09	0.85	895
0.06	0.00	0.28	0.25	0.04	0.52	0.24	0.40	0.50	0.59	0.60	0.44	0.74	0.15	0.70	0.70	0.76	0.77	0.66	0.86	0.10	0.82	975
0.11	0.00	0.18	0.20	-0.02	0.38	0.20	0.33	0.42	0.52	0.53	0.37	0.67	0.15	0.62	0.65	0.71	0.72	0.61	0.81	0.10	0.79	983
0.15	0.00	0.11	0.00	-0.05	0.28	0.17	0.25	0.33	0.45	0.44	0.30	0.59	0.15	0.55	0.59	0.66	0.67	0.55	0.78	0.11	0.74	908
0.18	0.00	0.07	0.00	-0.07	0.21	0.14	0.00	0.25	0.37	0.36	0.22	0.52	0.15	0.47	0.54	0.61	0.62	0.50	0.73	0.12	0.70	1014
0.32	0.00	0.03	0.00	-0.06	0.12	0.09	0.00	0.13	0.25	0.23	0.10	0.40	0.15	0.33	0.42	0.52	0.52	0.39	0.65	0.13	0.61	2630


==> data/mlm_plots/mlm_distil_fast/agnews/bert/s/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.12
top50	0.19


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	107.34	179.97	159.29	76.75	283.19	103.22	219.92	7.00	10.11	10.00	6.26	13.97	3.85	12.00	120.64	197.25	175.76	88.20	306.30	109.05	238.92	7.00	9.87	10.00	6.07	13.67	3.80	12.00	935
0.06	121.00	237.14	183.31	4.64	469.64	232.50	273.60	5.75	8.40	8.00	4.55	12.25	3.85	11.00	143.05	267.27	210.58	36.45	498.08	230.82	319.35	5.00	8.13	8.00	4.41	11.86	3.72	10.00	1072
0.11	120.36	232.95	181.71	16.71	449.18	216.24	272.06	6.00	8.52	8.00	4.68	12.36	3.84	11.00	160.64	285.90	227.54	62.93	508.88	222.97	332.50	5.00	8.10	8.00	4.42	11.79	3.69	10.00	1028
0.15	118.88	222.09	178.06	21.98	422.21	200.11	263.50	6.00	8.89	9.00	5.01	12.76	3.88	11.00	178.48	308.04	258.31	86.55	529.53	221.49	365.90	6.00	8.32	8.00	4.69	11.96	3.64	10.00	923
0.18	119.35	223.88	179.25	43.15	404.61	180.73	267.01	6.00	8.57	8.00	4.71	12.42	3.85	11.00	212.15	350.81	303.56	127.74	573.88	223.07	428.08	5.00	7.94	8.00	4.34	11.53	3.59	10.00	1029
0.32	119.41	230.19	179.95	18.08	442.29	212.11	269.50	6.00	8.58	8.00	4.65	12.50	3.93	11.00	294.06	491.12	420.74	190.16	792.09	300.96	611.24	5.00	7.68	7.00	4.10	11.25	3.58	10.00	2810


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	65.53
orig_ge	2.51
adv_pp	101.14
adv_ge	2.34


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.44	0.55	0.56	0.36	0.74	0.19	0.68	0.69	0.73	0.75	0.62	0.85	0.12	0.81	0.63	0.68	0.71	0.56	0.81	0.12	0.76	935
0.06	0.24	0.38	0.40	0.16	0.61	0.22	0.54	0.53	0.61	0.63	0.47	0.76	0.15	0.71	0.48	0.56	0.58	0.42	0.70	0.14	0.65	1072
0.11	0.01	0.18	0.19	-0.06	0.42	0.24	0.34	0.36	0.45	0.46	0.29	0.60	0.16	0.56	0.33	0.41	0.42	0.27	0.55	0.14	0.51	1028
0.15	-0.18	-0.02	-0.02	-0.25	0.21	0.23	0.11	0.17	0.27	0.27	0.11	0.42	0.16	0.37	0.18	0.26	0.27	0.13	0.39	0.13	0.34	923
0.18	-0.33	-0.17	-0.19	-0.39	0.04	0.22	-0.04	0.00	0.11	0.11	-0.05	0.27	0.16	0.21	0.04	0.12	0.13	-0.00	0.25	0.13	0.21	1029
0.32	-0.56	-0.40	-0.43	-0.62	-0.19	0.21	-0.28	-0.35	-0.19	-0.20	-0.40	0.02	0.21	-0.05	-0.23	-0.11	-0.12	-0.28	0.05	0.16	0.00	2810


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/correlations_auc.tex <==
name	auc
pcc	-0.01
spearman	0.06
kendall	0.06


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	2.05	3.65	2.97	1.06	6.25	2.59	4.50	1.83	4.03	3.00	0.63	7.42	3.39	4.87	1.93	6.51	3.82	-0.30	13.33	6.82	8.72	935
0.06	2.20	3.59	3.15	1.43	5.74	2.15	4.26	2.08	3.93	3.13	0.90	6.96	3.03	4.71	2.37	7.77	4.49	-0.79	16.34	8.57	9.70	1072
0.11	2.40	3.63	3.29	1.77	5.49	1.86	4.24	2.33	3.77	3.13	1.43	6.11	2.34	4.54	2.50	7.29	4.22	-0.72	15.30	8.01	8.61	1028
0.15	2.61	3.54	3.30	2.14	4.93	1.40	4.12	2.53	3.67	3.18	1.72	5.62	1.95	4.24	2.62	6.19	4.15	-0.08	12.45	6.27	7.08	923
0.18	2.68	3.42	3.24	2.28	4.56	1.14	3.95	2.58	3.49	3.17	2.01	4.97	1.48	3.97	2.64	5.58	3.91	0.20	10.96	5.38	6.17	1029
0.32	2.64	3.17	3.06	2.34	3.99	0.82	3.55	2.55	3.18	2.99	2.17	4.19	1.01	3.60	2.48	4.31	3.43	0.80	7.82	3.51	4.85	2810


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/ets_sts_auc.tex <==
name	auc
et_use	1.00
et_tse	1.04
et_ce	1.73


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.86	4.58	1.64	-8.41	17.57	12.99	3.79	3.67	8.96	6.46	0.74	17.18	8.22	11.35	3.52	11.41	6.73	-4.61	27.43	16.02	13.51	935
0.06	0.83	5.33	1.60	-14.70	25.37	20.03	3.37	4.26	9.52	7.20	1.12	17.92	8.40	11.58	3.89	12.23	7.47	-7.52	31.99	19.75	13.72	1072
0.11	0.73	4.82	1.39	-15.29	24.92	20.10	2.83	4.54	9.13	7.13	2.12	16.15	7.02	11.29	4.00	11.26	7.18	-3.62	26.15	14.88	12.70	1028
0.15	0.62	3.52	1.12	-11.50	18.53	15.01	2.59	4.91	8.59	6.75	2.65	14.52	5.93	10.27	4.19	10.50	6.57	-4.47	25.47	14.97	11.49	923
0.18	0.53	2.57	0.87	-6.27	11.40	8.84	1.79	4.93	8.13	6.52	2.45	13.82	5.69	9.63	4.16	10.04	6.15	-6.14	26.22	16.18	10.62	1029
0.32	0.33	2.05	0.56	-9.87	13.97	11.92	1.10	4.74	7.16	6.00	2.77	11.56	4.39	7.98	4.04	8.66	5.52	-5.43	22.76	14.10	8.76	2810


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.98
et_p_h	2.42
et_p_l2	2.99


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.06	0.16	0.13	0.02	0.30	0.14	0.22	0.02	0.04	0.03	0.01	0.08	0.03	0.05	0.02	0.04	0.03	0.01	0.06	0.02	0.05	935
0.06	0.09	0.24	0.18	0.03	0.44	0.20	0.34	0.02	0.05	0.04	0.01	0.09	0.04	0.07	0.03	0.05	0.04	0.02	0.08	0.03	0.06	1072
0.11	0.15	0.36	0.30	0.07	0.66	0.29	0.51	0.03	0.07	0.06	0.02	0.11	0.05	0.09	0.04	0.06	0.06	0.03	0.09	0.03	0.08	1028
0.15	0.21	0.55	0.44	0.10	1.00	0.45	0.78	0.04	0.08	0.08	0.03	0.13	0.05	0.12	0.05	0.08	0.07	0.04	0.11	0.03	0.10	923
0.18	0.33	0.80	0.66	0.14	1.45	0.65	1.10	0.05	0.10	0.09	0.05	0.16	0.06	0.14	0.06	0.09	0.09	0.05	0.13	0.04	0.12	1029
0.32	0.63	1.62	1.25	0.19	3.06	1.44	2.15	0.08	0.13	0.13	0.07	0.19	0.06	0.17	0.09	0.12	0.12	0.07	0.16	0.04	0.15	2810


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.23
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.91	0.93	0.93	0.90	0.96	0.03	0.95	0.90	0.92	0.93	0.88	0.96	0.04	0.95	0.89	0.93	0.94	0.86	0.99	0.06	0.98	935
0.06	0.88	0.90	0.90	0.87	0.94	0.03	0.92	0.87	0.90	0.90	0.85	0.95	0.05	0.93	0.88	0.91	0.93	0.84	0.98	0.07	0.97	1072
0.11	0.85	0.87	0.87	0.83	0.91	0.04	0.90	0.83	0.87	0.87	0.82	0.92	0.05	0.91	0.84	0.89	0.90	0.81	0.97	0.08	0.95	1028
0.15	0.82	0.84	0.84	0.80	0.88	0.04	0.87	0.80	0.84	0.84	0.79	0.89	0.05	0.88	0.81	0.86	0.88	0.77	0.95	0.09	0.93	923
0.18	0.79	0.82	0.82	0.78	0.86	0.04	0.84	0.78	0.81	0.81	0.76	0.87	0.05	0.85	0.78	0.84	0.85	0.75	0.93	0.09	0.90	1029
0.32	0.74	0.77	0.77	0.72	0.82	0.05	0.80	0.73	0.77	0.77	0.71	0.82	0.06	0.80	0.72	0.78	0.80	0.68	0.89	0.11	0.86	2810


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	1.18	1.22	1.23	1.09	1.34	0.13	1.28	5.38	8.00	7.19	4.32	11.68	3.68	10.05	0.70	2.45	1.71	-0.03	4.93	2.48	3.35	935
0.06	0.84	0.91	0.88	0.83	0.99	0.08	0.96	5.36	8.47	7.55	4.30	12.64	4.17	10.62	0.74	2.46	1.67	0.01	4.91	2.45	3.33	1072
0.11	1.03	1.11	1.08	1.00	1.22	0.11	1.16	6.31	9.77	8.84	5.24	14.29	4.52	12.14	1.04	2.94	2.18	0.28	5.60	2.66	3.95	1028
0.15	1.32	1.36	1.34	1.29	1.44	0.08	1.40	7.60	11.34	10.18	6.20	16.48	5.14	14.18	1.20	3.47	2.70	0.52	6.42	2.95	5.12	923
0.18	1.69	1.77	1.77	1.69	1.84	0.08	1.81	7.97	12.03	10.86	6.59	17.48	5.44	15.12	1.25	3.63	2.93	0.60	6.66	3.03	5.11	1029
0.32	2.10	2.86	3.07	2.18	3.55	0.69	3.38	8.96	13.38	12.01	7.38	19.38	6.00	16.71	1.41	3.80	3.11	0.71	6.89	3.09	5.33	2810


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/time_misc_auc.tex <==
name	auc
attack_time	0.50
l2	3.26
lom	0.96


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.40	0.56	0.60	0.41	0.70	0.15	0.60	0.75	0.80	0.81	0.71	0.89	0.09	0.88	0.84	0.86	0.88	0.79	0.93	0.07	0.92	935
0.06	0.25	0.36	0.40	0.15	0.57	0.21	0.50	0.67	0.72	0.73	0.61	0.83	0.11	0.80	0.78	0.81	0.82	0.74	0.89	0.08	0.87	1072
0.11	0.00	0.22	0.20	0.02	0.41	0.19	0.33	0.56	0.62	0.62	0.51	0.73	0.11	0.69	0.70	0.75	0.76	0.67	0.83	0.08	0.81	1028
0.15	0.00	0.12	0.00	-0.04	0.28	0.16	0.20	0.46	0.53	0.54	0.42	0.64	0.11	0.62	0.65	0.69	0.70	0.61	0.77	0.08	0.74	923
0.18	0.00	0.08	0.00	-0.05	0.21	0.13	0.20	0.36	0.43	0.44	0.32	0.55	0.11	0.50	0.58	0.63	0.63	0.55	0.71	0.08	0.68	1029
0.32	0.00	0.04	0.00	-0.06	0.14	0.10	0.00	0.19	0.28	0.27	0.14	0.41	0.13	0.38	0.44	0.51	0.52	0.41	0.61	0.10	0.58	2810


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/ig/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.14
top50	0.19


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	107.94	179.50	159.42	78.06	280.94	101.44	216.88	7.00	10.26	10.00	6.40	14.11	3.85	12.00	128.51	210.36	184.98	96.26	324.46	114.10	258.80	8.00	10.13	10.00	6.26	14.00	3.87	12.00	865
0.06	119.57	230.52	182.48	23.00	438.04	207.52	267.01	6.00	8.51	8.00	4.62	12.40	3.89	11.00	157.69	286.31	231.31	77.81	494.81	208.50	348.42	5.00	8.28	8.00	4.36	12.20	3.92	11.00	1005
0.11	119.84	233.25	182.54	16.34	450.16	216.91	271.88	6.00	8.54	8.00	4.69	12.40	3.85	11.00	186.87	336.89	275.14	74.06	599.72	262.83	400.79	5.00	8.23	8.00	4.36	12.09	3.86	10.00	999
0.15	118.32	222.42	177.88	21.28	423.56	201.14	263.15	6.00	8.89	9.00	5.02	12.76	3.87	11.00	226.74	382.74	321.94	101.01	664.48	281.74	457.99	6.00	8.49	8.00	4.62	12.36	3.87	11.00	917
0.18	119.24	223.64	179.35	42.97	404.31	180.67	266.62	6.00	8.57	8.00	4.71	12.44	3.87	11.00	273.97	461.39	386.57	136.15	786.64	325.24	561.42	5.00	8.08	8.00	4.25	11.91	3.83	10.00	1028
0.32	119.57	230.14	179.95	18.49	441.79	211.65	269.69	6.00	8.57	8.00	4.64	12.51	3.94	11.00	388.16	667.42	569.45	203.07	1131.76	464.35	810.89	5.00	7.86	7.00	3.99	11.73	3.87	10.00	2815


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/comparison_vals_auc.tex <==
name	auc
orig_pp	65.27
orig_ge	2.52
adv_pp	128.63
adv_ge	2.39


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.67	0.75	0.77	0.61	0.89	0.14	0.85	0.70	0.78	0.80	0.65	0.90	0.12	0.87	0.61	0.69	0.70	0.57	0.80	0.12	0.77	865
0.06	0.51	0.62	0.66	0.41	0.83	0.21	0.78	0.56	0.66	0.69	0.48	0.85	0.18	0.80	0.47	0.57	0.58	0.42	0.72	0.15	0.68	1005
0.11	0.33	0.48	0.52	0.24	0.72	0.24	0.66	0.39	0.53	0.56	0.31	0.75	0.22	0.69	0.33	0.43	0.44	0.26	0.60	0.17	0.55	999
0.15	0.16	0.33	0.36	0.07	0.59	0.26	0.53	0.23	0.38	0.40	0.13	0.63	0.25	0.57	0.18	0.30	0.31	0.11	0.49	0.19	0.43	917
0.18	-0.01	0.19	0.20	-0.10	0.47	0.29	0.40	0.05	0.23	0.25	-0.05	0.51	0.28	0.45	0.05	0.18	0.18	-0.02	0.38	0.20	0.33	1028
0.32	-0.36	-0.11	-0.13	-0.44	0.21	0.33	0.12	-0.35	-0.09	-0.10	-0.44	0.25	0.34	0.15	-0.23	-0.06	-0.06	-0.30	0.19	0.24	0.11	2815


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/correlations_auc.tex <==
name	auc
pcc	0.08
spearman	0.09
kendall	0.07


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	1.15	2.29	1.82	0.63	3.96	1.67	2.85	1.24	3.05	2.13	0.08	6.01	2.96	3.69	1.37	4.52	2.94	0.10	8.94	4.42	6.26	865
0.06	1.37	2.53	2.13	0.86	4.19	1.67	3.20	1.37	3.31	2.42	0.12	6.49	3.18	3.95	1.61	5.97	3.42	-0.37	12.31	6.34	8.16	1005
0.11	1.58	2.66	2.37	1.13	4.20	1.53	3.41	1.65	3.23	2.56	0.73	5.72	2.50	3.98	1.90	6.03	3.68	-0.67	12.74	6.70	7.35	999
0.15	1.79	2.75	2.55	1.37	4.12	1.38	3.46	1.84	3.25	2.71	1.08	5.41	2.17	3.99	2.00	5.63	3.30	-0.87	12.13	6.50	6.30	917
0.18	1.91	2.80	2.65	1.59	4.02	1.21	3.47	1.98	3.21	2.81	1.43	4.99	1.78	4.05	2.11	5.23	3.44	-0.75	11.20	5.98	5.84	1028
0.32	2.20	2.92	2.83	1.89	3.95	1.03	3.53	2.23	3.14	2.95	1.82	4.47	1.33	3.80	2.20	4.36	3.21	0.05	8.67	4.31	4.94	2815


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/ets_sts_auc.tex <==
name	auc
et_use	0.79
et_tse	0.93
et_ce	1.53


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.32	1.80	0.61	-3.56	7.15	5.35	1.46	1.52	3.80	2.61	-0.50	8.09	4.29	4.54	1.45	5.45	2.77	-5.78	16.68	11.23	5.68	865
0.06	0.31	1.87	0.55	-5.80	9.54	7.67	1.17	1.87	4.76	3.01	-1.10	10.62	5.86	5.52	1.69	7.29	3.19	-11.15	25.74	18.45	6.69	1005
0.11	0.29	1.40	0.50	-3.02	5.81	4.42	0.97	2.04	4.38	3.19	0.01	8.75	4.37	5.05	1.85	6.09	3.09	-7.72	19.90	13.81	5.82	999
0.15	0.25	0.82	0.41	-1.80	3.44	2.62	0.70	2.20	4.09	3.38	0.86	7.33	3.24	4.94	1.91	5.10	3.10	-5.16	15.37	10.26	5.62	917
0.18	0.20	0.73	0.35	-1.32	2.77	2.05	0.59	2.46	4.14	3.50	1.24	7.04	2.90	4.94	2.19	4.87	3.24	-3.27	13.01	8.14	5.13	1028
0.32	0.16	0.79	0.26	-4.50	6.09	5.30	0.46	3.05	4.51	3.92	1.74	7.28	2.77	5.19	2.65	5.35	3.56	-5.79	16.50	11.14	5.14	2815


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.31
et_p_h	1.25
et_p_l2	1.61


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.08	0.21	0.19	0.06	0.36	0.15	0.31	0.02	0.05	0.04	0.01	0.09	0.04	0.07	0.03	0.05	0.04	0.02	0.08	0.03	0.07	865
0.06	0.16	0.35	0.30	0.09	0.61	0.26	0.48	0.03	0.06	0.05	0.02	0.11	0.05	0.09	0.03	0.06	0.06	0.03	0.10	0.03	0.09	1005
0.11	0.27	0.57	0.49	0.16	0.98	0.41	0.79	0.04	0.09	0.08	0.03	0.14	0.05	0.13	0.05	0.08	0.08	0.04	0.12	0.04	0.11	999
0.15	0.45	0.89	0.81	0.33	1.44	0.56	1.20	0.06	0.11	0.10	0.05	0.17	0.06	0.15	0.07	0.10	0.10	0.06	0.14	0.04	0.13	917
0.18	0.68	1.31	1.15	0.46	2.15	0.85	1.76	0.08	0.13	0.13	0.07	0.19	0.06	0.17	0.09	0.11	0.11	0.08	0.15	0.04	0.14	1028
0.32	1.14	2.49	2.03	0.49	4.50	2.01	3.22	0.11	0.15	0.15	0.09	0.22	0.06	0.20	0.11	0.14	0.14	0.10	0.18	0.04	0.17	2815


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.36
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.94	0.94	0.91	0.96	0.03	0.95	0.92	0.94	0.95	0.90	0.98	0.04	0.97	0.92	0.94	0.97	0.88	1.00	0.06	0.98	865
0.06	0.90	0.92	0.92	0.89	0.95	0.03	0.94	0.90	0.92	0.93	0.87	0.96	0.05	0.95	0.90	0.93	0.95	0.86	1.00	0.07	0.98	1005
0.11	0.87	0.89	0.90	0.86	0.93	0.03	0.92	0.87	0.90	0.91	0.85	0.95	0.05	0.93	0.88	0.91	0.93	0.84	0.99	0.07	0.97	999
0.15	0.85	0.87	0.87	0.83	0.91	0.04	0.89	0.85	0.88	0.88	0.83	0.93	0.05	0.91	0.85	0.89	0.90	0.81	0.97	0.08	0.95	917
0.18	0.83	0.85	0.85	0.81	0.88	0.04	0.87	0.82	0.86	0.86	0.81	0.91	0.05	0.89	0.82	0.87	0.88	0.78	0.95	0.09	0.93	1028
0.32	0.77	0.80	0.80	0.75	0.85	0.05	0.83	0.77	0.81	0.81	0.75	0.86	0.06	0.85	0.76	0.82	0.83	0.72	0.91	0.10	0.89	2815


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.56	0.61	0.58	0.51	0.71	0.10	0.66	62.68	93.64	86.65	52.56	134.72	41.08	118.73	0.78	1.71	1.52	0.55	2.87	1.16	2.38	865
0.06	0.40	0.51	0.42	0.22	0.81	0.29	0.48	65.80	101.82	93.40	55.77	147.87	46.05	132.90	0.90	1.89	1.63	0.59	3.19	1.30	2.73	1005
0.11	0.57	0.68	0.61	0.43	0.94	0.25	0.69	80.48	120.34	112.18	68.87	171.80	51.47	152.80	1.01	2.26	1.93	0.69	3.83	1.57	3.29	999
0.15	0.70	0.77	0.74	0.65	0.88	0.12	0.78	98.57	146.34	137.20	84.52	208.16	61.82	186.80	1.34	2.79	2.50	0.89	4.70	1.90	3.97	917
0.18	0.81	0.88	0.86	0.78	0.98	0.10	0.90	107.53	161.53	153.16	92.85	230.21	68.68	207.03	1.37	3.08	2.78	1.00	5.16	2.08	4.44	1028
0.32	1.00	1.41	1.45	1.06	1.75	0.35	1.68	128.58	195.61	181.85	109.70	281.52	85.91	247.45	1.66	3.70	3.38	1.19	6.21	2.51	5.28	2815


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/time_misc_auc.tex <==
name	auc
attack_time	0.26
l2	43.43
lom	0.82


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.40	0.51	0.60	0.23	0.79	0.28	0.80	0.62	0.71	0.73	0.59	0.83	0.12	0.80	0.78	0.83	0.84	0.75	0.91	0.08	0.89	865
0.06	0.00	0.38	0.33	0.07	0.69	0.31	0.60	0.53	0.62	0.62	0.47	0.77	0.15	0.73	0.71	0.77	0.78	0.67	0.87	0.10	0.84	1005
0.11	0.00	0.27	0.20	-0.02	0.55	0.29	0.40	0.43	0.53	0.54	0.36	0.70	0.17	0.64	0.64	0.71	0.71	0.60	0.81	0.11	0.78	999
0.15	0.00	0.18	0.00	-0.06	0.42	0.24	0.33	0.31	0.43	0.43	0.26	0.60	0.17	0.55	0.57	0.64	0.65	0.53	0.76	0.12	0.72	917
0.18	0.00	0.12	0.00	-0.09	0.32	0.21	0.20	0.23	0.35	0.33	0.18	0.52	0.17	0.46	0.48	0.58	0.58	0.45	0.70	0.12	0.67	1028
0.32	0.00	0.05	0.00	-0.09	0.19	0.14	0.00	0.07	0.21	0.19	0.04	0.38	0.17	0.31	0.33	0.45	0.44	0.30	0.59	0.15	0.56	2815


==> data/mlm_plots/mlm_distil_fast/agnews/cnn/s/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.12
top50	0.18


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	107.88	180.07	158.92	80.72	279.42	99.35	224.26	7.00	10.14	10.00	6.15	14.13	3.99	12.00	122.22	199.85	175.26	87.47	312.23	112.38	248.71	7.00	10.02	10.00	6.03	14.01	3.99	12.00	956
0.06	120.35	234.96	183.01	4.81	465.12	230.16	274.62	5.00	8.48	8.00	4.57	12.39	3.91	11.00	142.56	267.89	210.28	33.90	501.87	233.99	309.83	5.00	8.37	8.00	4.50	12.24	3.87	11.00	1023
0.11	119.56	232.18	182.73	16.57	447.78	215.61	273.82	6.00	8.56	8.00	4.69	12.44	3.88	11.00	156.07	287.27	230.14	31.24	543.29	256.03	330.75	5.00	8.36	8.00	4.58	12.14	3.78	10.00	989
0.15	117.77	222.84	179.48	21.64	424.03	201.20	265.95	6.00	8.94	9.00	5.04	12.84	3.90	11.00	172.86	307.41	254.35	75.95	538.87	231.46	366.99	6.00	8.58	8.00	4.77	12.39	3.81	11.00	893
0.18	119.03	225.35	182.13	45.48	405.22	179.87	273.51	6.00	8.59	8.00	4.71	12.48	3.89	11.00	205.21	356.36	290.03	100.55	612.18	255.82	426.82	5.00	8.14	8.00	4.39	11.88	3.75	10.00	993
0.32	118.92	230.93	181.94	18.60	443.25	212.32	273.85	6.00	8.61	8.00	4.64	12.57	3.96	11.00	281.69	488.93	404.91	148.63	829.23	340.30	584.79	5.00	7.91	8.00	4.16	11.66	3.75	10.00	2714


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	65.62
orig_ge	2.52
adv_pp	101.56
adv_ge	2.41


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.14	0.32	0.34	0.03	0.61	0.29	0.52	0.59	0.64	0.70	0.44	0.85	0.21	0.77	0.49	0.57	0.63	0.37	0.77	0.20	0.71	956
0.06	-0.02	0.21	0.22	-0.11	0.52	0.32	0.42	0.49	0.56	0.60	0.36	0.77	0.21	0.69	0.41	0.50	0.54	0.31	0.69	0.19	0.63	1023
0.11	-0.22	-0.01	-0.01	-0.31	0.30	0.30	0.18	0.31	0.41	0.44	0.19	0.62	0.21	0.54	0.26	0.37	0.40	0.18	0.56	0.19	0.50	989
0.15	-0.39	-0.18	-0.21	-0.48	0.12	0.30	-0.01	0.12	0.24	0.25	0.03	0.45	0.21	0.38	0.14	0.24	0.25	0.06	0.41	0.18	0.35	893
0.18	-0.49	-0.29	-0.31	-0.56	-0.01	0.28	-0.12	-0.01	0.11	0.11	-0.10	0.31	0.21	0.24	0.03	0.13	0.13	-0.04	0.29	0.17	0.24	993
0.32	-0.64	-0.45	-0.48	-0.71	-0.19	0.26	-0.30	-0.31	-0.14	-0.14	-0.38	0.10	0.24	0.02	-0.20	-0.07	-0.07	-0.26	0.11	0.19	0.05	2714


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/correlations_auc.tex <==
name	auc
pcc	-0.05
spearman	0.06
kendall	0.06


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	2.99	5.07	4.33	1.80	8.34	3.27	6.14	2.75	5.17	4.22	1.26	9.07	3.91	6.44	3.32	9.54	5.88	0.26	18.83	9.29	12.76	956
0.06	2.64	4.41	3.88	1.70	7.12	2.71	5.35	2.40	4.34	3.51	1.11	7.56	3.23	5.29	2.95	8.77	5.12	-0.65	18.19	9.42	10.51	1023
0.11	2.93	4.32	3.95	2.11	6.53	2.21	5.13	2.67	4.13	3.48	1.73	6.54	2.41	4.97	3.13	8.33	4.87	-0.77	17.43	9.10	9.59	989
0.15	2.93	4.02	3.77	2.27	5.76	1.74	4.69	2.69	3.90	3.42	1.96	5.84	1.94	4.62	2.93	6.75	4.42	-0.39	13.88	7.14	7.33	893
0.18	2.78	3.67	3.45	2.21	5.14	1.46	4.21	2.62	3.51	3.16	2.03	5.00	1.48	4.03	2.72	5.43	3.85	0.08	10.78	5.35	6.14	993
0.32	2.61	3.22	3.10	2.20	4.24	1.02	3.67	2.49	3.12	2.93	2.08	4.16	1.04	3.52	2.47	4.20	3.35	0.61	7.78	3.59	4.68	2714


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/ets_sts_auc.tex <==
name	auc
et_use	1.13
et_tse	1.09
et_ce	1.86


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.31	7.13	2.53	-11.68	25.95	18.81	5.69	5.29	12.12	9.18	1.98	22.27	10.14	15.95	4.76	13.31	8.99	-0.06	26.69	13.37	17.39	956
0.06	1.08	6.15	2.16	-10.80	23.11	16.95	4.97	5.47	11.69	9.39	2.11	21.26	9.57	14.54	5.15	14.98	9.36	-10.03	39.99	25.01	16.52	1023
0.11	0.93	6.05	1.72	-15.57	27.67	21.62	3.85	5.64	10.45	8.48	3.34	17.56	7.11	13.10	5.06	13.15	8.42	-10.70	37.00	23.85	14.59	989
0.15	0.74	3.90	1.42	-7.08	14.88	10.98	2.94	5.53	9.46	7.98	3.89	15.04	5.57	11.73	4.64	10.80	7.49	-0.70	22.30	11.50	13.33	893
0.18	0.58	2.74	1.05	-8.46	13.93	11.20	2.10	5.36	8.74	7.33	3.19	14.29	5.55	10.22	4.48	10.23	6.83	-3.16	23.63	13.40	11.65	993
0.32	0.34	1.62	0.61	-4.54	7.78	6.16	1.21	4.84	7.33	6.23	3.27	11.40	4.06	8.51	4.13	8.47	5.61	-2.44	19.37	10.91	9.00	2714


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/ets_time_misc_auc.tex <==
name	auc
et_p	1.11
et_p_h	2.71
et_p_l2	3.23


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.06	0.16	0.13	0.02	0.30	0.14	0.23	0.02	0.05	0.03	0.01	0.08	0.03	0.06	0.02	0.04	0.03	0.02	0.07	0.02	0.05	956
0.06	0.09	0.24	0.17	0.01	0.47	0.23	0.32	0.02	0.05	0.04	0.01	0.09	0.04	0.07	0.03	0.05	0.04	0.02	0.08	0.03	0.06	1023
0.11	0.13	0.35	0.28	0.06	0.65	0.29	0.49	0.03	0.07	0.06	0.02	0.11	0.05	0.10	0.04	0.06	0.06	0.03	0.09	0.03	0.08	989
0.15	0.20	0.52	0.41	0.09	0.94	0.43	0.74	0.04	0.09	0.08	0.04	0.14	0.05	0.12	0.05	0.08	0.07	0.04	0.11	0.03	0.10	893
0.18	0.31	0.76	0.62	0.17	1.35	0.59	1.06	0.06	0.10	0.09	0.05	0.16	0.06	0.14	0.06	0.09	0.09	0.05	0.13	0.04	0.12	993
0.32	0.59	1.53	1.17	0.21	2.85	1.32	2.06	0.08	0.13	0.13	0.07	0.19	0.06	0.17	0.09	0.12	0.12	0.07	0.16	0.04	0.15	2714


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.22
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.90	0.92	0.93	0.89	0.95	0.03	0.94	0.89	0.92	0.92	0.88	0.96	0.04	0.95	0.90	0.93	0.95	0.88	0.99	0.06	0.98	956
0.06	0.87	0.90	0.90	0.86	0.93	0.03	0.92	0.85	0.89	0.89	0.84	0.94	0.05	0.93	0.87	0.91	0.92	0.84	0.98	0.07	0.97	1023
0.11	0.84	0.87	0.87	0.83	0.91	0.04	0.90	0.82	0.86	0.86	0.80	0.91	0.05	0.90	0.84	0.88	0.90	0.80	0.97	0.08	0.95	989
0.15	0.81	0.84	0.84	0.80	0.88	0.04	0.87	0.79	0.83	0.83	0.77	0.89	0.06	0.87	0.80	0.85	0.87	0.77	0.94	0.09	0.92	893
0.18	0.78	0.81	0.81	0.76	0.86	0.05	0.84	0.76	0.80	0.80	0.74	0.86	0.06	0.84	0.77	0.82	0.83	0.73	0.92	0.10	0.89	993
0.32	0.72	0.76	0.76	0.71	0.82	0.05	0.80	0.71	0.75	0.75	0.69	0.81	0.06	0.79	0.71	0.77	0.78	0.65	0.88	0.11	0.85	2714


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.24


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	2.93	2.96	3.06	2.28	3.65	0.68	3.17	1.35	2.18	1.85	0.77	3.58	1.40	2.61	0.89	3.65	2.13	-1.09	8.39	4.74	4.53	956
0.06	0.45	0.49	0.47	0.42	0.56	0.07	0.51	1.43	2.22	1.89	0.78	3.66	1.44	2.57	1.08	3.49	2.25	-0.58	7.55	4.07	4.38	1023
0.11	0.50	0.60	0.53	0.45	0.75	0.15	0.63	1.75	2.58	2.24	1.10	4.06	1.48	2.97	1.23	4.12	2.80	-0.33	8.57	4.45	5.19	989
0.15	0.78	0.91	0.89	0.70	1.12	0.21	0.90	1.99	2.90	2.54	1.30	4.51	1.60	3.34	1.73	5.04	3.60	-0.04	10.12	5.08	6.49	893
0.18	0.83	0.98	0.93	0.77	1.19	0.21	0.96	2.13	3.05	2.66	1.39	4.71	1.66	3.53	1.83	5.52	4.06	0.00	11.04	5.52	7.17	993
0.32	1.16	1.47	1.48	1.10	1.85	0.38	1.80	2.25	3.26	2.85	1.60	4.92	1.66	3.76	2.09	6.38	4.69	0.11	12.65	6.27	8.52	2714


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/time_misc_auc.tex <==
name	auc
attack_time	0.31
l2	0.83
lom	1.47


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.40	0.52	0.60	0.31	0.72	0.21	0.60	0.67	0.72	0.75	0.57	0.88	0.15	0.81	0.74	0.80	0.83	0.69	0.91	0.11	0.88	956
0.06	0.25	0.38	0.40	0.14	0.61	0.23	0.50	0.60	0.68	0.71	0.52	0.83	0.15	0.79	0.72	0.78	0.80	0.67	0.88	0.11	0.85	1023
0.11	0.00	0.23	0.20	0.01	0.44	0.21	0.40	0.50	0.59	0.62	0.44	0.75	0.16	0.69	0.67	0.72	0.74	0.61	0.83	0.11	0.80	989
0.15	0.00	0.14	0.00	-0.04	0.32	0.18	0.25	0.43	0.51	0.53	0.36	0.65	0.14	0.62	0.61	0.67	0.68	0.56	0.77	0.11	0.74	893
0.18	0.00	0.10	0.00	-0.05	0.26	0.16	0.20	0.33	0.43	0.44	0.29	0.57	0.14	0.53	0.56	0.62	0.63	0.51	0.73	0.11	0.69	993
0.32	0.00	0.06	0.00	-0.07	0.19	0.13	0.00	0.19	0.30	0.30	0.15	0.44	0.15	0.40	0.44	0.52	0.52	0.41	0.63	0.11	0.60	2714


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/ig/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.14
top50	0.19


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	110.03	179.70	159.45	83.34	276.05	96.35	220.92	7.00	10.18	10.00	6.19	14.17	3.99	12.25	125.28	201.35	178.15	96.89	305.80	104.45	246.58	7.00	10.11	10.00	6.15	14.07	3.96	12.00	880
0.06	121.89	238.96	186.04	2.08	475.83	236.88	276.41	6.00	8.56	8.00	4.66	12.47	3.91	11.00	154.38	281.69	216.31	31.32	532.06	250.37	327.43	6.00	8.49	8.00	4.67	12.32	3.82	11.00	966
0.11	120.32	231.73	182.59	18.94	444.52	212.79	273.87	6.00	8.62	8.00	4.74	12.51	3.89	11.00	170.89	306.12	243.82	56.74	555.51	249.38	362.38	6.00	8.48	8.00	4.70	12.26	3.78	11.00	966
0.15	117.95	221.95	179.30	22.02	421.88	199.93	264.26	6.00	8.95	9.00	5.06	12.85	3.89	11.00	194.98	341.28	276.90	85.90	596.66	255.38	400.97	6.00	8.78	8.00	4.96	12.60	3.82	11.00	889
0.18	119.41	223.44	181.50	49.41	397.47	174.03	271.89	6.00	8.59	8.00	4.70	12.49	3.90	11.00	238.89	404.52	342.09	132.93	676.11	271.59	479.40	5.00	8.38	8.00	4.56	12.19	3.81	11.00	998
0.32	118.90	229.73	181.27	19.41	440.05	210.32	273.66	6.00	8.62	8.00	4.66	12.59	3.96	11.00	338.91	582.55	486.37	205.86	959.25	376.69	712.92	5.00	8.22	8.00	4.41	12.02	3.80	11.00	2704


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/comparison_vals_auc.tex <==
name	auc
orig_pp	65.46
orig_ge	2.53
adv_pp	114.72
adv_ge	2.47


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.33	0.46	0.46	0.27	0.65	0.19	0.60	0.62	0.72	0.75	0.55	0.88	0.17	0.84	0.48	0.59	0.61	0.43	0.76	0.17	0.72	880
0.06	0.23	0.36	0.36	0.16	0.56	0.20	0.50	0.54	0.64	0.66	0.46	0.82	0.18	0.77	0.41	0.52	0.54	0.35	0.69	0.17	0.64	966
0.11	0.11	0.23	0.22	0.06	0.41	0.17	0.34	0.42	0.53	0.57	0.34	0.73	0.19	0.67	0.32	0.42	0.44	0.26	0.59	0.16	0.54	966
0.15	0.02	0.12	0.11	-0.03	0.27	0.15	0.22	0.30	0.41	0.43	0.22	0.61	0.20	0.56	0.22	0.32	0.33	0.16	0.48	0.16	0.43	889
0.18	-0.06	0.03	0.02	-0.10	0.17	0.14	0.11	0.16	0.28	0.29	0.08	0.48	0.20	0.43	0.12	0.21	0.21	0.06	0.36	0.15	0.32	998
0.32	-0.23	-0.13	-0.13	-0.27	0.02	0.15	-0.04	-0.16	0.02	0.02	-0.22	0.25	0.24	0.18	-0.11	0.02	0.01	-0.16	0.19	0.17	0.13	2704


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/correlations_auc.tex <==
name	auc
pcc	0.03
spearman	0.10
kendall	0.08


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	2.82	4.57	3.96	1.87	7.27	2.70	5.64	2.59	5.09	4.00	1.45	8.73	3.64	6.66	3.13	9.37	6.23	1.07	17.66	8.30	13.23	880
0.06	2.66	4.11	3.60	1.86	6.36	2.25	4.91	2.43	4.49	3.60	1.32	7.67	3.17	5.38	2.81	9.14	5.64	0.29	17.99	8.85	12.61	966
0.11	2.72	3.72	3.40	2.13	5.31	1.59	4.34	2.47	3.94	3.29	1.62	6.26	2.32	4.69	2.74	7.94	4.85	-0.08	15.97	8.02	10.21	966
0.15	2.64	3.44	3.19	2.14	4.74	1.30	3.89	2.46	3.58	3.13	1.79	5.37	1.79	4.18	2.56	6.93	4.40	-0.69	14.54	7.62	7.44	889
0.18	2.52	3.16	2.99	2.11	4.21	1.05	3.54	2.35	3.23	2.93	1.86	4.60	1.37	3.70	2.37	5.49	3.76	-0.19	11.18	5.69	5.96	998
0.32	2.31	2.79	2.68	2.02	3.57	0.77	3.11	2.22	2.82	2.62	1.88	3.76	0.94	3.16	2.12	3.95	3.00	0.47	7.43	3.48	4.45	2704


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/ets_sts_auc.tex <==
name	auc
et_use	0.99
et_tse	1.03
et_ce	1.85


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.05	6.06	1.79	-17.17	29.28	23.23	3.69	4.02	9.05	6.96	1.79	16.31	7.26	11.96	3.53	10.55	7.04	-1.01	22.12	11.56	13.74	880
0.06	0.79	5.17	1.46	-13.04	23.39	18.22	2.98	3.85	8.52	6.47	1.76	15.28	6.76	11.00	3.51	10.98	6.38	-4.24	26.21	15.23	12.95	966
0.11	0.61	3.45	1.04	-10.99	17.88	14.43	2.27	4.00	7.51	5.87	1.34	13.69	6.18	9.20	3.44	10.02	5.65	-10.38	30.42	20.40	10.56	966
0.15	0.46	1.72	0.73	-2.27	5.70	3.98	1.44	3.77	6.32	5.18	1.94	10.70	4.38	7.63	3.19	7.53	4.92	-3.39	18.45	10.92	8.13	889
0.18	0.33	1.92	0.54	-6.42	10.26	8.34	1.05	3.66	5.76	4.78	2.36	9.17	3.40	6.67	3.12	6.83	4.44	-2.85	16.51	9.68	7.31	998
0.32	0.21	1.05	0.34	-5.98	8.08	7.03	0.61	3.53	5.10	4.38	2.28	7.93	2.83	5.64	3.00	6.11	3.95	-4.63	16.85	10.74	5.93	2704


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.74
et_p_h	1.88
et_p_l2	2.32


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.07	0.17	0.14	0.04	0.30	0.13	0.23	0.02	0.05	0.04	0.01	0.09	0.04	0.07	0.02	0.04	0.04	0.02	0.07	0.03	0.06	880
0.06	0.10	0.27	0.22	0.05	0.49	0.22	0.39	0.03	0.06	0.05	0.02	0.10	0.04	0.09	0.03	0.05	0.05	0.02	0.08	0.03	0.07	966
0.11	0.17	0.44	0.36	0.09	0.79	0.35	0.61	0.04	0.08	0.07	0.03	0.13	0.05	0.11	0.04	0.07	0.07	0.04	0.10	0.03	0.09	966
0.15	0.31	0.68	0.59	0.18	1.17	0.50	0.93	0.05	0.10	0.09	0.04	0.15	0.06	0.14	0.06	0.09	0.08	0.05	0.12	0.04	0.11	889
0.18	0.45	1.02	0.90	0.26	1.78	0.76	1.45	0.07	0.11	0.11	0.06	0.17	0.06	0.15	0.07	0.10	0.10	0.06	0.14	0.04	0.13	998
0.32	0.90	2.05	1.63	0.35	3.75	1.70	2.69	0.09	0.14	0.14	0.08	0.21	0.06	0.19	0.10	0.13	0.13	0.09	0.17	0.04	0.16	2704


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.28
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.93	0.93	0.91	0.96	0.03	0.95	0.91	0.93	0.94	0.89	0.97	0.04	0.96	0.92	0.94	0.96	0.88	1.00	0.06	0.98	880
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.88	0.91	0.91	0.86	0.95	0.04	0.94	0.89	0.92	0.95	0.85	0.99	0.07	0.98	966
0.11	0.86	0.89	0.89	0.85	0.92	0.04	0.91	0.85	0.88	0.89	0.83	0.93	0.05	0.92	0.86	0.90	0.92	0.82	0.98	0.08	0.96	966
0.15	0.84	0.86	0.86	0.82	0.90	0.04	0.88	0.82	0.86	0.86	0.81	0.91	0.05	0.89	0.83	0.88	0.90	0.79	0.97	0.09	0.94	889
0.18	0.81	0.84	0.84	0.80	0.88	0.04	0.86	0.80	0.83	0.84	0.78	0.88	0.05	0.87	0.80	0.85	0.87	0.76	0.94	0.09	0.92	998
0.32	0.76	0.79	0.79	0.74	0.84	0.05	0.82	0.75	0.78	0.78	0.73	0.84	0.06	0.82	0.74	0.80	0.81	0.69	0.90	0.11	0.87	2704


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	1.28	1.31	1.34	1.09	1.53	0.22	1.37	31.40	62.53	46.29	3.48	121.58	59.05	72.81	1.25	3.63	2.73	0.42	6.83	3.21	5.03	880
0.06	0.57	0.74	0.77	0.53	0.94	0.20	0.93	33.15	61.48	46.67	1.18	121.79	60.30	72.31	1.13	3.06	2.29	0.28	5.85	2.79	4.17	966
0.11	0.40	0.46	0.41	0.30	0.62	0.16	0.46	39.03	69.88	55.37	9.64	130.13	60.24	82.33	1.26	3.46	2.64	0.45	6.46	3.01	4.65	966
0.15	0.50	0.51	0.51	0.48	0.55	0.03	0.52	45.10	78.67	63.43	24.71	132.62	53.96	94.98	1.38	3.85	3.00	0.59	7.10	3.26	5.45	889
0.18	0.70	0.74	0.74	0.66	0.81	0.07	0.77	48.98	84.63	67.58	27.67	141.58	56.95	102.78	1.51	4.00	3.09	0.50	7.50	3.50	5.50	998
0.32	0.91	1.39	1.30	0.90	1.88	0.49	1.71	50.19	87.55	71.15	27.71	147.40	59.84	104.59	1.60	4.31	3.43	0.65	7.97	3.66	5.99	2704


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/time_misc_auc.tex <==
name	auc
attack_time	0.24
l2	22.64
lom	1.11


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.20	0.40	0.40	0.17	0.62	0.22	0.60	0.56	0.67	0.69	0.52	0.82	0.15	0.80	0.74	0.80	0.81	0.70	0.90	0.10	0.88	880
0.06	0.00	0.29	0.25	0.06	0.52	0.23	0.40	0.50	0.61	0.62	0.46	0.76	0.15	0.73	0.70	0.76	0.78	0.66	0.87	0.10	0.84	966
0.11	0.00	0.20	0.20	-0.01	0.40	0.20	0.33	0.44	0.54	0.56	0.39	0.69	0.15	0.64	0.67	0.72	0.73	0.62	0.82	0.10	0.80	966
0.15	0.00	0.12	0.00	-0.04	0.29	0.17	0.20	0.38	0.45	0.46	0.32	0.59	0.14	0.55	0.60	0.67	0.67	0.57	0.77	0.10	0.74	889
0.18	0.00	0.07	0.00	-0.06	0.21	0.13	0.20	0.30	0.38	0.38	0.24	0.51	0.13	0.47	0.55	0.61	0.62	0.51	0.71	0.10	0.68	998
0.32	0.00	0.03	0.00	-0.06	0.12	0.09	0.00	0.14	0.24	0.23	0.11	0.38	0.13	0.33	0.44	0.51	0.50	0.40	0.62	0.11	0.58	2704


==> data/mlm_plots/mlm_distil_fast/agnews/lstm/s/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.12
top50	0.19


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	105.90	178.25	158.43	77.85	278.66	100.41	217.26	7.00	10.00	10.00	6.02	13.97	3.97	12.00	119.82	196.87	174.79	88.80	304.93	108.07	238.38	7.00	9.86	10.00	5.93	13.80	3.93	12.00	950
0.06	120.45	238.00	183.99	6.00	470.01	232.00	276.19	6.00	8.40	8.00	4.54	12.27	3.87	11.00	146.03	269.67	209.86	25.86	513.48	243.81	322.33	5.00	8.20	8.00	4.38	12.02	3.82	10.00	1032
0.11	119.24	233.04	183.57	20.16	445.92	212.88	273.99	6.00	8.52	8.00	4.69	12.35	3.83	11.00	161.33	290.51	235.18	55.94	525.08	234.57	344.09	5.00	8.25	8.00	4.48	12.02	3.77	10.00	988
0.15	117.62	220.09	177.88	24.78	415.40	195.31	263.08	6.00	8.85	9.00	4.98	12.72	3.87	11.00	177.39	315.88	255.35	53.46	578.30	262.42	382.01	6.00	8.46	8.00	4.67	12.24	3.79	11.00	895
0.18	118.85	223.33	180.57	48.31	398.36	175.03	269.69	6.00	8.52	8.00	4.67	12.37	3.85	11.00	215.40	362.41	305.72	133.03	591.80	229.38	438.21	5.00	8.06	8.00	4.31	11.81	3.75	10.00	997
0.32	118.32	226.78	181.09	36.30	417.26	190.48	272.66	6.00	8.53	8.00	4.60	12.45	3.92	11.00	300.63	517.53	432.42	187.98	847.08	329.55	643.01	5.00	7.76	7.00	4.08	11.43	3.68	10.00	2708


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/comparison_vals_auc.tex <==
name	auc
orig_pp	65.18
orig_ge	2.50
adv_pp	104.51
adv_ge	2.37


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.02	0.28	0.35	-0.13	0.69	0.41	0.60	0.05	0.30	0.36	-0.09	0.70	0.40	0.61	0.06	0.26	0.28	-0.05	0.57	0.31	0.49	950
0.06	-0.10	0.21	0.25	-0.22	0.63	0.42	0.55	-0.06	0.23	0.26	-0.20	0.66	0.43	0.59	-0.02	0.20	0.21	-0.13	0.53	0.33	0.46	1032
0.11	-0.35	0.01	0.01	-0.44	0.46	0.45	0.37	-0.31	0.04	0.02	-0.41	0.49	0.45	0.39	-0.20	0.05	0.03	-0.29	0.39	0.34	0.30	988
0.15	-0.53	-0.21	-0.24	-0.62	0.21	0.41	0.10	-0.48	-0.16	-0.21	-0.58	0.26	0.42	0.11	-0.32	-0.10	-0.13	-0.41	0.22	0.31	0.10	895
0.18	-0.66	-0.35	-0.43	-0.74	0.04	0.39	-0.11	-0.60	-0.30	-0.38	-0.70	0.11	0.41	-0.06	-0.42	-0.20	-0.25	-0.51	0.10	0.31	-0.03	997
0.32	-0.83	-0.57	-0.67	-0.92	-0.22	0.35	-0.42	-0.77	-0.52	-0.62	-0.88	-0.16	0.36	-0.39	-0.59	-0.39	-0.44	-0.67	-0.10	0.29	-0.26	2708


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/correlations_auc.tex <==
name	auc
pcc	-0.06
spearman	-0.05
kendall	-0.03


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	2.54	5.20	4.41	1.59	8.81	3.61	7.06	2.47	5.66	4.30	0.96	10.36	4.70	7.32	2.58	9.59	5.42	-1.41	20.58	10.99	12.34	950
0.06	2.12	4.24	3.73	1.34	7.14	2.90	5.55	2.11	4.57	3.67	0.95	8.19	3.62	5.86	2.55	8.72	4.86	-1.93	19.37	10.65	10.19	1032
0.11	2.37	4.13	3.67	1.66	6.60	2.47	5.35	2.37	4.29	3.67	1.49	7.10	2.81	5.57	2.61	8.22	4.56	-2.56	19.01	10.79	9.14	988
0.15	2.79	4.05	3.78	2.05	6.06	2.01	5.00	2.72	4.14	3.74	1.97	6.30	2.17	5.20	2.81	6.76	4.30	-0.79	14.30	7.55	7.23	895
0.18	2.88	3.87	3.75	2.19	5.56	1.68	4.63	2.78	3.93	3.69	2.19	5.67	1.74	4.81	2.75	6.14	4.31	-0.92	13.19	7.06	6.43	997
0.32	2.92	3.59	3.52	2.39	4.79	1.20	4.14	2.84	3.63	3.47	2.34	4.92	1.29	4.24	2.78	4.68	3.79	0.67	8.69	4.01	5.29	2708


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/ets_sts_auc.tex <==
name	auc
et_use	1.16
et_tse	1.19
et_ce	1.95


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.21	8.20	2.46	-16.77	33.18	24.97	5.58	4.87	13.03	8.95	0.05	26.01	12.98	16.32	4.47	15.95	9.49	-7.55	39.45	23.50	18.28	950
0.06	0.98	5.19	2.01	-7.29	17.68	12.49	4.48	5.00	11.79	8.56	0.93	22.64	10.85	14.74	4.66	15.53	8.84	-6.61	37.67	22.14	17.31	1032
0.11	0.84	6.29	1.53	-20.35	32.94	26.65	3.33	4.90	10.43	7.97	1.54	19.32	8.89	13.06	4.45	12.97	7.99	-5.64	31.58	18.61	14.80	988
0.15	0.70	3.30	1.27	-7.59	14.19	10.89	2.48	5.03	9.38	7.66	2.17	16.59	7.21	11.41	4.49	10.69	7.19	-1.13	22.51	11.82	12.05	895
0.18	0.57	2.50	0.99	-5.09	10.09	7.59	1.84	5.23	8.58	7.23	3.08	14.08	5.50	10.12	4.47	9.86	6.50	-1.80	21.52	11.66	11.21	997
0.32	0.33	2.01	0.58	-8.95	12.96	10.95	1.09	5.06	7.59	6.47	2.56	12.63	5.04	8.62	4.28	8.78	5.86	-5.29	22.85	14.07	8.80	2708


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/ets_time_misc_auc.tex <==
name	auc
et_p	1.08
et_p_h	2.72
et_p_l2	3.26


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.06	0.16	0.12	0.03	0.30	0.14	0.22	0.02	0.04	0.03	0.01	0.08	0.04	0.06	0.02	0.04	0.03	0.02	0.07	0.03	0.05	950
0.06	0.08	0.23	0.18	0.04	0.43	0.19	0.32	0.02	0.05	0.04	0.01	0.09	0.04	0.07	0.03	0.05	0.04	0.02	0.08	0.03	0.06	1032
0.11	0.14	0.37	0.29	0.06	0.68	0.31	0.53	0.03	0.07	0.06	0.02	0.11	0.05	0.10	0.04	0.06	0.06	0.03	0.10	0.03	0.08	988
0.15	0.22	0.56	0.47	0.13	0.98	0.43	0.77	0.05	0.09	0.08	0.04	0.14	0.05	0.12	0.05	0.08	0.08	0.05	0.11	0.03	0.10	895
0.18	0.37	0.82	0.70	0.17	1.48	0.65	1.10	0.06	0.11	0.10	0.05	0.16	0.05	0.14	0.07	0.10	0.09	0.06	0.13	0.04	0.12	997
0.32	0.71	1.73	1.34	0.19	3.26	1.53	2.26	0.09	0.14	0.14	0.07	0.20	0.06	0.18	0.09	0.12	0.12	0.08	0.17	0.04	0.15	2708


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.24
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.90	0.92	0.92	0.89	0.95	0.03	0.94	0.90	0.92	0.92	0.88	0.96	0.04	0.95	0.89	0.92	0.94	0.86	0.99	0.07	0.97	950
0.06	0.88	0.90	0.90	0.86	0.93	0.03	0.92	0.87	0.89	0.90	0.85	0.94	0.05	0.93	0.87	0.91	0.93	0.83	0.98	0.08	0.96	1032
0.11	0.85	0.87	0.87	0.83	0.91	0.04	0.89	0.83	0.87	0.87	0.82	0.92	0.05	0.90	0.84	0.88	0.90	0.80	0.97	0.08	0.95	988
0.15	0.82	0.84	0.84	0.80	0.88	0.04	0.86	0.81	0.84	0.84	0.79	0.89	0.05	0.88	0.80	0.85	0.87	0.77	0.94	0.09	0.92	895
0.18	0.79	0.81	0.82	0.77	0.86	0.04	0.84	0.78	0.81	0.81	0.76	0.87	0.05	0.85	0.78	0.83	0.84	0.74	0.92	0.09	0.90	997
0.32	0.74	0.77	0.77	0.72	0.82	0.05	0.80	0.73	0.77	0.77	0.71	0.83	0.06	0.81	0.72	0.78	0.79	0.68	0.88	0.10	0.85	2708


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.24


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	3.79	3.76	3.95	2.87	4.66	0.89	4.05	0.03	0.06	0.05	0.02	0.09	0.03	0.07	1.44	3.52	2.90	0.82	6.22	2.70	5.02	950
0.06	0.39	0.45	0.45	0.39	0.51	0.06	0.46	0.04	0.07	0.06	0.03	0.11	0.04	0.09	1.34	3.42	2.82	0.73	6.10	2.68	4.83	1032
0.11	0.55	0.59	0.57	0.52	0.66	0.07	0.62	0.05	0.08	0.07	0.04	0.12	0.04	0.10	1.71	4.14	3.35	0.98	7.30	3.16	5.73	988
0.15	0.61	0.67	0.65	0.59	0.75	0.08	0.70	0.06	0.09	0.08	0.05	0.13	0.04	0.12	2.13	5.07	4.24	1.28	8.86	3.79	7.14	895
0.18	0.88	0.94	0.93	0.87	1.01	0.07	0.99	0.06	0.10	0.09	0.05	0.15	0.05	0.13	2.32	5.40	4.58	1.45	9.34	3.95	7.61	997
0.32	1.11	1.46	1.47	1.13	1.79	0.33	1.70	0.07	0.11	0.10	0.06	0.16	0.05	0.14	2.68	6.00	5.01	1.63	10.38	4.38	8.42	2708


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/time_misc_auc.tex <==
name	auc
attack_time	0.30
l2	0.03
lom	1.43


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.24	0.00	-0.07	0.55	0.31	0.40	0.20	0.43	0.44	0.17	0.69	0.26	0.62	0.48	0.60	0.62	0.42	0.78	0.18	0.74	950
0.06	0.00	0.19	0.00	-0.10	0.48	0.29	0.33	0.14	0.37	0.36	0.11	0.63	0.26	0.56	0.42	0.57	0.56	0.36	0.77	0.20	0.72	1032
0.11	0.00	0.12	0.00	-0.12	0.36	0.24	0.20	0.06	0.27	0.23	0.03	0.52	0.24	0.44	0.33	0.49	0.48	0.28	0.70	0.21	0.62	988
0.15	0.00	0.07	0.00	-0.11	0.26	0.18	0.00	0.00	0.19	0.12	-0.02	0.40	0.21	0.31	0.28	0.41	0.41	0.22	0.60	0.19	0.52	895
0.18	0.00	0.04	0.00	-0.11	0.19	0.15	0.00	0.00	0.14	0.06	-0.05	0.33	0.19	0.23	0.22	0.35	0.33	0.17	0.54	0.19	0.46	997
0.32	0.00	0.02	0.00	-0.09	0.13	0.11	0.00	0.00	0.07	0.00	-0.08	0.22	0.15	0.08	0.13	0.26	0.23	0.09	0.43	0.17	0.35	2708


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/a/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.06
top50	0.12


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	105.63	177.45	157.20	76.80	278.10	100.65	216.76	7.00	10.08	10.00	6.10	14.07	3.99	12.00	122.57	199.53	173.57	85.80	313.27	113.74	245.00	7.00	9.91	10.00	5.93	13.88	3.98	12.00	944
0.06	121.88	237.21	186.19	7.23	467.19	229.98	273.94	5.25	8.42	8.00	4.55	12.30	3.88	11.00	147.64	276.38	220.04	43.92	508.83	232.45	326.44	5.00	8.21	8.00	4.37	12.05	3.84	10.00	1018
0.11	118.32	229.93	182.15	21.34	438.53	208.59	268.94	6.00	8.50	8.00	4.66	12.35	3.84	11.00	160.35	291.55	231.44	52.35	530.74	239.20	345.68	5.00	8.22	8.00	4.45	11.98	3.76	10.00	985
0.15	117.60	219.99	177.99	25.41	414.58	194.58	262.82	6.00	8.86	9.00	4.99	12.73	3.87	11.00	177.28	309.94	254.98	103.72	516.16	206.22	384.74	6.00	8.47	8.00	4.71	12.23	3.76	11.00	906
0.18	118.82	222.73	179.99	47.80	397.66	174.93	269.22	6.00	8.52	8.00	4.67	12.37	3.85	11.00	204.23	350.38	288.31	120.68	580.08	229.70	428.37	5.00	8.05	8.00	4.38	11.72	3.67	10.00	1000
0.32	118.57	229.32	181.27	21.84	436.80	207.48	272.59	6.00	8.53	8.00	4.61	12.44	3.91	11.00	283.84	479.33	405.19	182.73	775.92	296.60	586.96	5.00	7.88	7.00	4.21	11.54	3.66	10.00	2718


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	65.12
orig_ge	2.50
adv_pp	101.01
adv_ge	2.38


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.21	0.38	0.43	0.09	0.68	0.29	0.59	0.50	0.60	0.65	0.36	0.83	0.24	0.75	0.41	0.51	0.55	0.30	0.72	0.21	0.66	944
0.06	0.04	0.24	0.26	-0.07	0.55	0.31	0.45	0.37	0.49	0.54	0.24	0.74	0.25	0.65	0.31	0.42	0.45	0.21	0.64	0.21	0.57	1018
0.11	-0.13	0.06	0.06	-0.23	0.35	0.29	0.24	0.22	0.35	0.37	0.11	0.59	0.24	0.50	0.19	0.30	0.32	0.10	0.50	0.20	0.44	985
0.15	-0.32	-0.12	-0.14	-0.40	0.15	0.28	0.05	0.06	0.19	0.21	-0.05	0.43	0.24	0.34	0.08	0.18	0.20	-0.01	0.38	0.19	0.30	906
0.18	-0.42	-0.24	-0.26	-0.50	0.03	0.26	-0.07	-0.07	0.07	0.08	-0.16	0.30	0.23	0.22	-0.02	0.09	0.09	-0.10	0.27	0.18	0.20	1000
0.32	-0.57	-0.41	-0.43	-0.64	-0.17	0.23	-0.27	-0.29	-0.13	-0.13	-0.36	0.11	0.24	0.03	-0.19	-0.07	-0.07	-0.25	0.12	0.18	0.06	2718


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/correlations_auc.tex <==
name	auc
pcc	-0.04
spearman	0.05
kendall	0.05


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	2.59	4.67	4.12	1.53	7.80	3.13	5.92	2.56	5.30	3.97	0.48	10.13	4.82	6.43	2.77	8.57	5.26	-0.10	17.24	8.67	11.09	944
0.06	2.55	4.16	3.58	1.56	6.76	2.60	5.09	2.44	4.59	3.64	0.77	8.41	3.82	5.52	2.82	8.54	4.84	-0.95	18.04	9.50	10.62	1018
0.11	2.63	3.97	3.52	1.92	6.03	2.06	4.79	2.49	4.22	3.56	1.53	6.92	2.70	5.07	2.92	8.15	4.79	-1.08	17.37	9.22	8.96	985
0.15	2.67	3.79	3.41	2.07	5.50	1.72	4.43	2.48	3.83	3.36	1.87	5.78	1.95	4.68	2.78	6.49	4.36	-0.43	13.42	6.93	7.30	906
0.18	2.59	3.53	3.26	2.08	4.97	1.44	4.15	2.45	3.54	3.17	1.86	5.21	1.67	4.25	2.66	5.51	3.90	0.29	10.72	5.22	6.10	1000
0.32	2.51	3.16	2.98	2.10	4.21	1.05	3.56	2.41	3.15	2.90	1.98	4.32	1.17	3.57	2.49	4.11	3.38	1.25	6.98	2.87	4.81	2718


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/ets_sts_auc.tex <==
name	auc
et_use	1.07
et_tse	1.11
et_ce	1.82


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.11	6.75	1.94	-13.71	27.20	20.46	4.42	4.77	11.73	8.26	0.74	22.71	10.99	15.19	4.21	14.26	8.40	-4.34	32.86	18.60	17.46	944
0.06	0.91	5.56	1.76	-11.03	22.14	16.59	3.81	4.95	11.46	8.42	1.40	21.52	10.06	14.56	4.33	15.04	8.60	-8.38	38.46	23.42	16.54	1018
0.11	0.85	5.19	1.47	-10.34	20.73	15.53	3.30	5.25	10.10	7.96	1.79	18.41	8.31	12.45	4.57	12.49	7.95	-9.88	34.87	22.38	14.10	985
0.15	0.70	4.76	1.15	-12.58	22.09	17.33	2.33	5.31	8.98	7.47	3.21	14.74	5.76	10.79	4.40	10.69	7.01	-4.71	26.09	15.40	12.00	906
0.18	0.57	3.49	0.96	-16.45	23.43	19.94	1.98	5.09	8.55	7.01	2.98	14.11	5.56	10.42	4.31	10.39	6.42	-7.04	27.82	17.43	11.19	1000
0.32	0.33	2.65	0.59	-13.02	18.31	15.66	1.16	4.78	7.18	6.06	2.87	11.50	4.31	8.28	4.03	8.28	5.48	-5.25	21.81	13.53	8.67	2718


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/ets_time_misc_auc.tex <==
name	auc
et_p	1.21
et_p_h	2.63
et_p_l2	3.21


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.07	0.17	0.14	0.03	0.31	0.14	0.24	0.02	0.04	0.03	0.01	0.08	0.03	0.06	0.02	0.04	0.03	0.02	0.07	0.02	0.06	944
0.06	0.10	0.26	0.21	0.04	0.48	0.22	0.36	0.02	0.05	0.04	0.01	0.09	0.04	0.07	0.03	0.05	0.04	0.02	0.08	0.03	0.07	1018
0.11	0.14	0.38	0.31	0.07	0.69	0.31	0.52	0.03	0.07	0.06	0.02	0.11	0.04	0.10	0.04	0.06	0.06	0.03	0.09	0.03	0.08	985
0.15	0.23	0.57	0.48	0.12	1.02	0.45	0.78	0.05	0.09	0.08	0.04	0.14	0.05	0.12	0.05	0.08	0.08	0.04	0.11	0.03	0.10	906
0.18	0.31	0.77	0.65	0.17	1.38	0.61	1.06	0.06	0.10	0.10	0.05	0.15	0.05	0.14	0.06	0.09	0.09	0.05	0.13	0.04	0.11	1000
0.32	0.59	1.56	1.18	0.14	2.98	1.42	2.11	0.08	0.13	0.13	0.07	0.19	0.06	0.17	0.09	0.12	0.12	0.07	0.16	0.04	0.15	2718


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.22
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.91	0.92	0.93	0.90	0.95	0.03	0.94	0.90	0.92	0.93	0.89	0.96	0.04	0.95	0.90	0.93	0.95	0.88	0.98	0.05	0.97	944
0.06	0.87	0.90	0.90	0.86	0.93	0.03	0.92	0.86	0.89	0.90	0.85	0.94	0.05	0.93	0.87	0.91	0.92	0.85	0.98	0.07	0.97	1018
0.11	0.84	0.87	0.87	0.83	0.91	0.04	0.90	0.83	0.87	0.87	0.81	0.92	0.05	0.90	0.85	0.89	0.90	0.81	0.97	0.08	0.95	985
0.15	0.81	0.84	0.84	0.79	0.88	0.05	0.87	0.79	0.83	0.83	0.77	0.89	0.06	0.88	0.81	0.86	0.87	0.77	0.94	0.09	0.92	906
0.18	0.78	0.81	0.81	0.76	0.86	0.05	0.84	0.76	0.80	0.81	0.74	0.86	0.06	0.85	0.77	0.83	0.84	0.74	0.92	0.09	0.90	1000
0.32	0.73	0.76	0.76	0.71	0.82	0.05	0.80	0.72	0.76	0.76	0.70	0.82	0.06	0.80	0.72	0.78	0.79	0.67	0.88	0.11	0.85	2718


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	7.33	7.20	7.62	5.43	8.97	1.77	7.88	0.97	2.07	1.50	-0.06	4.20	2.13	2.36	1.80	6.14	4.09	-0.58	12.87	6.72	7.86	944
0.06	0.65	0.75	0.76	0.63	0.87	0.12	0.79	1.20	2.37	1.78	-0.05	4.80	2.42	2.62	1.57	5.39	3.62	-0.31	11.09	5.70	7.03	1018
0.11	0.63	0.74	0.66	0.53	0.96	0.22	0.74	1.46	2.78	2.12	-0.17	5.73	2.95	3.01	2.08	6.59	4.65	0.04	13.15	6.55	8.88	985
0.15	0.86	0.98	0.93	0.75	1.21	0.23	0.99	1.70	3.10	2.41	0.07	6.13	3.03	3.37	2.67	7.73	5.79	0.46	15.00	7.27	10.43	906
0.18	1.62	1.80	1.67	1.50	2.10	0.30	2.06	1.83	3.21	2.54	0.17	6.24	3.04	3.54	2.83	8.23	6.18	0.58	15.87	7.65	11.27	1000
0.32	1.63	2.21	2.19	1.56	2.85	0.64	2.75	1.93	3.24	2.65	0.55	5.93	2.69	3.57	3.40	9.24	7.12	1.07	17.42	8.17	12.67	2718


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/time_misc_auc.tex <==
name	auc
attack_time	0.51
l2	0.86
lom	2.22


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.40	0.49	0.60	0.30	0.68	0.19	0.60	0.60	0.69	0.73	0.54	0.83	0.15	0.80	0.70	0.77	0.79	0.64	0.89	0.12	0.85	944
0.06	0.20	0.34	0.33	0.11	0.56	0.22	0.50	0.55	0.62	0.64	0.46	0.78	0.16	0.73	0.65	0.72	0.74	0.60	0.85	0.13	0.81	1018
0.11	0.00	0.22	0.20	0.00	0.43	0.21	0.33	0.44	0.55	0.56	0.40	0.71	0.15	0.67	0.60	0.67	0.69	0.55	0.79	0.12	0.75	985
0.15	0.00	0.15	0.00	-0.04	0.33	0.18	0.25	0.38	0.47	0.47	0.32	0.62	0.15	0.57	0.56	0.62	0.63	0.50	0.74	0.12	0.70	906
0.18	0.00	0.11	0.00	-0.06	0.28	0.17	0.20	0.31	0.41	0.42	0.26	0.55	0.15	0.50	0.50	0.58	0.59	0.46	0.69	0.12	0.67	1000
0.32	0.00	0.07	0.00	-0.07	0.21	0.14	0.00	0.20	0.31	0.31	0.16	0.45	0.15	0.42	0.43	0.51	0.52	0.39	0.62	0.12	0.59	2718


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/ig/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.13
top50	0.18


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	106.05	181.38	159.68	78.00	284.76	103.38	225.64	7.00	10.15	10.00	6.21	14.09	3.94	12.00	121.04	203.36	179.45	93.15	313.57	110.21	250.61	7.00	10.06	10.00	6.14	13.99	3.92	12.00	872
0.06	118.89	236.08	183.85	1.77	470.39	234.31	273.51	6.00	8.44	8.00	4.55	12.33	3.89	11.00	149.66	275.99	227.37	55.68	496.29	220.30	325.90	5.00	8.30	8.00	4.47	12.14	3.83	11.00	964
0.11	117.98	230.56	182.41	17.42	443.69	213.13	269.56	6.00	8.58	8.00	4.73	12.42	3.84	11.00	165.60	304.48	242.04	71.77	537.18	232.70	362.19	5.00	8.41	8.00	4.60	12.23	3.82	11.00	960
0.15	117.41	220.47	177.81	24.33	416.62	196.14	263.13	6.00	8.86	9.00	4.99	12.74	3.88	11.00	195.23	339.39	278.38	93.94	584.83	245.45	405.93	6.00	8.64	8.00	4.84	12.43	3.80	11.00	891
0.18	118.71	223.18	180.56	48.96	397.41	174.23	271.19	6.00	8.53	8.00	4.68	12.38	3.85	11.00	229.57	400.08	331.05	118.85	681.30	281.22	484.87	5.00	8.31	8.00	4.52	12.11	3.80	10.00	999
0.32	118.22	228.30	180.54	22.68	433.92	205.62	272.10	6.00	8.56	8.00	4.63	12.48	3.93	11.00	328.70	590.05	490.28	154.61	1025.49	435.44	717.36	5.00	8.18	8.00	4.36	11.99	3.81	10.00	2716


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/comparison_vals_auc.tex <==
name	auc
orig_pp	65.15
orig_ge	2.51
adv_pp	114.51
adv_ge	2.44


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.33	0.46	0.47	0.26	0.66	0.20	0.60	0.59	0.69	0.74	0.50	0.89	0.19	0.83	0.43	0.55	0.57	0.37	0.72	0.18	0.67	872
0.06	0.26	0.39	0.40	0.19	0.59	0.20	0.52	0.57	0.67	0.70	0.47	0.86	0.19	0.81	0.42	0.52	0.54	0.35	0.70	0.17	0.65	964
0.11	0.15	0.27	0.26	0.08	0.45	0.18	0.39	0.45	0.57	0.61	0.36	0.79	0.22	0.73	0.33	0.44	0.46	0.26	0.62	0.18	0.57	960
0.15	0.05	0.16	0.15	-0.00	0.32	0.16	0.26	0.32	0.46	0.50	0.23	0.70	0.23	0.63	0.23	0.35	0.36	0.16	0.53	0.18	0.47	891
0.18	-0.02	0.08	0.07	-0.08	0.23	0.15	0.17	0.20	0.37	0.39	0.12	0.62	0.25	0.55	0.15	0.27	0.28	0.09	0.46	0.19	0.40	999
0.32	-0.19	-0.08	-0.09	-0.24	0.08	0.16	0.02	-0.09	0.12	0.11	-0.17	0.41	0.29	0.33	-0.06	0.09	0.08	-0.11	0.29	0.20	0.24	2716


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.12
kendall	0.09


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	2.72	4.87	4.15	1.93	7.81	2.94	6.09	2.80	5.73	4.38	1.16	10.29	4.56	7.11	3.19	10.04	6.59	0.98	19.10	9.06	14.68	872
0.06	2.57	4.04	3.51	1.83	6.25	2.21	4.86	2.49	4.49	3.64	1.25	7.73	3.24	5.58	3.18	9.91	6.23	0.87	18.96	9.05	14.41	964
0.11	2.62	3.72	3.32	2.00	5.45	1.72	4.43	2.50	4.04	3.44	1.54	6.54	2.50	4.79	2.92	8.92	5.10	-0.17	18.00	9.09	11.41	960
0.15	2.54	3.40	3.19	2.09	4.72	1.31	3.92	2.42	3.72	3.20	1.65	5.79	2.07	4.39	2.72	7.20	4.35	-0.20	14.60	7.40	8.35	891
0.18	2.44	3.13	2.94	2.05	4.21	1.08	3.56	2.30	3.35	3.00	1.70	4.99	1.65	3.95	2.51	5.86	3.76	-0.28	12.00	6.14	6.61	999
0.32	2.28	2.80	2.66	1.99	3.62	0.81	3.15	2.20	2.94	2.67	1.83	4.06	1.11	3.42	2.26	4.20	3.12	0.41	7.99	3.79	4.66	2716


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/ets_sts_auc.tex <==
name	auc
et_use	0.98
et_tse	1.07
et_ce	1.99


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.97	4.84	1.69	-7.97	17.66	12.82	3.93	4.24	9.20	6.87	0.88	17.53	8.32	11.59	3.89	11.21	7.05	-3.53	25.94	14.74	13.42	872
0.06	0.70	4.43	1.29	-10.90	19.76	15.33	2.74	3.86	8.33	6.28	1.32	15.35	7.01	10.35	3.47	10.95	6.46	-4.19	26.08	15.13	12.07	964
0.11	0.56	3.41	0.96	-10.80	17.62	14.21	2.02	3.75	7.24	5.46	1.68	12.80	5.56	8.74	3.33	9.63	5.43	-5.61	24.87	15.24	10.69	960
0.15	0.44	2.38	0.69	-6.06	10.82	8.44	1.39	3.58	6.21	5.00	1.95	10.47	4.26	7.61	3.12	7.81	4.92	-5.43	21.05	13.24	8.75	891
0.18	0.34	2.00	0.53	-6.95	10.95	8.95	0.96	3.54	5.70	4.53	1.87	9.53	3.83	6.46	3.03	7.31	4.38	-6.27	20.89	13.58	7.28	999
0.32	0.20	1.00	0.32	-3.75	5.74	4.75	0.58	3.34	5.02	4.17	1.87	8.17	3.15	5.63	2.89	6.27	3.84	-6.62	19.16	12.89	6.00	2716


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.72
et_p_h	1.85
et_p_l2	2.37


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.06	0.17	0.15	0.04	0.31	0.13	0.25	0.02	0.05	0.04	0.01	0.09	0.04	0.06	0.02	0.04	0.04	0.02	0.07	0.03	0.06	872
0.06	0.11	0.28	0.23	0.05	0.51	0.23	0.38	0.02	0.06	0.04	0.01	0.10	0.04	0.08	0.03	0.05	0.05	0.02	0.09	0.03	0.07	964
0.11	0.19	0.44	0.36	0.08	0.80	0.36	0.60	0.04	0.07	0.06	0.03	0.12	0.05	0.10	0.04	0.07	0.06	0.03	0.10	0.03	0.09	960
0.15	0.30	0.71	0.62	-0.11	1.52	0.82	0.93	0.05	0.09	0.08	0.04	0.15	0.05	0.13	0.06	0.09	0.08	0.05	0.12	0.04	0.11	891
0.18	0.46	1.00	0.86	0.26	1.74	0.74	1.37	0.06	0.11	0.11	0.05	0.17	0.06	0.15	0.07	0.10	0.10	0.06	0.14	0.04	0.13	999
0.32	0.91	2.07	1.63	0.35	3.78	1.72	2.77	0.09	0.14	0.14	0.07	0.21	0.07	0.19	0.10	0.13	0.13	0.08	0.17	0.05	0.16	2716


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.29
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.93	0.94	0.91	0.96	0.03	0.95	0.92	0.94	0.94	0.90	0.97	0.04	0.96	0.92	0.94	0.96	0.89	1.00	0.05	0.98	872
0.06	0.89	0.91	0.92	0.88	0.95	0.03	0.94	0.89	0.91	0.92	0.87	0.96	0.04	0.94	0.91	0.93	0.95	0.87	1.00	0.06	0.98	964
0.11	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.86	0.89	0.90	0.84	0.94	0.05	0.92	0.88	0.91	0.93	0.84	0.98	0.07	0.97	960
0.15	0.84	0.87	0.87	0.83	0.90	0.04	0.89	0.83	0.87	0.87	0.81	0.92	0.05	0.90	0.85	0.89	0.91	0.81	0.97	0.08	0.95	891
0.18	0.82	0.84	0.84	0.80	0.88	0.04	0.87	0.81	0.84	0.85	0.79	0.90	0.05	0.88	0.82	0.86	0.88	0.77	0.95	0.09	0.93	999
0.32	0.77	0.80	0.80	0.75	0.84	0.05	0.83	0.76	0.80	0.80	0.74	0.86	0.06	0.84	0.76	0.81	0.83	0.71	0.91	0.10	0.89	2716


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	6.43	6.48	6.70	5.07	7.90	1.42	6.99	13.48	42.51	26.52	-23.86	108.88	66.37	46.53	2.10	5.48	4.70	1.33	9.64	4.15	7.87	872
0.06	0.60	0.72	0.73	0.57	0.88	0.16	0.77	14.36	42.70	29.06	-5.55	90.94	48.24	50.63	1.62	4.62	3.63	0.76	8.48	3.86	6.60	964
0.11	0.73	0.86	0.86	0.71	1.01	0.15	0.98	16.51	49.19	33.90	-6.39	104.77	55.58	59.22	2.20	5.39	4.38	1.14	9.64	4.25	7.65	960
0.15	0.88	1.02	1.04	0.89	1.16	0.13	1.13	19.39	56.53	38.88	-7.17	120.22	63.69	66.42	2.64	6.33	5.32	1.68	10.98	4.65	9.21	891
0.18	1.20	1.37	1.33	1.17	1.57	0.20	1.47	21.38	59.86	41.21	-5.65	125.38	65.51	73.08	2.46	6.39	5.32	1.61	11.17	4.78	9.53	999
0.32	1.64	1.97	1.97	1.60	2.35	0.38	2.33	22.83	64.48	44.08	-7.42	136.38	71.90	79.17	2.86	7.00	5.95	1.93	12.06	5.06	10.46	2716


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/time_misc_auc.tex <==
name	auc
attack_time	0.45
l2	16.15
lom	1.77


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.20	0.36	0.40	0.14	0.58	0.22	0.60	0.53	0.63	0.67	0.48	0.79	0.16	0.75	0.70	0.78	0.78	0.67	0.88	0.11	0.85	872
0.06	0.00	0.27	0.25	0.05	0.50	0.23	0.40	0.50	0.61	0.62	0.44	0.77	0.16	0.73	0.70	0.77	0.78	0.66	0.88	0.11	0.85	964
0.11	0.00	0.20	0.20	0.00	0.39	0.20	0.33	0.43	0.53	0.54	0.36	0.70	0.17	0.67	0.65	0.73	0.74	0.61	0.84	0.12	0.81	960
0.15	0.00	0.12	0.00	-0.04	0.28	0.16	0.20	0.36	0.46	0.47	0.31	0.62	0.16	0.56	0.59	0.68	0.68	0.56	0.80	0.12	0.76	891
0.18	0.00	0.08	0.00	-0.06	0.21	0.14	0.20	0.31	0.40	0.40	0.24	0.56	0.16	0.50	0.56	0.64	0.64	0.52	0.76	0.12	0.73	999
0.32	0.00	0.03	0.00	-0.06	0.11	0.08	0.00	0.17	0.28	0.25	0.12	0.43	0.15	0.38	0.44	0.54	0.54	0.41	0.67	0.13	0.63	2716


==> data/mlm_plots/mlm_distil_fast/agnews/lstmatt/s/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.13
top50	0.19


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	58.71	113.45	115.09	56.40	170.50	57.05	150.53	2.00	3.11	3.00	1.41	4.80	1.69	4.00	87.13	131.41	129.13	69.14	193.68	62.27	171.27	2.00	3.29	3.00	1.58	5.00	1.71	4.75	66
0.06	93.32	168.54	136.83	41.41	295.66	127.13	202.74	3.00	4.65	5.00	2.66	6.63	1.99	6.00	114.31	204.15	170.06	57.58	350.73	146.57	243.74	3.00	4.68	5.00	2.65	6.72	2.04	6.00	1168
0.11	95.93	176.46	142.98	38.65	314.27	137.81	209.75	3.00	4.55	5.00	2.58	6.52	1.97	6.00	131.71	236.05	194.52	71.77	400.34	164.29	292.03	3.00	4.57	5.00	2.53	6.62	2.04	6.00	981
0.15	93.32	170.81	137.00	35.01	306.60	135.80	205.07	3.00	4.47	4.00	2.53	6.42	1.95	6.00	153.03	264.26	217.31	63.93	464.58	200.33	320.67	3.00	4.56	4.00	2.53	6.60	2.03	6.00	772
0.18	95.49	173.38	138.88	27.92	318.84	145.46	205.07	3.00	4.55	4.00	2.59	6.52	1.96	6.00	179.88	303.42	253.32	102.90	503.94	200.52	361.65	3.00	4.70	5.00	2.63	6.78	2.08	6.00	968
0.32	96.30	180.40	143.60	26.94	333.86	153.46	211.45	3.00	4.48	4.00	2.50	6.46	1.98	6.00	260.32	448.55	378.97	163.86	733.24	284.69	559.53	3.00	4.80	5.00	2.60	6.99	2.20	6.00	2660


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/comparison_vals_auc.tex <==
name	auc
orig_pp	49.71
orig_ge	1.29
adv_pp	86.89
adv_ge	1.34


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.21	0.43	0.39	0.13	0.73	0.30	0.65	0.81	0.86	0.89	0.77	0.95	0.09	0.93	0.64	0.71	0.71	0.60	0.82	0.11	0.80	66
0.06	0.11	0.33	0.31	0.07	0.60	0.27	0.54	0.65	0.73	0.77	0.56	0.91	0.18	0.86	0.50	0.59	0.61	0.43	0.75	0.16	0.69	1168
0.11	0.00	0.18	0.14	-0.05	0.41	0.23	0.31	0.49	0.62	0.66	0.39	0.85	0.23	0.79	0.36	0.48	0.50	0.29	0.67	0.19	0.61	981
0.15	-0.06	0.05	0.02	-0.12	0.23	0.17	0.14	0.36	0.52	0.56	0.26	0.78	0.26	0.72	0.26	0.39	0.41	0.19	0.60	0.20	0.55	772
0.18	-0.10	-0.01	-0.03	-0.17	0.14	0.16	0.06	0.21	0.42	0.45	0.13	0.71	0.29	0.66	0.15	0.31	0.33	0.09	0.53	0.22	0.48	968
0.32	-0.24	-0.15	-0.13	-0.31	0.01	0.16	-0.05	-0.11	0.17	0.18	-0.19	0.53	0.36	0.46	-0.07	0.12	0.12	-0.14	0.39	0.26	0.33	2660


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/correlations_auc.tex <==
name	auc
pcc	0.02
spearman	0.14
kendall	0.11


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	2.69	5.47	4.55	1.59	9.35	3.88	7.95	2.35	5.75	5.32	0.67	10.83	5.08	6.33	6.05	15.96	10.45	2.40	29.53	13.57	25.11	66
0.06	2.53	4.55	3.94	1.67	7.44	2.89	5.65	2.68	5.48	4.30	1.17	9.80	4.32	6.98	2.60	10.14	5.73	-0.60	20.88	10.74	13.97	1168
0.11	2.87	4.14	3.85	2.16	6.12	1.98	5.01	2.84	4.69	3.97	1.83	7.56	2.87	5.81	2.48	8.82	4.60	-1.28	18.91	10.09	10.85	981
0.15	2.86	3.76	3.55	2.36	5.16	1.40	4.33	2.81	4.20	3.67	2.03	6.37	2.17	4.91	2.56	7.66	4.40	-1.03	16.35	8.69	8.86	772
0.18	2.75	3.47	3.28	2.34	4.59	1.12	3.93	2.74	3.84	3.42	2.15	5.52	1.68	4.45	2.49	5.76	3.68	-0.49	12.01	6.25	6.20	968
0.32	2.44	3.00	2.85	2.16	3.83	0.84	3.36	2.51	3.27	3.02	2.12	4.41	1.14	3.70	2.19	3.96	3.02	0.50	7.42	3.46	4.49	2660


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/ets_sts_auc.tex <==
name	auc
et_use	1.09
et_tse	1.22
et_ce	2.08


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.52	2.69	1.64	-1.16	6.53	3.84	2.97	3.24	8.12	5.70	0.36	15.87	7.76	9.89	2.90	7.81	4.51	-1.15	16.77	8.96	8.92	66
0.06	0.69	5.13	1.30	-12.13	22.40	17.26	3.14	3.36	8.48	5.93	0.53	16.43	7.95	10.69	2.61	9.99	5.74	-6.34	26.33	16.34	11.77	1168
0.11	0.62	3.93	1.05	-9.14	17.01	13.07	2.49	3.70	7.25	5.72	1.62	12.89	5.63	9.08	2.83	7.84	5.01	-2.73	18.41	10.57	9.47	981
0.15	0.48	2.85	0.82	-11.49	17.19	14.34	1.57	3.75	6.30	5.04	2.19	10.41	4.11	7.44	2.84	7.67	4.34	-6.64	21.99	14.31	7.74	772
0.18	0.38	2.23	0.60	-10.73	15.18	12.95	1.16	3.55	5.50	4.53	2.22	8.78	3.28	6.25	2.73	5.92	3.67	-2.77	14.60	8.68	6.34	968
0.32	0.22	0.95	0.37	-2.93	4.82	3.87	0.65	3.30	4.81	4.09	2.05	7.57	2.76	5.30	2.61	5.56	3.27	-7.66	18.79	13.23	4.99	2660


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.78
et_p_h	1.81
et_p_l2	2.03


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.10	0.24	0.19	0.07	0.41	0.17	0.36	0.03	0.07	0.05	0.02	0.11	0.05	0.10	0.03	0.05	0.05	0.02	0.08	0.03	0.07	66
0.06	0.11	0.29	0.23	0.04	0.55	0.26	0.41	0.03	0.07	0.06	0.02	0.13	0.06	0.11	0.03	0.06	0.05	0.02	0.10	0.04	0.09	1168
0.11	0.17	0.45	0.37	0.05	0.85	0.40	0.63	0.04	0.10	0.08	0.03	0.16	0.06	0.14	0.05	0.08	0.07	0.04	0.12	0.04	0.11	981
0.15	0.29	0.70	0.57	0.13	1.27	0.57	0.96	0.06	0.12	0.11	0.05	0.18	0.06	0.17	0.06	0.10	0.09	0.06	0.14	0.04	0.12	772
0.18	0.42	0.96	0.85	0.25	1.67	0.71	1.31	0.08	0.14	0.14	0.07	0.20	0.06	0.19	0.08	0.11	0.11	0.07	0.15	0.04	0.14	968
0.32	0.87	1.97	1.53	0.33	3.61	1.64	2.61	0.12	0.17	0.17	0.10	0.24	0.07	0.22	0.11	0.14	0.14	0.09	0.19	0.05	0.17	2660


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.28
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.94	0.94	0.92	0.96	0.02	0.96	0.92	0.94	0.95	0.91	0.97	0.03	0.97	0.96	0.97	0.98	0.92	1.01	0.04	0.99	66
0.06	0.90	0.92	0.92	0.88	0.95	0.03	0.94	0.90	0.92	0.93	0.88	0.96	0.04	0.95	0.89	0.92	0.95	0.84	1.00	0.08	0.98	1168
0.11	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.87	0.89	0.90	0.85	0.94	0.04	0.93	0.84	0.89	0.91	0.80	0.98	0.09	0.96	981
0.15	0.84	0.86	0.87	0.83	0.90	0.04	0.89	0.84	0.87	0.87	0.82	0.92	0.05	0.90	0.83	0.87	0.89	0.78	0.97	0.09	0.95	772
0.18	0.82	0.84	0.85	0.81	0.88	0.04	0.87	0.82	0.85	0.85	0.80	0.90	0.05	0.89	0.80	0.85	0.86	0.75	0.95	0.10	0.92	968
0.32	0.77	0.80	0.80	0.75	0.84	0.05	0.83	0.77	0.81	0.81	0.76	0.86	0.05	0.85	0.74	0.80	0.81	0.69	0.90	0.11	0.87	2660


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.80	1.75	2.41	0.84	2.66	0.91	2.47	0.20	0.39	0.29	0.13	0.64	0.26	0.58	1.60	5.04	3.42	-0.37	10.45	5.41	7.61	66
0.06	0.81	1.77	1.98	1.01	2.53	0.76	2.16	0.11	0.32	0.23	0.06	0.59	0.26	0.47	1.00	3.52	2.32	-0.44	7.49	3.96	4.56	1168
0.11	0.63	0.73	0.68	0.58	0.89	0.16	0.81	0.15	0.38	0.30	0.11	0.65	0.27	0.55	1.26	4.24	2.80	-0.24	8.73	4.49	5.72	981
0.15	0.92	0.99	0.96	0.84	1.14	0.15	1.05	0.20	0.42	0.35	0.14	0.69	0.28	0.61	1.71	5.23	3.84	0.33	10.13	4.90	7.28	772
0.18	1.23	1.33	1.31	1.14	1.52	0.19	1.42	0.21	0.43	0.37	0.16	0.71	0.27	0.63	1.89	5.73	4.36	0.61	10.85	5.12	8.12	968
0.32	1.57	2.15	2.06	1.47	2.83	0.68	2.60	0.21	0.42	0.35	0.16	0.69	0.26	0.59	2.32	6.32	5.17	1.13	11.51	5.19	8.94	2660


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/time_misc_auc.tex <==
name	auc
attack_time	0.42
l2	0.12
lom	1.52


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.35	0.52	0.60	0.25	0.78	0.27	0.67	0.73	0.78	0.80	0.67	0.89	0.11	0.83	0.78	0.85	0.88	0.77	0.94	0.09	0.92	66
0.06	0.00	0.34	0.33	0.05	0.62	0.29	0.50	0.56	0.66	0.67	0.51	0.82	0.16	0.78	0.74	0.80	0.81	0.70	0.90	0.10	0.87	1168
0.11	0.00	0.23	0.25	-0.02	0.48	0.25	0.33	0.46	0.59	0.58	0.41	0.76	0.18	0.70	0.68	0.75	0.75	0.63	0.86	0.11	0.83	981
0.15	0.00	0.15	0.00	-0.07	0.37	0.22	0.33	0.40	0.51	0.50	0.32	0.71	0.19	0.67	0.62	0.70	0.71	0.58	0.83	0.12	0.80	772
0.18	0.00	0.10	0.00	-0.08	0.29	0.18	0.25	0.30	0.45	0.44	0.25	0.64	0.19	0.58	0.57	0.67	0.68	0.53	0.80	0.13	0.76	968
0.32	0.00	0.05	0.00	-0.08	0.17	0.13	0.00	0.17	0.32	0.30	0.11	0.52	0.21	0.45	0.45	0.57	0.57	0.41	0.73	0.16	0.69	2660


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/a/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.14
top50	0.20


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	59.86	124.43	134.68	60.59	188.28	63.85	161.50	2.00	3.32	3.00	1.44	5.19	1.88	5.00	77.75	139.32	145.51	67.43	211.21	71.89	173.12	2.00	3.38	3.00	1.42	5.33	1.95	5.00	72
0.06	93.52	168.72	137.15	41.77	295.67	126.95	204.44	3.00	4.62	5.00	2.65	6.60	1.97	6.00	118.11	205.74	167.52	64.70	346.78	141.04	252.06	3.00	4.72	5.00	2.70	6.74	2.02	6.00	1176
0.11	96.00	173.93	143.03	39.93	307.94	134.01	207.74	3.00	4.58	5.00	2.62	6.54	1.96	6.00	138.28	242.69	199.62	56.15	429.23	186.54	289.11	3.00	4.74	5.00	2.72	6.75	2.01	6.00	1042
0.15	92.52	169.40	138.73	44.28	294.51	125.12	205.03	3.00	4.53	4.00	2.59	6.47	1.94	6.00	155.01	267.31	219.10	80.37	454.26	186.95	328.91	3.00	4.78	5.00	2.69	6.88	2.10	6.00	866
0.18	95.62	169.82	136.92	33.76	305.87	136.06	203.66	3.00	4.51	4.00	2.57	6.45	1.94	6.00	180.67	305.72	244.13	76.92	534.51	228.80	359.31	3.00	4.80	5.00	2.66	6.95	2.14	6.00	1012
0.32	96.66	180.30	143.61	26.74	333.86	153.56	213.03	3.00	4.48	4.00	2.49	6.46	1.99	6.00	244.32	424.18	348.98	117.80	730.56	306.38	505.22	3.00	4.95	5.00	2.71	7.19	2.24	6.00	2626


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	49.40
orig_ge	1.30
adv_pp	86.04
adv_ge	1.37


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	-0.35	-0.07	-0.09	-0.48	0.34	0.41	0.13	0.07	0.23	0.19	-0.06	0.53	0.29	0.40	0.06	0.18	0.16	-0.05	0.42	0.23	0.31	72
0.06	-0.46	-0.19	-0.20	-0.57	0.19	0.38	0.04	-0.20	0.03	0.02	-0.28	0.35	0.32	0.24	-0.13	0.03	0.02	-0.21	0.28	0.24	0.18	1176
0.11	-0.55	-0.33	-0.33	-0.65	0.00	0.33	-0.12	-0.30	-0.09	-0.09	-0.38	0.20	0.29	0.10	-0.21	-0.06	-0.06	-0.27	0.16	0.22	0.07	1042
0.15	-0.65	-0.45	-0.45	-0.73	-0.16	0.28	-0.24	-0.39	-0.21	-0.22	-0.46	0.05	0.25	-0.03	-0.28	-0.15	-0.15	-0.34	0.04	0.19	-0.01	866
0.18	-0.65	-0.48	-0.48	-0.73	-0.22	0.25	-0.31	-0.39	-0.24	-0.25	-0.48	-0.00	0.24	-0.09	-0.28	-0.17	-0.18	-0.35	0.01	0.18	-0.06	1012
0.32	-0.73	-0.58	-0.59	-0.79	-0.37	0.21	-0.43	-0.50	-0.35	-0.36	-0.56	-0.14	0.21	-0.21	-0.36	-0.25	-0.26	-0.41	-0.09	0.16	-0.15	2626


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/correlations_auc.tex <==
name	auc
pcc	-0.12
spearman	-0.05
kendall	-0.04


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	5.27	9.95	8.38	3.66	16.25	6.30	12.70	5.17	12.99	8.84	1.99	23.99	11.00	16.15	5.29	21.24	10.48	-0.10	42.57	21.34	34.54	72
0.06	5.12	7.97	7.08	3.67	12.28	4.31	9.79	5.21	10.12	7.82	2.33	17.90	7.78	12.48	5.06	18.46	10.67	-0.34	37.26	18.80	26.35	1176
0.11	4.67	6.68	6.05	3.58	9.78	3.10	7.93	4.63	8.13	6.59	2.34	13.92	5.79	9.67	4.33	14.54	8.00	-1.31	30.39	15.85	18.07	1042
0.15	4.44	6.03	5.66	3.69	8.38	2.34	7.04	4.44	6.84	5.96	3.21	10.48	3.64	8.34	4.05	13.56	7.45	-2.21	29.33	15.77	14.87	866
0.18	4.01	5.26	4.90	3.31	7.21	1.95	6.03	4.04	5.87	5.18	3.05	8.69	2.82	6.88	3.62	9.69	5.76	-1.45	20.83	11.14	10.15	1012
0.32	3.51	4.38	4.12	3.02	5.74	1.36	4.94	3.54	4.86	4.42	2.90	6.82	1.96	5.63	3.19	6.82	4.62	-0.58	14.23	7.40	7.14	2626


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/ets_sts_auc.tex <==
name	auc
et_use	1.73
et_tse	2.04
et_ce	3.49


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.97	9.37	5.38	-7.10	25.85	16.48	10.51	7.96	18.15	13.01	2.24	34.05	15.90	22.71	6.93	19.99	14.85	-2.80	42.79	22.80	27.00	72
0.06	1.30	7.71	2.36	-18.04	33.45	25.75	5.21	6.35	15.32	10.68	1.58	29.07	13.74	19.41	4.98	19.47	10.26	-10.61	49.54	30.07	22.71	1176
0.11	0.97	5.20	1.65	-14.52	24.91	19.72	3.21	5.58	10.98	8.44	2.67	19.28	8.30	13.13	4.36	12.70	7.52	-4.91	30.31	17.61	14.30	1042
0.15	0.74	3.93	1.22	-13.95	21.81	17.88	2.34	5.28	9.21	7.21	2.68	15.75	6.53	10.70	4.19	11.40	6.23	-10.57	33.36	21.97	11.32	866
0.18	0.57	3.31	0.90	-17.37	23.99	20.68	1.74	4.95	8.00	6.60	2.79	13.21	5.21	9.15	3.93	9.13	5.44	-6.27	24.54	15.40	9.03	1012
0.32	0.34	1.83	0.58	-12.44	16.11	14.28	1.01	4.50	6.67	5.55	2.33	11.01	4.34	7.33	3.59	7.77	4.59	-11.49	27.03	19.26	6.83	2626


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/ets_time_misc_auc.tex <==
name	auc
et_p	1.23
et_p_h	2.84
et_p_l2	3.36


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.05	0.17	0.10	0.01	0.33	0.16	0.30	0.02	0.06	0.04	0.01	0.11	0.05	0.08	0.02	0.05	0.04	0.02	0.08	0.03	0.08	72
0.06	0.11	0.30	0.24	0.05	0.55	0.25	0.42	0.03	0.07	0.05	0.02	0.13	0.06	0.11	0.03	0.06	0.05	0.02	0.10	0.04	0.09	1176
0.11	0.20	0.50	0.41	0.04	0.95	0.45	0.66	0.05	0.10	0.09	0.04	0.16	0.06	0.15	0.05	0.08	0.08	0.04	0.12	0.04	0.11	1042
0.15	0.30	0.73	0.61	0.10	1.36	0.63	0.96	0.06	0.12	0.12	0.05	0.19	0.07	0.17	0.07	0.10	0.10	0.06	0.14	0.04	0.13	866
0.18	0.44	0.98	0.82	0.19	1.77	0.79	1.28	0.08	0.14	0.14	0.07	0.20	0.07	0.19	0.08	0.11	0.11	0.07	0.16	0.04	0.14	1012
0.32	0.77	1.75	1.36	0.27	3.22	1.47	2.28	0.12	0.17	0.17	0.10	0.24	0.07	0.22	0.11	0.14	0.14	0.09	0.19	0.05	0.17	2626


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.27
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.94	0.93	0.91	0.96	0.03	0.96	0.91	0.94	0.95	0.90	0.97	0.04	0.97	0.90	0.94	0.96	0.88	1.00	0.06	0.99	72
0.06	0.90	0.92	0.92	0.89	0.94	0.03	0.94	0.90	0.92	0.93	0.88	0.96	0.04	0.95	0.88	0.92	0.95	0.84	1.00	0.08	0.98	1176
0.11	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.87	0.90	0.90	0.85	0.94	0.04	0.93	0.86	0.90	0.92	0.81	0.98	0.08	0.96	1042
0.15	0.85	0.87	0.87	0.83	0.90	0.04	0.89	0.85	0.88	0.88	0.83	0.92	0.04	0.91	0.83	0.88	0.90	0.79	0.97	0.09	0.95	866
0.18	0.83	0.85	0.85	0.81	0.89	0.04	0.87	0.83	0.86	0.86	0.81	0.90	0.05	0.89	0.80	0.86	0.87	0.77	0.95	0.09	0.93	1012
0.32	0.78	0.81	0.81	0.76	0.85	0.04	0.84	0.78	0.82	0.82	0.77	0.87	0.05	0.86	0.76	0.81	0.83	0.71	0.92	0.10	0.89	2626


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.95	2.55	3.19	1.15	3.95	1.40	3.30	5.25	12.72	9.99	0.73	24.72	12.00	16.01	2.40	7.74	5.33	0.92	14.55	6.82	11.72	72
0.06	2.61	3.22	2.94	1.60	4.84	1.62	3.50	5.25	13.29	8.99	-37.52	64.11	50.82	14.08	2.74	7.56	6.06	1.44	13.68	6.12	10.75	1176
0.11	2.05	2.91	2.55	1.63	4.19	1.28	3.29	5.83	15.82	10.10	-30.14	61.78	45.96	16.51	2.65	7.40	5.75	1.18	13.62	6.22	10.53	1042
0.15	3.26	4.12	3.73	2.72	5.52	1.40	4.52	6.44	16.54	10.96	-9.01	42.10	25.55	18.19	2.98	7.97	6.31	1.56	14.38	6.41	11.55	866
0.18	4.49	5.36	5.27	4.14	6.58	1.22	6.02	6.65	14.79	10.85	1.35	28.23	13.44	17.71	3.04	8.18	6.49	1.59	14.77	6.59	11.91	1012
0.32	3.82	5.91	5.24	3.53	8.30	2.38	8.18	6.46	13.65	10.72	0.48	26.82	13.17	16.64	2.99	7.96	6.17	1.47	14.45	6.49	11.48	2626


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/time_misc_auc.tex <==
name	auc
attack_time	1.31
l2	4.24
lom	2.28


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.24	0.20	0.02	0.45	0.21	0.40	0.33	0.44	0.40	0.27	0.62	0.18	0.60	0.55	0.61	0.60	0.49	0.73	0.12	0.68	72
0.06	0.00	0.14	0.00	-0.06	0.35	0.21	0.33	0.22	0.35	0.33	0.17	0.52	0.17	0.45	0.44	0.53	0.53	0.39	0.67	0.14	0.62	1176
0.11	0.00	0.09	0.00	-0.08	0.25	0.16	0.19	0.18	0.30	0.29	0.14	0.45	0.16	0.40	0.40	0.48	0.48	0.35	0.61	0.13	0.56	1042
0.15	0.00	0.05	0.00	-0.08	0.18	0.13	0.00	0.15	0.24	0.23	0.11	0.38	0.14	0.33	0.36	0.44	0.44	0.32	0.56	0.12	0.53	866
0.18	0.00	0.04	0.00	-0.08	0.16	0.12	0.00	0.11	0.22	0.22	0.09	0.36	0.14	0.30	0.35	0.43	0.43	0.31	0.54	0.11	0.50	1012
0.32	0.00	0.02	0.00	-0.07	0.12	0.09	0.00	0.09	0.18	0.17	0.05	0.30	0.12	0.25	0.32	0.39	0.39	0.29	0.50	0.11	0.47	2626


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.07
top50	0.13


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	65.33	124.50	132.35	60.40	188.59	64.09	163.80	2.00	3.42	3.00	1.72	5.12	1.70	4.00	93.23	152.83	142.68	77.12	228.54	75.71	207.55	2.00	3.54	4.00	1.79	5.28	1.74	5.00	67
0.06	94.84	168.63	136.71	41.56	295.70	127.07	200.83	3.00	4.62	5.00	2.61	6.62	2.00	6.00	128.41	221.95	185.49	58.66	385.24	163.29	262.46	3.00	4.77	5.00	2.75	6.79	2.02	6.00	1134
0.11	96.35	179.70	142.85	32.58	326.82	147.12	210.15	3.00	4.56	5.00	2.58	6.55	1.98	6.00	151.15	273.59	221.07	61.93	485.24	211.65	327.56	3.00	4.79	5.00	2.73	6.85	2.06	6.00	968
0.15	94.38	170.54	138.11	35.49	305.59	135.05	204.33	3.00	4.49	4.00	2.53	6.46	1.96	6.00	183.47	315.95	262.35	99.39	532.50	216.56	373.65	3.00	4.84	5.00	2.72	6.96	2.12	6.00	766
0.18	95.57	172.69	138.67	28.00	317.39	144.69	204.45	3.00	4.54	4.00	2.59	6.49	1.95	6.00	213.58	366.72	308.56	112.30	621.15	254.42	436.88	4.00	4.97	5.00	2.86	7.07	2.11	6.00	973
0.32	96.29	178.90	142.95	30.56	327.24	148.34	210.94	3.00	4.48	4.00	2.51	6.45	1.97	6.00	311.57	540.14	442.13	166.55	913.72	373.58	651.44	4.00	5.12	5.00	2.89	7.35	2.23	7.00	2668


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/comparison_vals_auc.tex <==
name	auc
orig_pp	49.85
orig_ge	1.30
adv_pp	103.20
adv_ge	1.41


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.60	0.71	0.70	0.52	0.91	0.20	0.90	0.73	0.80	0.83	0.66	0.95	0.14	0.91	0.60	0.67	0.67	0.52	0.82	0.15	0.78	67
0.06	0.35	0.54	0.56	0.27	0.80	0.26	0.75	0.60	0.69	0.73	0.51	0.87	0.18	0.82	0.46	0.55	0.57	0.39	0.71	0.16	0.66	1134
0.11	0.18	0.37	0.36	0.11	0.64	0.27	0.58	0.45	0.56	0.60	0.33	0.79	0.23	0.73	0.33	0.43	0.45	0.25	0.62	0.19	0.56	968
0.15	0.04	0.21	0.21	-0.03	0.45	0.24	0.37	0.28	0.43	0.48	0.18	0.69	0.26	0.63	0.21	0.33	0.35	0.13	0.52	0.19	0.46	766
0.18	-0.04	0.11	0.10	-0.11	0.34	0.22	0.25	0.16	0.32	0.35	0.05	0.60	0.28	0.53	0.12	0.24	0.26	0.04	0.44	0.20	0.38	973
0.32	-0.24	-0.09	-0.10	-0.31	0.13	0.22	0.05	-0.20	0.04	0.05	-0.28	0.37	0.32	0.29	-0.13	0.04	0.04	-0.19	0.26	0.23	0.20	2668


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/correlations_auc.tex <==
name	auc
pcc	0.06
spearman	0.11
kendall	0.09


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	0.79	2.96	2.59	0.53	5.38	2.42	4.67	1.06	3.67	2.51	-0.04	7.39	3.71	4.77	0.95	6.91	5.41	0.00	13.82	6.91	9.74	67
0.06	1.56	3.13	2.71	0.96	5.29	2.16	4.24	1.69	3.84	2.92	0.65	7.03	3.19	5.02	1.82	6.23	3.61	-0.63	13.08	6.86	8.11	1134
0.11	1.97	3.18	2.94	1.48	4.88	1.70	4.06	2.12	3.79	3.10	1.10	6.48	2.69	4.64	1.98	6.80	3.90	-1.03	14.64	7.83	8.25	968
0.15	2.28	3.21	3.02	1.81	4.61	1.40	3.93	2.38	3.75	3.22	1.53	5.97	2.22	4.52	2.14	6.08	3.42	-0.87	13.03	6.95	6.87	766
0.18	2.34	3.13	2.99	1.97	4.28	1.16	3.73	2.43	3.61	3.20	1.78	5.44	1.83	4.36	2.17	5.22	3.43	-0.22	10.66	5.44	5.94	973
0.32	2.34	2.95	2.83	2.05	3.85	0.90	3.42	2.45	3.34	3.06	1.99	4.68	1.34	3.91	2.07	3.90	2.99	0.21	7.60	3.70	4.40	2668


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/ets_sts_auc.tex <==
name	auc
et_use	0.90
et_tse	1.05
et_ce	1.59


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.22	2.92	0.54	-7.10	12.94	10.02	0.87	1.11	3.13	2.59	-0.36	6.62	3.49	3.82	1.00	4.40	2.54	-4.36	13.15	8.75	4.02	67
0.06	0.30	1.88	0.64	-4.83	8.59	6.71	1.40	1.69	5.00	3.29	-0.57	10.56	5.57	6.09	1.44	6.76	2.99	-7.03	20.55	13.79	6.78	1134
0.11	0.31	1.78	0.55	-5.80	9.37	7.58	1.05	2.07	4.40	3.37	0.50	8.30	3.90	5.39	1.61	4.83	2.81	-1.77	11.43	6.60	5.37	968
0.15	0.27	1.11	0.44	-2.55	4.78	3.66	0.76	2.57	4.68	3.58	-1.08	10.44	5.76	5.12	1.97	6.61	2.94	-17.23	30.44	23.83	4.94	766
0.18	0.23	0.78	0.36	-1.78	3.34	2.56	0.64	2.70	4.29	3.54	1.20	7.38	3.09	4.89	2.10	4.96	2.98	-5.19	15.12	10.15	4.62	973
0.32	0.16	0.52	0.26	-1.85	2.89	2.37	0.44	2.86	4.12	3.52	1.58	6.67	2.55	4.57	2.28	4.67	2.92	-5.19	14.54	9.86	4.12	2668


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.34
et_p_h	1.26
et_p_l2	1.54


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.13	0.27	0.25	0.07	0.47	0.20	0.37	0.03	0.06	0.06	0.02	0.11	0.05	0.08	0.03	0.06	0.05	0.03	0.09	0.03	0.07	67
0.06	0.18	0.39	0.33	0.09	0.69	0.30	0.53	0.03	0.08	0.07	0.02	0.14	0.06	0.13	0.04	0.07	0.07	0.03	0.11	0.04	0.10	1134
0.11	0.30	0.62	0.53	0.18	1.07	0.44	0.87	0.06	0.11	0.11	0.05	0.18	0.06	0.17	0.06	0.09	0.09	0.05	0.14	0.04	0.12	968
0.15	0.50	1.03	0.87	0.26	1.80	0.77	1.37	0.08	0.13	0.13	0.07	0.20	0.07	0.18	0.08	0.11	0.11	0.07	0.15	0.04	0.14	766
0.18	0.70	1.37	1.17	0.39	2.36	0.98	1.84	0.10	0.15	0.15	0.08	0.22	0.07	0.20	0.09	0.13	0.13	0.08	0.17	0.04	0.16	973
0.32	1.22	2.57	2.02	0.44	4.70	2.13	3.25	0.14	0.18	0.19	0.11	0.25	0.07	0.23	0.12	0.15	0.15	0.11	0.20	0.05	0.18	2668


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.38
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.94	0.94	0.95	0.92	0.97	0.02	0.96	0.94	0.95	0.96	0.91	0.99	0.04	0.97	0.96	0.96	0.98	0.93	1.00	0.04	0.99	67
0.06	0.90	0.92	0.92	0.89	0.95	0.03	0.94	0.90	0.92	0.93	0.88	0.96	0.04	0.95	0.89	0.92	0.95	0.84	1.00	0.08	0.98	1134
0.11	0.87	0.89	0.89	0.86	0.93	0.03	0.92	0.87	0.90	0.91	0.86	0.94	0.04	0.93	0.86	0.90	0.92	0.81	0.98	0.08	0.96	968
0.15	0.85	0.87	0.87	0.83	0.91	0.04	0.89	0.85	0.88	0.88	0.83	0.92	0.05	0.91	0.83	0.87	0.89	0.78	0.97	0.09	0.94	766
0.18	0.83	0.85	0.85	0.81	0.89	0.04	0.87	0.83	0.86	0.86	0.81	0.91	0.05	0.89	0.81	0.85	0.87	0.76	0.95	0.10	0.92	973
0.32	0.78	0.81	0.81	0.76	0.85	0.05	0.84	0.79	0.82	0.82	0.77	0.87	0.05	0.86	0.75	0.80	0.82	0.70	0.91	0.10	0.87	2668


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	1.05	3.20	4.39	1.48	4.93	1.72	4.52	2.92	25.49	4.76	-65.49	116.48	90.99	12.83	0.63	1.53	1.03	0.39	2.67	1.14	2.15	67
0.06	0.96	2.36	2.68	1.31	3.40	1.05	2.93	1.95	41.95	5.10	-74.64	158.55	116.59	19.84	0.61	1.69	1.31	0.26	3.11	1.43	2.41	1134
0.11	0.80	0.92	0.88	0.70	1.15	0.22	1.02	2.75	55.78	7.24	-73.35	184.92	129.13	35.69	0.86	2.06	1.69	0.44	3.69	1.62	2.91	968
0.15	1.06	1.16	1.14	0.94	1.39	0.23	1.21	3.84	63.46	10.81	-86.58	213.50	150.04	43.59	1.01	2.59	2.09	0.53	4.65	2.06	3.68	766
0.18	1.41	1.54	1.53	1.30	1.78	0.24	1.63	4.69	88.03	12.45	-166.01	342.06	254.03	52.04	1.04	2.73	2.32	0.62	4.84	2.11	3.84	973
0.32	2.12	2.84	2.87	2.06	3.61	0.77	3.41	5.79	98.42	15.02	-175.64	372.47	274.06	68.48	1.26	3.01	2.53	0.73	5.30	2.28	4.24	2668


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/time_misc_auc.tex <==
name	auc
attack_time	0.55
l2	21.13
lom	0.72


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.45	0.59	0.60	0.37	0.81	0.22	0.78	0.67	0.76	0.75	0.64	0.88	0.12	0.83	0.80	0.84	0.84	0.75	0.92	0.09	0.89	67
0.06	0.00	0.36	0.33	0.07	0.65	0.29	0.67	0.55	0.64	0.64	0.49	0.80	0.15	0.75	0.71	0.78	0.79	0.68	0.87	0.10	0.84	1134
0.11	0.00	0.26	0.25	0.00	0.52	0.26	0.33	0.44	0.55	0.56	0.38	0.72	0.17	0.67	0.65	0.72	0.73	0.60	0.83	0.11	0.80	968
0.15	0.00	0.14	0.00	-0.07	0.36	0.22	0.25	0.36	0.47	0.50	0.30	0.64	0.17	0.60	0.59	0.67	0.68	0.55	0.79	0.12	0.76	766
0.18	0.00	0.10	0.00	-0.08	0.27	0.18	0.25	0.27	0.40	0.40	0.23	0.57	0.17	0.50	0.55	0.62	0.62	0.50	0.74	0.12	0.71	973
0.32	0.00	0.04	0.00	-0.08	0.15	0.11	0.00	0.12	0.26	0.25	0.09	0.43	0.17	0.38	0.41	0.51	0.50	0.37	0.65	0.14	0.61	2668


==> data/mlm_plots/mlm_distil_fast/agnews/roberta/s/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.13
top50	0.19


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	60.84	116.53	113.54	59.21	173.85	57.32	151.79	2.00	2.91	3.00	1.47	4.35	1.44	4.00	79.11	143.74	125.53	57.60	229.89	86.15	182.11	2.00	3.03	3.00	1.72	4.34	1.31	4.00	34
0.06	100.53	182.18	150.26	52.11	312.24	130.07	224.00	3.00	4.34	4.00	2.63	6.05	1.71	5.00	121.31	216.85	173.79	60.05	373.64	156.80	262.98	3.00	4.26	4.00	2.54	5.98	1.72	5.00	1226
0.11	103.39	192.14	152.88	46.41	337.88	145.73	230.31	3.00	4.16	4.00	2.42	5.90	1.74	5.00	142.33	265.81	214.19	72.01	459.61	193.80	324.34	3.00	3.86	4.00	2.15	5.58	1.72	5.00	1012
0.15	104.30	189.76	153.27	52.24	327.29	137.53	229.92	3.00	4.13	4.00	2.42	5.83	1.71	5.00	167.43	299.46	238.64	70.98	527.94	228.48	362.97	2.00	3.66	4.00	2.01	5.31	1.65	5.00	740
0.18	101.40	188.55	150.53	33.91	343.19	154.64	222.67	3.00	4.13	4.00	2.43	5.83	1.70	5.00	185.38	326.59	264.18	92.52	560.66	234.07	400.25	2.00	3.71	4.00	2.05	5.38	1.66	5.00	975
0.32	103.31	196.49	157.30	36.57	356.41	159.92	238.39	3.00	4.12	4.00	2.37	5.86	1.75	5.00	266.10	481.09	395.39	145.43	816.75	335.66	582.84	3.00	3.81	4.00	2.03	5.58	1.77	5.00	2691


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/comparison_vals_auc.tex <==
name	auc
orig_pp	54.11
orig_ge	1.19
adv_pp	94.46
adv_ge	1.10


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.26	0.53	0.56	0.20	0.87	0.33	0.80	0.44	0.68	0.80	0.38	0.97	0.30	0.91	0.32	0.55	0.63	0.28	0.82	0.27	0.76	34
0.06	0.12	0.31	0.29	0.04	0.59	0.27	0.49	0.43	0.57	0.63	0.30	0.85	0.28	0.79	0.31	0.45	0.47	0.22	0.68	0.23	0.62	1226
0.11	0.00	0.25	0.19	-0.07	0.57	0.32	0.46	0.30	0.47	0.51	0.17	0.77	0.30	0.70	0.21	0.36	0.38	0.12	0.60	0.24	0.54	1012
0.15	-0.11	0.12	0.06	-0.18	0.42	0.30	0.30	0.11	0.33	0.37	-0.01	0.66	0.34	0.58	0.08	0.25	0.27	-0.01	0.50	0.26	0.43	740
0.18	-0.15	0.07	-0.00	-0.22	0.36	0.29	0.23	0.00	0.26	0.29	-0.07	0.60	0.34	0.52	0.01	0.20	0.20	-0.05	0.45	0.25	0.38	975
0.32	-0.26	-0.06	-0.12	-0.35	0.23	0.29	0.06	-0.21	0.07	0.07	-0.28	0.43	0.36	0.35	-0.14	0.06	0.05	-0.20	0.32	0.26	0.25	2691


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.09
kendall	0.07


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	1.47	4.54	3.46	0.88	8.19	3.66	7.51	1.59	4.67	2.24	-0.88	10.22	5.55	6.35	1.11	5.85	2.31	-0.96	12.66	6.81	7.85	34
0.06	2.62	4.22	3.82	1.76	6.69	2.47	5.34	2.33	4.20	3.55	1.40	7.00	2.80	5.30	2.64	9.91	5.64	-0.35	20.18	10.26	13.60	1226
0.11	2.18	3.41	3.24	1.52	5.29	1.88	4.43	2.11	3.66	3.26	1.26	6.07	2.41	4.71	2.19	7.38	3.90	-1.48	16.25	8.87	8.79	1012
0.15	2.27	3.22	3.08	1.70	4.73	1.52	3.95	2.19	3.35	3.03	1.50	5.20	1.85	4.14	2.22	6.05	3.71	-0.60	12.69	6.64	7.30	740
0.18	2.21	2.95	2.89	1.71	4.20	1.25	3.62	2.11	3.09	2.87	1.51	4.67	1.58	3.79	2.04	5.04	3.21	-0.90	10.98	5.94	5.61	975
0.32	2.12	2.63	2.61	1.70	3.56	0.93	3.12	2.08	2.78	2.63	1.59	3.97	1.19	3.30	1.97	3.79	2.83	0.03	7.55	3.76	4.25	2691


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/ets_sts_auc.tex <==
name	auc
et_use	0.94
et_tse	0.98
et_ce	1.72


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.74	5.29	1.27	-6.64	17.22	11.93	4.22	2.05	9.18	4.36	-2.41	20.77	11.59	12.65	1.91	10.46	3.46	-4.49	25.42	14.95	12.36	34
0.06	0.74	5.38	1.55	-12.24	23.01	17.63	3.82	4.17	10.09	7.62	1.48	18.70	8.61	13.36	3.54	12.19	7.20	-5.41	29.79	17.60	14.00	1226
0.11	0.46	2.96	0.97	-7.11	13.02	10.07	2.21	3.21	8.10	5.87	0.28	15.93	7.83	10.21	2.68	10.61	5.36	-9.56	30.78	20.17	11.46	1012
0.15	0.37	3.00	0.80	-6.59	12.60	9.59	1.87	3.49	7.46	5.63	0.43	14.50	7.03	9.14	2.82	10.36	4.83	-13.60	34.32	23.96	9.52	740
0.18	0.32	2.19	0.62	-11.60	15.97	13.78	1.29	3.28	6.28	4.88	1.33	11.23	4.95	7.74	2.66	7.99	4.33	-10.04	26.02	18.03	8.30	975
0.32	0.18	1.09	0.35	-3.95	6.14	5.04	0.75	3.11	5.23	4.19	1.09	9.37	4.14	6.08	2.50	6.69	3.56	-11.68	25.05	18.36	6.04	2691


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.79
et_p_h	2.07
et_p_l2	2.64


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.04	0.23	0.19	0.02	0.45	0.22	0.32	0.02	0.05	0.04	0.01	0.09	0.04	0.07	0.03	0.04	0.03	0.02	0.06	0.02	0.06	34
0.06	0.09	0.29	0.21	-0.07	0.64	0.36	0.38	0.02	0.06	0.05	0.01	0.11	0.05	0.08	0.03	0.05	0.04	0.02	0.09	0.03	0.07	1226
0.11	0.17	0.51	0.38	-0.00	1.02	0.51	0.68	0.03	0.08	0.07	0.02	0.14	0.06	0.12	0.04	0.07	0.06	0.03	0.11	0.04	0.10	1012
0.15	0.25	0.76	0.54	-0.07	1.59	0.83	1.01	0.05	0.10	0.09	0.03	0.16	0.06	0.14	0.05	0.09	0.08	0.04	0.13	0.04	0.12	740
0.18	0.37	0.97	0.77	0.07	1.87	0.90	1.34	0.06	0.12	0.11	0.05	0.18	0.07	0.17	0.06	0.10	0.10	0.06	0.14	0.04	0.13	975
0.32	0.73	1.95	1.45	0.13	3.78	1.82	2.62	0.09	0.15	0.15	0.07	0.23	0.08	0.20	0.09	0.13	0.13	0.08	0.18	0.05	0.16	2691


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.28
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.93	0.94	0.95	0.92	0.96	0.02	0.96	0.90	0.93	0.95	0.88	0.98	0.05	0.96	0.87	0.90	0.93	0.80	1.01	0.10	0.98	34
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.87	0.90	0.90	0.85	0.95	0.05	0.93	0.89	0.92	0.94	0.84	1.00	0.08	0.98	1226
0.11	0.86	0.88	0.88	0.84	0.91	0.03	0.90	0.85	0.88	0.88	0.83	0.93	0.05	0.92	0.85	0.89	0.91	0.81	0.98	0.08	0.96	1012
0.15	0.83	0.85	0.86	0.82	0.89	0.04	0.88	0.82	0.85	0.86	0.80	0.90	0.05	0.89	0.82	0.87	0.88	0.78	0.96	0.09	0.94	740
0.18	0.81	0.83	0.84	0.79	0.87	0.04	0.86	0.80	0.83	0.83	0.78	0.89	0.05	0.87	0.80	0.84	0.86	0.75	0.94	0.10	0.92	975
0.32	0.76	0.79	0.79	0.75	0.83	0.04	0.82	0.75	0.79	0.80	0.74	0.85	0.06	0.84	0.74	0.80	0.81	0.70	0.90	0.10	0.87	2691


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	1.16	2.47	1.79	0.36	4.58	2.11	2.26	0.08	0.16	0.12	0.05	0.27	0.11	0.25	0.87	3.16	2.22	0.44	5.89	2.72	5.29	34
0.06	1.43	2.84	3.24	1.62	4.06	1.22	3.52	0.11	0.19	0.16	0.08	0.30	0.11	0.23	1.45	4.01	3.13	0.62	7.39	3.39	5.70	1226
0.11	0.99	1.39	1.23	0.73	2.04	0.65	1.55	0.11	0.17	0.15	0.07	0.26	0.09	0.21	1.30	4.17	3.12	0.34	7.99	3.83	5.87	1012
0.15	1.49	1.99	1.72	1.24	2.74	0.75	2.31	0.12	0.18	0.16	0.08	0.28	0.10	0.22	1.35	4.49	3.25	0.49	8.49	4.00	6.63	740
0.18	1.81	2.31	2.09	1.57	3.05	0.74	2.56	0.12	0.19	0.17	0.09	0.28	0.09	0.23	1.66	4.77	3.80	0.80	8.73	3.96	6.76	975
0.32	3.27	4.04	3.84	3.00	5.08	1.04	4.73	0.13	0.19	0.17	0.10	0.28	0.09	0.23	1.73	4.97	3.92	0.85	9.10	4.13	7.39	2691


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/time_misc_auc.tex <==
name	auc
attack_time	0.75
l2	0.05
lom	1.31


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.20	0.42	0.40	0.10	0.74	0.32	0.60	0.48	0.67	0.73	0.46	0.87	0.20	0.80	0.65	0.77	0.82	0.62	0.92	0.15	0.88	34
0.06	0.00	0.25	0.25	-0.03	0.52	0.27	0.33	0.44	0.56	0.57	0.36	0.76	0.20	0.71	0.64	0.72	0.73	0.58	0.86	0.14	0.82	1226
0.11	0.00	0.21	0.00	-0.06	0.47	0.27	0.33	0.33	0.49	0.50	0.28	0.71	0.21	0.67	0.59	0.68	0.69	0.54	0.82	0.14	0.78	1012
0.15	0.00	0.13	0.00	-0.10	0.36	0.23	0.33	0.25	0.41	0.40	0.20	0.62	0.21	0.56	0.53	0.62	0.63	0.47	0.77	0.15	0.73	740
0.18	0.00	0.11	0.00	-0.10	0.32	0.21	0.00	0.22	0.37	0.36	0.16	0.58	0.21	0.50	0.50	0.60	0.60	0.45	0.75	0.15	0.71	975
0.32	0.00	0.07	0.00	-0.11	0.25	0.18	0.00	0.12	0.28	0.25	0.08	0.48	0.20	0.42	0.42	0.53	0.53	0.37	0.68	0.15	0.63	2691


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/a/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.12
top50	0.18


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	71.05	166.12	131.45	53.03	279.21	113.09	233.00	3.00	3.28	3.00	2.08	4.47	1.20	4.00	77.30	193.58	150.97	44.62	342.55	148.97	243.61	2.00	3.19	3.00	1.71	4.67	1.48	4.00	58
0.06	99.23	182.58	149.02	48.47	316.69	134.11	219.98	3.00	4.32	4.00	2.62	6.03	1.71	5.00	124.07	220.46	175.39	63.59	377.33	156.87	269.49	3.00	4.21	4.00	2.45	5.96	1.75	5.00	1300
0.11	100.56	188.94	149.03	37.53	340.35	151.41	222.60	3.00	4.16	4.00	2.44	5.88	1.72	5.00	135.85	254.57	200.14	56.21	452.94	198.37	305.68	3.00	4.06	4.00	2.28	5.84	1.78	5.00	1056
0.15	104.30	193.17	157.26	45.06	341.27	148.11	229.92	3.00	4.07	4.00	2.34	5.81	1.73	5.00	161.29	298.79	243.67	86.70	510.89	212.10	365.21	3.00	3.93	4.00	2.12	5.73	1.81	5.00	748
0.18	103.81	191.58	152.19	29.58	353.58	162.00	225.40	3.00	4.18	4.00	2.47	5.89	1.71	5.00	191.43	327.66	271.18	100.99	554.33	226.67	408.01	3.00	4.04	4.00	2.21	5.87	1.83	5.00	946
0.32	104.09	194.77	156.47	38.54	351.01	156.23	232.82	3.00	4.18	4.00	2.44	5.92	1.74	5.00	256.09	459.45	385.36	147.30	771.61	312.15	564.51	3.00	4.13	4.00	2.22	6.04	1.91	5.00	2614


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	55.00
orig_ge	1.20
adv_pp	93.44
adv_ge	1.17


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	-0.02	0.35	0.25	-0.11	0.82	0.46	0.82	0.02	0.38	0.30	-0.01	0.78	0.39	0.77	0.02	0.31	0.21	-0.02	0.63	0.33	0.61	58
0.06	-0.24	0.02	0.01	-0.35	0.39	0.37	0.24	-0.13	0.12	0.13	-0.21	0.45	0.33	0.35	-0.08	0.10	0.09	-0.15	0.35	0.25	0.26	1300
0.11	-0.37	-0.07	-0.13	-0.46	0.32	0.39	0.16	-0.23	0.02	-0.00	-0.32	0.36	0.34	0.24	-0.16	0.02	0.01	-0.23	0.27	0.25	0.17	1056
0.15	-0.47	-0.23	-0.29	-0.58	0.13	0.35	-0.07	-0.35	-0.12	-0.16	-0.44	0.21	0.32	0.05	-0.25	-0.08	-0.11	-0.32	0.16	0.24	0.05	748
0.18	-0.57	-0.36	-0.42	-0.68	-0.03	0.32	-0.24	-0.43	-0.24	-0.28	-0.53	0.06	0.29	-0.09	-0.31	-0.17	-0.19	-0.38	0.05	0.22	-0.05	946
0.32	-0.72	-0.51	-0.59	-0.84	-0.18	0.33	-0.43	-0.60	-0.41	-0.47	-0.71	-0.10	0.31	-0.30	-0.45	-0.30	-0.34	-0.53	-0.07	0.23	-0.21	2614


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/correlations_auc.tex <==
name	auc
pcc	-0.07
spearman	-0.04
kendall	-0.03


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	1.72	5.63	5.84	1.20	10.06	4.43	8.63	1.96	6.56	6.10	1.56	11.55	5.00	10.06	2.55	11.72	5.04	-2.98	26.41	14.70	11.16	58
0.06	3.78	5.97	5.48	2.69	9.26	3.29	7.39	3.83	6.93	5.70	2.03	11.82	4.90	8.52	3.91	13.60	7.50	-0.43	27.63	14.03	19.34	1300
0.11	3.39	5.06	4.72	2.35	7.78	2.72	6.22	3.37	5.58	4.72	2.16	8.99	3.42	6.89	3.23	10.31	5.89	-1.28	21.89	11.58	12.31	1056
0.15	3.36	4.63	4.51	2.71	6.55	1.92	5.62	3.33	5.08	4.61	2.57	7.58	2.51	6.48	3.29	8.49	5.44	-1.00	17.98	9.49	9.74	748
0.18	3.44	4.38	4.24	2.80	5.95	1.57	5.20	3.43	4.72	4.33	2.71	6.72	2.01	5.77	3.17	7.41	5.05	-0.45	15.27	7.86	8.57	946
0.32	3.21	3.88	3.79	2.58	5.19	1.30	4.48	3.18	4.14	3.92	2.55	5.73	1.59	4.93	2.82	5.45	4.13	0.26	10.64	5.19	6.16	2614


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/ets_sts_auc.tex <==
name	auc
et_use	1.36
et_tse	1.49
et_ce	2.49


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.58	5.81	1.77	-5.25	16.88	11.06	7.50	3.53	16.71	11.61	0.94	32.48	15.77	28.43	6.12	23.66	11.99	-24.31	71.63	47.97	22.95	58
0.06	1.00	6.55	1.96	-13.07	26.17	19.62	4.45	5.69	13.84	10.09	1.58	26.10	12.26	18.29	4.85	17.87	10.16	-12.87	48.62	30.74	19.23	1300
0.11	0.74	5.75	1.46	-20.15	31.65	25.90	3.58	4.95	11.07	8.10	0.81	21.32	10.25	14.39	3.93	14.81	7.48	-17.55	47.16	32.35	15.71	1056
0.15	0.61	5.48	1.09	-21.84	32.79	27.32	2.34	4.84	9.31	7.10	1.38	17.24	7.93	10.64	3.91	13.16	6.09	-23.52	49.84	36.68	11.26	748
0.18	0.49	3.60	0.91	-14.08	21.28	17.68	1.92	4.91	8.51	6.96	2.22	14.79	6.29	9.87	3.87	10.60	5.79	-14.48	35.68	25.08	10.09	946
0.32	0.31	1.96	0.56	-9.58	13.49	11.54	1.07	4.51	7.16	5.79	1.72	12.59	5.44	8.03	3.58	9.40	4.73	-15.21	34.01	24.61	7.90	2614


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/ets_time_misc_auc.tex <==
name	auc
et_p	1.25
et_p_h	2.85
et_p_l2	3.75


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.06	0.17	0.17	0.02	0.32	0.15	0.20	0.01	0.03	0.02	-0.01	0.07	0.04	0.03	0.01	0.03	0.02	0.00	0.05	0.03	0.03	58
0.06	0.11	0.31	0.24	-0.00	0.62	0.31	0.41	0.02	0.07	0.05	0.01	0.12	0.05	0.09	0.03	0.06	0.05	0.02	0.09	0.04	0.08	1300
0.11	0.15	0.46	0.35	0.04	0.89	0.43	0.66	0.04	0.08	0.07	0.02	0.15	0.06	0.13	0.04	0.07	0.06	0.03	0.11	0.04	0.10	1056
0.15	0.27	0.69	0.54	0.03	1.35	0.66	0.89	0.05	0.11	0.10	0.04	0.17	0.06	0.15	0.06	0.09	0.09	0.05	0.13	0.04	0.12	748
0.18	0.37	0.93	0.77	0.14	1.72	0.79	1.24	0.07	0.12	0.11	0.05	0.19	0.07	0.17	0.07	0.10	0.10	0.06	0.14	0.04	0.13	946
0.32	0.71	1.79	1.36	0.18	3.39	1.61	2.36	0.10	0.15	0.16	0.08	0.23	0.07	0.21	0.10	0.13	0.13	0.08	0.18	0.05	0.16	2614


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.26
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.94	0.94	0.91	0.97	0.03	0.96	0.93	0.95	0.96	0.91	0.98	0.04	0.97	0.92	0.94	0.96	0.88	1.00	0.06	0.99	58
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.89	0.91	0.92	0.87	0.95	0.04	0.94	0.89	0.92	0.94	0.84	0.99	0.07	0.98	1300
0.11	0.86	0.88	0.88	0.85	0.92	0.04	0.91	0.86	0.89	0.89	0.84	0.93	0.05	0.92	0.85	0.89	0.91	0.81	0.98	0.08	0.96	1056
0.15	0.84	0.86	0.86	0.82	0.90	0.04	0.88	0.83	0.86	0.87	0.81	0.91	0.05	0.90	0.82	0.87	0.89	0.79	0.96	0.09	0.94	748
0.18	0.81	0.84	0.84	0.80	0.87	0.04	0.86	0.81	0.84	0.85	0.79	0.89	0.05	0.88	0.80	0.85	0.87	0.76	0.94	0.09	0.92	946
0.32	0.77	0.80	0.80	0.75	0.84	0.05	0.83	0.77	0.80	0.80	0.75	0.86	0.05	0.84	0.74	0.80	0.82	0.70	0.91	0.10	0.88	2614


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	1.89	4.06	3.14	1.39	6.73	2.67	5.24	1.43	3.95	2.16	0.46	7.44	3.49	5.55	0.56	2.48	1.63	-0.07	5.04	2.55	3.36	58
0.06	3.45	4.21	4.25	2.60	5.81	1.60	4.64	0.69	4.01	1.65	-7.82	15.84	11.83	4.25	1.25	3.50	2.65	0.44	6.57	3.06	4.76	1300
0.11	2.24	3.47	3.01	1.59	5.36	1.88	3.85	0.70	3.98	1.80	-1.49	9.45	5.47	5.12	1.23	3.46	2.77	0.51	6.41	2.95	4.91	1056
0.15	3.19	4.42	3.85	2.46	6.39	1.97	4.87	0.86	4.36	2.14	-1.47	10.19	5.83	6.01	1.43	3.85	3.12	0.66	7.04	3.19	5.51	748
0.18	4.54	5.45	5.02	3.87	7.03	1.58	6.01	0.88	4.60	2.19	-1.65	10.85	6.25	5.46	1.55	3.99	3.31	0.87	7.11	3.12	5.75	946
0.32	7.19	9.28	9.30	6.82	11.74	2.46	11.22	0.86	4.72	2.24	-1.68	11.11	6.39	6.09	1.51	4.10	3.32	0.75	7.46	3.35	6.06	2614


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/time_misc_auc.tex <==
name	auc
attack_time	1.64
l2	1.27
lom	1.09


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.37	0.33	0.00	0.73	0.37	0.60	0.27	0.49	0.47	0.25	0.72	0.24	0.67	0.54	0.65	0.57	0.49	0.80	0.15	0.77	58
0.06	0.00	0.16	0.00	-0.06	0.39	0.23	0.33	0.25	0.37	0.38	0.19	0.56	0.18	0.50	0.45	0.55	0.56	0.41	0.70	0.15	0.65	1300
0.11	0.00	0.13	0.00	-0.08	0.34	0.21	0.33	0.20	0.33	0.31	0.14	0.52	0.19	0.44	0.41	0.52	0.52	0.38	0.66	0.14	0.61	1056
0.15	0.00	0.09	0.00	-0.10	0.27	0.19	0.00	0.12	0.27	0.25	0.09	0.45	0.18	0.38	0.38	0.47	0.47	0.33	0.61	0.14	0.56	748
0.18	0.00	0.05	0.00	-0.10	0.20	0.15	0.00	0.11	0.22	0.20	0.06	0.38	0.16	0.33	0.35	0.43	0.42	0.30	0.56	0.13	0.50	946
0.32	0.00	0.03	0.00	-0.10	0.17	0.13	0.00	0.00	0.15	0.11	-0.01	0.30	0.15	0.22	0.28	0.37	0.35	0.23	0.50	0.13	0.43	2614


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.08
top50	0.13


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	55.91	121.23	100.16	47.19	195.27	74.04	161.33	1.75	2.71	3.00	1.53	3.90	1.18	4.00	81.12	144.91	131.45	70.04	219.79	74.87	200.79	2.00	2.86	3.00	1.68	4.03	1.18	4.00	28
0.06	100.92	184.93	151.00	45.29	324.58	139.64	225.14	3.00	4.28	4.00	2.57	5.99	1.71	5.00	128.09	226.77	189.70	58.31	395.24	168.47	274.98	3.00	4.25	4.00	2.50	5.99	1.74	5.00	1219
0.11	103.39	195.03	158.49	47.46	342.60	147.57	238.88	3.00	4.19	4.00	2.45	5.93	1.74	5.00	154.82	275.89	225.21	78.61	473.16	197.27	341.03	3.00	4.21	4.00	2.42	6.00	1.79	5.00	1049
0.15	104.01	191.66	157.77	50.32	333.00	141.34	232.85	3.00	4.09	4.00	2.38	5.80	1.71	5.00	180.26	309.27	246.68	97.48	521.07	211.79	383.41	3.00	4.11	4.00	2.30	5.93	1.82	5.00	793
0.18	102.01	190.64	151.30	37.52	343.76	153.12	230.31	3.00	4.19	4.00	2.48	5.90	1.71	5.00	203.71	359.06	290.62	87.44	630.67	271.62	418.83	3.00	4.23	4.00	2.44	6.02	1.79	5.00	1024
0.32	102.17	193.22	154.28	32.55	353.89	160.67	228.13	3.00	4.11	4.00	2.37	5.85	1.74	5.00	282.83	517.48	421.28	154.92	880.04	362.56	636.54	3.00	4.24	4.00	2.37	6.11	1.87	5.00	2512


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/comparison_vals_auc.tex <==
name	auc
orig_pp	54.44
orig_ge	1.19
adv_pp	100.91
adv_ge	1.20


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.63	0.70	0.74	0.53	0.87	0.17	0.78	0.74	0.81	0.79	0.72	0.91	0.10	0.88	0.58	0.65	0.63	0.54	0.77	0.11	0.73	28
0.06	0.25	0.43	0.43	0.17	0.68	0.26	0.62	0.53	0.63	0.68	0.41	0.85	0.22	0.79	0.38	0.49	0.52	0.30	0.68	0.19	0.63	1219
0.11	0.13	0.31	0.30	0.05	0.57	0.26	0.49	0.38	0.52	0.57	0.27	0.76	0.25	0.70	0.28	0.40	0.42	0.20	0.60	0.20	0.54	1049
0.15	0.03	0.20	0.18	-0.03	0.44	0.24	0.36	0.24	0.41	0.44	0.16	0.66	0.25	0.61	0.17	0.31	0.32	0.11	0.50	0.20	0.46	793
0.18	-0.04	0.12	0.11	-0.10	0.34	0.22	0.25	0.17	0.33	0.35	0.07	0.58	0.25	0.52	0.12	0.24	0.25	0.05	0.43	0.19	0.38	1024
0.32	-0.18	-0.04	-0.06	-0.25	0.18	0.22	0.08	-0.09	0.11	0.12	-0.17	0.39	0.28	0.31	-0.06	0.08	0.08	-0.12	0.28	0.20	0.23	2512


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/correlations_auc.tex <==
name	auc
pcc	0.06
spearman	0.11
kendall	0.08


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	1.53	2.62	2.54	1.19	4.04	1.42	3.35	1.67	2.73	2.39	1.25	4.21	1.48	3.94	1.32	5.32	2.65	-0.62	11.26	5.94	10.56	28
0.06	2.04	3.55	3.21	1.45	5.64	2.10	4.59	2.11	4.19	3.42	1.02	7.35	3.16	5.27	2.05	7.70	4.22	-1.10	16.51	8.80	9.58	1219
0.11	2.10	3.29	3.05	1.63	4.96	1.66	4.16	2.24	3.88	3.34	1.39	6.37	2.49	4.72	2.25	6.82	3.85	-1.13	14.77	7.95	7.62	1049
0.15	2.19	3.15	3.00	1.80	4.51	1.36	3.95	2.34	3.59	3.16	1.68	5.51	1.91	4.48	2.07	6.05	3.40	-1.06	13.15	7.11	6.76	793
0.18	2.18	2.93	2.81	1.84	4.02	1.09	3.54	2.23	3.29	2.91	1.72	4.85	1.56	4.03	2.07	5.23	3.22	-1.00	11.46	6.23	5.43	1024
0.32	2.16	2.70	2.59	1.85	3.55	0.85	3.11	2.19	2.95	2.75	1.80	4.11	1.16	3.45	2.02	3.92	2.91	0.07	7.76	3.84	4.36	2512


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/ets_sts_auc.tex <==
name	auc
et_use	0.88
et_tse	0.99
et_ce	1.63


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.25	0.88	0.63	0.11	1.65	0.77	1.18	1.81	4.26	3.31	0.88	7.64	3.38	6.31	1.50	4.34	3.31	0.43	8.25	3.91	5.91	28
0.06	0.51	3.74	1.07	-9.29	16.77	13.03	2.32	2.80	7.91	5.25	-0.26	16.08	8.17	10.39	2.39	10.53	5.13	-9.49	30.55	20.02	11.76	1219
0.11	0.40	2.98	0.80	-7.90	13.85	10.88	1.77	2.76	6.03	4.17	-0.62	12.68	6.65	6.76	2.24	7.28	3.73	-6.22	20.78	13.50	7.52	1049
0.15	0.34	1.64	0.65	-2.12	5.39	3.75	1.33	2.76	5.20	4.12	1.03	9.38	4.17	6.22	2.19	7.17	3.54	-14.05	28.40	21.23	6.21	793
0.18	0.27	1.69	0.49	-6.47	9.85	8.16	0.95	2.81	5.03	4.02	1.05	9.00	3.98	5.80	2.31	6.77	3.26	-10.70	24.24	17.47	6.06	1024
0.32	0.17	1.35	0.30	-9.54	12.25	10.90	0.60	2.89	4.57	3.73	1.12	8.02	3.45	5.00	2.36	6.48	3.17	-15.43	28.40	21.91	5.07	2512


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.59
et_p_h	1.58
et_p_l2	2.09


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.11	0.28	0.21	0.07	0.49	0.21	0.43	0.02	0.07	0.03	0.00	0.14	0.07	0.13	0.02	0.06	0.03	0.01	0.11	0.05	0.10	28
0.06	0.13	0.33	0.26	0.02	0.65	0.31	0.45	0.02	0.07	0.05	0.01	0.12	0.06	0.10	0.03	0.06	0.05	0.02	0.10	0.04	0.09	1219
0.11	0.19	0.54	0.42	0.08	1.00	0.46	0.77	0.05	0.10	0.09	0.04	0.17	0.07	0.15	0.05	0.09	0.08	0.04	0.13	0.04	0.12	1049
0.15	0.32	0.77	0.61	0.14	1.39	0.62	1.06	0.06	0.12	0.11	0.05	0.18	0.07	0.17	0.07	0.10	0.09	0.06	0.14	0.04	0.13	793
0.18	0.44	1.11	0.91	0.22	2.00	0.89	1.50	0.07	0.13	0.13	0.06	0.20	0.07	0.18	0.08	0.11	0.11	0.07	0.16	0.04	0.15	1024
0.32	0.87	2.20	1.70	0.20	4.20	2.00	2.89	0.10	0.16	0.17	0.08	0.24	0.08	0.21	0.10	0.14	0.14	0.09	0.19	0.05	0.17	2512


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.31
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.94	0.94	0.91	0.96	0.03	0.96	0.92	0.94	0.93	0.91	0.97	0.03	0.96	0.90	0.93	0.93	0.88	0.99	0.05	0.99	28
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.89	0.91	0.92	0.87	0.96	0.04	0.94	0.87	0.91	0.93	0.84	0.99	0.07	0.97	1219
0.11	0.86	0.88	0.89	0.85	0.92	0.04	0.91	0.87	0.89	0.90	0.85	0.94	0.04	0.92	0.85	0.90	0.91	0.82	0.97	0.08	0.96	1049
0.15	0.84	0.86	0.87	0.83	0.90	0.04	0.89	0.84	0.87	0.88	0.82	0.92	0.05	0.91	0.82	0.87	0.88	0.78	0.96	0.09	0.94	793
0.18	0.81	0.84	0.84	0.80	0.88	0.04	0.87	0.82	0.85	0.85	0.80	0.90	0.05	0.89	0.80	0.85	0.86	0.76	0.94	0.09	0.92	1024
0.32	0.77	0.80	0.80	0.75	0.85	0.05	0.83	0.77	0.81	0.81	0.75	0.87	0.06	0.85	0.75	0.81	0.82	0.71	0.91	0.10	0.88	2512


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	1.22	2.60	1.90	0.74	4.46	1.86	5.15	78.50	340.44	168.85	-269.78	950.66	610.22	263.46	0.17	1.11	1.24	0.24	1.98	0.87	1.52	28
0.06	2.03	3.73	3.94	1.56	5.90	2.17	4.45	53.58	655.37	193.85	-1098.40	2409.13	1753.76	594.55	0.58	1.55	1.15	0.16	2.94	1.39	2.14	1219
0.11	1.15	1.83	1.47	0.72	2.94	1.11	2.04	68.18	812.83	237.13	-1966.20	3591.85	2779.03	644.25	0.55	1.77	1.35	0.14	3.40	1.63	2.44	1049
0.15	1.68	2.56	2.12	1.27	3.85	1.29	2.97	90.03	809.94	299.74	-625.16	2245.03	1435.10	885.43	0.76	2.09	1.52	0.17	4.00	1.92	2.84	793
0.18	2.29	3.10	2.83	1.90	4.31	1.20	3.65	106.11	988.83	350.24	-1558.88	3536.54	2547.71	985.19	0.71	2.02	1.56	0.27	3.78	1.76	2.90	1024
0.32	3.85	4.81	4.72	3.49	6.14	1.32	5.62	129.78	1109.35	410.41	-1574.63	3793.33	2683.98	1103.96	0.71	2.04	1.58	0.25	3.83	1.79	2.83	2512


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/time_misc_auc.tex <==
name	auc
attack_time	0.95
l2	257.59
lom	0.55


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.50	0.63	0.60	0.44	0.83	0.20	0.80	0.66	0.71	0.73	0.60	0.82	0.11	0.78	0.80	0.83	0.84	0.75	0.91	0.08	0.88	28
0.06	0.00	0.28	0.33	0.01	0.56	0.27	0.50	0.48	0.59	0.62	0.41	0.77	0.18	0.73	0.68	0.75	0.77	0.64	0.87	0.11	0.84	1219
0.11	0.00	0.21	0.00	-0.04	0.46	0.25	0.33	0.40	0.52	0.55	0.33	0.71	0.19	0.67	0.62	0.70	0.71	0.58	0.83	0.12	0.80	1049
0.15	0.00	0.13	0.00	-0.08	0.33	0.21	0.33	0.33	0.45	0.45	0.28	0.62	0.17	0.57	0.57	0.66	0.67	0.53	0.79	0.13	0.76	793
0.18	0.00	0.10	0.00	-0.09	0.28	0.19	0.00	0.29	0.40	0.40	0.23	0.57	0.17	0.50	0.55	0.63	0.62	0.51	0.75	0.12	0.71	1024
0.32	0.00	0.05	0.00	-0.09	0.18	0.14	0.00	0.18	0.30	0.29	0.14	0.46	0.16	0.40	0.46	0.54	0.55	0.42	0.67	0.13	0.63	2512


==> data/mlm_plots/mlm_distil_fast/agnews/xlnet/s/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.13
top50	0.19


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	35.37	49.63	43.34	26.74	72.53	22.89	56.64	71.00	82.41	84.00	57.33	107.49	25.08	97.00	38.82	53.82	48.25	30.20	77.45	23.63	61.57	70.00	81.75	83.00	56.74	106.75	25.00	96.00	849
0.03	35.12	51.93	43.96	22.05	81.80	29.88	57.79	69.00	81.35	84.00	53.37	109.34	27.98	98.00	44.32	62.54	54.57	30.28	94.79	32.25	70.39	68.00	80.37	83.00	52.70	108.03	27.67	97.00	986
0.06	35.18	55.58	44.20	10.95	100.21	44.63	59.08	67.00	79.49	83.00	49.85	109.14	29.65	98.00	52.73	77.75	65.65	23.30	132.20	54.45	84.68	65.00	78.31	82.00	49.18	107.44	29.13	96.00	1009
0.11	35.23	57.20	43.95	-1.72	116.12	58.92	58.54	68.00	79.99	84.00	50.37	109.61	29.62	98.00	63.20	92.98	76.52	13.69	172.27	79.29	96.85	66.00	78.36	82.00	49.33	107.39	29.03	96.00	882
0.15	35.37	57.75	44.40	7.09	108.40	50.65	59.14	66.00	78.22	83.00	48.29	108.16	29.94	98.00	82.31	118.91	99.07	31.99	205.83	86.92	122.80	64.00	76.37	81.00	47.24	105.50	29.13	95.00	689
0.18	35.56	64.56	44.80	-95.51	224.63	160.07	59.57	65.00	77.85	83.00	48.32	107.38	29.53	98.00	102.14	148.45	123.60	-10.50	307.40	158.95	149.74	62.00	75.02	80.00	46.31	103.73	28.71	93.00	561
0.32	35.66	58.27	44.49	5.06	111.47	53.20	59.14	65.00	78.83	84.00	49.00	108.66	29.83	99.00	136.53	200.35	169.70	66.19	334.51	134.16	217.61	60.50	74.65	78.00	45.43	103.87	29.22	94.00	787


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/comparison_vals_auc.tex <==
name	auc
orig_pp	18.21
orig_ge	24.55
adv_pp	40.13
adv_ge	23.80


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.06	0.40	0.63	-0.04	0.84	0.44	0.73	0.35	0.47	0.49	0.24	0.70	0.23	0.62	0.25	0.35	0.36	0.17	0.53	0.18	0.46	849
0.03	-0.07	0.28	0.54	-0.18	0.75	0.46	0.65	0.32	0.44	0.48	0.20	0.69	0.25	0.61	0.23	0.33	0.34	0.14	0.52	0.19	0.45	986
0.06	-0.15	0.19	0.45	-0.27	0.66	0.47	0.56	0.29	0.41	0.47	0.16	0.66	0.25	0.58	0.20	0.30	0.33	0.11	0.50	0.19	0.42	1009
0.11	-0.21	0.13	0.35	-0.32	0.58	0.45	0.49	0.27	0.39	0.45	0.16	0.63	0.23	0.55	0.19	0.29	0.32	0.11	0.46	0.17	0.40	882
0.15	-0.17	0.09	0.23	-0.31	0.48	0.39	0.39	0.25	0.36	0.41	0.14	0.58	0.22	0.50	0.18	0.26	0.29	0.10	0.42	0.16	0.36	689
0.18	-0.23	0.02	0.13	-0.36	0.39	0.38	0.32	0.21	0.32	0.37	0.11	0.54	0.21	0.46	0.15	0.23	0.26	0.08	0.39	0.15	0.33	561
0.32	-0.23	-0.03	0.06	-0.37	0.31	0.34	0.23	0.17	0.28	0.32	0.06	0.50	0.22	0.42	0.12	0.20	0.22	0.04	0.35	0.15	0.30	787


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/correlations_auc.tex <==
name	auc
pcc	0.03
spearman	0.11
kendall	0.08


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	4.94	14.25	8.42	1.20	27.31	13.06	21.21	3.82	12.47	6.34	-1.17	26.11	13.64	16.45	2.63	7.88	4.73	-1.22	16.99	9.11	9.66	849
0.03	3.88	10.11	6.99	1.14	19.09	8.97	14.00	2.94	8.09	4.85	-0.91	17.09	9.00	9.44	2.27	6.30	3.87	-1.33	13.92	7.62	7.26	986
0.06	3.27	7.13	5.16	1.81	12.46	5.32	10.03	2.32	5.04	3.58	0.33	9.76	4.72	5.90	1.71	4.26	2.98	-0.45	8.96	4.70	4.77	1009
0.11	3.07	5.91	4.47	2.23	9.59	3.68	8.44	2.03	3.76	3.11	1.35	6.17	2.41	4.74	1.49	3.28	2.40	-0.03	6.58	3.30	3.94	882
0.15	2.86	4.83	3.95	2.12	7.54	2.71	6.50	1.82	3.07	2.60	1.36	4.78	1.71	3.93	1.41	2.69	2.07	-0.58	5.95	3.27	3.06	689
0.18	2.76	4.47	3.78	2.17	6.77	2.30	5.90	1.78	2.94	2.48	1.34	4.54	1.60	3.69	1.45	2.40	1.93	0.49	4.31	1.91	2.73	561
0.32	2.59	3.80	3.32	2.07	5.54	1.74	4.76	1.72	2.70	2.27	1.33	4.07	1.37	3.41	1.30	2.10	1.76	0.08	4.12	2.02	2.46	787


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/ets_sts_auc.tex <==
name	auc
et_use	1.76
et_tse	1.25
et_ce	1.00


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.39	5.70	2.99	-5.21	16.61	10.91	5.92	2.75	7.78	4.95	1.13	14.42	6.65	11.68	2.17	6.86	4.54	0.52	13.19	6.33	9.90	849
0.03	0.76	2.06	1.34	-1.12	5.23	3.17	2.48	2.38	5.74	3.81	1.21	10.28	4.54	8.58	1.89	4.95	3.29	-0.29	10.19	5.24	7.03	986
0.06	0.48	1.23	0.81	-1.25	3.71	2.48	1.42	2.27	4.74	3.44	1.33	8.14	3.40	6.87	1.82	4.20	2.99	-1.14	9.53	5.33	5.75	1009
0.11	0.36	0.73	0.57	-0.05	1.51	0.78	0.90	2.23	4.11	3.21	1.71	6.50	2.40	5.84	1.79	3.56	2.72	0.17	6.94	3.38	4.95	882
0.15	0.26	0.47	0.36	-0.26	1.20	0.73	0.52	2.21	3.51	2.97	1.59	5.44	1.93	4.55	1.80	3.08	2.47	-0.23	6.39	3.31	3.82	689
0.18	0.21	0.38	0.28	-0.52	1.28	0.90	0.39	2.21	3.34	2.90	1.63	5.06	1.71	4.22	1.77	2.93	2.49	0.46	5.40	2.47	3.49	561
0.32	0.14	0.33	0.18	-2.21	2.87	2.54	0.26	2.18	2.97	2.62	1.80	4.14	1.17	3.59	1.78	2.60	2.24	0.72	4.48	1.88	3.02	787


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.26
et_p_h	1.21
et_p_l2	1.06


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.10	0.09	0.04	0.15	0.06	0.13	0.04	0.06	0.05	0.03	0.08	0.03	0.07	0.03	0.05	0.04	0.03	0.06	0.02	0.05	849
0.03	0.17	0.23	0.23	0.14	0.33	0.10	0.29	0.07	0.09	0.08	0.05	0.12	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	986
0.06	0.36	0.45	0.45	0.29	0.62	0.17	0.55	0.09	0.12	0.11	0.08	0.16	0.04	0.14	0.08	0.09	0.09	0.07	0.12	0.02	0.11	1009
0.11	0.57	0.72	0.71	0.46	0.99	0.27	0.86	0.12	0.14	0.14	0.10	0.18	0.04	0.16	0.10	0.11	0.11	0.09	0.14	0.03	0.13	882
0.15	0.95	1.21	1.19	0.78	1.64	0.43	1.45	0.14	0.17	0.17	0.12	0.22	0.05	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.15	689
0.18	1.33	1.72	1.70	1.08	2.36	0.64	2.06	0.16	0.19	0.19	0.14	0.24	0.05	0.21	0.14	0.15	0.15	0.12	0.19	0.03	0.17	561
0.32	1.96	2.86	2.65	1.51	4.22	1.35	3.55	0.19	0.22	0.22	0.17	0.27	0.05	0.25	0.16	0.18	0.18	0.15	0.21	0.03	0.20	787


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.44
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.98	0.96	0.99	0.02	0.98	0.96	0.96	0.97	0.93	0.99	0.03	0.98	0.93	0.94	0.96	0.90	0.99	0.05	0.97	849
0.03	0.95	0.95	0.96	0.92	0.99	0.03	0.97	0.91	0.93	0.95	0.88	0.98	0.05	0.97	0.87	0.91	0.93	0.83	0.99	0.08	0.96	986
0.06	0.93	0.93	0.94	0.88	0.98	0.05	0.95	0.86	0.89	0.91	0.83	0.96	0.06	0.94	0.81	0.86	0.87	0.76	0.96	0.10	0.93	1009
0.11	0.91	0.92	0.93	0.87	0.96	0.04	0.94	0.83	0.87	0.87	0.81	0.93	0.06	0.91	0.77	0.82	0.82	0.73	0.92	0.09	0.89	882
0.15	0.89	0.89	0.91	0.84	0.94	0.05	0.92	0.80	0.83	0.84	0.77	0.89	0.06	0.87	0.74	0.78	0.79	0.68	0.88	0.10	0.84	689
0.18	0.87	0.88	0.89	0.82	0.93	0.05	0.90	0.78	0.81	0.82	0.75	0.87	0.06	0.85	0.71	0.76	0.77	0.66	0.85	0.09	0.81	561
0.32	0.84	0.85	0.86	0.80	0.90	0.05	0.88	0.75	0.79	0.79	0.72	0.85	0.06	0.83	0.68	0.72	0.73	0.62	0.81	0.10	0.77	787


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	32.95	39.35	41.06	20.43	58.26	18.91	48.01	0.06	0.17	0.09	-0.03	0.36	0.19	0.22	6.07	54.98	20.15	-12.27	122.23	67.25	93.38	849
0.03	40.60	47.96	49.88	21.63	74.28	26.32	57.37	0.07	0.19	0.10	-0.03	0.42	0.22	0.25	9.60	61.57	28.74	-5.95	129.09	67.52	105.01	986
0.06	49.68	63.53	64.28	18.18	108.88	45.35	74.26	0.07	0.22	0.10	-0.03	0.46	0.25	0.29	12.08	64.27	34.57	-2.47	131.01	66.74	104.91	1009
0.11	70.12	83.74	84.18	33.09	134.39	50.65	98.97	0.07	0.22	0.11	-0.02	0.46	0.24	0.29	15.46	66.44	41.66	0.81	132.07	65.63	100.39	882
0.15	89.65	106.14	110.23	53.12	159.15	53.02	128.69	0.07	0.23	0.11	-0.03	0.50	0.26	0.32	15.21	67.69	45.47	2.30	133.07	65.39	94.02	689
0.18	110.70	135.12	137.12	63.78	206.46	71.34	165.47	0.08	0.24	0.11	-0.02	0.49	0.26	0.34	15.57	68.43	49.35	4.50	132.37	63.94	97.44	561
0.32	146.65	193.47	186.35	93.66	293.28	99.81	244.34	0.08	0.24	0.12	-0.03	0.51	0.27	0.32	17.10	71.03	56.19	7.86	134.21	63.18	101.48	787


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/time_misc_auc.tex <==
name	auc
attack_time	36.55
l2	0.07
lom	20.84


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.56	0.64	0.67	0.47	0.81	0.17	0.76	0.53	0.60	0.62	0.47	0.74	0.14	0.69	0.60	0.66	0.66	0.56	0.76	0.10	0.72	849
0.03	0.50	0.58	0.62	0.41	0.76	0.17	0.70	0.51	0.59	0.61	0.45	0.73	0.14	0.68	0.59	0.65	0.66	0.55	0.76	0.10	0.71	986
0.06	0.44	0.52	0.56	0.34	0.71	0.18	0.64	0.49	0.57	0.60	0.43	0.72	0.14	0.67	0.59	0.65	0.66	0.54	0.75	0.10	0.71	1009
0.11	0.40	0.49	0.51	0.31	0.67	0.18	0.60	0.48	0.56	0.59	0.43	0.69	0.13	0.65	0.59	0.64	0.65	0.55	0.73	0.09	0.70	882
0.15	0.35	0.44	0.46	0.26	0.62	0.18	0.56	0.47	0.53	0.56	0.41	0.66	0.12	0.62	0.58	0.63	0.64	0.54	0.71	0.09	0.68	689
0.18	0.30	0.41	0.42	0.24	0.58	0.17	0.53	0.45	0.51	0.53	0.40	0.63	0.12	0.59	0.57	0.62	0.62	0.53	0.70	0.08	0.66	561
0.32	0.24	0.37	0.36	0.18	0.55	0.18	0.49	0.42	0.48	0.50	0.36	0.60	0.12	0.56	0.56	0.60	0.61	0.51	0.68	0.08	0.65	787


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/a/top_intersections_auc.tex <==
name	auc
top10	0.14
top30	0.17
top50	0.19


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	35.25	49.34	42.98	25.82	72.87	23.53	56.36	71.75	83.34	85.00	59.17	107.51	24.17	98.00	39.27	54.08	48.15	29.54	78.63	24.54	61.15	71.75	82.94	84.00	58.84	107.04	24.10	97.00	668
0.03	35.53	51.82	43.98	23.12	80.51	28.70	57.01	69.00	81.45	84.50	54.33	108.58	27.13	99.00	44.20	62.79	54.88	31.51	94.07	31.28	69.87	69.00	80.91	84.50	54.02	107.80	26.89	98.00	424
0.06	35.53	52.93	43.81	10.16	95.71	42.78	56.49	65.00	79.31	83.00	50.57	108.05	28.74	99.00	52.86	73.33	63.29	33.00	113.66	40.33	80.07	64.00	78.92	82.00	50.26	107.58	28.66	98.00	327
0.11	35.62	53.12	43.98	6.09	100.15	47.03	54.58	68.00	79.29	84.00	51.62	106.95	27.66	98.75	64.36	92.38	76.86	-15.50	200.26	107.88	94.10	69.00	79.24	82.50	51.50	106.98	27.74	99.00	262
0.15	37.29	56.20	44.49	10.17	102.23	46.03	58.70	65.00	77.87	82.00	47.96	107.79	29.91	98.00	83.66	125.79	104.74	-18.73	270.31	144.52	123.79	64.00	77.32	82.00	47.54	107.10	29.78	96.00	197
0.18	35.55	49.84	41.95	24.94	74.73	24.89	56.18	67.00	80.40	83.00	50.86	109.94	29.54	100.75	103.97	133.40	126.19	87.76	179.04	45.64	147.15	65.25	79.18	83.00	49.96	108.41	29.23	98.00	158
0.32	37.29	57.26	43.21	9.14	105.37	48.12	57.01	67.00	79.01	84.00	47.91	110.12	31.11	101.00	146.51	211.74	183.91	75.28	348.20	136.46	237.05	62.00	76.78	79.00	45.78	107.77	31.00	97.00	233


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	16.54
orig_ge	24.74
adv_pp	39.71
adv_ge	24.42


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.81	-0.53	-0.60	-0.89	-0.17	0.36	-0.32	-0.37	-0.15	-0.17	-0.49	0.19	0.34	0.07	-0.28	-0.12	-0.13	-0.39	0.15	0.27	0.05	668
0.03	-0.87	-0.61	-0.69	-0.94	-0.28	0.33	-0.46	-0.41	-0.18	-0.19	-0.53	0.17	0.35	0.04	-0.31	-0.14	-0.14	-0.42	0.14	0.28	0.03	424
0.06	-0.88	-0.65	-0.72	-0.96	-0.34	0.31	-0.53	-0.42	-0.20	-0.20	-0.54	0.14	0.34	0.04	-0.31	-0.15	-0.15	-0.43	0.12	0.27	0.04	327
0.11	-0.89	-0.68	-0.75	-0.95	-0.41	0.27	-0.55	-0.39	-0.21	-0.22	-0.52	0.09	0.30	-0.02	-0.30	-0.16	-0.16	-0.41	0.09	0.25	-0.01	262
0.15	-0.92	-0.70	-0.78	-0.96	-0.44	0.26	-0.53	-0.44	-0.26	-0.22	-0.56	0.04	0.30	-0.01	-0.33	-0.20	-0.16	-0.45	0.05	0.25	-0.01	197
0.18	-0.93	-0.72	-0.79	-0.97	-0.47	0.25	-0.60	-0.45	-0.27	-0.24	-0.56	0.02	0.29	-0.06	-0.33	-0.21	-0.18	-0.45	0.03	0.24	-0.04	158
0.32	-0.94	-0.77	-0.84	-0.99	-0.56	0.21	-0.67	-0.45	-0.29	-0.27	-0.56	-0.03	0.26	-0.12	-0.34	-0.22	-0.19	-0.44	-0.01	0.22	-0.08	233


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/correlations_auc.tex <==
name	auc
pcc	-0.22
spearman	-0.08
kendall	-0.06


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	23.35	35.15	32.41	19.14	51.15	16.00	44.81	15.37	32.70	28.79	12.54	52.86	20.16	46.66	8.81	19.99	15.62	5.36	34.61	14.62	28.04	668
0.03	15.87	23.25	21.16	11.92	34.59	11.33	28.01	8.56	20.18	15.92	5.51	34.84	14.67	28.79	5.41	14.11	10.36	2.81	25.41	11.30	19.30	424
0.06	11.87	14.78	14.24	8.51	21.05	6.27	18.01	5.49	11.49	8.85	3.09	19.88	8.40	15.82	3.97	8.81	5.73	0.84	16.77	7.96	11.21	327
0.11	8.76	11.16	11.46	7.10	15.23	4.07	13.55	4.70	7.80	6.57	3.26	12.33	4.53	9.54	3.59	6.30	4.75	1.68	10.92	4.62	7.22	262
0.15	7.40	9.07	9.58	6.15	11.98	2.92	11.08	4.22	5.93	5.15	3.29	8.57	2.64	6.89	3.46	4.70	4.12	2.47	6.93	2.23	5.42	197
0.18	6.33	7.73	7.89	5.20	10.26	2.53	9.61	3.90	5.32	4.94	3.12	7.52	2.20	6.26	3.17	4.02	3.73	2.54	5.50	1.48	4.72	158
0.32	5.53	6.61	6.71	4.73	8.49	1.88	7.95	3.91	4.92	4.56	2.94	6.90	1.98	5.41	2.96	3.61	3.41	2.12	5.10	1.49	3.99	233


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/ets_sts_auc.tex <==
name	auc
et_use	3.47
et_tse	2.65
et_ce	1.95


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	5.51	13.18	7.60	-19.76	46.13	32.95	10.98	12.66	18.26	16.66	9.46	27.07	8.81	21.68	9.63	15.90	13.58	5.14	26.67	10.77	18.88	668
0.03	2.82	4.84	3.52	-4.40	14.07	9.23	4.51	9.43	12.31	11.87	7.85	16.78	4.47	14.57	7.24	10.47	9.57	4.25	16.70	6.23	12.42	424
0.06	1.47	2.11	1.87	0.61	3.61	1.50	2.33	7.49	9.22	9.05	5.88	12.57	3.34	10.48	5.82	7.75	7.23	3.15	12.34	4.59	8.81	327
0.11	0.95	1.36	1.17	-0.19	2.92	1.55	1.44	6.46	7.53	7.39	5.69	9.37	1.84	8.72	4.98	6.24	6.07	4.20	8.28	2.04	7.32	262
0.15	0.57	0.80	0.69	0.13	1.47	0.67	0.84	5.41	6.24	6.15	4.85	7.62	1.38	6.87	4.41	5.26	5.03	3.54	6.98	1.72	5.66	197
0.18	0.38	0.53	0.47	0.26	0.81	0.28	0.59	4.98	5.53	5.53	4.44	6.62	1.09	6.13	3.98	4.62	4.48	3.24	6.01	1.39	5.14	158
0.32	0.23	0.42	0.30	-0.54	1.37	0.95	0.39	4.44	5.02	5.02	4.02	6.02	1.00	5.54	3.63	4.33	4.17	2.79	5.87	1.54	4.72	233


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.50
et_p_h	2.24
et_p_l2	1.89


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.10	0.10	0.05	0.16	0.05	0.14	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.06	0.02	0.06	668
0.03	0.18	0.23	0.23	0.14	0.33	0.09	0.29	0.07	0.09	0.09	0.05	0.12	0.04	0.11	0.06	0.07	0.07	0.05	0.09	0.02	0.08	424
0.06	0.36	0.46	0.45	0.30	0.62	0.16	0.56	0.09	0.12	0.12	0.08	0.16	0.04	0.14	0.08	0.10	0.09	0.07	0.12	0.02	0.11	327
0.11	0.60	0.76	0.74	0.44	1.09	0.32	0.86	0.12	0.15	0.14	0.10	0.19	0.04	0.17	0.10	0.12	0.12	0.09	0.14	0.03	0.13	262
0.15	1.02	1.28	1.27	0.82	1.74	0.46	1.51	0.15	0.17	0.17	0.13	0.22	0.04	0.20	0.13	0.14	0.14	0.11	0.17	0.03	0.15	197
0.18	1.46	1.84	1.86	1.27	2.41	0.57	2.20	0.17	0.20	0.20	0.15	0.24	0.04	0.22	0.14	0.16	0.16	0.13	0.18	0.03	0.17	158
0.32	2.30	3.11	2.96	1.83	4.39	1.28	3.84	0.20	0.22	0.22	0.17	0.27	0.05	0.25	0.17	0.18	0.18	0.15	0.21	0.03	0.20	233


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.48
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.98	0.96	0.99	0.02	0.98	0.96	0.96	0.97	0.93	0.99	0.03	0.98	0.91	0.94	0.95	0.88	0.99	0.05	0.97	668
0.03	0.95	0.96	0.96	0.92	0.99	0.03	0.97	0.91	0.94	0.95	0.89	0.98	0.05	0.97	0.86	0.90	0.92	0.82	0.98	0.08	0.96	424
0.06	0.93	0.93	0.94	0.88	0.98	0.05	0.95	0.86	0.89	0.90	0.83	0.96	0.06	0.95	0.79	0.85	0.86	0.74	0.95	0.10	0.92	327
0.11	0.91	0.91	0.93	0.86	0.96	0.05	0.94	0.83	0.87	0.87	0.81	0.92	0.06	0.91	0.77	0.82	0.82	0.72	0.91	0.10	0.88	262
0.15	0.89	0.90	0.91	0.85	0.94	0.04	0.92	0.80	0.84	0.84	0.78	0.89	0.05	0.88	0.75	0.79	0.80	0.70	0.88	0.09	0.84	197
0.18	0.87	0.87	0.89	0.82	0.93	0.06	0.90	0.79	0.82	0.82	0.76	0.88	0.06	0.86	0.72	0.76	0.76	0.66	0.85	0.09	0.82	158
0.32	0.84	0.85	0.87	0.80	0.91	0.05	0.89	0.77	0.80	0.80	0.75	0.86	0.05	0.84	0.70	0.73	0.74	0.64	0.82	0.09	0.77	233


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	55.95	91.19	74.97	38.45	143.94	52.74	123.13	0.72	19.32	5.46	-21.34	59.99	40.66	19.17	15.18	60.47	39.28	1.38	119.56	59.09	94.15	668
0.03	143.95	186.16	186.09	73.40	298.93	112.76	214.59	0.72	19.18	4.80	-27.16	65.52	46.34	15.90	15.29	58.09	37.89	0.66	115.52	57.43	88.96	424
0.06	198.23	265.80	246.69	68.74	462.86	197.06	295.76	0.62	19.67	3.97	-34.94	74.28	54.61	17.19	13.90	59.65	36.63	-3.36	122.66	63.01	90.07	327
0.11	246.95	355.68	301.23	93.25	618.10	262.42	389.80	0.67	15.16	4.11	-20.20	50.51	35.36	14.29	13.54	55.40	32.66	-3.95	114.76	59.36	85.73	262
0.15	298.06	409.63	390.81	174.52	644.74	235.11	476.41	0.62	16.35	3.77	-15.12	47.83	31.47	17.11	16.33	59.23	41.92	-0.42	118.88	59.65	84.58	197
0.18	378.17	498.12	484.07	252.05	744.19	246.07	589.06	0.78	16.02	4.31	-13.78	45.82	29.80	18.77	17.86	61.51	40.08	-0.48	123.49	61.99	83.77	158
0.32	490.97	644.71	638.12	336.34	953.08	308.37	791.00	0.66	16.44	3.97	-15.75	48.64	32.19	18.14	17.48	60.42	40.46	-3.01	123.85	63.43	79.80	233


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/time_misc_auc.tex <==
name	auc
attack_time	133.85
l2	5.23
lom	18.49


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.11	0.21	0.19	0.07	0.35	0.14	0.28	0.19	0.29	0.27	0.14	0.44	0.15	0.38	0.35	0.44	0.43	0.29	0.58	0.14	0.54	668
0.03	0.09	0.19	0.17	0.06	0.33	0.14	0.28	0.17	0.28	0.27	0.13	0.44	0.15	0.37	0.34	0.43	0.43	0.28	0.58	0.15	0.53	424
0.06	0.07	0.17	0.16	0.05	0.28	0.11	0.24	0.17	0.27	0.26	0.13	0.42	0.15	0.37	0.33	0.43	0.42	0.28	0.58	0.15	0.54	327
0.11	0.07	0.15	0.14	0.05	0.26	0.11	0.23	0.18	0.27	0.25	0.13	0.40	0.13	0.36	0.34	0.42	0.43	0.29	0.56	0.14	0.51	262
0.15	0.05	0.14	0.14	0.03	0.24	0.11	0.19	0.14	0.24	0.24	0.11	0.37	0.13	0.33	0.33	0.41	0.42	0.27	0.54	0.13	0.50	197
0.18	0.05	0.13	0.13	0.03	0.24	0.10	0.19	0.15	0.24	0.23	0.12	0.35	0.12	0.33	0.32	0.40	0.41	0.28	0.53	0.13	0.50	158
0.32	0.04	0.12	0.12	0.02	0.22	0.10	0.19	0.14	0.22	0.23	0.11	0.33	0.11	0.30	0.34	0.40	0.41	0.28	0.51	0.11	0.47	233


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/ig/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.08
top50	0.13


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	35.12	49.23	43.53	26.81	71.65	22.42	56.63	71.00	83.64	85.00	58.26	109.02	25.38	98.00	39.15	53.89	48.37	30.62	77.16	23.27	61.37	71.00	83.12	84.00	57.85	108.38	25.26	98.00	922
0.03	35.07	51.20	43.26	22.54	79.86	28.66	57.08	69.00	81.73	84.00	54.31	109.16	27.42	98.00	44.08	61.93	54.47	31.25	92.60	30.67	69.17	69.00	80.77	84.00	53.60	107.94	27.17	97.00	924
0.06	35.27	54.52	44.11	10.01	99.03	44.51	58.46	68.00	79.52	83.00	51.27	107.77	28.25	98.00	52.94	76.73	64.66	20.99	132.46	55.73	82.18	66.00	78.15	82.00	50.12	106.18	28.03	96.00	673
0.11	35.33	54.90	44.14	10.66	99.15	44.25	57.53	67.00	79.72	84.00	50.99	108.45	28.73	99.00	64.43	90.52	77.98	35.05	145.99	55.47	98.73	64.25	78.20	82.00	49.74	106.67	28.47	96.00	542
0.15	35.32	55.91	43.90	6.96	104.85	48.95	57.01	65.00	78.97	83.00	48.90	109.05	30.08	99.00	85.43	117.15	103.34	51.84	182.47	65.32	125.44	63.00	76.92	80.00	46.99	106.85	29.93	96.00	389
0.18	35.98	54.35	44.11	9.75	98.95	44.60	57.01	65.00	79.62	83.00	49.50	109.73	30.12	99.00	107.44	144.08	129.55	60.44	227.71	83.64	153.91	62.00	76.91	80.00	47.30	106.52	29.61	95.00	307
0.32	37.14	58.01	44.54	2.49	113.53	55.52	58.70	65.00	78.36	83.00	48.11	108.60	30.25	98.00	148.92	209.97	185.95	97.15	322.79	112.82	234.71	60.00	75.25	80.00	45.28	105.21	29.97	94.75	470


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/comparison_vals_auc.tex <==
name	auc
orig_pp	17.08
orig_ge	24.71
adv_pp	40.17
adv_ge	24.03


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.06	0.18	0.14	0.02	0.34	0.16	0.28	0.37	0.49	0.51	0.32	0.66	0.17	0.62	0.26	0.35	0.36	0.22	0.48	0.13	0.45	922
0.03	0.04	0.13	0.09	0.00	0.26	0.13	0.21	0.32	0.44	0.46	0.27	0.61	0.17	0.58	0.22	0.31	0.32	0.18	0.44	0.13	0.41	924
0.06	0.01	0.09	0.06	-0.02	0.20	0.11	0.15	0.26	0.39	0.39	0.22	0.56	0.17	0.53	0.17	0.27	0.27	0.15	0.40	0.13	0.37	673
0.11	0.00	0.07	0.05	-0.03	0.17	0.10	0.13	0.24	0.36	0.36	0.19	0.53	0.17	0.50	0.16	0.25	0.25	0.13	0.38	0.12	0.35	542
0.15	-0.01	0.05	0.03	-0.05	0.14	0.10	0.08	0.19	0.31	0.32	0.14	0.49	0.17	0.44	0.13	0.22	0.22	0.09	0.34	0.12	0.31	389
0.18	-0.02	0.03	0.01	-0.07	0.12	0.09	0.06	0.17	0.29	0.29	0.11	0.47	0.18	0.41	0.12	0.20	0.20	0.07	0.32	0.13	0.29	307
0.32	-0.04	-0.00	-0.00	-0.10	0.10	0.10	0.03	0.11	0.22	0.22	0.02	0.42	0.20	0.35	0.07	0.15	0.15	0.01	0.29	0.14	0.24	470


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/correlations_auc.tex <==
name	auc
pcc	0.02
spearman	0.10
kendall	0.07


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	12.27	16.97	16.06	10.00	23.95	6.97	20.50	8.85	15.58	14.42	6.81	24.35	8.77	20.79	4.89	10.74	8.67	2.72	18.76	8.02	13.99	922
0.03	8.18	10.91	10.33	6.31	15.51	4.60	12.74	4.85	9.28	7.80	3.12	15.44	6.16	11.91	3.03	7.06	5.10	1.00	13.11	6.05	9.12	924
0.06	6.04	7.41	7.44	4.85	9.97	2.56	8.81	3.35	5.63	4.86	2.32	8.94	3.31	7.06	2.27	4.58	3.23	-0.05	9.21	4.63	5.16	673
0.11	5.24	6.16	6.32	4.23	8.09	1.93	7.21	2.88	4.34	3.87	2.11	6.57	2.23	5.18	2.05	3.41	2.65	0.91	5.90	2.49	3.79	542
0.15	4.30	4.95	5.04	3.57	6.33	1.38	5.84	2.47	3.61	3.34	2.07	5.15	1.54	4.24	1.88	2.82	2.36	0.47	5.17	2.35	3.00	389
0.18	3.77	4.30	4.44	3.19	5.40	1.10	5.02	2.27	3.13	2.83	1.96	4.30	1.17	3.80	1.75	2.34	2.15	1.25	3.43	1.09	2.63	307
0.32	3.14	3.62	3.68	2.74	4.50	0.88	4.18	2.21	2.78	2.62	1.92	3.63	0.85	3.23	1.61	2.03	1.88	1.27	2.79	0.76	2.27	470


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/ets_sts_auc.tex <==
name	auc
et_use	1.81
et_tse	1.40
et_ce	1.06


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.90	6.12	3.95	-4.41	16.66	10.54	5.82	7.10	9.69	9.02	5.70	13.69	3.99	11.48	5.55	8.43	7.49	3.91	12.96	4.53	10.17	922
0.03	1.43	2.59	1.85	-2.23	7.40	4.82	2.50	5.19	6.71	6.27	3.99	9.43	2.72	7.63	4.05	5.75	5.13	2.39	9.11	3.36	6.63	924
0.06	0.81	1.86	0.99	-7.59	11.32	9.46	1.24	4.16	5.14	4.86	3.21	7.07	1.93	5.68	3.20	4.38	3.94	1.06	7.69	3.32	4.79	673
0.11	0.51	0.84	0.63	-0.42	2.09	1.25	0.77	3.51	4.29	4.06	2.61	5.96	1.68	4.67	2.76	3.62	3.28	0.98	6.26	2.64	3.88	542
0.15	0.31	0.49	0.37	-0.19	1.17	0.68	0.46	3.01	3.56	3.38	2.35	4.78	1.22	3.85	2.36	2.99	2.79	1.48	4.50	1.51	3.21	389
0.18	0.22	0.33	0.26	-0.02	0.68	0.35	0.32	2.73	3.17	3.06	2.29	4.06	0.89	3.40	2.12	2.63	2.50	1.65	3.62	0.99	2.84	307
0.32	0.13	0.23	0.17	-0.09	0.55	0.32	0.22	2.40	2.87	2.68	1.85	3.88	1.02	3.04	1.91	2.41	2.21	1.31	3.51	1.10	2.57	470


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.30
et_p_h	1.26
et_p_l2	1.06


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.11	0.10	0.06	0.15	0.05	0.14	0.04	0.06	0.06	0.03	0.08	0.02	0.07	0.04	0.05	0.05	0.03	0.06	0.02	0.06	922
0.03	0.18	0.24	0.24	0.14	0.33	0.10	0.29	0.07	0.09	0.09	0.06	0.12	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	924
0.06	0.36	0.47	0.46	0.29	0.64	0.18	0.57	0.09	0.12	0.12	0.08	0.16	0.04	0.14	0.08	0.09	0.09	0.07	0.12	0.02	0.11	673
0.11	0.60	0.75	0.75	0.49	1.00	0.25	0.90	0.12	0.14	0.14	0.10	0.19	0.04	0.16	0.10	0.12	0.11	0.09	0.14	0.03	0.13	542
0.15	1.06	1.30	1.29	0.86	1.73	0.43	1.55	0.15	0.17	0.17	0.13	0.22	0.04	0.20	0.12	0.14	0.14	0.11	0.17	0.03	0.16	389
0.18	1.52	1.87	1.85	1.25	2.48	0.62	2.17	0.17	0.20	0.19	0.15	0.24	0.05	0.23	0.14	0.16	0.16	0.13	0.19	0.03	0.18	307
0.32	2.24	3.14	2.91	1.79	4.49	1.35	3.85	0.19	0.22	0.22	0.17	0.28	0.05	0.26	0.16	0.18	0.18	0.15	0.22	0.03	0.21	470


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.48
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.94	1.00	0.03	0.98	0.96	0.96	0.97	0.93	1.00	0.03	0.98	0.92	0.93	0.95	0.87	1.00	0.06	0.97	922
0.03	0.95	0.95	0.96	0.91	0.99	0.04	0.96	0.91	0.93	0.95	0.88	0.98	0.05	0.96	0.86	0.89	0.92	0.81	0.98	0.08	0.95	924
0.06	0.93	0.93	0.94	0.88	0.98	0.05	0.95	0.87	0.89	0.91	0.84	0.95	0.06	0.94	0.80	0.85	0.86	0.75	0.94	0.10	0.91	673
0.11	0.91	0.91	0.93	0.87	0.96	0.05	0.94	0.84	0.87	0.88	0.81	0.93	0.06	0.91	0.78	0.82	0.82	0.73	0.91	0.09	0.88	542
0.15	0.89	0.89	0.91	0.84	0.95	0.05	0.92	0.81	0.85	0.86	0.79	0.91	0.06	0.89	0.75	0.79	0.80	0.69	0.88	0.10	0.84	389
0.18	0.88	0.87	0.89	0.82	0.93	0.06	0.90	0.79	0.83	0.83	0.77	0.88	0.06	0.87	0.73	0.76	0.77	0.66	0.86	0.10	0.81	307
0.32	0.84	0.85	0.87	0.79	0.91	0.06	0.88	0.77	0.80	0.81	0.75	0.86	0.06	0.84	0.70	0.73	0.74	0.63	0.82	0.09	0.78	470


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	46.59	57.21	58.13	35.77	78.65	21.44	69.75	0.16	195.91	0.68	-521.97	913.78	717.87	72.34	12.27	39.11	28.25	5.01	73.21	34.10	58.88	922
0.03	60.70	80.52	78.35	23.39	137.65	57.13	93.04	0.19	289.00	0.96	-732.20	1310.20	1021.20	102.12	12.10	42.08	30.68	4.93	79.23	37.15	63.72	924
0.06	84.62	122.00	110.40	29.28	214.73	92.72	135.77	0.24	270.09	1.22	-665.29	1205.47	935.38	132.31	12.98	45.32	36.54	6.99	83.65	38.33	69.58	673
0.11	108.06	166.68	142.45	39.61	293.75	127.07	181.71	0.24	282.48	1.95	-569.25	1134.22	851.73	97.80	12.02	43.80	36.68	7.23	80.36	36.57	68.01	542
0.15	146.11	213.89	193.04	82.19	345.58	131.70	253.03	0.25	285.22	1.50	-832.63	1403.06	1117.84	83.52	13.30	47.31	39.43	8.59	86.03	38.72	74.75	389
0.18	172.49	250.20	237.81	113.26	387.13	136.94	323.89	0.23	255.15	1.03	-824.16	1334.46	1079.31	61.29	12.95	46.59	40.33	10.04	83.14	36.55	70.50	307
0.32	206.48	296.24	296.42	146.83	445.65	149.41	404.61	0.27	263.26	0.94	-977.43	1503.95	1240.69	59.80	13.75	47.61	45.18	11.21	84.00	36.39	72.71	470


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/time_misc_auc.tex <==
name	auc
attack_time	64.51
l2	83.01
lom	14.20


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.20	0.31	0.30	0.16	0.46	0.15	0.42	0.46	0.54	0.54	0.43	0.65	0.11	0.62	0.63	0.68	0.69	0.61	0.75	0.07	0.73	922
0.03	0.16	0.26	0.24	0.12	0.40	0.14	0.36	0.43	0.51	0.50	0.40	0.62	0.11	0.59	0.61	0.66	0.67	0.59	0.73	0.07	0.71	924
0.06	0.12	0.22	0.20	0.09	0.36	0.13	0.30	0.39	0.47	0.47	0.36	0.58	0.11	0.56	0.59	0.64	0.64	0.57	0.71	0.07	0.70	673
0.11	0.12	0.20	0.17	0.08	0.33	0.13	0.27	0.38	0.46	0.45	0.35	0.56	0.11	0.54	0.59	0.63	0.63	0.56	0.70	0.07	0.69	542
0.15	0.09	0.17	0.14	0.05	0.28	0.11	0.22	0.36	0.43	0.42	0.32	0.53	0.10	0.50	0.57	0.61	0.62	0.55	0.68	0.07	0.67	389
0.18	0.07	0.15	0.12	0.04	0.26	0.11	0.21	0.35	0.41	0.41	0.31	0.52	0.11	0.49	0.56	0.61	0.61	0.54	0.67	0.07	0.65	307
0.32	0.05	0.12	0.10	0.02	0.23	0.11	0.17	0.30	0.37	0.37	0.26	0.49	0.11	0.45	0.54	0.58	0.59	0.51	0.66	0.07	0.63	470


==> data/mlm_plots/mlm_distil_fast/fakenews/bert/s/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.13
top50	0.19


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	33.87	46.59	41.43	25.15	68.02	21.44	53.46	74.00	89.59	89.00	53.27	125.92	36.33	103.00	36.97	50.14	44.93	27.79	72.48	22.35	56.93	74.00	89.38	89.00	53.46	125.31	35.92	103.00	841
0.03	34.67	48.99	42.67	22.93	75.04	26.06	54.49	72.00	86.34	89.50	51.88	120.80	34.46	101.00	41.36	57.58	50.37	27.97	87.19	29.61	64.60	71.00	85.30	87.50	51.43	119.16	33.86	101.00	468
0.06	34.00	51.55	41.88	12.74	90.37	38.81	55.62	68.00	84.64	87.00	47.00	122.29	37.64	102.00	48.90	68.58	59.86	30.10	107.05	38.47	75.33	67.00	82.44	85.00	45.72	119.16	36.72	99.00	994
0.11	34.92	56.14	42.88	-0.72	113.00	56.86	56.35	67.00	83.12	87.00	46.05	120.19	37.07	100.00	59.06	83.89	70.52	21.93	145.86	61.96	86.48	66.00	80.09	84.00	43.93	116.26	36.17	97.00	489
0.15	34.92	53.88	42.88	12.50	95.25	41.37	56.35	67.00	83.11	87.00	46.02	120.20	37.09	100.00	76.77	102.39	90.11	50.71	154.07	51.68	111.44	64.00	79.26	83.00	43.08	115.43	36.17	96.00	489
0.18	34.91	54.76	42.86	5.02	104.50	49.74	56.32	67.00	83.08	87.00	45.98	120.19	37.11	100.00	95.47	126.67	111.83	59.84	193.50	66.83	138.09	62.00	77.98	81.00	41.80	114.16	36.18	95.00	488
0.32	34.97	56.22	43.14	2.98	109.45	53.23	56.67	67.00	82.92	87.00	45.65	120.18	37.27	100.00	133.25	187.75	168.56	91.81	283.70	95.95	216.94	59.00	75.47	78.00	39.20	111.75	36.28	92.00	979


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	16.78
orig_ge	26.00
adv_pp	35.85
adv_ge	24.66


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.04	0.13	0.09	-0.15	0.40	0.27	0.29	0.70	0.76	0.78	0.66	0.86	0.10	0.83	0.60	0.69	0.70	0.57	0.82	0.12	0.79	841
0.03	-0.16	0.00	-0.02	-0.24	0.25	0.24	0.11	0.61	0.68	0.70	0.57	0.78	0.10	0.75	0.53	0.62	0.63	0.50	0.74	0.12	0.71	468
0.06	-0.24	-0.09	-0.12	-0.32	0.13	0.22	0.02	0.49	0.55	0.57	0.45	0.66	0.10	0.62	0.44	0.51	0.53	0.40	0.62	0.11	0.60	994
0.11	-0.29	-0.15	-0.18	-0.38	0.09	0.23	-0.05	0.38	0.44	0.45	0.34	0.54	0.10	0.51	0.36	0.42	0.43	0.32	0.52	0.10	0.49	489
0.15	-0.34	-0.19	-0.21	-0.42	0.04	0.23	-0.07	0.21	0.28	0.29	0.18	0.39	0.11	0.35	0.22	0.28	0.29	0.19	0.38	0.10	0.35	489
0.18	-0.37	-0.23	-0.25	-0.46	0.00	0.23	-0.10	0.07	0.15	0.15	0.04	0.26	0.11	0.21	0.11	0.17	0.18	0.08	0.26	0.09	0.23	488
0.32	-0.42	-0.27	-0.29	-0.50	-0.04	0.23	-0.13	-0.14	-0.04	-0.05	-0.18	0.09	0.14	0.05	-0.07	0.01	0.00	-0.10	0.12	0.11	0.09	979


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/correlations_auc.tex <==
name	auc
pcc	-0.05
spearman	0.09
kendall	0.09


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	13.63	20.44	18.73	10.42	30.47	10.02	26.63	7.00	18.12	15.97	5.40	30.83	12.72	26.29	4.48	13.56	9.94	2.37	24.76	11.20	20.71	841
0.03	9.71	13.88	12.93	6.63	21.13	7.25	17.15	4.98	11.49	8.58	2.51	20.46	8.97	15.70	3.10	10.46	6.04	-0.07	20.99	10.53	14.89	468
0.06	7.24	9.28	9.01	5.58	12.99	3.70	10.84	3.85	6.64	5.40	2.40	10.89	4.24	8.17	2.74	6.32	3.85	-0.31	12.94	6.62	7.19	994
0.11	6.19	7.59	7.59	4.90	10.28	2.69	9.11	3.25	5.04	4.40	2.31	7.78	2.73	5.98	2.53	5.13	3.26	-1.74	11.99	6.87	4.77	489
0.15	4.88	6.06	6.20	4.05	8.06	2.01	7.33	2.84	4.02	3.67	2.24	5.80	1.78	4.79	2.24	3.68	2.94	-0.14	7.51	3.83	3.83	489
0.18	4.36	5.28	5.29	3.67	6.89	1.61	6.28	2.65	3.55	3.35	2.20	4.91	1.36	4.19	2.11	2.95	2.58	1.22	4.68	1.73	3.28	488
0.32	3.59	4.40	4.37	3.10	5.70	1.30	5.17	2.44	3.08	2.95	2.07	4.09	1.01	3.57	1.93	2.59	2.31	0.99	4.19	1.60	2.87	979


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/ets_sts_auc.tex <==
name	auc
et_use	2.24
et_tse	1.62
et_ce	1.44


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	3.49	11.52	5.54	-14.27	37.30	25.79	9.17	8.42	13.17	11.86	5.87	20.48	7.31	16.75	6.74	12.26	10.17	3.11	21.42	9.15	14.85	841
0.03	1.92	3.77	2.73	-0.31	7.85	4.08	3.90	6.68	9.37	8.61	5.07	13.66	4.30	11.49	5.33	8.27	7.16	3.27	13.27	5.00	10.18	468
0.06	1.07	2.09	1.40	-3.29	7.47	5.38	1.91	5.43	7.18	6.73	3.90	10.46	3.28	8.13	4.27	6.47	5.55	-0.17	13.10	6.63	7.07	994
0.11	0.74	1.75	0.95	-7.10	10.60	8.85	1.24	4.84	6.24	5.76	2.99	9.48	3.25	7.00	3.87	5.73	4.82	-2.77	14.23	8.50	5.97	489
0.15	0.44	0.96	0.57	-2.27	4.18	3.23	0.73	3.99	5.17	4.84	2.63	7.71	2.54	5.76	3.24	4.83	4.01	-2.54	12.20	7.37	4.97	489
0.18	0.30	0.65	0.39	-2.10	3.41	2.75	0.51	3.66	4.67	4.38	2.37	6.97	2.30	5.13	2.97	4.29	3.64	-0.29	8.87	4.58	4.41	488
0.32	0.17	0.42	0.23	-1.38	2.22	1.80	0.33	3.22	4.00	3.77	2.21	5.79	1.79	4.36	2.65	3.60	3.16	0.21	7.00	3.40	3.77	979


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.49
et_p_h	1.80
et_p_l2	1.64


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.08	0.08	0.04	0.13	0.05	0.12	0.03	0.05	0.04	0.02	0.07	0.02	0.06	0.03	0.04	0.04	0.02	0.05	0.01	0.05	841
0.03	0.14	0.19	0.19	0.11	0.27	0.08	0.25	0.05	0.07	0.07	0.04	0.10	0.03	0.09	0.05	0.06	0.06	0.04	0.08	0.02	0.07	468
0.06	0.31	0.40	0.40	0.25	0.55	0.15	0.49	0.08	0.10	0.10	0.07	0.14	0.03	0.12	0.07	0.08	0.08	0.06	0.10	0.02	0.10	994
0.11	0.49	0.61	0.61	0.39	0.83	0.22	0.75	0.10	0.12	0.12	0.08	0.16	0.04	0.14	0.09	0.10	0.10	0.08	0.12	0.02	0.11	489
0.15	0.86	1.07	1.08	0.69	1.45	0.38	1.30	0.12	0.15	0.15	0.11	0.19	0.04	0.17	0.11	0.12	0.12	0.10	0.15	0.03	0.14	489
0.18	1.26	1.59	1.60	1.02	2.17	0.58	1.96	0.14	0.17	0.17	0.12	0.22	0.05	0.20	0.13	0.14	0.14	0.11	0.17	0.03	0.16	488
0.32	1.97	2.89	2.70	1.54	4.25	1.35	3.68	0.17	0.20	0.20	0.15	0.26	0.05	0.23	0.15	0.17	0.17	0.13	0.20	0.03	0.19	979


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.42
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.98	0.95	1.00	0.02	0.98	0.94	0.96	0.98	0.92	1.00	0.04	0.98	0.91	0.93	0.96	0.87	1.00	0.06	0.98	841
0.03	0.95	0.95	0.96	0.91	1.00	0.05	0.97	0.90	0.93	0.94	0.87	0.98	0.06	0.97	0.84	0.89	0.92	0.79	1.00	0.10	0.97	468
0.06	0.93	0.93	0.94	0.89	0.97	0.04	0.95	0.86	0.89	0.90	0.84	0.95	0.06	0.93	0.80	0.85	0.86	0.76	0.95	0.09	0.93	994
0.11	0.91	0.91	0.92	0.87	0.96	0.04	0.93	0.83	0.86	0.87	0.81	0.92	0.06	0.90	0.78	0.82	0.83	0.73	0.92	0.09	0.88	489
0.15	0.89	0.89	0.90	0.84	0.94	0.05	0.91	0.80	0.83	0.84	0.78	0.89	0.06	0.87	0.74	0.79	0.79	0.69	0.88	0.10	0.84	489
0.18	0.87	0.87	0.89	0.83	0.92	0.05	0.90	0.78	0.81	0.81	0.76	0.86	0.05	0.85	0.72	0.76	0.77	0.68	0.84	0.08	0.81	488
0.32	0.83	0.85	0.86	0.80	0.89	0.05	0.88	0.75	0.78	0.78	0.73	0.83	0.05	0.81	0.69	0.73	0.73	0.65	0.81	0.08	0.77	979


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	19.59	20.24	20.31	18.90	21.58	1.34	21.37	4.77	6.20	5.85	3.49	8.92	2.72	7.15	7.44	23.97	18.41	2.40	45.54	21.57	34.10	841
0.03	24.24	25.03	25.03	23.58	26.49	1.46	25.78	5.18	6.58	6.29	3.78	9.39	2.81	7.63	7.25	23.97	18.22	1.89	46.06	22.09	33.30	468
0.06	29.90	31.84	32.16	29.37	34.32	2.47	34.00	5.28	6.95	6.53	3.80	10.10	3.15	7.93	8.24	26.79	19.88	2.74	50.84	24.05	38.47	994
0.11	36.03	37.56	37.11	35.18	39.95	2.38	39.08	5.34	7.08	6.64	3.71	10.45	3.37	8.02	7.37	26.26	18.62	1.86	50.67	24.41	36.64	489
0.15	47.36	49.61	48.40	46.45	52.78	3.17	51.29	5.51	7.36	6.89	3.62	11.10	3.74	8.19	6.95	26.22	18.31	1.97	50.46	24.25	38.91	489
0.18	59.40	62.57	62.43	58.24	66.89	4.33	65.99	5.58	7.52	6.97	3.51	11.52	4.00	8.38	7.65	26.60	19.32	2.28	50.93	24.33	39.12	488
0.32	73.00	88.63	87.55	72.92	104.33	15.70	104.35	5.66	7.76	7.13	3.28	12.24	4.48	8.56	8.47	26.53	19.37	2.74	50.33	23.80	39.99	979


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/time_misc_auc.tex <==
name	auc
attack_time	17.01
l2	2.27
lom	8.14


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.69	0.74	0.75	0.66	0.82	0.08	0.80	0.77	0.83	0.83	0.75	0.90	0.07	0.89	0.80	0.86	0.86	0.79	0.93	0.07	0.91	841
0.03	0.60	0.65	0.67	0.57	0.74	0.08	0.71	0.74	0.79	0.80	0.72	0.87	0.07	0.85	0.79	0.83	0.84	0.76	0.90	0.07	0.89	468
0.06	0.47	0.53	0.53	0.44	0.62	0.09	0.59	0.69	0.73	0.74	0.67	0.80	0.07	0.79	0.75	0.80	0.81	0.73	0.86	0.07	0.85	994
0.11	0.37	0.42	0.42	0.31	0.54	0.11	0.49	0.64	0.68	0.69	0.62	0.75	0.06	0.73	0.72	0.76	0.77	0.70	0.82	0.06	0.81	489
0.15	0.24	0.30	0.31	0.19	0.41	0.11	0.38	0.55	0.60	0.61	0.54	0.67	0.06	0.65	0.67	0.71	0.71	0.65	0.77	0.06	0.76	489
0.18	0.16	0.23	0.22	0.13	0.33	0.10	0.29	0.49	0.53	0.53	0.47	0.59	0.06	0.57	0.62	0.66	0.67	0.61	0.72	0.06	0.71	488
0.32	0.11	0.18	0.18	0.09	0.28	0.09	0.23	0.36	0.42	0.41	0.34	0.50	0.08	0.48	0.54	0.59	0.58	0.52	0.65	0.06	0.63	979


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/ig/top_intersections_auc.tex <==
name	auc
top10	0.11
top30	0.18
top50	0.22


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	33.87	45.89	41.32	26.07	65.71	19.82	52.76	74.00	88.29	89.00	56.87	119.71	31.42	102.00	37.87	51.10	46.46	29.88	72.32	21.22	59.27	74.00	87.76	89.00	56.43	119.09	31.33	101.00	872
0.03	34.71	49.05	42.66	22.97	75.12	26.07	54.49	72.00	86.11	89.00	51.45	120.77	34.66	101.00	43.75	60.51	54.15	31.28	89.73	29.23	69.36	71.00	85.25	87.00	50.64	119.86	34.61	100.00	469
0.06	34.77	52.31	42.70	10.48	94.15	41.83	55.81	70.00	84.60	88.00	48.73	120.48	35.87	100.50	52.75	74.86	64.98	28.78	120.94	46.08	81.76	69.00	82.91	86.00	47.27	118.56	35.64	99.00	475
0.11	35.05	60.64	43.46	-12.05	133.34	72.69	57.45	67.00	82.18	87.00	44.22	120.13	37.96	100.00	63.50	98.34	76.36	-1.70	198.39	100.05	97.38	66.00	79.91	84.00	42.36	117.45	37.54	98.00	492
0.15	34.17	55.19	42.37	4.54	105.84	50.65	56.25	67.00	82.95	87.00	45.03	120.87	37.92	101.00	83.18	116.05	99.30	41.11	190.99	74.94	123.43	63.00	79.45	82.00	42.70	116.20	36.75	97.00	1004
0.18	34.13	55.54	42.52	-0.06	111.14	55.60	56.30	67.00	83.28	87.00	44.45	122.11	38.83	101.00	107.80	146.03	127.60	61.30	230.77	84.73	155.68	63.00	78.54	81.00	41.01	116.06	37.53	96.00	1005
0.32	34.18	58.29	42.62	-17.49	134.08	75.79	56.43	67.00	82.72	87.00	44.34	121.11	38.38	101.00	153.90	220.41	195.85	99.14	341.67	121.26	251.30	60.00	75.69	78.00	39.00	112.39	36.69	93.00	1992


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/comparison_vals_auc.tex <==
name	auc
orig_pp	17.26
orig_ge	25.93
adv_pp	41.22
adv_ge	24.72


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.60	0.70	0.74	0.55	0.86	0.15	0.82	0.86	0.90	0.92	0.84	0.96	0.06	0.95	0.71	0.80	0.81	0.69	0.90	0.10	0.89	872
0.03	0.44	0.57	0.60	0.39	0.75	0.18	0.71	0.77	0.83	0.84	0.75	0.91	0.08	0.89	0.62	0.71	0.72	0.60	0.81	0.11	0.79	469
0.06	0.32	0.46	0.48	0.28	0.65	0.18	0.61	0.66	0.72	0.73	0.62	0.82	0.10	0.80	0.53	0.60	0.61	0.50	0.70	0.10	0.67	475
0.11	0.25	0.39	0.39	0.20	0.57	0.18	0.53	0.55	0.62	0.63	0.50	0.74	0.12	0.70	0.43	0.50	0.51	0.39	0.61	0.11	0.58	492
0.15	0.15	0.28	0.28	0.11	0.46	0.17	0.41	0.40	0.47	0.48	0.34	0.61	0.13	0.56	0.31	0.37	0.38	0.27	0.47	0.10	0.44	1004
0.18	0.08	0.21	0.20	0.03	0.38	0.17	0.32	0.26	0.34	0.35	0.20	0.49	0.14	0.43	0.19	0.26	0.27	0.15	0.37	0.11	0.33	1005
0.32	-0.04	0.08	0.07	-0.10	0.27	0.19	0.20	0.01	0.13	0.14	-0.06	0.31	0.18	0.25	0.01	0.09	0.10	-0.04	0.23	0.13	0.18	1992


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/correlations_auc.tex <==
name	auc
pcc	0.09
spearman	0.14
kendall	0.11


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.20	6.40	5.20	1.94	10.86	4.46	8.36	2.24	5.96	4.64	1.01	10.90	4.94	8.05	1.37	4.72	2.99	-0.18	9.62	4.90	6.00	872
0.03	2.86	5.31	4.56	2.16	8.47	3.16	7.08	1.94	4.57	3.23	0.60	8.54	3.97	5.84	1.34	4.32	2.47	-0.62	9.25	4.94	5.10	469
0.06	2.82	4.44	4.15	2.19	6.69	2.25	5.74	1.76	3.18	2.66	1.12	5.25	2.06	4.01	1.35	3.19	2.06	-0.29	6.66	3.47	3.44	475
0.11	2.82	4.01	3.91	2.21	5.80	1.79	5.17	1.73	2.81	2.50	1.26	4.36	1.55	3.47	1.40	2.94	1.96	-0.45	6.32	3.39	3.18	492
0.15	2.88	3.76	3.78	2.41	5.11	1.35	4.66	1.82	2.62	2.43	1.47	3.77	1.15	3.20	1.48	2.47	1.89	-0.62	5.56	3.09	2.49	1004
0.18	2.81	3.54	3.60	2.42	4.66	1.12	4.32	1.87	2.50	2.35	1.59	3.41	0.91	2.97	1.46	2.10	1.81	0.60	3.61	1.50	2.31	1005
0.32	2.70	3.26	3.27	2.37	4.14	0.89	3.82	1.91	2.43	2.31	1.66	3.20	0.77	2.84	1.47	2.08	1.77	-0.16	4.32	2.24	2.14	1992


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/ets_sts_auc.tex <==
name	auc
et_use	1.22
et_tse	0.90
et_ce	0.83


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.72	2.00	1.13	-2.20	6.21	4.20	1.95	1.79	3.53	2.84	0.91	6.14	2.61	4.49	1.47	3.21	2.41	0.04	6.39	3.17	3.88	872
0.03	0.52	1.26	0.81	-2.19	4.71	3.45	1.24	2.02	3.32	3.00	1.52	5.11	1.79	4.23	1.68	2.90	2.46	1.09	4.71	1.81	3.56	469
0.06	0.37	0.83	0.53	-1.31	2.96	2.14	0.77	2.08	3.16	2.90	0.60	5.73	2.56	3.80	1.74	2.85	2.42	-1.95	7.66	4.80	3.22	475
0.11	0.30	0.75	0.41	-2.09	3.60	2.84	0.54	2.08	3.11	2.71	0.39	5.83	2.72	3.45	1.75	3.10	2.29	-3.77	9.98	6.87	2.94	492
0.15	0.21	0.54	0.27	-2.77	3.85	3.31	0.36	2.13	2.84	2.60	0.86	4.82	1.98	3.15	1.75	2.90	2.15	-7.13	12.93	10.03	2.67	1004
0.18	0.16	0.45	0.20	-2.47	3.37	2.92	0.26	2.11	2.73	2.52	1.18	4.28	1.55	3.00	1.72	2.50	2.12	-1.33	6.32	3.82	2.55	1005
0.32	0.10	0.30	0.13	-1.87	2.47	2.17	0.18	2.12	2.70	2.48	1.14	4.27	1.56	2.87	1.75	2.52	2.07	-0.99	6.02	3.50	2.45	1992


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.20
et_p_h	0.91
et_p_l2	0.85


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.12	0.12	0.07	0.17	0.05	0.15	0.04	0.06	0.05	0.03	0.08	0.02	0.07	0.04	0.05	0.05	0.03	0.06	0.02	0.06	872
0.03	0.20	0.26	0.26	0.17	0.34	0.09	0.31	0.07	0.08	0.08	0.05	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	469
0.06	0.40	0.49	0.50	0.34	0.65	0.16	0.59	0.09	0.11	0.11	0.08	0.15	0.04	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.10	475
0.11	0.61	0.74	0.74	0.50	0.98	0.24	0.89	0.11	0.13	0.13	0.09	0.17	0.04	0.16	0.10	0.11	0.11	0.09	0.14	0.03	0.12	492
0.15	1.08	1.31	1.32	0.89	1.72	0.42	1.57	0.14	0.17	0.16	0.12	0.21	0.05	0.19	0.12	0.14	0.14	0.11	0.16	0.03	0.15	1004
0.18	1.63	1.97	1.99	1.33	2.61	0.64	2.34	0.16	0.19	0.19	0.14	0.24	0.05	0.21	0.14	0.16	0.16	0.13	0.19	0.03	0.17	1005
0.32	2.51	3.58	3.36	1.96	5.19	1.62	4.55	0.19	0.22	0.22	0.16	0.27	0.06	0.25	0.16	0.18	0.18	0.15	0.22	0.04	0.20	1992


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.52
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.98	0.93	1.01	0.04	0.98	0.95	0.96	0.97	0.91	1.00	0.05	0.98	0.92	0.93	0.96	0.86	1.01	0.08	0.98	872
0.03	0.95	0.95	0.96	0.91	0.99	0.04	0.96	0.90	0.93	0.95	0.88	0.98	0.05	0.96	0.87	0.90	0.92	0.82	0.99	0.09	0.96	469
0.06	0.93	0.93	0.94	0.87	0.98	0.05	0.95	0.87	0.89	0.91	0.84	0.95	0.06	0.93	0.83	0.86	0.87	0.76	0.96	0.10	0.92	475
0.11	0.91	0.91	0.93	0.85	0.97	0.06	0.93	0.84	0.87	0.88	0.81	0.93	0.06	0.91	0.80	0.83	0.85	0.72	0.94	0.11	0.90	492
0.15	0.89	0.89	0.91	0.84	0.95	0.05	0.92	0.82	0.85	0.85	0.79	0.90	0.06	0.89	0.77	0.80	0.81	0.71	0.90	0.10	0.86	1004
0.18	0.87	0.88	0.89	0.83	0.93	0.05	0.90	0.80	0.83	0.84	0.78	0.88	0.05	0.86	0.75	0.78	0.79	0.69	0.87	0.09	0.82	1005
0.32	0.84	0.85	0.86	0.80	0.90	0.05	0.88	0.77	0.80	0.81	0.75	0.85	0.05	0.83	0.70	0.74	0.75	0.66	0.82	0.08	0.79	1992


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	12.70	13.21	13.42	12.33	14.10	0.89	13.75	32.76	54.49	42.14	14.47	94.50	40.02	58.82	6.92	19.13	14.04	1.69	36.57	17.44	26.15	872
0.03	16.89	17.64	17.17	16.34	18.94	1.30	19.02	39.64	70.33	52.11	17.65	123.02	52.69	76.12	7.46	23.76	18.46	2.28	45.24	21.48	34.04	469
0.06	20.13	20.99	20.86	19.31	22.67	1.68	22.74	46.91	82.73	61.88	21.13	144.34	61.61	95.53	8.66	26.94	19.88	2.21	51.67	24.73	38.35	475
0.11	23.02	24.68	24.09	21.85	27.51	2.83	25.23	52.08	88.20	66.77	23.40	153.01	64.80	105.35	8.17	28.16	21.43	3.16	53.15	25.00	40.45	492
0.15	30.55	32.47	33.19	29.51	35.44	2.97	34.21	59.72	99.36	79.88	28.16	170.57	71.21	114.45	9.68	31.10	24.11	4.68	57.52	26.42	45.42	1004
0.18	36.66	39.06	39.48	35.22	42.89	3.83	41.61	65.02	107.90	85.88	29.09	186.70	78.81	121.96	11.40	33.40	27.59	6.08	60.72	27.32	49.38	1005
0.32	49.86	57.60	55.42	47.44	67.75	10.15	65.36	72.46	119.94	96.57	31.12	208.77	88.82	133.20	13.42	37.33	32.65	8.83	65.84	28.50	55.24	1992


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/time_misc_auc.tex <==
name	auc
attack_time	10.99
l2	30.65
lom	9.68


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.60	0.67	0.69	0.56	0.79	0.11	0.76	0.80	0.85	0.86	0.77	0.92	0.08	0.91	0.86	0.91	0.92	0.85	0.96	0.06	0.96	872
0.03	0.44	0.53	0.55	0.39	0.67	0.14	0.62	0.72	0.78	0.79	0.70	0.86	0.08	0.84	0.83	0.87	0.88	0.81	0.93	0.06	0.91	469
0.06	0.33	0.42	0.43	0.27	0.56	0.15	0.51	0.64	0.69	0.70	0.61	0.77	0.08	0.75	0.79	0.82	0.83	0.77	0.88	0.06	0.86	475
0.11	0.24	0.35	0.36	0.19	0.50	0.16	0.44	0.56	0.61	0.62	0.52	0.70	0.09	0.67	0.74	0.77	0.78	0.72	0.83	0.06	0.81	492
0.15	0.18	0.26	0.26	0.12	0.41	0.14	0.36	0.46	0.51	0.52	0.42	0.60	0.09	0.56	0.67	0.71	0.71	0.65	0.76	0.06	0.74	1004
0.18	0.11	0.20	0.20	0.07	0.33	0.13	0.29	0.38	0.43	0.43	0.34	0.51	0.09	0.47	0.61	0.64	0.65	0.59	0.70	0.06	0.68	1005
0.32	0.04	0.14	0.12	0.02	0.26	0.12	0.20	0.25	0.31	0.31	0.21	0.42	0.10	0.38	0.50	0.55	0.55	0.48	0.62	0.07	0.60	1992


==> data/mlm_plots/mlm_distil_fast/fakenews/cnn/s/top_intersections_auc.tex <==
name	auc
top10	0.09
top30	0.16
top50	0.22


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	35.15	49.61	43.77	23.52	75.70	26.09	54.79	74.00	87.59	90.00	56.23	118.95	31.36	100.25	38.16	52.87	46.36	26.27	79.47	26.60	59.16	74.00	87.85	89.50	56.48	119.22	31.37	100.00	264
0.03	35.03	50.56	43.50	21.41	79.71	29.15	56.31	70.00	84.84	87.00	49.16	120.52	35.68	99.00	42.49	58.87	51.07	27.53	90.22	31.34	66.11	70.50	84.70	87.00	48.86	120.53	35.84	99.00	427
0.06	34.03	51.70	42.66	13.42	89.97	38.28	56.22	68.00	84.22	87.00	46.02	122.41	38.20	101.00	48.24	68.26	58.92	28.14	108.37	40.12	75.31	68.00	83.93	87.00	45.65	122.22	38.29	100.00	1006
0.11	35.05	57.00	43.51	-0.97	114.96	57.96	57.35	67.00	82.52	87.00	45.04	120.01	37.49	99.00	56.11	81.47	68.35	26.04	136.91	55.44	87.40	68.00	82.00	86.00	44.52	119.47	37.48	100.00	469
0.15	35.04	54.47	43.50	12.42	96.53	42.06	57.35	67.00	82.68	87.00	45.30	120.06	37.38	99.00	72.06	97.38	88.15	50.39	144.36	46.99	108.00	67.00	82.38	86.00	44.84	119.93	37.55	100.00	468
0.18	35.02	55.13	43.42	4.75	105.52	50.39	56.98	67.25	82.27	87.00	47.25	117.30	35.03	99.00	90.27	119.15	107.90	61.34	176.95	57.80	130.19	67.25	81.17	85.00	46.63	115.72	34.55	98.00	466
0.32	35.05	57.07	43.63	2.11	112.03	54.96	57.61	67.00	81.76	87.00	46.24	117.27	35.52	99.00	123.90	173.83	157.66	89.13	258.53	84.70	200.84	64.00	79.07	83.00	44.42	113.71	34.65	98.00	933


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	17.01
orig_ge	25.73
adv_pp	34.01
adv_ge	25.41


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.26	-0.07	-0.08	-0.34	0.21	0.28	0.08	0.61	0.69	0.70	0.57	0.81	0.12	0.79	0.49	0.61	0.59	0.46	0.75	0.14	0.73	264
0.03	-0.41	-0.23	-0.26	-0.50	0.03	0.27	-0.09	0.53	0.62	0.63	0.49	0.74	0.12	0.72	0.44	0.55	0.55	0.40	0.69	0.15	0.67	427
0.06	-0.49	-0.31	-0.35	-0.57	-0.06	0.26	-0.17	0.43	0.52	0.53	0.39	0.65	0.13	0.62	0.36	0.47	0.48	0.33	0.61	0.14	0.58	1006
0.11	-0.50	-0.32	-0.35	-0.58	-0.05	0.26	-0.18	0.34	0.44	0.44	0.31	0.56	0.13	0.54	0.30	0.40	0.39	0.27	0.53	0.13	0.50	469
0.15	-0.53	-0.33	-0.36	-0.60	-0.06	0.27	-0.17	0.23	0.31	0.31	0.19	0.43	0.12	0.40	0.22	0.29	0.29	0.18	0.40	0.11	0.37	468
0.18	-0.56	-0.37	-0.41	-0.63	-0.10	0.27	-0.21	0.13	0.21	0.21	0.08	0.33	0.12	0.29	0.13	0.20	0.20	0.10	0.30	0.10	0.27	466
0.32	-0.61	-0.41	-0.46	-0.67	-0.14	0.26	-0.23	-0.05	0.05	0.05	-0.10	0.19	0.15	0.15	-0.01	0.07	0.07	-0.04	0.19	0.11	0.15	933


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/correlations_auc.tex <==
name	auc
pcc	-0.10
spearman	0.10
kendall	0.09


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	19.23	28.55	25.89	15.59	41.51	12.96	36.88	9.67	24.85	24.67	8.97	40.74	15.88	35.17	6.41	18.71	15.25	4.83	32.59	13.88	27.64	264
0.03	14.08	22.50	18.79	9.76	35.24	12.74	28.44	5.62	18.99	15.78	3.58	34.39	15.41	27.82	4.02	14.37	11.42	2.27	26.48	12.11	21.42	427
0.06	9.55	13.26	11.85	6.15	20.36	7.10	14.92	4.09	10.10	6.35	1.25	18.95	8.85	13.72	3.15	8.55	5.07	0.63	16.47	7.92	11.53	1006
0.11	7.14	9.57	8.98	5.38	13.76	4.19	11.24	3.27	6.44	4.70	1.55	11.32	4.89	7.81	2.78	6.21	3.67	-0.08	12.50	6.29	7.34	469
0.15	5.22	6.84	6.79	4.37	9.31	2.47	8.47	2.74	4.14	3.59	1.86	6.42	2.28	4.83	2.31	3.96	2.99	0.45	7.47	3.51	4.25	468
0.18	4.65	5.89	5.86	4.03	7.76	1.86	7.10	2.64	3.60	3.24	1.96	5.24	1.64	4.13	2.23	3.39	2.78	0.09	6.70	3.30	3.51	466
0.32	3.81	4.87	4.82	3.39	6.35	1.48	5.86	2.49	3.17	3.03	2.06	4.29	1.11	3.66	2.09	2.83	2.55	1.07	4.60	1.76	3.11	933


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/ets_sts_auc.tex <==
name	auc
et_use	2.89
et_tse	2.09
et_ce	1.79


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	5.13	17.02	7.83	-23.54	57.59	40.57	14.46	10.06	15.75	14.37	7.27	24.23	8.48	19.76	7.85	13.86	11.82	5.12	22.59	8.74	16.94	264
0.03	2.50	5.22	3.58	-4.55	14.98	9.77	5.17	8.28	11.95	10.93	6.19	17.72	5.77	14.18	6.42	10.69	9.29	2.66	18.72	8.03	12.85	427
0.06	1.38	2.89	1.80	-8.75	14.54	11.65	2.43	6.48	8.60	8.03	4.78	12.42	3.82	9.99	5.03	7.55	6.52	2.60	12.50	4.95	8.55	1006
0.11	0.95	1.79	1.21	-1.27	4.86	3.06	1.64	5.58	7.16	6.68	4.21	10.10	2.94	8.03	4.39	6.63	5.58	-0.52	13.78	7.15	6.95	469
0.15	0.53	1.60	0.70	-6.90	10.10	8.50	0.94	4.46	5.78	5.34	2.79	8.78	2.99	6.55	3.63	5.31	4.42	-1.33	11.95	6.64	5.62	468
0.18	0.37	0.71	0.49	-0.36	1.77	1.07	0.65	4.03	5.08	4.83	3.13	7.04	1.95	5.77	3.27	4.47	4.00	1.39	7.55	3.08	4.96	466
0.32	0.20	0.53	0.29	-1.39	2.44	1.91	0.41	3.46	4.43	4.14	2.43	6.44	2.01	4.94	2.85	4.05	3.48	-0.32	8.42	4.37	4.20	933


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.66
et_p_h	2.07
et_p_l2	1.86


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.04	0.07	0.07	0.03	0.12	0.05	0.10	0.03	0.05	0.05	0.03	0.07	0.02	0.06	0.03	0.04	0.04	0.02	0.06	0.02	0.05	264
0.03	0.13	0.18	0.18	0.10	0.27	0.08	0.24	0.05	0.07	0.07	0.04	0.11	0.03	0.09	0.04	0.06	0.06	0.04	0.08	0.02	0.07	427
0.06	0.28	0.37	0.37	0.23	0.52	0.15	0.46	0.08	0.10	0.10	0.07	0.14	0.04	0.13	0.07	0.08	0.08	0.06	0.11	0.02	0.10	1006
0.11	0.41	0.55	0.56	0.32	0.79	0.23	0.70	0.10	0.12	0.12	0.08	0.16	0.04	0.14	0.08	0.10	0.10	0.07	0.13	0.03	0.11	469
0.15	0.72	0.96	0.96	0.56	1.35	0.40	1.20	0.12	0.15	0.15	0.10	0.20	0.05	0.18	0.11	0.12	0.12	0.10	0.15	0.03	0.14	468
0.18	1.09	1.43	1.43	0.85	2.01	0.58	1.76	0.14	0.17	0.17	0.12	0.22	0.05	0.20	0.13	0.14	0.14	0.11	0.17	0.03	0.16	466
0.32	1.72	2.59	2.40	1.32	3.86	1.27	3.27	0.17	0.20	0.20	0.15	0.26	0.06	0.23	0.15	0.17	0.17	0.13	0.20	0.04	0.19	933


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.38
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.98	0.98	0.97	0.99	0.01	0.99	0.95	0.96	0.98	0.92	1.00	0.04	0.99	0.93	0.94	0.97	0.89	1.00	0.06	0.98	264
0.03	0.96	0.96	0.97	0.94	0.99	0.03	0.98	0.89	0.93	0.96	0.87	0.99	0.06	0.98	0.85	0.91	0.95	0.82	0.99	0.09	0.97	427
0.06	0.93	0.94	0.94	0.91	0.97	0.03	0.95	0.84	0.89	0.90	0.82	0.96	0.07	0.95	0.79	0.86	0.87	0.76	0.96	0.10	0.94	1006
0.11	0.91	0.92	0.93	0.88	0.96	0.04	0.94	0.80	0.85	0.86	0.78	0.93	0.07	0.92	0.76	0.82	0.82	0.72	0.93	0.10	0.91	469
0.15	0.88	0.89	0.90	0.84	0.94	0.05	0.92	0.76	0.81	0.81	0.74	0.88	0.07	0.86	0.72	0.78	0.78	0.67	0.88	0.10	0.84	468
0.18	0.87	0.87	0.89	0.83	0.92	0.05	0.90	0.74	0.79	0.79	0.72	0.85	0.06	0.83	0.71	0.75	0.76	0.66	0.84	0.09	0.80	466
0.32	0.83	0.84	0.86	0.80	0.89	0.05	0.88	0.73	0.76	0.76	0.70	0.82	0.06	0.80	0.68	0.72	0.73	0.63	0.81	0.09	0.77	933


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	16.08	16.74	16.78	15.79	17.68	0.94	17.22	3.41	5.21	4.55	2.55	7.86	2.66	5.96	6.19	20.74	14.14	1.64	39.83	19.10	31.13	264
0.03	17.69	18.74	18.69	17.52	19.95	1.22	19.76	3.89	6.01	5.50	3.08	8.93	2.93	7.48	5.97	22.79	18.26	1.31	44.27	21.48	34.09	427
0.06	21.78	22.64	22.68	20.77	24.50	1.86	23.87	4.12	6.53	5.62	2.34	10.73	4.19	7.95	7.07	24.98	18.98	2.86	47.11	22.12	37.31	1006
0.11	28.40	29.97	30.12	27.05	32.90	2.92	31.32	4.17	6.77	5.79	0.65	12.90	6.12	8.09	7.80	26.03	19.45	2.95	49.10	23.07	37.47	469
0.15	52.16	55.73	53.25	48.38	63.08	7.35	57.96	4.28	8.19	5.90	-9.06	25.43	17.24	8.28	7.62	28.59	22.80	3.98	53.21	24.61	42.43	468
0.18	46.61	50.61	52.20	46.33	54.90	4.29	52.96	4.39	11.05	6.15	-39.98	62.08	51.03	8.65	8.76	31.47	25.51	4.28	58.65	27.18	44.67	466
0.32	59.07	72.68	67.37	57.83	87.53	14.85	85.08	4.48	12.92	6.18	-45.24	71.08	58.16	9.13	10.51	35.41	27.80	3.94	66.88	31.47	50.45	933


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/time_misc_auc.tex <==
name	auc
attack_time	14.28
l2	2.89
lom	9.10


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.60	0.67	0.67	0.58	0.76	0.09	0.73	0.69	0.76	0.77	0.66	0.86	0.10	0.85	0.76	0.82	0.81	0.73	0.90	0.08	0.89	264
0.03	0.53	0.59	0.60	0.49	0.69	0.10	0.65	0.65	0.73	0.74	0.63	0.83	0.10	0.81	0.73	0.80	0.80	0.71	0.88	0.08	0.87	427
0.06	0.42	0.48	0.49	0.38	0.58	0.10	0.56	0.61	0.68	0.69	0.59	0.78	0.10	0.77	0.70	0.77	0.77	0.68	0.85	0.08	0.83	1006
0.11	0.33	0.40	0.40	0.27	0.52	0.12	0.47	0.57	0.64	0.65	0.55	0.73	0.09	0.71	0.68	0.74	0.74	0.66	0.82	0.08	0.80	469
0.15	0.24	0.30	0.30	0.18	0.42	0.12	0.38	0.52	0.57	0.58	0.49	0.65	0.08	0.63	0.65	0.69	0.70	0.62	0.76	0.07	0.75	468
0.18	0.16	0.24	0.24	0.13	0.36	0.11	0.31	0.46	0.51	0.52	0.44	0.59	0.08	0.57	0.62	0.66	0.66	0.59	0.72	0.06	0.70	466
0.32	0.11	0.20	0.18	0.09	0.31	0.11	0.27	0.36	0.42	0.42	0.33	0.51	0.09	0.48	0.55	0.59	0.59	0.53	0.66	0.06	0.64	933


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/ig/top_intersections_auc.tex <==
name	auc
top10	0.10
top30	0.18
top50	0.21


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	34.85	47.88	42.76	26.59	69.17	21.29	55.94	73.00	87.91	87.00	51.41	124.41	36.50	101.00	39.02	52.97	47.63	30.62	75.31	22.35	61.23	72.00	87.49	87.00	51.07	123.90	36.41	100.00	767
0.03	34.25	49.41	42.67	22.03	76.79	27.38	55.82	70.00	85.49	87.00	47.89	123.10	37.61	102.00	42.98	60.15	52.98	30.88	89.43	29.28	68.69	69.00	84.79	86.00	47.30	122.28	37.49	101.00	967
0.06	34.18	53.06	42.75	10.43	95.69	42.63	56.39	67.00	83.63	87.00	44.99	122.28	38.65	100.00	51.28	74.26	62.99	22.23	126.28	52.02	80.87	66.00	82.74	86.00	44.19	121.30	38.56	100.00	1009
0.11	34.19	54.00	42.77	6.33	101.67	47.67	56.54	67.00	83.38	87.00	44.52	122.24	38.86	100.75	60.08	87.00	73.47	13.62	160.38	73.38	94.68	67.00	82.60	86.00	43.82	121.39	38.79	100.00	1018
0.15	35.04	55.30	43.50	9.83	100.76	45.47	57.42	67.00	82.43	87.00	44.88	119.98	37.55	99.00	79.43	110.72	96.89	49.62	171.81	61.10	118.86	68.00	82.16	86.00	44.49	119.82	37.67	100.00	468
0.18	35.06	55.25	43.50	4.86	105.64	50.39	57.27	67.25	82.80	87.00	45.57	120.03	37.23	99.00	100.56	138.68	121.93	42.96	234.40	95.72	146.57	68.00	82.02	85.50	44.74	119.30	37.28	99.00	466
0.32	35.08	57.48	43.63	1.30	113.65	56.17	57.73	67.00	82.20	87.00	45.74	118.66	36.46	99.00	139.22	207.54	180.92	75.73	339.36	131.81	236.94	65.00	80.44	83.00	43.77	117.11	36.67	99.00	931


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/comparison_vals_auc.tex <==
name	auc
orig_pp	16.95
orig_ge	25.83
adv_pp	38.99
adv_ge	25.55


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.25	0.37	0.36	0.21	0.53	0.16	0.48	0.77	0.83	0.84	0.73	0.93	0.10	0.91	0.62	0.71	0.71	0.58	0.84	0.13	0.81	767
0.03	0.18	0.29	0.26	0.14	0.43	0.15	0.38	0.72	0.78	0.80	0.67	0.90	0.11	0.86	0.57	0.66	0.66	0.53	0.79	0.13	0.75	967
0.06	0.12	0.21	0.19	0.08	0.34	0.13	0.28	0.64	0.72	0.73	0.59	0.85	0.13	0.81	0.50	0.59	0.59	0.45	0.72	0.13	0.68	1009
0.11	0.08	0.17	0.14	0.05	0.29	0.12	0.22	0.59	0.66	0.67	0.52	0.79	0.13	0.75	0.45	0.53	0.54	0.40	0.66	0.13	0.62	1018
0.15	0.04	0.11	0.09	0.01	0.22	0.11	0.16	0.48	0.55	0.57	0.42	0.69	0.14	0.65	0.36	0.43	0.44	0.31	0.55	0.12	0.51	468
0.18	0.01	0.07	0.04	-0.04	0.17	0.10	0.11	0.37	0.46	0.47	0.32	0.60	0.14	0.55	0.27	0.35	0.36	0.23	0.47	0.12	0.43	466
0.32	-0.06	0.00	-0.01	-0.10	0.11	0.11	0.05	0.17	0.28	0.28	0.11	0.45	0.17	0.40	0.12	0.21	0.21	0.08	0.34	0.13	0.30	931


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.17
kendall	0.13


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	10.11	14.88	13.49	8.00	21.76	6.88	18.46	6.32	13.56	12.12	4.87	22.25	8.69	18.84	3.76	9.41	7.87	2.51	16.31	6.90	13.44	767
0.03	7.77	11.08	9.77	5.50	16.66	5.58	12.87	3.99	9.69	7.59	2.32	17.05	7.36	13.25	2.59	7.12	5.03	1.26	12.97	5.86	9.98	967
0.06	5.90	7.84	7.34	4.15	11.54	3.70	8.94	2.91	6.05	4.22	1.19	10.91	4.86	7.81	2.09	4.84	2.97	0.24	9.44	4.60	5.65	1009
0.11	5.13	6.42	6.22	4.02	8.81	2.40	7.36	2.52	4.63	3.65	1.55	7.71	3.08	5.83	1.92	3.92	2.56	-0.00	7.83	3.92	4.09	1018
0.15	4.10	4.97	5.02	3.46	6.48	1.51	5.84	2.21	3.42	2.90	1.58	5.25	1.84	3.93	1.84	3.04	2.22	0.07	6.00	2.96	2.96	468
0.18	3.65	4.34	4.35	3.15	5.52	1.19	5.04	2.11	2.97	2.65	1.56	4.38	1.41	3.37	1.69	2.47	2.11	0.92	4.02	1.55	2.65	466
0.32	3.08	3.62	3.59	2.73	4.50	0.89	4.11	2.00	2.61	2.41	1.63	3.59	0.98	2.93	1.62	2.17	1.95	1.08	3.25	1.08	2.36	931


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/ets_sts_auc.tex <==
name	auc
et_use	1.83
et_tse	1.38
et_ce	1.11


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.02	4.07	2.83	-2.38	10.53	6.46	4.16	5.22	8.06	7.27	3.70	12.43	4.37	9.95	4.10	7.23	6.14	2.60	11.87	4.63	9.07	767
0.03	1.20	1.90	1.51	-0.24	4.05	2.14	2.01	4.33	5.90	5.59	3.47	8.32	2.42	7.04	3.44	5.13	4.64	2.35	7.91	2.78	6.12	967
0.06	0.71	1.10	0.88	-0.69	2.90	1.79	1.10	3.76	4.71	4.52	2.97	6.45	1.74	5.37	2.98	4.06	3.74	2.06	6.07	2.00	4.67	1009
0.11	0.49	1.03	0.60	-4.97	7.02	5.99	0.75	3.37	4.18	4.01	2.26	6.11	1.92	4.62	2.66	3.89	3.35	-4.55	12.34	8.45	4.05	1018
0.15	0.31	0.51	0.38	-0.43	1.44	0.93	0.48	3.00	3.56	3.46	2.48	4.63	1.08	3.91	2.42	3.16	2.88	0.91	5.40	2.24	3.48	468
0.18	0.22	0.38	0.27	-0.54	1.31	0.93	0.33	2.76	3.24	3.16	2.31	4.17	0.93	3.54	2.25	2.85	2.65	0.86	4.84	1.99	3.15	466
0.32	0.12	0.27	0.17	-0.99	1.52	1.25	0.23	2.53	2.97	2.84	2.08	3.87	0.90	3.23	2.09	2.67	2.42	0.72	4.62	1.95	2.83	931


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.25
et_p_h	1.21
et_p_l2	1.08


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.11	0.11	0.06	0.16	0.05	0.15	0.04	0.06	0.05	0.03	0.08	0.03	0.07	0.03	0.05	0.04	0.03	0.06	0.02	0.06	767
0.03	0.18	0.24	0.24	0.15	0.33	0.09	0.29	0.06	0.08	0.08	0.05	0.12	0.03	0.10	0.05	0.07	0.06	0.05	0.09	0.02	0.08	967
0.06	0.37	0.46	0.46	0.30	0.61	0.16	0.55	0.09	0.11	0.11	0.07	0.15	0.04	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.10	1009
0.11	0.56	0.70	0.70	0.46	0.94	0.24	0.85	0.10	0.13	0.13	0.09	0.17	0.04	0.15	0.09	0.11	0.11	0.08	0.13	0.03	0.12	1018
0.15	0.94	1.18	1.17	0.77	1.60	0.41	1.43	0.13	0.16	0.15	0.11	0.21	0.05	0.18	0.11	0.13	0.13	0.10	0.16	0.03	0.15	468
0.18	1.38	1.76	1.73	1.11	2.40	0.65	2.07	0.15	0.18	0.17	0.13	0.23	0.05	0.20	0.13	0.15	0.15	0.12	0.18	0.03	0.17	466
0.32	2.14	3.17	2.86	1.64	4.70	1.53	4.04	0.18	0.21	0.21	0.15	0.26	0.06	0.24	0.16	0.18	0.18	0.14	0.21	0.04	0.20	931


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.47
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.98	0.95	1.00	0.02	0.98	0.95	0.96	0.98	0.92	1.00	0.04	0.98	0.92	0.94	0.96	0.87	1.00	0.06	0.98	767
0.03	0.96	0.96	0.96	0.93	0.99	0.03	0.97	0.91	0.94	0.96	0.89	0.99	0.05	0.97	0.86	0.91	0.93	0.82	0.99	0.08	0.97	967
0.06	0.94	0.94	0.95	0.91	0.97	0.03	0.95	0.87	0.90	0.91	0.84	0.96	0.06	0.95	0.81	0.86	0.87	0.77	0.95	0.09	0.93	1009
0.11	0.92	0.93	0.93	0.89	0.96	0.04	0.94	0.84	0.88	0.88	0.82	0.94	0.06	0.93	0.78	0.83	0.83	0.75	0.92	0.09	0.90	1018
0.15	0.90	0.90	0.91	0.86	0.94	0.04	0.92	0.81	0.84	0.85	0.78	0.91	0.06	0.88	0.76	0.80	0.80	0.71	0.89	0.09	0.85	468
0.18	0.88	0.88	0.89	0.84	0.92	0.04	0.91	0.78	0.82	0.82	0.76	0.88	0.06	0.86	0.73	0.77	0.78	0.69	0.86	0.08	0.83	466
0.32	0.84	0.85	0.86	0.81	0.90	0.04	0.88	0.75	0.79	0.79	0.73	0.85	0.06	0.83	0.69	0.74	0.74	0.66	0.82	0.08	0.79	931


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	12.50	13.26	13.33	12.26	14.26	1.00	13.85	44.15	105.35	74.86	17.37	193.33	87.98	141.76	14.40	40.07	31.58	8.43	71.70	31.63	58.66	767
0.03	15.30	15.89	16.14	14.65	17.13	1.24	16.67	50.10	119.37	87.64	21.84	216.89	97.53	161.84	14.28	42.08	35.35	9.05	75.10	33.02	61.87	967
0.06	20.25	21.30	21.43	19.45	23.15	1.85	22.47	56.57	126.39	96.85	28.87	223.90	97.52	169.71	13.82	42.26	36.18	8.38	76.14	33.88	62.24	1009
0.11	26.15	26.98	27.17	24.73	29.22	2.24	28.58	62.13	132.39	107.59	37.00	227.78	95.39	174.62	11.99	41.95	33.79	6.98	76.93	34.97	64.07	1018
0.15	31.06	32.33	32.39	29.87	34.79	2.46	33.77	71.72	152.09	123.06	14.81	289.38	137.29	196.18	12.03	41.20	31.60	6.52	75.87	34.68	63.05	468
0.18	40.94	42.19	42.82	39.15	45.24	3.05	43.95	76.09	158.53	120.12	-28.38	345.44	186.91	201.61	13.52	39.28	30.23	6.40	72.16	32.88	59.14	466
0.32	50.54	59.37	55.52	49.11	69.62	10.25	70.94	73.40	166.49	123.62	-1.94	334.91	168.42	203.10	13.58	38.58	31.51	7.51	69.64	31.07	57.36	931


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/time_misc_auc.tex <==
name	auc
attack_time	11.44
l2	45.59
lom	12.54


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.46	0.55	0.56	0.41	0.70	0.14	0.65	0.71	0.78	0.79	0.68	0.88	0.10	0.85	0.82	0.87	0.87	0.80	0.93	0.07	0.92	767
0.03	0.36	0.47	0.47	0.32	0.62	0.15	0.58	0.67	0.74	0.74	0.64	0.84	0.10	0.81	0.80	0.85	0.85	0.78	0.91	0.07	0.90	967
0.06	0.29	0.37	0.38	0.23	0.52	0.14	0.47	0.61	0.68	0.69	0.58	0.78	0.10	0.75	0.76	0.81	0.82	0.74	0.89	0.07	0.86	1009
0.11	0.22	0.31	0.31	0.18	0.45	0.13	0.40	0.57	0.64	0.65	0.54	0.74	0.10	0.70	0.74	0.79	0.79	0.72	0.86	0.07	0.83	1018
0.15	0.13	0.22	0.22	0.10	0.35	0.13	0.31	0.50	0.56	0.56	0.46	0.65	0.10	0.62	0.70	0.74	0.75	0.67	0.81	0.07	0.79	468
0.18	0.08	0.16	0.14	0.05	0.27	0.11	0.23	0.43	0.49	0.50	0.40	0.58	0.09	0.55	0.66	0.70	0.70	0.64	0.77	0.07	0.75	466
0.32	0.02	0.09	0.07	-0.00	0.19	0.09	0.13	0.31	0.38	0.37	0.28	0.48	0.10	0.44	0.57	0.62	0.62	0.55	0.70	0.07	0.67	931


==> data/mlm_plots/mlm_distil_fast/fakenews/lstm/s/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.17
top50	0.23


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	35.02	48.18	42.70	25.48	70.89	22.70	55.06	72.25	88.02	88.00	51.16	124.88	36.86	101.00	37.74	51.62	46.03	28.00	75.24	23.62	58.67	73.00	88.03	88.00	51.09	124.98	36.95	101.00	670
0.03	34.19	48.94	41.93	21.01	76.87	27.93	54.90	72.00	86.44	89.00	50.94	121.94	35.50	102.00	40.99	56.64	49.93	26.82	86.46	29.82	62.88	71.25	86.25	88.00	50.69	121.81	35.56	101.00	946
0.06	34.18	52.31	42.15	10.22	94.39	42.08	55.89	69.25	84.61	88.00	47.88	121.34	36.73	102.00	47.91	67.36	57.91	24.93	109.78	42.43	72.70	69.00	84.50	88.00	47.75	121.25	36.75	102.00	1022
0.11	34.18	53.48	42.07	1.09	105.87	52.39	55.97	69.50	84.49	88.00	47.28	121.70	37.21	102.00	54.59	76.26	65.40	25.10	127.41	51.16	81.83	70.00	84.55	88.00	47.21	121.89	37.34	102.00	999
0.15	34.18	52.61	41.99	10.18	95.03	42.42	55.95	69.00	84.03	88.00	47.78	120.27	36.24	102.00	65.94	90.94	79.90	38.08	143.81	52.87	99.87	71.00	85.63	89.00	48.92	122.35	36.71	104.00	997
0.18	34.20	54.32	42.47	1.55	107.10	52.77	56.23	69.00	84.06	87.00	46.46	121.66	37.60	102.00	81.26	110.23	97.40	47.32	173.14	62.91	119.03	70.00	86.25	90.00	48.02	124.48	38.23	106.00	1002
0.32	34.19	56.75	42.52	-16.98	130.48	73.73	56.30	68.00	83.86	87.00	46.07	121.65	37.79	102.00	105.59	151.44	133.15	60.67	242.21	90.77	167.53	69.00	87.81	92.00	48.55	127.06	39.26	108.75	2010


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/comparison_vals_auc.tex <==
name	auc
orig_pp	16.65
orig_ge	26.23
adv_pp	31.15
adv_ge	26.74


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.03	0.14	0.09	-0.01	0.30	0.15	0.21	0.92	0.92	0.95	0.83	1.01	0.09	0.97	0.80	0.84	0.89	0.71	0.97	0.13	0.93	670
0.03	-0.00	0.05	0.01	-0.05	0.15	0.10	0.07	0.85	0.88	0.91	0.76	0.99	0.11	0.94	0.71	0.77	0.82	0.63	0.91	0.14	0.87	946
0.06	-0.01	0.02	-0.00	-0.05	0.10	0.08	0.02	0.81	0.84	0.87	0.74	0.95	0.10	0.91	0.67	0.72	0.76	0.60	0.85	0.12	0.81	1022
0.11	-0.02	0.01	-0.01	-0.07	0.09	0.08	0.01	0.76	0.81	0.83	0.70	0.91	0.11	0.87	0.62	0.68	0.71	0.56	0.80	0.12	0.76	999
0.15	-0.02	-0.00	-0.01	-0.08	0.08	0.08	0.00	0.70	0.75	0.77	0.65	0.86	0.10	0.82	0.56	0.62	0.64	0.51	0.73	0.11	0.69	997
0.18	-0.03	-0.01	-0.02	-0.08	0.05	0.07	-0.01	0.65	0.70	0.71	0.59	0.80	0.11	0.77	0.52	0.57	0.58	0.47	0.66	0.10	0.63	1002
0.32	-0.04	-0.03	-0.03	-0.09	0.04	0.07	-0.01	0.52	0.60	0.61	0.47	0.72	0.13	0.68	0.40	0.47	0.47	0.36	0.57	0.10	0.54	2010


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/correlations_auc.tex <==
name	auc
pcc	0.00
spearman	0.23
kendall	0.19


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	14.75	21.38	19.21	11.87	30.88	9.50	27.15	8.71	19.14	18.30	7.12	31.16	12.02	27.12	5.76	14.49	13.31	4.58	24.39	9.91	20.66	670
0.03	10.27	14.94	12.80	7.30	22.57	7.64	17.19	3.73	12.08	9.86	2.28	21.88	9.80	17.63	3.31	10.12	8.30	2.03	18.20	8.09	14.56	946
0.06	7.33	9.67	8.70	4.80	14.55	4.88	10.48	2.84	6.97	4.43	1.02	12.92	5.95	9.68	2.58	6.62	4.00	0.51	12.74	6.11	8.99	1022
0.11	5.74	7.14	6.89	4.33	9.96	2.82	8.06	2.47	4.66	3.28	1.08	8.23	3.57	5.59	2.27	4.60	3.02	0.29	8.91	4.31	5.55	999
0.15	4.56	5.46	5.44	3.73	7.19	1.73	6.23	2.19	3.43	2.75	1.36	5.50	2.07	3.91	2.06	3.38	2.54	0.42	6.33	2.95	3.55	997
0.18	3.87	4.55	4.55	3.27	5.82	1.28	5.24	2.07	2.89	2.52	1.45	4.33	1.44	3.22	1.89	2.83	2.30	0.01	5.64	2.81	2.89	1002
0.32	3.04	3.62	3.56	2.67	4.56	0.94	4.13	1.93	2.47	2.28	1.56	3.38	0.91	2.74	1.73	2.29	2.05	0.37	4.21	1.92	2.44	2010


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/ets_sts_auc.tex <==
name	auc
et_use	2.13
et_tse	1.52
et_ce	1.39


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	4.00	10.92	5.81	-7.41	29.25	18.33	9.24	8.45	12.71	11.39	6.72	18.69	5.98	15.35	6.71	11.29	9.68	4.81	17.77	6.48	13.92	670
0.03	2.09	3.99	2.77	-1.37	9.35	5.36	3.95	6.66	9.01	8.30	5.40	12.62	3.61	10.58	5.29	7.97	6.85	3.14	12.80	4.83	9.46	946
0.06	1.11	2.61	1.44	-8.85	14.07	11.46	1.97	5.07	6.44	5.96	3.93	8.94	2.51	7.25	3.97	5.70	4.96	1.76	9.65	3.94	6.27	1022
0.11	0.74	1.47	0.95	-1.89	4.83	3.36	1.31	4.37	5.37	5.00	3.13	7.62	2.25	5.80	3.45	4.84	4.12	0.12	9.57	4.73	5.03	999
0.15	0.45	1.05	0.59	-4.96	7.06	6.01	0.80	3.61	4.38	4.03	2.24	6.53	2.15	4.62	2.92	3.93	3.35	-0.12	7.98	4.05	4.03	997
0.18	0.31	0.74	0.41	-2.33	3.81	3.07	0.56	3.22	3.87	3.57	1.68	6.05	2.19	4.02	2.64	3.66	2.97	-3.36	10.68	7.02	3.50	1002
0.32	0.19	0.42	0.26	-0.63	1.46	1.05	0.37	2.74	3.32	3.05	1.43	5.20	1.89	3.43	2.24	3.11	2.56	-2.57	8.79	5.68	2.96	2010


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.51
et_p_h	1.57
et_p_l2	1.43


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.08	0.07	0.03	0.12	0.04	0.11	0.03	0.05	0.04	0.03	0.07	0.02	0.06	0.03	0.04	0.04	0.02	0.05	0.02	0.05	670
0.03	0.12	0.17	0.17	0.10	0.25	0.08	0.23	0.05	0.07	0.07	0.04	0.10	0.03	0.09	0.05	0.06	0.06	0.04	0.08	0.02	0.07	946
0.06	0.25	0.35	0.34	0.20	0.49	0.14	0.44	0.08	0.10	0.10	0.07	0.14	0.03	0.12	0.07	0.08	0.08	0.06	0.10	0.02	0.10	1022
0.11	0.38	0.53	0.52	0.31	0.74	0.22	0.67	0.10	0.12	0.12	0.08	0.16	0.04	0.14	0.09	0.10	0.10	0.08	0.12	0.02	0.11	999
0.15	0.63	0.87	0.84	0.50	1.23	0.36	1.10	0.13	0.15	0.15	0.11	0.19	0.04	0.17	0.11	0.12	0.12	0.10	0.15	0.03	0.14	997
0.18	0.91	1.26	1.23	0.73	1.79	0.53	1.59	0.14	0.17	0.17	0.13	0.21	0.04	0.19	0.13	0.14	0.14	0.11	0.17	0.03	0.16	1002
0.32	1.38	2.14	1.95	1.03	3.25	1.11	2.72	0.17	0.20	0.20	0.15	0.25	0.05	0.23	0.15	0.17	0.17	0.13	0.20	0.03	0.19	2010


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.33
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.98	0.98	0.95	1.00	0.02	0.98	0.96	0.96	0.98	0.91	1.01	0.05	0.98	0.93	0.94	0.97	0.88	1.01	0.06	0.98	670
0.03	0.95	0.96	0.96	0.92	0.99	0.03	0.97	0.87	0.92	0.95	0.85	0.99	0.07	0.97	0.86	0.91	0.94	0.82	0.99	0.09	0.97	946
0.06	0.93	0.94	0.94	0.90	0.98	0.04	0.95	0.83	0.88	0.89	0.81	0.96	0.07	0.95	0.81	0.87	0.88	0.78	0.96	0.09	0.95	1022
0.11	0.91	0.92	0.93	0.87	0.97	0.05	0.94	0.80	0.85	0.85	0.78	0.92	0.07	0.91	0.78	0.83	0.84	0.73	0.93	0.10	0.91	999
0.15	0.89	0.90	0.91	0.85	0.94	0.05	0.92	0.77	0.82	0.82	0.75	0.89	0.07	0.87	0.76	0.80	0.81	0.71	0.90	0.09	0.86	997
0.18	0.87	0.88	0.89	0.83	0.93	0.05	0.90	0.76	0.80	0.80	0.74	0.86	0.06	0.84	0.73	0.77	0.78	0.68	0.87	0.09	0.82	1002
0.32	0.83	0.85	0.86	0.80	0.89	0.04	0.88	0.73	0.77	0.78	0.72	0.83	0.06	0.81	0.70	0.74	0.75	0.67	0.82	0.08	0.79	2010


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	12.89	13.33	13.51	12.42	14.23	0.90	14.02	0.41	0.57	0.52	0.35	0.79	0.22	0.70	21.33	68.18	49.24	8.18	128.18	60.00	102.64	670
0.03	14.93	15.43	15.55	14.43	16.42	1.00	16.13	0.50	0.66	0.62	0.45	0.88	0.21	0.82	18.95	67.43	51.54	7.87	127.00	59.56	99.70	946
0.06	19.27	20.17	20.29	18.79	21.54	1.38	21.31	0.50	0.65	0.59	0.45	0.85	0.20	0.79	15.90	67.35	47.32	3.18	131.51	64.16	98.93	1022
0.11	22.75	23.46	23.41	21.99	24.92	1.47	24.17	0.48	0.62	0.56	0.42	0.82	0.20	0.75	16.94	70.67	46.80	2.75	138.59	67.92	103.58	999
0.15	29.02	30.17	30.33	28.04	32.31	2.14	32.01	0.43	0.58	0.52	0.39	0.78	0.20	0.72	19.98	81.13	58.20	6.89	155.37	74.24	127.01	997
0.18	36.23	38.66	38.58	34.58	42.73	4.08	40.27	0.41	0.56	0.49	0.36	0.75	0.20	0.70	18.80	84.03	58.27	6.14	161.92	77.89	131.24	1002
0.32	44.91	52.81	53.25	44.03	61.59	8.78	60.24	0.38	0.54	0.47	0.34	0.73	0.20	0.67	20.16	88.03	58.63	7.33	168.73	80.70	145.13	2010


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/time_misc_auc.tex <==
name	auc
attack_time	10.40
l2	0.18
lom	24.44


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.75	0.79	0.82	0.66	0.92	0.13	0.87	0.87	0.89	0.92	0.80	0.98	0.09	0.95	0.90	0.92	0.95	0.85	0.99	0.07	0.97	670
0.03	0.64	0.71	0.73	0.58	0.84	0.13	0.80	0.80	0.85	0.88	0.75	0.94	0.09	0.91	0.86	0.89	0.92	0.81	0.97	0.08	0.95	946
0.06	0.56	0.62	0.64	0.48	0.75	0.13	0.70	0.78	0.82	0.84	0.73	0.90	0.08	0.88	0.84	0.87	0.89	0.80	0.94	0.07	0.92	1022
0.11	0.46	0.53	0.56	0.39	0.66	0.14	0.62	0.74	0.78	0.80	0.71	0.86	0.08	0.84	0.83	0.86	0.87	0.79	0.92	0.07	0.90	999
0.15	0.29	0.37	0.38	0.23	0.52	0.14	0.47	0.70	0.73	0.74	0.66	0.81	0.07	0.78	0.81	0.83	0.85	0.77	0.90	0.06	0.88	997
0.18	0.16	0.26	0.25	0.12	0.40	0.14	0.36	0.64	0.68	0.69	0.61	0.75	0.07	0.73	0.78	0.81	0.82	0.76	0.87	0.06	0.85	1002
0.32	0.04	0.15	0.12	0.02	0.27	0.12	0.22	0.52	0.58	0.59	0.48	0.67	0.09	0.64	0.72	0.76	0.77	0.70	0.82	0.06	0.80	2010


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/a/top_intersections_auc.tex <==
name	auc
top10	0.12
top30	0.22
top50	0.26


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	34.69	47.51	41.93	25.75	69.26	21.75	54.52	74.00	87.93	89.00	55.59	120.28	32.35	102.00	37.44	51.13	45.86	28.19	74.07	22.94	58.74	74.00	88.30	90.00	55.83	120.78	32.47	102.00	694
0.03	34.29	48.61	41.93	22.10	75.11	26.51	54.74	72.00	85.87	88.00	50.85	120.89	35.02	102.00	41.08	56.50	49.59	26.97	86.04	29.53	63.21	72.00	85.97	88.50	50.88	121.06	35.09	102.00	944
0.06	34.12	52.21	41.93	10.18	94.24	42.03	55.78	69.75	84.69	88.00	47.96	121.42	36.73	102.00	47.31	68.46	57.69	20.80	116.12	47.66	73.06	70.75	85.04	89.00	48.09	121.98	36.94	102.00	1024
0.11	34.19	53.80	42.22	1.09	106.51	52.71	56.16	70.00	84.50	88.00	47.24	121.76	37.26	102.00	54.91	78.08	66.37	26.16	129.99	51.92	82.86	71.00	85.47	89.00	47.81	123.13	37.66	103.00	1009
0.15	34.19	52.77	42.47	10.21	95.33	42.56	55.96	69.75	84.44	88.00	47.18	121.70	37.26	102.00	66.48	93.10	81.35	37.55	148.64	55.55	101.14	72.00	86.67	90.50	48.65	124.69	38.02	104.00	1004
0.18	34.23	55.29	42.47	-15.33	125.91	70.62	56.10	69.00	84.05	87.00	46.45	121.65	37.60	101.75	81.11	113.23	98.80	37.47	188.99	75.76	120.62	72.00	85.95	90.00	47.51	124.38	38.43	104.00	986
0.32	34.29	57.35	42.65	-20.30	135.00	77.65	56.27	67.50	82.72	87.00	46.74	118.71	35.98	101.00	107.06	156.38	135.53	57.68	255.07	98.70	173.27	68.00	84.45	89.00	47.22	121.68	37.23	104.00	1715


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	16.77
orig_ge	26.15
adv_pp	31.94
adv_ge	26.58


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.11	0.09	0.08	-0.21	0.38	0.29	0.28	0.42	0.53	0.54	0.36	0.70	0.17	0.66	0.35	0.45	0.44	0.29	0.61	0.16	0.56	694
0.03	-0.30	-0.11	-0.14	-0.39	0.17	0.28	0.08	0.35	0.46	0.46	0.29	0.63	0.17	0.59	0.29	0.39	0.38	0.24	0.55	0.16	0.50	944
0.06	-0.39	-0.21	-0.22	-0.49	0.07	0.28	-0.03	0.30	0.40	0.41	0.23	0.58	0.18	0.53	0.25	0.35	0.35	0.19	0.51	0.16	0.47	1024
0.11	-0.44	-0.22	-0.23	-0.53	0.08	0.30	-0.02	0.25	0.35	0.37	0.18	0.52	0.17	0.47	0.21	0.31	0.32	0.16	0.46	0.15	0.42	1009
0.15	-0.48	-0.25	-0.26	-0.57	0.07	0.32	-0.02	0.18	0.27	0.29	0.12	0.43	0.16	0.38	0.17	0.25	0.26	0.11	0.38	0.14	0.34	1004
0.18	-0.52	-0.29	-0.30	-0.61	0.02	0.31	-0.07	0.13	0.22	0.23	0.07	0.37	0.15	0.32	0.13	0.21	0.22	0.08	0.33	0.13	0.29	986
0.32	-0.55	-0.33	-0.33	-0.64	-0.01	0.31	-0.10	0.05	0.14	0.15	-0.01	0.30	0.15	0.25	0.07	0.14	0.15	0.02	0.27	0.12	0.23	1715


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/correlations_auc.tex <==
name	auc
pcc	-0.08
spearman	0.09
kendall	0.08


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	14.26	23.20	20.90	11.21	35.19	11.99	30.38	6.09	19.69	18.63	5.50	33.88	14.19	29.58	4.28	16.29	13.63	3.22	29.37	13.07	24.70	694
0.03	11.17	18.28	15.24	7.23	29.33	11.05	21.63	4.23	14.65	10.74	1.53	27.76	13.12	21.11	3.42	12.35	8.49	1.42	23.28	10.93	18.87	944
0.06	8.24	12.13	10.74	5.38	18.88	6.75	14.29	3.23	8.64	5.15	0.27	17.00	8.37	11.56	2.77	7.72	4.27	-0.04	15.49	7.76	10.67	1024
0.11	6.23	8.84	8.16	4.38	13.30	4.46	10.72	2.68	5.59	3.84	0.62	10.56	4.97	6.47	2.40	5.47	3.35	-0.57	11.51	6.04	5.83	1009
0.15	4.98	6.66	6.42	3.92	9.39	2.73	8.08	2.39	4.01	3.23	1.18	6.84	2.83	4.53	2.20	3.92	2.95	0.17	7.68	3.76	4.15	1004
0.18	4.38	5.62	5.47	3.57	7.68	2.05	6.74	2.31	3.42	3.01	1.50	5.35	1.92	3.93	2.11	3.31	2.71	0.24	6.38	3.07	3.55	986
0.32	3.52	4.55	4.44	2.93	6.17	1.62	5.42	2.24	3.07	2.81	1.60	4.54	1.47	3.55	1.95	2.79	2.48	0.86	4.71	1.93	3.11	1715


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/ets_sts_auc.tex <==
name	auc
et_use	2.60
et_tse	1.81
et_ce	1.64


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	3.65	13.22	5.86	-17.85	44.29	31.07	9.99	9.07	14.34	12.65	6.38	22.31	7.97	17.81	7.33	12.82	11.10	4.48	21.16	8.34	15.98	694
0.03	2.22	5.09	3.25	-4.27	14.45	9.36	4.99	7.48	11.03	9.91	5.81	16.25	5.22	13.37	5.95	9.67	8.18	3.65	15.69	6.02	11.70	944
0.06	1.26	2.46	1.71	-1.49	6.42	3.95	2.48	5.99	8.34	7.60	4.17	12.51	4.17	9.62	4.71	7.40	6.19	1.19	13.60	6.20	8.49	1024
0.11	0.83	1.59	1.15	-1.07	4.25	2.66	1.59	4.92	6.85	6.19	3.31	10.38	3.53	7.94	3.90	6.42	5.06	-3.80	16.63	10.22	6.77	1009
0.15	0.51	1.31	0.72	-5.15	7.77	6.46	1.03	4.01	5.60	5.00	2.04	9.16	3.56	6.31	3.23	5.24	4.12	-2.97	13.45	8.21	5.37	1004
0.18	0.37	0.89	0.52	-3.42	5.20	4.31	0.73	3.69	4.97	4.56	2.53	7.41	2.44	5.67	3.00	4.53	3.81	-0.21	9.27	4.74	4.81	986
0.32	0.22	0.59	0.32	-2.84	4.01	3.43	0.47	3.24	4.39	3.99	1.32	7.47	3.08	4.93	2.66	4.13	3.33	-2.65	10.90	6.78	4.22	1715


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.60
et_p_h	1.99
et_p_l2	1.81


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.08	0.08	0.03	0.13	0.05	0.11	0.03	0.05	0.04	0.02	0.07	0.02	0.06	0.03	0.04	0.04	0.02	0.05	0.01	0.05	694
0.03	0.12	0.18	0.17	0.10	0.25	0.08	0.23	0.05	0.07	0.07	0.04	0.10	0.03	0.09	0.04	0.06	0.06	0.04	0.07	0.02	0.07	944
0.06	0.26	0.35	0.35	0.22	0.49	0.14	0.45	0.07	0.10	0.10	0.06	0.13	0.04	0.12	0.07	0.08	0.08	0.06	0.10	0.02	0.09	1024
0.11	0.41	0.55	0.54	0.34	0.75	0.21	0.67	0.10	0.12	0.12	0.08	0.16	0.04	0.14	0.08	0.10	0.10	0.07	0.12	0.02	0.11	1009
0.15	0.65	0.89	0.88	0.54	1.23	0.35	1.11	0.12	0.15	0.15	0.10	0.19	0.04	0.17	0.11	0.12	0.12	0.10	0.15	0.03	0.14	1004
0.18	0.96	1.29	1.27	0.79	1.79	0.50	1.60	0.14	0.17	0.17	0.12	0.22	0.05	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.15	986
0.32	1.46	2.20	2.04	1.13	3.28	1.08	2.78	0.17	0.20	0.19	0.14	0.25	0.05	0.22	0.15	0.16	0.16	0.13	0.20	0.03	0.18	1715


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.34
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.98	0.98	0.95	1.00	0.03	0.98	0.93	0.95	0.98	0.90	1.00	0.05	0.98	0.90	0.94	0.97	0.86	1.01	0.07	0.98	694
0.03	0.95	0.96	0.96	0.93	0.99	0.03	0.97	0.87	0.92	0.95	0.85	0.99	0.07	0.97	0.84	0.90	0.94	0.81	0.99	0.09	0.97	944
0.06	0.93	0.94	0.94	0.89	0.98	0.04	0.95	0.82	0.88	0.88	0.80	0.95	0.08	0.95	0.79	0.85	0.86	0.75	0.96	0.10	0.94	1024
0.11	0.91	0.92	0.93	0.86	0.97	0.05	0.94	0.79	0.84	0.84	0.77	0.92	0.08	0.90	0.76	0.82	0.82	0.71	0.93	0.11	0.89	1009
0.15	0.89	0.89	0.91	0.84	0.95	0.05	0.92	0.76	0.81	0.81	0.74	0.88	0.07	0.85	0.75	0.79	0.79	0.69	0.89	0.10	0.84	1004
0.18	0.87	0.87	0.89	0.82	0.93	0.05	0.90	0.75	0.79	0.78	0.72	0.85	0.06	0.83	0.72	0.76	0.76	0.66	0.86	0.10	0.81	986
0.32	0.83	0.84	0.85	0.79	0.90	0.05	0.87	0.73	0.77	0.77	0.71	0.83	0.06	0.81	0.69	0.73	0.74	0.64	0.82	0.09	0.78	1715


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	18.07	19.30	19.22	16.35	22.24	2.94	20.11	2.17	12.33	3.13	-24.65	49.31	36.98	4.88	18.51	57.94	43.92	5.22	110.65	52.72	80.43	694
0.03	25.19	37.50	27.29	20.54	54.46	16.96	48.67	2.65	14.83	3.49	-34.82	64.48	49.65	5.05	16.22	55.29	40.51	3.93	106.65	51.36	80.13	944
0.06	29.45	31.47	30.99	27.22	35.72	4.25	32.93	2.81	14.64	3.57	-33.31	62.58	47.95	5.23	15.12	54.54	39.46	3.52	105.55	51.01	78.44	1024
0.11	32.24	35.29	33.57	30.37	40.21	4.92	37.61	2.88	18.91	3.64	-104.87	142.69	123.78	5.24	15.64	55.57	36.90	0.51	110.64	55.07	78.22	1009
0.15	41.93	43.71	43.18	39.12	48.30	4.59	45.79	2.78	25.38	3.63	-298.20	348.97	323.59	5.27	18.38	62.86	45.60	4.02	121.69	58.83	89.28	1004
0.18	55.70	60.52	60.55	53.19	67.85	7.33	65.75	2.79	35.42	3.62	-451.75	522.59	487.17	5.29	19.87	66.75	49.30	5.56	127.95	61.20	97.39	986
0.32	65.60	77.53	75.60	63.39	91.67	14.14	88.74	2.76	20.12	3.62	-260.11	300.34	280.23	5.08	21.19	68.63	50.71	6.47	130.79	62.16	97.15	1715


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/time_misc_auc.tex <==
name	auc
attack_time	16.04
l2	7.28
lom	19.36


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.44	0.54	0.53	0.40	0.67	0.13	0.62	0.58	0.65	0.65	0.54	0.77	0.11	0.74	0.69	0.74	0.75	0.66	0.83	0.09	0.80	694
0.03	0.40	0.48	0.49	0.35	0.61	0.13	0.58	0.55	0.62	0.62	0.51	0.74	0.11	0.71	0.67	0.72	0.72	0.63	0.81	0.09	0.79	944
0.06	0.35	0.42	0.42	0.29	0.56	0.13	0.51	0.53	0.60	0.61	0.48	0.72	0.12	0.68	0.65	0.71	0.72	0.62	0.80	0.09	0.78	1024
0.11	0.31	0.37	0.38	0.24	0.50	0.13	0.44	0.51	0.57	0.58	0.46	0.69	0.11	0.66	0.64	0.69	0.70	0.60	0.78	0.09	0.76	1009
0.15	0.24	0.31	0.31	0.19	0.42	0.12	0.38	0.47	0.53	0.55	0.43	0.64	0.11	0.61	0.62	0.67	0.68	0.58	0.75	0.09	0.73	1004
0.18	0.20	0.27	0.27	0.16	0.38	0.11	0.33	0.44	0.50	0.52	0.40	0.61	0.10	0.58	0.60	0.65	0.66	0.57	0.73	0.08	0.71	986
0.32	0.16	0.23	0.22	0.12	0.33	0.11	0.29	0.39	0.46	0.47	0.35	0.56	0.10	0.53	0.57	0.62	0.63	0.54	0.70	0.08	0.68	1715


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/ig/top_intersections_auc.tex <==
name	auc
top10	0.10
top30	0.17
top50	0.21


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	34.30	46.93	41.86	25.95	67.92	20.98	54.00	74.00	88.72	89.00	54.04	123.40	34.68	102.00	37.22	50.80	45.85	28.82	72.77	21.97	58.30	74.00	88.57	89.00	53.95	123.20	34.63	101.00	720
0.03	34.20	48.50	41.88	22.37	74.63	26.13	54.64	72.00	86.53	89.00	51.00	122.06	35.53	102.00	41.22	57.24	50.52	28.72	85.75	28.51	64.51	71.00	86.19	89.00	50.72	121.67	35.48	101.75	950
0.06	34.20	52.24	42.22	10.60	93.89	41.64	55.89	70.00	84.68	88.00	47.97	121.38	36.70	102.00	48.50	69.16	58.34	22.74	115.57	46.41	75.14	69.50	84.51	88.00	47.71	121.32	36.80	101.00	1019
0.11	34.18	52.05	41.96	8.14	95.96	43.91	55.74	70.00	84.86	88.00	47.93	121.79	36.93	102.00	55.06	77.01	66.91	29.51	124.51	47.50	84.22	70.00	85.14	89.00	48.07	122.21	37.07	102.00	993
0.15	34.69	53.26	42.88	12.93	93.58	40.33	56.30	69.00	83.69	88.00	47.46	119.93	36.24	101.00	68.92	95.06	82.67	42.85	147.27	52.21	103.47	72.00	85.66	92.00	48.93	122.39	36.73	104.00	521
0.18	34.69	53.52	42.84	8.48	98.56	45.04	56.14	69.00	83.81	88.00	47.75	119.87	36.06	101.00	84.22	114.19	101.20	53.58	174.80	60.61	125.97	70.00	85.84	92.00	49.14	122.54	36.70	105.00	521
0.32	34.33	55.47	42.76	-0.43	111.36	55.90	56.34	68.00	83.54	87.00	46.80	120.28	36.74	101.00	110.34	156.13	137.67	72.68	239.58	83.45	178.71	69.00	85.86	91.00	47.83	123.88	38.02	105.00	1525


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/comparison_vals_auc.tex <==
name	auc
orig_pp	16.43
orig_ge	26.20
adv_pp	32.07
adv_ge	26.60


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.25	0.37	0.37	0.21	0.52	0.16	0.47	0.62	0.71	0.74	0.54	0.88	0.17	0.84	0.48	0.57	0.58	0.42	0.72	0.15	0.69	720
0.03	0.15	0.26	0.25	0.12	0.41	0.14	0.35	0.52	0.65	0.67	0.45	0.84	0.20	0.80	0.40	0.51	0.52	0.34	0.68	0.17	0.63	950
0.06	0.09	0.20	0.17	0.05	0.35	0.15	0.30	0.43	0.58	0.60	0.37	0.80	0.22	0.76	0.33	0.46	0.46	0.28	0.63	0.18	0.59	1019
0.11	0.05	0.17	0.13	0.01	0.32	0.15	0.25	0.40	0.55	0.57	0.32	0.78	0.23	0.74	0.30	0.42	0.43	0.24	0.61	0.18	0.56	993
0.15	0.00	0.11	0.06	-0.05	0.26	0.15	0.16	0.32	0.48	0.50	0.25	0.72	0.24	0.67	0.24	0.37	0.37	0.19	0.55	0.18	0.50	521
0.18	-0.03	0.07	0.02	-0.08	0.22	0.15	0.11	0.26	0.42	0.43	0.18	0.67	0.25	0.61	0.19	0.31	0.32	0.13	0.50	0.18	0.44	521
0.32	-0.08	0.01	-0.02	-0.14	0.16	0.15	0.05	0.12	0.32	0.33	0.05	0.58	0.26	0.51	0.10	0.23	0.24	0.05	0.42	0.19	0.37	1525


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.15
kendall	0.11


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	10.00	14.95	13.15	7.83	22.06	7.12	18.50	3.51	12.05	10.64	2.69	21.40	9.36	18.60	2.76	8.69	6.59	1.57	15.82	7.12	12.88	720
0.03	7.71	11.54	9.70	5.45	17.62	6.08	13.49	2.61	9.13	6.58	1.09	17.18	8.05	13.33	2.30	7.03	4.68	1.06	13.00	5.97	10.43	950
0.06	5.55	7.78	7.03	3.66	11.91	4.13	8.86	2.23	5.74	3.46	0.41	11.07	5.33	7.68	2.02	5.03	2.89	-0.06	10.12	5.09	6.49	1019
0.11	4.61	6.08	5.88	3.57	8.59	2.51	7.04	2.03	3.95	2.71	0.69	7.22	3.26	4.60	1.89	3.63	2.48	0.25	7.01	3.38	3.92	993
0.15	3.85	4.82	4.78	3.25	6.40	1.57	5.81	1.95	3.00	2.49	1.28	4.72	1.72	3.40	1.79	2.85	2.32	0.85	4.85	2.00	3.00	521
0.18	3.22	4.11	4.10	2.81	5.42	1.30	4.84	1.91	2.59	2.32	1.35	3.83	1.24	2.90	1.66	2.35	2.11	1.10	3.61	1.25	2.59	521
0.32	2.89	3.55	3.52	2.56	4.54	0.99	4.17	1.89	2.44	2.30	1.50	3.39	0.95	2.75	1.67	2.17	2.00	1.15	3.20	1.02	2.42	1525


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/ets_sts_auc.tex <==
name	auc
et_use	1.79
et_tse	1.25
et_ce	1.08


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.54	7.94	3.62	-10.92	26.80	18.86	5.81	5.80	8.90	7.95	4.39	13.41	4.51	11.02	4.56	7.89	6.52	3.04	12.73	4.84	9.96	720
0.03	1.42	3.14	1.93	-5.57	11.85	8.71	2.77	4.72	6.70	6.13	3.69	9.71	3.01	7.89	3.71	6.03	5.13	0.94	11.12	5.09	7.06	950
0.06	0.83	1.69	1.07	-3.60	6.99	5.29	1.48	3.93	5.21	4.87	2.90	7.51	2.30	5.85	3.15	4.62	4.02	1.53	7.71	3.09	5.11	1019
0.11	0.58	1.13	0.76	-3.85	6.11	4.98	1.01	3.49	4.39	4.20	2.79	5.98	1.60	5.05	2.76	3.82	3.48	1.65	5.99	2.17	4.37	993
0.15	0.38	1.13	0.50	-7.09	9.36	8.22	0.67	3.06	3.79	3.69	2.30	5.27	1.49	4.29	2.50	3.31	3.11	1.31	5.32	2.00	3.77	521
0.18	0.27	0.53	0.35	-0.60	1.65	1.13	0.47	2.88	3.44	3.38	2.25	4.64	1.20	3.86	2.32	3.04	2.84	1.13	4.95	1.91	3.36	521
0.32	0.17	0.54	0.23	-4.60	5.69	5.15	0.33	2.63	3.20	3.02	1.53	4.86	1.67	3.42	2.15	3.07	2.54	-4.41	10.54	7.47	2.95	1525


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.40
et_p_h	1.31
et_p_l2	1.18


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.09	0.09	0.04	0.13	0.05	0.12	0.03	0.05	0.05	0.03	0.08	0.02	0.07	0.03	0.04	0.04	0.03	0.06	0.02	0.05	720
0.03	0.14	0.19	0.19	0.11	0.28	0.08	0.25	0.05	0.08	0.07	0.04	0.11	0.03	0.09	0.05	0.06	0.06	0.04	0.08	0.02	0.07	950
0.06	0.28	0.37	0.37	0.23	0.51	0.14	0.46	0.08	0.10	0.10	0.07	0.14	0.04	0.12	0.07	0.08	0.08	0.06	0.11	0.02	0.10	1019
0.11	0.43	0.56	0.56	0.35	0.77	0.21	0.69	0.10	0.12	0.12	0.09	0.16	0.04	0.14	0.09	0.10	0.10	0.08	0.12	0.02	0.11	993
0.15	0.70	0.92	0.90	0.55	1.28	0.36	1.12	0.12	0.15	0.15	0.11	0.19	0.04	0.17	0.11	0.12	0.12	0.10	0.15	0.03	0.14	521
0.18	1.01	1.34	1.32	0.81	1.87	0.53	1.65	0.14	0.17	0.17	0.12	0.22	0.05	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.16	521
0.32	1.53	2.25	2.09	1.15	3.35	1.10	2.82	0.17	0.20	0.20	0.15	0.25	0.05	0.22	0.15	0.17	0.17	0.13	0.20	0.03	0.18	1525


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.35
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.98	0.95	1.00	0.02	0.98	0.91	0.94	0.97	0.89	1.00	0.06	0.98	0.89	0.93	0.96	0.85	1.00	0.07	0.98	720
0.03	0.95	0.96	0.96	0.93	0.99	0.03	0.97	0.86	0.91	0.95	0.84	0.99	0.07	0.97	0.84	0.90	0.92	0.81	0.98	0.09	0.97	950
0.06	0.93	0.94	0.94	0.89	0.98	0.05	0.95	0.83	0.88	0.88	0.80	0.96	0.08	0.95	0.81	0.86	0.86	0.75	0.96	0.10	0.94	1019
0.11	0.92	0.92	0.93	0.88	0.96	0.04	0.94	0.80	0.85	0.85	0.78	0.92	0.07	0.91	0.78	0.83	0.83	0.74	0.92	0.09	0.89	993
0.15	0.89	0.90	0.91	0.85	0.94	0.04	0.92	0.78	0.82	0.82	0.75	0.89	0.07	0.87	0.76	0.80	0.81	0.71	0.89	0.09	0.85	521
0.18	0.87	0.88	0.89	0.83	0.92	0.04	0.90	0.76	0.80	0.80	0.74	0.86	0.06	0.84	0.73	0.77	0.78	0.69	0.85	0.08	0.82	521
0.32	0.83	0.85	0.86	0.81	0.90	0.05	0.88	0.75	0.78	0.78	0.72	0.84	0.06	0.82	0.71	0.75	0.76	0.67	0.83	0.08	0.79	1525


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	15.21	15.62	15.73	14.72	16.52	0.90	16.31	36.04	293.79	55.81	-477.25	1064.83	771.04	129.13	22.72	61.24	50.27	11.65	110.82	49.58	89.98	720
0.03	17.42	18.39	18.35	17.07	19.70	1.32	19.40	43.11	313.87	64.20	-847.10	1474.85	1160.97	117.38	22.32	67.36	52.51	11.26	123.46	56.10	98.94	950
0.06	23.37	24.47	24.52	22.58	26.36	1.89	25.39	46.40	420.62	69.73	-3037.20	3878.43	3457.81	115.03	23.90	71.11	55.89	11.25	130.96	59.86	105.13	1019
0.11	26.49	28.58	28.28	25.87	31.29	2.71	29.76	49.60	516.20	73.17	-5452.63	6485.02	5968.83	123.30	22.48	74.93	60.77	12.39	137.48	62.55	112.29	993
0.15	32.94	35.04	34.98	32.20	37.87	2.83	37.25	50.52	229.99	71.19	-540.72	1000.70	770.71	122.53	30.19	85.16	67.23	15.43	154.89	69.73	127.62	521
0.18	41.27	44.01	43.10	39.69	48.34	4.32	46.15	49.48	333.40	74.37	-1608.08	2274.87	1941.47	121.38	30.67	88.37	71.85	18.06	158.69	70.31	129.42	521
0.32	57.51	66.31	64.19	55.44	77.18	10.87	73.29	46.21	483.61	69.23	-5272.33	6239.56	5755.94	113.62	30.88	89.95	73.73	19.23	160.67	70.72	136.77	1525


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/time_misc_auc.tex <==
name	auc
attack_time	12.45
l2	120.12
lom	25.36


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.38	0.49	0.49	0.32	0.67	0.17	0.60	0.60	0.67	0.68	0.55	0.80	0.13	0.77	0.73	0.78	0.79	0.69	0.87	0.09	0.85	720
0.03	0.29	0.42	0.41	0.23	0.62	0.19	0.56	0.54	0.63	0.64	0.49	0.77	0.14	0.73	0.69	0.76	0.76	0.66	0.85	0.10	0.83	950
0.06	0.20	0.36	0.33	0.16	0.55	0.19	0.49	0.49	0.59	0.58	0.45	0.73	0.14	0.69	0.66	0.73	0.73	0.63	0.83	0.10	0.80	1019
0.11	0.16	0.31	0.29	0.12	0.50	0.19	0.44	0.46	0.57	0.56	0.42	0.71	0.14	0.67	0.64	0.72	0.72	0.61	0.82	0.10	0.79	993
0.15	0.09	0.22	0.19	0.05	0.40	0.17	0.33	0.42	0.51	0.50	0.38	0.65	0.14	0.61	0.62	0.69	0.69	0.59	0.80	0.10	0.77	521
0.18	0.06	0.18	0.13	0.02	0.34	0.16	0.25	0.37	0.47	0.46	0.33	0.60	0.13	0.56	0.60	0.67	0.67	0.56	0.77	0.10	0.74	521
0.32	0.02	0.12	0.07	-0.02	0.27	0.15	0.17	0.30	0.40	0.39	0.26	0.53	0.14	0.48	0.55	0.63	0.63	0.52	0.73	0.11	0.70	1525


==> data/mlm_plots/mlm_distil_fast/fakenews/lstmatt/s/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.16
top50	0.21


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	31.90	44.48	39.39	20.91	68.05	23.57	50.58	30.00	38.62	37.00	23.23	54.02	15.39	46.25	35.31	47.73	42.57	23.05	72.41	24.68	54.11	30.00	39.15	38.00	23.71	54.58	15.43	47.00	336
0.03	31.78	44.38	39.09	20.29	68.47	24.09	50.11	29.00	37.86	37.00	22.08	53.65	15.79	46.00	38.31	51.74	46.05	25.60	77.87	26.13	58.56	30.00	38.53	38.00	22.82	54.24	15.71	46.00	511
0.06	31.69	46.85	39.28	14.05	79.65	32.80	51.04	28.00	37.35	37.00	20.69	54.01	16.66	46.00	43.65	61.40	53.39	27.41	95.39	33.99	68.61	30.00	38.77	38.00	22.01	55.53	16.76	47.00	568
0.11	31.55	48.25	39.10	6.32	90.19	41.94	50.60	29.00	37.39	37.00	20.60	54.19	16.80	46.00	50.97	74.01	61.31	10.13	137.89	63.88	78.52	31.00	39.88	40.00	22.79	56.97	17.09	48.00	566
0.15	31.88	49.49	39.46	8.21	90.78	41.29	51.96	27.00	36.47	36.00	19.38	53.55	17.09	45.00	66.99	93.73	80.16	27.82	159.65	65.91	99.65	31.00	40.77	40.00	22.98	58.56	17.79	50.00	590
0.18	31.69	49.98	39.28	1.33	98.63	48.65	51.90	28.00	36.90	37.00	19.85	53.95	17.05	46.00	82.30	112.38	97.67	30.77	193.99	81.61	117.88	33.00	42.48	42.00	24.32	60.65	18.17	52.00	576
0.32	31.45	50.72	39.03	-9.06	110.51	59.79	50.14	29.00	37.56	37.00	20.32	54.80	17.24	46.00	110.03	153.82	137.14	67.93	239.70	85.88	174.73	35.00	45.30	45.00	26.45	64.16	18.85	56.00	1032


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/comparison_vals_auc.tex <==
name	auc
orig_pp	15.16
orig_ge	11.57
adv_pp	31.11
adv_ge	12.92


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.28	0.44	0.44	0.24	0.63	0.19	0.59	0.96	0.95	0.98	0.81	1.10	0.14	0.99	0.84	0.86	0.89	0.72	1.00	0.14	0.92	336
0.03	0.13	0.27	0.24	0.09	0.44	0.18	0.38	0.95	0.94	0.97	0.81	1.07	0.13	0.98	0.81	0.83	0.85	0.70	0.96	0.13	0.88	511
0.06	0.05	0.17	0.13	0.01	0.33	0.16	0.27	0.92	0.89	0.94	0.69	1.10	0.20	0.96	0.77	0.77	0.81	0.59	0.95	0.18	0.84	568
0.11	0.02	0.13	0.09	-0.01	0.27	0.14	0.20	0.89	0.87	0.92	0.67	1.07	0.20	0.94	0.73	0.73	0.77	0.55	0.91	0.18	0.81	566
0.15	-0.00	0.09	0.05	-0.04	0.22	0.13	0.16	0.84	0.78	0.87	0.50	1.06	0.28	0.90	0.66	0.63	0.71	0.40	0.86	0.23	0.74	590
0.18	-0.01	0.07	0.03	-0.04	0.18	0.11	0.13	0.80	0.77	0.84	0.52	1.01	0.24	0.87	0.62	0.61	0.66	0.41	0.80	0.20	0.70	576
0.32	-0.02	0.04	0.01	-0.06	0.14	0.10	0.08	0.73	0.73	0.78	0.54	0.93	0.20	0.82	0.55	0.56	0.60	0.41	0.72	0.16	0.64	1032


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.25
kendall	0.21


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	8.39	14.30	12.49	6.28	22.33	8.02	18.70	3.95	12.11	9.84	2.74	21.47	9.36	18.08	2.16	7.10	4.89	0.59	13.61	6.51	10.76	336
0.03	7.12	11.97	9.66	4.31	19.64	7.67	14.37	2.78	9.68	5.83	0.53	18.84	9.16	14.77	1.73	6.22	3.60	-0.05	12.49	6.27	8.76	511
0.06	5.57	8.08	7.15	3.42	12.74	4.66	8.99	2.40	5.80	3.50	0.03	11.57	5.77	6.86	1.57	4.43	2.26	-0.33	9.18	4.75	5.50	568
0.11	4.56	5.95	5.87	3.32	8.58	2.63	7.10	2.15	3.94	2.99	0.89	6.99	3.05	4.31	1.42	3.24	1.94	-0.36	6.85	3.60	3.59	566
0.15	3.66	4.68	4.76	3.03	6.33	1.65	5.66	2.03	3.02	2.63	1.41	4.62	1.61	3.53	1.34	2.69	1.81	-1.32	6.70	4.01	2.59	590
0.18	3.29	4.07	4.13	2.73	5.41	1.34	4.90	1.95	2.61	2.37	1.50	3.72	1.11	2.99	1.24	2.02	1.60	-0.33	4.37	2.35	2.07	576
0.32	2.81	3.40	3.47	2.32	4.48	1.08	4.09	1.84	2.30	2.22	1.57	3.03	0.73	2.66	1.14	1.61	1.43	0.64	2.57	0.96	1.78	1032


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/ets_sts_auc.tex <==
name	auc
et_use	1.78
et_tse	1.26
et_ce	0.93


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.34	7.03	3.86	-5.61	19.67	12.64	6.36	4.95	8.82	7.52	2.69	14.96	6.13	10.68	3.92	8.04	6.48	1.95	14.13	6.09	9.93	336
0.03	1.57	3.06	2.12	-1.36	7.48	4.42	3.05	4.72	6.85	6.40	3.69	10.00	3.16	8.29	3.70	6.08	5.28	2.27	9.89	3.81	7.27	511
0.06	0.91	1.68	1.20	-1.70	5.07	3.38	1.66	3.99	5.35	5.04	3.02	7.68	2.33	6.30	3.04	4.51	4.13	2.03	6.98	2.47	5.23	568
0.11	0.59	0.97	0.76	-0.50	2.44	1.47	1.02	3.52	4.45	4.23	2.97	5.92	1.48	5.05	2.73	3.76	3.42	1.89	5.63	1.87	4.22	566
0.15	0.36	0.62	0.45	-0.86	2.11	1.48	0.59	3.00	3.67	3.52	2.32	5.02	1.35	4.04	2.35	3.12	2.88	1.09	5.15	2.03	3.38	590
0.18	0.25	0.53	0.32	-2.01	3.07	2.54	0.41	2.76	3.36	3.15	2.09	4.64	1.28	3.58	2.17	2.96	2.57	0.66	5.25	2.29	3.01	576
0.32	0.15	0.40	0.20	-2.40	3.20	2.80	0.27	2.46	2.92	2.72	1.71	4.13	1.21	3.10	1.96	2.50	2.23	0.58	4.42	1.92	2.61	1032


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.35
et_p_h	1.29
et_p_l2	1.12


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.08	0.08	0.03	0.12	0.04	0.10	0.03	0.05	0.05	0.02	0.07	0.02	0.06	0.03	0.04	0.04	0.02	0.05	0.02	0.05	336
0.03	0.13	0.18	0.17	0.10	0.25	0.08	0.22	0.05	0.08	0.07	0.04	0.11	0.03	0.09	0.05	0.06	0.06	0.04	0.08	0.02	0.07	511
0.06	0.26	0.35	0.35	0.21	0.49	0.14	0.44	0.08	0.11	0.10	0.07	0.15	0.04	0.13	0.07	0.08	0.08	0.06	0.11	0.02	0.10	568
0.11	0.45	0.57	0.57	0.35	0.80	0.23	0.70	0.10	0.13	0.12	0.09	0.17	0.04	0.15	0.09	0.10	0.10	0.08	0.13	0.03	0.12	566
0.15	0.79	1.01	1.01	0.59	1.43	0.42	1.23	0.13	0.16	0.16	0.12	0.21	0.05	0.18	0.11	0.13	0.13	0.10	0.16	0.03	0.14	590
0.18	1.15	1.48	1.45	0.85	2.10	0.63	1.72	0.16	0.18	0.18	0.13	0.23	0.05	0.21	0.13	0.15	0.15	0.12	0.18	0.03	0.16	576
0.32	1.77	2.55	2.32	1.36	3.73	1.18	3.18	0.18	0.21	0.21	0.16	0.27	0.05	0.24	0.15	0.17	0.17	0.14	0.21	0.04	0.19	1032


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.38
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.98	0.98	0.95	1.00	0.02	0.98	0.93	0.95	0.98	0.91	1.00	0.05	0.98	0.86	0.91	0.95	0.83	1.00	0.08	0.97	336
0.03	0.95	0.96	0.96	0.91	1.00	0.04	0.97	0.88	0.92	0.94	0.85	0.99	0.07	0.97	0.79	0.87	0.91	0.75	0.98	0.12	0.96	511
0.06	0.93	0.94	0.94	0.89	0.98	0.04	0.95	0.83	0.88	0.88	0.81	0.95	0.07	0.94	0.74	0.82	0.81	0.70	0.94	0.12	0.93	568
0.11	0.91	0.91	0.93	0.84	0.98	0.07	0.94	0.81	0.85	0.85	0.77	0.92	0.08	0.91	0.70	0.77	0.77	0.63	0.91	0.14	0.89	566
0.15	0.88	0.89	0.91	0.82	0.95	0.06	0.92	0.78	0.82	0.83	0.75	0.89	0.07	0.87	0.67	0.74	0.74	0.61	0.87	0.13	0.82	590
0.18	0.87	0.87	0.89	0.80	0.94	0.07	0.90	0.76	0.80	0.81	0.74	0.86	0.06	0.84	0.64	0.70	0.71	0.57	0.82	0.13	0.77	576
0.32	0.83	0.84	0.86	0.76	0.91	0.08	0.88	0.74	0.78	0.78	0.71	0.84	0.06	0.82	0.59	0.65	0.67	0.52	0.78	0.13	0.73	1032


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.26
sts_ce	0.23


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	22.13	23.47	25.18	16.97	29.98	6.50	27.62	0.19	0.26	0.25	0.16	0.36	0.10	0.32	4.17	23.48	10.30	-8.51	55.47	31.99	30.90	336
0.03	32.81	35.27	38.21	24.09	46.45	11.18	42.59	0.25	0.34	0.32	0.22	0.45	0.12	0.40	4.56	26.76	11.20	-14.47	67.99	41.23	28.42	511
0.06	38.88	42.29	45.47	27.09	57.49	15.20	50.36	0.28	0.38	0.36	0.25	0.50	0.13	0.45	5.06	25.25	12.61	-10.63	61.13	35.88	27.60	568
0.11	48.98	54.47	59.48	36.10	72.84	18.37	65.65	0.31	0.40	0.38	0.27	0.53	0.13	0.46	5.01	28.34	13.07	-14.35	71.03	42.69	31.02	566
0.15	65.91	75.61	79.71	48.40	102.82	27.21	90.90	0.31	0.41	0.39	0.28	0.54	0.13	0.48	6.31	34.75	16.58	-12.89	82.39	47.64	41.44	590
0.18	84.28	96.79	101.29	60.39	133.19	36.40	116.84	0.33	0.43	0.40	0.29	0.57	0.14	0.49	6.64	39.69	17.11	-13.73	93.12	53.42	49.05	576
0.32	113.84	136.71	141.17	85.64	187.78	51.07	171.13	0.33	0.45	0.41	0.29	0.61	0.16	0.54	7.92	46.19	23.74	-11.00	103.38	57.19	61.65	1032


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/time_misc_auc.tex <==
name	auc
attack_time	25.65
l2	0.13
lom	11.02


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.78	0.82	0.83	0.69	0.94	0.13	0.89	0.90	0.91	0.93	0.81	1.01	0.10	0.95	0.92	0.93	0.95	0.86	1.01	0.07	0.97	336
0.03	0.68	0.74	0.75	0.61	0.86	0.12	0.82	0.88	0.89	0.90	0.79	0.98	0.09	0.93	0.91	0.92	0.93	0.85	0.99	0.07	0.95	511
0.06	0.58	0.65	0.68	0.48	0.81	0.17	0.75	0.84	0.84	0.87	0.71	0.97	0.13	0.90	0.89	0.89	0.92	0.80	0.99	0.10	0.94	568
0.11	0.50	0.58	0.60	0.42	0.75	0.16	0.69	0.81	0.82	0.84	0.69	0.94	0.13	0.88	0.87	0.88	0.90	0.78	0.97	0.10	0.92	566
0.15	0.38	0.49	0.53	0.28	0.69	0.20	0.63	0.75	0.74	0.79	0.57	0.91	0.17	0.82	0.83	0.83	0.87	0.70	0.95	0.13	0.89	590
0.18	0.31	0.45	0.48	0.24	0.65	0.21	0.60	0.72	0.72	0.76	0.58	0.87	0.15	0.80	0.81	0.81	0.84	0.71	0.92	0.11	0.87	576
0.32	0.22	0.40	0.43	0.18	0.62	0.22	0.58	0.67	0.69	0.72	0.56	0.82	0.13	0.77	0.78	0.79	0.81	0.71	0.88	0.09	0.84	1032


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/a/top_intersections_auc.tex <==
name	auc
top10	0.16
top30	0.24
top50	0.26


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	31.51	42.63	38.69	21.70	63.55	20.93	48.92	31.00	38.94	38.00	25.02	52.86	13.92	46.00	35.23	46.87	42.72	24.90	68.84	21.97	53.72	31.00	39.25	38.00	25.37	53.12	13.87	47.00	485
0.03	31.78	43.36	38.25	20.40	66.32	22.96	48.48	30.00	38.25	37.00	21.91	54.60	16.34	46.00	39.29	52.44	46.96	27.39	77.49	25.05	60.05	30.00	38.68	37.00	22.32	55.04	16.36	46.00	429
0.06	30.97	43.46	38.33	21.63	65.30	21.83	49.55	29.50	38.88	37.00	19.86	57.91	19.02	46.00	46.39	60.09	53.21	36.32	83.86	23.77	68.85	31.00	40.17	38.00	21.35	58.98	18.81	49.00	315
0.11	32.86	46.67	39.86	12.30	81.04	34.37	49.91	29.25	36.93	36.00	20.94	52.91	15.99	45.00	55.92	75.40	69.64	34.50	116.29	40.90	83.10	32.00	39.12	39.00	22.82	55.41	16.29	47.75	206
0.15	31.78	46.12	40.56	25.16	67.08	20.96	53.13	29.50	37.58	36.00	21.49	53.67	16.09	46.00	74.30	98.39	85.76	44.12	152.66	54.27	114.87	33.50	41.36	40.00	24.75	57.97	16.61	51.00	119
0.18	34.23	49.72	39.57	4.27	95.18	45.46	52.81	22.00	34.25	34.00	16.27	52.23	17.98	42.00	86.98	113.04	102.12	56.46	169.61	56.57	121.38	26.00	38.02	39.00	19.16	56.89	18.86	51.00	87
0.32	34.42	54.99	39.57	-1.55	111.53	56.54	52.97	27.00	36.52	35.00	17.20	55.84	19.32	46.25	123.10	174.07	144.73	52.59	295.55	121.48	186.34	31.75	41.65	42.00	21.05	62.24	20.59	54.00	128


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	15.04
orig_ge	11.36
adv_pp	32.74
adv_ge	12.34


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.30	-0.09	-0.10	-0.40	0.21	0.30	0.06	0.10	0.25	0.20	0.01	0.48	0.23	0.36	0.07	0.19	0.15	0.00	0.38	0.19	0.27	485
0.03	-0.41	-0.22	-0.19	-0.48	0.04	0.26	-0.03	0.03	0.15	0.14	-0.05	0.35	0.20	0.26	0.02	0.12	0.10	-0.04	0.27	0.15	0.19	429
0.06	-0.44	-0.28	-0.24	-0.53	-0.03	0.25	-0.06	-0.01	0.08	0.07	-0.10	0.27	0.18	0.19	-0.01	0.06	0.05	-0.07	0.20	0.14	0.14	315
0.11	-0.59	-0.42	-0.47	-0.67	-0.18	0.24	-0.23	-0.08	0.01	0.02	-0.19	0.20	0.19	0.11	-0.06	0.01	0.02	-0.14	0.15	0.15	0.09	206
0.15	-0.67	-0.46	-0.47	-0.69	-0.22	0.24	-0.28	-0.10	-0.02	-0.04	-0.20	0.15	0.18	0.08	-0.07	-0.01	-0.03	-0.14	0.12	0.13	0.06	119
0.18	-0.72	-0.53	-0.60	-0.76	-0.30	0.23	-0.41	-0.13	-0.05	-0.05	-0.21	0.12	0.17	0.05	-0.09	-0.03	-0.03	-0.15	0.09	0.12	0.04	87
0.32	-0.78	-0.65	-0.71	-0.84	-0.46	0.19	-0.58	-0.18	-0.10	-0.10	-0.26	0.06	0.16	-0.02	-0.12	-0.07	-0.07	-0.18	0.05	0.12	-0.01	128


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/correlations_auc.tex <==
name	auc
pcc	-0.14
spearman	-0.00
kendall	0.00


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	16.44	23.93	21.89	12.77	35.08	11.16	29.57	13.00	24.64	21.70	9.75	39.53	14.89	33.94	5.76	14.82	12.18	2.85	26.79	11.97	19.73	485
0.03	11.74	15.80	14.27	8.54	23.07	7.26	17.70	8.96	15.73	13.70	5.96	25.50	9.77	20.05	4.30	10.91	9.05	1.88	19.95	9.03	14.20	429
0.06	8.71	11.55	11.07	7.53	15.58	4.02	13.52	6.69	11.38	9.65	3.88	18.88	7.50	14.05	3.50	8.03	6.54	2.03	14.03	6.00	10.38	315
0.11	7.45	9.54	9.55	6.09	13.00	3.45	11.62	5.59	8.60	7.70	3.77	13.43	4.83	9.99	3.48	6.22	5.31	1.72	10.71	4.49	7.33	206
0.15	5.27	7.51	7.74	4.88	10.14	2.63	9.64	4.27	6.36	5.61	3.17	9.55	3.19	7.73	2.71	4.78	4.02	1.49	8.06	3.28	5.81	119
0.18	4.86	6.49	6.53	4.41	8.57	2.08	8.19	4.06	5.30	4.83	3.47	7.13	1.83	6.23	2.58	4.24	3.38	0.27	8.20	3.97	4.62	87
0.32	4.63	5.78	5.83	4.02	7.54	1.76	7.10	3.74	4.70	4.49	3.30	6.09	1.40	5.54	2.23	3.78	2.84	0.80	6.75	2.97	4.02	128


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/ets_sts_auc.tex <==
name	auc
et_use	2.75
et_tse	2.49
et_ce	1.81


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	3.88	7.37	5.39	-0.29	15.03	7.66	7.84	9.10	13.90	12.16	6.70	21.11	7.20	17.88	7.14	12.59	10.71	4.60	20.59	7.99	15.88	485
0.03	2.06	4.23	2.67	-4.72	13.19	8.95	3.80	7.19	10.01	8.91	5.63	14.40	4.38	11.56	5.58	8.53	7.45	4.03	13.04	4.50	10.02	429
0.06	1.17	2.15	1.55	-1.29	5.58	3.43	1.97	5.55	7.75	7.16	4.04	11.46	3.71	8.68	4.42	6.77	5.98	2.14	11.39	4.62	7.39	315
0.11	0.83	1.28	1.05	-0.17	2.72	1.44	1.32	5.50	6.78	6.28	3.94	9.61	2.84	7.81	4.45	5.69	5.17	2.63	8.76	3.07	6.36	206
0.15	0.52	0.73	0.63	0.13	1.33	0.60	0.80	4.74	5.53	5.39	4.28	6.77	1.24	6.33	3.78	4.56	4.48	3.25	5.86	1.31	5.20	119
0.18	0.43	0.62	0.51	0.19	1.05	0.43	0.60	4.55	5.29	5.28	4.05	6.52	1.24	5.91	3.77	4.38	4.21	3.31	5.45	1.07	4.90	87
0.32	0.26	0.84	0.33	-3.98	5.66	4.82	0.45	4.39	4.88	4.86	3.91	5.84	0.97	5.39	3.58	4.06	3.99	3.13	4.99	0.93	4.57	128


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.46
et_p_h	1.99
et_p_l2	1.68


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.10	0.10	0.06	0.15	0.04	0.13	0.04	0.06	0.05	0.03	0.08	0.03	0.07	0.03	0.05	0.04	0.03	0.06	0.02	0.06	485
0.03	0.17	0.23	0.23	0.14	0.31	0.09	0.28	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	429
0.06	0.34	0.42	0.42	0.28	0.57	0.14	0.51	0.09	0.11	0.11	0.08	0.15	0.04	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.11	315
0.11	0.57	0.69	0.70	0.46	0.92	0.23	0.81	0.12	0.14	0.14	0.11	0.17	0.03	0.15	0.10	0.11	0.11	0.09	0.13	0.02	0.12	206
0.15	0.96	1.17	1.14	0.81	1.53	0.36	1.42	0.15	0.17	0.16	0.13	0.20	0.03	0.19	0.12	0.14	0.13	0.11	0.16	0.02	0.15	119
0.18	1.24	1.49	1.50	1.03	1.95	0.46	1.77	0.16	0.18	0.18	0.15	0.22	0.04	0.20	0.13	0.15	0.15	0.13	0.17	0.02	0.16	87
0.32	1.88	2.57	2.52	1.53	3.61	1.04	3.13	0.19	0.21	0.21	0.17	0.25	0.04	0.24	0.16	0.17	0.17	0.15	0.20	0.03	0.19	128


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.40
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.96	0.99	0.02	0.98	0.96	0.97	0.98	0.94	1.00	0.03	0.98	0.92	0.93	0.96	0.85	1.00	0.07	0.97	485
0.03	0.95	0.95	0.96	0.93	0.98	0.03	0.97	0.93	0.95	0.96	0.90	0.99	0.04	0.97	0.85	0.90	0.93	0.81	0.99	0.09	0.96	429
0.06	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.90	0.93	0.94	0.88	0.97	0.04	0.96	0.83	0.88	0.91	0.80	0.96	0.08	0.94	315
0.11	0.91	0.92	0.93	0.88	0.95	0.04	0.94	0.88	0.90	0.91	0.85	0.95	0.05	0.93	0.79	0.84	0.87	0.75	0.93	0.09	0.91	206
0.15	0.89	0.89	0.90	0.83	0.95	0.06	0.92	0.83	0.86	0.88	0.79	0.93	0.07	0.90	0.72	0.79	0.81	0.66	0.92	0.13	0.90	119
0.18	0.86	0.87	0.88	0.83	0.91	0.04	0.90	0.82	0.84	0.85	0.79	0.89	0.05	0.88	0.69	0.76	0.77	0.66	0.86	0.10	0.84	87
0.32	0.83	0.84	0.86	0.78	0.90	0.06	0.88	0.78	0.81	0.82	0.75	0.87	0.06	0.85	0.62	0.71	0.72	0.58	0.83	0.13	0.80	128


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.27
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	40.59	81.77	45.83	-93.34	256.88	175.11	56.41	1.17	4.18	2.69	-2.19	10.54	6.37	4.69	20.14	57.78	45.07	3.56	112.00	54.22	75.95	485
0.03	104.50	273.93	129.56	-49.75	597.62	323.68	263.63	1.68	5.07	3.30	-1.61	11.75	6.68	5.66	21.42	55.42	44.47	5.81	105.03	49.61	73.08	429
0.06	155.19	532.49	325.74	105.12	959.86	427.37	1022.28	2.10	5.98	3.69	-1.95	13.91	7.93	6.95	20.06	57.58	47.94	8.19	106.97	49.39	76.24	315
0.11	201.82	551.85	370.74	142.60	961.09	409.25	1059.02	2.31	7.13	4.82	-6.93	21.18	14.06	7.42	22.89	54.49	36.02	0.77	108.20	53.72	69.10	206
0.15	248.02	477.24	331.29	157.96	796.53	319.28	749.28	2.35	6.03	3.77	-5.81	17.87	11.84	5.15	20.51	45.62	42.43	15.18	76.05	30.44	65.41	119
0.18	283.66	428.18	350.20	176.61	679.76	251.58	548.08	1.66	5.89	3.13	-10.06	21.83	15.95	5.06	17.29	43.51	34.54	6.83	80.19	36.68	59.93	87
0.32	362.78	481.87	468.63	230.21	733.52	251.65	596.36	1.80	4.98	3.10	-6.54	16.51	11.53	4.67	16.13	38.06	32.47	9.77	66.35	28.29	53.85	128


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/time_misc_auc.tex <==
name	auc
attack_time	140.57
l2	1.79
lom	14.69


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.23	0.35	0.32	0.18	0.52	0.17	0.44	0.39	0.48	0.45	0.34	0.61	0.13	0.55	0.55	0.61	0.59	0.51	0.71	0.10	0.65	485
0.03	0.19	0.28	0.26	0.14	0.42	0.14	0.35	0.36	0.43	0.41	0.32	0.54	0.11	0.48	0.52	0.57	0.57	0.49	0.65	0.08	0.61	429
0.06	0.15	0.23	0.24	0.11	0.35	0.12	0.30	0.33	0.39	0.38	0.30	0.49	0.09	0.44	0.51	0.54	0.54	0.47	0.62	0.07	0.59	315
0.11	0.14	0.22	0.22	0.11	0.33	0.11	0.29	0.30	0.36	0.35	0.26	0.46	0.10	0.42	0.47	0.52	0.52	0.44	0.60	0.08	0.56	206
0.15	0.12	0.19	0.18	0.10	0.28	0.09	0.25	0.29	0.34	0.36	0.24	0.45	0.10	0.39	0.48	0.51	0.51	0.44	0.58	0.07	0.55	119
0.18	0.10	0.17	0.18	0.07	0.26	0.09	0.24	0.27	0.34	0.33	0.25	0.42	0.08	0.38	0.47	0.50	0.49	0.43	0.57	0.07	0.54	87
0.32	0.09	0.16	0.17	0.07	0.25	0.09	0.22	0.27	0.31	0.31	0.23	0.40	0.09	0.35	0.45	0.48	0.49	0.40	0.56	0.08	0.52	128


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/ig/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.11
top50	0.16


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	31.55	43.33	38.76	21.12	65.54	22.21	49.41	31.00	39.31	38.00	24.21	54.40	15.09	47.00	34.96	47.98	43.29	24.22	71.74	23.76	54.62	31.00	39.77	39.00	24.68	54.87	15.09	48.00	493
0.03	31.89	44.70	39.34	20.09	69.31	24.61	50.72	31.00	38.96	38.00	23.29	54.63	15.67	47.00	40.11	54.69	49.01	27.55	81.82	27.13	61.92	31.00	39.66	38.00	24.06	55.27	15.60	48.00	622
0.06	32.04	44.15	38.79	18.10	70.21	26.05	49.52	31.00	39.38	38.00	22.55	56.21	16.83	46.00	46.95	61.82	55.63	30.23	93.42	31.59	70.84	32.00	40.68	40.00	23.89	57.48	16.79	48.00	779
0.11	30.24	43.03	37.70	13.58	72.47	29.45	46.89	27.00	35.04	34.00	20.80	49.27	14.24	42.00	55.69	73.36	65.70	32.58	114.14	40.78	83.95	29.00	37.40	37.00	22.78	52.01	14.61	45.00	398
0.15	32.58	53.71	39.24	-7.45	114.87	61.16	48.48	21.25	34.43	36.00	15.86	53.01	18.57	45.00	71.99	105.23	86.00	23.06	187.40	82.17	103.34	24.25	37.25	39.50	17.85	56.66	19.41	48.00	122
0.18	31.78	54.71	37.97	-4.57	113.99	59.28	52.81	18.50	32.08	32.00	12.23	51.94	19.85	45.50	82.38	126.46	100.00	0.16	252.77	126.31	120.99	24.00	35.46	36.00	14.22	56.70	21.24	49.00	83
0.32	33.33	83.34	47.89	-13.06	179.75	96.41	72.21	10.50	25.79	24.00	5.53	46.04	20.26	39.25	115.79	235.82	146.20	-62.09	533.72	297.91	216.48	12.00	30.36	27.00	6.92	53.80	23.44	46.75	80


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/comparison_vals_auc.tex <==
name	auc
orig_pp	17.59
orig_ge	10.29
adv_pp	38.37
adv_ge	11.17


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.05	0.40	0.26	0.03	0.78	0.37	0.80	0.31	0.57	0.64	0.24	0.90	0.33	0.88	0.22	0.46	0.46	0.17	0.75	0.29	0.73	493
0.03	0.00	0.18	0.05	-0.09	0.45	0.27	0.23	0.08	0.35	0.32	0.03	0.68	0.32	0.63	0.06	0.26	0.22	0.01	0.52	0.26	0.46	622
0.06	-0.01	0.06	0.02	-0.10	0.21	0.15	0.05	0.02	0.21	0.17	-0.07	0.48	0.27	0.37	0.01	0.15	0.11	-0.05	0.35	0.20	0.25	779
0.11	-0.01	0.04	0.01	-0.07	0.15	0.11	0.07	-0.00	0.19	0.16	-0.08	0.46	0.27	0.36	-0.00	0.14	0.11	-0.05	0.33	0.19	0.25	398
0.15	-0.03	0.04	0.00	-0.11	0.20	0.15	0.08	0.01	0.18	0.18	-0.15	0.51	0.33	0.42	0.00	0.13	0.12	-0.11	0.38	0.24	0.28	122
0.18	-0.04	0.05	0.03	-0.14	0.24	0.19	0.09	-0.09	0.15	0.18	-0.18	0.49	0.34	0.37	-0.06	0.11	0.12	-0.13	0.36	0.24	0.25	83
0.32	-0.08	0.02	0.01	-0.15	0.20	0.17	0.05	-0.12	0.14	0.16	-0.18	0.46	0.32	0.38	-0.08	0.11	0.10	-0.12	0.34	0.23	0.26	80


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/correlations_auc.tex <==
name	auc
pcc	0.02
spearman	0.06
kendall	0.05


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	4.07	11.56	12.09	3.33	19.79	8.23	16.73	4.12	13.04	12.04	2.79	23.29	10.25	20.08	1.73	7.98	5.62	-0.08	16.05	8.06	11.59	493
0.03	7.47	9.88	9.85	5.44	14.32	4.44	12.45	7.20	11.25	10.46	4.63	17.87	6.62	14.49	3.00	7.49	6.43	1.61	13.37	5.88	10.10	622
0.06	6.28	7.90	7.95	5.23	10.57	2.67	9.39	5.56	8.53	7.79	3.61	13.46	4.92	10.06	2.53	5.51	4.44	1.30	9.73	4.21	7.15	779
0.11	4.58	5.98	6.12	3.87	8.09	2.11	7.32	3.93	5.84	5.40	2.89	8.79	2.95	6.87	2.03	3.67	2.74	1.28	6.06	2.39	4.96	398
0.15	4.10	4.91	4.95	3.36	6.45	1.55	5.90	3.35	4.31	4.43	2.81	5.80	1.49	5.07	1.79	3.16	2.37	0.92	5.39	2.24	3.81	122
0.18	3.37	4.25	4.54	2.83	5.67	1.42	5.36	2.72	3.83	3.79	2.14	5.52	1.69	4.37	1.64	2.43	2.04	1.03	3.83	1.40	3.06	83
0.32	2.70	3.46	3.50	2.22	4.70	1.24	4.17	2.47	3.11	2.92	2.04	4.19	1.08	3.65	1.67	2.40	2.04	1.12	3.69	1.29	2.73	80


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/ets_sts_auc.tex <==
name	auc
et_use	1.72
et_tse	1.71
et_ce	1.14


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.96	3.37	3.02	-0.26	7.00	3.63	4.55	1.96	6.58	6.68	1.56	11.59	5.02	9.81	1.57	5.98	5.35	-0.27	12.23	6.25	8.17	493
0.03	1.38	2.16	1.83	-2.81	7.13	4.97	2.50	4.71	6.07	6.15	3.18	8.96	2.89	7.50	3.61	5.32	4.97	0.44	10.19	4.88	6.34	622
0.06	0.90	1.42	1.16	-1.62	4.47	3.04	1.43	4.47	5.24	5.19	3.72	6.76	1.52	5.97	3.46	4.35	4.19	2.53	6.17	1.82	4.95	779
0.11	0.52	0.70	0.66	0.39	1.02	0.32	0.80	3.59	4.10	4.04	3.18	5.03	0.92	4.59	2.73	3.34	3.23	2.30	4.38	1.04	3.86	398
0.15	0.35	0.48	0.41	0.17	0.80	0.32	0.51	3.13	3.78	3.50	1.19	6.37	2.59	3.82	2.44	3.21	2.91	0.16	6.27	3.05	3.16	122
0.18	0.24	0.40	0.32	0.13	0.67	0.27	0.44	2.58	3.15	3.11	2.02	4.27	1.12	3.42	2.07	2.64	2.50	1.43	3.84	1.21	2.82	83
0.32	0.16	0.39	0.22	-0.26	1.04	0.65	0.32	2.54	3.28	2.90	1.19	5.37	2.09	3.36	2.03	2.96	2.37	0.07	5.85	2.89	2.85	80


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.25
et_p_h	1.24
et_p_l2	1.06


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.11	0.11	0.07	0.16	0.05	0.14	0.05	0.06	0.06	0.04	0.09	0.02	0.08	0.04	0.05	0.05	0.04	0.07	0.02	0.06	493
0.03	0.18	0.24	0.24	0.15	0.33	0.09	0.29	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.06	0.07	0.07	0.05	0.09	0.02	0.08	622
0.06	0.34	0.43	0.42	0.27	0.59	0.16	0.52	0.10	0.12	0.11	0.09	0.15	0.03	0.14	0.08	0.09	0.09	0.07	0.11	0.02	0.10	779
0.11	0.62	0.77	0.73	0.51	1.03	0.26	0.91	0.13	0.15	0.15	0.12	0.19	0.04	0.17	0.11	0.12	0.12	0.10	0.14	0.02	0.13	398
0.15	0.99	1.16	1.16	0.80	1.52	0.36	1.38	0.15	0.18	0.17	0.13	0.22	0.05	0.19	0.13	0.14	0.14	0.11	0.17	0.03	0.15	122
0.18	1.12	1.53	1.52	0.86	2.20	0.67	1.94	0.17	0.20	0.20	0.14	0.25	0.06	0.22	0.14	0.16	0.16	0.12	0.19	0.03	0.17	83
0.32	1.57	2.37	2.26	0.97	3.77	1.40	3.00	0.17	0.21	0.21	0.14	0.27	0.07	0.23	0.15	0.17	0.17	0.12	0.21	0.05	0.19	80


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.39
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.96	0.98	0.01	0.98	0.97	0.97	0.98	0.95	0.99	0.02	0.98	0.93	0.94	0.96	0.87	1.00	0.06	0.97	493
0.03	0.95	0.95	0.96	0.94	0.97	0.02	0.96	0.95	0.95	0.96	0.93	0.98	0.03	0.97	0.89	0.91	0.94	0.84	0.98	0.07	0.96	622
0.06	0.93	0.93	0.94	0.89	0.97	0.04	0.95	0.92	0.93	0.94	0.88	0.97	0.05	0.95	0.82	0.86	0.90	0.76	0.96	0.10	0.93	779
0.11	0.90	0.90	0.92	0.84	0.97	0.06	0.93	0.88	0.90	0.91	0.84	0.96	0.06	0.93	0.77	0.81	0.83	0.68	0.94	0.13	0.90	398
0.15	0.88	0.89	0.90	0.85	0.94	0.04	0.92	0.86	0.88	0.89	0.83	0.92	0.04	0.90	0.74	0.80	0.80	0.71	0.89	0.09	0.87	122
0.18	0.86	0.88	0.89	0.83	0.92	0.05	0.91	0.83	0.86	0.87	0.81	0.91	0.05	0.89	0.72	0.77	0.77	0.68	0.85	0.09	0.82	83
0.32	0.82	0.84	0.86	0.78	0.90	0.06	0.88	0.80	0.83	0.83	0.79	0.87	0.04	0.86	0.70	0.76	0.77	0.65	0.86	0.11	0.82	80


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.27
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	25.76	40.77	29.53	-11.78	93.33	52.55	37.01	2.18	132.72	16.53	-161.61	427.05	294.33	129.43	9.44	47.14	28.00	0.79	93.49	46.35	78.16	493
0.03	34.61	143.07	75.79	-6.90	293.05	149.97	200.78	31.32	317.43	144.51	-439.73	1074.60	757.17	345.23	18.32	65.98	57.04	14.90	117.07	51.09	108.79	622
0.06	188.86	325.63	384.96	162.80	488.46	162.83	454.40	107.59	380.75	228.54	-131.64	893.14	512.39	429.62	28.49	78.65	77.06	26.95	130.35	51.70	123.17	779
0.11	201.91	336.50	380.80	173.68	499.33	162.82	476.69	126.82	628.06	267.74	-512.03	1768.15	1140.09	588.58	27.14	70.96	66.09	23.41	118.50	47.55	111.45	398
0.15	84.60	246.97	276.90	75.74	418.20	171.23	388.37	47.67	458.48	190.13	-332.09	1249.05	790.57	457.24	24.63	62.68	51.06	16.07	109.30	46.61	100.72	122
0.18	105.97	230.19	198.79	75.88	384.51	154.32	355.25	7.43	446.37	93.69	-387.14	1279.88	833.51	287.42	16.78	57.83	44.31	10.84	104.82	46.99	95.61	83
0.32	38.12	146.91	132.18	19.48	274.35	127.43	200.72	8.76	190.81	54.36	-332.48	714.11	523.29	187.84	13.06	46.44	23.49	-2.66	95.54	49.10	70.10	80


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/time_misc_auc.tex <==
name	auc
attack_time	70.75
l2	121.08
lom	18.85


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.20	0.45	0.39	0.17	0.73	0.28	0.72	0.44	0.62	0.61	0.42	0.83	0.21	0.82	0.60	0.72	0.73	0.57	0.88	0.15	0.86	493
0.03	0.11	0.28	0.21	0.05	0.50	0.22	0.37	0.36	0.49	0.44	0.31	0.67	0.18	0.60	0.51	0.63	0.61	0.49	0.77	0.14	0.73	622
0.06	0.09	0.18	0.14	0.03	0.33	0.15	0.22	0.32	0.41	0.39	0.27	0.55	0.14	0.46	0.49	0.57	0.55	0.46	0.68	0.11	0.63	779
0.11	0.09	0.17	0.14	0.04	0.30	0.13	0.23	0.32	0.40	0.37	0.27	0.53	0.13	0.45	0.49	0.56	0.55	0.46	0.67	0.11	0.62	398
0.15	0.07	0.16	0.12	0.01	0.30	0.15	0.20	0.28	0.39	0.36	0.23	0.55	0.16	0.45	0.49	0.56	0.56	0.42	0.70	0.14	0.65	122
0.18	0.07	0.17	0.14	-0.02	0.37	0.19	0.21	0.28	0.38	0.38	0.23	0.53	0.15	0.44	0.47	0.55	0.56	0.41	0.69	0.14	0.63	83
0.32	0.00	0.13	0.06	-0.05	0.31	0.18	0.20	0.25	0.36	0.34	0.19	0.53	0.17	0.45	0.47	0.55	0.55	0.43	0.67	0.12	0.62	80


==> data/mlm_plots/mlm_distil_fast/fakenews/roberta/s/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.12
top50	0.18


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	32.26	43.95	40.19	23.86	64.05	20.10	50.95	29.00	35.86	35.00	22.75	48.96	13.11	41.00	36.18	48.80	44.60	27.28	70.32	21.52	56.34	29.00	36.11	35.00	23.03	49.19	13.08	42.00	823
0.03	32.15	44.78	39.58	21.68	67.87	23.09	51.03	28.00	35.30	35.00	21.37	49.23	13.93	42.00	40.05	55.06	49.65	29.50	80.63	25.56	62.94	29.00	35.88	35.00	22.00	49.77	13.88	43.00	930
0.06	32.12	46.86	39.94	16.35	77.37	30.51	51.99	28.00	34.52	34.00	20.00	49.05	14.52	41.00	47.55	66.83	59.15	29.75	103.91	37.08	74.33	28.00	35.69	36.00	21.11	50.27	14.58	43.00	959
0.11	32.16	48.90	40.27	8.73	89.06	40.17	52.01	27.00	34.37	34.00	19.39	49.35	14.98	41.00	56.57	82.27	68.46	-0.91	165.45	83.18	87.29	29.00	36.10	36.50	21.06	51.14	15.04	44.00	968
0.15	32.19	50.53	40.49	1.10	99.97	49.43	51.99	27.00	33.94	34.00	19.74	48.15	14.21	41.00	73.73	104.99	89.03	23.92	186.05	81.06	109.56	29.00	36.88	38.00	22.17	51.59	14.71	45.00	830
0.18	32.16	53.18	40.61	-7.72	114.09	60.91	52.50	27.00	33.74	34.00	19.55	47.94	14.20	41.00	91.89	131.32	110.74	19.81	242.84	111.52	134.38	30.00	37.65	39.00	22.65	52.64	14.99	47.00	776
0.32	32.39	51.46	40.53	2.36	100.57	49.10	52.11	27.00	33.80	34.00	19.22	48.38	14.58	41.00	124.04	181.42	155.98	38.68	324.15	142.73	204.51	31.00	39.04	40.00	23.51	54.57	15.53	49.00	1124


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/comparison_vals_auc.tex <==
name	auc
orig_pp	15.55
orig_ge	10.61
adv_pp	35.71
adv_ge	11.55


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.10	0.33	0.27	0.05	0.60	0.28	0.50	0.53	0.73	0.88	0.45	1.02	0.28	0.97	0.37	0.62	0.70	0.33	0.90	0.28	0.88	823
0.03	0.03	0.18	0.12	-0.02	0.39	0.20	0.29	0.50	0.69	0.80	0.40	0.98	0.29	0.93	0.35	0.56	0.62	0.29	0.83	0.27	0.80	930
0.06	-0.00	0.08	0.03	-0.06	0.22	0.14	0.12	0.46	0.64	0.76	0.35	0.93	0.29	0.88	0.31	0.50	0.57	0.25	0.76	0.25	0.72	959
0.11	-0.02	0.03	0.00	-0.07	0.13	0.10	0.06	0.40	0.59	0.69	0.30	0.89	0.30	0.84	0.27	0.46	0.51	0.21	0.70	0.25	0.67	968
0.15	-0.04	-0.01	-0.01	-0.10	0.09	0.09	0.01	0.34	0.53	0.61	0.23	0.83	0.30	0.78	0.23	0.40	0.45	0.16	0.64	0.24	0.60	830
0.18	-0.05	-0.03	-0.03	-0.12	0.06	0.09	-0.01	0.29	0.47	0.55	0.16	0.78	0.31	0.72	0.19	0.35	0.39	0.11	0.59	0.24	0.54	776
0.32	-0.09	-0.06	-0.05	-0.14	0.02	0.08	-0.02	0.16	0.37	0.43	0.05	0.69	0.32	0.63	0.10	0.27	0.30	0.03	0.50	0.24	0.45	1124


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/correlations_auc.tex <==
name	auc
pcc	0.01
spearman	0.16
kendall	0.12


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	8.97	14.54	13.70	6.10	22.98	8.44	18.84	6.34	14.44	13.15	4.66	24.22	9.78	19.90	2.70	8.71	6.65	1.27	16.15	7.44	12.71	823
0.03	7.74	10.46	9.82	5.58	15.34	4.88	12.59	5.27	10.10	9.01	3.67	16.54	6.44	13.55	2.40	6.59	4.83	0.91	12.26	5.68	8.84	930
0.06	6.04	7.93	7.87	4.35	11.50	3.58	9.32	3.91	7.50	6.05	1.94	13.06	5.56	9.24	2.10	4.48	3.19	0.63	8.32	3.85	5.70	959
0.11	5.40	6.51	6.52	4.26	8.77	2.25	7.71	3.18	6.27	4.92	1.20	11.34	5.07	7.40	1.93	3.39	2.53	0.34	6.44	3.05	3.79	968
0.15	4.34	5.26	5.40	3.68	6.84	1.58	6.31	2.70	5.09	3.93	0.61	9.56	4.48	5.66	1.75	2.76	2.25	0.74	4.78	2.02	3.07	830
0.18	3.84	4.59	4.73	3.30	5.88	1.29	5.43	2.49	4.64	3.43	0.45	8.84	4.19	5.04	1.66	2.31	2.02	1.14	3.48	1.17	2.63	776
0.32	3.27	3.91	3.95	2.84	4.98	1.07	4.62	2.26	4.01	2.99	0.69	7.32	3.32	4.51	1.48	1.99	1.82	0.89	3.10	1.11	2.20	1124


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/ets_sts_auc.tex <==
name	auc
et_use	1.87
et_tse	1.83
et_ce	1.02


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.89	4.86	2.94	-6.11	15.84	10.98	4.58	4.73	8.31	7.50	2.71	13.92	5.60	10.67	3.70	7.68	6.25	-0.08	15.44	7.76	9.63	823
0.03	1.29	2.14	1.70	-0.55	4.82	2.69	2.29	4.56	6.43	6.08	2.87	10.00	3.57	7.60	3.56	5.64	4.92	0.38	10.89	5.26	6.54	930
0.06	0.81	1.36	1.01	-4.02	6.73	5.37	1.31	4.09	5.21	5.00	3.35	7.06	1.86	6.02	3.20	4.43	4.02	2.08	6.77	2.34	5.13	959
0.11	0.56	0.88	0.69	-0.84	2.60	1.72	0.87	3.77	4.63	4.38	2.99	6.26	1.63	5.19	3.01	3.99	3.56	0.61	7.37	3.38	4.34	968
0.15	0.34	1.09	0.42	-10.80	12.98	11.89	0.53	3.31	3.92	3.73	2.70	5.13	1.22	4.27	2.63	3.66	3.05	-2.76	10.09	6.42	3.63	830
0.18	0.25	0.41	0.30	-0.72	1.54	1.13	0.38	3.04	3.57	3.42	2.36	4.78	1.21	3.87	2.44	3.13	2.82	0.52	5.75	2.61	3.31	776
0.32	0.15	0.25	0.19	-0.13	0.63	0.38	0.25	2.69	3.21	3.03	1.86	4.55	1.35	3.43	2.18	2.85	2.50	-0.39	6.10	3.25	2.91	1124


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.29
et_p_h	1.33
et_p_l2	1.17


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.12	0.11	0.06	0.17	0.05	0.15	0.04	0.06	0.06	0.03	0.09	0.03	0.07	0.04	0.05	0.05	0.03	0.07	0.02	0.06	823
0.03	0.18	0.25	0.25	0.16	0.34	0.09	0.31	0.07	0.09	0.09	0.05	0.12	0.04	0.11	0.06	0.07	0.07	0.05	0.09	0.02	0.08	930
0.06	0.36	0.46	0.46	0.31	0.62	0.16	0.56	0.09	0.12	0.12	0.08	0.16	0.04	0.14	0.08	0.10	0.09	0.07	0.12	0.03	0.11	959
0.11	0.57	0.72	0.71	0.44	1.00	0.28	0.86	0.11	0.14	0.14	0.10	0.18	0.04	0.16	0.10	0.11	0.11	0.08	0.14	0.03	0.13	968
0.15	0.96	1.22	1.20	0.81	1.63	0.41	1.45	0.14	0.17	0.16	0.12	0.22	0.05	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.15	830
0.18	1.36	1.73	1.72	1.12	2.34	0.61	2.09	0.16	0.19	0.18	0.14	0.24	0.05	0.21	0.13	0.15	0.15	0.12	0.18	0.03	0.17	776
0.32	2.08	2.96	2.71	1.62	4.31	1.35	3.67	0.18	0.21	0.21	0.16	0.27	0.06	0.24	0.16	0.18	0.18	0.14	0.21	0.04	0.20	1124


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.45
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.98	0.95	0.99	0.02	0.98	0.96	0.97	0.98	0.93	1.00	0.03	0.98	0.91	0.93	0.96	0.86	1.00	0.07	0.97	823
0.03	0.95	0.95	0.96	0.92	0.99	0.03	0.97	0.93	0.94	0.96	0.89	0.99	0.05	0.97	0.84	0.89	0.92	0.80	0.98	0.09	0.96	930
0.06	0.93	0.93	0.94	0.88	0.98	0.05	0.95	0.88	0.91	0.93	0.85	0.97	0.06	0.95	0.78	0.84	0.86	0.73	0.95	0.11	0.92	959
0.11	0.91	0.91	0.93	0.86	0.97	0.06	0.94	0.85	0.89	0.90	0.82	0.95	0.07	0.93	0.75	0.80	0.81	0.69	0.91	0.11	0.87	968
0.15	0.88	0.89	0.91	0.84	0.94	0.05	0.92	0.82	0.86	0.87	0.79	0.93	0.07	0.91	0.72	0.77	0.78	0.66	0.87	0.11	0.84	830
0.18	0.87	0.88	0.89	0.82	0.93	0.05	0.90	0.79	0.84	0.85	0.77	0.92	0.07	0.90	0.69	0.74	0.75	0.64	0.84	0.10	0.80	776
0.32	0.84	0.85	0.87	0.79	0.91	0.06	0.89	0.77	0.82	0.82	0.74	0.90	0.08	0.88	0.65	0.70	0.71	0.59	0.80	0.11	0.76	1124


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.27
sts_ce	0.24


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	27.83	29.98	31.46	23.17	36.80	6.81	33.82	0.11	0.20	0.16	0.05	0.35	0.15	0.25	12.59	49.18	33.19	1.39	96.97	47.79	74.68	823
0.03	38.86	42.04	44.37	30.29	53.78	11.74	49.73	0.13	0.27	0.21	0.09	0.45	0.18	0.37	18.27	65.05	52.18	8.14	121.95	56.91	95.40	930
0.06	56.84	63.84	67.85	42.31	85.37	21.53	77.49	0.17	0.34	0.29	0.12	0.55	0.21	0.46	20.28	76.05	61.61	10.69	141.42	65.36	117.01	959
0.11	70.72	78.86	84.27	52.12	105.60	26.74	95.30	0.18	0.35	0.30	0.14	0.57	0.22	0.47	22.93	79.56	65.53	13.23	145.89	66.33	121.74	968
0.15	103.59	113.18	121.90	74.30	152.06	38.88	135.87	0.18	0.35	0.29	0.13	0.57	0.22	0.47	29.49	85.73	72.41	19.11	152.35	66.62	130.79	830
0.18	104.80	131.16	130.41	76.92	185.41	54.24	168.91	0.17	0.32	0.27	0.12	0.52	0.20	0.41	27.82	82.44	70.05	18.51	146.38	63.93	127.33	776
0.32	173.25	209.90	213.42	126.64	293.16	83.26	264.43	0.16	0.27	0.23	0.10	0.44	0.17	0.33	27.53	79.35	67.85	18.01	140.69	61.34	122.93	1124


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/time_misc_auc.tex <==
name	auc
attack_time	37.16
l2	0.10
lom	24.37


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.36	0.59	0.66	0.32	0.86	0.27	0.83	0.56	0.73	0.80	0.52	0.93	0.20	0.91	0.69	0.81	0.85	0.67	0.95	0.14	0.94	823
0.03	0.31	0.51	0.56	0.26	0.76	0.25	0.72	0.53	0.69	0.75	0.49	0.88	0.19	0.85	0.68	0.78	0.80	0.65	0.92	0.14	0.91	930
0.06	0.22	0.42	0.44	0.18	0.65	0.24	0.61	0.50	0.64	0.69	0.45	0.83	0.19	0.80	0.66	0.76	0.78	0.63	0.89	0.13	0.87	959
0.11	0.16	0.34	0.34	0.12	0.56	0.22	0.52	0.47	0.61	0.64	0.42	0.79	0.19	0.77	0.64	0.73	0.76	0.61	0.86	0.13	0.84	968
0.15	0.07	0.25	0.23	0.06	0.44	0.19	0.39	0.42	0.56	0.60	0.37	0.75	0.19	0.71	0.63	0.71	0.73	0.58	0.84	0.13	0.81	830
0.18	0.03	0.19	0.15	0.01	0.36	0.17	0.30	0.38	0.52	0.55	0.33	0.70	0.19	0.67	0.61	0.69	0.71	0.56	0.82	0.13	0.79	776
0.32	0.00	0.12	0.06	-0.03	0.27	0.15	0.20	0.30	0.45	0.47	0.26	0.63	0.19	0.60	0.56	0.65	0.66	0.52	0.77	0.13	0.74	1124


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/a/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.17
top50	0.22


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	32.16	43.48	39.82	23.45	63.52	20.04	49.98	29.00	35.67	35.00	23.93	47.41	11.74	42.00	36.27	48.14	44.11	26.96	69.32	21.18	55.28	29.00	35.78	35.00	24.04	47.52	11.74	42.00	733
0.03	32.87	42.62	39.51	26.59	58.65	16.03	48.69	28.00	34.36	34.00	22.19	46.54	12.18	41.00	40.21	51.91	48.10	33.65	70.18	18.27	59.66	28.00	34.39	35.00	22.19	46.59	12.20	41.00	334
0.06	32.60	42.57	38.98	22.53	62.61	20.04	45.15	29.00	36.16	36.00	22.85	49.46	13.31	43.00	45.93	60.29	55.29	33.76	86.82	26.53	66.03	29.00	36.55	36.00	23.21	49.90	13.35	44.50	243
0.11	32.48	46.25	39.47	22.99	69.51	23.26	54.47	29.00	34.45	34.00	21.83	47.06	12.61	41.00	56.93	78.34	69.92	43.20	113.48	35.14	91.76	29.25	35.39	35.50	22.75	48.02	12.64	42.00	210
0.15	34.45	46.03	38.76	23.60	68.46	22.43	49.71	27.00	37.10	35.00	17.40	56.80	19.70	44.00	73.54	94.48	84.32	60.74	128.21	33.74	105.08	27.00	38.20	38.00	18.26	58.13	19.94	45.75	122
0.18	35.18	58.78	39.53	-0.37	117.94	59.16	55.16	22.50	31.54	33.00	16.88	46.21	14.67	41.00	89.47	127.80	110.09	59.48	196.13	68.32	134.77	23.00	33.30	38.00	18.03	48.58	15.27	45.00	79
0.32	32.64	59.02	38.98	-4.14	122.18	63.16	53.80	24.00	31.42	32.00	13.78	49.06	17.64	40.00	112.97	163.55	146.91	89.82	237.28	73.73	193.02	27.00	34.41	34.00	16.11	52.72	18.30	44.00	135


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	16.02
orig_ge	10.43
adv_pp	33.27
adv_ge	10.88


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.36	-0.16	-0.15	-0.48	0.17	0.32	0.06	0.05	0.21	0.23	-0.08	0.50	0.29	0.41	0.04	0.16	0.17	-0.06	0.38	0.22	0.31	733
0.03	-0.50	-0.32	-0.30	-0.60	-0.04	0.28	-0.10	-0.11	0.05	0.09	-0.24	0.34	0.29	0.25	-0.07	0.04	0.07	-0.18	0.26	0.22	0.19	334
0.06	-0.55	-0.39	-0.42	-0.63	-0.15	0.24	-0.20	-0.15	-0.02	-0.02	-0.24	0.19	0.22	0.10	-0.10	-0.01	-0.01	-0.17	0.14	0.16	0.07	243
0.11	-0.62	-0.45	-0.46	-0.67	-0.23	0.22	-0.29	-0.18	-0.06	-0.05	-0.25	0.13	0.19	0.07	-0.13	-0.04	-0.03	-0.18	0.10	0.14	0.05	210
0.15	-0.57	-0.44	-0.44	-0.65	-0.23	0.21	-0.29	-0.22	-0.11	-0.11	-0.27	0.04	0.16	-0.01	-0.15	-0.08	-0.08	-0.19	0.04	0.11	-0.00	122
0.18	-0.67	-0.56	-0.57	-0.74	-0.38	0.18	-0.44	-0.33	-0.20	-0.17	-0.41	0.00	0.21	-0.09	-0.24	-0.14	-0.12	-0.30	0.01	0.15	-0.05	79
0.32	-0.74	-0.62	-0.63	-0.80	-0.45	0.18	-0.52	-0.37	-0.28	-0.25	-0.47	-0.08	0.20	-0.17	-0.27	-0.20	-0.17	-0.34	-0.05	0.15	-0.11	135


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/correlations_auc.tex <==
name	auc
pcc	-0.15
spearman	-0.04
kendall	-0.03


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	15.23	22.45	20.69	11.88	33.01	10.56	26.82	13.16	24.14	21.60	9.36	38.92	14.78	31.64	4.85	14.05	10.85	2.37	25.72	11.67	19.15	733
0.03	10.97	16.39	14.39	7.35	25.44	9.04	19.14	9.38	18.11	14.41	4.69	31.53	13.42	21.36	3.71	10.46	7.64	1.17	19.76	9.29	13.55	334
0.06	8.66	11.99	11.68	7.60	16.37	4.38	14.22	7.41	12.42	10.87	4.48	20.37	7.95	15.60	3.11	7.08	4.82	-0.12	14.28	7.20	8.58	243
0.11	6.95	9.17	9.21	6.35	11.99	2.82	11.09	5.86	8.93	7.84	4.36	13.50	4.57	10.68	2.73	4.85	3.71	1.74	7.96	3.11	5.91	210
0.15	5.63	7.47	7.43	5.10	9.84	2.37	9.15	4.82	7.21	6.48	3.96	10.46	3.25	8.81	2.41	4.09	3.45	1.81	6.37	2.28	5.31	122
0.18	5.37	6.78	6.80	4.83	8.72	1.95	8.21	4.20	6.94	6.22	2.87	11.00	4.06	7.75	2.45	3.99	3.40	0.72	7.25	3.26	4.61	79
0.32	4.87	6.22	6.32	4.53	7.91	1.69	7.06	4.20	5.59	5.30	3.44	7.74	2.15	6.48	2.25	2.93	2.67	1.76	4.11	1.17	3.20	135


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/ets_sts_auc.tex <==
name	auc
et_use	2.80
et_tse	2.83
et_ce	1.59


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	3.70	8.48	5.13	-10.87	27.83	19.35	7.52	9.41	14.40	12.47	6.36	22.43	8.04	17.29	7.48	12.98	10.23	2.98	22.98	10.00	15.54	733
0.03	2.12	3.61	2.95	0.81	6.40	2.80	4.11	7.67	10.58	9.31	5.84	15.32	4.74	11.98	6.00	9.06	7.69	3.74	14.38	5.32	10.01	334
0.06	1.28	1.96	1.57	0.57	3.35	1.39	2.18	6.37	8.02	7.75	5.42	10.63	2.60	8.66	5.31	6.73	6.31	4.02	9.44	2.71	7.18	243
0.11	0.81	1.14	1.02	0.50	1.78	0.64	1.27	5.62	6.74	6.61	4.75	8.74	1.99	7.61	4.51	5.66	5.33	3.34	7.98	2.32	6.28	210
0.15	0.50	0.89	0.57	-0.15	1.93	1.04	0.79	4.47	5.56	5.39	4.19	6.94	1.37	6.34	3.64	4.60	4.46	3.09	6.11	1.51	5.16	122
0.18	0.41	0.68	0.51	-0.07	1.43	0.75	0.67	4.86	5.55	5.31	3.92	7.18	1.63	5.83	3.79	4.59	4.31	3.02	6.16	1.57	5.07	79
0.32	0.26	0.47	0.32	-0.02	0.97	0.50	0.45	4.17	5.03	4.71	3.50	6.57	1.54	5.45	3.34	4.33	3.86	1.86	6.79	2.47	4.57	135


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.43
et_p_h	2.05
et_p_l2	1.74


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.11	0.11	0.06	0.17	0.05	0.14	0.04	0.06	0.06	0.03	0.08	0.03	0.07	0.04	0.05	0.05	0.03	0.06	0.02	0.06	733
0.03	0.17	0.23	0.22	0.14	0.32	0.09	0.28	0.07	0.08	0.08	0.06	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	334
0.06	0.33	0.43	0.42	0.27	0.59	0.16	0.53	0.10	0.11	0.11	0.08	0.14	0.03	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.10	243
0.11	0.57	0.73	0.75	0.49	0.98	0.25	0.87	0.12	0.14	0.14	0.10	0.18	0.04	0.16	0.10	0.11	0.11	0.09	0.14	0.02	0.12	210
0.15	0.95	1.14	1.17	0.75	1.52	0.38	1.40	0.14	0.16	0.16	0.13	0.20	0.03	0.18	0.12	0.13	0.13	0.11	0.15	0.02	0.15	122
0.18	1.22	1.51	1.53	0.97	2.06	0.54	1.87	0.15	0.18	0.18	0.14	0.22	0.04	0.20	0.13	0.15	0.15	0.12	0.17	0.02	0.16	79
0.32	1.78	2.50	2.43	1.37	3.63	1.13	3.17	0.17	0.21	0.21	0.15	0.26	0.05	0.24	0.15	0.17	0.17	0.14	0.20	0.03	0.19	135


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.40
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.94	0.99	0.03	0.98	0.88	0.92	0.95	0.85	0.99	0.07	0.97	733
0.03	0.95	0.95	0.96	0.92	0.98	0.03	0.96	0.94	0.95	0.96	0.91	0.98	0.04	0.97	0.82	0.88	0.91	0.79	0.97	0.09	0.95	334
0.06	0.93	0.93	0.94	0.91	0.96	0.03	0.95	0.91	0.92	0.94	0.88	0.97	0.04	0.95	0.77	0.84	0.85	0.75	0.93	0.09	0.92	243
0.11	0.90	0.91	0.92	0.88	0.95	0.04	0.94	0.88	0.90	0.91	0.86	0.95	0.04	0.93	0.74	0.80	0.80	0.71	0.90	0.09	0.88	210
0.15	0.87	0.89	0.90	0.85	0.93	0.04	0.92	0.87	0.88	0.89	0.84	0.93	0.05	0.91	0.71	0.78	0.79	0.68	0.88	0.10	0.86	122
0.18	0.85	0.88	0.89	0.83	0.92	0.04	0.90	0.83	0.86	0.87	0.81	0.92	0.06	0.90	0.68	0.75	0.76	0.64	0.86	0.11	0.84	79
0.32	0.84	0.86	0.87	0.81	0.90	0.04	0.89	0.81	0.84	0.84	0.79	0.89	0.05	0.88	0.65	0.69	0.70	0.60	0.79	0.09	0.76	135


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.27
sts_ce	0.24


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	64.50	152.03	110.69	-32.41	336.48	184.45	170.47	0.18	8.30	0.94	-10.43	27.02	18.72	11.42	6.19	18.29	13.93	2.37	34.21	15.92	26.45	733
0.03	208.29	569.09	312.97	-15.48	1153.66	584.57	672.99	0.22	12.29	1.01	-24.90	49.49	37.19	12.48	7.66	19.87	14.10	1.53	38.21	18.34	27.47	334
0.06	373.51	875.64	765.49	277.96	1473.33	597.69	1156.76	0.36	10.99	2.05	-14.28	36.26	25.27	11.96	7.66	23.14	15.92	0.46	45.81	22.67	32.56	243
0.11	481.24	883.25	746.76	325.10	1441.40	558.15	1136.37	0.39	25.43	8.18	-78.63	129.48	104.05	23.38	7.01	20.58	15.23	1.13	40.03	19.45	27.40	210
0.15	583.06	883.80	771.54	367.89	1399.71	515.91	1029.74	0.42	9.56	2.29	-7.00	26.12	16.56	12.16	6.85	21.48	16.27	-2.36	45.32	23.84	27.92	122
0.18	352.47	701.05	676.84	227.11	1174.99	473.94	848.76	0.20	16.44	1.05	-42.73	75.61	59.17	15.51	6.77	21.62	14.24	-4.60	47.84	26.22	28.26	79
0.32	378.60	585.42	579.24	236.49	934.36	348.93	792.57	0.14	7.38	0.39	-3.55	18.31	10.93	12.70	5.72	18.31	14.25	2.69	33.93	15.62	24.41	135


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/time_misc_auc.tex <==
name	auc
attack_time	222.97
l2	4.23
lom	6.42


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.15	0.25	0.23	0.11	0.40	0.14	0.35	0.34	0.44	0.44	0.29	0.58	0.14	0.53	0.53	0.60	0.60	0.48	0.71	0.11	0.67	733
0.03	0.09	0.19	0.17	0.06	0.31	0.12	0.27	0.28	0.36	0.37	0.23	0.50	0.14	0.46	0.47	0.54	0.55	0.42	0.65	0.12	0.61	334
0.06	0.07	0.14	0.13	0.04	0.24	0.10	0.18	0.27	0.32	0.32	0.22	0.43	0.11	0.38	0.46	0.51	0.51	0.42	0.59	0.09	0.55	243
0.11	0.06	0.12	0.12	0.04	0.20	0.08	0.17	0.25	0.31	0.30	0.22	0.39	0.09	0.37	0.45	0.50	0.50	0.42	0.58	0.08	0.55	210
0.15	0.03	0.10	0.09	0.02	0.18	0.08	0.14	0.22	0.28	0.29	0.20	0.37	0.08	0.32	0.43	0.48	0.48	0.41	0.55	0.07	0.52	122
0.18	0.00	0.07	0.07	0.00	0.14	0.07	0.11	0.17	0.24	0.25	0.13	0.34	0.10	0.31	0.38	0.44	0.47	0.36	0.53	0.09	0.49	79
0.32	0.00	0.06	0.06	-0.00	0.13	0.07	0.10	0.18	0.21	0.23	0.12	0.31	0.10	0.29	0.38	0.42	0.43	0.34	0.51	0.09	0.48	135


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.09
top50	0.15


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	31.86	43.48	39.56	23.70	63.25	19.77	50.43	29.00	36.28	35.00	23.87	48.68	12.41	42.00	35.85	48.22	43.93	27.53	68.92	20.70	55.85	29.00	36.36	36.00	23.99	48.72	12.37	42.00	899
0.03	31.63	43.83	39.89	22.50	65.17	21.34	50.02	28.00	35.09	35.00	22.91	47.28	12.19	42.00	39.75	53.88	48.54	29.58	78.18	24.30	61.56	28.00	35.26	36.00	23.07	47.46	12.19	43.00	780
0.06	32.41	44.20	39.53	17.92	70.48	26.28	48.66	29.00	35.32	36.00	23.47	47.16	11.85	41.00	47.18	62.28	55.97	29.77	94.79	32.51	68.87	29.00	35.75	36.00	23.76	47.74	11.99	42.00	790
0.11	34.25	47.45	40.52	15.21	79.68	32.23	52.11	27.00	33.61	33.00	19.14	48.07	14.46	40.00	58.56	81.86	69.95	1.69	162.03	80.17	90.44	26.00	34.44	34.00	19.87	49.00	14.56	42.00	557
0.15	32.05	56.30	41.93	2.05	110.54	54.24	57.32	18.75	31.03	31.00	15.10	46.96	15.93	40.00	79.82	127.46	97.87	-10.71	265.64	138.18	112.50	19.00	32.74	35.00	16.44	49.03	16.29	43.25	172
0.18	30.55	57.15	36.69	-6.25	120.55	63.40	51.61	16.00	28.88	31.00	10.29	47.46	18.58	36.00	82.77	150.53	101.85	-32.42	333.48	182.95	138.03	19.25	30.54	30.00	12.08	49.00	18.46	39.00	72
0.32	33.91	99.30	48.24	-15.71	214.32	115.01	105.49	6.00	27.46	31.00	1.94	52.97	25.51	37.75	118.01	319.78	159.05	-79.20	718.76	398.98	253.11	7.00	29.24	29.00	3.75	54.73	25.49	42.50	70


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/comparison_vals_auc.tex <==
name	auc
orig_pp	19.16
orig_ge	9.64
adv_pp	47.35
adv_ge	10.03


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.06	0.24	0.16	0.00	0.47	0.23	0.36	0.26	0.44	0.43	0.20	0.69	0.25	0.64	0.18	0.33	0.31	0.13	0.52	0.20	0.46	899
0.03	0.01	0.11	0.07	-0.05	0.27	0.16	0.17	0.13	0.31	0.29	0.07	0.54	0.23	0.48	0.09	0.22	0.20	0.05	0.39	0.17	0.33	780
0.06	-0.03	0.02	-0.00	-0.07	0.12	0.09	0.05	0.03	0.17	0.15	-0.03	0.37	0.20	0.29	0.02	0.12	0.10	-0.02	0.26	0.14	0.20	790
0.11	-0.04	0.01	-0.01	-0.08	0.10	0.09	0.04	0.01	0.15	0.13	-0.05	0.34	0.20	0.27	0.01	0.10	0.09	-0.04	0.24	0.14	0.19	557
0.15	-0.04	-0.01	-0.01	-0.09	0.07	0.08	0.03	-0.08	0.12	0.11	-0.10	0.34	0.22	0.31	-0.04	0.08	0.08	-0.07	0.24	0.15	0.20	172
0.18	-0.05	-0.00	0.00	-0.09	0.08	0.08	0.03	0.09	0.19	0.18	-0.02	0.39	0.20	0.31	0.06	0.13	0.11	-0.02	0.27	0.14	0.21	72
0.32	-0.11	-0.07	-0.05	-0.19	0.06	0.13	-0.00	-0.08	0.05	0.02	-0.17	0.27	0.22	0.23	-0.05	0.03	0.02	-0.12	0.18	0.15	0.15	70


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/correlations_auc.tex <==
name	auc
pcc	0.00
spearman	0.05
kendall	0.03


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	10.59	14.74	14.44	8.08	21.40	6.66	18.43	9.49	16.90	15.81	7.35	26.45	9.55	22.68	3.46	9.54	7.56	1.39	17.69	8.15	12.73	899
0.03	7.91	10.19	9.90	6.56	13.82	3.63	12.36	7.40	11.71	10.41	5.33	18.09	6.38	14.84	2.80	6.96	5.52	1.57	12.34	5.39	9.47	780
0.06	6.46	8.09	8.13	5.46	10.72	2.63	9.74	5.52	8.70	7.83	3.08	14.31	5.61	10.35	2.21	4.58	3.26	1.12	8.04	3.46	6.11	790
0.11	5.12	6.27	6.43	4.57	7.96	1.69	7.44	4.59	6.45	5.73	2.75	10.15	3.70	7.56	2.00	3.90	2.88	1.01	6.79	2.89	4.98	557
0.15	4.11	5.21	5.10	3.78	6.63	1.43	6.09	3.74	5.00	4.39	2.88	7.12	2.12	5.80	2.00	4.11	2.55	-3.28	11.51	7.40	3.58	172
0.18	3.71	4.55	4.60	3.24	5.85	1.31	5.48	3.12	4.67	3.93	2.47	6.87	2.20	5.87	1.86	2.66	2.25	1.13	4.18	1.53	2.89	72
0.32	2.97	3.83	3.72	2.57	5.09	1.26	4.53	2.75	3.37	3.32	2.24	4.50	1.13	3.63	1.78	3.67	2.27	-2.12	9.47	5.80	3.30	70


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/ets_sts_auc.tex <==
name	auc
et_use	1.85
et_tse	1.91
et_ce	1.26


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.48	4.64	3.45	-2.72	12.01	7.36	4.78	6.03	8.65	7.92	3.72	13.57	4.93	10.22	4.66	7.66	6.41	1.74	13.58	5.92	9.07	899
0.03	1.49	2.21	1.93	0.67	3.76	1.54	2.51	5.24	6.78	6.40	3.29	10.27	3.49	7.84	4.08	5.78	5.14	0.77	10.80	5.01	6.35	780
0.06	0.95	1.28	1.14	0.65	1.91	0.63	1.47	4.61	5.56	5.28	3.75	7.38	1.82	6.20	3.66	4.63	4.25	2.50	6.75	2.12	5.12	790
0.11	0.57	0.85	0.69	-1.30	3.00	2.15	0.83	3.80	4.34	4.18	3.37	5.32	0.98	4.77	2.94	3.56	3.39	2.49	4.63	1.07	3.91	557
0.15	0.32	0.44	0.41	0.24	0.64	0.20	0.48	3.15	3.69	3.55	2.93	4.45	0.76	3.93	2.53	3.10	2.80	2.03	4.16	1.06	3.25	172
0.18	0.24	0.36	0.28	0.08	0.63	0.27	0.33	2.87	3.33	3.20	2.65	4.02	0.68	3.50	2.32	2.75	2.53	2.01	3.48	0.73	3.22	72
0.32	0.16	0.36	0.22	-0.10	0.81	0.45	0.32	2.70	3.31	3.07	2.33	4.30	0.98	3.62	2.13	2.84	2.58	1.46	4.23	1.39	2.99	70


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.26
et_p_h	1.32
et_p_l2	1.11


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.12	0.11	0.07	0.16	0.05	0.15	0.04	0.06	0.06	0.04	0.09	0.02	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.06	899
0.03	0.18	0.24	0.24	0.15	0.33	0.09	0.29	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.06	0.07	0.07	0.05	0.09	0.02	0.08	780
0.06	0.33	0.44	0.43	0.29	0.58	0.14	0.51	0.09	0.12	0.11	0.08	0.15	0.03	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.11	790
0.11	0.60	0.74	0.71	0.49	0.99	0.25	0.86	0.13	0.15	0.15	0.11	0.18	0.03	0.17	0.11	0.12	0.12	0.10	0.14	0.02	0.13	557
0.15	1.07	1.29	1.25	0.89	1.69	0.40	1.58	0.15	0.18	0.17	0.13	0.22	0.04	0.20	0.13	0.14	0.14	0.12	0.17	0.03	0.16	172
0.18	1.45	1.75	1.76	1.15	2.36	0.61	2.11	0.16	0.19	0.19	0.15	0.23	0.04	0.22	0.14	0.15	0.16	0.13	0.18	0.02	0.17	72
0.32	1.62	2.55	2.45	1.14	3.96	1.41	3.25	0.18	0.21	0.21	0.15	0.26	0.06	0.23	0.15	0.17	0.17	0.13	0.21	0.04	0.18	70


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.43
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.95	0.99	0.02	0.98	0.97	0.97	0.98	0.94	1.00	0.03	0.98	0.91	0.92	0.95	0.85	1.00	0.07	0.97	899
0.03	0.95	0.95	0.95	0.93	0.97	0.02	0.96	0.94	0.95	0.96	0.92	0.98	0.03	0.97	0.84	0.89	0.92	0.81	0.97	0.08	0.95	780
0.06	0.93	0.93	0.94	0.88	0.98	0.05	0.95	0.91	0.92	0.94	0.87	0.98	0.05	0.95	0.78	0.83	0.85	0.72	0.95	0.11	0.92	790
0.11	0.90	0.91	0.92	0.88	0.95	0.03	0.93	0.89	0.91	0.92	0.87	0.95	0.04	0.93	0.76	0.82	0.83	0.73	0.91	0.09	0.90	557
0.15	0.88	0.89	0.90	0.85	0.93	0.04	0.92	0.87	0.88	0.88	0.84	0.93	0.04	0.91	0.76	0.79	0.81	0.70	0.89	0.09	0.85	172
0.18	0.86	0.88	0.89	0.83	0.93	0.05	0.91	0.84	0.87	0.87	0.82	0.92	0.05	0.91	0.74	0.77	0.78	0.68	0.86	0.09	0.83	72
0.32	0.82	0.84	0.85	0.78	0.91	0.07	0.89	0.80	0.83	0.84	0.78	0.88	0.05	0.86	0.72	0.77	0.78	0.65	0.88	0.12	0.84	70


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.28
sts_tse	0.27
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	37.20	70.01	50.18	-9.87	149.90	79.89	71.07	10.06	78.38	21.59	-258.37	415.14	336.76	45.94	12.92	35.36	28.19	6.56	64.16	28.80	50.62	899
0.03	73.38	220.99	137.46	12.08	429.90	208.91	302.08	16.97	110.84	32.27	-508.22	729.90	619.06	63.10	13.25	38.03	29.56	7.00	69.07	31.04	54.71	780
0.06	242.82	416.54	451.01	201.09	631.99	215.45	534.11	28.69	167.96	49.44	-413.52	749.44	581.48	101.99	15.67	42.88	33.28	7.63	78.12	35.24	59.57	790
0.11	249.50	424.32	451.06	205.96	642.67	218.36	537.88	29.64	238.68	54.56	-1151.09	1628.45	1389.77	114.39	16.54	41.56	36.79	10.21	72.90	31.34	61.47	557
0.15	193.72	395.55	434.58	168.73	622.37	226.82	540.34	38.12	421.77	74.32	-1151.10	1994.64	1572.87	181.46	10.25	34.73	25.61	4.29	65.18	30.45	55.51	172
0.18	181.08	370.99	347.47	125.74	616.25	245.26	576.72	40.31	1159.24	91.79	-2174.37	4492.85	3333.61	325.83	8.72	41.27	38.86	8.45	74.10	32.82	69.90	72
0.32	55.08	291.30	305.39	53.03	529.57	238.27	484.55	24.80	679.97	113.98	-2917.07	4277.01	3597.04	351.40	2.23	23.14	16.01	-2.09	48.37	25.23	38.32	70


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/time_misc_auc.tex <==
name	auc
attack_time	108.03
l2	181.95
lom	11.26


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.12	0.27	0.22	0.08	0.46	0.19	0.38	0.38	0.49	0.48	0.34	0.64	0.15	0.59	0.58	0.66	0.65	0.56	0.77	0.10	0.73	899
0.03	0.06	0.17	0.13	0.03	0.32	0.15	0.23	0.32	0.42	0.39	0.28	0.55	0.13	0.51	0.55	0.61	0.60	0.52	0.70	0.09	0.67	780
0.06	0.03	0.10	0.07	0.00	0.19	0.09	0.14	0.26	0.35	0.33	0.24	0.45	0.11	0.40	0.51	0.56	0.56	0.48	0.64	0.08	0.61	790
0.11	0.03	0.09	0.07	-0.00	0.18	0.09	0.14	0.27	0.34	0.33	0.24	0.44	0.10	0.40	0.50	0.55	0.55	0.48	0.63	0.08	0.60	557
0.15	0.03	0.08	0.06	-0.00	0.17	0.08	0.11	0.24	0.34	0.33	0.21	0.46	0.12	0.42	0.48	0.54	0.55	0.46	0.63	0.09	0.60	172
0.18	0.00	0.09	0.07	0.01	0.17	0.08	0.14	0.27	0.36	0.33	0.25	0.47	0.11	0.43	0.52	0.57	0.59	0.49	0.65	0.08	0.61	72
0.32	0.00	0.06	0.03	-0.02	0.14	0.08	0.10	0.25	0.30	0.29	0.20	0.40	0.10	0.38	0.44	0.50	0.52	0.40	0.60	0.10	0.56	70


==> data/mlm_plots/mlm_distil_fast/fakenews/xlnet/s/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.11
top50	0.17


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	49.79	68.90	63.45	41.29	96.50	27.61	83.95	33.00	40.72	41.00	30.25	51.18	10.46	48.00	52.46	72.95	67.16	44.24	101.66	28.71	86.64	33.00	40.40	40.00	29.96	50.84	10.44	48.00	960
0.03	49.68	69.55	63.18	40.06	99.04	29.49	84.22	31.00	38.87	39.00	26.86	50.88	12.01	47.00	58.36	80.08	72.80	47.52	112.65	32.57	94.83	30.00	38.33	39.00	26.46	50.19	11.87	47.00	988
0.06	49.77	69.83	63.33	40.13	99.53	29.70	84.81	31.00	38.92	39.00	26.67	51.16	12.24	47.00	68.76	93.61	86.21	56.80	130.43	36.82	109.87	30.00	38.06	39.00	26.03	50.08	12.02	46.00	1004
0.11	49.70	69.96	64.01	40.53	99.39	29.43	84.86	30.00	38.77	39.00	26.48	51.05	12.29	47.00	80.72	109.75	101.88	67.97	151.52	41.77	131.19	29.00	37.50	38.00	25.55	49.45	11.95	46.00	1063
0.15	49.73	69.99	63.04	40.06	99.91	29.92	84.82	31.00	38.85	39.00	26.12	51.58	12.73	47.00	105.34	140.33	131.45	90.62	190.04	49.71	166.46	30.00	37.33	38.00	24.90	49.77	12.43	46.00	1061
0.18	49.44	69.41	62.96	39.59	99.23	29.82	83.89	31.00	39.07	39.00	26.80	51.34	12.27	48.00	130.95	171.92	162.32	114.56	229.27	57.36	201.36	29.00	36.99	37.00	25.02	48.96	11.97	45.00	1026
0.32	50.06	70.16	63.34	40.20	100.13	29.97	84.78	31.00	38.88	39.00	26.91	50.86	11.98	47.00	184.43	247.61	229.95	159.11	336.11	88.50	297.26	28.00	35.90	36.00	24.26	47.55	11.65	44.00	1812


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/comparison_vals_auc.tex <==
name	auc
orig_pp	21.66
orig_ge	12.10
adv_pp	48.16
adv_ge	11.56


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.01	0.21	0.04	-0.08	0.50	0.29	0.45	0.58	0.68	0.69	0.52	0.84	0.16	0.80	0.42	0.54	0.52	0.37	0.70	0.17	0.64	960
0.03	-0.01	0.11	-0.00	-0.11	0.34	0.23	0.12	0.50	0.62	0.64	0.45	0.80	0.17	0.75	0.36	0.48	0.48	0.32	0.65	0.17	0.60	988
0.06	-0.02	0.04	-0.01	-0.11	0.19	0.15	0.01	0.41	0.55	0.57	0.36	0.74	0.19	0.70	0.29	0.42	0.42	0.25	0.58	0.16	0.55	1004
0.11	-0.03	0.00	-0.02	-0.11	0.11	0.11	-0.01	0.36	0.50	0.54	0.30	0.71	0.20	0.67	0.25	0.38	0.39	0.21	0.55	0.17	0.51	1063
0.15	-0.07	-0.04	-0.02	-0.12	0.05	0.08	-0.02	0.30	0.44	0.50	0.22	0.66	0.22	0.61	0.21	0.33	0.36	0.16	0.51	0.17	0.47	1061
0.18	-0.11	-0.06	-0.03	-0.15	0.02	0.08	-0.02	0.25	0.39	0.45	0.15	0.63	0.24	0.57	0.17	0.29	0.33	0.11	0.47	0.18	0.43	1026
0.32	-0.15	-0.10	-0.05	-0.22	0.01	0.11	-0.03	0.18	0.30	0.38	0.03	0.58	0.28	0.50	0.12	0.22	0.28	0.02	0.42	0.20	0.37	1812


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/correlations_auc.tex <==
name	auc
pcc	-0.01
spearman	0.14
kendall	0.10


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	6.65	11.54	10.68	4.92	18.17	6.62	15.14	5.59	11.44	9.92	3.53	19.35	7.91	14.70	4.55	10.91	8.02	1.62	20.20	9.29	13.74	960
0.03	5.26	7.25	7.03	4.01	10.50	3.24	8.73	4.55	7.16	6.47	3.02	11.30	4.14	8.76	3.69	7.60	5.86	1.24	13.97	6.36	8.96	988
0.06	4.17	5.19	5.08	3.49	6.88	1.70	6.13	3.52	5.03	4.67	2.70	7.36	2.33	6.03	2.89	5.35	4.29	1.07	9.63	4.28	6.12	1004
0.11	3.60	4.40	4.33	3.20	5.60	1.20	5.10	2.99	4.11	3.79	2.38	5.84	1.73	4.82	2.55	4.25	3.43	1.03	7.46	3.22	4.80	1063
0.15	3.11	3.70	3.67	2.83	4.57	0.87	4.31	2.59	3.38	3.21	2.22	4.53	1.16	3.90	2.25	3.37	2.92	1.07	5.66	2.29	3.81	1061
0.18	2.80	3.33	3.31	2.55	4.12	0.79	3.84	2.39	3.03	2.86	2.07	3.99	0.96	3.48	2.07	2.95	2.64	1.00	4.90	1.95	3.32	1026
0.32	2.48	2.98	2.97	2.27	3.69	0.71	3.45	2.15	2.70	2.56	1.89	3.52	0.81	3.08	1.85	2.48	2.33	1.40	3.56	1.08	2.86	1812


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/ets_sts_auc.tex <==
name	auc
et_use	1.33
et_tse	1.25
et_ce	1.25


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	3.29	14.09	5.72	-16.50	44.68	30.59	11.92	8.11	14.35	11.67	4.49	24.21	9.86	17.86	6.96	14.33	10.97	3.12	25.53	11.20	18.14	960
0.03	1.84	6.41	2.81	-12.13	24.95	18.54	4.76	6.49	9.17	8.47	4.58	13.77	4.60	10.88	5.45	8.83	7.53	3.23	14.42	5.60	10.83	988
0.06	1.01	2.35	1.34	-8.43	13.14	10.78	1.92	5.19	6.49	6.15	4.07	8.90	2.42	7.34	4.32	5.98	5.28	2.52	9.44	3.46	6.81	1004
0.11	0.64	1.21	0.85	-5.13	7.54	6.34	1.16	4.46	5.33	5.11	3.80	6.87	1.53	5.97	3.70	4.82	4.40	2.55	7.09	2.27	5.47	1063
0.15	0.39	0.59	0.49	-0.22	1.40	0.81	0.64	3.75	4.35	4.25	3.38	5.33	0.98	4.77	3.09	3.87	3.64	2.56	5.18	1.31	4.30	1061
0.18	0.27	0.38	0.35	0.20	0.56	0.18	0.44	3.37	3.87	3.79	3.12	4.63	0.76	4.24	2.81	3.40	3.25	2.43	4.38	0.98	3.77	1026
0.32	0.16	0.24	0.22	0.11	0.37	0.13	0.28	2.97	3.44	3.33	2.76	4.12	0.68	3.76	2.50	3.03	2.88	2.21	3.84	0.81	3.36	1812


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.52
et_p_h	1.60
et_p_l2	1.46


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.03	0.08	0.07	0.02	0.14	0.06	0.11	0.02	0.04	0.03	0.02	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.04	960
0.03	0.09	0.17	0.16	0.07	0.28	0.11	0.24	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.06	0.05	0.04	0.07	0.02	0.07	988
0.06	0.26	0.37	0.36	0.19	0.54	0.18	0.47	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.07	0.08	0.08	0.06	0.10	0.02	0.09	1004
0.11	0.44	0.61	0.59	0.35	0.87	0.26	0.75	0.09	0.12	0.11	0.08	0.15	0.03	0.13	0.09	0.10	0.10	0.08	0.12	0.02	0.11	1063
0.15	0.82	1.09	1.06	0.66	1.53	0.43	1.32	0.12	0.14	0.14	0.11	0.18	0.04	0.17	0.11	0.12	0.12	0.10	0.15	0.02	0.14	1061
0.18	1.22	1.61	1.54	1.03	2.19	0.58	1.94	0.14	0.17	0.16	0.13	0.20	0.04	0.19	0.13	0.14	0.14	0.12	0.16	0.02	0.16	1026
0.32	1.92	2.78	2.54	1.57	3.98	1.20	3.43	0.16	0.19	0.19	0.15	0.23	0.04	0.22	0.15	0.16	0.16	0.14	0.19	0.03	0.18	1812


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.95	0.96	0.96	0.95	0.97	0.01	0.97	0.95	0.96	0.96	0.93	0.98	0.02	0.97	0.93	0.95	0.95	0.91	0.98	0.03	0.97	960
0.03	0.92	0.93	0.93	0.91	0.95	0.02	0.95	0.91	0.92	0.93	0.89	0.96	0.04	0.95	0.89	0.91	0.92	0.86	0.97	0.05	0.95	988
0.06	0.89	0.90	0.90	0.87	0.93	0.03	0.92	0.87	0.89	0.90	0.84	0.93	0.04	0.92	0.84	0.88	0.89	0.81	0.94	0.07	0.92	1004
0.11	0.86	0.88	0.88	0.84	0.91	0.03	0.90	0.84	0.86	0.87	0.81	0.91	0.05	0.90	0.80	0.84	0.85	0.77	0.92	0.08	0.89	1063
0.15	0.83	0.85	0.86	0.81	0.89	0.04	0.88	0.80	0.83	0.84	0.78	0.88	0.05	0.87	0.77	0.81	0.82	0.72	0.90	0.09	0.86	1061
0.18	0.81	0.83	0.84	0.78	0.88	0.05	0.86	0.78	0.81	0.81	0.75	0.86	0.05	0.85	0.74	0.78	0.80	0.69	0.88	0.10	0.84	1026
0.32	0.78	0.80	0.82	0.75	0.85	0.05	0.84	0.75	0.78	0.79	0.73	0.84	0.06	0.82	0.70	0.75	0.76	0.65	0.84	0.10	0.81	1812


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	9.67	13.17	13.69	8.62	17.72	4.55	15.85	0.08	0.61	0.68	0.20	1.02	0.41	0.96	4.82	26.40	16.41	-1.05	53.85	27.45	39.82	960
0.03	9.43	12.25	11.85	7.96	16.53	4.28	14.32	0.46	0.69	0.78	0.31	1.07	0.38	0.98	6.70	28.73	20.10	0.89	56.58	27.84	41.86	988
0.06	10.06	13.44	12.77	7.53	19.35	5.91	15.40	0.52	0.70	0.76	0.36	1.04	0.34	0.99	7.35	29.64	21.39	1.92	57.36	27.72	43.82	1004
0.11	13.37	20.65	16.91	5.53	35.77	15.12	21.98	0.52	0.69	0.72	0.37	1.00	0.31	0.95	8.78	30.05	23.55	3.42	56.69	26.63	43.07	1063
0.15	18.64	28.36	23.96	12.25	44.47	16.11	33.03	0.49	0.64	0.65	0.35	0.93	0.29	0.87	8.27	27.95	21.30	3.00	52.89	24.94	41.24	1061
0.18	29.89	43.29	38.54	23.15	63.43	20.14	53.39	0.45	0.60	0.59	0.32	0.88	0.28	0.81	9.07	27.94	21.69	3.60	52.28	24.34	40.20	1026
0.32	38.53	58.11	53.52	31.95	84.27	26.16	73.60	0.39	0.55	0.52	0.28	0.82	0.27	0.73	9.05	26.20	20.05	3.81	48.59	22.39	38.19	1812


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/time_misc_auc.tex <==
name	auc
attack_time	10.61
l2	0.19
lom	8.72


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.38	0.54	0.56	0.33	0.76	0.21	0.71	0.61	0.70	0.71	0.56	0.84	0.14	0.80	0.71	0.77	0.77	0.68	0.86	0.09	0.83	960
0.03	0.30	0.48	0.50	0.27	0.70	0.22	0.67	0.56	0.67	0.68	0.53	0.81	0.14	0.78	0.68	0.74	0.75	0.65	0.84	0.09	0.81	988
0.06	0.25	0.42	0.43	0.22	0.63	0.20	0.58	0.52	0.63	0.65	0.48	0.77	0.14	0.74	0.64	0.71	0.72	0.62	0.81	0.09	0.79	1004
0.11	0.22	0.38	0.40	0.18	0.58	0.20	0.55	0.49	0.60	0.63	0.45	0.75	0.15	0.72	0.63	0.70	0.70	0.60	0.79	0.10	0.77	1063
0.15	0.19	0.33	0.33	0.14	0.51	0.19	0.47	0.46	0.57	0.60	0.41	0.72	0.15	0.68	0.60	0.67	0.68	0.57	0.77	0.10	0.75	1061
0.18	0.14	0.29	0.29	0.12	0.47	0.18	0.43	0.43	0.54	0.57	0.38	0.69	0.16	0.66	0.58	0.65	0.66	0.54	0.75	0.10	0.73	1026
0.32	0.10	0.23	0.21	0.07	0.40	0.17	0.35	0.39	0.49	0.53	0.33	0.65	0.16	0.62	0.56	0.62	0.64	0.50	0.73	0.12	0.70	1812


==> data/mlm_plots/mlm_distil_fast/imdb/bert/a/top_intersections_auc.tex <==
name	auc
top10	0.10
top30	0.18
top50	0.21


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	49.84	68.72	63.27	41.13	96.31	27.59	82.33	33.00	40.67	41.00	30.31	51.03	10.36	48.00	52.94	72.71	66.40	43.98	101.43	28.72	87.34	33.00	40.34	40.00	30.01	50.68	10.34	48.00	954
0.03	49.47	69.66	63.03	39.70	99.62	29.96	84.26	31.00	39.07	39.50	26.92	51.22	12.15	47.00	57.42	80.19	72.61	47.20	113.18	32.99	96.20	31.00	38.53	39.00	26.44	50.61	12.09	47.00	992
0.06	49.77	69.72	63.55	40.18	99.26	29.54	84.19	31.00	38.94	39.00	26.70	51.19	12.25	47.50	68.32	93.25	85.17	57.14	129.36	36.11	111.38	30.00	38.09	39.00	26.02	50.15	12.07	46.00	1011
0.11	49.77	69.63	63.35	40.33	98.93	29.30	84.11	31.00	38.93	39.00	26.72	51.13	12.20	47.00	80.56	109.12	100.87	67.86	150.38	41.26	130.65	29.00	37.78	38.00	25.78	49.79	12.00	45.50	1039
0.15	48.96	68.68	62.27	38.93	98.44	29.76	82.47	31.00	38.83	39.00	26.72	50.93	12.11	47.00	104.74	138.29	128.06	88.67	187.91	49.62	162.20	29.00	37.40	37.00	25.55	49.25	11.85	45.00	1047
0.18	50.03	70.10	63.35	40.23	99.98	29.88	84.95	31.00	38.90	39.00	26.68	51.13	12.22	47.00	131.11	172.88	159.48	113.08	232.68	59.80	204.12	28.00	36.90	37.00	25.00	48.80	11.90	45.00	1013
0.32	50.20	70.84	64.00	40.77	100.92	30.08	85.66	31.00	38.98	40.00	26.59	51.37	12.39	48.00	183.18	248.19	230.10	157.79	338.58	90.40	298.75	28.00	36.06	36.00	24.20	47.93	11.86	44.00	1718


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	21.70
orig_ge	12.11
adv_pp	48.16
adv_ge	11.58


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.22	-0.01	-0.01	-0.37	0.34	0.35	0.22	-0.05	0.15	0.16	-0.17	0.47	0.32	0.36	-0.03	0.11	0.12	-0.13	0.36	0.24	0.26	954
0.03	-0.39	-0.18	-0.18	-0.51	0.14	0.32	0.01	-0.18	0.03	0.06	-0.27	0.34	0.30	0.24	-0.13	0.03	0.05	-0.20	0.26	0.23	0.18	992
0.06	-0.50	-0.31	-0.31	-0.60	-0.02	0.29	-0.15	-0.26	-0.06	-0.05	-0.35	0.23	0.29	0.15	-0.18	-0.04	-0.03	-0.26	0.18	0.22	0.11	1011
0.11	-0.57	-0.40	-0.40	-0.66	-0.15	0.25	-0.25	-0.30	-0.13	-0.11	-0.39	0.14	0.27	0.07	-0.21	-0.09	-0.07	-0.29	0.11	0.20	0.05	1039
0.15	-0.63	-0.49	-0.49	-0.71	-0.27	0.22	-0.35	-0.36	-0.21	-0.21	-0.45	0.03	0.24	-0.02	-0.26	-0.14	-0.15	-0.32	0.04	0.18	-0.01	1047
0.18	-0.70	-0.56	-0.56	-0.76	-0.36	0.20	-0.45	-0.43	-0.27	-0.26	-0.49	-0.04	0.23	-0.10	-0.30	-0.19	-0.18	-0.36	-0.02	0.17	-0.06	1013
0.32	-0.75	-0.63	-0.64	-0.80	-0.47	0.17	-0.54	-0.49	-0.34	-0.34	-0.54	-0.15	0.20	-0.20	-0.35	-0.24	-0.24	-0.40	-0.09	0.15	-0.14	1718


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/correlations_auc.tex <==
name	auc
pcc	-0.14
spearman	-0.06
kendall	-0.04


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	9.32	15.36	13.51	6.44	24.28	8.92	18.76	8.10	15.29	12.67	4.61	25.96	10.67	18.75	6.39	14.80	10.60	2.11	27.49	12.69	19.26	954
0.03	7.09	10.39	9.31	4.99	15.78	5.39	12.42	6.16	10.29	8.73	3.52	17.06	6.77	12.49	4.87	11.21	7.65	0.67	21.76	10.54	13.18	992
0.06	5.80	7.73	7.28	4.78	10.68	2.95	9.39	4.69	7.49	6.53	3.11	11.88	4.39	9.14	3.97	8.18	5.91	0.62	15.73	7.56	9.54	1011
0.11	5.08	6.63	6.34	4.26	9.00	2.37	7.80	4.19	6.31	5.61	3.07	9.54	3.24	7.57	3.58	6.38	5.04	1.49	11.27	4.89	7.44	1039
0.15	4.63	5.74	5.60	4.08	7.40	1.66	6.73	3.70	5.17	4.77	3.02	7.31	2.14	6.18	3.20	5.09	4.08	1.52	8.66	3.57	5.79	1047
0.18	4.26	5.20	5.20	3.71	6.69	1.49	6.13	3.48	4.68	4.42	2.91	6.45	1.77	5.44	2.85	4.25	3.66	1.61	6.90	2.65	4.89	1013
0.32	3.95	4.70	4.65	3.47	5.94	1.23	5.43	3.23	4.19	3.94	2.77	5.61	1.42	4.84	2.65	3.73	3.39	1.95	5.52	1.79	4.32	1718


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/ets_sts_auc.tex <==
name	auc
et_use	2.00
et_tse	1.87
et_ce	1.85


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	4.69	20.25	7.83	-26.87	67.38	47.12	15.79	10.53	18.54	15.58	7.00	30.07	11.54	23.85	9.07	18.74	14.77	4.38	33.09	14.36	23.69	954
0.03	2.57	8.46	3.73	-18.16	35.07	26.62	6.09	8.21	12.21	10.85	6.18	18.24	6.03	14.65	6.79	11.73	9.68	3.73	19.72	8.00	14.35	992
0.06	1.37	2.68	1.87	-1.91	7.27	4.59	2.61	6.83	8.89	8.35	5.66	12.13	3.24	10.42	5.73	8.10	7.16	3.80	12.40	4.30	9.34	1011
0.11	0.91	1.64	1.19	-1.67	4.94	3.30	1.60	6.08	7.52	7.19	5.29	9.75	2.23	8.66	5.04	6.68	6.16	3.78	9.58	2.90	7.75	1039
0.15	0.56	0.78	0.71	0.39	1.16	0.38	0.88	5.28	6.28	6.10	4.79	7.76	1.48	7.08	4.43	5.52	5.19	3.78	7.27	1.74	6.21	1047
0.18	0.41	0.55	0.51	0.33	0.78	0.22	0.63	5.02	5.77	5.66	4.62	6.92	1.15	6.40	4.19	5.06	4.82	3.69	6.43	1.37	5.63	1013
0.32	0.24	0.36	0.32	0.18	0.54	0.18	0.42	4.53	5.16	5.06	4.22	6.11	0.94	5.67	3.82	4.53	4.36	3.43	5.63	1.10	5.01	1718


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.70
et_p_h	2.26
et_p_l2	2.05


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.03	0.07	0.06	0.02	0.12	0.05	0.10	0.02	0.04	0.03	0.02	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.04	954
0.03	0.10	0.17	0.16	0.07	0.27	0.10	0.23	0.04	0.06	0.06	0.04	0.09	0.03	0.08	0.04	0.06	0.05	0.04	0.07	0.02	0.07	992
0.06	0.26	0.37	0.36	0.20	0.53	0.16	0.47	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.07	0.08	0.08	0.06	0.10	0.02	0.09	1011
0.11	0.45	0.61	0.59	0.36	0.87	0.25	0.76	0.09	0.11	0.11	0.08	0.15	0.03	0.13	0.08	0.10	0.10	0.08	0.12	0.02	0.11	1039
0.15	0.84	1.12	1.05	0.56	1.67	0.55	1.32	0.12	0.14	0.14	0.10	0.18	0.04	0.16	0.11	0.12	0.12	0.10	0.15	0.02	0.13	1047
0.18	1.23	1.59	1.54	1.07	2.10	0.52	1.90	0.14	0.16	0.16	0.13	0.20	0.03	0.18	0.13	0.14	0.14	0.12	0.16	0.02	0.15	1013
0.32	1.92	2.73	2.52	1.58	3.88	1.15	3.34	0.16	0.19	0.19	0.15	0.22	0.04	0.21	0.15	0.16	0.16	0.14	0.19	0.02	0.18	1718


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.95	0.96	0.96	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.93	0.95	0.96	0.91	0.98	0.04	0.97	954
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.92	0.93	0.94	0.90	0.96	0.03	0.95	0.89	0.92	0.93	0.87	0.97	0.05	0.95	992
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.92	0.87	0.89	0.90	0.85	0.94	0.04	0.92	0.84	0.88	0.89	0.81	0.95	0.07	0.93	1011
0.11	0.87	0.88	0.89	0.85	0.92	0.04	0.91	0.85	0.87	0.87	0.82	0.92	0.05	0.90	0.81	0.85	0.86	0.77	0.93	0.08	0.90	1039
0.15	0.85	0.86	0.87	0.82	0.90	0.04	0.89	0.81	0.84	0.85	0.78	0.89	0.05	0.87	0.78	0.81	0.82	0.72	0.90	0.09	0.87	1047
0.18	0.82	0.84	0.85	0.78	0.89	0.05	0.87	0.79	0.81	0.82	0.76	0.87	0.06	0.86	0.74	0.77	0.79	0.67	0.88	0.10	0.83	1013
0.32	0.80	0.81	0.83	0.76	0.87	0.05	0.85	0.75	0.79	0.79	0.73	0.85	0.06	0.83	0.70	0.74	0.76	0.63	0.85	0.11	0.81	1718


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	20.96	27.34	27.66	18.12	36.56	9.22	31.90	0.20	12.74	6.40	-2.87	28.36	15.62	21.46	6.49	21.93	16.18	1.64	42.22	20.29	31.41	954
0.03	12.03	15.58	14.67	7.47	23.70	8.12	18.05	0.23	13.83	6.06	-3.19	30.85	17.02	22.96	8.05	24.31	17.82	2.48	46.13	21.82	34.99	992
0.06	15.89	22.69	20.00	2.91	42.46	19.77	24.58	0.26	14.46	6.62	-3.15	32.06	17.61	25.05	8.47	25.87	18.68	3.04	48.69	22.83	37.10	1011
0.11	20.87	32.24	26.31	4.60	59.88	27.64	33.42	0.24	14.33	5.99	-3.32	31.99	17.66	25.21	9.23	26.15	19.88	3.42	48.88	22.73	37.67	1039
0.15	29.55	45.16	37.45	11.92	78.40	33.24	49.38	0.22	14.31	4.98	-4.26	32.87	18.57	25.43	9.41	26.48	20.02	3.76	49.20	22.72	37.87	1047
0.18	38.67	56.11	48.65	25.92	86.30	30.19	65.54	0.25	14.83	6.40	-3.71	33.38	18.55	25.55	9.54	26.87	20.97	4.09	49.65	22.78	37.34	1013
0.32	60.46	111.26	90.14	44.61	177.91	66.65	146.15	0.28	15.52	7.68	-3.93	34.97	19.45	26.38	10.46	28.01	21.56	4.72	51.31	23.30	39.69	1718


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/time_misc_auc.tex <==
name	auc
attack_time	17.06
l2	4.55
lom	8.22


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.14	0.28	0.27	0.10	0.47	0.19	0.40	0.30	0.41	0.41	0.26	0.57	0.16	0.52	0.48	0.56	0.56	0.44	0.68	0.12	0.63	954
0.03	0.08	0.21	0.19	0.05	0.37	0.16	0.31	0.26	0.36	0.37	0.21	0.51	0.15	0.46	0.45	0.52	0.53	0.41	0.64	0.11	0.60	992
0.06	0.05	0.16	0.13	0.02	0.30	0.14	0.25	0.22	0.32	0.31	0.18	0.46	0.14	0.42	0.42	0.49	0.50	0.38	0.60	0.11	0.57	1011
0.11	0.00	0.12	0.10	0.01	0.24	0.12	0.19	0.20	0.29	0.29	0.17	0.42	0.13	0.38	0.41	0.47	0.48	0.37	0.58	0.10	0.54	1039
0.15	0.00	0.09	0.06	-0.01	0.19	0.10	0.14	0.18	0.26	0.25	0.15	0.37	0.11	0.34	0.39	0.45	0.45	0.35	0.55	0.10	0.52	1047
0.18	0.00	0.07	0.05	-0.01	0.15	0.08	0.11	0.16	0.23	0.23	0.13	0.34	0.11	0.31	0.37	0.43	0.43	0.34	0.52	0.09	0.50	1013
0.32	0.00	0.04	0.00	-0.02	0.11	0.06	0.07	0.13	0.20	0.20	0.11	0.29	0.09	0.27	0.35	0.41	0.41	0.32	0.49	0.08	0.46	1718


==> data/mlm_plots/mlm_distil_fast/imdb/bert/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.08
top50	0.14


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	49.98	69.42	63.70	41.17	97.66	28.24	84.51	33.00	40.93	41.00	30.59	51.26	10.33	48.00	53.47	74.13	68.25	44.21	104.06	29.93	88.28	33.00	40.58	41.00	30.35	50.81	10.23	48.00	943
0.03	50.02	69.87	63.55	40.11	99.64	29.76	84.82	31.00	38.98	40.00	27.10	50.85	11.88	47.00	58.40	81.10	75.02	48.77	113.43	32.33	96.21	30.00	38.34	39.00	26.66	50.01	11.68	47.00	1013
0.06	50.02	69.47	63.70	40.87	98.07	28.60	84.25	32.00	39.68	41.00	27.82	51.54	11.86	48.00	69.85	94.39	88.08	59.25	129.52	35.13	111.17	31.00	38.70	39.00	27.03	50.38	11.67	47.00	1205
0.11	48.72	68.96	62.17	39.29	98.63	29.67	84.06	32.00	39.34	40.00	27.36	51.32	11.98	47.00	83.61	112.99	106.40	71.16	154.81	41.83	131.47	30.00	37.98	38.00	26.31	49.64	11.67	46.00	1397
0.15	49.73	69.44	63.85	40.23	98.65	29.21	82.11	30.25	38.70	39.00	26.41	50.99	12.29	48.00	112.46	143.53	136.60	95.93	191.13	47.60	165.20	29.00	36.82	37.00	24.94	48.70	11.88	45.00	1182
0.18	50.09	70.60	63.92	40.40	100.80	30.20	86.39	29.75	38.14	39.00	25.68	50.60	12.46	47.00	136.91	177.66	166.44	116.74	238.58	60.92	206.42	28.00	35.83	36.00	23.76	47.91	12.08	44.00	892
0.32	50.30	70.73	63.70	40.97	100.49	29.76	85.29	30.00	38.26	39.00	25.60	50.92	12.66	47.00	184.19	246.28	229.04	158.23	334.33	88.05	295.92	27.00	35.28	35.00	23.17	47.38	12.10	44.00	1255


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/comparison_vals_auc.tex <==
name	auc
orig_pp	21.74
orig_ge	12.03
adv_pp	48.90
adv_ge	11.44


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.08	0.19	0.18	0.05	0.34	0.14	0.28	0.32	0.42	0.42	0.27	0.56	0.15	0.52	0.22	0.30	0.29	0.18	0.41	0.11	0.37	943
0.03	0.01	0.10	0.07	-0.03	0.22	0.13	0.16	0.22	0.33	0.32	0.17	0.49	0.16	0.43	0.15	0.23	0.22	0.11	0.35	0.12	0.30	1013
0.06	-0.05	0.01	0.01	-0.08	0.10	0.09	0.07	0.13	0.24	0.24	0.08	0.39	0.15	0.34	0.09	0.16	0.16	0.05	0.27	0.11	0.23	1205
0.11	-0.08	-0.03	-0.04	-0.12	0.05	0.08	0.01	0.03	0.15	0.15	-0.01	0.31	0.16	0.26	0.02	0.10	0.10	-0.01	0.22	0.11	0.18	1397
0.15	-0.13	-0.08	-0.08	-0.16	0.00	0.08	-0.03	-0.05	0.07	0.06	-0.10	0.23	0.17	0.18	-0.03	0.05	0.04	-0.07	0.16	0.11	0.12	1182
0.18	-0.17	-0.12	-0.12	-0.20	-0.03	0.09	-0.06	-0.11	0.00	-0.01	-0.16	0.17	0.17	0.12	-0.08	0.00	-0.01	-0.11	0.12	0.11	0.08	892
0.32	-0.22	-0.16	-0.16	-0.25	-0.07	0.09	-0.11	-0.21	-0.09	-0.11	-0.26	0.07	0.16	0.01	-0.14	-0.07	-0.07	-0.18	0.05	0.11	0.01	1255


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/correlations_auc.tex <==
name	auc
pcc	-0.02
spearman	0.02
kendall	0.02


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	8.32	11.88	10.81	6.95	16.81	4.93	14.46	7.62	12.03	10.49	5.48	18.58	6.55	14.43	6.41	12.58	9.93	3.79	21.38	8.80	15.88	943
0.03	5.92	7.66	7.18	4.93	10.38	2.73	8.91	5.19	7.90	7.02	3.55	12.24	4.34	9.35	4.77	9.82	7.39	2.06	17.58	7.76	11.93	1013
0.06	4.65	5.76	5.56	4.05	7.47	1.71	6.58	4.01	5.79	5.21	2.99	8.59	2.80	6.93	3.44	7.17	5.12	0.80	13.53	6.37	8.22	1205
0.11	4.04	4.83	4.81	3.57	6.10	1.26	5.58	3.36	4.68	4.38	2.62	6.74	2.06	5.45	3.06	5.39	4.31	1.35	9.43	4.04	6.15	1397
0.15	3.49	4.14	4.14	3.18	5.10	0.96	4.74	2.98	3.92	3.64	2.53	5.30	1.38	4.52	2.50	3.99	3.35	1.32	6.66	2.67	4.53	1182
0.18	3.16	3.75	3.74	2.91	4.59	0.84	4.23	2.71	3.47	3.26	2.33	4.62	1.15	3.98	2.26	3.43	2.99	1.40	5.47	2.04	3.96	892
0.32	2.88	3.34	3.37	2.59	4.10	0.75	3.78	2.44	3.09	2.93	2.14	4.04	0.95	3.50	2.01	2.87	2.57	1.49	4.26	1.38	3.39	1255


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/ets_sts_auc.tex <==
name	auc
et_use	1.46
et_tse	1.41
et_ce	1.53


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	3.39	12.47	5.57	-9.79	34.73	22.26	11.28	8.29	13.67	11.76	6.09	21.26	7.58	16.98	7.04	13.84	11.01	4.32	23.36	9.52	17.82	943
0.03	1.87	6.84	2.60	-16.49	30.17	23.33	4.42	6.37	8.87	7.88	4.73	13.00	4.13	10.14	5.22	8.53	6.82	2.67	14.39	5.86	9.83	1013
0.06	0.99	1.86	1.31	-1.43	5.15	3.29	1.83	5.11	6.36	6.00	4.41	8.31	1.95	7.08	4.15	5.75	5.11	3.06	8.44	2.69	6.59	1205
0.11	0.60	0.90	0.77	0.34	1.46	0.56	1.05	4.31	5.19	5.02	3.90	6.47	1.28	5.76	3.54	4.58	4.28	2.87	6.30	1.72	5.16	1397
0.15	0.38	0.54	0.48	0.26	0.82	0.28	0.61	3.78	4.43	4.27	3.48	5.38	0.95	4.96	3.10	3.87	3.61	2.75	4.98	1.12	4.34	1182
0.18	0.27	0.38	0.35	0.23	0.54	0.15	0.45	3.50	4.06	3.95	3.24	4.87	0.82	4.46	2.91	3.56	3.35	2.57	4.55	0.99	3.94	892
0.32	0.18	0.26	0.23	0.13	0.39	0.13	0.31	3.20	3.68	3.56	2.95	4.41	0.73	4.04	2.67	3.22	3.07	2.38	4.07	0.84	3.57	1255


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.48
et_p_h	1.61
et_p_l2	1.45


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.04	0.08	0.07	0.03	0.14	0.06	0.12	0.02	0.04	0.04	0.02	0.07	0.02	0.06	0.02	0.04	0.03	0.02	0.05	0.02	0.05	943
0.03	0.10	0.18	0.17	0.07	0.29	0.11	0.24	0.05	0.07	0.07	0.04	0.10	0.03	0.09	0.04	0.06	0.06	0.04	0.08	0.02	0.07	1013
0.06	0.27	0.39	0.37	0.22	0.56	0.17	0.49	0.08	0.10	0.10	0.07	0.13	0.03	0.12	0.07	0.08	0.08	0.06	0.10	0.02	0.09	1205
0.11	0.49	0.69	0.66	0.41	0.98	0.28	0.86	0.10	0.12	0.12	0.09	0.16	0.03	0.14	0.09	0.10	0.10	0.08	0.13	0.02	0.12	1397
0.15	0.89	1.16	1.11	0.75	1.57	0.41	1.41	0.13	0.15	0.15	0.11	0.18	0.04	0.17	0.11	0.13	0.13	0.10	0.15	0.02	0.14	1182
0.18	1.25	1.64	1.59	1.10	2.18	0.54	1.96	0.14	0.17	0.16	0.13	0.20	0.04	0.19	0.13	0.14	0.14	0.12	0.16	0.02	0.15	892
0.32	1.90	2.70	2.51	1.59	3.81	1.11	3.28	0.17	0.19	0.19	0.15	0.23	0.04	0.21	0.15	0.16	0.16	0.14	0.19	0.03	0.18	1255


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.42
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.95	0.96	0.96	0.95	0.97	0.01	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.94	0.95	0.96	0.92	0.98	0.03	0.97	943
0.03	0.93	0.94	0.94	0.91	0.96	0.02	0.95	0.92	0.93	0.94	0.89	0.96	0.03	0.95	0.91	0.93	0.94	0.88	0.98	0.05	0.96	1013
0.06	0.90	0.91	0.91	0.88	0.94	0.03	0.92	0.88	0.90	0.91	0.86	0.94	0.04	0.93	0.86	0.89	0.90	0.83	0.96	0.07	0.94	1205
0.11	0.87	0.88	0.89	0.84	0.93	0.04	0.91	0.85	0.87	0.88	0.82	0.92	0.05	0.90	0.83	0.86	0.88	0.78	0.95	0.09	0.92	1397
0.15	0.85	0.86	0.87	0.82	0.90	0.04	0.89	0.82	0.85	0.85	0.80	0.90	0.05	0.88	0.79	0.83	0.84	0.74	0.91	0.08	0.88	1182
0.18	0.82	0.84	0.85	0.80	0.88	0.04	0.87	0.80	0.82	0.83	0.77	0.88	0.05	0.86	0.76	0.80	0.81	0.71	0.89	0.09	0.86	892
0.32	0.80	0.82	0.83	0.76	0.87	0.05	0.85	0.76	0.80	0.80	0.74	0.85	0.05	0.84	0.72	0.76	0.78	0.65	0.86	0.11	0.83	1255


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.26


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	9.64	14.18	13.30	5.70	22.67	8.49	16.33	0.72	69.34	1.36	-104.41	243.08	173.74	6.11	4.35	10.47	9.00	2.66	18.28	7.81	14.91	943
0.03	10.51	17.74	13.75	2.96	32.51	14.77	18.91	0.90	85.84	1.66	-158.69	330.36	244.53	10.85	4.83	11.64	10.48	3.30	19.99	8.35	16.79	1013
0.06	16.76	38.87	24.39	6.81	70.93	32.06	56.62	1.16	82.15	2.18	-158.93	323.24	241.08	11.96	5.42	12.77	11.02	3.61	21.93	9.16	18.41	1205
0.11	24.84	53.10	43.35	17.58	88.62	35.52	74.22	1.12	81.09	2.08	-180.07	342.24	261.15	8.92	5.18	12.81	11.24	3.28	22.34	9.53	18.85	1397
0.15	35.38	60.71	54.08	27.00	94.41	33.71	75.54	1.04	111.09	2.03	-264.39	486.57	375.48	10.28	4.95	12.44	10.21	2.93	21.95	9.51	18.65	1182
0.18	46.49	65.48	61.92	37.30	93.66	28.18	79.41	0.98	128.98	2.03	-256.99	514.96	385.97	15.28	4.76	12.44	10.30	2.85	22.03	9.59	18.16	892
0.32	62.17	82.96	80.14	51.48	114.44	31.48	98.50	1.01	145.67	2.13	-267.24	558.59	412.92	71.72	4.68	12.29	10.07	2.91	21.66	9.37	17.96	1255


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/time_misc_auc.tex <==
name	auc
attack_time	18.03
l2	34.85
lom	3.84


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.13	0.21	0.20	0.09	0.33	0.12	0.29	0.41	0.48	0.48	0.39	0.57	0.09	0.53	0.61	0.65	0.65	0.59	0.71	0.06	0.69	943
0.03	0.06	0.14	0.14	0.04	0.25	0.10	0.20	0.36	0.42	0.42	0.33	0.51	0.09	0.48	0.58	0.62	0.62	0.55	0.69	0.07	0.66	1013
0.06	0.05	0.09	0.09	0.01	0.17	0.08	0.14	0.32	0.37	0.37	0.28	0.45	0.08	0.42	0.55	0.59	0.59	0.52	0.65	0.06	0.63	1205
0.11	0.00	0.07	0.05	-0.00	0.14	0.07	0.10	0.27	0.33	0.32	0.24	0.42	0.09	0.38	0.51	0.56	0.56	0.49	0.62	0.07	0.60	1397
0.15	0.00	0.04	0.00	-0.01	0.10	0.06	0.07	0.24	0.29	0.29	0.21	0.37	0.08	0.34	0.48	0.53	0.53	0.47	0.59	0.06	0.57	1182
0.18	0.00	0.03	0.00	-0.02	0.08	0.05	0.05	0.20	0.26	0.25	0.18	0.34	0.08	0.31	0.47	0.51	0.50	0.44	0.57	0.06	0.55	892
0.32	0.00	0.02	0.00	-0.02	0.05	0.04	0.05	0.17	0.22	0.21	0.14	0.29	0.08	0.27	0.43	0.47	0.47	0.41	0.54	0.07	0.51	1255


==> data/mlm_plots/mlm_distil_fast/imdb/bert/s/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.09
top50	0.17


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	53.02	75.75	71.74	46.28	105.22	29.47	92.97	31.00	39.21	40.00	27.28	51.13	11.93	48.00	58.25	80.55	77.27	50.55	110.56	30.01	95.19	31.00	38.96	40.00	27.05	50.87	11.91	48.00	918
0.03	54.07	74.08	69.00	43.77	104.39	30.31	88.99	29.00	37.91	38.00	24.96	50.85	12.94	47.00	62.33	85.98	80.29	52.28	119.68	33.70	104.10	29.00	37.30	37.00	24.54	50.05	12.76	46.00	994
0.06	54.04	74.00	68.86	43.68	104.32	30.32	88.80	29.00	37.84	38.00	24.81	50.87	13.03	47.00	70.84	97.42	91.72	60.05	134.80	37.37	115.63	28.00	36.81	37.00	24.10	49.53	12.71	45.00	1010
0.11	54.14	74.37	69.10	43.39	105.35	30.98	89.03	29.00	37.84	38.00	24.80	50.89	13.04	47.00	82.42	112.21	105.47	69.38	155.04	42.83	133.23	28.00	36.38	36.00	23.76	49.00	12.62	45.00	1012
0.15	54.11	74.40	69.12	43.32	105.48	31.08	89.03	29.00	37.79	38.00	24.74	50.84	13.05	47.00	104.79	140.42	133.40	89.85	191.00	50.57	164.58	27.00	35.86	36.00	23.27	48.45	12.59	44.00	1016
0.18	54.14	74.38	69.10	43.32	105.45	31.06	89.01	29.00	37.80	38.00	24.75	50.84	13.04	47.00	131.29	171.45	162.14	110.87	232.04	60.58	199.47	26.00	35.22	35.00	22.81	47.63	12.41	43.00	1017
0.32	54.05	74.43	69.12	43.39	105.47	31.04	88.96	29.00	37.76	38.00	24.76	50.76	13.00	47.00	184.21	246.44	234.26	157.18	335.71	89.26	293.71	25.00	33.92	33.50	21.77	46.07	12.15	42.00	2016


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	23.09
orig_ge	11.75
adv_pp	48.53
adv_ge	11.08


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.32	0.48	0.48	0.24	0.71	0.23	0.63	0.57	0.69	0.76	0.49	0.89	0.20	0.84	0.47	0.61	0.65	0.40	0.82	0.21	0.78	918
0.03	0.08	0.25	0.23	-0.01	0.50	0.26	0.40	0.47	0.56	0.60	0.36	0.76	0.20	0.70	0.38	0.50	0.52	0.30	0.69	0.19	0.64	994
0.06	-0.12	0.04	0.03	-0.20	0.28	0.24	0.17	0.33	0.41	0.44	0.23	0.60	0.19	0.53	0.28	0.37	0.39	0.20	0.54	0.17	0.49	1010
0.11	-0.24	-0.09	-0.12	-0.32	0.14	0.23	0.01	0.19	0.29	0.31	0.11	0.47	0.18	0.40	0.18	0.27	0.29	0.11	0.43	0.16	0.37	1012
0.15	-0.39	-0.25	-0.28	-0.46	-0.05	0.21	-0.17	0.02	0.11	0.12	-0.05	0.27	0.16	0.20	0.05	0.12	0.13	-0.01	0.26	0.13	0.21	1016
0.18	-0.48	-0.36	-0.39	-0.55	-0.17	0.19	-0.28	-0.11	-0.03	-0.02	-0.18	0.12	0.15	0.06	-0.05	0.02	0.02	-0.10	0.14	0.12	0.09	1017
0.32	-0.61	-0.50	-0.52	-0.66	-0.33	0.17	-0.42	-0.35	-0.24	-0.25	-0.39	-0.08	0.15	-0.13	-0.24	-0.15	-0.16	-0.27	-0.03	0.12	-0.06	2016


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/correlations_auc.tex <==
name	auc
pcc	-0.07
spearman	0.04
kendall	0.04


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	4.72	8.14	7.66	3.60	12.67	4.53	10.00	4.84	8.61	7.93	3.48	13.73	5.12	10.86	3.18	7.69	6.04	1.48	13.91	6.22	10.09	918
0.03	4.70	6.80	6.36	3.38	10.21	3.42	8.21	4.53	7.38	6.50	2.83	11.93	4.55	9.04	3.23	7.27	5.24	1.05	13.50	6.23	9.10	994
0.06	4.45	5.89	5.63	3.53	8.26	2.36	6.99	4.11	6.30	5.48	2.49	10.11	3.81	7.61	3.01	5.81	4.61	1.34	10.28	4.47	7.24	1010
0.11	4.18	5.28	5.12	3.36	7.19	1.91	6.22	3.87	5.34	4.86	2.64	8.05	2.71	6.14	2.80	4.83	3.98	1.16	8.51	3.67	5.71	1012
0.15	3.88	4.72	4.69	3.36	6.09	1.36	5.52	3.44	4.60	4.24	2.18	7.01	2.41	5.29	2.63	3.90	3.40	1.32	6.49	2.59	4.50	1016
0.18	3.71	4.41	4.42	3.25	5.57	1.16	5.14	3.21	4.14	3.91	2.68	5.59	1.46	4.80	2.47	3.52	3.18	1.16	5.89	2.37	4.03	1017
0.32	3.46	4.02	4.05	3.10	4.94	0.92	4.61	2.97	3.69	3.53	2.60	4.77	1.08	4.19	2.32	3.08	2.87	1.29	4.87	1.79	3.50	2016


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/ets_sts_auc.tex <==
name	auc
et_use	1.55
et_tse	1.54
et_ce	1.36


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.04	9.60	3.78	-12.88	32.07	22.47	7.00	5.28	10.99	8.15	1.90	20.08	9.09	14.14	5.26	11.41	8.72	1.59	21.24	9.82	14.42	918
0.03	1.41	5.44	2.38	-12.80	23.68	18.24	3.91	5.43	8.96	7.67	2.95	14.97	6.01	11.06	4.69	9.15	7.12	1.56	16.74	7.59	11.33	994
0.06	1.05	2.13	1.48	-1.74	5.99	3.86	2.13	5.69	7.69	7.10	4.16	11.23	3.53	9.09	4.81	7.45	6.39	2.90	12.00	4.55	8.67	1010
0.11	0.79	1.38	1.06	-0.90	3.67	2.28	1.42	5.46	6.88	6.60	4.35	9.41	2.53	7.95	4.60	6.48	5.86	3.20	9.76	3.28	7.40	1012
0.15	0.54	0.79	0.68	0.16	1.41	0.62	0.89	5.15	6.22	6.00	4.31	8.12	1.91	7.03	4.37	5.79	5.29	3.38	8.20	2.41	6.59	1016
0.18	0.40	0.56	0.51	0.26	0.85	0.30	0.64	4.94	5.79	5.67	4.33	7.24	1.45	6.45	4.25	5.32	5.01	3.53	7.11	1.79	6.06	1017
0.32	0.24	0.36	0.32	0.05	0.68	0.31	0.43	4.60	5.28	5.15	4.17	6.38	1.11	5.80	3.97	4.83	4.61	3.44	6.22	1.39	5.34	2016


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.48
et_p_h	2.03
et_p_l2	1.93


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.03	0.08	0.07	0.02	0.13	0.05	0.11	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.04	918
0.03	0.11	0.17	0.16	0.08	0.27	0.10	0.24	0.03	0.06	0.05	0.03	0.08	0.03	0.07	0.04	0.05	0.05	0.03	0.07	0.02	0.06	994
0.06	0.24	0.34	0.33	0.19	0.49	0.15	0.43	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	1010
0.11	0.40	0.54	0.53	0.33	0.76	0.21	0.65	0.08	0.10	0.10	0.06	0.13	0.03	0.11	0.07	0.08	0.09	0.06	0.11	0.02	0.10	1012
0.15	0.73	0.95	0.93	0.62	1.28	0.33	1.14	0.10	0.12	0.12	0.08	0.16	0.04	0.14	0.09	0.11	0.11	0.08	0.13	0.02	0.12	1016
0.18	1.08	1.40	1.36	0.91	1.90	0.49	1.66	0.12	0.14	0.14	0.10	0.17	0.04	0.16	0.11	0.12	0.12	0.10	0.15	0.02	0.14	1017
0.32	1.72	2.52	2.33	1.43	3.61	1.09	3.13	0.14	0.16	0.16	0.13	0.20	0.04	0.19	0.13	0.15	0.15	0.12	0.17	0.03	0.16	2016


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.37
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.93	0.99	0.03	0.98	0.95	0.96	0.97	0.93	0.99	0.03	0.98	0.93	0.94	0.96	0.87	1.01	0.07	0.98	918
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.92	0.94	0.94	0.90	0.97	0.03	0.96	0.89	0.92	0.93	0.86	0.98	0.06	0.96	994
0.06	0.90	0.91	0.92	0.89	0.94	0.03	0.93	0.89	0.91	0.92	0.87	0.95	0.04	0.94	0.85	0.88	0.90	0.82	0.95	0.07	0.93	1010
0.11	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.86	0.88	0.89	0.84	0.93	0.04	0.91	0.81	0.85	0.86	0.77	0.93	0.08	0.91	1012
0.15	0.85	0.86	0.87	0.82	0.90	0.04	0.88	0.82	0.85	0.85	0.80	0.90	0.05	0.88	0.76	0.80	0.82	0.71	0.90	0.09	0.86	1016
0.18	0.82	0.84	0.85	0.79	0.88	0.05	0.86	0.79	0.82	0.83	0.77	0.87	0.05	0.86	0.73	0.77	0.79	0.67	0.87	0.10	0.83	1017
0.32	0.79	0.80	0.81	0.75	0.85	0.05	0.84	0.75	0.78	0.79	0.73	0.84	0.06	0.82	0.68	0.72	0.74	0.62	0.83	0.10	0.79	2016


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	4.85	5.57	5.61	4.32	6.81	1.25	6.42	4.31	7.04	6.05	3.25	10.82	3.79	8.93	2.93	7.46	5.19	0.14	14.77	7.31	9.92	918
0.03	6.44	6.63	6.66	6.36	6.90	0.27	6.75	5.59	9.10	7.77	4.20	14.00	4.90	11.42	3.24	9.94	7.26	0.55	19.33	9.39	13.90	994
0.06	8.20	8.47	8.38	8.05	8.89	0.42	8.65	6.39	10.64	9.00	4.95	16.33	5.69	13.82	3.86	10.72	8.39	1.11	20.34	9.62	14.48	1010
0.11	10.02	10.65	10.47	9.77	11.53	0.88	11.01	6.85	11.42	9.72	5.46	17.38	5.96	15.21	4.32	11.41	8.80	1.55	21.26	9.86	15.96	1012
0.15	13.32	14.01	14.06	13.28	14.75	0.74	14.37	7.49	12.43	10.49	5.92	18.94	6.51	16.43	4.12	11.89	9.28	1.76	22.01	10.13	16.94	1016
0.18	17.26	18.01	17.87	17.10	18.91	0.90	18.69	7.85	13.09	11.09	6.19	20.00	6.91	17.18	4.52	12.30	9.58	2.06	22.54	10.24	17.41	1017
0.32	22.83	26.38	25.15	22.49	30.27	3.89	29.80	8.23	13.85	11.85	6.52	21.18	7.33	18.17	4.28	12.41	9.92	2.16	22.65	10.24	17.71	2016


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/time_misc_auc.tex <==
name	auc
attack_time	4.89
l2	3.76
lom	3.60


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.50	0.65	0.68	0.49	0.80	0.16	0.77	0.68	0.76	0.79	0.62	0.90	0.14	0.87	0.75	0.81	0.83	0.70	0.93	0.11	0.91	918
0.03	0.42	0.53	0.55	0.38	0.68	0.15	0.64	0.62	0.70	0.72	0.57	0.83	0.13	0.80	0.71	0.77	0.78	0.67	0.88	0.11	0.85	994
0.06	0.32	0.41	0.41	0.27	0.54	0.13	0.50	0.56	0.63	0.64	0.51	0.75	0.12	0.71	0.67	0.72	0.73	0.62	0.82	0.10	0.79	1010
0.11	0.23	0.32	0.32	0.20	0.44	0.12	0.40	0.50	0.57	0.58	0.45	0.68	0.11	0.65	0.62	0.68	0.69	0.58	0.77	0.10	0.75	1012
0.15	0.14	0.21	0.20	0.10	0.32	0.11	0.27	0.42	0.48	0.49	0.38	0.57	0.10	0.54	0.57	0.62	0.62	0.53	0.70	0.08	0.68	1016
0.18	0.08	0.14	0.14	0.05	0.24	0.09	0.20	0.36	0.41	0.41	0.33	0.50	0.08	0.47	0.53	0.57	0.58	0.49	0.65	0.08	0.62	1017
0.32	0.00	0.08	0.07	0.01	0.15	0.07	0.12	0.24	0.30	0.30	0.22	0.39	0.08	0.37	0.44	0.49	0.49	0.42	0.57	0.07	0.54	2016


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/ig/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.15
top50	0.19


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	53.05	75.00	71.28	45.87	104.13	29.13	91.58	31.00	39.62	40.00	27.57	51.68	12.05	49.00	59.15	82.05	77.28	50.49	113.62	31.57	101.63	31.00	39.23	39.00	27.29	51.18	11.94	48.00	872
0.03	54.04	74.15	68.82	43.28	105.01	30.86	88.48	29.00	37.99	38.00	25.15	50.83	12.84	47.00	65.81	90.65	85.14	54.58	126.72	36.07	108.73	29.00	37.35	37.00	24.74	49.96	12.61	46.00	996
0.06	54.02	74.31	69.04	43.23	105.39	31.08	88.99	29.00	37.85	38.00	24.83	50.86	13.01	47.00	77.72	106.09	100.17	64.46	147.73	41.63	126.00	28.00	36.67	37.00	23.97	49.38	12.70	45.75	1014
0.11	54.18	74.42	69.22	43.42	105.42	31.00	89.03	29.00	37.83	38.00	24.80	50.85	13.02	47.00	90.91	124.64	116.50	76.63	172.65	48.01	148.27	27.00	36.19	36.00	23.60	48.78	12.59	45.00	1021
0.15	54.05	74.39	69.10	43.33	105.45	31.06	89.04	29.00	37.79	38.00	24.77	50.82	13.02	47.00	120.49	160.79	151.46	101.75	219.84	59.04	192.04	27.00	35.44	35.00	22.98	47.90	12.46	44.00	1013
0.18	54.05	74.38	69.10	43.32	105.45	31.06	89.04	29.00	37.79	38.00	24.76	50.82	13.03	47.00	152.83	202.23	191.95	130.02	274.43	72.21	237.62	26.00	34.66	35.00	22.37	46.96	12.29	43.00	1013
0.32	54.05	74.38	69.10	43.50	105.26	30.88	89.03	29.00	37.82	38.00	24.88	50.75	12.94	47.00	217.81	298.88	282.03	185.76	411.99	113.11	357.87	24.00	33.22	33.00	21.23	45.21	11.99	41.00	2017


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/comparison_vals_auc.tex <==
name	auc
orig_pp	23.09
orig_ge	11.76
adv_pp	56.51
adv_ge	10.96


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.75	0.81	0.81	0.71	0.90	0.10	0.88	0.83	0.88	0.89	0.80	0.95	0.07	0.93	0.70	0.77	0.77	0.66	0.87	0.11	0.84	872
0.03	0.62	0.69	0.71	0.57	0.82	0.12	0.78	0.74	0.79	0.81	0.69	0.89	0.10	0.86	0.60	0.67	0.67	0.56	0.78	0.11	0.74	996
0.06	0.49	0.58	0.59	0.44	0.72	0.14	0.67	0.62	0.69	0.70	0.58	0.80	0.11	0.77	0.49	0.56	0.56	0.45	0.66	0.11	0.63	1014
0.11	0.38	0.47	0.48	0.32	0.63	0.15	0.58	0.50	0.58	0.60	0.45	0.72	0.14	0.68	0.38	0.46	0.46	0.34	0.57	0.11	0.53	1021
0.15	0.22	0.33	0.33	0.17	0.49	0.16	0.44	0.33	0.43	0.43	0.28	0.58	0.15	0.53	0.25	0.32	0.32	0.21	0.43	0.11	0.40	1013
0.18	0.11	0.21	0.21	0.05	0.37	0.16	0.32	0.19	0.29	0.30	0.13	0.45	0.16	0.40	0.14	0.21	0.21	0.10	0.33	0.11	0.29	1013
0.32	-0.11	0.02	0.01	-0.16	0.20	0.18	0.14	-0.08	0.05	0.06	-0.14	0.25	0.19	0.19	-0.05	0.04	0.04	-0.09	0.18	0.14	0.13	2017


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/correlations_auc.tex <==
name	auc
pcc	0.10
spearman	0.13
kendall	0.10


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	1.91	3.31	2.81	1.29	5.33	2.02	4.30	1.93	3.73	3.02	1.11	6.35	2.62	4.79	1.35	3.34	2.45	0.56	6.12	2.78	4.55	872
0.03	1.88	2.86	2.64	1.42	4.31	1.45	3.57	1.77	3.09	2.71	1.18	4.99	1.90	3.89	1.57	3.78	2.81	0.53	7.02	3.25	4.84	996
0.06	1.94	2.67	2.53	1.53	3.81	1.14	3.26	1.79	2.74	2.47	1.26	4.22	1.48	3.47	1.53	3.20	2.46	0.56	5.85	2.65	3.94	1014
0.11	1.93	2.61	2.53	1.62	3.60	0.99	3.19	1.76	2.54	2.36	1.33	3.76	1.21	3.06	1.53	2.84	2.25	0.71	4.97	2.13	3.36	1021
0.15	2.06	2.64	2.59	1.80	3.48	0.84	3.14	1.77	2.42	2.29	1.44	3.40	0.98	2.89	1.55	2.59	2.22	0.91	4.26	1.68	3.04	1013
0.18	2.17	2.68	2.62	1.90	3.45	0.78	3.18	1.82	2.40	2.30	1.53	3.27	0.87	2.85	1.59	2.45	2.15	0.93	3.97	1.52	2.93	1013
0.32	2.27	2.71	2.71	2.02	3.40	0.69	3.15	1.91	2.40	2.33	1.69	3.10	0.71	2.77	1.65	2.30	2.10	1.14	3.47	1.16	2.67	2017


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/ets_sts_auc.tex <==
name	auc
et_use	0.84
et_tse	0.80
et_ce	0.84


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.53	2.14	0.93	-2.22	6.50	4.36	1.81	1.48	3.21	2.50	-0.04	6.45	3.25	3.60	1.28	3.36	2.34	0.03	6.69	3.33	3.83	872
0.03	0.42	1.00	0.63	-0.82	2.82	1.82	1.01	1.85	2.90	2.57	1.27	4.53	1.63	3.58	1.65	2.93	2.40	0.83	5.03	2.10	3.55	996
0.06	0.33	0.60	0.47	-0.30	1.49	0.90	0.66	2.06	2.83	2.68	1.70	3.97	1.13	3.48	1.78	2.71	2.47	1.34	4.08	1.37	3.27	1014
0.11	0.27	0.44	0.37	0.09	0.79	0.35	0.51	2.18	2.91	2.74	1.84	3.97	1.06	3.47	1.89	2.74	2.48	1.43	4.05	1.31	3.30	1021
0.15	0.21	0.31	0.28	0.13	0.49	0.18	0.36	2.39	2.94	2.84	2.10	3.78	0.84	3.41	2.08	2.71	2.56	1.75	3.67	0.96	3.16	1013
0.18	0.17	0.24	0.22	0.11	0.37	0.13	0.28	2.51	3.00	2.94	2.26	3.74	0.74	3.43	2.21	2.75	2.64	1.90	3.61	0.85	3.18	1013
0.32	0.12	0.18	0.16	0.09	0.26	0.09	0.21	2.73	3.15	3.11	2.51	3.79	0.64	3.53	2.41	2.88	2.80	2.14	3.62	0.74	3.25	2017


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.13
et_p_h	0.93
et_p_l2	0.87


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.10	0.10	0.04	0.16	0.06	0.14	0.02	0.04	0.04	0.02	0.06	0.02	0.06	0.03	0.04	0.04	0.02	0.05	0.01	0.05	872
0.03	0.16	0.24	0.23	0.13	0.34	0.10	0.30	0.04	0.06	0.06	0.04	0.09	0.03	0.08	0.05	0.06	0.06	0.04	0.08	0.02	0.07	996
0.06	0.35	0.45	0.44	0.29	0.61	0.16	0.54	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.07	0.08	0.08	0.06	0.10	0.02	0.09	1014
0.11	0.55	0.71	0.70	0.47	0.94	0.23	0.85	0.09	0.11	0.10	0.07	0.14	0.03	0.12	0.08	0.09	0.09	0.07	0.11	0.02	0.11	1021
0.15	0.97	1.23	1.20	0.83	1.63	0.40	1.45	0.11	0.13	0.13	0.10	0.17	0.03	0.15	0.10	0.12	0.12	0.10	0.14	0.02	0.13	1013
0.18	1.43	1.84	1.76	1.23	2.44	0.60	2.16	0.13	0.15	0.15	0.11	0.19	0.04	0.17	0.12	0.13	0.13	0.11	0.16	0.02	0.15	1013
0.32	2.25	3.27	3.02	1.85	4.68	1.42	4.01	0.15	0.18	0.18	0.14	0.21	0.04	0.20	0.14	0.16	0.16	0.13	0.18	0.02	0.17	2017


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.48
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.94	0.95	0.97	0.92	0.99	0.04	0.98	872
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.93	0.94	0.95	0.91	0.97	0.03	0.96	0.91	0.93	0.95	0.88	0.99	0.05	0.97	996
0.06	0.90	0.91	0.92	0.89	0.94	0.03	0.93	0.89	0.91	0.92	0.87	0.95	0.04	0.94	0.87	0.90	0.92	0.83	0.97	0.07	0.95	1014
0.11	0.88	0.89	0.90	0.86	0.93	0.04	0.91	0.86	0.88	0.89	0.84	0.93	0.04	0.91	0.84	0.87	0.88	0.79	0.95	0.08	0.92	1021
0.15	0.85	0.87	0.87	0.83	0.90	0.04	0.89	0.82	0.85	0.85	0.80	0.90	0.05	0.88	0.79	0.83	0.85	0.75	0.92	0.08	0.89	1013
0.18	0.83	0.84	0.85	0.80	0.89	0.04	0.87	0.79	0.82	0.83	0.77	0.87	0.05	0.86	0.76	0.80	0.82	0.72	0.89	0.09	0.86	1013
0.32	0.79	0.81	0.82	0.76	0.86	0.05	0.84	0.75	0.78	0.79	0.73	0.84	0.05	0.82	0.71	0.75	0.76	0.65	0.85	0.10	0.82	2017


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.26


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.04	3.53	3.65	2.72	4.34	0.81	4.02	65.33	115.93	89.78	41.88	189.98	74.05	149.42	1.43	4.04	3.08	0.60	7.47	3.43	6.14	872
0.03	4.24	4.38	4.32	4.20	4.57	0.19	4.49	89.86	154.30	133.31	69.58	239.01	84.71	202.14	1.94	5.50	4.28	-0.26	11.27	5.77	7.80	996
0.06	4.72	4.87	4.79	4.64	5.11	0.24	5.02	106.01	184.80	153.63	83.69	285.91	101.11	245.43	2.46	6.56	5.41	1.20	11.92	5.36	9.21	1014
0.11	5.60	5.86	5.72	5.20	6.52	0.66	5.96	122.40	209.91	175.03	96.24	323.59	113.67	280.03	2.88	7.84	6.15	-1.60	17.28	9.44	10.52	1021
0.15	8.37	8.85	8.47	7.81	9.89	1.04	8.95	141.47	245.45	205.03	110.19	380.70	135.25	320.93	3.36	8.76	7.33	1.77	15.74	6.99	12.62	1013
0.18	10.04	10.62	10.33	9.50	11.74	1.12	10.75	155.46	270.88	222.67	120.29	421.46	150.59	353.47	3.54	9.48	7.90	2.04	16.93	7.44	13.80	1013
0.32	12.07	13.67	13.72	11.94	15.40	1.73	14.65	178.45	314.82	263.54	137.41	492.23	177.41	414.12	3.94	10.31	8.73	2.21	18.41	8.10	14.84	2017


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/time_misc_auc.tex <==
name	auc
attack_time	2.77
l2	75.55
lom	2.63


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.50	0.62	0.64	0.47	0.77	0.15	0.71	0.76	0.82	0.83	0.74	0.90	0.08	0.87	0.85	0.89	0.89	0.83	0.95	0.06	0.93	872
0.03	0.36	0.47	0.47	0.31	0.64	0.16	0.59	0.68	0.74	0.74	0.65	0.82	0.08	0.79	0.81	0.85	0.85	0.79	0.91	0.06	0.89	996
0.06	0.23	0.36	0.36	0.19	0.52	0.17	0.45	0.59	0.65	0.65	0.56	0.74	0.09	0.71	0.75	0.79	0.80	0.73	0.85	0.06	0.83	1014
0.11	0.18	0.28	0.27	0.12	0.43	0.16	0.36	0.51	0.57	0.57	0.48	0.67	0.09	0.63	0.70	0.74	0.75	0.67	0.81	0.07	0.78	1021
0.15	0.09	0.19	0.18	0.05	0.32	0.14	0.27	0.41	0.47	0.47	0.38	0.57	0.09	0.53	0.62	0.67	0.67	0.60	0.74	0.07	0.71	1013
0.18	0.05	0.13	0.11	0.01	0.25	0.12	0.21	0.33	0.39	0.40	0.30	0.49	0.10	0.45	0.57	0.61	0.61	0.54	0.68	0.07	0.65	1013
0.32	0.00	0.08	0.05	-0.02	0.18	0.10	0.14	0.21	0.28	0.28	0.18	0.38	0.10	0.34	0.46	0.51	0.51	0.43	0.59	0.08	0.57	2017


==> data/mlm_plots/mlm_distil_fast/imdb/cnn/s/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.15
top50	0.21


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	54.03	75.89	68.81	46.56	105.22	29.33	93.29	32.00	39.32	40.00	27.59	51.05	11.73	49.00	56.58	79.57	71.59	49.25	109.88	30.32	98.12	32.00	39.31	40.00	27.57	51.06	11.75	49.00	926
0.03	53.73	73.97	68.64	43.84	104.09	30.12	89.24	29.00	37.72	38.00	25.07	50.37	12.65	46.00	61.54	84.19	78.46	50.89	117.49	33.30	100.30	29.00	37.58	38.00	25.00	50.17	12.59	46.00	999
0.06	53.65	73.95	68.70	43.82	104.07	30.12	89.29	29.00	37.74	38.00	24.93	50.55	12.81	46.00	70.01	94.97	88.37	58.61	131.32	36.36	115.01	28.00	37.52	38.00	24.80	50.24	12.72	46.00	1013
0.11	53.69	74.01	68.71	43.85	104.17	30.16	89.26	29.00	37.61	38.00	24.81	50.41	12.80	46.00	80.70	107.89	101.13	68.66	147.11	39.23	130.31	28.00	37.23	38.00	24.62	49.84	12.61	46.00	1014
0.15	53.51	73.94	68.49	43.73	104.16	30.21	89.23	28.00	37.49	38.00	24.71	50.26	12.77	46.00	101.94	135.85	127.75	88.65	183.04	47.19	159.82	28.00	37.22	37.00	24.52	49.91	12.69	46.00	1004
0.18	53.61	73.92	68.67	43.81	104.02	30.11	89.18	28.75	37.61	38.00	24.80	50.41	12.80	46.00	125.05	164.62	156.31	109.04	220.19	55.58	193.89	28.00	36.85	37.00	24.17	49.53	12.68	46.00	1016
0.32	53.65	74.10	68.70	44.01	104.18	30.09	89.29	29.00	37.60	38.00	24.88	50.31	12.71	46.00	177.01	236.86	224.89	152.83	320.89	84.03	282.36	27.00	35.70	36.00	23.22	48.19	12.48	44.00	2009


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	22.99
orig_ge	11.70
adv_pp	46.77
adv_ge	11.47


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.07	0.27	0.27	-0.04	0.57	0.30	0.48	0.71	0.77	0.78	0.67	0.87	0.10	0.84	0.63	0.71	0.71	0.60	0.82	0.11	0.78	926
0.03	-0.18	0.03	0.01	-0.26	0.33	0.30	0.22	0.57	0.64	0.64	0.52	0.76	0.12	0.72	0.52	0.58	0.58	0.47	0.70	0.11	0.66	999
0.06	-0.32	-0.14	-0.16	-0.40	0.12	0.26	-0.01	0.43	0.50	0.50	0.38	0.62	0.12	0.57	0.40	0.46	0.46	0.36	0.57	0.10	0.52	1013
0.11	-0.40	-0.24	-0.27	-0.47	-0.01	0.23	-0.12	0.31	0.39	0.39	0.27	0.51	0.12	0.46	0.30	0.37	0.37	0.27	0.47	0.10	0.43	1014
0.15	-0.47	-0.34	-0.36	-0.54	-0.13	0.20	-0.23	0.16	0.23	0.23	0.11	0.35	0.12	0.30	0.18	0.24	0.24	0.14	0.33	0.09	0.30	1004
0.18	-0.54	-0.42	-0.44	-0.61	-0.23	0.19	-0.33	0.03	0.11	0.11	-0.01	0.22	0.12	0.18	0.08	0.14	0.13	0.04	0.23	0.09	0.19	1016
0.32	-0.64	-0.52	-0.54	-0.69	-0.34	0.17	-0.43	-0.19	-0.09	-0.10	-0.24	0.05	0.14	0.01	-0.10	-0.02	-0.03	-0.14	0.09	0.11	0.05	2009


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/correlations_auc.tex <==
name	auc
pcc	-0.10
spearman	0.07
kendall	0.08


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	6.97	10.89	9.39	3.94	17.84	6.95	12.59	6.72	11.04	9.30	3.60	18.48	7.44	13.39	3.65	8.25	6.31	1.60	14.90	6.65	11.07	926
0.03	5.60	8.01	7.40	4.32	11.71	3.69	10.05	5.31	8.40	7.46	3.44	13.36	4.96	10.24	3.55	6.90	5.22	1.30	12.51	5.60	8.31	999
0.06	4.87	6.45	6.08	3.93	8.97	2.52	7.72	4.51	6.80	5.92	2.42	11.18	4.38	7.88	3.07	5.17	4.34	1.89	8.46	3.29	6.15	1013
0.11	4.43	5.65	5.39	3.71	7.58	1.94	6.61	3.91	5.56	4.95	2.76	8.37	2.81	6.49	2.74	4.23	3.63	1.78	6.68	2.45	4.95	1014
0.15	3.87	4.81	4.73	3.35	6.28	1.46	5.70	3.30	4.55	4.09	2.13	6.96	2.42	5.23	2.44	3.52	3.10	1.28	5.76	2.24	4.03	1004
0.18	3.54	4.43	4.41	3.21	5.65	1.22	5.25	3.04	4.07	3.75	2.51	5.63	1.56	4.70	2.32	3.15	2.86	1.64	4.66	1.51	3.61	1016
0.32	3.29	3.97	4.00	2.97	4.96	0.99	4.62	2.79	3.55	3.34	2.43	4.68	1.13	4.08	2.13	2.77	2.62	1.74	3.81	1.03	3.22	2009


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/ets_sts_auc.tex <==
name	auc
et_use	1.65
et_tse	1.60
et_ce	1.24


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	3.80	15.58	7.13	-10.74	41.89	26.31	15.92	8.35	17.19	13.04	3.90	30.47	13.28	22.51	7.34	17.32	13.63	1.91	32.73	15.41	21.67	926
0.03	2.24	6.72	3.45	-8.40	21.85	15.13	5.59	7.77	11.51	10.39	5.62	17.39	5.89	14.33	6.52	11.08	9.49	4.07	18.08	7.00	14.10	999
0.06	1.46	3.06	2.00	-9.63	15.75	12.69	2.79	6.90	9.23	8.85	5.69	12.78	3.54	10.91	5.91	8.69	7.85	4.31	13.07	4.38	10.48	1013
0.11	1.00	1.63	1.30	-0.42	3.68	2.05	1.74	6.46	7.95	7.69	5.42	10.48	2.53	9.19	5.45	7.38	6.82	4.26	10.49	3.11	8.74	1014
0.15	0.61	0.87	0.76	0.28	1.46	0.59	1.00	5.62	6.65	6.48	4.86	8.43	1.78	7.49	4.84	6.14	5.77	3.86	8.42	2.28	7.01	1004
0.18	0.45	0.61	0.55	0.26	0.96	0.35	0.71	5.26	6.08	5.97	4.68	7.47	1.39	6.81	4.55	5.61	5.33	3.83	7.39	1.78	6.35	1016
0.32	0.25	0.38	0.34	0.20	0.56	0.18	0.46	4.69	5.38	5.28	4.28	6.48	1.10	5.96	4.08	4.92	4.73	3.60	6.24	1.32	5.51	2009


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.63
et_p_h	2.32
et_p_l2	2.17


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.03	0.06	0.05	0.02	0.10	0.04	0.08	0.02	0.03	0.03	0.01	0.05	0.02	0.04	0.02	0.03	0.03	0.01	0.04	0.01	0.04	926
0.03	0.09	0.15	0.14	0.06	0.23	0.09	0.20	0.04	0.05	0.05	0.03	0.08	0.03	0.07	0.04	0.05	0.05	0.03	0.07	0.02	0.06	999
0.06	0.21	0.30	0.29	0.17	0.43	0.13	0.38	0.06	0.08	0.07	0.05	0.10	0.03	0.09	0.06	0.07	0.07	0.05	0.09	0.02	0.08	1013
0.11	0.37	0.49	0.48	0.30	0.68	0.19	0.60	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.07	0.08	0.08	0.06	0.10	0.02	0.09	1014
0.15	0.69	0.90	0.88	0.58	1.22	0.32	1.10	0.10	0.12	0.12	0.08	0.15	0.03	0.14	0.09	0.10	0.10	0.08	0.13	0.02	0.12	1004
0.18	1.03	1.32	1.30	0.88	1.76	0.44	1.56	0.11	0.14	0.13	0.10	0.17	0.04	0.15	0.11	0.12	0.12	0.10	0.14	0.02	0.13	1016
0.32	1.66	2.39	2.21	1.38	3.40	1.01	3.00	0.14	0.16	0.16	0.13	0.20	0.04	0.19	0.13	0.15	0.14	0.12	0.17	0.02	0.16	2009


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.35
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.95	0.96	0.96	0.95	0.98	0.02	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.91	0.93	0.95	0.89	0.98	0.05	0.97	926
0.03	0.92	0.93	0.94	0.91	0.95	0.02	0.95	0.92	0.93	0.93	0.90	0.96	0.03	0.95	0.87	0.90	0.91	0.84	0.96	0.06	0.94	999
0.06	0.89	0.90	0.91	0.88	0.93	0.03	0.92	0.88	0.90	0.91	0.86	0.94	0.04	0.93	0.82	0.86	0.87	0.79	0.93	0.07	0.91	1013
0.11	0.87	0.88	0.89	0.85	0.91	0.03	0.90	0.85	0.87	0.88	0.83	0.92	0.04	0.90	0.78	0.82	0.83	0.75	0.90	0.07	0.87	1014
0.15	0.83	0.85	0.86	0.81	0.89	0.04	0.88	0.80	0.83	0.84	0.78	0.89	0.05	0.87	0.73	0.77	0.79	0.68	0.87	0.09	0.84	1004
0.18	0.81	0.83	0.84	0.78	0.88	0.05	0.86	0.77	0.81	0.81	0.75	0.87	0.06	0.85	0.70	0.74	0.75	0.64	0.84	0.10	0.80	1016
0.32	0.78	0.80	0.81	0.74	0.85	0.05	0.83	0.73	0.77	0.77	0.71	0.83	0.06	0.81	0.65	0.70	0.71	0.59	0.80	0.11	0.76	2009


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.24


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	4.29	12.15	7.74	2.72	21.59	9.44	18.06	1.62	2.38	2.23	1.39	3.38	0.99	3.04	4.85	13.23	9.93	1.89	24.58	11.34	18.78	926
0.03	4.16	4.42	4.37	4.18	4.65	0.24	4.58	2.04	2.76	2.64	1.74	3.78	1.02	3.35	5.86	17.30	12.91	2.46	32.15	14.85	24.87	999
0.06	5.32	5.61	5.55	4.46	6.76	1.15	5.78	2.36	3.06	2.92	2.03	4.09	1.03	3.68	6.24	18.63	14.54	3.12	34.15	15.51	28.14	1013
0.11	6.74	7.05	6.96	6.69	7.42	0.36	7.50	2.52	3.21	3.11	2.19	4.24	1.03	3.77	7.05	19.87	15.74	3.73	36.01	16.14	29.12	1014
0.15	22.60	30.70	35.17	22.81	38.58	7.88	38.88	2.57	3.26	3.18	2.28	4.24	0.98	3.81	7.21	19.91	15.50	3.55	36.26	16.35	28.84	1004
0.18	11.38	12.06	11.73	11.34	12.79	0.72	12.64	2.70	3.39	3.29	2.39	4.39	1.00	3.95	7.96	20.36	16.66	4.33	36.40	16.04	29.26	1016
0.32	14.26	16.82	17.87	13.75	19.89	3.07	19.19	2.79	3.49	3.37	2.48	4.51	1.01	4.06	8.01	20.46	16.38	4.21	36.71	16.25	29.29	2009


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/time_misc_auc.tex <==
name	auc
attack_time	4.15
l2	1.01
lom	6.07


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.64	0.68	0.68	0.56	0.79	0.11	0.73	0.78	0.82	0.82	0.75	0.89	0.07	0.87	0.85	0.88	0.89	0.83	0.93	0.05	0.92	926
0.03	0.45	0.54	0.55	0.42	0.66	0.12	0.63	0.71	0.75	0.76	0.68	0.83	0.07	0.81	0.80	0.83	0.83	0.78	0.89	0.05	0.87	999
0.06	0.32	0.41	0.41	0.28	0.53	0.12	0.50	0.64	0.68	0.69	0.61	0.76	0.07	0.73	0.75	0.79	0.79	0.73	0.84	0.05	0.82	1013
0.11	0.23	0.31	0.32	0.19	0.43	0.12	0.37	0.58	0.63	0.63	0.55	0.70	0.07	0.68	0.72	0.75	0.75	0.70	0.80	0.05	0.78	1014
0.15	0.14	0.20	0.19	0.10	0.30	0.10	0.27	0.50	0.55	0.54	0.47	0.62	0.07	0.59	0.67	0.70	0.70	0.65	0.75	0.05	0.73	1004
0.18	0.08	0.15	0.14	0.05	0.25	0.10	0.20	0.44	0.48	0.49	0.41	0.55	0.07	0.53	0.62	0.65	0.66	0.60	0.70	0.05	0.68	1016
0.32	0.05	0.10	0.09	0.01	0.19	0.09	0.14	0.32	0.37	0.37	0.29	0.46	0.08	0.43	0.54	0.58	0.58	0.52	0.64	0.06	0.62	2009


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/ig/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.17
top50	0.22


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	53.82	75.32	69.86	46.53	104.11	28.79	93.29	32.00	39.08	40.00	27.09	51.06	11.99	49.00	57.87	81.64	75.48	50.80	112.48	30.84	98.87	31.00	38.90	40.00	26.88	50.92	12.02	49.00	946
0.03	53.69	73.66	68.71	43.94	103.37	29.72	89.06	29.00	37.65	38.00	24.92	50.38	12.73	46.00	65.81	89.06	83.72	54.92	123.20	34.14	106.70	28.00	37.31	37.00	24.65	49.97	12.66	46.00	1002
0.06	53.39	73.77	68.45	43.47	104.08	30.31	89.29	28.00	37.47	38.00	24.69	50.25	12.78	46.00	76.34	102.85	97.31	63.43	142.27	39.42	122.76	28.00	36.87	37.00	24.25	49.48	12.61	46.00	1009
0.11	53.49	73.90	68.22	43.80	103.99	30.09	89.18	29.00	37.72	38.00	24.94	50.49	12.77	47.00	88.79	118.79	111.42	74.66	162.93	44.14	140.79	28.00	37.02	37.00	24.32	49.72	12.70	46.00	1016
0.15	54.05	74.31	69.05	44.12	104.49	30.18	89.60	28.00	37.61	38.00	24.76	50.45	12.84	46.00	113.98	149.90	142.47	98.99	200.82	50.92	175.91	28.00	36.89	37.00	24.14	49.64	12.75	46.00	1000
0.18	54.16	74.33	69.09	44.23	104.43	30.10	89.53	29.00	37.68	38.00	24.89	50.47	12.79	46.00	144.15	184.49	176.53	124.31	244.67	60.18	214.00	27.00	36.33	36.00	23.64	49.02	12.69	45.00	995
0.32	54.11	74.33	69.10	44.40	104.27	29.93	89.50	29.00	37.68	38.00	24.92	50.44	12.76	46.25	200.49	267.96	253.39	174.98	360.93	92.98	323.38	26.00	34.97	35.00	22.43	47.51	12.54	43.25	1976


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/comparison_vals_auc.tex <==
name	auc
orig_pp	23.03
orig_ge	11.70
adv_pp	52.05
adv_ge	11.31


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.54	0.63	0.63	0.47	0.78	0.15	0.73	0.85	0.88	0.91	0.78	0.99	0.10	0.95	0.76	0.80	0.82	0.66	0.94	0.14	0.88	946
0.03	0.37	0.47	0.47	0.32	0.61	0.15	0.57	0.75	0.80	0.82	0.67	0.93	0.13	0.89	0.63	0.70	0.71	0.57	0.83	0.13	0.79	1002
0.06	0.25	0.34	0.33	0.21	0.47	0.13	0.42	0.65	0.71	0.72	0.59	0.83	0.12	0.80	0.53	0.59	0.60	0.47	0.72	0.12	0.67	1009
0.11	0.16	0.24	0.23	0.12	0.36	0.12	0.31	0.54	0.61	0.62	0.48	0.75	0.14	0.71	0.43	0.49	0.50	0.37	0.62	0.12	0.57	1016
0.15	0.06	0.13	0.12	0.03	0.24	0.10	0.19	0.37	0.47	0.47	0.33	0.61	0.14	0.55	0.29	0.37	0.37	0.26	0.48	0.11	0.44	1000
0.18	-0.01	0.06	0.05	-0.03	0.15	0.09	0.11	0.25	0.35	0.34	0.20	0.49	0.15	0.44	0.20	0.27	0.27	0.16	0.38	0.11	0.34	995
0.32	-0.11	-0.05	-0.06	-0.15	0.05	0.10	0.01	0.03	0.15	0.15	-0.02	0.32	0.17	0.26	0.03	0.11	0.11	-0.01	0.24	0.12	0.20	1976


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/correlations_auc.tex <==
name	auc
pcc	0.05
spearman	0.14
kendall	0.12


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.99	6.03	5.14	2.25	9.80	3.77	7.34	4.05	6.79	5.81	2.44	11.14	4.35	8.14	2.81	5.89	4.49	1.31	10.47	4.58	7.34	946
0.03	3.54	5.04	4.59	2.78	7.30	2.26	6.09	3.37	5.62	4.79	2.27	8.97	3.35	6.90	2.78	6.01	4.55	1.11	10.92	4.91	7.51	1002
0.06	3.23	4.29	4.04	2.70	5.87	1.58	5.01	3.05	4.63	4.08	2.07	7.18	2.56	5.53	2.24	4.58	3.54	0.83	8.32	3.75	5.52	1009
0.11	3.09	3.85	3.73	2.67	5.02	1.17	4.48	2.76	3.99	3.58	1.91	6.07	2.08	4.66	2.09	3.74	2.94	0.81	6.66	2.92	4.41	1016
0.15	2.88	3.46	3.44	2.51	4.40	0.94	4.06	2.43	3.38	3.13	1.90	4.86	1.48	3.87	1.87	2.87	2.45	1.04	4.70	1.83	3.29	1000
0.18	2.68	3.22	3.25	2.42	4.03	0.80	3.79	2.26	2.99	2.78	1.88	4.09	1.11	3.43	1.80	2.47	2.22	1.34	3.59	1.12	2.89	995
0.32	2.55	2.96	2.96	2.31	3.60	0.64	3.36	2.11	2.68	2.53	1.86	3.49	0.81	3.04	1.68	2.19	2.04	1.33	3.04	0.86	2.49	1976


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/ets_sts_auc.tex <==
name	auc
et_use	1.13
et_tse	1.13
et_ce	1.02


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.13	5.33	2.14	-15.56	26.21	20.88	4.02	3.58	7.32	5.12	-3.98	18.61	11.29	7.26	2.82	7.73	4.60	-4.52	19.98	12.25	7.95	946
0.03	0.87	2.24	1.20	-6.27	10.74	8.51	1.83	3.55	5.08	4.58	2.72	7.43	2.36	6.14	3.04	4.96	4.16	1.83	8.08	3.12	6.06	1002
0.06	0.62	1.09	0.81	-1.71	3.90	2.81	1.10	3.52	4.51	4.26	3.02	6.01	1.49	5.29	3.00	4.26	3.82	2.31	6.20	1.95	4.94	1009
0.11	0.48	0.70	0.60	-0.05	1.46	0.75	0.79	3.45	4.24	4.04	3.05	5.44	1.20	4.83	2.95	3.96	3.63	2.39	5.52	1.57	4.53	1016
0.15	0.33	0.45	0.41	0.18	0.72	0.27	0.51	3.26	3.89	3.79	2.97	4.82	0.92	4.36	2.83	3.58	3.37	2.41	4.75	1.17	4.06	1000
0.18	0.25	0.34	0.30	0.03	0.65	0.31	0.38	3.18	3.71	3.63	2.93	4.49	0.78	4.16	2.77	3.41	3.24	2.41	4.42	1.01	3.82	995
0.32	0.15	0.22	0.20	0.06	0.38	0.16	0.26	3.07	3.48	3.42	2.85	4.11	0.63	3.81	2.69	3.20	3.07	2.39	4.01	0.81	3.55	1976


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.25
et_p_h	1.27
et_p_l2	1.19


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.09	0.08	0.04	0.15	0.05	0.13	0.02	0.04	0.04	0.02	0.07	0.02	0.06	0.03	0.04	0.04	0.02	0.05	0.02	0.05	946
0.03	0.15	0.22	0.22	0.12	0.32	0.10	0.29	0.05	0.07	0.06	0.04	0.09	0.03	0.08	0.05	0.06	0.06	0.04	0.08	0.02	0.07	1002
0.06	0.32	0.42	0.40	0.26	0.57	0.16	0.51	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.07	0.08	0.08	0.06	0.10	0.02	0.09	1009
0.11	0.50	0.64	0.63	0.42	0.87	0.22	0.77	0.09	0.11	0.10	0.08	0.14	0.03	0.12	0.08	0.09	0.09	0.07	0.11	0.02	0.11	1016
0.15	0.86	1.09	1.06	0.73	1.46	0.36	1.30	0.11	0.13	0.13	0.10	0.16	0.03	0.15	0.10	0.12	0.12	0.09	0.14	0.02	0.13	1000
0.18	1.26	1.60	1.55	1.08	2.12	0.52	1.89	0.12	0.15	0.15	0.11	0.18	0.03	0.17	0.12	0.13	0.13	0.11	0.15	0.02	0.14	995
0.32	1.97	2.84	2.62	1.64	4.04	1.20	3.51	0.15	0.17	0.17	0.14	0.21	0.04	0.19	0.14	0.15	0.15	0.13	0.18	0.02	0.17	1976


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.42
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.01	0.97	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.94	0.95	0.96	0.92	0.99	0.03	0.98	946
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.93	0.94	0.95	0.91	0.97	0.03	0.96	0.91	0.93	0.94	0.87	0.98	0.06	0.97	1002
0.06	0.90	0.92	0.92	0.89	0.94	0.03	0.93	0.90	0.91	0.92	0.88	0.95	0.04	0.94	0.86	0.89	0.91	0.83	0.96	0.07	0.94	1009
0.11	0.88	0.89	0.90	0.86	0.93	0.03	0.91	0.87	0.89	0.89	0.84	0.93	0.04	0.92	0.82	0.86	0.87	0.79	0.94	0.07	0.91	1016
0.15	0.85	0.87	0.87	0.82	0.91	0.04	0.89	0.83	0.85	0.86	0.80	0.90	0.05	0.89	0.77	0.81	0.82	0.72	0.90	0.09	0.87	1000
0.18	0.83	0.84	0.86	0.80	0.89	0.04	0.87	0.80	0.83	0.83	0.77	0.88	0.05	0.86	0.74	0.78	0.79	0.69	0.87	0.09	0.84	995
0.32	0.80	0.81	0.82	0.77	0.86	0.05	0.84	0.75	0.79	0.79	0.73	0.85	0.06	0.83	0.69	0.73	0.74	0.63	0.83	0.10	0.79	1976


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.61	10.82	6.63	1.85	19.78	8.97	15.79	39.16	59.46	55.07	29.83	89.09	29.63	70.75	3.81	11.68	9.61	-2.88	26.24	14.56	14.24	946
0.03	3.82	5.94	4.03	1.42	10.46	4.52	4.32	51.68	74.65	67.91	42.44	106.86	32.21	91.74	4.14	12.48	9.07	-1.26	26.23	13.74	17.24	1002
0.06	4.69	6.54	5.00	4.05	9.03	2.49	9.35	61.20	87.31	80.58	50.92	123.71	36.40	106.66	5.04	14.26	11.33	1.36	27.16	12.90	20.41	1009
0.11	5.87	6.99	6.05	5.30	8.68	1.69	8.95	68.63	97.58	89.54	56.25	138.92	41.34	118.14	5.92	16.17	13.20	0.97	31.37	15.20	22.01	1016
0.15	7.61	8.59	7.97	7.22	9.96	1.37	9.98	76.14	107.19	100.26	63.87	150.51	43.32	131.09	6.72	16.33	13.52	3.95	28.71	12.38	23.44	1000
0.18	8.84	9.92	9.23	8.48	11.36	1.44	11.24	79.58	114.30	105.78	68.03	160.57	46.27	139.94	6.41	16.58	14.31	3.96	29.20	12.62	23.86	995
0.32	12.25	14.21	14.65	12.30	16.12	1.91	15.27	84.67	120.97	112.05	71.39	170.56	49.58	146.31	6.19	16.40	13.17	3.37	29.44	13.03	23.59	1976


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/time_misc_auc.tex <==
name	auc
attack_time	2.97
l2	32.33
lom	4.87


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.60	0.67	0.68	0.53	0.81	0.14	0.76	0.80	0.84	0.85	0.72	0.95	0.11	0.90	0.88	0.90	0.91	0.82	0.99	0.08	0.95	946
0.03	0.44	0.52	0.53	0.38	0.65	0.13	0.62	0.72	0.76	0.77	0.67	0.86	0.09	0.82	0.83	0.86	0.87	0.79	0.93	0.07	0.91	1002
0.06	0.31	0.38	0.38	0.25	0.51	0.13	0.46	0.63	0.69	0.69	0.59	0.78	0.10	0.75	0.78	0.82	0.82	0.74	0.89	0.07	0.86	1009
0.11	0.20	0.29	0.27	0.16	0.41	0.12	0.36	0.57	0.62	0.62	0.52	0.71	0.09	0.68	0.74	0.77	0.77	0.70	0.84	0.07	0.82	1016
0.15	0.11	0.18	0.18	0.08	0.28	0.10	0.24	0.47	0.52	0.51	0.44	0.60	0.08	0.58	0.68	0.71	0.71	0.65	0.77	0.06	0.75	1000
0.18	0.05	0.11	0.09	0.03	0.20	0.09	0.17	0.38	0.44	0.44	0.36	0.53	0.08	0.50	0.62	0.66	0.67	0.60	0.72	0.06	0.70	995
0.32	0.00	0.05	0.05	-0.01	0.11	0.06	0.09	0.25	0.32	0.32	0.23	0.41	0.09	0.38	0.53	0.58	0.58	0.51	0.65	0.07	0.63	1976


==> data/mlm_plots/mlm_distil_fast/imdb/lstm/s/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.16
top50	0.22


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	54.04	75.36	68.97	46.65	104.07	28.71	93.29	30.75	38.57	40.00	26.32	50.82	12.25	49.00	57.35	80.12	74.54	50.19	110.05	29.93	98.27	31.00	38.45	39.00	26.17	50.73	12.28	49.00	920
0.03	53.78	74.23	68.91	43.91	104.54	30.32	88.96	29.00	37.79	38.00	25.14	50.45	12.65	47.00	63.26	86.69	81.94	53.08	120.29	33.61	102.84	28.00	37.50	37.50	24.96	50.05	12.55	46.00	992
0.06	53.64	74.41	68.71	43.44	105.38	30.97	89.03	28.00	37.70	38.00	24.88	50.51	12.81	47.00	71.87	98.34	92.13	59.86	136.82	38.48	115.60	28.00	37.20	37.00	24.51	49.88	12.68	46.00	1000
0.11	53.64	74.34	68.70	43.31	105.37	31.03	88.98	28.00	37.77	38.00	24.89	50.64	12.88	47.00	83.17	111.85	104.49	69.52	154.18	42.33	132.67	28.00	37.08	37.00	24.36	49.80	12.72	46.00	1007
0.15	53.82	74.44	68.72	43.47	105.41	30.97	89.08	28.00	37.80	38.00	24.89	50.71	12.91	47.00	104.35	139.06	130.94	87.79	190.34	51.27	161.76	28.00	37.18	38.00	24.32	50.03	12.85	47.00	1001
0.18	53.82	74.44	68.72	43.47	105.41	30.97	89.08	28.00	37.80	38.00	24.89	50.71	12.91	47.00	130.22	170.07	160.69	110.45	229.69	59.62	200.03	27.00	36.72	37.00	23.94	49.50	12.78	45.00	1001
0.32	53.82	74.41	68.71	43.57	105.25	30.84	88.95	28.00	37.79	38.00	24.95	50.63	12.84	47.00	178.97	241.12	227.56	155.66	326.57	85.45	289.44	26.00	35.65	36.00	22.92	48.37	12.72	44.00	1993


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/comparison_vals_auc.tex <==
name	auc
orig_pp	23.11
orig_ge	11.74
adv_pp	48.03
adv_ge	11.42


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.38	0.54	0.55	0.35	0.73	0.19	0.68	0.90	0.92	0.93	0.87	0.98	0.05	0.96	0.80	0.84	0.84	0.77	0.91	0.07	0.88	920
0.03	0.22	0.35	0.33	0.18	0.51	0.17	0.46	0.80	0.84	0.85	0.75	0.93	0.09	0.90	0.67	0.73	0.74	0.63	0.82	0.10	0.79	992
0.06	0.10	0.20	0.18	0.06	0.34	0.14	0.28	0.66	0.73	0.75	0.62	0.85	0.12	0.82	0.55	0.62	0.62	0.51	0.72	0.11	0.69	1000
0.11	0.03	0.11	0.09	-0.00	0.23	0.11	0.17	0.55	0.63	0.64	0.50	0.77	0.14	0.73	0.45	0.52	0.52	0.40	0.63	0.12	0.60	1007
0.15	-0.03	0.02	0.00	-0.06	0.10	0.08	0.05	0.39	0.49	0.50	0.33	0.64	0.16	0.59	0.31	0.39	0.39	0.27	0.51	0.12	0.47	1001
0.18	-0.07	-0.03	-0.04	-0.10	0.03	0.06	-0.01	0.27	0.37	0.38	0.21	0.54	0.17	0.48	0.22	0.30	0.30	0.17	0.42	0.13	0.38	1001
0.32	-0.15	-0.11	-0.11	-0.17	-0.05	0.06	-0.07	0.09	0.21	0.21	0.02	0.41	0.19	0.35	0.07	0.17	0.17	0.03	0.31	0.14	0.27	1993


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/correlations_auc.tex <==
name	auc
pcc	0.02
spearman	0.15
kendall	0.13


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	4.39	6.83	6.01	3.17	10.48	3.66	8.55	4.22	7.69	6.54	2.95	12.42	4.73	10.59	3.22	6.92	5.46	1.54	12.30	5.38	9.62	920
0.03	3.89	5.66	5.17	2.92	8.40	2.74	6.75	3.71	5.96	5.20	2.48	9.43	3.47	7.21	2.86	5.94	4.56	1.06	10.81	4.87	7.26	992
0.06	3.60	4.75	4.48	2.85	6.65	1.90	5.50	3.24	4.95	4.39	1.92	7.97	3.02	5.74	2.48	4.49	3.55	1.07	7.91	3.42	5.42	1000
0.11	3.38	4.21	4.08	2.78	5.63	1.42	4.87	2.92	4.21	3.79	1.81	6.61	2.40	4.88	2.20	3.66	2.99	1.06	6.26	2.60	4.38	1007
0.15	3.11	3.72	3.67	2.73	4.71	0.99	4.27	2.55	3.48	3.22	2.10	4.86	1.38	3.98	1.97	2.91	2.51	1.29	4.54	1.62	3.32	1001
0.18	2.85	3.35	3.37	2.54	4.16	0.81	3.81	2.32	3.07	2.83	1.93	4.22	1.15	3.56	1.80	2.48	2.23	1.24	3.73	1.25	2.88	1001
0.32	2.57	2.95	2.98	2.30	3.60	0.65	3.36	2.06	2.64	2.46	1.81	3.48	0.83	3.02	1.63	2.12	1.97	1.23	3.01	0.89	2.41	1993


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/ets_sts_auc.tex <==
name	auc
et_use	1.21
et_tse	1.18
et_ce	1.02


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.10	11.38	3.36	-24.05	46.81	35.43	5.84	4.65	8.78	7.08	1.97	15.59	6.81	11.21	4.16	9.35	6.86	0.32	18.39	9.04	10.98	920
0.03	1.32	3.53	1.83	-6.34	13.40	9.87	2.88	4.66	6.79	6.17	3.49	10.08	3.30	8.02	3.92	6.63	5.57	2.27	10.99	4.36	7.92	992
0.06	0.92	1.75	1.18	-3.25	6.75	5.00	1.65	4.61	5.98	5.54	3.79	8.17	2.19	6.89	3.86	5.71	4.91	2.74	8.68	2.97	6.68	1000
0.11	0.66	1.04	0.84	-0.13	2.20	1.16	1.13	4.38	5.30	5.11	3.87	6.73	1.43	5.99	3.69	4.95	4.53	3.00	6.89	1.95	5.67	1007
0.15	0.43	0.66	0.54	-0.27	1.59	0.93	0.70	3.98	4.69	4.53	3.63	5.76	1.07	5.21	3.38	4.33	4.00	2.88	5.78	1.45	4.88	1001
0.18	0.31	0.44	0.38	0.18	0.69	0.25	0.49	3.71	4.32	4.22	3.44	5.19	0.88	4.73	3.19	3.97	3.74	2.82	5.13	1.16	4.46	1001
0.32	0.18	0.27	0.25	0.14	0.40	0.13	0.33	3.41	3.90	3.78	3.18	4.63	0.73	4.24	2.97	3.60	3.40	2.63	4.56	0.96	3.95	1993


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.40
et_p_h	1.54
et_p_l2	1.45


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.04	0.07	0.07	0.03	0.12	0.05	0.10	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.04	920
0.03	0.12	0.18	0.18	0.09	0.27	0.09	0.24	0.04	0.06	0.06	0.04	0.09	0.03	0.08	0.04	0.05	0.05	0.04	0.07	0.02	0.07	992
0.06	0.25	0.34	0.34	0.20	0.49	0.14	0.42	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.09	1000
0.11	0.41	0.54	0.53	0.34	0.74	0.20	0.66	0.08	0.10	0.10	0.07	0.13	0.03	0.12	0.08	0.09	0.09	0.07	0.11	0.02	0.10	1007
0.15	0.71	0.93	0.92	0.59	1.27	0.34	1.14	0.10	0.12	0.12	0.09	0.15	0.03	0.14	0.10	0.11	0.11	0.09	0.13	0.02	0.12	1001
0.18	1.05	1.39	1.35	0.89	1.88	0.49	1.67	0.12	0.14	0.14	0.11	0.17	0.03	0.16	0.11	0.12	0.12	0.10	0.14	0.02	0.14	1001
0.32	1.67	2.45	2.26	1.38	3.51	1.06	3.04	0.14	0.16	0.16	0.13	0.20	0.04	0.19	0.13	0.15	0.15	0.12	0.17	0.02	0.16	1993


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.36
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.95	0.96	0.96	0.95	0.98	0.02	0.97	0.95	0.96	0.97	0.95	0.98	0.02	0.98	0.93	0.95	0.96	0.90	1.00	0.05	0.98	920
0.03	0.92	0.93	0.94	0.91	0.96	0.02	0.95	0.92	0.93	0.94	0.90	0.96	0.03	0.95	0.89	0.92	0.93	0.86	0.97	0.06	0.96	992
0.06	0.89	0.91	0.91	0.87	0.94	0.03	0.93	0.88	0.90	0.91	0.86	0.95	0.04	0.93	0.84	0.87	0.89	0.80	0.95	0.07	0.93	1000
0.11	0.87	0.88	0.89	0.85	0.92	0.04	0.91	0.85	0.88	0.88	0.83	0.93	0.05	0.91	0.80	0.84	0.85	0.76	0.92	0.08	0.90	1007
0.15	0.84	0.86	0.87	0.82	0.90	0.04	0.88	0.81	0.84	0.85	0.79	0.89	0.05	0.88	0.75	0.80	0.80	0.71	0.88	0.09	0.85	1001
0.18	0.82	0.84	0.85	0.79	0.88	0.05	0.86	0.78	0.81	0.82	0.75	0.87	0.06	0.85	0.71	0.76	0.77	0.66	0.85	0.10	0.82	1001
0.32	0.78	0.80	0.81	0.75	0.86	0.06	0.84	0.73	0.77	0.77	0.71	0.83	0.06	0.82	0.66	0.70	0.72	0.59	0.82	0.11	0.77	1993


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.62	10.62	7.10	2.39	18.85	8.23	15.39	0.13	0.17	0.16	0.10	0.24	0.07	0.20	6.16	19.02	14.40	0.74	37.31	18.29	26.37	920
0.03	3.49	3.64	3.55	3.45	3.82	0.19	3.73	0.17	0.22	0.21	0.15	0.29	0.07	0.25	7.65	23.26	17.67	2.64	43.88	20.62	33.97	992
0.06	4.63	4.85	4.79	4.60	5.10	0.25	5.02	0.20	0.25	0.24	0.18	0.33	0.07	0.29	10.39	28.05	21.50	5.01	51.09	23.04	40.69	1000
0.11	5.64	5.87	5.80	5.57	6.16	0.29	6.10	0.22	0.27	0.26	0.20	0.34	0.07	0.31	9.33	28.91	22.99	4.82	53.00	24.09	41.92	1007
0.15	6.84	7.16	7.02	6.75	7.56	0.41	7.43	0.24	0.28	0.27	0.21	0.34	0.06	0.31	11.68	30.51	24.80	6.27	54.76	24.25	44.12	1001
0.18	9.03	9.37	9.26	8.89	9.84	0.47	9.59	0.23	0.28	0.27	0.22	0.33	0.06	0.31	11.63	29.80	24.28	6.72	52.88	23.08	43.60	1001
0.32	11.77	13.36	13.10	11.75	14.97	1.61	14.61	0.22	0.26	0.25	0.20	0.31	0.05	0.28	10.69	27.92	23.70	6.59	49.25	21.33	40.33	1993


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/time_misc_auc.tex <==
name	auc
attack_time	2.63
l2	0.08
lom	8.77


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.55	0.63	0.62	0.49	0.76	0.13	0.73	0.81	0.85	0.86	0.77	0.92	0.07	0.90	0.90	0.93	0.93	0.88	0.97	0.04	0.96	920
0.03	0.36	0.45	0.45	0.32	0.58	0.13	0.55	0.71	0.76	0.78	0.68	0.85	0.09	0.82	0.84	0.88	0.88	0.82	0.94	0.06	0.92	992
0.06	0.23	0.31	0.31	0.18	0.44	0.13	0.41	0.62	0.67	0.68	0.58	0.76	0.09	0.74	0.78	0.82	0.83	0.76	0.89	0.06	0.87	1000
0.11	0.12	0.20	0.19	0.08	0.32	0.12	0.27	0.53	0.60	0.60	0.50	0.69	0.10	0.66	0.73	0.78	0.78	0.71	0.85	0.07	0.82	1007
0.15	0.00	0.10	0.09	0.01	0.18	0.09	0.14	0.43	0.49	0.49	0.40	0.59	0.10	0.56	0.67	0.72	0.72	0.64	0.79	0.07	0.76	1001
0.18	0.00	0.05	0.00	-0.01	0.11	0.06	0.08	0.36	0.42	0.42	0.32	0.51	0.10	0.48	0.62	0.67	0.68	0.59	0.75	0.08	0.72	1001
0.32	0.00	0.01	0.00	-0.02	0.05	0.04	0.00	0.24	0.31	0.31	0.21	0.42	0.10	0.38	0.55	0.61	0.61	0.52	0.69	0.09	0.67	1993


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/a/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.16
top50	0.22


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	54.03	76.30	70.42	47.55	105.05	28.75	93.81	30.25	38.51	40.00	26.35	50.66	12.15	48.00	57.73	80.90	75.40	50.84	110.96	30.06	98.59	30.00	38.49	40.00	26.30	50.69	12.20	48.00	934
0.03	53.60	74.36	68.70	43.31	105.42	31.05	88.88	29.00	37.81	38.00	25.08	50.55	12.74	47.00	61.50	85.45	79.84	50.96	119.94	34.49	101.05	28.75	37.61	38.00	24.86	50.37	12.76	47.00	984
0.06	53.65	74.45	68.72	43.34	105.55	31.10	89.13	28.00	37.72	38.00	24.82	50.62	12.90	47.00	70.62	96.12	90.80	59.24	132.99	36.88	112.57	28.00	37.43	38.00	24.54	50.33	12.89	46.00	997
0.11	53.63	74.37	68.71	43.31	105.42	31.05	88.99	28.00	37.74	38.00	24.83	50.64	12.91	47.00	81.18	109.36	102.25	68.51	150.22	40.86	128.67	28.00	37.48	38.00	24.51	50.45	12.97	47.00	1002
0.15	53.82	74.43	68.81	43.44	105.42	30.99	89.01	28.00	37.76	38.00	24.89	50.63	12.87	47.00	102.99	136.28	128.27	87.98	184.59	48.31	160.39	28.00	37.48	38.00	24.43	50.54	13.06	46.00	1009
0.18	53.82	74.47	68.76	43.50	105.44	30.97	89.08	28.00	37.72	38.00	24.87	50.57	12.85	47.00	125.62	164.09	154.55	108.17	220.01	55.92	193.64	27.00	37.03	37.00	24.09	49.98	12.94	46.00	1005
0.32	53.66	74.32	68.72	43.69	104.95	30.63	89.05	28.00	37.76	38.00	24.94	50.57	12.82	47.00	174.31	233.11	220.78	150.65	315.58	82.47	278.48	26.00	36.01	36.00	23.24	48.78	12.77	45.00	2007


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	23.12
orig_ge	11.73
adv_pp	46.65
adv_ge	11.51


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.03	0.25	0.23	-0.07	0.56	0.32	0.44	0.48	0.59	0.62	0.39	0.79	0.20	0.74	0.39	0.50	0.50	0.32	0.68	0.18	0.63	934
0.03	-0.20	0.01	0.00	-0.30	0.32	0.31	0.20	0.35	0.45	0.48	0.24	0.67	0.21	0.59	0.28	0.38	0.39	0.20	0.56	0.18	0.50	984
0.06	-0.35	-0.17	-0.19	-0.44	0.11	0.28	0.01	0.21	0.32	0.33	0.12	0.52	0.20	0.45	0.18	0.27	0.28	0.11	0.44	0.16	0.38	997
0.11	-0.44	-0.27	-0.30	-0.54	-0.01	0.26	-0.13	0.11	0.22	0.23	0.03	0.41	0.19	0.33	0.11	0.20	0.20	0.05	0.34	0.15	0.29	1002
0.15	-0.50	-0.37	-0.39	-0.58	-0.15	0.22	-0.25	-0.01	0.09	0.10	-0.08	0.25	0.16	0.19	0.02	0.09	0.10	-0.03	0.22	0.12	0.17	1009
0.18	-0.58	-0.45	-0.47	-0.65	-0.26	0.20	-0.34	-0.11	-0.02	-0.01	-0.17	0.13	0.15	0.09	-0.06	0.02	0.02	-0.10	0.13	0.12	0.09	1005
0.32	-0.67	-0.55	-0.57	-0.73	-0.37	0.18	-0.44	-0.28	-0.17	-0.17	-0.32	-0.02	0.15	-0.07	-0.18	-0.10	-0.10	-0.22	0.01	0.12	-0.02	2007


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/correlations_auc.tex <==
name	auc
pcc	-0.11
spearman	0.03
kendall	0.03


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	6.83	11.30	10.45	4.74	17.87	6.57	14.26	6.75	11.89	10.45	3.94	19.83	7.95	15.45	4.10	9.32	6.44	1.05	17.59	8.27	11.74	934
0.03	5.85	8.93	7.90	4.12	13.74	4.81	10.77	5.73	9.29	7.96	3.37	15.22	5.92	11.34	3.78	8.08	6.06	1.28	14.87	6.80	9.80	984
0.06	5.08	7.04	6.53	3.99	10.09	3.05	8.28	4.66	7.21	6.32	3.04	11.37	4.16	8.51	3.30	6.11	4.75	1.59	10.64	4.52	7.16	997
0.11	4.59	6.01	5.75	3.83	8.20	2.18	7.06	4.11	5.90	5.29	2.96	8.84	2.94	6.94	2.93	4.90	4.00	1.33	8.48	3.57	5.58	1002
0.15	4.04	5.03	4.91	3.53	6.54	1.51	5.85	3.48	4.72	4.33	2.72	6.72	2.00	5.47	2.57	3.78	3.34	1.73	5.82	2.04	4.47	1009
0.18	3.74	4.56	4.51	3.33	5.78	1.22	5.32	3.16	4.14	3.83	2.51	5.77	1.63	4.70	2.40	3.29	3.02	1.69	4.90	1.61	3.81	1005
0.32	3.37	4.03	4.02	3.06	5.01	0.97	4.64	2.83	3.54	3.36	2.43	4.66	1.11	4.02	2.16	2.81	2.65	1.74	3.88	1.07	3.27	2007


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/ets_sts_auc.tex <==
name	auc
et_use	1.74
et_tse	1.67
et_ce	1.37


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	3.13	12.58	6.44	-9.75	34.90	22.33	13.10	7.89	15.81	13.20	4.33	27.28	11.48	20.40	6.92	16.19	12.95	3.76	28.62	12.43	21.72	934
0.03	2.09	6.20	3.26	-12.18	24.58	18.38	5.27	7.17	11.53	10.07	4.59	18.48	6.94	13.84	6.11	11.18	9.06	3.00	19.37	8.18	13.30	984
0.06	1.43	2.89	1.91	-4.17	9.96	7.07	2.72	6.73	9.30	8.66	5.24	13.36	4.06	11.06	5.81	8.83	7.68	3.43	14.23	5.40	10.29	997
0.11	0.97	1.74	1.31	-0.92	4.41	2.67	1.78	6.17	8.05	7.64	5.12	10.98	2.93	9.36	5.23	7.46	6.68	3.99	10.92	3.47	8.82	1002
0.15	0.62	0.90	0.80	0.33	1.48	0.58	1.03	5.64	6.80	6.53	4.88	8.72	1.92	7.64	4.78	6.26	5.79	3.90	8.61	2.35	7.17	1009
0.18	0.46	0.65	0.59	0.23	1.07	0.42	0.75	5.21	6.23	6.05	4.64	7.81	1.58	7.04	4.44	5.69	5.40	3.75	7.63	1.94	6.50	1005
0.32	0.26	0.41	0.36	0.02	0.80	0.39	0.49	4.73	5.51	5.39	4.30	6.73	1.22	6.16	4.08	5.03	4.81	3.53	6.54	1.51	5.71	2007


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.59
et_p_h	2.34
et_p_l2	2.19


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.03	0.07	0.06	0.02	0.12	0.05	0.09	0.02	0.03	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.04	934
0.03	0.10	0.16	0.16	0.07	0.25	0.09	0.22	0.04	0.06	0.05	0.03	0.08	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.06	984
0.06	0.22	0.32	0.30	0.18	0.46	0.14	0.39	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	997
0.11	0.37	0.51	0.50	0.31	0.71	0.20	0.64	0.08	0.10	0.10	0.07	0.13	0.03	0.12	0.07	0.08	0.08	0.06	0.11	0.02	0.10	1002
0.15	0.69	0.90	0.86	0.57	1.22	0.32	1.09	0.10	0.12	0.12	0.09	0.15	0.03	0.14	0.09	0.11	0.11	0.08	0.13	0.02	0.12	1009
0.18	0.99	1.30	1.27	0.85	1.75	0.45	1.56	0.11	0.14	0.14	0.10	0.17	0.03	0.16	0.11	0.12	0.12	0.10	0.14	0.02	0.14	1005
0.32	1.61	2.33	2.16	1.32	3.34	1.01	2.89	0.14	0.16	0.16	0.13	0.20	0.03	0.19	0.13	0.14	0.14	0.12	0.17	0.02	0.16	2007


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.34
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.98	0.92	0.94	0.95	0.89	0.98	0.05	0.97	934
0.03	0.92	0.94	0.94	0.91	0.96	0.02	0.95	0.92	0.93	0.94	0.91	0.96	0.03	0.96	0.88	0.91	0.92	0.85	0.97	0.06	0.95	984
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.88	0.90	0.91	0.86	0.94	0.04	0.93	0.83	0.87	0.88	0.80	0.94	0.07	0.92	997
0.11	0.87	0.89	0.89	0.85	0.92	0.03	0.91	0.85	0.88	0.88	0.83	0.92	0.05	0.91	0.79	0.83	0.84	0.75	0.91	0.08	0.89	1002
0.15	0.84	0.85	0.86	0.81	0.90	0.04	0.88	0.81	0.84	0.84	0.78	0.89	0.05	0.87	0.74	0.78	0.79	0.69	0.88	0.09	0.85	1009
0.18	0.81	0.83	0.84	0.78	0.88	0.05	0.86	0.77	0.81	0.81	0.75	0.86	0.06	0.84	0.71	0.75	0.76	0.64	0.85	0.10	0.81	1005
0.32	0.78	0.80	0.81	0.74	0.85	0.05	0.83	0.73	0.77	0.77	0.71	0.82	0.06	0.81	0.64	0.69	0.71	0.58	0.80	0.11	0.76	2007


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.24


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	5.12	19.59	12.43	2.14	37.04	17.45	30.02	2.31	7.11	4.18	-11.50	25.73	18.61	5.91	5.41	17.32	12.64	0.97	33.67	16.35	25.06	934
0.03	5.27	5.84	5.60	4.78	6.90	1.06	6.04	3.12	20.87	5.11	-113.03	154.77	133.90	7.56	5.71	19.64	13.70	0.03	39.25	19.61	28.23	984
0.06	6.37	6.94	6.65	5.97	7.92	0.97	7.00	3.82	43.33	5.71	-402.95	489.60	446.27	8.12	6.39	21.27	15.04	0.28	42.25	20.99	29.56	997
0.11	9.06	10.23	9.76	8.89	11.57	1.34	11.44	4.14	115.35	5.98	-2356.44	2587.14	2471.79	8.89	7.36	23.47	16.53	0.98	45.95	22.48	32.70	1002
0.15	11.29	12.23	11.92	10.87	13.59	1.36	12.66	4.21	277.44	6.02	-2760.06	3314.93	3037.49	9.09	8.24	23.84	17.93	2.03	45.66	21.82	33.12	1009
0.18	15.72	16.70	16.34	15.15	18.26	1.56	17.76	4.24	421.34	5.98	-6231.91	7074.58	6653.24	8.77	8.91	24.79	18.59	2.42	47.16	22.37	35.26	1005
0.32	17.37	20.63	20.47	17.27	23.98	3.36	23.15	4.29	792.44	5.89	-15281.69	16866.57	16074.13	8.26	9.03	25.14	19.19	2.99	47.29	22.15	35.93	2007


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/time_misc_auc.tex <==
name	auc
attack_time	4.37
l2	107.82
lom	7.29


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.41	0.53	0.53	0.34	0.71	0.19	0.64	0.60	0.68	0.70	0.56	0.81	0.13	0.78	0.72	0.77	0.78	0.69	0.86	0.09	0.84	934
0.03	0.31	0.41	0.41	0.24	0.57	0.16	0.50	0.54	0.61	0.62	0.48	0.74	0.13	0.70	0.68	0.73	0.73	0.63	0.82	0.09	0.79	984
0.06	0.22	0.30	0.31	0.16	0.44	0.14	0.40	0.48	0.55	0.56	0.43	0.66	0.12	0.62	0.63	0.68	0.69	0.60	0.77	0.09	0.74	997
0.11	0.14	0.24	0.23	0.11	0.37	0.13	0.32	0.43	0.50	0.50	0.39	0.61	0.11	0.56	0.60	0.65	0.65	0.56	0.73	0.08	0.70	1002
0.15	0.09	0.16	0.14	0.05	0.27	0.11	0.23	0.37	0.43	0.44	0.34	0.53	0.09	0.49	0.56	0.60	0.61	0.53	0.68	0.07	0.65	1009
0.18	0.05	0.12	0.11	0.03	0.22	0.10	0.18	0.32	0.38	0.38	0.29	0.47	0.09	0.44	0.53	0.57	0.57	0.50	0.64	0.07	0.61	1005
0.32	0.00	0.08	0.07	0.00	0.16	0.08	0.13	0.25	0.31	0.31	0.22	0.39	0.09	0.36	0.47	0.51	0.52	0.44	0.58	0.07	0.56	2007


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/ig/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.14
top50	0.19


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	54.37	75.83	71.12	48.13	103.52	27.69	93.29	31.00	38.60	40.00	26.25	50.96	12.36	49.00	59.99	83.02	76.21	53.19	112.85	29.83	102.33	31.00	38.39	39.00	26.14	50.63	12.25	48.00	894
0.03	53.67	74.21	68.78	43.95	104.47	30.26	89.13	29.00	37.89	38.00	25.10	50.68	12.79	47.00	66.29	90.51	85.03	56.25	124.76	34.26	108.17	28.00	37.52	37.50	24.86	50.18	12.66	46.00	978
0.06	53.69	74.24	68.77	43.77	104.72	30.47	89.03	28.00	37.75	38.00	24.89	50.61	12.86	47.00	76.60	103.48	97.72	65.23	141.72	38.24	123.47	28.00	37.15	38.00	24.45	49.84	12.69	46.00	1001
0.11	53.84	74.45	68.78	43.45	105.46	31.01	89.06	28.00	37.80	38.00	24.91	50.69	12.89	47.00	90.38	120.28	115.07	76.47	164.08	43.81	142.77	28.00	37.16	37.00	24.41	49.90	12.75	46.00	1006
0.15	53.65	74.39	68.74	43.35	105.43	31.04	89.06	28.00	37.75	38.00	24.85	50.65	12.90	47.00	114.07	150.53	143.52	96.55	204.51	53.98	175.99	28.00	37.24	37.00	24.33	50.16	12.92	46.00	1006
0.18	53.72	74.38	68.73	43.39	105.37	30.99	89.04	28.00	37.79	38.00	24.92	50.67	12.88	47.00	140.99	183.89	176.59	120.29	247.48	63.59	216.61	28.00	36.79	36.00	23.89	49.69	12.90	46.00	1006
0.32	53.66	74.19	68.67	43.58	104.81	30.61	88.88	29.00	37.82	38.00	25.00	50.65	12.83	47.00	194.89	262.61	246.71	165.19	360.03	97.42	316.16	27.00	35.69	36.00	22.97	48.40	12.72	44.00	1996


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/comparison_vals_auc.tex <==
name	auc
orig_pp	23.09
orig_ge	11.74
adv_pp	51.81
adv_ge	11.43


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.49	0.59	0.61	0.42	0.75	0.16	0.71	0.79	0.84	0.88	0.72	0.96	0.12	0.93	0.62	0.70	0.73	0.57	0.83	0.13	0.79	894
0.03	0.33	0.43	0.43	0.27	0.58	0.15	0.54	0.63	0.73	0.76	0.57	0.90	0.16	0.85	0.48	0.58	0.59	0.43	0.73	0.15	0.69	978
0.06	0.20	0.29	0.30	0.15	0.43	0.14	0.39	0.46	0.60	0.62	0.40	0.80	0.20	0.75	0.34	0.46	0.46	0.29	0.63	0.17	0.58	1001
0.11	0.12	0.20	0.20	0.07	0.33	0.13	0.29	0.34	0.48	0.50	0.26	0.70	0.22	0.64	0.25	0.36	0.37	0.20	0.53	0.17	0.47	1006
0.15	0.03	0.11	0.11	-0.01	0.23	0.12	0.19	0.15	0.32	0.32	0.09	0.55	0.23	0.49	0.12	0.24	0.24	0.08	0.41	0.17	0.36	1006
0.18	-0.03	0.04	0.04	-0.07	0.16	0.11	0.12	0.03	0.20	0.19	-0.03	0.43	0.23	0.35	0.04	0.16	0.15	-0.00	0.32	0.16	0.25	1006
0.32	-0.13	-0.05	-0.06	-0.17	0.06	0.11	0.02	-0.13	0.03	0.01	-0.19	0.25	0.22	0.17	-0.07	0.03	0.02	-0.11	0.18	0.15	0.13	1996


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.10
kendall	0.08


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	4.36	7.43	6.43	2.79	12.07	4.64	8.96	4.31	7.89	6.52	2.77	13.01	5.12	10.47	3.29	7.50	6.08	1.90	13.10	5.60	9.56	894
0.03	3.87	5.74	5.22	2.90	8.58	2.84	6.93	3.61	6.20	5.39	2.32	10.07	3.87	7.53	2.85	6.54	5.16	1.60	11.48	4.94	8.67	978
0.06	3.55	4.82	4.53	2.94	6.70	1.88	5.69	3.16	5.09	4.32	1.82	8.36	3.27	6.09	2.45	5.04	3.79	0.93	9.16	4.12	6.30	1001
0.11	3.29	4.21	4.07	2.74	5.68	1.47	4.84	2.69	4.15	3.63	1.73	6.57	2.42	4.87	2.15	4.05	3.10	0.70	7.39	3.34	4.67	1006
0.15	2.93	3.66	3.64	2.62	4.70	1.04	4.32	2.31	3.31	2.99	1.75	4.87	1.56	3.88	1.92	3.03	2.49	0.88	5.19	2.16	3.50	1006
0.18	2.72	3.32	3.35	2.48	4.16	0.84	3.83	2.19	2.98	2.69	1.59	4.37	1.39	3.44	1.80	2.63	2.27	0.91	4.35	1.72	3.00	1006
0.32	2.55	2.97	2.98	2.30	3.63	0.66	3.38	2.05	2.63	2.45	1.74	3.51	0.88	3.00	1.66	2.24	2.05	1.07	3.41	1.17	2.56	1996


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/ets_sts_auc.tex <==
name	auc
et_use	1.22
et_tse	1.18
et_ce	1.11


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.28	4.09	2.07	-4.63	12.81	8.72	3.35	3.82	7.26	5.74	1.67	12.86	5.60	8.64	3.46	7.43	5.39	1.08	13.78	6.35	8.93	894
0.03	0.90	1.65	1.24	-0.33	3.63	1.98	1.78	3.81	5.62	4.96	2.66	8.59	2.97	6.62	3.27	5.64	4.53	1.76	9.51	3.87	6.70	978
0.06	0.65	1.16	0.86	-1.04	3.36	2.20	1.13	3.72	5.01	4.64	2.83	7.19	2.18	5.72	3.26	4.87	4.13	1.84	7.90	3.03	5.59	1001
0.11	0.48	0.72	0.62	0.24	1.20	0.48	0.82	3.62	4.58	4.34	3.08	6.07	1.50	5.24	3.14	4.36	3.94	2.35	6.38	2.02	5.01	1006
0.15	0.32	0.51	0.42	-0.21	1.23	0.72	0.54	3.41	4.09	3.95	3.08	5.09	1.01	4.65	2.95	3.82	3.52	2.44	5.20	1.38	4.40	1006
0.18	0.24	0.35	0.31	0.15	0.55	0.20	0.40	3.27	3.86	3.73	3.02	4.70	0.84	4.33	2.86	3.59	3.37	2.49	4.69	1.10	4.11	1006
0.32	0.15	0.24	0.21	0.04	0.43	0.20	0.28	3.12	3.59	3.50	2.90	4.27	0.68	3.95	2.75	3.33	3.17	2.44	4.22	0.89	3.72	1996


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.23
et_p_h	1.34
et_p_l2	1.28


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.10	0.10	0.05	0.15	0.05	0.13	0.02	0.04	0.03	0.02	0.06	0.02	0.05	0.03	0.04	0.04	0.02	0.05	0.01	0.04	894
0.03	0.16	0.23	0.23	0.14	0.33	0.10	0.30	0.04	0.06	0.06	0.04	0.09	0.03	0.08	0.05	0.06	0.06	0.04	0.07	0.02	0.07	978
0.06	0.32	0.42	0.41	0.27	0.57	0.15	0.51	0.07	0.08	0.08	0.06	0.11	0.03	0.10	0.06	0.08	0.08	0.06	0.09	0.02	0.09	1001
0.11	0.50	0.66	0.65	0.43	0.88	0.23	0.79	0.08	0.10	0.10	0.07	0.13	0.03	0.12	0.08	0.09	0.09	0.07	0.11	0.02	0.10	1006
0.15	0.83	1.09	1.06	0.73	1.46	0.37	1.33	0.10	0.13	0.12	0.09	0.16	0.03	0.15	0.10	0.11	0.11	0.09	0.13	0.02	0.13	1006
0.18	1.20	1.58	1.54	1.05	2.11	0.53	1.90	0.12	0.14	0.14	0.11	0.17	0.03	0.16	0.11	0.13	0.13	0.11	0.15	0.02	0.14	1006
0.32	1.89	2.76	2.55	1.54	3.97	1.21	3.43	0.14	0.17	0.17	0.13	0.20	0.03	0.19	0.13	0.15	0.15	0.13	0.17	0.02	0.17	1996


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.42
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.99	0.02	0.98	0.94	0.95	0.97	0.92	0.99	0.04	0.98	894
0.03	0.93	0.94	0.95	0.92	0.97	0.02	0.96	0.93	0.94	0.95	0.90	0.98	0.04	0.96	0.91	0.93	0.94	0.87	0.99	0.06	0.97	978
0.06	0.91	0.92	0.92	0.89	0.95	0.03	0.94	0.89	0.91	0.92	0.87	0.96	0.05	0.94	0.86	0.89	0.91	0.82	0.96	0.07	0.94	1001
0.11	0.89	0.90	0.90	0.86	0.93	0.03	0.92	0.86	0.88	0.89	0.83	0.93	0.05	0.92	0.82	0.86	0.87	0.78	0.94	0.08	0.92	1006
0.15	0.86	0.87	0.88	0.83	0.91	0.04	0.89	0.81	0.84	0.85	0.79	0.90	0.06	0.88	0.77	0.81	0.82	0.72	0.90	0.09	0.87	1006
0.18	0.83	0.85	0.86	0.80	0.89	0.05	0.87	0.79	0.82	0.82	0.76	0.88	0.06	0.86	0.74	0.78	0.79	0.69	0.87	0.09	0.84	1006
0.32	0.80	0.81	0.82	0.76	0.86	0.05	0.84	0.74	0.78	0.79	0.72	0.84	0.06	0.82	0.68	0.73	0.74	0.62	0.83	0.11	0.79	1996


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	5.17	18.24	10.55	1.98	34.51	16.26	28.27	42.87	93.40	75.62	24.30	162.49	69.09	129.12	5.72	16.48	13.06	2.78	30.18	13.70	22.62	894
0.03	4.59	4.75	4.69	4.53	4.96	0.21	4.86	50.58	117.46	96.72	32.05	202.86	85.40	160.68	7.38	21.22	17.12	3.77	38.66	17.44	30.38	978
0.06	5.57	5.76	5.69	5.50	6.01	0.26	5.88	66.04	141.09	122.48	45.04	237.13	96.05	188.48	9.12	25.09	20.37	4.73	45.45	20.36	35.87	1001
0.11	7.01	7.28	7.38	6.89	7.67	0.39	7.58	75.55	152.32	133.31	56.30	248.34	96.02	206.22	10.72	27.44	21.86	5.90	48.98	21.54	40.22	1006
0.15	8.84	9.16	9.03	8.65	9.66	0.51	9.41	89.92	175.33	154.28	62.76	287.90	112.57	230.54	12.55	30.70	26.42	7.73	53.67	22.97	44.06	1006
0.18	10.87	11.28	11.21	10.74	11.82	0.54	11.38	95.49	182.49	163.23	66.56	298.41	115.93	238.21	12.72	31.66	26.44	7.75	55.57	23.91	45.83	1006
0.32	12.71	15.27	14.55	12.66	17.88	2.61	17.64	98.83	182.83	164.56	70.55	295.12	112.28	235.80	12.41	30.58	24.51	7.80	53.37	22.78	45.57	1996


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/time_misc_auc.tex <==
name	auc
attack_time	3.21
l2	50.93
lom	8.86


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.43	0.55	0.57	0.39	0.72	0.17	0.68	0.72	0.76	0.78	0.65	0.87	0.11	0.84	0.81	0.85	0.87	0.78	0.93	0.07	0.90	894
0.03	0.32	0.42	0.42	0.26	0.58	0.16	0.54	0.60	0.67	0.68	0.55	0.79	0.12	0.76	0.74	0.80	0.80	0.71	0.88	0.09	0.86	978
0.06	0.20	0.31	0.31	0.16	0.45	0.15	0.41	0.50	0.58	0.58	0.46	0.71	0.12	0.66	0.67	0.73	0.74	0.64	0.83	0.10	0.80	1001
0.11	0.14	0.24	0.23	0.10	0.37	0.14	0.32	0.43	0.51	0.52	0.39	0.64	0.12	0.59	0.62	0.68	0.69	0.59	0.78	0.10	0.75	1006
0.15	0.07	0.16	0.14	0.04	0.27	0.11	0.23	0.35	0.43	0.43	0.31	0.55	0.12	0.51	0.55	0.62	0.62	0.52	0.72	0.10	0.69	1006
0.18	0.05	0.11	0.09	0.01	0.21	0.10	0.17	0.29	0.37	0.37	0.26	0.48	0.11	0.44	0.51	0.57	0.57	0.48	0.67	0.10	0.64	1006
0.32	0.00	0.06	0.05	-0.02	0.13	0.08	0.09	0.21	0.28	0.28	0.18	0.38	0.10	0.34	0.45	0.51	0.51	0.42	0.60	0.09	0.56	1996


==> data/mlm_plots/mlm_distil_fast/imdb/lstmatt/s/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.14
top50	0.20


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.26	59.11	53.25	35.37	82.85	23.74	71.12	15.00	19.64	19.00	13.39	25.90	6.26	23.00	45.90	64.34	58.55	39.06	89.63	25.28	78.37	15.00	19.70	19.00	13.42	25.98	6.28	23.00	903
0.03	42.58	59.46	53.30	34.88	84.04	24.58	72.94	14.00	18.64	19.00	11.75	25.54	6.90	23.00	50.63	71.78	65.84	43.01	100.55	28.77	88.85	14.00	18.76	19.00	11.74	25.77	7.02	23.00	974
0.06	42.38	60.15	54.01	34.71	85.59	25.44	73.03	14.00	18.43	18.00	11.53	25.33	6.90	23.00	58.85	82.78	76.19	50.32	115.24	32.46	100.85	14.00	18.78	18.00	11.66	25.91	7.13	23.00	994
0.11	42.31	60.12	54.00	34.69	85.54	25.43	73.02	14.00	18.43	18.00	11.48	25.38	6.95	23.00	68.51	94.69	87.73	58.57	130.81	36.12	113.35	14.00	18.98	19.00	11.68	26.27	7.30	24.00	999
0.15	42.22	59.90	53.66	34.52	85.29	25.39	72.56	14.00	18.51	18.00	11.62	25.40	6.89	23.00	87.56	118.71	110.76	74.62	162.80	44.09	140.61	15.00	19.65	19.00	12.25	27.04	7.40	24.00	988
0.18	42.24	59.92	53.75	34.56	85.29	25.37	72.63	14.00	18.47	18.00	11.56	25.39	6.92	23.00	108.35	144.48	134.84	93.27	195.69	51.21	172.76	15.00	19.77	19.00	12.24	27.30	7.53	24.00	990
0.32	42.29	60.10	54.00	34.88	85.32	25.22	72.99	14.00	18.46	18.00	11.58	25.34	6.88	23.00	152.07	206.81	194.63	130.68	282.95	76.14	249.44	15.00	20.18	20.00	12.43	27.93	7.75	25.00	1971


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/comparison_vals_auc.tex <==
name	auc
orig_pp	18.61
orig_ge	5.75
adv_pp	40.83
adv_ge	6.06


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.46	0.58	0.60	0.38	0.77	0.19	0.72	0.93	0.95	0.96	0.91	0.99	0.04	0.98	0.82	0.85	0.86	0.79	0.91	0.06	0.89	903
0.03	0.26	0.38	0.39	0.20	0.56	0.18	0.51	0.87	0.90	0.92	0.84	0.97	0.06	0.95	0.72	0.77	0.78	0.69	0.85	0.08	0.83	974
0.06	0.09	0.22	0.20	0.07	0.37	0.15	0.31	0.80	0.84	0.86	0.76	0.93	0.09	0.91	0.63	0.69	0.70	0.60	0.78	0.09	0.76	994
0.11	0.03	0.13	0.10	0.00	0.25	0.12	0.20	0.73	0.79	0.81	0.68	0.90	0.11	0.87	0.56	0.63	0.64	0.52	0.73	0.11	0.71	999
0.15	-0.02	0.05	0.02	-0.05	0.14	0.09	0.09	0.64	0.71	0.73	0.58	0.85	0.14	0.82	0.48	0.55	0.56	0.43	0.67	0.12	0.64	988
0.18	-0.04	0.00	-0.01	-0.07	0.08	0.08	0.03	0.55	0.64	0.66	0.48	0.81	0.16	0.77	0.40	0.48	0.49	0.35	0.62	0.14	0.58	990
0.32	-0.09	-0.05	-0.05	-0.12	0.03	0.08	-0.02	0.37	0.50	0.53	0.29	0.72	0.21	0.67	0.25	0.37	0.38	0.20	0.53	0.16	0.49	1971


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/correlations_auc.tex <==
name	auc
pcc	0.03
spearman	0.22
kendall	0.17


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.78	7.18	6.02	2.35	12.00	4.82	9.26	3.35	7.30	5.85	1.68	12.92	5.62	9.48	2.57	6.58	4.69	0.84	12.31	5.73	8.76	903
0.03	3.79	5.90	5.34	2.65	9.15	3.25	7.17	2.99	5.78	4.68	1.55	10.00	4.23	7.14	2.42	5.67	4.04	0.87	10.47	4.80	7.50	974
0.06	3.54	4.81	4.65	2.91	6.71	1.90	5.67	2.77	4.61	3.95	1.51	7.71	3.10	5.55	2.20	4.08	3.15	0.99	7.17	3.09	4.92	994
0.11	3.32	4.23	4.12	2.88	5.59	1.36	4.94	2.63	3.88	3.48	1.67	6.09	2.21	4.59	2.10	3.41	2.84	1.13	5.69	2.28	4.01	999
0.15	3.13	3.70	3.71	2.75	4.65	0.95	4.31	2.42	3.24	3.00	1.94	4.54	1.30	3.73	1.93	2.72	2.37	1.25	4.18	1.46	3.11	988
0.18	2.83	3.31	3.34	2.50	4.11	0.80	3.86	2.28	2.93	2.73	1.88	3.99	1.05	3.35	1.80	2.44	2.20	1.10	3.78	1.34	2.73	990
0.32	2.50	2.90	2.92	2.24	3.56	0.66	3.33	2.11	2.60	2.48	1.84	3.36	0.76	2.92	1.62	2.04	1.91	1.22	2.87	0.83	2.33	1971


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/ets_sts_auc.tex <==
name	auc
et_use	1.22
et_tse	1.12
et_ce	0.97


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.32	4.01	2.27	-4.07	12.09	8.08	3.97	3.43	6.89	5.83	1.88	11.90	5.01	8.51	3.12	7.17	5.35	0.86	13.49	6.32	8.86	903
0.03	1.01	2.04	1.44	-2.36	6.45	4.41	2.10	3.81	5.98	5.43	2.99	8.96	2.98	7.23	3.28	5.74	4.79	2.09	9.40	3.66	6.91	974
0.06	0.76	1.29	0.99	-2.14	4.72	3.43	1.35	4.04	5.41	5.16	3.39	7.43	2.02	6.27	3.44	5.01	4.46	2.42	7.60	2.59	5.89	994
0.11	0.58	0.83	0.72	0.39	1.27	0.44	0.97	3.95	4.91	4.75	3.48	6.34	1.43	5.60	3.29	4.44	4.10	2.63	6.25	1.81	5.08	999
0.15	0.38	0.51	0.47	0.30	0.73	0.21	0.59	3.65	4.30	4.20	3.28	5.31	1.01	4.81	3.03	3.82	3.57	2.57	5.06	1.24	4.30	988
0.18	0.27	0.37	0.34	0.22	0.51	0.14	0.42	3.36	3.89	3.81	3.07	4.71	0.82	4.31	2.81	3.43	3.26	2.43	4.43	1.00	3.81	990
0.32	0.16	0.23	0.21	0.13	0.34	0.11	0.28	3.01	3.45	3.36	2.79	4.10	0.66	3.77	2.53	3.03	2.89	2.26	3.80	0.77	3.35	1971


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.25
et_p_h	1.38
et_p_l2	1.26


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.09	0.09	0.05	0.14	0.05	0.12	0.02	0.04	0.04	0.02	0.06	0.02	0.06	0.03	0.04	0.04	0.02	0.05	0.02	0.05	903
0.03	0.15	0.22	0.21	0.13	0.31	0.09	0.27	0.04	0.07	0.06	0.04	0.10	0.03	0.09	0.04	0.06	0.06	0.04	0.08	0.02	0.07	974
0.06	0.30	0.40	0.39	0.25	0.55	0.15	0.49	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.07	0.08	0.08	0.06	0.10	0.02	0.09	994
0.11	0.45	0.61	0.61	0.40	0.82	0.21	0.75	0.09	0.11	0.11	0.08	0.14	0.03	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.11	999
0.15	0.82	1.05	1.02	0.69	1.40	0.35	1.24	0.11	0.13	0.13	0.10	0.17	0.03	0.15	0.10	0.12	0.11	0.09	0.14	0.02	0.13	988
0.18	1.19	1.52	1.48	0.99	2.05	0.53	1.81	0.13	0.15	0.15	0.12	0.19	0.04	0.18	0.12	0.13	0.13	0.11	0.15	0.02	0.14	990
0.32	1.85	2.65	2.45	1.56	3.74	1.09	3.26	0.16	0.18	0.18	0.14	0.22	0.04	0.21	0.14	0.16	0.16	0.13	0.18	0.02	0.17	1971


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.40
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.02	0.98	0.95	0.96	0.97	0.93	0.99	0.03	0.98	0.93	0.95	0.96	0.91	0.99	0.04	0.98	903
0.03	0.93	0.94	0.94	0.91	0.96	0.02	0.95	0.90	0.93	0.94	0.89	0.97	0.04	0.96	0.88	0.91	0.93	0.85	0.97	0.06	0.96	974
0.06	0.90	0.91	0.92	0.87	0.95	0.04	0.93	0.87	0.89	0.90	0.84	0.94	0.05	0.93	0.83	0.87	0.87	0.79	0.95	0.08	0.92	994
0.11	0.88	0.89	0.89	0.85	0.93	0.04	0.91	0.84	0.87	0.87	0.81	0.92	0.05	0.90	0.80	0.84	0.84	0.75	0.92	0.09	0.89	999
0.15	0.85	0.86	0.87	0.82	0.91	0.04	0.89	0.81	0.84	0.84	0.78	0.89	0.05	0.87	0.76	0.79	0.80	0.71	0.88	0.09	0.84	988
0.18	0.82	0.84	0.85	0.79	0.89	0.05	0.87	0.78	0.81	0.82	0.76	0.87	0.05	0.85	0.73	0.76	0.77	0.66	0.86	0.10	0.82	990
0.32	0.79	0.81	0.82	0.76	0.86	0.05	0.84	0.75	0.78	0.79	0.73	0.84	0.06	0.82	0.68	0.71	0.73	0.61	0.82	0.10	0.77	1971


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	6.73	8.74	9.38	6.55	10.93	2.19	10.45	0.11	0.18	0.16	0.08	0.28	0.10	0.22	5.24	16.31	11.68	0.86	31.76	15.45	22.40	903
0.03	6.53	9.00	8.63	5.70	12.30	3.30	11.62	0.15	0.24	0.21	0.12	0.36	0.12	0.30	5.55	18.76	13.86	1.72	35.81	17.04	26.42	974
0.06	8.10	10.18	10.10	6.99	13.36	3.19	11.99	0.21	0.32	0.29	0.18	0.46	0.14	0.40	8.54	24.62	18.35	3.82	45.43	20.80	36.29	994
0.11	11.33	14.19	13.97	9.79	18.58	4.39	16.70	0.26	0.38	0.36	0.22	0.55	0.16	0.48	8.70	28.02	21.80	4.41	51.63	23.61	41.62	999
0.15	17.16	21.91	21.81	15.12	28.71	6.79	25.80	0.32	0.45	0.42	0.28	0.63	0.18	0.57	12.46	30.97	25.44	7.36	54.57	23.61	44.36	988
0.18	20.04	25.34	25.04	17.35	33.32	7.99	29.59	0.32	0.46	0.42	0.28	0.65	0.19	0.58	12.15	31.30	26.11	7.01	55.59	24.29	44.96	990
0.32	28.58	37.91	36.33	24.45	51.38	13.46	45.70	0.28	0.42	0.36	0.22	0.62	0.20	0.51	11.62	30.75	25.99	6.51	54.98	24.24	43.66	1971


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/time_misc_auc.tex <==
name	auc
attack_time	6.93
l2	0.12
lom	8.80


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.62	0.69	0.71	0.57	0.81	0.12	0.78	0.84	0.87	0.88	0.82	0.93	0.06	0.92	0.92	0.93	0.94	0.90	0.97	0.04	0.96	903
0.03	0.45	0.54	0.56	0.40	0.69	0.15	0.64	0.76	0.81	0.82	0.73	0.89	0.08	0.86	0.87	0.90	0.90	0.85	0.95	0.05	0.93	974
0.06	0.31	0.41	0.42	0.25	0.57	0.16	0.50	0.68	0.74	0.75	0.65	0.83	0.09	0.81	0.83	0.86	0.87	0.81	0.92	0.06	0.90	994
0.11	0.20	0.32	0.32	0.16	0.49	0.16	0.44	0.62	0.69	0.70	0.59	0.79	0.10	0.76	0.79	0.83	0.84	0.77	0.90	0.06	0.88	999
0.15	0.10	0.23	0.22	0.06	0.40	0.17	0.33	0.56	0.62	0.63	0.51	0.74	0.11	0.70	0.75	0.79	0.80	0.72	0.87	0.07	0.85	988
0.18	0.05	0.17	0.14	0.01	0.32	0.15	0.26	0.48	0.57	0.57	0.44	0.70	0.13	0.66	0.71	0.76	0.76	0.68	0.84	0.08	0.82	990
0.32	0.00	0.10	0.05	-0.04	0.24	0.14	0.17	0.37	0.47	0.48	0.32	0.62	0.15	0.58	0.64	0.70	0.71	0.61	0.80	0.09	0.77	1971


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/a/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.19
top50	0.25


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.18	58.70	53.15	35.19	82.21	23.51	71.02	15.00	19.56	19.00	13.47	25.64	6.09	23.00	45.82	63.85	57.96	38.59	89.11	25.26	77.77	15.00	19.51	19.00	13.46	25.56	6.05	23.00	908
0.03	42.58	59.39	52.75	34.06	84.73	25.33	72.55	14.00	18.59	19.00	11.98	25.19	6.61	23.00	51.43	70.99	64.68	41.84	100.14	29.15	86.52	14.00	18.74	19.00	12.04	25.43	6.69	23.00	987
0.06	42.57	60.23	53.75	34.48	85.99	25.75	72.94	14.00	18.47	18.00	11.54	25.41	6.94	23.00	59.35	81.82	74.07	48.54	115.10	33.28	98.74	14.00	18.98	19.00	11.83	26.13	7.15	23.00	1010
0.11	42.38	60.15	53.84	34.83	85.47	25.32	73.03	14.00	18.42	18.00	11.50	25.34	6.92	23.00	66.92	93.60	84.85	56.41	130.80	37.19	111.66	14.00	19.55	20.00	12.23	26.86	7.31	24.00	1018
0.15	42.07	59.74	53.53	34.60	84.88	25.14	72.46	14.00	18.50	18.00	11.68	25.33	6.83	23.00	83.95	114.81	108.06	72.73	156.90	42.09	137.51	15.00	20.60	21.00	13.21	28.00	7.39	25.00	1004
0.18	42.57	60.03	54.01	34.91	85.16	25.12	72.75	14.00	18.47	18.00	11.56	25.37	6.90	23.00	104.80	140.48	132.76	90.00	190.96	50.48	167.77	16.00	21.36	21.00	13.66	29.06	7.70	26.00	994
0.32	42.57	60.24	54.14	34.97	85.50	25.27	73.13	14.00	18.53	18.00	11.61	25.45	6.92	23.00	144.91	199.97	188.38	125.02	274.91	74.94	242.18	17.00	22.74	23.00	14.56	30.93	8.19	28.00	1948


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	18.62
orig_ge	5.75
adv_pp	39.76
adv_ge	6.44


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.13	0.37	0.39	0.04	0.71	0.33	0.63	0.36	0.57	0.62	0.28	0.85	0.29	0.80	0.25	0.46	0.47	0.20	0.72	0.26	0.65	908
0.03	-0.09	0.12	0.10	-0.22	0.45	0.33	0.32	0.14	0.38	0.39	0.07	0.68	0.30	0.62	0.10	0.30	0.28	0.04	0.55	0.25	0.48	987
0.06	-0.24	-0.05	-0.05	-0.35	0.25	0.30	0.13	0.02	0.23	0.22	-0.05	0.51	0.28	0.45	0.02	0.18	0.16	-0.04	0.40	0.22	0.33	1010
0.11	-0.32	-0.16	-0.14	-0.43	0.12	0.27	-0.00	-0.05	0.14	0.12	-0.12	0.41	0.26	0.35	-0.03	0.11	0.09	-0.09	0.32	0.20	0.26	1018
0.15	-0.40	-0.26	-0.25	-0.51	-0.00	0.25	-0.10	-0.15	0.02	0.01	-0.22	0.26	0.24	0.18	-0.10	0.02	0.01	-0.16	0.20	0.18	0.14	1004
0.18	-0.48	-0.34	-0.34	-0.57	-0.10	0.24	-0.18	-0.22	-0.06	-0.08	-0.29	0.17	0.23	0.10	-0.15	-0.04	-0.05	-0.21	0.13	0.17	0.07	994
0.32	-0.59	-0.44	-0.46	-0.66	-0.22	0.22	-0.29	-0.36	-0.19	-0.21	-0.41	0.04	0.23	-0.04	-0.25	-0.13	-0.15	-0.29	0.04	0.16	-0.02	1948


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/correlations_auc.tex <==
name	auc
pcc	-0.07
spearman	0.01
kendall	0.01


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	5.58	11.20	9.43	3.15	19.24	8.04	14.83	4.63	11.22	8.77	2.32	20.12	8.90	15.14	3.77	9.73	6.79	0.42	19.04	9.31	12.26	908
0.03	5.99	10.24	8.71	3.96	16.51	6.28	13.39	5.00	10.34	8.22	2.43	18.25	7.91	13.06	4.01	9.78	6.96	0.61	18.95	9.17	11.62	987
0.06	5.30	7.71	6.96	3.96	11.45	3.74	9.35	4.29	7.52	6.51	2.87	12.16	4.65	9.55	3.47	7.05	5.48	1.20	12.89	5.84	8.69	1010
0.11	4.87	6.75	6.18	3.80	9.71	2.96	7.89	3.97	6.39	5.74	2.78	10.00	3.61	7.76	3.19	5.91	4.67	1.19	10.64	4.73	7.31	1018
0.15	4.30	5.61	5.29	3.47	7.75	2.14	6.50	3.45	5.19	4.80	2.74	7.63	2.44	6.30	2.90	4.56	3.78	1.71	7.40	2.85	5.47	1004
0.18	3.93	4.98	4.80	3.33	6.64	1.65	5.80	3.18	4.57	4.23	2.58	6.57	1.99	5.45	2.57	3.87	3.36	1.79	5.94	2.08	4.59	994
0.32	3.39	4.24	4.08	2.95	5.52	1.28	4.89	2.96	3.92	3.72	2.52	5.33	1.41	4.61	2.32	3.19	2.88	1.67	4.71	1.52	3.60	1948


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/ets_sts_auc.tex <==
name	auc
et_use	1.90
et_tse	1.81
et_ce	1.60


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.65	8.37	3.44	-12.84	29.59	21.21	6.86	4.58	11.46	8.54	0.95	21.97	10.51	14.71	4.01	11.56	8.05	0.03	23.09	11.53	14.39	908
0.03	1.36	4.21	2.16	-10.00	18.41	14.21	3.45	5.69	9.36	7.98	2.79	15.94	6.58	11.01	4.69	9.24	6.97	0.48	18.01	8.76	10.53	987
0.06	1.01	2.00	1.40	-2.93	6.93	4.93	1.97	5.42	7.54	7.03	3.11	11.97	4.43	8.74	4.45	6.89	6.06	2.83	10.95	4.06	8.10	1010
0.11	0.76	1.22	1.02	-0.02	2.46	1.24	1.37	5.16	6.66	6.34	4.22	9.10	2.44	7.68	4.27	5.97	5.48	3.34	8.59	2.62	6.98	1018
0.15	0.50	0.78	0.65	-0.15	1.71	0.93	0.87	4.64	5.74	5.52	4.09	7.38	1.64	6.67	3.86	5.08	4.81	3.30	6.87	1.78	5.99	1004
0.18	0.37	0.54	0.48	0.15	0.94	0.40	0.63	4.41	5.28	5.10	3.90	6.66	1.38	6.01	3.70	4.68	4.43	3.18	6.17	1.50	5.34	994
0.32	0.23	0.35	0.31	0.16	0.53	0.18	0.43	4.04	4.76	4.63	3.67	5.85	1.09	5.31	3.44	4.21	4.06	2.97	5.46	1.24	4.75	1948


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.42
et_p_h	1.94
et_p_l2	1.76


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.10	0.09	0.03	0.16	0.06	0.13	0.02	0.04	0.04	0.02	0.07	0.02	0.06	0.02	0.04	0.03	0.02	0.05	0.02	0.05	908
0.03	0.14	0.21	0.21	0.11	0.31	0.10	0.27	0.04	0.06	0.06	0.03	0.10	0.03	0.08	0.04	0.06	0.06	0.04	0.08	0.02	0.07	987
0.06	0.28	0.38	0.37	0.23	0.53	0.15	0.47	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.06	0.08	0.08	0.06	0.10	0.02	0.09	1010
0.11	0.43	0.59	0.56	0.35	0.82	0.23	0.71	0.08	0.11	0.10	0.07	0.14	0.03	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.10	1018
0.15	0.74	0.99	0.95	0.61	1.38	0.38	1.21	0.11	0.13	0.13	0.10	0.17	0.04	0.16	0.10	0.11	0.11	0.09	0.14	0.02	0.13	1004
0.18	1.08	1.45	1.38	0.89	2.00	0.56	1.74	0.13	0.15	0.15	0.11	0.19	0.04	0.17	0.12	0.13	0.13	0.11	0.15	0.02	0.15	994
0.32	1.71	2.53	2.32	1.38	3.67	1.14	3.13	0.15	0.18	0.18	0.14	0.22	0.04	0.20	0.14	0.16	0.16	0.13	0.18	0.03	0.17	1948


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.38
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.96	0.96	0.97	0.93	0.99	0.03	0.98	0.94	0.95	0.96	0.91	0.99	0.04	0.98	908
0.03	0.94	0.95	0.95	0.93	0.97	0.02	0.96	0.93	0.94	0.95	0.90	0.98	0.04	0.97	0.90	0.93	0.94	0.87	0.98	0.05	0.96	987
0.06	0.91	0.92	0.93	0.89	0.95	0.03	0.94	0.89	0.91	0.92	0.86	0.96	0.05	0.94	0.86	0.89	0.91	0.82	0.96	0.07	0.94	1010
0.11	0.89	0.91	0.91	0.87	0.94	0.03	0.92	0.86	0.89	0.90	0.84	0.94	0.05	0.93	0.82	0.87	0.88	0.80	0.93	0.07	0.92	1018
0.15	0.86	0.88	0.88	0.85	0.91	0.03	0.90	0.83	0.86	0.87	0.80	0.91	0.06	0.90	0.78	0.83	0.84	0.76	0.90	0.07	0.88	1004
0.18	0.84	0.86	0.86	0.82	0.89	0.04	0.88	0.80	0.83	0.84	0.77	0.89	0.06	0.88	0.75	0.79	0.80	0.71	0.88	0.08	0.85	994
0.32	0.80	0.82	0.83	0.78	0.86	0.04	0.85	0.76	0.80	0.80	0.74	0.86	0.06	0.84	0.70	0.74	0.75	0.66	0.83	0.09	0.80	1948


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.26


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	16.36	20.02	21.05	15.89	24.15	4.13	23.12	1.17	7.43	2.11	-4.92	19.78	12.35	7.38	3.43	15.51	8.68	-1.67	32.69	17.18	21.58	908
0.03	18.58	23.29	22.85	14.44	32.14	8.85	27.21	1.84	13.63	3.52	-8.71	35.97	22.34	16.71	4.88	19.55	12.07	0.28	38.81	19.26	28.66	987
0.06	25.00	32.57	30.43	11.71	53.44	20.86	35.80	2.42	16.26	5.72	-9.66	42.18	25.92	20.36	6.70	22.52	15.65	1.88	43.16	20.64	33.25	1010
0.11	31.54	41.00	38.16	20.13	61.87	20.87	44.73	2.84	17.81	6.96	-8.67	44.29	26.48	22.59	7.38	23.32	17.14	2.76	43.88	20.56	35.18	1018
0.15	49.79	65.11	61.96	41.28	88.94	23.83	75.91	3.33	19.77	10.05	-10.15	49.69	29.92	25.33	8.38	25.46	20.28	4.53	46.38	20.93	38.15	1004
0.18	32.56	53.82	47.83	26.91	80.73	26.91	70.87	3.43	18.75	10.54	-4.15	41.64	22.89	25.49	8.89	25.73	21.11	5.41	46.06	20.33	38.36	994
0.32	42.56	71.86	61.24	31.97	111.74	39.88	91.25	3.87	17.82	10.90	-2.65	38.29	20.47	24.42	9.91	26.30	21.57	6.03	46.57	20.27	39.19	1948


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/time_misc_auc.tex <==
name	auc
attack_time	15.89
l2	5.42
lom	7.53


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.29	0.48	0.47	0.24	0.72	0.24	0.67	0.49	0.63	0.63	0.44	0.81	0.19	0.78	0.63	0.74	0.74	0.60	0.87	0.13	0.84	908
0.03	0.15	0.33	0.30	0.11	0.55	0.22	0.50	0.38	0.52	0.51	0.34	0.70	0.18	0.65	0.56	0.66	0.65	0.53	0.79	0.13	0.76	987
0.06	0.11	0.24	0.21	0.07	0.42	0.18	0.35	0.33	0.44	0.43	0.28	0.60	0.16	0.55	0.52	0.61	0.60	0.49	0.72	0.12	0.69	1010
0.11	0.07	0.19	0.17	0.04	0.35	0.15	0.29	0.30	0.40	0.39	0.26	0.55	0.15	0.50	0.49	0.57	0.56	0.46	0.68	0.11	0.65	1018
0.15	0.05	0.14	0.12	0.01	0.27	0.13	0.21	0.25	0.34	0.33	0.21	0.47	0.13	0.43	0.46	0.53	0.53	0.43	0.63	0.10	0.60	1004
0.18	0.00	0.11	0.08	-0.00	0.23	0.11	0.18	0.22	0.31	0.30	0.19	0.43	0.12	0.38	0.44	0.50	0.49	0.41	0.60	0.09	0.57	994
0.32	0.00	0.07	0.06	-0.02	0.17	0.10	0.12	0.17	0.25	0.24	0.14	0.36	0.11	0.33	0.39	0.46	0.45	0.36	0.55	0.09	0.52	1948


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/ig/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.11
top50	0.17


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.28	58.40	53.12	35.18	81.61	23.21	70.23	15.00	19.58	19.00	13.30	25.86	6.28	23.00	46.66	64.09	58.07	39.00	89.18	25.09	77.15	15.00	19.60	19.00	13.35	25.86	6.25	23.00	876
0.03	42.23	59.10	52.56	34.01	84.20	25.10	72.42	14.00	18.65	19.00	11.77	25.53	6.88	23.00	51.38	71.90	64.80	42.71	101.08	29.19	88.33	14.00	18.77	19.00	11.93	25.60	6.84	23.00	972
0.06	42.58	60.26	53.82	34.49	86.02	25.77	73.03	14.00	18.51	18.00	11.64	25.38	6.87	23.00	61.42	84.46	77.50	50.87	118.04	33.59	101.02	14.00	18.73	19.00	11.87	25.58	6.85	23.00	1018
0.11	42.07	60.05	53.53	34.57	85.54	25.48	73.58	14.00	18.42	18.00	11.56	25.29	6.87	23.00	70.35	97.53	90.20	59.70	135.36	37.83	117.17	14.00	18.82	19.00	11.93	25.70	6.89	23.00	1030
0.15	42.56	59.71	54.00	34.84	84.59	24.87	71.65	14.00	18.39	18.00	11.62	25.16	6.77	23.00	90.07	122.72	115.13	77.24	168.20	45.48	144.51	15.00	19.23	19.00	12.40	26.07	6.84	23.00	1033
0.18	42.57	59.98	53.92	34.70	85.27	25.29	73.00	14.00	18.44	18.00	11.58	25.29	6.86	23.00	111.43	150.12	140.06	95.74	204.50	54.38	176.85	15.00	19.53	20.00	12.52	26.54	7.01	24.00	996
0.32	42.30	59.96	53.64	34.67	85.26	25.29	72.63	14.00	18.41	18.00	11.53	25.29	6.88	23.00	158.39	216.57	202.78	135.59	297.55	80.98	256.31	15.00	19.88	20.00	12.70	27.07	7.19	25.00	1890


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/comparison_vals_auc.tex <==
name	auc
orig_pp	18.59
orig_ge	5.74
adv_pp	42.32
adv_ge	6.00


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.48	0.64	0.67	0.41	0.87	0.23	0.83	0.75	0.81	0.86	0.65	0.97	0.16	0.91	0.58	0.65	0.68	0.49	0.81	0.16	0.77	876
0.03	0.30	0.47	0.47	0.26	0.68	0.21	0.62	0.61	0.70	0.75	0.52	0.89	0.19	0.84	0.45	0.54	0.56	0.38	0.70	0.16	0.66	972
0.06	0.15	0.28	0.27	0.10	0.47	0.19	0.41	0.42	0.55	0.60	0.33	0.78	0.23	0.72	0.29	0.41	0.43	0.23	0.58	0.18	0.54	1018
0.11	0.06	0.18	0.16	0.02	0.34	0.16	0.27	0.29	0.45	0.48	0.21	0.68	0.24	0.62	0.20	0.32	0.34	0.15	0.50	0.18	0.45	1030
0.15	-0.01	0.08	0.07	-0.05	0.22	0.14	0.16	0.14	0.32	0.33	0.06	0.57	0.25	0.51	0.10	0.22	0.23	0.05	0.40	0.18	0.35	1033
0.18	-0.07	0.02	0.01	-0.11	0.15	0.13	0.10	0.02	0.20	0.21	-0.05	0.46	0.26	0.38	0.02	0.14	0.15	-0.03	0.32	0.18	0.26	996
0.32	-0.19	-0.09	-0.09	-0.23	0.06	0.14	0.00	-0.18	0.02	-0.01	-0.25	0.29	0.27	0.20	-0.12	0.02	-0.00	-0.17	0.20	0.18	0.14	1890


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.10
kendall	0.07


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	2.62	6.30	5.25	1.64	10.95	4.66	8.93	2.87	7.18	5.73	1.54	12.82	5.64	10.05	2.11	6.40	4.62	0.48	12.32	5.92	9.01	876
0.03	3.17	5.33	4.74	2.23	8.43	3.10	6.88	3.00	5.89	4.88	1.92	9.87	3.97	7.72	2.46	5.80	4.25	0.76	10.83	5.04	7.96	972
0.06	3.27	4.52	4.35	2.70	6.34	1.82	5.47	3.16	4.98	4.45	2.07	7.88	2.90	6.15	2.44	4.95	3.91	1.01	8.89	3.94	5.90	1018
0.11	3.21	4.09	3.99	2.79	5.40	1.30	4.88	3.01	4.33	3.94	2.32	6.34	2.01	5.22	2.39	4.00	3.35	1.34	6.66	2.66	4.81	1030
0.15	2.90	3.58	3.50	2.62	4.54	0.96	4.24	2.74	3.69	3.39	2.17	5.21	1.52	4.24	2.15	3.27	2.84	1.38	5.16	1.89	3.86	1033
0.18	2.71	3.30	3.25	2.45	4.14	0.84	3.83	2.59	3.33	3.12	2.15	4.52	1.18	3.87	2.04	2.85	2.53	1.37	4.32	1.47	3.33	996
0.32	2.53	3.03	2.99	2.30	3.75	0.72	3.51	2.40	3.02	2.86	2.08	3.96	0.94	3.42	1.82	2.35	2.20	1.48	3.23	0.87	2.70	1890


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/ets_sts_auc.tex <==
name	auc
et_use	1.18
et_tse	1.24
et_ce	1.11


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.83	3.34	1.56	-3.01	9.68	6.34	2.99	2.14	5.62	4.10	0.05	11.20	5.57	7.11	1.81	5.71	3.61	-0.64	12.07	6.35	7.15	876
0.03	0.75	1.75	1.17	-1.57	5.08	3.32	1.78	2.84	4.71	4.14	1.87	7.56	2.84	5.96	2.27	4.44	3.54	0.90	7.97	3.53	5.28	972
0.06	0.64	1.06	0.87	-0.33	2.45	1.39	1.17	3.33	4.61	4.39	2.72	6.50	1.89	5.42	2.76	4.18	3.76	1.87	6.48	2.30	4.96	1018
0.11	0.49	0.72	0.63	0.32	1.12	0.40	0.84	3.38	4.28	4.10	2.88	5.69	1.40	4.93	2.79	3.78	3.45	2.09	5.47	1.69	4.37	1030
0.15	0.33	0.46	0.42	0.24	0.69	0.23	0.53	3.22	3.86	3.78	2.92	4.81	0.94	4.39	2.67	3.35	3.20	2.27	4.43	1.08	3.86	1033
0.18	0.25	0.34	0.31	0.19	0.50	0.16	0.40	3.08	3.62	3.52	2.81	4.43	0.81	4.06	2.55	3.15	2.99	2.21	4.08	0.93	3.54	996
0.32	0.16	0.23	0.20	0.11	0.34	0.12	0.27	2.95	3.42	3.35	2.74	4.09	0.68	3.80	2.49	2.98	2.87	2.24	3.71	0.73	3.35	1890


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.21
et_p_h	1.24
et_p_l2	1.10


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.10	0.10	0.05	0.16	0.05	0.14	0.02	0.05	0.04	0.02	0.08	0.03	0.07	0.03	0.04	0.04	0.02	0.06	0.02	0.05	876
0.03	0.17	0.23	0.22	0.13	0.32	0.10	0.29	0.05	0.08	0.08	0.04	0.11	0.03	0.10	0.05	0.06	0.06	0.04	0.08	0.02	0.08	972
0.06	0.32	0.42	0.41	0.27	0.58	0.16	0.52	0.08	0.10	0.10	0.07	0.13	0.03	0.12	0.07	0.08	0.08	0.06	0.11	0.02	0.10	1018
0.11	0.51	0.66	0.64	0.43	0.90	0.23	0.79	0.10	0.12	0.12	0.09	0.16	0.04	0.14	0.09	0.10	0.10	0.08	0.12	0.02	0.12	1030
0.15	0.89	1.12	1.10	0.76	1.48	0.36	1.33	0.12	0.15	0.15	0.11	0.18	0.04	0.17	0.11	0.12	0.12	0.10	0.15	0.02	0.14	1033
0.18	1.25	1.61	1.57	1.09	2.13	0.52	1.91	0.14	0.16	0.16	0.13	0.20	0.04	0.19	0.13	0.14	0.14	0.12	0.16	0.02	0.15	996
0.32	2.01	2.83	2.64	1.67	4.00	1.17	3.47	0.16	0.19	0.19	0.15	0.23	0.04	0.21	0.15	0.16	0.16	0.14	0.19	0.03	0.18	1890


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.43
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.96	0.97	0.97	0.95	0.99	0.02	0.98	0.94	0.96	0.97	0.92	0.99	0.04	0.98	876
0.03	0.93	0.94	0.95	0.92	0.97	0.02	0.96	0.93	0.94	0.95	0.91	0.97	0.03	0.96	0.91	0.93	0.94	0.87	0.98	0.05	0.96	972
0.06	0.90	0.91	0.92	0.89	0.94	0.03	0.93	0.90	0.91	0.92	0.88	0.95	0.04	0.94	0.86	0.90	0.91	0.83	0.96	0.06	0.94	1018
0.11	0.88	0.89	0.90	0.86	0.93	0.03	0.91	0.87	0.89	0.90	0.85	0.93	0.04	0.92	0.83	0.87	0.88	0.79	0.94	0.07	0.91	1030
0.15	0.85	0.86	0.87	0.83	0.90	0.04	0.89	0.84	0.86	0.87	0.82	0.91	0.05	0.89	0.79	0.83	0.84	0.75	0.91	0.08	0.88	1033
0.18	0.83	0.84	0.85	0.80	0.88	0.04	0.87	0.81	0.84	0.84	0.79	0.89	0.05	0.87	0.76	0.80	0.81	0.72	0.88	0.08	0.85	996
0.32	0.79	0.81	0.82	0.77	0.86	0.05	0.84	0.78	0.81	0.81	0.76	0.86	0.05	0.84	0.70	0.74	0.75	0.66	0.83	0.09	0.80	1890


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.26


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	9.25	11.68	12.46	8.79	14.58	2.90	13.76	1.32	54.34	2.71	-145.22	253.91	199.56	10.21	2.88	9.47	6.55	0.40	18.55	9.08	13.36	876
0.03	9.22	12.69	11.99	7.79	17.59	4.90	16.36	1.94	68.81	4.42	-153.54	291.16	222.35	15.55	3.63	11.99	9.49	1.21	22.77	10.78	16.06	972
0.06	11.39	17.19	14.35	2.61	31.78	14.59	17.45	3.41	165.19	8.99	-436.68	767.06	601.87	43.32	5.21	15.65	12.99	2.98	28.31	12.66	23.02	1018
0.11	15.57	22.82	19.21	8.38	37.26	14.44	24.19	5.15	180.60	14.21	-427.86	789.05	608.46	79.09	6.91	17.89	15.35	4.56	31.21	13.33	26.05	1030
0.15	22.12	33.50	27.78	11.67	55.32	21.82	35.70	6.60	267.17	20.74	-1024.42	1558.75	1291.58	103.29	8.31	19.85	17.07	5.49	34.22	14.36	28.85	1033
0.18	29.90	41.60	36.85	21.79	61.41	19.81	48.28	6.87	227.86	20.29	-726.97	1182.68	954.82	93.42	8.39	19.80	17.18	5.70	33.90	14.10	29.27	996
0.32	41.28	56.35	53.06	34.26	78.44	22.09	68.83	6.72	229.31	19.94	-750.72	1209.34	980.03	98.12	8.12	19.55	16.90	5.77	33.33	13.78	29.18	1890


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/time_misc_auc.tex <==
name	auc
attack_time	10.79
l2	62.15
lom	5.59


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.41	0.55	0.56	0.35	0.76	0.21	0.71	0.67	0.74	0.75	0.61	0.86	0.13	0.83	0.79	0.83	0.85	0.75	0.92	0.09	0.89	876
0.03	0.27	0.41	0.41	0.22	0.60	0.19	0.54	0.58	0.65	0.67	0.52	0.79	0.13	0.75	0.73	0.78	0.79	0.69	0.87	0.09	0.85	972
0.06	0.14	0.27	0.27	0.11	0.44	0.17	0.38	0.45	0.55	0.56	0.41	0.69	0.14	0.65	0.64	0.71	0.72	0.61	0.81	0.10	0.78	1018
0.11	0.08	0.20	0.18	0.05	0.34	0.15	0.29	0.39	0.48	0.48	0.35	0.62	0.13	0.57	0.60	0.67	0.67	0.56	0.77	0.10	0.74	1030
0.15	0.00	0.13	0.11	0.01	0.25	0.12	0.21	0.31	0.41	0.41	0.28	0.55	0.14	0.50	0.54	0.62	0.62	0.51	0.72	0.11	0.69	1033
0.18	0.00	0.10	0.06	-0.01	0.20	0.11	0.17	0.26	0.36	0.35	0.23	0.49	0.13	0.44	0.50	0.58	0.57	0.47	0.68	0.10	0.64	996
0.32	0.00	0.06	0.00	-0.03	0.14	0.09	0.09	0.18	0.27	0.25	0.14	0.40	0.13	0.35	0.43	0.51	0.50	0.40	0.61	0.11	0.58	1890


==> data/mlm_plots/mlm_distil_fast/imdb/roberta/s/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.13
top50	0.19


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.66	58.92	54.80	36.18	81.65	22.74	71.06	15.00	18.58	18.00	13.22	23.94	5.36	22.00	45.49	63.11	58.76	38.92	87.30	24.19	76.06	15.00	18.59	18.00	13.22	23.96	5.37	22.00	926
0.03	42.51	60.24	54.65	34.96	85.51	25.27	72.79	14.00	17.77	17.00	11.70	23.83	6.07	22.00	49.82	70.46	64.59	41.80	99.13	28.67	84.60	14.00	17.76	18.00	11.61	23.92	6.16	21.00	985
0.06	42.38	60.59	54.75	34.63	86.54	25.96	73.83	13.00	17.55	17.00	11.33	23.76	6.22	21.00	58.83	81.41	75.15	49.52	113.30	31.89	97.63	13.00	17.58	17.50	11.28	23.88	6.30	21.00	1000
0.11	42.37	60.50	54.75	34.66	86.34	25.84	73.75	13.00	17.52	17.00	11.30	23.73	6.21	21.00	68.39	93.97	87.03	58.10	129.85	35.88	112.56	13.00	17.58	18.00	11.22	23.93	6.35	22.00	1001
0.15	42.32	60.42	54.48	34.48	86.36	25.94	73.55	13.00	17.60	17.00	11.41	23.78	6.18	21.00	89.36	119.81	111.81	76.59	163.03	43.22	143.68	13.00	17.92	18.00	11.45	24.39	6.47	22.00	995
0.18	42.32	60.35	54.56	34.60	86.09	25.75	73.65	13.00	17.55	17.00	11.33	23.77	6.22	21.00	109.55	146.29	139.66	95.91	196.66	50.37	174.25	13.00	17.93	18.00	11.34	24.52	6.59	22.00	996
0.32	42.32	60.26	54.48	34.76	85.76	25.50	73.47	13.00	17.55	17.00	11.38	23.73	6.17	21.00	157.73	213.79	200.53	136.30	291.27	77.48	256.25	13.00	18.01	18.00	11.40	24.62	6.61	22.00	1985


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/comparison_vals_auc.tex <==
name	auc
orig_pp	18.73
orig_ge	5.47
adv_pp	41.37
adv_ge	5.55


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.17	0.33	0.30	0.12	0.54	0.21	0.46	0.58	0.70	0.78	0.44	0.96	0.26	0.88	0.42	0.54	0.59	0.32	0.77	0.23	0.71	926
0.03	0.07	0.20	0.16	0.02	0.37	0.17	0.31	0.45	0.60	0.67	0.32	0.88	0.28	0.81	0.31	0.45	0.49	0.23	0.68	0.23	0.63	985
0.06	0.01	0.10	0.07	-0.03	0.24	0.14	0.17	0.34	0.52	0.58	0.23	0.80	0.29	0.74	0.23	0.38	0.41	0.16	0.61	0.22	0.55	1000
0.11	-0.02	0.05	0.03	-0.07	0.17	0.12	0.10	0.26	0.45	0.52	0.15	0.75	0.30	0.68	0.18	0.33	0.36	0.10	0.56	0.23	0.50	1001
0.15	-0.06	0.00	-0.01	-0.11	0.11	0.11	0.03	0.19	0.38	0.42	0.09	0.67	0.29	0.60	0.13	0.27	0.29	0.06	0.49	0.21	0.43	995
0.18	-0.09	-0.03	-0.04	-0.14	0.07	0.11	0.00	0.11	0.31	0.34	0.01	0.60	0.29	0.53	0.07	0.22	0.23	0.01	0.43	0.21	0.37	996
0.32	-0.15	-0.09	-0.09	-0.20	0.02	0.11	-0.04	-0.04	0.18	0.18	-0.13	0.49	0.31	0.40	-0.03	0.12	0.12	-0.09	0.34	0.22	0.28	1985


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/correlations_auc.tex <==
name	auc
pcc	0.01
spearman	0.12
kendall	0.08


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	7.01	11.98	10.54	5.16	18.80	6.82	15.26	5.77	11.61	9.91	3.61	19.61	8.00	14.93	4.56	10.61	8.26	2.50	18.72	8.11	14.32	926
0.03	5.60	8.51	7.28	3.76	13.25	4.75	10.03	3.99	7.88	6.38	2.27	13.50	5.62	10.14	3.51	7.69	5.63	1.26	14.12	6.43	9.47	985
0.06	4.48	6.06	5.56	3.32	8.80	2.74	6.90	2.88	5.07	4.23	1.78	8.36	3.29	6.15	2.67	5.08	3.99	0.99	9.18	4.09	5.93	1000
0.11	3.96	4.95	4.83	3.25	6.66	1.70	5.67	2.55	3.90	3.40	1.91	5.89	1.99	4.72	2.34	3.74	3.03	1.33	6.15	2.41	4.37	1001
0.15	3.35	3.99	3.93	2.87	5.11	1.12	4.61	2.26	3.08	2.86	1.82	4.33	1.25	3.60	2.06	2.93	2.54	1.32	4.54	1.61	3.40	995
0.18	3.03	3.53	3.51	2.64	4.42	0.89	4.03	2.13	2.74	2.59	1.83	3.65	0.91	3.21	1.88	2.50	2.29	1.36	3.64	1.14	2.84	996
0.32	2.64	3.06	3.05	2.35	3.77	0.71	3.49	1.99	2.47	2.36	1.77	3.17	0.70	2.83	1.67	2.10	1.99	1.37	2.83	0.73	2.42	1985


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/ets_sts_auc.tex <==
name	auc
et_use	1.45
et_tse	1.21
et_ce	1.13


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.84	10.93	4.68	-13.97	35.83	24.90	8.78	7.17	13.26	10.86	4.12	22.40	9.14	16.65	6.07	12.73	10.09	2.89	22.56	9.84	16.90	926
0.03	1.59	4.50	2.33	-8.27	17.28	12.77	3.57	6.07	9.32	8.11	3.85	14.79	5.47	10.90	4.94	9.01	7.10	2.15	15.88	6.86	10.86	985
0.06	0.95	1.80	1.24	-1.97	5.56	3.77	1.70	5.19	6.80	6.29	4.10	9.51	2.71	7.75	4.22	6.36	5.41	2.76	9.95	3.59	7.40	1000
0.11	0.63	1.26	0.82	-5.05	7.56	6.30	1.09	4.49	5.69	5.33	3.68	7.70	2.01	6.34	3.73	5.17	4.64	2.63	7.71	2.54	5.85	1001
0.15	0.38	0.56	0.49	-0.01	1.14	0.58	0.62	3.89	4.66	4.49	3.45	5.86	1.21	5.20	3.23	4.15	3.86	2.64	5.66	1.51	4.68	995
0.18	0.28	0.39	0.35	0.16	0.61	0.23	0.44	3.53	4.16	4.04	3.22	5.11	0.94	4.62	2.90	3.69	3.49	2.49	4.90	1.21	4.15	996
0.32	0.16	0.24	0.21	0.10	0.37	0.14	0.28	3.17	3.68	3.57	2.91	4.45	0.77	4.07	2.66	3.25	3.09	2.28	4.22	0.97	3.63	1985


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.42
et_p_h	1.67
et_p_l2	1.53


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.04	0.08	0.07	0.03	0.13	0.05	0.11	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.04	926
0.03	0.11	0.18	0.17	0.08	0.28	0.10	0.24	0.04	0.06	0.05	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.06	985
0.06	0.27	0.37	0.36	0.21	0.53	0.16	0.46	0.06	0.08	0.08	0.05	0.12	0.03	0.11	0.06	0.07	0.07	0.05	0.09	0.02	0.09	1000
0.11	0.43	0.60	0.57	0.35	0.84	0.24	0.74	0.08	0.10	0.10	0.07	0.14	0.03	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.10	1001
0.15	0.80	1.06	1.03	0.68	1.45	0.38	1.28	0.11	0.13	0.13	0.09	0.17	0.04	0.15	0.10	0.11	0.11	0.09	0.14	0.02	0.13	995
0.18	1.18	1.54	1.48	1.00	2.09	0.54	1.84	0.12	0.15	0.15	0.11	0.19	0.04	0.17	0.11	0.13	0.13	0.10	0.15	0.02	0.14	996
0.32	1.91	2.79	2.55	1.58	3.99	1.21	3.45	0.15	0.18	0.18	0.14	0.22	0.04	0.20	0.13	0.15	0.15	0.13	0.18	0.03	0.17	1985


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.95	0.96	0.97	0.92	1.00	0.04	0.98	0.93	0.95	0.96	0.90	0.99	0.04	0.98	926
0.03	0.93	0.94	0.95	0.91	0.97	0.03	0.96	0.90	0.92	0.94	0.87	0.98	0.05	0.96	0.89	0.92	0.93	0.85	0.99	0.07	0.96	985
0.06	0.90	0.92	0.92	0.88	0.95	0.04	0.93	0.84	0.88	0.90	0.82	0.94	0.06	0.93	0.84	0.87	0.89	0.79	0.95	0.08	0.93	1000
0.11	0.88	0.89	0.90	0.86	0.93	0.04	0.91	0.81	0.85	0.86	0.79	0.91	0.06	0.90	0.80	0.84	0.85	0.75	0.92	0.08	0.89	1001
0.15	0.85	0.87	0.87	0.82	0.91	0.04	0.89	0.78	0.82	0.82	0.76	0.88	0.06	0.86	0.76	0.80	0.80	0.70	0.89	0.09	0.85	995
0.18	0.83	0.84	0.85	0.80	0.89	0.05	0.87	0.76	0.79	0.80	0.74	0.85	0.06	0.83	0.73	0.76	0.78	0.67	0.85	0.09	0.82	996
0.32	0.79	0.81	0.82	0.76	0.86	0.05	0.84	0.73	0.76	0.77	0.71	0.82	0.06	0.80	0.68	0.71	0.73	0.61	0.81	0.10	0.77	1985


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	10.13	12.31	12.32	9.65	14.97	2.66	14.23	0.14	0.23	0.19	0.10	0.36	0.13	0.29	10.07	26.07	22.34	6.44	45.70	19.63	37.75	926
0.03	12.75	15.47	16.02	10.86	20.08	4.61	18.57	0.17	0.27	0.23	0.13	0.42	0.15	0.34	11.58	28.74	25.15	7.88	49.60	20.86	42.31	985
0.06	16.25	19.99	20.68	13.62	26.37	6.37	24.56	0.19	0.31	0.26	0.14	0.47	0.16	0.37	13.39	32.29	28.33	9.61	54.98	22.68	46.56	1000
0.11	21.84	26.96	28.03	18.14	35.78	8.82	32.94	0.20	0.33	0.28	0.16	0.50	0.17	0.42	14.13	33.70	30.51	10.81	56.60	22.90	50.16	1001
0.15	29.96	37.69	38.61	25.35	50.03	12.34	46.01	0.20	0.33	0.28	0.15	0.51	0.18	0.41	15.13	33.80	31.03	10.89	56.71	22.91	48.90	995
0.18	38.60	48.38	49.46	32.85	63.92	15.54	59.13	0.20	0.32	0.26	0.14	0.50	0.18	0.38	15.35	33.40	30.33	11.04	55.76	22.36	49.37	996
0.32	51.09	68.59	66.49	42.07	95.11	26.52	85.62	0.18	0.28	0.23	0.11	0.46	0.17	0.32	13.50	31.88	27.89	9.74	54.02	22.14	47.12	1985


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/time_misc_auc.tex <==
name	auc
attack_time	12.73
l2	0.10
lom	10.06


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.25	0.43	0.43	0.21	0.65	0.22	0.61	0.54	0.65	0.67	0.48	0.83	0.17	0.78	0.70	0.77	0.80	0.65	0.90	0.12	0.86	926
0.03	0.17	0.32	0.31	0.12	0.52	0.20	0.46	0.46	0.58	0.60	0.41	0.76	0.18	0.71	0.65	0.73	0.75	0.60	0.86	0.13	0.83	985
0.06	0.08	0.24	0.20	0.05	0.42	0.19	0.33	0.40	0.52	0.52	0.35	0.69	0.17	0.65	0.61	0.70	0.71	0.57	0.83	0.13	0.80	1000
0.11	0.06	0.18	0.14	0.02	0.34	0.16	0.29	0.35	0.48	0.49	0.31	0.65	0.17	0.60	0.58	0.67	0.69	0.54	0.80	0.13	0.76	1001
0.15	0.00	0.12	0.08	-0.01	0.25	0.13	0.19	0.31	0.43	0.42	0.27	0.59	0.16	0.54	0.55	0.64	0.65	0.52	0.77	0.13	0.74	995
0.18	0.00	0.09	0.06	-0.03	0.21	0.12	0.14	0.26	0.38	0.37	0.22	0.54	0.16	0.49	0.53	0.61	0.62	0.49	0.74	0.13	0.70	996
0.32	0.00	0.05	0.00	-0.04	0.15	0.10	0.07	0.19	0.31	0.29	0.15	0.47	0.16	0.41	0.48	0.57	0.57	0.44	0.70	0.13	0.66	1985


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/a/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.13
top50	0.20


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.58	59.37	54.74	35.96	82.79	23.42	71.50	15.00	18.70	18.00	13.31	24.08	5.38	22.00	46.25	64.34	59.22	39.31	89.37	25.03	78.01	15.00	18.56	18.00	13.22	23.91	5.34	22.00	915
0.03	42.34	59.71	53.87	34.17	85.24	25.54	72.07	14.00	17.89	18.00	11.82	23.96	6.07	22.00	50.65	70.81	64.40	41.83	99.79	28.98	85.53	14.00	17.72	18.00	11.65	23.78	6.06	21.00	1007
0.06	41.92	59.35	53.68	33.74	84.95	25.61	71.83	14.00	17.76	18.00	11.71	23.81	6.05	22.00	58.88	81.26	74.07	48.17	114.35	33.09	96.49	13.00	17.65	18.00	11.55	23.75	6.10	22.00	1139
0.11	41.99	59.72	53.23	34.31	85.13	25.41	72.67	14.00	17.71	17.00	11.49	23.92	6.22	21.00	69.66	95.07	86.73	58.07	132.07	37.00	112.98	13.00	17.78	18.00	11.38	24.17	6.40	22.00	1201
0.15	41.94	60.12	54.35	34.46	85.79	25.66	73.08	13.00	17.51	17.00	11.50	23.52	6.01	22.00	86.86	118.34	110.15	75.39	161.30	42.96	143.84	13.00	17.66	17.00	11.48	23.83	6.17	22.00	981
0.18	42.42	61.11	55.03	34.56	87.65	26.54	74.26	13.00	17.54	17.00	11.49	23.59	6.05	21.00	107.56	145.72	137.42	93.02	198.43	52.70	174.96	13.00	17.88	18.00	11.59	24.17	6.29	22.00	891
0.32	42.80	61.34	55.38	35.21	87.47	26.13	74.26	13.00	17.45	17.00	11.48	23.42	5.97	21.00	148.63	202.94	188.68	125.32	280.55	77.62	242.55	14.00	18.01	18.00	11.67	24.35	6.34	22.00	1423


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	18.77
orig_ge	5.48
adv_pp	40.59
adv_ge	5.54


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.01	0.21	0.23	-0.14	0.55	0.34	0.44	0.20	0.39	0.45	0.08	0.71	0.32	0.63	0.15	0.30	0.34	0.05	0.55	0.25	0.49	915
0.03	-0.23	-0.05	-0.04	-0.36	0.25	0.30	0.13	-0.03	0.16	0.17	-0.14	0.46	0.30	0.38	-0.02	0.12	0.12	-0.10	0.34	0.22	0.29	1007
0.06	-0.38	-0.23	-0.20	-0.49	0.04	0.26	-0.06	-0.16	-0.02	0.00	-0.27	0.24	0.26	0.16	-0.11	-0.01	0.01	-0.20	0.18	0.19	0.12	1139
0.11	-0.46	-0.31	-0.30	-0.54	-0.08	0.23	-0.13	-0.24	-0.11	-0.08	-0.33	0.11	0.22	0.03	-0.17	-0.08	-0.05	-0.24	0.08	0.16	0.03	1201
0.15	-0.58	-0.44	-0.46	-0.63	-0.25	0.19	-0.32	-0.37	-0.23	-0.22	-0.44	-0.03	0.20	-0.09	-0.26	-0.16	-0.15	-0.31	-0.02	0.15	-0.06	981
0.18	-0.66	-0.54	-0.57	-0.71	-0.38	0.17	-0.45	-0.47	-0.35	-0.34	-0.53	-0.17	0.18	-0.23	-0.34	-0.25	-0.24	-0.38	-0.11	0.14	-0.15	891
0.32	-0.75	-0.65	-0.67	-0.79	-0.50	0.15	-0.57	-0.60	-0.48	-0.49	-0.65	-0.32	0.16	-0.38	-0.44	-0.35	-0.35	-0.48	-0.22	0.13	-0.27	1423


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/correlations_auc.tex <==
name	auc
pcc	-0.13
spearman	-0.07
kendall	-0.05


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	7.37	13.58	11.45	4.70	22.46	8.88	17.47	6.25	13.71	10.90	3.18	24.24	10.53	18.00	4.66	11.93	8.49	1.08	22.78	10.85	15.91	915
0.03	6.52	10.16	9.04	4.62	15.71	5.55	12.15	5.08	10.22	8.06	2.69	17.74	7.52	12.95	4.20	10.02	7.05	1.12	18.91	8.90	12.86	1007
0.06	5.53	7.70	7.08	4.19	11.21	3.51	8.97	4.28	7.65	6.05	1.74	13.57	5.91	8.88	3.60	7.38	5.47	0.80	13.96	6.58	9.00	1139
0.11	4.96	6.38	6.18	4.20	8.56	2.18	7.51	3.80	5.71	5.08	2.88	8.54	2.83	6.84	3.21	5.63	4.42	1.29	9.96	4.34	6.48	1201
0.15	4.44	5.51	5.41	3.92	7.10	1.59	6.46	3.44	4.72	4.36	2.76	6.67	1.95	5.55	2.98	4.40	3.80	1.85	6.96	2.55	5.11	981
0.18	4.20	5.09	5.03	3.76	6.43	1.33	5.97	3.32	4.33	4.10	2.86	5.80	1.47	5.00	2.88	3.87	3.60	2.25	5.49	1.62	4.52	891
0.32	3.97	4.68	4.66	3.59	5.76	1.08	5.35	3.20	4.04	3.78	2.83	5.26	1.22	4.58	2.70	3.44	3.27	2.28	4.61	1.16	3.98	1423


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/ets_sts_auc.tex <==
name	auc
et_use	1.94
et_tse	1.77
et_ce	1.64


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.63	10.66	4.55	-12.16	33.48	22.82	8.73	6.96	14.02	11.26	3.33	24.70	10.69	18.00	5.84	14.44	10.40	1.79	27.10	12.66	18.93	915
0.03	1.87	4.25	2.72	-2.06	10.56	6.31	4.25	7.13	11.23	9.74	5.00	17.46	6.23	13.70	5.96	11.05	8.70	2.55	19.55	8.50	13.33	1007
0.06	1.21	2.08	1.61	-0.33	4.49	2.41	2.25	6.47	8.80	8.06	5.14	12.45	3.65	10.17	5.34	8.23	7.05	3.48	12.99	4.76	9.47	1139
0.11	0.81	1.28	1.07	0.21	2.34	1.07	1.46	5.81	7.58	6.98	3.75	11.40	3.83	8.62	4.80	7.31	6.09	-10.10	24.72	17.41	7.78	1201
0.15	0.56	0.81	0.72	0.35	1.27	0.46	0.93	5.34	6.69	6.45	4.83	8.55	1.86	7.77	4.46	5.95	5.55	3.71	8.20	2.25	6.85	981
0.18	0.42	0.59	0.53	0.33	0.84	0.26	0.69	5.29	6.27	6.10	4.81	7.72	1.45	7.10	4.39	5.52	5.20	3.80	7.23	1.72	6.32	891
0.32	0.27	0.39	0.36	0.22	0.56	0.17	0.47	4.92	5.67	5.53	4.53	6.81	1.14	6.30	4.13	4.97	4.76	3.61	6.34	1.37	5.54	1423


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.46
et_p_h	2.28
et_p_l2	2.11


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.09	0.08	0.03	0.15	0.06	0.13	0.02	0.04	0.03	0.02	0.07	0.03	0.06	0.02	0.04	0.03	0.02	0.05	0.02	0.05	915
0.03	0.13	0.20	0.19	0.10	0.31	0.10	0.27	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.08	0.02	0.07	1007
0.06	0.28	0.39	0.38	0.22	0.57	0.17	0.49	0.06	0.09	0.09	0.05	0.12	0.04	0.11	0.06	0.08	0.08	0.05	0.10	0.02	0.09	1139
0.11	0.46	0.63	0.60	0.37	0.89	0.26	0.77	0.09	0.11	0.11	0.07	0.14	0.04	0.13	0.08	0.09	0.09	0.07	0.12	0.02	0.11	1201
0.15	0.79	1.04	1.01	0.68	1.41	0.37	1.25	0.11	0.13	0.13	0.10	0.17	0.04	0.15	0.10	0.11	0.11	0.09	0.14	0.02	0.13	981
0.18	1.14	1.49	1.46	0.99	2.00	0.51	1.80	0.13	0.15	0.15	0.11	0.19	0.04	0.17	0.11	0.13	0.13	0.10	0.15	0.02	0.14	891
0.32	1.76	2.50	2.27	1.44	3.56	1.06	3.04	0.15	0.17	0.17	0.14	0.21	0.04	0.20	0.13	0.15	0.15	0.12	0.18	0.03	0.17	1423


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.39
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.95	0.96	0.97	0.93	0.99	0.03	0.98	0.92	0.94	0.96	0.90	0.99	0.05	0.98	915
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.91	0.93	0.94	0.88	0.97	0.04	0.96	0.88	0.91	0.93	0.85	0.97	0.06	0.96	1007
0.06	0.90	0.91	0.92	0.88	0.94	0.03	0.93	0.86	0.89	0.90	0.84	0.95	0.05	0.93	0.84	0.88	0.89	0.81	0.95	0.07	0.93	1139
0.11	0.88	0.89	0.90	0.85	0.93	0.04	0.91	0.84	0.86	0.87	0.81	0.92	0.05	0.90	0.81	0.85	0.86	0.77	0.92	0.08	0.90	1201
0.15	0.85	0.86	0.87	0.81	0.90	0.05	0.89	0.79	0.83	0.84	0.77	0.89	0.06	0.87	0.76	0.80	0.81	0.70	0.89	0.10	0.86	981
0.18	0.82	0.84	0.85	0.79	0.89	0.05	0.87	0.77	0.81	0.81	0.75	0.86	0.06	0.84	0.74	0.77	0.79	0.67	0.87	0.10	0.83	891
0.32	0.80	0.81	0.82	0.77	0.86	0.05	0.84	0.75	0.78	0.78	0.73	0.84	0.06	0.82	0.70	0.74	0.75	0.64	0.83	0.09	0.79	1423


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	11.77	14.51	14.33	6.93	22.09	7.58	15.90	1.07	4.54	2.01	-5.66	14.74	10.20	4.35	2.38	7.29	5.37	0.59	13.99	6.70	10.19	915
0.03	16.24	27.93	20.17	-8.90	64.76	36.83	24.03	1.56	8.35	3.16	-9.94	26.64	18.29	7.39	2.62	8.35	6.04	0.30	16.39	8.05	11.49	1007
0.06	20.02	57.26	25.82	-20.20	134.73	77.46	41.09	2.09	15.42	4.62	-20.12	50.95	35.53	11.90	3.10	9.18	6.94	0.87	17.49	8.31	12.48	1139
0.11	33.58	85.82	48.12	0.50	171.14	85.32	109.02	2.25	15.57	5.13	-23.43	54.58	39.01	12.97	3.46	9.76	7.36	1.16	18.36	8.60	13.44	1201
0.15	40.30	81.05	56.05	14.05	148.05	67.00	102.55	1.95	10.18	4.05	-11.06	31.42	21.24	9.65	3.45	9.44	7.18	1.05	17.83	8.39	12.81	981
0.18	57.89	93.12	76.60	33.55	152.69	59.57	109.00	1.90	7.02	3.35	-9.60	23.64	16.62	7.60	3.46	9.39	6.80	1.01	17.77	8.38	12.78	891
0.32	75.34	122.93	105.81	53.84	192.02	69.09	157.89	1.82	5.37	3.18	-0.73	11.47	6.10	6.79	3.21	9.53	7.08	0.93	18.13	8.60	13.65	1423


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/time_misc_auc.tex <==
name	auc
attack_time	26.32
l2	2.90
lom	2.89


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.20	0.35	0.36	0.16	0.55	0.19	0.50	0.42	0.53	0.55	0.36	0.69	0.17	0.65	0.58	0.66	0.68	0.53	0.79	0.13	0.76	915
0.03	0.09	0.21	0.19	0.06	0.36	0.15	0.31	0.30	0.40	0.40	0.25	0.56	0.15	0.52	0.50	0.58	0.58	0.45	0.70	0.12	0.67	1007
0.06	0.06	0.13	0.12	0.02	0.24	0.11	0.20	0.24	0.32	0.32	0.20	0.45	0.13	0.40	0.46	0.52	0.52	0.41	0.62	0.11	0.59	1139
0.11	0.00	0.09	0.07	-0.00	0.18	0.09	0.14	0.21	0.28	0.28	0.17	0.38	0.11	0.34	0.43	0.48	0.49	0.39	0.57	0.09	0.54	1201
0.15	0.00	0.05	0.00	-0.02	0.12	0.07	0.08	0.16	0.23	0.24	0.14	0.33	0.10	0.30	0.39	0.44	0.45	0.36	0.53	0.08	0.50	981
0.18	0.00	0.03	0.00	-0.02	0.08	0.05	0.06	0.12	0.19	0.19	0.10	0.27	0.09	0.24	0.35	0.40	0.41	0.32	0.48	0.08	0.45	891
0.32	0.00	0.01	0.00	-0.02	0.04	0.03	0.00	0.07	0.13	0.12	0.05	0.21	0.08	0.18	0.30	0.35	0.35	0.28	0.43	0.08	0.40	1423


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.07
top50	0.14


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.45	59.00	54.60	35.35	82.65	23.65	71.10	15.00	18.66	18.00	13.32	23.99	5.33	22.00	46.37	64.30	59.74	39.14	89.45	25.16	77.86	15.00	18.58	18.00	13.26	23.90	5.32	22.00	904
0.03	42.48	60.28	54.70	34.87	85.70	25.42	72.94	14.00	17.83	18.00	11.73	23.94	6.10	22.00	51.79	72.31	66.17	43.30	101.31	29.00	87.41	14.00	17.80	17.00	11.73	23.88	6.08	22.00	998
0.06	42.39	60.44	54.84	34.83	86.04	25.60	72.75	13.00	17.62	17.00	11.48	23.76	6.14	21.00	60.37	83.94	77.17	50.52	117.36	33.42	100.05	14.00	17.78	18.00	11.60	23.96	6.18	22.00	1069
0.11	42.39	60.39	54.89	34.70	86.08	25.69	73.47	13.00	17.67	18.00	11.52	23.82	6.15	21.00	70.96	98.74	92.56	60.58	136.90	38.16	119.04	14.00	17.94	18.00	11.79	24.10	6.16	22.00	1157
0.15	42.62	61.66	54.85	34.67	88.64	26.99	75.45	13.00	17.69	17.00	11.40	23.97	6.28	22.00	92.78	126.75	118.24	79.25	174.25	47.50	150.58	14.00	18.26	18.00	11.97	24.55	6.29	22.00	1118
0.18	42.16	60.42	54.85	34.54	86.31	25.89	73.02	13.00	17.42	17.00	11.43	23.41	5.99	21.00	115.67	152.86	144.01	98.56	207.15	54.30	178.37	14.00	18.22	18.00	12.11	24.34	6.12	22.00	980
0.32	42.38	60.38	54.75	34.74	86.02	25.64	73.73	13.00	17.32	17.00	11.27	23.38	6.06	21.00	158.76	219.21	205.81	136.97	301.46	82.24	265.13	14.00	18.38	18.00	12.05	24.71	6.33	23.00	1552


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/comparison_vals_auc.tex <==
name	auc
orig_pp	18.79
orig_ge	5.45
adv_pp	42.94
adv_ge	5.63


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.44	0.57	0.61	0.34	0.81	0.23	0.75	0.76	0.79	0.87	0.60	0.99	0.20	0.92	0.58	0.65	0.70	0.46	0.83	0.19	0.78	904
0.03	0.26	0.41	0.43	0.19	0.62	0.22	0.56	0.60	0.68	0.77	0.44	0.92	0.24	0.85	0.43	0.53	0.59	0.33	0.74	0.20	0.68	998
0.06	0.11	0.26	0.27	0.07	0.45	0.19	0.39	0.38	0.55	0.63	0.28	0.82	0.27	0.76	0.26	0.41	0.46	0.20	0.63	0.21	0.58	1069
0.11	0.05	0.17	0.17	0.01	0.34	0.16	0.29	0.25	0.45	0.49	0.19	0.71	0.26	0.66	0.18	0.33	0.34	0.13	0.53	0.20	0.49	1157
0.15	0.01	0.10	0.09	-0.03	0.23	0.13	0.18	0.16	0.34	0.37	0.09	0.59	0.25	0.55	0.11	0.25	0.25	0.06	0.43	0.18	0.39	1118
0.18	-0.03	0.05	0.03	-0.07	0.16	0.11	0.12	0.09	0.27	0.27	0.04	0.50	0.23	0.44	0.06	0.19	0.19	0.03	0.36	0.16	0.31	980
0.32	-0.09	-0.02	-0.03	-0.13	0.09	0.11	0.05	-0.01	0.15	0.14	-0.07	0.37	0.22	0.31	-0.01	0.11	0.10	-0.05	0.26	0.16	0.21	1552


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.11
kendall	0.08


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.59	7.12	5.84	2.03	12.21	5.09	9.34	3.19	7.32	5.71	1.24	13.41	6.08	9.54	2.67	6.92	4.93	0.43	13.41	6.49	8.88	904
0.03	3.53	5.72	5.07	2.37	9.06	3.34	7.00	2.93	5.72	4.58	1.32	10.12	4.40	7.06	2.44	6.10	4.26	0.13	12.07	5.97	7.13	998
0.06	3.35	4.59	4.33	2.70	6.48	1.89	5.44	2.59	4.35	3.81	1.74	6.96	2.61	5.40	2.30	4.72	3.50	0.67	8.77	4.05	5.63	1069
0.11	3.16	4.07	3.93	2.62	5.52	1.45	4.80	2.46	3.73	3.40	1.79	5.67	1.94	4.52	2.13	3.79	3.05	1.01	6.58	2.78	4.53	1157
0.15	2.88	3.54	3.50	2.60	4.48	0.94	4.14	2.22	3.09	2.89	1.89	4.28	1.20	3.69	2.05	3.11	2.65	1.18	5.05	1.94	3.56	1118
0.18	2.66	3.16	3.16	2.36	3.95	0.80	3.70	2.07	2.76	2.62	1.82	3.70	0.94	3.26	1.83	2.59	2.29	1.22	3.97	1.37	2.98	980
0.32	2.44	2.86	2.87	2.18	3.54	0.68	3.30	1.96	2.47	2.33	1.73	3.20	0.73	2.84	1.67	2.19	2.00	1.30	3.08	0.89	2.54	1552


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/ets_sts_auc.tex <==
name	auc
et_use	1.18
et_tse	1.07
et_ce	1.07


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.17	5.51	2.18	-9.95	20.98	15.46	4.25	3.13	7.50	5.69	0.25	14.75	7.25	9.54	2.76	7.98	5.51	-1.00	16.97	8.99	10.05	904
0.03	0.95	2.91	1.46	-6.34	12.16	9.25	2.25	3.64	6.07	5.28	2.43	9.72	3.65	7.42	3.19	6.11	4.69	0.48	11.74	5.63	7.32	998
0.06	0.66	1.39	0.93	-2.15	4.93	3.54	1.30	3.74	5.12	4.78	3.08	7.17	2.05	6.05	3.14	4.80	4.18	2.29	7.30	2.50	5.74	1069
0.11	0.48	0.83	0.62	-1.91	3.56	2.74	0.85	3.58	4.50	4.32	3.11	5.90	1.40	5.17	3.00	4.12	3.75	2.27	5.97	1.85	4.75	1157
0.15	0.32	0.47	0.40	0.13	0.81	0.34	0.54	3.30	3.97	3.80	2.87	5.07	1.10	4.41	2.77	3.57	3.29	2.14	4.99	1.42	4.02	1118
0.18	0.23	0.33	0.29	0.15	0.52	0.19	0.38	3.15	3.68	3.56	2.81	4.54	0.86	4.06	2.61	3.27	3.05	2.18	4.35	1.08	3.66	980
0.32	0.14	0.22	0.19	0.10	0.33	0.12	0.25	2.90	3.37	3.27	2.64	4.09	0.73	3.69	2.47	2.99	2.84	2.12	3.87	0.88	3.30	1552


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.28
et_p_h	1.32
et_p_l2	1.22


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.10	0.09	0.04	0.16	0.06	0.14	0.02	0.04	0.04	0.02	0.07	0.03	0.06	0.02	0.04	0.04	0.02	0.05	0.02	0.05	904
0.03	0.14	0.21	0.21	0.10	0.32	0.11	0.28	0.04	0.06	0.06	0.03	0.10	0.03	0.08	0.04	0.06	0.06	0.04	0.08	0.02	0.07	998
0.06	0.29	0.41	0.40	0.23	0.60	0.19	0.53	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.06	0.08	0.08	0.06	0.10	0.02	0.09	1069
0.11	0.49	0.68	0.65	0.39	0.97	0.29	0.83	0.09	0.11	0.11	0.07	0.15	0.04	0.14	0.08	0.10	0.10	0.07	0.12	0.02	0.11	1157
0.15	0.86	1.15	1.10	0.67	1.63	0.48	1.39	0.12	0.14	0.14	0.10	0.18	0.04	0.16	0.10	0.12	0.12	0.09	0.15	0.03	0.13	1118
0.18	1.27	1.65	1.60	1.11	2.19	0.54	1.99	0.13	0.16	0.16	0.12	0.19	0.04	0.18	0.12	0.13	0.13	0.11	0.16	0.02	0.15	980
0.32	1.99	2.89	2.63	1.58	4.19	1.30	3.56	0.15	0.18	0.18	0.14	0.22	0.04	0.21	0.14	0.16	0.16	0.13	0.18	0.03	0.17	1552


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.43
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.95	0.96	0.97	0.93	0.99	0.03	0.98	0.94	0.95	0.96	0.91	0.99	0.04	0.98	904
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.91	0.93	0.94	0.89	0.97	0.04	0.96	0.90	0.92	0.93	0.86	0.98	0.06	0.96	998
0.06	0.90	0.91	0.92	0.88	0.94	0.03	0.93	0.87	0.89	0.90	0.84	0.94	0.05	0.93	0.85	0.88	0.90	0.81	0.95	0.07	0.93	1069
0.11	0.88	0.89	0.90	0.85	0.93	0.04	0.91	0.84	0.87	0.88	0.82	0.92	0.05	0.91	0.81	0.85	0.87	0.77	0.94	0.09	0.91	1157
0.15	0.85	0.86	0.87	0.83	0.90	0.04	0.89	0.80	0.84	0.84	0.78	0.89	0.05	0.88	0.79	0.82	0.83	0.74	0.90	0.08	0.87	1118
0.18	0.83	0.84	0.85	0.79	0.89	0.05	0.87	0.78	0.81	0.82	0.75	0.87	0.06	0.85	0.74	0.78	0.80	0.68	0.88	0.10	0.84	980
0.32	0.80	0.81	0.82	0.76	0.86	0.05	0.85	0.74	0.78	0.78	0.72	0.84	0.06	0.82	0.70	0.74	0.75	0.64	0.83	0.10	0.80	1552


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	11.92	14.67	14.37	3.73	25.61	10.94	15.99	74.94	560.99	165.06	-1035.85	2157.82	1596.84	407.11	2.36	7.85	5.28	0.44	15.26	7.41	11.25	904
0.03	14.25	20.12	17.70	2.02	38.23	18.11	20.68	123.67	1284.08	268.72	-2476.66	5044.83	3760.75	763.63	3.34	10.14	7.83	1.33	18.96	8.82	14.77	998
0.06	19.00	39.96	24.09	-7.97	87.88	47.93	32.57	201.08	2621.54	490.43	-3601.92	8845.01	6223.46	1942.04	4.62	13.00	10.54	2.65	23.34	10.34	19.34	1069
0.11	26.88	63.03	34.75	1.90	124.16	61.13	73.21	278.65	3344.35	870.10	-3443.47	10132.18	6787.83	3290.54	5.50	14.19	12.03	3.20	25.19	11.00	20.23	1157
0.15	35.77	76.84	50.26	17.61	136.07	59.23	112.45	380.58	3848.78	1074.49	-5402.99	13100.54	9251.77	3595.07	6.37	15.66	13.50	4.03	27.30	11.63	22.39	1118
0.18	48.79	89.31	67.33	30.66	147.96	58.65	121.52	411.56	3586.84	1165.42	-3652.96	10826.64	7239.80	3640.17	6.13	16.21	14.17	4.28	28.15	11.94	23.78	980
0.32	62.90	106.23	90.97	46.79	165.67	59.44	142.10	464.06	3831.26	1178.97	-4153.33	11815.84	7984.58	3686.28	5.96	15.87	13.40	3.71	28.02	12.15	23.40	1552


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/time_misc_auc.tex <==
name	auc
attack_time	22.83
l2	1004.42
lom	4.54


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.42	0.54	0.57	0.33	0.76	0.22	0.71	0.68	0.74	0.78	0.59	0.89	0.15	0.84	0.79	0.83	0.86	0.73	0.93	0.10	0.90	904
0.03	0.25	0.40	0.42	0.20	0.61	0.20	0.56	0.57	0.65	0.69	0.49	0.81	0.16	0.77	0.72	0.78	0.80	0.67	0.89	0.11	0.86	998
0.06	0.13	0.28	0.27	0.10	0.45	0.18	0.40	0.45	0.56	0.59	0.40	0.72	0.16	0.69	0.63	0.72	0.74	0.60	0.83	0.12	0.81	1069
0.11	0.08	0.20	0.19	0.06	0.35	0.15	0.30	0.38	0.50	0.51	0.35	0.65	0.15	0.62	0.59	0.67	0.68	0.56	0.78	0.11	0.76	1157
0.15	0.06	0.15	0.12	0.02	0.27	0.13	0.22	0.34	0.44	0.44	0.30	0.57	0.13	0.53	0.56	0.63	0.64	0.53	0.74	0.10	0.71	1118
0.18	0.00	0.12	0.09	0.01	0.23	0.11	0.18	0.32	0.40	0.39	0.28	0.52	0.12	0.49	0.53	0.60	0.60	0.51	0.70	0.10	0.68	980
0.32	0.00	0.08	0.06	-0.01	0.18	0.10	0.13	0.26	0.34	0.33	0.22	0.45	0.11	0.42	0.50	0.56	0.56	0.47	0.65	0.09	0.62	1552


==> data/mlm_plots/mlm_distil_fast/imdb/xlnet/s/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.14
top50	0.20


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	95.93	188.56	145.11	50.17	326.94	138.39	232.28	3.00	4.54	4.00	2.51	6.57	2.03	6.00	137.25	261.04	202.80	77.74	444.34	183.30	335.77	3.00	4.06	4.00	2.14	5.98	1.92	5.00	251
0.11	107.30	248.22	184.20	-35.21	531.65	283.43	299.34	3.00	4.32	4.00	2.41	6.23	1.91	5.00	166.26	361.70	268.33	-35.70	759.10	397.40	441.18	2.00	3.73	3.00	1.80	5.65	1.92	5.00	1017
0.15	111.14	262.60	204.48	47.54	477.66	215.06	337.03	3.00	4.13	4.00	2.16	6.11	1.98	5.00	184.94	400.60	312.85	67.61	733.59	332.99	506.56	2.00	3.42	3.00	1.34	5.49	2.07	4.00	670
0.18	99.29	237.76	180.39	3.14	472.37	234.61	297.05	2.00	4.04	4.00	2.08	6.00	1.96	6.00	218.59	433.70	338.98	57.27	810.13	376.43	544.43	2.00	3.27	3.00	1.35	5.19	1.92	4.00	726
0.32	108.62	257.18	191.09	-12.58	526.94	269.76	313.64	3.00	3.99	4.00	2.09	5.90	1.90	5.00	318.37	655.21	512.91	133.31	1177.10	521.89	827.70	2.00	3.19	3.00	1.24	5.14	1.95	4.00	2671


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/comparison_vals_auc.tex <==
name	auc
orig_pp	63.49
orig_ge	1.07
adv_pp	119.26
adv_ge	0.89


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	-0.10	0.09	-0.01	-0.18	0.37	0.27	0.31	0.40	0.54	0.59	0.30	0.78	0.24	0.72	0.30	0.44	0.48	0.23	0.65	0.21	0.60	251
0.11	-0.15	0.04	-0.07	-0.25	0.32	0.29	0.19	0.34	0.49	0.54	0.21	0.76	0.28	0.69	0.27	0.40	0.43	0.17	0.63	0.23	0.57	1017
0.15	-0.19	-0.06	-0.12	-0.30	0.19	0.24	-0.02	0.25	0.40	0.45	0.12	0.69	0.28	0.61	0.19	0.33	0.35	0.10	0.56	0.23	0.49	670
0.18	-0.20	-0.13	-0.15	-0.27	0.01	0.14	-0.08	0.13	0.32	0.35	0.02	0.62	0.30	0.55	0.10	0.26	0.27	0.02	0.49	0.23	0.43	726
0.32	-0.31	-0.23	-0.22	-0.39	-0.07	0.16	-0.15	-0.05	0.16	0.17	-0.15	0.46	0.30	0.37	-0.03	0.13	0.13	-0.10	0.36	0.23	0.29	2671


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/correlations_auc.tex <==
name	auc
pcc	-0.03
spearman	0.09
kendall	0.07


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	2.93	4.34	4.08	2.27	6.40	2.06	5.34	3.31	5.43	4.68	2.15	8.70	3.28	6.43	4.95	19.97	13.83	2.83	37.10	17.14	31.51	251
0.11	2.84	4.19	3.90	2.13	6.24	2.05	5.17	2.99	5.13	4.44	2.03	8.23	3.10	6.60	3.73	17.37	9.65	0.50	34.25	16.88	27.25	1017
0.15	2.77	3.68	3.41	2.12	5.24	1.56	4.50	2.78	4.31	3.95	2.07	6.55	2.24	5.29	3.16	14.47	7.71	-1.11	30.05	15.58	21.15	670
0.18	2.74	3.33	3.27	2.39	4.27	0.94	3.79	2.90	4.12	3.76	2.39	5.86	1.73	5.00	3.09	11.27	5.81	-1.61	24.15	12.88	14.12	726
0.32	2.25	2.76	2.64	1.97	3.55	0.79	3.13	2.37	3.19	2.96	2.03	4.36	1.16	3.74	2.21	6.82	3.46	-2.65	16.29	9.47	6.54	2671


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/ets_sts_auc.tex <==
name	auc
et_use	0.90
et_tse	1.09
et_ce	3.23


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.62	4.15	1.09	-9.74	18.04	13.89	3.25	4.29	10.82	7.70	-0.17	21.81	10.99	12.94	3.92	17.00	8.79	-13.92	47.91	30.91	17.65	251
0.11	0.56	3.86	1.06	-13.59	21.31	17.45	2.25	4.73	10.90	7.77	0.29	21.51	10.61	13.09	4.14	18.64	9.54	-16.24	53.51	34.87	18.20	1017
0.15	0.54	3.16	0.93	-12.71	19.03	15.87	1.86	4.48	10.25	7.69	-1.04	21.53	11.28	12.16	4.00	17.51	9.34	-8.00	43.02	25.51	19.48	670
0.18	0.33	4.14	0.56	-27.64	35.93	31.79	1.40	4.51	9.56	6.83	1.75	17.37	7.81	11.40	3.86	18.43	7.18	-10.45	47.30	28.87	20.54	726
0.32	0.19	1.73	0.37	-8.79	12.25	10.52	0.83	3.78	7.54	5.26	-0.19	15.28	7.73	8.42	3.12	14.28	5.24	-23.18	51.73	37.45	11.70	2671


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.86
et_p_h	2.47
et_p_l2	4.45


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.15	0.48	0.41	0.09	0.87	0.39	0.67	0.03	0.07	0.05	0.01	0.13	0.06	0.11	0.04	0.07	0.06	0.03	0.11	0.04	0.10	251
0.11	0.21	0.59	0.45	0.04	1.15	0.56	0.82	0.02	0.07	0.05	0.01	0.14	0.06	0.11	0.04	0.07	0.06	0.03	0.11	0.04	0.10	1017
0.15	0.26	0.78	0.57	-0.21	1.76	0.98	0.96	0.02	0.08	0.06	0.01	0.16	0.07	0.13	0.04	0.08	0.07	0.03	0.13	0.05	0.11	670
0.18	0.41	1.20	1.00	0.10	2.31	1.11	1.69	0.03	0.09	0.08	0.02	0.17	0.08	0.14	0.05	0.09	0.08	0.04	0.14	0.05	0.12	726
0.32	0.74	2.44	1.64	-0.34	5.22	2.78	3.17	0.05	0.13	0.12	0.04	0.22	0.09	0.20	0.07	0.12	0.12	0.06	0.18	0.06	0.16	2671


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.34
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.86	0.88	0.89	0.85	0.92	0.04	0.91	0.86	0.90	0.90	0.85	0.95	0.05	0.94	0.91	0.93	0.97	0.85	1.02	0.08	0.99	251
0.11	0.84	0.87	0.87	0.83	0.91	0.04	0.90	0.85	0.88	0.89	0.83	0.94	0.05	0.92	0.88	0.92	0.95	0.82	1.01	0.09	0.98	1017
0.15	0.81	0.84	0.85	0.79	0.89	0.05	0.88	0.82	0.85	0.87	0.79	0.92	0.06	0.90	0.85	0.89	0.93	0.78	1.00	0.11	0.98	670
0.18	0.80	0.82	0.83	0.78	0.86	0.04	0.85	0.81	0.84	0.85	0.79	0.90	0.06	0.88	0.83	0.87	0.90	0.77	0.98	0.10	0.96	726
0.32	0.73	0.76	0.77	0.71	0.82	0.05	0.80	0.74	0.79	0.79	0.72	0.85	0.06	0.83	0.72	0.80	0.82	0.67	0.94	0.13	0.90	2671


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.22
sts_ce	0.23


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	2.03	2.19	2.17	1.61	2.76	0.58	2.24	0.40	0.46	0.47	0.34	0.58	0.12	0.52	1.61	4.46	3.52	0.92	8.00	3.54	6.80	251
0.11	1.91	2.21	2.08	1.62	2.80	0.59	2.47	0.40	0.46	0.47	0.33	0.59	0.13	0.52	1.87	4.53	3.90	1.20	7.87	3.33	6.63	1017
0.15	1.64	2.26	2.34	1.23	3.29	1.03	2.75	0.44	0.46	0.49	0.34	0.59	0.13	0.53	1.74	4.63	4.22	1.24	8.02	3.39	6.79	670
0.18	0.61	1.99	1.66	0.48	3.50	1.51	3.21	0.44	0.49	0.50	0.38	0.60	0.11	0.55	2.14	4.93	4.48	1.53	8.32	3.40	7.33	726
0.32	0.59	0.87	0.96	0.60	1.13	0.27	1.10	0.45	0.48	0.50	0.37	0.59	0.11	0.53	1.92	4.47	4.02	1.37	7.57	3.10	6.52	2671


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/time_misc_auc.tex <==
name	auc
attack_time	0.47
l2	0.12
lom	1.21


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.17	0.00	-0.08	0.41	0.24	0.50	0.43	0.54	0.57	0.35	0.73	0.19	0.71	0.67	0.73	0.77	0.60	0.87	0.14	0.83	251
0.11	0.00	0.14	0.00	-0.11	0.38	0.25	0.00	0.43	0.53	0.57	0.32	0.74	0.21	0.67	0.62	0.71	0.73	0.56	0.86	0.15	0.82	1017
0.15	0.00	0.07	0.00	-0.13	0.27	0.20	0.00	0.33	0.47	0.50	0.26	0.68	0.21	0.67	0.60	0.68	0.70	0.53	0.82	0.15	0.78	670
0.18	0.00	0.04	0.00	-0.10	0.17	0.13	0.00	0.25	0.41	0.43	0.19	0.63	0.22	0.57	0.54	0.63	0.62	0.47	0.79	0.16	0.75	726
0.32	0.00	0.02	0.00	-0.09	0.13	0.11	0.00	0.17	0.32	0.33	0.11	0.54	0.21	0.50	0.50	0.57	0.58	0.42	0.73	0.16	0.67	2671


==> data/mlm_plots/mlm_distil_fast/mr/bert/a/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.11
top50	0.17


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	97.01	186.95	145.76	59.63	314.27	127.32	246.13	3.00	4.53	4.00	2.56	6.50	1.97	6.00	133.84	247.83	208.71	91.25	404.42	156.58	319.78	3.00	4.51	4.00	2.55	6.46	1.96	6.00	285
0.11	105.88	246.70	184.30	-23.01	516.42	269.71	304.13	3.00	4.26	4.00	2.40	6.12	1.86	5.00	159.08	327.68	253.95	40.31	615.06	287.37	406.82	3.00	4.23	4.00	2.35	6.11	1.88	5.00	1166
0.15	112.56	258.48	202.42	46.28	470.68	212.20	331.00	3.00	4.04	4.00	2.11	5.97	1.93	5.00	180.83	388.12	306.93	71.76	704.47	316.36	458.32	2.00	3.95	4.00	2.07	5.83	1.88	5.00	761
0.18	99.29	228.37	170.50	26.70	430.04	201.67	290.17	3.00	4.05	4.00	2.12	5.98	1.93	6.00	197.45	400.40	319.31	120.44	680.37	279.96	524.30	2.00	4.00	4.00	2.04	5.95	1.95	5.00	754
0.32	109.57	259.85	192.05	-21.80	541.49	281.65	314.36	3.00	3.99	4.00	2.10	5.89	1.90	5.00	296.90	609.35	477.59	126.11	1092.59	483.24	759.04	2.00	3.77	3.00	1.85	5.70	1.93	5.00	2687


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	62.60
orig_ge	1.07
adv_pp	111.01
adv_ge	1.04


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	-0.35	0.00	0.01	-0.45	0.45	0.45	0.33	-0.01	0.19	0.30	-0.22	0.61	0.42	0.51	0.01	0.16	0.24	-0.16	0.49	0.33	0.41	285
0.11	-0.45	-0.11	-0.15	-0.56	0.33	0.45	0.22	-0.21	0.08	0.14	-0.34	0.49	0.42	0.39	-0.15	0.07	0.11	-0.25	0.40	0.33	0.31	1166
0.15	-0.58	-0.21	-0.24	-0.65	0.24	0.44	0.09	-0.36	-0.03	0.03	-0.46	0.40	0.43	0.28	-0.26	-0.01	0.03	-0.35	0.33	0.34	0.23	761
0.18	-0.65	-0.35	-0.45	-0.75	0.05	0.40	-0.11	-0.49	-0.19	-0.21	-0.58	0.20	0.39	0.12	-0.37	-0.13	-0.13	-0.44	0.18	0.31	0.09	754
0.32	-0.78	-0.50	-0.58	-0.86	-0.15	0.35	-0.32	-0.62	-0.35	-0.38	-0.70	0.01	0.35	-0.11	-0.47	-0.26	-0.27	-0.54	0.02	0.28	-0.07	2687


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/correlations_auc.tex <==
name	auc
pcc	-0.08
spearman	-0.03
kendall	-0.02


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	2.62	4.50	3.85	1.39	7.61	3.11	5.74	2.77	5.56	4.44	1.20	9.91	4.35	6.71	2.70	13.29	6.18	-2.31	28.89	15.60	19.02	285
0.11	2.60	4.13	3.89	1.80	6.45	2.33	5.13	2.84	5.02	4.30	1.58	8.46	3.44	6.33	2.90	12.32	5.86	-3.14	27.78	15.46	15.05	1166
0.15	2.37	3.64	3.44	1.78	5.49	1.86	4.69	2.50	4.19	3.53	1.74	6.65	2.45	5.44	2.51	9.71	4.79	-3.14	22.56	12.85	11.23	761
0.18	2.60	3.70	3.52	2.05	5.35	1.65	4.50	2.78	4.42	3.91	1.83	7.01	2.59	5.36	2.77	9.49	4.91	-3.91	22.88	13.40	9.59	754
0.32	2.48	3.15	3.04	2.02	4.28	1.13	3.68	2.65	3.62	3.36	2.06	5.18	1.56	4.27	2.15	5.76	3.37	-2.68	14.21	8.45	5.76	2687


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/ets_sts_auc.tex <==
name	auc
et_use	0.96
et_tse	1.14
et_ce	2.44


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.69	5.77	1.47	-16.36	27.90	22.13	3.50	4.33	13.45	7.93	-5.33	32.23	18.78	14.72	3.59	18.82	7.93	-30.65	68.28	49.47	18.68	285
0.11	0.72	5.27	1.41	-16.59	27.13	21.86	3.01	5.00	14.55	8.89	-5.90	35.00	20.45	17.22	4.24	26.61	9.53	-45.29	98.52	71.90	22.02	1166
0.15	0.51	4.05	0.97	-10.42	18.51	14.46	2.85	4.94	13.35	8.87	-3.62	30.31	16.97	16.00	4.28	26.30	9.61	-42.66	95.25	68.95	23.25	761
0.18	0.39	2.51	0.77	-5.22	10.23	7.73	1.80	4.99	11.25	7.60	-0.03	22.52	11.27	13.12	4.30	28.02	8.31	-47.63	103.67	75.65	17.54	754
0.32	0.25	2.05	0.52	-8.18	12.29	10.23	1.15	4.61	9.06	6.47	-0.92	19.04	9.98	9.95	3.84	17.08	6.22	-31.71	65.86	48.78	12.79	2687


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.88
et_p_h	3.06
et_p_l2	6.21


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.15	0.44	0.31	0.05	0.83	0.39	0.62	0.03	0.07	0.05	0.02	0.13	0.06	0.11	0.03	0.07	0.05	0.03	0.11	0.04	0.09	285
0.11	0.17	0.53	0.40	0.04	1.01	0.48	0.73	0.03	0.08	0.06	0.01	0.14	0.06	0.11	0.03	0.07	0.06	0.02	0.11	0.04	0.10	1166
0.15	0.19	0.74	0.55	0.05	1.43	0.69	1.03	0.03	0.08	0.05	0.01	0.16	0.07	0.13	0.04	0.08	0.06	0.03	0.13	0.05	0.11	761
0.18	0.40	1.16	0.90	0.15	2.17	1.01	1.69	0.04	0.10	0.09	0.03	0.18	0.07	0.16	0.05	0.10	0.09	0.04	0.15	0.05	0.13	754
0.32	0.62	2.17	1.45	-0.17	4.50	2.33	2.85	0.06	0.13	0.12	0.04	0.22	0.09	0.20	0.07	0.12	0.12	0.06	0.18	0.06	0.16	2687


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.31
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.85	0.87	0.88	0.83	0.91	0.04	0.90	0.85	0.89	0.90	0.83	0.94	0.05	0.92	0.82	0.88	0.93	0.75	1.01	0.13	0.98	285
0.11	0.82	0.85	0.85	0.81	0.89	0.04	0.88	0.83	0.87	0.87	0.81	0.92	0.05	0.91	0.83	0.88	0.91	0.76	0.99	0.12	0.97	1166
0.15	0.79	0.82	0.82	0.77	0.87	0.05	0.85	0.79	0.83	0.84	0.77	0.89	0.06	0.88	0.79	0.85	0.88	0.74	0.97	0.12	0.95	761
0.18	0.77	0.80	0.81	0.76	0.85	0.05	0.83	0.78	0.82	0.83	0.76	0.89	0.07	0.87	0.77	0.83	0.87	0.70	0.96	0.13	0.93	754
0.32	0.71	0.75	0.75	0.70	0.80	0.05	0.78	0.72	0.77	0.78	0.71	0.84	0.07	0.82	0.67	0.76	0.78	0.60	0.91	0.15	0.87	2687


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.22


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	2.60	2.99	2.83	1.20	4.77	1.79	2.95	1.55	8.73	6.48	-0.28	17.73	9.01	12.79	1.83	5.48	3.67	0.30	10.65	5.17	7.62	285
0.11	2.48	3.04	2.73	1.60	4.49	1.45	3.40	1.09	9.25	7.29	-0.19	18.68	9.44	14.21	1.54	4.91	3.83	0.73	9.08	4.18	7.09	1166
0.15	2.08	3.12	3.18	1.54	4.71	1.59	3.75	1.26	9.47	7.47	-0.44	19.37	9.90	14.39	1.79	4.88	3.88	0.82	8.93	4.06	7.07	761
0.18	1.25	2.94	2.23	0.72	5.15	2.21	4.15	0.92	10.17	7.64	-1.46	21.80	11.63	15.36	1.33	5.08	3.78	0.82	9.35	4.26	7.56	754
0.32	1.37	1.81	1.80	1.33	2.29	0.48	2.18	1.30	10.89	8.35	-0.56	22.33	11.45	16.55	2.01	5.41	4.40	1.06	9.76	4.35	7.90	2687


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/time_misc_auc.tex <==
name	auc
attack_time	0.70
l2	2.59
lom	1.34


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.16	0.00	-0.09	0.41	0.25	0.50	0.29	0.42	0.43	0.20	0.65	0.22	0.57	0.50	0.59	0.62	0.40	0.77	0.18	0.75	285
0.11	0.00	0.15	0.00	-0.11	0.42	0.27	0.50	0.17	0.37	0.33	0.14	0.60	0.23	0.50	0.42	0.55	0.56	0.36	0.73	0.19	0.67	1166
0.15	0.00	0.10	0.00	-0.14	0.33	0.24	0.00	0.17	0.31	0.33	0.07	0.54	0.24	0.50	0.36	0.51	0.55	0.32	0.70	0.19	0.67	761
0.18	0.00	0.04	0.00	-0.12	0.21	0.17	0.00	0.00	0.23	0.17	0.03	0.43	0.20	0.33	0.31	0.44	0.43	0.27	0.62	0.18	0.55	754
0.32	0.00	0.03	0.00	-0.11	0.16	0.14	0.00	0.00	0.17	0.14	-0.01	0.35	0.18	0.29	0.27	0.39	0.38	0.22	0.55	0.17	0.50	2687


==> data/mlm_plots/mlm_distil_fast/mr/bert/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.07
top50	0.12


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	92.40	181.14	143.67	50.09	312.20	131.06	224.32	3.00	4.54	4.00	2.60	6.47	1.93	6.00	133.34	243.72	194.17	79.24	408.20	164.48	319.01	3.00	4.54	4.00	2.64	6.44	1.90	6.00	264
0.11	108.02	253.17	191.39	-25.61	531.96	278.79	308.82	3.00	4.29	4.00	2.42	6.15	1.87	5.00	169.47	365.91	280.09	-8.78	740.61	374.70	436.53	3.00	4.20	4.00	2.33	6.07	1.87	5.00	1130
0.15	115.20	262.86	205.13	48.90	476.82	213.96	337.58	2.25	4.04	4.00	2.08	6.01	1.96	5.00	224.95	465.32	349.19	50.11	880.53	415.21	564.96	2.00	3.87	4.00	1.95	5.78	1.91	5.00	750
0.18	99.35	241.85	180.52	-15.25	498.94	257.09	297.73	2.00	4.04	3.00	2.04	6.05	2.01	6.00	220.70	464.17	342.73	102.45	825.89	361.72	591.22	2.00	3.87	4.00	1.97	5.77	1.90	5.00	737
0.32	108.92	262.91	192.16	-34.61	560.43	297.52	315.87	3.00	3.97	4.00	2.07	5.88	1.91	5.00	353.75	749.67	565.29	132.66	1366.67	617.00	943.45	2.00	3.74	3.00	1.85	5.64	1.90	5.00	2718


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/comparison_vals_auc.tex <==
name	auc
orig_pp	64.29
orig_ge	1.07
adv_pp	130.62
adv_ge	1.03


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.12	0.33	0.34	0.06	0.59	0.27	0.52	0.35	0.51	0.55	0.24	0.78	0.27	0.71	0.27	0.39	0.41	0.17	0.61	0.22	0.56	264
0.11	0.06	0.24	0.23	-0.03	0.50	0.27	0.42	0.25	0.42	0.46	0.14	0.71	0.28	0.64	0.18	0.32	0.33	0.11	0.54	0.22	0.48	1130
0.15	-0.04	0.14	0.11	-0.14	0.42	0.28	0.30	0.13	0.32	0.35	0.02	0.63	0.30	0.54	0.10	0.25	0.26	0.01	0.48	0.23	0.42	750
0.18	-0.11	0.04	0.03	-0.19	0.27	0.23	0.21	-0.01	0.21	0.23	-0.08	0.51	0.30	0.44	-0.01	0.16	0.16	-0.06	0.38	0.22	0.32	737
0.32	-0.31	-0.14	-0.16	-0.38	0.10	0.24	0.00	-0.26	-0.02	-0.03	-0.35	0.31	0.33	0.21	-0.18	-0.01	-0.01	-0.25	0.23	0.24	0.15	2718


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/correlations_auc.tex <==
name	auc
pcc	0.02
spearman	0.06
kendall	0.05


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	1.78	3.04	2.83	1.35	4.73	1.69	3.77	1.77	3.80	3.05	1.04	6.56	2.76	4.94	1.95	10.89	4.35	-1.73	23.51	12.62	16.67	264
0.11	1.88	2.87	2.63	1.44	4.29	1.42	3.63	2.05	3.57	2.99	1.24	5.90	2.33	4.48	2.29	10.34	5.23	-1.45	22.13	11.79	14.83	1130
0.15	1.86	2.74	2.56	1.45	4.03	1.29	3.51	1.99	3.28	2.95	1.44	5.13	1.85	4.09	2.08	8.39	3.92	-1.93	18.70	10.32	10.23	750
0.18	1.92	2.67	2.52	1.55	3.80	1.12	3.26	2.06	3.32	2.92	1.33	5.32	2.00	3.96	2.05	7.43	3.36	-2.21	17.08	9.64	8.99	737
0.32	1.92	2.44	2.35	1.66	3.21	0.77	2.87	2.03	2.84	2.61	1.62	4.05	1.22	3.41	1.82	4.69	2.75	-1.46	10.84	6.15	4.80	2718


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/ets_sts_auc.tex <==
name	auc
et_use	0.70
et_tse	0.85
et_ce	1.99


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.46	3.02	0.81	-5.39	11.43	8.41	1.78	3.10	7.28	5.39	0.86	13.71	6.42	9.63	2.58	11.01	5.56	-9.46	31.49	20.48	12.52	264
0.11	0.39	2.40	0.79	-4.95	9.75	7.35	1.79	3.33	7.92	5.44	-0.24	16.08	8.16	9.37	2.98	13.94	5.60	-20.70	48.58	34.64	12.18	1130
0.15	0.28	1.96	0.52	-7.27	11.18	9.22	1.25	3.24	7.60	5.02	-2.74	17.93	10.33	9.10	2.71	13.01	5.55	-14.25	40.26	27.26	13.18	750
0.18	0.23	1.45	0.45	-2.31	5.21	3.76	0.91	3.27	6.86	4.72	-0.34	14.06	7.20	7.49	2.65	14.25	5.10	-30.77	59.27	45.02	11.15	737
0.32	0.15	1.16	0.27	-5.94	8.25	7.09	0.59	3.31	6.42	4.44	-0.61	13.46	7.04	6.65	2.75	12.76	4.24	-25.29	50.80	38.05	9.31	2718


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.46
et_p_h	1.84
et_p_l2	3.47


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.18	0.46	0.39	0.08	0.83	0.37	0.62	0.03	0.08	0.05	0.01	0.14	0.06	0.11	0.04	0.07	0.06	0.03	0.11	0.04	0.10	264
0.11	0.21	0.65	0.47	0.03	1.27	0.62	0.91	0.03	0.08	0.06	0.02	0.15	0.07	0.12	0.04	0.08	0.07	0.03	0.12	0.05	0.11	1130
0.15	0.33	1.05	0.80	0.03	2.06	1.01	1.49	0.03	0.10	0.07	0.02	0.18	0.08	0.16	0.05	0.09	0.08	0.04	0.15	0.05	0.13	750
0.18	0.44	1.50	1.06	0.00	3.01	1.50	2.16	0.04	0.11	0.09	0.03	0.19	0.08	0.17	0.06	0.11	0.10	0.05	0.16	0.05	0.14	737
0.32	0.92	3.04	2.01	-0.75	6.83	3.79	3.84	0.06	0.14	0.13	0.05	0.23	0.09	0.21	0.08	0.13	0.13	0.07	0.19	0.06	0.17	2718


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.85	0.88	0.88	0.84	0.91	0.04	0.90	0.86	0.89	0.90	0.83	0.94	0.05	0.93	0.84	0.89	0.93	0.77	1.01	0.12	0.98	264
0.11	0.83	0.85	0.86	0.81	0.90	0.04	0.88	0.84	0.87	0.88	0.81	0.93	0.06	0.91	0.85	0.89	0.93	0.78	1.00	0.11	0.98	1130
0.15	0.80	0.83	0.83	0.79	0.87	0.04	0.86	0.81	0.85	0.85	0.79	0.91	0.06	0.89	0.81	0.86	0.89	0.74	0.98	0.12	0.96	750
0.18	0.78	0.81	0.81	0.76	0.85	0.04	0.84	0.79	0.83	0.84	0.77	0.89	0.06	0.87	0.79	0.85	0.87	0.74	0.96	0.11	0.94	737
0.32	0.72	0.75	0.76	0.70	0.81	0.05	0.79	0.73	0.78	0.78	0.71	0.84	0.06	0.82	0.70	0.77	0.79	0.63	0.91	0.14	0.88	2718


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.22
sts_ce	0.22


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	2.26	2.50	2.45	2.05	2.95	0.45	2.67	6.06	68.59	50.06	-23.69	160.87	92.28	96.76	0.91	2.18	1.94	0.69	3.67	1.49	3.11	264
0.11	2.01	2.34	2.33	1.60	3.08	0.74	2.57	2.76	62.44	19.91	-24.90	149.79	87.34	95.18	0.74	1.82	1.48	0.44	3.20	1.38	2.67	1130
0.15	1.53	2.19	2.33	1.03	3.35	1.16	2.61	2.45	82.44	30.60	-31.81	196.69	114.25	129.67	0.55	1.68	1.33	0.27	3.09	1.41	2.42	750
0.18	0.69	1.96	1.57	0.55	3.37	1.41	3.05	1.62	80.09	19.84	-26.16	186.35	106.25	127.62	0.74	1.86	1.51	0.43	3.28	1.43	2.75	737
0.32	0.73	0.97	1.02	0.71	1.24	0.27	1.21	2.50	88.08	43.36	-29.30	205.45	117.37	139.92	0.78	2.02	1.78	0.51	3.52	1.51	2.91	2718


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/time_misc_auc.tex <==
name	auc
attack_time	0.48
l2	20.40
lom	0.49


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.19	0.00	-0.07	0.45	0.26	0.50	0.43	0.50	0.57	0.31	0.70	0.20	0.71	0.58	0.69	0.69	0.55	0.83	0.14	0.77	264
0.11	0.00	0.12	0.00	-0.12	0.35	0.23	0.00	0.33	0.46	0.50	0.25	0.66	0.20	0.57	0.58	0.66	0.67	0.53	0.80	0.13	0.75	1130
0.15	0.00	0.08	0.00	-0.14	0.31	0.23	0.00	0.25	0.38	0.33	0.18	0.59	0.21	0.50	0.55	0.63	0.64	0.48	0.78	0.15	0.73	750
0.18	0.00	0.05	0.00	-0.11	0.22	0.17	0.00	0.17	0.33	0.33	0.13	0.53	0.20	0.50	0.50	0.58	0.58	0.44	0.71	0.14	0.67	737
0.32	0.00	0.02	0.00	-0.09	0.12	0.11	0.00	0.00	0.22	0.17	0.03	0.40	0.19	0.33	0.38	0.49	0.50	0.33	0.64	0.15	0.60	2718


==> data/mlm_plots/mlm_distil_fast/mr/bert/s/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.09
top50	0.15


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	121.02	221.48	177.90	65.93	377.03	155.55	299.94	4.00	5.35	5.00	2.49	8.20	2.85	6.00	125.50	248.29	186.77	67.54	429.04	180.75	332.10	4.00	5.36	5.00	2.52	8.20	2.84	6.00	312
0.06	98.76	187.23	152.11	54.18	320.27	133.05	228.00	3.00	4.70	4.00	2.50	6.91	2.20	6.00	126.84	219.37	174.10	66.55	372.18	152.81	270.83	3.00	4.70	4.00	2.49	6.92	2.22	6.00	748
0.11	96.39	209.18	171.91	47.36	371.00	161.82	262.95	3.00	4.51	4.00	2.26	6.75	2.24	6.00	131.36	280.08	220.58	52.17	508.00	227.91	350.33	3.00	4.44	4.00	2.24	6.63	2.19	6.00	952
0.15	104.61	249.89	177.22	-58.14	557.92	308.03	285.58	2.00	3.74	3.00	1.98	5.50	1.76	5.00	153.68	360.08	257.41	-3.88	724.04	363.96	414.55	2.00	3.60	3.00	1.88	5.32	1.72	4.75	458
0.18	99.69	249.97	183.61	1.21	498.73	248.76	311.98	3.00	4.20	4.00	2.08	6.33	2.13	6.00	193.87	425.39	309.25	64.45	786.33	360.94	520.75	2.00	4.09	3.00	1.93	6.24	2.16	5.00	596
0.32	101.82	245.44	175.77	-34.91	525.78	280.35	293.35	3.00	4.13	4.00	2.00	6.26	2.13	5.00	281.33	565.90	431.99	86.57	1045.23	479.33	706.78	2.00	3.84	3.00	1.74	5.93	2.09	5.00	2171


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	67.57
orig_ge	1.24
adv_pp	113.31
adv_ge	1.21


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.00	0.00	0.00	0.00	0.00	0.00	-0.25	-0.04	-0.03	-0.30	0.22	0.26	0.12	0.00	0.00	0.00	0.00	0.00	0.00	0.00	312
0.06	0.00	0.25	0.13	-0.07	0.58	0.32	0.50	0.10	0.37	0.43	0.03	0.71	0.34	0.62	0.00	0.31	0.33	0.03	0.59	0.28	0.54	748
0.11	0.00	0.20	0.14	-0.14	0.53	0.34	0.42	0.16	0.35	0.38	0.04	0.65	0.30	0.54	0.11	0.31	0.32	0.08	0.54	0.23	0.48	952
0.15	-0.14	0.11	0.00	-0.29	0.51	0.40	0.35	-0.03	0.22	0.21	-0.12	0.57	0.35	0.47	0.00	0.21	0.18	-0.06	0.49	0.27	0.37	458
0.18	-0.37	-0.08	-0.11	-0.44	0.28	0.36	0.15	-0.14	0.05	0.02	-0.25	0.35	0.30	0.22	-0.07	0.05	0.02	-0.17	0.28	0.22	0.19	596
0.32	-0.58	-0.33	-0.38	-0.67	0.01	0.34	-0.13	-0.40	-0.18	-0.21	-0.49	0.13	0.31	0.01	-0.29	-0.13	-0.14	-0.37	0.11	0.24	0.02	2171


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/correlations_auc.tex <==
name	auc
pcc	-0.01
spearman	0.03
kendall	0.03


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	5.08	6.58	6.29	4.51	8.65	2.07	8.14	5.76	9.59	8.01	4.46	14.73	5.14	12.35	4.46	19.34	13.90	3.45	35.22	15.88	33.88	312
0.06	1.92	3.31	3.27	1.43	5.19	1.88	4.31	2.00	4.20	3.44	0.56	7.85	3.64	5.06	2.37	10.87	4.69	-1.65	23.38	12.52	15.60	748
0.11	1.79	2.73	2.61	1.23	4.22	1.50	3.47	1.80	3.21	2.86	1.00	5.41	2.21	4.12	1.80	7.04	3.78	-1.85	15.93	8.89	7.66	952
0.15	1.58	2.52	2.40	1.05	4.00	1.47	3.15	1.63	2.94	2.55	0.43	5.46	2.52	3.62	1.42	5.67	2.39	-2.96	14.29	8.63	5.89	458
0.18	1.96	2.72	2.69	1.56	3.88	1.16	3.30	2.11	3.14	2.96	1.52	4.77	1.63	3.66	2.04	6.05	3.40	-2.00	14.10	8.05	6.13	596
0.32	2.10	2.59	2.54	1.73	3.45	0.86	3.01	2.14	2.83	2.66	1.69	3.97	1.14	3.31	1.81	3.90	2.68	-1.28	9.08	5.18	4.03	2171


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/ets_sts_auc.tex <==
name	auc
et_use	0.85
et_tse	1.02
et_ce	2.02


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.86	16.84	3.76	-40.37	74.05	57.21	5.39	8.49	24.09	18.14	4.46	43.73	19.63	36.31	12.16	39.25	21.42	-6.47	84.96	45.72	53.37	312
0.06	0.70	5.45	1.89	-10.87	21.77	16.32	4.14	4.32	14.81	9.09	-3.35	32.98	18.16	19.44	3.99	22.35	9.63	-19.54	64.23	41.88	22.15	748
0.11	0.47	3.24	1.08	-7.12	13.60	10.36	2.44	4.00	10.40	7.00	0.67	20.13	9.73	13.68	3.44	18.10	7.84	-11.59	47.79	29.69	18.98	952
0.15	0.39	13.27	0.83	-75.13	101.68	88.40	2.26	3.66	10.19	6.94	-1.01	21.40	11.20	13.81	3.55	19.15	7.57	-25.81	64.12	44.96	16.95	458
0.18	0.31	1.99	0.75	-2.35	6.34	4.35	1.56	3.96	10.71	6.25	-4.42	25.85	15.13	11.21	3.42	21.42	6.26	-28.55	71.38	49.97	14.89	596
0.32	0.22	1.87	0.44	-6.90	10.64	8.77	1.10	4.06	8.40	5.81	-1.51	18.31	9.91	8.96	3.42	17.71	5.67	-42.79	78.21	60.50	11.79	2171


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/ets_time_misc_auc.tex <==
name	auc
et_p	1.43
et_p_h	3.27
et_p_l2	6.02


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.09	0.21	0.13	0.03	0.39	0.18	0.27	0.01	0.04	0.02	-0.01	0.08	0.04	0.04	0.01	0.04	0.03	0.01	0.08	0.04	0.06	312
0.06	0.09	0.30	0.19	-0.08	0.69	0.38	0.38	0.02	0.05	0.03	0.00	0.10	0.05	0.07	0.02	0.05	0.04	0.01	0.08	0.04	0.07	748
0.11	0.16	0.51	0.36	-0.01	1.02	0.52	0.66	0.02	0.07	0.05	0.01	0.13	0.06	0.10	0.03	0.06	0.05	0.02	0.11	0.04	0.09	952
0.15	0.22	0.73	0.50	0.03	1.44	0.71	1.09	0.03	0.08	0.06	0.01	0.14	0.07	0.11	0.03	0.07	0.06	0.03	0.12	0.04	0.10	458
0.18	0.31	1.12	0.77	-0.08	2.31	1.19	1.57	0.04	0.10	0.08	0.02	0.18	0.08	0.16	0.05	0.09	0.09	0.04	0.14	0.05	0.13	596
0.32	0.58	2.20	1.47	-0.25	4.66	2.46	2.88	0.05	0.13	0.12	0.04	0.22	0.09	0.19	0.07	0.12	0.12	0.06	0.18	0.06	0.16	2171


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.31
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.90	0.92	0.92	0.89	0.94	0.02	0.94	0.91	0.93	0.94	0.90	0.97	0.03	0.96	0.89	0.94	0.96	0.87	1.00	0.06	0.99	312
0.06	0.85	0.88	0.88	0.84	0.91	0.04	0.90	0.85	0.88	0.89	0.83	0.94	0.05	0.92	0.85	0.90	0.93	0.81	1.00	0.10	0.98	748
0.11	0.81	0.84	0.84	0.80	0.88	0.04	0.87	0.81	0.85	0.86	0.79	0.91	0.06	0.89	0.81	0.86	0.89	0.74	0.98	0.12	0.96	952
0.15	0.78	0.81	0.81	0.76	0.86	0.05	0.84	0.78	0.82	0.83	0.76	0.88	0.06	0.86	0.73	0.81	0.84	0.65	0.96	0.15	0.93	458
0.18	0.76	0.79	0.79	0.74	0.84	0.05	0.82	0.76	0.81	0.81	0.75	0.87	0.06	0.85	0.74	0.82	0.84	0.69	0.95	0.13	0.91	596
0.32	0.70	0.73	0.73	0.68	0.79	0.05	0.77	0.70	0.75	0.74	0.68	0.81	0.07	0.80	0.64	0.73	0.75	0.57	0.88	0.16	0.84	2171


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.23
sts_tse	0.24
sts_ce	0.24


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	1.59	2.57	1.79	1.40	3.73	1.17	3.87	0.04	0.08	0.05	-0.07	0.23	0.15	0.08	2.37	4.26	3.69	1.70	6.82	2.56	6.06	312
0.06	0.52	1.10	0.59	0.19	2.01	0.91	1.55	0.07	1.20	0.83	-0.13	2.54	1.34	1.81	0.73	2.29	1.76	0.28	4.30	2.01	3.34	748
0.11	0.47	0.71	0.57	0.23	1.18	0.47	0.66	0.63	1.75	1.44	0.29	3.21	1.46	2.54	0.68	2.27	1.67	0.19	4.34	2.08	3.14	952
0.15	0.46	0.82	0.58	0.27	1.37	0.55	1.26	0.55	1.52	1.16	0.18	2.86	1.34	2.11	0.65	2.33	1.81	0.06	4.59	2.26	3.13	458
0.18	0.77	1.13	1.02	0.67	1.58	0.46	1.50	0.30	1.00	1.01	0.30	1.70	0.70	1.51	1.02	2.91	2.18	0.43	5.40	2.48	4.11	596
0.32	1.32	1.43	1.52	1.12	1.74	0.31	1.64	0.40	1.58	1.19	0.04	3.13	1.54	1.96	1.01	2.91	2.24	0.43	5.40	2.48	4.23	2171


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/time_misc_auc.tex <==
name	auc
attack_time	0.34
l2	0.38
lom	0.79


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.05	0.00	-0.13	0.22	0.18	0.00	0.14	0.28	0.29	0.12	0.45	0.17	0.43	0.38	0.51	0.54	0.37	0.64	0.13	0.62	312
0.06	0.00	0.22	0.00	-0.08	0.52	0.30	0.50	0.29	0.48	0.57	0.23	0.73	0.25	0.71	0.56	0.67	0.69	0.50	0.85	0.17	0.83	748
0.11	0.00	0.20	0.00	-0.10	0.50	0.30	0.50	0.40	0.49	0.50	0.28	0.71	0.21	0.67	0.60	0.69	0.69	0.54	0.83	0.15	0.77	952
0.15	0.00	0.19	0.00	-0.15	0.54	0.35	0.50	0.29	0.44	0.50	0.21	0.68	0.23	0.60	0.54	0.64	0.64	0.48	0.80	0.16	0.73	458
0.18	0.00	0.12	0.00	-0.14	0.38	0.26	0.00	0.25	0.34	0.33	0.14	0.54	0.20	0.43	0.46	0.54	0.54	0.41	0.67	0.13	0.62	596
0.32	0.00	0.05	0.00	-0.13	0.23	0.18	0.00	0.00	0.24	0.25	0.05	0.42	0.19	0.33	0.38	0.47	0.46	0.32	0.61	0.15	0.56	2171


==> data/mlm_plots/mlm_distil_fast/mr/cnn/ig/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.11
top50	0.17


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	99.38	199.54	158.58	58.28	340.80	141.26	262.93	3.00	4.99	5.00	2.65	7.33	2.34	6.00	112.83	215.67	172.28	61.52	369.83	154.16	276.29	3.00	5.08	5.00	2.71	7.45	2.37	6.00	1091
0.06	99.81	208.52	170.50	25.50	391.54	183.02	265.92	3.00	4.18	4.00	2.24	6.11	1.93	5.00	115.43	239.58	184.66	42.67	436.49	196.91	300.37	3.00	4.18	4.00	2.28	6.08	1.90	5.00	1264
0.11	94.59	235.01	162.03	-116.75	586.77	351.76	268.41	3.00	3.96	4.00	2.10	5.82	1.86	5.00	132.15	290.99	203.45	-19.69	601.66	310.67	332.56	3.00	3.95	4.00	2.08	5.81	1.86	5.00	711
0.15	119.27	322.76	228.23	-96.99	742.51	419.75	319.47	2.00	3.38	3.00	1.69	5.07	1.69	4.00	184.51	415.45	323.63	-45.42	876.32	460.87	508.76	2.00	3.38	3.00	1.74	5.01	1.63	4.00	222
0.18	191.44	309.06	230.65	130.23	487.89	178.83	426.12	2.00	3.14	3.00	1.80	4.49	1.34	4.00	225.59	483.51	273.86	113.11	853.91	370.40	705.71	2.00	3.11	3.00	1.80	4.43	1.32	3.50	71
0.32	106.44	255.21	175.26	-27.45	537.87	282.66	289.28	3.00	3.90	3.00	2.10	5.71	1.80	5.00	350.62	742.26	562.09	28.34	1456.17	713.92	896.99	2.00	3.52	3.00	1.83	5.21	1.69	4.00	546


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/comparison_vals_auc.tex <==
name	auc
orig_pp	77.80
orig_ge	1.08
adv_pp	133.13
adv_ge	1.05


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.00	0.00	0.00	0.00	0.00	0.00	-0.23	0.00	-0.01	-0.35	0.35	0.35	0.25	0.00	0.00	0.00	0.00	0.00	0.00	0.00	1091
0.06	0.00	0.10	0.00	-0.14	0.34	0.24	0.00	-0.27	0.05	0.05	-0.34	0.45	0.40	0.33	0.00	0.09	0.00	-0.11	0.28	0.19	0.00	1264
0.11	0.00	0.21	0.00	-0.09	0.51	0.30	0.46	-0.05	0.25	0.28	-0.09	0.59	0.34	0.54	0.00	0.18	0.06	-0.05	0.42	0.23	0.38	711
0.15	0.00	0.15	0.00	-0.16	0.45	0.30	0.34	-0.14	0.15	0.13	-0.20	0.50	0.35	0.42	0.00	0.13	0.00	-0.09	0.35	0.22	0.28	222
0.18	-0.22	-0.12	0.00	-0.36	0.12	0.24	0.00	-0.70	-0.33	-0.29	-0.66	0.01	0.34	-0.10	-0.13	-0.07	0.00	-0.24	0.11	0.18	0.00	71
0.32	-0.54	-0.27	-0.28	-0.62	0.09	0.36	-0.04	-0.54	-0.25	-0.29	-0.61	0.10	0.35	-0.03	-0.38	-0.17	-0.18	-0.44	0.09	0.26	0.00	546


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/correlations_auc.tex <==
name	auc
pcc	-0.01
spearman	-0.03
kendall	-0.00


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	4.41	6.07	5.44	3.51	8.64	2.57	7.09	4.46	8.05	6.63	2.95	13.15	5.10	10.24	4.66	18.44	12.33	2.81	34.06	15.63	32.49	1091
0.06	2.94	3.88	3.88	2.21	5.56	1.68	4.87	2.75	4.96	4.05	0.96	8.96	4.00	5.70	2.85	11.99	6.31	-1.05	25.02	13.04	15.91	1264
0.11	1.74	2.66	2.47	1.34	3.98	1.32	3.54	1.74	3.28	2.82	1.01	5.55	2.27	4.36	1.82	8.34	3.95	-2.59	19.26	10.93	10.60	711
0.15	1.85	2.45	2.40	1.36	3.54	1.09	3.03	1.84	3.17	2.86	1.30	5.03	1.86	3.86	2.31	7.61	3.70	-2.03	17.25	9.64	7.19	222
0.18	2.03	2.78	2.13	1.63	3.93	1.15	3.18	2.28	3.42	3.12	1.73	5.11	1.69	3.74	2.09	6.35	4.28	0.69	12.01	5.66	7.31	71
0.32	1.93	2.43	2.36	1.58	3.28	0.85	2.86	1.96	2.63	2.50	1.56	3.70	1.07	3.10	1.66	3.45	2.41	-0.98	7.88	4.43	3.52	546


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/ets_sts_auc.tex <==
name	auc
et_use	0.85
et_tse	1.05
et_ce	2.18


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.99	7.41	3.57	-3.39	18.21	10.80	7.15	10.77	27.32	18.62	4.32	50.31	23.00	38.31	11.71	54.36	24.97	-21.29	130.02	75.66	55.02	1091
0.06	1.03	7.75	2.25	-23.85	39.35	31.60	5.02	6.71	20.48	15.23	1.89	39.08	18.59	29.15	6.23	41.88	18.66	-21.01	104.78	62.90	46.01	1264
0.11	0.44	3.06	1.16	-10.17	16.29	13.23	2.43	3.05	11.10	6.11	-1.91	24.11	13.01	13.48	2.80	20.57	7.05	-21.97	63.10	42.53	19.36	711
0.15	0.35	6.21	0.77	-13.26	25.69	19.48	1.99	3.56	17.89	7.25	-5.46	41.24	23.35	17.45	3.18	59.80	9.48	-60.35	179.95	120.15	31.48	222
0.18	0.36	1.71	1.06	-0.35	3.77	2.06	1.77	4.32	18.13	8.76	1.97	34.29	16.16	30.26	4.97	53.38	11.19	-19.85	126.62	73.23	65.20	71
0.32	0.15	1.15	0.28	-3.49	5.78	4.64	0.65	3.48	7.25	4.71	-1.19	15.69	8.44	7.66	2.96	15.46	4.39	-29.85	60.77	45.31	9.69	546


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/ets_time_misc_auc.tex <==
name	auc
et_p	1.01
et_p_h	4.42
et_p_l2	11.28


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.07	0.18	0.14	0.03	0.33	0.15	0.25	0.01	0.03	0.02	-0.00	0.07	0.04	0.04	0.01	0.03	0.03	0.01	0.06	0.03	0.05	1091
0.06	0.09	0.30	0.20	-0.00	0.60	0.30	0.39	0.01	0.05	0.02	-0.01	0.10	0.06	0.06	0.02	0.05	0.03	0.01	0.08	0.04	0.06	1264
0.11	0.18	0.58	0.36	-0.08	1.23	0.65	0.70	0.02	0.08	0.05	0.00	0.15	0.07	0.12	0.03	0.07	0.05	0.02	0.12	0.05	0.10	711
0.15	0.18	0.74	0.56	-0.11	1.60	0.85	1.00	0.02	0.07	0.04	-0.00	0.14	0.07	0.10	0.03	0.07	0.05	0.01	0.12	0.05	0.09	222
0.18	0.28	1.16	0.47	-0.08	2.40	1.24	1.78	0.01	0.09	0.06	-0.01	0.18	0.09	0.17	0.02	0.08	0.06	0.01	0.14	0.07	0.13	71
0.32	0.99	2.96	2.16	0.11	5.81	2.85	3.94	0.06	0.15	0.14	0.05	0.25	0.10	0.22	0.08	0.13	0.14	0.07	0.20	0.07	0.18	546


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.37
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.89	0.91	0.91	0.87	0.94	0.03	0.93	0.89	0.91	0.92	0.87	0.96	0.05	0.95	0.89	0.92	0.96	0.82	1.01	0.10	0.98	1091
0.06	0.85	0.87	0.88	0.84	0.91	0.04	0.90	0.85	0.88	0.88	0.82	0.94	0.06	0.92	0.85	0.89	0.93	0.78	1.00	0.11	0.97	1264
0.11	0.80	0.84	0.84	0.79	0.89	0.05	0.88	0.82	0.85	0.86	0.79	0.91	0.06	0.90	0.81	0.86	0.90	0.73	1.00	0.14	0.96	711
0.15	0.79	0.82	0.82	0.78	0.86	0.04	0.85	0.81	0.84	0.84	0.78	0.90	0.06	0.89	0.83	0.87	0.89	0.76	0.98	0.11	0.94	222
0.18	0.76	0.78	0.76	0.73	0.83	0.05	0.84	0.78	0.81	0.83	0.74	0.88	0.07	0.87	0.76	0.83	0.87	0.72	0.95	0.12	0.93	71
0.32	0.70	0.73	0.73	0.68	0.78	0.05	0.76	0.70	0.74	0.74	0.68	0.81	0.06	0.79	0.64	0.72	0.73	0.57	0.87	0.15	0.82	546


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.23
sts_tse	0.24
sts_ce	0.24


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.94	1.58	1.06	0.84	2.33	0.74	2.38	29.52	43.48	44.17	24.14	62.82	19.34	58.58	11.88	12.43	12.52	11.42	13.44	1.01	12.98	1091
0.06	0.81	1.05	0.95	0.47	1.64	0.59	1.41	25.07	38.53	36.32	20.55	56.51	17.98	49.25	5.59	6.97	7.49	3.29	10.66	3.68	9.72	1264
0.11	0.26	0.62	0.36	0.14	1.10	0.48	0.92	24.66	37.94	35.11	21.31	54.57	16.63	49.63	0.79	3.14	1.76	-0.21	6.49	3.35	4.42	711
0.15	0.31	0.57	0.34	0.17	0.98	0.40	0.87	25.84	36.87	35.11	20.95	52.79	15.92	46.61	0.59	2.42	1.32	-0.77	5.60	3.19	2.42	222
0.18	0.79	0.85	0.91	0.62	1.09	0.23	0.99	18.84	29.10	28.74	13.86	44.34	15.24	30.63	0.75	2.55	1.62	-0.37	5.47	2.92	2.02	71
0.32	0.37	0.54	0.42	0.31	0.76	0.23	0.72	29.23	41.73	41.53	25.38	58.07	16.34	53.39	0.49	1.33	1.17	0.11	2.54	1.21	1.82	546


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/time_misc_auc.tex <==
name	auc
attack_time	0.22
l2	10.57
lom	0.99


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.13	0.00	-0.12	0.38	0.25	0.00	0.14	0.31	0.29	0.10	0.52	0.21	0.43	0.42	0.52	0.54	0.37	0.67	0.15	0.62	1091
0.06	0.00	0.13	0.00	-0.14	0.39	0.27	0.00	0.17	0.33	0.33	0.10	0.57	0.23	0.50	0.45	0.57	0.58	0.40	0.75	0.17	0.69	1264
0.11	0.00	0.17	0.00	-0.14	0.48	0.31	0.50	0.17	0.36	0.33	0.12	0.61	0.25	0.50	0.44	0.55	0.56	0.36	0.74	0.19	0.69	711
0.15	0.00	0.25	0.00	-0.12	0.63	0.38	0.50	0.00	0.33	0.33	0.04	0.61	0.28	0.50	0.43	0.55	0.55	0.38	0.72	0.17	0.67	222
0.18	0.00	0.27	0.00	-0.18	0.71	0.45	1.00	0.00	0.39	0.25	-0.01	0.78	0.40	0.88	0.39	0.59	0.50	0.32	0.86	0.27	0.82	71
0.32	0.00	0.04	0.00	-0.14	0.22	0.18	0.00	0.00	0.16	0.14	-0.04	0.36	0.20	0.25	0.27	0.39	0.38	0.22	0.56	0.17	0.50	546


==> data/mlm_plots/mlm_distil_fast/mr/cnn/s/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.09
top50	0.15


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	97.61	154.30	130.84	74.07	234.54	80.24	202.25	3.00	4.62	4.00	2.57	6.66	2.04	6.00	116.51	176.72	149.58	87.30	266.14	89.42	236.75	3.00	4.59	4.00	2.58	6.60	2.01	6.00	312
0.06	101.44	236.62	183.41	20.33	452.91	216.29	283.67	3.00	4.33	4.00	2.10	6.56	2.23	5.00	124.80	275.09	209.58	27.17	523.01	247.92	334.53	3.00	4.30	4.00	2.11	6.48	2.18	5.00	1219
0.11	104.11	237.21	178.58	41.37	433.06	195.84	305.61	3.00	4.42	4.00	2.02	6.82	2.40	5.00	139.73	300.61	220.94	60.55	540.67	240.06	390.75	3.00	4.33	4.00	1.99	6.67	2.34	5.00	989
0.15	109.11	303.78	189.01	-48.57	656.12	352.35	358.83	2.00	3.73	3.00	1.97	5.50	1.77	5.00	155.16	371.54	273.84	26.18	716.91	345.37	472.57	2.00	3.65	3.00	1.90	5.41	1.76	4.00	326
0.18	97.81	235.90	186.77	24.78	447.02	211.12	334.78	3.00	4.59	4.00	1.95	7.23	2.64	6.00	184.42	381.77	315.52	103.64	659.90	278.13	508.51	2.25	4.38	4.00	1.79	6.96	2.58	5.00	502
0.32	100.73	245.25	173.04	-55.39	545.89	300.64	295.30	3.00	4.39	4.00	2.01	6.76	2.37	5.00	272.38	543.24	430.37	134.26	952.22	408.98	681.77	3.00	4.14	4.00	1.83	6.45	2.31	5.00	1787


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	70.62
orig_ge	1.27
adv_pp	110.47
adv_ge	1.22


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.00	0.00	0.00	0.00	0.00	0.00	-0.30	-0.13	-0.16	-0.35	0.10	0.23	0.04	0.00	0.00	0.00	0.00	0.00	0.00	0.00	312
0.06	0.00	-0.00	0.00	-0.31	0.30	0.30	0.00	-0.16	0.10	0.11	-0.27	0.46	0.37	0.35	0.00	0.10	0.00	-0.16	0.36	0.26	0.20	1219
0.11	-0.49	-0.19	-0.14	-0.61	0.22	0.42	0.00	-0.31	-0.02	0.01	-0.45	0.40	0.43	0.32	-0.19	0.00	0.00	-0.33	0.33	0.33	0.21	989
0.15	-0.75	-0.36	-0.34	-0.75	0.03	0.39	0.00	-0.50	-0.20	-0.27	-0.59	0.19	0.39	0.11	-0.33	-0.12	-0.08	-0.40	0.17	0.28	0.00	326
0.18	-0.71	-0.48	-0.48	-0.77	-0.20	0.29	-0.28	-0.56	-0.35	-0.36	-0.66	-0.04	0.31	-0.18	-0.41	-0.25	-0.24	-0.50	0.01	0.25	-0.08	502
0.32	-0.81	-0.58	-0.64	-0.88	-0.29	0.29	-0.42	-0.64	-0.41	-0.45	-0.72	-0.10	0.31	-0.23	-0.49	-0.31	-0.32	-0.56	-0.05	0.26	-0.15	1787


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/correlations_auc.tex <==
name	auc
pcc	-0.10
spearman	-0.06
kendall	-0.04


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	4.76	6.38	5.82	3.63	9.13	2.75	7.19	4.65	9.23	7.01	2.11	16.36	7.12	10.06	6.17	22.27	19.31	7.05	37.49	15.22	33.68	312
0.06	3.23	4.35	4.15	2.03	6.67	2.32	5.20	3.04	5.47	4.56	1.80	9.14	3.67	6.63	3.25	13.92	7.67	-1.07	28.90	14.99	20.29	1219
0.11	2.71	3.99	3.70	2.04	5.94	1.95	5.05	2.66	4.86	4.11	1.52	8.20	3.34	6.49	2.57	12.35	5.14	-3.26	27.96	15.61	15.03	989
0.15	2.88	3.95	3.49	2.18	5.71	1.77	4.97	2.61	4.68	4.02	1.77	7.58	2.90	5.60	2.47	12.32	5.27	-3.06	27.69	15.37	15.70	326
0.18	3.02	3.88	3.72	2.67	5.08	1.20	4.63	3.23	4.61	4.28	2.50	6.72	2.11	5.28	2.95	10.10	5.01	-2.65	22.85	12.75	11.57	502
0.32	2.57	3.24	3.10	2.19	4.29	1.05	3.75	2.64	3.63	3.29	2.08	5.17	1.54	4.27	2.18	5.67	3.26	-2.76	14.10	8.43	5.62	1787


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/ets_sts_auc.tex <==
name	auc
et_use	1.14
et_tse	1.39
et_ce	3.15


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.84	10.39	4.28	-4.95	25.73	15.34	10.92	7.51	19.89	15.34	4.45	35.32	15.44	29.44	7.53	43.08	21.44	-16.81	102.96	59.88	39.02	312
0.06	0.98	9.58	2.15	-27.38	46.54	36.96	4.95	7.54	19.45	13.37	-0.53	39.44	19.99	23.65	6.80	40.63	15.08	-33.53	114.79	74.16	36.71	1219
0.11	0.92	6.51	1.93	-12.69	25.71	19.20	4.48	6.82	17.88	12.14	0.41	35.34	17.46	22.99	5.95	29.54	12.44	-18.17	77.26	47.72	30.02	989
0.15	0.77	3.59	1.47	-3.23	10.40	6.81	3.21	7.15	16.35	11.15	0.33	32.37	16.02	19.71	7.00	30.31	15.18	-26.11	86.74	56.43	27.24	326
0.18	0.50	3.47	0.94	-9.70	16.64	13.17	1.92	5.78	13.32	8.74	-1.37	28.02	14.69	14.23	5.28	25.89	10.63	-27.37	79.15	53.26	17.50	502
0.32	0.27	2.35	0.56	-10.10	14.79	12.44	1.31	5.15	9.89	6.88	-0.81	20.58	10.69	10.64	4.26	18.70	6.91	-38.07	75.47	56.77	13.64	1787


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/ets_time_misc_auc.tex <==
name	auc
et_p	1.40
et_p_h	4.29
et_p_l2	8.17


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.05	0.22	0.12	-0.12	0.56	0.34	0.27	0.01	0.05	0.02	-0.00	0.09	0.05	0.07	0.02	0.05	0.03	0.01	0.08	0.04	0.07	312
0.06	0.10	0.34	0.22	0.00	0.68	0.34	0.47	0.01	0.05	0.03	-0.01	0.11	0.06	0.07	0.02	0.05	0.04	0.01	0.09	0.04	0.06	1219
0.11	0.13	0.47	0.29	-0.10	1.04	0.57	0.58	0.02	0.07	0.04	0.00	0.13	0.06	0.09	0.03	0.06	0.05	0.02	0.10	0.04	0.08	989
0.15	0.21	0.62	0.41	0.02	1.21	0.60	0.92	0.02	0.07	0.05	0.00	0.13	0.07	0.09	0.04	0.07	0.06	0.02	0.11	0.04	0.09	326
0.18	0.40	1.04	0.79	0.13	1.94	0.90	1.43	0.04	0.09	0.08	0.03	0.16	0.07	0.14	0.05	0.09	0.08	0.04	0.13	0.05	0.12	502
0.32	0.60	2.11	1.39	-0.18	4.40	2.29	2.89	0.06	0.13	0.11	0.04	0.21	0.08	0.19	0.07	0.12	0.11	0.06	0.17	0.06	0.15	1787


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.29
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.90	0.91	0.91	0.89	0.94	0.03	0.93	0.89	0.92	0.93	0.88	0.96	0.04	0.95	0.92	0.94	0.97	0.84	1.04	0.10	0.99	312
0.06	0.85	0.87	0.88	0.83	0.91	0.04	0.90	0.85	0.88	0.89	0.82	0.94	0.06	0.92	0.86	0.90	0.94	0.79	1.01	0.11	0.98	1219
0.11	0.81	0.84	0.84	0.79	0.88	0.04	0.87	0.81	0.85	0.86	0.78	0.91	0.07	0.90	0.79	0.86	0.89	0.73	0.99	0.13	0.96	989
0.15	0.78	0.81	0.82	0.77	0.86	0.05	0.84	0.77	0.82	0.82	0.75	0.89	0.07	0.88	0.75	0.83	0.86	0.69	0.97	0.14	0.95	326
0.18	0.77	0.80	0.80	0.75	0.85	0.05	0.83	0.78	0.81	0.82	0.75	0.88	0.07	0.86	0.74	0.83	0.86	0.71	0.96	0.12	0.94	502
0.32	0.70	0.74	0.74	0.68	0.80	0.06	0.78	0.71	0.76	0.76	0.69	0.83	0.07	0.81	0.65	0.74	0.76	0.57	0.90	0.16	0.85	1787


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.23
sts_tse	0.24
sts_ce	0.24


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.87	2.66	1.04	0.54	4.77	2.12	4.89	0.00	0.01	0.00	-0.01	0.03	0.02	0.01	5.11	8.27	8.74	3.91	12.64	4.37	11.17	312
0.06	0.72	1.35	0.84	0.23	2.47	1.12	1.11	0.01	0.96	0.02	-2.04	3.95	2.99	0.16	1.64	4.53	3.41	0.55	8.51	3.98	6.61	1219
0.11	0.64	0.92	0.81	0.40	1.43	0.52	0.98	0.01	1.39	0.04	-2.91	5.70	4.30	1.60	1.45	4.89	3.38	0.06	9.72	4.83	6.47	989
0.15	0.66	0.87	0.78	0.49	1.24	0.38	0.94	0.01	0.83	0.03	-2.18	3.84	3.01	0.12	1.50	4.77	2.94	-0.13	9.66	4.90	6.25	326
0.18	0.75	1.13	1.01	0.62	1.63	0.51	1.42	0.02	0.07	0.04	-0.02	0.16	0.09	0.08	1.90	6.70	4.87	0.41	12.99	6.29	8.87	502
0.32	0.70	0.79	0.83	0.61	0.96	0.17	0.92	0.02	1.12	0.05	-3.00	5.23	4.12	0.17	1.73	5.86	4.23	0.47	11.24	5.38	8.36	1787


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/time_misc_auc.tex <==
name	auc
attack_time	0.32
l2	0.21
lom	1.67


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.11	0.00	-0.10	0.31	0.21	0.00	0.14	0.34	0.29	0.17	0.51	0.17	0.43	0.46	0.56	0.54	0.45	0.67	0.11	0.67	312
0.06	0.00	0.17	0.00	-0.12	0.46	0.29	0.50	0.17	0.37	0.33	0.11	0.63	0.26	0.57	0.43	0.56	0.56	0.38	0.73	0.18	0.69	1219
0.11	0.00	0.11	0.00	-0.13	0.35	0.24	0.00	0.00	0.31	0.29	0.05	0.57	0.26	0.50	0.38	0.52	0.50	0.31	0.73	0.21	0.67	989
0.15	0.00	0.11	0.00	-0.18	0.39	0.28	0.00	0.00	0.26	0.20	0.01	0.52	0.25	0.50	0.33	0.46	0.44	0.27	0.66	0.19	0.67	326
0.18	0.00	0.04	0.00	-0.13	0.20	0.16	0.00	0.00	0.18	0.14	-0.01	0.36	0.18	0.29	0.31	0.40	0.38	0.25	0.55	0.15	0.50	502
0.32	0.00	0.03	0.00	-0.10	0.15	0.13	0.00	0.00	0.16	0.14	-0.02	0.34	0.18	0.29	0.27	0.38	0.38	0.22	0.54	0.16	0.46	1787


==> data/mlm_plots/mlm_distil_fast/mr/lstm/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.07
top50	0.13


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	88.64	171.23	138.33	53.98	288.48	117.25	217.45	3.00	4.32	4.00	2.48	6.16	1.84	5.00	105.18	186.66	154.18	71.53	301.79	115.13	236.75	3.00	4.37	4.00	2.55	6.18	1.81	5.00	648
0.06	100.73	238.88	184.20	32.39	445.37	206.49	305.21	3.00	4.39	4.00	2.01	6.77	2.38	5.00	132.20	283.33	213.59	46.67	519.99	236.66	349.52	3.00	4.31	4.00	2.04	6.57	2.27	5.00	1347
0.11	97.56	255.00	183.61	-97.46	607.45	352.45	292.47	3.00	4.34	4.00	1.96	6.73	2.38	5.00	152.98	352.75	259.51	22.77	682.74	329.99	435.16	3.00	4.20	4.00	1.95	6.44	2.25	5.00	929
0.15	118.76	308.23	187.02	-44.73	661.19	352.96	351.60	2.00	3.68	3.00	2.07	5.30	1.62	5.00	211.48	410.15	325.07	129.41	690.88	280.74	535.09	2.00	3.48	3.00	1.98	4.97	1.50	5.00	301
0.18	105.74	234.42	186.36	66.91	401.92	167.50	338.91	3.00	4.68	5.00	2.04	7.31	2.64	6.00	217.47	443.81	359.21	152.10	735.51	291.70	615.97	2.50	4.36	4.00	1.87	6.86	2.50	6.00	379
0.32	102.38	244.60	177.24	6.35	482.85	238.25	293.87	3.00	4.45	4.00	2.00	6.90	2.45	6.00	354.22	740.11	568.89	114.06	1366.17	626.06	922.49	2.00	3.92	4.00	1.68	6.15	2.23	5.00	1334


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/comparison_vals_auc.tex <==
name	auc
orig_pp	71.77
orig_ge	1.27
adv_pp	133.39
adv_ge	1.19


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.00	0.00	0.00	0.00	0.00	0.00	-0.17	0.11	0.15	-0.26	0.48	0.37	0.40	0.00	0.00	0.00	0.00	0.00	0.00	0.00	648
0.06	0.00	0.14	0.00	-0.10	0.38	0.24	0.25	-0.19	0.18	0.19	-0.25	0.61	0.43	0.56	0.00	0.17	0.00	-0.09	0.43	0.26	0.39	1347
0.11	0.00	0.21	0.11	-0.05	0.47	0.26	0.41	0.20	0.38	0.47	0.00	0.75	0.38	0.66	0.00	0.28	0.29	0.02	0.55	0.26	0.51	929
0.15	0.00	0.12	0.00	-0.14	0.38	0.26	0.24	0.00	0.23	0.32	-0.15	0.61	0.38	0.50	0.00	0.19	0.17	-0.05	0.43	0.24	0.38	301
0.18	-0.06	0.10	0.04	-0.13	0.33	0.23	0.26	0.14	0.30	0.35	-0.03	0.63	0.33	0.50	0.10	0.25	0.25	0.03	0.47	0.22	0.37	379
0.32	-0.21	-0.06	-0.09	-0.28	0.17	0.23	0.07	-0.09	0.11	0.13	-0.18	0.41	0.30	0.32	-0.05	0.09	0.08	-0.13	0.30	0.21	0.22	1334


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/correlations_auc.tex <==
name	auc
pcc	0.02
spearman	0.07
kendall	0.05


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	4.67	6.33	5.67	3.78	8.88	2.55	7.12	4.65	8.82	7.01	1.83	15.81	6.99	9.68	5.14	18.36	12.32	3.34	33.39	15.03	31.88	648
0.06	2.85	4.03	3.90	1.93	6.13	2.10	4.80	2.80	5.11	4.21	1.67	8.55	3.44	6.14	3.29	14.07	9.17	0.45	27.69	13.62	20.65	1347
0.11	1.98	2.76	2.72	1.61	3.91	1.15	3.38	1.93	3.31	2.81	1.27	5.34	2.03	4.10	2.46	9.00	5.03	-0.57	18.57	9.57	12.14	929
0.15	1.93	2.62	2.38	1.55	3.70	1.08	3.11	2.13	3.14	2.69	1.47	4.82	1.67	3.79	2.33	9.77	4.61	-2.16	21.69	11.92	10.94	301
0.18	2.00	2.58	2.38	1.59	3.56	0.99	2.95	2.06	3.18	2.91	1.68	4.68	1.50	3.75	2.28	7.44	3.36	-1.70	16.59	9.15	8.64	379
0.32	1.83	2.26	2.18	1.58	2.94	0.68	2.58	1.96	2.56	2.40	1.64	3.49	0.93	2.96	1.76	4.11	2.50	-1.35	9.56	5.45	3.99	1334


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/ets_sts_auc.tex <==
name	auc
et_use	0.85
et_tse	1.04
et_ce	2.51


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.71	8.01	3.61	-3.72	19.74	11.73	8.32	9.84	21.85	15.48	4.65	39.05	17.20	30.09	11.69	42.63	21.58	-19.13	104.38	61.76	33.90	648
0.06	0.65	8.63	1.69	-27.23	44.50	35.86	4.46	4.72	18.17	11.84	-2.01	38.36	20.19	22.35	4.85	39.02	12.70	-34.34	112.38	73.36	37.64	1347
0.11	0.32	3.27	0.75	-9.73	16.28	13.00	2.08	3.42	11.93	6.09	-3.46	27.33	15.40	12.61	3.14	24.66	6.99	-22.73	72.06	47.40	19.06	929
0.15	0.29	2.00	0.77	-3.00	6.99	4.99	1.94	3.69	10.09	7.33	1.55	18.63	8.54	14.02	3.36	20.89	8.65	-19.68	61.47	40.57	21.08	301
0.18	0.22	1.51	0.39	-2.99	6.00	4.49	0.88	3.19	6.93	5.02	-0.63	14.50	7.56	7.43	2.78	11.76	5.37	-6.31	29.83	18.07	11.81	379
0.32	0.13	0.94	0.24	-3.30	5.17	4.24	0.51	3.22	6.08	4.29	-0.51	12.67	6.59	6.38	2.79	11.73	4.52	-21.09	44.54	32.81	8.59	1334


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.86
et_p_h	2.95
et_p_l2	5.84


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.06	0.21	0.14	-0.05	0.48	0.27	0.29	0.01	0.04	0.02	-0.01	0.09	0.05	0.04	0.02	0.04	0.03	0.01	0.07	0.03	0.05	648
0.06	0.11	0.39	0.25	0.01	0.76	0.38	0.55	0.01	0.06	0.03	-0.01	0.12	0.06	0.07	0.02	0.05	0.04	0.01	0.10	0.04	0.07	1347
0.11	0.21	0.70	0.50	-0.00	1.41	0.71	0.91	0.02	0.07	0.05	0.01	0.14	0.07	0.11	0.03	0.07	0.06	0.02	0.12	0.05	0.10	929
0.15	0.24	0.85	0.53	-0.00	1.70	0.85	1.35	0.02	0.08	0.05	0.01	0.14	0.07	0.12	0.03	0.07	0.06	0.02	0.12	0.05	0.10	301
0.18	0.54	1.29	1.07	0.28	2.30	1.01	1.80	0.04	0.10	0.09	0.03	0.17	0.07	0.15	0.06	0.10	0.09	0.05	0.14	0.05	0.14	379
0.32	1.04	3.04	2.13	-0.09	6.17	3.13	4.01	0.06	0.13	0.12	0.05	0.21	0.08	0.19	0.08	0.12	0.12	0.07	0.18	0.06	0.16	1334


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.40
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.89	0.92	0.93	0.87	0.96	0.05	0.95	0.90	0.93	0.96	0.85	1.01	0.08	0.98	648
0.06	0.86	0.88	0.89	0.85	0.92	0.04	0.90	0.86	0.89	0.90	0.84	0.94	0.05	0.93	0.88	0.91	0.96	0.82	1.01	0.09	0.98	1347
0.11	0.82	0.85	0.85	0.80	0.89	0.05	0.88	0.82	0.86	0.86	0.79	0.92	0.06	0.90	0.83	0.89	0.92	0.78	1.00	0.11	0.97	929
0.15	0.79	0.82	0.83	0.77	0.87	0.05	0.86	0.80	0.84	0.85	0.78	0.90	0.06	0.88	0.80	0.86	0.91	0.72	1.00	0.14	0.97	301
0.18	0.78	0.81	0.81	0.76	0.86	0.05	0.84	0.80	0.84	0.85	0.78	0.90	0.06	0.88	0.81	0.86	0.88	0.76	0.96	0.10	0.95	379
0.32	0.72	0.76	0.76	0.71	0.81	0.05	0.79	0.74	0.78	0.78	0.71	0.84	0.06	0.82	0.70	0.78	0.79	0.64	0.91	0.13	0.87	1334


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.82	2.59	1.01	0.57	4.61	2.02	4.94	1.24	1.97	1.76	0.89	3.05	1.08	2.40	9.09	11.73	11.53	8.04	15.41	3.68	14.25	648
0.06	0.67	1.45	0.81	0.20	2.70	1.25	1.69	1.17	11.30	1.80	-11.06	33.66	22.36	3.49	3.04	5.97	5.99	2.42	9.51	3.54	8.47	1347
0.11	0.63	0.90	0.77	0.27	1.53	0.63	0.85	1.18	15.48	2.01	-13.30	44.27	28.78	19.25	1.43	3.20	2.48	0.68	5.73	2.53	4.52	929
0.15	0.71	0.91	0.77	0.33	1.48	0.57	0.90	1.10	9.24	1.78	-16.16	34.64	25.40	3.12	1.45	3.10	2.54	0.65	5.55	2.45	3.92	301
0.18	0.78	1.11	1.00	0.56	1.65	0.54	1.21	1.78	2.63	2.35	1.20	4.05	1.42	3.05	1.13	3.04	2.51	0.66	5.42	2.38	4.17	379
0.32	0.65	0.71	0.76	0.52	0.90	0.19	0.84	2.02	17.73	2.86	-17.10	52.55	34.83	6.20	1.14	2.99	2.44	0.65	5.33	2.34	4.29	1334


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/time_misc_auc.tex <==
name	auc
attack_time	0.31
l2	2.94
lom	1.13


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.09	0.00	-0.11	0.29	0.20	0.00	0.14	0.27	0.29	0.08	0.45	0.19	0.43	0.31	0.46	0.46	0.30	0.62	0.16	0.54	648
0.06	0.00	0.15	0.00	-0.13	0.44	0.29	0.00	0.17	0.36	0.33	0.12	0.61	0.25	0.57	0.43	0.59	0.60	0.41	0.78	0.19	0.75	1347
0.11	0.00	0.16	0.00	-0.12	0.44	0.28	0.50	0.29	0.43	0.43	0.17	0.69	0.26	0.60	0.50	0.62	0.67	0.39	0.84	0.22	0.77	929
0.15	0.00	0.15	0.00	-0.18	0.47	0.33	0.00	0.20	0.39	0.33	0.13	0.65	0.26	0.50	0.46	0.60	0.64	0.43	0.78	0.17	0.70	301
0.18	0.00	0.11	0.00	-0.15	0.36	0.25	0.00	0.25	0.37	0.33	0.16	0.58	0.21	0.50	0.55	0.63	0.62	0.46	0.80	0.17	0.70	379
0.32	0.00	0.03	0.00	-0.11	0.18	0.15	0.00	0.14	0.26	0.29	0.07	0.46	0.20	0.43	0.45	0.54	0.54	0.39	0.68	0.14	0.62	1334


==> data/mlm_plots/mlm_distil_fast/mr/lstm/s/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.10
top50	0.17


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	101.00	198.57	158.54	55.72	341.41	142.85	249.00	3.00	4.87	4.00	2.72	7.03	2.15	6.00	131.20	238.52	196.49	77.59	399.45	160.93	293.91	3.00	4.87	4.00	2.72	7.02	2.15	6.00	595
0.11	97.42	218.78	172.62	37.67	399.88	181.11	279.18	3.00	4.60	4.00	2.52	6.68	2.08	6.00	137.60	281.83	232.55	69.08	494.58	212.75	352.26	3.00	4.58	4.00	2.49	6.68	2.09	6.00	1061
0.15	110.90	271.25	202.15	-2.75	545.25	274.00	305.24	2.00	3.75	3.00	2.02	5.48	1.73	5.00	163.30	383.79	278.35	33.82	733.76	349.97	467.83	2.00	3.76	3.00	2.00	5.52	1.76	5.00	531
0.18	111.24	234.88	185.04	48.10	421.67	186.78	292.47	3.00	4.54	4.00	2.10	6.97	2.44	6.00	179.21	379.63	304.65	68.49	690.77	311.14	453.28	3.00	4.53	4.00	2.12	6.94	2.41	6.00	742
0.32	104.46	244.27	181.47	-16.97	505.51	261.24	292.02	3.00	4.26	4.00	2.08	6.45	2.18	5.00	257.14	544.16	412.88	62.61	1025.71	481.55	680.28	3.00	4.13	4.00	1.97	6.28	2.15	5.00	2729


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/comparison_vals_auc.tex <==
name	auc
orig_pp	61.62
orig_ge	1.14
adv_pp	102.40
adv_ge	1.13


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.27	0.42	0.43	0.20	0.64	0.22	0.58	0.51	0.63	0.65	0.42	0.84	0.21	0.79	0.41	0.53	0.54	0.34	0.72	0.19	0.66	595
0.11	0.16	0.33	0.34	0.09	0.57	0.24	0.50	0.41	0.57	0.61	0.33	0.82	0.25	0.77	0.34	0.48	0.50	0.26	0.69	0.21	0.63	1061
0.15	0.04	0.24	0.24	-0.02	0.50	0.26	0.44	0.34	0.52	0.51	0.26	0.78	0.26	0.72	0.27	0.44	0.43	0.21	0.66	0.23	0.61	531
0.18	-0.14	0.08	0.04	-0.20	0.36	0.28	0.30	0.13	0.35	0.36	0.03	0.67	0.32	0.57	0.10	0.28	0.28	0.02	0.53	0.26	0.43	742
0.32	-0.32	-0.13	-0.16	-0.40	0.15	0.28	0.03	-0.21	0.08	0.05	-0.30	0.45	0.37	0.35	-0.14	0.07	0.05	-0.21	0.35	0.28	0.27	2729


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/correlations_auc.tex <==
name	auc
pcc	0.03
spearman	0.10
kendall	0.08


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	1.55	2.49	2.20	1.08	3.89	1.40	3.12	1.49	2.80	2.43	0.93	4.68	1.87	3.50	1.46	5.83	2.83	-1.15	12.80	6.97	7.27	595
0.11	1.53	2.28	2.07	1.15	3.42	1.13	2.88	1.51	2.59	2.17	0.99	4.19	1.60	3.31	1.46	5.25	2.47	-1.94	12.44	7.19	5.59	1061
0.15	1.57	2.11	2.00	1.23	2.98	0.88	2.51	1.51	2.35	2.06	0.83	3.88	1.53	2.64	1.38	5.43	2.14	-2.81	13.68	8.25	4.47	531
0.18	1.77	2.35	2.40	1.45	3.25	0.90	2.86	1.83	2.57	2.41	1.45	3.70	1.12	3.08	1.56	4.19	2.40	-1.77	10.16	5.96	4.01	742
0.32	1.77	2.21	2.13	1.47	2.95	0.74	2.55	1.83	2.37	2.21	1.46	3.28	0.91	2.78	1.39	2.79	1.93	-0.71	6.30	3.51	2.93	2729


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/ets_sts_auc.tex <==
name	auc
et_use	0.59
et_tse	0.65
et_ce	1.13


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.55	4.15	1.14	-9.87	18.18	14.03	2.67	3.61	8.47	6.58	1.20	15.74	7.27	11.07	3.30	10.74	6.40	-4.23	25.71	14.97	12.55	595
0.11	0.45	3.02	0.95	-8.23	14.27	11.25	2.02	3.80	8.24	6.22	1.36	15.12	6.88	10.80	3.38	11.61	6.84	-9.48	32.71	21.09	12.69	1061
0.15	0.43	2.94	0.78	-6.04	11.92	8.98	1.73	3.95	10.11	6.65	-1.87	22.10	11.99	11.80	3.44	17.17	7.09	-11.98	46.32	29.15	15.15	531
0.18	0.38	1.80	0.73	-1.11	4.71	2.91	1.97	4.21	8.48	5.74	0.20	16.75	8.28	9.89	3.46	13.03	5.76	-13.50	39.56	26.53	13.30	742
0.32	0.22	2.41	0.42	-13.12	17.94	15.53	1.01	3.94	7.33	5.46	-0.50	15.16	7.83	8.27	3.34	12.26	5.42	-20.51	45.04	32.77	10.50	2729


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.66
et_p_h	2.18
et_p_l2	3.39


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.10	0.32	0.25	0.03	0.61	0.29	0.46	0.02	0.06	0.04	0.01	0.10	0.05	0.07	0.03	0.05	0.04	0.02	0.09	0.03	0.07	595
0.11	0.18	0.47	0.35	0.06	0.88	0.41	0.66	0.03	0.06	0.05	0.01	0.12	0.05	0.09	0.03	0.06	0.05	0.02	0.10	0.04	0.08	1061
0.15	0.20	0.68	0.45	-0.07	1.42	0.75	0.90	0.03	0.07	0.05	0.01	0.13	0.06	0.09	0.03	0.06	0.05	0.02	0.11	0.04	0.08	531
0.18	0.23	0.88	0.60	-0.01	1.76	0.89	1.20	0.04	0.09	0.08	0.03	0.15	0.06	0.14	0.04	0.08	0.07	0.04	0.12	0.04	0.11	742
0.32	0.53	1.91	1.29	-0.17	4.00	2.08	2.51	0.05	0.12	0.10	0.04	0.19	0.08	0.17	0.06	0.11	0.10	0.05	0.16	0.05	0.14	2729


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.26
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.84	0.87	0.87	0.83	0.91	0.04	0.90	0.84	0.87	0.88	0.82	0.93	0.06	0.92	0.82	0.88	0.90	0.76	0.99	0.11	0.96	595
0.11	0.81	0.84	0.84	0.80	0.88	0.04	0.87	0.80	0.85	0.85	0.78	0.91	0.06	0.89	0.78	0.85	0.87	0.73	0.96	0.11	0.94	1061
0.15	0.78	0.81	0.81	0.77	0.85	0.04	0.84	0.77	0.81	0.82	0.75	0.88	0.06	0.86	0.73	0.81	0.83	0.68	0.95	0.13	0.92	531
0.18	0.77	0.80	0.80	0.75	0.84	0.04	0.82	0.77	0.81	0.81	0.75	0.86	0.06	0.85	0.73	0.80	0.81	0.67	0.92	0.13	0.89	742
0.32	0.70	0.73	0.73	0.68	0.79	0.06	0.77	0.70	0.75	0.74	0.68	0.81	0.07	0.80	0.60	0.69	0.71	0.53	0.85	0.16	0.81	2729


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.20


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.47	0.51	0.49	0.40	0.63	0.11	0.51	0.11	0.16	0.15	0.09	0.24	0.07	0.20	1.05	2.48	2.19	0.71	4.25	1.77	3.54	595
0.11	0.41	0.49	0.46	0.33	0.65	0.16	0.62	0.14	0.21	0.19	0.12	0.29	0.09	0.26	1.04	2.57	2.19	0.63	4.51	1.94	3.62	1061
0.15	0.26	0.38	0.33	0.23	0.53	0.15	0.51	0.18	0.25	0.24	0.15	0.36	0.10	0.32	0.81	2.16	1.90	0.52	3.80	1.64	3.05	531
0.18	0.25	0.30	0.28	0.23	0.38	0.08	0.33	0.18	0.26	0.25	0.16	0.36	0.10	0.33	1.43	3.45	3.08	1.01	5.88	2.44	4.96	742
0.32	0.34	0.42	0.41	0.32	0.51	0.10	0.47	0.20	0.27	0.26	0.17	0.37	0.10	0.34	1.41	3.52	3.08	1.02	6.02	2.50	5.13	2729


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/time_misc_auc.tex <==
name	auc
attack_time	0.10
l2	0.06
lom	0.79


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.17	0.00	-0.09	0.43	0.26	0.50	0.43	0.59	0.57	0.41	0.76	0.17	0.71	0.69	0.77	0.77	0.65	0.89	0.12	0.85	595
0.11	0.00	0.11	0.00	-0.12	0.34	0.23	0.00	0.43	0.53	0.57	0.33	0.73	0.20	0.67	0.67	0.74	0.75	0.60	0.88	0.14	0.83	1061
0.15	0.00	0.05	0.00	-0.13	0.23	0.18	0.00	0.33	0.42	0.50	0.20	0.65	0.23	0.57	0.64	0.72	0.71	0.57	0.88	0.15	0.83	531
0.18	0.00	0.04	0.00	-0.13	0.21	0.17	0.00	0.17	0.35	0.33	0.13	0.56	0.22	0.50	0.50	0.63	0.62	0.47	0.79	0.16	0.73	742
0.32	0.00	0.02	0.00	-0.09	0.12	0.10	0.00	0.00	0.20	0.17	0.01	0.40	0.19	0.33	0.40	0.53	0.50	0.36	0.70	0.17	0.64	2729


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/a/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.10
top50	0.17


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	101.52	199.38	159.17	56.10	342.66	143.28	246.75	3.00	4.87	4.00	2.66	7.08	2.21	6.00	126.31	241.26	200.88	71.72	410.80	169.54	310.32	3.00	4.87	4.50	2.65	7.09	2.22	6.00	588
0.11	97.08	223.35	172.79	29.43	417.28	193.93	280.19	3.00	4.65	4.00	2.38	6.92	2.27	6.00	137.71	297.94	238.90	56.03	539.86	241.91	367.19	3.00	4.61	4.00	2.34	6.89	2.27	6.00	1055
0.15	115.07	271.93	201.25	-8.82	552.68	280.75	292.02	2.00	3.86	4.00	2.11	5.61	1.75	5.00	189.81	380.73	293.84	34.93	726.52	345.80	429.51	2.00	3.80	4.00	2.08	5.51	1.71	5.00	493
0.18	109.84	232.23	183.70	44.85	419.62	187.38	289.99	3.00	4.55	4.00	2.12	6.99	2.44	6.00	197.94	392.32	281.33	123.80	660.84	268.52	535.39	3.00	4.42	4.00	2.04	6.80	2.38	6.00	738
0.32	103.89	238.65	178.60	-9.59	486.89	248.24	287.55	3.00	4.28	4.00	2.09	6.47	2.19	5.00	266.73	541.52	426.94	115.72	967.32	425.80	676.62	3.00	3.98	4.00	1.83	6.12	2.15	5.00	2692


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	61.26
orig_ge	1.15
adv_pp	103.96
adv_ge	1.11


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.01	0.30	0.28	-0.07	0.66	0.37	0.57	0.41	0.54	0.53	0.31	0.78	0.24	0.70	0.33	0.48	0.49	0.27	0.69	0.21	0.61	588
0.11	-0.10	0.15	0.12	-0.22	0.52	0.37	0.39	0.21	0.39	0.38	0.13	0.65	0.26	0.56	0.20	0.35	0.35	0.13	0.58	0.23	0.50	1055
0.15	-0.22	0.07	-0.00	-0.33	0.47	0.40	0.29	0.07	0.30	0.28	0.00	0.60	0.30	0.47	0.08	0.29	0.27	0.03	0.54	0.25	0.43	493
0.18	-0.40	-0.11	-0.20	-0.54	0.31	0.43	0.11	-0.07	0.13	0.12	-0.20	0.47	0.33	0.30	-0.01	0.15	0.14	-0.13	0.42	0.28	0.29	738
0.32	-0.58	-0.31	-0.38	-0.67	0.05	0.36	-0.12	-0.35	-0.11	-0.14	-0.43	0.21	0.32	0.08	-0.24	-0.05	-0.07	-0.30	0.20	0.25	0.10	2692


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/correlations_auc.tex <==
name	auc
pcc	-0.01
spearman	0.05
kendall	0.05


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	1.56	2.84	2.64	1.08	4.60	1.76	3.84	1.72	3.52	3.19	1.04	6.00	2.48	4.82	1.42	7.16	3.42	-2.09	16.40	9.25	8.76	588
0.11	1.91	2.86	2.72	1.33	4.39	1.53	3.64	2.13	3.49	3.12	1.31	5.68	2.18	4.55	1.69	6.96	3.29	-2.68	16.60	9.64	7.17	1055
0.15	1.92	2.60	2.58	1.17	4.03	1.43	3.24	1.96	3.01	2.84	1.14	4.88	1.87	3.96	1.68	5.22	2.89	-2.02	12.46	7.24	5.39	493
0.18	1.95	2.78	2.87	1.48	4.08	1.30	3.42	2.33	3.29	3.22	1.59	4.98	1.69	4.20	2.00	6.01	3.21	-2.90	14.91	8.90	6.08	738
0.32	2.08	2.62	2.58	1.65	3.60	0.97	3.07	2.18	2.99	2.80	1.67	4.31	1.32	3.56	1.64	3.52	2.45	-0.95	7.98	4.47	3.70	2692


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/ets_sts_auc.tex <==
name	auc
et_use	0.71
et_tse	0.84
et_ce	1.43


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.62	4.11	1.42	-7.10	15.32	11.21	3.22	3.78	11.31	7.21	-0.41	23.04	11.73	14.51	3.30	18.46	7.83	-13.97	50.90	32.43	18.79	588
0.11	0.52	4.61	1.10	-10.44	19.67	15.06	2.86	3.71	11.97	6.86	-10.53	34.48	22.50	12.95	3.19	24.61	7.86	-47.67	96.89	72.28	17.77	1055
0.15	0.42	2.99	0.89	-5.08	11.06	8.07	2.57	3.24	11.29	7.74	-2.55	25.14	13.84	14.67	2.55	24.45	9.67	-24.61	73.51	49.06	23.76	493
0.18	0.33	3.70	0.77	-13.01	20.40	16.70	1.93	4.07	11.62	7.09	-7.37	30.60	18.99	11.74	3.25	22.17	7.70	-26.53	70.88	48.71	16.89	738
0.32	0.23	2.06	0.47	-9.70	13.82	11.76	1.18	3.91	8.46	5.75	-1.14	18.06	9.60	9.48	3.29	16.08	6.06	-24.58	56.74	40.66	13.16	2692


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.87
et_p_h	2.80
et_p_l2	5.47


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.11	0.32	0.22	0.01	0.63	0.31	0.45	0.02	0.06	0.04	0.01	0.11	0.05	0.08	0.02	0.05	0.04	0.02	0.09	0.04	0.07	588
0.11	0.14	0.51	0.37	-0.01	1.02	0.51	0.67	0.02	0.07	0.05	0.01	0.14	0.07	0.11	0.03	0.07	0.06	0.02	0.12	0.05	0.10	1055
0.15	0.18	0.70	0.42	-0.11	1.50	0.81	0.95	0.02	0.08	0.05	0.00	0.16	0.08	0.12	0.04	0.07	0.06	0.02	0.13	0.05	0.10	493
0.18	0.32	0.98	0.75	0.07	1.90	0.92	1.35	0.03	0.09	0.07	0.01	0.17	0.08	0.15	0.04	0.09	0.08	0.04	0.14	0.05	0.12	738
0.32	0.56	1.95	1.33	-0.07	3.96	2.02	2.63	0.05	0.13	0.11	0.04	0.22	0.09	0.20	0.07	0.12	0.11	0.06	0.18	0.06	0.16	2692


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.27
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.84	0.87	0.87	0.83	0.90	0.04	0.89	0.85	0.88	0.89	0.83	0.93	0.05	0.92	0.82	0.87	0.91	0.75	1.00	0.13	0.96	588
0.11	0.82	0.84	0.84	0.80	0.88	0.04	0.87	0.82	0.86	0.86	0.80	0.91	0.06	0.90	0.79	0.85	0.88	0.71	0.98	0.13	0.95	1055
0.15	0.78	0.81	0.81	0.77	0.85	0.04	0.84	0.78	0.82	0.83	0.76	0.88	0.06	0.87	0.72	0.81	0.83	0.68	0.94	0.13	0.92	493
0.18	0.76	0.79	0.79	0.74	0.83	0.05	0.81	0.77	0.81	0.81	0.75	0.87	0.06	0.85	0.74	0.81	0.83	0.68	0.94	0.13	0.90	738
0.32	0.70	0.74	0.74	0.68	0.79	0.06	0.78	0.71	0.76	0.76	0.69	0.83	0.07	0.81	0.61	0.70	0.73	0.54	0.87	0.17	0.83	2692


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.21


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.85	0.94	0.94	0.77	1.12	0.18	1.01	1.21	3.12	1.99	-0.07	6.31	3.19	3.73	1.36	4.68	3.32	0.21	9.15	4.47	6.61	588
0.11	0.75	0.99	0.95	0.60	1.37	0.38	1.34	1.48	3.50	2.47	0.01	7.00	3.49	4.09	1.55	4.81	3.62	0.47	9.14	4.33	6.91	1055
0.15	0.35	0.72	0.54	0.31	1.13	0.41	1.09	1.70	3.17	2.56	0.74	5.59	2.42	3.81	0.97	3.90	2.71	-0.04	7.85	3.94	5.21	493
0.18	0.31	0.43	0.37	0.26	0.60	0.17	0.50	2.11	4.49	3.34	-1.31	10.29	5.80	5.12	1.60	5.38	3.98	0.51	10.24	4.87	7.92	738
0.32	0.38	0.47	0.47	0.36	0.57	0.11	0.54	2.10	4.60	3.24	-0.10	9.29	4.70	5.41	2.03	5.83	4.39	0.76	10.90	5.07	8.06	2692


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/time_misc_auc.tex <==
name	auc
attack_time	0.16
l2	1.05
lom	1.33


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.29	0.00	-0.03	0.60	0.31	0.50	0.43	0.62	0.57	0.44	0.80	0.18	0.71	0.69	0.77	0.77	0.65	0.88	0.11	0.85	588
0.11	0.00	0.20	0.00	-0.10	0.49	0.30	0.50	0.43	0.53	0.57	0.33	0.72	0.20	0.67	0.62	0.71	0.73	0.59	0.84	0.13	0.80	1055
0.15	0.00	0.13	0.00	-0.16	0.43	0.29	0.00	0.33	0.45	0.50	0.23	0.67	0.22	0.60	0.57	0.67	0.67	0.52	0.82	0.15	0.78	493
0.18	0.00	0.11	0.00	-0.15	0.38	0.27	0.00	0.25	0.39	0.33	0.17	0.61	0.22	0.57	0.54	0.62	0.62	0.46	0.78	0.16	0.71	738
0.32	0.00	0.06	0.00	-0.14	0.25	0.20	0.00	0.14	0.25	0.25	0.05	0.45	0.20	0.40	0.42	0.52	0.50	0.37	0.67	0.15	0.62	2692


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.11
top50	0.16


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	102.13	196.00	157.41	59.97	332.03	136.03	245.96	3.00	4.92	4.00	2.68	7.17	2.25	6.00	155.71	287.76	227.60	98.83	476.70	188.94	359.94	3.00	4.94	5.00	2.70	7.17	2.24	6.00	556
0.11	96.12	219.35	171.81	29.22	409.47	190.12	278.77	3.00	4.57	4.00	2.50	6.65	2.08	6.00	165.77	358.02	284.42	62.33	653.71	295.69	444.78	3.00	4.51	4.00	2.46	6.57	2.05	6.00	1021
0.15	104.94	246.18	190.00	15.73	476.64	230.45	280.39	2.00	3.82	3.00	2.07	5.58	1.75	5.00	226.74	437.85	340.65	95.73	779.97	342.12	553.38	2.00	3.75	4.00	1.96	5.54	1.79	5.00	489
0.18	109.52	233.82	185.04	47.84	419.79	185.98	292.47	3.00	4.56	4.00	2.12	7.00	2.44	6.00	259.19	517.59	439.25	148.79	886.39	368.80	659.53	3.00	4.42	4.00	2.03	6.81	2.39	6.00	734
0.32	104.11	240.11	179.91	2.04	478.18	238.07	290.69	3.00	4.26	4.00	2.10	6.42	2.16	5.00	380.48	818.29	625.01	96.16	1540.43	722.13	1019.46	2.00	3.86	3.00	1.81	5.90	2.04	5.00	2723


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/comparison_vals_auc.tex <==
name	auc
orig_pp	60.21
orig_ge	1.14
adv_pp	139.33
adv_ge	1.10


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.37	0.51	0.51	0.30	0.72	0.21	0.66	0.56	0.65	0.70	0.45	0.85	0.20	0.80	0.43	0.54	0.56	0.36	0.72	0.18	0.67	556
0.11	0.20	0.37	0.40	0.12	0.62	0.25	0.54	0.37	0.53	0.57	0.26	0.80	0.27	0.74	0.29	0.43	0.45	0.21	0.66	0.23	0.60	1021
0.15	0.06	0.25	0.29	-0.02	0.52	0.27	0.44	0.20	0.39	0.44	0.07	0.71	0.32	0.63	0.17	0.32	0.36	0.07	0.57	0.25	0.49	489
0.18	-0.03	0.13	0.11	-0.10	0.36	0.23	0.31	0.07	0.30	0.31	0.01	0.58	0.29	0.52	0.07	0.24	0.24	0.02	0.45	0.21	0.38	734
0.32	-0.23	-0.05	-0.05	-0.32	0.22	0.27	0.13	-0.18	0.07	0.08	-0.28	0.42	0.35	0.33	-0.12	0.06	0.06	-0.20	0.32	0.26	0.25	2723


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/correlations_auc.tex <==
name	auc
pcc	0.05
spearman	0.08
kendall	0.07


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	1.47	2.32	2.12	1.14	3.51	1.19	3.01	1.67	3.01	2.46	0.94	5.07	2.06	3.88	2.00	8.02	4.74	-0.41	16.45	8.43	11.33	556
0.11	1.51	2.38	2.19	1.14	3.62	1.24	3.00	1.66	3.07	2.47	0.83	5.31	2.24	3.91	2.08	7.96	4.38	-1.01	16.92	8.97	10.75	1021
0.15	1.61	2.31	2.18	1.29	3.33	1.02	2.75	1.77	2.93	2.57	1.27	4.59	1.66	3.61	1.99	9.46	4.23	-1.62	20.54	11.08	12.60	489
0.18	1.79	2.42	2.29	1.49	3.35	0.93	2.89	2.07	2.96	2.59	1.50	4.43	1.47	3.61	1.91	6.32	3.64	-0.94	13.58	7.26	7.76	734
0.32	1.82	2.29	2.19	1.53	3.04	0.76	2.67	1.97	2.72	2.52	1.57	3.87	1.15	3.21	1.81	4.53	2.65	-1.25	10.31	5.78	4.66	2723


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/ets_sts_auc.tex <==
name	auc
et_use	0.61
et_tse	0.76
et_ce	1.76


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.24	1.46	0.50	-2.70	5.62	4.16	1.21	2.11	4.85	3.39	-0.17	9.87	5.02	5.64	2.00	7.06	3.72	-5.02	19.15	12.09	7.38	556
0.11	0.24	1.71	0.48	-6.70	10.12	8.41	0.98	2.44	6.74	4.07	-2.39	15.88	9.14	7.04	2.30	12.32	4.46	-15.88	40.52	28.20	9.11	1021
0.15	0.22	1.91	0.40	-3.70	7.52	5.61	0.97	2.21	7.51	4.27	-2.91	17.94	10.42	7.21	1.95	14.42	4.17	-20.69	49.54	35.12	11.55	489
0.18	0.19	1.32	0.34	-4.53	7.17	5.85	0.63	2.94	6.52	4.25	-2.08	15.13	8.60	6.60	2.66	14.85	4.57	-35.59	65.28	50.43	10.26	734
0.32	0.12	1.07	0.21	-10.18	12.32	11.25	0.42	2.86	5.58	3.88	-0.84	12.00	6.42	5.92	2.46	12.30	3.77	-30.05	54.65	42.35	8.02	2723


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.37
et_p_h	1.64
et_p_l2	3.38


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.22	0.58	0.48	0.12	1.03	0.45	0.83	0.03	0.08	0.06	0.02	0.14	0.06	0.11	0.04	0.08	0.07	0.04	0.12	0.04	0.10	556
0.11	0.33	0.80	0.66	0.08	1.51	0.71	1.06	0.03	0.09	0.07	0.02	0.15	0.07	0.13	0.04	0.08	0.07	0.03	0.13	0.05	0.12	1021
0.15	0.34	1.16	0.93	-0.10	2.43	1.27	1.47	0.03	0.11	0.08	0.02	0.19	0.09	0.18	0.05	0.10	0.09	0.04	0.16	0.06	0.15	489
0.18	0.63	1.61	1.26	0.19	3.02	1.41	2.08	0.04	0.11	0.09	0.03	0.19	0.08	0.17	0.06	0.11	0.10	0.05	0.16	0.05	0.14	734
0.32	1.21	3.42	2.34	-0.18	7.03	3.60	4.39	0.06	0.14	0.13	0.05	0.23	0.09	0.21	0.09	0.13	0.13	0.07	0.19	0.06	0.18	2723


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.46
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.86	0.89	0.89	0.85	0.92	0.03	0.91	0.87	0.90	0.91	0.85	0.95	0.05	0.94	0.88	0.91	0.96	0.81	1.02	0.10	0.98	556
0.11	0.83	0.86	0.86	0.81	0.90	0.04	0.88	0.84	0.87	0.88	0.81	0.93	0.06	0.92	0.85	0.90	0.93	0.79	1.01	0.11	0.97	1021
0.15	0.80	0.83	0.83	0.79	0.87	0.04	0.86	0.82	0.85	0.85	0.80	0.91	0.06	0.90	0.82	0.88	0.92	0.77	1.00	0.12	0.98	489
0.18	0.78	0.81	0.81	0.76	0.86	0.05	0.84	0.80	0.83	0.84	0.77	0.89	0.06	0.87	0.78	0.85	0.88	0.72	0.97	0.13	0.95	734
0.32	0.73	0.76	0.76	0.71	0.81	0.05	0.80	0.75	0.79	0.79	0.73	0.85	0.06	0.83	0.72	0.79	0.81	0.65	0.92	0.13	0.89	2723


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.22
sts_ce	0.22


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	1.07	1.09	1.11	0.96	1.21	0.13	1.15	20.82	38.05	30.05	9.49	66.61	28.56	44.18	0.73	1.81	1.47	0.41	3.21	1.40	2.64	556
0.11	0.84	0.95	1.03	0.61	1.30	0.35	1.24	24.66	51.75	37.17	4.37	99.13	47.38	60.68	0.75	2.05	1.71	0.49	3.60	1.56	3.04	1021
0.15	0.27	0.63	0.44	0.23	1.02	0.40	1.04	29.31	61.12	44.72	0.55	121.68	60.56	63.69	0.84	1.99	1.56	0.50	3.47	1.49	2.86	489
0.18	0.26	0.34	0.29	0.21	0.47	0.13	0.38	37.02	66.56	53.85	14.68	118.43	51.88	79.90	0.90	2.54	2.08	0.67	4.41	1.87	3.82	734
0.32	0.34	0.42	0.40	0.32	0.53	0.11	0.51	38.50	72.77	56.84	14.11	131.42	58.66	86.62	1.07	2.77	2.41	0.75	4.79	2.02	4.10	2723


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/time_misc_auc.tex <==
name	auc
attack_time	0.15
l2	16.20
lom	0.62


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.28	0.50	0.00	0.56	0.28	0.50	0.57	0.61	0.57	0.43	0.78	0.17	0.71	0.69	0.77	0.77	0.65	0.88	0.12	0.85	556
0.11	0.00	0.19	0.00	-0.09	0.47	0.28	0.50	0.43	0.52	0.57	0.33	0.71	0.19	0.67	0.62	0.71	0.75	0.57	0.85	0.14	0.80	1021
0.15	0.00	0.09	0.00	-0.14	0.32	0.23	0.00	0.29	0.41	0.50	0.20	0.62	0.21	0.50	0.55	0.64	0.67	0.48	0.81	0.16	0.73	489
0.18	0.00	0.07	0.00	-0.14	0.29	0.21	0.00	0.25	0.36	0.33	0.17	0.55	0.19	0.50	0.50	0.60	0.62	0.46	0.75	0.15	0.69	734
0.32	0.00	0.03	0.00	-0.11	0.17	0.14	0.00	0.14	0.24	0.25	0.06	0.43	0.19	0.37	0.38	0.51	0.50	0.34	0.68	0.17	0.62	2723


==> data/mlm_plots/mlm_distil_fast/mr/lstmatt/s/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.10
top50	0.16


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	38.05	84.72	58.63	4.45	164.98	80.26	97.24	1.00	1.53	1.00	0.75	2.30	0.77	2.00	60.85	129.62	85.74	26.41	232.83	103.21	150.99	1.00	1.74	2.00	1.00	2.47	0.73	2.00	19
0.11	56.10	117.46	90.71	26.69	208.22	90.77	149.20	1.00	1.83	2.00	0.76	2.91	1.08	2.00	92.67	178.49	144.23	52.98	304.00	125.51	230.68	1.00	1.98	2.00	0.83	3.13	1.15	3.00	930
0.15	59.45	140.33	96.61	-15.97	296.63	156.30	168.91	1.00	1.77	1.00	0.66	2.88	1.11	2.00	115.13	243.80	176.12	-3.81	491.42	247.62	285.21	1.00	1.91	2.00	0.74	3.08	1.17	2.00	883
0.18	52.82	130.70	87.92	0.88	260.52	129.82	157.40	1.00	1.88	1.00	0.58	3.18	1.30	2.00	114.61	260.61	181.20	38.19	483.04	222.42	340.56	1.00	2.04	2.00	0.76	3.32	1.28	3.00	793
0.32	55.35	134.74	94.56	-10.48	279.96	145.22	165.48	1.00	1.73	1.00	0.53	2.92	1.20	2.00	177.97	377.58	277.13	50.91	704.25	326.67	473.40	1.00	2.01	2.00	0.65	3.38	1.36	3.00	2635


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/comparison_vals_auc.tex <==
name	auc
orig_pp	33.01
orig_ge	0.46
adv_pp	68.34
adv_ge	0.51


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.35	0.53	0.55	0.22	0.84	0.31	0.79	0.64	0.70	0.74	0.47	0.92	0.22	0.85	0.49	0.56	0.58	0.36	0.76	0.20	0.71	19
0.11	0.17	0.39	0.40	0.10	0.68	0.29	0.61	0.43	0.59	0.65	0.32	0.86	0.27	0.81	0.31	0.47	0.49	0.25	0.69	0.22	0.65	930
0.15	0.01	0.23	0.22	-0.07	0.52	0.29	0.43	0.22	0.42	0.46	0.10	0.75	0.32	0.69	0.16	0.33	0.34	0.08	0.58	0.25	0.53	883
0.18	-0.08	0.15	0.12	-0.16	0.46	0.31	0.35	0.13	0.34	0.36	0.00	0.68	0.34	0.62	0.09	0.26	0.27	-0.00	0.52	0.26	0.46	793
0.32	-0.33	-0.13	-0.15	-0.45	0.19	0.32	0.04	-0.31	-0.00	-0.01	-0.42	0.41	0.42	0.30	-0.22	0.00	0.00	-0.32	0.32	0.32	0.21	2635


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.09
kendall	0.07


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	0.78	1.93	1.89	0.61	3.25	1.32	2.90	0.72	2.56	2.52	0.53	4.59	2.03	3.98	1.23	9.39	4.95	-3.32	22.11	12.72	9.52	19
0.11	1.36	2.41	2.20	1.00	3.82	1.41	3.17	1.46	2.93	2.49	0.85	5.02	2.08	3.81	1.50	8.04	3.67	-1.94	18.02	9.98	10.50	930
0.15	1.58	2.43	2.29	1.26	3.60	1.17	3.05	1.79	3.03	2.63	1.23	4.82	1.79	3.82	1.68	7.13	3.61	-2.21	16.47	9.34	8.25	883
0.18	1.66	2.42	2.38	1.36	3.47	1.06	3.02	1.94	2.97	2.70	1.45	4.48	1.51	3.97	1.69	7.10	3.23	-3.69	17.88	10.78	6.45	793
0.32	1.90	2.42	2.37	1.59	3.24	0.83	2.89	2.06	2.85	2.65	1.64	4.07	1.22	3.49	1.54	3.86	2.41	-1.58	9.30	5.44	3.85	2635


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/ets_sts_auc.tex <==
name	auc
et_use	0.62
et_tse	0.76
et_ce	1.72


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.16	0.66	0.42	-0.24	1.57	0.91	0.77	1.11	4.39	2.53	-0.38	9.15	4.76	6.64	1.08	9.15	2.67	-9.37	27.68	18.52	7.05	19
0.11	0.27	1.32	0.51	-2.87	5.52	4.20	1.06	2.35	5.57	4.08	0.21	10.93	5.36	6.85	2.04	7.83	3.81	-7.08	22.75	14.91	8.77	930
0.15	0.25	2.12	0.48	-7.12	11.36	9.24	0.95	2.51	5.97	3.94	-2.09	14.03	8.06	6.40	2.09	7.17	3.38	-6.31	20.66	13.49	7.04	883
0.18	0.22	2.52	0.38	-14.21	19.24	16.72	0.81	2.75	5.57	4.09	-0.12	11.27	5.69	6.18	2.16	9.12	3.54	-15.73	33.97	24.85	7.44	793
0.32	0.14	1.18	0.27	-7.22	9.59	8.40	0.61	3.01	5.85	4.11	-2.08	13.77	7.92	5.96	2.28	8.29	3.27	-11.62	28.20	19.91	5.91	2635


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.45
et_p_h	1.46
et_p_l2	2.18


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.41	0.74	0.57	0.20	1.28	0.54	0.95	0.04	0.09	0.08	0.03	0.16	0.06	0.14	0.06	0.08	0.07	0.04	0.13	0.04	0.12	19
0.11	0.28	0.68	0.57	0.14	1.23	0.54	0.94	0.03	0.09	0.07	0.02	0.16	0.07	0.13	0.04	0.08	0.07	0.03	0.13	0.05	0.11	930
0.15	0.40	1.01	0.80	0.16	1.85	0.85	1.42	0.05	0.13	0.10	0.04	0.22	0.09	0.19	0.06	0.10	0.10	0.05	0.16	0.05	0.14	883
0.18	0.54	1.42	1.08	0.08	2.76	1.34	1.89	0.06	0.13	0.12	0.04	0.23	0.09	0.19	0.07	0.11	0.10	0.05	0.17	0.06	0.15	793
0.32	0.91	2.85	2.02	-0.15	5.84	2.99	3.67	0.09	0.18	0.17	0.07	0.28	0.11	0.25	0.10	0.14	0.14	0.08	0.20	0.06	0.18	2635


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.40
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.85	0.87	0.88	0.84	0.90	0.03	0.89	0.86	0.89	0.89	0.84	0.93	0.05	0.92	0.88	0.92	0.96	0.84	1.00	0.08	0.98	19
0.11	0.84	0.86	0.86	0.82	0.90	0.04	0.89	0.84	0.87	0.88	0.82	0.93	0.05	0.91	0.83	0.88	0.92	0.77	1.00	0.12	0.98	930
0.15	0.80	0.83	0.83	0.79	0.87	0.04	0.86	0.81	0.85	0.86	0.79	0.91	0.06	0.90	0.80	0.86	0.89	0.74	0.98	0.12	0.95	883
0.18	0.79	0.81	0.82	0.77	0.86	0.04	0.84	0.80	0.84	0.84	0.78	0.90	0.06	0.88	0.77	0.84	0.88	0.72	0.97	0.13	0.94	793
0.32	0.72	0.76	0.75	0.70	0.81	0.05	0.79	0.73	0.78	0.78	0.72	0.85	0.07	0.83	0.66	0.74	0.77	0.59	0.89	0.15	0.86	2635


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.22
sts_ce	0.22


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	1.62	1.75	1.72	1.56	1.95	0.19	1.88	0.14	0.22	0.18	0.10	0.35	0.12	0.28	0.83	3.08	2.07	0.18	5.98	2.90	4.40	19
0.11	1.51	1.69	1.64	1.39	1.99	0.30	1.78	0.12	0.20	0.18	0.10	0.30	0.10	0.25	0.89	2.50	1.89	0.34	4.67	2.17	3.49	930
0.15	1.49	1.97	2.04	1.24	2.71	0.74	2.33	0.13	0.20	0.18	0.10	0.29	0.10	0.25	0.72	2.37	1.69	0.14	4.61	2.24	3.24	883
0.18	1.34	2.08	1.94	0.92	3.24	1.16	2.63	0.14	0.20	0.18	0.11	0.29	0.09	0.25	0.81	2.41	1.73	0.24	4.57	2.17	3.27	793
0.32	0.72	1.42	0.97	0.38	2.47	1.04	1.78	0.17	0.24	0.22	0.15	0.34	0.10	0.29	0.96	2.68	1.97	0.35	5.01	2.33	3.78	2635


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/time_misc_auc.tex <==
name	auc
attack_time	0.47
l2	0.06
lom	0.66


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.25	0.45	0.50	0.12	0.78	0.33	0.50	0.57	0.65	0.71	0.47	0.82	0.17	0.79	0.72	0.76	0.75	0.63	0.90	0.13	0.83	19
0.11	0.00	0.20	0.00	-0.12	0.51	0.31	0.50	0.40	0.53	0.50	0.31	0.76	0.22	0.67	0.62	0.73	0.75	0.58	0.87	0.15	0.82	930
0.15	0.00	0.12	0.00	-0.15	0.40	0.28	0.00	0.25	0.42	0.40	0.18	0.66	0.24	0.60	0.56	0.66	0.67	0.49	0.83	0.17	0.80	883
0.18	0.00	0.06	0.00	-0.15	0.27	0.21	0.00	0.25	0.40	0.33	0.16	0.63	0.23	0.50	0.50	0.61	0.60	0.43	0.79	0.18	0.73	793
0.32	0.00	0.03	0.00	-0.12	0.17	0.14	0.00	0.00	0.22	0.17	-0.01	0.45	0.23	0.33	0.33	0.48	0.50	0.28	0.68	0.20	0.60	2635


==> data/mlm_plots/mlm_distil_fast/mr/roberta/a/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.10
top50	0.16


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	48.03	103.01	96.33	23.23	182.80	79.78	123.93	1.00	1.42	1.00	0.91	1.93	0.51	2.00	73.51	128.17	99.34	49.03	207.31	79.14	149.48	1.00	1.47	1.00	0.96	1.99	0.51	2.00	19
0.11	55.94	116.43	90.55	28.75	204.11	87.68	149.17	1.00	1.84	2.00	0.76	2.91	1.07	2.00	89.80	179.89	139.81	39.30	320.49	140.59	231.52	1.00	1.92	2.00	0.80	3.04	1.12	2.00	939
0.15	59.73	139.49	96.12	-15.16	294.14	154.65	169.47	1.00	1.75	1.00	0.66	2.85	1.10	2.00	111.68	251.79	173.67	-49.82	553.39	301.60	297.76	1.00	1.86	2.00	0.73	2.98	1.13	2.00	917
0.18	52.22	131.36	89.19	1.59	261.13	129.77	162.33	1.00	1.89	2.00	0.58	3.19	1.31	2.00	112.57	250.67	183.91	29.47	471.88	221.20	315.62	1.00	2.00	2.00	0.66	3.33	1.33	2.00	795
0.32	55.37	133.64	94.56	-8.30	275.58	141.94	165.48	1.00	1.72	1.00	0.55	2.90	1.18	2.00	171.30	383.52	278.56	12.62	754.42	370.90	476.76	1.00	1.92	2.00	0.65	3.19	1.27	2.00	2634


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	33.32
orig_ge	0.46
adv_pp	68.25
adv_ge	0.49


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	-0.12	-0.00	0.07	-0.46	0.45	0.46	0.22	0.03	0.20	0.22	0.00	0.39	0.20	0.35	0.03	0.15	0.17	0.00	0.30	0.15	0.26	19
0.11	-0.30	-0.06	-0.06	-0.41	0.29	0.35	0.17	-0.11	0.09	0.09	-0.21	0.39	0.30	0.30	-0.07	0.07	0.07	-0.15	0.30	0.23	0.23	939
0.15	-0.45	-0.22	-0.24	-0.55	0.11	0.33	0.01	-0.29	-0.09	-0.09	-0.40	0.22	0.31	0.12	-0.21	-0.06	-0.06	-0.30	0.18	0.24	0.10	917
0.18	-0.56	-0.32	-0.33	-0.64	-0.01	0.32	-0.12	-0.38	-0.17	-0.19	-0.47	0.14	0.31	0.04	-0.28	-0.12	-0.13	-0.35	0.12	0.23	0.03	795
0.32	-0.74	-0.55	-0.59	-0.82	-0.28	0.27	-0.40	-0.62	-0.41	-0.43	-0.70	-0.12	0.29	-0.24	-0.47	-0.31	-0.32	-0.55	-0.07	0.24	-0.17	2634


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/correlations_auc.tex <==
name	auc
pcc	-0.08
spearman	-0.04
kendall	-0.03


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	2.56	4.74	2.79	0.47	9.01	4.27	4.32	2.02	4.67	3.31	1.10	8.24	3.57	6.20	2.75	11.15	6.32	-0.12	22.41	11.26	14.68	19
0.11	2.87	4.23	3.92	2.19	6.26	2.03	5.22	2.96	5.09	4.23	1.90	8.29	3.19	6.35	2.90	13.54	6.66	-1.84	28.93	15.38	19.19	939
0.15	2.90	4.05	3.77	2.29	5.80	1.76	4.83	3.04	5.21	4.47	1.94	8.47	3.26	6.28	3.00	12.73	5.89	-2.99	28.45	15.72	15.60	917
0.18	2.80	3.74	3.50	2.34	5.14	1.40	4.52	3.02	4.58	4.01	2.10	7.06	2.48	5.50	2.74	9.69	4.44	-2.75	22.12	12.43	10.24	795
0.32	2.78	3.45	3.29	2.40	4.49	1.04	3.92	3.04	4.08	3.80	2.48	5.69	1.61	4.70	2.48	6.19	3.66	-2.06	14.45	8.26	6.26	2634


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/ets_sts_auc.tex <==
name	auc
et_use	1.01
et_tse	1.21
et_ce	2.61


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.60	2.59	1.42	-2.60	7.77	5.18	1.71	3.44	13.42	4.43	-19.12	45.96	32.54	8.17	2.74	10.50	3.76	-10.80	31.81	21.31	6.90	19
0.11	0.50	3.66	0.94	-8.18	15.50	11.84	2.14	4.33	10.01	6.77	-0.38	20.41	10.40	11.68	3.40	15.18	6.37	-20.22	50.59	35.40	13.85	939
0.15	0.43	2.43	0.73	-7.26	12.12	9.69	1.42	4.37	9.54	6.46	-1.86	20.93	11.39	10.14	3.29	15.88	5.43	-34.68	66.45	50.57	11.74	917
0.18	0.34	2.57	0.62	-7.10	12.25	9.67	1.45	4.28	8.25	6.49	1.79	14.70	6.45	9.37	3.22	12.63	5.20	-16.60	41.87	29.23	10.90	795
0.32	0.20	1.40	0.43	-3.75	6.54	5.15	0.91	4.23	8.37	5.74	-1.71	18.45	10.08	8.70	3.17	12.45	4.62	-20.77	45.66	33.22	10.10	2634


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.63
et_p_h	2.40
et_p_l2	3.47


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.33	0.51	0.54	0.18	0.83	0.32	0.57	0.06	0.12	0.12	0.05	0.20	0.07	0.17	0.06	0.10	0.10	0.05	0.15	0.05	0.14	19
0.11	0.25	0.69	0.53	0.06	1.33	0.63	0.95	0.04	0.10	0.08	0.03	0.17	0.07	0.15	0.04	0.08	0.07	0.04	0.13	0.05	0.11	939
0.15	0.43	1.04	0.82	0.02	2.06	1.02	1.35	0.05	0.12	0.11	0.04	0.21	0.09	0.19	0.06	0.10	0.09	0.05	0.15	0.05	0.14	917
0.18	0.46	1.33	1.06	0.06	2.60	1.27	1.83	0.06	0.14	0.13	0.05	0.23	0.09	0.20	0.07	0.11	0.11	0.06	0.16	0.05	0.15	795
0.32	0.84	2.77	1.81	-0.26	5.81	3.04	3.56	0.07	0.17	0.17	0.06	0.28	0.11	0.25	0.09	0.14	0.13	0.07	0.20	0.07	0.18	2634


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.38
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.85	0.86	0.86	0.82	0.91	0.05	0.89	0.82	0.86	0.88	0.79	0.93	0.07	0.92	0.87	0.89	0.94	0.78	0.99	0.11	0.96	19
0.11	0.84	0.86	0.86	0.82	0.90	0.04	0.89	0.84	0.87	0.88	0.82	0.93	0.05	0.91	0.83	0.88	0.92	0.76	1.00	0.12	0.98	939
0.15	0.81	0.84	0.84	0.79	0.88	0.04	0.86	0.82	0.86	0.86	0.79	0.92	0.06	0.90	0.80	0.86	0.90	0.74	0.99	0.12	0.96	917
0.18	0.78	0.81	0.81	0.76	0.86	0.05	0.84	0.79	0.83	0.84	0.77	0.89	0.06	0.88	0.76	0.84	0.87	0.71	0.97	0.13	0.93	795
0.32	0.73	0.76	0.76	0.71	0.82	0.05	0.80	0.75	0.79	0.79	0.72	0.86	0.07	0.84	0.69	0.77	0.79	0.62	0.91	0.15	0.88	2634


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.22
sts_ce	0.22


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	2.08	3.35	2.65	0.31	6.38	3.04	3.05	4.06	11.90	8.32	1.09	22.72	10.81	15.88	5.18	9.54	6.79	2.29	16.79	7.25	12.60	19
0.11	2.27	2.77	2.48	1.17	4.36	1.59	2.69	2.13	7.80	4.17	-2.16	17.76	9.96	9.75	2.08	5.47	4.56	1.24	9.71	4.24	7.94	939
0.15	2.18	3.11	2.93	1.31	4.91	1.80	3.54	2.71	10.91	5.37	-12.60	34.42	23.51	11.29	2.31	5.50	4.65	1.39	9.62	4.11	7.94	917
0.18	1.63	2.96	2.84	1.15	4.76	1.80	3.85	2.99	11.13	6.58	-14.03	36.29	25.16	12.02	2.48	5.85	4.89	1.46	10.24	4.39	8.01	795
0.32	1.20	2.14	1.88	0.84	3.44	1.30	2.62	4.11	11.66	7.43	-8.51	31.83	20.17	12.90	2.20	5.65	4.75	1.35	9.96	4.30	8.28	2634


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/time_misc_auc.tex <==
name	auc
attack_time	0.72
l2	2.79
lom	1.56


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.21	0.00	-0.04	0.46	0.25	0.50	0.29	0.38	0.40	0.23	0.53	0.15	0.43	0.50	0.55	0.58	0.42	0.68	0.13	0.64	19
0.11	0.00	0.12	0.00	-0.14	0.38	0.26	0.00	0.20	0.36	0.33	0.16	0.55	0.20	0.50	0.44	0.55	0.56	0.40	0.69	0.14	0.64	939
0.15	0.00	0.06	0.00	-0.14	0.27	0.20	0.00	0.17	0.28	0.25	0.07	0.48	0.21	0.40	0.40	0.48	0.50	0.33	0.63	0.15	0.57	917
0.18	0.00	0.05	0.00	-0.14	0.23	0.18	0.00	0.00	0.22	0.20	0.03	0.41	0.19	0.33	0.36	0.44	0.43	0.29	0.59	0.15	0.55	795
0.32	0.00	0.01	0.00	-0.09	0.11	0.10	0.00	0.00	0.13	0.00	-0.04	0.29	0.16	0.20	0.27	0.36	0.36	0.20	0.51	0.16	0.45	2634


==> data/mlm_plots/mlm_distil_fast/mr/roberta/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.06
top50	0.12


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	38.04	82.55	52.79	-0.37	165.48	82.93	93.29	1.00	1.50	1.00	0.71	2.29	0.79	2.00	67.00	167.91	96.66	-27.83	363.65	195.74	161.71	1.00	1.83	1.50	0.79	2.88	1.04	2.00	18
0.11	55.74	116.08	88.87	27.04	205.12	89.04	147.32	1.00	1.83	2.00	0.75	2.91	1.08	2.00	112.12	210.39	168.06	58.70	362.09	151.69	263.35	1.00	2.00	2.00	0.84	3.16	1.16	3.00	891
0.15	58.64	135.36	95.48	0.66	270.05	134.69	168.21	1.00	1.79	2.00	0.70	2.88	1.09	2.00	149.24	298.89	229.13	58.38	539.40	240.51	367.17	1.00	1.98	2.00	0.87	3.10	1.12	3.00	855
0.18	52.82	130.04	86.26	0.45	259.62	129.58	157.49	1.00	1.86	1.00	0.59	3.14	1.27	2.00	155.43	348.46	260.60	60.60	636.33	287.86	420.69	1.00	2.10	2.00	0.77	3.42	1.32	3.00	784
0.32	55.35	133.99	93.60	-11.24	279.22	145.23	163.43	1.00	1.74	1.00	0.53	2.94	1.20	2.00	259.73	600.80	450.98	51.67	1149.93	549.13	749.32	1.00	2.07	2.00	0.81	3.33	1.26	3.00	2601


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/comparison_vals_auc.tex <==
name	auc
orig_pp	32.59
orig_ge	0.46
adv_pp	95.37
adv_ge	0.53


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.16	0.38	0.48	0.14	0.63	0.24	0.57	0.44	0.55	0.57	0.32	0.78	0.23	0.71	0.36	0.43	0.45	0.24	0.62	0.19	0.55	18
0.11	0.15	0.37	0.38	0.06	0.68	0.31	0.61	0.27	0.45	0.51	0.16	0.75	0.30	0.68	0.20	0.35	0.38	0.12	0.58	0.23	0.52	891
0.15	-0.05	0.18	0.18	-0.13	0.49	0.31	0.40	0.07	0.29	0.31	-0.02	0.60	0.31	0.53	0.05	0.22	0.23	-0.01	0.45	0.23	0.39	855
0.18	-0.13	0.07	0.06	-0.24	0.39	0.32	0.29	-0.08	0.17	0.22	-0.19	0.53	0.36	0.44	-0.04	0.14	0.16	-0.13	0.40	0.26	0.31	784
0.32	-0.37	-0.18	-0.21	-0.48	0.13	0.30	-0.00	-0.38	-0.11	-0.13	-0.48	0.25	0.36	0.14	-0.26	-0.08	-0.09	-0.35	0.19	0.27	0.10	2601


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/correlations_auc.tex <==
name	auc
pcc	0.03
spearman	0.05
kendall	0.04


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	1.35	2.63	2.42	1.02	4.25	1.62	3.31	1.47	2.86	2.61	1.10	4.63	1.77	3.85	2.77	12.37	6.85	-0.95	25.68	13.31	20.42	18
0.11	1.42	2.68	2.39	0.93	4.43	1.75	3.54	1.69	3.41	2.77	0.86	5.96	2.55	4.53	1.91	9.10	4.61	-1.36	19.55	10.46	12.20	891
0.15	1.90	2.85	2.69	1.38	4.32	1.47	3.59	2.13	3.60	3.03	1.28	5.91	2.32	4.52	2.31	9.00	4.85	-1.21	19.21	10.21	12.18	855
0.18	1.95	2.88	2.67	1.45	4.31	1.43	3.47	2.17	3.70	3.19	1.42	5.98	2.28	4.62	2.08	8.71	4.12	-3.24	20.66	11.95	9.77	784
0.32	2.14	2.77	2.66	1.68	3.85	1.08	3.19	2.41	3.40	3.07	1.80	5.01	1.60	4.02	1.94	5.62	2.89	-2.40	13.64	8.02	5.40	2601


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/ets_sts_auc.tex <==
name	auc
et_use	0.73
et_tse	0.91
et_ce	2.17


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.21	0.62	0.29	-0.26	1.49	0.88	0.69	1.65	3.23	2.81	1.19	5.27	2.04	4.04	1.37	3.31	2.21	-0.07	6.69	3.38	3.32	18
0.11	0.19	1.02	0.35	-3.91	5.95	4.93	0.61	1.91	4.70	3.26	-0.44	9.85	5.15	5.47	1.66	7.00	3.13	-9.56	23.57	16.56	6.68	891
0.15	0.17	0.69	0.28	-2.58	3.95	3.26	0.52	2.35	5.75	3.63	-2.81	14.31	8.56	5.99	1.89	7.51	3.17	-9.21	24.24	16.72	6.78	855
0.18	0.14	0.50	0.24	-1.66	2.66	2.16	0.39	2.56	4.99	3.61	0.58	9.40	4.41	6.20	1.98	7.30	3.19	-5.68	20.28	12.98	7.48	784
0.32	0.08	0.36	0.16	-0.79	1.51	1.15	0.30	2.99	5.62	4.04	-0.94	12.18	6.56	6.00	2.30	8.50	3.43	-16.60	33.60	25.10	7.42	2601


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.15
et_p_h	1.32
et_p_l2	1.88


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.45	1.01	1.18	0.39	1.62	0.62	1.42	0.08	0.14	0.14	0.08	0.19	0.06	0.18	0.08	0.11	0.12	0.07	0.15	0.04	0.13	18
0.11	0.47	1.02	0.86	0.25	1.80	0.78	1.38	0.05	0.11	0.09	0.03	0.19	0.08	0.17	0.06	0.10	0.09	0.05	0.15	0.05	0.14	891
0.15	0.76	1.68	1.33	0.36	3.00	1.32	2.29	0.06	0.14	0.12	0.05	0.22	0.09	0.21	0.07	0.11	0.11	0.06	0.17	0.06	0.15	855
0.18	1.09	2.32	1.82	0.44	4.20	1.88	2.85	0.06	0.15	0.14	0.05	0.25	0.10	0.23	0.07	0.13	0.12	0.07	0.19	0.06	0.18	784
0.32	1.81	5.19	3.48	-0.11	10.49	5.30	6.80	0.08	0.17	0.17	0.07	0.28	0.11	0.25	0.10	0.15	0.14	0.08	0.21	0.07	0.20	2601


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.68
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.85	0.87	0.87	0.82	0.91	0.04	0.89	0.87	0.87	0.89	0.81	0.93	0.06	0.91	0.90	0.91	0.95	0.78	1.03	0.12	0.99	18
0.11	0.85	0.87	0.87	0.83	0.91	0.04	0.89	0.86	0.89	0.89	0.84	0.94	0.05	0.92	0.86	0.90	0.94	0.80	1.00	0.10	0.98	891
0.15	0.82	0.84	0.84	0.80	0.89	0.04	0.87	0.84	0.87	0.87	0.82	0.92	0.05	0.90	0.83	0.89	0.91	0.78	0.99	0.11	0.97	855
0.18	0.80	0.83	0.83	0.78	0.87	0.04	0.85	0.82	0.85	0.86	0.79	0.91	0.06	0.89	0.80	0.86	0.89	0.75	0.97	0.11	0.96	784
0.32	0.74	0.78	0.78	0.72	0.83	0.05	0.81	0.77	0.81	0.81	0.75	0.87	0.06	0.85	0.70	0.79	0.80	0.66	0.92	0.13	0.89	2601


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.22
sts_ce	0.22


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	2.71	2.83	2.90	2.34	3.32	0.49	3.09	13.53	104.31	42.30	-132.05	340.66	236.35	82.14	0.86	1.57	1.56	0.65	2.49	0.92	2.16	18
0.11	1.86	2.31	2.26	1.76	2.86	0.55	2.67	8.74	88.45	25.37	-124.62	301.52	213.07	83.68	0.61	1.37	1.15	0.35	2.39	1.02	1.91	891
0.15	1.85	2.44	2.48	1.58	3.29	0.86	2.87	11.19	108.58	31.06	-121.68	338.83	230.25	114.57	0.49	1.39	1.14	0.28	2.49	1.11	2.01	855
0.18	1.90	2.82	2.82	1.35	4.30	1.47	3.74	15.55	119.59	39.57	-91.92	331.11	211.51	136.22	0.51	1.44	1.06	0.18	2.71	1.26	1.98	784
0.32	0.89	1.88	1.26	0.40	3.37	1.48	2.40	18.53	173.82	63.24	-254.47	602.12	428.30	191.46	0.61	1.64	1.29	0.26	3.01	1.38	2.31	2601


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/time_misc_auc.tex <==
name	auc
attack_time	0.63
l2	32.57
lom	0.39


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.36	0.50	0.07	0.65	0.29	0.50	0.43	0.53	0.57	0.37	0.69	0.16	0.71	0.60	0.70	0.75	0.59	0.81	0.11	0.76	18
0.11	0.00	0.23	0.00	-0.12	0.58	0.35	0.50	0.33	0.50	0.50	0.28	0.71	0.21	0.67	0.56	0.67	0.67	0.52	0.81	0.15	0.78	891
0.15	0.00	0.11	0.00	-0.16	0.37	0.26	0.00	0.20	0.38	0.33	0.15	0.61	0.23	0.50	0.50	0.61	0.60	0.46	0.76	0.15	0.71	855
0.18	0.00	0.07	0.00	-0.16	0.30	0.23	0.00	0.17	0.33	0.33	0.10	0.56	0.23	0.50	0.43	0.55	0.60	0.38	0.72	0.17	0.64	784
0.32	0.00	0.03	0.00	-0.13	0.18	0.16	0.00	0.00	0.19	0.17	-0.02	0.39	0.20	0.33	0.33	0.45	0.44	0.27	0.62	0.17	0.57	2601


==> data/mlm_plots/mlm_distil_fast/mr/roberta/s/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.09
top50	0.15


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	34.47	121.00	113.60	24.20	217.81	96.80	221.75	1.00	1.38	1.00	0.86	1.89	0.52	2.00	54.43	134.72	120.85	36.98	232.46	97.74	238.12	1.00	1.38	1.00	0.86	1.89	0.52	2.00	8
0.11	53.45	120.02	87.23	8.35	231.69	111.67	145.14	1.00	1.57	1.00	0.75	2.40	0.82	2.00	81.12	177.31	130.04	19.44	335.18	157.87	214.91	1.00	1.65	1.00	0.77	2.54	0.89	2.00	770
0.15	57.56	142.47	97.07	-15.56	300.50	158.03	172.82	1.00	1.67	1.00	0.76	2.58	0.91	2.00	98.75	217.72	152.11	19.37	416.07	198.35	265.70	1.00	1.71	1.00	0.76	2.65	0.94	2.00	921
0.18	58.49	135.11	98.43	5.05	265.16	130.06	165.04	1.00	1.69	1.00	0.67	2.71	1.02	2.00	110.30	240.23	183.12	51.77	428.69	188.46	311.78	1.00	1.77	1.00	0.74	2.79	1.02	2.00	771
0.32	55.55	143.07	102.13	-6.55	292.69	149.62	174.18	1.00	1.63	1.00	0.67	2.58	0.96	2.00	157.08	360.19	264.10	37.20	683.17	322.99	450.09	1.00	1.74	1.00	0.77	2.72	0.97	2.00	2593


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/comparison_vals_auc.tex <==
name	auc
orig_pp	34.96
orig_ge	0.42
adv_pp	64.45
adv_ge	0.44


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.46	0.66	0.71	0.34	0.98	0.32	0.97	0.78	0.83	0.86	0.75	0.91	0.08	0.89	0.62	0.68	0.72	0.58	0.78	0.10	0.75	8
0.11	0.15	0.36	0.38	0.06	0.67	0.30	0.59	0.37	0.54	0.61	0.23	0.85	0.31	0.78	0.27	0.42	0.45	0.17	0.67	0.25	0.61	770
0.15	-0.04	0.21	0.20	-0.12	0.55	0.34	0.47	0.12	0.39	0.46	0.01	0.76	0.38	0.70	0.09	0.30	0.33	0.01	0.59	0.29	0.54	921
0.18	-0.14	0.11	0.08	-0.22	0.44	0.33	0.33	0.03	0.30	0.35	-0.08	0.68	0.38	0.62	0.02	0.24	0.25	-0.06	0.53	0.29	0.47	771
0.32	-0.37	-0.10	-0.16	-0.47	0.26	0.37	0.12	-0.34	-0.00	-0.04	-0.44	0.43	0.44	0.33	-0.23	0.01	-0.03	-0.32	0.33	0.33	0.24	2593


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.08
kendall	0.07


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	0.26	1.34	0.97	0.06	2.63	1.28	1.88	0.26	1.66	0.93	-0.37	3.69	2.03	1.91	0.16	6.13	1.75	-5.32	17.59	11.45	5.18	8
0.11	1.34	2.31	2.08	0.91	3.70	1.40	3.00	1.37	2.63	2.18	0.71	4.56	1.93	3.40	1.34	7.49	3.22	-2.52	17.50	10.01	9.00	770
0.15	1.52	2.41	2.26	1.14	3.68	1.27	3.09	1.56	2.72	2.43	1.04	4.39	1.68	3.50	1.63	6.23	3.12	-1.87	14.34	8.11	7.03	921
0.18	1.60	2.40	2.33	1.24	3.56	1.16	3.00	1.62	2.68	2.35	1.15	4.21	1.53	3.39	1.49	5.79	2.65	-3.42	15.01	9.22	5.87	771
0.32	1.78	2.32	2.28	1.37	3.26	0.94	2.80	1.84	2.56	2.41	1.35	3.77	1.21	3.12	1.49	3.58	2.26	-1.08	8.24	4.66	3.70	2593


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/ets_sts_auc.tex <==
name	auc
et_use	0.59
et_tse	0.67
et_ce	1.46


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.18	1.59	0.35	-1.80	4.98	3.39	0.62	0.58	3.14	1.55	-0.94	7.22	4.08	3.50	1.51	4.57	1.59	-3.15	12.29	7.72	2.74	8
0.11	0.28	2.48	0.61	-8.29	13.24	10.77	1.52	2.36	6.30	4.23	-0.68	13.29	6.99	7.92	2.01	8.14	4.16	-7.91	24.18	16.04	9.12	770
0.15	0.26	2.79	0.57	-9.29	14.87	12.08	1.57	2.58	6.27	4.47	0.21	12.34	6.07	7.61	2.10	8.77	4.24	-6.63	24.18	15.40	9.29	921
0.18	0.25	2.43	0.52	-9.35	14.22	11.78	1.18	3.02	6.81	4.73	0.00	13.61	6.80	7.77	2.37	9.10	3.98	-5.21	23.41	14.31	9.36	771
0.32	0.16	1.60	0.33	-6.96	10.16	8.56	0.78	2.93	5.77	4.14	-0.23	11.76	6.00	6.69	2.28	8.30	3.56	-11.34	27.94	19.64	7.48	2593


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.57
et_p_h	1.57
et_p_l2	2.15


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.07	0.29	0.11	-0.02	0.60	0.31	0.53	0.01	0.06	0.05	0.00	0.11	0.06	0.10	0.02	0.06	0.04	0.02	0.10	0.04	0.09	8
0.11	0.21	0.65	0.47	0.05	1.24	0.60	0.88	0.04	0.09	0.07	0.02	0.16	0.07	0.13	0.04	0.08	0.07	0.03	0.12	0.05	0.11	770
0.15	0.25	0.89	0.63	-0.04	1.81	0.92	1.22	0.04	0.11	0.09	0.03	0.20	0.08	0.17	0.05	0.09	0.09	0.04	0.15	0.05	0.13	921
0.18	0.37	1.23	0.84	-0.26	2.72	1.49	1.53	0.04	0.12	0.09	0.03	0.21	0.09	0.18	0.06	0.10	0.09	0.04	0.15	0.06	0.13	771
0.32	0.65	2.55	1.53	-0.76	5.87	3.32	3.12	0.07	0.16	0.16	0.05	0.28	0.11	0.25	0.08	0.14	0.13	0.07	0.20	0.07	0.18	2593


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.35
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.86	0.89	0.89	0.83	0.95	0.06	0.95	0.85	0.88	0.92	0.80	0.97	0.09	0.95	0.92	0.92	0.92	0.86	0.98	0.06	0.95	8
0.11	0.82	0.85	0.85	0.81	0.89	0.04	0.88	0.82	0.85	0.86	0.79	0.92	0.06	0.90	0.81	0.87	0.91	0.74	1.00	0.13	0.97	770
0.15	0.80	0.83	0.83	0.78	0.87	0.04	0.85	0.79	0.83	0.84	0.77	0.90	0.06	0.88	0.79	0.85	0.88	0.72	0.97	0.13	0.95	921
0.18	0.78	0.80	0.80	0.76	0.85	0.04	0.84	0.76	0.81	0.82	0.75	0.88	0.06	0.86	0.75	0.82	0.83	0.69	0.94	0.13	0.92	771
0.32	0.72	0.75	0.75	0.70	0.80	0.05	0.79	0.72	0.77	0.77	0.70	0.83	0.07	0.81	0.65	0.74	0.76	0.60	0.88	0.14	0.84	2593


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.21


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	2.13	3.37	2.72	1.91	4.83	1.46	4.76	0.03	0.18	0.17	0.02	0.33	0.15	0.26	0.29	4.95	2.89	-0.68	10.59	5.63	7.88	8
0.11	1.93	2.31	2.28	1.65	2.96	0.66	2.43	0.16	0.24	0.22	0.13	0.35	0.11	0.30	1.26	2.90	2.39	0.71	5.08	2.18	4.08	770
0.15	2.08	2.65	2.33	1.57	3.73	1.08	3.26	0.16	0.24	0.21	0.12	0.35	0.12	0.29	1.05	2.79	2.25	0.59	4.99	2.20	4.03	921
0.18	2.11	2.95	2.97	1.76	4.13	1.18	3.74	0.17	0.25	0.23	0.13	0.37	0.12	0.30	1.16	2.88	2.29	0.56	5.20	2.32	4.06	771
0.32	1.27	2.45	1.90	0.89	4.01	1.56	3.17	0.15	0.22	0.21	0.12	0.33	0.10	0.27	1.07	3.02	2.42	0.58	5.46	2.44	4.42	2593


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/time_misc_auc.tex <==
name	auc
attack_time	0.70
l2	0.06
lom	0.80


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.50	0.69	0.75	0.32	1.06	0.37	1.00	0.68	0.71	0.75	0.57	0.85	0.14	0.78	0.75	0.82	0.86	0.73	0.91	0.09	0.88	8
0.11	0.00	0.20	0.00	-0.15	0.56	0.36	0.50	0.40	0.53	0.50	0.29	0.76	0.24	0.67	0.60	0.69	0.70	0.53	0.86	0.17	0.80	770
0.15	0.00	0.14	0.00	-0.18	0.47	0.33	0.00	0.25	0.42	0.40	0.15	0.68	0.26	0.67	0.50	0.64	0.67	0.45	0.82	0.19	0.78	921
0.18	0.00	0.08	0.00	-0.17	0.33	0.25	0.00	0.20	0.37	0.33	0.12	0.62	0.25	0.50	0.43	0.59	0.60	0.41	0.78	0.19	0.75	771
0.32	0.00	0.06	0.00	-0.17	0.30	0.23	0.00	0.00	0.23	0.20	-0.02	0.48	0.25	0.33	0.33	0.48	0.50	0.27	0.69	0.21	0.62	2593


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/a/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.10
top50	0.16


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	34.47	80.06	86.96	16.48	143.64	63.58	86.96	1.00	1.00	1.00	1.00	1.00	0.00	1.00	57.32	161.96	200.65	53.34	270.59	108.62	217.17	1.00	1.25	1.00	0.79	1.71	0.46	1.25	8
0.11	53.62	117.78	88.87	11.10	224.47	106.69	141.61	1.00	1.59	1.00	0.78	2.41	0.82	2.00	82.96	170.14	127.03	24.92	315.36	145.22	211.41	1.00	1.65	1.00	0.77	2.52	0.87	2.00	765
0.15	56.18	146.76	96.95	-20.63	314.14	167.38	175.56	1.00	1.69	1.00	0.75	2.62	0.93	2.00	97.78	221.09	157.48	16.60	425.57	204.48	271.29	1.00	1.76	1.00	0.75	2.77	1.01	2.00	914
0.18	58.49	134.20	96.93	5.15	263.26	129.05	164.46	1.00	1.65	1.00	0.67	2.63	0.98	2.00	111.90	252.80	195.93	43.13	462.46	209.67	321.92	1.00	1.70	1.00	0.72	2.69	0.99	2.00	790
0.32	54.96	143.13	101.16	-10.23	296.49	153.36	175.03	1.00	1.60	1.00	0.66	2.54	0.94	2.00	153.96	349.24	254.31	1.48	697.00	347.76	427.28	1.00	1.74	1.00	0.70	2.77	1.03	2.00	2580


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	34.04
orig_ge	0.41
adv_pp	65.21
adv_ge	0.43


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	-0.02	0.30	0.51	-0.31	0.90	0.61	0.77	0.21	0.33	0.49	-0.24	0.90	0.57	0.71	0.21	0.23	0.34	-0.22	0.68	0.45	0.49	8
0.11	-0.34	-0.11	-0.13	-0.44	0.22	0.33	0.10	-0.25	-0.03	-0.03	-0.34	0.29	0.31	0.19	-0.18	-0.02	-0.01	-0.25	0.22	0.24	0.14	765
0.15	-0.48	-0.24	-0.27	-0.57	0.09	0.33	-0.04	-0.37	-0.15	-0.15	-0.47	0.17	0.32	0.06	-0.27	-0.11	-0.11	-0.35	0.14	0.24	0.05	914
0.18	-0.51	-0.28	-0.32	-0.59	0.04	0.32	-0.10	-0.41	-0.19	-0.23	-0.51	0.12	0.31	0.00	-0.31	-0.14	-0.16	-0.37	0.09	0.23	0.01	790
0.32	-0.68	-0.44	-0.50	-0.76	-0.12	0.32	-0.29	-0.58	-0.36	-0.40	-0.67	-0.04	0.32	-0.19	-0.43	-0.26	-0.29	-0.52	-0.01	0.25	-0.13	2580


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/correlations_auc.tex <==
name	auc
pcc	-0.06
spearman	-0.04
kendall	-0.03


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	1.03	4.28	2.55	-1.49	10.05	5.77	3.59	1.58	5.55	2.83	-1.23	12.32	6.77	5.66	3.67	5.67	5.05	3.09	8.25	2.58	7.15	8
0.11	2.74	3.86	3.57	2.06	5.66	1.80	4.69	2.65	4.41	3.81	1.45	7.37	2.96	5.45	2.50	11.78	5.21	-2.84	26.40	14.62	14.46	765
0.15	2.72	3.66	3.44	2.13	5.19	1.53	4.36	2.73	4.18	3.80	2.01	6.35	2.17	5.01	2.57	9.56	4.39	-2.89	22.01	12.45	10.43	914
0.18	2.52	3.32	3.21	2.11	4.53	1.21	3.97	2.59	3.78	3.40	2.03	5.53	1.75	4.61	2.28	7.97	3.67	-2.94	18.87	10.91	8.12	790
0.32	2.45	3.01	2.94	1.99	4.03	1.02	3.43	2.51	3.46	3.17	1.88	5.03	1.57	4.07	2.06	5.03	3.07	-1.86	11.93	6.90	4.80	2580


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/ets_sts_auc.tex <==
name	auc
et_use	0.90
et_tse	1.05
et_ce	2.06


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.09	0.57	0.17	-0.11	1.25	0.68	0.93	4.94	7.11	5.84	1.36	12.86	5.75	6.70	5.65	8.75	6.16	0.92	16.57	7.82	9.97	8
0.11	0.59	3.86	1.22	-11.04	18.75	14.90	2.73	4.73	10.72	7.78	1.08	20.37	9.64	13.50	3.82	14.35	7.56	-11.98	40.68	26.33	16.04	765
0.15	0.51	3.27	0.96	-6.78	13.31	10.04	2.24	4.68	10.86	7.16	0.10	21.61	10.75	13.13	3.21	16.88	6.53	-22.57	56.33	39.45	14.70	914
0.18	0.35	2.69	0.73	-10.49	15.88	13.18	1.54	4.31	9.94	6.70	-1.79	21.68	11.74	10.98	3.24	15.02	6.08	-23.29	53.34	38.31	13.83	790
0.32	0.23	1.79	0.48	-5.45	9.03	7.24	1.15	4.09	9.17	5.63	-3.71	22.04	12.88	9.27	3.00	15.26	4.70	-27.09	57.62	42.35	10.67	2580


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.67
et_p_h	2.54
et_p_l2	3.82


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.68	1.04	1.18	0.59	1.48	0.44	1.35	0.03	0.06	0.04	0.01	0.12	0.06	0.09	0.04	0.06	0.04	0.02	0.10	0.04	0.07	8
0.11	0.21	0.63	0.46	0.04	1.22	0.59	0.86	0.03	0.09	0.07	0.02	0.16	0.07	0.14	0.04	0.08	0.07	0.03	0.12	0.05	0.11	765
0.15	0.27	0.84	0.63	0.05	1.64	0.80	1.15	0.04	0.12	0.09	0.03	0.21	0.09	0.19	0.05	0.09	0.09	0.04	0.15	0.05	0.13	914
0.18	0.42	1.29	0.89	-0.10	2.67	1.38	1.66	0.05	0.12	0.10	0.03	0.22	0.09	0.19	0.06	0.10	0.09	0.05	0.16	0.06	0.14	790
0.32	0.61	2.35	1.47	-0.51	5.21	2.86	2.99	0.07	0.16	0.16	0.06	0.27	0.11	0.25	0.08	0.13	0.13	0.06	0.19	0.07	0.18	2580


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.35
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.87	0.89	0.90	0.85	0.93	0.04	0.90	0.90	0.90	0.93	0.82	0.97	0.08	0.94	0.91	0.93	0.94	0.87	0.99	0.06	0.98	8
0.11	0.82	0.84	0.85	0.80	0.88	0.04	0.87	0.81	0.85	0.86	0.79	0.91	0.06	0.89	0.79	0.85	0.90	0.72	0.99	0.14	0.96	765
0.15	0.79	0.82	0.82	0.77	0.86	0.05	0.85	0.79	0.83	0.83	0.76	0.89	0.06	0.87	0.77	0.84	0.86	0.70	0.97	0.13	0.94	914
0.18	0.77	0.80	0.80	0.75	0.84	0.05	0.83	0.77	0.81	0.82	0.74	0.88	0.07	0.86	0.73	0.81	0.83	0.67	0.95	0.14	0.92	790
0.32	0.72	0.75	0.75	0.70	0.80	0.05	0.78	0.72	0.77	0.77	0.70	0.84	0.07	0.82	0.65	0.74	0.76	0.59	0.90	0.15	0.85	2580


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.21


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	2.43	5.23	3.32	-0.07	10.52	5.29	4.74	5.37	6.10	6.56	3.76	8.44	2.34	7.45	0.85	2.73	1.61	-0.44	5.89	3.16	2.96	8
0.11	2.77	3.32	3.25	2.40	4.24	0.92	3.85	3.06	6.71	5.16	1.19	12.23	5.52	8.74	0.90	2.46	1.87	0.38	4.54	2.08	3.50	765
0.15	2.38	3.23	3.00	1.69	4.76	1.54	4.02	2.83	6.38	4.98	1.37	11.40	5.01	8.46	0.94	2.53	1.98	0.37	4.70	2.16	3.68	914
0.18	2.38	3.46	3.32	1.80	5.12	1.66	4.24	2.69	6.44	4.86	1.53	11.34	4.90	8.61	0.84	2.39	1.87	0.24	4.54	2.15	3.42	790
0.32	2.04	3.30	2.64	1.34	5.27	1.96	4.03	3.19	7.02	5.01	1.18	12.85	5.84	9.09	0.86	2.45	1.92	0.28	4.62	2.17	3.37	2580


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/time_misc_auc.tex <==
name	auc
attack_time	0.91
l2	1.72
lom	0.64


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.06	0.00	-0.11	0.24	0.18	0.00	0.39	0.60	0.80	0.28	0.92	0.32	0.80	0.58	0.61	0.69	0.39	0.84	0.23	0.75	8
0.11	0.00	0.07	0.00	-0.15	0.28	0.22	0.00	0.17	0.30	0.29	0.10	0.50	0.20	0.40	0.38	0.50	0.50	0.35	0.64	0.15	0.60	765
0.15	0.00	0.06	0.00	-0.15	0.27	0.21	0.00	0.00	0.24	0.25	0.03	0.45	0.21	0.33	0.33	0.46	0.44	0.30	0.61	0.16	0.57	914
0.18	0.00	0.04	0.00	-0.14	0.22	0.18	0.00	0.00	0.21	0.20	0.01	0.42	0.21	0.33	0.30	0.43	0.40	0.27	0.58	0.15	0.57	790
0.32	0.00	0.02	0.00	-0.12	0.17	0.14	0.00	0.00	0.15	0.00	-0.04	0.33	0.19	0.25	0.27	0.38	0.38	0.21	0.54	0.16	0.50	2580


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/ig/top_intersections_auc.tex <==
name	auc
top10	0.01
top30	0.06
top50	0.12


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	27.32	72.34	45.84	7.47	137.21	64.87	111.79	1.00	1.33	1.00	0.52	2.15	0.82	1.00	48.64	125.92	83.61	-4.85	256.68	130.76	121.17	1.00	1.50	1.00	0.66	2.34	0.84	1.75	6
0.11	53.38	119.59	86.62	8.04	231.14	111.55	143.14	1.00	1.58	1.00	0.76	2.40	0.82	2.00	101.06	201.95	155.55	30.00	373.89	171.94	245.20	1.00	1.70	1.00	0.77	2.63	0.93	2.00	758
0.15	58.64	148.59	98.42	-20.82	317.99	169.40	175.64	1.00	1.68	1.00	0.76	2.59	0.92	2.00	115.04	275.18	189.26	-26.32	576.68	301.50	318.66	1.00	1.79	2.00	0.80	2.78	0.99	2.00	903
0.18	58.49	135.86	98.09	5.25	266.46	130.60	168.10	1.00	1.67	1.00	0.69	2.65	0.98	2.00	135.00	297.61	216.87	45.63	549.59	251.98	372.60	1.00	1.77	1.00	0.66	2.88	1.11	2.00	763
0.32	55.42	141.57	102.25	-5.42	288.56	146.99	173.84	1.00	1.62	1.00	0.68	2.57	0.94	2.00	188.69	447.76	320.05	14.71	880.81	433.05	561.81	1.00	1.78	2.00	0.73	2.84	1.06	2.00	2582


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/comparison_vals_auc.tex <==
name	auc
orig_pp	34.06
orig_ge	0.42
adv_pp	78.45
adv_ge	0.45


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.54	0.59	0.63	0.35	0.83	0.24	0.76	0.61	0.69	0.74	0.49	0.89	0.20	0.83	0.46	0.54	0.59	0.37	0.71	0.17	0.67	6
0.11	0.21	0.38	0.40	0.12	0.64	0.26	0.57	0.33	0.49	0.52	0.24	0.75	0.26	0.69	0.25	0.38	0.40	0.18	0.59	0.21	0.53	758
0.15	0.07	0.27	0.28	-0.01	0.55	0.28	0.47	0.20	0.39	0.41	0.11	0.68	0.28	0.62	0.14	0.30	0.31	0.08	0.52	0.22	0.45	903
0.18	-0.06	0.15	0.14	-0.14	0.43	0.29	0.36	0.05	0.25	0.27	-0.05	0.55	0.30	0.47	0.05	0.19	0.20	-0.04	0.41	0.23	0.35	763
0.32	-0.27	-0.07	-0.09	-0.37	0.24	0.31	0.13	-0.24	0.01	0.01	-0.34	0.36	0.35	0.26	-0.16	0.01	0.01	-0.25	0.27	0.26	0.19	2582


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/correlations_auc.tex <==
name	auc
pcc	0.05
spearman	0.08
kendall	0.06


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	1.34	2.21	1.62	0.54	3.89	1.68	2.63	1.43	2.60	1.75	0.41	4.78	2.19	3.22	4.44	5.40	4.59	1.54	9.26	3.86	5.42	6
0.11	1.45	2.30	2.08	1.11	3.48	1.18	2.85	1.53	2.76	2.28	0.93	4.59	1.83	3.44	1.63	7.70	3.68	-1.47	16.86	9.17	10.45	758
0.15	1.51	2.26	2.10	1.17	3.34	1.08	2.78	1.60	2.71	2.31	1.02	4.40	1.69	3.39	1.55	6.23	2.90	-2.18	14.64	8.41	7.12	903
0.18	1.63	2.33	2.17	1.30	3.36	1.03	2.82	1.72	2.76	2.39	1.16	4.36	1.60	3.25	1.64	5.60	2.82	-2.22	13.42	7.82	5.59	763
0.32	1.74	2.28	2.22	1.47	3.09	0.81	2.73	1.88	2.62	2.43	1.46	3.78	1.16	3.15	1.58	3.66	2.40	-0.97	8.29	4.63	3.77	2582


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/ets_sts_auc.tex <==
name	auc
et_use	0.60
et_tse	0.70
et_ce	1.44


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.21	2.89	0.28	-3.55	9.34	6.45	0.44	1.44	2.53	2.78	1.13	3.92	1.40	3.43	1.44	3.26	2.80	0.75	5.76	2.50	4.66	6
0.11	0.22	1.46	0.38	-5.88	8.81	7.34	0.83	2.15	5.14	3.38	-0.43	10.72	5.57	6.47	1.88	7.58	3.42	-11.05	26.21	18.63	7.67	758
0.15	0.19	1.77	0.36	-5.92	9.46	7.69	0.76	2.30	5.22	3.67	-0.43	10.87	5.65	6.09	1.87	7.31	3.30	-8.11	22.73	15.42	7.46	903
0.18	0.18	1.13	0.33	-3.08	5.33	4.21	0.65	2.54	5.74	3.98	-0.56	12.05	6.30	6.70	1.99	8.62	3.58	-13.16	30.40	21.78	7.98	763
0.32	0.11	1.04	0.22	-4.85	6.93	5.89	0.50	2.70	5.65	3.75	-1.44	12.75	7.10	5.81	2.17	9.53	3.19	-23.99	43.05	33.52	6.79	2582


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.37
et_p_h	1.37
et_p_l2	2.08


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.39	0.90	0.83	0.17	1.64	0.74	1.40	0.04	0.11	0.08	0.01	0.20	0.09	0.16	0.06	0.10	0.09	0.04	0.16	0.06	0.14	6
0.11	0.37	0.93	0.74	0.13	1.73	0.80	1.28	0.04	0.10	0.08	0.03	0.18	0.07	0.15	0.05	0.09	0.08	0.04	0.14	0.05	0.13	758
0.15	0.42	1.28	0.98	0.10	2.45	1.18	1.81	0.05	0.12	0.10	0.03	0.22	0.09	0.20	0.06	0.11	0.10	0.05	0.16	0.06	0.15	903
0.18	0.65	1.64	1.27	0.17	3.11	1.47	2.18	0.05	0.13	0.11	0.04	0.23	0.09	0.20	0.07	0.11	0.10	0.06	0.17	0.06	0.15	763
0.32	1.00	3.39	2.28	-0.43	7.22	3.82	4.33	0.07	0.17	0.16	0.06	0.27	0.11	0.25	0.09	0.14	0.14	0.08	0.21	0.07	0.19	2582


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.48
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.88	0.89	0.91	0.86	0.93	0.04	0.92	0.86	0.90	0.93	0.84	0.95	0.06	0.93	0.93	0.94	0.95	0.88	0.99	0.05	0.97	6
0.11	0.83	0.85	0.86	0.82	0.89	0.04	0.88	0.83	0.87	0.87	0.81	0.92	0.05	0.91	0.83	0.88	0.92	0.76	1.00	0.12	0.97	758
0.15	0.80	0.83	0.83	0.78	0.87	0.04	0.86	0.81	0.85	0.85	0.79	0.90	0.06	0.89	0.80	0.85	0.88	0.73	0.97	0.12	0.95	903
0.18	0.78	0.81	0.81	0.76	0.85	0.05	0.84	0.78	0.82	0.83	0.76	0.88	0.06	0.87	0.76	0.83	0.84	0.71	0.95	0.12	0.93	763
0.32	0.72	0.76	0.76	0.70	0.81	0.05	0.79	0.73	0.78	0.78	0.71	0.84	0.07	0.83	0.68	0.76	0.78	0.62	0.90	0.14	0.86	2582


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.22
sts_ce	0.22


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	2.04	2.49	2.94	1.68	3.30	0.81	3.02	219.57	370.96	272.42	68.57	673.34	302.39	362.76	0.27	0.74	0.47	-0.00	1.49	0.75	1.08	6
0.11	2.58	2.74	2.74	2.19	3.28	0.55	2.88	113.67	472.49	250.98	-84.30	1029.27	556.78	597.50	0.34	0.90	0.73	0.19	1.61	0.71	1.30	758
0.15	2.32	2.74	2.58	1.69	3.80	1.05	3.59	115.72	474.86	266.52	-94.08	1043.81	568.95	597.50	0.35	0.85	0.72	0.19	1.52	0.67	1.17	903
0.18	2.25	3.07	3.23	1.71	4.44	1.36	3.99	117.76	481.60	295.36	-44.51	1007.70	526.10	621.96	0.31	0.83	0.67	0.16	1.50	0.67	1.19	763
0.32	1.26	2.33	1.87	0.86	3.80	1.47	3.11	159.31	607.81	382.32	-13.30	1228.92	621.11	844.30	0.32	0.93	0.73	0.15	1.71	0.78	1.35	2582


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/time_misc_auc.tex <==
name	auc
attack_time	0.71
l2	130.57
lom	0.22


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.25	0.25	-0.02	0.52	0.27	0.50	0.57	0.59	0.57	0.49	0.69	0.10	0.64	0.67	0.77	0.75	0.60	0.95	0.18	0.90	6
0.11	0.00	0.16	0.00	-0.15	0.47	0.31	0.00	0.40	0.50	0.50	0.31	0.70	0.19	0.67	0.62	0.69	0.70	0.56	0.83	0.13	0.78	758
0.15	0.00	0.13	0.00	-0.17	0.42	0.30	0.00	0.25	0.43	0.50	0.20	0.66	0.23	0.50	0.56	0.65	0.67	0.50	0.79	0.15	0.71	903
0.18	0.00	0.08	0.00	-0.16	0.32	0.24	0.00	0.25	0.36	0.33	0.14	0.57	0.22	0.50	0.50	0.59	0.60	0.44	0.74	0.15	0.71	763
0.32	0.00	0.04	0.00	-0.14	0.22	0.18	0.00	0.00	0.24	0.25	0.02	0.46	0.22	0.33	0.38	0.50	0.50	0.32	0.68	0.18	0.62	2582


==> data/mlm_plots/mlm_distil_fast/mr/xlnet/s/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.10
top50	0.16


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	39.76	52.70	49.07	33.80	71.61	18.90	60.52	29.00	37.85	38.00	26.20	49.50	11.65	47.00	43.74	57.23	53.87	37.17	77.29	20.06	65.12	29.00	37.75	38.00	26.15	49.35	11.60	47.00	928
0.03	41.60	59.65	53.54	31.74	87.56	27.91	69.82	19.00	31.39	30.00	17.42	45.36	13.97	42.00	49.86	70.10	63.29	38.86	101.34	31.24	81.27	19.00	31.24	30.00	17.36	45.13	13.88	42.00	977
0.06	42.61	66.78	55.38	21.58	111.98	45.20	75.88	15.00	28.17	26.00	13.23	43.11	14.94	39.00	59.11	88.90	75.30	34.44	143.35	54.45	99.34	15.00	27.92	26.00	13.13	42.71	14.79	40.00	1022
0.11	42.49	68.60	55.56	16.33	120.86	52.26	76.43	15.00	27.65	26.00	12.43	42.88	15.22	39.00	69.61	104.71	86.60	36.82	172.61	67.89	115.89	14.00	27.23	26.00	12.37	42.09	14.86	39.00	1015
0.15	42.56	66.33	54.13	17.33	115.32	49.00	73.39	16.00	29.05	28.00	14.34	43.76	14.71	41.00	88.07	125.24	107.92	56.80	193.67	68.43	140.53	16.00	28.39	27.00	14.19	42.60	14.21	39.00	959
0.18	42.55	69.41	55.63	14.78	124.04	54.63	76.83	15.00	27.62	25.00	12.33	42.92	15.29	39.00	110.38	161.71	136.98	60.43	262.98	101.28	177.08	14.00	26.59	25.00	12.07	41.11	14.52	38.00	994
0.32	42.54	70.80	55.87	5.46	136.15	65.34	77.21	15.00	27.58	25.00	12.29	42.86	15.28	39.00	156.81	235.04	204.02	92.64	377.44	142.40	270.39	14.00	25.63	24.00	11.54	39.71	14.08	36.00	1977


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/comparison_vals_auc.tex <==
name	auc
orig_pp	20.97
orig_ge	8.85
adv_pp	45.02
adv_ge	8.57


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.10	0.26	0.21	0.06	0.45	0.20	0.37	0.84	0.86	0.90	0.74	0.98	0.12	0.94	0.67	0.72	0.75	0.59	0.85	0.13	0.81	928
0.03	0.02	0.13	0.09	-0.02	0.27	0.14	0.18	0.74	0.79	0.82	0.65	0.92	0.13	0.87	0.57	0.63	0.65	0.49	0.76	0.13	0.72	977
0.06	-0.01	0.04	0.01	-0.06	0.15	0.10	0.07	0.62	0.68	0.72	0.52	0.84	0.16	0.79	0.45	0.52	0.54	0.38	0.66	0.14	0.62	1022
0.11	-0.04	-0.00	-0.02	-0.08	0.07	0.07	0.01	0.49	0.58	0.62	0.40	0.76	0.18	0.70	0.35	0.43	0.45	0.28	0.57	0.15	0.53	1015
0.15	-0.07	-0.04	-0.04	-0.10	0.02	0.06	-0.02	0.32	0.44	0.47	0.25	0.64	0.20	0.59	0.22	0.32	0.33	0.17	0.47	0.15	0.43	959
0.18	-0.10	-0.07	-0.07	-0.13	-0.02	0.06	-0.04	0.20	0.33	0.35	0.12	0.54	0.21	0.48	0.14	0.23	0.24	0.08	0.38	0.15	0.34	994
0.32	-0.16	-0.13	-0.12	-0.20	-0.06	0.07	-0.08	-0.01	0.14	0.14	-0.08	0.37	0.23	0.30	-0.01	0.10	0.10	-0.06	0.25	0.16	0.20	1977


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/correlations_auc.tex <==
name	auc
pcc	-0.01
spearman	0.14
kendall	0.10


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	8.13	12.47	11.34	6.51	18.43	5.96	15.55	8.12	13.23	11.62	6.05	20.40	7.17	17.04	6.05	11.63	9.49	3.70	19.56	7.93	14.95	928
0.03	5.95	8.33	7.52	4.66	12.00	3.67	9.83	5.75	8.96	7.74	4.01	13.91	4.95	10.79	4.50	9.59	7.14	1.67	17.52	7.92	11.44	977
0.06	4.47	5.78	5.41	3.57	7.99	2.21	6.57	4.19	6.07	5.38	2.98	9.15	3.09	7.07	3.40	6.54	4.90	0.88	12.20	5.66	7.44	1022
0.11	3.53	4.49	4.30	2.98	6.00	1.51	5.21	3.31	4.51	4.04	2.48	6.54	2.03	5.20	2.58	4.71	3.60	0.28	9.14	4.43	5.06	1015
0.15	2.92	3.56	3.44	2.64	4.48	0.92	4.08	2.73	3.47	3.27	2.34	4.61	1.13	3.92	2.14	3.24	2.68	1.00	5.47	2.23	3.64	959
0.18	2.60	3.14	3.06	2.36	3.92	0.78	3.63	2.42	3.04	2.83	2.05	4.02	0.98	3.44	1.90	2.74	2.36	0.91	4.56	1.82	3.00	994
0.32	2.30	2.73	2.72	2.11	3.35	0.62	3.10	2.18	2.64	2.52	1.93	3.36	0.72	2.98	1.64	2.26	2.02	0.96	3.55	1.29	2.51	1977


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/ets_sts_auc.tex <==
name	auc
et_use	1.35
et_tse	1.37
et_ce	1.33


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.74	7.54	4.21	-4.19	19.28	11.74	7.30	7.33	11.59	9.94	4.85	18.33	6.74	14.44	6.21	12.00	9.53	3.06	20.95	8.95	15.01	928
0.03	1.66	4.91	2.34	-6.92	16.74	11.83	3.62	6.49	9.31	8.25	4.01	14.61	5.30	10.60	5.50	9.85	7.65	-2.01	21.71	11.86	10.82	977
0.06	0.99	2.36	1.34	-3.74	8.46	6.10	1.96	5.42	7.39	6.58	3.81	10.96	3.58	8.17	4.63	7.52	5.90	1.57	13.47	5.95	8.37	1022
0.11	0.67	1.42	0.87	-3.76	6.60	5.18	1.18	4.83	6.31	5.64	3.11	9.52	3.21	6.77	4.08	6.28	5.13	1.55	11.00	4.73	6.67	1015
0.15	0.41	1.15	0.51	-8.59	10.90	9.74	0.67	4.11	5.11	4.69	3.27	6.94	1.83	5.50	3.49	4.98	4.22	1.57	8.39	3.41	5.27	959
0.18	0.29	0.47	0.36	0.02	0.91	0.45	0.48	3.72	4.58	4.21	2.86	6.30	1.72	4.91	3.16	4.66	3.75	0.04	9.28	4.62	4.60	994
0.32	0.16	0.29	0.22	-0.17	0.76	0.47	0.31	3.25	4.04	3.68	2.35	5.73	1.69	4.30	2.82	4.10	3.27	-2.99	11.18	7.08	4.02	1977


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.46
et_p_h	1.78
et_p_l2	1.81


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.10	0.09	0.04	0.15	0.06	0.13	0.03	0.04	0.04	0.02	0.06	0.02	0.06	0.03	0.04	0.04	0.02	0.05	0.02	0.05	928
0.03	0.12	0.19	0.19	0.09	0.30	0.11	0.26	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.04	0.07	0.02	0.07	977
0.06	0.25	0.37	0.36	0.19	0.55	0.18	0.48	0.06	0.08	0.08	0.05	0.12	0.03	0.10	0.06	0.07	0.07	0.05	0.10	0.02	0.09	1022
0.11	0.43	0.59	0.58	0.33	0.86	0.27	0.74	0.07	0.10	0.10	0.06	0.14	0.04	0.12	0.07	0.09	0.09	0.06	0.11	0.02	0.10	1015
0.15	0.76	1.02	1.01	0.60	1.44	0.42	1.26	0.10	0.12	0.12	0.08	0.16	0.04	0.15	0.10	0.11	0.11	0.08	0.13	0.03	0.13	959
0.18	1.11	1.51	1.47	0.89	2.12	0.61	1.86	0.12	0.14	0.14	0.10	0.18	0.04	0.17	0.11	0.13	0.13	0.10	0.15	0.03	0.14	994
0.32	1.82	2.73	2.52	1.41	4.05	1.32	3.44	0.14	0.17	0.17	0.12	0.22	0.05	0.20	0.13	0.15	0.15	0.12	0.18	0.03	0.17	1977


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.40
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.94	0.95	0.96	0.92	0.98	0.03	0.98	928
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.96	0.93	0.94	0.94	0.91	0.97	0.03	0.96	0.90	0.93	0.94	0.88	0.98	0.05	0.96	977
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.89	0.91	0.91	0.86	0.95	0.04	0.93	0.86	0.89	0.90	0.82	0.96	0.07	0.94	1022
0.11	0.86	0.88	0.88	0.84	0.92	0.04	0.90	0.85	0.87	0.88	0.82	0.92	0.05	0.90	0.81	0.85	0.86	0.76	0.93	0.08	0.90	1015
0.15	0.82	0.84	0.85	0.80	0.89	0.04	0.87	0.81	0.84	0.84	0.79	0.88	0.05	0.87	0.75	0.80	0.81	0.71	0.89	0.09	0.86	959
0.18	0.79	0.82	0.83	0.77	0.87	0.05	0.85	0.78	0.81	0.81	0.75	0.86	0.05	0.84	0.72	0.76	0.77	0.66	0.86	0.10	0.82	994
0.32	0.75	0.78	0.79	0.73	0.84	0.06	0.82	0.74	0.77	0.78	0.72	0.83	0.06	0.81	0.66	0.71	0.72	0.59	0.82	0.12	0.78	1977


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	8.02	12.00	12.57	8.07	15.92	3.92	15.55	0.27	0.42	0.37	0.22	0.61	0.20	0.55	7.29	22.29	16.66	2.25	42.33	20.04	31.02	928
0.03	5.21	10.42	9.29	4.83	16.02	5.60	16.23	0.37	0.53	0.51	0.33	0.73	0.20	0.67	7.07	22.93	15.47	0.93	44.93	22.00	31.68	977
0.06	5.68	13.91	11.28	4.59	23.22	9.31	22.03	0.45	0.62	0.60	0.41	0.83	0.21	0.78	6.33	23.30	15.28	-0.24	46.85	23.55	32.61	1022
0.11	5.70	11.57	10.28	3.87	19.27	7.70	15.74	0.47	0.63	0.61	0.42	0.84	0.21	0.80	5.99	23.33	16.22	0.20	46.46	23.13	33.49	1015
0.15	7.67	17.94	14.69	6.19	29.68	11.74	28.64	0.39	0.56	0.52	0.35	0.77	0.21	0.70	7.50	22.85	16.38	1.56	44.14	21.29	32.25	959
0.18	12.22	22.28	20.24	8.96	35.60	13.32	29.40	0.35	0.49	0.45	0.30	0.69	0.19	0.59	6.13	20.44	14.13	1.03	39.85	19.41	28.17	994
0.32	16.97	33.58	30.80	12.07	55.09	21.51	44.79	0.29	0.41	0.37	0.25	0.57	0.16	0.49	5.74	18.91	13.33	1.02	36.79	17.89	26.62	1977


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/time_misc_auc.tex <==
name	auc
attack_time	6.31
l2	0.16
lom	6.66


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.50	0.60	0.64	0.43	0.78	0.18	0.73	0.74	0.79	0.81	0.67	0.90	0.11	0.86	0.83	0.86	0.88	0.79	0.94	0.07	0.91	928
0.03	0.33	0.46	0.46	0.27	0.64	0.18	0.60	0.66	0.71	0.73	0.59	0.83	0.12	0.80	0.78	0.82	0.84	0.74	0.90	0.08	0.87	977
0.06	0.18	0.31	0.32	0.12	0.50	0.19	0.44	0.55	0.63	0.65	0.50	0.76	0.13	0.72	0.73	0.77	0.78	0.68	0.85	0.08	0.82	1022
0.11	0.05	0.20	0.19	0.03	0.37	0.17	0.32	0.47	0.55	0.57	0.41	0.69	0.14	0.65	0.67	0.73	0.74	0.64	0.81	0.09	0.79	1015
0.15	0.00	0.11	0.07	-0.02	0.24	0.13	0.20	0.38	0.46	0.48	0.33	0.60	0.14	0.56	0.62	0.67	0.68	0.58	0.77	0.09	0.74	959
0.18	0.00	0.06	0.00	-0.04	0.15	0.09	0.09	0.30	0.39	0.40	0.25	0.53	0.14	0.49	0.57	0.63	0.63	0.53	0.72	0.09	0.70	994
0.32	0.00	0.02	0.00	-0.04	0.08	0.06	0.00	0.19	0.28	0.28	0.15	0.42	0.13	0.38	0.50	0.56	0.56	0.46	0.65	0.10	0.62	1977


==> data/mlm_plots/mlm_distil_fast/yelp/bert/a/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.15
top50	0.21


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	39.74	52.41	48.97	33.80	71.03	18.62	60.15	29.00	38.06	38.00	26.59	49.53	11.47	47.00	42.82	56.67	53.13	36.86	76.48	19.81	64.81	29.00	37.80	38.00	26.43	49.16	11.37	47.00	919
0.03	41.55	59.65	53.50	31.55	87.74	28.09	69.86	19.00	31.47	30.00	17.54	45.41	13.93	42.00	50.00	69.90	62.56	38.68	101.12	31.22	81.07	19.00	31.06	30.00	17.34	44.77	13.71	42.00	977
0.06	42.74	67.55	55.72	21.55	113.55	46.00	76.36	15.00	28.19	26.00	13.28	43.10	14.91	39.00	59.67	88.93	76.16	38.28	139.59	50.66	101.86	15.00	27.59	26.00	12.93	42.24	14.65	39.00	1023
0.11	43.43	70.65	57.04	16.40	124.89	54.24	77.92	14.00	27.23	25.00	12.17	42.29	15.06	39.00	69.90	108.55	90.02	33.23	183.87	75.32	119.54	14.00	26.45	24.00	11.65	41.24	14.79	37.25	1028
0.15	42.80	69.09	56.08	20.15	118.03	48.94	76.70	15.00	27.81	25.00	12.92	42.70	14.89	39.00	90.01	132.92	113.26	51.94	213.91	80.98	150.35	15.00	26.67	24.00	12.31	41.03	14.36	38.00	988
0.18	42.58	69.35	55.97	15.57	123.12	53.78	77.83	15.00	27.30	25.00	12.20	42.40	15.10	39.00	110.67	159.34	137.76	74.10	244.59	85.24	180.06	14.00	25.78	24.00	11.42	40.13	14.35	37.00	1022
0.32	43.12	72.40	55.74	-5.29	150.10	77.70	77.75	15.00	27.91	26.00	12.60	43.23	15.32	40.00	148.53	224.03	190.81	86.53	361.53	137.50	253.56	14.00	25.67	24.00	11.43	39.92	14.24	37.00	1775


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	21.30
orig_ge	8.78
adv_pp	44.55
adv_ge	8.39


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.44	-0.04	-0.05	-0.52	0.44	0.48	0.29	-0.29	0.09	0.12	-0.35	0.53	0.44	0.40	-0.21	0.07	0.09	-0.26	0.41	0.34	0.30	919
0.03	-0.56	-0.21	-0.29	-0.65	0.23	0.44	0.07	-0.37	-0.04	-0.06	-0.45	0.36	0.40	0.27	-0.26	-0.03	-0.04	-0.33	0.28	0.30	0.20	977
0.06	-0.64	-0.37	-0.45	-0.74	-0.01	0.36	-0.18	-0.45	-0.17	-0.19	-0.51	0.17	0.34	0.06	-0.32	-0.12	-0.13	-0.38	0.13	0.25	0.05	1023
0.11	-0.71	-0.51	-0.56	-0.79	-0.23	0.28	-0.36	-0.52	-0.30	-0.31	-0.58	-0.01	0.29	-0.10	-0.37	-0.21	-0.22	-0.43	0.00	0.22	-0.06	1028
0.15	-0.78	-0.62	-0.65	-0.84	-0.41	0.22	-0.51	-0.58	-0.40	-0.41	-0.64	-0.17	0.23	-0.25	-0.42	-0.29	-0.29	-0.47	-0.11	0.18	-0.17	988
0.18	-0.81	-0.69	-0.71	-0.86	-0.51	0.18	-0.60	-0.62	-0.47	-0.48	-0.68	-0.27	0.20	-0.34	-0.46	-0.35	-0.35	-0.51	-0.19	0.16	-0.23	1022
0.32	-0.84	-0.75	-0.77	-0.88	-0.63	0.13	-0.70	-0.67	-0.55	-0.57	-0.71	-0.39	0.16	-0.45	-0.50	-0.40	-0.41	-0.53	-0.28	0.13	-0.32	1775


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/correlations_auc.tex <==
name	auc
pcc	-0.18
spearman	-0.11
kendall	-0.08


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	8.82	16.70	14.37	5.61	27.79	11.09	22.32	8.28	17.14	13.72	4.43	29.86	12.71	22.56	6.46	15.46	11.57	1.71	29.21	13.75	19.92	919
0.03	6.93	11.04	10.14	4.97	17.12	6.08	14.20	6.48	11.75	9.73	3.67	19.83	8.08	14.86	5.23	12.78	8.18	-0.20	25.77	12.99	15.07	977
0.06	5.75	8.21	7.78	4.50	11.92	3.71	10.18	5.14	8.48	7.26	3.06	13.91	5.42	10.11	4.39	10.42	6.53	-1.47	22.30	11.89	11.11	1023
0.11	5.25	7.00	6.67	4.43	9.57	2.57	8.57	4.74	6.98	6.13	3.30	10.66	3.68	8.22	3.80	8.32	5.47	-1.01	17.65	9.33	9.13	1028
0.15	4.73	5.99	5.83	4.16	7.82	1.83	7.20	4.15	5.87	5.33	3.24	8.50	2.63	6.91	3.51	6.65	4.67	-1.59	14.89	8.24	6.82	988
0.18	4.34	5.40	5.32	3.85	6.96	1.55	6.34	3.97	5.25	4.87	3.12	7.37	2.13	6.04	3.29	5.63	4.26	-0.62	11.88	6.25	5.89	1022
0.32	3.85	4.77	4.69	3.48	6.06	1.29	5.54	3.62	4.67	4.36	3.15	6.19	1.52	5.42	2.95	4.50	3.71	-0.34	9.34	4.84	4.72	1775


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/ets_sts_auc.tex <==
name	auc
et_use	2.09
et_tse	2.10
et_ce	2.29


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	3.43	14.66	6.31	-21.56	50.89	36.22	10.93	8.91	16.14	14.36	5.19	27.08	10.95	20.59	7.78	16.29	13.07	1.80	30.77	14.49	20.75	919
0.03	2.20	7.22	3.40	-12.15	26.59	19.37	5.39	8.16	12.72	11.47	5.13	20.30	7.59	15.76	7.09	12.73	10.31	2.90	22.57	9.83	15.74	977
0.06	1.41	5.20	1.94	-19.95	30.36	25.15	2.84	7.43	10.66	9.59	4.42	16.91	6.25	12.14	6.36	10.80	8.52	1.74	19.86	9.06	12.20	1023
0.11	0.99	2.45	1.33	-8.60	13.49	11.05	1.86	7.11	9.31	8.62	5.18	13.45	4.13	10.43	6.06	9.38	7.72	1.47	17.29	7.91	10.19	1028
0.15	0.62	1.26	0.81	-5.10	7.63	6.37	1.11	6.26	7.88	7.28	4.79	10.97	3.09	8.60	5.30	7.79	6.39	0.62	14.97	7.18	8.04	988
0.18	0.45	0.76	0.58	-0.26	1.78	1.02	0.78	5.75	7.10	6.54	4.43	9.76	2.67	7.56	4.86	7.05	5.74	-0.04	14.13	7.08	7.11	1022
0.32	0.28	0.50	0.38	-0.40	1.41	0.91	0.52	5.18	6.32	5.79	3.95	8.70	2.38	6.69	4.40	6.25	5.09	0.43	12.06	5.81	6.21	1775


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.79
et_p_h	2.65
et_p_l2	2.65


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.09	0.09	0.04	0.15	0.05	0.12	0.03	0.04	0.04	0.02	0.06	0.02	0.06	0.03	0.04	0.04	0.02	0.05	0.01	0.05	919
0.03	0.12	0.19	0.19	0.09	0.29	0.10	0.25	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.04	0.07	0.02	0.07	977
0.06	0.24	0.37	0.36	0.18	0.56	0.19	0.48	0.06	0.08	0.08	0.05	0.12	0.04	0.10	0.06	0.07	0.08	0.05	0.10	0.02	0.09	1023
0.11	0.41	0.60	0.58	0.32	0.88	0.28	0.75	0.07	0.10	0.10	0.06	0.14	0.04	0.12	0.07	0.09	0.09	0.06	0.11	0.02	0.10	1028
0.15	0.74	1.04	1.03	0.61	1.47	0.43	1.28	0.10	0.13	0.13	0.09	0.17	0.04	0.15	0.09	0.11	0.11	0.08	0.14	0.03	0.13	988
0.18	1.09	1.50	1.48	0.89	2.10	0.60	1.84	0.12	0.14	0.15	0.10	0.19	0.04	0.18	0.11	0.13	0.13	0.10	0.16	0.03	0.15	1022
0.32	1.71	2.49	2.32	1.30	3.69	1.19	3.08	0.14	0.17	0.17	0.12	0.22	0.05	0.20	0.13	0.15	0.15	0.12	0.18	0.03	0.17	1775


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.38
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.01	0.97	0.95	0.96	0.97	0.94	0.98	0.02	0.98	0.94	0.95	0.96	0.92	0.98	0.03	0.97	919
0.03	0.93	0.94	0.94	0.91	0.96	0.02	0.95	0.92	0.94	0.94	0.90	0.97	0.03	0.96	0.90	0.92	0.93	0.87	0.98	0.05	0.96	977
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.88	0.90	0.91	0.86	0.94	0.04	0.93	0.85	0.89	0.90	0.81	0.96	0.07	0.94	1023
0.11	0.87	0.88	0.89	0.84	0.92	0.04	0.91	0.85	0.87	0.88	0.82	0.92	0.05	0.91	0.81	0.85	0.87	0.76	0.94	0.09	0.92	1028
0.15	0.83	0.85	0.86	0.81	0.90	0.05	0.88	0.82	0.84	0.85	0.79	0.90	0.05	0.88	0.77	0.82	0.83	0.72	0.91	0.10	0.88	988
0.18	0.81	0.83	0.84	0.78	0.88	0.05	0.86	0.79	0.82	0.83	0.77	0.88	0.06	0.86	0.75	0.79	0.80	0.69	0.89	0.10	0.86	1022
0.32	0.78	0.80	0.81	0.75	0.86	0.05	0.84	0.76	0.80	0.80	0.74	0.85	0.06	0.84	0.71	0.75	0.76	0.64	0.86	0.11	0.82	1775


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.26


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	16.01	24.05	24.68	15.28	32.82	8.77	29.33	7.09	21.09	16.36	4.03	38.16	17.07	32.02	5.97	19.42	13.58	0.78	38.05	18.63	26.80	919
0.03	13.32	27.61	23.86	10.66	44.55	16.94	38.80	8.59	24.32	20.11	4.68	43.96	19.64	35.85	5.70	18.69	12.88	0.35	37.03	18.34	25.52	977
0.06	11.31	31.55	20.27	4.49	58.61	27.06	47.99	9.93	26.98	21.90	5.90	48.05	21.07	39.12	5.70	17.80	12.15	0.34	35.26	17.46	24.00	1023
0.11	12.47	19.61	18.15	8.44	30.78	11.17	24.45	10.31	28.39	23.07	3.81	52.97	24.58	39.66	5.63	18.40	12.93	0.50	36.29	17.89	24.67	1028
0.15	17.40	27.75	25.40	10.08	45.43	17.67	33.23	9.58	27.75	22.93	5.17	50.33	22.58	40.14	6.60	19.13	14.17	1.74	36.52	17.39	26.38	988
0.18	24.02	38.48	35.03	14.49	62.46	23.98	46.12	10.07	27.81	23.29	6.14	49.48	21.67	38.90	5.93	19.08	13.97	1.35	36.80	17.72	26.10	1022
0.32	42.16	80.13	62.37	24.29	135.98	55.84	104.38	11.13	29.21	24.85	6.18	52.24	23.03	41.11	5.89	19.04	13.76	1.06	37.03	17.98	26.35	1775


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/time_misc_auc.tex <==
name	auc
attack_time	12.80
l2	8.57
lom	5.84


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.08	0.26	0.23	0.04	0.49	0.22	0.40	0.21	0.39	0.39	0.18	0.60	0.21	0.54	0.40	0.54	0.55	0.37	0.71	0.17	0.66	919
0.03	0.00	0.19	0.14	-0.01	0.38	0.19	0.29	0.18	0.33	0.31	0.14	0.52	0.19	0.47	0.37	0.50	0.49	0.34	0.65	0.15	0.61	977
0.06	0.00	0.11	0.05	-0.04	0.26	0.15	0.18	0.15	0.27	0.25	0.11	0.42	0.16	0.37	0.35	0.45	0.45	0.32	0.58	0.13	0.54	1023
0.11	0.00	0.06	0.00	-0.04	0.16	0.10	0.09	0.11	0.21	0.20	0.08	0.34	0.13	0.30	0.33	0.41	0.41	0.30	0.53	0.12	0.49	1028
0.15	0.00	0.03	0.00	-0.04	0.11	0.07	0.05	0.09	0.17	0.16	0.06	0.29	0.11	0.24	0.30	0.38	0.38	0.28	0.47	0.10	0.44	988
0.18	0.00	0.02	0.00	-0.04	0.08	0.06	0.00	0.07	0.14	0.13	0.04	0.24	0.10	0.20	0.28	0.35	0.36	0.26	0.44	0.09	0.41	1022
0.32	0.00	0.01	0.00	-0.02	0.04	0.03	0.00	0.05	0.11	0.10	0.03	0.19	0.08	0.15	0.27	0.32	0.32	0.25	0.40	0.08	0.38	1775


==> data/mlm_plots/mlm_distil_fast/yelp/bert/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.06
top50	0.12


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	39.84	52.77	49.59	33.85	71.70	18.92	60.41	29.75	38.18	38.00	26.74	49.63	11.44	47.00	44.37	58.20	54.77	38.01	78.40	20.20	66.94	29.00	37.99	38.00	26.65	49.34	11.34	46.25	928
0.03	41.66	59.76	53.58	31.79	87.74	27.98	69.89	20.00	31.63	30.00	17.73	45.54	13.91	42.00	51.48	72.48	65.11	39.93	105.02	32.54	84.47	20.00	31.34	30.00	17.67	45.01	13.67	42.00	972
0.06	42.61	66.92	55.43	21.44	112.39	45.47	75.88	15.00	28.19	26.00	13.26	43.13	14.93	39.00	62.50	93.07	78.99	41.40	144.74	51.67	106.66	15.00	27.66	25.00	13.11	42.22	14.56	39.00	1022
0.11	42.82	69.21	56.18	17.19	121.23	52.02	77.21	15.00	27.49	25.00	12.44	42.54	15.05	39.00	74.15	115.08	93.56	36.51	193.66	78.57	127.95	14.00	26.84	25.00	12.25	41.44	14.60	38.00	1025
0.15	42.34	69.21	54.68	2.63	135.79	66.58	75.89	16.00	28.44	27.00	13.66	43.22	14.78	39.00	95.70	142.95	118.29	30.39	255.50	112.56	154.68	15.00	27.53	26.00	13.29	41.78	14.25	39.00	979
0.18	42.56	68.52	55.23	14.59	122.45	53.93	76.10	15.00	27.78	26.00	12.54	43.03	15.25	39.00	118.07	177.03	151.87	74.47	279.59	102.56	196.22	14.00	26.55	25.00	12.01	41.09	14.54	38.00	999
0.32	42.79	70.86	56.47	12.51	129.22	58.36	77.21	15.00	27.56	25.00	12.28	42.84	15.28	39.00	176.81	270.97	230.15	105.95	435.99	165.02	310.11	13.00	25.46	23.00	11.32	39.60	14.14	36.00	1933


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/comparison_vals_auc.tex <==
name	auc
orig_pp	21.05
orig_ge	8.84
adv_pp	50.15
adv_ge	8.50


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.44	0.55	0.56	0.37	0.74	0.18	0.68	0.70	0.77	0.78	0.65	0.88	0.11	0.85	0.52	0.60	0.60	0.48	0.71	0.11	0.68	928
0.03	0.28	0.41	0.40	0.23	0.59	0.18	0.53	0.61	0.68	0.70	0.55	0.82	0.13	0.79	0.44	0.52	0.52	0.40	0.64	0.12	0.61	972
0.06	0.15	0.28	0.26	0.11	0.45	0.17	0.38	0.48	0.58	0.60	0.42	0.75	0.16	0.70	0.34	0.43	0.44	0.30	0.56	0.13	0.52	1022
0.11	0.07	0.18	0.16	0.03	0.32	0.15	0.26	0.36	0.48	0.50	0.30	0.66	0.18	0.61	0.25	0.35	0.35	0.21	0.49	0.14	0.44	1025
0.15	-0.00	0.08	0.06	-0.05	0.22	0.14	0.16	0.24	0.37	0.38	0.16	0.57	0.20	0.52	0.17	0.26	0.27	0.11	0.41	0.15	0.37	979
0.18	-0.06	0.02	0.00	-0.11	0.15	0.13	0.09	0.11	0.25	0.26	0.04	0.47	0.22	0.40	0.08	0.18	0.18	0.02	0.33	0.15	0.28	999
0.32	-0.17	-0.09	-0.09	-0.22	0.04	0.13	-0.01	-0.13	0.04	0.04	-0.20	0.28	0.24	0.21	-0.09	0.03	0.03	-0.13	0.19	0.16	0.14	1933


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/correlations_auc.tex <==
name	auc
pcc	0.03
spearman	0.11
kendall	0.08


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	4.36	7.10	6.32	3.00	11.19	4.10	8.70	4.40	7.55	6.58	2.89	12.22	4.67	9.44	3.30	7.39	5.70	1.83	12.95	5.56	9.87	928
0.03	3.59	5.32	5.01	2.89	7.74	2.42	6.61	3.45	5.81	5.18	2.35	9.27	3.46	7.12	2.88	6.89	4.88	0.87	12.92	6.03	8.64	972
0.06	3.18	4.35	4.13	2.65	6.06	1.70	5.25	3.02	4.61	4.09	2.25	6.96	2.36	5.68	2.63	5.88	4.02	0.30	11.46	5.58	6.76	1022
0.11	2.90	3.75	3.65	2.54	4.96	1.21	4.50	2.75	3.85	3.59	2.17	5.52	1.67	4.52	2.43	4.84	3.40	-0.00	9.67	4.84	5.16	1025
0.15	2.66	3.32	3.26	2.36	4.28	0.96	3.92	2.51	3.37	3.09	2.04	4.70	1.33	3.93	2.09	3.67	2.85	0.41	6.92	3.25	4.05	979
0.18	2.47	3.05	3.02	2.19	3.90	0.86	3.61	2.34	3.06	2.87	1.93	4.20	1.14	3.53	1.93	3.30	2.51	-0.65	7.26	3.96	3.41	999
0.32	2.32	2.78	2.74	2.10	3.47	0.69	3.23	2.21	2.79	2.62	1.91	3.67	0.88	3.19	1.74	2.60	2.22	1.03	4.18	1.58	2.95	1933


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/ets_sts_auc.tex <==
name	auc
et_use	1.12
et_tse	1.15
et_ce	1.29


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.22	3.81	2.01	-3.47	11.08	7.27	3.57	3.61	6.15	5.16	2.38	9.92	3.77	7.83	3.13	6.10	4.79	1.67	10.52	4.42	7.99	928
0.03	0.90	2.57	1.31	-5.73	10.88	8.30	2.11	3.66	5.52	5.02	2.77	8.28	2.75	6.69	3.15	5.45	4.48	1.92	8.98	3.53	6.71	972
0.06	0.60	1.77	0.85	-5.02	8.56	6.79	1.25	3.62	5.08	4.65	2.69	7.46	2.39	5.92	3.13	5.11	4.20	0.89	9.32	4.22	5.65	1022
0.11	0.45	0.83	0.61	-0.64	2.30	1.47	0.83	3.57	4.58	4.31	2.51	6.64	2.06	5.16	3.03	4.47	3.77	0.88	8.06	3.59	4.93	1025
0.15	0.30	0.48	0.39	0.01	0.95	0.47	0.52	3.38	4.13	3.87	2.54	5.72	1.59	4.52	2.88	4.25	3.37	-4.29	12.79	8.54	4.19	979
0.18	0.22	0.33	0.29	0.09	0.58	0.24	0.37	3.18	3.79	3.60	2.70	4.88	1.09	4.16	2.74	3.66	3.16	0.95	6.38	2.72	3.82	999
0.32	0.13	0.22	0.18	-0.01	0.45	0.23	0.25	3.02	3.60	3.41	2.42	4.78	1.18	3.89	2.60	3.48	3.01	0.85	6.10	2.62	3.61	1933


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.27
et_p_h	1.33
et_p_l2	1.31


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.11	0.11	0.05	0.17	0.06	0.15	0.03	0.05	0.04	0.02	0.07	0.02	0.06	0.03	0.04	0.04	0.03	0.06	0.01	0.05	928
0.03	0.15	0.23	0.22	0.12	0.34	0.11	0.30	0.05	0.07	0.07	0.04	0.10	0.03	0.09	0.05	0.06	0.06	0.04	0.08	0.02	0.07	972
0.06	0.31	0.45	0.44	0.23	0.66	0.21	0.57	0.06	0.09	0.09	0.05	0.12	0.04	0.11	0.06	0.08	0.08	0.06	0.10	0.02	0.09	1022
0.11	0.51	0.72	0.69	0.40	1.03	0.32	0.88	0.09	0.11	0.11	0.07	0.15	0.04	0.13	0.08	0.10	0.10	0.07	0.12	0.02	0.11	1025
0.15	0.89	1.20	1.17	0.73	1.66	0.46	1.46	0.11	0.13	0.13	0.09	0.17	0.04	0.16	0.10	0.12	0.12	0.09	0.14	0.03	0.13	979
0.18	1.32	1.78	1.73	1.09	2.47	0.69	2.15	0.13	0.15	0.15	0.11	0.19	0.04	0.18	0.12	0.14	0.14	0.11	0.16	0.03	0.15	999
0.32	2.15	3.23	2.93	1.70	4.77	1.54	4.15	0.15	0.18	0.18	0.13	0.22	0.05	0.21	0.14	0.16	0.16	0.13	0.19	0.03	0.18	1933


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.47
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.01	0.97	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.94	0.96	0.96	0.93	0.99	0.03	0.98	928
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.93	0.94	0.94	0.91	0.97	0.03	0.96	0.90	0.93	0.94	0.88	0.98	0.05	0.97	972
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.89	0.91	0.91	0.86	0.95	0.04	0.93	0.86	0.90	0.91	0.83	0.97	0.07	0.95	1022
0.11	0.86	0.88	0.89	0.85	0.92	0.04	0.90	0.85	0.88	0.89	0.83	0.92	0.04	0.91	0.83	0.87	0.88	0.79	0.95	0.08	0.92	1025
0.15	0.83	0.85	0.86	0.81	0.89	0.04	0.88	0.82	0.85	0.85	0.80	0.90	0.05	0.88	0.78	0.83	0.84	0.74	0.92	0.09	0.88	979
0.18	0.80	0.83	0.84	0.78	0.88	0.05	0.86	0.80	0.82	0.83	0.77	0.88	0.05	0.86	0.75	0.79	0.80	0.69	0.90	0.11	0.85	999
0.32	0.76	0.79	0.80	0.74	0.85	0.05	0.83	0.76	0.79	0.79	0.73	0.85	0.06	0.83	0.69	0.74	0.76	0.63	0.85	0.11	0.81	1933


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.26


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	8.44	12.13	12.88	8.43	15.83	3.70	15.03	17.69	139.67	83.55	-25.30	304.64	164.97	209.96	2.76	7.73	6.29	1.38	14.09	6.35	11.07	928
0.03	7.92	15.59	14.05	6.98	24.19	8.60	22.90	23.50	189.58	116.80	-55.15	434.31	244.73	277.84	2.73	8.92	6.53	0.92	16.92	8.00	13.10	972
0.06	7.52	17.95	14.45	5.62	30.29	12.34	27.00	34.88	240.39	149.27	-90.86	571.65	331.25	343.74	2.43	9.60	6.76	0.62	18.58	8.98	14.80	1022
0.11	9.74	14.71	13.03	5.05	24.36	9.65	18.19	45.02	287.90	164.86	-80.14	655.95	368.04	385.51	2.80	10.48	7.21	0.69	20.28	9.80	15.54	1025
0.15	14.51	27.40	23.04	8.30	46.51	19.11	34.38	49.05	333.22	177.30	-192.00	858.45	525.23	408.05	3.40	11.25	8.50	1.20	21.29	10.04	16.60	979
0.18	11.68	19.61	17.17	4.79	34.43	14.82	24.10	59.95	361.97	198.48	-202.57	926.51	564.54	434.29	3.13	11.86	8.66	0.89	22.84	10.97	17.69	999
0.32	21.45	45.07	36.07	10.37	79.76	34.69	57.13	62.98	325.88	198.04	-130.86	782.63	456.74	405.90	3.67	11.51	8.16	1.25	21.77	10.26	16.70	1933


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/time_misc_auc.tex <==
name	auc
attack_time	7.66
l2	94.28
lom	3.37


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.40	0.51	0.52	0.36	0.66	0.15	0.62	0.65	0.71	0.71	0.61	0.80	0.09	0.77	0.76	0.80	0.81	0.74	0.87	0.06	0.85	928
0.03	0.29	0.40	0.40	0.24	0.56	0.16	0.50	0.57	0.64	0.64	0.54	0.74	0.10	0.71	0.72	0.76	0.77	0.69	0.83	0.07	0.81	972
0.06	0.18	0.29	0.29	0.13	0.45	0.16	0.40	0.48	0.57	0.57	0.45	0.68	0.12	0.64	0.67	0.72	0.73	0.64	0.80	0.08	0.77	1022
0.11	0.10	0.21	0.20	0.05	0.37	0.16	0.30	0.43	0.50	0.50	0.38	0.62	0.12	0.58	0.62	0.68	0.68	0.59	0.77	0.09	0.74	1025
0.15	0.00	0.14	0.12	0.01	0.26	0.12	0.21	0.36	0.43	0.44	0.31	0.55	0.12	0.51	0.58	0.64	0.64	0.55	0.72	0.09	0.69	979
0.18	0.00	0.09	0.05	-0.03	0.22	0.12	0.14	0.29	0.37	0.37	0.26	0.49	0.12	0.45	0.53	0.60	0.59	0.50	0.69	0.09	0.66	999
0.32	0.00	0.04	0.00	-0.03	0.12	0.08	0.07	0.19	0.27	0.26	0.16	0.39	0.12	0.35	0.45	0.52	0.51	0.42	0.61	0.10	0.58	1933


==> data/mlm_plots/mlm_distil_fast/yelp/bert/s/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.13
top50	0.20


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	40.14	55.08	51.46	33.75	76.41	21.33	64.90	26.00	35.23	35.00	23.89	46.58	11.34	44.00	43.94	59.82	55.71	37.15	82.49	22.67	70.59	26.00	34.88	35.00	23.59	46.17	11.29	43.00	888
0.03	42.64	61.61	55.05	33.17	90.05	28.44	72.34	18.00	29.04	26.00	15.54	42.54	13.50	40.00	51.81	73.22	66.02	41.45	105.00	31.78	84.93	17.00	28.35	26.00	15.13	41.57	13.22	38.00	962
0.06	43.65	68.44	57.29	29.41	107.47	39.03	78.13	14.75	26.10	23.00	11.52	40.68	14.58	36.00	61.59	91.59	79.56	44.51	138.67	47.08	104.98	13.00	25.04	22.00	11.00	39.09	14.04	35.00	1036
0.11	43.56	70.92	58.79	27.10	114.73	43.82	81.27	13.00	25.03	22.00	10.13	39.93	14.90	35.00	73.77	110.52	96.46	50.45	170.59	60.07	128.20	12.00	23.67	21.00	9.52	37.83	14.15	33.50	1043
0.15	43.72	73.02	57.57	2.38	143.66	70.64	78.21	15.00	26.34	23.00	11.39	41.29	14.95	37.00	93.80	138.29	118.48	60.64	215.93	77.64	157.25	13.00	24.28	22.00	10.34	38.21	13.94	34.00	947
0.18	43.89	72.69	57.81	11.03	134.36	61.66	79.39	13.00	25.20	22.00	10.41	40.00	14.79	36.00	117.26	173.84	145.55	50.79	296.89	123.05	192.13	12.00	22.54	20.00	9.05	36.02	13.48	33.00	997
0.32	44.08	73.57	58.41	8.00	139.14	65.57	80.33	13.00	24.79	21.00	10.14	39.44	14.65	35.00	170.09	253.67	221.11	114.64	392.70	139.03	292.80	11.00	20.92	18.00	8.22	33.63	12.70	30.00	1994


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	21.94
orig_ge	8.07
adv_pp	48.30
adv_ge	7.38


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.19	0.40	0.43	0.10	0.71	0.31	0.63	0.42	0.60	0.66	0.35	0.85	0.25	0.81	0.33	0.54	0.55	0.28	0.79	0.26	0.78	888
0.03	-0.01	0.21	0.19	-0.11	0.52	0.31	0.41	0.25	0.44	0.47	0.19	0.69	0.25	0.64	0.20	0.39	0.38	0.15	0.63	0.24	0.59	962
0.06	-0.17	0.04	0.03	-0.27	0.35	0.31	0.22	0.13	0.30	0.30	0.06	0.53	0.24	0.47	0.11	0.26	0.25	0.05	0.48	0.21	0.42	1036
0.11	-0.30	-0.10	-0.14	-0.41	0.21	0.31	0.06	0.02	0.17	0.19	-0.07	0.41	0.24	0.32	0.03	0.16	0.17	-0.04	0.36	0.20	0.28	1043
0.15	-0.44	-0.26	-0.29	-0.53	0.01	0.27	-0.13	-0.11	0.02	0.03	-0.19	0.23	0.21	0.15	-0.07	0.05	0.05	-0.12	0.21	0.17	0.16	947
0.18	-0.53	-0.37	-0.41	-0.62	-0.13	0.24	-0.25	-0.22	-0.10	-0.10	-0.29	0.09	0.19	0.01	-0.15	-0.05	-0.05	-0.20	0.10	0.15	0.04	997
0.32	-0.66	-0.52	-0.54	-0.72	-0.31	0.20	-0.41	-0.40	-0.28	-0.29	-0.45	-0.10	0.17	-0.17	-0.28	-0.19	-0.20	-0.33	-0.06	0.14	-0.10	1994


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/correlations_auc.tex <==
name	auc
pcc	-0.07
spearman	0.01
kendall	0.02


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	5.43	10.42	8.96	3.48	17.36	6.94	13.64	5.58	11.81	9.65	2.98	20.64	8.83	15.36	3.76	10.40	7.70	0.98	19.82	9.42	13.57	888
0.03	4.94	7.90	7.11	3.01	12.79	4.89	9.82	4.85	8.86	7.66	2.84	14.89	6.03	11.51	3.34	9.40	6.44	0.58	18.22	8.82	12.97	962
0.06	4.26	6.04	5.73	3.04	9.03	3.00	7.35	4.04	6.68	5.66	2.29	11.07	4.39	8.09	3.04	7.89	4.89	-1.45	17.24	9.34	8.36	1036
0.11	3.80	5.20	5.07	3.04	7.37	2.17	6.32	3.58	5.48	4.98	2.61	8.35	2.87	6.60	2.73	5.89	4.11	0.02	11.76	5.87	6.66	1043
0.15	3.86	4.69	4.64	3.19	6.19	1.50	5.46	3.57	4.77	4.45	2.84	6.69	1.92	5.56	2.60	4.62	3.45	0.35	8.89	4.27	4.77	947
0.18	3.54	4.35	4.38	3.10	5.60	1.25	5.11	3.36	4.43	4.10	2.70	6.17	1.73	5.13	2.50	3.99	3.25	0.66	7.32	3.33	4.28	997
0.32	3.30	3.93	3.93	3.00	4.86	0.93	4.53	3.18	3.95	3.76	2.79	5.11	1.16	4.50	2.35	3.46	2.95	0.93	5.99	2.53	3.77	1994


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/ets_sts_auc.tex <==
name	auc
et_use	1.59
et_tse	1.68
et_ce	1.66


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.88	7.09	3.33	-9.35	23.54	16.44	6.01	5.24	10.87	8.75	1.26	20.47	9.60	13.57	4.85	12.34	8.47	-8.62	33.30	20.96	14.62	888
0.03	1.29	3.76	1.91	-10.92	18.43	14.67	3.02	5.50	9.29	7.95	2.70	15.88	6.59	11.27	4.94	10.02	7.64	0.62	19.43	9.41	12.02	962
0.06	0.87	2.30	1.28	-3.63	8.24	5.94	1.95	5.24	8.46	7.11	2.69	14.23	5.77	10.08	4.75	9.50	6.90	-2.27	21.27	11.77	10.64	1036
0.11	0.65	1.65	0.92	-5.02	8.33	6.68	1.30	5.10	7.69	6.63	1.69	13.68	5.99	8.65	4.55	8.58	6.25	-3.77	20.93	12.35	9.02	1043
0.15	0.45	0.98	0.59	-1.64	3.59	2.61	0.84	5.05	6.69	6.12	2.95	10.43	3.74	7.44	4.51	7.28	5.74	-1.36	15.92	8.64	7.33	947
0.18	0.35	0.66	0.45	-0.72	2.03	1.37	0.60	4.84	6.32	5.71	2.67	9.96	3.65	6.83	4.27	7.93	5.32	-21.90	37.77	29.83	6.88	997
0.32	0.20	0.43	0.28	-1.10	1.96	1.53	0.40	4.49	5.67	5.21	2.99	8.35	2.68	6.14	4.00	5.83	4.78	-0.28	11.93	6.10	5.95	1994


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.45
et_p_h	2.20
et_p_l2	2.48


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.09	0.09	0.04	0.15	0.05	0.13	0.02	0.04	0.03	0.02	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.01	0.04	888
0.03	0.14	0.21	0.20	0.11	0.31	0.10	0.27	0.03	0.05	0.05	0.03	0.08	0.03	0.07	0.04	0.05	0.05	0.03	0.07	0.02	0.06	962
0.06	0.26	0.39	0.38	0.20	0.58	0.19	0.50	0.05	0.07	0.07	0.04	0.11	0.03	0.09	0.05	0.07	0.07	0.04	0.09	0.02	0.08	1036
0.11	0.44	0.62	0.62	0.35	0.90	0.27	0.79	0.07	0.09	0.09	0.05	0.13	0.04	0.11	0.07	0.08	0.09	0.06	0.11	0.03	0.10	1043
0.15	0.80	1.08	1.07	0.63	1.53	0.45	1.32	0.09	0.11	0.11	0.07	0.15	0.04	0.14	0.09	0.10	0.11	0.08	0.13	0.03	0.12	947
0.18	1.16	1.58	1.55	0.91	2.25	0.67	1.94	0.10	0.13	0.13	0.09	0.17	0.04	0.16	0.10	0.12	0.12	0.09	0.15	0.03	0.14	997
0.32	1.90	2.91	2.69	1.45	4.37	1.46	3.72	0.13	0.16	0.16	0.11	0.20	0.05	0.19	0.13	0.14	0.15	0.11	0.18	0.03	0.17	1994


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.42
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.99	0.02	0.98	0.94	0.95	0.97	0.91	1.00	0.05	0.98	888
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.96	0.93	0.94	0.95	0.91	0.97	0.03	0.96	0.90	0.92	0.94	0.86	0.99	0.07	0.97	962
0.06	0.90	0.91	0.92	0.88	0.94	0.03	0.93	0.89	0.91	0.92	0.87	0.95	0.04	0.94	0.85	0.89	0.91	0.81	0.97	0.08	0.95	1036
0.11	0.87	0.88	0.89	0.84	0.93	0.04	0.91	0.86	0.88	0.89	0.83	0.93	0.05	0.92	0.80	0.85	0.87	0.75	0.95	0.10	0.92	1043
0.15	0.84	0.86	0.86	0.82	0.89	0.04	0.88	0.83	0.85	0.86	0.81	0.90	0.05	0.89	0.76	0.81	0.82	0.72	0.90	0.09	0.87	947
0.18	0.81	0.83	0.84	0.79	0.88	0.04	0.86	0.80	0.83	0.84	0.78	0.88	0.05	0.87	0.73	0.78	0.79	0.68	0.87	0.10	0.83	997
0.32	0.77	0.80	0.81	0.75	0.84	0.05	0.83	0.76	0.80	0.80	0.74	0.85	0.05	0.83	0.68	0.73	0.74	0.63	0.84	0.10	0.80	1994


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	4.57	6.97	6.96	4.57	9.37	2.40	9.25	21.54	47.09	35.53	6.42	87.76	40.67	59.23	2.59	9.17	6.16	-1.31	19.66	10.49	12.24	888
0.03	3.10	6.04	5.14	2.60	9.47	3.43	9.50	24.02	52.04	41.62	11.13	92.96	40.92	68.25	2.70	9.36	5.83	-4.51	23.23	13.87	12.03	962
0.06	3.77	8.68	6.96	1.64	15.73	7.04	12.61	26.79	57.48	44.59	11.87	103.09	45.61	75.76	2.96	10.26	6.29	-10.97	31.50	21.23	11.87	1036
0.11	4.47	9.31	7.58	2.78	15.85	6.53	12.51	28.66	60.23	48.91	12.97	107.49	47.26	74.71	2.65	9.65	6.67	-1.18	20.47	10.83	13.15	1043
0.15	6.90	10.89	9.66	4.61	17.18	6.29	13.92	32.61	66.90	54.21	17.81	115.99	49.09	88.32	2.93	9.80	6.81	-1.21	20.81	11.01	13.71	947
0.18	11.65	13.60	13.56	11.02	16.17	2.57	15.61	36.14	70.10	57.54	21.39	118.81	48.71	90.51	3.10	10.56	6.90	-2.24	23.36	12.80	13.90	997
0.32	15.93	18.71	18.35	14.78	22.65	3.94	22.11	39.62	73.81	61.62	24.57	123.05	49.24	94.60	3.24	10.04	7.12	-0.25	20.33	10.29	13.36	1994


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/time_misc_auc.tex <==
name	auc
attack_time	3.82
l2	20.28
lom	3.12


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.43	0.59	0.60	0.39	0.79	0.20	0.75	0.58	0.71	0.72	0.55	0.88	0.17	0.87	0.68	0.78	0.79	0.65	0.92	0.13	0.91	888
0.03	0.33	0.47	0.47	0.28	0.66	0.19	0.60	0.50	0.63	0.62	0.47	0.79	0.16	0.76	0.62	0.72	0.71	0.59	0.85	0.13	0.83	962
0.06	0.22	0.35	0.33	0.16	0.54	0.19	0.47	0.44	0.55	0.55	0.41	0.70	0.14	0.67	0.58	0.66	0.66	0.54	0.78	0.12	0.76	1036
0.11	0.15	0.27	0.27	0.09	0.46	0.18	0.38	0.40	0.48	0.49	0.34	0.63	0.14	0.57	0.54	0.62	0.62	0.51	0.73	0.11	0.69	1043
0.15	0.08	0.18	0.18	0.04	0.33	0.14	0.25	0.33	0.42	0.41	0.29	0.54	0.13	0.50	0.50	0.57	0.57	0.47	0.67	0.10	0.64	947
0.18	0.00	0.12	0.11	0.00	0.25	0.12	0.19	0.29	0.35	0.35	0.24	0.46	0.11	0.42	0.46	0.52	0.53	0.43	0.61	0.09	0.58	997
0.32	0.00	0.07	0.00	-0.03	0.17	0.10	0.12	0.20	0.26	0.26	0.16	0.37	0.10	0.33	0.40	0.45	0.45	0.37	0.53	0.08	0.50	1994


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/ig/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.13
top50	0.18


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	40.87	55.65	52.01	34.59	76.70	21.06	64.81	26.00	34.71	34.00	22.99	46.42	11.71	43.00	45.37	61.72	58.81	38.78	84.67	22.95	71.76	25.00	34.25	34.00	22.68	45.83	11.58	42.75	970
0.03	42.40	61.36	54.58	33.22	89.49	28.13	72.03	17.00	28.60	26.00	15.02	42.18	13.58	39.00	53.39	75.45	67.98	42.18	108.72	33.27	88.02	17.00	27.69	25.00	14.46	40.91	13.22	38.00	975
0.06	43.38	68.43	57.12	28.21	108.65	40.22	76.99	14.00	25.95	23.00	11.34	40.56	14.61	36.00	63.50	96.76	84.07	44.27	149.24	52.48	111.01	13.00	24.45	22.00	10.43	38.46	14.01	35.00	1033
0.11	43.38	71.16	59.09	27.19	115.12	43.96	81.77	12.00	24.86	21.00	9.94	39.78	14.92	35.00	79.70	120.92	103.33	53.57	188.27	67.35	140.78	11.00	22.85	19.00	8.79	36.91	14.06	33.00	977
0.15	43.38	69.61	57.98	24.38	114.83	45.22	78.54	14.00	26.01	23.00	11.22	40.80	14.79	36.00	101.80	149.85	131.27	71.07	228.63	78.78	168.04	12.00	23.17	20.00	9.73	36.61	13.44	33.00	889
0.18	43.66	71.53	57.55	11.41	131.65	60.12	79.11	13.00	25.14	22.00	10.42	39.86	14.72	36.00	129.56	190.93	165.51	81.70	300.17	109.24	216.04	11.00	21.78	19.00	8.49	35.07	13.29	32.00	964
0.32	44.16	73.35	58.20	11.94	134.76	61.41	81.26	13.00	24.75	21.00	10.05	39.44	14.70	36.00	188.05	290.73	247.89	112.64	468.83	178.09	341.08	10.00	20.29	17.00	7.55	33.04	12.75	30.00	1910


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/comparison_vals_auc.tex <==
name	auc
orig_pp	21.70
orig_ge	8.02
adv_pp	53.46
adv_ge	7.14


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.68	0.70	0.80	0.42	0.98	0.28	0.88	0.83	0.79	0.90	0.47	1.10	0.31	0.95	0.67	0.70	0.78	0.41	0.98	0.28	0.89	970
0.03	0.58	0.66	0.70	0.45	0.87	0.21	0.80	0.76	0.79	0.85	0.56	1.01	0.22	0.90	0.61	0.67	0.71	0.48	0.87	0.19	0.80	975
0.06	0.43	0.54	0.57	0.32	0.75	0.22	0.69	0.63	0.69	0.74	0.45	0.92	0.24	0.83	0.50	0.57	0.59	0.38	0.75	0.19	0.68	1033
0.11	0.31	0.44	0.47	0.23	0.66	0.22	0.59	0.53	0.61	0.65	0.39	0.82	0.21	0.75	0.41	0.48	0.50	0.31	0.65	0.17	0.59	977
0.15	0.22	0.33	0.34	0.12	0.54	0.21	0.46	0.39	0.49	0.52	0.29	0.70	0.20	0.63	0.30	0.38	0.38	0.22	0.53	0.16	0.48	889
0.18	0.11	0.22	0.23	0.01	0.43	0.21	0.35	0.25	0.36	0.38	0.13	0.58	0.22	0.51	0.19	0.27	0.28	0.11	0.43	0.16	0.37	964
0.32	-0.09	0.04	0.04	-0.18	0.27	0.23	0.19	-0.03	0.13	0.14	-0.12	0.39	0.26	0.31	-0.01	0.10	0.10	-0.08	0.28	0.18	0.22	1910


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/correlations_auc.tex <==
name	auc
pcc	0.10
spearman	0.14
kendall	0.11


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	2.01	5.67	3.40	-1.55	12.89	7.22	5.64	2.12	6.08	3.62	-1.79	13.96	7.88	6.27	1.86	5.34	3.70	-0.31	10.99	5.65	6.87	970
0.03	1.79	3.39	2.71	0.77	6.01	2.62	4.07	1.74	3.91	2.82	0.02	7.80	3.89	4.64	1.54	4.60	3.13	-0.09	9.28	4.68	6.02	975
0.06	1.88	2.95	2.66	1.40	4.51	1.56	3.71	1.76	3.12	2.54	0.96	5.27	2.15	3.92	1.52	4.35	2.69	-0.87	9.57	5.22	4.85	1033
0.11	1.93	2.72	2.62	1.58	3.86	1.14	3.36	1.84	2.76	2.46	1.43	4.09	1.33	3.50	1.51	3.70	2.48	-0.78	8.18	4.48	4.39	977
0.15	2.02	2.62	2.57	1.53	3.71	1.09	3.12	1.86	2.56	2.39	1.45	3.68	1.12	3.14	1.47	3.13	2.17	-0.47	6.74	3.60	3.37	889
0.18	2.03	2.56	2.54	1.73	3.38	0.82	3.04	1.85	2.49	2.38	1.55	3.44	0.94	2.99	1.52	2.80	2.12	-0.10	5.71	2.90	3.14	964
0.32	2.09	2.53	2.50	1.81	3.25	0.72	2.96	1.96	2.49	2.39	1.67	3.31	0.82	2.90	1.59	2.51	2.04	0.53	4.49	1.98	2.85	1910


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/ets_sts_auc.tex <==
name	auc
et_use	0.87
et_tse	0.88
et_ce	1.03


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.49	2.73	0.90	-4.74	10.19	7.47	2.19	1.57	5.31	2.72	-2.48	13.11	7.80	5.46	1.45	6.30	2.75	-4.88	17.47	11.18	6.53	970
0.03	0.37	1.76	0.60	-6.05	9.56	7.81	1.03	1.80	3.84	2.72	-1.27	8.96	5.11	4.08	1.68	6.98	2.68	-26.29	40.25	33.27	4.40	975
0.06	0.31	0.85	0.46	-1.57	3.28	2.42	0.74	2.06	3.57	2.88	0.69	6.45	2.88	4.14	1.92	4.29	2.82	-3.51	12.10	7.80	4.45	1033
0.11	0.24	0.56	0.36	-0.52	1.63	1.08	0.54	2.26	3.39	2.88	1.16	5.61	2.22	3.86	2.05	3.73	2.80	0.13	7.34	3.61	3.96	977
0.15	0.19	0.34	0.26	-0.16	0.84	0.50	0.38	2.34	3.24	2.90	1.42	5.05	1.82	3.69	2.14	3.65	2.71	-2.88	10.18	6.53	3.75	889
0.18	0.15	0.33	0.20	-1.41	2.06	1.74	0.28	2.43	3.33	2.95	0.73	5.92	2.59	3.67	2.19	4.75	2.74	-22.14	31.64	26.89	3.62	964
0.32	0.11	0.19	0.15	-0.08	0.47	0.28	0.21	2.59	3.34	3.07	1.75	4.93	1.59	3.67	2.33	3.45	2.85	-0.38	7.29	3.84	3.58	1910


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.18
et_p_h	1.08
et_p_l2	1.35


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.12	0.11	0.06	0.17	0.06	0.16	0.02	0.04	0.04	0.02	0.06	0.02	0.05	0.03	0.04	0.04	0.02	0.05	0.01	0.05	970
0.03	0.17	0.25	0.25	0.13	0.36	0.11	0.32	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.06	0.06	0.04	0.08	0.02	0.07	975
0.06	0.34	0.47	0.46	0.26	0.68	0.21	0.58	0.05	0.08	0.08	0.05	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.10	0.02	0.09	1033
0.11	0.58	0.77	0.74	0.44	1.09	0.33	0.95	0.07	0.10	0.10	0.06	0.13	0.04	0.12	0.08	0.09	0.09	0.07	0.11	0.02	0.11	977
0.15	0.94	1.27	1.23	0.80	1.75	0.48	1.56	0.09	0.12	0.12	0.08	0.16	0.04	0.14	0.10	0.11	0.11	0.09	0.14	0.02	0.13	889
0.18	1.42	1.90	1.83	1.16	2.64	0.74	2.34	0.11	0.14	0.14	0.09	0.18	0.04	0.17	0.11	0.13	0.13	0.10	0.16	0.03	0.15	964
0.32	2.20	3.43	3.10	1.71	5.14	1.71	4.34	0.14	0.16	0.17	0.12	0.21	0.05	0.19	0.13	0.15	0.15	0.12	0.18	0.03	0.17	1910


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.50
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.99	0.02	0.98	0.95	0.96	0.97	0.91	1.00	0.05	0.98	970
0.03	0.93	0.94	0.95	0.92	0.97	0.02	0.96	0.93	0.94	0.95	0.91	0.98	0.03	0.96	0.91	0.93	0.95	0.87	1.00	0.07	0.97	975
0.06	0.91	0.92	0.92	0.89	0.94	0.03	0.93	0.89	0.91	0.92	0.87	0.95	0.04	0.94	0.86	0.90	0.92	0.83	0.97	0.07	0.96	1033
0.11	0.88	0.89	0.90	0.86	0.93	0.04	0.91	0.86	0.89	0.89	0.84	0.93	0.04	0.92	0.83	0.87	0.89	0.79	0.96	0.08	0.94	977
0.15	0.85	0.86	0.87	0.83	0.90	0.04	0.89	0.83	0.86	0.86	0.81	0.90	0.05	0.89	0.79	0.84	0.85	0.75	0.93	0.09	0.90	889
0.18	0.83	0.84	0.85	0.80	0.88	0.04	0.87	0.81	0.83	0.84	0.78	0.88	0.05	0.87	0.76	0.81	0.82	0.71	0.90	0.10	0.87	964
0.32	0.78	0.80	0.81	0.76	0.85	0.05	0.84	0.77	0.80	0.80	0.74	0.85	0.05	0.83	0.71	0.76	0.77	0.66	0.86	0.10	0.83	1910


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.26


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	1.85	5.36	3.05	-4.03	14.74	9.39	3.83	504.61	1434.04	847.93	-125.07	2993.16	1559.12	1631.17	2.13	13.41	4.84	-11.77	38.58	25.17	9.57	970
0.03	1.95	4.50	3.35	-1.14	10.14	5.64	6.20	618.43	1738.08	1061.56	-116.09	3592.26	1854.17	2096.09	2.30	8.22	4.83	-5.69	22.12	13.90	8.93	975
0.06	1.81	4.89	3.65	-0.25	10.02	5.13	7.04	724.88	1879.08	1215.32	75.30	3682.86	1803.78	2339.24	2.42	9.33	5.22	-6.28	24.93	15.60	10.41	1033
0.11	2.55	5.80	4.73	1.76	9.84	4.04	8.80	881.75	2226.08	1462.41	132.77	4319.39	2093.31	2803.87	2.37	8.16	5.53	-2.28	18.59	10.43	10.83	977
0.15	3.44	6.32	5.59	2.32	10.33	4.01	7.97	1123.97	2646.67	1924.85	501.58	4791.77	2145.09	3526.43	2.58	8.47	6.49	-0.46	17.39	8.93	11.91	889
0.18	7.57	8.87	8.73	6.66	11.08	2.21	10.30	1231.66	2881.04	2045.14	442.03	5320.05	2439.01	3746.88	3.51	10.60	7.46	-2.14	23.33	12.73	13.83	964
0.32	11.11	12.57	12.37	10.02	15.13	2.56	14.21	1504.27	3510.15	2527.85	541.77	6478.54	2968.38	4399.73	3.97	10.11	7.80	1.26	18.97	8.86	13.53	1910


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/time_misc_auc.tex <==
name	auc
attack_time	2.47
l2	816.92
lom	2.98


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.46	0.56	0.62	0.33	0.79	0.23	0.73	0.76	0.77	0.84	0.56	0.98	0.21	0.90	0.84	0.85	0.90	0.71	1.00	0.15	0.95	970
0.03	0.32	0.45	0.45	0.24	0.66	0.21	0.59	0.69	0.74	0.76	0.60	0.88	0.14	0.82	0.81	0.85	0.86	0.74	0.95	0.10	0.91	975
0.06	0.15	0.31	0.31	0.09	0.53	0.22	0.45	0.57	0.64	0.67	0.48	0.79	0.15	0.74	0.75	0.79	0.81	0.69	0.89	0.10	0.86	1033
0.11	0.00	0.22	0.20	0.00	0.44	0.22	0.33	0.50	0.56	0.59	0.41	0.71	0.15	0.67	0.70	0.75	0.76	0.64	0.86	0.11	0.82	977
0.15	0.00	0.17	0.13	-0.02	0.36	0.19	0.27	0.41	0.48	0.49	0.34	0.62	0.14	0.56	0.65	0.70	0.71	0.60	0.79	0.10	0.75	889
0.18	0.00	0.12	0.07	-0.04	0.28	0.16	0.20	0.32	0.40	0.41	0.26	0.54	0.14	0.49	0.59	0.64	0.64	0.53	0.74	0.11	0.70	964
0.32	0.00	0.07	0.00	-0.05	0.20	0.13	0.12	0.21	0.29	0.29	0.16	0.43	0.13	0.38	0.47	0.54	0.55	0.43	0.66	0.11	0.61	1910


==> data/mlm_plots/mlm_distil_fast/yelp/cnn/s/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.15
top50	0.21


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	41.00	54.99	51.35	33.82	76.16	21.17	63.59	27.00	36.05	36.00	24.72	47.38	11.33	45.00	44.83	59.99	55.64	37.30	82.68	22.69	69.34	27.00	35.69	35.00	24.52	46.86	11.17	44.00	902
0.03	42.67	61.92	54.65	32.47	91.37	29.45	72.08	19.00	30.04	28.00	16.54	43.53	13.50	41.00	51.99	74.22	66.33	40.59	107.85	33.63	85.66	18.00	29.44	28.00	16.28	42.61	13.17	40.00	1045
0.06	43.07	67.49	55.79	26.17	108.81	41.32	76.10	15.00	28.50	27.00	13.63	43.36	14.87	40.00	61.86	91.52	78.80	43.64	139.39	47.87	105.81	15.00	27.50	26.00	13.10	41.90	14.40	39.00	1250
0.11	42.54	69.79	55.32	6.14	133.45	63.66	77.70	16.00	29.16	29.00	14.19	44.13	14.97	42.00	73.94	111.90	95.44	44.16	179.63	67.73	125.68	15.00	27.89	27.00	13.49	42.30	14.41	40.00	1390
0.15	43.84	71.38	55.79	22.10	120.66	49.28	80.32	15.00	26.85	25.00	12.50	41.20	14.35	38.00	97.49	142.67	122.13	64.35	220.98	78.32	163.53	14.00	25.21	23.00	11.57	38.84	13.63	36.00	1152
0.18	45.44	79.06	59.60	7.71	150.40	71.34	85.41	12.00	24.13	21.00	9.73	38.54	14.40	34.00	122.98	184.77	153.31	64.75	304.79	120.02	205.97	11.00	22.15	19.00	8.83	35.47	13.32	32.00	903
0.32	46.10	85.70	63.04	-2.87	174.28	88.58	93.89	11.00	20.28	17.00	7.38	33.19	12.91	28.00	162.35	258.80	212.11	89.26	428.35	169.54	292.22	9.00	18.00	15.00	6.40	29.60	11.60	25.00	1197


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	23.16
orig_ge	8.00
adv_pp	49.84
adv_ge	7.50


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.71	-0.32	-0.31	-0.77	0.14	0.46	-0.00	-0.38	-0.06	-0.01	-0.49	0.37	0.43	0.27	-0.25	-0.03	0.01	-0.37	0.30	0.34	0.22	902
0.03	-0.68	-0.36	-0.34	-0.76	0.04	0.40	-0.10	-0.40	-0.12	-0.06	-0.51	0.27	0.39	0.18	-0.28	-0.08	-0.03	-0.39	0.22	0.31	0.14	1045
0.06	-0.73	-0.46	-0.44	-0.81	-0.10	0.36	-0.21	-0.51	-0.24	-0.20	-0.59	0.12	0.36	0.03	-0.37	-0.18	-0.14	-0.46	0.11	0.29	0.03	1250
0.11	-0.77	-0.54	-0.53	-0.83	-0.25	0.29	-0.33	-0.57	-0.32	-0.29	-0.63	-0.02	0.30	-0.10	-0.42	-0.24	-0.20	-0.49	0.00	0.25	-0.06	1390
0.15	-0.73	-0.58	-0.57	-0.81	-0.36	0.23	-0.44	-0.51	-0.35	-0.33	-0.60	-0.10	0.25	-0.19	-0.37	-0.26	-0.23	-0.46	-0.06	0.20	-0.12	1152
0.18	-0.72	-0.59	-0.59	-0.79	-0.38	0.20	-0.47	-0.47	-0.34	-0.33	-0.55	-0.13	0.21	-0.20	-0.33	-0.25	-0.23	-0.41	-0.08	0.16	-0.14	903
0.32	-0.74	-0.63	-0.63	-0.79	-0.47	0.16	-0.53	-0.49	-0.38	-0.38	-0.55	-0.21	0.17	-0.28	-0.35	-0.27	-0.27	-0.40	-0.14	0.13	-0.19	1197


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/correlations_auc.tex <==
name	auc
pcc	-0.17
spearman	-0.10
kendall	-0.07


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	14.81	23.82	21.58	10.95	36.68	12.87	30.15	14.37	26.46	22.42	9.25	43.68	17.22	33.58	10.08	25.54	19.30	5.31	45.78	20.23	36.23	902
0.03	9.28	14.45	13.03	6.67	22.24	7.79	17.48	8.93	16.57	13.72	5.27	27.87	11.30	20.69	6.84	18.84	12.72	2.39	35.30	16.46	26.14	1045
0.06	7.04	10.01	9.33	5.63	14.40	4.38	12.37	6.76	12.39	9.86	2.01	22.78	10.38	14.19	4.52	11.66	7.39	0.13	23.20	11.53	13.59	1250
0.11	5.50	7.67	7.36	4.77	10.56	2.90	9.30	5.42	9.28	7.27	1.04	17.53	8.24	10.33	3.83	7.79	5.40	0.17	15.41	7.62	8.64	1390
0.15	4.72	6.09	5.90	4.21	7.98	1.89	7.30	4.60	7.02	5.77	2.01	12.03	5.01	7.77	3.23	6.40	4.35	-0.81	13.61	7.21	6.58	1152
0.18	4.18	5.24	5.03	3.67	6.81	1.57	6.10	4.04	5.58	5.07	2.96	8.20	2.62	6.40	2.95	5.32	4.12	-0.17	10.80	5.49	5.48	903
0.32	3.63	4.45	4.37	3.25	5.65	1.20	5.25	3.52	4.76	4.39	2.91	6.61	1.85	5.52	2.79	4.42	3.70	1.05	7.80	3.37	4.94	1197


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/ets_sts_auc.tex <==
name	auc
et_use	2.32
et_tse	2.65
et_ce	2.53


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	4.55	12.66	7.10	-12.62	37.93	25.28	11.88	12.17	19.92	17.46	8.78	31.05	11.14	25.22	10.67	20.14	16.23	6.31	33.97	13.83	25.45	902
0.03	2.29	5.21	3.26	-4.80	15.21	10.01	4.86	9.43	13.56	12.39	7.05	20.07	6.51	16.02	8.16	13.56	11.67	5.44	21.69	8.13	16.52	1045
0.06	1.39	3.44	1.89	-14.39	21.26	17.82	2.62	7.81	10.81	9.82	5.72	15.89	5.08	12.23	6.72	11.02	9.05	2.96	19.09	8.06	12.31	1250
0.11	0.87	1.74	1.13	-5.61	9.08	7.35	1.52	6.85	8.92	8.30	5.14	12.69	3.77	9.80	5.99	9.20	7.33	-0.93	19.33	10.13	9.54	1390
0.15	0.55	1.24	0.71	-3.99	6.46	5.22	0.93	5.91	7.58	6.95	4.53	10.63	3.05	8.18	5.12	7.65	6.15	1.19	14.11	6.46	7.76	1152
0.18	0.40	0.74	0.53	-0.70	2.19	1.44	0.68	5.38	6.99	6.33	3.81	10.16	3.18	7.37	4.67	7.99	5.68	-12.06	28.03	20.05	7.12	903
0.32	0.26	0.56	0.36	-1.33	2.45	1.89	0.50	4.91	6.36	5.67	3.11	9.61	3.25	6.70	4.30	7.19	5.17	-5.21	19.58	12.39	6.51	1197


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.62
et_p_h	2.68
et_p_l2	2.85


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.10	0.09	0.04	0.15	0.05	0.13	0.03	0.04	0.04	0.02	0.07	0.02	0.06	0.03	0.04	0.04	0.02	0.05	0.02	0.05	902
0.03	0.15	0.21	0.21	0.11	0.31	0.10	0.28	0.04	0.06	0.06	0.04	0.09	0.03	0.08	0.04	0.06	0.06	0.04	0.07	0.02	0.07	1045
0.06	0.29	0.40	0.40	0.22	0.59	0.18	0.51	0.06	0.08	0.08	0.05	0.12	0.03	0.10	0.06	0.07	0.08	0.05	0.10	0.02	0.09	1250
0.11	0.51	0.71	0.68	0.40	1.01	0.31	0.87	0.08	0.10	0.11	0.07	0.14	0.04	0.13	0.08	0.09	0.10	0.07	0.12	0.02	0.11	1390
0.15	0.85	1.15	1.14	0.69	1.61	0.46	1.42	0.10	0.13	0.13	0.09	0.17	0.04	0.15	0.10	0.11	0.12	0.09	0.14	0.03	0.13	1152
0.18	1.17	1.58	1.52	0.92	2.24	0.66	1.99	0.11	0.14	0.14	0.09	0.18	0.04	0.17	0.11	0.12	0.13	0.09	0.15	0.03	0.14	903
0.32	1.63	2.48	2.28	1.19	3.78	1.29	3.09	0.13	0.15	0.16	0.10	0.20	0.05	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.16	1197


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.40
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.99	0.02	0.98	0.94	0.95	0.97	0.91	1.00	0.05	0.98	902
0.03	0.94	0.95	0.95	0.92	0.97	0.02	0.96	0.93	0.95	0.95	0.92	0.98	0.03	0.97	0.91	0.93	0.95	0.87	0.99	0.06	0.98	1045
0.06	0.91	0.92	0.92	0.88	0.95	0.03	0.94	0.90	0.92	0.93	0.88	0.96	0.04	0.95	0.84	0.88	0.90	0.80	0.97	0.08	0.95	1250
0.11	0.87	0.89	0.90	0.85	0.93	0.04	0.91	0.87	0.89	0.90	0.84	0.94	0.05	0.92	0.79	0.85	0.86	0.75	0.94	0.09	0.91	1390
0.15	0.84	0.86	0.87	0.82	0.90	0.04	0.89	0.84	0.86	0.87	0.81	0.91	0.05	0.90	0.76	0.81	0.82	0.72	0.91	0.09	0.88	1152
0.18	0.82	0.84	0.84	0.79	0.88	0.04	0.87	0.81	0.84	0.84	0.79	0.89	0.05	0.87	0.75	0.79	0.80	0.69	0.89	0.10	0.85	903
0.32	0.78	0.80	0.81	0.75	0.86	0.05	0.84	0.77	0.81	0.81	0.75	0.87	0.06	0.85	0.72	0.76	0.78	0.65	0.87	0.11	0.83	1197


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.26


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	6.92	12.89	8.53	-10.93	36.71	23.82	12.21	48.63	20934.42	115.46	-553037.73	594906.57	573972.15	403.73	9.21	26.45	20.96	4.50	48.40	21.95	38.87	902
0.03	12.78	22.89	18.17	-9.67	55.45	32.56	24.00	40.05	9587.62	108.48	-124181.89	143357.13	133769.51	496.18	6.98	23.25	16.63	1.53	44.96	21.71	33.77	1045
0.06	17.49	46.47	22.12	-22.09	115.04	68.56	31.47	42.51	7609.67	123.74	-87237.74	102457.07	94847.40	641.12	5.85	22.53	15.45	1.17	43.88	21.35	34.47	1250
0.11	18.05	50.28	23.80	-24.19	124.75	74.47	32.42	47.20	13212.54	114.33	-115830.91	142255.98	129043.45	465.79	6.15	22.75	16.93	0.84	44.65	21.90	31.73	1390
0.15	19.54	50.64	23.95	-22.47	123.76	73.11	30.25	38.13	3191.15	75.67	-68995.19	75377.49	72186.34	241.50	5.15	21.22	14.43	0.23	42.22	20.99	31.11	1152
0.18	25.03	52.28	27.34	-12.46	117.03	64.75	34.08	33.39	967.14	59.09	-12038.32	13972.59	13005.45	106.93	3.64	16.91	10.66	-1.89	35.71	18.80	23.73	903
0.32	26.13	46.76	27.86	-6.17	99.69	52.93	32.06	29.34	1371.70	44.96	-18788.31	21531.72	20160.02	77.05	2.83	12.44	7.58	-1.07	25.96	13.52	17.70	1197


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/time_misc_auc.tex <==
name	auc
attack_time	14.34
l2	1639.03
lom	5.85


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.00	0.19	0.14	-0.00	0.38	0.19	0.31	0.18	0.34	0.34	0.14	0.54	0.20	0.49	0.39	0.50	0.52	0.33	0.67	0.17	0.62	902
0.03	0.00	0.15	0.11	-0.01	0.31	0.16	0.24	0.16	0.31	0.30	0.13	0.49	0.18	0.44	0.38	0.47	0.49	0.32	0.63	0.16	0.59	1045
0.06	0.00	0.10	0.05	-0.04	0.24	0.14	0.17	0.12	0.25	0.25	0.09	0.42	0.16	0.38	0.33	0.43	0.45	0.28	0.58	0.15	0.54	1250
0.11	0.00	0.07	0.00	-0.03	0.17	0.10	0.11	0.10	0.21	0.21	0.07	0.35	0.14	0.31	0.30	0.40	0.40	0.26	0.53	0.13	0.49	1390
0.15	0.00	0.05	0.00	-0.04	0.13	0.09	0.09	0.11	0.20	0.20	0.08	0.32	0.12	0.29	0.32	0.39	0.40	0.28	0.50	0.11	0.46	1152
0.18	0.00	0.05	0.00	-0.05	0.15	0.10	0.09	0.12	0.20	0.20	0.09	0.31	0.11	0.27	0.34	0.40	0.41	0.30	0.50	0.10	0.46	903
0.32	0.00	0.04	0.00	-0.04	0.12	0.08	0.06	0.12	0.18	0.18	0.08	0.28	0.10	0.24	0.33	0.39	0.39	0.30	0.47	0.08	0.44	1197


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.07
top50	0.13


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.14	58.71	52.93	33.21	84.22	25.50	69.46	24.00	33.80	34.00	21.60	46.00	12.20	44.00	45.35	63.02	56.80	36.11	89.94	26.91	75.28	24.00	33.49	33.00	21.39	45.59	12.10	43.00	1221
0.03	43.18	64.25	55.53	32.82	95.68	31.43	74.64	16.00	27.20	25.00	13.14	41.26	14.06	38.00	52.30	75.92	68.21	41.56	110.27	34.35	89.66	15.00	26.58	24.00	12.86	40.29	13.72	37.00	910
0.06	44.10	72.28	57.11	25.80	118.77	46.48	81.00	13.00	25.50	23.00	11.13	39.87	14.37	37.00	63.75	98.90	83.13	39.95	157.85	58.95	112.92	13.00	24.47	22.00	10.62	38.31	13.84	35.00	896
0.11	45.17	80.75	59.79	-16.14	177.65	96.90	86.67	13.00	24.87	22.00	10.36	39.38	14.51	36.00	74.66	121.52	96.75	26.43	216.62	95.09	135.85	12.00	23.56	21.00	9.64	37.49	13.93	34.00	895
0.15	44.28	73.57	57.40	20.42	126.72	53.15	80.50	14.00	25.77	23.00	11.29	40.25	14.48	37.00	94.04	142.94	123.77	63.12	222.75	79.81	162.42	12.00	23.75	21.00	10.08	37.42	13.67	34.00	806
0.18	44.53	76.77	58.55	19.64	133.91	57.13	84.98	12.75	24.84	21.00	10.09	39.58	14.75	36.00	120.25	179.85	152.51	78.85	280.86	101.01	205.91	11.00	22.36	19.00	8.61	36.11	13.75	32.00	820
0.32	44.27	76.02	58.20	18.96	133.08	57.06	84.38	13.00	24.98	22.00	10.27	39.70	14.72	36.00	175.62	261.86	228.85	121.23	402.49	140.63	307.85	11.00	21.45	19.00	8.33	34.56	13.11	31.00	1594


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/comparison_vals_auc.tex <==
name	auc
orig_pp	23.17
orig_ge	7.94
adv_pp	50.42
adv_ge	7.29


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.00	0.27	0.30	0.01	0.52	0.26	0.49	0.09	0.44	0.62	0.04	0.84	0.40	0.77	0.00	0.34	0.47	0.04	0.65	0.30	0.61	1221
0.03	0.16	0.28	0.29	0.10	0.47	0.19	0.41	0.46	0.54	0.61	0.27	0.81	0.27	0.71	0.34	0.41	0.44	0.22	0.61	0.19	0.54	910
0.06	0.08	0.19	0.18	0.03	0.35	0.16	0.27	0.34	0.45	0.47	0.23	0.67	0.22	0.59	0.25	0.33	0.34	0.18	0.49	0.16	0.44	896
0.11	0.01	0.10	0.08	-0.05	0.25	0.15	0.18	0.20	0.32	0.34	0.08	0.56	0.24	0.48	0.14	0.24	0.24	0.07	0.40	0.16	0.35	895
0.15	-0.08	-0.00	-0.01	-0.14	0.13	0.13	0.06	0.04	0.17	0.17	-0.03	0.37	0.20	0.31	0.03	0.12	0.12	-0.02	0.26	0.14	0.21	806
0.18	-0.15	-0.08	-0.08	-0.22	0.06	0.14	-0.01	-0.09	0.04	0.04	-0.18	0.25	0.22	0.16	-0.05	0.03	0.03	-0.11	0.18	0.15	0.11	820
0.32	-0.28	-0.20	-0.20	-0.34	-0.06	0.14	-0.13	-0.31	-0.16	-0.17	-0.37	0.05	0.21	-0.04	-0.21	-0.11	-0.12	-0.25	0.04	0.15	-0.02	1594


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/correlations_auc.tex <==
name	auc
pcc	0.00
spearman	0.05
kendall	0.04


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	7.81	16.78	12.38	4.97	28.59	11.81	23.63	8.19	17.29	13.88	5.81	28.77	11.48	24.73	5.50	15.24	11.13	2.57	27.91	12.67	20.39	1221
0.03	4.98	7.24	6.49	3.63	10.85	3.61	8.61	4.55	8.06	6.91	2.84	13.28	5.22	9.86	3.54	9.81	6.43	0.39	19.24	9.43	12.55	910
0.06	4.00	5.26	5.06	3.43	7.10	1.83	6.33	3.48	5.60	4.83	1.94	9.26	3.66	6.73	2.75	7.07	4.34	-0.87	15.01	7.94	7.58	896
0.11	3.47	4.40	4.29	3.00	5.80	1.40	5.21	3.04	4.53	4.05	2.03	7.04	2.50	5.35	2.33	5.25	3.31	-0.51	11.01	5.76	5.66	895
0.15	3.15	3.84	3.82	2.77	4.92	1.07	4.47	2.69	3.70	3.47	2.18	5.21	1.52	4.25	2.08	3.91	2.78	-0.50	8.33	4.41	4.20	806
0.18	2.90	3.53	3.56	2.40	4.67	1.14	4.08	2.50	3.41	3.12	1.83	4.99	1.58	3.91	2.01	3.52	2.57	-0.08	7.12	3.60	3.60	820
0.32	2.68	3.17	3.18	2.42	3.92	0.75	3.64	2.44	3.05	2.91	2.08	4.01	0.96	3.48	1.88	2.80	2.36	0.72	4.89	2.08	3.03	1594


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/ets_sts_auc.tex <==
name	auc
et_use	1.42
et_tse	1.44
et_ce	1.55


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.44	17.23	4.86	-28.38	62.84	45.61	10.89	6.41	17.61	10.67	-0.88	36.11	18.50	19.32	5.99	20.94	10.86	-8.58	50.47	29.52	23.62	1221
0.03	1.19	4.56	1.70	-14.35	23.46	18.91	2.86	5.00	8.48	6.56	1.72	15.24	6.76	9.16	4.40	9.40	6.33	-0.81	19.62	10.21	10.24	910
0.06	0.77	2.32	1.03	-6.88	11.52	9.20	1.42	4.63	6.60	5.65	2.65	10.54	3.94	7.35	4.02	7.14	5.29	0.11	14.17	7.03	7.92	896
0.11	0.55	1.15	0.72	-1.07	3.36	2.21	0.99	4.25	6.09	5.09	1.54	10.63	4.55	6.38	3.71	7.37	4.74	-9.26	24.00	16.63	6.67	895
0.15	0.36	0.80	0.46	-4.14	5.75	4.95	0.66	3.94	5.20	4.59	2.24	8.16	2.96	5.52	3.46	5.97	4.25	-7.62	19.55	13.59	5.43	806
0.18	0.27	0.76	0.34	-8.24	9.76	9.00	0.47	3.75	4.92	4.27	0.95	8.90	3.97	5.13	3.19	5.62	3.90	-7.84	19.08	13.46	5.03	820
0.32	0.16	0.30	0.22	-0.39	1.00	0.69	0.31	3.50	4.45	4.00	2.19	6.70	2.25	4.76	3.08	5.16	3.64	-8.03	18.34	13.18	4.62	1594


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.55
et_p_h	1.84
et_p_l2	2.12


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.04	0.08	0.07	0.03	0.14	0.06	0.12	0.02	0.03	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.04	1221
0.03	0.13	0.21	0.20	0.10	0.31	0.11	0.28	0.03	0.06	0.05	0.03	0.08	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.07	910
0.06	0.29	0.41	0.40	0.21	0.61	0.20	0.51	0.05	0.08	0.08	0.04	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.09	896
0.11	0.44	0.63	0.62	0.35	0.90	0.28	0.79	0.07	0.09	0.09	0.06	0.13	0.04	0.12	0.07	0.09	0.09	0.06	0.11	0.03	0.10	895
0.15	0.78	1.09	1.08	0.65	1.53	0.44	1.38	0.09	0.12	0.12	0.08	0.16	0.04	0.15	0.09	0.11	0.11	0.08	0.14	0.03	0.13	806
0.18	1.16	1.59	1.57	0.93	2.25	0.66	1.94	0.11	0.13	0.14	0.09	0.18	0.04	0.16	0.11	0.12	0.13	0.09	0.15	0.03	0.14	820
0.32	1.91	2.95	2.66	1.41	4.48	1.54	3.71	0.13	0.16	0.16	0.11	0.21	0.05	0.19	0.13	0.15	0.15	0.11	0.18	0.03	0.17	1594


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.43
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.98	0.95	0.99	0.02	0.98	0.95	0.96	0.97	0.91	1.00	0.04	0.98	1221
0.03	0.93	0.94	0.95	0.92	0.96	0.02	0.96	0.93	0.94	0.95	0.91	0.98	0.03	0.96	0.90	0.93	0.95	0.87	0.99	0.06	0.97	910
0.06	0.90	0.92	0.92	0.89	0.94	0.03	0.93	0.89	0.91	0.92	0.86	0.95	0.05	0.94	0.85	0.89	0.91	0.81	0.97	0.08	0.95	896
0.11	0.88	0.89	0.90	0.85	0.93	0.04	0.91	0.86	0.88	0.89	0.83	0.93	0.05	0.92	0.81	0.85	0.87	0.76	0.95	0.09	0.93	895
0.15	0.85	0.86	0.87	0.82	0.90	0.04	0.89	0.82	0.85	0.86	0.79	0.90	0.05	0.88	0.76	0.81	0.81	0.71	0.91	0.10	0.88	806
0.18	0.82	0.84	0.85	0.79	0.88	0.05	0.87	0.79	0.82	0.83	0.77	0.88	0.06	0.86	0.73	0.78	0.79	0.67	0.89	0.11	0.85	820
0.32	0.78	0.80	0.81	0.75	0.85	0.05	0.83	0.76	0.79	0.79	0.73	0.84	0.05	0.83	0.68	0.73	0.75	0.62	0.84	0.11	0.80	1594


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	18.63	54.79	36.62	-22.24	131.82	77.03	43.32	566.03	3243.22	1453.25	-13678.61	20165.04	16921.82	2769.83	9.07	38.96	23.85	0.99	76.92	37.97	61.38	1221
0.03	13.91	21.33	16.23	0.23	42.43	21.10	21.24	966.50	12031.78	1900.69	-105609.07	129672.62	117640.84	3209.28	4.97	16.82	11.89	-2.44	36.08	19.26	20.63	910
0.06	11.37	20.89	14.57	1.72	40.05	19.16	21.66	1248.22	49413.67	2229.47	-426118.89	524946.23	475532.56	4017.09	4.05	16.55	10.50	-2.56	35.66	19.11	21.64	896
0.11	12.17	27.17	14.56	-7.54	61.89	34.71	25.36	1255.30	108507.55	2361.83	-733203.21	950218.31	841710.76	4863.20	4.01	17.30	9.83	-3.81	38.40	21.11	21.83	895
0.15	11.52	28.06	13.58	-1.83	57.95	29.89	28.12	1479.08	525516.22	2515.43	-14129800.79	15180833.22	14655317.01	4225.42	4.97	16.35	11.28	-0.24	32.95	16.59	22.53	806
0.18	16.63	35.63	17.68	1.77	69.49	33.86	43.15	1421.79	80083.66	2387.37	-1010069.31	1170236.64	1090152.98	4358.55	4.47	15.93	10.73	-1.34	33.19	17.27	21.65	820
0.32	18.85	44.68	23.28	-15.42	104.77	60.10	36.98	1425.54	243492.09	2457.38	-8301266.93	8788251.12	8544759.02	4165.57	4.62	15.17	10.46	-0.09	30.44	15.26	21.08	1594


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/time_misc_auc.tex <==
name	auc
attack_time	10.27
l2	51336.37
lom	5.26


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.08	0.29	0.29	0.07	0.50	0.22	0.46	0.32	0.52	0.59	0.29	0.75	0.23	0.71	0.53	0.68	0.74	0.51	0.85	0.17	0.82	1221
0.03	0.14	0.26	0.27	0.10	0.43	0.17	0.38	0.49	0.56	0.58	0.41	0.71	0.15	0.66	0.68	0.72	0.73	0.60	0.83	0.11	0.79	910
0.06	0.06	0.18	0.17	0.02	0.34	0.16	0.27	0.41	0.48	0.50	0.35	0.62	0.14	0.57	0.62	0.67	0.68	0.58	0.77	0.10	0.73	896
0.11	0.00	0.12	0.10	-0.01	0.26	0.13	0.20	0.33	0.41	0.42	0.28	0.55	0.13	0.50	0.57	0.62	0.63	0.53	0.72	0.10	0.69	895
0.15	0.00	0.07	0.05	-0.03	0.18	0.10	0.12	0.27	0.33	0.33	0.22	0.45	0.11	0.40	0.51	0.56	0.57	0.48	0.65	0.09	0.61	806
0.18	0.00	0.04	0.00	-0.03	0.11	0.07	0.06	0.21	0.27	0.26	0.16	0.38	0.11	0.33	0.46	0.52	0.52	0.42	0.61	0.09	0.57	820
0.32	0.00	0.02	0.00	-0.03	0.07	0.05	0.00	0.12	0.19	0.18	0.09	0.29	0.10	0.25	0.39	0.44	0.44	0.35	0.53	0.09	0.50	1594


==> data/mlm_plots/mlm_distil_fast/yelp/lstm/s/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.11
top50	0.17


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	40.85	54.35	50.71	33.91	74.79	20.44	63.00	27.00	35.94	36.00	24.82	47.06	11.12	44.00	44.12	58.76	55.12	37.22	80.29	21.54	67.74	27.00	35.69	36.00	24.67	46.72	11.03	44.00	934
0.03	42.37	60.82	54.58	33.13	88.50	27.68	70.68	18.00	29.56	28.00	16.31	42.81	13.25	40.00	50.94	70.99	64.24	40.71	101.27	30.28	82.19	18.00	29.02	27.00	15.99	42.05	13.03	39.00	968
0.06	43.55	69.32	56.75	23.58	115.06	45.74	78.83	14.00	26.36	24.00	12.02	40.69	14.33	38.00	59.81	91.41	75.57	32.96	149.86	58.45	102.19	13.00	25.51	23.00	11.61	39.42	13.90	37.00	1015
0.11	43.09	74.26	57.16	-9.75	158.27	84.01	80.38	13.00	25.55	23.00	10.79	40.30	14.76	37.00	69.73	110.48	88.34	19.25	201.70	91.22	120.65	13.00	24.57	22.00	10.29	38.85	14.28	36.00	1041
0.15	42.77	68.64	56.22	19.71	117.56	48.92	76.46	15.00	26.79	25.00	12.44	41.13	14.34	38.00	88.06	126.12	111.39	60.43	191.81	65.69	141.40	13.00	25.29	24.00	11.57	39.01	13.72	36.00	974
0.18	43.53	74.47	57.47	11.34	137.60	63.13	80.41	13.00	25.61	23.00	10.92	40.30	14.69	37.00	110.48	163.21	138.46	69.08	257.33	94.13	178.52	12.00	23.73	21.00	9.96	37.50	13.77	34.00	998
0.32	43.56	75.93	57.64	0.12	151.73	75.80	81.35	13.00	25.44	23.00	10.72	40.16	14.72	37.00	157.91	240.30	206.80	97.06	383.53	143.23	275.07	11.00	22.55	20.00	9.18	35.93	13.37	33.00	2014


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/comparison_vals_auc.tex <==
name	auc
orig_pp	22.23
orig_ge	8.22
adv_pp	45.93
adv_ge	7.71


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.15	0.33	0.32	0.11	0.55	0.22	0.48	0.94	0.95	0.96	0.92	0.99	0.03	0.98	0.83	0.86	0.87	0.80	0.92	0.06	0.90	934
0.03	0.07	0.23	0.18	0.03	0.42	0.20	0.35	0.90	0.92	0.93	0.87	0.96	0.05	0.95	0.76	0.79	0.80	0.73	0.86	0.07	0.84	968
0.06	0.02	0.14	0.08	-0.02	0.31	0.17	0.21	0.83	0.86	0.88	0.79	0.93	0.07	0.91	0.68	0.72	0.73	0.64	0.80	0.08	0.77	1015
0.11	-0.00	0.09	0.04	-0.06	0.24	0.15	0.12	0.78	0.81	0.83	0.71	0.91	0.10	0.87	0.62	0.66	0.67	0.56	0.75	0.10	0.71	1041
0.15	-0.02	0.03	-0.00	-0.08	0.15	0.11	0.05	0.69	0.73	0.74	0.62	0.84	0.11	0.80	0.52	0.57	0.57	0.47	0.66	0.09	0.62	974
0.18	-0.04	-0.00	-0.02	-0.10	0.09	0.09	0.00	0.60	0.65	0.67	0.51	0.80	0.14	0.73	0.45	0.49	0.50	0.38	0.61	0.12	0.55	998
0.32	-0.07	-0.04	-0.04	-0.11	0.03	0.07	-0.02	0.45	0.53	0.54	0.38	0.67	0.15	0.62	0.32	0.38	0.39	0.27	0.50	0.12	0.46	2014


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/correlations_auc.tex <==
name	auc
pcc	0.02
spearman	0.22
kendall	0.18


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	7.11	11.13	10.03	5.07	17.19	6.06	13.86	6.67	11.59	9.96	4.54	18.64	7.05	14.69	3.67	8.59	6.58	1.56	15.62	7.03	11.29	934
0.03	5.12	7.48	7.06	3.74	11.21	3.73	8.99	4.45	7.79	6.70	2.88	12.70	4.91	9.75	2.84	6.56	4.75	0.78	12.34	5.78	8.31	968
0.06	3.98	5.37	5.23	3.20	7.54	2.17	6.41	3.35	5.44	4.79	2.29	8.59	3.15	6.69	2.34	4.90	3.38	-0.09	9.89	4.99	5.39	1015
0.11	3.30	4.35	4.35	2.74	5.96	1.61	5.31	2.86	4.43	3.75	1.51	7.35	2.92	5.11	2.00	3.89	2.70	-0.18	7.96	4.07	4.15	1041
0.15	2.99	3.62	3.68	2.57	4.67	1.05	4.24	2.48	3.40	3.09	1.92	4.88	1.48	3.90	1.75	2.75	2.23	0.76	4.75	2.00	3.12	974
0.18	2.67	3.16	3.21	2.37	3.96	0.80	3.67	2.23	2.92	2.74	1.90	3.94	1.02	3.36	1.64	2.57	2.09	0.53	4.61	2.04	2.79	998
0.32	2.24	2.65	2.65	2.02	3.29	0.64	3.05	2.00	2.50	2.37	1.74	3.26	0.76	2.83	1.45	2.05	1.79	0.83	3.26	1.21	2.29	2014


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/ets_sts_auc.tex <==
name	auc
et_use	1.29
et_tse	1.27
et_ce	1.08


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.57	7.86	3.92	-7.96	23.67	15.82	6.82	6.51	11.03	9.49	3.98	18.08	7.05	13.57	5.84	11.65	9.15	0.44	22.87	11.22	14.54	934
0.03	1.53	4.24	2.19	-7.55	16.03	11.79	3.37	5.82	8.70	7.68	3.95	13.44	4.74	10.34	5.18	9.38	7.26	-1.64	20.39	11.02	10.96	968
0.06	0.96	2.27	1.28	-4.39	8.93	6.66	1.85	5.15	7.06	6.39	3.58	10.55	3.48	8.08	4.50	7.46	5.92	-0.96	15.88	8.42	8.37	1015
0.11	0.62	1.49	0.83	-4.33	7.31	5.82	1.11	4.52	5.96	5.52	3.24	8.69	2.73	6.65	3.96	6.09	5.05	2.13	10.05	3.96	6.66	1041
0.15	0.40	0.69	0.50	-0.86	2.24	1.55	0.68	4.04	5.16	4.56	-1.24	11.57	6.41	5.34	3.50	5.41	4.21	-4.80	15.61	10.21	5.22	974
0.18	0.29	0.63	0.36	-2.00	3.25	2.63	0.49	3.65	4.60	4.13	2.10	7.11	2.51	4.82	3.16	5.23	3.79	-6.96	17.43	12.19	4.76	998
0.32	0.16	0.33	0.21	-1.30	1.96	1.63	0.30	3.15	3.88	3.56	2.40	5.35	1.47	4.14	2.76	3.97	3.30	0.13	7.82	3.84	4.04	2014


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.44
et_p_h	1.73
et_p_l2	1.84


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.09	0.08	0.04	0.14	0.05	0.12	0.02	0.04	0.04	0.02	0.06	0.02	0.05	0.03	0.04	0.04	0.02	0.05	0.02	0.05	934
0.03	0.11	0.19	0.18	0.09	0.28	0.10	0.25	0.04	0.06	0.05	0.03	0.08	0.03	0.07	0.04	0.05	0.05	0.03	0.07	0.02	0.06	968
0.06	0.24	0.35	0.34	0.18	0.53	0.17	0.46	0.05	0.08	0.07	0.04	0.11	0.03	0.10	0.05	0.07	0.07	0.05	0.09	0.02	0.08	1015
0.11	0.41	0.58	0.56	0.31	0.85	0.27	0.72	0.07	0.09	0.09	0.05	0.13	0.04	0.11	0.07	0.09	0.09	0.06	0.11	0.03	0.10	1041
0.15	0.70	0.97	0.97	0.58	1.37	0.39	1.22	0.09	0.11	0.12	0.08	0.15	0.04	0.14	0.09	0.10	0.11	0.08	0.13	0.03	0.12	974
0.18	1.02	1.43	1.40	0.82	2.03	0.61	1.75	0.10	0.13	0.13	0.09	0.17	0.04	0.16	0.10	0.12	0.12	0.09	0.15	0.03	0.14	998
0.32	1.71	2.62	2.39	1.32	3.91	1.30	3.35	0.13	0.16	0.16	0.11	0.20	0.05	0.19	0.12	0.14	0.14	0.11	0.18	0.03	0.16	2014


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.38
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.94	0.99	0.02	0.97	0.96	0.96	0.97	0.93	0.99	0.03	0.98	0.92	0.93	0.95	0.87	0.99	0.06	0.97	934
0.03	0.93	0.94	0.94	0.91	0.97	0.03	0.95	0.92	0.93	0.94	0.90	0.97	0.04	0.96	0.86	0.90	0.92	0.83	0.97	0.07	0.96	968
0.06	0.90	0.91	0.91	0.87	0.95	0.04	0.93	0.88	0.90	0.91	0.85	0.95	0.05	0.94	0.82	0.86	0.87	0.76	0.95	0.10	0.92	1015
0.11	0.87	0.88	0.89	0.83	0.93	0.05	0.91	0.85	0.87	0.88	0.81	0.93	0.06	0.91	0.77	0.82	0.83	0.70	0.94	0.12	0.89	1041
0.15	0.84	0.86	0.87	0.81	0.90	0.05	0.89	0.81	0.84	0.84	0.78	0.89	0.06	0.88	0.73	0.77	0.78	0.67	0.88	0.10	0.84	974
0.18	0.81	0.83	0.84	0.78	0.88	0.05	0.86	0.78	0.81	0.82	0.75	0.87	0.06	0.85	0.70	0.75	0.76	0.64	0.86	0.11	0.82	998
0.32	0.77	0.79	0.80	0.73	0.85	0.06	0.83	0.74	0.78	0.78	0.72	0.84	0.06	0.82	0.64	0.70	0.71	0.58	0.82	0.12	0.77	2014


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.24


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	15.53	21.78	21.58	14.19	29.36	7.59	27.80	0.33	0.49	0.43	0.26	0.71	0.22	0.58	6.95	24.06	17.16	0.38	47.74	23.68	32.78	934
0.03	10.94	19.74	18.32	9.99	29.50	9.75	29.95	0.39	0.55	0.51	0.34	0.77	0.21	0.68	5.86	23.07	15.00	-1.10	47.24	24.17	31.57	968
0.06	8.70	19.67	17.04	7.46	31.89	12.21	30.31	0.45	0.61	0.58	0.41	0.81	0.20	0.75	5.73	22.98	13.72	-2.60	48.56	25.58	29.86	1015
0.11	8.04	23.26	17.92	6.06	40.46	17.20	36.59	0.49	0.64	0.62	0.45	0.83	0.19	0.77	5.47	22.17	14.40	-1.41	45.75	23.58	29.93	1041
0.15	6.95	28.21	15.18	0.96	55.46	27.25	44.29	0.52	0.65	0.63	0.47	0.84	0.18	0.77	6.33	23.93	16.72	0.29	47.57	23.64	32.89	974
0.18	6.74	7.41	7.54	6.51	8.31	0.90	7.90	0.50	0.64	0.61	0.45	0.82	0.18	0.75	6.39	23.79	15.17	-0.19	47.77	23.98	33.55	998
0.32	9.63	10.95	10.61	8.98	12.92	1.97	12.04	0.45	0.58	0.54	0.40	0.76	0.18	0.68	6.09	21.87	13.76	-1.11	44.85	22.98	29.55	2014


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/time_misc_auc.tex <==
name	auc
attack_time	5.00
l2	0.19
lom	7.14


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.73	0.79	0.80	0.70	0.89	0.09	0.86	0.88	0.90	0.91	0.85	0.95	0.05	0.93	0.92	0.94	0.94	0.90	0.97	0.03	0.96	934
0.03	0.60	0.68	0.68	0.55	0.80	0.12	0.75	0.82	0.85	0.86	0.79	0.91	0.06	0.89	0.88	0.91	0.91	0.87	0.95	0.04	0.93	968
0.06	0.45	0.53	0.55	0.37	0.70	0.17	0.67	0.75	0.79	0.80	0.72	0.87	0.07	0.84	0.85	0.87	0.88	0.82	0.92	0.05	0.90	1015
0.11	0.33	0.42	0.45	0.24	0.61	0.19	0.56	0.70	0.74	0.75	0.64	0.84	0.10	0.80	0.81	0.84	0.85	0.77	0.91	0.07	0.88	1041
0.15	0.20	0.31	0.33	0.14	0.48	0.17	0.43	0.63	0.68	0.68	0.58	0.77	0.09	0.73	0.77	0.80	0.81	0.74	0.87	0.07	0.84	974
0.18	0.09	0.22	0.22	0.05	0.38	0.16	0.32	0.57	0.62	0.63	0.51	0.72	0.11	0.68	0.74	0.77	0.78	0.70	0.85	0.08	0.81	998
0.32	0.00	0.11	0.07	-0.02	0.24	0.13	0.18	0.47	0.53	0.54	0.41	0.64	0.12	0.60	0.68	0.72	0.73	0.65	0.79	0.07	0.76	2014


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/a/top_intersections_auc.tex <==
name	auc
top10	0.10
top30	0.21
top50	0.25


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	40.86	54.70	51.15	34.06	75.34	20.64	63.42	27.00	36.02	36.00	24.80	47.25	11.23	45.00	44.38	59.02	54.84	36.95	81.09	22.07	68.55	27.00	35.84	36.00	24.65	47.02	11.18	44.00	926
0.03	42.68	61.01	54.59	33.30	88.71	27.71	70.97	18.00	29.32	28.00	16.04	42.61	13.29	40.00	50.33	71.37	64.89	40.24	102.50	31.13	83.09	18.00	28.94	28.00	15.86	42.01	13.07	39.00	983
0.06	43.08	69.21	56.67	23.13	115.29	46.08	78.82	14.00	26.25	24.00	11.89	40.62	14.37	38.00	59.12	91.05	76.66	36.32	145.78	54.73	102.99	14.00	25.74	23.00	11.63	39.84	14.11	37.00	1024
0.11	43.57	71.71	57.60	15.14	128.27	56.57	80.23	13.00	25.90	24.00	11.30	40.51	14.60	38.00	70.29	108.57	89.02	29.18	187.97	79.39	121.13	13.00	25.03	23.00	10.81	39.25	14.22	36.00	1046
0.15	42.63	68.64	56.27	19.45	117.82	49.18	76.86	14.00	26.54	24.00	12.19	40.90	14.35	38.00	86.08	129.36	112.76	47.27	211.45	82.09	144.11	14.00	25.39	24.00	11.59	39.19	13.80	36.00	979
0.18	43.59	74.68	57.51	11.24	138.12	63.44	80.50	13.00	25.52	23.00	10.85	40.18	14.67	37.00	109.89	167.74	140.70	54.88	280.61	112.87	184.44	12.00	23.94	22.00	10.07	37.80	13.86	34.00	989
0.32	43.58	75.09	57.68	6.50	143.68	68.59	81.47	13.00	25.41	23.00	10.71	40.11	14.70	37.00	160.71	243.86	208.88	100.05	387.66	143.80	280.23	12.00	22.86	21.00	9.56	36.15	13.30	33.00	1995


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	22.09
orig_ge	8.21
adv_pp	46.60
adv_ge	7.78


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.02	0.23	0.26	-0.14	0.60	0.37	0.50	0.41	0.53	0.56	0.33	0.74	0.21	0.69	0.32	0.43	0.44	0.26	0.61	0.18	0.56	926
0.03	-0.17	0.08	0.07	-0.29	0.45	0.37	0.32	0.26	0.40	0.41	0.18	0.62	0.22	0.55	0.20	0.32	0.32	0.15	0.49	0.17	0.44	983
0.06	-0.33	-0.08	-0.11	-0.42	0.25	0.34	0.12	0.11	0.25	0.26	0.04	0.47	0.22	0.40	0.10	0.20	0.20	0.04	0.37	0.17	0.32	1024
0.11	-0.41	-0.19	-0.25	-0.51	0.12	0.32	-0.01	0.01	0.15	0.14	-0.06	0.36	0.21	0.28	0.02	0.12	0.12	-0.03	0.28	0.16	0.22	1046
0.15	-0.49	-0.31	-0.33	-0.57	-0.05	0.26	-0.18	-0.12	-0.00	-0.01	-0.19	0.19	0.19	0.11	-0.08	0.01	0.01	-0.13	0.15	0.14	0.10	979
0.18	-0.58	-0.42	-0.46	-0.66	-0.18	0.24	-0.31	-0.25	-0.12	-0.12	-0.30	0.06	0.18	-0.01	-0.17	-0.08	-0.08	-0.21	0.06	0.14	0.00	989
0.32	-0.68	-0.55	-0.59	-0.75	-0.35	0.20	-0.45	-0.39	-0.27	-0.28	-0.45	-0.09	0.18	-0.16	-0.28	-0.19	-0.19	-0.33	-0.05	0.14	-0.10	1995


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/correlations_auc.tex <==
name	auc
pcc	-0.09
spearman	0.00
kendall	0.01


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	7.12	13.13	11.47	4.58	21.69	8.56	16.92	6.83	13.76	11.46	4.02	23.50	9.74	17.90	3.94	9.56	7.19	1.58	17.54	7.98	12.59	926
0.03	5.35	8.99	7.89	3.10	14.88	5.89	11.42	4.83	9.30	7.53	2.14	16.45	7.15	11.65	3.27	7.48	5.66	0.91	14.04	6.56	9.58	983
0.06	4.60	6.93	6.44	3.39	10.47	3.54	8.63	4.10	6.97	5.75	2.24	11.70	4.73	8.43	2.82	6.18	4.41	0.08	12.27	6.10	7.03	1024
0.11	4.06	5.72	5.59	3.29	8.15	2.43	7.10	3.57	5.51	4.84	2.01	9.01	3.50	6.49	2.42	5.15	3.57	-0.11	10.41	5.26	5.66	1046
0.15	3.70	4.78	4.70	3.16	6.41	1.62	5.73	3.34	4.52	4.12	2.28	6.76	2.24	5.29	2.32	4.15	3.25	-0.13	8.44	4.29	4.38	979
0.18	3.49	4.43	4.41	3.05	5.81	1.38	5.31	3.15	4.20	3.96	2.58	5.83	1.63	4.83	2.28	3.54	3.03	1.09	5.99	2.45	4.07	989
0.32	3.27	3.98	3.98	2.91	5.04	1.06	4.65	3.01	3.80	3.65	2.65	4.95	1.15	4.40	2.20	3.13	2.76	1.28	4.98	1.85	3.55	1995


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/ets_sts_auc.tex <==
name	auc
et_use	1.72
et_tse	1.68
et_ce	1.43


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.72	11.23	4.74	-19.31	41.77	30.54	8.82	6.78	13.41	11.61	3.69	23.13	9.72	17.68	5.92	13.60	10.72	1.87	25.34	11.74	17.52	926
0.03	1.69	5.75	2.63	-16.64	28.14	22.39	4.09	6.42	10.38	9.18	3.93	16.82	6.44	12.82	5.60	10.70	8.71	1.84	19.56	8.86	12.81	983
0.06	1.09	3.05	1.63	-7.71	13.81	10.76	2.37	5.88	8.95	8.10	4.20	13.70	4.75	10.82	5.19	9.26	7.48	2.14	16.39	7.12	11.09	1024
0.11	0.80	1.54	1.09	-1.23	4.31	2.77	1.48	5.80	8.45	7.54	2.65	14.24	5.80	9.47	5.03	9.66	7.06	-7.07	26.39	16.73	9.56	1046
0.15	0.54	1.17	0.67	-6.19	8.53	7.36	0.91	5.23	6.83	6.34	3.92	9.74	2.91	7.76	4.55	7.06	5.82	1.26	12.86	5.80	7.70	979
0.18	0.40	0.84	0.51	-2.75	4.42	3.58	0.68	5.10	6.42	6.03	3.99	8.85	2.43	7.06	4.47	6.72	5.47	1.13	12.30	5.58	6.95	989
0.32	0.23	0.41	0.31	-0.11	0.92	0.52	0.44	4.65	5.69	5.29	3.75	7.63	1.94	6.23	4.11	5.71	4.85	1.54	9.87	4.16	5.96	1995


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.59
et_p_h	2.32
et_p_l2	2.43


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.08	0.08	0.03	0.13	0.05	0.11	0.02	0.04	0.03	0.02	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.01	0.04	926
0.03	0.11	0.18	0.18	0.09	0.28	0.10	0.25	0.04	0.06	0.05	0.03	0.08	0.03	0.07	0.04	0.05	0.05	0.03	0.07	0.02	0.06	983
0.06	0.24	0.35	0.34	0.18	0.52	0.17	0.45	0.05	0.08	0.07	0.04	0.11	0.03	0.10	0.05	0.07	0.07	0.05	0.09	0.02	0.08	1024
0.11	0.41	0.57	0.56	0.32	0.82	0.25	0.72	0.06	0.09	0.09	0.05	0.13	0.04	0.11	0.07	0.08	0.08	0.06	0.11	0.03	0.10	1046
0.15	0.71	0.99	0.97	0.60	1.38	0.39	1.22	0.09	0.11	0.11	0.07	0.15	0.04	0.14	0.09	0.10	0.11	0.08	0.13	0.03	0.12	979
0.18	1.05	1.43	1.42	0.83	2.03	0.60	1.76	0.10	0.13	0.13	0.09	0.17	0.04	0.16	0.10	0.12	0.12	0.09	0.15	0.03	0.14	989
0.32	1.77	2.66	2.46	1.36	3.96	1.30	3.36	0.13	0.16	0.16	0.11	0.21	0.05	0.19	0.13	0.14	0.15	0.11	0.18	0.03	0.17	1995


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.39
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.96	0.96	0.97	0.94	0.99	0.02	0.98	0.92	0.94	0.95	0.88	0.99	0.05	0.97	926
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.92	0.94	0.94	0.90	0.97	0.04	0.96	0.87	0.90	0.92	0.83	0.97	0.07	0.95	983
0.06	0.90	0.91	0.92	0.88	0.94	0.03	0.93	0.88	0.90	0.91	0.86	0.95	0.04	0.93	0.81	0.86	0.88	0.78	0.94	0.08	0.93	1024
0.11	0.87	0.88	0.89	0.84	0.92	0.04	0.91	0.85	0.87	0.88	0.82	0.93	0.05	0.91	0.76	0.82	0.83	0.72	0.92	0.10	0.89	1046
0.15	0.84	0.85	0.86	0.80	0.90	0.05	0.88	0.81	0.84	0.84	0.78	0.89	0.06	0.87	0.72	0.78	0.79	0.66	0.89	0.12	0.85	979
0.18	0.81	0.83	0.84	0.77	0.88	0.05	0.86	0.78	0.81	0.82	0.76	0.87	0.06	0.85	0.69	0.75	0.76	0.63	0.87	0.12	0.82	989
0.32	0.77	0.79	0.80	0.74	0.85	0.05	0.83	0.75	0.78	0.79	0.73	0.84	0.06	0.82	0.65	0.70	0.72	0.59	0.82	0.12	0.78	1995


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.24


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	5.06	28.37	28.91	3.88	52.86	24.49	50.86	2.36	4.49	3.76	1.48	7.49	3.01	5.69	4.41	14.23	9.81	0.04	28.42	14.19	19.67	926
0.03	5.46	27.04	13.83	-0.41	54.50	27.46	45.54	2.79	5.12	4.49	1.89	8.36	3.23	6.60	3.66	12.78	9.02	0.15	25.42	12.64	17.88	983
0.06	5.06	29.95	6.39	-7.42	67.33	37.38	46.44	3.28	5.82	5.05	2.23	9.42	3.59	7.36	3.49	12.60	8.18	-0.66	25.87	13.26	17.35	1024
0.11	6.67	28.20	7.97	-10.13	66.53	38.33	30.20	3.52	6.25	5.58	2.60	9.89	3.65	8.10	3.18	12.66	8.30	-0.16	25.48	12.82	19.13	1046
0.15	8.57	33.20	10.42	-15.97	82.37	49.17	29.82	3.87	6.68	6.00	2.77	10.59	3.91	8.59	4.29	14.20	10.48	1.00	27.39	13.20	21.24	979
0.18	11.15	12.43	12.12	10.55	14.30	1.88	13.77	4.06	6.95	6.29	2.72	11.19	4.24	8.83	3.59	14.81	10.26	-0.57	30.18	15.37	21.02	989
0.32	15.56	18.87	18.56	14.74	22.99	4.13	22.08	4.27	7.16	6.40	3.05	11.27	4.11	9.01	3.92	15.41	10.32	-0.52	31.34	15.93	21.32	1995


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/time_misc_auc.tex <==
name	auc
attack_time	7.02
l2	2.02
lom	4.38


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.36	0.47	0.47	0.31	0.64	0.16	0.59	0.56	0.64	0.65	0.52	0.76	0.12	0.73	0.68	0.74	0.74	0.65	0.83	0.09	0.81	926
0.03	0.23	0.36	0.36	0.20	0.53	0.17	0.45	0.48	0.56	0.56	0.44	0.68	0.12	0.64	0.63	0.69	0.69	0.60	0.78	0.09	0.75	983
0.06	0.16	0.26	0.25	0.10	0.42	0.16	0.35	0.41	0.49	0.49	0.37	0.60	0.11	0.56	0.57	0.63	0.64	0.54	0.72	0.09	0.69	1024
0.11	0.09	0.20	0.18	0.04	0.36	0.16	0.29	0.36	0.43	0.44	0.32	0.55	0.12	0.51	0.54	0.60	0.60	0.51	0.69	0.09	0.66	1046
0.15	0.00	0.14	0.12	-0.00	0.28	0.14	0.19	0.29	0.36	0.35	0.25	0.47	0.11	0.42	0.49	0.54	0.54	0.46	0.62	0.08	0.58	979
0.18	0.00	0.09	0.05	-0.03	0.20	0.12	0.14	0.24	0.30	0.30	0.20	0.41	0.10	0.36	0.45	0.50	0.50	0.42	0.58	0.08	0.55	989
0.32	0.00	0.05	0.00	-0.04	0.15	0.10	0.09	0.17	0.24	0.23	0.14	0.34	0.10	0.29	0.39	0.44	0.44	0.36	0.52	0.08	0.50	1995


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/ig/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.11
top50	0.17


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	40.92	54.81	51.12	34.13	75.49	20.68	63.43	27.00	35.96	36.00	24.78	47.15	11.19	44.00	44.64	59.55	55.31	37.85	81.24	21.69	69.08	27.00	35.62	36.00	24.51	46.74	11.11	44.00	911
0.03	42.62	60.81	54.56	33.12	88.51	27.69	70.32	18.00	29.49	28.00	16.15	42.82	13.33	40.00	51.40	71.97	64.62	41.39	102.55	30.58	84.23	18.00	28.84	27.00	15.79	41.89	13.05	39.00	974
0.06	43.37	69.32	56.73	22.99	115.65	46.33	78.53	14.00	26.63	24.00	12.26	41.00	14.37	38.00	60.78	92.25	77.56	35.68	148.81	56.57	104.29	14.00	25.77	23.00	11.82	39.72	13.95	37.00	1030
0.11	43.03	72.22	57.14	2.92	141.53	69.30	79.78	13.00	25.58	23.00	10.82	40.35	14.76	37.00	70.95	112.81	93.98	-3.93	229.54	116.73	124.47	13.00	24.38	22.00	10.35	38.41	14.03	35.00	1072
0.15	42.86	68.74	56.37	19.66	117.82	49.08	76.53	14.00	26.62	24.00	12.21	41.04	14.41	38.00	89.86	135.66	114.44	45.27	226.05	90.39	150.96	14.00	25.01	24.00	11.53	38.50	13.49	35.00	989
0.18	43.55	74.06	57.45	12.42	135.70	61.64	80.36	13.00	25.58	23.00	10.90	40.26	14.68	37.00	113.11	170.84	144.04	66.71	274.98	104.14	191.75	12.00	23.29	21.00	9.73	36.86	13.57	34.00	987
0.32	43.62	75.32	57.64	6.18	144.46	69.14	81.32	13.00	25.44	23.00	10.70	40.18	14.74	37.00	166.42	252.29	215.93	97.52	407.05	154.76	288.57	11.00	22.03	20.00	8.98	35.07	13.04	32.00	1989


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/comparison_vals_auc.tex <==
name	auc
orig_pp	22.08
orig_ge	8.22
adv_pp	47.94
adv_ge	7.62


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.30	0.45	0.47	0.22	0.69	0.23	0.62	0.52	0.65	0.70	0.42	0.89	0.24	0.84	0.40	0.51	0.54	0.32	0.71	0.20	0.66	911
0.03	0.15	0.32	0.30	0.08	0.56	0.24	0.49	0.32	0.49	0.52	0.22	0.77	0.28	0.71	0.24	0.38	0.39	0.17	0.59	0.21	0.53	974
0.06	0.03	0.20	0.17	-0.03	0.43	0.23	0.35	0.13	0.34	0.36	0.04	0.64	0.30	0.57	0.11	0.26	0.26	0.04	0.48	0.22	0.41	1030
0.11	-0.05	0.12	0.09	-0.12	0.36	0.24	0.26	0.01	0.22	0.23	-0.08	0.52	0.30	0.42	0.02	0.17	0.17	-0.04	0.39	0.22	0.31	1072
0.15	-0.14	-0.00	-0.05	-0.21	0.21	0.21	0.11	-0.14	0.06	0.02	-0.23	0.35	0.29	0.25	-0.08	0.06	0.04	-0.14	0.26	0.20	0.18	989
0.18	-0.22	-0.10	-0.13	-0.30	0.09	0.20	-0.01	-0.28	-0.08	-0.12	-0.36	0.20	0.28	0.08	-0.17	-0.03	-0.06	-0.23	0.16	0.19	0.07	987
0.32	-0.36	-0.24	-0.26	-0.42	-0.05	0.18	-0.15	-0.43	-0.25	-0.30	-0.50	-0.00	0.25	-0.12	-0.28	-0.16	-0.18	-0.33	0.02	0.17	-0.07	1989


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/correlations_auc.tex <==
name	auc
pcc	0.00
spearman	0.02
kendall	0.02


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	5.33	9.32	8.23	3.57	15.08	5.76	11.70	5.13	9.81	8.20	3.24	16.38	6.57	12.59	3.13	8.15	5.81	1.05	15.25	7.10	11.26	911
0.03	4.19	6.65	6.14	3.02	10.27	3.62	8.24	3.67	7.26	5.85	2.14	12.38	5.12	9.30	2.53	6.43	4.40	0.20	12.67	6.23	7.99	974
0.06	3.55	5.20	4.99	2.66	7.75	2.55	6.46	3.02	5.34	4.53	1.70	8.99	3.65	6.58	2.14	5.53	3.49	-0.62	11.69	6.16	6.26	1030
0.11	2.94	4.33	4.32	2.46	6.20	1.87	5.42	2.57	4.37	3.67	1.20	7.54	3.17	5.13	1.93	4.25	2.71	-0.65	9.16	4.91	4.80	1072
0.15	3.01	3.86	3.80	2.52	5.20	1.34	4.72	2.57	3.66	3.28	1.90	5.42	1.76	4.36	1.91	3.79	2.70	-0.62	8.20	4.41	4.01	989
0.18	2.89	3.59	3.67	2.52	4.66	1.07	4.25	2.52	3.42	3.11	1.90	4.93	1.52	4.02	1.89	3.19	2.51	0.45	5.92	2.73	3.41	987
0.32	2.74	3.27	3.29	2.43	4.11	0.84	3.83	2.48	3.13	2.97	2.10	4.15	1.02	3.59	1.85	2.73	2.33	0.94	4.51	1.79	3.01	1989


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/ets_sts_auc.tex <==
name	auc
et_use	1.33
et_tse	1.33
et_ce	1.25


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.88	6.33	3.03	-10.40	23.05	16.72	5.07	4.80	8.67	7.25	2.90	14.43	5.77	11.03	4.30	9.00	6.89	1.76	16.24	7.24	11.35	911
0.03	1.14	3.81	1.72	-7.88	15.49	11.68	2.81	4.49	7.25	6.37	3.08	11.42	4.17	8.99	3.98	7.58	6.03	1.68	13.47	5.89	9.08	974
0.06	0.79	1.61	1.13	-0.75	3.97	2.36	1.58	4.18	6.38	5.76	2.80	9.96	3.58	7.56	3.71	6.97	5.38	-2.17	16.10	9.13	7.66	1030
0.11	0.55	1.22	0.75	-6.21	8.64	7.42	1.06	4.10	5.45	5.11	2.87	8.04	2.58	6.23	3.47	5.74	4.74	0.38	11.09	5.35	6.24	1072
0.15	0.36	0.72	0.48	-2.99	4.42	3.70	0.64	3.90	4.94	4.63	2.97	6.91	1.97	5.53	3.40	5.07	4.20	1.02	9.12	4.05	5.59	989
0.18	0.29	0.62	0.36	-2.49	3.73	3.11	0.50	3.78	4.85	4.43	2.16	7.53	2.69	5.24	3.28	6.03	4.03	-18.44	30.51	24.48	5.02	987
0.32	0.17	0.48	0.23	-4.66	5.61	5.13	0.33	3.62	4.43	4.15	2.88	5.98	1.55	4.84	3.20	4.45	3.79	0.53	8.36	3.91	4.67	1989


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.39
et_p_h	1.66
et_p_l2	1.82


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.09	0.09	0.04	0.15	0.05	0.12	0.02	0.04	0.04	0.02	0.06	0.02	0.05	0.03	0.04	0.04	0.02	0.05	0.02	0.05	911
0.03	0.13	0.20	0.20	0.10	0.31	0.10	0.27	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.07	974
0.06	0.26	0.38	0.37	0.20	0.56	0.18	0.48	0.05	0.08	0.08	0.04	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.09	1030
0.11	0.42	0.62	0.59	0.33	0.91	0.29	0.79	0.07	0.10	0.10	0.06	0.14	0.04	0.12	0.07	0.09	0.09	0.06	0.11	0.03	0.10	1072
0.15	0.81	1.08	1.05	0.67	1.48	0.41	1.34	0.09	0.12	0.12	0.08	0.16	0.04	0.14	0.10	0.11	0.11	0.08	0.13	0.03	0.13	989
0.18	1.10	1.52	1.52	0.90	2.14	0.62	1.87	0.11	0.14	0.14	0.09	0.18	0.04	0.16	0.11	0.12	0.13	0.10	0.15	0.03	0.14	987
0.32	1.88	2.79	2.57	1.42	4.17	1.38	3.54	0.13	0.16	0.16	0.12	0.21	0.05	0.19	0.13	0.15	0.15	0.12	0.18	0.03	0.17	1989


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.96	0.96	0.97	0.94	0.99	0.03	0.98	0.93	0.94	0.96	0.89	0.99	0.05	0.98	911
0.03	0.93	0.94	0.94	0.91	0.97	0.03	0.95	0.93	0.94	0.95	0.90	0.98	0.04	0.96	0.88	0.91	0.93	0.83	0.98	0.07	0.96	974
0.06	0.90	0.91	0.92	0.88	0.95	0.04	0.93	0.88	0.90	0.92	0.86	0.95	0.05	0.93	0.83	0.87	0.89	0.78	0.96	0.09	0.94	1030
0.11	0.87	0.89	0.90	0.83	0.94	0.05	0.91	0.85	0.87	0.89	0.82	0.93	0.06	0.91	0.77	0.83	0.84	0.71	0.95	0.12	0.91	1072
0.15	0.84	0.86	0.87	0.81	0.90	0.04	0.89	0.81	0.84	0.85	0.79	0.90	0.05	0.88	0.75	0.80	0.81	0.70	0.90	0.10	0.87	989
0.18	0.82	0.84	0.85	0.79	0.88	0.05	0.87	0.79	0.82	0.82	0.77	0.88	0.05	0.86	0.72	0.77	0.78	0.66	0.88	0.11	0.84	987
0.32	0.78	0.80	0.81	0.75	0.85	0.05	0.83	0.75	0.79	0.79	0.73	0.84	0.05	0.83	0.67	0.73	0.73	0.62	0.83	0.11	0.79	1989


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	4.72	28.15	5.58	-0.20	56.50	28.35	52.87	51.68	101.00	82.28	27.70	174.30	73.30	125.35	7.25	21.79	16.21	1.39	42.19	20.40	30.66	911
0.03	4.15	28.52	16.29	-1.53	58.58	30.06	48.58	58.14	113.69	93.47	33.09	194.30	80.61	140.91	6.26	22.39	14.91	-0.09	44.88	22.49	31.38	974
0.06	4.39	30.46	6.28	-6.60	67.52	37.06	51.09	66.36	131.02	105.37	26.44	235.61	104.58	162.86	5.95	22.82	14.38	-0.94	46.58	23.76	32.05	1030
0.11	6.07	26.49	6.72	-11.79	64.78	38.29	26.99	68.27	140.78	115.50	29.17	252.38	111.61	180.77	5.87	22.47	14.45	-0.54	45.48	23.01	30.77	1072
0.15	6.99	31.08	8.54	-20.20	82.37	51.28	20.93	76.57	153.62	123.14	28.02	279.21	125.59	191.42	7.08	24.08	15.63	0.23	47.93	23.85	34.53	989
0.18	9.75	10.40	10.46	9.10	11.69	1.30	11.00	82.30	170.83	126.81	23.09	318.57	147.74	206.40	6.79	23.59	15.79	1.16	46.01	22.43	33.71	987
0.32	12.10	15.37	15.07	11.39	19.35	3.98	18.45	89.03	190.81	138.77	-4.55	386.18	195.37	220.61	6.74	22.73	14.98	0.75	44.70	21.97	32.28	1989


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/time_misc_auc.tex <==
name	auc
attack_time	6.51
l2	48.70
lom	7.16


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.23	0.38	0.36	0.17	0.58	0.20	0.50	0.53	0.62	0.63	0.47	0.77	0.15	0.73	0.69	0.76	0.77	0.64	0.87	0.11	0.84	911
0.03	0.12	0.26	0.23	0.07	0.45	0.19	0.38	0.41	0.52	0.52	0.36	0.68	0.16	0.63	0.60	0.68	0.69	0.56	0.81	0.13	0.77	974
0.06	0.05	0.18	0.14	0.01	0.34	0.17	0.27	0.32	0.43	0.43	0.27	0.59	0.16	0.53	0.53	0.62	0.62	0.49	0.75	0.13	0.71	1030
0.11	0.00	0.13	0.07	-0.05	0.31	0.18	0.18	0.26	0.38	0.36	0.21	0.55	0.17	0.48	0.48	0.57	0.57	0.44	0.71	0.13	0.65	1072
0.15	0.00	0.08	0.00	-0.05	0.20	0.12	0.11	0.21	0.31	0.29	0.16	0.46	0.15	0.38	0.43	0.52	0.50	0.39	0.64	0.12	0.59	989
0.18	0.00	0.05	0.00	-0.05	0.15	0.10	0.06	0.15	0.24	0.22	0.10	0.38	0.14	0.31	0.38	0.46	0.46	0.34	0.58	0.12	0.54	987
0.32	0.00	0.02	0.00	-0.04	0.09	0.07	0.00	0.09	0.17	0.15	0.05	0.28	0.12	0.22	0.32	0.40	0.39	0.29	0.51	0.11	0.46	1989


==> data/mlm_plots/mlm_distil_fast/yelp/lstmatt/s/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.10
top50	0.16


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	33.05	43.94	41.19	28.27	59.61	15.67	51.03	15.00	18.90	18.00	13.08	24.72	5.82	23.00	36.44	48.07	45.11	31.40	64.73	16.66	56.08	15.00	18.85	18.00	13.04	24.67	5.81	23.00	907
0.03	33.84	47.33	43.47	26.69	67.97	20.64	54.38	10.00	15.64	15.00	8.78	22.50	6.86	20.00	41.17	56.70	52.23	33.42	79.98	23.28	66.20	10.00	15.50	15.00	8.66	22.34	6.84	20.00	982
0.06	34.47	53.40	44.78	18.38	88.43	35.03	58.63	7.00	13.75	12.00	6.37	21.13	7.38	19.00	48.69	72.46	62.33	29.08	115.85	43.38	79.69	7.00	13.64	12.00	6.25	21.02	7.39	19.00	1033
0.11	34.83	53.95	45.81	21.19	86.71	32.76	60.07	7.00	13.30	12.00	5.88	20.72	7.42	18.00	58.25	85.85	73.17	35.96	135.74	49.89	95.44	7.00	13.25	12.00	5.76	20.74	7.49	19.00	1014
0.15	34.74	54.95	45.19	13.61	96.29	41.34	58.86	7.00	13.48	12.00	6.04	20.91	7.44	19.00	72.96	108.08	92.79	43.82	172.33	64.25	119.74	7.00	13.75	13.00	6.08	21.42	7.67	19.00	966
0.18	34.73	56.20	45.37	9.06	103.33	47.13	60.08	7.00	13.37	12.00	5.89	20.84	7.47	18.25	91.70	132.94	113.66	54.18	211.69	78.75	147.08	7.00	13.69	12.00	5.94	21.45	7.75	19.00	972
0.32	34.78	55.96	45.47	15.38	96.55	40.58	60.44	7.00	13.17	12.00	5.64	20.71	7.54	18.00	128.94	194.96	170.27	81.70	308.21	113.26	224.75	7.00	13.75	12.00	5.73	21.77	8.02	20.00	1973


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/comparison_vals_auc.tex <==
name	auc
orig_pp	16.83
orig_ge	4.27
adv_pp	37.29
adv_ge	4.33


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.07	0.22	0.18	0.04	0.40	0.18	0.32	0.91	0.93	0.94	0.88	0.97	0.05	0.96	0.76	0.79	0.80	0.72	0.86	0.07	0.84	907
0.03	0.02	0.12	0.08	-0.02	0.26	0.14	0.18	0.83	0.87	0.88	0.79	0.95	0.08	0.92	0.66	0.71	0.72	0.62	0.80	0.09	0.77	982
0.06	-0.01	0.05	0.02	-0.05	0.15	0.10	0.08	0.72	0.78	0.82	0.64	0.92	0.14	0.87	0.55	0.61	0.64	0.49	0.74	0.13	0.70	1033
0.11	-0.03	0.01	-0.01	-0.07	0.09	0.08	0.03	0.63	0.71	0.75	0.53	0.88	0.17	0.82	0.47	0.54	0.57	0.39	0.68	0.15	0.64	1014
0.15	-0.05	-0.02	-0.02	-0.09	0.04	0.07	-0.01	0.53	0.63	0.68	0.43	0.82	0.20	0.77	0.38	0.46	0.50	0.31	0.62	0.16	0.57	966
0.18	-0.07	-0.05	-0.04	-0.11	0.02	0.07	-0.02	0.43	0.55	0.59	0.33	0.76	0.21	0.70	0.30	0.40	0.42	0.23	0.56	0.16	0.51	972
0.32	-0.12	-0.09	-0.07	-0.17	-0.01	0.08	-0.04	0.24	0.40	0.45	0.13	0.66	0.27	0.60	0.16	0.28	0.31	0.09	0.47	0.19	0.42	1973


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/correlations_auc.tex <==
name	auc
pcc	-0.00
spearman	0.19
kendall	0.14


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	8.97	13.57	12.42	7.07	20.07	6.50	16.40	7.55	13.56	11.70	5.60	21.52	7.96	18.17	5.28	11.76	8.89	2.82	20.70	8.94	15.52	907
0.03	6.41	8.80	8.19	5.08	12.51	3.72	10.20	5.21	8.84	7.57	3.54	14.14	5.30	10.96	3.91	8.78	6.02	0.96	16.59	7.81	10.76	982
0.06	4.86	6.24	5.92	3.92	8.56	2.32	7.22	3.91	6.06	5.39	2.73	9.39	3.33	7.28	2.76	6.12	4.22	0.02	12.23	6.10	6.64	1033
0.11	4.03	5.01	4.83	3.34	6.68	1.67	5.84	3.32	4.90	4.38	2.28	7.52	2.62	5.71	2.39	4.57	3.35	0.20	8.95	4.37	5.21	1014
0.15	3.32	4.08	4.01	2.87	5.29	1.21	4.71	2.90	3.88	3.57	2.22	5.54	1.66	4.40	2.12	3.48	2.67	-0.01	6.98	3.50	3.64	966
0.18	2.88	3.48	3.42	2.54	4.41	0.94	4.02	2.63	3.34	3.16	2.19	4.49	1.15	3.82	1.91	2.85	2.34	0.24	5.46	2.61	3.05	972
0.32	2.46	2.94	2.91	2.20	3.69	0.75	3.38	2.32	2.90	2.75	2.02	3.77	0.87	3.29	1.61	2.23	1.95	0.84	3.63	1.40	2.45	1973


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/ets_sts_auc.tex <==
name	auc
et_use	1.48
et_tse	1.44
et_ce	1.31


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.89	8.06	4.19	-11.07	27.20	19.14	6.40	7.77	12.63	10.98	5.70	19.57	6.94	15.96	6.76	13.07	10.82	4.05	22.10	9.03	16.62	907
0.03	1.62	3.43	2.13	-3.71	10.58	7.14	3.07	6.27	9.05	8.04	4.79	13.31	4.26	10.70	5.18	8.92	7.28	3.25	14.59	5.67	10.85	982
0.06	0.93	2.15	1.23	-3.36	7.66	5.51	1.73	5.28	7.24	6.34	3.60	10.88	3.64	8.09	4.34	7.11	5.54	1.54	12.68	5.57	8.01	1033
0.11	0.62	1.16	0.80	-3.22	5.55	4.38	1.06	4.52	5.99	5.35	3.22	8.76	2.77	6.62	3.71	5.78	4.61	0.50	11.07	5.29	6.31	1014
0.15	0.39	0.69	0.48	-0.57	1.94	1.26	0.63	3.87	4.86	4.41	2.88	6.85	1.99	5.27	3.18	4.41	3.76	1.60	7.23	2.81	4.69	966
0.18	0.27	0.54	0.34	-1.31	2.38	1.84	0.44	3.45	4.27	3.89	2.54	6.00	1.73	4.56	2.84	3.89	3.35	-0.22	8.00	4.11	4.05	972
0.32	0.15	0.29	0.21	-0.26	0.83	0.54	0.29	3.02	3.66	3.39	2.50	4.82	1.16	3.90	2.53	3.34	2.91	1.42	5.25	1.91	3.49	1973


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.39
et_p_h	1.70
et_p_l2	1.62


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.10	0.09	0.05	0.15	0.05	0.13	0.02	0.04	0.04	0.02	0.06	0.02	0.06	0.03	0.04	0.04	0.02	0.05	0.02	0.05	907
0.03	0.14	0.21	0.21	0.11	0.31	0.10	0.27	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.06	0.05	0.04	0.08	0.02	0.07	982
0.06	0.27	0.40	0.39	0.21	0.58	0.18	0.51	0.06	0.09	0.09	0.05	0.12	0.04	0.11	0.06	0.07	0.08	0.05	0.10	0.02	0.09	1033
0.11	0.47	0.64	0.62	0.37	0.91	0.27	0.79	0.08	0.11	0.11	0.07	0.15	0.04	0.13	0.08	0.09	0.09	0.07	0.12	0.03	0.11	1014
0.15	0.80	1.09	1.06	0.63	1.54	0.46	1.32	0.11	0.14	0.13	0.09	0.18	0.04	0.16	0.10	0.11	0.12	0.09	0.14	0.03	0.13	966
0.18	1.19	1.58	1.54	0.89	2.28	0.69	1.93	0.13	0.16	0.16	0.11	0.20	0.04	0.18	0.12	0.13	0.13	0.10	0.16	0.03	0.15	972
0.32	1.88	2.85	2.58	1.46	4.24	1.39	3.63	0.16	0.18	0.18	0.13	0.23	0.05	0.21	0.14	0.16	0.16	0.12	0.19	0.03	0.18	1973


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.42
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.99	0.02	0.98	0.95	0.96	0.97	0.93	0.99	0.03	0.98	0.93	0.94	0.96	0.89	1.00	0.05	0.98	907
0.03	0.93	0.94	0.95	0.92	0.97	0.02	0.96	0.92	0.93	0.94	0.89	0.97	0.04	0.96	0.88	0.91	0.93	0.85	0.98	0.07	0.96	982
0.06	0.90	0.91	0.92	0.88	0.95	0.03	0.93	0.88	0.90	0.91	0.85	0.95	0.05	0.94	0.83	0.87	0.89	0.79	0.95	0.08	0.93	1033
0.11	0.88	0.89	0.90	0.85	0.93	0.04	0.91	0.85	0.88	0.89	0.83	0.93	0.05	0.91	0.79	0.84	0.85	0.76	0.93	0.09	0.90	1014
0.15	0.85	0.86	0.87	0.81	0.91	0.05	0.89	0.82	0.85	0.86	0.80	0.90	0.05	0.88	0.76	0.80	0.81	0.70	0.90	0.10	0.86	966
0.18	0.82	0.84	0.85	0.79	0.89	0.05	0.87	0.80	0.83	0.83	0.77	0.88	0.05	0.86	0.73	0.77	0.78	0.66	0.87	0.10	0.83	972
0.32	0.78	0.80	0.81	0.75	0.86	0.06	0.84	0.77	0.80	0.80	0.74	0.85	0.06	0.84	0.67	0.71	0.72	0.60	0.82	0.11	0.78	1973


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	6.83	9.48	9.94	6.78	12.17	2.70	11.55	0.34	0.50	0.47	0.28	0.71	0.21	0.64	8.47	29.31	21.33	1.87	56.75	27.44	42.43	907
0.03	6.44	12.06	10.98	5.89	18.23	6.17	17.34	0.42	0.58	0.56	0.37	0.80	0.22	0.75	7.77	29.23	18.52	-0.34	58.79	29.56	42.22	982
0.06	5.52	13.65	11.42	4.66	22.63	8.98	21.58	0.46	0.62	0.60	0.41	0.83	0.21	0.79	6.67	26.53	15.27	-2.16	55.22	28.69	36.55	1033
0.11	6.94	16.05	13.67	4.69	27.40	11.35	23.02	0.48	0.64	0.62	0.43	0.85	0.21	0.79	6.51	26.97	16.45	-1.28	55.22	28.25	35.96	1014
0.15	7.07	11.12	10.47	5.42	16.83	5.71	14.10	0.44	0.61	0.57	0.40	0.83	0.21	0.77	6.40	25.42	15.27	-1.04	51.87	26.45	35.52	966
0.18	9.24	14.33	13.33	6.89	21.76	7.43	18.30	0.41	0.57	0.51	0.36	0.77	0.21	0.68	6.16	24.25	14.64	-0.86	49.35	25.11	32.90	972
0.32	17.78	32.07	28.76	12.25	51.90	19.82	41.64	0.36	0.49	0.44	0.30	0.68	0.19	0.56	5.76	22.97	13.96	-0.61	46.56	23.59	32.11	1973


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/time_misc_auc.tex <==
name	auc
attack_time	5.46
l2	0.18
lom	7.87


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.55	0.64	0.67	0.48	0.79	0.15	0.75	0.80	0.84	0.85	0.76	0.91	0.07	0.89	0.88	0.91	0.91	0.87	0.95	0.04	0.94	907
0.03	0.38	0.50	0.50	0.32	0.68	0.18	0.63	0.72	0.77	0.78	0.68	0.86	0.09	0.83	0.84	0.87	0.88	0.81	0.92	0.06	0.91	982
0.06	0.20	0.35	0.38	0.14	0.56	0.21	0.50	0.62	0.69	0.71	0.57	0.81	0.12	0.78	0.78	0.82	0.84	0.74	0.90	0.08	0.87	1033
0.11	0.09	0.27	0.25	0.07	0.47	0.20	0.43	0.56	0.63	0.65	0.48	0.77	0.14	0.73	0.75	0.79	0.81	0.70	0.87	0.09	0.85	1014
0.15	0.00	0.18	0.15	-0.00	0.37	0.18	0.32	0.50	0.57	0.60	0.41	0.72	0.16	0.68	0.70	0.75	0.77	0.65	0.85	0.10	0.82	966
0.18	0.00	0.13	0.06	-0.03	0.29	0.16	0.22	0.42	0.51	0.53	0.34	0.68	0.17	0.63	0.67	0.72	0.73	0.61	0.82	0.10	0.79	972
0.32	0.00	0.07	0.00	-0.06	0.20	0.13	0.11	0.30	0.42	0.44	0.24	0.60	0.18	0.56	0.59	0.66	0.68	0.54	0.78	0.12	0.74	1973


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/a/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.18
top50	0.23


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	32.84	44.20	41.34	28.19	60.20	16.01	51.10	15.00	18.99	19.00	13.11	24.87	5.88	23.00	36.20	48.49	45.63	31.36	65.63	17.14	56.25	15.00	18.91	19.00	13.07	24.76	5.84	23.00	913
0.03	33.88	47.30	43.49	26.96	67.63	20.34	54.40	10.00	15.68	15.00	8.83	22.53	6.85	20.00	41.29	56.55	52.24	33.40	79.70	23.15	64.53	10.00	15.64	15.00	8.77	22.51	6.87	20.00	993
0.06	34.35	53.30	44.77	18.34	88.27	34.97	58.40	7.00	13.87	13.00	6.44	21.30	7.43	19.00	49.47	72.57	62.74	29.98	115.16	42.59	78.47	8.00	14.01	13.00	6.40	21.62	7.61	19.00	1068
0.11	34.75	54.32	45.68	20.61	88.04	33.71	60.19	7.00	13.13	12.00	5.76	20.51	7.38	18.00	58.05	87.01	73.85	31.12	142.91	55.90	94.41	7.00	13.51	12.00	5.83	21.18	7.67	19.00	1050
0.15	35.20	55.51	45.05	9.59	101.42	45.91	58.40	7.00	13.43	12.00	6.01	20.85	7.42	19.00	75.08	110.75	95.30	26.69	194.80	84.06	119.99	7.00	14.08	13.00	6.16	22.00	7.92	20.00	1015
0.18	34.62	56.29	45.46	9.25	103.33	47.04	60.08	7.00	13.17	12.00	5.78	20.55	7.38	18.00	92.24	136.26	115.73	27.64	244.87	108.61	146.85	7.00	14.09	13.00	5.97	22.22	8.13	21.00	995
0.32	35.20	56.78	46.16	15.23	98.34	41.55	61.10	7.00	12.91	12.00	5.48	20.34	7.43	18.00	124.67	187.25	159.47	71.88	302.63	115.37	209.26	7.00	14.13	13.00	5.83	22.42	8.30	20.00	1835


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	16.93
orig_ge	4.23
adv_pp	37.21
adv_ge	4.44


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.24	0.03	0.02	-0.41	0.46	0.43	0.33	0.03	0.25	0.26	-0.06	0.56	0.31	0.47	0.02	0.19	0.18	-0.05	0.43	0.24	0.35	913
0.03	-0.33	-0.09	-0.10	-0.47	0.28	0.38	0.12	-0.05	0.14	0.12	-0.14	0.42	0.28	0.31	-0.03	0.11	0.08	-0.11	0.32	0.21	0.23	993
0.06	-0.45	-0.22	-0.23	-0.58	0.14	0.36	-0.03	-0.13	0.04	0.01	-0.24	0.31	0.27	0.20	-0.09	0.03	0.01	-0.17	0.24	0.20	0.15	1068
0.11	-0.54	-0.34	-0.35	-0.65	-0.02	0.31	-0.16	-0.24	-0.07	-0.08	-0.31	0.18	0.25	0.07	-0.16	-0.04	-0.05	-0.22	0.14	0.18	0.06	1050
0.15	-0.62	-0.46	-0.47	-0.71	-0.21	0.25	-0.30	-0.34	-0.19	-0.21	-0.41	0.04	0.22	-0.05	-0.23	-0.13	-0.14	-0.29	0.04	0.16	-0.03	1015
0.18	-0.70	-0.54	-0.56	-0.77	-0.30	0.23	-0.41	-0.41	-0.26	-0.29	-0.48	-0.04	0.22	-0.15	-0.29	-0.18	-0.20	-0.35	-0.02	0.16	-0.10	995
0.32	-0.74	-0.62	-0.64	-0.81	-0.43	0.19	-0.53	-0.50	-0.36	-0.39	-0.56	-0.17	0.20	-0.26	-0.36	-0.26	-0.28	-0.41	-0.11	0.15	-0.18	1835


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/correlations_auc.tex <==
name	auc
pcc	-0.13
spearman	-0.05
kendall	-0.03


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	10.32	18.00	15.57	6.70	29.29	11.29	23.75	8.88	19.07	15.25	4.72	33.43	14.35	25.28	5.61	15.24	10.80	1.21	29.27	14.03	19.41	913
0.03	7.71	11.82	10.41	5.19	18.44	6.63	14.41	6.44	12.62	10.51	3.71	21.52	8.90	15.70	4.61	11.44	7.92	0.94	21.94	10.50	14.41	993
0.06	5.91	8.72	8.05	4.40	13.04	4.32	10.59	5.17	9.05	7.77	3.02	15.08	6.03	11.03	3.91	8.92	6.54	0.74	17.11	8.18	10.74	1068
0.11	5.14	7.29	6.87	4.10	10.49	3.20	8.92	4.73	7.51	6.51	3.04	11.98	4.47	8.97	3.60	7.02	5.52	1.35	12.69	5.67	8.31	1050
0.15	4.54	5.96	5.69	3.87	8.06	2.09	7.05	4.28	6.09	5.55	3.22	8.96	2.87	7.21	3.23	5.58	4.48	0.91	10.25	4.67	6.36	1015
0.18	4.20	5.21	5.05	3.59	6.84	1.62	6.09	4.06	5.35	5.11	3.38	7.32	1.97	6.16	3.02	4.85	4.01	1.12	8.58	3.73	5.45	995
0.32	3.66	4.54	4.37	3.23	5.85	1.31	5.22	3.72	4.73	4.53	3.23	6.24	1.51	5.43	2.70	3.91	3.37	1.47	6.34	2.43	4.50	1835


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/ets_sts_auc.tex <==
name	auc
et_use	2.13
et_tse	2.21
et_ce	1.99


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.96	9.62	4.85	-13.26	32.50	22.88	7.98	7.98	15.02	12.81	4.73	25.30	10.29	19.32	6.85	15.43	11.63	2.10	28.77	13.33	19.61	913
0.03	1.85	4.49	2.73	-11.20	20.18	15.69	4.24	6.97	10.99	9.72	4.49	17.49	6.50	13.37	5.98	11.08	8.70	1.18	20.97	9.90	13.38	993
0.06	1.14	2.37	1.58	-4.68	9.41	7.05	2.25	5.99	8.77	8.09	4.50	13.05	4.28	10.61	5.07	8.59	7.22	2.01	15.18	6.58	10.36	1068
0.11	0.79	1.54	1.09	-3.10	6.18	4.64	1.50	5.69	7.68	7.11	4.15	11.22	3.54	8.83	4.68	7.32	6.12	1.77	12.88	5.55	8.20	1050
0.15	0.53	0.89	0.68	-0.65	2.43	1.54	0.89	5.30	6.68	6.23	4.11	9.25	2.57	7.47	4.36	6.16	5.39	2.22	10.11	3.94	6.92	1015
0.18	0.39	0.70	0.50	-1.92	3.31	2.61	0.65	4.99	6.07	5.77	4.20	7.95	1.88	6.77	4.13	5.55	4.97	2.46	8.64	3.09	6.16	995
0.32	0.25	0.52	0.34	-3.55	4.60	4.07	0.46	4.62	5.46	5.26	4.01	6.92	1.45	5.98	3.86	4.96	4.51	2.42	7.51	2.54	5.31	1835


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.50
et_p_h	2.26
et_p_l2	2.14


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.10	0.10	0.05	0.16	0.06	0.14	0.03	0.04	0.04	0.02	0.07	0.03	0.06	0.03	0.04	0.04	0.02	0.06	0.02	0.05	913
0.03	0.14	0.21	0.20	0.11	0.31	0.10	0.27	0.04	0.07	0.06	0.03	0.10	0.03	0.09	0.04	0.06	0.06	0.04	0.08	0.02	0.07	993
0.06	0.28	0.40	0.40	0.22	0.58	0.18	0.50	0.06	0.09	0.09	0.05	0.13	0.04	0.11	0.06	0.08	0.08	0.05	0.10	0.02	0.09	1068
0.11	0.46	0.64	0.63	0.36	0.92	0.28	0.80	0.09	0.11	0.11	0.07	0.16	0.04	0.14	0.08	0.10	0.10	0.07	0.12	0.03	0.11	1050
0.15	0.85	1.11	1.08	0.67	1.55	0.44	1.36	0.11	0.14	0.14	0.09	0.18	0.04	0.16	0.10	0.12	0.12	0.09	0.14	0.03	0.13	1015
0.18	1.19	1.59	1.55	0.97	2.21	0.62	1.93	0.13	0.16	0.16	0.11	0.20	0.05	0.18	0.12	0.13	0.14	0.10	0.16	0.03	0.15	995
0.32	1.79	2.60	2.37	1.37	3.83	1.23	3.19	0.15	0.18	0.18	0.13	0.23	0.05	0.21	0.14	0.15	0.16	0.13	0.18	0.03	0.17	1835


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.94	0.99	0.02	0.98	0.93	0.95	0.96	0.90	0.99	0.04	0.98	913
0.03	0.94	0.95	0.95	0.92	0.97	0.02	0.96	0.93	0.94	0.95	0.90	0.98	0.04	0.97	0.89	0.92	0.94	0.86	0.98	0.06	0.96	993
0.06	0.91	0.92	0.92	0.90	0.95	0.03	0.94	0.90	0.92	0.92	0.87	0.96	0.04	0.94	0.86	0.89	0.91	0.82	0.96	0.07	0.94	1068
0.11	0.88	0.90	0.90	0.86	0.93	0.04	0.92	0.87	0.89	0.90	0.84	0.94	0.05	0.92	0.82	0.86	0.88	0.78	0.94	0.08	0.92	1050
0.15	0.85	0.87	0.87	0.83	0.91	0.04	0.89	0.84	0.86	0.87	0.81	0.91	0.05	0.90	0.78	0.83	0.83	0.74	0.91	0.09	0.88	1015
0.18	0.82	0.84	0.85	0.80	0.89	0.04	0.87	0.82	0.84	0.85	0.79	0.89	0.05	0.88	0.75	0.80	0.81	0.70	0.89	0.10	0.86	995
0.32	0.78	0.81	0.81	0.76	0.86	0.05	0.84	0.79	0.81	0.82	0.76	0.87	0.05	0.85	0.70	0.75	0.76	0.65	0.85	0.10	0.82	1835


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.26


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	15.73	21.08	21.72	12.96	29.21	8.12	24.51	7.43	20.20	13.74	-9.64	50.05	29.85	21.75	6.49	20.28	14.90	1.62	38.94	18.66	29.26	913
0.03	6.66	14.25	11.75	-3.65	32.15	17.90	18.38	9.70	22.89	16.36	-11.95	57.74	34.84	24.09	5.33	18.03	12.51	0.24	35.82	17.79	24.40	993
0.06	14.13	31.85	24.65	3.94	59.76	27.91	42.90	12.88	31.40	19.53	-33.83	96.63	65.23	28.87	5.27	17.80	12.24	0.44	35.15	17.36	24.23	1068
0.11	9.32	17.46	14.11	4.22	30.69	13.23	21.33	13.46	28.08	19.69	-15.26	71.42	43.34	28.80	4.90	16.84	11.61	-0.41	34.09	17.25	22.69	1050
0.15	21.39	43.71	37.81	15.08	72.34	28.63	59.55	14.24	24.74	20.98	5.32	44.17	19.42	30.50	5.20	16.83	12.00	1.17	32.49	15.66	23.54	1015
0.18	19.78	27.16	24.83	14.54	39.79	12.63	32.42	15.32	25.58	21.97	6.95	44.21	18.63	30.57	5.43	16.92	12.55	1.02	32.81	15.90	23.58	995
0.32	27.35	37.82	35.89	23.13	52.51	14.69	46.26	16.20	27.22	22.82	-1.46	55.89	28.68	31.07	5.28	16.63	11.85	0.95	32.31	15.68	23.13	1835


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/time_misc_auc.tex <==
name	auc
attack_time	9.17
l2	8.23
lom	5.32


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.12	0.28	0.25	0.08	0.47	0.19	0.40	0.33	0.45	0.44	0.29	0.61	0.16	0.56	0.53	0.61	0.60	0.49	0.73	0.12	0.69	913
0.03	0.08	0.21	0.17	0.03	0.39	0.18	0.29	0.30	0.40	0.38	0.25	0.54	0.15	0.48	0.49	0.57	0.56	0.46	0.67	0.11	0.63	993
0.06	0.00	0.15	0.11	-0.01	0.32	0.16	0.23	0.25	0.35	0.33	0.21	0.49	0.14	0.43	0.46	0.53	0.53	0.43	0.64	0.11	0.60	1068
0.11	0.00	0.11	0.06	-0.04	0.25	0.14	0.17	0.21	0.30	0.29	0.17	0.43	0.13	0.38	0.43	0.50	0.49	0.40	0.60	0.10	0.56	1050
0.15	0.00	0.07	0.00	-0.05	0.19	0.12	0.11	0.17	0.25	0.24	0.13	0.37	0.12	0.31	0.40	0.46	0.45	0.36	0.55	0.10	0.51	1015
0.18	0.00	0.04	0.00	-0.04	0.13	0.09	0.06	0.14	0.22	0.20	0.10	0.33	0.11	0.28	0.37	0.43	0.42	0.34	0.52	0.09	0.49	995
0.32	0.00	0.03	0.00	-0.05	0.11	0.08	0.00	0.11	0.18	0.16	0.07	0.28	0.11	0.23	0.33	0.39	0.38	0.31	0.48	0.09	0.44	1835


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.08
top50	0.14


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	32.92	44.18	41.19	28.09	60.26	16.08	51.12	15.00	19.02	18.00	13.14	24.90	5.88	23.00	36.91	49.03	45.93	31.54	66.51	17.49	56.61	15.00	19.02	18.00	13.18	24.85	5.83	23.00	887
0.03	33.60	46.90	43.22	26.98	66.83	19.92	54.02	10.00	15.91	15.00	9.06	22.76	6.85	21.00	42.61	58.18	53.58	34.02	82.33	24.16	66.66	10.00	15.99	15.00	9.07	22.90	6.92	21.00	1031
0.06	33.60	50.42	43.08	18.71	82.14	31.72	55.71	9.00	15.19	15.00	7.71	22.67	7.48	21.00	50.28	72.74	62.22	29.53	115.94	43.21	80.78	9.00	15.25	15.00	7.72	22.78	7.53	21.00	1292
0.11	34.09	53.52	44.72	18.27	88.77	35.25	58.45	8.00	14.42	14.00	6.73	22.12	7.70	19.00	61.99	93.09	77.73	37.30	148.88	55.79	101.68	8.00	14.57	14.00	6.84	22.30	7.73	20.00	1208
0.15	35.75	56.11	46.05	14.95	97.27	41.16	61.54	7.00	12.93	12.00	5.59	20.27	7.34	18.00	82.19	121.22	101.89	48.37	194.06	72.85	136.49	7.00	13.18	12.00	5.70	20.67	7.48	18.00	930
0.18	35.63	57.88	46.95	9.03	106.73	48.85	62.19	7.00	12.24	11.00	5.11	19.37	7.13	17.00	102.23	155.49	128.25	42.28	268.70	113.21	169.88	7.00	12.57	11.00	5.16	19.98	7.41	18.00	858
0.32	35.76	57.85	47.41	18.46	97.25	39.40	63.79	6.00	11.68	10.00	4.74	18.62	6.94	16.00	145.19	223.78	190.88	100.36	347.20	123.42	257.66	6.00	12.18	11.00	4.92	19.44	7.26	17.00	1624


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/comparison_vals_auc.tex <==
name	auc
orig_pp	17.01
orig_ge	4.16
adv_pp	42.06
adv_ge	4.24


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.48	0.62	0.68	0.38	0.87	0.24	0.80	0.71	0.76	0.81	0.57	0.95	0.19	0.88	0.53	0.60	0.64	0.43	0.77	0.17	0.72	887
0.03	0.27	0.43	0.46	0.19	0.67	0.24	0.61	0.53	0.61	0.69	0.36	0.87	0.25	0.79	0.38	0.47	0.52	0.26	0.67	0.20	0.61	1031
0.06	0.05	0.24	0.23	0.01	0.47	0.23	0.40	0.20	0.42	0.49	0.12	0.72	0.30	0.66	0.14	0.31	0.35	0.09	0.54	0.23	0.48	1292
0.11	0.02	0.17	0.14	-0.03	0.37	0.20	0.29	0.18	0.36	0.40	0.09	0.63	0.27	0.57	0.12	0.27	0.29	0.07	0.47	0.20	0.42	1208
0.15	-0.01	0.09	0.07	-0.07	0.25	0.16	0.19	0.14	0.30	0.31	0.06	0.54	0.24	0.48	0.10	0.22	0.22	0.04	0.39	0.17	0.34	930
0.18	-0.08	0.02	0.00	-0.13	0.16	0.15	0.10	0.02	0.19	0.19	-0.05	0.43	0.24	0.37	0.02	0.14	0.13	-0.03	0.30	0.17	0.26	858
0.32	-0.19	-0.09	-0.09	-0.24	0.07	0.15	-0.00	-0.17	0.01	-0.00	-0.24	0.27	0.25	0.19	-0.11	0.01	0.00	-0.16	0.19	0.17	0.13	1624


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/correlations_auc.tex <==
name	auc
pcc	0.03
spearman	0.08
kendall	0.06


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.21	7.11	5.49	1.45	12.77	5.66	8.98	3.38	8.15	5.68	0.67	15.64	7.49	10.21	2.46	6.90	4.61	0.17	13.62	6.72	8.92	887
0.03	3.53	5.96	5.12	2.50	9.42	3.46	7.50	3.63	6.89	5.53	2.08	11.70	4.81	8.67	2.75	6.94	5.10	0.86	13.02	6.08	9.01	1031
0.06	3.50	5.26	4.80	2.62	7.90	2.64	6.62	3.45	5.85	5.12	2.36	9.33	3.48	7.36	2.81	6.20	4.62	1.03	11.36	5.16	7.84	1292
0.11	3.12	4.22	4.06	2.60	5.83	1.62	5.18	3.05	4.60	4.17	2.07	7.12	2.53	5.56	2.44	4.62	3.59	0.93	8.31	3.69	5.47	1208
0.15	2.83	3.54	3.47	2.42	4.67	1.12	4.24	2.73	3.74	3.48	2.20	5.29	1.55	4.45	2.02	3.57	2.81	0.64	6.49	2.92	4.16	930
0.18	2.62	3.27	3.12	2.29	4.25	0.98	3.87	2.62	3.49	3.23	2.16	4.81	1.33	4.05	1.97	3.22	2.60	0.50	5.94	2.72	3.60	858
0.32	2.41	2.93	2.87	2.15	3.72	0.79	3.42	2.46	3.16	2.96	2.09	4.22	1.07	3.64	1.76	2.63	2.25	0.77	4.49	1.86	2.94	1624


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/ets_sts_auc.tex <==
name	auc
et_use	1.23
et_tse	1.34
et_ce	1.28


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.86	2.68	1.47	-2.63	8.00	5.32	2.67	2.38	5.38	4.04	0.44	10.31	4.94	6.79	2.09	5.58	3.79	-0.84	12.00	6.42	6.87	887
0.03	0.77	1.55	1.11	-1.12	4.22	2.67	1.64	3.13	5.09	4.52	2.27	7.92	2.82	6.50	2.70	4.95	4.07	1.54	8.36	3.41	6.28	1031
0.06	0.58	1.01	0.83	-0.11	2.13	1.12	1.17	3.56	5.01	4.78	2.80	7.21	2.20	6.06	3.02	4.76	4.19	1.83	7.69	2.93	5.66	1292
0.11	0.42	0.70	0.55	-0.85	2.25	1.55	0.72	3.27	4.33	4.16	2.80	5.86	1.53	5.05	2.72	4.05	3.68	1.88	6.23	2.18	4.76	1208
0.15	0.29	0.46	0.37	-0.54	1.45	0.99	0.48	3.19	3.97	3.77	2.52	5.41	1.45	4.42	2.66	3.68	3.24	1.58	5.78	2.10	4.08	930
0.18	0.21	0.32	0.27	-0.01	0.65	0.33	0.36	3.02	3.74	3.58	2.58	4.90	1.16	4.21	2.49	3.44	3.06	1.70	5.18	1.74	3.80	858
0.32	0.13	0.22	0.18	0.03	0.40	0.19	0.25	2.93	3.54	3.34	2.33	4.75	1.21	3.90	2.45	3.30	2.89	0.68	5.93	2.62	3.50	1624


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.20
et_p_h	1.28
et_p_l2	1.21


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.11	0.11	0.06	0.17	0.06	0.15	0.03	0.05	0.04	0.02	0.07	0.03	0.06	0.03	0.04	0.04	0.03	0.06	0.02	0.05	887
0.03	0.18	0.25	0.24	0.15	0.35	0.10	0.31	0.05	0.07	0.07	0.04	0.10	0.03	0.09	0.05	0.06	0.06	0.04	0.08	0.02	0.07	1031
0.06	0.35	0.47	0.46	0.28	0.66	0.19	0.57	0.07	0.10	0.10	0.06	0.13	0.04	0.12	0.07	0.08	0.08	0.06	0.11	0.02	0.10	1292
0.11	0.60	0.79	0.76	0.48	1.11	0.31	0.95	0.09	0.12	0.12	0.08	0.16	0.04	0.14	0.09	0.10	0.10	0.08	0.13	0.03	0.12	1208
0.15	0.96	1.28	1.24	0.79	1.76	0.48	1.53	0.11	0.14	0.14	0.10	0.18	0.04	0.17	0.11	0.12	0.12	0.09	0.15	0.03	0.14	930
0.18	1.37	1.88	1.78	1.11	2.65	0.77	2.25	0.13	0.16	0.16	0.11	0.21	0.05	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.16	858
0.32	2.14	3.28	2.96	1.64	4.92	1.64	4.01	0.16	0.19	0.19	0.14	0.24	0.05	0.22	0.14	0.16	0.16	0.13	0.19	0.03	0.18	1624


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.49
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.99	0.02	0.98	0.97	0.97	0.97	0.95	0.99	0.02	0.98	0.95	0.96	0.97	0.91	1.00	0.04	0.98	887
0.03	0.94	0.95	0.95	0.93	0.97	0.02	0.96	0.94	0.95	0.95	0.92	0.98	0.03	0.97	0.91	0.93	0.95	0.88	0.99	0.05	0.97	1031
0.06	0.91	0.92	0.92	0.89	0.95	0.03	0.94	0.90	0.92	0.93	0.88	0.96	0.04	0.94	0.87	0.90	0.92	0.83	0.97	0.07	0.95	1292
0.11	0.88	0.89	0.90	0.86	0.93	0.03	0.91	0.87	0.89	0.90	0.85	0.94	0.04	0.92	0.83	0.87	0.88	0.79	0.95	0.08	0.92	1208
0.15	0.84	0.86	0.87	0.82	0.90	0.04	0.89	0.84	0.86	0.87	0.82	0.91	0.05	0.90	0.78	0.83	0.84	0.73	0.92	0.09	0.89	930
0.18	0.82	0.84	0.84	0.80	0.88	0.04	0.87	0.82	0.84	0.85	0.80	0.89	0.05	0.88	0.75	0.80	0.81	0.71	0.90	0.09	0.86	858
0.32	0.78	0.80	0.81	0.76	0.85	0.05	0.84	0.79	0.81	0.82	0.76	0.87	0.05	0.85	0.70	0.75	0.76	0.64	0.85	0.10	0.82	1624


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.26


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	7.68	11.63	10.96	-1.86	25.13	13.50	12.20	17.10	357.23	71.61	-1114.34	1828.80	1471.57	232.40	3.37	10.42	7.36	-0.27	21.10	10.69	13.82	887
0.03	7.05	20.50	12.36	-11.49	52.49	31.99	18.87	31.68	1024.46	152.31	-3465.31	5514.22	4489.76	433.92	3.50	13.10	8.50	-0.65	26.86	13.76	18.13	1031
0.06	9.30	33.39	21.24	-5.08	71.87	38.47	39.74	74.58	3315.97	329.53	-10196.24	16828.18	13512.21	1185.37	4.24	17.24	10.79	0.86	33.61	16.38	28.33	1292
0.11	9.35	27.11	16.12	2.00	52.22	25.11	39.81	96.59	3502.61	346.28	-15223.49	22228.71	18726.10	1079.77	4.14	16.81	10.54	1.04	32.57	15.77	26.74	1208
0.15	9.42	22.26	16.67	4.58	39.93	17.68	31.28	85.53	1918.21	283.43	-4784.36	8620.77	6702.57	690.54	4.14	14.60	9.43	0.74	28.46	13.86	21.37	930
0.18	14.73	29.21	25.97	10.56	47.87	18.66	38.81	98.72	1243.10	273.63	-5795.26	8281.46	7038.36	691.62	3.71	12.82	8.23	-0.06	25.71	12.89	17.25	858
0.32	17.97	33.72	28.99	13.07	54.36	20.65	44.75	97.77	818.83	279.58	-3759.01	5396.67	4577.84	652.68	3.41	12.20	8.32	0.21	24.19	11.99	16.59	1624


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/time_misc_auc.tex <==
name	auc
attack_time	8.76
l2	549.16
lom	4.34


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.40	0.53	0.55	0.32	0.73	0.21	0.68	0.65	0.71	0.73	0.57	0.85	0.14	0.80	0.77	0.80	0.82	0.71	0.90	0.09	0.87	887
0.03	0.20	0.37	0.36	0.16	0.57	0.20	0.50	0.53	0.61	0.63	0.45	0.76	0.16	0.72	0.68	0.74	0.76	0.62	0.85	0.11	0.82	1031
0.06	0.06	0.21	0.18	0.03	0.39	0.18	0.33	0.35	0.48	0.50	0.31	0.66	0.17	0.61	0.56	0.66	0.67	0.53	0.79	0.13	0.76	1292
0.11	0.00	0.16	0.12	0.00	0.32	0.16	0.25	0.33	0.45	0.44	0.29	0.60	0.15	0.56	0.56	0.64	0.65	0.52	0.75	0.12	0.72	1208
0.15	0.00	0.12	0.07	-0.03	0.26	0.15	0.20	0.31	0.41	0.40	0.27	0.54	0.14	0.50	0.54	0.61	0.62	0.50	0.71	0.10	0.68	930
0.18	0.00	0.08	0.00	-0.04	0.20	0.12	0.12	0.25	0.35	0.33	0.21	0.48	0.14	0.44	0.50	0.57	0.57	0.47	0.67	0.10	0.64	858
0.32	0.00	0.04	0.00	-0.05	0.14	0.10	0.06	0.18	0.27	0.26	0.14	0.40	0.13	0.35	0.43	0.51	0.50	0.40	0.61	0.11	0.57	1624


==> data/mlm_plots/mlm_distil_fast/yelp/roberta/s/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.12
top50	0.19


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	33.32	44.55	41.41	28.18	60.92	16.37	51.23	14.00	18.04	18.00	12.83	23.26	5.22	22.00	36.62	48.42	45.28	31.07	65.77	17.35	55.74	14.00	17.93	18.00	12.74	23.12	5.19	22.00	900
0.03	33.90	47.27	42.84	26.49	68.06	20.78	54.43	10.00	15.04	15.00	8.90	21.18	6.14	19.00	41.84	57.23	52.93	33.20	81.26	24.03	66.33	10.00	14.59	14.00	8.82	20.35	5.76	18.00	994
0.06	34.72	52.09	44.59	21.06	83.11	31.03	58.28	8.00	13.33	12.00	6.55	20.12	6.79	18.00	48.55	71.63	62.13	33.21	110.05	38.42	80.21	7.00	12.60	12.00	6.31	18.88	6.29	17.00	1075
0.11	34.85	53.25	45.24	23.03	83.47	30.22	60.14	7.00	13.11	12.00	6.23	19.99	6.88	18.00	59.33	84.77	74.72	43.24	126.29	41.52	96.25	7.00	12.16	11.00	5.90	18.42	6.26	16.00	1027
0.15	35.35	53.84	44.63	16.34	91.34	37.50	58.81	7.00	13.02	12.00	6.19	19.86	6.84	18.00	76.44	109.72	94.06	11.42	208.02	98.30	121.78	7.00	12.08	11.00	5.71	18.45	6.37	16.00	992
0.18	35.06	55.33	45.47	14.78	95.87	40.54	60.34	7.00	12.55	12.00	5.86	19.24	6.69	17.00	93.34	134.96	117.94	52.39	217.54	82.58	152.33	6.00	11.66	11.00	5.37	17.95	6.29	16.00	959
0.32	35.22	56.09	46.12	13.09	99.10	43.01	61.29	7.00	12.50	12.00	5.61	19.39	6.89	17.00	133.38	196.33	172.13	83.93	308.72	112.40	226.69	7.00	12.43	12.00	5.76	19.10	6.67	17.00	1916


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/comparison_vals_auc.tex <==
name	auc
orig_pp	16.64
orig_ge	4.09
adv_pp	37.55
adv_ge	3.88


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.13	0.30	0.27	0.07	0.53	0.23	0.44	0.68	0.76	0.83	0.54	0.98	0.22	0.91	0.50	0.61	0.65	0.40	0.81	0.20	0.76	900
0.03	0.09	0.36	0.30	0.05	0.67	0.31	0.61	0.69	0.76	0.81	0.56	0.95	0.20	0.89	0.52	0.61	0.64	0.43	0.78	0.18	0.73	994
0.06	-0.00	0.20	0.12	-0.08	0.48	0.28	0.35	0.45	0.59	0.66	0.30	0.87	0.28	0.80	0.32	0.45	0.49	0.22	0.68	0.23	0.62	1075
0.11	-0.04	0.12	0.04	-0.15	0.38	0.26	0.21	0.32	0.48	0.55	0.18	0.79	0.31	0.71	0.22	0.36	0.40	0.13	0.60	0.23	0.53	1027
0.15	-0.11	0.03	-0.03	-0.22	0.28	0.25	0.08	0.15	0.35	0.38	0.02	0.67	0.32	0.60	0.11	0.26	0.27	0.02	0.50	0.24	0.43	992
0.18	-0.16	-0.03	-0.08	-0.28	0.21	0.24	0.02	-0.00	0.23	0.26	-0.11	0.57	0.34	0.49	0.00	0.17	0.17	-0.08	0.41	0.25	0.34	959
0.32	-0.18	-0.03	-0.08	-0.31	0.25	0.28	0.03	-0.08	0.18	0.20	-0.18	0.54	0.36	0.45	-0.05	0.13	0.14	-0.13	0.39	0.26	0.32	1916


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/correlations_auc.tex <==
name	auc
pcc	0.02
spearman	0.12
kendall	0.09


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	7.68	12.97	11.25	5.10	20.83	7.86	16.53	5.75	12.94	10.83	3.56	22.32	9.38	17.56	4.20	10.47	7.78	1.43	19.52	9.05	13.05	900
0.03	3.62	6.32	5.99	2.34	10.31	3.98	8.17	2.79	6.23	5.01	0.96	11.49	5.26	8.22	2.26	5.91	3.96	-0.72	12.55	6.64	6.82	994
0.06	3.55	5.06	4.98	2.58	7.55	2.48	6.42	2.58	4.61	3.86	1.56	7.66	3.05	5.91	2.10	4.87	3.36	-0.40	10.13	5.26	5.71	1075
0.11	3.18	4.30	4.35	2.45	6.15	1.85	5.28	2.42	3.77	3.32	1.63	5.91	2.14	4.62	2.01	3.87	2.76	-0.43	8.16	4.29	4.03	1027
0.15	2.92	3.65	3.72	2.37	4.92	1.27	4.38	2.35	3.23	3.04	1.82	4.64	1.41	3.92	1.88	3.07	2.45	0.09	6.04	2.98	3.22	992
0.18	2.78	3.31	3.38	2.29	4.34	1.03	3.93	2.31	2.97	2.84	1.86	4.08	1.11	3.51	1.81	2.72	2.27	0.60	4.84	2.12	2.95	959
0.32	2.27	2.74	2.81	1.83	3.66	0.92	3.30	2.14	2.70	2.67	1.66	3.75	1.04	3.21	1.58	2.24	2.01	0.80	3.69	1.44	2.58	1916


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/ets_sts_auc.tex <==
name	auc
et_use	1.29
et_tse	1.20
et_ce	1.12


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.53	8.90	4.10	-8.91	26.72	17.82	7.41	6.70	12.23	10.75	4.71	19.75	7.52	16.08	5.81	12.14	9.81	3.23	21.05	8.91	16.15	900
0.03	0.85	2.51	1.45	-4.71	9.73	7.22	2.36	3.44	6.30	5.88	2.16	10.44	4.14	8.32	2.89	6.20	5.07	1.09	11.31	5.11	7.82	994
0.06	0.71	1.58	1.03	-3.05	6.21	4.63	1.53	4.10	6.03	5.62	2.64	9.42	3.39	7.43	3.33	5.93	4.83	1.28	10.59	4.65	7.23	1075
0.11	0.50	1.06	0.72	-1.41	3.53	2.47	1.01	3.84	5.38	5.06	2.39	8.37	2.99	6.32	3.18	5.20	4.34	1.22	9.17	3.98	6.14	1027
0.15	0.33	0.60	0.46	-0.31	1.51	0.91	0.63	3.60	4.58	4.41	2.57	6.59	2.01	5.30	2.90	4.24	3.79	1.55	6.92	2.68	4.87	992
0.18	0.25	0.48	0.33	-1.42	2.38	1.90	0.46	3.39	4.27	4.10	2.44	6.11	1.83	4.90	2.83	3.96	3.52	1.37	6.54	2.58	4.42	959
0.32	0.13	0.27	0.19	-0.67	1.20	0.94	0.27	2.84	3.55	3.42	1.93	5.17	1.62	4.15	2.40	3.33	2.97	0.51	6.15	2.82	3.72	1916


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.34
et_p_h	1.54
et_p_l2	1.47


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.09	0.09	0.03	0.15	0.06	0.13	0.02	0.04	0.03	0.02	0.06	0.02	0.05	0.02	0.04	0.03	0.02	0.05	0.02	0.05	900
0.03	0.15	0.22	0.22	0.11	0.33	0.11	0.29	0.04	0.07	0.06	0.04	0.10	0.03	0.09	0.04	0.06	0.06	0.04	0.08	0.02	0.07	994
0.06	0.27	0.41	0.40	0.22	0.61	0.19	0.53	0.06	0.09	0.09	0.05	0.13	0.04	0.11	0.06	0.08	0.07	0.05	0.10	0.02	0.09	1075
0.11	0.47	0.66	0.63	0.36	0.97	0.31	0.82	0.08	0.11	0.11	0.07	0.15	0.04	0.13	0.07	0.09	0.09	0.07	0.12	0.03	0.11	1027
0.15	0.79	1.13	1.09	0.62	1.64	0.51	1.40	0.11	0.13	0.13	0.09	0.18	0.04	0.16	0.10	0.11	0.11	0.09	0.14	0.03	0.13	992
0.18	1.17	1.63	1.59	0.93	2.33	0.70	2.00	0.12	0.15	0.15	0.10	0.20	0.05	0.18	0.11	0.13	0.13	0.10	0.16	0.03	0.15	959
0.32	1.92	2.88	2.64	1.47	4.28	1.40	3.61	0.15	0.18	0.18	0.13	0.23	0.05	0.21	0.13	0.15	0.16	0.12	0.19	0.03	0.18	1916


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.43
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.95	0.96	0.97	0.92	0.99	0.04	0.98	0.93	0.94	0.96	0.89	0.99	0.05	0.97	900
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.96	0.91	0.93	0.94	0.89	0.97	0.04	0.96	0.88	0.91	0.93	0.85	0.97	0.06	0.96	994
0.06	0.90	0.91	0.92	0.88	0.94	0.03	0.93	0.86	0.89	0.90	0.84	0.94	0.05	0.93	0.83	0.87	0.88	0.80	0.95	0.08	0.93	1075
0.11	0.88	0.89	0.89	0.85	0.92	0.04	0.91	0.83	0.86	0.87	0.81	0.92	0.05	0.90	0.79	0.84	0.84	0.75	0.92	0.09	0.90	1027
0.15	0.85	0.86	0.87	0.82	0.90	0.04	0.88	0.80	0.84	0.84	0.78	0.89	0.05	0.87	0.75	0.80	0.80	0.71	0.89	0.09	0.86	992
0.18	0.82	0.84	0.84	0.80	0.88	0.04	0.86	0.78	0.81	0.82	0.76	0.87	0.05	0.85	0.72	0.77	0.77	0.68	0.86	0.09	0.83	959
0.32	0.78	0.80	0.81	0.76	0.85	0.04	0.84	0.77	0.80	0.80	0.75	0.85	0.05	0.83	0.68	0.74	0.74	0.64	0.83	0.09	0.80	1916


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	12.32	15.95	15.94	11.08	20.82	4.87	18.93	0.15	0.25	0.22	0.10	0.40	0.15	0.32	10.71	30.72	24.23	5.67	55.76	25.04	46.12	900
0.03	4.44	6.64	5.43	-0.35	13.63	6.99	6.90	0.12	0.23	0.19	0.08	0.37	0.14	0.29	4.81	23.55	14.44	-1.62	48.72	25.17	34.19	994
0.06	6.37	14.90	11.29	1.78	28.01	13.11	18.93	0.16	0.26	0.22	0.11	0.42	0.15	0.33	5.18	23.67	14.44	-1.15	48.49	24.82	34.18	1075
0.11	8.26	19.64	15.20	3.84	35.44	15.80	26.35	0.17	0.28	0.24	0.12	0.44	0.16	0.35	6.04	24.55	14.94	-0.64	49.74	25.19	34.89	1027
0.15	11.26	25.07	20.54	7.80	42.35	17.28	35.61	0.18	0.28	0.24	0.12	0.44	0.16	0.33	5.95	25.94	17.43	0.58	51.31	25.37	38.29	992
0.18	13.34	29.25	24.28	9.71	48.80	19.54	43.41	0.18	0.27	0.23	0.12	0.43	0.16	0.32	6.10	25.21	15.83	0.64	49.77	24.57	38.21	959
0.32	17.04	23.41	22.14	13.95	32.88	9.46	27.72	0.17	0.26	0.23	0.12	0.39	0.13	0.30	6.02	22.88	15.26	0.20	45.56	22.68	32.88	1916


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/time_misc_auc.tex <==
name	auc
attack_time	6.84
l2	0.08
lom	7.63


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.27	0.44	0.45	0.21	0.67	0.23	0.61	0.58	0.69	0.72	0.52	0.85	0.17	0.81	0.75	0.81	0.84	0.70	0.92	0.11	0.89	900
0.03	0.25	0.42	0.41	0.18	0.66	0.24	0.60	0.60	0.69	0.70	0.53	0.84	0.15	0.79	0.77	0.81	0.83	0.72	0.91	0.10	0.88	994
0.06	0.06	0.27	0.25	0.03	0.50	0.24	0.43	0.44	0.56	0.58	0.38	0.75	0.18	0.70	0.67	0.74	0.76	0.61	0.86	0.13	0.83	1075
0.11	0.00	0.18	0.12	-0.03	0.40	0.21	0.29	0.38	0.50	0.50	0.31	0.69	0.19	0.64	0.62	0.69	0.71	0.56	0.83	0.13	0.79	1027
0.15	0.00	0.14	0.00	-0.06	0.34	0.20	0.22	0.28	0.42	0.41	0.23	0.61	0.19	0.56	0.56	0.64	0.65	0.50	0.77	0.14	0.73	992
0.18	0.00	0.10	0.00	-0.08	0.27	0.17	0.13	0.21	0.35	0.33	0.16	0.54	0.19	0.49	0.50	0.59	0.60	0.45	0.73	0.14	0.69	959
0.32	0.00	0.10	0.00	-0.08	0.29	0.18	0.14	0.17	0.33	0.32	0.13	0.53	0.20	0.46	0.47	0.57	0.57	0.42	0.72	0.15	0.67	1916


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/a/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.14
top50	0.20


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	33.92	44.72	41.57	28.62	60.83	16.11	51.43	14.00	17.97	18.00	12.67	23.27	5.30	22.00	36.77	48.74	45.23	31.42	66.07	17.33	56.27	14.00	17.84	18.00	12.58	23.11	5.26	21.00	947
0.03	34.21	48.21	43.60	24.82	71.61	23.39	54.85	10.00	14.72	14.00	8.52	20.91	6.19	19.00	41.22	57.28	51.92	31.91	82.65	25.37	65.43	10.00	14.53	14.00	8.41	20.65	6.12	19.00	1020
0.06	35.33	53.41	45.12	20.95	85.87	32.46	59.60	7.00	12.90	12.00	6.26	19.55	6.64	18.00	48.93	72.78	62.71	28.25	117.30	44.53	82.28	7.00	12.70	12.00	6.13	19.26	6.56	17.00	1125
0.11	35.23	53.87	45.40	21.56	86.17	32.31	59.77	7.00	12.79	12.00	6.11	19.48	6.68	18.00	58.20	85.34	72.45	38.28	132.40	47.06	95.23	7.00	12.55	12.00	5.96	19.13	6.58	17.00	1034
0.15	35.34	55.45	46.17	15.83	95.06	39.61	60.44	7.00	12.73	12.00	5.89	19.58	6.85	18.00	74.62	107.14	92.91	47.00	167.27	60.14	119.46	7.00	12.63	12.00	5.64	19.63	6.99	18.00	946
0.18	34.71	55.68	44.70	9.73	101.63	45.95	59.39	7.00	13.08	12.00	6.33	19.83	6.75	18.00	90.56	129.76	112.40	42.66	216.86	87.10	139.61	7.00	13.02	12.00	6.19	19.84	6.83	18.00	934
0.32	35.33	55.41	46.14	15.54	95.29	39.87	60.85	7.00	12.62	12.00	5.75	19.49	6.87	18.00	130.49	187.24	164.59	91.47	283.01	95.77	217.36	7.00	12.66	12.00	5.53	19.80	7.14	18.00	1827


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	16.79
orig_ge	4.09
adv_pp	36.47
adv_ge	4.06


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.22	0.08	0.07	-0.32	0.48	0.40	0.35	-0.02	0.25	0.28	-0.12	0.62	0.37	0.54	-0.01	0.20	0.20	-0.09	0.48	0.28	0.41	947
0.03	-0.37	-0.07	-0.11	-0.46	0.33	0.39	0.16	-0.14	0.13	0.14	-0.22	0.47	0.35	0.38	-0.09	0.10	0.10	-0.16	0.36	0.26	0.28	1020
0.06	-0.47	-0.17	-0.25	-0.57	0.22	0.40	0.02	-0.24	-0.00	-0.03	-0.34	0.34	0.34	0.19	-0.17	0.01	-0.02	-0.25	0.26	0.25	0.14	1125
0.11	-0.57	-0.27	-0.39	-0.68	0.14	0.41	-0.12	-0.35	-0.11	-0.17	-0.44	0.23	0.34	0.05	-0.24	-0.07	-0.12	-0.32	0.18	0.25	0.04	1034
0.15	-0.66	-0.43	-0.52	-0.78	-0.09	0.35	-0.35	-0.45	-0.27	-0.32	-0.56	0.03	0.30	-0.17	-0.32	-0.19	-0.22	-0.41	0.03	0.22	-0.11	946
0.18	-0.73	-0.57	-0.63	-0.84	-0.30	0.27	-0.52	-0.55	-0.41	-0.44	-0.64	-0.17	0.24	-0.33	-0.40	-0.29	-0.31	-0.47	-0.12	0.17	-0.23	934
0.32	-0.80	-0.69	-0.73	-0.90	-0.48	0.21	-0.64	-0.67	-0.55	-0.58	-0.74	-0.35	0.20	-0.48	-0.49	-0.40	-0.42	-0.55	-0.25	0.15	-0.34	1827


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/correlations_auc.tex <==
name	auc
pcc	-0.13
spearman	-0.08
kendall	-0.06


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	8.86	15.51	13.38	5.63	25.39	9.88	20.11	6.88	15.45	12.58	3.76	27.13	11.69	20.68	4.52	12.20	8.52	0.81	23.59	11.39	15.92	947
0.03	6.80	10.72	9.66	4.40	17.04	6.32	13.44	5.52	10.72	8.59	2.84	18.60	7.88	14.00	3.89	9.14	6.71	0.70	17.58	8.44	11.03	1020
0.06	5.08	7.52	7.21	3.83	11.21	3.69	9.56	4.18	7.29	6.30	2.67	11.91	4.62	9.27	3.24	6.73	4.90	0.40	13.06	6.33	7.90	1125
0.11	4.37	6.23	6.24	3.40	9.05	2.83	7.95	3.68	5.89	5.37	2.34	9.45	3.55	7.26	2.86	5.63	4.19	-0.27	11.54	5.91	6.19	1034
0.15	4.19	5.45	5.55	3.45	7.44	2.00	6.76	3.47	4.94	4.56	2.70	7.18	2.24	5.96	2.77	4.29	3.71	1.21	7.37	3.08	4.97	946
0.18	4.14	5.17	5.27	3.53	6.81	1.64	6.20	3.52	4.66	4.38	2.84	6.49	1.83	5.56	2.77	3.87	3.49	1.81	5.93	2.06	4.47	934
0.32	3.69	4.49	4.48	3.29	5.69	1.20	5.30	3.41	4.28	4.06	2.95	5.60	1.32	4.93	2.46	3.41	3.07	1.43	5.39	1.98	3.88	1827


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/ets_sts_auc.tex <==
name	auc
et_use	1.95
et_tse	1.85
et_ce	1.59


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	3.12	12.29	4.99	-19.89	44.47	32.18	8.95	7.83	14.51	12.49	4.43	24.59	10.08	18.82	6.83	14.77	11.16	1.85	27.69	12.92	18.90	947
0.03	1.80	5.24	2.77	-10.86	21.34	16.10	4.23	7.22	11.37	10.05	3.46	19.29	7.92	13.99	5.94	11.25	8.86	1.31	21.19	9.94	13.80	1020
0.06	1.09	2.32	1.61	-2.11	6.74	4.43	2.30	6.24	9.20	8.40	3.80	14.60	5.40	10.93	5.14	9.04	7.30	1.16	16.93	7.88	10.37	1125
0.11	0.77	1.47	1.09	-2.21	5.16	3.68	1.50	5.74	7.63	7.42	3.65	11.61	3.98	9.20	4.63	7.21	6.34	2.26	12.17	4.96	8.36	1034
0.15	0.54	1.24	0.72	-3.66	6.14	4.90	0.96	5.59	7.07	6.82	3.85	10.28	3.22	8.26	4.55	6.62	5.82	2.31	10.94	4.32	7.43	946
0.18	0.42	0.96	0.54	-3.38	5.29	4.33	0.70	5.56	6.75	6.39	3.47	10.02	3.28	7.46	4.56	6.31	5.54	1.61	11.02	4.70	6.86	934
0.32	0.24	0.43	0.33	-0.36	1.22	0.79	0.46	4.94	5.84	5.61	4.12	7.56	1.72	6.44	4.09	5.31	4.86	2.54	8.08	2.77	5.77	1827


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.57
et_p_h	2.37
et_p_l2	2.26


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.09	0.09	0.04	0.15	0.06	0.13	0.02	0.04	0.04	0.02	0.07	0.02	0.06	0.03	0.04	0.04	0.02	0.05	0.02	0.05	947
0.03	0.13	0.20	0.19	0.10	0.31	0.10	0.27	0.04	0.06	0.06	0.03	0.09	0.03	0.09	0.04	0.06	0.06	0.03	0.08	0.02	0.07	1020
0.06	0.27	0.39	0.37	0.21	0.58	0.18	0.50	0.06	0.09	0.08	0.05	0.12	0.04	0.11	0.06	0.07	0.07	0.05	0.10	0.02	0.09	1125
0.11	0.44	0.64	0.61	0.32	0.96	0.32	0.79	0.08	0.11	0.11	0.07	0.15	0.04	0.13	0.08	0.09	0.09	0.07	0.12	0.03	0.11	1034
0.15	0.77	1.06	1.05	0.62	1.50	0.44	1.31	0.10	0.13	0.13	0.08	0.17	0.04	0.15	0.09	0.11	0.11	0.08	0.14	0.03	0.13	946
0.18	1.15	1.53	1.49	0.84	2.22	0.69	1.88	0.12	0.15	0.15	0.10	0.19	0.04	0.17	0.11	0.13	0.13	0.10	0.15	0.03	0.14	934
0.32	1.82	2.75	2.53	1.42	4.08	1.33	3.43	0.15	0.18	0.18	0.13	0.22	0.05	0.21	0.13	0.15	0.15	0.12	0.18	0.03	0.17	1827


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.95	0.96	0.97	0.93	0.99	0.03	0.98	0.92	0.94	0.95	0.89	0.99	0.05	0.97	947
0.03	0.93	0.94	0.94	0.92	0.97	0.03	0.96	0.92	0.93	0.94	0.89	0.98	0.04	0.96	0.88	0.91	0.92	0.84	0.98	0.07	0.95	1020
0.06	0.90	0.91	0.92	0.88	0.95	0.03	0.93	0.88	0.90	0.91	0.85	0.95	0.05	0.94	0.83	0.87	0.88	0.79	0.95	0.08	0.93	1125
0.11	0.87	0.89	0.89	0.85	0.92	0.04	0.91	0.85	0.87	0.88	0.82	0.93	0.05	0.91	0.80	0.84	0.85	0.76	0.92	0.08	0.90	1034
0.15	0.84	0.86	0.87	0.82	0.90	0.04	0.88	0.81	0.84	0.84	0.78	0.89	0.05	0.88	0.75	0.79	0.80	0.70	0.89	0.10	0.85	946
0.18	0.82	0.84	0.85	0.79	0.89	0.05	0.87	0.78	0.81	0.82	0.76	0.87	0.06	0.85	0.72	0.76	0.77	0.65	0.86	0.10	0.82	934
0.32	0.78	0.80	0.81	0.75	0.85	0.05	0.84	0.75	0.79	0.79	0.73	0.84	0.05	0.83	0.66	0.71	0.73	0.60	0.82	0.11	0.78	1827


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	10.89	14.25	14.08	7.32	21.19	6.94	15.96	1.47	3.01	2.46	0.54	5.49	2.48	3.86	1.56	4.71	3.37	0.22	9.20	4.49	6.41	947
0.03	9.31	17.01	15.46	5.90	28.12	11.11	22.17	1.96	3.71	3.04	1.05	6.36	2.65	4.64	1.49	4.58	3.31	0.15	9.01	4.43	6.22	1020
0.06	9.97	23.03	19.76	5.57	40.49	17.46	32.22	2.28	4.35	3.52	0.55	8.15	3.80	5.41	1.38	4.21	3.04	0.01	8.40	4.19	5.70	1125
0.11	14.81	26.05	22.03	6.65	45.45	19.40	33.03	2.44	4.54	3.76	1.45	7.64	3.10	5.74	1.41	4.41	3.16	0.26	8.56	4.15	6.14	1034
0.15	20.49	32.67	29.93	14.16	51.19	18.51	40.82	2.79	4.84	4.10	1.58	8.11	3.27	6.05	1.57	4.64	3.37	0.17	9.10	4.46	6.21	946
0.18	28.19	43.81	38.88	17.49	70.12	26.31	54.43	2.96	5.05	4.46	2.02	8.07	3.03	6.39	1.66	4.87	3.71	0.52	9.22	4.35	6.85	934
0.32	43.30	78.51	65.83	27.11	129.92	51.41	103.24	3.10	5.22	4.65	2.04	8.39	3.17	6.65	1.63	4.80	3.56	0.35	9.25	4.45	6.64	1827


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/time_misc_auc.tex <==
name	auc
attack_time	12.94
l2	1.47
lom	1.44


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.13	0.31	0.29	0.10	0.52	0.21	0.45	0.31	0.46	0.47	0.27	0.65	0.19	0.60	0.50	0.61	0.61	0.46	0.75	0.15	0.71	947
0.03	0.07	0.22	0.18	0.03	0.41	0.19	0.33	0.27	0.40	0.39	0.23	0.58	0.17	0.52	0.47	0.57	0.56	0.43	0.70	0.14	0.66	1020
0.06	0.00	0.15	0.10	-0.03	0.34	0.19	0.22	0.22	0.34	0.32	0.18	0.51	0.17	0.44	0.43	0.52	0.51	0.39	0.65	0.13	0.60	1125
0.11	0.00	0.12	0.00	-0.06	0.30	0.18	0.17	0.18	0.29	0.26	0.13	0.45	0.16	0.36	0.39	0.48	0.47	0.35	0.61	0.13	0.56	1034
0.15	0.00	0.06	0.00	-0.08	0.20	0.14	0.06	0.13	0.22	0.19	0.08	0.36	0.14	0.27	0.35	0.43	0.41	0.31	0.54	0.11	0.48	946
0.18	0.00	0.03	0.00	-0.06	0.12	0.09	0.00	0.09	0.16	0.14	0.05	0.27	0.11	0.20	0.31	0.38	0.37	0.28	0.48	0.10	0.43	934
0.32	0.00	0.01	0.00	-0.05	0.08	0.07	0.00	0.05	0.11	0.09	0.01	0.20	0.10	0.14	0.27	0.32	0.31	0.23	0.41	0.09	0.36	1827


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.07
top50	0.13


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	33.65	44.69	41.57	28.33	61.06	16.37	51.42	14.00	18.07	18.00	12.86	23.27	5.21	21.00	37.26	49.41	46.02	31.82	67.00	17.59	57.49	14.00	17.92	18.00	12.75	23.10	5.18	21.00	921
0.03	34.08	47.77	43.46	26.79	68.74	20.98	54.90	10.00	15.03	15.00	8.82	21.24	6.21	19.00	42.61	58.80	53.72	33.37	84.22	25.42	66.99	10.00	14.78	14.00	8.70	20.87	6.08	19.00	993
0.06	34.86	52.43	44.81	20.70	84.16	31.73	58.36	8.00	13.39	12.00	6.64	20.14	6.75	18.00	50.93	75.05	64.12	31.51	118.59	43.54	82.41	8.00	13.12	12.00	6.51	19.73	6.61	18.00	1109
0.11	35.18	53.68	45.83	23.09	84.27	30.59	60.73	7.00	13.30	13.00	6.46	20.13	6.84	18.00	61.46	90.01	77.22	40.39	139.63	49.62	100.97	7.00	12.97	12.00	6.17	19.77	6.80	18.00	1113
0.15	35.06	53.80	44.73	20.56	87.03	33.23	59.17	7.00	12.87	12.00	6.19	19.55	6.68	17.00	77.77	114.86	98.61	48.01	181.71	66.85	126.57	7.00	12.66	12.00	5.97	19.35	6.69	18.00	987
0.18	34.73	55.18	45.13	10.59	99.77	44.59	59.77	7.00	12.60	12.00	5.78	19.43	6.83	17.00	98.28	143.97	123.79	61.23	226.70	82.73	159.78	7.00	12.32	11.00	5.48	19.17	6.84	17.00	950
0.32	35.42	55.78	45.96	15.09	96.47	40.69	60.82	7.00	12.34	12.00	5.46	19.21	6.87	17.00	148.48	224.48	192.88	94.87	354.08	129.60	260.18	6.00	11.99	11.00	5.05	18.93	6.94	17.00	1801


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/comparison_vals_auc.tex <==
name	auc
orig_pp	16.65
orig_ge	4.08
adv_pp	40.84
adv_ge	4.00


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.52	0.62	0.64	0.45	0.79	0.17	0.74	0.82	0.85	0.88	0.76	0.95	0.10	0.92	0.64	0.70	0.72	0.59	0.81	0.11	0.78	921
0.03	0.38	0.50	0.50	0.32	0.67	0.17	0.62	0.73	0.78	0.81	0.65	0.91	0.13	0.87	0.56	0.62	0.64	0.49	0.75	0.13	0.71	993
0.06	0.24	0.38	0.38	0.19	0.57	0.19	0.50	0.61	0.68	0.72	0.51	0.86	0.18	0.81	0.45	0.53	0.55	0.37	0.68	0.15	0.63	1109
0.11	0.16	0.29	0.28	0.12	0.46	0.17	0.40	0.51	0.61	0.64	0.43	0.78	0.18	0.74	0.37	0.46	0.47	0.31	0.61	0.15	0.56	1113
0.15	0.09	0.20	0.19	0.04	0.35	0.15	0.29	0.42	0.52	0.54	0.35	0.69	0.17	0.65	0.29	0.38	0.40	0.25	0.52	0.14	0.48	987
0.18	0.03	0.13	0.12	-0.00	0.26	0.13	0.21	0.32	0.43	0.45	0.26	0.61	0.18	0.56	0.23	0.31	0.32	0.18	0.45	0.13	0.41	950
0.32	-0.07	0.02	0.01	-0.11	0.16	0.14	0.10	0.12	0.25	0.26	0.05	0.46	0.20	0.39	0.09	0.18	0.18	0.04	0.33	0.15	0.28	1801


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/correlations_auc.tex <==
name	auc
pcc	0.07
spearman	0.16
kendall	0.12


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.36	5.99	5.20	2.36	9.61	3.63	7.82	2.83	6.03	4.85	1.42	10.64	4.61	8.06	2.04	5.10	3.70	0.41	9.79	4.69	6.63	921
0.03	2.95	4.77	4.22	1.99	7.55	2.78	5.70	2.43	4.77	3.70	1.17	8.38	3.61	6.12	1.89	4.35	3.12	0.31	8.38	4.04	5.42	993
0.06	2.63	3.85	3.56	2.00	5.71	1.85	4.72	2.16	3.73	3.07	1.24	6.22	2.49	4.53	1.71	3.78	2.60	-0.36	7.92	4.14	4.17	1109
0.11	2.51	3.45	3.26	2.06	4.83	1.38	4.21	2.10	3.31	2.87	1.39	5.23	1.92	3.94	1.69	3.15	2.34	0.26	6.04	2.89	3.59	1113
0.15	2.38	3.06	3.01	1.96	4.16	1.10	3.58	1.98	2.82	2.53	1.35	4.29	1.47	3.33	1.57	2.49	2.06	0.48	4.51	2.02	2.80	987
0.18	2.22	2.79	2.75	1.96	3.62	0.83	3.32	1.93	2.58	2.38	1.60	3.57	0.98	3.02	1.53	2.25	1.92	0.49	4.02	1.77	2.40	950
0.32	2.07	2.55	2.52	1.87	3.24	0.68	2.98	1.90	2.41	2.29	1.63	3.19	0.78	2.78	1.46	1.94	1.77	0.97	2.91	0.97	2.19	1801


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/ets_sts_auc.tex <==
name	auc
et_use	1.01
et_tse	0.97
et_ce	0.87


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.04	3.85	1.71	-7.20	14.90	11.05	3.09	3.11	5.86	4.89	1.60	10.11	4.26	7.31	2.69	6.07	4.69	0.67	11.48	5.41	7.70	921
0.03	0.72	1.82	1.05	-2.82	6.45	4.64	1.64	3.16	4.94	4.35	2.03	7.84	2.90	5.99	2.72	4.88	3.93	1.18	8.58	3.70	6.00	993
0.06	0.49	1.04	0.70	-1.84	3.92	2.88	1.04	3.04	4.40	4.00	1.98	6.81	2.42	5.24	2.56	4.31	3.53	0.92	7.71	3.40	5.09	1109
0.11	0.37	0.66	0.52	-0.35	1.67	1.01	0.71	3.05	4.06	3.78	2.40	5.73	1.66	4.74	2.58	3.91	3.39	1.66	6.16	2.25	4.59	1113
0.15	0.26	0.51	0.33	-1.17	2.19	1.68	0.46	2.89	3.66	3.45	2.28	5.04	1.38	4.04	2.42	3.48	3.03	1.33	5.64	2.16	3.82	987
0.18	0.19	0.37	0.25	-0.64	1.38	1.01	0.33	2.79	3.44	3.26	2.26	4.63	1.19	3.81	2.34	3.24	2.87	1.45	5.02	1.79	3.54	950
0.32	0.11	0.20	0.15	-0.07	0.47	0.27	0.22	2.67	3.27	3.09	2.19	4.34	1.07	3.55	2.29	3.02	2.72	1.51	4.53	1.51	3.25	1801


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.22
et_p_h	1.19
et_p_l2	1.14


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.11	0.11	0.05	0.18	0.06	0.15	0.03	0.04	0.04	0.02	0.07	0.02	0.06	0.03	0.04	0.04	0.02	0.06	0.02	0.05	921
0.03	0.16	0.24	0.24	0.13	0.36	0.11	0.32	0.04	0.07	0.06	0.04	0.10	0.03	0.09	0.04	0.06	0.06	0.04	0.08	0.02	0.07	993
0.06	0.31	0.46	0.44	0.24	0.68	0.22	0.58	0.06	0.09	0.09	0.05	0.13	0.04	0.11	0.06	0.08	0.08	0.05	0.10	0.02	0.09	1109
0.11	0.51	0.73	0.70	0.40	1.06	0.33	0.90	0.08	0.11	0.11	0.07	0.15	0.04	0.13	0.08	0.10	0.10	0.07	0.12	0.03	0.11	1113
0.15	0.89	1.24	1.20	0.70	1.78	0.54	1.52	0.11	0.13	0.13	0.09	0.18	0.04	0.16	0.10	0.12	0.12	0.09	0.14	0.03	0.13	987
0.18	1.34	1.84	1.76	1.04	2.63	0.80	2.23	0.13	0.15	0.15	0.11	0.20	0.05	0.18	0.12	0.13	0.13	0.10	0.16	0.03	0.15	950
0.32	2.17	3.47	3.10	1.64	5.29	1.82	4.42	0.15	0.18	0.18	0.13	0.23	0.05	0.21	0.14	0.16	0.16	0.13	0.19	0.03	0.18	1801


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.50
pp_l2_d	0.04
pp_h_d	0.04


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.92	0.99	0.03	0.98	0.92	0.94	0.95	0.89	0.99	0.05	0.97	921
0.03	0.93	0.94	0.94	0.91	0.97	0.03	0.95	0.91	0.93	0.94	0.88	0.97	0.04	0.96	0.88	0.91	0.92	0.84	0.98	0.07	0.95	993
0.06	0.90	0.91	0.92	0.88	0.94	0.03	0.93	0.87	0.89	0.90	0.84	0.95	0.05	0.93	0.83	0.87	0.88	0.79	0.95	0.08	0.92	1109
0.11	0.87	0.89	0.89	0.85	0.92	0.04	0.91	0.84	0.87	0.88	0.82	0.92	0.05	0.91	0.80	0.84	0.85	0.76	0.93	0.08	0.90	1113
0.15	0.84	0.86	0.87	0.81	0.90	0.05	0.89	0.81	0.84	0.84	0.78	0.89	0.06	0.88	0.75	0.80	0.81	0.70	0.89	0.10	0.85	987
0.18	0.82	0.83	0.84	0.78	0.88	0.05	0.87	0.78	0.81	0.82	0.76	0.87	0.06	0.85	0.72	0.76	0.77	0.66	0.86	0.10	0.82	950
0.32	0.77	0.80	0.81	0.74	0.85	0.05	0.83	0.75	0.78	0.79	0.72	0.84	0.06	0.82	0.67	0.71	0.73	0.60	0.82	0.11	0.78	1801


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.25


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	12.10	15.54	15.78	9.93	21.16	5.61	17.74	121.21	348.25	232.49	-57.82	754.33	406.08	414.67	3.15	9.07	7.34	1.49	16.66	7.58	12.65	921
0.03	9.97	19.17	16.83	0.51	37.84	18.66	23.68	159.77	473.33	293.54	-227.90	1174.56	701.23	528.05	3.18	9.40	6.74	0.41	18.38	8.99	12.78	993
0.06	9.81	26.16	18.59	-3.77	56.10	29.94	32.78	206.24	848.37	389.89	-2169.70	3866.45	3018.07	718.62	2.85	10.41	6.88	-0.46	21.28	10.87	14.71	1109
0.11	8.11	18.77	11.66	-4.86	42.39	23.62	20.13	237.76	974.98	459.46	-1278.70	3228.66	2253.68	887.37	2.87	10.95	7.29	0.30	21.60	10.65	16.41	1113
0.15	11.05	22.67	17.04	-2.35	47.69	25.02	26.20	292.20	806.47	512.93	-330.86	1943.80	1137.33	919.74	2.82	11.35	7.86	0.35	22.36	11.00	16.18	987
0.18	13.54	25.22	20.25	2.47	47.96	22.74	31.23	333.33	905.98	576.45	-472.84	2284.79	1378.82	985.02	2.95	12.19	7.85	0.12	24.26	12.07	17.59	950
0.32	22.22	39.07	33.73	13.20	64.93	25.87	49.17	362.66	988.78	637.27	-589.11	2566.68	1577.89	1066.15	2.94	11.84	7.80	0.12	23.55	11.71	17.20	1801


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/time_misc_auc.tex <==
name	auc
attack_time	8.16
l2	267.22
lom	3.50


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.47	0.57	0.58	0.41	0.74	0.16	0.70	0.71	0.77	0.78	0.67	0.86	0.09	0.84	0.82	0.86	0.86	0.79	0.92	0.06	0.90	921
0.03	0.32	0.43	0.43	0.25	0.61	0.18	0.56	0.64	0.70	0.71	0.59	0.81	0.11	0.78	0.78	0.82	0.83	0.75	0.89	0.07	0.87	993
0.06	0.18	0.31	0.31	0.12	0.49	0.18	0.43	0.55	0.62	0.64	0.49	0.76	0.14	0.72	0.72	0.77	0.79	0.68	0.86	0.09	0.84	1109
0.11	0.11	0.24	0.25	0.07	0.41	0.17	0.33	0.50	0.57	0.57	0.44	0.69	0.13	0.66	0.69	0.74	0.75	0.65	0.83	0.09	0.80	1113
0.15	0.00	0.16	0.14	0.01	0.31	0.15	0.25	0.43	0.51	0.50	0.38	0.63	0.12	0.58	0.65	0.70	0.71	0.62	0.79	0.08	0.76	987
0.18	0.00	0.12	0.10	-0.02	0.26	0.14	0.19	0.37	0.45	0.45	0.33	0.57	0.12	0.52	0.62	0.67	0.67	0.58	0.75	0.08	0.72	950
0.32	0.00	0.07	0.00	-0.03	0.17	0.10	0.12	0.27	0.35	0.35	0.22	0.48	0.13	0.43	0.54	0.60	0.60	0.50	0.69	0.09	0.66	1801


==> data/mlm_plots/mlm_distil_fast/yelp/xlnet/s/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.16
top50	0.22


==> data/mlm_plots/tef/agnews/bert/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	138.20	241.34	202.62	91.56	391.12	149.78	303.44	5.00	7.92	7.00	4.54	11.31	3.38	10.00	170.03	283.61	240.56	117.96	449.26	165.65	358.90	5.00	8.06	8.00	4.63	11.49	3.43	10.00	756
0.06	139.59	245.92	209.15	85.52	406.33	160.40	303.66	5.00	7.69	7.00	4.40	10.98	3.29	10.00	200.51	334.75	291.15	134.67	534.83	200.08	418.06	5.00	7.91	7.00	4.54	11.27	3.36	10.00	1001
0.11	135.76	240.85	203.55	82.69	399.02	158.17	299.09	5.00	7.78	7.00	4.48	11.08	3.30	10.00	228.49	378.80	326.00	155.62	601.97	223.17	468.89	6.00	8.10	8.00	4.71	11.48	3.39	10.00	988
0.15	136.90	240.87	203.19	84.63	397.10	156.24	303.36	5.00	7.87	8.00	4.58	11.16	3.29	10.00	282.04	465.21	406.30	197.32	733.10	267.89	586.94	6.00	8.31	8.00	4.93	11.69	3.38	10.00	912
0.18	137.79	245.88	207.87	80.11	411.64	165.76	305.89	5.00	7.74	7.00	4.42	11.05	3.31	10.00	340.76	558.69	493.09	252.16	865.22	306.53	690.28	6.00	8.32	8.00	4.91	11.72	3.41	10.00	1032
0.32	136.85	246.07	206.35	79.87	412.27	166.20	304.33	5.00	7.69	7.00	4.40	10.97	3.29	10.00	520.22	868.60	750.81	341.87	1395.34	526.73	1068.77	6.00	8.63	8.00	5.22	12.04	3.41	11.00	2896


==> data/mlm_plots/tef/agnews/bert/a/comparison_vals_auc.tex <==
name	auc
orig_pp	70.82
orig_ge	2.25
adv_pp	158.58
adv_ge	2.40


==> data/mlm_plots/tef/agnews/bert/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.37	0.54	0.59	0.27	0.81	0.27	0.75	0.84	0.88	0.90	0.80	0.97	0.09	0.95	0.71	0.76	0.78	0.67	0.86	0.10	0.83	756
0.06	0.15	0.34	0.34	0.09	0.60	0.25	0.53	0.74	0.80	0.83	0.68	0.92	0.12	0.89	0.59	0.66	0.67	0.53	0.78	0.12	0.74	1001
0.11	0.04	0.22	0.18	-0.01	0.45	0.23	0.37	0.66	0.74	0.76	0.59	0.88	0.15	0.85	0.50	0.58	0.60	0.45	0.72	0.14	0.68	988
0.15	-0.03	0.11	0.07	-0.08	0.30	0.19	0.21	0.56	0.65	0.68	0.48	0.83	0.17	0.78	0.42	0.50	0.51	0.35	0.65	0.15	0.61	912
0.18	-0.07	0.04	-0.00	-0.12	0.20	0.16	0.10	0.46	0.58	0.61	0.38	0.77	0.20	0.72	0.34	0.43	0.45	0.27	0.59	0.16	0.55	1032
0.32	-0.13	-0.06	-0.07	-0.19	0.08	0.13	-0.01	0.26	0.41	0.44	0.17	0.66	0.24	0.60	0.17	0.30	0.31	0.11	0.48	0.18	0.43	2896


==> data/mlm_plots/tef/agnews/bert/a/correlations_auc.tex <==
name	auc
pcc	0.03
spearman	0.18
kendall	0.14


==> data/mlm_plots/tef/agnews/bert/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	2.09	4.23	3.46	1.02	7.43	3.20	5.35	1.74	4.21	2.94	0.13	8.29	4.08	5.12	2.19	8.13	4.60	-0.90	17.16	9.03	10.84	756
0.06	2.44	3.88	3.43	1.70	6.06	2.18	4.85	2.04	3.70	3.02	0.93	6.47	2.77	4.62	2.53	9.05	5.14	-0.88	18.97	9.93	11.16	1001
0.11	2.50	3.54	3.31	1.93	5.16	1.62	4.31	2.07	3.30	2.82	1.32	5.28	1.98	3.95	2.33	7.62	4.19	-0.96	16.21	8.59	9.11	988
0.15	2.44	3.17	3.05	2.00	4.34	1.17	3.67	2.05	2.95	2.66	1.50	4.41	1.45	3.50	2.47	6.45	3.97	-0.61	13.51	7.06	7.19	912
0.18	2.28	2.86	2.75	1.93	3.78	0.92	3.25	1.95	2.63	2.42	1.61	3.66	1.02	3.05	2.32	5.53	3.70	-0.57	11.63	6.10	5.82	1032
0.32	2.00	2.42	2.29	1.74	3.09	0.67	2.71	1.82	2.29	2.13	1.56	3.01	0.73	2.58	2.08	4.02	2.99	-0.07	8.12	4.09	4.49	2896


==> data/mlm_plots/tef/agnews/bert/a/ets_sts_auc.tex <==
name	auc
et_use	0.90
et_tse	0.85
et_ce	1.80


==> data/mlm_plots/tef/agnews/bert/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.55	2.66	1.07	-4.41	9.74	7.07	2.22	3.42	11.07	7.31	-1.10	23.25	12.17	13.61	3.61	15.84	8.13	-10.94	42.61	26.78	17.32	756
0.06	0.49	2.86	0.81	-11.87	17.59	14.73	1.55	4.11	9.67	6.83	1.07	18.27	8.60	12.36	3.66	12.76	7.38	-6.05	31.57	18.81	15.53	1001
0.11	0.39	2.57	0.64	-13.60	18.73	16.17	1.10	3.93	7.91	6.00	1.36	14.45	6.54	9.91	3.36	9.63	5.85	-2.38	21.63	12.00	11.33	988
0.15	0.29	0.99	0.45	-2.31	4.29	3.30	0.74	3.85	6.87	5.35	1.95	11.79	4.92	8.16	3.30	8.08	4.98	-1.65	17.81	9.73	9.73	912
0.18	0.23	0.88	0.35	-3.36	5.13	4.25	0.57	3.75	6.12	4.83	2.10	10.13	4.01	7.22	3.14	7.20	4.42	-4.48	18.89	11.68	7.75	1032
0.32	0.13	0.39	0.21	-1.51	2.29	1.90	0.35	3.36	5.07	4.19	2.09	8.04	2.97	5.76	2.82	5.69	3.70	-1.99	13.36	7.68	5.88	2896


==> data/mlm_plots/tef/agnews/bert/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.40
et_p_h	2.02
et_p_l2	2.47


==> data/mlm_plots/tef/agnews/bert/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.09	0.23	0.19	0.06	0.40	0.17	0.33	0.01	0.04	0.02	0.00	0.08	0.04	0.05	0.01	0.04	0.03	0.01	0.07	0.03	0.05	756
0.06	0.21	0.43	0.39	0.15	0.72	0.29	0.60	0.02	0.06	0.04	0.01	0.10	0.05	0.08	0.03	0.05	0.04	0.02	0.09	0.03	0.08	1001
0.11	0.34	0.70	0.61	0.21	1.18	0.48	0.95	0.03	0.08	0.06	0.02	0.13	0.05	0.11	0.04	0.07	0.06	0.03	0.11	0.04	0.10	988
0.15	0.60	1.11	0.94	0.35	1.88	0.76	1.46	0.05	0.09	0.09	0.04	0.15	0.06	0.13	0.05	0.09	0.08	0.05	0.12	0.04	0.11	912
0.18	0.85	1.57	1.36	0.53	2.60	1.03	2.05	0.06	0.11	0.11	0.05	0.17	0.06	0.15	0.07	0.10	0.10	0.06	0.14	0.04	0.13	1032
0.32	1.47	3.24	2.53	0.61	5.86	2.63	4.09	0.09	0.14	0.14	0.07	0.21	0.07	0.18	0.09	0.12	0.12	0.08	0.17	0.05	0.16	2896


==> data/mlm_plots/tef/agnews/bert/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.45
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/agnews/bert/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.94	0.94	0.91	0.96	0.03	0.96	0.90	0.93	0.93	0.88	0.97	0.04	0.96	0.91	0.94	0.96	0.87	1.00	0.06	0.98	756
0.06	0.89	0.91	0.91	0.87	0.94	0.03	0.93	0.86	0.89	0.90	0.84	0.94	0.05	0.93	0.88	0.92	0.94	0.84	0.99	0.07	0.97	1001
0.11	0.86	0.88	0.88	0.84	0.92	0.04	0.90	0.82	0.86	0.86	0.81	0.91	0.05	0.90	0.85	0.89	0.91	0.80	0.98	0.09	0.96	988
0.15	0.83	0.85	0.85	0.81	0.89	0.04	0.87	0.79	0.83	0.83	0.77	0.89	0.06	0.87	0.83	0.87	0.89	0.78	0.96	0.09	0.94	912
0.18	0.80	0.82	0.82	0.78	0.86	0.04	0.85	0.76	0.80	0.80	0.75	0.86	0.05	0.84	0.80	0.85	0.87	0.75	0.95	0.10	0.92	1032
0.32	0.74	0.77	0.77	0.72	0.82	0.05	0.81	0.71	0.75	0.75	0.69	0.81	0.06	0.80	0.75	0.80	0.82	0.69	0.91	0.11	0.88	2896


==> data/mlm_plots/tef/agnews/bert/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.25


==> data/mlm_plots/tef/agnews/bert/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.34	0.37	0.36	0.33	0.41	0.04	0.39	0.17	0.27	0.25	0.13	0.40	0.13	0.34	1.29	4.14	2.89	-0.18	8.47	4.32	5.50	756
0.06	0.50	0.56	0.53	0.44	0.68	0.12	0.56	0.23	0.33	0.32	0.20	0.47	0.13	0.41	1.86	5.29	3.96	0.48	10.10	4.81	7.21	1001
0.11	0.89	0.95	0.94	0.83	1.06	0.11	0.99	0.28	0.38	0.37	0.24	0.52	0.14	0.45	2.27	6.12	4.80	0.90	11.33	5.22	8.63	988
0.15	0.92	1.02	0.99	0.80	1.23	0.21	1.05	0.32	0.42	0.40	0.28	0.56	0.14	0.49	2.67	6.85	5.42	1.30	12.39	5.54	9.69	912
0.18	1.87	2.00	2.01	1.79	2.22	0.21	2.12	0.34	0.43	0.42	0.29	0.57	0.14	0.51	2.81	7.34	6.12	1.65	13.03	5.69	10.62	1032
0.32	2.19	2.53	2.60	2.17	2.89	0.36	2.81	0.34	0.44	0.42	0.30	0.57	0.14	0.50	3.18	7.58	6.69	2.06	13.09	5.51	10.80	2896


==> data/mlm_plots/tef/agnews/bert/a/time_misc_auc.tex <==
name	auc
attack_time	0.45
l2	0.12
lom	1.95


==> data/mlm_plots/tef/agnews/bert/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.40	0.56	0.60	0.33	0.79	0.23	0.75	0.73	0.81	0.82	0.70	0.91	0.10	0.88	0.85	0.89	0.89	0.83	0.95	0.06	0.93	756
0.06	0.25	0.39	0.40	0.15	0.63	0.24	0.50	0.64	0.72	0.73	0.59	0.85	0.13	0.81	0.79	0.84	0.85	0.76	0.92	0.08	0.89	1001
0.11	0.00	0.29	0.25	0.05	0.53	0.24	0.50	0.57	0.66	0.67	0.51	0.80	0.14	0.77	0.75	0.81	0.81	0.72	0.90	0.09	0.88	988
0.15	0.00	0.20	0.20	-0.01	0.41	0.21	0.33	0.50	0.59	0.60	0.44	0.74	0.15	0.69	0.71	0.77	0.78	0.67	0.87	0.10	0.84	912
0.18	0.00	0.14	0.00	-0.05	0.32	0.18	0.25	0.43	0.53	0.54	0.38	0.69	0.16	0.64	0.67	0.74	0.74	0.64	0.84	0.10	0.81	1032
0.32	0.00	0.07	0.00	-0.07	0.21	0.14	0.00	0.30	0.42	0.43	0.25	0.60	0.17	0.55	0.59	0.67	0.68	0.56	0.78	0.11	0.75	2896


==> data/mlm_plots/tef/agnews/bert/a/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.17
top50	0.22


==> data/mlm_plots/tef/agnews/bert/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	136.16	238.94	202.60	86.11	391.77	152.83	297.69	5.00	7.87	7.00	4.48	11.27	3.39	10.00	162.18	278.59	237.07	108.06	449.12	170.53	352.66	5.00	7.99	8.00	4.56	11.42	3.43	10.00	769
0.06	137.90	243.81	205.59	85.24	402.38	158.57	305.58	5.00	7.70	7.00	4.44	10.96	3.26	10.00	188.04	325.34	281.24	127.58	523.11	197.77	410.37	5.00	7.90	8.00	4.61	11.20	3.30	10.00	1025
0.11	136.86	242.23	201.01	84.21	400.24	158.02	299.16	5.00	7.75	7.00	4.50	11.00	3.25	10.00	218.95	382.95	320.69	141.21	624.69	241.74	477.28	6.00	8.06	8.00	4.74	11.38	3.32	10.00	1027
0.15	138.28	243.61	204.66	84.36	402.87	159.25	300.65	5.00	7.89	7.00	4.42	11.36	3.47	10.00	274.58	460.16	400.83	167.92	752.41	292.25	550.87	6.00	8.32	8.00	4.80	11.85	3.52	10.00	1042
0.18	137.34	241.66	207.32	86.74	396.59	154.92	300.24	5.00	7.76	7.00	4.56	10.96	3.20	10.00	337.37	551.22	485.26	227.57	874.88	323.65	677.52	6.00	8.30	8.00	5.02	11.58	3.28	10.00	1113
0.32	136.45	246.02	206.35	82.58	409.47	163.45	307.14	5.00	7.64	7.00	4.34	10.94	3.30	10.00	447.45	774.81	651.10	276.24	1273.38	498.57	940.43	6.00	8.40	8.00	5.01	11.78	3.39	10.50	2663


==> data/mlm_plots/tef/agnews/bert/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	70.52
orig_ge	2.25
adv_pp	151.17
adv_ge	2.38


==> data/mlm_plots/tef/agnews/bert/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.01	0.24	0.26	-0.08	0.57	0.33	0.49	0.18	0.35	0.37	0.08	0.61	0.26	0.54	0.13	0.27	0.28	0.06	0.48	0.21	0.40	769
0.06	-0.24	-0.04	-0.03	-0.33	0.26	0.30	0.16	-0.04	0.12	0.12	-0.12	0.36	0.24	0.28	-0.02	0.09	0.09	-0.09	0.27	0.18	0.21	1025
0.11	-0.41	-0.21	-0.20	-0.47	0.06	0.26	-0.03	-0.19	-0.03	-0.03	-0.26	0.21	0.23	0.14	-0.13	-0.01	-0.02	-0.19	0.16	0.17	0.10	1027
0.15	-0.51	-0.36	-0.37	-0.58	-0.13	0.23	-0.22	-0.33	-0.18	-0.19	-0.40	0.04	0.22	-0.02	-0.23	-0.12	-0.13	-0.29	0.04	0.16	-0.01	1042
0.18	-0.58	-0.44	-0.46	-0.65	-0.24	0.20	-0.32	-0.41	-0.27	-0.28	-0.47	-0.06	0.20	-0.14	-0.29	-0.19	-0.20	-0.33	-0.04	0.15	-0.09	1113
0.32	-0.67	-0.54	-0.57	-0.72	-0.37	0.18	-0.44	-0.50	-0.37	-0.39	-0.56	-0.19	0.18	-0.27	-0.36	-0.27	-0.28	-0.40	-0.13	0.14	-0.18	2663


==> data/mlm_plots/tef/agnews/bert/ig/correlations_auc.tex <==
name	auc
pcc	-0.10
spearman	-0.05
kendall	-0.03


==> data/mlm_plots/tef/agnews/bert/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	4.12	7.09	5.96	2.36	11.83	4.74	8.59	3.31	7.27	5.60	1.26	13.28	6.01	8.98	3.79	13.76	9.16	0.75	26.77	13.01	20.16	769
0.06	4.26	6.11	5.56	3.08	9.15	3.03	7.09	3.59	6.10	5.06	1.99	10.21	4.11	7.26	4.16	13.78	8.52	0.20	27.37	13.58	18.46	1025
0.11	4.02	5.43	4.98	3.07	7.79	2.36	6.31	3.36	5.20	4.54	2.38	8.02	2.82	6.06	3.92	11.72	6.96	-0.95	24.38	12.67	13.79	1027
0.15	3.78	4.81	4.57	3.16	6.46	1.65	5.44	3.24	4.62	4.18	2.58	6.65	2.03	5.47	3.78	10.14	5.80	-1.23	21.51	11.37	11.49	1042
0.18	3.48	4.36	4.19	3.04	5.69	1.32	4.98	3.21	4.20	3.88	2.62	5.78	1.58	4.87	3.72	9.01	5.75	-1.05	19.07	10.06	9.60	1113
0.32	3.13	3.81	3.65	2.76	4.86	1.05	4.26	2.93	3.71	3.46	2.53	4.89	1.18	4.24	3.28	6.97	4.84	-0.75	14.68	7.71	7.57	2663


==> data/mlm_plots/tef/agnews/bert/ig/ets_sts_auc.tex <==
name	auc
et_use	1.40
et_tse	1.36
et_ce	2.89


==> data/mlm_plots/tef/agnews/bert/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.10	5.49	2.01	-10.05	21.02	15.54	3.93	7.30	20.82	14.28	0.92	40.73	19.91	27.01	7.93	30.25	16.39	-11.70	72.19	41.94	35.69	769
0.06	0.87	5.07	1.41	-14.73	24.87	19.80	2.81	7.25	16.23	11.63	3.18	29.27	13.05	20.77	6.34	21.85	13.45	-5.48	49.18	27.33	25.62	1025
0.11	0.66	2.52	0.99	-7.71	12.75	10.23	1.75	6.72	13.00	10.14	3.91	22.08	9.08	16.33	5.99	16.28	11.25	0.71	31.86	15.58	20.35	1027
0.15	0.49	1.17	0.73	-1.01	3.35	2.18	1.20	6.37	10.85	8.78	3.95	17.74	6.90	13.27	5.35	12.95	8.64	-0.06	25.96	13.01	14.54	1042
0.18	0.38	1.21	0.56	-5.40	7.83	6.61	0.83	5.76	9.38	7.72	3.43	15.33	5.95	11.16	4.83	10.60	6.98	0.27	20.94	10.33	12.52	1113
0.32	0.23	0.60	0.36	-1.97	3.16	2.57	0.59	5.34	7.96	6.65	3.67	12.25	4.29	9.07	4.44	8.72	6.00	0.52	16.92	8.20	9.58	2663


==> data/mlm_plots/tef/agnews/bert/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.58
et_p_h	3.27
et_p_l2	4.01


==> data/mlm_plots/tef/agnews/bert/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.09	0.21	0.18	0.04	0.39	0.17	0.30	0.01	0.03	0.02	-0.00	0.07	0.03	0.04	0.01	0.03	0.02	0.01	0.06	0.03	0.04	769
0.06	0.18	0.41	0.35	0.10	0.71	0.30	0.56	0.02	0.05	0.04	0.01	0.10	0.04	0.08	0.02	0.05	0.04	0.02	0.08	0.03	0.07	1025
0.11	0.34	0.67	0.59	0.19	1.16	0.48	0.90	0.03	0.07	0.05	0.02	0.12	0.05	0.10	0.04	0.07	0.06	0.03	0.10	0.04	0.09	1027
0.15	0.56	1.02	0.93	0.40	1.64	0.62	1.35	0.05	0.09	0.08	0.04	0.14	0.05	0.13	0.05	0.08	0.08	0.04	0.12	0.04	0.11	1042
0.18	0.85	1.50	1.31	0.55	2.46	0.95	1.92	0.06	0.11	0.10	0.05	0.17	0.06	0.15	0.07	0.10	0.10	0.06	0.14	0.04	0.12	1113
0.32	1.32	2.58	2.11	0.70	4.46	1.88	3.32	0.08	0.13	0.13	0.07	0.19	0.06	0.17	0.08	0.12	0.12	0.07	0.16	0.04	0.14	2663


==> data/mlm_plots/tef/agnews/bert/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.39
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/tef/agnews/bert/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.94	0.94	0.91	0.96	0.03	0.96	0.90	0.93	0.94	0.88	0.97	0.04	0.96	0.91	0.94	0.96	0.87	1.00	0.06	0.98	769
0.06	0.89	0.91	0.91	0.87	0.94	0.03	0.93	0.86	0.89	0.90	0.85	0.94	0.05	0.93	0.88	0.92	0.94	0.84	0.99	0.07	0.97	1025
0.11	0.85	0.88	0.88	0.84	0.91	0.04	0.90	0.83	0.86	0.87	0.81	0.91	0.05	0.90	0.86	0.89	0.91	0.81	0.98	0.08	0.96	1027
0.15	0.82	0.85	0.85	0.81	0.89	0.04	0.87	0.80	0.83	0.84	0.78	0.89	0.05	0.88	0.82	0.87	0.89	0.78	0.96	0.09	0.94	1042
0.18	0.80	0.82	0.83	0.79	0.86	0.04	0.85	0.78	0.81	0.81	0.76	0.86	0.05	0.85	0.81	0.86	0.87	0.76	0.95	0.09	0.92	1113
0.32	0.76	0.79	0.79	0.74	0.83	0.04	0.82	0.74	0.78	0.78	0.72	0.83	0.05	0.82	0.77	0.82	0.84	0.71	0.93	0.11	0.90	2663


==> data/mlm_plots/tef/agnews/bert/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.25


==> data/mlm_plots/tef/agnews/bert/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.48	0.54	0.51	0.36	0.72	0.18	0.53	0.33	4.21	0.74	-4.66	13.07	8.86	3.17	3.06	8.33	6.44	1.39	15.28	6.95	11.74	769
0.06	1.58	1.78	1.67	1.22	2.34	0.56	1.77	0.46	5.41	1.02	-6.23	17.06	11.65	4.29	3.88	9.88	7.97	2.22	17.54	7.66	14.32	1025
0.11	2.07	2.40	2.20	1.63	3.18	0.77	2.40	0.57	5.93	1.33	-4.88	16.73	10.80	6.23	4.39	10.91	9.57	2.83	19.00	8.09	16.16	1027
0.15	2.95	3.51	3.11	2.41	4.60	1.10	3.42	0.63	6.07	1.29	-5.15	17.30	11.22	6.08	4.44	11.41	9.56	2.80	20.03	8.61	16.38	1042
0.18	4.02	4.58	4.41	3.80	5.36	0.78	4.68	0.66	6.51	1.42	-4.73	17.74	11.24	6.92	5.09	12.21	10.39	3.32	21.11	8.89	17.29	1113
0.32	5.57	6.15	6.21	5.41	6.89	0.74	6.72	0.69	7.14	1.71	-4.13	18.42	11.27	8.89	4.43	11.58	9.76	2.74	20.42	8.84	16.82	2663


==> data/mlm_plots/tef/agnews/bert/ig/time_misc_auc.tex <==
name	auc
attack_time	1.13
l2	1.81
lom	3.26


==> data/mlm_plots/tef/agnews/bert/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.20	0.33	0.33	0.08	0.57	0.24	0.50	0.40	0.50	0.50	0.35	0.66	0.16	0.62	0.56	0.64	0.65	0.52	0.75	0.11	0.71	769
0.06	0.00	0.18	0.20	-0.02	0.38	0.20	0.33	0.29	0.39	0.38	0.24	0.54	0.15	0.50	0.48	0.56	0.56	0.45	0.66	0.11	0.63	1025
0.11	0.00	0.12	0.00	-0.05	0.28	0.17	0.25	0.22	0.32	0.33	0.18	0.46	0.14	0.42	0.44	0.51	0.50	0.40	0.61	0.10	0.58	1027
0.15	0.00	0.06	0.00	-0.06	0.18	0.12	0.00	0.17	0.26	0.25	0.13	0.39	0.13	0.33	0.38	0.45	0.45	0.36	0.55	0.10	0.52	1042
0.18	0.00	0.04	0.00	-0.06	0.14	0.10	0.00	0.14	0.22	0.21	0.10	0.34	0.12	0.30	0.36	0.43	0.42	0.34	0.52	0.09	0.50	1113
0.32	0.00	0.03	0.00	-0.06	0.11	0.08	0.00	0.09	0.17	0.15	0.06	0.28	0.11	0.23	0.32	0.39	0.38	0.30	0.47	0.09	0.44	2663


==> data/mlm_plots/tef/agnews/bert/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.08
top50	0.13


==> data/mlm_plots/tef/agnews/bert/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	138.62	242.53	205.30	83.73	401.33	158.80	298.27	5.00	7.87	8.00	4.45	11.30	3.43	10.00	168.63	280.72	244.65	111.50	449.94	169.22	338.98	5.00	7.98	8.00	4.53	11.42	3.44	10.00	771
0.06	138.45	246.01	203.65	73.06	418.96	172.95	301.11	5.00	7.73	7.00	4.38	11.07	3.35	10.00	195.60	332.90	281.93	120.27	545.54	212.64	409.16	5.00	7.94	7.00	4.55	11.32	3.39	10.00	1056
0.11	137.20	242.39	204.29	78.95	405.83	163.44	298.91	5.00	7.62	7.00	4.37	10.86	3.25	9.00	227.64	390.38	332.78	134.15	646.60	256.22	482.44	6.00	7.95	7.00	4.64	11.26	3.31	10.00	1070
0.15	135.31	238.14	199.83	82.20	394.07	155.93	300.77	6.00	7.93	8.00	4.64	11.22	3.29	10.00	276.64	457.05	385.24	178.80	735.29	278.25	552.93	6.00	8.45	8.00	5.05	11.84	3.39	10.00	997
0.18	136.04	246.65	205.81	77.47	415.84	169.18	303.58	5.00	7.72	7.00	4.45	10.98	3.26	10.00	354.75	582.02	507.60	246.14	917.90	335.88	712.93	6.00	8.34	8.00	4.97	11.71	3.37	10.00	1075
0.32	136.16	247.30	208.59	85.53	409.07	161.77	309.35	5.00	7.69	7.00	4.37	11.01	3.32	10.00	522.48	885.23	758.12	345.39	1425.07	539.84	1101.50	6.00	8.64	8.00	5.19	12.10	3.46	11.00	2658


==> data/mlm_plots/tef/agnews/bert/s/comparison_vals_auc.tex <==
name	auc
orig_pp	70.95
orig_ge	2.24
adv_pp	161.77
adv_ge	2.40


==> data/mlm_plots/tef/agnews/bert/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.53	0.65	0.68	0.45	0.85	0.20	0.81	0.74	0.79	0.83	0.64	0.94	0.15	0.89	0.57	0.64	0.66	0.50	0.78	0.14	0.74	771
0.06	0.32	0.46	0.48	0.24	0.68	0.22	0.62	0.57	0.66	0.71	0.47	0.86	0.19	0.81	0.42	0.51	0.54	0.35	0.67	0.16	0.63	1056
0.11	0.17	0.33	0.33	0.11	0.55	0.22	0.49	0.45	0.57	0.61	0.35	0.78	0.22	0.73	0.33	0.43	0.45	0.26	0.60	0.17	0.55	1070
0.15	0.08	0.21	0.21	0.02	0.41	0.20	0.35	0.34	0.47	0.50	0.25	0.70	0.22	0.63	0.25	0.35	0.36	0.18	0.52	0.17	0.46	997
0.18	0.01	0.14	0.13	-0.05	0.33	0.19	0.26	0.23	0.38	0.40	0.15	0.62	0.23	0.56	0.16	0.28	0.28	0.11	0.45	0.17	0.40	1075
0.32	-0.11	0.02	-0.00	-0.17	0.20	0.18	0.13	0.01	0.20	0.21	-0.06	0.46	0.26	0.38	0.01	0.14	0.14	-0.04	0.32	0.18	0.26	2658


==> data/mlm_plots/tef/agnews/bert/s/correlations_auc.tex <==
name	auc
pcc	0.06
spearman	0.13
kendall	0.10


==> data/mlm_plots/tef/agnews/bert/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	1.51	3.24	2.63	0.79	5.70	2.46	4.14	1.26	3.31	2.44	-0.21	6.83	3.52	4.04	1.51	5.87	3.45	-0.65	12.38	6.51	7.92	771
0.06	1.95	3.19	2.80	1.37	5.00	1.82	4.01	1.66	3.18	2.50	0.77	5.59	2.41	4.04	1.97	7.20	3.97	-0.62	15.02	7.82	9.46	1056
0.11	2.01	3.03	2.76	1.53	4.52	1.49	3.71	1.76	2.99	2.46	1.13	4.86	1.87	3.74	2.09	6.98	3.79	-0.91	14.86	7.88	8.60	1070
0.15	2.03	2.80	2.56	1.64	3.96	1.16	3.38	1.77	2.68	2.36	1.29	4.08	1.39	3.24	2.10	5.35	3.42	-0.82	11.51	6.16	5.91	997
0.18	1.95	2.56	2.40	1.62	3.51	0.94	3.01	1.75	2.45	2.21	1.35	3.55	1.10	2.87	2.04	4.53	3.05	-0.62	9.68	5.15	5.10	1075
0.32	1.82	2.28	2.17	1.58	2.98	0.70	2.62	1.70	2.21	2.07	1.43	2.98	0.77	2.52	1.89	3.61	2.77	0.39	6.84	3.23	4.10	2658


==> data/mlm_plots/tef/agnews/bert/s/ets_sts_auc.tex <==
name	auc
et_use	0.79
et_tse	0.77
et_ce	1.51


==> data/mlm_plots/tef/agnews/bert/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.46	2.68	0.86	-4.35	9.71	7.03	1.92	2.74	8.67	5.51	-0.53	17.88	9.21	11.49	2.76	12.38	6.25	-6.24	31.00	18.62	14.15	771
0.06	0.39	2.19	0.65	-7.49	11.87	9.68	1.32	3.12	7.82	5.29	-0.23	15.87	8.05	9.51	2.91	11.05	5.61	-11.87	33.96	22.92	11.49	1056
0.11	0.32	1.52	0.51	-5.82	8.85	7.33	0.92	3.33	6.82	4.82	0.92	12.72	5.90	8.11	2.88	8.60	5.05	-3.80	20.99	12.39	10.06	1070
0.15	0.26	1.36	0.40	-7.52	10.25	8.89	0.68	3.23	5.84	4.53	1.78	9.89	4.05	7.10	2.77	6.75	4.25	-0.48	13.97	7.23	8.14	997
0.18	0.19	0.70	0.29	-2.05	3.44	2.74	0.48	3.19	5.07	4.17	1.77	8.37	3.30	5.71	2.67	5.87	3.71	-3.88	15.62	9.75	6.42	1075
0.32	0.12	0.35	0.19	-1.25	1.96	1.61	0.31	3.08	4.56	3.86	2.01	7.12	2.55	5.19	2.58	4.99	3.39	-0.04	10.01	5.03	5.34	2658


==> data/mlm_plots/tef/agnews/bert/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.33
et_p_h	1.70
et_p_l2	2.09


==> data/mlm_plots/tef/agnews/bert/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.08	0.22	0.18	0.04	0.40	0.18	0.31	0.01	0.04	0.02	-0.00	0.08	0.04	0.05	0.01	0.04	0.03	0.01	0.07	0.03	0.05	771
0.06	0.20	0.44	0.39	0.13	0.76	0.31	0.60	0.02	0.06	0.04	0.01	0.11	0.05	0.09	0.03	0.06	0.05	0.02	0.09	0.04	0.08	1056
0.11	0.35	0.74	0.65	0.19	1.29	0.55	1.00	0.03	0.08	0.06	0.02	0.13	0.05	0.11	0.04	0.07	0.07	0.03	0.11	0.04	0.10	1070
0.15	0.57	1.11	0.97	0.33	1.89	0.78	1.52	0.05	0.10	0.09	0.04	0.16	0.06	0.14	0.05	0.09	0.09	0.05	0.13	0.04	0.12	997
0.18	0.88	1.68	1.47	0.47	2.89	1.21	2.18	0.07	0.12	0.11	0.06	0.18	0.06	0.16	0.07	0.10	0.10	0.06	0.14	0.04	0.13	1075
0.32	1.53	3.23	2.55	0.72	5.74	2.51	4.12	0.09	0.14	0.14	0.08	0.21	0.07	0.19	0.09	0.13	0.13	0.08	0.17	0.05	0.16	2658


==> data/mlm_plots/tef/agnews/bert/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.46
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/agnews/bert/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.94	0.94	0.91	0.96	0.03	0.95	0.90	0.93	0.94	0.88	0.97	0.04	0.96	0.91	0.94	0.96	0.87	1.00	0.06	0.98	771
0.06	0.89	0.91	0.91	0.87	0.94	0.03	0.93	0.86	0.89	0.90	0.85	0.94	0.05	0.93	0.88	0.92	0.94	0.85	0.99	0.07	0.97	1056
0.11	0.86	0.88	0.88	0.84	0.91	0.04	0.90	0.83	0.87	0.87	0.81	0.92	0.05	0.90	0.85	0.90	0.92	0.82	0.98	0.08	0.96	1070
0.15	0.83	0.85	0.85	0.81	0.89	0.04	0.88	0.80	0.83	0.84	0.78	0.89	0.05	0.87	0.82	0.87	0.89	0.78	0.95	0.09	0.93	997
0.18	0.80	0.82	0.82	0.78	0.86	0.04	0.85	0.77	0.81	0.81	0.75	0.86	0.05	0.85	0.79	0.84	0.86	0.75	0.94	0.09	0.92	1075
0.32	0.74	0.77	0.77	0.73	0.82	0.05	0.81	0.72	0.76	0.76	0.71	0.82	0.06	0.80	0.75	0.80	0.82	0.69	0.91	0.11	0.88	2658


==> data/mlm_plots/tef/agnews/bert/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.25


==> data/mlm_plots/tef/agnews/bert/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.47	0.50	0.50	0.46	0.55	0.05	0.53	1.37	17.99	3.15	-26.57	62.56	44.56	12.27	0.66	1.84	1.39	0.18	3.51	1.66	2.54	771
0.06	0.72	0.83	0.77	0.32	1.34	0.51	0.81	2.15	24.72	4.32	-33.89	83.33	58.61	16.86	0.83	2.37	1.93	0.40	4.34	1.97	3.33	1056
0.11	0.71	0.95	0.78	0.19	1.71	0.76	0.88	3.03	34.62	6.94	-44.84	114.07	79.45	27.23	1.12	2.95	2.52	0.59	5.30	2.35	4.21	1070
0.15	1.03	1.36	1.13	0.36	2.35	1.00	1.26	4.09	47.25	10.03	-46.84	141.35	94.09	41.12	1.32	3.52	2.98	0.87	6.17	2.65	5.30	997
0.18	1.41	1.77	1.53	0.74	2.81	1.04	1.69	4.86	55.91	13.53	-49.36	161.19	105.27	53.11	1.41	3.66	3.10	0.93	6.39	2.73	5.31	1075
0.32	1.97	3.55	2.28	1.39	5.71	2.16	6.36	7.66	86.19	23.47	-54.63	227.02	140.82	104.60	1.83	4.20	3.72	1.25	7.16	2.95	6.16	2658


==> data/mlm_plots/tef/agnews/bert/s/time_misc_auc.tex <==
name	auc
attack_time	0.53
l2	15.22
lom	0.98


==> data/mlm_plots/tef/agnews/bert/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.25	0.46	0.50	0.22	0.70	0.24	0.67	0.62	0.71	0.73	0.58	0.85	0.14	0.80	0.77	0.82	0.84	0.74	0.91	0.09	0.88	771
0.06	0.00	0.29	0.25	0.06	0.52	0.23	0.50	0.53	0.61	0.62	0.47	0.75	0.14	0.70	0.69	0.76	0.78	0.66	0.86	0.10	0.83	1056
0.11	0.00	0.21	0.20	0.00	0.41	0.21	0.33	0.44	0.53	0.54	0.38	0.68	0.15	0.64	0.65	0.72	0.73	0.62	0.82	0.10	0.80	1070
0.15	0.00	0.14	0.00	-0.03	0.32	0.18	0.25	0.38	0.47	0.47	0.32	0.62	0.15	0.57	0.62	0.68	0.68	0.58	0.78	0.10	0.75	997
0.18	0.00	0.10	0.00	-0.05	0.25	0.15	0.20	0.31	0.42	0.42	0.27	0.56	0.14	0.50	0.57	0.64	0.64	0.53	0.75	0.11	0.71	1075
0.32	0.00	0.06	0.00	-0.06	0.18	0.12	0.00	0.20	0.32	0.31	0.17	0.47	0.15	0.42	0.48	0.57	0.57	0.45	0.68	0.11	0.65	2658


==> data/mlm_plots/tef/agnews/bert/s/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.13
top50	0.19


==> data/mlm_plots/tef/agnews/cnn/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	123.44	220.56	181.13	66.90	374.21	153.66	268.50	6.00	8.35	8.00	4.40	12.31	3.95	10.00	147.21	253.23	216.09	91.13	415.33	162.10	312.07	6.00	8.42	8.00	4.44	12.41	3.99	10.00	817
0.06	127.96	231.35	188.79	57.13	405.57	174.22	278.15	5.00	8.10	8.00	4.34	11.86	3.76	10.00	174.20	302.35	253.33	102.44	502.25	199.91	365.73	5.00	8.24	8.00	4.44	12.04	3.80	10.00	1067
0.11	125.68	235.72	188.11	45.11	426.34	190.62	280.18	6.00	8.20	8.00	4.46	11.94	3.74	10.00	201.07	347.84	291.86	109.70	585.98	238.14	424.53	6.00	8.46	8.00	4.65	12.27	3.81	10.00	1038
0.15	124.37	221.43	181.21	65.71	377.15	155.72	269.20	6.00	8.39	8.00	4.59	12.19	3.80	10.00	244.36	398.28	340.17	158.93	637.63	239.35	495.05	6.00	8.80	8.00	4.89	12.71	3.91	11.00	943
0.18	125.80	229.04	185.66	53.94	404.14	175.10	275.88	6.00	8.26	8.00	4.42	12.09	3.83	10.00	295.57	490.01	421.85	192.08	787.95	297.94	606.93	6.00	8.80	8.00	4.83	12.78	3.97	11.00	1045
0.32	125.80	228.09	185.66	59.33	396.86	168.77	275.95	6.00	8.19	8.00	4.45	11.92	3.73	10.00	451.29	768.41	661.08	298.31	1238.51	470.10	956.63	6.00	9.23	9.00	5.27	13.19	3.96	11.00	2968


==> data/mlm_plots/tef/agnews/cnn/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	66.31
orig_ge	2.39
adv_pp	140.24
adv_ge	2.54


==> data/mlm_plots/tef/agnews/cnn/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.64	0.73	0.77	0.54	0.91	0.18	0.86	0.76	0.82	0.84	0.71	0.94	0.11	0.90	0.70	0.76	0.79	0.64	0.88	0.12	0.84	817
0.06	0.41	0.54	0.56	0.32	0.77	0.22	0.71	0.59	0.67	0.68	0.53	0.82	0.15	0.78	0.52	0.60	0.61	0.46	0.74	0.14	0.70	1067
0.11	0.22	0.39	0.40	0.13	0.64	0.25	0.58	0.42	0.53	0.55	0.36	0.70	0.17	0.64	0.37	0.46	0.47	0.31	0.60	0.15	0.56	1038
0.15	0.04	0.22	0.23	-0.05	0.50	0.27	0.43	0.24	0.36	0.36	0.18	0.54	0.18	0.49	0.22	0.31	0.31	0.17	0.45	0.14	0.41	943
0.18	-0.08	0.10	0.10	-0.17	0.38	0.28	0.31	0.10	0.22	0.22	0.03	0.41	0.19	0.35	0.09	0.19	0.19	0.05	0.33	0.14	0.29	1045
0.32	-0.28	-0.08	-0.09	-0.36	0.21	0.29	0.12	-0.17	-0.02	-0.02	-0.24	0.21	0.23	0.14	-0.11	0.00	-0.00	-0.17	0.17	0.17	0.12	2968


==> data/mlm_plots/tef/agnews/cnn/ig/correlations_auc.tex <==
name	auc
pcc	0.06
spearman	0.09
kendall	0.08


==> data/mlm_plots/tef/agnews/cnn/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	1.11	2.21	1.83	0.53	3.89	1.68	2.84	0.91	2.18	1.64	0.35	4.01	1.83	2.82	1.31	4.92	2.96	-0.71	10.54	5.63	6.43	817
0.06	1.44	2.42	2.20	1.00	3.85	1.43	3.10	1.21	2.23	1.84	0.71	3.74	1.52	2.88	1.73	5.75	3.34	-0.72	12.22	6.47	7.07	1067
0.11	1.60	2.47	2.31	1.27	3.68	1.21	3.10	1.37	2.25	1.95	0.96	3.54	1.29	2.87	1.84	5.22	3.17	-0.74	11.18	5.96	5.91	1038
0.15	1.74	2.51	2.38	1.42	3.61	1.09	3.06	1.55	2.26	2.08	1.20	3.33	1.07	2.80	2.01	5.12	3.15	-0.82	11.06	5.94	5.54	943
0.18	1.79	2.42	2.33	1.50	3.35	0.93	2.97	1.61	2.19	2.10	1.29	3.10	0.91	2.63	2.06	4.36	3.16	0.03	8.69	4.33	4.86	1045
0.32	1.78	2.27	2.21	1.53	3.01	0.74	2.71	1.64	2.10	2.06	1.40	2.80	0.70	2.46	1.93	3.59	2.88	0.59	6.60	3.00	4.19	2968


==> data/mlm_plots/tef/agnews/cnn/ig/ets_sts_auc.tex <==
name	auc
et_use	0.69
et_tse	0.64
et_ce	1.34


==> data/mlm_plots/tef/agnews/cnn/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.35	2.44	0.70	-4.66	9.55	7.11	1.63	2.49	7.97	5.09	-1.25	17.19	9.22	9.67	2.52	11.26	5.36	-6.34	28.86	17.60	12.13	817
0.06	0.35	2.10	0.67	-5.95	10.14	8.05	1.35	2.92	7.81	5.28	-0.05	15.67	7.86	9.76	2.68	10.38	5.66	-5.42	26.17	15.79	12.09	1067
0.11	0.31	1.65	0.56	-6.04	9.35	7.69	1.04	3.10	7.34	5.01	0.33	14.36	7.01	9.02	2.75	9.57	5.23	-7.60	26.74	17.17	10.54	1038
0.15	0.27	1.12	0.44	-3.63	5.88	4.75	0.74	3.28	6.56	4.98	1.45	11.67	5.11	8.16	2.80	7.96	4.71	-3.33	19.25	11.29	9.45	943
0.18	0.22	0.92	0.36	-3.79	5.64	4.72	0.60	3.32	5.96	4.81	1.67	10.25	4.29	7.04	2.87	7.21	4.37	-5.71	20.12	12.91	8.00	1045
0.32	0.13	0.41	0.22	-1.12	1.94	1.53	0.38	3.29	5.06	4.38	2.19	7.94	2.88	5.97	2.81	5.65	3.91	-2.31	13.61	7.96	6.13	2968


==> data/mlm_plots/tef/agnews/cnn/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.34
et_p_h	1.85
et_p_l2	2.30


==> data/mlm_plots/tef/agnews/cnn/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.08	0.20	0.16	0.03	0.36	0.16	0.28	0.01	0.03	0.02	-0.00	0.07	0.03	0.04	0.01	0.03	0.02	0.00	0.06	0.03	0.04	817
0.06	0.15	0.38	0.32	0.09	0.67	0.29	0.54	0.02	0.05	0.04	0.01	0.09	0.04	0.07	0.02	0.05	0.04	0.02	0.08	0.03	0.07	1067
0.11	0.28	0.61	0.53	0.15	1.07	0.46	0.80	0.03	0.07	0.05	0.02	0.12	0.05	0.10	0.03	0.06	0.06	0.03	0.10	0.04	0.09	1038
0.15	0.48	0.98	0.86	0.28	1.67	0.69	1.28	0.04	0.09	0.08	0.03	0.14	0.06	0.13	0.05	0.08	0.08	0.04	0.12	0.04	0.11	943
0.18	0.71	1.43	1.25	0.43	2.42	1.00	1.89	0.06	0.10	0.10	0.05	0.16	0.06	0.15	0.06	0.09	0.09	0.05	0.14	0.04	0.12	1045
0.32	1.36	3.04	2.37	0.55	5.54	2.49	3.93	0.08	0.14	0.14	0.07	0.20	0.07	0.19	0.09	0.12	0.12	0.08	0.17	0.05	0.16	2968


==> data/mlm_plots/tef/agnews/cnn/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/tef/agnews/cnn/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.93	0.94	0.91	0.96	0.02	0.95	0.89	0.92	0.93	0.87	0.96	0.05	0.95	0.92	0.94	0.96	0.89	1.00	0.05	0.98	817
0.06	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.85	0.88	0.89	0.83	0.93	0.05	0.92	0.89	0.92	0.94	0.85	0.99	0.07	0.97	1067
0.11	0.85	0.87	0.87	0.83	0.90	0.03	0.89	0.82	0.85	0.85	0.80	0.90	0.05	0.89	0.85	0.89	0.91	0.81	0.97	0.08	0.95	1038
0.15	0.81	0.84	0.84	0.80	0.87	0.04	0.86	0.78	0.82	0.82	0.77	0.86	0.05	0.85	0.82	0.87	0.88	0.79	0.95	0.08	0.93	943
0.18	0.78	0.81	0.81	0.77	0.85	0.04	0.83	0.75	0.78	0.79	0.73	0.83	0.05	0.82	0.80	0.85	0.86	0.76	0.93	0.09	0.91	1045
0.32	0.72	0.75	0.75	0.71	0.80	0.05	0.79	0.70	0.73	0.73	0.68	0.79	0.05	0.77	0.74	0.80	0.81	0.70	0.90	0.10	0.87	2968


==> data/mlm_plots/tef/agnews/cnn/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.23
sts_ce	0.25


==> data/mlm_plots/tef/agnews/cnn/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.66	0.69	0.69	0.64	0.73	0.04	0.71	3.65	5.90	5.37	2.90	8.91	3.01	7.38	0.54	1.73	1.10	-0.15	3.60	1.88	2.27	817
0.06	0.86	0.91	0.90	0.83	0.98	0.07	0.92	5.11	7.88	7.28	4.28	11.48	3.60	9.96	0.81	2.49	1.81	0.22	4.76	2.27	3.58	1067
0.11	1.10	1.16	1.13	1.02	1.29	0.13	1.15	6.31	9.54	8.98	5.46	13.63	4.08	12.09	1.18	3.17	2.58	0.58	5.76	2.59	4.50	1038
0.15	1.49	1.53	1.55	1.46	1.60	0.07	1.57	7.70	11.26	10.44	6.58	15.93	4.68	14.28	1.57	3.98	3.31	0.92	7.05	3.07	5.76	943
0.18	1.82	1.88	1.88	1.76	2.00	0.12	1.92	8.40	12.46	11.60	7.37	17.56	5.10	15.87	1.93	4.43	3.84	1.22	7.65	3.22	6.33	1045
0.32	2.32	2.90	2.99	2.39	3.41	0.51	3.44	10.02	14.41	13.36	8.64	20.19	5.77	18.24	2.18	4.92	4.40	1.51	8.34	3.42	7.13	2968


==> data/mlm_plots/tef/agnews/cnn/ig/time_misc_auc.tex <==
name	auc
attack_time	0.51
l2	3.30
lom	1.13


==> data/mlm_plots/tef/agnews/cnn/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.60	0.66	0.67	0.50	0.82	0.16	0.75	0.80	0.85	0.87	0.75	0.94	0.09	0.92	0.86	0.89	0.90	0.82	0.96	0.07	0.94	817
0.06	0.33	0.47	0.50	0.26	0.69	0.21	0.60	0.69	0.75	0.75	0.64	0.86	0.11	0.82	0.78	0.83	0.84	0.75	0.90	0.08	0.88	1067
0.11	0.25	0.37	0.33	0.15	0.59	0.22	0.50	0.59	0.66	0.67	0.55	0.78	0.11	0.75	0.71	0.76	0.78	0.68	0.85	0.08	0.82	1038
0.15	0.20	0.30	0.25	0.07	0.52	0.22	0.50	0.50	0.56	0.57	0.45	0.68	0.11	0.64	0.65	0.70	0.70	0.61	0.78	0.08	0.76	943
0.18	0.00	0.25	0.25	0.04	0.46	0.21	0.40	0.40	0.48	0.50	0.36	0.60	0.12	0.56	0.59	0.64	0.64	0.55	0.72	0.08	0.70	1045
0.32	0.00	0.18	0.20	-0.01	0.38	0.20	0.33	0.27	0.36	0.36	0.23	0.50	0.14	0.45	0.47	0.53	0.53	0.43	0.63	0.10	0.60	2968


==> data/mlm_plots/tef/agnews/cnn/ig/top_intersections_auc.tex <==
name	auc
top10	0.09
top30	0.16
top50	0.20


==> data/mlm_plots/tef/agnews/cnn/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	122.77	216.49	181.21	71.51	361.46	144.97	263.02	6.00	8.54	8.00	4.63	12.45	3.91	10.00	149.60	253.48	216.48	88.46	418.50	165.02	307.05	6.00	8.66	8.00	4.73	12.60	3.93	11.00	762
0.06	127.61	227.08	188.07	68.25	385.91	158.83	277.70	5.25	8.20	8.00	4.42	11.98	3.78	10.00	179.41	301.61	253.15	115.71	487.51	185.90	371.15	6.00	8.43	8.00	4.59	12.26	3.83	10.00	1034
0.11	125.32	232.06	185.43	51.41	412.71	180.65	277.50	6.00	8.24	8.00	4.50	11.99	3.75	10.00	207.81	358.25	296.04	123.47	593.04	234.79	432.88	6.00	8.61	8.00	4.74	12.48	3.87	11.00	1022
0.15	123.44	220.41	180.70	66.72	374.11	153.69	269.04	6.00	8.40	8.00	4.60	12.21	3.80	10.00	250.23	414.38	356.25	170.16	658.60	244.22	510.65	6.00	9.03	9.00	5.10	12.96	3.93	11.00	940
0.18	125.61	226.61	185.18	59.34	393.88	167.27	272.64	6.00	8.30	8.00	4.48	12.12	3.82	10.00	312.40	502.86	436.15	214.97	790.76	287.89	630.08	6.00	9.09	9.00	5.08	13.10	4.01	11.00	1044
0.32	125.50	229.52	185.49	53.62	405.42	175.90	275.95	6.00	8.17	8.00	4.46	11.88	3.71	10.00	451.13	763.18	661.34	293.53	1232.83	469.65	930.62	7.00	9.59	9.00	5.54	13.63	4.04	12.00	2962


==> data/mlm_plots/tef/agnews/cnn/s/comparison_vals_auc.tex <==
name	auc
orig_pp	65.78
orig_ge	2.40
adv_pp	142.07
adv_ge	2.61


==> data/mlm_plots/tef/agnews/cnn/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.80	0.85	0.88	0.72	0.97	0.13	0.94	0.80	0.85	0.88	0.73	0.98	0.12	0.94	0.70	0.77	0.78	0.65	0.89	0.12	0.86	762
0.06	0.66	0.73	0.78	0.55	0.92	0.18	0.86	0.67	0.75	0.79	0.58	0.92	0.17	0.87	0.54	0.64	0.65	0.48	0.79	0.15	0.74	1034
0.11	0.53	0.64	0.69	0.43	0.85	0.21	0.79	0.54	0.65	0.70	0.45	0.85	0.20	0.80	0.42	0.53	0.55	0.36	0.70	0.17	0.64	1022
0.15	0.36	0.51	0.57	0.27	0.76	0.24	0.69	0.39	0.53	0.57	0.29	0.76	0.23	0.70	0.29	0.40	0.43	0.22	0.58	0.18	0.53	940
0.18	0.22	0.39	0.44	0.12	0.67	0.27	0.60	0.25	0.41	0.43	0.14	0.67	0.26	0.61	0.18	0.30	0.31	0.11	0.50	0.20	0.45	1044
0.32	-0.14	0.11	0.13	-0.24	0.45	0.34	0.38	-0.16	0.10	0.12	-0.25	0.45	0.35	0.37	-0.09	0.08	0.09	-0.16	0.32	0.24	0.26	2962


==> data/mlm_plots/tef/agnews/cnn/s/correlations_auc.tex <==
name	auc
pcc	0.13
spearman	0.13
kendall	0.11


==> data/mlm_plots/tef/agnews/cnn/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	0.54	1.45	1.01	0.01	2.89	1.44	1.84	0.47	1.59	0.92	-0.40	3.58	1.99	1.82	0.60	2.87	1.50	-0.61	6.36	3.48	3.81	762
0.06	0.73	1.63	1.27	0.32	2.94	1.31	2.05	0.65	1.65	1.16	-0.19	3.49	1.84	1.92	0.89	3.72	1.99	-0.99	8.43	4.71	4.47	1034
0.11	0.86	1.65	1.35	0.52	2.78	1.13	2.15	0.75	1.60	1.22	0.27	2.93	1.33	2.02	1.07	3.43	2.03	-0.77	7.62	4.20	3.98	1022
0.15	1.01	1.77	1.48	0.70	2.83	1.07	2.33	0.91	1.66	1.34	0.50	2.82	1.16	2.08	1.21	3.56	2.16	-1.06	8.18	4.62	3.91	940
0.18	1.09	1.80	1.59	0.84	2.76	0.96	2.30	0.99	1.69	1.47	0.71	2.67	0.98	2.16	1.31	3.27	2.17	-0.47	7.02	3.75	3.73	1044
0.32	1.33	1.95	1.84	1.13	2.77	0.82	2.43	1.25	1.87	1.74	1.01	2.73	0.86	2.30	1.52	3.01	2.29	0.13	5.89	2.88	3.52	2962


==> data/mlm_plots/tef/agnews/cnn/s/ets_sts_auc.tex <==
name	auc
et_use	0.51
et_tse	0.49
et_ce	0.96


==> data/mlm_plots/tef/agnews/cnn/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.17	0.90	0.32	-1.80	3.61	2.70	0.69	0.92	3.29	2.13	-0.41	6.98	3.69	4.33	0.95	5.60	2.27	-6.80	18.00	12.40	5.61	762
0.06	0.18	0.85	0.33	-1.81	3.51	2.66	0.62	1.30	3.66	2.39	-0.31	7.63	3.97	4.36	1.28	5.44	2.46	-5.37	16.24	10.80	5.40	1034
0.11	0.15	0.68	0.29	-1.98	3.35	2.67	0.52	1.51	3.50	2.45	-0.17	7.18	3.67	4.18	1.38	4.70	2.39	-4.85	14.25	9.55	4.74	1022
0.15	0.14	0.58	0.24	-2.14	3.29	2.72	0.43	1.70	3.33	2.61	0.75	5.92	2.58	4.15	1.48	3.96	2.47	-1.26	9.18	5.22	4.35	940
0.18	0.13	0.38	0.22	-0.54	1.30	0.92	0.36	1.93	3.46	2.83	0.99	5.94	2.47	4.08	1.68	4.11	2.65	-1.83	10.04	5.94	4.40	1044
0.32	0.11	0.36	0.17	-1.58	2.31	1.94	0.29	2.42	3.88	3.36	1.43	6.33	2.45	4.59	2.09	4.61	3.01	-4.35	13.57	8.96	4.57	2962


==> data/mlm_plots/tef/agnews/cnn/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.16
et_p_h	1.03
et_p_l2	1.32


==> data/mlm_plots/tef/agnews/cnn/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.10	0.22	0.19	0.06	0.38	0.16	0.30	0.01	0.04	0.02	-0.00	0.08	0.04	0.05	0.01	0.04	0.03	0.01	0.07	0.03	0.05	762
0.06	0.20	0.41	0.35	0.11	0.70	0.30	0.55	0.02	0.06	0.04	0.01	0.11	0.05	0.09	0.03	0.05	0.05	0.02	0.09	0.03	0.08	1034
0.11	0.34	0.68	0.57	0.20	1.16	0.48	0.90	0.03	0.08	0.06	0.03	0.13	0.05	0.12	0.04	0.07	0.07	0.03	0.11	0.04	0.10	1022
0.15	0.57	1.06	0.91	0.37	1.76	0.70	1.41	0.05	0.10	0.09	0.04	0.16	0.06	0.15	0.06	0.09	0.09	0.05	0.13	0.04	0.12	940
0.18	0.80	1.52	1.32	0.52	2.52	1.00	1.97	0.06	0.12	0.12	0.06	0.18	0.06	0.16	0.07	0.10	0.10	0.06	0.15	0.04	0.13	1044
0.32	1.44	2.98	2.45	0.71	5.26	2.28	3.91	0.09	0.15	0.15	0.08	0.22	0.07	0.19	0.10	0.13	0.13	0.09	0.18	0.05	0.16	2962


==> data/mlm_plots/tef/agnews/cnn/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.42
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/agnews/cnn/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.96	0.91	0.93	0.94	0.89	0.97	0.04	0.96	0.93	0.95	0.96	0.89	1.00	0.05	0.98	762
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.87	0.90	0.90	0.85	0.94	0.05	0.93	0.89	0.93	0.94	0.86	0.99	0.06	0.97	1034
0.11	0.86	0.88	0.88	0.85	0.91	0.03	0.90	0.83	0.87	0.87	0.82	0.91	0.05	0.90	0.87	0.90	0.92	0.83	0.97	0.07	0.95	1022
0.15	0.83	0.85	0.85	0.82	0.89	0.03	0.87	0.80	0.83	0.84	0.79	0.88	0.05	0.87	0.84	0.88	0.89	0.80	0.96	0.08	0.94	940
0.18	0.80	0.82	0.82	0.78	0.86	0.04	0.85	0.77	0.80	0.80	0.75	0.86	0.05	0.84	0.81	0.86	0.87	0.77	0.94	0.08	0.92	1044
0.32	0.73	0.76	0.76	0.71	0.81	0.05	0.80	0.71	0.75	0.75	0.69	0.81	0.06	0.79	0.75	0.80	0.81	0.69	0.90	0.10	0.87	2962


==> data/mlm_plots/tef/agnews/cnn/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.25


==> data/mlm_plots/tef/agnews/cnn/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.30	0.32	0.32	0.29	0.34	0.03	0.32	39.18	65.83	57.94	29.09	102.58	36.75	83.57	0.51	1.11	0.89	0.24	1.97	0.87	1.49	762
0.06	0.46	0.48	0.49	0.44	0.53	0.04	0.50	55.33	89.92	80.56	44.90	134.95	45.03	115.30	0.61	1.48	1.23	0.37	2.58	1.11	2.04	1034
0.11	0.57	0.62	0.59	0.52	0.71	0.10	0.61	71.89	111.29	101.40	59.97	162.62	51.33	140.91	0.68	1.76	1.46	0.40	3.11	1.35	2.57	1022
0.15	0.86	0.89	0.89	0.86	0.93	0.04	0.92	91.45	138.82	128.81	77.94	199.70	60.88	181.27	0.93	2.15	1.80	0.57	3.72	1.57	3.06	940
0.18	1.04	1.09	1.09	0.99	1.19	0.10	1.11	104.66	159.60	147.98	89.72	229.47	69.87	204.09	0.95	2.38	2.03	0.63	4.12	1.75	3.42	1044
0.32	1.33	1.79	1.74	1.33	2.25	0.46	2.35	137.48	214.37	196.80	116.73	312.01	97.64	277.13	1.24	2.92	2.58	0.82	5.02	2.10	4.25	2962


==> data/mlm_plots/tef/agnews/cnn/s/time_misc_auc.tex <==
name	auc
attack_time	0.30
l2	42.96
lom	0.64


==> data/mlm_plots/tef/agnews/cnn/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.40	0.62	0.67	0.32	0.92	0.30	0.80	0.69	0.78	0.79	0.64	0.92	0.14	0.88	0.81	0.87	0.88	0.78	0.96	0.09	0.93	762
0.06	0.25	0.47	0.50	0.15	0.78	0.31	0.67	0.58	0.67	0.69	0.52	0.83	0.15	0.78	0.74	0.80	0.81	0.70	0.91	0.10	0.88	1034
0.11	0.00	0.36	0.33	0.06	0.66	0.30	0.60	0.50	0.60	0.62	0.44	0.77	0.17	0.71	0.69	0.75	0.75	0.65	0.86	0.11	0.82	1022
0.15	0.00	0.27	0.20	-0.01	0.55	0.28	0.50	0.40	0.51	0.50	0.34	0.68	0.17	0.62	0.62	0.69	0.70	0.58	0.81	0.12	0.77	940
0.18	0.00	0.21	0.00	-0.05	0.47	0.26	0.33	0.31	0.43	0.44	0.25	0.61	0.18	0.56	0.56	0.64	0.64	0.51	0.76	0.12	0.72	1044
0.32	0.00	0.12	0.00	-0.09	0.33	0.21	0.20	0.14	0.29	0.27	0.10	0.48	0.19	0.42	0.40	0.51	0.50	0.35	0.66	0.15	0.62	2962


==> data/mlm_plots/tef/agnews/cnn/s/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.14
top50	0.19


==> data/mlm_plots/tef/agnews/lstm/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	123.47	220.18	184.15	59.68	380.67	160.49	266.64	6.00	8.36	8.00	4.55	12.17	3.81	10.00	146.41	248.91	211.43	78.99	418.84	169.93	305.18	6.00	8.42	8.00	4.60	12.23	3.81	10.00	790
0.06	127.80	231.47	190.79	55.90	407.04	175.57	280.09	5.00	8.00	8.00	4.31	11.69	3.69	10.00	172.83	300.10	246.96	86.57	513.62	213.52	363.38	5.00	8.10	8.00	4.40	11.81	3.70	10.00	1019
0.11	125.32	232.40	188.74	51.37	413.42	181.03	276.96	6.00	8.15	8.00	4.47	11.83	3.68	10.00	206.28	348.53	289.82	113.34	583.72	235.19	425.07	6.00	8.36	8.00	4.65	12.07	3.71	10.00	1002
0.15	125.50	221.78	182.60	68.15	375.42	153.63	271.87	6.00	8.32	8.00	4.58	12.05	3.74	10.00	242.28	401.49	343.49	159.41	643.58	242.08	492.78	6.00	8.69	8.00	4.91	12.46	3.77	11.00	899
0.18	127.55	231.04	189.60	56.15	405.92	174.89	275.20	6.00	8.33	8.00	4.43	12.22	3.90	10.00	300.88	499.85	437.82	197.53	802.16	302.31	596.07	6.00	8.82	8.00	4.86	12.79	3.97	11.00	1043
0.32	125.80	227.91	188.10	60.57	395.24	167.33	276.88	6.00	8.07	8.00	4.49	11.65	3.58	10.00	456.25	764.23	649.34	299.82	1228.65	464.41	936.02	6.00	9.02	9.00	5.23	12.81	3.79	11.00	2813


==> data/mlm_plots/tef/agnews/lstm/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	66.33
orig_ge	2.38
adv_pp	140.80
adv_ge	2.51


==> data/mlm_plots/tef/agnews/lstm/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.34	0.54	0.61	0.23	0.85	0.31	0.80	0.66	0.73	0.78	0.52	0.94	0.21	0.85	0.56	0.65	0.71	0.45	0.86	0.20	0.79	790
0.06	0.08	0.32	0.35	-0.02	0.67	0.34	0.59	0.48	0.57	0.62	0.34	0.81	0.24	0.73	0.41	0.51	0.55	0.29	0.72	0.21	0.65	1019
0.11	-0.08	0.17	0.18	-0.17	0.52	0.34	0.44	0.33	0.44	0.47	0.20	0.67	0.23	0.59	0.28	0.38	0.41	0.18	0.58	0.20	0.52	1002
0.15	-0.22	0.01	-0.02	-0.31	0.34	0.33	0.24	0.14	0.28	0.31	0.04	0.51	0.24	0.43	0.13	0.25	0.28	0.06	0.44	0.19	0.38	899
0.18	-0.31	-0.09	-0.12	-0.41	0.23	0.32	0.11	-0.00	0.15	0.17	-0.09	0.38	0.24	0.31	0.02	0.14	0.17	-0.05	0.33	0.19	0.27	1043
0.32	-0.45	-0.21	-0.25	-0.52	0.09	0.30	-0.02	-0.18	-0.02	-0.02	-0.26	0.22	0.24	0.15	-0.11	0.01	0.01	-0.17	0.19	0.18	0.13	2813


==> data/mlm_plots/tef/agnews/lstm/ig/correlations_auc.tex <==
name	auc
pcc	0.01
spearman	0.07
kendall	0.07


==> data/mlm_plots/tef/agnews/lstm/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	1.59	3.85	2.88	0.72	6.97	3.13	5.27	1.22	3.18	2.25	0.24	6.13	2.95	4.30	2.04	8.36	5.29	-1.12	17.84	9.48	10.70	790
0.06	2.12	3.69	3.25	1.34	6.04	2.35	4.73	1.69	3.10	2.62	0.95	5.26	2.15	3.99	2.54	9.17	5.33	-1.01	19.35	10.18	11.91	1019
0.11	2.12	3.46	3.15	1.55	5.38	1.92	4.39	1.83	2.95	2.56	1.17	4.73	1.78	3.64	2.67	8.56	4.90	-1.26	18.38	9.82	9.97	1002
0.15	2.27	3.28	3.13	1.80	4.76	1.48	3.99	1.96	2.85	2.60	1.46	4.23	1.38	3.45	2.72	7.16	4.49	-0.90	15.22	8.06	7.84	899
0.18	2.26	3.00	2.87	1.82	4.18	1.18	3.58	1.98	2.68	2.49	1.56	3.81	1.13	3.23	2.63	5.85	4.15	0.03	11.67	5.82	6.68	1043
0.32	2.07	2.65	2.56	1.73	3.58	0.93	3.11	1.91	2.46	2.33	1.60	3.33	0.86	2.88	2.38	4.43	3.49	1.00	7.86	3.43	5.12	2813


==> data/mlm_plots/tef/agnews/lstm/ig/ets_sts_auc.tex <==
name	auc
et_use	0.92
et_tse	0.81
et_ce	1.94


==> data/mlm_plots/tef/agnews/lstm/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.56	4.56	1.34	-10.39	19.52	14.95	3.17	3.92	12.46	7.81	-0.88	25.81	13.35	16.26	3.74	15.18	8.10	-6.73	37.08	21.90	18.81	790
0.06	0.52	2.55	0.99	-4.92	10.01	7.46	2.12	4.15	10.88	7.61	0.65	21.11	10.23	14.73	3.91	13.53	7.64	-6.76	33.82	20.29	16.44	1019
0.11	0.40	1.90	0.77	-3.99	7.80	5.89	1.49	4.06	9.24	6.83	0.99	17.48	8.24	11.39	3.59	11.47	6.57	-7.90	30.83	19.36	13.23	1002
0.15	0.32	1.35	0.56	-3.56	6.27	4.92	1.04	4.22	8.09	6.23	1.47	14.70	6.61	9.85	3.66	9.88	5.85	-7.53	27.29	17.41	10.59	899
0.18	0.25	0.92	0.41	-2.14	3.98	3.06	0.75	4.07	7.35	5.83	1.60	13.11	5.75	8.42	3.48	9.39	5.26	-9.96	28.74	19.35	9.25	1043
0.32	0.15	0.49	0.25	-1.82	2.80	2.31	0.44	3.72	5.94	4.93	1.93	9.96	4.02	6.87	3.18	7.02	4.45	-5.82	19.86	12.84	7.14	2813


==> data/mlm_plots/tef/agnews/lstm/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.42
et_p_h	2.36
et_p_l2	2.92


==> data/mlm_plots/tef/agnews/lstm/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.07	0.19	0.15	0.03	0.35	0.16	0.26	0.01	0.03	0.02	0.00	0.06	0.03	0.04	0.01	0.03	0.02	0.01	0.05	0.02	0.04	790
0.06	0.16	0.38	0.32	0.07	0.68	0.30	0.52	0.02	0.05	0.04	0.01	0.09	0.04	0.07	0.02	0.05	0.04	0.02	0.08	0.03	0.07	1019
0.11	0.28	0.63	0.51	0.12	1.14	0.51	0.85	0.03	0.07	0.05	0.02	0.12	0.05	0.10	0.04	0.06	0.06	0.03	0.10	0.04	0.09	1002
0.15	0.47	0.99	0.86	0.28	1.70	0.71	1.34	0.04	0.09	0.08	0.04	0.14	0.05	0.13	0.05	0.08	0.08	0.04	0.12	0.04	0.11	899
0.18	0.74	1.47	1.26	0.43	2.51	1.04	1.97	0.06	0.11	0.10	0.05	0.16	0.06	0.15	0.06	0.10	0.09	0.06	0.14	0.04	0.12	1043
0.32	1.38	3.03	2.33	0.58	5.49	2.46	3.93	0.08	0.14	0.14	0.07	0.21	0.07	0.18	0.09	0.12	0.12	0.08	0.17	0.05	0.16	2813


==> data/mlm_plots/tef/agnews/lstm/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/tef/agnews/lstm/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.93	0.93	0.91	0.96	0.02	0.95	0.88	0.91	0.92	0.87	0.95	0.04	0.94	0.92	0.94	0.96	0.89	1.00	0.05	0.98	790
0.06	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.84	0.87	0.88	0.82	0.92	0.05	0.91	0.89	0.92	0.94	0.86	0.99	0.06	0.97	1019
0.11	0.85	0.87	0.87	0.83	0.91	0.04	0.89	0.81	0.84	0.85	0.79	0.90	0.05	0.88	0.87	0.91	0.92	0.83	0.98	0.07	0.96	1002
0.15	0.81	0.84	0.84	0.80	0.88	0.04	0.87	0.77	0.81	0.81	0.76	0.86	0.05	0.85	0.83	0.88	0.89	0.80	0.96	0.08	0.94	899
0.18	0.78	0.81	0.81	0.77	0.85	0.04	0.83	0.75	0.78	0.78	0.73	0.84	0.05	0.82	0.81	0.86	0.87	0.77	0.94	0.08	0.92	1043
0.32	0.73	0.76	0.76	0.71	0.81	0.05	0.79	0.70	0.74	0.74	0.69	0.80	0.06	0.78	0.76	0.81	0.83	0.71	0.91	0.10	0.88	2813


==> data/mlm_plots/tef/agnews/lstm/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.23
sts_ce	0.25


==> data/mlm_plots/tef/agnews/lstm/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.27	0.29	0.29	0.26	0.31	0.02	0.30	0.93	1.66	1.36	0.54	2.79	1.13	2.07	0.71	2.89	1.60	-1.13	6.91	4.02	3.21	790
0.06	0.40	0.43	0.42	0.34	0.53	0.09	0.44	1.27	2.16	1.79	0.71	3.60	1.44	2.52	1.02	3.99	2.49	-1.31	9.29	5.30	4.87	1019
0.11	0.56	0.59	0.56	0.48	0.70	0.11	0.58	1.56	2.54	2.15	0.93	4.15	1.61	2.91	1.52	4.86	3.37	-0.39	10.11	5.25	6.22	1002
0.15	0.79	0.81	0.81	0.73	0.89	0.08	0.83	1.85	2.87	2.42	1.15	4.60	1.72	3.32	2.08	5.92	4.24	-0.04	11.88	5.96	7.54	899
0.18	1.12	1.17	1.14	1.02	1.32	0.15	1.19	2.00	3.11	2.61	1.28	4.95	1.84	3.57	2.39	7.06	4.94	0.19	13.93	6.87	9.48	1043
0.32	1.44	1.73	1.79	1.46	1.99	0.26	1.98	2.18	3.32	2.74	1.36	5.28	1.96	3.79	2.71	7.82	5.84	0.59	15.06	7.23	10.49	2813


==> data/mlm_plots/tef/agnews/lstm/ig/time_misc_auc.tex <==
name	auc
attack_time	0.30
l2	0.82
lom	1.78


==> data/mlm_plots/tef/agnews/lstm/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.50	0.60	0.60	0.38	0.83	0.23	0.75	0.69	0.77	0.80	0.62	0.92	0.15	0.88	0.79	0.84	0.86	0.73	0.95	0.11	0.91	790
0.06	0.25	0.41	0.40	0.16	0.67	0.26	0.60	0.60	0.68	0.71	0.51	0.84	0.17	0.80	0.72	0.77	0.80	0.65	0.89	0.12	0.86	1019
0.11	0.20	0.32	0.25	0.07	0.56	0.25	0.50	0.50	0.60	0.62	0.44	0.76	0.16	0.71	0.65	0.72	0.74	0.60	0.84	0.12	0.80	1002
0.15	0.00	0.24	0.25	0.01	0.47	0.23	0.40	0.43	0.52	0.54	0.36	0.67	0.15	0.62	0.59	0.66	0.67	0.54	0.78	0.12	0.74	899
0.18	0.00	0.21	0.20	-0.02	0.44	0.23	0.33	0.33	0.44	0.45	0.29	0.59	0.15	0.56	0.55	0.61	0.62	0.49	0.72	0.11	0.69	1043
0.32	0.00	0.17	0.00	-0.04	0.38	0.21	0.33	0.25	0.36	0.36	0.21	0.50	0.15	0.45	0.47	0.54	0.55	0.43	0.65	0.11	0.62	2813


==> data/mlm_plots/tef/agnews/lstm/ig/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.15
top50	0.19


==> data/mlm_plots/tef/agnews/lstm/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	125.07	219.76	184.94	70.50	369.03	149.27	266.54	6.00	8.49	8.00	4.62	12.37	3.87	10.00	148.59	253.44	212.57	85.42	421.47	168.03	309.91	6.00	8.58	8.00	4.67	12.49	3.91	11.00	735
0.06	127.74	230.39	189.98	54.87	405.90	175.52	276.98	5.00	8.04	8.00	4.33	11.74	3.71	10.00	173.03	304.93	251.87	95.16	514.71	209.77	373.43	5.00	8.20	8.00	4.45	11.95	3.75	10.00	990
0.11	124.25	229.30	187.59	50.80	407.80	178.50	272.21	6.00	8.14	8.00	4.47	11.81	3.67	10.00	203.03	350.32	298.06	118.55	582.09	231.77	432.93	6.00	8.41	8.00	4.67	12.14	3.73	10.00	988
0.15	124.28	220.65	182.21	67.75	373.55	152.90	269.51	6.00	8.40	8.00	4.62	12.18	3.78	10.00	249.52	415.23	344.49	158.53	671.93	256.70	510.69	6.00	8.85	8.00	4.98	12.71	3.87	11.00	905
0.18	126.16	228.03	186.67	56.51	399.55	171.52	272.73	6.00	8.17	8.00	4.42	11.92	3.75	10.00	312.43	524.78	434.03	199.43	850.13	325.35	644.69	6.00	8.81	8.00	4.93	12.69	3.88	11.00	1001
0.32	126.54	229.73	188.47	58.58	400.89	171.16	277.70	6.00	8.11	8.00	4.49	11.73	3.62	10.00	467.90	792.50	675.22	303.33	1281.67	489.17	972.32	6.00	9.20	9.00	5.36	13.05	3.85	11.00	2846


==> data/mlm_plots/tef/agnews/lstm/s/comparison_vals_auc.tex <==
name	auc
orig_pp	65.97
orig_ge	2.37
adv_pp	145.71
adv_ge	2.54


==> data/mlm_plots/tef/agnews/lstm/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.40	0.55	0.57	0.35	0.75	0.20	0.71	0.69	0.77	0.81	0.62	0.92	0.15	0.88	0.55	0.65	0.67	0.49	0.81	0.16	0.77	735
0.06	0.25	0.39	0.39	0.19	0.58	0.20	0.52	0.55	0.66	0.68	0.48	0.83	0.17	0.79	0.42	0.52	0.53	0.36	0.69	0.16	0.64	990
0.11	0.13	0.26	0.25	0.08	0.43	0.18	0.37	0.42	0.54	0.56	0.34	0.74	0.20	0.68	0.31	0.41	0.42	0.25	0.58	0.16	0.53	988
0.15	0.04	0.14	0.13	-0.01	0.30	0.16	0.25	0.29	0.42	0.43	0.22	0.62	0.20	0.57	0.20	0.31	0.31	0.16	0.47	0.15	0.42	905
0.18	-0.03	0.06	0.04	-0.09	0.20	0.15	0.14	0.17	0.30	0.31	0.10	0.51	0.20	0.45	0.12	0.22	0.22	0.07	0.37	0.15	0.32	1001
0.32	-0.18	-0.08	-0.09	-0.23	0.06	0.14	0.00	-0.07	0.08	0.09	-0.14	0.30	0.22	0.24	-0.05	0.06	0.05	-0.10	0.21	0.16	0.16	2846


==> data/mlm_plots/tef/agnews/lstm/s/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.11
kendall	0.08


==> data/mlm_plots/tef/agnews/lstm/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	2.35	4.01	3.58	1.56	6.46	2.45	5.11	1.86	3.81	2.92	0.72	6.90	3.09	4.83	3.06	8.96	6.18	1.04	16.89	7.92	12.45	735
0.06	2.48	3.58	3.27	1.85	5.30	1.72	4.35	1.92	3.23	2.70	1.11	5.34	2.11	3.90	2.94	9.06	5.76	0.33	17.80	8.73	11.64	990
0.11	2.45	3.34	3.08	1.99	4.70	1.36	3.90	1.99	3.00	2.63	1.43	4.56	1.56	3.55	2.92	8.14	4.92	0.11	16.18	8.04	10.34	988
0.15	2.32	3.00	2.80	1.96	4.04	1.04	3.45	1.94	2.69	2.45	1.50	3.88	1.19	3.08	2.61	6.77	4.34	-0.34	13.88	7.11	7.58	905
0.18	2.20	2.75	2.60	1.87	3.63	0.88	3.06	1.93	2.49	2.31	1.54	3.45	0.96	2.83	2.58	5.66	3.96	0.12	11.19	5.53	6.48	1001
0.32	2.00	2.39	2.30	1.75	3.03	0.64	2.63	1.82	2.23	2.13	1.62	2.84	0.61	2.48	2.21	4.00	3.03	0.63	7.38	3.38	4.51	2846


==> data/mlm_plots/tef/agnews/lstm/s/ets_sts_auc.tex <==
name	auc
et_use	0.86
et_tse	0.78
et_ce	1.86


==> data/mlm_plots/tef/agnews/lstm/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.70	4.07	1.27	-7.51	15.64	11.57	2.87	4.22	11.74	8.20	0.28	23.20	11.46	15.03	4.22	15.61	9.10	-7.64	38.86	23.25	16.42	735
0.06	0.53	2.75	0.89	-7.28	12.78	10.03	1.89	4.01	9.59	6.98	0.59	18.59	9.00	11.48	3.76	13.12	7.05	-9.70	35.95	22.82	14.13	990
0.11	0.40	1.96	0.67	-5.28	9.19	7.24	1.27	3.84	7.93	5.98	1.67	14.19	6.26	9.67	3.41	10.00	5.88	-4.46	24.47	14.47	11.22	988
0.15	0.30	0.94	0.46	-1.20	3.07	2.14	0.79	3.70	6.57	5.19	2.16	10.99	4.42	7.94	3.11	7.80	4.98	-1.87	17.47	9.67	9.15	905
0.18	0.22	0.98	0.34	-8.28	10.24	9.26	0.56	3.51	5.94	4.73	1.93	9.94	4.00	7.05	2.93	7.18	4.20	-4.78	19.13	11.96	7.83	1001
0.32	0.13	0.38	0.21	-0.79	1.55	1.17	0.36	3.32	5.15	4.22	1.90	8.40	3.25	5.77	2.79	6.23	3.83	-6.88	19.34	13.11	6.19	2846


==> data/mlm_plots/tef/agnews/lstm/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.40
et_p_h	2.01
et_p_l2	2.52


==> data/mlm_plots/tef/agnews/lstm/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.07	0.20	0.15	0.03	0.36	0.17	0.28	0.01	0.03	0.02	0.00	0.07	0.03	0.04	0.01	0.03	0.02	0.01	0.06	0.03	0.04	735
0.06	0.16	0.40	0.33	0.08	0.71	0.32	0.56	0.02	0.05	0.04	0.01	0.10	0.05	0.08	0.03	0.05	0.04	0.02	0.08	0.03	0.07	990
0.11	0.29	0.65	0.54	0.14	1.17	0.51	0.88	0.03	0.07	0.06	0.02	0.13	0.05	0.11	0.04	0.07	0.06	0.03	0.10	0.04	0.09	988
0.15	0.56	1.05	0.91	0.34	1.77	0.72	1.38	0.05	0.09	0.09	0.04	0.15	0.06	0.14	0.05	0.09	0.08	0.05	0.12	0.04	0.11	905
0.18	0.84	1.60	1.36	0.48	2.72	1.12	2.13	0.06	0.11	0.11	0.05	0.18	0.06	0.16	0.07	0.10	0.10	0.06	0.14	0.04	0.13	1001
0.32	1.46	3.15	2.49	0.62	5.67	2.52	4.13	0.09	0.14	0.14	0.07	0.21	0.07	0.19	0.09	0.13	0.13	0.08	0.17	0.05	0.16	2846


==> data/mlm_plots/tef/agnews/lstm/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.44
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/agnews/lstm/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.94	0.94	0.91	0.96	0.02	0.95	0.90	0.92	0.93	0.88	0.96	0.04	0.95	0.93	0.95	0.97	0.89	1.00	0.06	0.99	735
0.06	0.89	0.91	0.91	0.88	0.93	0.03	0.92	0.85	0.88	0.89	0.84	0.93	0.05	0.92	0.90	0.93	0.95	0.87	0.99	0.06	0.98	990
0.11	0.86	0.88	0.88	0.85	0.91	0.03	0.90	0.82	0.86	0.86	0.81	0.91	0.05	0.89	0.88	0.91	0.93	0.84	0.98	0.07	0.96	988
0.15	0.83	0.85	0.85	0.81	0.88	0.04	0.87	0.79	0.82	0.82	0.77	0.87	0.05	0.86	0.85	0.89	0.90	0.81	0.96	0.08	0.94	905
0.18	0.80	0.82	0.82	0.78	0.86	0.04	0.84	0.76	0.80	0.80	0.75	0.85	0.05	0.83	0.83	0.87	0.88	0.78	0.95	0.08	0.93	1001
0.32	0.73	0.76	0.76	0.72	0.81	0.05	0.79	0.71	0.75	0.74	0.69	0.80	0.06	0.78	0.76	0.81	0.82	0.71	0.91	0.10	0.88	2846


==> data/mlm_plots/tef/agnews/lstm/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.25


==> data/mlm_plots/tef/agnews/lstm/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.25	0.26	0.26	0.23	0.28	0.02	0.27	26.84	51.61	42.00	11.44	91.78	40.17	63.47	1.01	2.72	2.12	0.31	5.14	2.41	3.59	735
0.06	0.37	0.39	0.38	0.35	0.44	0.04	0.40	34.75	65.09	54.01	14.61	115.57	50.48	76.69	1.12	3.17	2.43	0.43	5.92	2.75	4.29	990
0.11	0.51	0.55	0.52	0.46	0.64	0.09	0.55	42.72	78.99	63.85	14.12	143.86	64.87	91.86	1.39	3.72	2.87	0.46	6.99	3.27	5.02	988
0.15	0.70	0.73	0.73	0.65	0.82	0.09	0.75	51.74	91.49	72.02	24.29	158.70	67.20	107.57	1.51	4.08	3.17	0.68	7.48	3.40	5.64	905
0.18	1.06	1.11	1.11	1.03	1.19	0.08	1.16	56.50	99.97	79.20	22.35	177.60	77.62	117.03	1.72	4.34	3.56	0.89	7.79	3.45	6.11	1001
0.32	1.22	1.51	1.55	1.25	1.78	0.26	1.78	62.76	112.33	88.95	27.17	197.49	85.16	130.67	1.95	5.06	4.28	1.14	8.98	3.92	7.24	2846


==> data/mlm_plots/tef/agnews/lstm/s/time_misc_auc.tex <==
name	auc
attack_time	0.27
l2	26.51
lom	1.20


==> data/mlm_plots/tef/agnews/lstm/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.33	0.46	0.50	0.22	0.70	0.24	0.67	0.62	0.71	0.73	0.57	0.85	0.14	0.81	0.78	0.83	0.85	0.74	0.93	0.09	0.90	735
0.06	0.00	0.30	0.33	0.07	0.53	0.23	0.50	0.53	0.62	0.62	0.47	0.77	0.15	0.73	0.71	0.77	0.78	0.67	0.87	0.10	0.84	990
0.11	0.00	0.19	0.20	-0.00	0.39	0.20	0.33	0.44	0.53	0.55	0.39	0.68	0.14	0.64	0.65	0.72	0.73	0.62	0.82	0.10	0.79	988
0.15	0.00	0.12	0.00	-0.04	0.28	0.16	0.25	0.36	0.45	0.46	0.32	0.59	0.14	0.55	0.59	0.67	0.67	0.57	0.77	0.10	0.74	905
0.18	0.00	0.07	0.00	-0.07	0.21	0.14	0.20	0.29	0.37	0.38	0.24	0.51	0.13	0.46	0.56	0.62	0.62	0.52	0.72	0.10	0.68	1001
0.32	0.00	0.03	0.00	-0.06	0.12	0.09	0.00	0.15	0.25	0.25	0.12	0.38	0.13	0.33	0.46	0.53	0.52	0.43	0.63	0.10	0.59	2846


==> data/mlm_plots/tef/agnews/lstm/s/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.12
top50	0.19


==> data/mlm_plots/tef/agnews/lstmatt/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	128.35	222.59	182.20	60.60	384.57	161.98	266.25	6.00	8.42	8.00	4.47	12.36	3.95	10.00	149.53	259.65	214.60	72.75	446.55	186.90	310.10	6.00	8.51	8.00	4.57	12.45	3.94	10.00	737
0.06	129.31	229.14	188.80	67.50	390.77	161.63	280.54	5.00	8.05	8.00	4.29	11.80	3.76	10.00	176.13	307.42	261.55	97.73	517.11	209.69	378.08	5.00	8.21	8.00	4.43	11.98	3.78	10.00	1009
0.11	127.56	235.05	188.69	53.68	416.42	181.37	281.93	5.00	8.12	8.00	4.39	11.85	3.73	10.00	204.56	361.14	300.93	107.04	615.25	254.10	438.01	6.00	8.40	8.00	4.61	12.20	3.80	10.00	1001
0.15	124.93	219.89	179.29	67.19	372.59	152.70	269.20	6.00	8.38	8.00	4.61	12.14	3.77	10.00	244.98	413.97	355.78	157.77	670.17	256.20	508.67	6.00	8.79	8.00	4.94	12.65	3.86	11.00	923
0.18	126.26	226.89	188.24	60.01	393.77	166.88	272.52	6.00	8.16	8.00	4.35	11.98	3.81	10.00	304.97	504.97	434.03	184.58	825.36	320.39	601.44	6.00	8.73	8.00	4.82	12.64	3.91	11.00	1038
0.32	125.64	228.60	188.29	61.24	395.96	167.36	279.92	6.00	8.15	8.00	4.41	11.90	3.75	10.00	451.92	794.49	665.31	276.24	1312.75	518.25	981.83	6.00	9.11	9.00	5.20	13.02	3.91	11.00	2860


==> data/mlm_plots/tef/agnews/lstmatt/a/comparison_vals_auc.tex <==
name	auc
orig_pp	66.02
orig_ge	2.37
adv_pp	144.78
adv_ge	2.52


==> data/mlm_plots/tef/agnews/lstmatt/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.29	0.48	0.58	0.08	0.88	0.40	0.79	0.25	0.48	0.56	0.07	0.88	0.40	0.80	0.20	0.41	0.45	0.08	0.73	0.32	0.66	737
0.06	-0.07	0.23	0.30	-0.21	0.68	0.44	0.58	-0.08	0.24	0.28	-0.20	0.68	0.44	0.60	-0.02	0.21	0.22	-0.13	0.55	0.34	0.47	1009
0.11	-0.32	0.03	0.04	-0.43	0.49	0.46	0.41	-0.31	0.05	0.04	-0.41	0.50	0.46	0.41	-0.19	0.06	0.05	-0.29	0.40	0.34	0.31	1001
0.15	-0.55	-0.20	-0.23	-0.64	0.24	0.44	0.14	-0.51	-0.17	-0.25	-0.62	0.27	0.44	0.13	-0.35	-0.11	-0.15	-0.44	0.22	0.33	0.11	923
0.18	-0.68	-0.35	-0.43	-0.76	0.06	0.41	-0.08	-0.64	-0.31	-0.40	-0.73	0.10	0.42	-0.07	-0.46	-0.22	-0.26	-0.54	0.10	0.32	-0.04	1038
0.32	-0.81	-0.56	-0.67	-0.91	-0.20	0.35	-0.39	-0.77	-0.52	-0.62	-0.88	-0.16	0.36	-0.37	-0.59	-0.39	-0.45	-0.67	-0.10	0.29	-0.25	2860


==> data/mlm_plots/tef/agnews/lstmatt/a/correlations_auc.tex <==
name	auc
pcc	-0.06
spearman	-0.05
kendall	-0.03


==> data/mlm_plots/tef/agnews/lstmatt/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	1.68	4.29	3.16	0.66	7.93	3.64	5.85	1.44	4.15	2.85	0.04	8.26	4.11	5.32	2.05	8.76	4.85	-1.75	19.27	10.51	11.14	737
0.06	1.97	4.17	3.56	1.37	6.97	2.80	5.76	1.76	3.83	3.17	0.93	6.73	2.90	5.14	2.50	9.62	5.33	-1.60	20.85	11.23	11.73	1009
0.11	2.28	4.07	3.85	1.78	6.36	2.29	5.52	2.04	3.69	3.29	1.40	5.98	2.29	4.93	2.78	9.28	5.22	-1.80	20.35	11.07	10.64	1001
0.15	2.81	4.00	3.93	2.17	5.82	1.83	4.96	2.47	3.65	3.42	1.86	5.43	1.79	4.53	3.18	8.27	5.13	-1.47	18.00	9.73	8.96	923
0.18	2.90	3.84	3.75	2.28	5.40	1.56	4.61	2.55	3.52	3.35	1.99	5.04	1.52	4.23	3.20	7.38	5.02	-0.91	15.68	8.30	8.14	1038
0.32	2.88	3.47	3.43	2.37	4.56	1.10	4.00	2.62	3.26	3.16	2.14	4.37	1.11	3.79	3.09	5.96	4.63	0.46	11.46	5.50	6.77	2860


==> data/mlm_plots/tef/agnews/lstmatt/a/ets_sts_auc.tex <==
name	auc
et_use	1.12
et_tse	1.04
et_ce	2.27


==> data/mlm_plots/tef/agnews/lstmatt/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.60	4.30	1.21	-11.39	19.99	15.69	2.68	3.48	12.67	7.41	-2.87	28.22	15.55	14.97	3.50	17.81	8.38	-12.41	48.03	30.22	17.97	737
0.06	0.54	2.88	1.04	-6.05	11.81	8.93	2.06	4.25	11.77	7.75	-0.53	24.08	12.31	15.25	3.88	15.32	8.18	-9.73	40.38	25.05	18.01	1009
0.11	0.45	2.18	0.82	-5.31	9.68	7.49	1.55	4.51	10.19	7.52	0.69	19.69	9.50	12.84	4.09	12.93	7.37	-5.83	31.68	18.76	15.24	1001
0.15	0.39	1.38	0.62	-2.91	5.66	4.29	1.08	4.92	9.38	7.42	1.80	16.96	7.58	11.06	4.33	11.49	7.12	-3.68	26.66	15.17	12.52	923
0.18	0.32	1.09	0.50	-4.62	6.81	5.72	0.84	4.92	8.56	6.93	2.52	14.59	6.03	10.22	4.22	9.80	6.28	-2.64	22.24	12.44	11.06	1038
0.32	0.19	0.63	0.31	-3.23	4.50	3.86	0.53	4.77	7.31	6.11	2.67	11.94	4.64	8.33	4.05	8.57	5.38	-6.59	23.72	15.15	8.46	2860


==> data/mlm_plots/tef/agnews/lstmatt/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.46
et_p_h	2.69
et_p_l2	3.29


==> data/mlm_plots/tef/agnews/lstmatt/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.08	0.20	0.17	0.05	0.35	0.15	0.29	0.01	0.04	0.02	0.00	0.07	0.04	0.05	0.02	0.03	0.03	0.01	0.06	0.03	0.05	737
0.06	0.18	0.40	0.35	0.11	0.68	0.28	0.57	0.02	0.05	0.04	0.01	0.10	0.04	0.08	0.02	0.05	0.04	0.02	0.08	0.03	0.07	1009
0.11	0.32	0.64	0.57	0.18	1.10	0.46	0.84	0.03	0.07	0.06	0.02	0.12	0.05	0.11	0.04	0.07	0.06	0.03	0.10	0.04	0.09	1001
0.15	0.58	1.05	0.93	0.36	1.73	0.68	1.39	0.04	0.09	0.09	0.04	0.15	0.06	0.13	0.05	0.08	0.08	0.04	0.12	0.04	0.11	923
0.18	0.81	1.49	1.27	0.50	2.48	0.99	1.98	0.06	0.11	0.11	0.05	0.17	0.06	0.15	0.07	0.10	0.10	0.06	0.14	0.04	0.13	1038
0.32	1.45	3.07	2.47	0.77	5.36	2.30	4.03	0.09	0.14	0.14	0.08	0.21	0.07	0.19	0.09	0.13	0.13	0.08	0.17	0.05	0.16	2860


==> data/mlm_plots/tef/agnews/lstmatt/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.42
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/agnews/lstmatt/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.93	0.94	0.91	0.96	0.02	0.95	0.89	0.92	0.93	0.87	0.96	0.04	0.95	0.92	0.94	0.96	0.88	1.00	0.06	0.98	737
0.06	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.85	0.88	0.89	0.83	0.93	0.05	0.92	0.89	0.92	0.94	0.85	0.99	0.07	0.97	1009
0.11	0.85	0.87	0.87	0.84	0.91	0.03	0.90	0.82	0.85	0.86	0.80	0.90	0.05	0.89	0.86	0.90	0.91	0.83	0.97	0.07	0.96	1001
0.15	0.82	0.84	0.84	0.81	0.88	0.04	0.86	0.79	0.82	0.82	0.77	0.87	0.05	0.86	0.83	0.87	0.89	0.79	0.95	0.08	0.93	923
0.18	0.79	0.82	0.82	0.78	0.85	0.04	0.84	0.76	0.79	0.79	0.74	0.85	0.05	0.83	0.81	0.85	0.86	0.77	0.94	0.08	0.91	1038
0.32	0.73	0.77	0.77	0.72	0.81	0.05	0.80	0.71	0.75	0.75	0.69	0.80	0.06	0.79	0.77	0.82	0.83	0.72	0.91	0.10	0.88	2860


==> data/mlm_plots/tef/agnews/lstmatt/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.25


==> data/mlm_plots/tef/agnews/lstmatt/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.27	0.29	0.29	0.26	0.31	0.02	0.30	0.03	0.05	0.05	0.02	0.08	0.03	0.07	0.91	2.65	2.00	0.37	4.94	2.28	3.68	737
0.06	0.40	0.43	0.42	0.37	0.48	0.05	0.43	0.04	0.07	0.06	0.03	0.10	0.04	0.09	1.48	3.51	2.84	0.79	6.23	2.72	4.97	1009
0.11	0.57	0.61	0.58	0.50	0.71	0.10	0.59	0.05	0.08	0.07	0.04	0.12	0.04	0.10	1.71	4.19	3.43	0.99	7.40	3.21	5.95	1001
0.15	0.82	0.86	0.85	0.75	0.96	0.11	0.86	0.06	0.09	0.08	0.04	0.14	0.05	0.12	2.17	5.18	4.44	1.44	8.93	3.74	7.48	923
0.18	1.05	1.11	1.10	0.98	1.24	0.13	1.12	0.06	0.10	0.10	0.05	0.15	0.05	0.13	2.48	5.70	5.09	1.73	9.67	3.97	8.17	1038
0.32	1.29	1.61	1.67	1.33	1.88	0.27	1.83	0.07	0.11	0.11	0.06	0.16	0.05	0.15	2.87	6.36	5.59	2.01	10.70	4.34	9.14	2860


==> data/mlm_plots/tef/agnews/lstmatt/a/time_misc_auc.tex <==
name	auc
attack_time	0.28
l2	0.03
lom	1.48


==> data/mlm_plots/tef/agnews/lstmatt/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.34	0.25	-0.01	0.69	0.35	0.67	0.33	0.52	0.56	0.25	0.80	0.27	0.75	0.56	0.67	0.69	0.48	0.87	0.20	0.82	737
0.06	0.00	0.21	0.00	-0.10	0.52	0.31	0.40	0.15	0.38	0.38	0.11	0.65	0.27	0.58	0.42	0.57	0.58	0.36	0.78	0.21	0.72	1009
0.11	0.00	0.14	0.00	-0.11	0.40	0.26	0.25	0.07	0.29	0.25	0.04	0.54	0.25	0.44	0.33	0.49	0.48	0.28	0.70	0.21	0.64	1001
0.15	0.00	0.07	0.00	-0.11	0.26	0.19	0.00	0.00	0.19	0.12	-0.03	0.41	0.22	0.33	0.26	0.40	0.38	0.20	0.60	0.20	0.52	923
0.18	0.00	0.05	0.00	-0.11	0.21	0.16	0.00	0.00	0.14	0.06	-0.06	0.33	0.19	0.21	0.21	0.35	0.33	0.16	0.54	0.19	0.47	1038
0.32	0.00	0.02	0.00	-0.09	0.13	0.11	0.00	0.00	0.07	0.00	-0.08	0.23	0.15	0.09	0.14	0.26	0.24	0.09	0.43	0.17	0.35	2860


==> data/mlm_plots/tef/agnews/lstmatt/a/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.06
top50	0.12


==> data/mlm_plots/tef/agnews/lstmatt/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	126.07	218.91	182.20	60.61	377.21	158.30	263.39	6.00	8.32	8.00	4.48	12.17	3.85	10.00	152.39	256.43	218.92	90.49	422.37	165.94	317.73	6.00	8.42	8.00	4.55	12.30	3.88	10.00	776
0.06	129.15	230.95	189.98	59.17	402.73	171.78	283.42	5.00	8.08	8.00	4.34	11.82	3.74	10.00	179.98	308.43	263.90	99.69	517.18	208.74	381.04	6.00	8.26	8.00	4.49	12.03	3.77	10.00	1022
0.11	128.35	235.97	188.80	55.25	416.69	180.72	285.36	6.00	8.16	8.00	4.32	12.00	3.84	10.00	206.90	361.08	303.44	125.48	596.69	235.61	444.24	6.00	8.44	8.00	4.56	12.32	3.88	10.00	1048
0.15	121.80	219.03	178.91	64.46	373.60	154.57	267.49	6.00	8.37	8.00	4.63	12.10	3.74	10.00	240.91	403.25	340.90	161.93	644.58	241.33	506.41	6.00	8.80	8.00	5.01	12.59	3.79	11.00	962
0.18	127.61	228.06	187.59	59.12	397.01	168.95	272.25	6.00	8.22	8.00	4.52	11.92	3.70	10.00	301.35	494.78	428.25	212.33	777.23	282.45	614.83	6.00	8.78	8.00	5.00	12.56	3.78	11.00	1046
0.32	126.16	228.29	188.65	62.23	394.36	166.06	279.40	5.00	8.10	8.00	4.39	11.80	3.71	10.00	438.77	749.79	643.34	300.19	1199.38	449.60	936.26	6.00	9.02	9.00	5.21	12.83	3.81	11.00	2744


==> data/mlm_plots/tef/agnews/lstmatt/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	66.12
orig_ge	2.38
adv_pp	140.46
adv_ge	2.52


==> data/mlm_plots/tef/agnews/lstmatt/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.33	0.51	0.57	0.19	0.83	0.32	0.75	0.60	0.68	0.74	0.46	0.91	0.23	0.82	0.50	0.59	0.63	0.38	0.80	0.21	0.74	776
0.06	0.07	0.28	0.31	-0.05	0.61	0.33	0.53	0.39	0.51	0.56	0.27	0.76	0.24	0.68	0.32	0.44	0.47	0.23	0.65	0.21	0.58	1022
0.11	-0.11	0.12	0.14	-0.22	0.46	0.34	0.37	0.23	0.36	0.40	0.09	0.64	0.28	0.55	0.19	0.31	0.34	0.08	0.54	0.23	0.46	1048
0.15	-0.26	-0.03	-0.04	-0.36	0.30	0.33	0.20	0.08	0.22	0.25	-0.05	0.49	0.27	0.40	0.08	0.19	0.22	-0.02	0.41	0.21	0.34	962
0.18	-0.33	-0.12	-0.14	-0.42	0.19	0.31	0.10	0.00	0.14	0.14	-0.10	0.38	0.24	0.30	0.02	0.13	0.13	-0.06	0.32	0.19	0.25	1046
0.32	-0.46	-0.25	-0.27	-0.53	0.04	0.29	-0.06	-0.16	-0.00	-0.00	-0.25	0.24	0.24	0.16	-0.10	0.02	0.02	-0.17	0.20	0.19	0.14	2744


==> data/mlm_plots/tef/agnews/lstmatt/ig/correlations_auc.tex <==
name	auc
pcc	-0.00
spearman	0.07
kendall	0.06


==> data/mlm_plots/tef/agnews/lstmatt/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	1.92	4.18	3.37	0.90	7.46	3.28	5.28	1.57	4.17	2.88	0.07	8.27	4.10	5.13	2.63	8.69	5.35	-0.16	17.54	8.85	12.09	776
0.06	2.35	3.89	3.45	1.58	6.20	2.31	4.89	1.95	3.69	2.97	0.83	6.55	2.86	4.51	2.70	9.71	5.73	-0.58	20.00	10.29	13.26	1022
0.11	2.44	3.65	3.36	1.82	5.48	1.83	4.44	2.08	3.38	2.96	1.36	5.39	2.02	4.15	2.87	9.22	4.92	-1.45	19.88	10.66	10.73	1048
0.15	2.45	3.43	3.21	1.96	4.91	1.47	4.23	2.04	3.13	2.88	1.61	4.65	1.52	3.76	2.80	7.51	4.58	-1.67	16.69	9.18	7.53	962
0.18	2.38	3.13	2.98	1.97	4.28	1.15	3.75	2.10	2.90	2.71	1.66	4.13	1.23	3.43	2.74	6.20	4.20	-0.08	12.47	6.28	7.00	1046
0.32	2.21	2.79	2.67	1.86	3.71	0.93	3.26	2.02	2.62	2.47	1.67	3.56	0.94	3.03	2.55	4.98	3.59	0.16	9.81	4.82	5.70	2744


==> data/mlm_plots/tef/agnews/lstmatt/ig/ets_sts_auc.tex <==
name	auc
et_use	0.96
et_tse	0.90
et_ce	2.07


==> data/mlm_plots/tef/agnews/lstmatt/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.61	3.63	1.17	-10.85	18.12	14.48	2.37	3.83	11.56	8.06	-0.02	23.14	11.58	15.55	3.92	15.73	8.76	-7.55	39.01	23.28	18.13	776
0.06	0.52	2.64	0.96	-7.15	12.42	9.79	1.90	4.37	10.92	7.80	0.46	21.38	10.46	13.71	4.17	14.59	8.25	-9.08	38.26	23.67	15.90	1022
0.11	0.43	1.74	0.75	-3.48	6.97	5.22	1.38	4.48	9.58	6.92	1.25	17.90	8.33	11.68	4.00	12.08	6.97	-5.60	29.76	17.68	13.93	1048
0.15	0.36	1.65	0.56	-8.58	11.89	10.24	0.94	4.43	8.14	6.51	2.19	14.09	5.95	9.84	3.83	9.70	6.20	-2.08	21.48	11.78	10.71	962
0.18	0.27	1.20	0.42	-7.89	10.29	9.09	0.71	4.31	7.32	5.80	2.25	12.39	5.07	8.52	3.70	8.56	5.48	-2.96	20.09	11.52	9.68	1046
0.32	0.16	0.62	0.26	-3.90	5.13	4.52	0.45	3.94	6.09	5.11	2.17	10.02	3.93	6.89	3.37	7.11	4.58	-4.46	18.67	11.56	7.23	2744


==> data/mlm_plots/tef/agnews/lstmatt/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.44
et_p_h	2.37
et_p_l2	2.92


==> data/mlm_plots/tef/agnews/lstmatt/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.09	0.22	0.18	0.05	0.39	0.17	0.31	0.01	0.04	0.02	0.00	0.07	0.03	0.05	0.02	0.03	0.03	0.01	0.06	0.03	0.04	776
0.06	0.18	0.41	0.35	0.10	0.73	0.32	0.56	0.02	0.05	0.04	0.01	0.10	0.04	0.07	0.03	0.05	0.04	0.02	0.08	0.03	0.07	1022
0.11	0.33	0.66	0.54	0.15	1.16	0.50	0.87	0.03	0.07	0.06	0.02	0.12	0.05	0.10	0.04	0.06	0.06	0.03	0.10	0.03	0.09	1048
0.15	0.57	1.02	0.90	0.32	1.71	0.69	1.35	0.05	0.09	0.08	0.04	0.14	0.05	0.13	0.05	0.08	0.08	0.05	0.12	0.04	0.11	962
0.18	0.79	1.45	1.26	0.50	2.40	0.95	1.89	0.06	0.10	0.10	0.05	0.16	0.06	0.14	0.07	0.09	0.09	0.06	0.13	0.04	0.12	1046
0.32	1.32	2.90	2.31	0.61	5.18	2.29	3.70	0.08	0.14	0.14	0.07	0.20	0.07	0.18	0.09	0.12	0.12	0.08	0.17	0.05	0.15	2744


==> data/mlm_plots/tef/agnews/lstmatt/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/tef/agnews/lstmatt/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.93	0.94	0.91	0.96	0.02	0.95	0.90	0.92	0.93	0.88	0.96	0.04	0.95	0.93	0.95	0.96	0.89	1.00	0.05	0.98	776
0.06	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.85	0.88	0.89	0.83	0.93	0.05	0.92	0.89	0.92	0.94	0.86	0.99	0.06	0.97	1022
0.11	0.85	0.87	0.87	0.84	0.91	0.03	0.90	0.82	0.85	0.85	0.80	0.90	0.05	0.89	0.86	0.90	0.92	0.83	0.97	0.07	0.96	1048
0.15	0.82	0.84	0.84	0.80	0.88	0.04	0.87	0.78	0.82	0.82	0.77	0.87	0.05	0.86	0.83	0.88	0.89	0.79	0.96	0.08	0.94	962
0.18	0.79	0.81	0.81	0.78	0.85	0.04	0.84	0.76	0.79	0.79	0.74	0.85	0.05	0.83	0.81	0.86	0.87	0.77	0.94	0.08	0.92	1046
0.32	0.73	0.77	0.77	0.72	0.81	0.05	0.80	0.71	0.75	0.75	0.69	0.81	0.06	0.79	0.76	0.82	0.83	0.72	0.92	0.10	0.89	2744


==> data/mlm_plots/tef/agnews/lstmatt/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.25


==> data/mlm_plots/tef/agnews/lstmatt/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.33	0.35	0.35	0.24	0.47	0.12	0.36	0.75	1.71	1.25	-0.08	3.50	1.79	1.99	1.27	4.07	2.92	-0.19	8.32	4.25	5.11	776
0.06	0.52	0.57	0.54	0.43	0.70	0.14	0.57	1.13	2.28	1.76	0.24	4.33	2.05	2.64	1.76	5.24	3.75	0.23	10.25	5.01	7.19	1022
0.11	0.69	0.80	0.72	0.53	1.06	0.26	0.79	1.42	2.64	2.13	0.05	5.24	2.59	3.11	2.10	6.72	5.00	0.56	12.87	6.15	9.83	1048
0.15	0.99	1.07	1.01	0.82	1.33	0.25	1.05	1.61	2.87	2.31	0.13	5.61	2.74	3.34	2.87	8.15	6.31	0.95	15.35	7.20	11.49	962
0.18	1.36	1.46	1.43	1.27	1.66	0.20	1.47	1.75	2.97	2.43	0.12	5.82	2.85	3.47	3.28	8.41	6.81	1.63	15.19	6.78	11.74	1046
0.32	1.60	2.02	2.14	1.67	2.37	0.35	2.32	1.95	3.23	2.62	0.41	6.04	2.82	3.76	3.55	8.72	7.12	1.77	15.67	6.95	12.46	2744


==> data/mlm_plots/tef/agnews/lstmatt/ig/time_misc_auc.tex <==
name	auc
attack_time	0.37
l2	0.82
lom	2.19


==> data/mlm_plots/tef/agnews/lstmatt/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.40	0.56	0.60	0.33	0.78	0.23	0.75	0.67	0.74	0.77	0.59	0.90	0.16	0.85	0.75	0.80	0.82	0.68	0.92	0.12	0.88	776
0.06	0.25	0.38	0.40	0.14	0.61	0.23	0.50	0.56	0.64	0.67	0.49	0.80	0.15	0.75	0.67	0.73	0.75	0.61	0.85	0.12	0.82	1022
0.11	0.00	0.30	0.25	0.06	0.53	0.24	0.50	0.46	0.56	0.57	0.40	0.72	0.16	0.67	0.60	0.67	0.70	0.54	0.81	0.13	0.76	1048
0.15	0.00	0.24	0.25	0.01	0.46	0.22	0.40	0.38	0.49	0.50	0.34	0.64	0.15	0.60	0.54	0.62	0.63	0.49	0.75	0.13	0.71	962
0.18	0.00	0.22	0.20	0.00	0.43	0.21	0.33	0.36	0.44	0.44	0.30	0.59	0.14	0.54	0.52	0.59	0.60	0.47	0.71	0.12	0.67	1046
0.32	0.00	0.16	0.00	-0.04	0.35	0.19	0.25	0.27	0.38	0.38	0.23	0.53	0.15	0.50	0.47	0.54	0.55	0.43	0.65	0.11	0.62	2744


==> data/mlm_plots/tef/agnews/lstmatt/ig/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.14
top50	0.18


==> data/mlm_plots/tef/agnews/lstmatt/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	126.48	220.24	182.05	63.71	376.77	156.53	266.64	6.00	8.36	8.00	4.43	12.29	3.93	10.00	150.42	260.68	220.95	92.20	429.16	168.48	329.72	6.00	8.46	8.00	4.51	12.41	3.95	10.00	758
0.06	128.95	227.37	188.80	60.62	394.11	166.75	276.99	5.00	8.03	8.00	4.27	11.80	3.76	10.00	178.39	308.27	257.02	97.27	519.27	211.00	381.32	5.00	8.22	8.00	4.42	12.03	3.80	10.00	1006
0.11	125.98	231.56	188.39	52.34	410.77	179.21	277.35	6.00	8.16	8.00	4.42	11.89	3.74	10.00	204.30	361.75	298.06	100.33	623.18	261.42	439.15	6.00	8.44	8.00	4.65	12.24	3.79	10.00	987
0.15	127.48	222.97	181.90	69.08	376.87	153.89	272.43	6.00	8.41	8.00	4.63	12.19	3.78	10.00	260.30	422.38	362.43	171.59	673.18	250.80	523.92	6.00	8.87	8.00	5.03	12.72	3.84	11.00	927
0.18	125.72	226.12	185.27	57.88	394.37	168.24	271.87	6.00	8.27	8.00	4.36	12.18	3.91	10.00	316.31	517.12	453.88	192.85	841.39	324.27	612.84	6.00	8.90	8.00	4.94	12.87	3.96	11.00	1023
0.32	125.86	228.44	188.41	61.89	394.99	166.55	278.60	6.00	8.11	8.00	4.40	11.82	3.71	10.00	456.90	780.06	674.25	285.21	1274.91	494.85	939.24	6.00	9.12	9.00	5.25	12.98	3.87	11.00	2878


==> data/mlm_plots/tef/agnews/lstmatt/s/comparison_vals_auc.tex <==
name	auc
orig_pp	65.81
orig_ge	2.38
adv_pp	145.25
adv_ge	2.54


==> data/mlm_plots/tef/agnews/lstmatt/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.41	0.55	0.56	0.33	0.76	0.22	0.70	0.68	0.76	0.80	0.59	0.94	0.18	0.90	0.51	0.62	0.63	0.44	0.80	0.18	0.76	758
0.06	0.24	0.38	0.39	0.18	0.59	0.20	0.52	0.55	0.66	0.70	0.45	0.88	0.21	0.82	0.39	0.52	0.53	0.33	0.70	0.19	0.65	1006
0.11	0.14	0.27	0.27	0.08	0.45	0.19	0.39	0.43	0.57	0.61	0.34	0.80	0.23	0.74	0.30	0.43	0.45	0.24	0.62	0.19	0.57	987
0.15	0.03	0.15	0.15	-0.02	0.32	0.17	0.26	0.28	0.45	0.49	0.20	0.70	0.25	0.65	0.20	0.33	0.35	0.14	0.52	0.19	0.48	927
0.18	-0.02	0.08	0.08	-0.08	0.24	0.16	0.18	0.19	0.36	0.39	0.10	0.62	0.26	0.56	0.14	0.26	0.26	0.07	0.45	0.19	0.40	1023
0.32	-0.15	-0.04	-0.05	-0.20	0.12	0.16	0.06	-0.01	0.18	0.19	-0.09	0.46	0.27	0.38	-0.01	0.13	0.13	-0.06	0.32	0.19	0.26	2878


==> data/mlm_plots/tef/agnews/lstmatt/s/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.12
kendall	0.09


==> data/mlm_plots/tef/agnews/lstmatt/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	2.27	4.17	3.65	1.44	6.91	2.74	5.50	1.83	4.00	3.10	0.46	7.54	3.54	4.93	2.62	8.92	5.90	0.61	17.24	8.32	12.57	758
0.06	2.48	3.73	3.40	1.83	5.63	1.90	4.51	2.06	3.54	2.87	0.96	6.12	2.58	4.23	3.06	8.81	5.52	0.52	17.09	8.29	12.32	1006
0.11	2.37	3.40	3.15	1.92	4.88	1.48	4.14	2.00	3.16	2.80	1.42	4.91	1.75	3.75	2.84	8.06	5.03	0.04	16.07	8.01	9.90	987
0.15	2.31	3.05	2.83	1.93	4.17	1.12	3.55	2.04	2.84	2.60	1.64	4.04	1.20	3.38	2.67	6.53	4.28	0.02	13.04	6.51	7.53	927
0.18	2.19	2.79	2.67	1.88	3.69	0.90	3.18	1.90	2.61	2.43	1.59	3.63	1.02	3.05	2.53	5.64	3.88	-0.01	11.28	5.64	6.53	1023
0.32	1.99	2.41	2.31	1.75	3.06	0.65	2.73	1.82	2.28	2.16	1.60	2.97	0.68	2.63	2.24	4.31	3.25	0.47	8.15	3.84	4.84	2878


==> data/mlm_plots/tef/agnews/lstmatt/s/ets_sts_auc.tex <==
name	auc
et_use	0.88
et_tse	0.83
et_ce	1.86


==> data/mlm_plots/tef/agnews/lstmatt/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.63	3.04	1.14	-5.99	12.07	9.03	2.11	4.17	11.22	7.59	-0.36	22.80	11.58	13.72	3.90	14.70	8.66	-8.49	37.89	23.19	16.64	758
0.06	0.49	2.23	0.83	-6.94	11.41	9.18	1.57	4.06	9.36	6.49	0.60	18.13	8.77	11.70	3.62	12.26	6.93	-5.90	30.42	18.16	13.27	1006
0.11	0.38	1.49	0.61	-3.87	6.86	5.37	1.08	3.75	7.50	5.56	0.97	14.03	6.53	9.04	3.16	9.51	5.55	-6.29	25.32	15.80	10.99	987
0.15	0.29	1.45	0.44	-11.77	14.68	13.22	0.73	3.59	6.30	4.89	1.25	11.36	5.05	7.32	3.04	7.38	4.44	-2.75	17.52	10.14	8.49	927
0.18	0.22	0.81	0.34	-7.52	9.13	8.33	0.53	3.43	5.50	4.49	1.79	9.21	3.71	6.32	2.88	6.62	3.96	-4.96	18.20	11.58	6.62	1023
0.32	0.13	0.44	0.21	-2.43	3.32	2.88	0.36	3.23	4.82	4.06	1.79	7.84	3.03	5.48	2.74	5.52	3.56	-3.66	14.69	9.17	5.55	2878


==> data/mlm_plots/tef/agnews/lstmatt/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.35
et_p_h	1.90
et_p_l2	2.34


==> data/mlm_plots/tef/agnews/lstmatt/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.09	0.23	0.19	0.05	0.40	0.18	0.32	0.01	0.04	0.02	-0.00	0.08	0.04	0.05	0.01	0.04	0.03	0.01	0.06	0.03	0.05	758
0.06	0.19	0.42	0.36	0.11	0.73	0.31	0.58	0.02	0.06	0.04	0.01	0.10	0.05	0.08	0.03	0.05	0.04	0.02	0.09	0.03	0.08	1006
0.11	0.33	0.66	0.58	0.20	1.13	0.46	0.91	0.03	0.08	0.06	0.03	0.13	0.05	0.11	0.04	0.07	0.06	0.03	0.11	0.04	0.10	987
0.15	0.56	1.07	0.92	0.37	1.78	0.70	1.43	0.05	0.10	0.10	0.04	0.16	0.06	0.14	0.06	0.09	0.09	0.05	0.13	0.04	0.12	927
0.18	0.85	1.58	1.34	0.54	2.63	1.04	2.12	0.07	0.12	0.11	0.06	0.18	0.06	0.16	0.07	0.10	0.10	0.06	0.14	0.04	0.13	1023
0.32	1.39	3.05	2.46	0.61	5.49	2.44	3.94	0.09	0.14	0.14	0.08	0.21	0.07	0.19	0.10	0.13	0.13	0.08	0.17	0.05	0.16	2878


==> data/mlm_plots/tef/agnews/lstmatt/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.43
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/agnews/lstmatt/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.93	0.94	0.94	0.91	0.96	0.02	0.96	0.90	0.92	0.93	0.88	0.96	0.04	0.95	0.92	0.95	0.97	0.90	1.00	0.05	0.98	758
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.86	0.89	0.89	0.84	0.94	0.05	0.92	0.90	0.93	0.95	0.87	0.99	0.06	0.98	1006
0.11	0.86	0.88	0.88	0.85	0.92	0.03	0.90	0.83	0.86	0.87	0.81	0.91	0.05	0.90	0.88	0.91	0.93	0.84	0.98	0.07	0.96	987
0.15	0.83	0.85	0.85	0.81	0.89	0.04	0.87	0.80	0.83	0.84	0.78	0.88	0.05	0.87	0.85	0.89	0.90	0.81	0.96	0.08	0.94	927
0.18	0.80	0.83	0.83	0.79	0.86	0.04	0.85	0.77	0.81	0.81	0.75	0.86	0.05	0.84	0.82	0.87	0.88	0.79	0.95	0.08	0.93	1023
0.32	0.74	0.77	0.77	0.73	0.82	0.05	0.81	0.72	0.76	0.76	0.70	0.81	0.06	0.80	0.77	0.82	0.84	0.73	0.92	0.10	0.89	2878


==> data/mlm_plots/tef/agnews/lstmatt/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.24
sts_tse	0.24
sts_ce	0.25


==> data/mlm_plots/tef/agnews/lstmatt/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.33	0.34	0.34	0.32	0.37	0.03	0.35	10.44	34.19	23.39	-13.22	81.61	47.41	42.03	1.38	3.94	3.02	0.56	7.32	3.38	5.77	758
0.06	0.47	0.50	0.48	0.45	0.56	0.06	0.52	15.17	43.88	32.26	-0.45	88.21	44.33	56.02	1.66	4.82	3.94	1.02	8.62	3.80	7.02	1006
0.11	0.65	0.70	0.67	0.60	0.80	0.10	0.69	17.99	53.50	38.73	-1.41	108.41	54.91	68.17	2.24	5.62	4.92	1.51	9.72	4.11	8.18	987
0.15	0.95	1.00	0.98	0.84	1.17	0.16	1.01	21.07	65.46	46.24	-7.35	138.27	72.81	83.81	2.91	6.89	6.14	2.18	11.61	4.72	10.42	927
0.18	1.41	1.45	1.44	1.33	1.58	0.13	1.49	24.48	73.26	50.71	-1.92	148.44	75.18	91.46	3.29	7.17	6.45	2.42	11.93	4.75	10.49	1023
0.32	1.97	2.05	2.05	1.92	2.18	0.13	2.16	30.64	89.73	62.71	-11.89	191.35	101.62	110.70	3.91	8.29	7.78	3.07	13.51	5.22	12.07	2878


==> data/mlm_plots/tef/agnews/lstmatt/s/time_misc_auc.tex <==
name	auc
attack_time	0.36
l2	19.47
lom	1.94


==> data/mlm_plots/tef/agnews/lstmatt/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.21	0.41	0.40	0.16	0.66	0.25	0.60	0.60	0.69	0.70	0.53	0.85	0.16	0.81	0.74	0.81	0.82	0.70	0.92	0.11	0.89	758
0.06	0.00	0.27	0.25	0.05	0.49	0.22	0.40	0.50	0.61	0.62	0.44	0.77	0.17	0.73	0.69	0.76	0.78	0.64	0.88	0.12	0.85	1006
0.11	0.00	0.19	0.20	0.00	0.38	0.19	0.33	0.44	0.54	0.56	0.37	0.71	0.17	0.67	0.64	0.72	0.73	0.60	0.84	0.12	0.81	987
0.15	0.00	0.11	0.00	-0.04	0.27	0.16	0.25	0.33	0.45	0.45	0.28	0.62	0.17	0.58	0.58	0.67	0.67	0.54	0.79	0.13	0.76	927
0.18	0.00	0.07	0.00	-0.06	0.21	0.13	0.20	0.29	0.40	0.38	0.23	0.56	0.16	0.50	0.55	0.63	0.65	0.50	0.76	0.13	0.72	1023
0.32	0.00	0.03	0.00	-0.06	0.13	0.09	0.00	0.18	0.29	0.29	0.13	0.45	0.16	0.38	0.48	0.56	0.56	0.43	0.68	0.13	0.65	2878


==> data/mlm_plots/tef/agnews/lstmatt/s/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.13
top50	0.19


==> data/mlm_plots/tef/agnews/roberta/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	95.63	173.46	142.01	48.10	298.82	125.36	212.67	3.00	4.40	4.00	2.44	6.36	1.96	6.00	116.40	205.49	172.34	65.92	345.06	139.57	254.16	3.00	4.52	4.00	2.56	6.48	1.96	6.00	650
0.06	99.56	178.71	148.76	56.90	300.51	121.81	226.28	3.00	4.65	5.00	2.63	6.66	2.01	6.00	139.78	245.99	204.34	87.72	404.26	158.27	307.36	3.00	4.84	5.00	2.77	6.92	2.08	6.00	1068
0.11	99.92	176.97	147.88	57.33	296.62	119.65	219.80	3.00	4.61	4.00	2.59	6.64	2.02	6.00	165.76	284.34	240.58	105.68	463.00	178.66	352.97	3.00	4.92	5.00	2.80	7.04	2.12	6.00	988
0.15	99.13	180.62	147.74	50.65	310.58	129.97	224.45	3.00	4.62	4.00	2.54	6.69	2.08	6.00	202.85	348.48	289.85	110.64	586.32	237.84	418.95	3.00	5.03	5.00	2.82	7.24	2.21	6.00	771
0.18	98.16	176.12	147.48	53.04	299.21	123.09	223.34	3.00	4.67	4.00	2.60	6.75	2.08	6.00	241.14	403.27	339.27	142.01	664.52	261.26	497.22	4.00	5.19	5.00	2.98	7.40	2.21	7.00	1039
0.32	98.91	179.99	147.88	48.80	311.18	131.19	223.27	3.00	4.62	4.00	2.56	6.68	2.06	6.00	330.12	582.90	479.80	192.50	973.30	390.40	716.54	4.00	5.39	5.00	3.13	7.65	2.26	7.00	2868


==> data/mlm_plots/tef/agnews/roberta/a/comparison_vals_auc.tex <==
name	auc
orig_pp	51.61
orig_ge	1.34
adv_pp	112.66
adv_ge	1.48


==> data/mlm_plots/tef/agnews/roberta/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.66	0.76	0.82	0.56	0.97	0.21	0.92	0.82	0.87	0.89	0.77	0.97	0.10	0.94	0.67	0.73	0.75	0.62	0.85	0.11	0.82	650
0.06	0.38	0.57	0.60	0.31	0.83	0.26	0.78	0.70	0.77	0.81	0.61	0.94	0.16	0.89	0.54	0.63	0.65	0.47	0.78	0.16	0.74	1068
0.11	0.20	0.42	0.41	0.15	0.69	0.27	0.63	0.60	0.70	0.74	0.50	0.89	0.19	0.84	0.45	0.55	0.57	0.38	0.72	0.17	0.67	988
0.15	0.09	0.30	0.27	0.03	0.57	0.27	0.47	0.50	0.63	0.67	0.40	0.85	0.23	0.80	0.36	0.48	0.50	0.29	0.67	0.19	0.63	771
0.18	0.01	0.19	0.13	-0.07	0.45	0.26	0.33	0.38	0.54	0.58	0.28	0.80	0.26	0.75	0.27	0.41	0.43	0.20	0.62	0.21	0.57	1039
0.32	-0.11	0.04	-0.00	-0.20	0.29	0.25	0.16	0.13	0.37	0.41	0.03	0.70	0.34	0.64	0.09	0.27	0.29	0.02	0.52	0.25	0.47	2868


==> data/mlm_plots/tef/agnews/roberta/a/correlations_auc.tex <==
name	auc
pcc	0.08
spearman	0.17
kendall	0.13


==> data/mlm_plots/tef/agnews/roberta/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	0.79	2.39	1.64	0.02	4.76	2.37	3.44	0.74	2.56	1.61	-0.42	5.54	2.98	3.18	1.02	5.90	2.88	-1.84	13.63	7.74	7.09	650
0.06	1.36	2.83	2.45	0.80	4.87	2.04	3.87	1.23	2.92	2.29	0.29	5.56	2.63	3.77	1.84	7.42	4.33	-0.94	15.78	8.36	9.78	1068
0.11	1.71	2.89	2.68	1.22	4.56	1.67	3.80	1.53	2.86	2.43	0.80	4.91	2.06	3.67	2.22	7.30	4.26	-0.51	15.11	7.81	9.05	988
0.15	1.92	2.78	2.70	1.39	4.18	1.40	3.53	1.70	2.72	2.44	1.15	4.29	1.57	3.43	2.38	6.95	4.42	-0.51	14.42	7.46	8.44	771
0.18	2.06	2.71	2.68	1.61	3.80	1.10	3.32	1.88	2.63	2.51	1.44	3.82	1.19	3.22	2.44	6.43	4.04	-0.51	13.37	6.94	7.52	1039
0.32	2.02	2.48	2.41	1.61	3.35	0.87	2.91	1.88	2.44	2.31	1.46	3.41	0.97	2.88	2.33	4.89	3.44	0.16	9.61	4.72	5.68	2868


==> data/mlm_plots/tef/agnews/roberta/a/ets_sts_auc.tex <==
name	auc
et_use	0.78
et_tse	0.77
et_ce	1.85


==> data/mlm_plots/tef/agnews/roberta/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.20	1.62	0.51	-3.32	6.56	4.94	1.21	1.09	5.41	2.91	-2.05	12.88	7.47	6.41	1.10	7.10	2.82	-5.58	19.77	12.68	8.04	650
0.06	0.24	1.60	0.52	-6.62	9.83	8.22	1.06	1.71	5.78	3.63	-0.89	12.44	6.66	7.11	1.54	7.51	3.62	-8.67	23.69	16.18	8.19	1068
0.11	0.25	0.85	0.44	-0.98	2.68	1.83	0.85	2.19	5.54	3.90	-0.17	11.24	5.71	6.99	1.90	6.46	3.56	-2.70	15.63	9.16	7.76	988
0.15	0.21	0.62	0.35	-0.89	2.12	1.50	0.59	2.51	4.99	3.63	0.49	9.50	4.51	6.13	2.11	6.20	3.22	-6.22	18.63	12.43	6.31	771
0.18	0.19	0.69	0.31	-6.25	7.62	6.94	0.49	2.72	4.67	3.84	0.96	8.39	3.72	5.60	2.26	5.90	3.37	-7.62	19.42	13.52	6.11	1039
0.32	0.13	0.42	0.21	-1.83	2.67	2.25	0.36	2.82	4.49	3.71	0.93	8.05	3.56	5.16	2.31	5.80	3.21	-9.60	21.21	15.40	5.06	2868


==> data/mlm_plots/tef/agnews/roberta/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.23
et_p_h	1.45
et_p_l2	1.82


==> data/mlm_plots/tef/agnews/roberta/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.09	0.23	0.19	0.04	0.42	0.19	0.31	0.01	0.05	0.03	-0.00	0.09	0.05	0.06	0.02	0.04	0.03	0.01	0.08	0.03	0.06	650
0.06	0.21	0.44	0.38	0.13	0.74	0.31	0.58	0.02	0.07	0.05	0.01	0.12	0.06	0.10	0.03	0.06	0.05	0.02	0.10	0.04	0.09	1068
0.11	0.35	0.71	0.61	0.20	1.22	0.51	0.93	0.04	0.09	0.07	0.03	0.14	0.06	0.13	0.04	0.08	0.07	0.04	0.12	0.04	0.11	988
0.15	0.59	1.08	0.95	0.41	1.75	0.67	1.43	0.05	0.11	0.10	0.04	0.17	0.06	0.16	0.06	0.09	0.09	0.05	0.14	0.04	0.13	771
0.18	0.82	1.51	1.29	0.52	2.50	0.99	1.94	0.07	0.12	0.12	0.06	0.19	0.07	0.17	0.07	0.11	0.11	0.06	0.15	0.04	0.14	1039
0.32	1.30	2.73	2.17	0.66	4.80	2.07	3.50	0.09	0.15	0.15	0.08	0.22	0.07	0.20	0.10	0.13	0.13	0.08	0.18	0.05	0.17	2868


==> data/mlm_plots/tef/agnews/roberta/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/agnews/roberta/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.93	0.94	0.95	0.92	0.97	0.02	0.96	0.91	0.94	0.94	0.90	0.97	0.04	0.96	0.94	0.96	0.98	0.91	1.00	0.05	0.99	650
0.06	0.90	0.92	0.92	0.89	0.94	0.03	0.93	0.88	0.91	0.91	0.86	0.95	0.04	0.94	0.92	0.94	0.96	0.88	1.00	0.06	0.98	1068
0.11	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.85	0.88	0.88	0.83	0.93	0.05	0.91	0.89	0.92	0.94	0.86	0.99	0.07	0.97	988
0.15	0.85	0.87	0.87	0.83	0.90	0.03	0.89	0.82	0.85	0.86	0.81	0.90	0.05	0.89	0.87	0.91	0.93	0.84	0.98	0.07	0.96	771
0.18	0.82	0.84	0.84	0.81	0.88	0.03	0.87	0.80	0.83	0.83	0.79	0.88	0.05	0.87	0.85	0.89	0.90	0.81	0.96	0.07	0.95	1039
0.32	0.77	0.80	0.80	0.76	0.84	0.04	0.83	0.75	0.79	0.79	0.74	0.84	0.05	0.83	0.80	0.85	0.86	0.77	0.94	0.09	0.92	2868


==> data/mlm_plots/tef/agnews/roberta/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/agnews/roberta/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.27	0.29	0.28	0.25	0.33	0.04	0.29	0.05	0.14	0.09	-0.00	0.27	0.14	0.17	0.37	1.49	0.87	-0.53	3.50	2.01	1.92	650
0.06	0.38	0.43	0.40	0.36	0.50	0.07	0.47	0.07	0.19	0.14	0.03	0.35	0.16	0.25	0.62	2.26	1.49	-0.28	4.79	2.53	2.99	1068
0.11	0.51	0.61	0.57	0.45	0.77	0.16	0.70	0.10	0.24	0.18	0.05	0.43	0.19	0.32	0.84	2.93	2.00	-0.18	6.03	3.10	4.10	988
0.15	0.73	0.79	0.76	0.62	0.97	0.18	0.81	0.13	0.29	0.23	0.08	0.51	0.22	0.41	0.97	3.54	2.49	-0.17	7.24	3.70	5.09	771
0.18	1.10	1.23	1.20	0.99	1.47	0.24	1.31	0.16	0.33	0.26	0.10	0.57	0.24	0.47	1.21	4.03	2.97	0.07	8.00	3.96	5.63	1039
0.32	1.50	1.82	1.77	1.40	2.23	0.41	2.13	0.17	0.35	0.28	0.12	0.59	0.24	0.48	1.42	4.61	3.47	0.44	8.78	4.17	6.75	2868


==> data/mlm_plots/tef/agnews/roberta/a/time_misc_auc.tex <==
name	auc
attack_time	0.31
l2	0.08
lom	1.03


==> data/mlm_plots/tef/agnews/roberta/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.50	0.61	0.67	0.33	0.88	0.28	0.75	0.73	0.79	0.80	0.66	0.92	0.13	0.89	0.82	0.86	0.88	0.79	0.94	0.08	0.92	650
0.06	0.25	0.45	0.50	0.15	0.75	0.30	0.67	0.60	0.70	0.71	0.54	0.85	0.16	0.82	0.75	0.81	0.82	0.71	0.91	0.10	0.88	1068
0.11	0.00	0.35	0.33	0.06	0.64	0.29	0.50	0.55	0.63	0.67	0.46	0.80	0.17	0.75	0.70	0.77	0.78	0.66	0.88	0.11	0.85	988
0.15	0.00	0.28	0.25	-0.01	0.57	0.29	0.50	0.50	0.59	0.60	0.41	0.77	0.18	0.73	0.67	0.74	0.75	0.63	0.85	0.11	0.82	771
0.18	0.00	0.23	0.00	-0.05	0.50	0.28	0.33	0.40	0.53	0.50	0.33	0.72	0.19	0.67	0.63	0.71	0.71	0.58	0.83	0.12	0.80	1039
0.32	0.00	0.15	0.00	-0.09	0.39	0.24	0.33	0.25	0.43	0.42	0.21	0.64	0.22	0.58	0.53	0.64	0.65	0.49	0.78	0.14	0.75	2868


==> data/mlm_plots/tef/agnews/roberta/a/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.16
top50	0.21


==> data/mlm_plots/tef/agnews/roberta/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	93.47	169.37	139.92	52.31	286.42	117.06	209.86	3.00	4.36	4.00	2.44	6.28	1.92	6.00	112.57	195.41	161.54	67.58	323.25	127.83	235.53	3.00	4.47	4.00	2.52	6.41	1.94	6.00	651
0.06	99.76	178.46	148.91	55.43	301.49	123.03	220.69	3.00	4.71	5.00	2.64	6.79	2.08	6.00	133.86	231.13	195.53	79.87	382.38	151.25	281.12	3.00	4.88	5.00	2.79	6.98	2.09	6.00	1199
0.11	100.55	182.48	150.72	59.42	305.54	123.06	224.08	3.00	4.58	4.00	2.54	6.62	2.04	6.00	165.65	283.06	242.19	105.91	460.22	177.16	342.30	3.00	4.88	5.00	2.78	6.98	2.10	6.00	1388
0.15	99.28	174.52	146.42	50.43	298.61	124.09	220.26	3.00	4.71	5.00	2.70	6.72	2.01	6.00	205.24	327.04	294.30	136.21	517.88	190.83	401.69	4.00	5.10	5.00	3.01	7.19	2.09	7.00	1244
0.18	96.43	173.62	145.35	52.65	294.59	120.97	214.16	3.00	4.74	5.00	2.64	6.85	2.10	6.00	233.93	381.16	330.10	157.63	604.69	223.53	471.46	4.00	5.27	5.00	3.07	7.47	2.20	7.00	1094
0.32	99.61	182.90	147.48	48.41	317.40	134.50	226.84	3.00	4.41	4.00	2.33	6.49	2.08	6.00	310.81	539.14	451.32	178.47	899.81	360.67	664.87	3.00	5.01	5.00	2.80	7.21	2.21	6.00	1788


==> data/mlm_plots/tef/agnews/roberta/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	51.53
orig_ge	1.34
adv_pp	106.21
adv_ge	1.46


==> data/mlm_plots/tef/agnews/roberta/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	-0.27	0.01	0.03	-0.40	0.43	0.42	0.30	-0.04	0.19	0.19	-0.13	0.51	0.32	0.41	-0.03	0.15	0.14	-0.10	0.40	0.25	0.30	651
0.06	-0.45	-0.20	-0.17	-0.57	0.17	0.37	0.06	-0.16	0.02	0.03	-0.29	0.33	0.31	0.23	-0.11	0.02	0.03	-0.21	0.25	0.23	0.17	1199
0.11	-0.57	-0.34	-0.31	-0.66	-0.01	0.33	-0.10	-0.28	-0.10	-0.08	-0.40	0.20	0.30	0.11	-0.20	-0.07	-0.05	-0.29	0.16	0.23	0.09	1388
0.15	-0.63	-0.42	-0.39	-0.70	-0.13	0.29	-0.22	-0.34	-0.18	-0.17	-0.43	0.08	0.25	-0.02	-0.24	-0.12	-0.11	-0.32	0.07	0.19	-0.01	1244
0.18	-0.60	-0.42	-0.40	-0.67	-0.17	0.25	-0.25	-0.33	-0.19	-0.18	-0.43	0.05	0.24	-0.04	-0.23	-0.13	-0.12	-0.31	0.04	0.18	-0.02	1094
0.32	-0.62	-0.47	-0.47	-0.69	-0.26	0.21	-0.33	-0.39	-0.25	-0.27	-0.46	-0.03	0.22	-0.09	-0.28	-0.18	-0.18	-0.34	-0.01	0.16	-0.07	1788


==> data/mlm_plots/tef/agnews/roberta/ig/correlations_auc.tex <==
name	auc
pcc	-0.11
spearman	-0.04
kendall	-0.03


==> data/mlm_plots/tef/agnews/roberta/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	5.72	10.03	8.71	3.86	16.20	6.17	13.07	4.43	10.73	7.68	1.10	20.35	9.63	13.13	6.87	22.58	16.43	3.21	41.96	19.37	33.97	651
0.06	5.38	8.06	7.24	4.09	12.03	3.97	9.62	4.38	8.48	6.43	1.84	15.12	6.64	10.15	5.97	21.64	14.23	1.96	41.33	19.69	31.08	1199
0.11	4.87	6.66	6.22	4.00	9.32	2.66	7.86	4.10	6.80	5.63	2.74	10.87	4.07	8.32	6.15	18.92	12.21	0.99	36.85	17.93	25.63	1388
0.15	4.29	5.69	5.41	3.69	7.69	2.00	6.65	3.76	5.59	5.09	2.90	8.28	2.69	6.67	5.66	16.69	10.37	0.28	33.11	16.41	21.66	1244
0.18	3.81	4.89	4.59	3.25	6.52	1.64	5.62	3.35	4.79	4.35	2.72	6.86	2.07	5.60	4.79	12.00	7.54	-0.28	24.28	12.28	14.12	1094
0.32	3.33	4.19	3.98	2.89	5.49	1.30	4.70	3.03	4.08	3.70	2.52	5.63	1.56	4.72	4.14	9.54	6.09	-0.56	19.64	10.10	10.24	1788


==> data/mlm_plots/tef/agnews/roberta/ig/ets_sts_auc.tex <==
name	auc
et_use	1.68
et_tse	1.69
et_ce	4.33


==> data/mlm_plots/tef/agnews/roberta/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.56	7.94	2.93	-12.39	28.27	20.33	6.51	7.41	25.58	15.92	-1.75	52.92	27.34	32.52	7.03	32.58	16.77	-12.21	77.36	44.78	39.75	651
0.06	1.08	6.64	2.06	-21.18	34.45	27.82	4.03	7.31	18.63	13.12	0.09	37.17	18.54	21.49	6.46	26.22	13.14	-30.29	82.73	56.51	26.19	1199
0.11	0.75	3.18	1.17	-12.00	18.37	15.19	2.20	6.27	13.05	9.33	1.37	24.73	11.68	15.23	5.38	16.69	9.70	-9.32	42.70	26.01	17.78	1388
0.15	0.50	1.43	0.76	-5.97	8.83	7.40	1.20	5.64	10.08	8.04	2.45	17.71	7.63	12.17	4.51	12.86	7.55	-10.22	35.94	23.08	14.01	1244
0.18	0.37	0.98	0.58	-1.30	3.26	2.28	0.88	5.11	8.45	6.75	3.21	13.69	5.24	10.25	4.18	9.58	5.84	-1.36	20.51	10.93	11.32	1094
0.32	0.24	0.96	0.37	-7.10	9.02	8.06	0.60	4.65	7.54	6.02	1.86	13.22	5.68	8.39	3.83	9.89	5.13	-16.36	36.14	26.25	8.56	1788


==> data/mlm_plots/tef/agnews/roberta/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.72
et_p_h	3.30
et_p_l2	4.22


==> data/mlm_plots/tef/agnews/roberta/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.07	0.20	0.15	0.03	0.38	0.18	0.29	0.01	0.04	0.03	-0.00	0.09	0.04	0.06	0.01	0.04	0.03	0.01	0.07	0.03	0.05	651
0.06	0.14	0.36	0.31	0.08	0.65	0.28	0.52	0.02	0.06	0.04	0.01	0.11	0.05	0.09	0.03	0.06	0.05	0.02	0.09	0.04	0.08	1199
0.11	0.31	0.65	0.57	0.19	1.11	0.46	0.89	0.04	0.08	0.07	0.03	0.14	0.06	0.12	0.04	0.07	0.07	0.04	0.11	0.04	0.10	1388
0.15	0.58	1.06	0.91	0.34	1.78	0.72	1.38	0.05	0.11	0.10	0.04	0.17	0.06	0.15	0.06	0.09	0.09	0.05	0.14	0.04	0.12	1244
0.18	0.79	1.46	1.27	0.49	2.42	0.97	1.87	0.06	0.12	0.12	0.06	0.19	0.07	0.17	0.07	0.11	0.11	0.06	0.15	0.04	0.14	1094
0.32	1.19	2.36	1.98	0.66	4.06	1.70	3.02	0.09	0.14	0.14	0.07	0.21	0.07	0.19	0.09	0.12	0.12	0.08	0.17	0.05	0.15	1788


==> data/mlm_plots/tef/agnews/roberta/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.37
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/agnews/roberta/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.96	0.91	0.93	0.94	0.89	0.97	0.04	0.96	0.93	0.95	0.98	0.90	1.00	0.05	0.99	651
0.06	0.90	0.92	0.92	0.89	0.94	0.03	0.93	0.88	0.90	0.91	0.86	0.95	0.05	0.94	0.91	0.93	0.96	0.87	1.00	0.07	0.98	1199
0.11	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.85	0.88	0.88	0.83	0.93	0.05	0.92	0.89	0.93	0.95	0.86	0.99	0.06	0.97	1388
0.15	0.85	0.87	0.87	0.83	0.90	0.03	0.89	0.83	0.86	0.86	0.81	0.90	0.05	0.89	0.87	0.91	0.93	0.84	0.98	0.07	0.97	1244
0.18	0.82	0.84	0.85	0.81	0.88	0.04	0.87	0.80	0.83	0.84	0.78	0.88	0.05	0.87	0.86	0.89	0.91	0.83	0.96	0.07	0.95	1094
0.32	0.79	0.81	0.82	0.77	0.85	0.04	0.84	0.77	0.80	0.80	0.75	0.86	0.05	0.84	0.82	0.87	0.88	0.79	0.95	0.08	0.93	1788


==> data/mlm_plots/tef/agnews/roberta/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/agnews/roberta/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.41	0.46	0.42	0.25	0.67	0.21	0.44	3.63	9.10	6.36	-0.34	18.53	9.43	11.15	2.24	6.64	5.14	1.00	12.27	5.63	9.56	651
0.06	0.56	0.79	0.61	0.34	1.24	0.45	0.81	4.80	12.92	8.22	-9.51	35.35	22.43	14.20	2.59	7.08	5.57	1.29	12.88	5.79	10.03	1199
0.11	0.86	1.33	1.16	0.77	1.89	0.56	1.75	6.38	32.08	9.99	-224.61	288.77	256.69	17.72	2.53	7.39	5.54	1.27	13.52	6.13	10.68	1388
0.15	1.36	1.75	1.63	1.29	2.21	0.46	2.17	6.93	16.43	10.91	-9.68	42.54	26.11	18.57	2.94	7.75	6.27	1.46	14.04	6.29	11.44	1244
0.18	1.73	1.98	1.94	1.69	2.28	0.30	2.20	5.98	12.59	9.03	1.23	23.95	11.36	15.70	2.47	7.55	6.27	1.38	13.72	6.17	10.90	1094
0.32	2.08	2.25	2.25	2.02	2.47	0.23	2.40	5.84	12.25	9.27	1.11	23.40	11.14	14.85	2.49	7.32	5.98	1.19	13.44	6.12	10.33	1788


==> data/mlm_plots/tef/agnews/roberta/ig/time_misc_auc.tex <==
name	auc
attack_time	0.49
l2	4.62
lom	2.14


==> data/mlm_plots/tef/agnews/roberta/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.24	0.25	-0.02	0.49	0.26	0.33	0.29	0.42	0.42	0.24	0.61	0.19	0.56	0.48	0.58	0.58	0.45	0.72	0.14	0.67	651
0.06	0.00	0.15	0.00	-0.06	0.37	0.21	0.33	0.22	0.34	0.33	0.17	0.52	0.17	0.45	0.43	0.52	0.53	0.39	0.65	0.13	0.60	1199
0.11	0.00	0.11	0.00	-0.07	0.28	0.18	0.25	0.18	0.30	0.30	0.14	0.46	0.16	0.42	0.40	0.48	0.48	0.35	0.61	0.13	0.56	1388
0.15	0.00	0.06	0.00	-0.07	0.20	0.13	0.00	0.17	0.26	0.25	0.12	0.40	0.14	0.33	0.39	0.45	0.45	0.34	0.57	0.11	0.53	1244
0.18	0.00	0.06	0.00	-0.08	0.19	0.13	0.00	0.17	0.25	0.25	0.11	0.39	0.14	0.33	0.38	0.45	0.45	0.34	0.56	0.11	0.53	1094
0.32	0.00	0.04	0.00	-0.07	0.16	0.11	0.00	0.11	0.21	0.20	0.08	0.34	0.13	0.30	0.36	0.43	0.43	0.33	0.54	0.11	0.50	1788


==> data/mlm_plots/tef/agnews/roberta/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.08
top50	0.14


==> data/mlm_plots/tef/agnews/roberta/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	97.55	174.01	141.95	57.78	290.24	116.23	215.73	3.00	4.45	4.00	2.47	6.42	1.98	6.00	119.24	210.53	173.25	66.67	354.38	143.86	260.03	3.00	4.56	4.00	2.57	6.55	1.99	6.00	644
0.06	99.64	176.94	147.56	57.70	296.18	119.24	223.34	3.00	4.65	4.00	2.58	6.71	2.07	6.00	144.18	249.61	213.58	93.09	406.13	156.52	312.83	3.00	4.84	5.00	2.76	6.92	2.08	6.00	1063
0.11	99.43	176.86	145.19	52.68	301.04	124.18	218.01	3.00	4.61	4.50	2.59	6.63	2.02	6.00	172.92	304.10	252.85	104.76	503.43	199.34	373.58	3.00	4.95	5.00	2.88	7.03	2.08	6.00	1026
0.15	99.62	176.39	147.33	53.58	299.20	122.81	223.66	3.00	4.67	4.00	2.59	6.76	2.09	6.00	217.30	364.56	315.92	141.79	587.32	222.77	454.10	4.00	5.14	5.00	3.00	7.27	2.13	7.00	849
0.18	98.38	174.75	143.86	54.56	294.93	120.18	219.24	3.00	4.59	4.00	2.53	6.65	2.06	6.00	254.08	441.39	369.92	160.80	721.98	280.59	551.64	4.00	5.19	5.00	3.03	7.34	2.15	7.00	1122
0.32	99.33	179.38	149.17	52.28	306.48	127.10	223.21	3.00	4.59	4.00	2.50	6.67	2.09	6.00	347.70	609.12	510.99	207.57	1010.66	401.55	741.97	4.00	5.40	5.00	3.15	7.66	2.25	7.00	2691


==> data/mlm_plots/tef/agnews/roberta/s/comparison_vals_auc.tex <==
name	auc
orig_pp	51.22
orig_ge	1.34
adv_pp	119.42
adv_ge	1.48


==> data/mlm_plots/tef/agnews/roberta/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.70	0.78	0.84	0.59	0.97	0.19	0.92	0.79	0.85	0.88	0.73	0.96	0.12	0.93	0.64	0.71	0.73	0.58	0.83	0.13	0.80	644
0.06	0.41	0.58	0.62	0.33	0.83	0.25	0.78	0.65	0.72	0.77	0.54	0.91	0.18	0.86	0.49	0.57	0.60	0.41	0.74	0.16	0.69	1063
0.11	0.21	0.40	0.42	0.13	0.67	0.27	0.61	0.47	0.59	0.66	0.34	0.84	0.25	0.78	0.34	0.45	0.49	0.25	0.65	0.20	0.60	1026
0.15	0.12	0.29	0.29	0.05	0.52	0.23	0.45	0.35	0.51	0.56	0.25	0.76	0.25	0.70	0.26	0.38	0.41	0.18	0.57	0.19	0.52	849
0.18	0.02	0.18	0.17	-0.05	0.40	0.22	0.33	0.22	0.40	0.43	0.13	0.66	0.27	0.60	0.16	0.29	0.31	0.09	0.49	0.20	0.44	1122
0.32	-0.10	0.05	0.04	-0.16	0.26	0.21	0.18	0.04	0.24	0.26	-0.05	0.53	0.29	0.47	0.03	0.17	0.18	-0.03	0.38	0.21	0.33	2691


==> data/mlm_plots/tef/agnews/roberta/s/correlations_auc.tex <==
name	auc
pcc	0.08
spearman	0.14
kendall	0.10


==> data/mlm_plots/tef/agnews/roberta/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	0.76	2.28	1.48	-0.06	4.62	2.34	2.97	0.75	2.47	1.53	-0.51	5.44	2.98	2.97	1.07	4.75	2.74	-1.12	10.62	5.87	5.77	644
0.06	1.39	2.81	2.36	0.83	4.79	1.98	3.75	1.28	3.04	2.21	0.13	5.96	2.92	3.80	1.99	7.15	4.42	-0.44	14.75	7.60	9.35	1063
0.11	1.83	3.02	2.70	1.22	4.83	1.80	3.80	1.64	3.03	2.48	0.71	5.36	2.32	3.74	2.41	7.97	4.92	-0.55	16.50	8.53	10.18	1026
0.15	1.96	2.89	2.75	1.55	4.23	1.34	3.51	1.80	2.83	2.46	1.03	4.63	1.80	3.37	2.57	7.98	4.62	-0.57	16.53	8.55	9.50	849
0.18	2.04	2.84	2.66	1.64	4.04	1.20	3.32	1.90	2.87	2.52	1.21	4.53	1.66	3.27	2.70	7.06	4.34	-0.19	14.31	7.25	7.72	1122
0.32	2.02	2.55	2.42	1.71	3.40	0.84	2.93	1.86	2.52	2.30	1.48	3.57	1.04	2.91	2.45	5.33	3.55	-0.12	10.78	5.45	6.11	2691


==> data/mlm_plots/tef/agnews/roberta/s/ets_sts_auc.tex <==
name	auc
et_use	0.80
et_tse	0.82
et_ce	1.98


==> data/mlm_plots/tef/agnews/roberta/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.16	1.12	0.39	-1.64	3.88	2.76	0.91	0.97	5.10	2.47	-1.97	12.18	7.08	6.21	0.89	7.61	2.66	-5.78	20.99	13.38	7.88	644
0.06	0.24	1.12	0.48	-2.06	4.30	3.18	0.94	1.66	5.45	3.36	-1.25	12.14	6.69	6.57	1.41	7.53	3.25	-9.08	24.15	16.61	7.24	1063
0.11	0.23	0.92	0.39	-1.98	3.82	2.90	0.71	2.24	5.31	3.64	-0.75	11.36	6.06	5.92	1.94	7.31	3.21	-12.77	27.39	20.08	6.64	1026
0.15	0.20	0.50	0.32	-0.31	1.32	0.82	0.54	2.52	4.55	3.60	0.22	8.88	4.33	5.40	2.08	5.61	3.12	-5.56	16.79	11.17	5.35	849
0.18	0.17	0.46	0.26	-1.18	2.10	1.64	0.43	2.68	4.36	3.60	1.35	7.38	3.01	5.06	2.24	5.48	3.07	-8.89	19.85	14.37	5.16	1122
0.32	0.12	0.43	0.20	-2.35	3.22	2.78	0.33	2.72	4.30	3.56	1.39	7.21	2.91	4.86	2.25	5.13	3.07	-4.72	14.98	9.85	4.80	2691


==> data/mlm_plots/tef/agnews/roberta/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.19
et_p_h	1.36
et_p_l2	1.76


==> data/mlm_plots/tef/agnews/roberta/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.12	0.25	0.21	0.07	0.43	0.18	0.34	0.01	0.05	0.03	0.00	0.09	0.05	0.06	0.02	0.04	0.03	0.01	0.08	0.03	0.06	644
0.06	0.23	0.48	0.39	0.11	0.86	0.37	0.65	0.03	0.07	0.06	0.02	0.13	0.06	0.12	0.03	0.07	0.06	0.02	0.11	0.04	0.09	1063
0.11	0.41	0.83	0.71	0.24	1.43	0.60	1.12	0.04	0.10	0.09	0.04	0.16	0.06	0.15	0.05	0.08	0.08	0.04	0.13	0.04	0.12	1026
0.15	0.67	1.25	1.07	0.44	2.07	0.82	1.73	0.06	0.12	0.11	0.05	0.18	0.07	0.17	0.07	0.10	0.10	0.06	0.14	0.04	0.13	849
0.18	0.94	1.78	1.55	0.61	2.95	1.17	2.36	0.08	0.13	0.13	0.07	0.20	0.07	0.18	0.08	0.11	0.12	0.07	0.16	0.04	0.15	1122
0.32	1.44	2.92	2.37	0.70	5.15	2.22	3.80	0.10	0.15	0.16	0.08	0.23	0.07	0.20	0.10	0.13	0.13	0.09	0.18	0.05	0.17	2691


==> data/mlm_plots/tef/agnews/roberta/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.46
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/agnews/roberta/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.93	0.94	0.95	0.92	0.97	0.02	0.96	0.92	0.94	0.95	0.90	0.98	0.04	0.97	0.94	0.95	0.97	0.90	1.00	0.05	0.99	644
0.06	0.90	0.92	0.92	0.89	0.94	0.03	0.94	0.89	0.91	0.92	0.87	0.95	0.04	0.94	0.92	0.94	0.96	0.89	0.99	0.05	0.98	1063
0.11	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.85	0.88	0.88	0.84	0.93	0.05	0.92	0.89	0.92	0.94	0.86	0.99	0.06	0.97	1026
0.15	0.85	0.87	0.87	0.83	0.90	0.03	0.89	0.83	0.86	0.86	0.81	0.90	0.05	0.89	0.87	0.91	0.93	0.84	0.98	0.07	0.97	849
0.18	0.82	0.85	0.85	0.81	0.88	0.03	0.87	0.80	0.84	0.84	0.79	0.89	0.05	0.87	0.86	0.90	0.91	0.83	0.96	0.07	0.95	1122
0.32	0.77	0.80	0.81	0.76	0.85	0.04	0.83	0.76	0.80	0.79	0.74	0.85	0.05	0.83	0.81	0.86	0.87	0.77	0.94	0.08	0.92	2691


==> data/mlm_plots/tef/agnews/roberta/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/agnews/roberta/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.31	0.33	0.32	0.29	0.37	0.04	0.34	1.07	22.39	2.61	-44.27	89.05	66.66	10.36	0.36	1.09	0.81	0.01	2.18	1.09	1.42	644
0.06	0.41	0.48	0.45	0.33	0.63	0.15	0.51	1.90	36.38	4.26	-81.54	154.30	117.92	15.12	0.50	1.56	1.16	0.11	3.01	1.45	2.09	1063
0.11	0.54	0.67	0.57	0.40	0.94	0.27	0.76	2.87	63.57	7.46	-118.26	245.40	181.83	30.36	0.77	2.12	1.68	0.28	3.95	1.83	3.05	1026
0.15	0.80	0.97	0.86	0.62	1.33	0.35	0.94	4.03	85.39	10.80	-150.50	321.29	235.90	42.75	0.88	2.40	1.93	0.46	4.34	1.94	3.40	849
0.18	1.04	1.23	1.11	0.90	1.55	0.32	1.25	4.96	114.18	11.44	-180.25	408.61	294.43	54.68	0.95	2.52	1.99	0.55	4.48	1.97	3.68	1122
0.32	1.81	1.94	1.92	1.75	2.12	0.18	2.05	6.42	130.47	18.11	-199.85	460.78	330.32	79.22	1.15	2.87	2.42	0.70	5.04	2.17	4.12	2691


==> data/mlm_plots/tef/agnews/roberta/s/time_misc_auc.tex <==
name	auc
attack_time	0.33
l2	26.49
lom	0.67


==> data/mlm_plots/tef/agnews/roberta/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.40	0.59	0.67	0.32	0.85	0.26	0.75	0.70	0.77	0.80	0.64	0.90	0.13	0.88	0.81	0.85	0.86	0.77	0.94	0.08	0.91	644
0.06	0.00	0.40	0.33	0.10	0.69	0.30	0.67	0.56	0.66	0.67	0.50	0.82	0.16	0.78	0.73	0.79	0.80	0.68	0.89	0.10	0.86	1063
0.11	0.00	0.26	0.25	-0.00	0.52	0.26	0.33	0.44	0.56	0.58	0.38	0.75	0.18	0.70	0.67	0.73	0.75	0.60	0.85	0.12	0.82	1026
0.15	0.00	0.18	0.00	-0.04	0.41	0.22	0.33	0.40	0.50	0.50	0.32	0.68	0.18	0.62	0.62	0.69	0.71	0.57	0.81	0.12	0.78	849
0.18	0.00	0.11	0.00	-0.08	0.30	0.19	0.25	0.30	0.43	0.44	0.25	0.60	0.17	0.55	0.56	0.64	0.65	0.52	0.77	0.12	0.73	1122
0.32	0.00	0.06	0.00	-0.08	0.20	0.14	0.00	0.22	0.35	0.33	0.18	0.52	0.17	0.45	0.50	0.59	0.59	0.46	0.71	0.13	0.68	2691


==> data/mlm_plots/tef/agnews/roberta/s/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.14
top50	0.20


==> data/mlm_plots/tef/agnews/xlnet/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	103.53	196.61	153.86	56.87	336.36	139.75	251.40	3.00	4.11	4.00	2.21	6.01	1.90	5.00	122.21	232.73	189.22	65.83	399.64	166.90	307.91	3.00	4.13	4.00	2.23	6.03	1.90	6.00	145
0.06	107.16	191.24	159.06	64.47	318.00	126.77	239.49	3.00	4.29	4.00	2.51	6.08	1.78	5.00	142.50	249.75	208.09	88.11	411.39	161.64	315.73	3.00	4.31	4.00	2.55	6.07	1.76	5.00	1080
0.11	105.17	194.63	159.32	60.07	329.20	134.56	246.31	3.00	4.20	4.00	2.41	6.00	1.80	5.00	169.89	295.64	253.63	110.28	481.00	185.36	370.50	3.00	4.37	4.00	2.59	6.16	1.78	5.00	1147
0.15	105.49	187.16	148.71	53.03	321.30	134.14	232.02	3.00	4.24	4.00	2.47	6.00	1.76	5.00	204.23	341.67	294.08	128.24	555.10	213.43	414.46	3.00	4.46	4.00	2.71	6.20	1.75	5.00	902
0.18	104.87	191.53	159.06	61.70	321.35	129.83	241.94	3.00	4.27	4.00	2.45	6.10	1.83	5.00	246.79	413.37	357.98	164.10	662.65	249.28	512.69	3.00	4.62	4.00	2.75	6.50	1.87	6.00	1087
0.32	107.96	197.37	163.68	64.99	329.75	132.38	254.72	3.00	4.29	4.00	2.46	6.12	1.83	5.00	334.92	572.03	487.86	207.94	936.12	364.09	707.17	3.00	4.87	5.00	2.96	6.77	1.91	6.00	2432


==> data/mlm_plots/tef/agnews/xlnet/a/comparison_vals_auc.tex <==
name	auc
orig_pp	55.97
orig_ge	1.23
adv_pp	113.58
adv_ge	1.32


==> data/mlm_plots/tef/agnews/xlnet/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.54	0.70	0.81	0.39	1.00	0.31	0.93	0.71	0.77	0.85	0.53	1.01	0.24	0.93	0.54	0.64	0.69	0.41	0.87	0.23	0.81	145
0.06	0.28	0.51	0.54	0.19	0.83	0.32	0.78	0.54	0.67	0.75	0.41	0.94	0.27	0.88	0.38	0.54	0.58	0.30	0.77	0.24	0.72	1080
0.11	0.17	0.41	0.42	0.09	0.73	0.32	0.68	0.45	0.60	0.68	0.31	0.89	0.29	0.81	0.33	0.47	0.51	0.23	0.71	0.24	0.64	1147
0.15	0.05	0.32	0.30	-0.02	0.65	0.33	0.59	0.33	0.51	0.61	0.19	0.84	0.32	0.76	0.24	0.40	0.45	0.14	0.65	0.26	0.58	902
0.18	0.01	0.25	0.21	-0.07	0.56	0.31	0.49	0.26	0.46	0.53	0.14	0.78	0.32	0.71	0.18	0.35	0.38	0.10	0.60	0.25	0.54	1087
0.32	-0.13	0.11	0.06	-0.20	0.41	0.31	0.31	0.04	0.31	0.35	-0.05	0.67	0.36	0.59	0.03	0.23	0.25	-0.04	0.50	0.27	0.43	2432


==> data/mlm_plots/tef/agnews/xlnet/a/correlations_auc.tex <==
name	auc
pcc	0.09
spearman	0.14
kendall	0.11


==> data/mlm_plots/tef/agnews/xlnet/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	0.56	2.61	1.77	-0.23	5.46	2.84	3.54	0.51	2.98	1.40	-0.87	6.83	3.85	4.06	1.27	6.89	3.48	-1.62	15.40	8.51	8.97	145
0.06	1.25	3.05	2.60	0.67	5.43	2.38	4.16	1.07	2.97	2.37	0.24	5.70	2.73	4.01	1.73	7.34	4.08	-1.05	15.73	8.39	9.54	1080
0.11	1.38	2.75	2.46	0.89	4.60	1.85	3.62	1.23	2.60	2.19	0.59	4.61	2.01	3.37	1.84	6.52	3.61	-1.44	14.48	7.96	7.81	1147
0.15	1.51	2.51	2.41	1.11	3.92	1.40	3.38	1.40	2.39	2.18	0.90	3.89	1.49	3.05	1.91	5.36	3.51	-0.76	11.49	6.13	6.37	902
0.18	1.56	2.39	2.35	1.22	3.55	1.16	3.07	1.47	2.30	2.19	1.07	3.52	1.23	2.89	1.91	5.46	3.44	-0.85	11.78	6.32	6.24	1087
0.32	1.71	2.32	2.33	1.37	3.26	0.95	2.85	1.59	2.24	2.19	1.26	3.21	0.98	2.72	2.06	4.77	3.30	-0.46	10.00	5.23	5.31	2432


==> data/mlm_plots/tef/agnews/xlnet/a/ets_sts_auc.tex <==
name	auc
et_use	0.74
et_tse	0.71
et_ce	1.67


==> data/mlm_plots/tef/agnews/xlnet/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.15	2.01	0.59	-2.32	6.34	4.33	2.11	0.97	8.99	3.28	-4.08	22.05	13.06	11.24	1.08	11.88	4.48	-8.87	32.62	20.74	14.80	145
0.06	0.31	2.11	0.70	-7.71	11.94	9.82	1.51	2.27	9.51	5.57	-1.80	20.82	11.31	13.17	2.05	12.01	5.72	-6.99	31.02	19.00	15.12	1080
0.11	0.25	2.08	0.52	-11.06	15.22	13.14	1.08	2.15	7.79	4.60	-1.69	17.27	9.48	10.38	1.91	10.00	4.50	-7.07	27.07	17.07	11.09	1147
0.15	0.20	1.01	0.37	-3.79	5.81	4.80	0.74	2.28	6.01	4.21	-0.35	12.38	6.36	7.76	1.90	8.23	3.84	-7.96	24.41	16.19	8.56	902
0.18	0.17	0.76	0.30	-3.48	4.99	4.23	0.57	2.44	5.34	3.78	0.36	10.31	4.97	6.62	2.02	7.04	3.42	-8.07	22.16	15.12	7.05	1087
0.32	0.14	0.47	0.22	-1.72	2.67	2.20	0.39	2.59	4.94	3.66	-0.21	10.08	5.15	5.54	2.19	7.66	3.13	-18.81	34.13	26.47	5.63	2432


==> data/mlm_plots/tef/agnews/xlnet/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.34
et_p_h	1.87
et_p_l2	2.52


==> data/mlm_plots/tef/agnews/xlnet/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.09	0.22	0.20	0.04	0.41	0.18	0.31	0.01	0.04	0.02	-0.00	0.08	0.04	0.05	0.01	0.04	0.02	0.00	0.07	0.03	0.06	145
0.06	0.16	0.37	0.31	0.06	0.68	0.31	0.51	0.02	0.05	0.03	0.00	0.10	0.05	0.07	0.02	0.05	0.03	0.01	0.08	0.04	0.07	1080
0.11	0.29	0.64	0.54	0.14	1.13	0.49	0.86	0.03	0.07	0.06	0.02	0.13	0.06	0.11	0.03	0.07	0.06	0.02	0.11	0.04	0.10	1147
0.15	0.49	1.01	0.85	0.29	1.74	0.73	1.36	0.04	0.10	0.08	0.03	0.16	0.06	0.15	0.05	0.09	0.08	0.04	0.13	0.05	0.12	902
0.18	0.69	1.45	1.20	0.34	2.55	1.11	1.90	0.05	0.12	0.11	0.05	0.18	0.07	0.17	0.06	0.10	0.10	0.05	0.15	0.05	0.13	1087
0.32	1.08	2.38	1.86	0.40	4.36	1.98	3.06	0.08	0.14	0.14	0.06	0.22	0.08	0.20	0.08	0.12	0.12	0.07	0.17	0.05	0.16	2432


==> data/mlm_plots/tef/agnews/xlnet/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.37
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/agnews/xlnet/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.94	0.94	0.91	0.96	0.02	0.95	0.90	0.93	0.93	0.88	0.97	0.04	0.96	0.94	0.96	0.98	0.92	1.00	0.04	0.99	145
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.87	0.90	0.91	0.85	0.94	0.05	0.93	0.90	0.93	0.95	0.87	0.99	0.06	0.98	1080
0.11	0.86	0.88	0.88	0.85	0.92	0.04	0.91	0.83	0.87	0.87	0.82	0.92	0.05	0.91	0.87	0.91	0.93	0.84	0.98	0.07	0.97	1147
0.15	0.83	0.86	0.86	0.82	0.89	0.04	0.88	0.81	0.84	0.84	0.79	0.89	0.05	0.88	0.85	0.89	0.90	0.81	0.97	0.08	0.95	902
0.18	0.81	0.83	0.84	0.80	0.87	0.04	0.86	0.79	0.82	0.82	0.77	0.87	0.05	0.86	0.84	0.88	0.89	0.80	0.96	0.08	0.94	1087
0.32	0.77	0.80	0.80	0.76	0.84	0.04	0.83	0.75	0.79	0.79	0.73	0.84	0.05	0.82	0.80	0.85	0.86	0.76	0.94	0.09	0.91	2432


==> data/mlm_plots/tef/agnews/xlnet/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.24
sts_ce	0.26


==> data/mlm_plots/tef/agnews/xlnet/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.48	0.54	0.52	0.46	0.63	0.09	0.57	0.04	0.09	0.07	0.02	0.15	0.06	0.11	0.49	2.01	1.18	-0.19	4.22	2.21	2.63	145
0.06	0.56	0.71	0.64	0.43	0.99	0.28	0.76	0.07	0.13	0.11	0.05	0.21	0.08	0.17	1.00	3.17	2.19	0.08	6.25	3.08	4.32	1080
0.11	0.84	1.18	1.01	0.69	1.68	0.50	1.33	0.09	0.14	0.13	0.06	0.23	0.08	0.18	1.15	3.61	2.70	0.15	7.07	3.46	4.95	1147
0.15	1.20	1.57	1.43	1.10	2.04	0.47	1.83	0.10	0.16	0.14	0.07	0.24	0.08	0.20	1.29	4.01	3.11	0.44	7.57	3.57	5.58	902
0.18	1.69	1.96	1.88	1.59	2.33	0.37	2.19	0.11	0.16	0.15	0.08	0.25	0.08	0.20	1.29	4.14	3.15	0.50	7.77	3.63	5.93	1087
0.32	2.16	2.41	2.42	2.04	2.78	0.37	2.65	0.12	0.18	0.16	0.09	0.27	0.09	0.22	1.78	4.75	3.84	0.98	8.51	3.77	6.94	2432


==> data/mlm_plots/tef/agnews/xlnet/a/time_misc_auc.tex <==
name	auc
attack_time	0.48
l2	0.05
lom	1.14


==> data/mlm_plots/tef/agnews/xlnet/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.33	0.55	0.50	0.20	0.90	0.35	1.00	0.62	0.71	0.75	0.51	0.92	0.20	0.86	0.76	0.82	0.85	0.68	0.95	0.13	0.92	145
0.06	0.00	0.37	0.33	0.04	0.69	0.33	0.67	0.49	0.62	0.64	0.41	0.83	0.21	0.78	0.68	0.77	0.79	0.63	0.90	0.14	0.88	1080
0.11	0.00	0.31	0.33	0.01	0.61	0.30	0.50	0.43	0.56	0.58	0.36	0.77	0.21	0.71	0.67	0.73	0.75	0.59	0.87	0.14	0.83	1147
0.15	0.00	0.24	0.00	-0.04	0.51	0.28	0.50	0.36	0.52	0.50	0.30	0.73	0.22	0.67	0.60	0.70	0.71	0.54	0.85	0.15	0.81	902
0.18	0.00	0.20	0.00	-0.07	0.48	0.27	0.33	0.33	0.48	0.50	0.26	0.69	0.21	0.64	0.57	0.67	0.69	0.53	0.81	0.14	0.78	1087
0.32	0.00	0.13	0.00	-0.10	0.35	0.23	0.25	0.22	0.38	0.38	0.17	0.60	0.22	0.55	0.50	0.61	0.62	0.45	0.77	0.16	0.73	2432


==> data/mlm_plots/tef/agnews/xlnet/a/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.15
top50	0.20


==> data/mlm_plots/tef/agnews/xlnet/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	106.35	203.71	165.09	67.51	339.91	136.20	277.75	3.00	4.01	4.00	2.03	5.98	1.98	5.00	123.27	235.76	192.09	90.56	380.96	145.20	321.94	3.00	4.05	4.00	2.05	6.06	2.00	5.00	170
0.06	103.57	187.63	152.77	55.98	319.29	131.65	235.65	3.00	4.19	4.00	2.40	5.97	1.79	5.00	139.81	246.52	207.49	84.41	408.62	162.10	304.35	3.00	4.31	4.00	2.48	6.14	1.83	5.00	1151
0.11	103.53	196.99	163.97	59.74	334.23	137.24	249.71	3.00	4.21	4.00	2.48	5.94	1.73	5.00	169.04	302.29	255.71	105.67	498.90	196.62	380.01	3.00	4.39	4.00	2.60	6.19	1.80	5.00	1189
0.15	103.56	188.97	149.42	58.21	319.74	130.76	241.94	3.00	4.25	4.00	2.45	6.05	1.80	5.00	191.34	347.14	299.38	127.93	566.35	219.21	432.70	3.00	4.56	4.00	2.64	6.48	1.92	6.00	888
0.18	98.42	186.22	146.94	40.82	331.63	145.40	226.21	3.00	4.17	4.00	2.47	5.86	1.70	5.00	232.47	392.52	331.35	142.42	642.62	250.10	470.46	3.00	4.60	4.00	2.79	6.40	1.81	6.00	1043
0.32	109.02	194.52	160.57	63.14	325.89	131.38	247.71	3.00	4.33	4.00	2.51	6.14	1.82	6.00	332.99	570.68	481.87	213.34	928.01	357.34	701.25	4.00	4.93	5.00	2.97	6.88	1.95	6.00	2349


==> data/mlm_plots/tef/agnews/xlnet/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	55.47
orig_ge	1.22
adv_pp	112.15
adv_ge	1.33


==> data/mlm_plots/tef/agnews/xlnet/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.19	0.41	0.48	0.01	0.81	0.40	0.72	0.34	0.47	0.56	0.12	0.83	0.35	0.71	0.24	0.37	0.43	0.09	0.65	0.28	0.56	170
0.06	-0.07	0.17	0.17	-0.19	0.54	0.36	0.43	0.08	0.27	0.30	-0.04	0.58	0.31	0.49	0.05	0.21	0.22	-0.03	0.44	0.24	0.37	1151
0.11	-0.32	-0.05	-0.05	-0.43	0.33	0.38	0.20	-0.15	0.08	0.08	-0.23	0.40	0.32	0.31	-0.10	0.06	0.07	-0.17	0.30	0.23	0.23	1189
0.15	-0.43	-0.20	-0.24	-0.54	0.14	0.34	-0.01	-0.26	-0.06	-0.09	-0.35	0.23	0.29	0.11	-0.18	-0.04	-0.06	-0.25	0.18	0.22	0.09	888
0.18	-0.47	-0.28	-0.31	-0.57	0.01	0.29	-0.12	-0.32	-0.14	-0.16	-0.40	0.12	0.26	0.03	-0.23	-0.10	-0.11	-0.29	0.09	0.19	0.03	1043
0.32	-0.61	-0.44	-0.47	-0.69	-0.19	0.25	-0.32	-0.48	-0.31	-0.34	-0.55	-0.07	0.24	-0.18	-0.34	-0.22	-0.24	-0.40	-0.04	0.18	-0.12	2349


==> data/mlm_plots/tef/agnews/xlnet/ig/correlations_auc.tex <==
name	auc
pcc	-0.05
spearman	-0.01
kendall	-0.01


==> data/mlm_plots/tef/agnews/xlnet/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	2.12	4.99	3.89	1.18	8.80	3.81	6.52	2.09	5.30	4.08	0.90	9.71	4.40	7.57	4.03	14.36	8.78	-1.23	29.94	15.58	19.53	170
0.06	3.13	5.19	4.64	2.23	8.15	2.96	6.72	2.80	5.31	4.31	1.51	9.11	3.80	6.74	3.83	12.85	7.44	-0.41	26.12	13.27	17.18	1151
0.11	3.31	4.92	4.52	2.43	7.41	2.49	6.04	2.86	4.90	4.27	1.96	7.84	2.94	5.97	4.01	11.92	7.16	-0.55	24.39	12.47	14.40	1189
0.15	3.37	4.55	4.34	2.62	6.47	1.92	5.54	2.89	4.38	3.99	2.24	6.53	2.15	5.43	3.78	10.24	6.40	-1.10	21.57	11.33	11.12	888
0.18	3.30	4.24	4.00	2.65	5.83	1.59	4.89	2.92	4.07	3.71	2.30	5.84	1.77	4.82	3.69	8.87	5.94	-0.14	17.89	9.01	10.08	1043
0.32	3.03	3.72	3.57	2.61	4.83	1.11	4.22	2.82	3.61	3.33	2.36	4.85	1.24	4.14	3.60	7.26	5.17	0.27	14.25	6.99	8.07	2349


==> data/mlm_plots/tef/agnews/xlnet/ig/ets_sts_auc.tex <==
name	auc
et_use	1.28
et_tse	1.26
et_ce	2.89


==> data/mlm_plots/tef/agnews/xlnet/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.73	4.32	1.40	-6.86	15.49	11.17	3.40	3.87	17.39	9.02	-4.16	38.93	21.55	21.81	3.75	22.31	9.57	-13.00	57.63	35.32	26.81	170
0.06	0.67	4.27	1.23	-12.63	21.18	16.90	2.31	4.88	13.89	9.16	-0.29	28.07	14.18	17.51	4.36	19.96	9.63	-15.84	55.75	35.80	20.28	1151
0.11	0.53	3.09	0.96	-10.56	16.74	13.65	1.75	4.90	11.77	8.23	0.36	23.19	11.41	14.38	4.13	16.70	8.67	-13.35	46.75	30.05	17.13	1189
0.15	0.38	3.22	0.69	-18.00	24.45	21.22	1.31	4.94	10.27	7.12	-0.02	20.55	10.28	11.62	4.11	15.54	6.60	-22.44	53.52	37.98	13.56	888
0.18	0.33	1.18	0.53	-4.42	6.77	5.60	0.89	4.69	8.68	6.47	0.95	16.41	7.73	9.95	3.90	11.44	6.11	-12.47	35.35	23.91	11.07	1043
0.32	0.22	0.76	0.37	-2.34	3.85	3.10	0.63	4.58	7.78	5.93	1.06	14.50	6.72	8.51	3.74	10.93	5.22	-16.16	38.02	27.09	8.87	2349


==> data/mlm_plots/tef/agnews/xlnet/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.64
et_p_h	2.99
et_p_l2	4.17


==> data/mlm_plots/tef/agnews/xlnet/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.10	0.20	0.19	0.06	0.35	0.15	0.29	0.01	0.04	0.02	-0.00	0.09	0.05	0.06	0.01	0.04	0.03	0.00	0.07	0.03	0.05	170
0.06	0.18	0.38	0.33	0.10	0.66	0.28	0.52	0.02	0.06	0.04	0.01	0.11	0.05	0.08	0.02	0.05	0.04	0.02	0.09	0.04	0.07	1151
0.11	0.29	0.63	0.55	0.17	1.10	0.47	0.85	0.03	0.08	0.06	0.02	0.14	0.06	0.12	0.04	0.07	0.06	0.03	0.11	0.04	0.10	1189
0.15	0.48	1.02	0.89	0.28	1.75	0.73	1.35	0.04	0.10	0.09	0.04	0.16	0.06	0.15	0.05	0.09	0.08	0.04	0.13	0.04	0.12	888
0.18	0.71	1.37	1.19	0.46	2.29	0.92	1.85	0.06	0.11	0.11	0.05	0.18	0.07	0.16	0.07	0.10	0.10	0.06	0.15	0.04	0.13	1043
0.32	1.14	2.38	1.90	0.51	4.25	1.87	2.99	0.08	0.14	0.14	0.07	0.21	0.07	0.19	0.09	0.12	0.12	0.07	0.17	0.05	0.15	2349


==> data/mlm_plots/tef/agnews/xlnet/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.36
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/agnews/xlnet/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.94	0.94	0.92	0.96	0.02	0.95	0.90	0.93	0.94	0.89	0.97	0.04	0.96	0.95	0.95	0.98	0.90	1.01	0.05	0.99	170
0.06	0.90	0.91	0.91	0.88	0.94	0.03	0.93	0.88	0.90	0.91	0.86	0.95	0.04	0.94	0.90	0.93	0.95	0.87	0.99	0.06	0.98	1151
0.11	0.86	0.88	0.88	0.85	0.92	0.03	0.90	0.84	0.87	0.88	0.83	0.92	0.05	0.91	0.87	0.91	0.93	0.84	0.98	0.07	0.97	1189
0.15	0.84	0.86	0.86	0.82	0.90	0.04	0.88	0.82	0.85	0.85	0.80	0.90	0.05	0.89	0.85	0.89	0.91	0.82	0.97	0.07	0.95	888
0.18	0.81	0.84	0.84	0.80	0.88	0.04	0.86	0.79	0.83	0.83	0.78	0.88	0.05	0.86	0.83	0.88	0.89	0.79	0.96	0.08	0.94	1043
0.32	0.77	0.80	0.80	0.75	0.84	0.04	0.83	0.75	0.79	0.79	0.73	0.84	0.05	0.82	0.80	0.85	0.86	0.76	0.93	0.08	0.91	2349


==> data/mlm_plots/tef/agnews/xlnet/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.24
sts_ce	0.26


==> data/mlm_plots/tef/agnews/xlnet/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.62	0.98	0.72	0.26	1.71	0.72	0.86	0.39	3.43	0.93	-4.80	11.66	8.23	2.95	0.88	2.34	1.61	0.21	4.48	2.14	3.19	170
0.06	0.72	1.09	0.81	0.33	1.85	0.76	1.09	0.53	3.29	1.31	-2.02	8.60	5.31	3.74	1.07	2.96	2.24	0.41	5.51	2.55	4.16	1151
0.11	1.11	1.72	1.47	0.84	2.60	0.88	1.99	0.70	4.13	1.50	-2.79	11.05	6.92	4.41	1.17	3.34	2.63	0.51	6.16	2.83	4.89	1189
0.15	1.50	2.07	1.75	1.14	3.00	0.93	2.34	0.72	3.93	1.57	-2.03	9.90	5.96	4.69	1.31	3.66	2.86	0.56	6.77	3.11	5.30	888
0.18	2.27	3.48	2.96	1.97	4.99	1.51	4.71	0.70	3.86	1.51	-1.76	9.48	5.62	4.72	1.31	3.66	2.81	0.64	6.67	3.01	5.16	1043
0.32	2.66	2.98	3.00	2.52	3.44	0.46	3.28	0.70	3.96	1.57	-1.85	9.77	5.81	4.46	1.35	3.75	2.92	0.55	6.94	3.19	5.27	2349


==> data/mlm_plots/tef/agnews/xlnet/ig/time_misc_auc.tex <==
name	auc
attack_time	0.71
l2	1.11
lom	1.01


==> data/mlm_plots/tef/agnews/xlnet/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.34	0.37	0.03	0.64	0.30	0.50	0.43	0.55	0.58	0.34	0.77	0.21	0.71	0.62	0.70	0.73	0.53	0.86	0.16	0.79	170
0.06	0.00	0.22	0.00	-0.03	0.48	0.25	0.33	0.31	0.45	0.44	0.26	0.63	0.19	0.58	0.53	0.61	0.62	0.47	0.74	0.13	0.71	1151
0.11	0.00	0.15	0.00	-0.07	0.37	0.22	0.33	0.22	0.36	0.33	0.18	0.53	0.18	0.45	0.47	0.55	0.55	0.42	0.68	0.13	0.62	1189
0.15	0.00	0.09	0.00	-0.10	0.27	0.18	0.00	0.18	0.30	0.29	0.13	0.46	0.16	0.40	0.41	0.50	0.50	0.37	0.62	0.12	0.57	888
0.18	0.00	0.06	0.00	-0.10	0.22	0.16	0.00	0.14	0.26	0.25	0.11	0.40	0.15	0.33	0.39	0.47	0.47	0.35	0.59	0.12	0.55	1043
0.32	0.00	0.03	0.00	-0.07	0.12	0.10	0.00	0.10	0.18	0.17	0.05	0.32	0.14	0.27	0.33	0.41	0.40	0.30	0.52	0.11	0.47	2349


==> data/mlm_plots/tef/agnews/xlnet/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.09
top50	0.15


==> data/mlm_plots/tef/agnews/xlnet/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	110.48	191.49	170.59	84.87	298.11	106.62	243.86	3.00	4.24	4.00	2.29	6.20	1.96	6.00	131.34	226.90	202.64	104.06	349.73	122.83	300.90	3.00	4.36	4.00	2.39	6.32	1.96	6.00	156
0.06	105.67	196.97	160.35	45.61	348.33	151.36	238.11	3.00	4.28	4.00	2.55	6.00	1.73	5.00	147.09	261.50	216.64	83.94	439.06	177.56	318.55	3.00	4.43	4.00	2.65	6.21	1.78	6.00	1147
0.11	101.24	193.60	153.48	57.11	330.08	136.49	247.87	3.00	4.15	4.00	2.47	5.84	1.69	5.00	170.62	307.78	264.23	113.26	502.31	194.52	387.00	3.00	4.37	4.00	2.62	6.12	1.75	5.00	1236
0.15	107.96	185.07	150.62	67.85	302.30	117.23	240.06	3.00	4.29	4.00	2.40	6.17	1.89	5.00	219.96	352.25	300.43	147.39	557.12	204.86	441.24	3.00	4.61	4.00	2.57	6.65	2.04	6.00	911
0.18	103.62	191.81	155.56	62.78	320.84	129.03	247.78	3.00	4.24	4.00	2.42	6.06	1.82	5.00	254.78	438.16	368.22	173.60	702.73	264.56	550.97	3.00	4.64	4.00	2.71	6.57	1.93	6.00	1040
0.32	105.79	196.81	161.95	63.01	330.60	133.80	251.60	3.00	4.30	4.00	2.50	6.09	1.80	5.00	346.92	613.29	513.84	217.78	1008.81	395.51	766.09	3.00	4.91	5.00	2.93	6.89	1.98	6.00	2268


==> data/mlm_plots/tef/agnews/xlnet/s/comparison_vals_auc.tex <==
name	auc
orig_pp	55.96
orig_ge	1.23
adv_pp	119.79
adv_ge	1.34


==> data/mlm_plots/tef/agnews/xlnet/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.50	0.66	0.75	0.40	0.91	0.26	0.84	0.76	0.81	0.87	0.63	0.98	0.17	0.92	0.61	0.67	0.72	0.50	0.84	0.17	0.79	156
0.06	0.39	0.55	0.59	0.31	0.79	0.24	0.72	0.63	0.73	0.78	0.54	0.92	0.19	0.87	0.48	0.58	0.62	0.41	0.76	0.18	0.71	1147
0.11	0.25	0.42	0.44	0.17	0.67	0.25	0.62	0.52	0.63	0.68	0.41	0.86	0.22	0.80	0.38	0.49	0.52	0.30	0.68	0.19	0.63	1236
0.15	0.19	0.35	0.34	0.11	0.60	0.25	0.54	0.43	0.57	0.62	0.34	0.80	0.23	0.75	0.31	0.43	0.46	0.24	0.62	0.19	0.57	911
0.18	0.13	0.29	0.28	0.06	0.52	0.23	0.44	0.38	0.52	0.55	0.29	0.74	0.23	0.69	0.27	0.39	0.41	0.21	0.56	0.18	0.51	1040
0.32	0.02	0.18	0.16	-0.05	0.41	0.23	0.33	0.25	0.41	0.44	0.16	0.65	0.25	0.60	0.17	0.30	0.31	0.11	0.48	0.19	0.43	2268


==> data/mlm_plots/tef/agnews/xlnet/s/correlations_auc.tex <==
name	auc
pcc	0.10
spearman	0.16
kendall	0.12


==> data/mlm_plots/tef/agnews/xlnet/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	1.14	3.01	1.89	0.08	5.94	2.93	3.52	1.07	3.65	1.77	-1.06	8.35	4.71	3.82	1.59	7.08	4.36	-1.60	15.75	8.67	8.57	156
0.06	1.47	2.79	2.34	0.90	4.67	1.88	3.58	1.31	2.83	2.15	0.44	5.22	2.39	3.54	1.75	7.05	3.79	-1.26	15.35	8.31	9.17	1147
0.11	1.58	2.71	2.47	1.23	4.20	1.49	3.53	1.44	2.75	2.29	0.84	4.65	1.91	3.55	2.03	6.83	3.72	-1.27	14.93	8.10	8.05	1236
0.15	1.55	2.48	2.24	1.13	3.84	1.36	3.11	1.44	2.42	2.04	0.83	4.01	1.59	3.02	1.94	5.70	3.38	-0.94	12.34	6.64	6.54	911
0.18	1.62	2.24	2.12	1.30	3.19	0.95	2.77	1.44	2.19	1.99	1.09	3.28	1.09	2.64	2.00	5.00	3.15	-0.51	10.51	5.51	5.55	1040
0.32	1.56	2.05	1.95	1.29	2.81	0.76	2.47	1.45	1.98	1.84	1.14	2.82	0.84	2.37	1.79	3.93	2.71	-0.19	8.04	4.12	4.41	2268


==> data/mlm_plots/tef/agnews/xlnet/s/ets_sts_auc.tex <==
name	auc
et_use	0.70
et_tse	0.70
et_ce	1.60


==> data/mlm_plots/tef/agnews/xlnet/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	0.37	3.14	0.74	-11.58	17.86	14.72	1.91	1.95	12.06	5.53	-7.26	31.37	19.31	11.16	2.51	16.62	5.41	-12.81	46.04	29.43	15.82	156
0.06	0.31	1.90	0.60	-4.98	8.78	6.88	1.38	2.32	7.72	4.42	-1.63	17.08	9.35	9.44	2.14	11.25	4.78	-8.44	30.94	19.69	11.56	1147
0.11	0.26	1.76	0.46	-7.71	11.24	9.47	0.83	2.44	6.27	3.80	-1.29	13.83	7.56	7.07	2.03	8.51	3.77	-7.45	24.47	15.96	8.74	1236
0.15	0.18	1.15	0.36	-7.74	10.04	8.89	0.65	2.32	5.50	3.69	-1.20	12.19	6.70	6.01	1.97	6.80	3.48	-5.40	19.00	12.20	6.96	911
0.18	0.16	0.68	0.27	-2.79	4.15	3.47	0.46	2.43	4.78	3.49	0.62	8.93	4.16	5.39	2.02	6.09	3.20	-2.89	15.07	8.98	6.46	1040
0.32	0.11	0.52	0.19	-3.22	4.26	3.74	0.34	2.40	4.05	3.27	0.80	7.29	3.25	4.55	2.00	5.51	2.87	-9.24	20.26	14.75	4.78	2268


==> data/mlm_plots/tef/agnews/xlnet/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.34
et_p_h	1.65
et_p_l2	2.22


==> data/mlm_plots/tef/agnews/xlnet/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.10	0.22	0.16	0.03	0.41	0.19	0.31	0.01	0.04	0.02	-0.01	0.09	0.05	0.05	0.01	0.04	0.03	0.00	0.07	0.03	0.05	156
0.06	0.16	0.42	0.33	0.08	0.77	0.35	0.61	0.02	0.06	0.04	0.00	0.11	0.05	0.09	0.02	0.05	0.04	0.02	0.09	0.04	0.08	1147
0.11	0.35	0.73	0.62	0.17	1.28	0.56	0.96	0.03	0.09	0.07	0.02	0.15	0.06	0.14	0.04	0.08	0.07	0.03	0.12	0.05	0.11	1236
0.15	0.53	1.10	0.87	0.26	1.94	0.84	1.50	0.05	0.10	0.09	0.03	0.17	0.07	0.16	0.05	0.09	0.09	0.04	0.14	0.05	0.13	911
0.18	0.76	1.58	1.27	0.42	2.74	1.16	2.07	0.06	0.11	0.11	0.04	0.18	0.07	0.17	0.06	0.10	0.10	0.05	0.15	0.05	0.14	1040
0.32	1.19	2.68	2.07	0.41	4.94	2.26	3.47	0.08	0.14	0.15	0.07	0.22	0.07	0.20	0.09	0.13	0.13	0.08	0.18	0.05	0.16	2268


==> data/mlm_plots/tef/agnews/xlnet/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/agnews/xlnet/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.92	0.93	0.93	0.90	0.96	0.03	0.95	0.90	0.93	0.93	0.88	0.97	0.04	0.96	0.93	0.95	0.97	0.89	1.00	0.05	0.98	156
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.87	0.90	0.91	0.86	0.94	0.04	0.93	0.90	0.93	0.95	0.86	0.99	0.06	0.98	1147
0.11	0.86	0.88	0.88	0.85	0.92	0.03	0.91	0.84	0.87	0.88	0.82	0.92	0.05	0.91	0.88	0.91	0.93	0.84	0.98	0.07	0.97	1236
0.15	0.84	0.86	0.86	0.82	0.89	0.04	0.88	0.81	0.85	0.85	0.80	0.90	0.05	0.88	0.85	0.89	0.91	0.82	0.96	0.07	0.95	911
0.18	0.81	0.83	0.83	0.79	0.87	0.04	0.86	0.79	0.82	0.82	0.77	0.87	0.05	0.86	0.84	0.88	0.89	0.80	0.96	0.08	0.94	1040
0.32	0.76	0.79	0.79	0.75	0.84	0.05	0.82	0.74	0.78	0.78	0.72	0.84	0.06	0.82	0.79	0.84	0.85	0.75	0.93	0.09	0.91	2268


==> data/mlm_plots/tef/agnews/xlnet/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.24
sts_ce	0.26


==> data/mlm_plots/tef/agnews/xlnet/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.59	0.82	0.72	0.34	1.29	0.47	0.87	29.41	236.64	71.91	-217.60	690.88	454.24	244.66	0.30	1.10	0.59	-0.30	2.51	1.41	1.33	156
0.06	0.79	1.06	0.90	0.51	1.60	0.54	1.07	39.24	354.08	120.32	-265.84	974.01	619.92	407.56	0.44	1.28	0.91	0.09	2.47	1.19	1.74	1147
0.11	1.09	1.64	1.39	0.86	2.41	0.78	1.91	48.86	497.05	172.81	-409.43	1403.53	906.48	553.33	0.57	1.58	1.25	0.27	2.88	1.31	2.25	1236
0.15	1.33	1.92	1.60	1.07	2.77	0.85	2.46	61.74	417.70	174.15	-189.03	1024.43	606.73	466.93	0.63	1.79	1.34	0.20	3.38	1.59	2.52	911
0.18	1.80	2.25	2.08	1.62	2.88	0.63	2.55	63.10	565.23	204.09	-357.45	1487.91	922.68	684.32	0.65	1.86	1.38	0.19	3.53	1.67	2.56	1040
0.32	2.78	3.14	2.99	2.53	3.76	0.61	3.42	74.49	697.57	246.05	-564.17	1959.30	1261.73	823.10	0.74	1.99	1.59	0.42	3.56	1.57	2.86	2268


==> data/mlm_plots/tef/agnews/xlnet/s/time_misc_auc.tex <==
name	auc
attack_time	0.61
l2	151.03
lom	0.50


==> data/mlm_plots/tef/agnews/xlnet/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.44	0.50	0.11	0.77	0.33	0.53	0.66	0.74	0.75	0.59	0.89	0.15	0.86	0.79	0.83	0.85	0.73	0.94	0.11	0.92	156
0.06	0.00	0.35	0.33	0.07	0.63	0.28	0.50	0.56	0.66	0.67	0.50	0.83	0.16	0.78	0.73	0.80	0.81	0.69	0.90	0.11	0.88	1147
0.11	0.00	0.27	0.33	0.01	0.53	0.26	0.43	0.50	0.59	0.60	0.42	0.76	0.17	0.70	0.67	0.75	0.76	0.63	0.87	0.12	0.83	1236
0.15	0.00	0.20	0.00	-0.05	0.45	0.25	0.33	0.42	0.55	0.56	0.37	0.72	0.18	0.67	0.65	0.72	0.73	0.61	0.84	0.12	0.82	911
0.18	0.00	0.16	0.00	-0.06	0.37	0.22	0.33	0.40	0.51	0.50	0.34	0.67	0.17	0.62	0.62	0.70	0.71	0.59	0.82	0.11	0.78	1040
0.32	0.00	0.10	0.00	-0.08	0.29	0.19	0.25	0.33	0.44	0.44	0.26	0.61	0.18	0.56	0.59	0.66	0.67	0.55	0.78	0.11	0.75	2268


==> data/mlm_plots/tef/agnews/xlnet/s/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.16
top50	0.21


==> data/mlm_plots/tef/fakenews/bert/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	35.05	49.01	43.15	26.42	71.61	22.60	56.36	70.75	83.00	85.00	58.15	107.85	24.85	98.00	40.50	55.28	49.61	31.31	79.24	23.97	63.62	71.00	83.42	85.00	58.55	108.28	24.86	99.00	944
0.03	35.07	51.36	43.84	22.66	80.06	28.70	57.70	69.00	81.37	84.00	53.61	109.13	27.76	98.00	47.22	66.19	58.03	34.29	98.08	31.90	74.47	69.00	82.28	85.00	54.54	110.02	27.74	99.00	1000
0.06	35.25	55.15	43.90	13.62	96.68	41.53	59.11	67.00	79.54	83.00	49.86	109.21	29.68	98.00	59.94	86.73	73.29	30.77	142.70	55.96	92.69	69.00	81.20	85.00	51.41	110.99	29.79	100.00	1031
0.11	35.21	56.42	44.45	6.13	106.72	50.30	59.15	65.00	79.19	83.00	49.12	109.26	30.07	98.00	73.38	107.05	89.81	28.56	185.54	78.49	112.36	68.00	81.69	86.00	51.27	112.10	30.42	101.00	1032
0.15	35.08	55.61	43.68	10.79	100.43	44.82	57.66	68.00	79.70	83.00	50.35	109.05	29.35	98.00	101.25	139.61	121.39	60.98	218.24	78.63	148.59	72.00	83.54	88.00	53.71	113.37	29.83	102.00	789
0.18	35.76	64.23	44.76	-87.54	215.99	151.76	60.10	65.25	78.08	83.00	47.99	108.16	30.09	98.00	138.61	193.74	166.17	45.35	342.13	148.39	198.89	71.00	83.25	89.00	52.04	114.47	31.22	103.00	618
0.32	35.54	62.32	44.82	-64.24	188.88	126.56	60.18	65.00	78.29	83.00	47.92	108.66	30.37	98.00	193.75	281.82	243.81	109.57	454.08	172.26	319.77	73.00	85.66	93.00	53.49	117.84	32.18	107.00	934


==> data/mlm_plots/tef/fakenews/bert/a/comparison_vals_auc.tex <==
name	auc
orig_pp	18.30
orig_ge	24.56
adv_pp	51.38
adv_ge	25.85


==> data/mlm_plots/tef/fakenews/bert/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.18	0.50	0.74	0.08	0.92	0.42	0.82	0.42	0.57	0.59	0.33	0.81	0.24	0.76	0.30	0.43	0.43	0.23	0.63	0.20	0.59	944
0.03	0.07	0.43	0.68	-0.02	0.88	0.45	0.77	0.38	0.53	0.56	0.29	0.78	0.25	0.73	0.27	0.41	0.41	0.20	0.61	0.20	0.56	1000
0.06	0.04	0.38	0.62	-0.07	0.82	0.44	0.72	0.37	0.51	0.54	0.26	0.77	0.25	0.72	0.26	0.39	0.39	0.19	0.59	0.20	0.54	1031
0.11	-0.01	0.33	0.57	-0.11	0.78	0.44	0.68	0.35	0.49	0.53	0.25	0.74	0.25	0.69	0.25	0.37	0.38	0.17	0.57	0.20	0.52	1032
0.15	-0.02	0.30	0.52	-0.13	0.73	0.43	0.64	0.34	0.48	0.52	0.25	0.72	0.24	0.66	0.25	0.36	0.37	0.17	0.55	0.19	0.50	789
0.18	-0.05	0.28	0.51	-0.14	0.70	0.42	0.61	0.35	0.47	0.51	0.24	0.71	0.24	0.65	0.25	0.35	0.37	0.17	0.53	0.18	0.49	618
0.32	-0.03	0.27	0.46	-0.14	0.68	0.41	0.58	0.33	0.45	0.48	0.22	0.68	0.23	0.62	0.23	0.33	0.34	0.16	0.51	0.18	0.46	934


==> data/mlm_plots/tef/fakenews/bert/a/correlations_auc.tex <==
name	auc
pcc	0.10
spearman	0.15
kendall	0.11


==> data/mlm_plots/tef/fakenews/bert/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.25	11.17	5.66	-0.74	23.08	11.91	16.34	2.75	9.86	4.77	-1.07	20.79	10.93	14.26	2.27	7.72	4.31	-1.26	16.71	8.98	9.44	944
0.03	2.31	7.07	3.86	-0.07	14.22	7.14	10.17	2.00	6.43	3.41	-0.56	13.42	6.99	8.85	2.02	6.33	3.92	-0.73	13.39	7.06	8.11	1000
0.06	1.79	4.54	3.00	0.72	8.37	3.82	6.32	1.62	4.27	2.65	0.53	8.01	3.74	6.12	1.77	4.89	3.34	0.10	9.69	4.80	6.51	1031
0.11	1.56	3.47	2.37	0.88	6.07	2.59	4.94	1.44	3.35	2.23	0.79	5.91	2.56	4.90	1.61	4.04	2.89	0.34	7.74	3.70	5.35	1032
0.15	1.26	2.53	1.75	0.86	4.20	1.67	3.64	1.20	2.48	1.73	0.81	4.15	1.67	3.57	1.33	3.02	2.24	0.60	5.45	2.43	4.05	789
0.18	1.07	2.06	1.45	0.77	3.36	1.30	2.97	1.02	2.05	1.41	0.73	3.36	1.32	2.96	1.15	2.37	1.70	0.69	4.05	1.68	3.24	618
0.32	0.91	1.69	1.19	0.63	2.76	1.07	2.36	0.90	1.70	1.18	0.61	2.78	1.08	2.41	0.95	1.90	1.34	0.50	3.29	1.39	2.54	934


==> data/mlm_plots/tef/fakenews/bert/a/ets_sts_auc.tex <==
name	auc
et_use	1.01
et_tse	0.96
et_ce	1.05


==> data/mlm_plots/tef/fakenews/bert/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.65	2.69	1.19	-3.06	8.43	5.75	3.35	2.01	7.14	3.83	0.03	14.25	7.11	10.85	1.59	6.44	3.49	-0.57	13.44	7.01	9.26	944
0.03	0.36	1.10	0.59	-0.48	2.68	1.58	1.61	1.69	4.93	2.84	0.43	9.43	4.50	7.72	1.33	4.22	2.42	0.02	8.41	4.19	6.41	1000
0.06	0.22	0.63	0.35	-1.23	2.48	1.85	0.80	1.56	3.81	2.50	0.65	6.97	3.16	5.69	1.25	3.31	2.04	-0.41	7.03	3.72	4.73	1031
0.11	0.16	0.42	0.25	-1.03	1.86	1.45	0.53	1.49	3.32	2.26	0.87	5.77	2.45	4.85	1.18	2.85	1.86	-1.19	6.90	4.05	4.16	1032
0.15	0.11	0.23	0.16	0.01	0.45	0.22	0.31	1.39	2.84	2.04	0.85	4.84	1.99	4.05	1.10	2.42	1.67	-0.22	5.07	2.64	3.41	789
0.18	0.07	0.16	0.11	-0.03	0.34	0.18	0.21	1.30	2.54	1.80	0.85	4.23	1.69	3.76	1.02	2.20	1.48	-1.00	5.40	3.20	3.10	618
0.32	0.05	0.12	0.07	-0.23	0.46	0.34	0.14	1.22	2.26	1.66	0.93	3.59	1.33	3.27	0.97	1.90	1.34	0.55	3.25	1.35	2.72	934


==> data/mlm_plots/tef/fakenews/bert/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.13
et_p_h	0.97
et_p_l2	0.84


==> data/mlm_plots/tef/fakenews/bert/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.10	0.14	0.14	0.08	0.20	0.06	0.18	0.03	0.05	0.05	0.03	0.08	0.03	0.07	0.03	0.04	0.04	0.03	0.06	0.02	0.05	944
0.03	0.25	0.32	0.32	0.21	0.43	0.11	0.38	0.06	0.08	0.08	0.05	0.12	0.03	0.10	0.05	0.07	0.06	0.05	0.09	0.02	0.08	1000
0.06	0.52	0.64	0.64	0.43	0.85	0.21	0.75	0.09	0.11	0.11	0.07	0.15	0.04	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.10	1031
0.11	0.82	1.01	1.00	0.64	1.39	0.38	1.17	0.11	0.14	0.13	0.09	0.18	0.04	0.16	0.09	0.11	0.11	0.08	0.13	0.03	0.12	1032
0.15	1.43	1.73	1.74	1.18	2.29	0.56	2.04	0.14	0.16	0.16	0.12	0.21	0.04	0.19	0.12	0.13	0.13	0.10	0.16	0.03	0.15	789
0.18	2.13	2.64	2.62	1.75	3.54	0.90	3.15	0.16	0.19	0.19	0.14	0.24	0.05	0.21	0.13	0.15	0.15	0.12	0.18	0.03	0.16	618
0.32	3.23	4.46	4.08	2.56	6.36	1.90	5.43	0.19	0.21	0.21	0.16	0.27	0.05	0.24	0.15	0.17	0.17	0.14	0.20	0.03	0.19	934


==> data/mlm_plots/tef/fakenews/bert/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.67
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/bert/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.94	0.96	0.96	0.93	0.98	0.02	0.97	944
0.03	0.94	0.95	0.95	0.94	0.97	0.02	0.96	0.93	0.95	0.95	0.92	0.97	0.02	0.96	0.92	0.94	0.95	0.91	0.97	0.03	0.96	1000
0.06	0.91	0.92	0.92	0.90	0.95	0.02	0.94	0.90	0.92	0.92	0.89	0.94	0.03	0.93	0.90	0.92	0.92	0.88	0.96	0.04	0.95	1031
0.11	0.88	0.90	0.90	0.87	0.92	0.03	0.91	0.88	0.89	0.90	0.86	0.92	0.03	0.91	0.88	0.90	0.90	0.85	0.94	0.05	0.93	1032
0.15	0.84	0.86	0.86	0.83	0.88	0.03	0.87	0.83	0.85	0.85	0.82	0.88	0.03	0.87	0.84	0.87	0.87	0.81	0.92	0.05	0.90	789
0.18	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.80	0.82	0.82	0.78	0.85	0.03	0.84	0.80	0.83	0.84	0.77	0.89	0.06	0.87	618
0.32	0.75	0.77	0.77	0.74	0.81	0.04	0.80	0.74	0.77	0.77	0.73	0.81	0.04	0.80	0.74	0.78	0.79	0.71	0.85	0.07	0.83	934


==> data/mlm_plots/tef/fakenews/bert/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/fakenews/bert/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	29.76	31.37	34.36	21.73	41.01	9.64	37.01	0.04	0.12	0.07	-0.01	0.25	0.13	0.13	3.67	47.67	10.26	-19.93	115.27	67.60	65.05	944
0.03	37.43	57.26	43.94	21.06	93.45	36.19	93.20	0.05	0.14	0.08	-0.02	0.29	0.16	0.16	4.03	48.97	11.46	-18.54	116.48	67.51	75.86	1000
0.06	47.16	61.20	60.89	30.12	92.29	31.08	76.87	0.05	0.15	0.08	-0.02	0.32	0.17	0.19	4.63	51.20	12.88	-17.09	119.50	68.30	82.47	1031
0.11	55.74	72.40	75.73	36.10	108.70	36.30	88.49	0.06	0.16	0.09	-0.02	0.33	0.18	0.20	5.49	50.86	14.41	-15.80	117.52	66.66	73.28	1032
0.15	81.33	95.69	104.32	54.56	136.82	41.13	119.00	0.06	0.16	0.09	-0.02	0.34	0.18	0.19	5.84	52.80	16.08	-16.11	121.72	68.91	79.26	789
0.18	95.84	120.29	129.60	66.44	174.15	53.86	152.65	0.06	0.16	0.09	-0.03	0.35	0.19	0.15	5.92	50.28	16.87	-16.59	117.14	66.87	59.17	618
0.32	127.04	152.28	166.63	87.12	217.44	65.16	198.41	0.06	0.15	0.09	-0.04	0.34	0.19	0.13	6.65	45.52	17.22	-15.83	106.86	61.35	46.87	934


==> data/mlm_plots/tef/fakenews/bert/a/time_misc_auc.tex <==
name	auc
attack_time	31.65
l2	0.05
lom	15.39


==> data/mlm_plots/tef/fakenews/bert/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.60	0.69	0.74	0.52	0.86	0.17	0.81	0.56	0.65	0.67	0.51	0.79	0.14	0.76	0.63	0.71	0.70	0.60	0.81	0.11	0.79	944
0.03	0.56	0.65	0.70	0.47	0.82	0.18	0.77	0.55	0.64	0.65	0.49	0.78	0.14	0.75	0.62	0.69	0.69	0.59	0.80	0.11	0.77	1000
0.06	0.52	0.62	0.66	0.44	0.80	0.18	0.75	0.53	0.63	0.64	0.48	0.77	0.14	0.73	0.61	0.69	0.68	0.58	0.80	0.11	0.77	1031
0.11	0.51	0.60	0.64	0.42	0.78	0.18	0.73	0.52	0.61	0.63	0.47	0.76	0.14	0.72	0.61	0.68	0.68	0.57	0.78	0.11	0.75	1032
0.15	0.50	0.58	0.62	0.40	0.76	0.18	0.71	0.52	0.61	0.62	0.47	0.74	0.14	0.71	0.61	0.67	0.67	0.57	0.78	0.10	0.75	789
0.18	0.48	0.56	0.59	0.38	0.74	0.18	0.68	0.51	0.60	0.62	0.47	0.73	0.13	0.69	0.61	0.67	0.67	0.57	0.77	0.10	0.74	618
0.32	0.45	0.55	0.57	0.37	0.72	0.18	0.67	0.51	0.59	0.60	0.46	0.71	0.13	0.68	0.60	0.66	0.66	0.56	0.76	0.10	0.73	934


==> data/mlm_plots/tef/fakenews/bert/a/top_intersections_auc.tex <==
name	auc
top10	0.18
top30	0.19
top50	0.21


==> data/mlm_plots/tef/fakenews/bert/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	34.97	48.61	42.76	26.11	71.11	22.50	55.85	71.00	83.10	85.00	58.69	107.50	24.40	98.00	40.37	54.75	49.24	31.11	78.40	23.65	63.10	71.75	83.44	85.00	59.04	107.85	24.41	99.00	716
0.03	35.01	50.64	43.68	22.77	78.51	27.87	56.75	70.00	81.22	84.00	54.73	107.72	26.50	98.00	46.94	64.62	57.31	33.62	95.62	31.00	72.86	71.00	81.86	85.00	55.31	108.40	26.55	99.00	616
0.06	36.43	55.27	44.41	12.07	98.47	43.20	58.55	69.00	81.01	86.00	52.57	109.46	28.45	100.00	59.18	84.20	71.42	30.34	138.06	53.86	90.44	71.00	82.41	87.00	53.73	111.08	28.68	101.00	471
0.11	35.26	53.92	43.27	9.76	98.09	44.16	56.68	65.25	79.46	84.00	50.43	108.48	29.03	99.00	72.77	99.36	87.83	46.51	152.21	52.85	106.76	68.00	81.71	87.00	52.18	111.24	29.53	101.00	394
0.15	35.53	56.77	43.34	1.92	111.63	54.86	55.67	65.00	79.56	83.00	49.04	110.07	30.51	99.50	99.18	136.21	120.48	56.60	215.82	79.61	144.84	70.00	82.81	87.00	51.42	114.20	31.39	103.50	315
0.18	37.22	55.01	44.51	7.99	102.04	47.02	60.10	63.25	77.37	81.50	48.11	106.62	29.25	95.00	139.84	182.40	167.06	87.37	277.43	95.03	198.72	68.25	82.36	88.50	51.52	113.20	30.84	102.00	238
0.32	39.40	59.28	46.24	4.41	114.15	54.87	60.24	67.00	78.33	83.00	48.17	108.50	30.16	96.00	196.87	262.88	240.90	139.09	386.66	123.78	299.22	71.75	85.53	90.00	53.07	118.00	32.46	106.25	324


==> data/mlm_plots/tef/fakenews/bert/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	17.22
orig_ge	24.56
adv_pp	48.52
adv_ge	25.78


==> data/mlm_plots/tef/fakenews/bert/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.75	-0.41	-0.50	-0.84	0.02	0.43	-0.14	-0.34	-0.11	-0.13	-0.44	0.22	0.33	0.11	-0.25	-0.08	-0.09	-0.34	0.18	0.26	0.08	716
0.03	-0.82	-0.50	-0.60	-0.91	-0.09	0.41	-0.28	-0.37	-0.13	-0.16	-0.47	0.21	0.34	0.09	-0.28	-0.10	-0.11	-0.36	0.17	0.27	0.07	616
0.06	-0.86	-0.56	-0.68	-0.96	-0.16	0.40	-0.39	-0.37	-0.15	-0.18	-0.48	0.18	0.33	0.07	-0.27	-0.12	-0.13	-0.38	0.15	0.26	0.06	471
0.11	-0.89	-0.60	-0.72	-0.97	-0.22	0.37	-0.46	-0.41	-0.17	-0.18	-0.50	0.15	0.32	0.04	-0.32	-0.13	-0.13	-0.39	0.12	0.26	0.03	394
0.15	-0.90	-0.65	-0.76	-0.99	-0.30	0.35	-0.52	-0.43	-0.21	-0.23	-0.54	0.11	0.32	-0.01	-0.32	-0.17	-0.17	-0.42	0.09	0.26	-0.00	315
0.18	-0.90	-0.65	-0.75	-0.96	-0.34	0.31	-0.51	-0.42	-0.19	-0.21	-0.49	0.11	0.30	0.02	-0.31	-0.15	-0.15	-0.38	0.09	0.24	0.01	238
0.32	-0.91	-0.67	-0.75	-0.98	-0.35	0.31	-0.55	-0.43	-0.21	-0.22	-0.51	0.08	0.29	0.02	-0.32	-0.16	-0.16	-0.39	0.07	0.23	0.02	324


==> data/mlm_plots/tef/fakenews/bert/ig/correlations_auc.tex <==
name	auc
pcc	-0.19
spearman	-0.06
kendall	-0.04


==> data/mlm_plots/tef/fakenews/bert/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	18.68	28.60	26.78	14.65	42.55	13.95	35.87	15.61	25.54	22.75	11.77	39.32	13.77	32.55	11.06	21.69	17.52	7.19	36.18	14.49	28.48	716
0.03	12.83	18.04	16.73	9.55	26.53	8.49	21.81	11.26	16.63	14.93	8.23	25.04	8.40	20.74	9.16	16.98	14.00	5.73	28.24	11.25	21.29	616
0.06	8.44	11.32	11.02	6.83	15.81	4.49	13.78	7.87	10.74	10.45	6.36	15.13	4.38	13.12	7.55	12.17	10.65	5.28	19.06	6.89	14.80	471
0.11	6.53	8.23	8.13	5.47	10.99	2.76	9.90	6.22	7.96	7.78	5.20	10.73	2.77	9.64	6.33	9.59	8.68	4.72	14.46	4.87	12.16	394
0.15	5.02	5.97	6.07	4.21	7.73	1.76	6.96	4.96	5.96	6.02	4.13	7.79	1.83	7.09	5.10	7.19	6.67	3.89	10.50	3.31	8.64	315
0.18	4.05	4.69	4.77	3.50	5.88	1.19	5.49	4.05	4.67	4.76	3.31	6.03	1.36	5.47	4.10	5.61	5.13	3.19	8.03	2.42	6.83	238
0.32	3.30	3.84	3.90	2.83	4.85	1.01	4.35	3.32	3.90	3.97	2.72	5.07	1.18	4.39	3.30	4.42	4.16	2.51	6.34	1.92	5.16	324


==> data/mlm_plots/tef/fakenews/bert/ig/ets_sts_auc.tex <==
name	auc
et_use	2.44
et_tse	2.34
et_ce	2.60


==> data/mlm_plots/tef/fakenews/bert/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	3.68	8.29	5.27	-10.28	26.86	18.57	7.75	12.22	19.97	17.59	7.50	32.45	12.47	24.30	9.57	18.31	14.15	3.28	33.34	15.03	22.22	716
0.03	1.90	3.70	2.59	-15.69	23.09	19.39	3.35	8.90	13.10	12.31	4.47	21.72	8.63	15.65	6.79	11.40	9.59	0.12	22.69	11.28	13.04	616
0.06	1.07	1.55	1.36	0.05	3.04	1.49	1.78	7.50	9.66	9.31	5.57	13.75	4.09	11.74	5.71	8.33	7.35	0.40	16.27	7.94	9.58	471
0.11	0.68	1.02	0.85	-0.59	2.62	1.60	1.05	6.46	7.84	7.69	5.28	10.40	2.56	9.11	5.01	6.41	6.04	3.74	9.07	2.66	7.48	394
0.15	0.40	0.57	0.50	0.21	0.93	0.36	0.63	5.60	6.61	6.65	4.63	8.58	1.98	7.57	4.29	5.42	5.27	3.32	7.53	2.10	6.13	315
0.18	0.26	0.35	0.32	0.19	0.51	0.16	0.41	4.97	5.82	5.67	4.04	7.59	1.78	6.50	3.87	4.74	4.61	2.91	6.58	1.83	5.30	238
0.32	0.16	0.26	0.21	-0.04	0.56	0.30	0.27	4.50	5.28	5.19	3.49	7.07	1.79	5.94	3.51	4.38	4.19	2.28	6.48	2.10	4.81	324


==> data/mlm_plots/tef/fakenews/bert/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.35
et_p_h	2.37
et_p_l2	1.99


==> data/mlm_plots/tef/fakenews/bert/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.10	0.14	0.13	0.08	0.20	0.06	0.17	0.03	0.05	0.05	0.03	0.08	0.03	0.07	0.03	0.04	0.04	0.03	0.06	0.02	0.05	716
0.03	0.24	0.30	0.30	0.20	0.41	0.11	0.36	0.06	0.08	0.08	0.05	0.12	0.03	0.10	0.05	0.07	0.06	0.04	0.09	0.02	0.08	616
0.06	0.47	0.59	0.58	0.40	0.79	0.19	0.71	0.09	0.11	0.11	0.07	0.15	0.04	0.13	0.07	0.09	0.09	0.06	0.11	0.02	0.10	471
0.11	0.80	0.98	0.98	0.67	1.28	0.31	1.17	0.11	0.14	0.14	0.10	0.18	0.04	0.16	0.09	0.11	0.11	0.08	0.13	0.03	0.12	394
0.15	1.41	1.67	1.67	1.17	2.17	0.50	1.99	0.14	0.16	0.16	0.12	0.21	0.04	0.18	0.12	0.13	0.13	0.10	0.16	0.03	0.14	315
0.18	2.12	2.64	2.65	1.83	3.46	0.81	3.23	0.16	0.19	0.18	0.14	0.23	0.04	0.21	0.13	0.15	0.15	0.12	0.18	0.03	0.16	238
0.32	3.06	4.18	3.97	2.39	5.96	1.78	5.13	0.18	0.21	0.21	0.16	0.26	0.05	0.23	0.15	0.17	0.17	0.13	0.20	0.03	0.19	324


==> data/mlm_plots/tef/fakenews/bert/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.65
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/bert/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.94	0.96	0.96	0.93	0.98	0.03	0.98	716
0.03	0.94	0.95	0.95	0.94	0.97	0.02	0.96	0.94	0.95	0.95	0.93	0.97	0.02	0.96	0.92	0.94	0.94	0.91	0.97	0.03	0.97	616
0.06	0.91	0.93	0.93	0.90	0.95	0.02	0.94	0.91	0.92	0.92	0.89	0.95	0.03	0.94	0.90	0.92	0.93	0.88	0.96	0.04	0.95	471
0.11	0.88	0.90	0.90	0.87	0.92	0.02	0.91	0.88	0.89	0.89	0.86	0.92	0.03	0.91	0.87	0.90	0.91	0.85	0.95	0.05	0.93	394
0.15	0.84	0.86	0.86	0.83	0.88	0.03	0.88	0.84	0.86	0.86	0.83	0.89	0.03	0.87	0.84	0.87	0.88	0.82	0.92	0.05	0.90	315
0.18	0.80	0.82	0.82	0.79	0.85	0.03	0.83	0.80	0.82	0.82	0.78	0.85	0.03	0.83	0.80	0.83	0.84	0.77	0.89	0.06	0.87	238
0.32	0.75	0.78	0.78	0.74	0.81	0.04	0.80	0.75	0.78	0.78	0.74	0.82	0.04	0.80	0.76	0.79	0.80	0.71	0.86	0.07	0.83	324


==> data/mlm_plots/tef/fakenews/bert/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/fakenews/bert/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	91.31	95.52	101.70	67.84	123.20	27.68	107.88	0.60	20.29	3.37	-34.00	74.59	54.30	17.25	17.72	59.24	41.62	3.85	114.63	55.39	85.11	716
0.03	109.88	133.76	129.94	53.77	213.74	79.99	144.36	0.64	17.79	3.96	-23.51	59.09	41.30	16.83	17.64	59.20	40.92	2.75	115.65	56.45	87.19	616
0.06	146.03	183.94	172.72	77.43	290.44	106.51	201.67	0.62	19.73	3.60	-34.67	74.13	54.40	16.78	15.67	60.02	41.61	0.69	119.36	59.34	88.84	471
0.11	171.00	229.93	215.82	108.63	351.23	121.30	261.08	0.66	20.50	4.27	-32.71	73.72	53.22	15.05	15.35	58.81	35.31	-1.90	119.53	60.72	88.31	394
0.15	237.16	297.37	303.12	165.25	429.50	132.13	361.38	0.54	20.02	3.19	-29.67	69.71	49.69	13.20	12.54	57.34	34.71	-1.98	116.66	59.32	88.54	315
0.18	253.86	329.76	355.93	194.66	464.86	135.10	404.24	0.57	20.42	2.57	-31.85	72.69	52.27	17.48	14.04	59.87	40.43	-2.58	122.31	62.44	91.16	238
0.32	314.30	385.20	430.33	240.85	529.56	144.35	485.98	0.53	24.88	2.78	-36.61	86.37	61.49	24.60	20.48	65.98	45.70	1.76	130.20	64.22	98.97	324


==> data/mlm_plots/tef/fakenews/bert/ig/time_misc_auc.tex <==
name	auc
attack_time	87.53
l2	6.54
lom	18.84


==> data/mlm_plots/tef/fakenews/bert/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.12	0.22	0.20	0.08	0.36	0.14	0.30	0.20	0.31	0.29	0.16	0.45	0.15	0.39	0.37	0.46	0.45	0.32	0.60	0.14	0.55	716
0.03	0.12	0.21	0.19	0.07	0.35	0.14	0.28	0.19	0.30	0.28	0.15	0.45	0.15	0.38	0.36	0.45	0.45	0.31	0.59	0.14	0.54	616
0.06	0.10	0.20	0.18	0.07	0.34	0.14	0.27	0.18	0.29	0.28	0.15	0.44	0.15	0.38	0.35	0.44	0.44	0.30	0.58	0.14	0.54	471
0.11	0.09	0.19	0.17	0.06	0.33	0.14	0.26	0.18	0.28	0.27	0.14	0.42	0.14	0.38	0.34	0.43	0.43	0.30	0.57	0.14	0.53	394
0.15	0.08	0.17	0.15	0.04	0.30	0.13	0.24	0.16	0.26	0.25	0.12	0.40	0.14	0.36	0.34	0.42	0.42	0.28	0.56	0.14	0.51	315
0.18	0.08	0.17	0.15	0.06	0.28	0.11	0.25	0.17	0.27	0.26	0.14	0.40	0.13	0.37	0.35	0.43	0.43	0.31	0.56	0.13	0.52	238
0.32	0.08	0.16	0.14	0.05	0.27	0.11	0.24	0.16	0.26	0.25	0.13	0.39	0.13	0.36	0.35	0.43	0.42	0.30	0.55	0.12	0.51	324


==> data/mlm_plots/tef/fakenews/bert/ig/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.09
top50	0.13


==> data/mlm_plots/tef/fakenews/bert/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	35.07	48.89	43.14	26.43	71.35	22.46	56.32	71.00	82.52	85.00	58.20	106.84	24.32	98.00	40.68	55.28	49.71	31.25	79.31	24.03	63.08	71.00	82.89	85.00	58.55	107.22	24.33	99.00	958
0.03	35.09	51.26	43.77	23.24	79.28	28.02	57.63	69.00	81.52	84.00	54.26	108.78	27.26	99.00	47.41	65.81	57.59	34.57	97.05	31.24	74.04	69.00	82.29	86.00	54.97	109.62	27.32	99.00	1015
0.06	34.75	51.63	42.64	15.30	87.96	36.33	56.36	69.00	80.99	84.00	53.24	108.75	27.76	99.00	57.69	80.53	70.05	37.14	123.92	43.39	88.65	70.75	82.43	86.00	54.44	110.42	27.99	99.00	896
0.11	35.00	53.06	43.16	10.52	95.60	42.54	56.46	69.00	80.62	84.00	53.57	107.67	27.05	98.00	75.18	102.29	90.02	46.03	158.55	56.26	111.85	72.00	83.09	87.00	55.46	110.73	27.64	101.00	846
0.15	36.21	57.69	44.83	8.55	106.82	49.13	57.41	71.00	80.05	84.00	50.70	109.39	29.35	99.00	105.79	145.39	127.85	62.42	228.37	82.98	155.29	73.00	83.56	89.00	53.33	113.79	30.23	103.00	586
0.18	34.50	55.84	43.34	8.49	103.19	47.35	58.12	64.50	77.90	82.00	47.13	108.67	30.77	98.00	127.58	183.36	161.24	80.05	286.67	103.31	197.92	70.50	82.57	88.00	50.68	114.46	31.89	103.00	367
0.32	38.64	64.40	46.31	1.69	127.10	62.70	63.84	55.00	75.12	79.50	40.42	109.81	34.69	99.00	171.28	255.35	217.20	111.76	398.93	143.58	288.18	58.00	80.47	87.00	44.22	116.73	36.25	106.00	438


==> data/mlm_plots/tef/fakenews/bert/s/comparison_vals_auc.tex <==
name	auc
orig_pp	17.52
orig_ge	24.46
adv_pp	48.49
adv_ge	25.55


==> data/mlm_plots/tef/fakenews/bert/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.09	0.29	0.23	0.06	0.51	0.23	0.45	0.43	0.55	0.58	0.37	0.72	0.17	0.69	0.30	0.40	0.41	0.26	0.53	0.14	0.50	958
0.03	0.06	0.22	0.15	0.02	0.43	0.21	0.34	0.37	0.49	0.52	0.31	0.68	0.18	0.64	0.25	0.35	0.37	0.21	0.50	0.14	0.47	1015
0.06	0.04	0.18	0.10	-0.01	0.36	0.19	0.27	0.32	0.46	0.46	0.27	0.64	0.18	0.61	0.21	0.32	0.32	0.19	0.46	0.14	0.44	896
0.11	0.03	0.15	0.09	-0.02	0.33	0.17	0.23	0.29	0.43	0.43	0.25	0.62	0.19	0.58	0.20	0.31	0.30	0.17	0.45	0.14	0.42	846
0.15	0.02	0.13	0.07	-0.02	0.28	0.15	0.19	0.29	0.42	0.42	0.25	0.59	0.17	0.55	0.20	0.29	0.29	0.17	0.42	0.13	0.39	586
0.18	0.04	0.14	0.08	-0.01	0.28	0.14	0.21	0.27	0.40	0.40	0.23	0.57	0.17	0.54	0.19	0.28	0.28	0.16	0.41	0.13	0.38	367
0.32	0.03	0.14	0.10	-0.01	0.28	0.15	0.22	0.26	0.39	0.39	0.20	0.57	0.18	0.53	0.17	0.27	0.27	0.14	0.40	0.13	0.37	438


==> data/mlm_plots/tef/fakenews/bert/s/correlations_auc.tex <==
name	auc
pcc	0.05
spearman	0.13
kendall	0.09


==> data/mlm_plots/tef/fakenews/bert/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	9.36	13.99	12.92	7.39	20.58	6.60	17.60	7.72	12.46	11.34	5.93	18.98	6.53	15.53	5.95	11.03	9.06	3.53	18.53	7.50	14.08	958
0.03	6.23	8.37	8.06	5.05	11.69	3.32	10.29	5.50	7.78	7.40	4.42	11.14	3.36	9.55	4.89	8.64	7.41	3.07	14.20	5.56	10.91	1015
0.06	4.48	5.52	5.38	3.63	7.41	1.89	6.44	4.15	5.35	5.17	3.39	7.30	1.96	6.41	4.15	6.58	5.76	2.67	10.48	3.90	8.09	896
0.11	3.34	3.95	3.87	2.85	5.05	1.10	4.51	3.17	3.87	3.76	2.69	5.04	1.17	4.43	3.31	5.00	4.38	2.06	7.93	2.94	5.93	846
0.15	2.62	3.02	3.00	2.30	3.74	0.72	3.44	2.57	3.01	3.01	2.23	3.79	0.78	3.42	2.68	3.80	3.67	2.25	5.35	1.55	4.66	586
0.18	2.17	2.48	2.48	1.92	3.04	0.56	2.80	2.17	2.50	2.50	1.91	3.10	0.60	2.87	2.23	3.13	2.87	1.82	4.43	1.30	3.74	367
0.32	1.80	2.10	2.11	1.63	2.57	0.47	2.40	1.80	2.12	2.12	1.61	2.64	0.52	2.42	1.90	2.58	2.45	1.54	3.61	1.03	3.10	438


==> data/mlm_plots/tef/fakenews/bert/s/ets_sts_auc.tex <==
name	auc
et_use	1.21
et_tse	1.18
et_ce	1.39


==> data/mlm_plots/tef/fakenews/bert/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.88	3.30	2.71	-0.69	7.28	3.99	3.61	6.27	9.66	8.58	4.32	15.00	5.34	11.60	4.93	8.64	7.11	2.80	14.48	5.84	10.45	958
0.03	0.98	1.48	1.28	-0.13	3.09	1.61	1.64	4.76	6.48	6.23	3.62	9.34	2.86	7.67	3.71	5.56	4.97	2.11	9.01	3.45	6.42	1015
0.06	0.55	0.77	0.68	-0.02	1.56	0.79	0.86	3.87	4.93	4.80	3.04	6.83	1.90	5.76	2.94	4.10	3.80	1.71	6.48	2.39	4.75	896
0.11	0.34	0.45	0.41	0.21	0.69	0.24	0.51	3.34	4.08	3.96	2.62	5.53	1.45	4.68	2.60	3.49	3.18	-0.21	7.20	3.71	3.77	846
0.15	0.21	0.28	0.25	0.14	0.42	0.14	0.32	2.89	3.57	3.48	2.06	5.08	1.51	3.96	2.28	3.14	2.80	-1.64	7.92	4.78	3.23	586
0.18	0.14	0.19	0.17	0.10	0.27	0.09	0.20	2.49	3.03	2.96	1.89	4.17	1.14	3.30	1.91	2.59	2.31	-0.05	5.24	2.64	2.68	367
0.32	0.10	0.15	0.12	0.02	0.29	0.14	0.17	2.26	2.84	2.75	1.70	3.99	1.14	3.11	1.80	2.55	2.19	-0.78	5.89	3.34	2.49	438


==> data/mlm_plots/tef/fakenews/bert/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.16
et_p_h	1.22
et_p_l2	1.06


==> data/mlm_plots/tef/fakenews/bert/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.10	0.14	0.14	0.08	0.19	0.05	0.17	0.03	0.05	0.05	0.03	0.08	0.03	0.07	0.03	0.04	0.04	0.03	0.06	0.02	0.05	958
0.03	0.25	0.31	0.31	0.21	0.42	0.11	0.38	0.06	0.08	0.08	0.05	0.12	0.03	0.10	0.05	0.07	0.07	0.05	0.09	0.02	0.08	1015
0.06	0.51	0.62	0.62	0.43	0.82	0.20	0.74	0.09	0.11	0.11	0.08	0.15	0.04	0.13	0.07	0.09	0.09	0.07	0.11	0.02	0.10	896
0.11	0.87	1.06	1.03	0.73	1.38	0.32	1.24	0.12	0.14	0.14	0.10	0.18	0.04	0.16	0.10	0.11	0.11	0.08	0.13	0.03	0.12	846
0.15	1.45	1.76	1.74	1.24	2.27	0.51	2.02	0.14	0.16	0.16	0.12	0.21	0.04	0.19	0.12	0.13	0.13	0.10	0.16	0.03	0.15	586
0.18	2.19	2.61	2.60	1.84	3.37	0.77	3.11	0.16	0.19	0.19	0.14	0.24	0.05	0.22	0.13	0.15	0.15	0.12	0.18	0.03	0.17	367
0.32	2.70	3.59	3.49	2.18	4.99	1.40	4.37	0.18	0.20	0.20	0.15	0.26	0.05	0.23	0.15	0.16	0.17	0.13	0.20	0.04	0.18	438


==> data/mlm_plots/tef/fakenews/bert/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.61
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/bert/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.94	0.96	0.96	0.93	0.98	0.02	0.97	958
0.03	0.94	0.95	0.95	0.93	0.97	0.02	0.96	0.93	0.94	0.95	0.92	0.96	0.02	0.96	0.92	0.94	0.95	0.91	0.97	0.03	0.96	1015
0.06	0.91	0.92	0.92	0.90	0.94	0.02	0.93	0.90	0.92	0.92	0.89	0.94	0.03	0.93	0.90	0.92	0.93	0.88	0.96	0.04	0.95	896
0.11	0.87	0.89	0.89	0.86	0.91	0.03	0.91	0.87	0.88	0.88	0.86	0.91	0.03	0.90	0.87	0.90	0.90	0.86	0.94	0.04	0.93	846
0.15	0.84	0.85	0.85	0.83	0.88	0.03	0.87	0.84	0.85	0.85	0.82	0.88	0.03	0.87	0.85	0.87	0.88	0.83	0.91	0.04	0.90	586
0.18	0.81	0.82	0.82	0.79	0.85	0.03	0.84	0.81	0.82	0.82	0.79	0.85	0.03	0.84	0.82	0.84	0.85	0.79	0.90	0.05	0.88	367
0.32	0.77	0.79	0.79	0.76	0.82	0.03	0.81	0.77	0.79	0.79	0.75	0.83	0.04	0.81	0.78	0.81	0.82	0.74	0.88	0.07	0.86	438


==> data/mlm_plots/tef/fakenews/bert/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.27


==> data/mlm_plots/tef/fakenews/bert/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	30.16	34.92	35.88	21.83	48.02	13.09	41.23	0.10	218.15	0.46	-597.03	1033.34	815.19	63.85	8.55	35.05	24.51	2.15	67.95	32.90	53.75	958
0.03	50.10	65.26	60.87	24.81	105.71	40.45	73.64	0.14	336.62	0.59	-1307.14	1980.38	1643.76	90.06	10.24	40.04	28.18	3.30	76.78	36.74	61.72	1015
0.06	71.48	106.92	90.84	39.51	174.32	67.41	124.76	0.18	237.52	1.78	-504.75	979.78	742.27	132.68	11.38	45.79	32.92	5.54	86.03	40.25	71.54	896
0.11	81.81	130.86	113.31	55.41	206.32	75.46	177.65	0.21	312.37	1.46	-801.67	1426.42	1114.05	156.70	12.14	46.55	37.31	7.51	85.58	39.04	71.92	846
0.15	132.25	175.69	187.73	98.22	253.15	77.47	235.85	0.17	198.73	0.51	-488.92	886.38	687.65	64.66	11.34	44.60	35.38	6.72	82.47	37.88	69.14	586
0.18	138.90	182.20	203.28	102.16	262.25	80.05	242.77	0.16	174.66	0.42	-778.09	1127.42	952.75	33.13	8.86	40.24	31.20	4.45	76.04	35.79	65.49	367
0.32	111.79	182.45	215.11	98.55	266.36	83.91	248.16	0.13	181.05	0.41	-616.37	978.47	797.42	43.39	8.54	34.91	25.72	3.76	66.06	31.15	55.15	438


==> data/mlm_plots/tef/fakenews/bert/s/time_misc_auc.tex <==
name	auc
attack_time	46.73
l2	68.72
lom	12.74


==> data/mlm_plots/tef/fakenews/bert/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.25	0.37	0.37	0.21	0.54	0.16	0.50	0.50	0.58	0.59	0.47	0.69	0.11	0.67	0.65	0.70	0.71	0.63	0.78	0.07	0.76	958
0.03	0.20	0.32	0.30	0.16	0.48	0.16	0.44	0.45	0.54	0.55	0.42	0.66	0.12	0.63	0.63	0.68	0.69	0.60	0.76	0.08	0.74	1015
0.06	0.17	0.29	0.26	0.13	0.44	0.15	0.40	0.42	0.52	0.51	0.40	0.63	0.12	0.60	0.61	0.67	0.67	0.59	0.74	0.08	0.73	896
0.11	0.14	0.26	0.23	0.11	0.42	0.15	0.37	0.41	0.50	0.50	0.38	0.62	0.12	0.59	0.60	0.66	0.66	0.58	0.73	0.08	0.71	846
0.15	0.14	0.25	0.23	0.10	0.39	0.15	0.33	0.41	0.49	0.49	0.38	0.61	0.12	0.58	0.60	0.65	0.66	0.58	0.73	0.07	0.71	586
0.18	0.14	0.25	0.21	0.11	0.38	0.14	0.33	0.41	0.49	0.49	0.38	0.60	0.11	0.57	0.59	0.65	0.65	0.58	0.72	0.07	0.69	367
0.32	0.14	0.24	0.21	0.09	0.39	0.15	0.33	0.40	0.48	0.48	0.37	0.59	0.11	0.57	0.59	0.64	0.65	0.57	0.72	0.08	0.70	438


==> data/mlm_plots/tef/fakenews/bert/s/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.16
top50	0.20


==> data/mlm_plots/tef/fakenews/cnn/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	33.73	46.45	41.34	25.21	67.68	21.24	53.20	73.00	88.36	89.00	54.57	122.15	33.79	102.50	39.17	52.90	47.49	30.08	75.71	22.81	59.92	73.00	88.69	90.00	54.82	122.56	33.87	103.00	935
0.03	33.95	48.70	41.81	21.67	75.72	27.02	54.64	70.00	85.80	88.00	49.18	122.41	36.62	102.00	45.84	62.80	55.94	33.34	92.26	29.46	70.42	71.00	86.70	89.00	49.82	123.57	36.87	102.00	1006
0.06	34.07	52.76	42.07	10.23	95.29	42.53	55.98	67.00	83.70	87.00	45.44	121.95	38.26	101.00	57.54	80.35	69.20	31.28	129.42	49.07	86.31	69.00	85.73	90.00	46.87	124.60	38.87	103.00	1033
0.11	34.13	55.42	42.22	-12.58	123.42	68.00	56.14	67.00	83.42	87.00	44.78	122.05	38.63	101.00	69.86	97.36	82.61	25.81	168.91	71.55	101.35	70.00	86.66	91.00	47.10	126.22	39.56	105.00	1009
0.15	34.07	52.80	41.97	11.32	94.29	41.49	55.95	67.00	83.81	87.00	45.48	122.14	38.33	102.00	93.53	124.98	111.06	57.02	192.93	67.96	133.07	73.00	89.42	94.00	49.67	129.18	39.76	108.00	1004
0.18	34.29	60.11	42.65	-44.49	164.71	104.60	56.33	67.00	82.52	87.00	44.71	120.33	37.81	100.50	122.90	164.12	144.93	62.56	265.68	101.56	170.59	76.00	90.69	97.00	50.91	130.46	39.77	110.00	811
0.32	34.31	55.76	42.67	-0.70	112.22	56.46	56.32	67.00	82.03	87.00	45.15	118.90	36.88	101.00	171.97	240.93	214.42	118.44	363.42	122.49	275.85	80.00	95.33	102.00	55.06	135.61	40.28	117.00	1412


==> data/mlm_plots/tef/fakenews/cnn/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	17.16
orig_ge	25.87
adv_pp	44.73
adv_ge	27.93


==> data/mlm_plots/tef/fakenews/cnn/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.55	0.73	0.81	0.50	0.96	0.23	0.93	0.79	0.84	0.87	0.76	0.93	0.08	0.91	0.70	0.79	0.81	0.67	0.90	0.12	0.89	935
0.03	0.48	0.68	0.76	0.43	0.93	0.25	0.89	0.71	0.76	0.78	0.66	0.85	0.09	0.82	0.62	0.70	0.71	0.59	0.82	0.11	0.79	1006
0.06	0.41	0.63	0.68	0.37	0.89	0.26	0.86	0.58	0.64	0.65	0.54	0.75	0.11	0.71	0.52	0.59	0.60	0.48	0.70	0.11	0.67	1033
0.11	0.38	0.59	0.62	0.33	0.85	0.26	0.83	0.49	0.55	0.56	0.44	0.66	0.11	0.62	0.43	0.50	0.50	0.39	0.60	0.11	0.57	1009
0.15	0.32	0.53	0.54	0.27	0.79	0.26	0.77	0.34	0.41	0.42	0.30	0.53	0.12	0.49	0.30	0.37	0.37	0.27	0.47	0.10	0.43	1004
0.18	0.28	0.49	0.48	0.23	0.75	0.26	0.72	0.24	0.32	0.32	0.20	0.44	0.12	0.39	0.21	0.28	0.28	0.17	0.38	0.10	0.33	811
0.32	0.23	0.43	0.39	0.17	0.68	0.25	0.63	0.13	0.22	0.22	0.09	0.35	0.13	0.30	0.11	0.18	0.17	0.07	0.28	0.11	0.24	1412


==> data/mlm_plots/tef/fakenews/cnn/ig/correlations_auc.tex <==
name	auc
pcc	0.17
spearman	0.14
kendall	0.12


==> data/mlm_plots/tef/fakenews/cnn/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	1.40	5.49	3.40	0.07	10.90	5.41	7.96	1.32	5.46	3.36	-0.14	11.06	5.60	7.99	1.03	4.06	2.34	-0.75	8.87	4.81	5.22	935
0.03	1.08	3.33	2.41	0.45	6.21	2.88	4.94	1.00	3.16	2.26	0.44	5.88	2.72	4.67	0.97	3.06	2.02	-0.01	6.13	3.07	4.06	1006
0.06	0.84	2.30	1.84	0.55	4.06	1.75	3.40	0.77	2.19	1.75	0.49	3.88	1.69	3.27	0.86	2.37	1.74	0.15	4.59	2.22	3.19	1033
0.11	0.78	1.91	1.68	0.57	3.24	1.34	2.80	0.71	1.80	1.59	0.51	3.09	1.29	2.58	0.80	2.01	1.62	0.34	3.67	1.67	2.76	1009
0.15	0.74	1.58	1.48	0.62	2.54	0.96	2.26	0.70	1.48	1.42	0.57	2.39	0.91	2.12	0.77	1.67	1.43	0.45	2.88	1.22	2.28	1004
0.18	0.72	1.40	1.40	0.64	2.15	0.76	1.97	0.69	1.32	1.31	0.59	2.04	0.73	1.83	0.72	1.44	1.28	0.48	2.40	0.96	1.96	811
0.32	0.75	1.22	1.24	0.62	1.81	0.59	1.63	0.70	1.16	1.18	0.59	1.73	0.57	1.55	0.70	1.19	1.10	0.51	1.87	0.68	1.57	1412


==> data/mlm_plots/tef/fakenews/cnn/ig/ets_sts_auc.tex <==
name	auc
et_use	0.58
et_tse	0.55
et_ce	0.57


==> data/mlm_plots/tef/fakenews/cnn/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.25	1.19	0.72	-0.28	2.67	1.48	1.61	0.81	3.85	2.39	-0.64	8.34	4.49	5.33	0.65	3.54	1.98	-1.11	8.19	4.65	4.58	935
0.03	0.16	0.58	0.42	-0.00	1.17	0.59	0.85	0.78	2.72	1.99	0.30	5.13	2.41	4.05	0.61	2.41	1.65	-0.18	5.01	2.60	3.35	1006
0.06	0.12	0.34	0.28	0.05	0.64	0.29	0.49	0.82	2.31	1.90	0.51	4.10	1.79	3.40	0.67	2.07	1.59	-0.21	4.34	2.27	2.81	1033
0.11	0.10	0.26	0.21	-0.33	0.86	0.59	0.34	0.84	2.08	1.89	0.59	3.58	1.50	2.97	0.68	1.95	1.54	-2.29	6.18	4.23	2.49	1009
0.15	0.07	0.17	0.15	0.03	0.30	0.13	0.22	0.91	1.91	1.81	0.71	3.11	1.20	2.66	0.74	1.65	1.48	0.15	3.16	1.51	2.20	1004
0.18	0.06	0.13	0.11	0.02	0.24	0.11	0.16	0.98	1.85	1.79	0.72	2.98	1.13	2.48	0.83	1.65	1.49	-0.08	3.37	1.72	2.06	811
0.32	0.04	0.09	0.07	-0.10	0.29	0.20	0.11	1.04	1.72	1.71	0.71	2.72	1.01	2.20	0.86	1.55	1.42	-1.01	4.12	2.57	1.84	1412


==> data/mlm_plots/tef/fakenews/cnn/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.08
et_p_h	0.64
et_p_l2	0.57


==> data/mlm_plots/tef/fakenews/cnn/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.11	0.15	0.15	0.09	0.21	0.06	0.18	0.04	0.06	0.05	0.03	0.08	0.03	0.07	0.03	0.05	0.04	0.03	0.06	0.02	0.06	935
0.03	0.25	0.32	0.32	0.21	0.43	0.11	0.39	0.06	0.08	0.08	0.05	0.12	0.03	0.10	0.05	0.07	0.07	0.05	0.09	0.02	0.08	1006
0.06	0.49	0.61	0.61	0.41	0.81	0.20	0.74	0.09	0.11	0.11	0.07	0.15	0.04	0.13	0.07	0.09	0.09	0.06	0.11	0.03	0.10	1033
0.11	0.75	0.93	0.93	0.63	1.23	0.30	1.12	0.11	0.13	0.13	0.09	0.17	0.04	0.15	0.09	0.11	0.11	0.08	0.13	0.03	0.12	1009
0.15	1.27	1.58	1.57	1.07	2.09	0.51	1.89	0.13	0.16	0.16	0.11	0.20	0.04	0.18	0.11	0.13	0.13	0.10	0.16	0.03	0.15	1004
0.18	1.85	2.33	2.33	1.49	3.17	0.84	2.83	0.15	0.18	0.18	0.13	0.23	0.05	0.21	0.13	0.15	0.15	0.11	0.18	0.03	0.17	811
0.32	2.89	4.08	3.80	2.27	5.89	1.81	5.04	0.18	0.21	0.21	0.16	0.27	0.05	0.24	0.16	0.18	0.18	0.14	0.21	0.04	0.20	1412


==> data/mlm_plots/tef/fakenews/cnn/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.61
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/cnn/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.94	0.96	0.96	0.93	0.98	0.03	0.98	935
0.03	0.94	0.95	0.95	0.93	0.96	0.02	0.96	0.93	0.94	0.95	0.92	0.96	0.02	0.96	0.92	0.93	0.94	0.90	0.97	0.04	0.96	1006
0.06	0.90	0.91	0.91	0.89	0.94	0.02	0.93	0.89	0.91	0.91	0.88	0.93	0.03	0.92	0.88	0.90	0.91	0.86	0.95	0.04	0.94	1033
0.11	0.87	0.89	0.89	0.86	0.91	0.02	0.90	0.86	0.88	0.88	0.85	0.91	0.03	0.90	0.85	0.88	0.89	0.83	0.93	0.05	0.91	1009
0.15	0.83	0.85	0.85	0.82	0.87	0.03	0.86	0.82	0.83	0.84	0.80	0.87	0.03	0.85	0.80	0.84	0.85	0.78	0.90	0.06	0.88	1004
0.18	0.79	0.81	0.81	0.78	0.84	0.03	0.83	0.78	0.80	0.80	0.76	0.83	0.03	0.82	0.76	0.80	0.81	0.74	0.86	0.06	0.85	811
0.32	0.73	0.76	0.76	0.72	0.80	0.04	0.78	0.71	0.74	0.74	0.70	0.79	0.04	0.77	0.69	0.74	0.74	0.66	0.81	0.08	0.79	1412


==> data/mlm_plots/tef/fakenews/cnn/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.26


==> data/mlm_plots/tef/fakenews/cnn/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	19.68	20.83	20.88	19.48	22.17	1.34	21.71	2.28	3.69	3.26	1.48	5.90	2.21	4.61	3.27	14.51	9.39	-0.19	29.22	14.71	21.54	935
0.03	24.69	26.12	26.18	24.27	27.97	1.85	27.56	2.74	4.34	3.78	1.62	7.06	2.72	5.27	4.11	16.61	11.30	0.49	32.73	16.12	24.42	1006
0.06	31.77	33.95	34.23	31.31	36.58	2.63	36.18	3.19	4.99	4.31	1.67	8.30	3.31	5.81	4.51	18.34	13.42	1.02	35.66	17.32	26.45	1033
0.11	38.92	41.38	41.03	37.80	44.96	3.58	43.30	3.52	5.47	4.73	1.76	9.19	3.72	6.21	5.27	19.17	14.12	1.35	37.00	17.83	27.92	1009
0.15	52.71	55.32	54.61	50.99	59.64	4.33	58.87	4.09	6.25	5.34	1.85	10.64	4.40	6.75	6.32	20.38	14.81	2.18	38.59	18.21	29.31	1004
0.18	64.54	68.95	70.50	63.00	74.89	5.94	73.84	4.47	6.94	5.73	1.98	11.90	4.96	7.47	6.56	20.50	15.75	2.69	38.31	17.81	30.13	811
0.32	85.05	97.01	94.25	81.82	112.19	15.18	110.86	5.05	7.85	6.56	2.48	13.23	5.37	8.77	6.45	20.96	15.86	2.72	39.20	18.24	30.74	1412


==> data/mlm_plots/tef/fakenews/cnn/ig/time_misc_auc.tex <==
name	auc
attack_time	18.63
l2	1.95
lom	6.09


==> data/mlm_plots/tef/fakenews/cnn/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.76	0.80	0.82	0.72	0.89	0.08	0.87	0.83	0.88	0.89	0.81	0.95	0.07	0.94	0.86	0.90	0.91	0.84	0.97	0.06	0.96	935
0.03	0.64	0.71	0.71	0.62	0.80	0.09	0.78	0.79	0.83	0.85	0.76	0.90	0.07	0.89	0.83	0.87	0.88	0.81	0.93	0.06	0.92	1006
0.06	0.54	0.61	0.61	0.50	0.71	0.11	0.67	0.73	0.77	0.78	0.70	0.84	0.07	0.82	0.79	0.83	0.84	0.76	0.89	0.06	0.87	1033
0.11	0.48	0.55	0.55	0.43	0.66	0.11	0.61	0.67	0.72	0.72	0.65	0.78	0.07	0.77	0.75	0.79	0.79	0.73	0.85	0.06	0.83	1009
0.15	0.40	0.48	0.47	0.36	0.59	0.11	0.53	0.59	0.63	0.64	0.57	0.70	0.07	0.68	0.69	0.73	0.74	0.67	0.79	0.06	0.77	1004
0.18	0.36	0.43	0.42	0.30	0.56	0.13	0.49	0.53	0.57	0.57	0.50	0.64	0.07	0.61	0.65	0.68	0.68	0.62	0.73	0.06	0.71	811
0.32	0.29	0.37	0.36	0.23	0.51	0.14	0.44	0.44	0.49	0.49	0.42	0.57	0.08	0.54	0.58	0.62	0.62	0.56	0.67	0.06	0.66	1412


==> data/mlm_plots/tef/fakenews/cnn/ig/top_intersections_auc.tex <==
name	auc
top10	0.15
top30	0.20
top50	0.23


==> data/mlm_plots/tef/fakenews/cnn/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	33.63	45.96	41.34	26.09	65.84	19.87	53.33	73.00	88.61	89.00	54.12	123.10	34.49	102.50	39.52	52.86	48.38	31.50	74.22	21.36	60.87	74.00	89.30	90.00	54.54	124.06	34.76	103.00	967
0.03	33.91	48.47	41.79	21.94	75.00	26.53	54.47	70.75	86.25	88.00	49.92	122.57	36.33	102.00	46.72	63.62	57.19	33.16	94.08	30.46	71.01	72.00	87.69	90.00	50.82	124.57	36.88	104.00	1000
0.06	34.07	52.48	41.93	10.00	94.97	42.49	55.85	68.00	84.38	87.00	46.55	122.22	37.84	102.00	59.28	82.99	70.66	28.29	137.69	54.70	88.90	71.00	87.11	91.00	48.27	125.94	38.83	104.00	998
0.11	34.15	56.19	42.52	-14.08	126.46	70.27	56.15	67.00	83.23	87.00	45.62	120.84	37.61	101.00	72.18	103.53	85.83	21.06	185.99	82.46	107.19	71.00	87.16	92.00	48.14	126.18	39.02	105.50	1007
0.15	34.15	55.34	42.52	4.13	106.54	51.21	56.30	67.00	83.27	87.00	44.58	121.95	38.69	101.00	99.56	133.36	116.68	55.95	210.76	77.40	141.58	73.00	89.39	94.00	48.80	129.99	40.60	108.00	1015
0.18	34.18	59.13	42.54	-36.88	155.14	96.01	56.30	67.00	83.04	87.00	44.11	121.97	38.93	101.00	129.91	172.06	151.80	72.82	271.29	99.23	179.72	76.00	91.60	97.50	50.18	133.02	41.42	112.00	1014
0.32	34.22	56.12	42.62	-3.03	115.27	59.15	56.32	67.00	82.58	87.00	44.29	120.87	38.29	101.00	179.03	247.73	221.02	120.56	374.90	127.17	281.27	81.00	96.02	103.00	54.18	137.86	41.84	118.00	1708


==> data/mlm_plots/tef/fakenews/cnn/s/comparison_vals_auc.tex <==
name	auc
orig_pp	17.22
orig_ge	25.96
adv_pp	46.60
adv_ge	28.16


==> data/mlm_plots/tef/fakenews/cnn/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.80	0.84	0.87	0.74	0.95	0.11	0.92	0.90	0.92	0.93	0.87	0.97	0.05	0.95	0.78	0.84	0.87	0.75	0.93	0.09	0.90	967
0.03	0.72	0.78	0.81	0.66	0.90	0.12	0.87	0.83	0.86	0.87	0.80	0.92	0.06	0.90	0.71	0.75	0.77	0.67	0.84	0.08	0.81	1000
0.06	0.63	0.71	0.73	0.57	0.85	0.14	0.80	0.74	0.78	0.78	0.71	0.85	0.07	0.83	0.60	0.65	0.66	0.57	0.73	0.08	0.71	998
0.11	0.57	0.65	0.66	0.51	0.80	0.14	0.75	0.66	0.71	0.71	0.62	0.80	0.09	0.76	0.52	0.57	0.57	0.48	0.66	0.09	0.62	1007
0.15	0.47	0.57	0.57	0.41	0.72	0.15	0.68	0.55	0.61	0.61	0.51	0.71	0.10	0.67	0.41	0.46	0.46	0.38	0.55	0.09	0.51	1015
0.18	0.38	0.50	0.50	0.33	0.66	0.16	0.60	0.45	0.52	0.52	0.40	0.63	0.12	0.58	0.32	0.38	0.37	0.29	0.48	0.09	0.43	1014
0.32	0.26	0.39	0.37	0.21	0.56	0.18	0.51	0.25	0.36	0.36	0.21	0.51	0.15	0.46	0.18	0.26	0.25	0.14	0.37	0.11	0.33	1708


==> data/mlm_plots/tef/fakenews/cnn/s/correlations_auc.tex <==
name	auc
pcc	0.18
spearman	0.18
kendall	0.15


==> data/mlm_plots/tef/fakenews/cnn/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	1.27	2.91	2.12	0.45	5.36	2.45	3.59	1.23	2.80	2.00	0.27	5.32	2.52	3.51	0.98	2.57	1.70	-0.09	5.22	2.66	3.22	967
0.03	1.14	2.13	1.76	0.66	3.59	1.46	2.70	1.08	2.03	1.66	0.59	3.46	1.43	2.62	1.05	2.30	1.69	0.40	4.20	1.90	2.97	1000
0.06	1.08	1.72	1.49	0.74	2.71	0.99	2.14	1.01	1.64	1.39	0.65	2.63	0.99	2.04	1.11	2.01	1.61	0.57	3.46	1.44	2.50	998
0.11	1.02	1.55	1.44	0.80	2.30	0.75	1.94	0.95	1.47	1.35	0.74	2.19	0.73	1.86	1.08	1.83	1.56	0.61	3.06	1.22	2.28	1007
0.15	1.02	1.42	1.36	0.84	1.99	0.58	1.75	0.96	1.34	1.27	0.78	1.90	0.56	1.65	1.04	1.61	1.44	0.74	2.48	0.87	1.98	1015
0.18	1.01	1.35	1.32	0.85	1.84	0.50	1.64	0.96	1.28	1.24	0.79	1.76	0.48	1.55	1.00	1.56	1.36	-0.05	3.18	1.62	1.84	1014
0.32	1.01	1.28	1.27	0.86	1.70	0.42	1.54	0.96	1.23	1.22	0.82	1.65	0.42	1.47	0.93	1.31	1.21	0.72	1.89	0.58	1.56	1708


==> data/mlm_plots/tef/fakenews/cnn/s/ets_sts_auc.tex <==
name	auc
et_use	0.48
et_tse	0.45
et_ce	0.53


==> data/mlm_plots/tef/fakenews/cnn/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.25	0.59	0.41	-0.04	1.21	0.62	0.68	0.87	1.92	1.41	0.16	3.67	1.75	2.40	0.70	1.80	1.16	-0.55	4.14	2.34	2.08	967
0.03	0.19	0.37	0.28	0.06	0.67	0.30	0.44	0.95	1.73	1.41	0.50	2.96	1.23	2.12	0.74	1.53	1.17	-0.08	3.14	1.61	1.75	1000
0.06	0.15	0.25	0.21	0.03	0.47	0.22	0.30	1.03	1.68	1.49	0.69	2.67	0.99	2.06	0.84	1.46	1.21	0.18	2.74	1.28	1.70	998
0.11	0.12	0.20	0.17	0.01	0.40	0.19	0.24	1.10	1.70	1.57	0.76	2.64	0.94	2.05	0.89	1.50	1.27	-0.00	3.00	1.50	1.71	1007
0.15	0.09	0.16	0.13	-0.03	0.34	0.18	0.17	1.22	1.80	1.60	0.31	3.29	1.49	2.06	0.99	1.84	1.30	-3.41	7.09	5.25	1.71	1015
0.18	0.07	0.17	0.10	-1.46	1.81	1.63	0.14	1.29	1.76	1.67	0.90	2.62	0.86	2.07	1.05	1.61	1.36	-0.56	3.79	2.18	1.71	1014
0.32	0.05	0.10	0.07	-0.04	0.23	0.13	0.10	1.38	1.81	1.74	0.89	2.73	0.92	2.09	1.14	1.63	1.44	-0.40	3.66	2.03	1.74	1708


==> data/mlm_plots/tef/fakenews/cnn/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.06
et_p_h	0.55
et_p_l2	0.50


==> data/mlm_plots/tef/fakenews/cnn/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.12	0.16	0.16	0.10	0.22	0.06	0.20	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.06	0.02	0.06	967
0.03	0.28	0.34	0.34	0.24	0.45	0.11	0.41	0.07	0.09	0.09	0.06	0.12	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	1000
0.06	0.54	0.66	0.66	0.46	0.86	0.20	0.79	0.09	0.12	0.11	0.08	0.15	0.04	0.14	0.08	0.09	0.09	0.07	0.12	0.02	0.11	998
0.11	0.82	1.01	1.00	0.69	1.32	0.31	1.20	0.11	0.14	0.14	0.10	0.18	0.04	0.16	0.10	0.11	0.11	0.08	0.14	0.03	0.13	1007
0.15	1.36	1.70	1.70	1.14	2.25	0.56	2.04	0.14	0.16	0.17	0.12	0.21	0.05	0.19	0.12	0.13	0.14	0.10	0.16	0.03	0.15	1015
0.18	2.01	2.51	2.50	1.67	3.35	0.84	3.04	0.16	0.19	0.19	0.14	0.24	0.05	0.21	0.14	0.15	0.15	0.12	0.19	0.03	0.17	1014
0.32	3.01	4.24	4.02	2.41	6.06	1.82	5.28	0.19	0.22	0.22	0.16	0.27	0.05	0.25	0.16	0.18	0.18	0.14	0.22	0.04	0.20	1708


==> data/mlm_plots/tef/fakenews/cnn/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.65
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/cnn/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.95	0.96	0.97	0.93	0.98	0.02	0.98	967
0.03	0.93	0.94	0.94	0.93	0.96	0.02	0.95	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.92	0.94	0.95	0.91	0.97	0.03	0.96	1000
0.06	0.90	0.91	0.91	0.89	0.93	0.02	0.92	0.89	0.90	0.90	0.88	0.93	0.02	0.92	0.89	0.91	0.92	0.88	0.95	0.04	0.94	998
0.11	0.87	0.88	0.88	0.86	0.91	0.02	0.90	0.86	0.87	0.88	0.85	0.90	0.03	0.89	0.86	0.89	0.90	0.85	0.93	0.04	0.92	1007
0.15	0.83	0.84	0.84	0.82	0.87	0.03	0.86	0.81	0.83	0.83	0.80	0.86	0.03	0.85	0.82	0.85	0.85	0.80	0.90	0.05	0.88	1015
0.18	0.79	0.81	0.81	0.78	0.83	0.03	0.82	0.78	0.80	0.79	0.77	0.83	0.03	0.81	0.78	0.81	0.81	0.76	0.87	0.06	0.85	1014
0.32	0.73	0.76	0.76	0.72	0.79	0.04	0.78	0.71	0.74	0.74	0.70	0.79	0.04	0.77	0.70	0.74	0.75	0.67	0.82	0.08	0.80	1708


==> data/mlm_plots/tef/fakenews/cnn/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.26


==> data/mlm_plots/tef/fakenews/cnn/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	13.11	13.86	14.00	12.89	14.84	0.97	14.67	21.70	39.14	29.69	8.06	70.22	31.08	44.47	3.48	11.06	7.99	0.33	21.80	10.74	14.88	967
0.03	17.20	18.10	18.02	16.66	19.55	1.45	19.17	27.90	48.94	37.35	10.32	87.56	38.62	53.66	4.23	13.29	9.73	0.69	25.90	12.60	18.37	1000
0.06	24.07	25.37	25.27	22.87	27.86	2.49	27.36	35.18	59.09	45.43	13.12	105.06	45.97	65.35	5.12	15.98	12.05	1.13	30.83	14.85	22.24	998
0.11	28.63	30.26	30.55	27.71	32.80	2.55	31.95	40.40	67.99	52.76	15.50	120.48	52.49	75.24	5.72	17.90	13.53	1.82	33.99	16.09	26.20	1007
0.15	37.89	41.09	40.91	36.25	45.92	4.84	43.71	48.88	81.74	65.63	20.22	143.27	61.53	91.46	6.19	20.11	15.43	2.50	37.72	17.61	29.50	1015
0.18	51.83	53.97	53.83	49.36	58.57	4.61	57.10	56.01	94.31	75.75	24.85	163.76	69.45	108.97	6.29	22.57	18.25	3.09	42.05	19.48	33.26	1014
0.32	65.59	75.66	71.48	62.91	88.42	12.75	87.18	68.59	116.82	97.93	35.57	198.08	81.25	137.25	8.37	26.50	21.66	4.24	48.76	22.26	39.03	1708


==> data/mlm_plots/tef/fakenews/cnn/s/time_misc_auc.tex <==
name	auc
attack_time	14.25
l2	26.08
lom	6.37


==> data/mlm_plots/tef/fakenews/cnn/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.69	0.75	0.76	0.65	0.85	0.10	0.82	0.84	0.87	0.89	0.81	0.94	0.07	0.92	0.90	0.92	0.94	0.88	0.97	0.05	0.96	967
0.03	0.60	0.67	0.67	0.56	0.78	0.11	0.73	0.77	0.81	0.82	0.75	0.88	0.06	0.85	0.86	0.89	0.90	0.84	0.94	0.05	0.92	1000
0.06	0.51	0.59	0.58	0.46	0.72	0.13	0.67	0.69	0.74	0.74	0.67	0.80	0.07	0.78	0.81	0.84	0.84	0.79	0.89	0.05	0.87	998
0.11	0.45	0.54	0.53	0.40	0.68	0.14	0.62	0.63	0.67	0.67	0.60	0.75	0.07	0.72	0.76	0.79	0.80	0.74	0.85	0.05	0.83	1007
0.15	0.38	0.46	0.44	0.32	0.60	0.14	0.53	0.54	0.59	0.58	0.52	0.67	0.07	0.63	0.70	0.73	0.73	0.68	0.78	0.05	0.76	1015
0.18	0.33	0.41	0.40	0.26	0.55	0.14	0.49	0.48	0.53	0.53	0.44	0.62	0.09	0.58	0.65	0.68	0.68	0.63	0.74	0.05	0.71	1014
0.32	0.22	0.32	0.31	0.16	0.48	0.16	0.41	0.39	0.45	0.45	0.35	0.55	0.10	0.50	0.57	0.61	0.61	0.55	0.68	0.07	0.65	1708


==> data/mlm_plots/tef/fakenews/cnn/s/top_intersections_auc.tex <==
name	auc
top10	0.15
top30	0.19
top50	0.23


==> data/mlm_plots/tef/fakenews/lstm/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	34.69	47.88	43.04	25.91	69.84	21.96	55.47	71.00	86.53	87.00	52.12	120.95	34.41	101.00	40.00	54.54	49.37	31.13	77.95	23.41	63.24	72.00	87.01	88.00	52.52	121.50	34.49	101.00	781
0.03	34.01	49.47	42.59	21.70	77.24	27.77	55.90	70.00	85.19	87.00	47.94	122.44	37.25	101.25	45.86	63.58	56.19	33.08	94.07	30.49	72.71	71.00	86.29	89.00	48.78	123.79	37.50	102.00	1008
0.06	34.18	52.91	42.73	10.81	95.00	42.09	56.34	67.00	83.59	87.00	44.84	122.33	38.75	101.00	58.01	81.26	69.60	31.75	130.77	49.51	88.70	70.00	85.85	91.00	46.63	125.08	39.23	103.00	1014
0.11	34.19	55.61	42.85	-0.76	111.98	56.37	56.96	67.00	82.87	86.00	43.59	122.15	39.28	100.00	70.54	99.26	84.10	30.24	168.28	69.02	104.98	69.00	86.17	91.00	46.22	126.12	39.95	105.00	1024
0.15	34.28	56.35	42.87	3.11	109.59	53.24	57.01	67.00	83.19	87.00	43.83	122.55	39.36	101.00	97.02	131.81	113.29	50.82	212.80	80.99	138.37	72.00	88.54	94.00	47.95	129.14	40.60	108.00	1002
0.18	34.23	55.97	42.84	0.46	111.48	55.51	56.98	67.00	82.70	86.00	43.73	121.67	38.97	100.00	128.28	167.96	148.88	72.79	263.14	95.17	177.54	74.00	90.24	96.00	49.55	130.92	40.68	110.00	1003
0.32	34.37	56.59	42.84	-0.13	113.30	56.72	56.91	67.00	81.76	86.00	44.04	119.49	37.73	100.00	177.03	243.93	214.75	123.57	364.29	120.36	275.92	77.00	92.69	100.00	52.39	132.98	40.30	113.00	1541


==> data/mlm_plots/tef/fakenews/lstm/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	17.06
orig_ge	25.78
adv_pp	45.69
adv_ge	27.64


==> data/mlm_plots/tef/fakenews/lstm/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.36	0.60	0.75	0.26	0.94	0.34	0.85	0.82	0.85	0.86	0.78	0.91	0.07	0.89	0.75	0.79	0.80	0.71	0.87	0.08	0.85	781
0.03	0.17	0.48	0.63	0.10	0.85	0.37	0.78	0.73	0.77	0.78	0.69	0.84	0.08	0.81	0.66	0.71	0.72	0.62	0.79	0.08	0.77	1008
0.06	0.11	0.42	0.55	0.05	0.79	0.37	0.70	0.63	0.67	0.68	0.59	0.76	0.09	0.73	0.56	0.61	0.62	0.53	0.69	0.08	0.67	1014
0.11	0.08	0.38	0.48	0.02	0.74	0.36	0.66	0.55	0.60	0.61	0.51	0.69	0.09	0.66	0.48	0.53	0.54	0.45	0.62	0.09	0.59	1024
0.15	0.06	0.33	0.42	-0.01	0.68	0.34	0.60	0.43	0.49	0.50	0.39	0.60	0.11	0.57	0.37	0.43	0.43	0.34	0.52	0.09	0.49	1002
0.18	0.05	0.30	0.37	-0.03	0.64	0.34	0.56	0.33	0.42	0.42	0.30	0.53	0.12	0.50	0.28	0.35	0.35	0.25	0.45	0.10	0.42	1003
0.32	0.03	0.27	0.33	-0.06	0.60	0.33	0.52	0.24	0.33	0.34	0.19	0.47	0.14	0.43	0.19	0.27	0.27	0.16	0.38	0.11	0.35	1541


==> data/mlm_plots/tef/fakenews/lstm/ig/correlations_auc.tex <==
name	auc
pcc	0.11
spearman	0.16
kendall	0.14


==> data/mlm_plots/tef/fakenews/lstm/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.17	11.45	6.25	-0.57	23.47	12.02	15.80	2.73	10.87	5.65	-1.03	22.78	11.90	15.72	2.29	6.69	4.39	-0.37	13.75	7.06	8.44	781
0.03	2.66	9.13	5.19	-0.64	18.89	9.76	12.14	2.40	8.39	4.77	-0.71	17.49	9.10	11.21	2.33	6.46	4.47	-0.32	13.23	6.78	7.90	1008
0.06	2.02	4.98	3.53	0.66	9.30	4.32	6.75	1.86	4.63	3.27	0.54	8.72	4.09	6.42	1.97	4.46	3.38	0.62	8.30	3.84	5.78	1014
0.11	1.73	3.51	2.74	0.92	6.10	2.59	4.75	1.62	3.29	2.58	0.85	5.72	2.44	4.40	1.74	3.47	2.82	0.72	6.21	2.75	4.50	1024
0.15	1.44	2.48	2.09	1.03	3.92	1.44	3.33	1.34	2.33	1.99	0.97	3.69	1.36	3.10	1.46	2.55	2.23	0.91	4.18	1.64	3.22	1002
0.18	1.24	2.01	1.77	0.96	3.06	1.05	2.65	1.17	1.90	1.67	0.90	2.91	1.00	2.51	1.28	2.08	1.89	0.89	3.27	1.19	2.64	1003
0.32	1.03	1.63	1.47	0.82	2.44	0.81	2.10	1.01	1.57	1.41	0.79	2.35	0.78	2.03	1.05	1.64	1.51	0.78	2.50	0.86	2.08	1541


==> data/mlm_plots/tef/fakenews/lstm/ig/ets_sts_auc.tex <==
name	auc
et_use	1.07
et_tse	1.01
et_ce	0.94


==> data/mlm_plots/tef/fakenews/lstm/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.48	2.08	0.91	-8.40	12.57	10.49	2.24	1.50	5.86	2.91	-0.93	12.65	6.79	8.39	1.17	5.25	2.44	-1.38	11.87	6.62	6.85	781
0.03	0.36	0.94	0.65	-0.10	1.98	1.04	1.36	1.63	4.45	2.96	0.73	8.17	3.72	6.78	1.27	3.77	2.55	0.39	7.14	3.37	5.61	1008
0.06	0.24	0.52	0.40	0.10	0.94	0.42	0.73	1.59	3.48	2.67	1.07	5.90	2.41	5.11	1.26	2.96	2.27	0.68	5.25	2.28	4.28	1014
0.11	0.19	0.38	0.30	-0.31	1.07	0.69	0.49	1.61	3.06	2.50	1.18	4.94	1.88	4.31	1.28	2.59	2.07	0.72	4.46	1.87	3.61	1024
0.15	0.13	0.23	0.20	0.03	0.43	0.20	0.29	1.57	2.68	2.35	1.24	4.12	1.44	3.69	1.26	2.35	1.94	-0.10	4.80	2.45	3.05	1002
0.18	0.10	0.16	0.14	0.07	0.25	0.09	0.20	1.51	2.42	2.18	1.18	3.66	1.24	3.18	1.20	2.07	1.81	0.49	3.64	1.58	2.64	1003
0.32	0.06	0.10	0.09	0.04	0.17	0.07	0.13	1.43	2.17	2.00	1.07	3.27	1.10	2.81	1.15	1.91	1.66	-0.41	4.23	2.32	2.35	1541


==> data/mlm_plots/tef/fakenews/lstm/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.11
et_p_h	0.90
et_p_l2	0.77


==> data/mlm_plots/tef/fakenews/lstm/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.11	0.15	0.14	0.09	0.21	0.06	0.18	0.03	0.06	0.05	0.03	0.09	0.03	0.08	0.03	0.05	0.04	0.03	0.07	0.02	0.06	781
0.03	0.25	0.32	0.32	0.21	0.42	0.11	0.39	0.06	0.09	0.08	0.05	0.12	0.04	0.10	0.05	0.07	0.07	0.05	0.09	0.02	0.08	1008
0.06	0.51	0.62	0.62	0.42	0.82	0.20	0.73	0.09	0.11	0.11	0.07	0.15	0.04	0.14	0.08	0.09	0.09	0.07	0.12	0.03	0.10	1014
0.11	0.77	0.94	0.95	0.64	1.24	0.30	1.12	0.11	0.13	0.13	0.09	0.18	0.04	0.16	0.09	0.11	0.11	0.08	0.13	0.03	0.12	1024
0.15	1.32	1.60	1.60	1.09	2.11	0.51	1.90	0.13	0.16	0.16	0.11	0.21	0.05	0.18	0.11	0.13	0.13	0.10	0.16	0.03	0.15	1002
0.18	1.93	2.41	2.42	1.60	3.21	0.81	2.89	0.16	0.18	0.18	0.13	0.23	0.05	0.21	0.13	0.15	0.15	0.12	0.18	0.03	0.17	1003
0.32	2.93	4.07	3.84	2.35	5.80	1.73	4.96	0.18	0.21	0.21	0.16	0.27	0.05	0.24	0.16	0.17	0.17	0.14	0.21	0.04	0.19	1541


==> data/mlm_plots/tef/fakenews/lstm/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.62
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/lstm/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.98	0.98	0.97	0.99	0.01	0.99	0.97	0.98	0.98	0.96	0.99	0.01	0.98	0.95	0.96	0.97	0.94	0.98	0.02	0.98	781
0.03	0.95	0.96	0.96	0.95	0.98	0.02	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.93	0.95	0.95	0.92	0.98	0.03	0.97	1008
0.06	0.92	0.93	0.93	0.91	0.95	0.02	0.95	0.91	0.92	0.93	0.90	0.95	0.03	0.94	0.90	0.92	0.93	0.88	0.96	0.04	0.95	1014
0.11	0.89	0.90	0.90	0.88	0.93	0.03	0.92	0.88	0.89	0.90	0.86	0.92	0.03	0.92	0.87	0.89	0.90	0.85	0.94	0.05	0.93	1024
0.15	0.84	0.86	0.86	0.83	0.89	0.03	0.88	0.83	0.85	0.85	0.82	0.88	0.03	0.87	0.82	0.86	0.86	0.80	0.91	0.05	0.89	1002
0.18	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.79	0.81	0.81	0.78	0.85	0.03	0.83	0.79	0.82	0.82	0.76	0.87	0.05	0.86	1003
0.32	0.74	0.77	0.77	0.73	0.81	0.04	0.79	0.73	0.76	0.76	0.72	0.80	0.04	0.79	0.72	0.76	0.77	0.69	0.83	0.07	0.81	1541


==> data/mlm_plots/tef/fakenews/lstm/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.26


==> data/mlm_plots/tef/fakenews/lstm/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	16.67	17.32	17.22	16.02	18.63	1.30	18.34	1.44	3.70	2.45	0.80	6.61	2.91	5.76	2.85	9.87	6.82	-0.02	19.75	9.89	13.53	781
0.03	21.19	22.27	22.36	20.28	24.25	1.98	23.50	1.85	4.44	3.28	1.14	7.74	3.30	6.54	3.38	11.54	8.07	0.02	23.07	11.52	16.00	1008
0.06	27.28	29.16	29.27	26.79	31.53	2.37	31.01	2.12	4.74	3.61	1.34	8.15	3.40	6.80	4.27	13.88	9.87	0.47	27.29	13.41	19.25	1014
0.11	33.92	36.09	36.43	32.83	39.34	3.26	37.73	2.35	4.97	3.86	1.45	8.48	3.52	7.01	4.39	15.15	11.12	0.99	29.31	14.16	21.31	1024
0.15	45.94	51.26	51.81	45.05	57.46	6.20	55.53	2.56	5.34	4.39	1.48	9.21	3.87	7.26	4.89	17.08	12.18	1.02	33.13	16.06	24.97	1002
0.18	59.89	64.36	64.93	57.41	71.31	6.95	69.02	2.76	5.67	4.75	1.12	10.22	4.55	7.51	5.17	18.00	12.91	0.82	35.18	17.18	26.27	1003
0.32	75.79	86.09	83.45	72.81	99.38	13.29	98.69	3.02	6.38	5.23	-0.53	13.28	6.91	7.80	5.50	19.75	14.43	0.43	39.08	19.33	28.20	1541


==> data/mlm_plots/tef/fakenews/lstm/ig/time_misc_auc.tex <==
name	auc
attack_time	16.79
l2	1.68
lom	5.14


==> data/mlm_plots/tef/fakenews/lstm/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.73	0.78	0.80	0.68	0.87	0.09	0.84	0.85	0.88	0.88	0.82	0.93	0.06	0.92	0.89	0.91	0.92	0.87	0.96	0.04	0.94	781
0.03	0.62	0.69	0.71	0.58	0.79	0.11	0.76	0.80	0.83	0.84	0.77	0.89	0.06	0.87	0.85	0.88	0.89	0.83	0.92	0.05	0.91	1008
0.06	0.53	0.61	0.62	0.49	0.72	0.12	0.67	0.73	0.77	0.77	0.71	0.83	0.06	0.81	0.81	0.84	0.84	0.79	0.88	0.05	0.87	1014
0.11	0.47	0.55	0.56	0.42	0.68	0.13	0.62	0.69	0.72	0.72	0.66	0.78	0.06	0.76	0.77	0.80	0.81	0.75	0.85	0.05	0.84	1024
0.15	0.42	0.50	0.50	0.37	0.63	0.13	0.58	0.61	0.65	0.66	0.58	0.73	0.07	0.71	0.72	0.75	0.76	0.71	0.80	0.05	0.79	1002
0.18	0.38	0.47	0.45	0.33	0.60	0.13	0.53	0.54	0.60	0.60	0.52	0.68	0.08	0.66	0.68	0.71	0.71	0.66	0.77	0.05	0.75	1003
0.32	0.33	0.43	0.42	0.28	0.57	0.14	0.50	0.48	0.54	0.54	0.45	0.63	0.09	0.60	0.62	0.66	0.66	0.60	0.72	0.06	0.70	1541


==> data/mlm_plots/tef/fakenews/lstm/ig/top_intersections_auc.tex <==
name	auc
top10	0.16
top30	0.20
top50	0.23


==> data/mlm_plots/tef/fakenews/lstm/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	34.56	47.62	42.66	25.89	69.35	21.73	55.23	73.00	88.59	89.00	52.19	125.00	36.41	102.00	40.75	55.02	49.86	31.37	78.67	23.65	63.26	73.00	89.30	89.00	52.82	125.79	36.49	103.00	876
0.03	34.00	49.15	42.52	22.01	76.29	27.14	55.55	70.00	85.17	87.00	48.28	122.06	36.89	101.75	46.82	64.91	57.28	33.45	96.38	31.46	73.53	72.00	86.63	89.00	49.49	123.77	37.14	103.00	1014
0.06	34.18	52.76	42.75	10.80	94.72	41.96	56.33	68.00	83.89	87.00	45.40	122.38	38.49	101.00	59.13	84.48	72.17	29.94	139.02	54.54	92.04	71.00	86.59	90.00	47.62	125.57	38.97	104.00	1011
0.11	34.19	55.49	42.84	-10.87	121.85	66.36	56.91	67.00	83.14	86.00	44.11	122.18	39.04	100.00	72.09	104.83	87.46	21.13	188.53	83.70	111.90	71.00	87.02	91.00	47.20	126.84	39.82	105.00	1021
0.15	34.26	55.61	42.85	4.17	107.05	51.44	56.91	67.00	83.06	86.00	44.20	121.93	38.87	100.00	99.19	139.23	118.97	32.15	246.32	107.08	146.65	73.00	89.20	93.50	48.95	129.44	40.24	107.00	1000
0.18	34.31	60.29	42.94	-36.75	157.32	97.04	57.35	66.00	82.70	86.00	43.14	122.27	39.56	100.00	132.84	180.20	157.90	67.81	292.59	112.39	190.08	75.00	91.08	96.00	49.50	132.66	41.58	111.00	1005
0.32	34.39	57.18	42.87	-5.59	119.95	62.77	57.20	67.00	82.03	86.00	43.54	120.53	38.49	100.00	186.10	261.30	228.60	112.69	409.91	148.61	291.57	79.00	94.19	101.00	52.91	135.47	41.28	115.00	1654


==> data/mlm_plots/tef/fakenews/lstm/s/comparison_vals_auc.tex <==
name	auc
orig_pp	17.41
orig_ge	25.84
adv_pp	48.61
adv_ge	27.93


==> data/mlm_plots/tef/fakenews/lstm/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.30	0.43	0.43	0.26	0.60	0.17	0.54	0.84	0.88	0.89	0.79	0.96	0.08	0.94	0.70	0.77	0.78	0.65	0.88	0.11	0.85	876
0.03	0.21	0.34	0.32	0.17	0.50	0.16	0.43	0.78	0.83	0.85	0.74	0.93	0.10	0.90	0.64	0.71	0.72	0.59	0.82	0.12	0.79	1014
0.06	0.15	0.27	0.23	0.11	0.42	0.15	0.34	0.71	0.76	0.78	0.66	0.87	0.10	0.84	0.55	0.62	0.63	0.51	0.73	0.11	0.70	1011
0.11	0.12	0.22	0.19	0.08	0.36	0.14	0.29	0.64	0.70	0.71	0.59	0.81	0.11	0.77	0.49	0.55	0.56	0.44	0.66	0.11	0.62	1021
0.15	0.07	0.17	0.13	0.04	0.30	0.13	0.23	0.51	0.59	0.60	0.46	0.71	0.13	0.67	0.38	0.44	0.45	0.34	0.55	0.11	0.51	1000
0.18	0.04	0.13	0.10	0.00	0.26	0.13	0.18	0.41	0.48	0.49	0.35	0.61	0.13	0.57	0.29	0.35	0.35	0.25	0.45	0.10	0.42	1005
0.32	-0.00	0.08	0.05	-0.04	0.21	0.12	0.13	0.22	0.33	0.34	0.16	0.49	0.17	0.44	0.15	0.23	0.23	0.11	0.35	0.12	0.31	1654


==> data/mlm_plots/tef/fakenews/lstm/s/correlations_auc.tex <==
name	auc
pcc	0.06
spearman	0.18
kendall	0.14


==> data/mlm_plots/tef/fakenews/lstm/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	8.47	13.22	11.86	6.87	19.57	6.35	16.79	7.70	12.52	11.00	6.01	19.03	6.51	16.12	5.64	9.58	8.19	3.98	15.18	5.60	12.53	876
0.03	6.21	9.46	8.37	4.54	14.37	4.92	11.48	5.71	8.88	7.76	4.03	13.72	4.85	10.71	4.93	8.08	7.10	3.45	12.72	4.64	10.19	1014
0.06	4.44	6.00	5.50	3.44	8.57	2.57	6.98	4.16	5.63	5.16	3.26	8.00	2.37	6.63	3.84	6.09	5.24	2.68	9.50	3.41	7.40	1011
0.11	3.49	4.50	4.23	2.87	6.14	1.64	5.25	3.26	4.24	4.00	2.74	5.74	1.50	4.97	3.28	4.88	4.24	2.21	7.54	2.66	5.81	1021
0.15	2.66	3.24	3.11	2.24	4.24	1.00	3.65	2.51	3.07	2.94	2.14	4.00	0.93	3.49	2.57	3.59	3.27	1.93	5.24	1.66	4.18	1000
0.18	2.20	2.58	2.51	1.89	3.26	0.68	2.90	2.11	2.46	2.40	1.81	3.11	0.65	2.77	2.12	2.85	2.66	1.71	3.99	1.14	3.36	1005
0.32	1.77	2.06	2.00	1.56	2.57	0.50	2.30	1.71	1.99	1.94	1.51	2.48	0.49	2.21	1.68	2.18	2.03	1.33	3.03	0.85	2.49	1654


==> data/mlm_plots/tef/fakenews/lstm/s/ets_sts_auc.tex <==
name	auc
et_use	1.29
et_tse	1.22
et_ce	1.28


==> data/mlm_plots/tef/fakenews/lstm/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.28	2.20	1.78	-1.91	6.32	4.12	2.42	4.12	6.88	6.00	2.80	10.97	4.09	8.42	3.30	6.14	4.95	1.39	10.88	4.74	7.51	876
0.03	0.76	1.07	0.99	0.24	1.90	0.83	1.23	3.66	5.14	4.88	2.78	7.50	2.36	6.19	2.86	4.40	3.97	1.61	7.20	2.80	5.16	1014
0.06	0.45	0.64	0.56	-0.65	1.94	1.29	0.69	3.28	4.23	4.02	2.27	6.19	1.96	4.88	2.54	3.65	3.27	0.64	6.65	3.01	4.10	1011
0.11	0.32	0.43	0.39	0.15	0.71	0.28	0.47	2.99	3.73	3.61	2.15	5.31	1.58	4.20	2.34	3.38	2.90	-3.09	9.86	6.47	3.54	1021
0.15	0.21	0.28	0.24	0.04	0.53	0.24	0.30	2.72	3.37	3.17	1.74	5.01	1.64	3.63	2.14	3.13	2.59	-1.11	7.36	4.23	3.06	1000
0.18	0.14	0.20	0.17	0.05	0.35	0.15	0.21	2.52	3.09	2.89	1.20	4.98	1.89	3.27	2.00	3.01	2.37	-4.43	10.46	7.44	2.73	1005
0.32	0.08	0.13	0.11	0.02	0.25	0.11	0.14	2.31	2.80	2.60	0.85	4.74	1.94	2.93	1.86	2.82	2.13	-7.04	12.68	9.86	2.44	1654


==> data/mlm_plots/tef/fakenews/lstm/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.13
et_p_h	1.11
et_p_l2	1.03


==> data/mlm_plots/tef/fakenews/lstm/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.13	0.16	0.16	0.11	0.22	0.06	0.20	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.06	876
0.03	0.28	0.35	0.35	0.25	0.45	0.10	0.41	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.06	0.07	0.07	0.05	0.09	0.02	0.08	1014
0.06	0.56	0.67	0.67	0.47	0.87	0.20	0.78	0.09	0.12	0.11	0.08	0.16	0.04	0.14	0.08	0.09	0.09	0.07	0.12	0.02	0.11	1011
0.11	0.85	1.02	1.02	0.72	1.33	0.31	1.19	0.11	0.14	0.14	0.10	0.18	0.04	0.16	0.10	0.11	0.11	0.08	0.14	0.03	0.13	1021
0.15	1.43	1.73	1.73	1.19	2.26	0.53	2.03	0.14	0.17	0.16	0.12	0.21	0.05	0.19	0.12	0.13	0.13	0.10	0.16	0.03	0.15	1000
0.18	2.13	2.58	2.61	1.75	3.42	0.84	3.09	0.16	0.19	0.19	0.14	0.24	0.05	0.21	0.14	0.15	0.15	0.12	0.19	0.03	0.17	1005
0.32	3.17	4.38	4.10	2.54	6.22	1.84	5.37	0.19	0.22	0.22	0.16	0.27	0.05	0.25	0.16	0.18	0.18	0.14	0.21	0.04	0.20	1654


==> data/mlm_plots/tef/fakenews/lstm/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.67
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/lstm/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.98	0.98	0.97	0.98	0.01	0.98	0.97	0.97	0.98	0.96	0.98	0.01	0.98	0.95	0.96	0.97	0.94	0.99	0.02	0.98	876
0.03	0.95	0.96	0.96	0.94	0.97	0.02	0.97	0.94	0.96	0.96	0.94	0.97	0.02	0.97	0.93	0.95	0.95	0.92	0.98	0.03	0.97	1014
0.06	0.92	0.93	0.93	0.91	0.95	0.02	0.95	0.91	0.93	0.93	0.90	0.95	0.02	0.94	0.91	0.93	0.93	0.89	0.96	0.03	0.95	1011
0.11	0.89	0.91	0.91	0.88	0.93	0.02	0.92	0.89	0.90	0.90	0.87	0.93	0.03	0.92	0.88	0.90	0.91	0.87	0.94	0.04	0.93	1021
0.15	0.85	0.86	0.86	0.84	0.89	0.03	0.88	0.84	0.86	0.86	0.83	0.89	0.03	0.88	0.84	0.87	0.87	0.82	0.91	0.05	0.90	1000
0.18	0.81	0.83	0.82	0.80	0.86	0.03	0.84	0.80	0.82	0.82	0.78	0.85	0.03	0.84	0.80	0.83	0.84	0.78	0.88	0.05	0.87	1005
0.32	0.74	0.77	0.77	0.73	0.81	0.04	0.80	0.73	0.76	0.76	0.72	0.80	0.04	0.79	0.73	0.77	0.77	0.70	0.84	0.07	0.81	1654


==> data/mlm_plots/tef/fakenews/lstm/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/fakenews/lstm/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	14.10	15.16	14.65	13.54	16.77	1.61	16.89	39.03	86.48	68.88	26.50	146.46	59.98	118.21	9.93	32.30	25.48	4.99	59.60	27.31	47.81	876
0.03	17.34	18.40	18.37	16.66	20.13	1.73	19.60	48.64	99.77	85.94	32.31	167.23	67.46	133.51	10.14	34.30	27.61	5.32	63.28	28.98	48.69	1014
0.06	25.27	26.54	26.90	24.20	28.87	2.33	27.75	55.72	112.06	97.44	33.61	190.51	78.45	146.58	12.06	36.55	28.80	6.35	66.76	30.21	54.29	1011
0.11	31.48	32.77	32.83	29.94	35.61	2.84	34.51	61.49	122.86	105.72	35.02	210.70	87.84	160.44	11.52	37.17	28.90	6.04	68.30	31.13	54.87	1021
0.15	42.99	45.47	45.25	41.14	49.80	4.33	48.30	70.45	140.57	117.74	38.81	242.33	101.76	183.76	11.88	37.62	29.19	6.03	69.20	31.59	57.28	1000
0.18	55.23	58.24	58.50	53.40	63.08	4.84	62.27	76.60	159.26	131.90	32.20	286.31	127.05	203.25	11.36	37.70	29.52	5.86	69.53	31.83	54.82	1005
0.32	67.39	79.70	76.38	64.93	94.48	14.78	92.63	87.10	193.25	152.30	18.31	368.20	174.94	242.05	13.10	41.18	32.47	6.84	75.52	34.34	61.85	1654


==> data/mlm_plots/tef/fakenews/lstm/s/time_misc_auc.tex <==
name	auc
attack_time	15.24
l2	45.34
lom	11.73


==> data/mlm_plots/tef/fakenews/lstm/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.53	0.62	0.64	0.48	0.77	0.14	0.73	0.77	0.82	0.83	0.73	0.91	0.09	0.89	0.85	0.89	0.90	0.83	0.95	0.06	0.94	876
0.03	0.44	0.53	0.55	0.39	0.67	0.14	0.62	0.72	0.77	0.79	0.68	0.87	0.09	0.84	0.83	0.87	0.88	0.80	0.93	0.06	0.91	1014
0.06	0.33	0.42	0.42	0.28	0.55	0.13	0.51	0.66	0.71	0.72	0.62	0.80	0.09	0.77	0.79	0.83	0.83	0.77	0.89	0.06	0.87	1011
0.11	0.26	0.34	0.33	0.21	0.47	0.13	0.42	0.60	0.65	0.66	0.56	0.74	0.09	0.71	0.76	0.79	0.80	0.73	0.86	0.06	0.84	1021
0.15	0.18	0.25	0.24	0.13	0.37	0.12	0.33	0.51	0.56	0.57	0.48	0.65	0.08	0.62	0.71	0.74	0.74	0.68	0.80	0.06	0.78	1000
0.18	0.12	0.20	0.20	0.08	0.33	0.12	0.27	0.44	0.49	0.50	0.41	0.57	0.08	0.55	0.66	0.69	0.69	0.63	0.75	0.06	0.73	1005
0.32	0.07	0.14	0.13	0.04	0.25	0.11	0.20	0.35	0.40	0.40	0.31	0.50	0.09	0.47	0.58	0.63	0.62	0.56	0.69	0.07	0.67	1654


==> data/mlm_plots/tef/fakenews/lstm/s/top_intersections_auc.tex <==
name	auc
top10	0.09
top30	0.18
top50	0.23


==> data/mlm_plots/tef/fakenews/lstmatt/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	34.63	47.62	42.73	25.86	69.39	21.76	54.71	73.00	88.50	89.00	52.63	124.37	35.87	102.00	39.99	54.09	48.70	30.93	77.25	23.16	61.79	74.00	89.00	89.00	53.09	124.91	35.91	102.00	836
0.03	34.04	48.67	41.81	21.05	76.28	27.61	54.60	72.00	86.37	89.00	51.16	121.59	35.21	102.00	45.83	62.45	55.50	32.59	92.30	29.86	70.00	73.00	87.60	90.00	52.20	123.00	35.40	103.00	995
0.06	34.18	51.85	41.99	11.21	92.48	40.64	55.81	69.00	84.58	88.00	47.77	121.39	36.81	102.00	56.98	79.61	69.36	31.55	127.67	48.06	86.84	72.00	87.25	91.00	50.01	124.48	37.23	104.00	1023
0.11	34.19	53.70	42.07	-10.51	117.90	64.21	55.95	69.00	84.47	88.00	47.20	121.74	37.27	102.00	68.88	96.38	83.49	27.71	165.05	68.67	102.32	74.00	88.57	93.00	50.60	126.54	37.97	106.00	997
0.15	34.18	52.28	42.03	11.88	92.69	40.40	55.94	70.00	84.55	88.00	47.36	121.74	37.19	102.00	94.21	126.15	112.98	56.41	195.89	69.74	135.50	78.00	91.47	96.00	52.93	130.01	38.54	110.00	998
0.18	34.20	54.25	42.22	-9.83	118.33	64.08	56.15	69.00	84.26	87.00	46.93	121.59	37.33	102.00	124.90	164.20	147.18	72.07	256.33	92.13	175.43	81.00	94.00	99.00	54.68	133.32	39.32	113.00	1003
0.32	34.21	55.16	42.52	-14.03	124.34	69.19	56.10	68.00	83.36	87.00	47.12	119.61	36.25	101.00	173.39	241.47	214.83	117.72	365.22	123.75	277.76	85.00	97.92	105.00	58.43	137.41	39.49	119.00	1722


==> data/mlm_plots/tef/fakenews/lstmatt/a/comparison_vals_auc.tex <==
name	auc
orig_pp	16.50
orig_ge	26.23
adv_pp	44.76
adv_ge	28.64


==> data/mlm_plots/tef/fakenews/lstmatt/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.32	0.58	0.69	0.27	0.89	0.31	0.83	0.92	0.92	0.96	0.81	1.03	0.11	0.98	0.78	0.83	0.88	0.68	0.97	0.15	0.92	836
0.03	0.14	0.44	0.48	0.15	0.74	0.30	0.69	0.86	0.88	0.93	0.75	1.01	0.13	0.96	0.70	0.77	0.82	0.61	0.92	0.15	0.87	995
0.06	0.10	0.38	0.38	0.10	0.65	0.27	0.58	0.82	0.85	0.89	0.73	0.97	0.12	0.93	0.66	0.72	0.76	0.58	0.86	0.14	0.82	1023
0.11	0.08	0.34	0.32	0.08	0.60	0.26	0.52	0.78	0.82	0.86	0.70	0.94	0.12	0.90	0.63	0.68	0.72	0.56	0.81	0.13	0.78	997
0.15	0.07	0.30	0.27	0.05	0.55	0.25	0.46	0.73	0.77	0.80	0.66	0.88	0.11	0.85	0.57	0.63	0.65	0.51	0.74	0.11	0.70	998
0.18	0.06	0.28	0.24	0.04	0.52	0.24	0.42	0.68	0.73	0.75	0.62	0.84	0.11	0.80	0.52	0.58	0.59	0.47	0.68	0.10	0.64	1003
0.32	0.04	0.26	0.22	0.02	0.50	0.24	0.39	0.58	0.65	0.67	0.54	0.77	0.12	0.73	0.43	0.50	0.51	0.40	0.61	0.11	0.57	1722


==> data/mlm_plots/tef/fakenews/lstmatt/a/correlations_auc.tex <==
name	auc
pcc	0.10
spearman	0.24
kendall	0.19


==> data/mlm_plots/tef/fakenews/lstmatt/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.20	10.90	6.51	0.39	21.40	10.51	16.28	3.00	9.84	6.08	0.48	19.20	9.36	15.27	2.40	6.64	4.93	0.70	12.58	5.94	8.88	836
0.03	3.39	8.10	6.30	1.66	14.54	6.44	11.01	3.10	7.36	5.84	1.60	13.11	5.75	10.17	2.88	6.20	4.89	1.43	10.98	4.77	8.04	995
0.06	2.83	4.94	4.41	1.87	8.00	3.06	6.38	2.56	4.56	4.09	1.74	7.38	2.82	6.06	2.63	4.47	3.87	1.62	7.31	2.85	5.78	1023
0.11	2.36	3.73	3.59	1.76	5.70	1.97	4.79	2.20	3.47	3.33	1.65	5.30	1.82	4.48	2.33	3.59	3.26	1.53	5.64	2.05	4.54	997
0.15	1.90	2.68	2.68	1.51	3.84	1.17	3.37	1.80	2.52	2.53	1.42	3.61	1.09	3.18	1.90	2.69	2.55	1.34	4.04	1.35	3.33	998
0.18	1.59	2.12	2.15	1.26	2.98	0.86	2.63	1.51	2.00	2.04	1.20	2.81	0.81	2.51	1.59	2.15	2.10	1.13	3.17	1.02	2.69	1003
0.32	1.27	1.65	1.66	1.00	2.29	0.65	2.04	1.19	1.58	1.60	0.96	2.19	0.62	1.96	1.20	1.63	1.59	0.92	2.34	0.71	2.01	1722


==> data/mlm_plots/tef/fakenews/lstmatt/a/ets_sts_auc.tex <==
name	auc
et_use	1.07
et_tse	0.99
et_ce	0.95


==> data/mlm_plots/tef/fakenews/lstmatt/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.56	1.88	1.14	-0.54	4.30	2.42	2.60	1.83	5.77	3.69	0.43	11.11	5.34	8.38	1.44	5.10	3.16	-0.15	10.35	5.25	7.29	836
0.03	0.50	0.98	0.87	0.36	1.60	0.62	1.35	2.38	4.71	4.11	1.62	7.79	3.08	6.74	1.87	4.01	3.38	0.84	7.18	3.17	5.53	995
0.06	0.35	0.59	0.53	-0.17	1.35	0.76	0.72	2.28	3.76	3.53	1.54	5.98	2.22	5.06	1.81	3.23	2.89	-0.05	6.51	3.28	4.19	1023
0.11	0.25	0.40	0.37	-0.10	0.90	0.50	0.48	2.17	3.26	3.21	1.51	5.02	1.76	4.25	1.74	2.80	2.62	-0.23	5.82	3.03	3.52	997
0.15	0.17	0.25	0.23	0.00	0.49	0.25	0.29	2.02	2.77	2.82	1.66	3.89	1.12	3.55	1.64	2.34	2.30	1.05	3.64	1.30	2.93	998
0.18	0.12	0.17	0.16	0.04	0.29	0.13	0.20	1.86	2.48	2.52	1.54	3.42	0.94	3.10	1.52	2.11	2.07	0.87	3.35	1.24	2.59	1003
0.32	0.07	0.11	0.09	-0.10	0.33	0.22	0.13	1.71	2.19	2.22	1.32	3.05	0.86	2.67	1.38	1.90	1.82	0.30	3.51	1.61	2.24	1722


==> data/mlm_plots/tef/fakenews/lstmatt/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.12
et_p_h	0.93
et_p_l2	0.80


==> data/mlm_plots/tef/fakenews/lstmatt/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.11	0.15	0.14	0.09	0.20	0.06	0.18	0.04	0.06	0.05	0.03	0.08	0.03	0.07	0.03	0.04	0.04	0.03	0.06	0.02	0.06	836
0.03	0.24	0.32	0.31	0.21	0.42	0.11	0.38	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.05	0.07	0.06	0.05	0.09	0.02	0.08	995
0.06	0.50	0.61	0.61	0.43	0.79	0.18	0.72	0.09	0.11	0.11	0.08	0.15	0.04	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.10	1023
0.11	0.78	0.93	0.94	0.66	1.21	0.27	1.10	0.11	0.13	0.13	0.09	0.17	0.04	0.15	0.09	0.11	0.11	0.08	0.13	0.03	0.12	997
0.15	1.33	1.60	1.61	1.13	2.08	0.48	1.90	0.14	0.16	0.16	0.12	0.20	0.04	0.18	0.12	0.13	0.13	0.10	0.16	0.03	0.15	998
0.18	1.96	2.41	2.41	1.66	3.15	0.75	2.87	0.16	0.18	0.18	0.14	0.23	0.05	0.21	0.14	0.15	0.15	0.12	0.18	0.03	0.17	1003
0.32	3.02	4.11	3.84	2.43	5.78	1.67	5.06	0.19	0.21	0.21	0.16	0.26	0.05	0.24	0.16	0.17	0.18	0.14	0.21	0.03	0.20	1722


==> data/mlm_plots/tef/fakenews/lstmatt/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.62
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/lstmatt/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.98	0.98	0.96	0.99	0.01	0.98	0.97	0.97	0.97	0.96	0.98	0.01	0.98	0.95	0.96	0.97	0.94	0.98	0.02	0.98	836
0.03	0.95	0.96	0.96	0.94	0.97	0.02	0.97	0.94	0.95	0.96	0.94	0.97	0.02	0.97	0.93	0.94	0.95	0.91	0.97	0.03	0.96	995
0.06	0.92	0.93	0.93	0.91	0.95	0.02	0.94	0.91	0.92	0.92	0.90	0.95	0.02	0.94	0.90	0.92	0.92	0.88	0.95	0.04	0.94	1023
0.11	0.89	0.90	0.90	0.88	0.93	0.03	0.92	0.88	0.90	0.90	0.87	0.92	0.03	0.91	0.87	0.89	0.90	0.85	0.94	0.04	0.92	997
0.15	0.84	0.86	0.86	0.83	0.89	0.03	0.88	0.83	0.85	0.85	0.82	0.89	0.03	0.87	0.83	0.86	0.86	0.81	0.90	0.05	0.89	998
0.18	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.79	0.81	0.81	0.78	0.85	0.03	0.83	0.78	0.82	0.82	0.77	0.87	0.05	0.86	1003
0.32	0.74	0.77	0.77	0.73	0.81	0.04	0.80	0.73	0.76	0.76	0.71	0.80	0.04	0.79	0.71	0.76	0.76	0.69	0.82	0.07	0.80	1722


==> data/mlm_plots/tef/fakenews/lstmatt/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.26


==> data/mlm_plots/tef/fakenews/lstmatt/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	14.16	14.63	14.77	13.79	15.48	0.84	15.17	0.21	0.39	0.31	0.15	0.64	0.24	0.53	15.93	70.50	43.73	2.61	138.38	67.88	116.22	836
0.03	21.33	22.32	22.25	20.30	24.33	2.01	23.51	0.29	0.47	0.41	0.24	0.71	0.23	0.65	22.54	84.08	60.37	11.68	156.48	72.40	137.36	995
0.06	24.13	25.49	25.41	23.10	27.88	2.39	26.77	0.34	0.51	0.46	0.29	0.73	0.22	0.67	24.20	89.19	70.63	15.13	163.26	74.07	144.55	1023
0.11	32.38	34.44	34.29	31.54	37.34	2.90	36.37	0.37	0.53	0.48	0.32	0.74	0.21	0.68	25.93	93.72	77.64	18.03	169.41	75.69	152.57	997
0.15	41.44	44.15	43.91	39.68	48.62	4.47	46.84	0.39	0.54	0.50	0.34	0.75	0.21	0.69	30.99	98.79	84.00	22.42	175.17	76.37	160.38	998
0.18	53.52	56.57	55.95	52.35	60.80	4.22	59.59	0.40	0.54	0.51	0.34	0.75	0.20	0.69	32.71	101.16	89.90	23.82	178.50	77.34	162.86	1003
0.32	64.96	76.07	72.87	62.95	89.19	13.12	88.36	0.38	0.53	0.49	0.33	0.74	0.20	0.68	33.36	103.28	92.28	26.87	179.69	76.41	168.95	1722


==> data/mlm_plots/tef/fakenews/lstmatt/a/time_misc_auc.tex <==
name	auc
attack_time	14.93
l2	0.16
lom	29.93


==> data/mlm_plots/tef/fakenews/lstmatt/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.73	0.82	0.87	0.68	0.96	0.14	0.91	0.85	0.89	0.92	0.79	0.98	0.09	0.95	0.89	0.91	0.94	0.84	0.99	0.08	0.97	836
0.03	0.64	0.75	0.80	0.60	0.90	0.15	0.87	0.80	0.85	0.88	0.75	0.95	0.10	0.92	0.86	0.89	0.91	0.81	0.97	0.08	0.94	995
0.06	0.60	0.70	0.73	0.56	0.85	0.15	0.82	0.77	0.82	0.84	0.73	0.91	0.09	0.88	0.84	0.87	0.89	0.79	0.94	0.07	0.92	1023
0.11	0.56	0.66	0.67	0.52	0.81	0.15	0.76	0.74	0.79	0.81	0.71	0.88	0.08	0.85	0.82	0.85	0.87	0.78	0.92	0.07	0.90	997
0.15	0.49	0.59	0.60	0.44	0.74	0.15	0.69	0.71	0.75	0.77	0.68	0.83	0.08	0.80	0.79	0.82	0.83	0.76	0.89	0.06	0.86	998
0.18	0.42	0.53	0.53	0.38	0.68	0.15	0.62	0.67	0.72	0.72	0.64	0.79	0.07	0.77	0.77	0.80	0.81	0.74	0.86	0.06	0.84	1003
0.32	0.36	0.45	0.44	0.30	0.60	0.15	0.53	0.61	0.66	0.66	0.58	0.74	0.08	0.71	0.72	0.76	0.77	0.70	0.82	0.06	0.80	1722


==> data/mlm_plots/tef/fakenews/lstmatt/a/top_intersections_auc.tex <==
name	auc
top10	0.18
top30	0.23
top50	0.26


==> data/mlm_plots/tef/fakenews/lstmatt/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	34.90	47.67	42.86	26.22	69.12	21.45	54.91	73.00	88.26	90.00	53.73	122.78	34.53	102.00	40.15	54.17	48.78	30.75	77.58	23.41	61.77	74.00	88.74	90.00	54.15	123.33	34.59	103.00	801
0.03	34.18	48.63	41.86	21.91	75.34	26.71	54.82	72.00	86.35	89.00	51.04	121.67	35.32	102.00	45.61	62.40	55.59	32.60	92.20	29.80	70.80	73.00	87.55	90.00	52.02	123.08	35.53	103.00	985
0.06	34.13	52.23	42.22	10.33	94.14	41.91	55.95	70.00	84.55	88.00	47.84	121.25	36.71	102.00	56.36	79.98	68.96	27.72	132.24	52.26	86.20	72.00	86.89	91.00	49.77	124.01	37.12	104.00	1025
0.11	34.19	54.47	42.15	-14.52	123.46	68.99	55.98	69.75	84.46	88.00	47.21	121.71	37.25	102.00	68.48	97.33	82.25	10.29	184.37	87.04	103.14	74.00	88.08	93.00	50.23	125.92	37.84	106.00	1004
0.15	34.17	51.83	42.03	13.90	89.76	37.93	55.90	70.00	84.78	88.00	47.87	121.70	36.91	102.00	93.49	124.30	110.37	53.00	195.60	71.30	133.58	78.00	90.70	95.00	52.87	128.53	37.83	108.00	1004
0.18	34.18	55.49	42.01	-14.93	125.91	70.42	55.98	68.00	83.76	88.00	46.90	120.62	36.86	101.00	122.90	162.56	143.71	65.40	259.71	97.15	171.04	79.00	92.13	98.00	53.77	130.48	38.36	111.00	881
0.32	34.70	56.45	42.96	-10.52	123.43	66.98	56.54	67.00	82.09	87.00	45.85	118.32	36.23	100.00	171.73	237.22	211.90	112.54	361.90	124.68	274.46	81.00	94.79	103.00	55.58	134.01	39.22	116.00	1288


==> data/mlm_plots/tef/fakenews/lstmatt/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	16.73
orig_ge	26.11
adv_pp	44.31
adv_ge	28.20


==> data/mlm_plots/tef/fakenews/lstmatt/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.53	0.70	0.81	0.42	0.97	0.28	0.91	0.67	0.76	0.82	0.59	0.93	0.17	0.89	0.57	0.68	0.74	0.51	0.85	0.17	0.81	801
0.03	0.42	0.59	0.67	0.27	0.90	0.31	0.83	0.59	0.68	0.72	0.51	0.85	0.17	0.81	0.50	0.60	0.63	0.44	0.76	0.16	0.72	985
0.06	0.35	0.52	0.59	0.20	0.84	0.32	0.76	0.53	0.61	0.65	0.45	0.78	0.16	0.72	0.45	0.53	0.56	0.38	0.68	0.15	0.64	1025
0.11	0.32	0.48	0.56	0.16	0.81	0.32	0.72	0.49	0.57	0.59	0.41	0.72	0.15	0.67	0.41	0.49	0.51	0.35	0.63	0.14	0.58	1004
0.15	0.29	0.45	0.51	0.12	0.77	0.33	0.67	0.43	0.51	0.53	0.36	0.66	0.15	0.61	0.36	0.43	0.45	0.31	0.56	0.13	0.52	1004
0.18	0.28	0.43	0.49	0.10	0.76	0.33	0.66	0.39	0.47	0.49	0.32	0.62	0.15	0.57	0.33	0.39	0.41	0.27	0.52	0.12	0.47	881
0.32	0.27	0.42	0.48	0.09	0.74	0.33	0.64	0.35	0.44	0.45	0.29	0.58	0.14	0.53	0.28	0.35	0.36	0.23	0.47	0.12	0.43	1288


==> data/mlm_plots/tef/fakenews/lstmatt/ig/correlations_auc.tex <==
name	auc
pcc	0.15
spearman	0.16
kendall	0.14


==> data/mlm_plots/tef/fakenews/lstmatt/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	1.74	8.44	4.59	-0.78	17.66	9.22	12.74	1.58	7.84	4.31	-0.88	16.57	8.72	11.64	1.38	4.98	2.95	-0.50	10.45	5.47	6.57	801
0.03	2.11	7.33	4.70	-0.89	15.56	8.22	9.28	1.89	6.80	4.33	-0.72	14.32	7.52	8.76	1.78	4.97	3.39	-0.07	10.01	5.04	6.36	985
0.06	1.75	4.43	3.20	0.00	8.86	4.43	5.59	1.63	4.14	3.05	0.14	8.14	4.00	5.21	1.56	3.76	2.80	0.38	7.14	3.38	4.67	1025
0.11	1.53	3.17	2.45	0.49	5.84	2.67	3.97	1.38	3.00	2.37	0.54	5.45	2.45	3.75	1.38	2.92	2.29	0.56	5.28	2.36	3.73	1004
0.15	1.19	2.18	1.82	0.63	3.73	1.55	2.72	1.11	2.08	1.72	0.62	3.55	1.47	2.65	1.17	2.15	1.80	0.60	3.69	1.55	2.73	1004
0.18	0.97	1.69	1.47	0.59	2.80	1.11	2.09	0.91	1.62	1.40	0.55	2.69	1.07	2.05	0.95	1.69	1.49	0.58	2.81	1.11	2.14	881
0.32	0.76	1.32	1.12	0.46	2.18	0.86	1.64	0.73	1.27	1.07	0.43	2.11	0.84	1.58	0.75	1.30	1.12	0.49	2.11	0.81	1.65	1288


==> data/mlm_plots/tef/fakenews/lstmatt/ig/ets_sts_auc.tex <==
name	auc
et_use	0.90
et_tse	0.85
et_ce	0.77


==> data/mlm_plots/tef/fakenews/lstmatt/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.29	1.51	0.78	-1.84	4.85	3.34	1.82	0.99	4.46	2.37	-0.53	9.46	5.00	6.25	0.81	3.93	2.07	-0.64	8.50	4.57	5.45	801
0.03	0.29	0.75	0.57	0.09	1.41	0.66	1.04	1.34	3.58	2.71	0.47	6.69	3.11	4.98	1.06	3.06	2.24	0.16	5.96	2.90	4.27	985
0.06	0.21	0.44	0.35	0.01	0.88	0.43	0.58	1.40	2.91	2.34	0.73	5.09	2.18	3.84	1.13	2.48	2.01	0.21	4.75	2.27	3.25	1025
0.11	0.17	0.32	0.25	-0.29	0.94	0.62	0.39	1.37	2.56	2.16	0.87	4.25	1.69	3.30	1.11	2.17	1.79	0.30	4.04	1.87	2.79	1004
0.15	0.11	0.19	0.16	0.05	0.33	0.14	0.24	1.29	2.20	1.92	0.88	3.53	1.32	2.76	1.04	1.86	1.59	0.53	3.18	1.32	2.31	1004
0.18	0.07	0.13	0.11	0.03	0.24	0.11	0.16	1.18	1.97	1.72	0.82	3.13	1.15	2.49	0.96	1.69	1.43	0.42	2.96	1.27	2.11	881
0.32	0.05	0.10	0.07	-0.11	0.30	0.21	0.11	1.08	1.75	1.51	0.74	2.77	1.02	2.16	0.89	1.52	1.26	0.25	2.79	1.27	1.84	1288


==> data/mlm_plots/tef/fakenews/lstmatt/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.09
et_p_h	0.73
et_p_l2	0.63


==> data/mlm_plots/tef/fakenews/lstmatt/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.10	0.14	0.14	0.09	0.20	0.05	0.18	0.03	0.05	0.05	0.03	0.08	0.03	0.07	0.03	0.04	0.04	0.03	0.06	0.02	0.05	801
0.03	0.24	0.31	0.30	0.20	0.41	0.10	0.37	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.05	0.06	0.06	0.04	0.08	0.02	0.08	985
0.06	0.49	0.60	0.60	0.41	0.78	0.18	0.71	0.09	0.11	0.11	0.07	0.15	0.04	0.13	0.07	0.09	0.09	0.06	0.11	0.02	0.10	1025
0.11	0.77	0.92	0.91	0.64	1.19	0.27	1.07	0.11	0.13	0.13	0.09	0.17	0.04	0.15	0.09	0.11	0.10	0.08	0.13	0.03	0.12	1004
0.15	1.28	1.57	1.57	1.10	2.03	0.46	1.84	0.14	0.16	0.16	0.12	0.20	0.04	0.18	0.12	0.13	0.13	0.10	0.16	0.03	0.14	1004
0.18	1.92	2.35	2.32	1.61	3.08	0.74	2.80	0.16	0.18	0.18	0.14	0.23	0.05	0.21	0.13	0.15	0.15	0.12	0.18	0.03	0.16	881
0.32	2.81	3.95	3.69	2.25	5.64	1.69	4.81	0.18	0.21	0.21	0.16	0.26	0.05	0.24	0.15	0.17	0.17	0.14	0.21	0.03	0.19	1288


==> data/mlm_plots/tef/fakenews/lstmatt/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.60
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/lstmatt/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.98	0.98	0.97	0.99	0.01	0.98	0.97	0.97	0.98	0.96	0.99	0.01	0.98	0.95	0.96	0.97	0.94	0.99	0.03	0.98	801
0.03	0.95	0.96	0.96	0.95	0.98	0.02	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.93	0.95	0.95	0.92	0.98	0.03	0.97	985
0.06	0.92	0.93	0.94	0.91	0.96	0.02	0.95	0.92	0.93	0.93	0.90	0.95	0.03	0.95	0.90	0.92	0.93	0.88	0.96	0.04	0.95	1025
0.11	0.89	0.91	0.91	0.88	0.93	0.03	0.93	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.87	0.90	0.90	0.85	0.94	0.05	0.93	1004
0.15	0.84	0.86	0.86	0.83	0.89	0.03	0.88	0.83	0.86	0.86	0.82	0.89	0.03	0.88	0.82	0.85	0.86	0.80	0.91	0.05	0.89	1004
0.18	0.80	0.82	0.82	0.79	0.86	0.03	0.84	0.79	0.81	0.82	0.78	0.85	0.03	0.84	0.78	0.82	0.82	0.76	0.87	0.06	0.86	881
0.32	0.74	0.77	0.77	0.73	0.81	0.04	0.79	0.73	0.76	0.76	0.72	0.80	0.04	0.79	0.71	0.76	0.76	0.69	0.83	0.07	0.80	1288


==> data/mlm_plots/tef/fakenews/lstmatt/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.26


==> data/mlm_plots/tef/fakenews/lstmatt/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	19.05	20.46	20.80	18.88	22.03	1.57	21.44	0.75	8.70	1.46	-14.74	32.15	23.44	5.50	6.87	25.93	16.11	-1.52	53.38	27.45	35.60	801
0.03	24.00	25.74	25.35	23.24	28.24	2.50	26.88	1.17	13.04	2.15	-57.08	83.15	70.12	6.45	8.64	29.74	21.95	0.92	58.56	28.82	41.13	985
0.06	32.42	35.36	35.25	31.15	39.56	4.20	37.33	1.46	22.54	2.43	-171.36	216.44	193.90	6.83	9.59	33.44	24.61	1.61	65.27	31.83	48.16	1025
0.11	41.32	44.51	44.36	39.75	49.27	4.76	46.38	1.65	21.38	2.63	-169.65	212.40	191.02	7.03	9.96	35.40	26.50	1.85	68.96	33.56	51.30	1004
0.15	54.32	57.38	55.96	51.39	63.37	5.99	61.97	1.82	14.62	2.83	-29.37	58.61	43.99	7.49	11.84	37.86	28.20	2.14	73.58	35.72	54.49	1004
0.18	67.73	75.95	76.19	67.03	84.86	8.91	82.12	1.89	15.99	2.94	-35.81	67.80	51.80	7.76	12.37	39.52	30.48	1.73	77.32	37.79	56.49	881
0.32	89.83	102.63	96.77	84.47	120.79	18.16	112.62	2.02	15.14	3.04	-35.48	65.76	50.62	7.76	12.16	40.56	31.86	1.30	79.82	39.26	56.80	1288


==> data/mlm_plots/tef/fakenews/lstmatt/ig/time_misc_auc.tex <==
name	auc
attack_time	19.87
l2	5.19
lom	11.48


==> data/mlm_plots/tef/fakenews/lstmatt/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.64	0.73	0.76	0.59	0.87	0.14	0.84	0.73	0.80	0.83	0.69	0.91	0.11	0.88	0.81	0.86	0.88	0.77	0.94	0.08	0.92	801
0.03	0.56	0.66	0.67	0.52	0.79	0.13	0.76	0.69	0.75	0.76	0.65	0.85	0.10	0.82	0.77	0.82	0.83	0.74	0.90	0.08	0.88	985
0.06	0.51	0.60	0.61	0.47	0.74	0.13	0.69	0.65	0.71	0.72	0.61	0.81	0.10	0.78	0.75	0.79	0.80	0.71	0.87	0.08	0.85	1025
0.11	0.49	0.57	0.58	0.44	0.71	0.14	0.67	0.63	0.68	0.69	0.59	0.78	0.09	0.74	0.73	0.77	0.78	0.69	0.85	0.08	0.82	1004
0.15	0.47	0.55	0.56	0.41	0.68	0.14	0.62	0.59	0.64	0.65	0.55	0.73	0.09	0.70	0.70	0.74	0.75	0.67	0.81	0.07	0.79	1004
0.18	0.44	0.54	0.53	0.40	0.68	0.14	0.62	0.56	0.61	0.62	0.52	0.71	0.09	0.67	0.68	0.72	0.73	0.65	0.79	0.07	0.77	881
0.32	0.42	0.52	0.53	0.38	0.67	0.15	0.60	0.53	0.59	0.59	0.49	0.68	0.09	0.64	0.66	0.69	0.70	0.63	0.76	0.07	0.74	1288


==> data/mlm_plots/tef/fakenews/lstmatt/ig/top_intersections_auc.tex <==
name	auc
top10	0.18
top30	0.20
top50	0.23


==> data/mlm_plots/tef/fakenews/lstmatt/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	34.65	47.24	42.47	26.10	68.38	21.14	54.04	74.00	88.45	90.00	54.16	122.74	34.29	102.00	40.06	53.98	48.89	31.20	76.77	22.78	62.04	74.00	88.95	90.00	54.64	123.25	34.31	102.00	838
0.03	34.04	48.54	41.84	21.93	75.15	26.61	54.75	72.00	86.43	89.00	51.18	121.68	35.25	102.00	45.93	62.94	56.00	32.62	93.27	30.33	71.03	73.00	87.61	90.00	52.21	123.01	35.40	103.00	991
0.06	34.19	52.38	42.42	10.25	94.52	42.14	55.95	69.00	84.38	88.00	47.42	121.34	36.96	102.00	57.16	80.41	69.20	33.16	127.67	47.25	87.34	72.00	86.80	91.00	49.40	124.20	37.40	104.00	1029
0.11	34.08	53.77	41.96	2.01	105.52	51.75	56.07	68.50	84.13	87.00	46.96	121.30	37.17	102.00	69.43	96.80	83.42	31.70	161.89	65.09	103.50	73.00	87.82	92.00	49.99	125.66	37.83	105.00	1035
0.15	34.19	52.57	42.52	11.19	93.96	41.38	56.14	70.00	84.58	88.00	47.57	121.60	37.01	102.00	94.95	126.34	113.33	61.68	190.99	64.65	136.66	77.00	90.69	95.00	52.68	128.70	38.01	109.00	1017
0.18	34.21	54.93	42.07	-0.17	110.03	55.10	56.25	68.00	83.70	88.00	46.25	121.14	37.44	101.00	125.36	167.66	148.16	73.44	261.89	94.22	175.85	80.00	92.33	98.00	53.31	131.35	39.02	112.00	913
0.32	34.62	59.09	42.62	-25.61	143.80	84.71	56.41	67.00	82.15	87.00	45.76	118.55	36.39	101.00	176.08	250.16	220.17	115.57	384.75	134.59	283.04	82.00	94.79	102.00	55.54	134.04	39.25	116.00	1485


==> data/mlm_plots/tef/fakenews/lstmatt/s/comparison_vals_auc.tex <==
name	auc
orig_pp	16.85
orig_ge	26.08
adv_pp	45.70
adv_ge	28.20


==> data/mlm_plots/tef/fakenews/lstmatt/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.44	0.54	0.56	0.37	0.72	0.17	0.67	0.77	0.83	0.85	0.71	0.95	0.12	0.91	0.60	0.68	0.69	0.55	0.80	0.13	0.77	838
0.03	0.33	0.45	0.47	0.28	0.63	0.18	0.59	0.69	0.77	0.80	0.63	0.91	0.14	0.87	0.53	0.61	0.62	0.47	0.75	0.14	0.71	991
0.06	0.26	0.39	0.39	0.21	0.58	0.19	0.53	0.61	0.71	0.73	0.55	0.87	0.16	0.83	0.46	0.55	0.56	0.41	0.70	0.15	0.66	1029
0.11	0.21	0.36	0.35	0.17	0.55	0.19	0.49	0.57	0.67	0.70	0.50	0.84	0.17	0.80	0.42	0.51	0.52	0.37	0.66	0.15	0.62	1035
0.15	0.17	0.32	0.30	0.12	0.51	0.20	0.46	0.48	0.61	0.63	0.42	0.79	0.18	0.74	0.35	0.46	0.46	0.30	0.61	0.15	0.56	1017
0.18	0.13	0.29	0.28	0.09	0.49	0.20	0.43	0.41	0.53	0.55	0.33	0.73	0.20	0.67	0.29	0.39	0.39	0.24	0.55	0.15	0.50	913
0.32	0.09	0.26	0.24	0.05	0.46	0.21	0.40	0.25	0.41	0.42	0.17	0.65	0.24	0.58	0.18	0.30	0.30	0.12	0.48	0.18	0.42	1485


==> data/mlm_plots/tef/fakenews/lstmatt/s/correlations_auc.tex <==
name	auc
pcc	0.10
spearman	0.18
kendall	0.14


==> data/mlm_plots/tef/fakenews/lstmatt/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	6.75	11.87	10.07	4.88	18.85	6.99	15.43	5.96	10.65	9.04	4.43	16.88	6.22	14.26	4.20	7.73	6.47	2.81	12.65	4.92	10.09	838
0.03	5.03	8.20	7.05	3.41	13.00	4.79	9.94	4.60	7.48	6.42	3.25	11.71	4.23	9.19	3.68	6.33	5.47	2.52	10.14	3.81	8.02	991
0.06	3.40	5.14	4.71	2.55	7.73	2.59	6.30	3.14	4.80	4.40	2.39	7.22	2.42	5.96	2.79	4.70	4.09	1.99	7.42	2.72	5.85	1029
0.11	2.65	3.83	3.59	2.13	5.53	1.70	4.79	2.45	3.60	3.36	1.99	5.21	1.61	4.52	2.34	3.75	3.31	1.67	5.84	2.08	4.66	1035
0.15	1.95	2.70	2.61	1.63	3.76	1.07	3.30	1.84	2.56	2.46	1.55	3.58	1.02	3.14	1.86	2.77	2.49	1.31	4.23	1.46	3.38	1017
0.18	1.59	2.15	2.10	1.35	2.96	0.80	2.65	1.52	2.06	2.02	1.28	2.83	0.78	2.53	1.55	2.23	2.08	1.18	3.28	1.05	2.70	913
0.32	1.25	1.68	1.65	1.07	2.30	0.62	2.05	1.22	1.62	1.59	1.03	2.21	0.59	1.95	1.20	1.72	1.61	0.90	2.55	0.82	2.10	1485


==> data/mlm_plots/tef/fakenews/lstmatt/s/ets_sts_auc.tex <==
name	auc
et_use	1.10
et_tse	1.03
et_ce	1.00


==> data/mlm_plots/tef/fakenews/lstmatt/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.01	1.84	1.49	0.35	3.34	1.50	2.21	3.59	5.93	5.12	2.39	9.48	3.55	7.50	2.82	5.15	4.24	1.71	8.60	3.44	6.68	838
0.03	0.63	0.98	0.84	0.00	1.95	0.97	1.14	3.05	4.54	4.15	2.18	6.90	2.36	5.53	2.40	3.86	3.42	1.40	6.32	2.46	4.59	991
0.06	0.38	0.55	0.49	0.21	0.89	0.34	0.64	2.61	3.67	3.48	1.94	5.40	1.73	4.37	2.07	3.20	2.85	0.07	6.33	3.13	3.63	1029
0.11	0.26	0.38	0.35	0.15	0.60	0.23	0.44	2.35	3.23	3.05	1.71	4.75	1.52	3.86	1.86	2.98	2.49	-3.60	9.56	6.58	3.19	1035
0.15	0.16	0.24	0.21	0.05	0.43	0.19	0.28	2.04	2.75	2.65	1.47	4.04	1.28	3.27	1.65	2.46	2.16	-1.13	6.04	3.59	2.71	1017
0.18	0.11	0.17	0.15	-0.02	0.36	0.19	0.19	1.86	2.49	2.42	1.42	3.56	1.07	2.99	1.49	2.19	1.97	0.01	4.37	2.18	2.46	913
0.32	0.07	0.15	0.09	-0.78	1.09	0.93	0.12	1.71	2.28	2.17	1.00	3.57	1.29	2.66	1.38	2.20	1.78	-1.79	6.18	3.98	2.22	1485


==> data/mlm_plots/tef/fakenews/lstmatt/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.12
et_p_h	0.93
et_p_l2	0.84


==> data/mlm_plots/tef/fakenews/lstmatt/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.11	0.15	0.15	0.09	0.21	0.06	0.19	0.04	0.06	0.05	0.03	0.08	0.03	0.07	0.03	0.05	0.04	0.03	0.06	0.02	0.06	838
0.03	0.26	0.32	0.32	0.22	0.42	0.10	0.39	0.06	0.08	0.08	0.05	0.12	0.03	0.10	0.05	0.07	0.07	0.05	0.09	0.02	0.08	991
0.06	0.50	0.62	0.62	0.44	0.79	0.18	0.72	0.09	0.11	0.11	0.07	0.15	0.04	0.13	0.07	0.09	0.09	0.07	0.11	0.02	0.10	1029
0.11	0.78	0.94	0.95	0.68	1.20	0.26	1.10	0.11	0.13	0.13	0.09	0.17	0.04	0.15	0.09	0.11	0.11	0.08	0.13	0.03	0.12	1035
0.15	1.33	1.61	1.62	1.14	2.08	0.47	1.90	0.14	0.16	0.16	0.12	0.20	0.04	0.18	0.12	0.13	0.13	0.10	0.16	0.03	0.15	1017
0.18	2.03	2.44	2.44	1.70	3.18	0.74	2.90	0.16	0.18	0.18	0.14	0.23	0.05	0.21	0.13	0.15	0.15	0.12	0.18	0.03	0.17	913
0.32	3.04	4.15	3.93	2.45	5.85	1.70	5.15	0.19	0.21	0.21	0.16	0.27	0.05	0.24	0.16	0.17	0.18	0.14	0.21	0.04	0.19	1485


==> data/mlm_plots/tef/fakenews/lstmatt/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.63
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/lstmatt/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.98	0.98	0.97	0.99	0.01	0.98	0.97	0.97	0.98	0.96	0.99	0.01	0.98	0.95	0.96	0.97	0.94	0.99	0.02	0.98	838
0.03	0.95	0.96	0.96	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.97	0.02	0.97	0.93	0.95	0.95	0.92	0.97	0.03	0.97	991
0.06	0.92	0.93	0.94	0.91	0.95	0.02	0.95	0.92	0.93	0.93	0.91	0.95	0.02	0.94	0.90	0.92	0.93	0.89	0.96	0.03	0.95	1029
0.11	0.89	0.91	0.91	0.88	0.93	0.03	0.92	0.89	0.90	0.90	0.87	0.93	0.03	0.92	0.88	0.90	0.90	0.86	0.94	0.04	0.93	1035
0.15	0.85	0.87	0.87	0.84	0.89	0.03	0.88	0.84	0.86	0.86	0.83	0.89	0.03	0.88	0.83	0.86	0.86	0.81	0.91	0.05	0.89	1017
0.18	0.81	0.83	0.83	0.80	0.86	0.03	0.85	0.80	0.82	0.82	0.78	0.85	0.03	0.84	0.79	0.82	0.83	0.77	0.87	0.05	0.86	913
0.32	0.74	0.77	0.77	0.73	0.81	0.04	0.80	0.73	0.76	0.76	0.72	0.80	0.04	0.79	0.72	0.76	0.76	0.70	0.83	0.07	0.81	1485


==> data/mlm_plots/tef/fakenews/lstmatt/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.26
sts_ce	0.26


==> data/mlm_plots/tef/fakenews/lstmatt/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	16.64	17.55	17.63	16.19	18.92	1.37	18.36	23.59	212.20	46.84	-545.04	969.44	757.24	109.59	12.35	47.79	32.54	1.11	94.48	46.68	68.06	838
0.03	20.72	21.49	21.77	19.96	23.03	1.54	22.65	33.23	240.40	60.71	-579.81	1060.62	820.22	123.51	14.78	54.63	39.01	2.31	106.94	52.31	79.59	991
0.06	28.38	29.50	29.69	25.10	33.90	4.40	29.97	39.36	270.36	64.81	-913.11	1453.83	1183.47	127.97	15.26	59.37	41.74	2.79	115.94	56.58	88.11	1029
0.11	36.54	39.06	39.04	33.65	44.48	5.42	41.29	42.52	315.13	67.05	-2588.31	3218.56	2903.43	129.44	15.87	62.34	44.02	3.43	121.26	58.91	90.00	1035
0.15	48.23	52.49	52.69	46.13	58.85	6.36	54.89	47.33	656.90	76.05	-6759.22	8073.02	7416.12	140.17	17.67	66.52	46.58	4.20	128.84	62.32	95.26	1017
0.18	65.44	70.21	70.63	64.29	76.13	5.92	73.82	47.15	160.83	74.99	-261.57	583.23	422.40	125.81	18.92	69.13	49.79	5.43	132.83	63.70	101.53	913
0.32	81.28	88.67	86.98	77.54	99.81	11.13	96.98	48.78	308.13	75.30	-2957.44	3573.69	3265.56	126.30	18.13	71.33	53.73	5.58	137.09	65.76	103.62	1485


==> data/mlm_plots/tef/fakenews/lstmatt/s/time_misc_auc.tex <==
name	auc
attack_time	17.64
l2	93.31
lom	20.25


==> data/mlm_plots/tef/fakenews/lstmatt/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.53	0.62	0.64	0.47	0.78	0.16	0.73	0.70	0.76	0.77	0.66	0.87	0.10	0.83	0.80	0.84	0.85	0.77	0.91	0.07	0.89	838
0.03	0.44	0.55	0.56	0.38	0.72	0.17	0.67	0.64	0.71	0.72	0.60	0.82	0.11	0.79	0.76	0.81	0.82	0.73	0.89	0.08	0.86	991
0.06	0.36	0.48	0.49	0.30	0.66	0.18	0.60	0.59	0.67	0.67	0.55	0.78	0.12	0.75	0.73	0.78	0.78	0.70	0.86	0.08	0.83	1029
0.11	0.30	0.44	0.44	0.25	0.63	0.19	0.58	0.56	0.64	0.64	0.52	0.76	0.12	0.72	0.70	0.76	0.76	0.68	0.84	0.08	0.82	1035
0.15	0.24	0.40	0.39	0.20	0.59	0.20	0.53	0.51	0.59	0.60	0.47	0.72	0.12	0.68	0.67	0.73	0.73	0.64	0.81	0.08	0.79	1017
0.18	0.21	0.36	0.36	0.17	0.55	0.19	0.50	0.47	0.55	0.55	0.42	0.67	0.12	0.63	0.64	0.69	0.70	0.61	0.78	0.09	0.75	913
0.32	0.18	0.33	0.31	0.13	0.53	0.20	0.47	0.40	0.50	0.50	0.36	0.63	0.14	0.59	0.58	0.64	0.64	0.54	0.74	0.10	0.71	1485


==> data/mlm_plots/tef/fakenews/lstmatt/s/top_intersections_auc.tex <==
name	auc
top10	0.13
top30	0.18
top50	0.22


==> data/mlm_plots/tef/fakenews/roberta/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	31.98	43.12	39.19	24.68	61.55	18.43	49.93	30.00	38.28	37.00	23.43	53.13	14.85	45.00	36.49	48.36	43.86	28.36	68.36	20.00	56.37	30.00	38.65	38.00	23.79	53.51	14.86	46.00	656
0.03	31.42	43.60	38.74	20.88	66.32	22.72	49.69	30.00	38.37	38.00	22.39	54.36	15.98	46.00	40.42	54.67	48.96	28.90	80.45	25.77	62.07	30.00	39.16	39.00	23.14	55.19	16.02	46.00	967
0.06	31.11	45.02	38.92	16.28	73.76	28.74	50.05	29.00	37.59	37.00	20.90	54.27	16.68	46.00	48.59	67.09	59.30	30.61	103.57	36.48	74.46	31.00	39.16	39.00	22.39	55.93	16.77	47.25	1000
0.11	31.14	47.54	39.03	7.31	87.76	40.23	50.53	29.00	37.11	37.00	20.38	53.84	16.73	45.00	58.89	83.49	71.22	14.57	152.42	68.92	87.98	31.00	39.33	40.00	22.39	56.28	16.94	48.00	999
0.15	31.27	48.97	39.13	3.02	94.92	45.95	50.76	29.00	37.25	37.00	20.09	54.41	17.16	45.00	78.21	109.16	94.88	28.63	189.68	80.52	115.63	32.00	40.57	41.00	23.06	58.08	17.51	49.00	1016
0.18	31.09	52.57	39.33	-10.94	116.07	63.51	51.70	28.00	36.38	37.00	20.00	52.77	16.39	45.00	98.42	144.97	120.66	9.13	280.82	135.84	146.33	33.00	40.58	42.00	23.49	57.66	17.09	50.00	864
0.32	31.62	48.75	39.46	8.00	89.50	40.75	51.25	28.00	36.64	37.00	20.19	53.09	16.45	46.00	126.37	180.48	155.99	63.10	297.86	117.38	198.26	34.00	42.12	44.00	24.90	59.34	17.22	52.00	1337


==> data/mlm_plots/tef/fakenews/roberta/a/comparison_vals_auc.tex <==
name	auc
orig_pp	15.09
orig_ge	11.50
adv_pp	37.02
adv_ge	12.54


==> data/mlm_plots/tef/fakenews/roberta/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.60	0.73	0.74	0.56	0.90	0.17	0.88	0.97	0.98	0.99	0.94	1.01	0.04	0.99	0.87	0.90	0.92	0.84	0.96	0.06	0.93	656
0.03	0.50	0.63	0.63	0.45	0.82	0.19	0.79	0.95	0.96	0.97	0.92	1.00	0.04	0.98	0.83	0.86	0.88	0.81	0.92	0.06	0.90	967
0.06	0.43	0.57	0.57	0.38	0.77	0.20	0.73	0.93	0.94	0.95	0.89	0.99	0.05	0.97	0.79	0.82	0.84	0.76	0.89	0.06	0.87	1000
0.11	0.39	0.54	0.54	0.34	0.74	0.20	0.69	0.91	0.92	0.93	0.87	0.98	0.06	0.95	0.76	0.79	0.80	0.72	0.86	0.07	0.83	999
0.15	0.34	0.49	0.48	0.29	0.69	0.20	0.62	0.87	0.89	0.90	0.80	0.98	0.09	0.93	0.71	0.74	0.75	0.66	0.83	0.09	0.79	1016
0.18	0.31	0.45	0.44	0.25	0.66	0.21	0.58	0.85	0.87	0.88	0.78	0.96	0.09	0.91	0.68	0.71	0.72	0.62	0.80	0.09	0.76	864
0.32	0.25	0.41	0.40	0.21	0.61	0.20	0.53	0.83	0.85	0.86	0.77	0.93	0.08	0.89	0.65	0.68	0.69	0.61	0.76	0.08	0.72	1337


==> data/mlm_plots/tef/fakenews/roberta/a/correlations_auc.tex <==
name	auc
pcc	0.15
spearman	0.28
kendall	0.23


==> data/mlm_plots/tef/fakenews/roberta/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	2.97	7.86	6.20	1.71	14.00	6.15	11.25	2.68	7.66	6.20	1.55	13.78	6.12	11.49	1.86	4.72	3.60	0.72	8.71	3.99	6.34	656
0.03	3.03	6.41	5.34	1.63	11.19	4.78	8.53	2.89	6.33	5.37	1.56	11.09	4.77	8.39	2.36	4.79	4.08	1.41	8.18	3.39	6.38	967
0.06	2.07	3.86	3.47	1.47	6.25	2.39	5.22	2.09	3.84	3.37	1.41	6.27	2.43	5.18	2.12	3.85	3.39	1.38	6.32	2.47	4.98	1000
0.11	1.72	2.86	2.62	1.28	4.45	1.58	3.92	1.72	2.85	2.58	1.25	4.46	1.60	3.82	1.88	3.15	2.84	1.30	4.99	1.85	4.04	999
0.15	1.42	2.15	2.05	1.12	3.18	1.03	2.84	1.42	2.15	2.05	1.11	3.19	1.04	2.82	1.65	2.56	2.40	1.11	4.01	1.45	3.21	1016
0.18	1.27	1.83	1.74	1.00	2.66	0.83	2.38	1.26	1.84	1.76	0.98	2.69	0.85	2.38	1.48	2.17	2.06	1.11	3.23	1.06	2.73	864
0.32	1.20	1.65	1.59	0.98	2.31	0.66	2.09	1.21	1.66	1.59	0.97	2.36	0.69	2.12	1.36	1.96	1.88	1.07	2.86	0.89	2.46	1337


==> data/mlm_plots/tef/fakenews/roberta/a/ets_sts_auc.tex <==
name	auc
et_use	0.87
et_tse	0.86
et_ce	0.88


==> data/mlm_plots/tef/fakenews/roberta/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.46	1.55	1.06	-1.36	4.47	2.91	1.90	1.33	4.47	3.29	0.12	8.81	4.34	6.09	1.04	4.14	2.86	-0.32	8.60	4.46	5.56	656
0.03	0.37	0.79	0.68	0.12	1.46	0.67	1.05	1.54	3.41	2.93	0.95	5.86	2.45	4.61	1.20	2.95	2.39	0.47	5.42	2.48	3.90	967
0.06	0.26	0.45	0.41	0.14	0.76	0.31	0.60	1.49	2.65	2.51	1.14	4.16	1.51	3.57	1.15	2.20	2.01	0.79	3.62	1.41	2.94	1000
0.11	0.19	0.32	0.29	-0.11	0.76	0.43	0.41	1.50	2.35	2.27	1.19	3.50	1.16	3.12	1.15	1.93	1.84	0.87	2.99	1.06	2.54	999
0.15	0.13	0.20	0.19	0.09	0.31	0.11	0.26	1.47	2.13	2.08	1.13	3.12	1.00	2.71	1.15	1.78	1.68	0.47	3.09	1.31	2.24	1016
0.18	0.09	0.15	0.14	0.03	0.28	0.13	0.19	1.43	2.03	1.94	0.73	3.33	1.30	2.54	1.13	1.73	1.58	-0.69	4.15	2.42	2.11	864
0.32	0.07	0.12	0.11	0.01	0.23	0.11	0.14	1.43	1.92	1.90	1.20	2.65	0.72	2.40	1.11	1.58	1.53	0.87	2.29	0.71	1.96	1337


==> data/mlm_plots/tef/fakenews/roberta/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.10
et_p_h	0.72
et_p_l2	0.61


==> data/mlm_plots/tef/fakenews/roberta/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.09	0.13	0.12	0.08	0.18	0.05	0.16	0.03	0.05	0.05	0.02	0.08	0.03	0.07	0.03	0.04	0.04	0.02	0.06	0.02	0.05	656
0.03	0.21	0.27	0.27	0.18	0.36	0.09	0.33	0.06	0.08	0.08	0.05	0.12	0.04	0.10	0.05	0.06	0.06	0.04	0.09	0.02	0.08	967
0.06	0.42	0.53	0.52	0.37	0.69	0.16	0.62	0.09	0.11	0.11	0.07	0.15	0.04	0.13	0.07	0.09	0.09	0.06	0.11	0.03	0.10	1000
0.11	0.66	0.82	0.81	0.57	1.07	0.25	0.96	0.11	0.13	0.13	0.09	0.18	0.04	0.15	0.09	0.11	0.10	0.08	0.13	0.03	0.12	999
0.15	1.11	1.38	1.38	0.97	1.80	0.42	1.63	0.13	0.16	0.16	0.11	0.21	0.05	0.18	0.11	0.13	0.13	0.10	0.16	0.03	0.14	1016
0.18	1.60	2.03	2.00	1.37	2.68	0.65	2.41	0.15	0.18	0.18	0.13	0.23	0.05	0.20	0.13	0.14	0.14	0.11	0.18	0.03	0.16	864
0.32	2.14	3.01	2.85	1.77	4.26	1.24	3.63	0.17	0.20	0.20	0.15	0.25	0.05	0.23	0.14	0.16	0.16	0.13	0.19	0.03	0.18	1337


==> data/mlm_plots/tef/fakenews/roberta/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.50
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/roberta/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.98	0.98	0.97	0.99	0.01	0.99	0.97	0.98	0.98	0.97	0.99	0.01	0.99	0.95	0.96	0.97	0.94	0.98	0.02	0.98	656
0.03	0.96	0.96	0.97	0.95	0.98	0.01	0.98	0.96	0.96	0.97	0.95	0.98	0.02	0.98	0.94	0.95	0.96	0.93	0.98	0.03	0.97	967
0.06	0.92	0.94	0.94	0.92	0.96	0.02	0.95	0.92	0.94	0.94	0.91	0.96	0.02	0.95	0.92	0.93	0.94	0.90	0.96	0.03	0.96	1000
0.11	0.90	0.91	0.91	0.89	0.94	0.02	0.93	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.90	0.92	0.92	0.88	0.95	0.03	0.94	999
0.15	0.86	0.87	0.87	0.85	0.90	0.03	0.89	0.86	0.87	0.87	0.85	0.90	0.03	0.89	0.87	0.89	0.89	0.85	0.93	0.04	0.91	1016
0.18	0.83	0.84	0.84	0.82	0.87	0.03	0.86	0.82	0.84	0.84	0.81	0.87	0.03	0.86	0.84	0.86	0.87	0.82	0.90	0.04	0.89	864
0.32	0.79	0.81	0.81	0.78	0.85	0.03	0.83	0.79	0.81	0.81	0.78	0.85	0.04	0.84	0.81	0.84	0.84	0.79	0.88	0.05	0.87	1337


==> data/mlm_plots/tef/fakenews/roberta/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.28


==> data/mlm_plots/tef/fakenews/roberta/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	22.17	23.35	25.27	17.16	29.54	6.19	27.43	0.10	0.16	0.15	0.09	0.22	0.07	0.20	2.21	11.80	5.18	-5.69	29.28	17.48	13.37	656
0.03	28.10	30.06	32.60	20.73	39.38	9.32	35.80	0.13	0.19	0.18	0.12	0.26	0.07	0.24	2.21	12.27	5.50	-7.06	31.61	19.34	13.04	967
0.06	34.92	37.63	41.76	24.52	50.74	13.11	45.45	0.15	0.21	0.20	0.13	0.29	0.08	0.26	2.11	13.68	5.65	-8.42	35.78	22.10	15.03	1000
0.11	46.27	51.34	56.79	32.47	70.22	18.87	63.52	0.16	0.22	0.21	0.14	0.30	0.08	0.28	2.16	15.40	6.25	-9.40	40.21	24.81	16.40	999
0.15	63.61	70.63	76.97	44.10	97.15	26.52	86.37	0.18	0.25	0.24	0.16	0.34	0.09	0.30	2.50	17.09	6.93	-10.42	44.60	27.51	17.56	1016
0.18	80.11	90.60	99.85	54.53	126.67	36.07	113.47	0.19	0.26	0.25	0.17	0.36	0.09	0.32	2.34	18.28	6.81	-10.58	47.13	28.86	18.58	864
0.32	87.84	105.14	114.04	62.63	147.65	42.51	133.05	0.21	0.28	0.27	0.18	0.39	0.10	0.35	3.24	20.77	8.62	-10.93	52.48	31.71	23.74	1337


==> data/mlm_plots/tef/fakenews/roberta/a/time_misc_auc.tex <==
name	auc
attack_time	22.34
l2	0.08
lom	5.28


==> data/mlm_plots/tef/fakenews/roberta/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.81	0.85	0.86	0.77	0.92	0.07	0.91	0.92	0.93	0.94	0.89	0.98	0.04	0.96	0.93	0.95	0.96	0.92	0.98	0.03	0.97	656
0.03	0.75	0.80	0.81	0.71	0.89	0.09	0.86	0.89	0.91	0.92	0.87	0.95	0.04	0.94	0.92	0.94	0.94	0.90	0.97	0.03	0.96	967
0.06	0.71	0.77	0.78	0.66	0.87	0.10	0.83	0.86	0.88	0.89	0.83	0.94	0.05	0.91	0.90	0.92	0.92	0.88	0.96	0.04	0.94	1000
0.11	0.69	0.75	0.76	0.63	0.86	0.12	0.82	0.84	0.86	0.87	0.80	0.92	0.06	0.89	0.88	0.90	0.90	0.86	0.94	0.04	0.92	999
0.15	0.67	0.72	0.74	0.59	0.86	0.13	0.81	0.81	0.83	0.84	0.76	0.91	0.07	0.87	0.85	0.87	0.88	0.82	0.93	0.05	0.90	1016
0.18	0.65	0.72	0.74	0.57	0.86	0.14	0.81	0.79	0.82	0.82	0.74	0.90	0.08	0.86	0.83	0.86	0.86	0.80	0.91	0.05	0.89	864
0.32	0.63	0.70	0.72	0.56	0.84	0.14	0.79	0.77	0.80	0.81	0.72	0.88	0.08	0.84	0.82	0.84	0.85	0.79	0.89	0.05	0.87	1337


==> data/mlm_plots/tef/fakenews/roberta/a/top_intersections_auc.tex <==
name	auc
top10	0.23
top30	0.26
top50	0.27


==> data/mlm_plots/tef/fakenews/roberta/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	30.83	41.75	38.03	22.87	60.62	18.87	49.15	30.00	38.49	38.00	24.63	52.35	13.86	46.00	35.24	46.93	43.36	26.98	66.89	19.95	55.02	31.00	39.00	38.00	25.13	52.87	13.87	46.00	939
0.03	30.97	42.26	38.74	23.31	61.21	18.95	48.89	29.00	37.35	36.00	22.75	51.96	14.60	45.00	39.11	52.28	49.44	30.43	74.14	21.85	59.66	30.00	38.10	36.00	23.53	52.68	14.57	45.00	772
0.06	32.05	44.72	39.12	17.97	71.46	26.74	49.78	31.00	38.94	38.00	22.41	55.47	16.53	47.00	48.72	64.26	57.80	31.81	96.72	32.45	70.98	33.00	40.21	40.00	23.65	56.77	16.56	47.50	623
0.11	32.26	50.41	40.32	6.29	94.54	44.13	55.35	19.00	34.61	33.00	12.99	56.24	21.62	43.00	62.01	88.28	75.86	11.96	164.60	76.32	89.97	21.00	36.42	35.00	14.30	58.54	22.12	46.00	237
0.15	32.21	60.35	39.42	-6.33	127.04	66.69	56.96	23.75	33.81	35.50	16.41	51.22	17.40	43.00	84.54	123.82	91.13	22.66	224.98	101.16	113.41	26.00	37.13	41.00	18.70	55.56	18.43	48.00	124
0.18	32.83	57.71	39.94	-3.06	118.48	60.77	55.16	31.00	35.48	38.00	17.42	53.55	18.07	43.00	101.30	143.65	125.25	66.81	220.49	76.84	146.77	36.50	40.07	44.00	20.58	59.56	19.49	47.00	87
0.32	32.55	68.26	38.68	-21.01	157.54	89.27	58.85	29.00	35.80	40.00	17.79	53.81	18.01	45.00	131.22	204.89	153.57	48.01	361.77	156.88	204.46	37.00	41.43	45.50	21.45	61.42	19.99	52.00	120


==> data/mlm_plots/tef/fakenews/roberta/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	17.37
orig_ge	11.14
adv_pp	39.18
adv_ge	12.20


==> data/mlm_plots/tef/fakenews/roberta/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.17	0.02	0.02	-0.31	0.35	0.33	0.15	0.11	0.28	0.24	0.04	0.53	0.25	0.45	0.08	0.22	0.17	0.02	0.41	0.20	0.33	939
0.03	-0.20	-0.07	-0.04	-0.30	0.16	0.23	0.06	0.08	0.22	0.20	0.02	0.41	0.20	0.33	0.06	0.16	0.15	0.01	0.31	0.15	0.25	772
0.06	-0.41	-0.18	-0.09	-0.48	0.12	0.30	0.04	0.02	0.15	0.14	-0.07	0.36	0.21	0.28	0.02	0.11	0.10	-0.05	0.27	0.16	0.20	623
0.11	-0.45	-0.26	-0.27	-0.51	-0.01	0.25	-0.06	-0.02	0.08	0.08	-0.10	0.27	0.19	0.18	-0.01	0.06	0.06	-0.07	0.20	0.14	0.14	237
0.15	-0.51	-0.36	-0.37	-0.59	-0.14	0.23	-0.19	-0.04	0.00	0.00	-0.15	0.15	0.15	0.07	-0.03	0.01	0.01	-0.10	0.12	0.11	0.05	124
0.18	-0.58	-0.42	-0.49	-0.67	-0.18	0.25	-0.28	-0.03	0.03	0.02	-0.07	0.14	0.11	0.07	-0.02	0.03	0.02	-0.05	0.10	0.08	0.05	87
0.32	-0.64	-0.49	-0.55	-0.72	-0.27	0.23	-0.33	-0.08	-0.03	-0.02	-0.17	0.11	0.14	0.04	-0.05	-0.02	-0.01	-0.12	0.08	0.10	0.03	120


==> data/mlm_plots/tef/fakenews/roberta/ig/correlations_auc.tex <==
name	auc
pcc	-0.10
spearman	0.02
kendall	0.01


==> data/mlm_plots/tef/fakenews/roberta/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	15.15	22.96	21.26	11.37	34.55	11.59	29.75	14.45	23.64	21.03	10.76	36.53	12.89	31.48	9.83	17.72	15.45	6.66	28.79	11.06	23.86	939
0.03	10.53	15.10	13.75	8.61	21.58	6.49	17.87	10.98	15.76	14.08	8.62	22.90	7.14	19.26	9.62	15.46	13.48	6.91	24.01	8.55	19.18	772
0.06	7.64	10.41	9.72	6.27	14.55	4.14	12.38	7.89	10.85	10.12	6.27	15.44	4.58	13.47	8.69	14.65	12.12	5.58	23.73	9.08	18.44	623
0.11	5.13	7.33	7.07	4.66	10.00	2.67	9.11	5.41	7.78	7.14	4.59	10.96	3.18	9.89	5.69	8.72	7.65	3.80	13.64	4.92	10.49	237
0.15	5.09	6.04	5.81	4.23	7.86	1.82	6.88	5.17	6.40	6.26	4.04	8.77	2.37	7.29	4.98	7.70	6.58	2.83	12.56	4.87	9.05	124
0.18	3.83	5.14	5.07	3.48	6.80	1.66	6.40	4.17	5.30	5.03	3.64	6.96	1.66	6.46	4.61	6.39	6.33	4.09	8.68	2.29	7.96	87
0.32	3.54	4.42	4.44	3.18	5.67	1.24	5.19	3.79	4.60	4.48	3.28	5.91	1.31	5.40	3.81	5.24	4.70	3.23	7.24	2.00	6.81	120


==> data/mlm_plots/tef/fakenews/roberta/ig/ets_sts_auc.tex <==
name	auc
et_use	2.31
et_tse	2.41
et_ce	2.72


==> data/mlm_plots/tef/fakenews/roberta/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.76	4.51	3.82	0.29	8.73	4.22	5.30	8.02	13.03	11.25	4.71	21.34	8.32	15.68	6.15	11.90	9.25	1.98	21.81	9.91	14.21	939
0.03	1.70	2.54	2.18	1.27	3.82	1.28	3.22	7.00	9.50	8.93	5.20	13.80	4.30	10.97	5.55	7.99	7.12	1.03	14.95	6.96	9.16	772
0.06	1.00	1.42	1.29	0.63	2.22	0.80	1.60	5.72	7.91	7.20	4.40	11.41	3.51	9.25	4.44	6.56	5.77	2.82	10.31	3.74	7.65	623
0.11	0.63	0.94	0.80	-0.25	2.14	1.20	0.99	5.18	6.80	6.33	2.01	11.60	4.79	7.87	3.83	5.85	5.13	-0.24	11.95	6.10	6.57	237
0.15	0.40	0.62	0.52	0.11	1.13	0.51	0.69	4.94	6.32	5.96	3.07	9.56	3.25	6.99	3.82	5.32	4.85	1.81	8.83	3.51	5.73	124
0.18	0.30	0.45	0.39	0.10	0.79	0.34	0.46	4.53	5.58	5.62	4.01	7.16	1.57	6.59	3.68	5.03	4.41	1.77	8.29	3.26	5.37	87
0.32	0.21	0.40	0.28	-0.32	1.12	0.72	0.35	4.21	5.12	5.15	3.51	6.73	1.61	5.65	3.43	4.17	4.14	2.50	5.84	1.67	4.51	120


==> data/mlm_plots/tef/fakenews/roberta/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.30
et_p_h	2.05
et_p_l2	1.75


==> data/mlm_plots/tef/fakenews/roberta/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.10	0.13	0.13	0.08	0.18	0.05	0.16	0.04	0.06	0.05	0.03	0.08	0.03	0.07	0.03	0.05	0.04	0.03	0.06	0.02	0.05	939
0.03	0.17	0.25	0.25	0.15	0.34	0.09	0.31	0.06	0.08	0.07	0.05	0.11	0.03	0.10	0.05	0.06	0.06	0.04	0.08	0.02	0.07	772
0.06	0.35	0.47	0.45	0.31	0.62	0.16	0.56	0.08	0.10	0.10	0.07	0.14	0.03	0.12	0.06	0.08	0.08	0.06	0.10	0.02	0.10	623
0.11	0.64	0.84	0.80	0.53	1.15	0.31	0.98	0.10	0.13	0.13	0.09	0.18	0.05	0.16	0.09	0.10	0.10	0.08	0.13	0.03	0.12	237
0.15	0.97	1.34	1.31	0.87	1.81	0.47	1.68	0.12	0.15	0.15	0.10	0.20	0.05	0.18	0.10	0.12	0.12	0.09	0.15	0.03	0.14	124
0.18	1.50	1.92	1.93	1.26	2.57	0.66	2.34	0.14	0.17	0.17	0.12	0.21	0.05	0.19	0.12	0.13	0.13	0.11	0.16	0.03	0.15	87
0.32	2.10	2.83	2.73	1.69	3.97	1.14	3.60	0.16	0.19	0.20	0.15	0.24	0.04	0.22	0.13	0.15	0.16	0.12	0.19	0.03	0.17	120


==> data/mlm_plots/tef/fakenews/roberta/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.47
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/roberta/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.98	0.98	0.97	0.98	0.01	0.98	0.97	0.98	0.98	0.96	0.99	0.01	0.98	0.96	0.96	0.97	0.94	0.99	0.02	0.98	939
0.03	0.95	0.96	0.96	0.95	0.97	0.01	0.97	0.95	0.96	0.96	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.93	0.98	0.02	0.97	772
0.06	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.93	0.95	0.95	0.92	0.97	0.03	0.97	623
0.11	0.89	0.91	0.91	0.88	0.93	0.02	0.92	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.90	0.91	0.92	0.88	0.95	0.04	0.94	237
0.15	0.87	0.88	0.88	0.85	0.91	0.03	0.90	0.87	0.88	0.89	0.85	0.92	0.04	0.90	0.87	0.89	0.90	0.83	0.95	0.06	0.92	124
0.18	0.83	0.85	0.86	0.82	0.89	0.04	0.88	0.84	0.86	0.86	0.83	0.89	0.03	0.88	0.85	0.88	0.89	0.83	0.92	0.04	0.91	87
0.32	0.80	0.82	0.82	0.78	0.86	0.04	0.85	0.80	0.83	0.83	0.79	0.87	0.04	0.85	0.81	0.84	0.84	0.76	0.91	0.07	0.88	120


==> data/mlm_plots/tef/fakenews/roberta/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.28


==> data/mlm_plots/tef/fakenews/roberta/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	35.83	86.90	48.57	-7.91	181.70	94.80	88.48	1.20	4.84	2.56	-4.75	14.43	9.59	4.91	20.83	62.64	46.95	5.03	120.25	57.61	83.74	939
0.03	150.81	285.77	327.25	153.11	418.44	132.67	398.51	1.44	7.24	2.94	-13.63	28.12	20.87	5.91	28.60	72.52	56.25	8.48	136.55	64.04	87.62	772
0.06	180.92	292.68	345.69	168.89	416.47	123.79	392.98	1.89	8.58	4.01	-4.69	21.84	13.26	10.17	25.45	74.68	57.43	6.00	143.35	68.67	90.47	623
0.11	138.93	209.81	187.49	90.72	328.90	119.09	300.29	2.69	8.44	3.43	-13.82	30.70	22.26	5.57	11.32	41.41	28.92	0.88	81.94	40.53	57.91	237
0.15	135.23	213.78	211.43	100.42	327.13	113.35	288.99	2.61	4.84	3.58	-0.29	9.97	5.13	5.05	17.93	41.15	25.61	-0.17	82.47	41.32	55.79	124
0.18	163.89	226.94	252.16	120.95	332.94	105.99	303.71	2.52	4.81	3.36	-0.08	9.71	4.90	4.34	14.90	36.68	30.47	9.94	63.42	26.74	54.79	87
0.32	210.06	263.47	291.87	137.79	389.16	125.68	351.64	2.49	3.74	3.23	1.24	6.24	2.50	4.19	11.99	35.63	27.32	6.61	64.66	29.03	56.89	120


==> data/mlm_plots/tef/fakenews/roberta/ig/time_misc_auc.tex <==
name	auc
attack_time	74.15
l2	1.79
lom	14.31


==> data/mlm_plots/tef/fakenews/roberta/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.25	0.38	0.34	0.19	0.56	0.18	0.49	0.39	0.50	0.46	0.35	0.64	0.14	0.59	0.55	0.62	0.60	0.52	0.72	0.10	0.68	939
0.03	0.21	0.31	0.29	0.17	0.44	0.14	0.40	0.38	0.45	0.44	0.34	0.57	0.11	0.53	0.54	0.59	0.58	0.51	0.67	0.08	0.63	772
0.06	0.21	0.30	0.28	0.16	0.43	0.14	0.38	0.36	0.43	0.42	0.31	0.54	0.12	0.52	0.52	0.57	0.56	0.48	0.65	0.09	0.62	623
0.11	0.17	0.24	0.24	0.12	0.37	0.13	0.32	0.34	0.40	0.39	0.28	0.51	0.11	0.44	0.49	0.54	0.54	0.46	0.63	0.09	0.59	237
0.15	0.15	0.21	0.22	0.09	0.33	0.12	0.27	0.32	0.35	0.35	0.27	0.44	0.09	0.39	0.49	0.51	0.52	0.44	0.58	0.07	0.54	124
0.18	0.16	0.21	0.22	0.11	0.31	0.10	0.27	0.31	0.35	0.33	0.28	0.42	0.07	0.38	0.50	0.52	0.52	0.47	0.58	0.05	0.54	87
0.32	0.14	0.19	0.18	0.09	0.29	0.10	0.24	0.30	0.33	0.33	0.25	0.41	0.08	0.36	0.48	0.50	0.51	0.43	0.57	0.07	0.54	120


==> data/mlm_plots/tef/fakenews/roberta/ig/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.12
top50	0.17


==> data/mlm_plots/tef/fakenews/roberta/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	31.03	41.26	37.93	23.84	58.67	17.42	48.31	31.00	39.21	38.00	25.29	53.13	13.92	46.00	35.78	46.87	43.14	28.21	65.54	18.67	55.03	32.00	39.92	39.00	26.04	53.80	13.88	47.00	1063
0.03	31.23	42.43	38.91	21.50	63.35	20.93	48.44	31.00	39.24	38.00	23.96	54.53	15.29	47.00	39.17	52.66	49.39	29.33	76.00	23.34	60.40	32.00	40.26	39.00	25.05	55.47	15.21	48.00	1622
0.06	30.78	44.69	38.70	18.46	70.93	26.24	50.19	29.00	37.29	37.00	21.40	53.17	15.89	46.00	45.89	64.71	56.66	30.09	99.32	34.61	75.20	31.00	38.93	39.00	22.86	54.99	16.06	47.00	1376
0.11	33.49	51.78	40.51	5.04	98.51	46.74	52.76	27.00	37.85	37.00	16.99	58.71	20.86	45.75	65.90	90.90	76.55	20.18	161.61	70.71	91.48	29.25	40.08	39.00	18.96	61.20	21.12	50.00	438
0.15	34.97	80.81	49.96	-16.16	177.79	96.98	69.37	17.00	28.23	29.00	10.10	46.37	18.13	40.00	89.23	172.50	115.74	-8.76	353.75	181.25	150.78	20.00	31.41	30.00	11.55	51.26	19.86	46.00	150
0.18	35.16	82.96	48.98	-7.64	173.55	90.60	78.77	10.50	30.05	30.00	9.01	51.08	21.04	45.00	110.91	210.28	150.58	22.38	398.17	187.89	237.80	12.50	33.38	34.00	10.72	56.03	22.66	51.00	104
0.32	38.43	97.55	52.81	-8.89	203.98	106.43	105.44	6.00	23.78	21.00	2.32	45.23	21.45	38.00	151.94	315.58	208.30	-23.46	654.62	339.04	311.06	7.00	27.05	23.00	3.34	50.77	23.72	45.00	129


==> data/mlm_plots/tef/fakenews/roberta/s/comparison_vals_auc.tex <==
name	auc
orig_pp	22.37
orig_ge	9.78
adv_pp	54.40
adv_ge	10.61


==> data/mlm_plots/tef/fakenews/roberta/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.04	0.38	0.20	0.01	0.76	0.38	0.78	0.24	0.54	0.59	0.20	0.89	0.35	0.88	0.16	0.44	0.42	0.13	0.74	0.30	0.73	1063
0.03	0.00	0.15	0.04	-0.11	0.42	0.26	0.14	0.10	0.31	0.26	0.01	0.61	0.30	0.49	0.07	0.23	0.18	-0.01	0.47	0.24	0.33	1622
0.06	0.01	0.13	0.05	-0.08	0.33	0.21	0.13	0.10	0.30	0.26	0.02	0.57	0.28	0.49	0.06	0.22	0.18	0.01	0.43	0.21	0.34	1376
0.11	0.02	0.19	0.07	-0.07	0.46	0.26	0.26	0.17	0.38	0.34	0.08	0.68	0.30	0.60	0.11	0.28	0.23	0.05	0.52	0.24	0.44	438
0.15	0.05	0.34	0.17	0.01	0.66	0.32	0.65	0.20	0.52	0.57	0.19	0.84	0.32	0.81	0.13	0.40	0.42	0.13	0.66	0.27	0.63	150
0.18	0.06	0.36	0.32	0.05	0.66	0.31	0.64	0.29	0.50	0.62	0.15	0.85	0.35	0.82	0.21	0.38	0.45	0.11	0.66	0.28	0.63	104
0.32	0.16	0.41	0.44	0.12	0.70	0.29	0.64	0.39	0.55	0.66	0.22	0.88	0.33	0.80	0.28	0.42	0.48	0.16	0.68	0.26	0.62	129


==> data/mlm_plots/tef/fakenews/roberta/s/correlations_auc.tex <==
name	auc
pcc	0.09
spearman	0.14
kendall	0.11


==> data/mlm_plots/tef/fakenews/roberta/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	4.18	12.86	12.75	3.32	22.39	9.54	18.95	3.95	13.13	12.59	2.96	23.30	10.17	19.03	2.76	10.57	9.08	1.54	19.60	9.03	15.54	1063
0.03	8.44	11.26	11.28	5.97	16.55	5.29	14.34	8.28	11.70	11.55	5.75	17.64	5.94	14.65	6.53	11.99	10.34	4.14	19.84	7.85	15.62	1622
0.06	5.54	7.51	7.35	4.43	10.60	3.08	8.94	5.71	7.67	7.29	4.39	10.96	3.29	9.37	6.07	9.29	8.04	3.83	14.75	5.46	11.48	1376
0.11	3.62	4.46	4.63	2.72	6.20	1.74	5.50	3.44	4.61	4.65	2.62	6.60	1.99	5.75	4.09	5.97	5.58	2.70	9.24	3.27	7.30	438
0.15	1.59	2.72	2.80	1.29	4.14	1.43	3.78	1.60	2.77	2.89	1.29	4.25	1.48	3.70	1.78	3.70	3.45	1.37	6.03	2.33	4.91	150
0.18	1.15	2.23	2.29	1.03	3.43	1.20	3.17	1.26	2.27	2.27	1.11	3.43	1.16	3.20	1.65	3.38	3.01	0.49	6.28	2.89	4.27	104
0.32	0.85	1.70	1.51	0.63	2.78	1.08	2.26	0.82	1.72	1.49	0.67	2.78	1.06	2.30	1.18	2.47	1.92	0.06	4.87	2.41	3.01	129


==> data/mlm_plots/tef/fakenews/roberta/s/ets_sts_auc.tex <==
name	auc
et_use	1.31
et_tse	1.35
et_ce	1.63


==> data/mlm_plots/tef/fakenews/roberta/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.82	2.52	2.41	0.42	4.61	2.09	3.60	2.20	7.27	7.06	1.12	13.42	6.15	10.07	1.79	6.56	5.47	-0.24	13.36	6.80	8.38	1063
0.03	1.35	1.92	1.85	0.88	2.95	1.04	2.41	5.70	7.49	7.07	3.19	11.80	4.31	8.95	4.33	6.48	5.69	1.27	11.68	5.21	7.39	1622
0.06	0.74	1.10	0.97	0.50	1.69	0.60	1.36	4.47	5.69	5.49	3.07	8.32	2.63	6.59	3.37	4.73	4.39	1.94	7.51	2.79	5.58	1376
0.11	0.38	0.55	0.49	0.17	0.92	0.38	0.67	3.24	4.07	4.17	2.29	5.84	1.77	5.02	2.52	3.47	3.38	0.47	6.47	3.00	3.98	438
0.15	0.13	0.27	0.29	0.11	0.44	0.17	0.38	1.41	2.74	3.02	1.26	4.22	1.48	3.83	1.19	2.26	2.41	0.98	3.53	1.27	3.11	150
0.18	0.10	0.26	0.18	-0.31	0.82	0.56	0.23	1.33	2.36	2.62	1.10	3.63	1.26	3.12	1.01	2.18	2.10	0.17	4.19	2.01	2.53	104
0.32	0.06	0.25	0.12	-0.58	1.07	0.82	0.18	1.10	2.13	1.79	0.64	3.61	1.49	2.75	0.80	2.02	1.46	-0.24	4.28	2.26	2.18	129


==> data/mlm_plots/tef/fakenews/roberta/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.19
et_p_h	1.11
et_p_l2	0.98


==> data/mlm_plots/tef/fakenews/roberta/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.11	0.14	0.14	0.09	0.20	0.05	0.18	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.06	1063
0.03	0.19	0.25	0.25	0.17	0.34	0.09	0.32	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.05	0.06	0.06	0.05	0.08	0.02	0.08	1622
0.06	0.34	0.47	0.46	0.29	0.65	0.18	0.57	0.08	0.11	0.11	0.07	0.14	0.04	0.12	0.07	0.08	0.08	0.06	0.11	0.02	0.10	1376
0.11	0.67	0.85	0.86	0.56	1.14	0.29	1.03	0.11	0.13	0.13	0.09	0.17	0.04	0.15	0.09	0.11	0.10	0.08	0.13	0.03	0.12	438
0.15	1.00	1.36	1.40	0.83	1.90	0.53	1.63	0.13	0.16	0.16	0.10	0.22	0.06	0.18	0.11	0.13	0.13	0.09	0.17	0.04	0.15	150
0.18	1.50	2.00	2.09	1.16	2.84	0.84	2.49	0.16	0.19	0.19	0.11	0.27	0.08	0.22	0.13	0.15	0.15	0.10	0.20	0.05	0.17	104
0.32	1.85	2.77	2.72	1.41	4.13	1.36	3.51	0.16	0.20	0.20	0.12	0.28	0.08	0.25	0.12	0.16	0.16	0.11	0.21	0.05	0.19	129


==> data/mlm_plots/tef/fakenews/roberta/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.48
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/roberta/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.96	0.98	0.01	0.98	0.97	0.97	0.97	0.96	0.98	0.01	0.98	0.95	0.96	0.97	0.94	0.98	0.02	0.98	1063
0.03	0.95	0.96	0.96	0.95	0.97	0.01	0.97	0.95	0.96	0.96	0.94	0.97	0.01	0.97	0.94	0.95	0.96	0.93	0.98	0.03	0.97	1622
0.06	0.93	0.94	0.94	0.92	0.95	0.02	0.95	0.92	0.94	0.94	0.92	0.96	0.02	0.95	0.93	0.94	0.94	0.91	0.97	0.03	0.96	1376
0.11	0.89	0.91	0.91	0.88	0.93	0.02	0.92	0.89	0.91	0.91	0.88	0.93	0.03	0.93	0.91	0.92	0.92	0.89	0.95	0.03	0.94	438
0.15	0.86	0.87	0.87	0.84	0.90	0.03	0.90	0.85	0.87	0.87	0.84	0.91	0.03	0.90	0.87	0.90	0.90	0.86	0.93	0.04	0.92	150
0.18	0.83	0.85	0.85	0.81	0.88	0.04	0.87	0.82	0.85	0.85	0.81	0.89	0.04	0.87	0.85	0.88	0.89	0.83	0.93	0.05	0.92	104
0.32	0.77	0.81	0.81	0.76	0.86	0.05	0.84	0.78	0.81	0.81	0.76	0.86	0.05	0.84	0.81	0.85	0.85	0.78	0.91	0.07	0.89	129


==> data/mlm_plots/tef/fakenews/roberta/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.28


==> data/mlm_plots/tef/fakenews/roberta/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	25.42	50.36	29.45	-0.44	101.15	50.79	42.01	2.22	112.99	26.01	-94.94	320.91	207.92	145.46	9.11	48.11	31.23	1.24	94.98	46.87	79.80	1063
0.03	73.99	139.44	160.99	72.32	206.56	67.12	190.10	65.13	323.23	182.69	-127.03	773.48	450.25	371.47	30.74	74.44	65.54	22.78	126.09	51.65	119.52	1622
0.06	96.45	142.71	162.73	83.72	201.71	58.99	186.20	85.83	366.14	203.26	-135.31	867.59	501.45	452.35	22.71	69.74	62.96	20.00	119.48	49.74	107.54	1376
0.11	72.21	129.27	142.01	61.64	196.91	67.63	187.06	31.64	442.67	142.61	-612.15	1497.49	1054.82	316.14	12.05	56.29	43.71	8.10	104.47	48.19	92.33	438
0.15	27.04	88.42	86.71	24.32	152.52	64.10	130.65	4.28	167.15	34.70	-78.54	412.83	245.69	248.90	3.25	31.74	14.55	-6.39	69.88	38.14	50.20	150
0.18	22.73	91.97	90.03	23.41	160.53	68.56	158.82	3.08	272.04	10.83	-516.25	1060.34	788.30	95.12	3.37	38.69	13.24	-6.95	84.33	45.64	63.18	104
0.32	15.19	84.82	64.38	11.62	158.02	73.20	159.93	2.76	58.35	5.76	-208.00	324.69	266.35	25.32	1.55	23.49	7.62	-13.29	60.26	36.77	27.15	129


==> data/mlm_plots/tef/fakenews/roberta/s/time_misc_auc.tex <==
name	auc
attack_time	32.29
l2	76.72
lom	13.66


==> data/mlm_plots/tef/fakenews/roberta/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.17	0.44	0.35	0.14	0.73	0.30	0.73	0.41	0.61	0.57	0.39	0.82	0.22	0.82	0.57	0.71	0.71	0.55	0.88	0.16	0.87	1063
0.03	0.11	0.25	0.20	0.04	0.47	0.21	0.30	0.36	0.47	0.42	0.30	0.63	0.17	0.52	0.51	0.61	0.58	0.48	0.74	0.13	0.68	1622
0.06	0.12	0.24	0.20	0.06	0.42	0.18	0.29	0.36	0.46	0.43	0.31	0.61	0.15	0.51	0.52	0.60	0.58	0.48	0.72	0.12	0.67	1376
0.11	0.14	0.30	0.24	0.08	0.52	0.22	0.37	0.40	0.50	0.47	0.34	0.67	0.17	0.61	0.55	0.64	0.61	0.51	0.76	0.13	0.73	438
0.15	0.14	0.40	0.35	0.11	0.69	0.29	0.62	0.39	0.57	0.57	0.37	0.77	0.20	0.75	0.55	0.70	0.71	0.55	0.84	0.15	0.82	150
0.18	0.19	0.39	0.42	0.14	0.64	0.25	0.60	0.45	0.57	0.59	0.38	0.77	0.19	0.75	0.56	0.69	0.70	0.54	0.84	0.15	0.83	104
0.32	0.22	0.45	0.50	0.18	0.72	0.27	0.63	0.43	0.59	0.65	0.40	0.79	0.20	0.75	0.60	0.71	0.75	0.56	0.86	0.15	0.83	129


==> data/mlm_plots/tef/fakenews/roberta/s/top_intersections_auc.tex <==
name	auc
top10	0.11
top30	0.17
top50	0.21


==> data/mlm_plots/tef/fakenews/xlnet/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	32.08	43.35	39.58	25.14	61.56	18.21	50.51	29.00	35.83	35.00	22.92	48.73	12.90	41.00	36.90	49.50	45.87	29.64	69.35	19.85	57.43	29.75	36.52	36.00	23.63	49.41	12.89	42.00	900
0.03	31.92	43.96	39.52	24.18	63.73	19.78	50.89	28.00	35.46	35.00	21.42	49.50	14.04	42.00	42.73	56.92	52.17	33.90	79.95	23.03	65.60	29.00	36.69	36.00	22.63	50.74	14.05	43.00	989
0.06	31.94	46.50	39.73	16.66	76.34	29.84	51.76	28.00	34.69	34.00	20.19	49.20	14.50	41.00	52.37	72.31	63.69	27.43	117.19	44.88	80.05	30.00	36.78	37.00	22.15	51.41	14.63	44.00	1003
0.11	31.81	50.69	39.94	-23.18	124.55	73.86	52.11	27.00	34.20	34.00	19.57	48.84	14.63	41.00	63.32	90.97	76.51	3.83	178.11	87.14	96.46	30.00	37.06	38.00	22.15	51.97	14.91	44.00	1013
0.15	31.81	50.54	39.68	1.85	99.24	48.70	52.11	28.00	34.45	34.00	19.43	49.47	15.02	41.00	85.20	116.98	102.35	39.07	194.89	77.91	125.89	31.00	38.52	39.00	23.12	53.93	15.40	46.00	1012
0.18	32.14	54.57	40.47	-34.30	143.44	88.87	52.16	27.00	33.54	34.00	19.00	48.08	14.54	41.00	111.98	156.42	134.80	7.95	304.89	148.47	163.89	32.00	38.62	40.00	23.26	53.98	15.36	47.00	889
0.32	32.39	53.03	40.71	-19.88	125.95	72.91	52.61	26.00	33.35	34.00	19.48	47.21	13.87	41.00	151.14	215.78	187.25	69.33	362.22	146.45	241.19	33.00	39.99	42.00	24.88	55.11	15.11	49.00	1354


==> data/mlm_plots/tef/fakenews/xlnet/a/comparison_vals_auc.tex <==
name	auc
orig_pp	15.82
orig_ge	10.58
adv_pp	41.29
adv_ge	11.87


==> data/mlm_plots/tef/fakenews/xlnet/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.24	0.53	0.54	0.21	0.85	0.32	0.82	0.66	0.81	0.95	0.56	1.05	0.25	0.98	0.47	0.69	0.83	0.43	0.96	0.26	0.91	900
0.03	0.14	0.40	0.35	0.10	0.70	0.30	0.64	0.61	0.77	0.91	0.52	1.03	0.26	0.96	0.44	0.65	0.75	0.39	0.90	0.26	0.86	989
0.06	0.07	0.29	0.21	0.02	0.57	0.28	0.48	0.56	0.73	0.86	0.46	1.00	0.27	0.94	0.39	0.60	0.70	0.34	0.85	0.26	0.81	1003
0.11	0.03	0.23	0.14	-0.03	0.48	0.25	0.39	0.49	0.69	0.82	0.40	0.98	0.29	0.91	0.34	0.55	0.64	0.29	0.81	0.26	0.77	1013
0.15	0.00	0.16	0.07	-0.06	0.38	0.22	0.25	0.39	0.63	0.76	0.33	0.93	0.30	0.87	0.27	0.49	0.57	0.23	0.75	0.26	0.71	1012
0.18	-0.02	0.11	0.03	-0.09	0.31	0.20	0.18	0.29	0.57	0.69	0.24	0.90	0.33	0.85	0.20	0.44	0.51	0.17	0.71	0.27	0.68	889
0.32	-0.04	0.06	0.01	-0.12	0.24	0.18	0.12	0.16	0.47	0.58	0.10	0.84	0.37	0.81	0.10	0.36	0.41	0.07	0.65	0.29	0.63	1354


==> data/mlm_plots/tef/fakenews/xlnet/a/correlations_auc.tex <==
name	auc
pcc	0.06
spearman	0.19
kendall	0.15


==> data/mlm_plots/tef/fakenews/xlnet/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.37	10.75	9.02	1.98	19.53	8.78	16.08	3.17	10.50	8.58	1.78	19.21	8.72	15.90	2.44	8.85	6.53	0.69	17.01	8.16	13.07	900
0.03	3.78	7.87	7.33	2.36	13.38	5.51	10.61	3.68	7.63	6.92	2.50	12.76	5.13	10.47	3.39	8.01	6.55	1.73	14.28	6.27	10.94	989
0.06	3.43	5.59	5.49	2.31	8.88	3.29	7.10	3.41	5.45	5.27	2.35	8.56	3.10	7.04	3.51	6.49	5.61	2.14	10.84	4.35	8.50	1003
0.11	3.12	4.38	4.28	2.16	6.61	2.23	5.38	3.01	4.31	4.14	2.14	6.48	2.17	5.31	3.31	5.38	4.79	2.08	8.67	3.30	6.79	1013
0.15	2.66	3.36	3.36	2.14	4.58	1.22	4.03	2.59	3.32	3.24	2.06	4.59	1.26	3.97	2.86	4.18	3.86	2.11	6.26	2.07	5.03	1012
0.18	2.36	2.83	2.84	1.92	3.73	0.91	3.29	2.26	2.81	2.78	1.87	3.74	0.94	3.29	2.55	3.49	3.23	1.95	5.03	1.54	4.17	889
0.32	2.07	2.43	2.42	1.75	3.11	0.68	2.79	2.04	2.43	2.40	1.73	3.13	0.70	2.79	2.21	2.94	2.74	1.77	4.11	1.17	3.45	1354


==> data/mlm_plots/tef/fakenews/xlnet/a/ets_sts_auc.tex <==
name	auc
et_use	1.25
et_tse	1.23
et_ce	1.44


==> data/mlm_plots/tef/fakenews/xlnet/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.61	2.07	1.62	-1.87	6.00	3.93	2.65	1.83	6.19	4.85	0.06	12.33	6.14	8.89	1.42	5.61	3.92	-0.72	11.93	6.32	7.45	900
0.03	0.60	1.13	1.02	-0.46	2.73	1.60	1.39	2.60	4.87	4.54	1.57	8.18	3.31	6.63	2.02	4.21	3.63	0.18	8.23	4.03	5.34	989
0.06	0.44	0.66	0.64	0.23	1.09	0.43	0.82	2.72	4.18	4.18	1.93	6.43	2.25	5.39	2.11	3.51	3.27	0.97	6.05	2.54	4.40	1003
0.11	0.33	0.48	0.45	0.07	0.88	0.40	0.56	2.74	3.79	3.80	2.01	5.58	1.79	4.74	2.10	3.26	3.03	-0.01	6.52	3.27	3.86	1013
0.15	0.22	0.31	0.29	0.05	0.58	0.26	0.35	2.71	3.42	3.43	2.10	4.75	1.33	4.07	2.11	2.97	2.70	0.19	5.76	2.78	3.31	1012
0.18	0.16	0.22	0.20	0.07	0.38	0.16	0.25	2.63	3.15	3.16	2.05	4.25	1.10	3.62	2.03	2.71	2.52	0.39	5.02	2.32	2.95	889
0.32	0.10	0.15	0.13	0.03	0.28	0.12	0.17	2.47	2.91	2.89	1.95	3.87	0.96	3.25	1.94	2.49	2.31	0.48	4.50	2.01	2.66	1354


==> data/mlm_plots/tef/fakenews/xlnet/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.14
et_p_h	1.11
et_p_l2	0.96


==> data/mlm_plots/tef/fakenews/xlnet/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.11	0.15	0.15	0.09	0.20	0.05	0.18	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.03	0.05	0.05	0.03	0.06	0.02	0.06	900
0.03	0.25	0.31	0.32	0.22	0.41	0.09	0.37	0.06	0.09	0.08	0.05	0.12	0.03	0.11	0.05	0.07	0.07	0.05	0.09	0.02	0.08	989
0.06	0.48	0.59	0.59	0.42	0.77	0.17	0.70	0.09	0.12	0.11	0.08	0.16	0.04	0.14	0.08	0.09	0.09	0.07	0.12	0.02	0.10	1003
0.11	0.74	0.91	0.91	0.65	1.18	0.27	1.07	0.11	0.14	0.14	0.09	0.18	0.04	0.16	0.09	0.11	0.11	0.08	0.14	0.03	0.12	1013
0.15	1.25	1.53	1.53	1.07	1.99	0.46	1.81	0.14	0.16	0.16	0.12	0.21	0.04	0.19	0.12	0.13	0.13	0.10	0.16	0.03	0.15	1012
0.18	1.83	2.30	2.30	1.56	3.05	0.74	2.77	0.16	0.19	0.18	0.14	0.24	0.05	0.21	0.13	0.15	0.15	0.12	0.18	0.03	0.16	889
0.32	2.65	3.69	3.46	2.14	5.23	1.54	4.39	0.18	0.21	0.21	0.16	0.26	0.05	0.24	0.15	0.17	0.17	0.13	0.20	0.03	0.19	1354


==> data/mlm_plots/tef/fakenews/xlnet/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.58
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/xlnet/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.98	0.96	0.98	0.01	0.98	0.97	0.97	0.98	0.96	0.99	0.01	0.98	0.96	0.96	0.97	0.94	0.99	0.02	0.98	900
0.03	0.95	0.96	0.96	0.94	0.97	0.02	0.97	0.94	0.95	0.96	0.94	0.97	0.02	0.97	0.94	0.95	0.96	0.92	0.98	0.03	0.97	989
0.06	0.92	0.93	0.93	0.91	0.95	0.02	0.94	0.91	0.93	0.93	0.90	0.95	0.02	0.94	0.92	0.93	0.94	0.90	0.96	0.03	0.96	1003
0.11	0.89	0.90	0.91	0.88	0.93	0.02	0.92	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.89	0.91	0.92	0.88	0.95	0.04	0.94	1013
0.15	0.85	0.87	0.87	0.84	0.90	0.03	0.89	0.84	0.87	0.87	0.83	0.90	0.03	0.89	0.86	0.88	0.89	0.84	0.93	0.04	0.91	1012
0.18	0.82	0.84	0.84	0.81	0.87	0.03	0.85	0.81	0.83	0.83	0.80	0.87	0.03	0.85	0.83	0.86	0.86	0.81	0.90	0.05	0.89	889
0.32	0.78	0.80	0.80	0.77	0.83	0.03	0.82	0.78	0.80	0.80	0.76	0.84	0.04	0.82	0.79	0.83	0.83	0.77	0.88	0.05	0.86	1354


==> data/mlm_plots/tef/fakenews/xlnet/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.27


==> data/mlm_plots/tef/fakenews/xlnet/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	27.75	30.02	31.21	23.19	36.85	6.83	34.07	0.06	0.13	0.11	0.03	0.23	0.10	0.17	7.73	34.77	23.01	-1.48	71.01	36.24	49.06	900
0.03	37.08	40.89	43.08	29.11	52.67	11.78	47.87	0.09	0.17	0.14	0.05	0.29	0.12	0.22	8.37	41.94	27.13	-1.58	85.46	43.52	61.90	989
0.06	53.29	58.07	61.85	39.14	77.01	18.94	69.29	0.11	0.21	0.18	0.07	0.35	0.14	0.27	11.02	48.34	34.02	0.43	96.24	47.90	70.83	1003
0.11	66.94	73.01	77.65	46.46	99.57	26.55	86.78	0.12	0.24	0.19	0.08	0.40	0.16	0.31	12.89	52.22	37.41	1.97	102.46	50.24	78.27	1013
0.15	97.32	106.52	113.84	68.23	144.81	38.29	127.76	0.14	0.27	0.21	0.09	0.45	0.18	0.36	15.90	58.01	43.47	3.54	112.47	54.46	84.90	1012
0.18	120.83	129.58	141.24	83.36	175.80	46.22	158.05	0.15	0.29	0.23	0.10	0.48	0.19	0.39	14.52	58.02	41.59	2.75	113.29	55.27	84.07	889
0.32	146.68	167.88	179.11	106.07	229.69	61.81	207.34	0.15	0.30	0.23	0.09	0.50	0.21	0.39	14.89	58.69	39.58	1.19	116.19	57.50	84.65	1354


==> data/mlm_plots/tef/fakenews/xlnet/a/time_misc_auc.tex <==
name	auc
attack_time	33.41
l2	0.08
lom	16.79


==> data/mlm_plots/tef/fakenews/xlnet/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.45	0.67	0.79	0.40	0.94	0.27	0.88	0.62	0.78	0.88	0.59	0.97	0.19	0.93	0.74	0.85	0.91	0.71	0.98	0.13	0.96	900
0.03	0.39	0.61	0.71	0.34	0.87	0.27	0.83	0.60	0.75	0.83	0.56	0.94	0.19	0.90	0.72	0.82	0.88	0.69	0.96	0.13	0.93	989
0.06	0.33	0.54	0.63	0.28	0.81	0.27	0.77	0.56	0.71	0.78	0.52	0.90	0.19	0.86	0.70	0.80	0.85	0.67	0.93	0.13	0.91	1003
0.11	0.25	0.49	0.54	0.22	0.76	0.27	0.72	0.51	0.68	0.74	0.48	0.87	0.20	0.84	0.67	0.78	0.82	0.65	0.91	0.13	0.89	1013
0.15	0.18	0.43	0.45	0.15	0.70	0.27	0.67	0.47	0.63	0.69	0.44	0.83	0.20	0.80	0.64	0.75	0.79	0.62	0.88	0.13	0.86	1012
0.18	0.10	0.38	0.38	0.10	0.66	0.28	0.64	0.41	0.59	0.65	0.38	0.80	0.21	0.77	0.60	0.72	0.76	0.59	0.86	0.14	0.84	889
0.32	0.04	0.33	0.26	0.04	0.61	0.29	0.60	0.33	0.53	0.56	0.31	0.76	0.22	0.74	0.55	0.68	0.71	0.54	0.83	0.15	0.81	1354


==> data/mlm_plots/tef/fakenews/xlnet/a/top_intersections_auc.tex <==
name	auc
top10	0.14
top30	0.20
top50	0.23


==> data/mlm_plots/tef/fakenews/xlnet/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	31.76	42.71	39.40	25.17	60.25	17.54	49.84	29.00	36.00	36.00	24.28	47.72	11.72	43.00	36.21	48.13	44.46	29.37	66.89	18.76	55.46	29.75	36.44	36.00	24.78	48.10	11.66	43.00	1032
0.03	32.16	43.32	39.53	24.59	62.05	18.73	50.19	28.00	34.68	34.00	22.59	46.77	12.09	41.00	41.47	54.12	49.47	32.30	75.94	21.82	62.55	29.00	35.54	35.00	23.38	47.69	12.15	42.00	1163
0.06	32.12	46.35	39.43	17.70	75.00	28.65	50.12	28.00	35.76	35.00	21.14	50.37	14.61	42.75	48.51	66.11	57.74	29.41	102.81	36.70	73.13	30.00	37.26	36.00	22.62	51.90	14.64	44.00	1482
0.11	32.54	49.19	39.53	9.13	89.26	40.07	51.81	27.00	33.09	34.00	18.29	47.89	14.80	40.00	62.57	88.90	72.47	20.87	156.93	68.03	96.05	29.00	35.30	36.00	20.25	50.35	15.05	43.00	735
0.15	33.74	60.26	44.64	-13.47	133.98	73.73	54.89	23.00	32.02	32.00	16.51	47.53	15.51	41.00	86.23	136.70	101.43	-16.09	289.48	152.79	129.11	28.00	35.17	36.00	19.34	51.01	15.83	46.00	255
0.18	32.91	69.68	45.85	-18.11	157.46	87.78	63.17	20.00	28.94	31.50	15.10	42.78	13.84	39.00	103.36	166.24	140.45	37.46	295.03	128.79	165.23	24.50	32.89	36.00	17.68	48.10	15.21	45.00	132
0.32	34.99	65.17	41.05	-14.32	144.66	79.49	56.13	14.00	24.29	25.50	9.62	38.95	14.66	36.00	129.42	188.83	149.08	69.44	308.21	119.38	189.66	18.00	28.39	30.50	11.93	44.86	16.46	43.00	84


==> data/mlm_plots/tef/fakenews/xlnet/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	18.22
orig_ge	9.45
adv_pp	40.68
adv_ge	10.38


==> data/mlm_plots/tef/fakenews/xlnet/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.31	-0.07	-0.04	-0.44	0.31	0.37	0.18	0.06	0.24	0.29	-0.11	0.59	0.35	0.50	0.05	0.18	0.21	-0.09	0.45	0.27	0.37	1032
0.03	-0.38	-0.19	-0.16	-0.50	0.12	0.31	0.02	-0.02	0.12	0.15	-0.16	0.41	0.28	0.31	-0.01	0.09	0.11	-0.12	0.30	0.21	0.22	1163
0.06	-0.42	-0.24	-0.21	-0.52	0.04	0.28	-0.03	-0.06	0.05	0.07	-0.18	0.29	0.24	0.19	-0.04	0.04	0.05	-0.13	0.21	0.17	0.14	1482
0.11	-0.43	-0.28	-0.27	-0.52	-0.05	0.23	-0.11	-0.11	0.01	0.03	-0.20	0.21	0.21	0.12	-0.07	0.01	0.02	-0.14	0.16	0.15	0.09	735
0.15	-0.48	-0.36	-0.33	-0.57	-0.15	0.21	-0.24	-0.19	-0.05	-0.07	-0.26	0.15	0.21	0.10	-0.13	-0.04	-0.04	-0.19	0.12	0.15	0.07	255
0.18	-0.59	-0.44	-0.43	-0.66	-0.22	0.22	-0.26	-0.23	-0.08	-0.06	-0.30	0.15	0.23	0.10	-0.16	-0.05	-0.04	-0.22	0.11	0.17	0.08	132
0.32	-0.64	-0.51	-0.50	-0.73	-0.29	0.22	-0.37	-0.30	-0.14	-0.12	-0.33	0.05	0.19	-0.02	-0.21	-0.09	-0.08	-0.23	0.04	0.13	-0.01	84


==> data/mlm_plots/tef/fakenews/xlnet/ig/correlations_auc.tex <==
name	auc
pcc	-0.11
spearman	-0.01
kendall	-0.01


==> data/mlm_plots/tef/fakenews/xlnet/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	13.91	22.65	20.90	10.84	34.45	11.80	28.70	13.66	24.04	22.08	10.84	37.24	13.20	31.83	9.60	19.14	15.18	5.70	32.58	13.44	24.60	1032
0.03	9.58	15.08	13.18	7.30	22.87	7.78	18.78	9.84	16.02	14.05	7.23	24.80	8.79	19.41	8.84	15.74	13.55	6.24	25.23	9.49	20.24	1163
0.06	6.82	9.47	8.62	5.72	13.22	3.75	11.64	6.90	9.93	8.73	5.66	14.19	4.26	12.43	7.47	12.66	10.54	4.92	20.41	7.74	15.51	1482
0.11	5.02	6.64	6.29	4.42	8.87	2.23	7.58	5.03	6.77	6.32	4.40	9.15	2.37	7.95	5.95	9.27	7.78	3.59	14.95	5.68	10.71	735
0.15	4.28	5.03	4.88	3.79	6.27	1.24	5.69	4.35	5.22	5.03	3.85	6.59	1.37	5.95	5.34	8.31	6.78	1.06	15.57	7.26	8.83	255
0.18	3.84	4.55	4.47	3.36	5.73	1.19	5.09	3.78	4.54	4.45	3.37	5.70	1.17	5.14	4.51	6.24	5.56	3.72	8.76	2.52	7.61	132
0.32	3.63	4.09	3.96	2.76	5.41	1.32	4.31	3.52	4.18	4.04	2.71	5.66	1.47	4.55	4.05	5.24	5.30	3.50	6.97	1.73	6.29	84


==> data/mlm_plots/tef/fakenews/xlnet/ig/ets_sts_auc.tex <==
name	auc
et_use	2.13
et_tse	2.20
et_ce	2.70


==> data/mlm_plots/tef/fakenews/xlnet/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.72	5.11	3.91	0.08	10.13	5.02	5.97	8.58	14.43	12.25	5.24	23.62	9.19	17.51	6.75	13.26	10.17	1.93	24.60	11.33	15.39	1032
0.03	1.65	2.83	2.26	0.47	5.19	2.36	3.31	7.38	10.88	9.55	5.16	16.61	5.72	12.83	5.78	9.39	7.94	2.92	15.87	6.47	10.85	1163
0.06	1.02	1.65	1.38	0.16	3.15	1.49	1.94	5.91	8.25	7.68	4.45	12.05	3.80	9.56	4.65	7.07	6.16	2.07	12.07	5.00	7.95	1482
0.11	0.59	0.83	0.76	0.40	1.26	0.43	0.95	4.97	6.35	6.03	4.21	8.50	2.15	7.26	3.93	5.40	4.88	2.15	8.66	3.26	6.13	735
0.15	0.40	0.53	0.48	0.31	0.75	0.22	0.58	4.69	5.75	5.29	3.75	7.76	2.01	6.45	3.57	4.71	4.37	2.50	6.91	2.20	5.20	255
0.18	0.33	0.44	0.39	0.18	0.69	0.25	0.45	4.71	5.67	5.30	2.96	8.38	2.71	5.95	3.67	6.19	4.25	-8.70	21.07	14.88	4.70	132
0.32	0.23	0.38	0.29	0.08	0.67	0.29	0.35	4.02	4.94	4.49	3.36	6.51	1.57	5.38	3.23	4.18	3.70	1.88	6.48	2.30	4.31	84


==> data/mlm_plots/tef/fakenews/xlnet/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.31
et_p_h	2.06
et_p_l2	1.88


==> data/mlm_plots/tef/fakenews/xlnet/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.10	0.13	0.13	0.08	0.19	0.05	0.17	0.04	0.05	0.05	0.03	0.08	0.03	0.07	0.03	0.04	0.04	0.03	0.06	0.02	0.05	1032
0.03	0.19	0.26	0.26	0.16	0.36	0.10	0.33	0.06	0.08	0.08	0.05	0.11	0.03	0.09	0.05	0.06	0.06	0.04	0.08	0.02	0.07	1163
0.06	0.34	0.46	0.44	0.29	0.63	0.17	0.57	0.08	0.10	0.10	0.07	0.14	0.04	0.13	0.07	0.08	0.08	0.06	0.11	0.02	0.10	1482
0.11	0.69	0.88	0.86	0.59	1.16	0.29	1.02	0.11	0.14	0.13	0.09	0.18	0.04	0.16	0.09	0.11	0.10	0.08	0.13	0.03	0.12	735
0.15	1.24	1.43	1.42	0.98	1.87	0.45	1.60	0.13	0.16	0.16	0.12	0.20	0.04	0.19	0.11	0.13	0.12	0.10	0.15	0.03	0.14	255
0.18	1.60	1.88	1.91	1.32	2.44	0.56	2.23	0.15	0.17	0.17	0.12	0.23	0.05	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.16	132
0.32	2.14	2.64	2.53	1.52	3.75	1.11	3.15	0.17	0.20	0.20	0.15	0.26	0.05	0.23	0.14	0.16	0.16	0.13	0.19	0.03	0.18	84


==> data/mlm_plots/tef/fakenews/xlnet/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.46
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/xlnet/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.96	0.98	0.01	0.98	0.97	0.97	0.98	0.96	0.98	0.01	0.98	0.95	0.96	0.97	0.94	0.99	0.02	0.98	1032
0.03	0.95	0.95	0.96	0.94	0.97	0.02	0.97	0.95	0.96	0.96	0.94	0.97	0.02	0.97	0.94	0.95	0.96	0.92	0.98	0.03	0.97	1163
0.06	0.92	0.93	0.93	0.91	0.95	0.02	0.94	0.92	0.93	0.93	0.91	0.95	0.02	0.95	0.92	0.94	0.94	0.91	0.97	0.03	0.96	1482
0.11	0.88	0.90	0.90	0.87	0.92	0.03	0.91	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.89	0.91	0.92	0.88	0.95	0.04	0.94	735
0.15	0.85	0.86	0.86	0.83	0.89	0.03	0.88	0.85	0.86	0.87	0.84	0.89	0.03	0.88	0.87	0.90	0.90	0.85	0.94	0.04	0.92	255
0.18	0.82	0.84	0.84	0.80	0.87	0.03	0.85	0.82	0.83	0.84	0.80	0.87	0.03	0.85	0.85	0.87	0.87	0.84	0.91	0.04	0.90	132
0.32	0.79	0.80	0.81	0.76	0.85	0.04	0.82	0.79	0.81	0.81	0.77	0.85	0.04	0.83	0.83	0.83	0.85	0.76	0.91	0.08	0.88	84


==> data/mlm_plots/tef/fakenews/xlnet/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.28


==> data/mlm_plots/tef/fakenews/xlnet/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	55.07	95.39	64.07	18.06	172.72	77.33	90.59	0.15	5.44	0.58	-6.67	17.54	12.10	6.61	5.61	16.54	12.42	1.52	31.55	15.02	23.22	1032
0.03	79.82	167.85	132.55	62.83	272.87	105.02	265.30	0.22	7.92	0.91	-14.02	29.85	21.94	9.53	6.84	19.42	12.97	1.16	37.67	18.26	26.61	1163
0.06	153.75	232.27	251.79	134.83	329.70	97.43	307.61	0.29	9.53	1.66	-14.53	33.59	24.06	12.04	7.71	20.53	15.61	2.58	38.49	17.95	27.83	1482
0.11	143.33	220.37	237.19	124.91	315.84	95.46	297.91	0.26	10.20	3.19	-7.26	27.67	17.47	15.37	5.16	21.00	14.88	1.55	40.45	19.45	31.79	735
0.15	156.93	222.79	251.24	121.42	324.17	101.37	301.81	0.25	10.09	2.19	-10.81	30.99	20.90	15.64	5.45	22.92	15.01	0.19	45.65	22.73	33.78	255
0.18	126.14	212.60	236.03	104.43	320.77	108.17	302.80	0.13	5.70	0.30	-4.46	15.86	10.16	10.25	5.92	20.65	12.72	-2.51	43.81	23.16	25.02	132
0.32	102.63	206.30	238.89	81.96	330.64	124.34	321.52	0.13	6.62	0.29	-5.33	18.58	11.95	7.86	3.59	22.96	12.59	-8.67	54.58	31.63	25.39	84


==> data/mlm_plots/tef/fakenews/xlnet/ig/time_misc_auc.tex <==
name	auc
attack_time	64.75
l2	2.41
lom	6.60


==> data/mlm_plots/tef/fakenews/xlnet/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.15	0.28	0.27	0.11	0.45	0.17	0.40	0.35	0.45	0.46	0.29	0.62	0.17	0.58	0.54	0.61	0.62	0.47	0.74	0.14	0.70	1032
0.03	0.12	0.21	0.19	0.08	0.34	0.13	0.28	0.31	0.39	0.39	0.26	0.53	0.13	0.47	0.50	0.56	0.57	0.45	0.67	0.11	0.63	1163
0.06	0.10	0.17	0.16	0.06	0.28	0.11	0.23	0.30	0.36	0.36	0.25	0.47	0.11	0.43	0.49	0.54	0.54	0.45	0.63	0.09	0.59	1482
0.11	0.07	0.14	0.12	0.04	0.25	0.10	0.20	0.26	0.33	0.34	0.23	0.44	0.10	0.40	0.48	0.52	0.53	0.44	0.60	0.08	0.57	735
0.15	0.06	0.12	0.10	0.03	0.21	0.09	0.18	0.25	0.32	0.31	0.22	0.42	0.10	0.38	0.45	0.50	0.50	0.42	0.58	0.08	0.56	255
0.18	0.03	0.12	0.09	0.02	0.21	0.10	0.17	0.23	0.31	0.32	0.19	0.42	0.12	0.39	0.43	0.49	0.51	0.39	0.59	0.10	0.57	132
0.32	0.00	0.09	0.07	0.00	0.18	0.09	0.14	0.20	0.28	0.27	0.18	0.38	0.10	0.35	0.43	0.47	0.48	0.40	0.55	0.08	0.52	84


==> data/mlm_plots/tef/fakenews/xlnet/ig/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.10
top50	0.16


==> data/mlm_plots/tef/fakenews/xlnet/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	31.69	42.19	38.77	25.09	59.30	17.11	49.27	29.00	35.81	35.00	24.51	47.11	11.30	41.00	36.47	47.78	44.16	29.46	66.10	18.32	54.96	30.00	36.37	36.00	25.12	47.63	11.26	42.00	1071
0.03	32.51	43.37	40.58	25.86	60.88	17.51	50.68	29.00	35.56	36.00	24.42	46.71	11.15	43.00	41.40	54.37	50.05	33.63	75.10	20.74	63.78	30.00	36.46	36.00	25.30	47.61	11.15	44.00	1510
0.06	33.01	46.25	40.13	20.11	72.38	26.13	51.73	28.00	35.09	35.00	22.26	47.91	12.82	42.00	49.39	66.63	59.43	33.55	99.71	33.08	72.79	30.00	36.47	36.00	23.60	49.34	12.87	44.00	1773
0.11	30.95	51.00	39.25	6.01	95.99	44.99	54.59	22.00	33.56	32.00	14.78	52.33	18.78	39.00	56.57	87.73	76.32	30.95	144.51	56.78	97.56	25.00	35.59	35.00	17.01	54.17	18.58	41.00	560
0.15	33.63	80.12	40.37	-11.05	171.29	91.17	73.93	7.00	24.29	21.00	2.58	45.99	21.71	31.00	86.62	173.34	105.63	-16.28	362.96	189.62	197.18	8.00	26.20	24.50	3.70	48.71	22.50	38.00	108
0.18	34.12	140.64	66.11	-3.26	284.54	143.90	184.18	4.00	16.09	9.00	0.60	31.57	15.49	28.00	125.73	290.74	228.85	91.43	490.06	199.31	377.59	4.00	17.71	10.00	1.04	34.38	16.67	32.00	69
0.32	55.40	143.53	89.74	20.21	266.85	123.32	198.24	3.00	14.27	6.00	-1.47	30.00	15.74	22.00	242.53	396.73	319.46	153.72	639.74	243.01	586.70	4.00	16.04	7.00	-0.93	33.00	16.96	27.00	56


==> data/mlm_plots/tef/fakenews/xlnet/s/comparison_vals_auc.tex <==
name	auc
orig_pp	30.40
orig_ge	7.39
adv_pp	66.73
adv_ge	7.90


==> data/mlm_plots/tef/fakenews/xlnet/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.11	0.31	0.25	0.05	0.58	0.26	0.48	0.34	0.50	0.50	0.26	0.75	0.24	0.70	0.24	0.38	0.36	0.18	0.58	0.20	0.52	1071
0.03	0.03	0.15	0.08	-0.04	0.33	0.18	0.21	0.17	0.35	0.34	0.12	0.57	0.23	0.49	0.12	0.25	0.23	0.07	0.42	0.17	0.34	1510
0.06	0.03	0.13	0.11	-0.02	0.28	0.15	0.20	0.18	0.33	0.34	0.11	0.56	0.22	0.51	0.12	0.24	0.23	0.07	0.40	0.16	0.36	1773
0.11	0.05	0.16	0.12	-0.01	0.33	0.17	0.23	0.23	0.37	0.36	0.14	0.59	0.23	0.52	0.16	0.26	0.26	0.10	0.43	0.17	0.37	560
0.15	0.03	0.17	0.13	-0.08	0.42	0.25	0.27	0.18	0.35	0.36	0.06	0.63	0.28	0.57	0.14	0.26	0.25	0.05	0.46	0.21	0.41	108
0.18	0.03	0.11	0.11	-0.08	0.30	0.19	0.21	0.16	0.31	0.39	-0.00	0.62	0.31	0.50	0.11	0.23	0.26	-0.00	0.46	0.23	0.35	69
0.32	0.05	0.15	0.13	-0.07	0.38	0.22	0.20	0.22	0.33	0.32	0.12	0.53	0.21	0.48	0.15	0.24	0.23	0.08	0.39	0.15	0.33	56


==> data/mlm_plots/tef/fakenews/xlnet/s/correlations_auc.tex <==
name	auc
pcc	0.05
spearman	0.10
kendall	0.08


==> data/mlm_plots/tef/fakenews/xlnet/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	8.82	14.19	13.61	6.61	21.76	7.58	18.35	8.79	14.87	13.78	6.53	23.21	8.34	19.74	6.29	11.86	10.33	3.67	20.04	8.19	15.49	1071
0.03	7.48	10.44	9.62	5.86	15.01	4.57	12.56	7.51	11.12	9.85	5.35	16.88	5.77	13.07	6.60	11.45	9.88	4.60	18.31	6.86	14.33	1510
0.06	5.12	6.75	6.34	4.22	9.28	2.53	7.90	5.15	7.14	6.80	4.19	10.09	2.95	8.61	5.54	8.71	7.57	3.80	13.62	4.91	10.52	1773
0.11	3.40	4.32	4.40	3.05	5.58	1.27	4.98	3.38	4.39	4.30	2.67	6.11	1.72	5.09	4.16	5.91	5.50	2.89	8.93	3.02	7.02	560
0.15	2.64	3.32	3.29	2.05	4.59	1.27	4.25	2.46	3.40	3.11	1.71	5.10	1.69	4.23	3.37	5.31	4.80	1.51	9.12	3.80	6.66	108
0.18	2.42	3.03	2.80	1.92	4.14	1.11	3.38	2.32	3.31	2.85	1.84	4.77	1.47	3.61	3.06	6.48	4.24	-0.21	13.16	6.68	5.75	69
0.32	1.77	2.36	2.30	1.35	3.36	1.01	2.73	1.79	2.44	2.19	1.25	3.64	1.19	2.84	1.82	3.92	3.13	-1.08	8.91	4.99	4.90	56


==> data/mlm_plots/tef/fakenews/xlnet/s/ets_sts_auc.tex <==
name	auc
et_use	1.41
et_tse	1.48
et_ce	2.03


==> data/mlm_plots/tef/fakenews/xlnet/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.72	3.13	2.56	-1.29	7.54	4.42	3.69	5.28	8.94	7.97	2.89	14.99	6.05	11.07	4.00	8.14	6.36	0.50	15.78	7.64	9.37	1071
0.03	1.27	1.87	1.77	1.00	2.73	0.87	2.33	5.47	7.55	7.12	4.14	10.96	3.41	8.94	4.26	6.44	5.76	2.38	10.50	4.06	7.62	1510
0.06	0.76	1.15	0.99	-2.44	4.74	3.59	1.26	4.45	5.74	5.44	3.61	7.87	2.13	6.67	3.47	4.82	4.31	2.46	7.17	2.36	5.63	1773
0.11	0.38	0.61	0.48	0.11	1.11	0.50	0.68	3.22	4.39	3.87	1.45	7.32	2.93	4.98	2.39	3.70	3.00	0.27	7.13	3.43	4.13	560
0.15	0.20	0.65	0.28	-1.33	2.63	1.98	0.37	2.66	3.83	3.04	0.00	7.65	3.83	3.61	1.99	4.51	2.40	-7.79	16.81	12.30	2.92	108
0.18	0.16	0.71	0.22	-0.92	2.34	1.63	0.40	2.62	4.78	3.08	0.39	9.17	4.39	4.63	2.13	5.45	2.57	-1.92	12.82	7.37	4.15	69
0.32	0.12	0.35	0.17	-0.24	0.94	0.59	0.25	1.97	3.60	3.18	0.71	6.49	2.89	4.16	1.51	4.35	2.54	-2.97	11.66	7.32	3.69	56


==> data/mlm_plots/tef/fakenews/xlnet/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.26
et_p_h	1.50
et_p_l2	1.53


==> data/mlm_plots/tef/fakenews/xlnet/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.10	0.14	0.14	0.09	0.19	0.05	0.17	0.04	0.06	0.06	0.03	0.08	0.03	0.07	0.03	0.05	0.05	0.03	0.06	0.02	0.06	1071
0.03	0.20	0.26	0.25	0.17	0.36	0.09	0.32	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.05	0.06	0.06	0.04	0.08	0.02	0.07	1510
0.06	0.34	0.47	0.44	0.29	0.64	0.18	0.56	0.08	0.10	0.10	0.07	0.14	0.03	0.12	0.07	0.08	0.08	0.06	0.10	0.02	0.09	1773
0.11	0.68	0.86	0.83	0.54	1.18	0.32	1.04	0.11	0.14	0.14	0.09	0.19	0.05	0.16	0.09	0.11	0.11	0.08	0.14	0.03	0.13	560
0.15	1.11	1.54	1.40	0.79	2.30	0.75	1.87	0.14	0.18	0.18	0.11	0.25	0.07	0.21	0.12	0.14	0.14	0.09	0.19	0.05	0.17	108
0.18	1.11	1.94	1.92	0.67	3.21	1.27	2.28	0.10	0.16	0.17	0.07	0.25	0.09	0.20	0.09	0.13	0.14	0.08	0.19	0.06	0.16	69
0.32	1.53	2.57	2.46	1.05	4.08	1.51	3.49	0.12	0.18	0.17	0.09	0.27	0.09	0.23	0.10	0.15	0.14	0.10	0.20	0.05	0.18	56


==> data/mlm_plots/tef/fakenews/xlnet/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.46
pp_l2_d	0.05
pp_h_d	0.04


==> data/mlm_plots/tef/fakenews/xlnet/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.96	0.98	0.01	0.98	0.97	0.97	0.98	0.96	0.98	0.01	0.98	0.95	0.96	0.97	0.94	0.99	0.03	0.98	1071
0.03	0.94	0.95	0.95	0.94	0.97	0.01	0.96	0.94	0.96	0.96	0.94	0.97	0.02	0.97	0.94	0.95	0.96	0.93	0.98	0.03	0.97	1510
0.06	0.92	0.93	0.93	0.91	0.95	0.02	0.94	0.92	0.93	0.93	0.91	0.95	0.02	0.95	0.92	0.94	0.94	0.91	0.97	0.03	0.96	1773
0.11	0.89	0.90	0.90	0.88	0.92	0.02	0.91	0.88	0.90	0.90	0.88	0.92	0.02	0.91	0.90	0.92	0.92	0.88	0.95	0.03	0.94	560
0.15	0.85	0.87	0.86	0.83	0.90	0.03	0.89	0.84	0.86	0.86	0.82	0.91	0.05	0.89	0.87	0.90	0.91	0.84	0.95	0.05	0.93	108
0.18	0.82	0.84	0.83	0.80	0.88	0.04	0.86	0.81	0.85	0.84	0.80	0.89	0.05	0.89	0.85	0.89	0.90	0.82	0.95	0.06	0.92	69
0.32	0.78	0.81	0.80	0.75	0.86	0.05	0.84	0.77	0.81	0.80	0.75	0.86	0.05	0.85	0.79	0.84	0.85	0.74	0.93	0.10	0.91	56


==> data/mlm_plots/tef/fakenews/xlnet/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.28


==> data/mlm_plots/tef/fakenews/xlnet/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	37.57	79.69	51.50	5.68	153.70	74.01	81.46	8.31	77.47	16.11	-346.65	501.59	424.12	34.30	12.47	36.36	27.26	6.34	66.37	30.02	55.52	1071
0.03	118.54	187.86	195.88	99.62	276.10	88.24	256.50	14.65	84.35	25.83	-266.15	434.85	350.50	53.65	14.23	39.26	31.17	7.64	70.87	31.62	58.31	1510
0.06	168.87	216.02	222.78	135.55	296.48	80.47	271.13	17.11	146.72	31.07	-409.23	702.68	555.96	58.11	14.23	39.30	27.84	6.01	72.59	33.29	59.35	1773
0.11	128.66	199.80	204.72	107.23	292.37	92.57	284.31	16.53	147.20	31.24	-331.34	625.75	478.55	73.12	10.68	32.69	24.92	4.95	60.42	27.74	45.20	560
0.15	27.40	110.11	83.69	12.95	207.27	97.16	173.57	9.02	869.33	33.05	-1664.34	3403.00	2533.67	97.54	3.84	19.58	13.98	-0.20	39.36	19.78	29.20	108
0.18	16.37	96.79	39.50	-16.57	210.15	113.36	121.44	8.84	277.70	12.95	-456.68	1012.09	734.39	189.37	2.99	12.26	7.10	-2.31	26.84	14.57	15.07	69
0.32	11.03	72.82	24.37	-23.29	168.93	96.11	65.34	4.25	298.08	11.63	-438.80	1034.96	736.88	58.30	0.66	9.07	5.03	-4.70	22.83	13.76	11.73	56


==> data/mlm_plots/tef/fakenews/xlnet/s/time_misc_auc.tex <==
name	auc
attack_time	40.20
l2	93.55
lom	6.75


==> data/mlm_plots/tef/fakenews/xlnet/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.15	0.31	0.27	0.10	0.52	0.21	0.44	0.41	0.53	0.52	0.38	0.69	0.16	0.64	0.61	0.69	0.68	0.58	0.79	0.11	0.76	1071
0.03	0.07	0.19	0.14	0.03	0.34	0.16	0.24	0.34	0.44	0.42	0.30	0.57	0.13	0.51	0.56	0.62	0.61	0.53	0.72	0.09	0.68	1510
0.06	0.07	0.18	0.14	0.04	0.32	0.14	0.26	0.34	0.43	0.42	0.30	0.56	0.13	0.51	0.55	0.62	0.62	0.53	0.71	0.09	0.68	1773
0.11	0.10	0.21	0.19	0.07	0.36	0.14	0.30	0.35	0.45	0.44	0.32	0.58	0.13	0.52	0.57	0.63	0.63	0.54	0.73	0.10	0.70	560
0.15	0.00	0.19	0.12	-0.03	0.40	0.21	0.30	0.34	0.44	0.44	0.25	0.63	0.19	0.55	0.57	0.63	0.64	0.52	0.75	0.11	0.70	108
0.18	0.00	0.12	0.05	-0.03	0.26	0.14	0.21	0.33	0.42	0.43	0.29	0.56	0.14	0.51	0.56	0.61	0.62	0.45	0.76	0.16	0.71	69
0.32	0.00	0.13	0.00	-0.10	0.37	0.23	0.14	0.29	0.41	0.39	0.26	0.55	0.14	0.48	0.55	0.63	0.64	0.53	0.72	0.09	0.69	56


==> data/mlm_plots/tef/fakenews/xlnet/s/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.13
top50	0.19


==> data/mlm_plots/tef/imdb/bert/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	49.37	68.81	63.03	40.15	97.46	28.65	82.50	33.00	40.14	40.00	29.09	51.18	11.04	48.00	55.03	75.68	69.95	45.66	105.69	30.01	90.21	33.00	40.36	41.00	29.29	51.42	11.06	48.00	949
0.03	49.69	69.81	63.35	39.94	99.67	29.87	84.38	31.00	38.94	39.00	27.05	50.83	11.89	47.00	63.28	85.74	78.94	52.42	119.07	33.33	103.07	32.00	39.40	40.00	27.43	51.37	11.97	48.00	990
0.06	49.60	69.94	63.86	40.17	99.71	29.77	85.25	32.00	39.41	41.00	27.35	51.47	12.06	48.00	76.86	104.14	97.57	66.46	141.83	37.68	123.83	32.00	40.30	41.00	28.12	52.48	12.18	49.00	1118
0.11	49.43	67.51	61.81	39.50	95.51	28.01	80.10	30.75	38.88	39.00	26.48	51.28	12.40	48.00	96.63	124.81	118.00	81.27	168.36	43.54	144.93	32.00	40.21	41.00	27.58	52.85	12.64	49.00	1644
0.15	49.78	70.03	63.68	40.20	99.86	29.83	84.61	32.00	39.16	40.00	27.10	51.23	12.06	47.00	131.70	168.85	160.66	115.18	222.52	53.67	197.01	33.00	41.03	42.00	28.76	53.30	12.27	49.00	1449
0.18	50.15	71.62	64.61	41.12	102.12	30.50	86.80	30.00	38.03	39.00	26.32	49.74	11.71	46.00	167.35	214.39	204.07	148.05	280.74	66.34	247.19	33.00	40.40	42.00	28.20	52.60	12.20	49.00	944
0.32	50.01	71.96	63.99	40.03	103.90	31.93	87.68	30.00	38.32	39.00	26.25	50.39	12.07	48.00	212.59	285.99	264.76	188.17	383.82	97.82	339.53	33.00	41.37	42.00	28.57	54.17	12.80	51.00	836


==> data/mlm_plots/tef/imdb/bert/a/comparison_vals_auc.tex <==
name	auc
orig_pp	21.88
orig_ge	12.01
adv_pp	56.74
adv_ge	12.60


==> data/mlm_plots/tef/imdb/bert/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.01	0.24	0.08	-0.06	0.54	0.30	0.54	0.61	0.69	0.70	0.54	0.83	0.14	0.78	0.45	0.53	0.54	0.39	0.67	0.14	0.62	949
0.03	-0.01	0.13	-0.00	-0.11	0.38	0.24	0.17	0.52	0.62	0.64	0.46	0.78	0.16	0.73	0.37	0.47	0.48	0.33	0.62	0.14	0.58	990
0.06	-0.02	0.04	-0.01	-0.12	0.21	0.17	0.01	0.43	0.56	0.59	0.38	0.74	0.18	0.70	0.31	0.42	0.43	0.27	0.57	0.15	0.54	1118
0.11	-0.05	-0.01	-0.02	-0.12	0.11	0.11	-0.01	0.39	0.52	0.53	0.33	0.70	0.19	0.66	0.28	0.39	0.38	0.23	0.54	0.15	0.50	1644
0.15	-0.08	-0.04	-0.03	-0.13	0.06	0.09	-0.02	0.33	0.46	0.48	0.25	0.67	0.21	0.61	0.23	0.34	0.35	0.17	0.50	0.16	0.46	1449
0.18	-0.09	-0.05	-0.03	-0.14	0.05	0.10	-0.02	0.26	0.41	0.46	0.18	0.65	0.24	0.60	0.18	0.31	0.33	0.13	0.49	0.18	0.45	944
0.32	-0.10	-0.06	-0.03	-0.15	0.03	0.09	-0.02	0.12	0.34	0.40	0.05	0.62	0.29	0.58	0.08	0.25	0.28	0.04	0.46	0.21	0.43	836


==> data/mlm_plots/tef/imdb/bert/a/correlations_auc.tex <==
name	auc
pcc	-0.00
spearman	0.14
kendall	0.11


==> data/mlm_plots/tef/imdb/bert/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	6.64	11.49	10.80	5.07	17.92	6.42	14.91	5.45	10.15	8.88	3.43	16.88	6.72	13.10	5.68	12.57	9.82	2.99	22.14	9.57	16.89	949
0.03	5.17	6.87	6.74	3.88	9.85	2.98	8.25	4.41	6.12	5.85	3.29	8.96	2.83	7.53	4.80	9.13	7.40	2.49	15.77	6.64	11.24	990
0.06	3.95	4.69	4.61	3.28	6.09	1.40	5.39	3.49	4.37	4.26	2.89	5.84	1.47	5.12	4.11	6.78	5.70	2.28	11.29	4.51	7.94	1118
0.11	3.18	3.74	3.69	2.86	4.62	0.88	4.20	2.93	3.57	3.43	2.59	4.56	0.98	4.10	3.63	5.76	4.76	2.01	9.52	3.76	6.69	1644
0.15	2.60	2.97	2.90	2.40	3.54	0.57	3.29	2.50	2.90	2.80	2.26	3.53	0.63	3.20	3.04	4.35	3.90	2.19	6.51	2.16	5.19	1449
0.18	2.27	2.58	2.52	2.11	3.04	0.46	2.80	2.21	2.52	2.44	2.02	3.03	0.51	2.75	2.57	3.62	3.25	1.84	5.40	1.78	4.19	944
0.32	2.03	2.27	2.23	1.90	2.64	0.37	2.46	1.98	2.24	2.19	1.85	2.64	0.39	2.44	2.19	2.97	2.76	1.84	4.11	1.13	3.51	836


==> data/mlm_plots/tef/imdb/bert/a/ets_sts_auc.tex <==
name	auc
et_use	1.13
et_tse	1.06
et_ce	1.56


==> data/mlm_plots/tef/imdb/bert/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.30	6.87	3.60	-10.21	23.95	17.08	6.33	8.25	17.14	12.91	3.75	30.54	13.39	21.89	7.23	17.95	12.91	1.55	34.34	16.39	23.48	949
0.03	1.26	3.36	1.83	-8.58	15.30	11.94	2.74	6.91	11.21	9.33	3.66	18.76	7.55	13.44	5.71	11.37	8.36	1.07	21.66	10.30	13.68	990
0.06	0.71	1.16	0.93	-0.45	2.78	1.62	1.28	5.49	7.49	6.91	4.21	10.78	3.29	8.49	4.50	7.03	6.03	2.38	11.67	4.65	7.84	1118
0.11	0.45	0.66	0.56	0.24	1.07	0.41	0.74	4.80	5.97	5.61	4.03	7.91	1.94	6.76	3.87	5.31	4.75	2.76	7.86	2.55	6.02	1644
0.15	0.27	0.39	0.35	0.04	0.75	0.36	0.46	4.12	4.92	4.71	3.62	6.21	1.29	5.55	3.36	4.26	3.98	2.70	5.83	1.56	4.77	1449
0.18	0.20	0.27	0.25	0.15	0.39	0.12	0.32	3.77	4.49	4.31	3.33	5.65	1.16	5.02	3.07	3.88	3.57	2.51	5.24	1.36	4.33	944
0.32	0.13	0.19	0.18	0.10	0.28	0.09	0.22	3.32	3.92	3.81	3.03	4.81	0.89	4.32	2.71	3.36	3.19	2.30	4.42	1.06	3.67	836


==> data/mlm_plots/tef/imdb/bert/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.28
et_p_h	1.85
et_p_l2	1.70


==> data/mlm_plots/tef/imdb/bert/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.11	0.10	0.05	0.18	0.07	0.16	0.02	0.03	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.01	0.05	0.02	0.04	949
0.03	0.16	0.25	0.24	0.12	0.38	0.13	0.32	0.03	0.05	0.05	0.03	0.08	0.03	0.07	0.03	0.05	0.05	0.03	0.07	0.02	0.06	990
0.06	0.39	0.54	0.52	0.32	0.75	0.22	0.66	0.06	0.08	0.08	0.05	0.12	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.09	1118
0.11	0.68	0.92	0.91	0.58	1.25	0.34	1.10	0.09	0.11	0.11	0.07	0.14	0.03	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.11	1644
0.15	1.14	1.56	1.49	0.97	2.15	0.59	1.88	0.11	0.13	0.13	0.09	0.17	0.04	0.15	0.09	0.11	0.11	0.09	0.14	0.03	0.13	1449
0.18	1.61	2.20	2.10	1.37	3.02	0.83	2.60	0.12	0.15	0.15	0.11	0.18	0.04	0.17	0.11	0.12	0.12	0.10	0.15	0.03	0.14	944
0.32	2.37	3.32	3.06	1.88	4.75	1.44	3.91	0.14	0.17	0.17	0.13	0.21	0.04	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.16	836


==> data/mlm_plots/tef/imdb/bert/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.54
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/bert/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.96	0.95	0.98	0.01	0.97	0.94	0.96	0.96	0.94	0.97	0.02	0.97	0.95	0.96	0.96	0.93	0.98	0.03	0.98	949
0.03	0.92	0.93	0.93	0.91	0.95	0.02	0.94	0.91	0.92	0.92	0.90	0.95	0.03	0.94	0.92	0.94	0.94	0.90	0.97	0.04	0.96	990
0.06	0.88	0.89	0.89	0.87	0.92	0.02	0.91	0.87	0.88	0.88	0.85	0.91	0.03	0.90	0.89	0.91	0.92	0.87	0.95	0.04	0.94	1118
0.11	0.84	0.86	0.86	0.83	0.89	0.03	0.88	0.83	0.85	0.85	0.82	0.88	0.03	0.87	0.86	0.89	0.89	0.84	0.94	0.05	0.92	1644
0.15	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.79	0.81	0.81	0.78	0.85	0.03	0.84	0.83	0.86	0.87	0.81	0.91	0.05	0.90	1449
0.18	0.77	0.79	0.79	0.76	0.82	0.03	0.81	0.77	0.79	0.79	0.75	0.82	0.03	0.81	0.80	0.83	0.84	0.77	0.89	0.06	0.87	944
0.32	0.74	0.76	0.76	0.73	0.79	0.03	0.78	0.73	0.76	0.76	0.72	0.79	0.03	0.78	0.76	0.80	0.81	0.73	0.87	0.07	0.85	836


==> data/mlm_plots/tef/imdb/bert/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/imdb/bert/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	6.80	8.40	8.29	5.97	10.82	2.42	9.60	0.07	0.56	0.59	0.15	0.96	0.41	0.93	4.11	26.32	15.63	-2.42	55.07	28.74	40.42	949
0.03	6.48	8.27	8.12	5.55	10.98	2.72	9.62	0.35	0.63	0.70	0.25	1.01	0.38	0.96	5.79	28.53	18.43	0.09	56.98	28.45	43.20	990
0.06	9.93	15.05	12.80	6.52	23.57	8.52	16.63	0.48	0.67	0.72	0.34	1.00	0.33	0.95	8.13	31.88	22.79	2.90	60.87	28.99	47.73	1118
0.11	15.50	24.02	21.44	12.61	35.43	11.41	30.36	0.48	0.67	0.68	0.37	0.96	0.29	0.93	11.05	33.16	27.40	6.35	59.96	26.81	48.37	1644
0.15	21.81	28.69	27.63	18.66	38.73	10.03	35.01	0.44	0.61	0.62	0.33	0.88	0.27	0.80	8.86	29.43	23.98	3.65	55.20	25.78	40.96	1449
0.18	23.88	30.71	30.22	20.60	40.81	10.10	36.44	0.41	0.59	0.60	0.29	0.89	0.30	0.81	9.88	28.98	22.16	3.81	54.15	25.17	41.48	944
0.32	27.50	35.54	33.90	23.64	47.45	11.91	42.09	0.30	0.52	0.54	0.21	0.84	0.32	0.76	7.33	24.50	18.18	1.61	47.39	22.89	35.29	836


==> data/mlm_plots/tef/imdb/bert/a/time_misc_auc.tex <==
name	auc
attack_time	8.10
l2	0.19
lom	8.97


==> data/mlm_plots/tef/imdb/bert/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.42	0.55	0.57	0.35	0.75	0.20	0.70	0.63	0.70	0.72	0.58	0.83	0.13	0.79	0.72	0.77	0.78	0.69	0.85	0.08	0.83	949
0.03	0.33	0.49	0.50	0.28	0.69	0.20	0.64	0.58	0.66	0.68	0.53	0.80	0.13	0.77	0.68	0.74	0.74	0.65	0.82	0.09	0.80	990
0.06	0.27	0.43	0.45	0.23	0.64	0.20	0.59	0.53	0.64	0.66	0.50	0.77	0.14	0.75	0.65	0.71	0.72	0.62	0.80	0.09	0.78	1118
0.11	0.24	0.38	0.38	0.19	0.57	0.19	0.52	0.51	0.61	0.62	0.47	0.75	0.14	0.72	0.63	0.69	0.69	0.60	0.78	0.09	0.76	1644
0.15	0.19	0.34	0.33	0.15	0.53	0.19	0.50	0.47	0.57	0.59	0.42	0.72	0.15	0.69	0.60	0.67	0.67	0.57	0.76	0.10	0.74	1449
0.18	0.16	0.32	0.31	0.13	0.52	0.19	0.48	0.44	0.55	0.57	0.38	0.72	0.17	0.69	0.58	0.65	0.67	0.55	0.76	0.11	0.74	944
0.32	0.14	0.29	0.29	0.10	0.48	0.19	0.43	0.37	0.51	0.54	0.33	0.70	0.18	0.67	0.53	0.63	0.64	0.50	0.75	0.12	0.73	836


==> data/mlm_plots/tef/imdb/bert/a/top_intersections_auc.tex <==
name	auc
top10	0.11
top30	0.18
top50	0.21


==> data/mlm_plots/tef/imdb/bert/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	49.29	68.57	62.82	40.16	96.98	28.41	82.59	32.00	39.81	40.00	28.62	51.01	11.19	48.00	54.77	75.65	69.59	45.31	105.99	30.34	90.74	32.00	40.07	40.00	28.85	51.28	11.21	48.00	944
0.03	49.89	69.93	63.68	40.25	99.61	29.68	84.27	31.00	39.03	39.00	26.89	51.16	12.13	47.00	62.09	85.57	78.42	51.91	119.23	33.66	103.55	32.00	39.52	40.00	27.30	51.75	12.23	48.00	1007
0.06	49.41	69.99	63.61	39.99	99.99	30.00	84.04	30.00	38.56	39.00	26.37	50.75	12.19	47.00	75.46	102.74	94.74	63.21	142.27	39.53	122.33	31.00	39.41	40.00	27.06	51.76	12.35	48.00	1150
0.11	49.26	68.79	62.85	38.86	98.72	29.93	82.50	31.00	39.04	39.00	27.21	50.87	11.83	47.00	93.48	124.61	116.64	79.88	169.35	44.74	148.19	32.00	40.33	41.00	28.18	52.48	12.15	49.00	1361
0.15	48.79	68.70	62.72	39.59	97.82	29.11	84.96	32.00	39.48	40.00	27.53	51.42	11.94	48.00	124.10	163.83	152.87	107.44	220.23	56.39	193.91	33.00	41.27	42.00	29.06	53.48	12.21	50.00	1360
0.18	50.00	70.02	64.00	40.15	99.89	29.87	83.18	30.00	38.50	39.00	26.29	50.72	12.22	47.00	164.62	207.78	194.45	140.69	274.88	67.09	239.12	33.00	40.91	42.00	28.42	53.40	12.49	50.00	945
0.32	52.25	73.45	64.59	43.50	103.40	29.95	90.03	30.00	38.78	40.00	25.79	51.78	12.99	48.00	212.72	279.67	259.31	183.01	376.33	96.66	326.40	33.00	41.76	43.00	28.28	55.24	13.48	51.00	792


==> data/mlm_plots/tef/imdb/bert/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	21.85
orig_ge	12.07
adv_pp	55.49
adv_ge	12.65


==> data/mlm_plots/tef/imdb/bert/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.15	0.06	0.06	-0.28	0.39	0.33	0.30	-0.01	0.17	0.20	-0.12	0.45	0.29	0.38	-0.01	0.12	0.14	-0.09	0.34	0.21	0.28	944
0.03	-0.31	-0.13	-0.12	-0.44	0.18	0.31	0.07	-0.14	0.04	0.06	-0.24	0.33	0.29	0.27	-0.10	0.04	0.04	-0.18	0.25	0.21	0.19	1007
0.06	-0.47	-0.30	-0.28	-0.58	-0.02	0.28	-0.12	-0.26	-0.08	-0.07	-0.35	0.19	0.27	0.13	-0.18	-0.05	-0.05	-0.25	0.15	0.20	0.10	1150
0.11	-0.55	-0.40	-0.40	-0.64	-0.16	0.24	-0.24	-0.33	-0.16	-0.17	-0.41	0.09	0.25	0.02	-0.23	-0.11	-0.12	-0.29	0.07	0.18	0.02	1361
0.15	-0.62	-0.47	-0.46	-0.69	-0.26	0.22	-0.34	-0.38	-0.22	-0.22	-0.46	0.01	0.24	-0.05	-0.27	-0.16	-0.16	-0.33	0.02	0.18	-0.03	1360
0.18	-0.62	-0.49	-0.49	-0.68	-0.29	0.20	-0.37	-0.40	-0.23	-0.22	-0.45	-0.02	0.21	-0.07	-0.29	-0.16	-0.15	-0.32	-0.01	0.16	-0.05	945
0.32	-0.58	-0.46	-0.46	-0.64	-0.29	0.17	-0.35	-0.30	-0.19	-0.18	-0.37	-0.02	0.17	-0.07	-0.21	-0.13	-0.13	-0.26	-0.01	0.13	-0.04	792


==> data/mlm_plots/tef/imdb/bert/ig/correlations_auc.tex <==
name	auc
pcc	-0.12
spearman	-0.05
kendall	-0.03


==> data/mlm_plots/tef/imdb/bert/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	9.09	14.57	12.66	6.42	22.73	8.15	17.94	7.51	12.97	10.73	4.71	21.23	8.26	16.01	7.94	17.02	12.89	4.25	29.79	12.77	22.10	944
0.03	6.33	9.17	8.43	5.27	13.06	3.90	11.17	5.44	8.28	7.48	4.28	12.28	4.00	10.09	6.56	13.24	10.23	3.19	23.28	10.05	16.13	1007
0.06	5.04	6.76	6.29	4.18	9.34	2.58	7.99	4.55	6.43	5.81	3.27	9.59	3.16	7.57	5.89	11.43	8.33	1.80	21.06	9.63	13.25	1150
0.11	4.22	5.27	5.13	3.85	6.70	1.43	5.97	3.97	5.07	4.86	3.56	6.58	1.51	5.92	5.17	8.65	7.01	2.97	14.34	5.69	10.08	1361
0.15	3.55	4.25	4.14	3.28	5.21	0.96	4.81	3.37	4.15	4.03	3.05	5.26	1.11	4.83	4.32	6.72	5.72	2.46	10.97	4.26	7.68	1360
0.18	3.11	3.70	3.58	2.89	4.51	0.81	4.19	3.05	3.68	3.55	2.77	4.59	0.91	4.17	3.72	5.68	4.92	2.70	8.65	2.97	6.74	945
0.32	2.69	3.14	3.07	2.54	3.74	0.60	3.49	2.62	3.12	3.03	2.46	3.78	0.66	3.52	2.99	4.13	3.75	2.46	5.81	1.68	4.77	792


==> data/mlm_plots/tef/imdb/bert/ig/ets_sts_auc.tex <==
name	auc
et_use	1.57
et_tse	1.50
et_ce	2.36


==> data/mlm_plots/tef/imdb/bert/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.69	11.10	4.34	-20.33	42.52	31.42	7.77	10.12	20.51	16.43	6.13	34.90	14.39	26.80	9.00	20.96	16.44	4.36	37.55	16.60	27.60	944
0.03	1.69	3.71	2.38	-6.10	13.52	9.81	3.50	8.71	14.10	11.89	5.64	22.57	8.47	16.99	7.28	13.78	10.49	3.36	24.20	10.42	16.40	1007
0.06	1.00	1.67	1.28	-0.94	4.28	2.61	1.81	7.30	10.28	9.19	5.83	14.73	4.45	12.25	5.93	9.51	7.92	3.92	15.10	5.59	11.20	1150
0.11	0.63	0.95	0.81	0.10	1.80	0.85	1.08	6.45	8.34	7.84	5.53	11.15	2.81	9.62	5.26	7.29	6.47	3.91	10.68	3.38	8.47	1361
0.15	0.40	0.55	0.50	0.32	0.79	0.24	0.65	5.72	7.09	6.69	5.04	9.14	2.05	7.99	4.65	6.12	5.61	3.90	8.33	2.22	7.00	1360
0.18	0.29	0.39	0.36	0.22	0.57	0.18	0.45	5.20	6.30	6.05	4.71	7.88	1.59	7.10	4.23	5.40	5.00	3.71	7.08	1.68	6.23	945
0.32	0.20	0.28	0.25	0.14	0.41	0.14	0.33	4.66	5.58	5.43	4.25	6.90	1.33	6.32	3.77	4.79	4.56	3.40	6.17	1.39	5.50	792


==> data/mlm_plots/tef/imdb/bert/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.39
et_p_h	2.52
et_p_l2	2.27


==> data/mlm_plots/tef/imdb/bert/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.11	0.11	0.05	0.18	0.07	0.16	0.02	0.03	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.01	0.05	0.02	0.04	944
0.03	0.16	0.24	0.23	0.13	0.36	0.12	0.31	0.03	0.06	0.05	0.03	0.08	0.03	0.07	0.03	0.05	0.05	0.03	0.07	0.02	0.06	1007
0.06	0.37	0.50	0.49	0.31	0.70	0.20	0.62	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	1150
0.11	0.65	0.89	0.84	0.55	1.23	0.34	1.09	0.09	0.11	0.11	0.07	0.14	0.04	0.13	0.07	0.09	0.09	0.07	0.11	0.02	0.10	1361
0.15	1.15	1.50	1.46	1.00	2.01	0.51	1.78	0.11	0.13	0.13	0.09	0.17	0.04	0.15	0.09	0.11	0.11	0.08	0.13	0.02	0.12	1360
0.18	1.66	2.13	2.08	1.45	2.82	0.69	2.48	0.12	0.15	0.15	0.11	0.18	0.03	0.17	0.11	0.12	0.12	0.10	0.15	0.02	0.14	945
0.32	2.30	3.02	2.87	1.96	4.08	1.06	3.58	0.14	0.16	0.16	0.13	0.20	0.03	0.19	0.12	0.14	0.13	0.11	0.16	0.02	0.15	792


==> data/mlm_plots/tef/imdb/bert/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.51
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/bert/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.96	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.97	0.02	0.97	0.95	0.96	0.97	0.93	0.99	0.03	0.98	944
0.03	0.92	0.93	0.93	0.91	0.95	0.02	0.95	0.91	0.92	0.93	0.90	0.95	0.03	0.94	0.92	0.94	0.94	0.91	0.97	0.03	0.96	1007
0.06	0.88	0.90	0.90	0.87	0.92	0.02	0.91	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.90	0.92	0.92	0.88	0.96	0.04	0.95	1150
0.11	0.84	0.86	0.86	0.84	0.89	0.03	0.88	0.83	0.85	0.86	0.82	0.89	0.03	0.88	0.87	0.90	0.90	0.85	0.94	0.05	0.93	1361
0.15	0.81	0.82	0.82	0.80	0.85	0.02	0.84	0.80	0.82	0.82	0.78	0.85	0.03	0.84	0.84	0.87	0.87	0.81	0.92	0.05	0.90	1360
0.18	0.78	0.79	0.79	0.77	0.82	0.03	0.81	0.77	0.79	0.79	0.76	0.82	0.03	0.82	0.81	0.84	0.85	0.79	0.90	0.06	0.89	945
0.32	0.74	0.76	0.76	0.73	0.79	0.03	0.78	0.74	0.76	0.76	0.73	0.79	0.03	0.78	0.77	0.80	0.81	0.74	0.87	0.07	0.84	792


==> data/mlm_plots/tef/imdb/bert/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/imdb/bert/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	16.97	20.05	20.20	15.63	24.48	4.43	23.15	0.15	11.04	5.23	-2.04	24.12	13.08	19.96	6.61	20.59	15.06	1.58	39.60	19.01	28.29	944
0.03	9.55	12.85	11.90	4.59	21.11	8.26	14.02	0.18	11.94	5.30	-2.20	26.08	14.14	21.37	8.71	23.12	16.95	2.45	43.79	20.67	31.64	1007
0.06	14.31	25.61	18.31	2.35	48.87	23.26	23.33	0.17	11.34	3.07	-3.77	26.45	15.11	20.50	8.47	24.61	19.34	3.23	45.99	21.38	34.71	1150
0.11	19.17	42.96	26.01	8.85	77.08	34.12	72.48	0.16	11.41	2.69	-3.92	26.73	15.33	21.53	9.64	26.72	20.32	4.53	48.92	22.19	38.23	1361
0.15	60.74	77.50	77.36	54.68	100.31	22.82	95.42	0.21	12.47	3.43	-3.54	28.48	16.01	22.22	7.98	26.99	20.61	2.66	51.31	24.32	37.89	1360
0.18	68.02	83.53	84.91	61.77	105.29	21.76	98.88	0.30	15.01	8.89	-1.46	31.48	16.47	26.14	11.08	28.25	21.59	4.60	51.90	23.65	39.57	945
0.32	75.80	90.58	91.78	69.07	112.10	21.51	104.93	3.29	20.08	18.79	2.83	37.32	17.24	29.11	7.29	23.33	18.19	2.38	44.28	20.95	32.03	792


==> data/mlm_plots/tef/imdb/bert/ig/time_misc_auc.tex <==
name	auc
attack_time	19.74
l2	4.48
lom	7.98


==> data/mlm_plots/tef/imdb/bert/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.14	0.28	0.27	0.11	0.45	0.17	0.41	0.32	0.42	0.42	0.28	0.55	0.14	0.52	0.50	0.57	0.57	0.46	0.67	0.11	0.64	944
0.03	0.09	0.21	0.19	0.06	0.37	0.16	0.32	0.26	0.36	0.36	0.23	0.50	0.14	0.47	0.46	0.52	0.53	0.42	0.63	0.11	0.60	1007
0.06	0.05	0.15	0.14	0.02	0.27	0.13	0.24	0.22	0.31	0.31	0.19	0.44	0.13	0.41	0.42	0.49	0.49	0.39	0.59	0.10	0.56	1150
0.11	0.00	0.11	0.08	-0.00	0.21	0.11	0.18	0.19	0.28	0.27	0.16	0.39	0.12	0.35	0.40	0.46	0.46	0.37	0.55	0.09	0.53	1361
0.15	0.00	0.08	0.06	-0.01	0.17	0.09	0.14	0.17	0.25	0.24	0.14	0.36	0.11	0.33	0.38	0.44	0.44	0.35	0.53	0.09	0.51	1360
0.18	0.00	0.07	0.05	-0.01	0.16	0.09	0.12	0.17	0.24	0.24	0.14	0.35	0.10	0.33	0.37	0.44	0.44	0.36	0.52	0.08	0.50	945
0.32	0.00	0.08	0.06	0.00	0.16	0.08	0.14	0.20	0.26	0.26	0.17	0.35	0.09	0.33	0.41	0.46	0.46	0.39	0.52	0.07	0.50	792


==> data/mlm_plots/tef/imdb/bert/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.09
top50	0.14


==> data/mlm_plots/tef/imdb/bert/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	49.73	69.17	63.55	40.84	97.49	28.32	83.70	33.00	40.28	41.00	29.02	51.55	11.27	48.00	55.88	76.48	70.60	46.08	106.88	30.40	91.25	33.00	40.53	41.00	29.25	51.81	11.28	48.00	981
0.03	47.51	69.03	62.74	38.91	99.15	30.12	83.30	33.00	39.90	40.00	27.99	51.81	11.91	48.00	60.46	85.31	77.52	50.10	120.53	35.21	101.22	33.00	40.44	41.00	28.44	52.43	11.99	49.00	1220
0.06	48.72	67.19	61.40	39.36	95.02	27.83	81.65	32.00	39.60	40.00	27.94	51.27	11.66	48.00	72.83	99.61	92.67	61.30	137.92	38.31	117.90	33.00	40.42	41.00	28.68	52.16	11.74	48.00	1955
0.11	50.03	69.38	63.14	40.11	98.64	29.27	84.12	30.00	38.41	39.00	26.02	50.79	12.38	47.00	97.44	129.04	121.34	81.52	176.56	47.52	149.62	31.00	39.79	40.00	27.26	52.33	12.53	49.00	2010
0.15	49.43	69.51	62.93	40.81	98.22	28.71	84.12	30.00	38.12	38.00	25.97	50.28	12.15	46.00	128.85	167.47	158.72	113.19	221.76	54.29	195.72	32.00	39.94	40.00	27.47	52.41	12.47	48.00	1159
0.18	56.88	80.67	72.17	45.50	115.84	35.17	95.14	28.00	37.45	40.00	24.32	50.57	13.13	47.00	174.96	229.41	215.75	153.69	305.12	75.72	260.12	30.00	39.51	42.00	25.77	53.25	13.74	50.00	434
0.32	61.37	88.43	79.08	50.05	126.82	38.38	100.10	27.75	36.42	37.00	21.43	51.41	14.99	45.00	230.80	300.36	270.14	197.52	403.19	102.83	351.69	30.50	38.82	40.00	23.33	54.31	15.49	48.00	176


==> data/mlm_plots/tef/imdb/bert/s/comparison_vals_auc.tex <==
name	auc
orig_pp	23.70
orig_ge	11.80
adv_pp	58.95
adv_ge	12.32


==> data/mlm_plots/tef/imdb/bert/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.09	0.20	0.18	0.05	0.36	0.15	0.30	0.32	0.42	0.42	0.27	0.57	0.15	0.52	0.23	0.30	0.29	0.19	0.41	0.11	0.37	981
0.03	0.00	0.08	0.07	-0.03	0.20	0.12	0.14	0.23	0.32	0.33	0.17	0.47	0.15	0.42	0.15	0.23	0.22	0.12	0.33	0.11	0.30	1220
0.06	-0.04	0.01	-0.00	-0.08	0.09	0.08	0.05	0.13	0.22	0.23	0.08	0.37	0.15	0.32	0.09	0.15	0.15	0.05	0.25	0.10	0.22	1955
0.11	-0.09	-0.04	-0.04	-0.12	0.05	0.08	0.01	0.04	0.14	0.14	-0.02	0.31	0.16	0.25	0.03	0.10	0.10	-0.02	0.21	0.11	0.17	2010
0.15	-0.11	-0.05	-0.06	-0.15	0.04	0.09	-0.00	-0.02	0.11	0.11	-0.06	0.28	0.17	0.23	-0.02	0.07	0.07	-0.04	0.19	0.12	0.16	1159
0.18	-0.12	-0.07	-0.07	-0.17	0.03	0.10	-0.02	-0.03	0.08	0.08	-0.10	0.26	0.18	0.19	-0.02	0.05	0.05	-0.07	0.18	0.12	0.13	434
0.32	-0.12	-0.08	-0.07	-0.17	0.02	0.09	-0.02	-0.03	0.06	0.10	-0.12	0.24	0.18	0.16	-0.02	0.04	0.07	-0.08	0.16	0.12	0.11	176


==> data/mlm_plots/tef/imdb/bert/s/correlations_auc.tex <==
name	auc
pcc	-0.01
spearman	0.04
kendall	0.03


==> data/mlm_plots/tef/imdb/bert/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	8.76	12.06	11.25	7.28	16.85	4.79	14.58	7.21	10.91	9.82	5.41	16.40	5.50	12.96	7.13	14.13	11.55	4.76	23.49	9.36	18.23	981
0.03	5.87	7.60	7.15	4.93	10.27	2.67	8.81	5.18	7.19	6.58	3.99	10.39	3.20	8.35	6.11	11.58	9.31	3.84	19.31	7.74	14.18	1220
0.06	4.32	5.29	5.07	3.77	6.81	1.52	5.92	4.09	5.06	4.79	3.49	6.64	1.58	5.67	5.22	8.90	7.42	3.18	14.62	5.72	10.56	1955
0.11	3.32	3.90	3.79	3.08	4.72	0.82	4.37	3.19	3.84	3.64	2.90	4.78	0.94	4.35	4.23	6.49	5.60	2.71	10.28	3.78	7.58	2010
0.15	2.73	3.11	3.02	2.55	3.68	0.56	3.39	2.67	3.08	3.03	2.47	3.68	0.61	3.43	3.41	4.94	4.53	2.64	7.25	2.30	5.72	1159
0.18	2.49	2.76	2.68	2.28	3.24	0.48	2.98	2.42	2.76	2.66	2.21	3.31	0.55	3.04	2.99	4.08	3.75	2.24	5.93	1.84	4.84	434
0.32	2.27	2.51	2.49	2.15	2.88	0.37	2.67	2.25	2.50	2.45	2.11	2.88	0.38	2.72	2.82	3.61	3.41	2.45	4.77	1.16	4.59	176


==> data/mlm_plots/tef/imdb/bert/s/ets_sts_auc.tex <==
name	auc
et_use	1.22
et_tse	1.18
et_ce	1.85


==> data/mlm_plots/tef/imdb/bert/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.53	8.11	3.81	-12.58	28.80	20.69	6.53	8.99	17.21	14.01	5.65	28.77	11.56	21.91	7.73	17.62	13.77	4.89	30.36	12.74	24.56	981
0.03	1.42	2.82	1.93	-3.73	9.36	6.55	2.73	7.18	10.79	9.21	5.58	16.01	5.21	13.52	5.99	10.74	8.47	3.57	17.91	7.17	13.59	1220
0.06	0.79	1.19	1.01	-0.08	2.47	1.28	1.33	5.89	7.79	7.09	4.49	11.08	3.30	8.76	4.82	7.12	6.00	3.47	10.77	3.65	8.21	1955
0.11	0.46	0.66	0.58	0.31	1.01	0.35	0.76	4.81	6.08	5.55	4.05	8.11	2.03	6.81	3.92	5.42	4.72	2.78	8.06	2.64	6.00	2010
0.15	0.29	0.39	0.37	0.23	0.54	0.15	0.45	4.19	5.00	4.81	3.79	6.21	1.21	5.50	3.44	4.32	3.96	2.82	5.82	1.50	4.83	1159
0.18	0.22	0.30	0.27	0.18	0.42	0.12	0.36	3.89	4.67	4.41	3.53	5.81	1.14	5.20	3.10	4.02	3.74	2.69	5.34	1.32	4.59	434
0.32	0.17	0.24	0.21	0.10	0.38	0.14	0.26	3.74	4.38	4.16	3.44	5.32	0.94	4.83	3.06	3.73	3.43	2.63	4.83	1.10	4.10	176


==> data/mlm_plots/tef/imdb/bert/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.29
et_p_h	1.91
et_p_l2	1.73


==> data/mlm_plots/tef/imdb/bert/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.12	0.10	0.04	0.19	0.07	0.15	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.01	0.05	0.02	0.04	981
0.03	0.17	0.25	0.24	0.13	0.37	0.12	0.32	0.03	0.06	0.05	0.03	0.09	0.03	0.07	0.03	0.05	0.05	0.03	0.07	0.02	0.06	1220
0.06	0.37	0.52	0.49	0.30	0.73	0.21	0.62	0.06	0.08	0.08	0.05	0.12	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	1955
0.11	0.68	0.92	0.89	0.57	1.28	0.35	1.14	0.08	0.11	0.11	0.07	0.15	0.04	0.13	0.08	0.09	0.09	0.07	0.12	0.02	0.11	2010
0.15	1.18	1.52	1.43	1.00	2.05	0.53	1.81	0.11	0.13	0.13	0.10	0.16	0.03	0.15	0.09	0.11	0.11	0.09	0.13	0.02	0.12	1159
0.18	1.51	2.01	1.93	1.33	2.70	0.68	2.37	0.12	0.14	0.14	0.11	0.18	0.03	0.16	0.10	0.12	0.12	0.10	0.14	0.02	0.13	434
0.32	2.00	2.58	2.49	1.77	3.38	0.81	3.22	0.13	0.15	0.16	0.12	0.19	0.03	0.18	0.11	0.13	0.13	0.11	0.15	0.02	0.14	176


==> data/mlm_plots/tef/imdb/bert/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.47
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/bert/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.95	0.96	0.96	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.97	0.02	0.97	0.95	0.96	0.97	0.93	0.99	0.03	0.98	981
0.03	0.92	0.93	0.94	0.92	0.95	0.02	0.95	0.91	0.93	0.93	0.90	0.95	0.02	0.94	0.93	0.94	0.95	0.91	0.98	0.03	0.97	1220
0.06	0.89	0.90	0.90	0.88	0.92	0.02	0.92	0.88	0.89	0.90	0.87	0.92	0.03	0.91	0.91	0.93	0.93	0.89	0.96	0.04	0.95	1955
0.11	0.84	0.86	0.86	0.84	0.89	0.03	0.88	0.84	0.86	0.86	0.83	0.89	0.03	0.88	0.88	0.90	0.91	0.85	0.95	0.05	0.93	2010
0.15	0.81	0.83	0.83	0.80	0.85	0.02	0.84	0.81	0.82	0.83	0.79	0.85	0.03	0.84	0.85	0.88	0.88	0.83	0.92	0.05	0.91	1159
0.18	0.79	0.80	0.80	0.78	0.83	0.03	0.82	0.78	0.80	0.80	0.77	0.83	0.03	0.82	0.82	0.85	0.86	0.79	0.91	0.06	0.89	434
0.32	0.77	0.78	0.78	0.76	0.81	0.03	0.80	0.77	0.78	0.78	0.75	0.81	0.03	0.80	0.81	0.83	0.85	0.78	0.89	0.06	0.88	176


==> data/mlm_plots/tef/imdb/bert/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/imdb/bert/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	5.76	8.34	7.10	2.80	13.87	5.53	8.69	0.68	77.48	1.33	-184.40	339.36	261.88	5.63	3.70	10.01	8.46	2.28	17.73	7.72	14.93	981
0.03	11.85	20.31	15.78	8.37	32.26	11.94	27.08	0.91	79.19	1.58	-158.12	316.49	237.30	8.07	4.35	11.82	10.19	2.80	20.84	9.02	17.49	1220
0.06	18.48	29.82	29.58	15.97	43.67	13.85	39.38	1.07	68.13	2.02	-185.33	321.60	253.47	6.39	5.37	13.31	11.88	3.68	22.94	9.63	19.03	1955
0.11	25.52	33.76	33.59	21.89	45.64	11.88	41.27	1.05	75.01	1.80	-141.20	291.22	216.21	6.56	5.56	12.84	10.95	3.58	22.11	9.27	18.56	2010
0.15	27.85	35.00	35.50	24.51	45.49	10.49	41.35	1.19	161.61	2.45	-210.99	534.21	372.60	95.64	5.15	13.11	11.51	3.41	22.81	9.70	18.69	1159
0.18	28.29	35.86	35.69	24.24	47.47	11.61	41.76	1.41	190.89	3.92	-177.99	559.78	368.89	261.79	3.91	12.25	9.64	2.25	22.24	10.00	19.13	434
0.32	28.19	35.88	36.10	24.79	46.98	11.09	42.58	1.58	298.62	31.13	-158.76	755.99	457.37	507.60	4.34	12.38	9.69	2.13	22.63	10.25	17.42	176


==> data/mlm_plots/tef/imdb/bert/s/time_misc_auc.tex <==
name	auc
attack_time	10.11
l2	51.57
lom	3.88


==> data/mlm_plots/tef/imdb/bert/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.13	0.21	0.20	0.09	0.34	0.12	0.29	0.42	0.48	0.47	0.38	0.57	0.09	0.54	0.61	0.65	0.65	0.59	0.72	0.06	0.69	981
0.03	0.07	0.14	0.14	0.04	0.24	0.10	0.20	0.35	0.42	0.42	0.33	0.51	0.09	0.47	0.58	0.62	0.62	0.56	0.68	0.06	0.66	1220
0.06	0.00	0.09	0.07	0.01	0.17	0.08	0.14	0.31	0.36	0.36	0.28	0.44	0.08	0.42	0.54	0.58	0.58	0.52	0.64	0.06	0.62	1955
0.11	0.00	0.06	0.05	-0.01	0.12	0.06	0.10	0.26	0.32	0.32	0.23	0.41	0.09	0.38	0.51	0.55	0.56	0.49	0.62	0.07	0.59	2010
0.15	0.00	0.05	0.05	-0.01	0.12	0.07	0.08	0.25	0.31	0.31	0.22	0.40	0.09	0.36	0.50	0.54	0.54	0.48	0.61	0.07	0.59	1159
0.18	0.00	0.05	0.00	-0.02	0.11	0.07	0.09	0.23	0.29	0.30	0.20	0.39	0.10	0.35	0.49	0.53	0.53	0.46	0.60	0.07	0.58	434
0.32	0.00	0.04	0.00	-0.01	0.09	0.05	0.06	0.23	0.28	0.29	0.18	0.38	0.10	0.34	0.49	0.52	0.53	0.45	0.59	0.07	0.57	176


==> data/mlm_plots/tef/imdb/bert/s/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.10
top50	0.17


==> data/mlm_plots/tef/imdb/cnn/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	53.39	72.90	68.21	43.46	102.33	29.44	86.86	31.00	38.90	38.00	26.61	51.18	12.28	47.00	58.38	79.52	74.67	48.53	110.51	30.99	94.35	31.00	39.17	39.00	26.81	51.53	12.36	47.00	929
0.03	54.04	74.15	69.10	43.59	104.72	30.56	88.95	29.00	38.01	38.00	25.12	50.90	12.89	47.00	66.15	89.76	84.85	55.41	124.12	34.36	106.32	30.00	38.60	38.00	25.55	51.65	13.05	47.00	1009
0.06	54.04	74.16	69.04	43.63	104.70	30.54	88.90	29.00	37.74	38.00	24.97	50.50	12.77	47.00	77.15	103.98	98.14	65.59	142.37	38.39	121.60	30.00	38.79	39.00	25.78	51.81	13.02	48.00	1016
0.11	53.72	74.24	68.96	43.18	105.30	31.06	88.93	29.00	37.75	38.00	24.72	50.78	13.03	47.00	92.17	121.87	115.77	78.65	165.08	43.21	140.99	31.00	39.34	39.00	25.93	52.75	13.41	49.00	1022
0.15	54.14	74.15	68.76	43.09	105.22	31.06	88.98	28.50	37.68	38.00	24.64	50.71	13.03	47.00	122.31	156.49	149.93	106.11	206.86	50.37	179.66	31.00	40.12	40.00	26.52	53.73	13.60	50.00	1031
0.18	53.63	74.06	68.78	42.94	105.17	31.12	88.55	29.00	37.79	38.00	24.69	50.88	13.09	47.00	158.86	198.76	189.26	138.30	259.22	60.46	227.87	32.00	41.20	41.00	27.44	54.96	13.76	51.00	1034
0.32	54.26	74.61	69.48	43.72	105.50	30.89	89.13	29.00	37.90	38.00	24.93	50.87	12.97	47.00	218.24	283.74	269.27	192.84	374.64	90.90	333.92	34.00	43.01	43.00	28.93	57.09	14.08	53.00	1992


==> data/mlm_plots/tef/imdb/cnn/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	23.04
orig_ge	11.75
adv_pp	54.77
adv_ge	12.61


==> data/mlm_plots/tef/imdb/cnn/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.41	0.54	0.57	0.32	0.76	0.22	0.70	0.65	0.73	0.78	0.56	0.91	0.18	0.86	0.54	0.66	0.69	0.46	0.85	0.19	0.82	929
0.03	0.13	0.29	0.30	0.04	0.54	0.25	0.45	0.47	0.57	0.60	0.38	0.75	0.19	0.70	0.38	0.50	0.51	0.32	0.68	0.18	0.64	1009
0.06	-0.06	0.10	0.09	-0.14	0.34	0.24	0.25	0.31	0.40	0.43	0.22	0.58	0.18	0.52	0.26	0.35	0.37	0.19	0.52	0.16	0.46	1016
0.11	-0.19	-0.03	-0.05	-0.26	0.20	0.23	0.11	0.16	0.26	0.28	0.08	0.43	0.17	0.38	0.15	0.24	0.25	0.09	0.39	0.15	0.34	1022
0.15	-0.30	-0.16	-0.17	-0.37	0.06	0.21	-0.03	-0.02	0.07	0.08	-0.09	0.23	0.16	0.18	0.01	0.09	0.09	-0.04	0.22	0.13	0.17	1031
0.18	-0.36	-0.23	-0.25	-0.43	-0.03	0.20	-0.12	-0.14	-0.05	-0.06	-0.19	0.09	0.14	0.03	-0.08	-0.02	-0.02	-0.13	0.09	0.11	0.05	1034
0.32	-0.42	-0.29	-0.31	-0.48	-0.09	0.19	-0.19	-0.27	-0.18	-0.19	-0.32	-0.04	0.14	-0.10	-0.19	-0.12	-0.13	-0.23	-0.02	0.10	-0.06	1992


==> data/mlm_plots/tef/imdb/cnn/ig/correlations_auc.tex <==
name	auc
pcc	-0.03
spearman	0.03
kendall	0.04


==> data/mlm_plots/tef/imdb/cnn/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	4.07	7.24	6.08	2.62	11.85	4.61	9.11	3.73	7.04	5.83	2.23	11.85	4.81	9.19	3.96	8.33	6.61	2.22	14.44	6.11	10.98	929
0.03	3.93	5.83	5.38	3.00	8.65	2.82	7.22	3.64	5.64	5.09	2.55	8.72	3.09	7.12	4.20	8.14	6.51	2.06	14.23	6.09	10.02	1009
0.06	3.52	4.69	4.47	2.94	6.45	1.75	5.62	3.19	4.46	4.13	2.59	6.32	1.87	5.39	3.94	6.52	5.42	2.19	10.86	4.33	7.94	1016
0.11	3.22	4.01	3.90	2.79	5.23	1.22	4.69	2.93	3.82	3.63	2.48	5.15	1.33	4.47	3.46	5.32	4.61	2.10	8.54	3.22	6.27	1022
0.15	2.84	3.33	3.30	2.53	4.13	0.80	3.78	2.61	3.17	3.08	2.30	4.04	0.87	3.63	2.98	4.15	3.82	2.28	6.02	1.87	4.96	1031
0.18	2.53	2.93	2.94	2.31	3.54	0.62	3.29	2.39	2.79	2.76	2.14	3.44	0.65	3.17	2.60	3.49	3.28	2.12	4.87	1.37	4.12	1034
0.32	2.20	2.51	2.51	2.02	3.00	0.49	2.81	2.11	2.43	2.40	1.92	2.93	0.51	2.74	2.12	2.83	2.69	1.81	3.86	1.03	3.35	1992


==> data/mlm_plots/tef/imdb/cnn/ig/ets_sts_auc.tex <==
name	auc
et_use	1.13
et_tse	1.08
et_ce	1.43


==> data/mlm_plots/tef/imdb/cnn/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.39	5.99	2.36	-13.47	25.45	19.46	4.32	5.13	11.47	8.48	1.66	21.28	9.81	14.20	4.69	12.53	8.77	0.91	24.14	11.61	16.20	929
0.03	1.09	2.71	1.63	-4.52	9.94	7.23	2.52	5.45	9.52	7.98	2.87	16.17	6.65	11.56	4.67	9.94	7.45	1.71	18.17	8.23	12.63	1009
0.06	0.79	1.42	1.07	-1.59	4.44	3.01	1.49	5.56	7.94	7.26	4.04	11.83	3.90	9.51	4.68	7.70	6.37	2.80	12.59	4.90	9.17	1016
0.11	0.58	0.93	0.77	-0.94	2.80	1.87	1.03	5.32	6.97	6.57	4.36	9.59	2.61	8.22	4.46	6.56	5.75	3.07	10.04	3.48	7.65	1022
0.15	0.39	0.55	0.50	0.15	0.95	0.40	0.63	4.83	6.03	5.78	4.11	7.94	1.91	6.95	4.08	5.45	5.03	3.17	7.73	2.28	6.27	1031
0.18	0.27	0.38	0.35	0.17	0.59	0.21	0.45	4.48	5.38	5.25	3.93	6.84	1.46	6.16	3.81	4.78	4.55	3.08	6.48	1.70	5.53	1034
0.32	0.17	0.24	0.22	0.12	0.36	0.12	0.29	3.98	4.67	4.60	3.51	5.83	1.16	5.29	3.35	4.10	3.94	2.79	5.41	1.31	4.64	1992


==> data/mlm_plots/tef/imdb/cnn/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.30
et_p_h	1.98
et_p_l2	1.86


==> data/mlm_plots/tef/imdb/cnn/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.10	0.09	0.04	0.16	0.06	0.14	0.01	0.03	0.02	0.01	0.05	0.02	0.04	0.02	0.03	0.02	0.01	0.05	0.02	0.04	929
0.03	0.15	0.23	0.22	0.11	0.35	0.12	0.29	0.03	0.05	0.05	0.02	0.08	0.03	0.07	0.03	0.05	0.05	0.03	0.07	0.02	0.06	1009
0.06	0.32	0.44	0.42	0.25	0.63	0.19	0.54	0.05	0.07	0.07	0.04	0.10	0.03	0.09	0.05	0.06	0.06	0.04	0.09	0.02	0.08	1016
0.11	0.52	0.70	0.67	0.42	0.98	0.28	0.85	0.07	0.09	0.09	0.06	0.13	0.03	0.11	0.07	0.08	0.08	0.06	0.10	0.02	0.09	1022
0.15	0.91	1.23	1.17	0.74	1.72	0.49	1.46	0.09	0.12	0.12	0.08	0.15	0.04	0.14	0.09	0.10	0.10	0.08	0.13	0.02	0.12	1031
0.18	1.38	1.87	1.78	1.15	2.59	0.72	2.25	0.11	0.14	0.14	0.10	0.18	0.04	0.16	0.10	0.12	0.12	0.09	0.14	0.02	0.13	1034
0.32	2.22	3.09	2.86	1.84	4.33	1.25	3.75	0.14	0.17	0.17	0.13	0.20	0.04	0.19	0.13	0.14	0.14	0.12	0.17	0.03	0.16	1992


==> data/mlm_plots/tef/imdb/cnn/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.47
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/cnn/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.94	0.99	0.03	0.98	929
0.03	0.92	0.93	0.93	0.91	0.95	0.02	0.95	0.91	0.93	0.93	0.90	0.96	0.03	0.95	0.92	0.94	0.95	0.91	0.98	0.04	0.97	1009
0.06	0.88	0.90	0.90	0.87	0.92	0.02	0.91	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.89	0.91	0.92	0.87	0.95	0.04	0.94	1016
0.11	0.85	0.87	0.87	0.84	0.89	0.03	0.88	0.84	0.86	0.86	0.82	0.89	0.03	0.88	0.86	0.88	0.89	0.84	0.93	0.05	0.92	1022
0.15	0.80	0.82	0.82	0.80	0.85	0.03	0.84	0.79	0.81	0.81	0.77	0.85	0.04	0.83	0.81	0.84	0.85	0.79	0.90	0.05	0.88	1031
0.18	0.77	0.79	0.79	0.76	0.81	0.03	0.80	0.75	0.77	0.77	0.74	0.81	0.03	0.80	0.77	0.80	0.81	0.74	0.86	0.06	0.85	1034
0.32	0.72	0.74	0.74	0.71	0.77	0.03	0.76	0.71	0.73	0.73	0.69	0.76	0.03	0.75	0.71	0.75	0.76	0.68	0.82	0.07	0.80	1992


==> data/mlm_plots/tef/imdb/cnn/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/imdb/cnn/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	5.26	5.47	5.45	5.17	5.78	0.31	5.71	4.35	7.12	6.13	3.28	10.96	3.84	9.17	2.45	7.82	5.40	0.03	15.61	7.79	10.77	929
0.03	6.35	6.65	6.56	6.29	7.00	0.35	6.93	5.77	9.30	7.84	4.38	14.22	4.92	12.06	2.97	9.53	7.09	0.73	18.32	8.80	13.37	1009
0.06	8.99	9.43	9.29	8.97	9.89	0.46	9.73	6.80	10.96	9.17	5.23	16.69	5.73	14.31	3.78	10.68	8.48	1.46	19.91	9.23	14.63	1016
0.11	11.11	11.59	11.52	10.47	12.72	1.12	12.12	7.49	12.21	10.18	5.71	18.71	6.50	15.78	4.40	11.52	9.29	1.91	21.13	9.61	16.10	1022
0.15	15.38	16.29	15.91	14.70	17.88	1.59	16.81	8.25	13.39	11.19	6.26	20.52	7.13	17.46	4.52	12.04	9.33	2.12	21.96	9.92	17.32	1031
0.18	19.59	20.28	19.74	18.49	22.07	1.79	20.49	8.48	14.21	11.98	6.53	21.89	7.68	18.53	4.35	12.19	9.73	1.93	22.46	10.26	17.70	1034
0.32	28.25	29.48	29.20	27.22	31.75	2.26	30.40	9.01	15.28	12.74	6.97	23.58	8.31	19.76	4.18	11.92	9.63	2.01	21.83	9.91	17.13	1992


==> data/mlm_plots/tef/imdb/cnn/ig/time_misc_auc.tex <==
name	auc
attack_time	5.46
l2	4.04
lom	3.56


==> data/mlm_plots/tef/imdb/cnn/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.59	0.68	0.70	0.53	0.83	0.15	0.79	0.71	0.79	0.82	0.67	0.92	0.12	0.90	0.77	0.84	0.86	0.73	0.94	0.10	0.92	929
0.03	0.44	0.52	0.52	0.38	0.66	0.14	0.62	0.62	0.70	0.71	0.58	0.82	0.12	0.79	0.71	0.77	0.78	0.67	0.87	0.10	0.85	1009
0.06	0.30	0.39	0.40	0.27	0.52	0.13	0.47	0.54	0.62	0.63	0.50	0.73	0.11	0.70	0.66	0.71	0.72	0.62	0.81	0.09	0.78	1016
0.11	0.23	0.29	0.29	0.17	0.41	0.12	0.36	0.49	0.54	0.56	0.44	0.65	0.10	0.62	0.61	0.66	0.68	0.57	0.75	0.09	0.73	1022
0.15	0.14	0.20	0.18	0.10	0.31	0.11	0.27	0.39	0.45	0.45	0.35	0.54	0.09	0.51	0.55	0.60	0.61	0.52	0.67	0.08	0.65	1031
0.18	0.09	0.16	0.14	0.06	0.26	0.10	0.22	0.32	0.37	0.37	0.29	0.45	0.08	0.42	0.50	0.54	0.54	0.47	0.61	0.07	0.59	1034
0.32	0.07	0.13	0.12	0.04	0.22	0.09	0.18	0.24	0.30	0.29	0.22	0.37	0.07	0.34	0.43	0.47	0.47	0.41	0.54	0.06	0.52	1992


==> data/mlm_plots/tef/imdb/cnn/ig/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.14
top50	0.19


==> data/mlm_plots/tef/imdb/cnn/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	53.63	73.26	68.49	43.56	102.96	29.70	88.21	30.00	38.62	38.00	26.21	51.02	12.40	47.00	59.33	80.84	76.05	49.03	112.66	31.82	96.09	30.00	38.99	39.00	26.49	51.49	12.50	47.50	931
0.03	54.04	74.11	69.04	43.79	104.43	30.32	89.03	29.00	37.92	38.00	25.01	50.82	12.90	47.00	68.80	92.34	87.43	57.58	127.09	34.76	110.62	29.75	38.71	39.00	25.61	51.81	13.10	48.00	1004
0.06	54.05	74.40	69.10	43.31	105.49	31.09	89.04	29.00	37.82	38.00	24.81	50.84	13.01	47.00	82.52	109.05	101.84	68.42	149.68	40.63	129.71	30.00	39.20	39.00	25.88	52.51	13.31	49.00	1017
0.11	54.07	74.38	69.09	43.30	105.46	31.08	89.04	29.00	37.80	38.00	24.76	50.83	13.04	47.00	97.32	127.76	121.18	83.13	172.39	44.63	150.91	30.25	39.78	39.00	26.24	53.31	13.53	49.00	1018
0.15	54.16	74.51	69.07	43.28	105.75	31.24	89.10	29.00	37.66	38.00	24.80	50.51	12.86	47.00	127.09	163.76	155.62	109.89	217.64	53.87	188.95	31.00	40.74	41.00	27.09	54.38	13.64	50.00	1023
0.18	54.03	74.29	69.07	43.26	105.32	31.03	88.94	29.00	37.73	38.00	24.98	50.49	12.75	47.00	161.38	203.39	194.79	141.67	265.12	61.72	233.69	32.00	41.94	42.00	28.14	55.75	13.80	52.00	1015
0.32	54.02	74.30	69.07	43.26	105.34	31.04	88.99	29.00	37.75	38.00	25.01	50.49	12.74	47.00	218.34	280.65	265.10	189.32	371.99	91.34	328.66	34.00	44.12	44.00	29.72	58.53	14.41	54.75	2026


==> data/mlm_plots/tef/imdb/cnn/s/comparison_vals_auc.tex <==
name	auc
orig_pp	23.07
orig_ge	11.73
adv_pp	55.78
adv_ge	12.81


==> data/mlm_plots/tef/imdb/cnn/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.80	0.85	0.86	0.76	0.93	0.08	0.91	0.86	0.89	0.90	0.83	0.95	0.06	0.94	0.72	0.79	0.80	0.69	0.88	0.10	0.86	931
0.03	0.68	0.75	0.76	0.64	0.86	0.11	0.82	0.76	0.81	0.82	0.72	0.89	0.09	0.87	0.61	0.67	0.68	0.58	0.77	0.10	0.74	1004
0.06	0.55	0.64	0.65	0.50	0.77	0.13	0.73	0.63	0.71	0.71	0.60	0.81	0.11	0.79	0.49	0.56	0.57	0.46	0.66	0.10	0.63	1017
0.11	0.45	0.54	0.55	0.40	0.69	0.15	0.65	0.52	0.61	0.62	0.48	0.74	0.13	0.70	0.39	0.47	0.47	0.36	0.57	0.11	0.54	1018
0.15	0.30	0.41	0.42	0.25	0.57	0.16	0.52	0.37	0.47	0.47	0.31	0.62	0.15	0.58	0.26	0.34	0.34	0.22	0.46	0.12	0.42	1023
0.18	0.18	0.30	0.30	0.13	0.47	0.17	0.42	0.23	0.34	0.35	0.17	0.50	0.17	0.46	0.16	0.24	0.24	0.12	0.36	0.12	0.32	1015
0.32	-0.00	0.13	0.13	-0.06	0.33	0.19	0.27	-0.02	0.13	0.13	-0.08	0.33	0.20	0.27	-0.01	0.09	0.09	-0.05	0.23	0.14	0.18	2026


==> data/mlm_plots/tef/imdb/cnn/s/correlations_auc.tex <==
name	auc
pcc	0.13
spearman	0.14
kendall	0.11


==> data/mlm_plots/tef/imdb/cnn/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	1.34	2.39	2.05	0.86	3.92	1.53	2.99	1.17	2.29	1.86	0.64	3.94	1.65	2.90	1.19	2.91	2.20	0.42	5.40	2.49	3.78	931
0.03	1.27	2.02	1.80	0.92	3.12	1.10	2.54	1.13	1.89	1.62	0.70	3.07	1.18	2.35	1.36	2.95	2.22	0.51	5.39	2.44	3.71	1004
0.06	1.27	1.85	1.73	1.00	2.70	0.85	2.23	1.15	1.70	1.56	0.89	2.52	0.81	2.07	1.41	2.65	2.17	0.60	4.70	2.05	3.20	1017
0.11	1.31	1.73	1.66	1.08	2.39	0.65	2.07	1.18	1.60	1.51	0.96	2.25	0.64	1.94	1.43	2.40	2.05	0.69	4.10	1.70	2.85	1018
0.15	1.32	1.67	1.64	1.16	2.19	0.51	1.99	1.24	1.56	1.53	1.06	2.06	0.50	1.84	1.43	2.14	1.91	0.86	3.43	1.29	2.51	1023
0.18	1.35	1.64	1.64	1.21	2.08	0.43	1.91	1.26	1.54	1.53	1.12	1.96	0.42	1.79	1.39	1.95	1.81	0.96	2.94	0.99	2.29	1015
0.32	1.40	1.64	1.64	1.27	2.01	0.37	1.89	1.31	1.56	1.55	1.19	1.93	0.37	1.79	1.30	1.73	1.63	1.08	2.38	0.65	2.04	2026


==> data/mlm_plots/tef/imdb/cnn/s/ets_sts_auc.tex <==
name	auc
et_use	0.54
et_tse	0.51
et_ce	0.68


==> data/mlm_plots/tef/imdb/cnn/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.44	1.16	0.70	-0.94	3.27	2.11	1.16	1.56	3.14	2.56	0.68	5.59	2.46	3.99	1.39	3.45	2.55	0.38	6.52	3.07	4.51	931
0.03	0.33	0.68	0.47	-0.76	2.11	1.43	0.70	1.74	2.80	2.51	1.19	4.41	1.61	3.36	1.50	2.87	2.31	0.67	5.06	2.20	3.41	1004
0.06	0.27	0.42	0.38	0.11	0.74	0.32	0.50	1.88	2.80	2.56	1.32	4.27	1.47	3.32	1.65	2.69	2.22	0.82	4.57	1.88	3.12	1017
0.11	0.23	0.33	0.30	0.12	0.55	0.21	0.39	2.05	2.78	2.62	1.59	3.97	1.19	3.30	1.74	2.59	2.27	1.07	4.12	1.52	3.10	1018
0.15	0.18	0.25	0.23	0.14	0.37	0.12	0.30	2.19	2.83	2.70	1.85	3.81	0.98	3.31	1.87	2.59	2.36	1.23	3.95	1.36	3.03	1023
0.18	0.15	0.21	0.19	0.12	0.29	0.09	0.24	2.31	2.87	2.78	2.00	3.74	0.87	3.32	1.96	2.56	2.40	1.59	3.53	0.97	2.98	1015
0.32	0.11	0.16	0.15	0.09	0.23	0.07	0.20	2.47	2.97	2.91	2.20	3.74	0.77	3.42	2.11	2.62	2.51	1.78	3.47	0.84	3.04	2026


==> data/mlm_plots/tef/imdb/cnn/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.10
et_p_h	0.89
et_p_l2	0.82


==> data/mlm_plots/tef/imdb/cnn/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.11	0.11	0.05	0.17	0.06	0.15	0.02	0.03	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.01	0.05	0.02	0.04	931
0.03	0.19	0.26	0.26	0.15	0.38	0.11	0.34	0.03	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.07	1004
0.06	0.37	0.50	0.49	0.31	0.70	0.19	0.61	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	1017
0.11	0.59	0.78	0.75	0.50	1.06	0.28	0.93	0.08	0.10	0.10	0.07	0.13	0.03	0.12	0.07	0.09	0.09	0.07	0.11	0.02	0.10	1018
0.15	1.00	1.31	1.26	0.84	1.78	0.47	1.58	0.10	0.13	0.13	0.09	0.16	0.04	0.15	0.09	0.11	0.11	0.09	0.13	0.02	0.12	1023
0.18	1.45	1.92	1.81	1.20	2.63	0.72	2.28	0.12	0.15	0.14	0.11	0.18	0.04	0.17	0.11	0.13	0.12	0.10	0.15	0.02	0.14	1015
0.32	2.16	3.08	2.85	1.77	4.38	1.30	3.72	0.15	0.17	0.17	0.13	0.21	0.04	0.20	0.13	0.15	0.15	0.12	0.18	0.03	0.17	2026


==> data/mlm_plots/tef/imdb/cnn/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.48
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/cnn/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.93	0.99	0.03	0.98	931
0.03	0.92	0.93	0.93	0.91	0.95	0.02	0.95	0.91	0.92	0.93	0.90	0.95	0.03	0.94	0.92	0.94	0.95	0.90	0.98	0.04	0.97	1004
0.06	0.88	0.90	0.90	0.87	0.92	0.02	0.91	0.87	0.88	0.89	0.85	0.92	0.03	0.91	0.89	0.91	0.92	0.87	0.95	0.04	0.94	1017
0.11	0.85	0.86	0.86	0.84	0.89	0.02	0.88	0.83	0.85	0.85	0.82	0.88	0.03	0.87	0.86	0.88	0.89	0.83	0.93	0.05	0.92	1018
0.15	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.78	0.81	0.80	0.77	0.84	0.03	0.83	0.81	0.84	0.85	0.78	0.90	0.06	0.88	1023
0.18	0.77	0.78	0.78	0.76	0.81	0.03	0.80	0.75	0.77	0.77	0.73	0.80	0.03	0.79	0.76	0.80	0.81	0.74	0.86	0.06	0.84	1015
0.32	0.71	0.73	0.73	0.70	0.76	0.03	0.75	0.69	0.72	0.72	0.68	0.75	0.04	0.74	0.68	0.73	0.74	0.65	0.80	0.08	0.78	2026


==> data/mlm_plots/tef/imdb/cnn/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/imdb/cnn/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.01	3.15	3.11	2.98	3.33	0.17	3.20	60.24	108.02	94.68	45.19	170.86	62.83	147.91	1.20	3.67	2.69	0.22	7.11	3.44	5.02	931
0.03	4.41	4.67	4.59	4.40	4.95	0.28	4.92	79.88	140.51	119.14	62.22	218.79	78.28	187.11	1.68	4.92	3.61	0.49	9.35	4.43	7.00	1004
0.06	6.00	6.27	6.19	5.95	6.58	0.32	6.50	101.08	175.66	148.00	82.66	268.65	92.99	236.16	2.46	6.11	4.87	1.16	11.05	4.95	8.67	1017
0.11	8.32	8.61	8.52	8.22	9.00	0.39	8.94	117.30	201.25	167.29	95.36	307.14	105.89	272.23	2.69	6.78	5.69	1.30	12.25	5.47	9.48	1018
0.15	10.56	11.03	10.70	10.19	11.87	0.84	11.41	137.74	237.08	197.87	112.42	361.74	124.66	321.97	3.08	8.59	6.66	-1.00	18.18	9.59	11.98	1023
0.18	13.33	13.84	13.48	13.13	14.55	0.71	14.29	158.69	268.22	226.29	129.85	406.58	138.37	364.93	3.10	9.03	7.45	1.78	16.27	7.24	13.32	1015
0.32	16.43	18.72	18.81	16.61	20.83	2.11	20.38	190.00	324.59	271.46	150.25	498.93	174.34	430.21	3.33	9.70	8.14	1.87	17.53	7.83	14.27	2026


==> data/mlm_plots/tef/imdb/cnn/s/time_misc_auc.tex <==
name	auc
attack_time	3.65
l2	74.49
lom	2.46


==> data/mlm_plots/tef/imdb/cnn/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.59	0.67	0.68	0.52	0.81	0.15	0.77	0.79	0.83	0.84	0.76	0.91	0.07	0.89	0.87	0.90	0.90	0.84	0.95	0.05	0.94	931
0.03	0.41	0.53	0.54	0.36	0.70	0.17	0.64	0.69	0.75	0.75	0.66	0.83	0.09	0.81	0.81	0.85	0.85	0.79	0.90	0.06	0.88	1004
0.06	0.27	0.40	0.41	0.23	0.58	0.18	0.50	0.60	0.65	0.66	0.56	0.75	0.09	0.72	0.75	0.79	0.79	0.73	0.85	0.06	0.83	1017
0.11	0.19	0.32	0.32	0.15	0.49	0.17	0.44	0.51	0.58	0.58	0.48	0.67	0.10	0.64	0.69	0.74	0.74	0.67	0.80	0.06	0.78	1018
0.15	0.12	0.23	0.21	0.07	0.39	0.16	0.33	0.41	0.48	0.48	0.37	0.58	0.10	0.54	0.61	0.66	0.67	0.59	0.74	0.07	0.71	1023
0.18	0.06	0.18	0.14	0.03	0.32	0.15	0.27	0.33	0.40	0.40	0.30	0.51	0.11	0.47	0.56	0.61	0.61	0.53	0.68	0.07	0.65	1015
0.32	0.00	0.12	0.09	-0.01	0.26	0.13	0.19	0.24	0.31	0.31	0.20	0.42	0.11	0.38	0.46	0.52	0.52	0.44	0.60	0.08	0.57	2026


==> data/mlm_plots/tef/imdb/cnn/s/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.15
top50	0.21


==> data/mlm_plots/tef/imdb/lstm/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	53.03	72.47	67.78	43.72	101.22	28.75	87.96	30.00	38.51	38.00	26.16	50.86	12.35	47.00	58.62	79.56	74.48	48.91	110.21	30.65	95.78	30.00	38.80	39.00	26.40	51.21	12.40	47.00	942
0.03	53.47	73.82	68.64	43.79	103.86	30.03	89.15	29.00	37.77	38.00	25.08	50.45	12.68	46.00	67.52	90.97	85.31	56.31	125.62	34.65	107.89	29.00	38.42	39.00	25.56	51.28	12.86	48.00	1007
0.06	53.55	73.95	68.70	43.83	104.06	30.11	89.18	29.00	37.68	38.00	24.95	50.41	12.73	46.00	81.02	106.55	99.75	67.50	145.61	39.06	125.16	29.25	38.86	39.00	25.83	51.90	13.04	48.00	1014
0.11	53.78	73.98	68.70	43.85	104.12	30.13	89.21	28.75	37.61	38.00	24.80	50.41	12.80	46.00	97.71	125.95	118.68	82.36	169.54	43.59	145.88	30.00	39.38	40.00	26.15	52.60	13.22	49.00	1016
0.15	53.62	73.99	68.77	43.98	103.99	30.00	89.27	28.00	37.53	38.00	24.70	50.35	12.83	46.00	129.22	164.13	157.64	111.56	216.70	52.57	188.93	31.00	40.36	40.00	26.76	53.95	13.59	50.00	1005
0.18	53.62	73.97	68.77	43.95	103.99	30.02	89.27	28.00	37.51	38.00	24.70	50.33	12.82	46.00	166.63	209.14	200.48	144.38	273.91	64.76	241.36	31.00	41.29	42.00	27.47	55.11	13.82	51.00	1005
0.32	53.51	73.73	68.45	43.96	103.50	29.77	89.11	29.00	37.65	38.00	24.93	50.37	12.72	46.00	224.16	291.14	275.01	195.16	387.12	95.98	342.80	33.00	42.88	43.00	28.78	56.99	14.11	53.00	2023


==> data/mlm_plots/tef/imdb/lstm/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	22.93
orig_ge	11.68
adv_pp	56.77
adv_ge	12.62


==> data/mlm_plots/tef/imdb/lstm/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.25	0.42	0.44	0.15	0.69	0.27	0.61	0.76	0.81	0.82	0.72	0.90	0.09	0.87	0.68	0.74	0.75	0.65	0.84	0.09	0.81	942
0.03	-0.02	0.17	0.16	-0.11	0.45	0.28	0.36	0.60	0.67	0.67	0.56	0.77	0.10	0.73	0.54	0.60	0.60	0.50	0.70	0.10	0.66	1007
0.06	-0.19	0.00	-0.02	-0.27	0.28	0.27	0.18	0.45	0.52	0.52	0.41	0.64	0.11	0.59	0.41	0.47	0.47	0.37	0.56	0.10	0.53	1014
0.11	-0.27	-0.09	-0.12	-0.34	0.17	0.26	0.08	0.33	0.40	0.40	0.29	0.52	0.11	0.48	0.30	0.36	0.36	0.27	0.46	0.09	0.42	1016
0.15	-0.35	-0.18	-0.20	-0.42	0.06	0.24	-0.03	0.18	0.26	0.25	0.14	0.37	0.12	0.33	0.18	0.24	0.24	0.15	0.33	0.09	0.29	1005
0.18	-0.40	-0.23	-0.25	-0.46	0.00	0.23	-0.08	0.07	0.15	0.15	0.03	0.27	0.12	0.23	0.09	0.14	0.15	0.05	0.24	0.09	0.20	1005
0.32	-0.43	-0.26	-0.28	-0.48	-0.04	0.22	-0.12	-0.04	0.05	0.05	-0.09	0.18	0.14	0.14	-0.01	0.06	0.06	-0.05	0.16	0.10	0.13	2023


==> data/mlm_plots/tef/imdb/lstm/ig/correlations_auc.tex <==
name	auc
pcc	-0.04
spearman	0.09
kendall	0.08


==> data/mlm_plots/tef/imdb/lstm/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	5.07	8.69	7.48	3.46	13.92	5.23	11.38	4.43	8.51	6.99	2.50	14.52	6.01	10.92	4.87	11.41	8.93	2.61	20.21	8.80	15.43	942
0.03	4.56	6.64	6.05	3.37	9.91	3.27	8.14	4.05	6.37	5.68	2.81	9.93	3.56	7.81	4.86	9.95	7.70	2.33	17.57	7.62	12.47	1007
0.06	3.84	5.02	4.79	3.14	6.91	1.89	6.03	3.44	4.80	4.42	2.63	6.97	2.17	5.83	4.10	7.23	5.85	1.78	12.68	5.45	8.56	1014
0.11	3.31	4.14	4.03	2.84	5.44	1.30	4.86	3.01	3.90	3.72	2.53	5.28	1.38	4.67	3.53	5.63	4.93	2.27	8.99	3.36	6.71	1016
0.15	2.77	3.31	3.24	2.46	4.17	0.85	3.84	2.54	3.14	3.07	2.26	4.02	0.88	3.65	2.90	4.15	3.74	2.07	6.22	2.08	4.94	1005
0.18	2.42	2.85	2.84	2.21	3.49	0.64	3.27	2.25	2.72	2.70	2.04	3.41	0.68	3.13	2.44	3.40	3.12	1.85	4.95	1.55	3.96	1005
0.32	2.07	2.42	2.39	1.91	2.93	0.51	2.76	1.97	2.34	2.32	1.80	2.88	0.54	2.66	2.01	2.71	2.52	1.67	3.75	1.04	3.19	2023


==> data/mlm_plots/tef/imdb/lstm/ig/ets_sts_auc.tex <==
name	auc
et_use	1.17
et_tse	1.12
et_ce	1.53


==> data/mlm_plots/tef/imdb/lstm/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.69	5.60	2.87	-7.69	18.88	13.28	4.69	6.00	12.60	9.47	2.26	22.94	10.34	16.15	5.37	13.69	9.86	1.09	26.30	12.61	18.16	942
0.03	1.18	2.29	1.68	-0.57	5.15	2.86	2.52	6.09	9.92	8.43	3.60	16.23	6.32	12.07	5.22	10.24	7.84	2.24	18.25	8.01	12.91	1007
0.06	0.79	1.26	1.06	0.47	2.05	0.79	1.47	5.65	7.99	7.29	4.28	11.71	3.72	9.49	4.77	7.60	6.60	3.15	12.05	4.45	9.06	1014
0.11	0.56	0.84	0.74	0.23	1.46	0.62	0.99	5.19	6.83	6.51	4.35	9.30	2.48	8.09	4.41	6.29	5.77	3.40	9.19	2.90	7.51	1016
0.15	0.35	0.50	0.46	0.28	0.73	0.23	0.60	4.62	5.76	5.61	4.04	7.47	1.71	6.70	3.90	5.16	4.77	3.22	7.10	1.94	5.98	1005
0.18	0.25	0.35	0.32	0.20	0.50	0.15	0.42	4.19	5.09	5.00	3.73	6.46	1.37	5.85	3.52	4.50	4.33	2.98	6.03	1.52	5.19	1005
0.32	0.16	0.23	0.21	0.12	0.33	0.11	0.27	3.69	4.45	4.39	3.34	5.56	1.11	5.09	3.13	3.90	3.75	2.70	5.10	1.20	4.48	2023


==> data/mlm_plots/tef/imdb/lstm/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.27
et_p_h	1.95
et_p_l2	1.82


==> data/mlm_plots/tef/imdb/lstm/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.06	0.11	0.10	0.05	0.17	0.06	0.14	0.02	0.03	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.01	0.05	0.02	0.04	942
0.03	0.17	0.25	0.24	0.14	0.37	0.11	0.32	0.03	0.05	0.05	0.03	0.08	0.03	0.07	0.04	0.05	0.05	0.03	0.07	0.02	0.06	1007
0.06	0.34	0.48	0.46	0.29	0.66	0.19	0.58	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.05	0.07	0.07	0.05	0.09	0.02	0.08	1014
0.11	0.57	0.76	0.73	0.48	1.05	0.28	0.91	0.08	0.10	0.10	0.07	0.13	0.03	0.12	0.07	0.09	0.09	0.06	0.11	0.02	0.10	1016
0.15	1.00	1.33	1.28	0.85	1.81	0.48	1.56	0.10	0.12	0.12	0.09	0.16	0.03	0.14	0.09	0.11	0.11	0.08	0.13	0.02	0.12	1005
0.18	1.51	2.01	1.91	1.27	2.75	0.74	2.35	0.12	0.15	0.15	0.11	0.18	0.04	0.17	0.11	0.12	0.12	0.10	0.15	0.02	0.14	1005
0.32	2.30	3.24	3.00	1.90	4.58	1.34	3.92	0.15	0.17	0.17	0.13	0.21	0.04	0.19	0.13	0.15	0.15	0.12	0.17	0.03	0.16	2023


==> data/mlm_plots/tef/imdb/lstm/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.50
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/lstm/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.96	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.94	0.99	0.03	0.98	942
0.03	0.92	0.93	0.93	0.91	0.95	0.02	0.95	0.91	0.93	0.93	0.90	0.95	0.03	0.94	0.92	0.94	0.95	0.90	0.98	0.04	0.97	1007
0.06	0.88	0.90	0.90	0.87	0.92	0.02	0.91	0.87	0.89	0.89	0.85	0.92	0.03	0.91	0.88	0.91	0.92	0.86	0.96	0.05	0.94	1014
0.11	0.85	0.86	0.86	0.84	0.89	0.03	0.88	0.83	0.85	0.86	0.82	0.89	0.04	0.88	0.85	0.88	0.89	0.82	0.94	0.06	0.92	1016
0.15	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.78	0.81	0.81	0.77	0.84	0.04	0.83	0.80	0.84	0.84	0.77	0.90	0.06	0.88	1005
0.18	0.76	0.78	0.78	0.75	0.81	0.03	0.80	0.75	0.77	0.77	0.73	0.80	0.04	0.79	0.75	0.80	0.80	0.73	0.86	0.07	0.84	1005
0.32	0.71	0.74	0.73	0.70	0.77	0.03	0.76	0.70	0.72	0.72	0.69	0.76	0.04	0.75	0.70	0.74	0.75	0.67	0.82	0.07	0.80	2023


==> data/mlm_plots/tef/imdb/lstm/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/imdb/lstm/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.62	3.75	3.75	3.56	3.93	0.18	3.78	1.44	1.96	1.86	1.22	2.70	0.74	2.39	3.93	13.00	9.64	1.10	24.91	11.90	18.61	942
0.03	4.59	4.83	4.82	4.58	5.09	0.26	5.08	1.86	2.42	2.35	1.61	3.23	0.81	2.89	5.60	16.02	12.46	2.13	29.91	13.89	22.82	1007
0.06	6.10	6.40	6.47	5.99	6.80	0.40	6.75	2.14	2.72	2.65	1.90	3.54	0.82	3.21	6.18	17.72	14.35	2.81	32.63	14.91	24.75	1014
0.11	13.43	13.82	13.70	12.57	15.06	1.24	14.96	2.30	2.88	2.79	2.07	3.70	0.82	3.40	6.50	18.33	14.54	3.03	33.63	15.30	25.92	1016
0.15	10.93	11.41	11.18	10.80	12.02	0.61	12.02	2.46	3.05	2.96	2.22	3.88	0.83	3.58	6.93	18.75	15.02	3.34	34.16	15.41	26.88	1005
0.18	15.73	16.43	16.57	15.35	17.51	1.08	17.19	2.58	3.14	3.06	2.31	3.97	0.83	3.66	6.55	18.86	14.92	3.14	34.58	15.72	26.91	1005
0.32	16.34	18.21	18.19	16.31	20.11	1.90	19.60	2.63	3.22	3.15	2.38	4.06	0.84	3.72	6.50	18.47	14.82	3.14	33.80	15.33	25.95	2023


==> data/mlm_plots/tef/imdb/lstm/ig/time_misc_auc.tex <==
name	auc
attack_time	4.10
l2	0.92
lom	5.63


==> data/mlm_plots/tef/imdb/lstm/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.64	0.71	0.71	0.60	0.81	0.11	0.77	0.80	0.84	0.85	0.78	0.90	0.06	0.89	0.87	0.89	0.90	0.85	0.94	0.05	0.93	942
0.03	0.46	0.55	0.55	0.42	0.67	0.12	0.64	0.72	0.76	0.76	0.70	0.83	0.07	0.81	0.81	0.84	0.84	0.79	0.89	0.05	0.87	1007
0.06	0.33	0.41	0.41	0.29	0.54	0.13	0.50	0.64	0.68	0.69	0.61	0.75	0.07	0.72	0.75	0.79	0.79	0.74	0.83	0.05	0.82	1014
0.11	0.27	0.33	0.33	0.21	0.45	0.12	0.41	0.57	0.62	0.62	0.55	0.69	0.07	0.67	0.71	0.74	0.74	0.69	0.79	0.05	0.77	1016
0.15	0.19	0.27	0.27	0.16	0.39	0.11	0.33	0.49	0.54	0.53	0.46	0.61	0.07	0.58	0.66	0.68	0.68	0.64	0.73	0.05	0.72	1005
0.18	0.18	0.24	0.23	0.13	0.35	0.11	0.32	0.43	0.47	0.47	0.40	0.54	0.07	0.51	0.61	0.64	0.64	0.59	0.69	0.05	0.67	1005
0.32	0.14	0.21	0.20	0.10	0.32	0.11	0.27	0.35	0.41	0.40	0.33	0.49	0.08	0.46	0.54	0.58	0.58	0.52	0.64	0.06	0.62	2023


==> data/mlm_plots/tef/imdb/lstm/ig/top_intersections_auc.tex <==
name	auc
top10	0.10
top30	0.17
top50	0.21


==> data/mlm_plots/tef/imdb/lstm/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	53.07	72.22	67.78	43.66	100.79	28.57	86.78	30.00	38.30	38.00	26.12	50.48	12.18	47.00	58.94	80.23	74.97	49.51	110.94	30.71	96.30	30.00	38.65	39.00	26.40	50.90	12.25	47.00	960
0.03	53.97	73.95	68.76	43.95	103.94	30.00	89.11	29.00	37.68	38.00	25.00	50.36	12.68	46.00	69.08	92.68	87.58	58.22	127.14	34.46	110.75	29.00	38.45	39.00	25.54	51.37	12.92	47.00	1015
0.06	53.95	73.97	68.55	43.87	104.07	30.10	89.18	29.00	37.55	38.00	24.77	50.33	12.78	46.00	84.05	109.27	103.34	70.43	148.11	38.84	128.40	30.00	38.91	39.00	25.78	52.04	13.13	48.00	1018
0.11	53.12	73.59	68.08	43.42	103.76	30.17	89.09	29.00	37.68	38.00	24.91	50.44	12.77	47.00	98.85	128.97	123.20	84.13	173.81	44.84	151.75	30.00	39.68	40.00	26.40	52.95	13.27	49.00	1028
0.15	53.73	74.07	68.72	43.91	104.23	30.16	89.30	28.00	37.57	38.00	24.76	50.37	12.80	46.00	131.04	166.99	160.23	113.74	220.23	53.25	192.20	31.00	40.59	41.00	27.01	54.16	13.57	50.00	1011
0.18	54.05	74.15	68.89	43.98	104.32	30.17	89.35	28.00	37.58	38.00	24.75	50.42	12.84	46.00	168.86	209.93	202.08	147.62	272.24	62.31	239.86	32.00	41.56	42.00	27.74	55.39	13.83	51.00	1008
0.32	54.04	74.28	69.10	44.14	104.41	30.14	89.59	28.00	37.51	38.00	24.81	50.22	12.71	46.00	230.66	296.96	282.67	202.56	391.36	94.40	347.65	34.00	43.32	44.00	29.17	57.48	14.15	53.00	1999


==> data/mlm_plots/tef/imdb/lstm/s/comparison_vals_auc.tex <==
name	auc
orig_pp	22.97
orig_ge	11.68
adv_pp	57.63
adv_ge	12.69


==> data/mlm_plots/tef/imdb/lstm/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.56	0.64	0.66	0.49	0.79	0.15	0.74	0.85	0.88	0.90	0.77	0.99	0.11	0.94	0.74	0.79	0.81	0.65	0.93	0.14	0.87	960
0.03	0.39	0.48	0.48	0.35	0.62	0.14	0.57	0.75	0.80	0.82	0.68	0.92	0.12	0.87	0.62	0.68	0.69	0.56	0.80	0.12	0.75	1015
0.06	0.27	0.35	0.35	0.23	0.48	0.13	0.44	0.63	0.70	0.70	0.57	0.82	0.12	0.78	0.50	0.56	0.56	0.45	0.67	0.11	0.63	1018
0.11	0.19	0.27	0.26	0.15	0.39	0.12	0.35	0.52	0.59	0.60	0.45	0.74	0.14	0.68	0.40	0.46	0.46	0.34	0.58	0.12	0.53	1028
0.15	0.10	0.18	0.17	0.07	0.29	0.11	0.24	0.37	0.46	0.46	0.32	0.59	0.14	0.54	0.27	0.34	0.33	0.23	0.44	0.11	0.40	1011
0.18	0.04	0.12	0.10	0.01	0.23	0.11	0.18	0.24	0.33	0.33	0.19	0.47	0.14	0.42	0.17	0.24	0.23	0.13	0.34	0.10	0.30	1008
0.32	-0.05	0.03	0.02	-0.09	0.14	0.12	0.10	0.01	0.13	0.13	-0.04	0.29	0.17	0.24	0.01	0.09	0.09	-0.02	0.20	0.11	0.17	1999


==> data/mlm_plots/tef/imdb/lstm/s/correlations_auc.tex <==
name	auc
pcc	0.06
spearman	0.14
kendall	0.11


==> data/mlm_plots/tef/imdb/lstm/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.43	5.63	4.74	1.79	9.47	3.84	6.62	3.15	5.60	4.52	0.95	10.26	4.66	6.68	3.25	7.19	5.35	0.60	13.78	6.59	8.96	960
0.03	2.92	4.13	3.79	2.23	6.03	1.90	4.86	2.66	4.03	3.52	1.73	6.34	2.31	4.70	3.03	5.89	4.62	1.28	10.49	4.60	7.14	1015
0.06	2.52	3.29	3.09	2.04	4.54	1.25	3.80	2.32	3.16	2.87	1.61	4.71	1.55	3.61	2.67	4.45	3.69	1.43	7.46	3.02	5.43	1018
0.11	2.23	2.78	2.65	1.94	3.62	0.84	3.18	2.06	2.66	2.53	1.68	3.64	0.98	2.97	2.37	3.61	3.14	1.61	5.61	2.00	4.32	1028
0.15	1.97	2.31	2.23	1.79	2.82	0.52	2.60	1.83	2.20	2.13	1.64	2.76	0.56	2.49	1.96	2.81	2.55	1.54	4.09	1.27	3.36	1011
0.18	1.80	2.06	2.02	1.66	2.45	0.40	2.27	1.69	1.97	1.92	1.54	2.39	0.43	2.19	1.77	2.40	2.23	1.44	3.36	0.96	2.83	1008
0.32	1.65	1.83	1.81	1.54	2.12	0.29	1.98	1.58	1.77	1.74	1.46	2.08	0.31	1.93	1.51	1.99	1.85	1.26	2.72	0.73	2.30	1999


==> data/mlm_plots/tef/imdb/lstm/s/ets_sts_auc.tex <==
name	auc
et_use	0.80
et_tse	0.77
et_ce	1.00


==> data/mlm_plots/tef/imdb/lstm/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.01	2.95	1.51	-3.88	9.78	6.83	2.61	3.60	7.04	5.26	1.69	12.39	5.35	8.79	3.31	7.83	5.25	0.22	15.43	7.61	9.75	960
0.03	0.73	1.31	0.96	-0.56	3.18	1.87	1.38	3.76	5.78	4.98	2.57	8.99	3.21	6.77	3.23	5.72	4.51	1.72	9.72	4.00	6.79	1015
0.06	0.50	0.74	0.65	0.21	1.28	0.53	0.84	3.65	4.94	4.52	2.90	6.97	2.04	5.73	3.08	4.66	3.96	2.03	7.28	2.62	5.33	1018
0.11	0.37	0.52	0.47	0.24	0.80	0.28	0.59	3.52	4.44	4.18	3.02	5.87	1.42	5.12	2.98	4.06	3.67	2.30	5.81	1.76	4.63	1028
0.15	0.25	0.34	0.31	0.18	0.50	0.16	0.39	3.26	3.96	3.80	2.89	5.03	1.07	4.45	2.76	3.54	3.29	2.24	4.85	1.30	4.03	1011
0.18	0.18	0.25	0.23	0.14	0.36	0.11	0.29	3.08	3.66	3.54	2.75	4.58	0.92	4.11	2.58	3.25	3.07	2.19	4.31	1.06	3.67	1008
0.32	0.12	0.17	0.16	0.10	0.25	0.08	0.20	2.91	3.39	3.31	2.64	4.13	0.75	3.75	2.45	2.98	2.84	2.12	3.84	0.86	3.32	1999


==> data/mlm_plots/tef/imdb/lstm/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.16
et_p_h	1.30
et_p_l2	1.20


==> data/mlm_plots/tef/imdb/lstm/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.12	0.11	0.05	0.18	0.06	0.16	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.05	960
0.03	0.20	0.27	0.27	0.16	0.39	0.11	0.34	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.07	1015
0.06	0.38	0.52	0.50	0.33	0.71	0.19	0.62	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.09	1018
0.11	0.63	0.82	0.78	0.52	1.11	0.29	0.97	0.08	0.10	0.10	0.07	0.13	0.03	0.12	0.07	0.09	0.09	0.07	0.11	0.02	0.10	1028
0.15	1.05	1.37	1.32	0.90	1.85	0.48	1.64	0.10	0.13	0.13	0.09	0.16	0.03	0.15	0.09	0.11	0.11	0.09	0.13	0.02	0.12	1011
0.18	1.53	2.02	1.90	1.30	2.74	0.72	2.40	0.12	0.15	0.15	0.11	0.18	0.04	0.17	0.11	0.13	0.12	0.10	0.15	0.02	0.14	1008
0.32	2.36	3.30	3.06	1.98	4.63	1.33	3.99	0.15	0.17	0.17	0.13	0.21	0.04	0.20	0.13	0.15	0.15	0.12	0.17	0.03	0.16	1999


==> data/mlm_plots/tef/imdb/lstm/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.51
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/lstm/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.96	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.93	0.99	0.03	0.98	960
0.03	0.92	0.93	0.93	0.91	0.95	0.02	0.94	0.91	0.93	0.93	0.90	0.95	0.03	0.94	0.92	0.94	0.95	0.90	0.97	0.04	0.96	1015
0.06	0.88	0.89	0.90	0.87	0.92	0.03	0.91	0.87	0.89	0.89	0.85	0.92	0.03	0.91	0.88	0.91	0.91	0.86	0.95	0.05	0.94	1018
0.11	0.84	0.86	0.86	0.83	0.89	0.03	0.88	0.83	0.85	0.85	0.82	0.89	0.03	0.88	0.85	0.88	0.88	0.82	0.93	0.05	0.92	1028
0.15	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.78	0.81	0.81	0.77	0.84	0.04	0.83	0.80	0.83	0.84	0.77	0.89	0.06	0.88	1011
0.18	0.76	0.78	0.78	0.75	0.81	0.03	0.80	0.75	0.77	0.77	0.73	0.80	0.04	0.79	0.75	0.79	0.80	0.73	0.86	0.07	0.84	1008
0.32	0.71	0.73	0.73	0.70	0.76	0.03	0.75	0.69	0.72	0.72	0.68	0.76	0.04	0.74	0.68	0.73	0.74	0.65	0.81	0.08	0.79	1999


==> data/mlm_plots/tef/imdb/lstm/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/imdb/lstm/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.20	3.51	3.33	2.21	4.81	1.30	3.52	37.63	55.65	50.22	29.93	81.37	25.72	68.21	3.14	9.98	6.67	-4.70	24.67	14.69	11.98	960
0.03	4.15	4.37	4.27	3.41	5.33	0.96	4.53	52.05	72.60	66.07	42.88	102.33	29.73	88.13	3.98	11.23	8.37	-0.93	23.40	12.16	15.13	1015
0.06	5.27	5.58	5.48	4.73	6.43	0.85	5.85	62.62	84.89	77.95	52.76	117.02	32.13	103.09	4.25	12.61	9.47	0.33	24.89	12.28	17.29	1018
0.11	8.00	8.53	8.35	7.18	9.87	1.35	8.81	68.38	93.93	87.04	58.65	129.20	35.28	113.61	5.27	14.92	11.20	-1.13	30.96	16.05	19.26	1028
0.15	18.32	19.25	19.43	17.60	20.90	1.65	20.21	77.56	105.34	98.23	67.23	143.44	38.11	125.83	5.22	14.42	11.81	2.18	26.66	12.24	19.80	1011
0.18	13.43	13.82	13.57	13.15	14.49	0.67	14.12	84.09	113.28	106.23	72.62	153.95	40.66	134.50	5.55	14.57	11.75	1.91	27.23	12.66	20.42	1008
0.32	17.28	18.75	18.62	17.10	20.40	1.65	20.14	93.98	127.21	121.13	82.31	172.12	44.90	151.63	5.83	14.89	12.12	3.06	26.73	11.84	20.88	1999


==> data/mlm_plots/tef/imdb/lstm/s/time_misc_auc.tex <==
name	auc
attack_time	3.95
l2	32.24
lom	4.35


==> data/mlm_plots/tef/imdb/lstm/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.59	0.67	0.68	0.53	0.81	0.14	0.76	0.79	0.83	0.84	0.72	0.94	0.11	0.89	0.88	0.90	0.91	0.81	0.98	0.08	0.94	960
0.03	0.43	0.52	0.53	0.38	0.65	0.13	0.60	0.71	0.76	0.76	0.67	0.84	0.09	0.81	0.82	0.85	0.86	0.79	0.92	0.06	0.89	1015
0.06	0.28	0.38	0.36	0.25	0.51	0.13	0.47	0.61	0.67	0.67	0.58	0.75	0.09	0.72	0.76	0.80	0.80	0.74	0.86	0.06	0.84	1018
0.11	0.19	0.28	0.27	0.15	0.41	0.13	0.36	0.54	0.59	0.59	0.50	0.68	0.09	0.65	0.71	0.75	0.75	0.68	0.82	0.07	0.79	1028
0.15	0.10	0.18	0.18	0.08	0.29	0.11	0.25	0.44	0.49	0.49	0.41	0.58	0.08	0.54	0.65	0.69	0.69	0.63	0.75	0.06	0.73	1011
0.18	0.05	0.13	0.12	0.03	0.22	0.10	0.18	0.37	0.42	0.41	0.34	0.50	0.08	0.47	0.59	0.63	0.63	0.57	0.69	0.06	0.67	1008
0.32	0.00	0.08	0.07	0.00	0.17	0.08	0.14	0.26	0.32	0.32	0.23	0.40	0.08	0.38	0.51	0.55	0.55	0.48	0.62	0.07	0.60	1999


==> data/mlm_plots/tef/imdb/lstm/s/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.16
top50	0.21


==> data/mlm_plots/tef/imdb/lstmatt/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	53.57	73.36	68.22	44.00	102.72	29.36	88.07	29.00	38.47	38.00	26.10	50.85	12.38	47.00	59.95	81.44	77.04	50.06	112.81	31.38	96.75	30.00	38.81	38.00	26.34	51.27	12.47	48.00	943
0.03	53.64	74.08	68.64	43.58	104.57	30.50	88.49	29.00	37.96	38.00	25.28	50.65	12.69	47.00	68.27	92.80	86.52	57.58	128.02	35.22	109.94	30.00	38.72	39.00	25.84	51.60	12.88	48.00	999
0.06	53.66	74.38	68.71	43.38	105.38	31.00	89.03	28.00	37.75	38.00	24.86	50.63	12.88	47.00	82.13	109.71	103.33	69.91	149.52	39.81	128.26	30.00	39.07	39.00	25.91	52.24	13.17	49.00	1008
0.11	53.65	74.36	68.72	43.36	105.37	31.00	89.01	28.00	37.78	38.00	24.90	50.67	12.88	47.00	98.70	129.66	122.35	84.70	174.62	44.96	153.08	30.00	39.71	40.00	26.44	52.99	13.28	49.00	1009
0.15	53.65	74.36	68.71	43.37	105.35	30.99	88.99	28.00	37.77	38.00	24.88	50.65	12.89	47.00	131.65	167.81	160.03	114.14	221.47	53.66	196.04	31.00	40.73	41.00	27.16	54.29	13.57	50.00	1010
0.18	53.60	74.28	68.70	43.27	105.29	31.01	88.96	28.00	37.78	38.00	24.90	50.66	12.88	47.00	167.84	211.10	202.70	147.72	274.48	63.38	243.81	32.00	41.75	42.00	28.04	55.47	13.71	52.00	1012
0.32	54.03	74.54	69.01	43.75	105.34	30.79	89.08	29.00	37.83	38.00	25.08	50.57	12.75	47.00	232.78	301.46	285.82	203.33	399.59	98.13	354.97	34.00	43.54	44.00	29.53	57.55	14.01	54.00	1996


==> data/mlm_plots/tef/imdb/lstmatt/a/comparison_vals_auc.tex <==
name	auc
orig_pp	23.08
orig_ge	11.74
adv_pp	58.13
adv_ge	12.75


==> data/mlm_plots/tef/imdb/lstmatt/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.46	0.58	0.59	0.40	0.75	0.17	0.70	0.88	0.91	0.93	0.86	0.97	0.06	0.96	0.78	0.82	0.83	0.75	0.89	0.07	0.87	943
0.03	0.23	0.37	0.36	0.19	0.54	0.18	0.48	0.76	0.82	0.83	0.72	0.92	0.10	0.89	0.63	0.69	0.70	0.59	0.79	0.10	0.77	999
0.06	0.10	0.21	0.19	0.06	0.36	0.15	0.30	0.61	0.69	0.70	0.56	0.82	0.13	0.79	0.49	0.56	0.57	0.45	0.68	0.12	0.64	1008
0.11	0.02	0.12	0.09	-0.01	0.25	0.13	0.19	0.47	0.57	0.59	0.41	0.73	0.16	0.69	0.37	0.45	0.46	0.32	0.58	0.13	0.54	1009
0.15	-0.04	0.03	0.01	-0.08	0.14	0.11	0.07	0.29	0.41	0.42	0.23	0.59	0.18	0.53	0.23	0.31	0.31	0.18	0.45	0.13	0.40	1010
0.18	-0.09	-0.03	-0.05	-0.13	0.07	0.10	0.01	0.15	0.28	0.28	0.08	0.47	0.20	0.42	0.11	0.21	0.21	0.07	0.34	0.14	0.30	1012
0.32	-0.17	-0.10	-0.11	-0.21	-0.00	0.10	-0.06	-0.11	0.05	0.04	-0.17	0.28	0.22	0.21	-0.07	0.04	0.04	-0.11	0.20	0.15	0.15	1996


==> data/mlm_plots/tef/imdb/lstmatt/a/correlations_auc.tex <==
name	auc
pcc	0.02
spearman	0.13
kendall	0.10


==> data/mlm_plots/tef/imdb/lstmatt/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.75	6.44	5.65	2.66	10.22	3.78	8.08	3.38	6.11	5.18	2.10	10.13	4.02	7.74	3.55	7.55	5.86	1.89	13.21	5.66	10.08	943
0.03	3.58	5.05	4.67	2.78	7.32	2.27	6.02	3.14	4.73	4.32	2.38	7.09	2.36	5.68	3.47	6.68	5.29	1.72	11.65	4.97	8.18	999
0.06	3.09	4.04	3.85	2.63	5.46	1.41	4.68	2.81	3.77	3.54	2.30	5.25	1.47	4.47	3.05	5.21	4.35	1.53	8.89	3.68	6.09	1008
0.11	2.76	3.39	3.27	2.43	4.35	0.96	3.81	2.53	3.15	3.01	2.20	4.11	0.96	3.63	2.68	4.05	3.51	1.86	6.23	2.19	4.77	1009
0.15	2.36	2.75	2.66	2.14	3.37	0.61	3.03	2.16	2.58	2.48	1.93	3.24	0.65	2.88	2.21	3.12	2.76	1.59	4.64	1.52	3.60	1010
0.18	2.14	2.39	2.36	1.98	2.80	0.41	2.60	1.96	2.26	2.20	1.80	2.71	0.45	2.48	1.94	2.59	2.40	1.62	3.57	0.97	3.02	1012
0.32	1.88	2.07	2.04	1.78	2.36	0.29	2.22	1.78	1.98	1.94	1.67	2.29	0.31	2.13	1.66	2.13	1.99	1.42	2.85	0.71	2.43	1996


==> data/mlm_plots/tef/imdb/lstmatt/a/ets_sts_auc.tex <==
name	auc
et_use	0.95
et_tse	0.89
et_ce	1.11


==> data/mlm_plots/tef/imdb/lstmatt/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.17	3.19	1.87	-4.08	10.45	7.26	3.09	4.46	8.63	6.80	2.48	14.78	6.15	11.02	3.94	9.55	7.03	0.86	18.24	8.69	12.35	943
0.03	0.87	1.50	1.20	-0.59	3.60	2.10	1.64	4.84	7.18	6.22	3.41	10.96	3.78	8.42	4.12	7.19	5.62	2.20	12.17	4.98	8.61	999
0.06	0.62	0.89	0.80	0.34	1.45	0.56	1.03	4.67	6.17	5.66	3.68	8.66	2.49	7.07	3.90	5.88	5.04	2.46	9.30	3.42	6.54	1008
0.11	0.44	0.64	0.56	0.06	1.21	0.57	0.73	4.34	5.45	5.11	3.57	7.34	1.88	6.19	3.63	5.02	4.45	2.50	7.55	2.53	5.61	1009
0.15	0.29	0.40	0.37	0.19	0.62	0.21	0.47	3.91	4.75	4.51	3.37	6.13	1.38	5.30	3.29	4.25	3.88	2.57	5.94	1.69	4.75	1010
0.18	0.21	0.29	0.27	0.16	0.42	0.13	0.34	3.65	4.29	4.14	3.27	5.32	1.03	4.79	3.05	3.79	3.54	2.60	4.98	1.19	4.22	1012
0.32	0.13	0.19	0.18	0.10	0.29	0.10	0.23	3.35	3.87	3.76	3.08	4.66	0.79	4.28	2.81	3.39	3.24	2.46	4.33	0.93	3.77	1996


==> data/mlm_plots/tef/imdb/lstmatt/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.19
et_p_h	1.56
et_p_l2	1.45


==> data/mlm_plots/tef/imdb/lstmatt/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.12	0.11	0.05	0.18	0.06	0.16	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.04	943
0.03	0.19	0.27	0.26	0.16	0.38	0.11	0.34	0.03	0.06	0.06	0.03	0.08	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.06	999
0.06	0.39	0.51	0.49	0.33	0.70	0.19	0.62	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	1008
0.11	0.61	0.81	0.78	0.53	1.08	0.27	0.97	0.08	0.10	0.10	0.07	0.13	0.03	0.12	0.07	0.09	0.09	0.07	0.11	0.02	0.10	1009
0.15	1.04	1.37	1.32	0.91	1.83	0.46	1.65	0.10	0.12	0.13	0.09	0.16	0.03	0.15	0.09	0.11	0.11	0.08	0.13	0.02	0.12	1010
0.18	1.54	2.03	1.95	1.31	2.75	0.72	2.42	0.12	0.15	0.15	0.11	0.18	0.03	0.17	0.11	0.12	0.13	0.10	0.15	0.02	0.14	1012
0.32	2.39	3.35	3.13	1.99	4.71	1.36	4.10	0.15	0.17	0.17	0.13	0.21	0.04	0.19	0.13	0.15	0.15	0.12	0.17	0.03	0.16	1996


==> data/mlm_plots/tef/imdb/lstmatt/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.52
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/lstmatt/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.95	0.96	0.96	0.95	0.98	0.02	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.93	0.99	0.03	0.98	943
0.03	0.92	0.93	0.93	0.91	0.95	0.02	0.95	0.91	0.92	0.93	0.90	0.95	0.03	0.94	0.91	0.93	0.94	0.89	0.97	0.04	0.96	999
0.06	0.88	0.90	0.90	0.87	0.92	0.03	0.91	0.87	0.89	0.89	0.85	0.92	0.03	0.91	0.87	0.90	0.91	0.85	0.95	0.05	0.94	1008
0.11	0.85	0.86	0.86	0.84	0.89	0.03	0.88	0.83	0.85	0.85	0.82	0.89	0.04	0.88	0.84	0.87	0.88	0.81	0.92	0.06	0.91	1009
0.15	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.78	0.80	0.80	0.77	0.84	0.04	0.83	0.78	0.82	0.83	0.76	0.88	0.06	0.87	1010
0.18	0.76	0.78	0.78	0.75	0.81	0.03	0.80	0.74	0.77	0.76	0.73	0.80	0.04	0.79	0.74	0.78	0.79	0.71	0.85	0.07	0.83	1012
0.32	0.71	0.73	0.73	0.70	0.76	0.03	0.75	0.69	0.72	0.71	0.68	0.75	0.04	0.74	0.67	0.72	0.72	0.64	0.80	0.08	0.78	1996


==> data/mlm_plots/tef/imdb/lstmatt/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.25
sts_tse	0.25
sts_ce	0.25


==> data/mlm_plots/tef/imdb/lstmatt/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.11	3.22	3.20	3.05	3.39	0.17	3.33	0.12	0.16	0.15	0.10	0.22	0.06	0.19	5.75	17.42	12.75	0.84	34.01	16.59	24.29	943
0.03	4.19	4.36	4.33	4.14	4.59	0.23	4.47	0.16	0.21	0.20	0.14	0.28	0.07	0.25	7.36	22.78	16.57	1.51	44.05	21.27	30.74	999
0.06	5.39	5.60	5.54	5.25	5.94	0.34	5.80	0.20	0.25	0.24	0.18	0.32	0.07	0.29	9.88	27.29	20.96	4.17	50.41	23.12	38.80	1008
0.11	6.69	6.99	6.97	6.64	7.34	0.35	7.27	0.22	0.27	0.26	0.20	0.34	0.07	0.31	10.76	29.75	23.70	5.76	53.74	23.99	43.14	1009
0.15	9.22	9.84	9.70	9.19	10.48	0.65	10.40	0.23	0.28	0.27	0.21	0.34	0.06	0.31	11.62	31.25	26.52	7.35	55.15	23.90	45.75	1010
0.18	12.56	12.96	12.82	12.27	13.66	0.70	13.23	0.23	0.26	0.26	0.21	0.32	0.06	0.29	12.41	30.99	27.00	8.25	53.72	22.74	44.95	1012
0.32	17.02	19.38	19.19	17.01	21.75	2.37	21.36	0.21	0.24	0.23	0.19	0.30	0.05	0.27	12.77	30.98	26.23	8.29	53.67	22.69	45.29	1996


==> data/mlm_plots/tef/imdb/lstmatt/a/time_misc_auc.tex <==
name	auc
attack_time	3.47
l2	0.08
lom	9.09


==> data/mlm_plots/tef/imdb/lstmatt/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.55	0.62	0.64	0.49	0.75	0.13	0.72	0.80	0.84	0.85	0.77	0.91	0.07	0.89	0.89	0.91	0.92	0.87	0.96	0.05	0.95	943
0.03	0.33	0.43	0.43	0.29	0.57	0.14	0.53	0.68	0.73	0.74	0.65	0.82	0.09	0.79	0.82	0.85	0.86	0.79	0.92	0.06	0.90	999
0.06	0.18	0.28	0.27	0.14	0.41	0.13	0.36	0.57	0.63	0.63	0.53	0.73	0.10	0.69	0.74	0.79	0.79	0.72	0.86	0.07	0.84	1008
0.11	0.09	0.18	0.17	0.05	0.31	0.13	0.27	0.47	0.54	0.54	0.44	0.65	0.11	0.61	0.69	0.74	0.74	0.66	0.82	0.08	0.79	1009
0.15	0.00	0.10	0.07	-0.00	0.20	0.10	0.15	0.36	0.43	0.43	0.33	0.54	0.11	0.50	0.61	0.67	0.67	0.58	0.75	0.08	0.72	1010
0.18	0.00	0.06	0.05	-0.02	0.14	0.08	0.09	0.28	0.35	0.35	0.25	0.46	0.11	0.42	0.55	0.61	0.61	0.52	0.70	0.09	0.67	1012
0.32	0.00	0.03	0.00	-0.03	0.09	0.06	0.05	0.18	0.26	0.25	0.15	0.36	0.11	0.32	0.46	0.52	0.52	0.43	0.61	0.09	0.59	1996


==> data/mlm_plots/tef/imdb/lstmatt/a/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.14
top50	0.21


==> data/mlm_plots/tef/imdb/lstmatt/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	53.41	73.00	68.19	44.18	101.82	28.82	87.65	30.00	38.66	38.00	26.35	50.96	12.30	47.00	59.86	80.72	76.00	50.41	111.02	30.31	96.43	30.00	38.99	39.00	26.59	51.38	12.40	48.00	927
0.03	53.51	74.12	68.45	43.21	105.04	30.92	88.60	29.00	37.90	38.00	25.07	50.72	12.83	47.00	67.79	91.83	86.29	57.00	126.65	34.83	109.72	29.00	38.61	39.00	25.58	51.65	13.03	48.00	1001
0.06	53.39	74.17	68.45	43.16	105.18	31.01	88.86	29.00	37.72	38.00	24.86	50.59	12.87	47.00	80.15	107.70	101.44	68.02	147.37	39.68	127.06	29.00	38.96	39.00	25.79	52.13	13.17	48.00	1013
0.11	53.74	74.37	69.52	43.62	105.11	30.75	89.18	29.00	37.79	38.00	25.04	50.54	12.75	47.00	96.61	127.51	121.15	83.29	171.73	44.22	149.29	31.00	39.64	40.00	26.49	52.78	13.14	49.00	1043
0.15	53.65	73.89	67.89	43.36	104.42	30.53	88.21	28.00	37.56	38.00	24.78	50.35	12.79	47.00	129.50	163.89	157.41	112.59	215.18	51.29	189.30	31.00	40.32	41.00	26.82	53.83	13.50	50.00	1083
0.18	53.64	74.06	68.12	43.17	104.95	30.89	88.16	28.00	37.70	38.00	24.87	50.53	12.83	47.00	167.06	207.56	199.90	146.06	269.05	61.50	239.18	32.00	41.34	42.00	27.61	55.06	13.73	51.00	1039
0.32	53.82	74.96	69.66	43.53	106.39	31.43	89.35	28.00	37.85	38.00	24.89	50.81	12.96	47.00	222.07	286.89	272.27	193.59	380.19	93.30	332.52	33.00	42.86	43.00	28.65	57.08	14.21	53.00	1867


==> data/mlm_plots/tef/imdb/lstmatt/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	23.06
orig_ge	11.73
adv_pp	56.49
adv_ge	12.64


==> data/mlm_plots/tef/imdb/lstmatt/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.14	0.34	0.36	0.03	0.65	0.31	0.55	0.56	0.65	0.68	0.46	0.83	0.19	0.77	0.45	0.55	0.57	0.38	0.71	0.17	0.66	927
0.03	-0.09	0.10	0.10	-0.21	0.40	0.30	0.29	0.39	0.48	0.50	0.29	0.67	0.19	0.61	0.31	0.40	0.41	0.24	0.56	0.16	0.50	1001
0.06	-0.26	-0.08	-0.09	-0.36	0.20	0.28	0.10	0.22	0.33	0.34	0.14	0.52	0.19	0.46	0.19	0.27	0.28	0.12	0.42	0.15	0.37	1013
0.11	-0.35	-0.19	-0.19	-0.44	0.07	0.25	-0.03	0.11	0.21	0.22	0.03	0.39	0.18	0.33	0.10	0.18	0.19	0.04	0.32	0.14	0.27	1043
0.15	-0.44	-0.28	-0.30	-0.52	-0.04	0.24	-0.14	-0.03	0.08	0.09	-0.10	0.25	0.18	0.20	0.00	0.08	0.09	-0.05	0.21	0.13	0.17	1083
0.18	-0.48	-0.33	-0.34	-0.55	-0.11	0.22	-0.20	-0.10	0.01	0.01	-0.15	0.17	0.16	0.11	-0.05	0.02	0.02	-0.10	0.14	0.12	0.10	1039
0.32	-0.52	-0.37	-0.39	-0.58	-0.17	0.21	-0.24	-0.17	-0.06	-0.07	-0.22	0.09	0.15	0.04	-0.11	-0.03	-0.04	-0.15	0.08	0.11	0.04	1867


==> data/mlm_plots/tef/imdb/lstmatt/ig/correlations_auc.tex <==
name	auc
pcc	-0.07
spearman	0.04
kendall	0.04


==> data/mlm_plots/tef/imdb/lstmatt/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	6.27	10.59	9.04	3.87	17.32	6.72	13.44	5.58	10.15	8.47	3.14	17.16	7.01	12.75	5.50	12.31	9.69	2.56	22.05	9.75	16.41	927
0.03	5.22	7.80	6.98	3.84	11.77	3.97	9.70	4.61	7.44	6.53	3.07	11.80	4.37	9.18	5.11	10.60	8.27	2.08	19.13	8.52	12.83	1001
0.06	4.27	5.81	5.44	3.52	8.10	2.29	6.96	3.90	5.46	5.06	3.02	7.91	2.44	6.55	4.41	7.86	6.49	2.45	13.26	5.41	9.60	1013
0.11	3.73	4.77	4.54	3.20	6.33	1.56	5.55	3.38	4.48	4.25	2.85	6.11	1.63	5.26	3.88	6.14	5.21	2.43	9.85	3.71	7.39	1043
0.15	3.09	3.77	3.68	2.72	4.81	1.05	4.27	2.88	3.58	3.48	2.49	4.68	1.09	4.12	3.17	4.65	4.16	2.34	6.97	2.32	5.62	1083
0.18	2.72	3.18	3.10	2.47	3.88	0.71	3.58	2.56	3.03	2.98	2.28	3.79	0.76	3.46	2.75	3.80	3.46	2.07	5.54	1.74	4.46	1039
0.32	2.36	2.72	2.68	2.18	3.25	0.53	3.02	2.26	2.62	2.58	2.06	3.18	0.56	2.93	2.27	3.05	2.84	1.94	4.15	1.11	3.63	1867


==> data/mlm_plots/tef/imdb/lstmatt/ig/ets_sts_auc.tex <==
name	auc
et_use	1.34
et_tse	1.28
et_ce	1.68


==> data/mlm_plots/tef/imdb/lstmatt/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.80	5.21	2.94	-4.37	14.80	9.58	5.02	6.86	13.66	10.69	3.15	24.16	10.51	17.58	6.06	14.68	10.39	1.90	27.45	12.77	19.67	927
0.03	1.23	2.40	1.77	-1.16	5.96	3.56	2.53	6.50	10.60	9.20	4.12	17.08	6.48	12.31	5.65	10.72	8.43	2.63	18.81	8.09	13.15	1001
0.06	0.85	1.47	1.12	-1.76	4.70	3.23	1.53	6.12	8.70	7.88	4.53	12.87	4.17	10.37	5.26	8.35	6.97	3.12	13.57	5.23	9.96	1013
0.11	0.61	0.90	0.78	0.31	1.50	0.60	1.04	5.77	7.53	7.04	4.60	10.46	2.93	8.60	4.93	6.97	6.09	3.23	10.72	3.75	7.86	1043
0.15	0.38	0.55	0.50	0.25	0.86	0.30	0.64	5.12	6.39	6.04	4.26	8.52	2.13	7.25	4.30	5.77	5.17	3.14	8.39	2.62	6.41	1083
0.18	0.27	0.38	0.34	0.22	0.54	0.16	0.45	4.63	5.63	5.46	4.13	7.14	1.51	6.30	3.92	5.02	4.71	3.19	6.85	1.83	5.61	1039
0.32	0.18	0.26	0.23	0.14	0.38	0.12	0.31	4.17	4.99	4.84	3.72	6.26	1.27	5.57	3.52	4.38	4.14	2.91	5.85	1.47	4.88	1867


==> data/mlm_plots/tef/imdb/lstmatt/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.28
et_p_h	2.14
et_p_l2	2.00


==> data/mlm_plots/tef/imdb/lstmatt/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.12	0.11	0.05	0.18	0.06	0.15	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.04	927
0.03	0.18	0.26	0.25	0.15	0.37	0.11	0.33	0.03	0.06	0.05	0.03	0.08	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.06	1001
0.06	0.36	0.49	0.48	0.30	0.68	0.19	0.60	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.05	0.07	0.07	0.05	0.09	0.02	0.08	1013
0.11	0.59	0.78	0.74	0.49	1.06	0.28	0.94	0.08	0.10	0.10	0.07	0.13	0.03	0.12	0.07	0.08	0.08	0.06	0.11	0.02	0.10	1043
0.15	1.01	1.33	1.29	0.87	1.80	0.47	1.59	0.10	0.12	0.12	0.09	0.16	0.03	0.14	0.09	0.11	0.11	0.08	0.13	0.02	0.12	1083
0.18	1.50	1.99	1.90	1.28	2.69	0.70	2.40	0.12	0.14	0.14	0.11	0.18	0.04	0.16	0.11	0.12	0.12	0.10	0.15	0.02	0.14	1039
0.32	2.22	3.13	2.93	1.82	4.44	1.31	3.80	0.14	0.17	0.17	0.13	0.20	0.04	0.19	0.13	0.14	0.14	0.12	0.17	0.02	0.16	1867


==> data/mlm_plots/tef/imdb/lstmatt/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.49
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/lstmatt/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.93	0.99	0.03	0.98	927
0.03	0.92	0.94	0.94	0.91	0.96	0.02	0.95	0.91	0.93	0.93	0.90	0.96	0.03	0.95	0.92	0.94	0.95	0.90	0.98	0.04	0.96	1001
0.06	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.89	0.91	0.92	0.86	0.96	0.05	0.94	1013
0.11	0.85	0.87	0.87	0.84	0.90	0.03	0.89	0.83	0.86	0.86	0.82	0.89	0.04	0.88	0.85	0.88	0.89	0.83	0.93	0.05	0.92	1043
0.15	0.81	0.82	0.82	0.79	0.85	0.03	0.84	0.79	0.81	0.81	0.77	0.85	0.04	0.84	0.81	0.84	0.85	0.78	0.90	0.06	0.88	1083
0.18	0.77	0.79	0.79	0.76	0.82	0.03	0.81	0.75	0.78	0.78	0.74	0.81	0.04	0.80	0.77	0.80	0.81	0.74	0.87	0.06	0.85	1039
0.32	0.72	0.74	0.74	0.71	0.77	0.03	0.76	0.71	0.73	0.73	0.70	0.77	0.04	0.76	0.70	0.75	0.76	0.68	0.83	0.07	0.80	1867


==> data/mlm_plots/tef/imdb/lstmatt/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/imdb/lstmatt/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	4.10	4.33	4.24	4.04	4.62	0.29	4.49	1.89	6.84	3.22	-17.68	31.36	24.52	5.53	4.31	15.86	10.21	-1.28	33.00	17.14	21.36	927
0.03	5.16	5.37	5.32	5.02	5.71	0.35	5.57	2.79	15.92	4.57	-99.37	131.20	115.29	6.93	5.90	18.99	12.97	-0.36	38.34	19.35	25.90	1001
0.06	7.87	8.58	8.72	7.47	9.69	1.11	8.92	3.66	46.17	5.29	-448.05	540.39	494.22	8.23	6.80	21.57	15.56	0.52	42.62	21.05	29.22	1013
0.11	9.35	10.25	9.81	8.08	12.41	2.16	10.54	4.13	263.81	5.86	-1996.39	2524.01	2260.20	9.11	6.99	24.03	17.45	-0.23	48.30	24.27	32.66	1043
0.15	12.65	14.13	13.28	11.51	16.74	2.62	14.51	4.35	180.22	6.06	-981.41	1341.86	1161.64	9.77	7.86	24.24	18.23	1.40	47.07	22.83	33.52	1083
0.18	16.01	17.45	17.01	15.13	19.76	2.31	18.36	4.38	49.01	5.98	-303.23	401.25	352.24	8.82	8.26	23.53	18.09	2.28	44.77	21.24	33.15	1039
0.32	21.68	24.13	24.66	21.51	26.76	2.63	25.90	4.25	32.81	5.67	-211.98	277.60	244.79	7.82	7.69	23.04	17.60	1.91	44.17	21.13	31.73	1867


==> data/mlm_plots/tef/imdb/lstmatt/ig/time_misc_auc.tex <==
name	auc
attack_time	4.64
l2	27.66
lom	7.06


==> data/mlm_plots/tef/imdb/lstmatt/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.45	0.56	0.57	0.39	0.72	0.17	0.68	0.65	0.71	0.72	0.60	0.82	0.11	0.79	0.75	0.80	0.81	0.72	0.88	0.08	0.85	927
0.03	0.32	0.41	0.41	0.26	0.57	0.16	0.50	0.56	0.62	0.63	0.51	0.73	0.11	0.69	0.68	0.73	0.74	0.65	0.82	0.08	0.79	1001
0.06	0.21	0.30	0.30	0.16	0.44	0.14	0.40	0.47	0.54	0.56	0.43	0.65	0.11	0.62	0.63	0.68	0.68	0.59	0.76	0.08	0.73	1013
0.11	0.14	0.23	0.23	0.10	0.36	0.13	0.32	0.42	0.48	0.49	0.37	0.59	0.11	0.56	0.59	0.63	0.64	0.56	0.71	0.08	0.69	1043
0.15	0.09	0.18	0.18	0.07	0.30	0.11	0.25	0.35	0.41	0.42	0.31	0.51	0.10	0.49	0.54	0.58	0.59	0.51	0.66	0.08	0.63	1083
0.18	0.09	0.17	0.16	0.06	0.27	0.11	0.23	0.32	0.38	0.37	0.29	0.47	0.09	0.44	0.51	0.56	0.56	0.49	0.63	0.07	0.60	1039
0.32	0.07	0.15	0.14	0.05	0.25	0.10	0.21	0.28	0.34	0.34	0.25	0.42	0.09	0.40	0.48	0.52	0.52	0.45	0.59	0.07	0.56	1867


==> data/mlm_plots/tef/imdb/lstmatt/ig/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.14
top50	0.19


==> data/mlm_plots/tef/imdb/lstmatt/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	53.11	72.57	67.80	43.76	101.38	28.81	86.96	30.00	38.70	38.00	26.34	51.07	12.36	47.00	60.36	81.02	75.25	50.04	112.01	30.98	95.72	31.00	39.10	39.00	26.64	51.55	12.45	48.00	936
0.03	53.57	74.04	68.64	43.65	104.43	30.39	88.90	29.00	37.94	38.00	25.19	50.69	12.75	47.00	69.77	93.64	87.55	58.91	128.38	34.74	110.66	29.00	38.79	39.00	25.82	51.77	12.98	48.00	1003
0.06	53.65	74.36	68.71	43.35	105.36	31.00	89.01	28.00	37.78	38.00	24.90	50.67	12.88	47.00	83.65	110.66	105.13	71.13	150.19	39.53	130.05	30.00	39.22	39.00	25.97	52.47	13.25	49.00	1009
0.11	53.65	74.36	68.71	43.37	105.35	30.99	88.99	28.00	37.77	38.00	24.88	50.65	12.89	47.00	100.95	130.54	123.50	86.28	174.80	44.26	151.94	30.00	39.79	40.00	26.44	53.14	13.35	49.00	1010
0.15	53.65	74.36	68.71	43.37	105.35	30.99	88.99	28.00	37.77	38.00	24.88	50.65	12.89	47.00	134.40	169.24	162.50	117.02	221.47	52.22	197.28	31.00	40.83	41.00	27.21	54.46	13.63	50.00	1010
0.18	53.60	74.28	68.70	43.27	105.29	31.01	88.96	28.00	37.78	38.00	24.90	50.66	12.88	47.00	170.82	213.18	205.65	151.24	275.12	61.94	247.64	32.00	41.85	43.00	28.01	55.69	13.84	51.00	1012
0.32	54.03	74.62	68.81	43.78	105.47	30.85	89.08	28.00	37.72	38.00	24.97	50.47	12.75	47.00	231.24	297.25	281.15	202.54	391.96	94.71	347.11	34.00	43.42	44.00	29.29	57.56	14.13	54.00	2002


==> data/mlm_plots/tef/imdb/lstmatt/s/comparison_vals_auc.tex <==
name	auc
orig_pp	23.07
orig_ge	11.74
adv_pp	58.17
adv_ge	12.76


==> data/mlm_plots/tef/imdb/lstmatt/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.51	0.61	0.62	0.46	0.76	0.15	0.71	0.76	0.82	0.85	0.70	0.94	0.12	0.91	0.60	0.68	0.69	0.55	0.80	0.12	0.77	936
0.03	0.32	0.42	0.43	0.27	0.58	0.16	0.53	0.56	0.67	0.70	0.50	0.85	0.18	0.81	0.42	0.53	0.53	0.37	0.68	0.15	0.64	1003
0.06	0.18	0.29	0.28	0.14	0.44	0.15	0.39	0.38	0.51	0.52	0.31	0.72	0.21	0.67	0.28	0.39	0.38	0.23	0.55	0.16	0.50	1009
0.11	0.10	0.21	0.19	0.05	0.36	0.15	0.31	0.22	0.38	0.38	0.15	0.60	0.23	0.54	0.17	0.28	0.27	0.12	0.45	0.17	0.39	1010
0.15	0.00	0.11	0.09	-0.03	0.26	0.15	0.20	0.05	0.21	0.21	-0.03	0.45	0.24	0.37	0.05	0.16	0.15	0.00	0.33	0.16	0.26	1010
0.18	-0.06	0.04	0.03	-0.10	0.19	0.14	0.13	-0.07	0.09	0.07	-0.14	0.31	0.22	0.23	-0.03	0.08	0.06	-0.07	0.23	0.15	0.17	1012
0.32	-0.16	-0.06	-0.07	-0.20	0.09	0.15	0.03	-0.25	-0.09	-0.11	-0.31	0.13	0.22	0.05	-0.15	-0.05	-0.06	-0.19	0.10	0.15	0.04	2002


==> data/mlm_plots/tef/imdb/lstmatt/s/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.07
kendall	0.06


==> data/mlm_plots/tef/imdb/lstmatt/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.62	6.04	5.35	2.66	9.42	3.38	7.55	3.27	5.77	4.87	2.26	9.27	3.51	7.43	3.38	7.10	5.70	2.16	12.05	4.94	9.60	936
0.03	3.23	4.62	4.23	2.51	6.74	2.11	5.64	2.92	4.38	3.84	2.06	6.70	2.32	5.32	3.18	6.14	4.92	1.84	10.45	4.30	7.83	1003
0.06	2.82	3.70	3.52	2.35	5.05	1.35	4.39	2.56	3.49	3.22	2.03	4.94	1.45	4.17	2.85	4.84	4.02	1.59	8.09	3.25	5.80	1009
0.11	2.47	3.10	2.98	2.14	4.06	0.96	3.60	2.24	2.91	2.77	1.92	3.91	1.00	3.41	2.45	3.86	3.30	1.59	6.13	2.27	4.66	1010
0.15	2.15	2.56	2.53	1.93	3.19	0.63	2.90	2.00	2.42	2.35	1.78	3.06	0.64	2.77	2.12	3.03	2.74	1.65	4.41	1.38	3.60	1010
0.18	1.96	2.27	2.24	1.79	2.76	0.49	2.54	1.85	2.15	2.10	1.66	2.65	0.49	2.45	1.91	2.56	2.36	1.56	3.56	1.00	2.98	1012
0.32	1.80	2.02	2.01	1.67	2.38	0.36	2.22	1.72	1.94	1.92	1.57	2.31	0.37	2.13	1.69	2.17	2.04	1.45	2.89	0.72	2.51	2002


==> data/mlm_plots/tef/imdb/lstmatt/s/ets_sts_auc.tex <==
name	auc
et_use	0.89
et_tse	0.84
et_ce	1.07


==> data/mlm_plots/tef/imdb/lstmatt/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.07	3.11	1.61	-4.92	11.15	8.04	2.47	3.89	7.44	5.86	2.10	12.77	5.33	9.41	3.48	8.09	5.58	0.91	15.26	7.18	10.25	936
0.03	0.75	1.31	1.04	-0.10	2.71	1.40	1.44	3.99	6.27	5.39	2.63	9.90	3.63	7.39	3.42	6.30	4.86	1.55	11.06	4.76	7.55	1003
0.06	0.53	0.87	0.69	-0.60	2.35	1.48	0.91	3.94	5.44	4.86	2.88	7.99	2.56	6.31	3.35	5.12	4.36	1.96	8.28	3.16	5.81	1009
0.11	0.38	0.62	0.50	-0.78	2.01	1.40	0.65	3.74	4.87	4.56	2.99	6.76	1.89	5.57	3.13	4.46	3.94	2.17	6.75	2.29	5.10	1010
0.15	0.26	0.38	0.33	-0.16	0.92	0.54	0.42	3.48	4.30	4.08	2.93	5.66	1.37	4.83	2.92	3.83	3.50	2.21	5.45	1.62	4.29	1010
0.18	0.19	0.27	0.24	-0.02	0.56	0.29	0.31	3.33	3.98	3.86	2.91	5.04	1.07	4.43	2.78	3.52	3.31	2.29	4.74	1.23	3.93	1012
0.32	0.13	0.19	0.17	0.10	0.27	0.09	0.22	3.17	3.72	3.64	2.87	4.57	0.85	4.14	2.65	3.27	3.14	2.33	4.21	0.94	3.65	2002


==> data/mlm_plots/tef/imdb/lstmatt/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.18
et_p_h	1.42
et_p_l2	1.31


==> data/mlm_plots/tef/imdb/lstmatt/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.13	0.12	0.06	0.19	0.07	0.16	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.05	936
0.03	0.21	0.29	0.28	0.17	0.40	0.12	0.36	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.07	1003
0.06	0.39	0.53	0.52	0.34	0.72	0.19	0.64	0.06	0.08	0.08	0.05	0.11	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.09	1009
0.11	0.63	0.82	0.80	0.53	1.12	0.30	0.99	0.08	0.10	0.10	0.07	0.13	0.03	0.12	0.07	0.09	0.09	0.07	0.11	0.02	0.10	1010
0.15	1.08	1.40	1.34	0.91	1.90	0.49	1.68	0.11	0.13	0.13	0.09	0.16	0.03	0.15	0.10	0.11	0.11	0.09	0.13	0.02	0.12	1010
0.18	1.56	2.07	1.96	1.28	2.87	0.79	2.47	0.12	0.15	0.15	0.11	0.18	0.04	0.17	0.11	0.13	0.13	0.10	0.15	0.02	0.14	1012
0.32	2.36	3.29	3.08	1.96	4.61	1.32	3.95	0.15	0.17	0.17	0.13	0.21	0.04	0.19	0.13	0.15	0.15	0.12	0.17	0.02	0.16	2002


==> data/mlm_plots/tef/imdb/lstmatt/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.52
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/lstmatt/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.95	0.96	0.96	0.95	0.98	0.02	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.93	0.99	0.03	0.98	936
0.03	0.92	0.93	0.93	0.91	0.95	0.02	0.95	0.91	0.92	0.93	0.90	0.95	0.03	0.94	0.91	0.93	0.94	0.89	0.97	0.04	0.96	1003
0.06	0.88	0.90	0.90	0.87	0.92	0.03	0.91	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.88	0.90	0.91	0.86	0.95	0.05	0.94	1009
0.11	0.85	0.87	0.87	0.84	0.89	0.03	0.88	0.83	0.85	0.86	0.82	0.89	0.04	0.88	0.84	0.87	0.88	0.82	0.93	0.05	0.91	1010
0.15	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.79	0.81	0.81	0.77	0.85	0.04	0.83	0.80	0.83	0.84	0.77	0.89	0.06	0.88	1010
0.18	0.76	0.78	0.78	0.75	0.82	0.03	0.80	0.75	0.77	0.77	0.73	0.81	0.04	0.80	0.75	0.79	0.80	0.73	0.86	0.06	0.84	1012
0.32	0.71	0.74	0.73	0.70	0.77	0.03	0.76	0.70	0.72	0.72	0.69	0.76	0.04	0.75	0.69	0.74	0.74	0.66	0.81	0.07	0.79	2002


==> data/mlm_plots/tef/imdb/lstmatt/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/imdb/lstmatt/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.28	3.43	3.39	3.25	3.61	0.18	3.58	38.53	86.17	69.46	23.01	149.32	63.16	121.22	5.53	16.26	12.76	2.51	30.01	13.75	23.65	936
0.03	4.51	4.73	4.66	4.42	5.04	0.31	4.87	52.78	115.38	96.79	34.96	195.80	80.42	156.15	8.22	22.55	17.88	4.23	40.88	18.32	32.36	1003
0.06	6.71	6.97	6.80	6.55	7.40	0.43	7.12	69.07	146.64	129.24	50.17	243.11	96.47	198.64	9.96	27.34	23.01	6.19	48.48	21.14	40.12	1009
0.11	7.73	8.01	7.87	7.60	8.43	0.42	8.27	81.85	161.18	143.71	60.76	261.60	100.42	212.04	11.48	29.94	25.80	7.38	52.50	22.56	43.86	1010
0.15	12.45	12.96	12.80	12.32	13.60	0.64	13.16	93.00	179.08	169.60	75.73	282.42	103.34	231.25	13.08	32.52	28.23	8.79	56.24	23.72	47.77	1010
0.18	14.55	14.83	14.67	13.96	15.70	0.87	15.38	107.36	186.74	176.57	85.67	287.81	101.07	242.04	13.22	32.77	29.16	9.45	56.09	23.32	47.59	1012
0.32	17.13	20.20	20.55	17.09	23.31	3.11	22.44	118.94	190.98	180.43	90.77	291.19	100.21	243.28	13.70	32.40	28.50	9.51	55.30	22.89	46.30	2002


==> data/mlm_plots/tef/imdb/lstmatt/s/time_misc_auc.tex <==
name	auc
attack_time	3.92
l2	52.48
lom	9.38


==> data/mlm_plots/tef/imdb/lstmatt/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.45	0.56	0.57	0.40	0.72	0.16	0.67	0.68	0.75	0.76	0.65	0.85	0.10	0.82	0.79	0.84	0.85	0.77	0.91	0.07	0.89	936
0.03	0.28	0.40	0.40	0.24	0.56	0.16	0.50	0.55	0.63	0.63	0.52	0.75	0.12	0.72	0.70	0.76	0.77	0.68	0.85	0.09	0.82	1003
0.06	0.18	0.29	0.27	0.13	0.44	0.15	0.38	0.46	0.53	0.53	0.41	0.66	0.12	0.62	0.62	0.69	0.69	0.59	0.79	0.10	0.75	1009
0.11	0.12	0.22	0.20	0.08	0.36	0.14	0.30	0.38	0.46	0.46	0.33	0.59	0.13	0.54	0.57	0.63	0.63	0.53	0.73	0.10	0.70	1010
0.15	0.06	0.15	0.14	0.03	0.27	0.12	0.23	0.30	0.38	0.38	0.26	0.50	0.12	0.46	0.50	0.57	0.56	0.47	0.67	0.10	0.63	1010
0.18	0.00	0.11	0.09	0.00	0.22	0.11	0.18	0.25	0.32	0.32	0.22	0.43	0.11	0.40	0.46	0.52	0.52	0.43	0.61	0.09	0.58	1012
0.32	0.00	0.07	0.05	-0.02	0.16	0.09	0.11	0.17	0.25	0.25	0.15	0.36	0.11	0.32	0.39	0.45	0.45	0.36	0.55	0.09	0.51	2002


==> data/mlm_plots/tef/imdb/lstmatt/s/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.12
top50	0.18


==> data/mlm_plots/tef/imdb/roberta/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.29	59.50	53.30	34.65	84.34	24.85	71.79	14.00	18.87	18.00	12.14	25.60	6.73	23.00	48.41	66.81	60.64	39.89	93.73	26.92	81.11	15.00	19.33	19.00	12.52	26.15	6.81	23.00	937
0.03	42.25	59.62	53.36	34.66	84.59	24.96	71.87	14.00	18.58	18.00	11.72	25.43	6.85	23.00	55.15	75.57	68.60	46.11	105.02	29.46	90.69	15.00	19.36	19.00	12.39	26.34	6.97	24.00	991
0.06	42.29	60.01	53.82	34.64	85.38	25.37	72.67	14.00	18.46	18.00	11.55	25.38	6.91	23.00	66.37	89.64	82.51	55.31	123.96	34.32	106.01	15.00	19.71	20.00	12.58	26.85	7.14	24.00	1001
0.11	42.38	60.09	54.01	34.73	85.45	25.36	72.94	14.00	18.48	18.00	11.53	25.43	6.95	23.00	79.00	105.15	97.90	66.76	143.55	38.40	123.23	15.00	20.18	20.00	12.94	27.43	7.25	25.00	1006
0.15	42.04	59.01	52.72	33.90	84.11	25.11	71.30	14.00	18.43	18.00	11.52	25.34	6.91	23.00	99.65	131.42	123.54	85.56	177.28	45.86	151.89	16.00	20.73	20.00	13.40	28.05	7.33	25.00	1109
0.18	41.42	58.76	53.10	33.50	84.01	25.25	70.94	14.00	18.67	18.00	11.77	25.58	6.91	23.00	121.55	159.20	151.31	106.45	211.95	52.75	185.11	17.00	21.64	22.00	14.32	28.97	7.33	26.00	1212
0.32	43.32	61.49	55.28	36.02	86.96	25.47	75.95	14.00	18.39	18.00	11.52	25.26	6.87	23.00	155.04	205.58	192.29	134.56	276.60	71.02	241.14	17.00	21.83	22.00	14.51	29.15	7.32	26.00	1668


==> data/mlm_plots/tef/imdb/roberta/a/comparison_vals_auc.tex <==
name	auc
orig_pp	18.57
orig_ge	5.75
adv_pp	43.35
adv_ge	6.48


==> data/mlm_plots/tef/imdb/roberta/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.64	0.73	0.77	0.57	0.90	0.16	0.85	0.96	0.97	0.97	0.94	0.99	0.02	0.98	0.85	0.88	0.88	0.83	0.92	0.04	0.91	937
0.03	0.46	0.59	0.62	0.40	0.78	0.19	0.74	0.92	0.94	0.95	0.90	0.98	0.04	0.96	0.78	0.81	0.82	0.75	0.87	0.06	0.85	991
0.06	0.31	0.45	0.47	0.26	0.65	0.19	0.60	0.87	0.90	0.91	0.84	0.96	0.06	0.94	0.71	0.75	0.76	0.68	0.83	0.07	0.81	1001
0.11	0.22	0.36	0.36	0.18	0.54	0.18	0.49	0.84	0.87	0.88	0.80	0.94	0.07	0.92	0.66	0.71	0.72	0.63	0.79	0.08	0.77	1006
0.15	0.13	0.26	0.25	0.10	0.43	0.17	0.38	0.78	0.82	0.84	0.73	0.91	0.09	0.89	0.59	0.65	0.66	0.55	0.74	0.10	0.71	1109
0.18	0.09	0.21	0.19	0.05	0.38	0.16	0.32	0.73	0.79	0.81	0.68	0.89	0.10	0.86	0.55	0.61	0.62	0.51	0.72	0.10	0.69	1212
0.32	0.05	0.17	0.14	0.02	0.33	0.16	0.26	0.68	0.75	0.78	0.63	0.88	0.13	0.84	0.50	0.57	0.59	0.46	0.69	0.12	0.66	1668


==> data/mlm_plots/tef/imdb/roberta/a/correlations_auc.tex <==
name	auc
pcc	0.10
spearman	0.26
kendall	0.21


==> data/mlm_plots/tef/imdb/roberta/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	1.96	4.25	3.23	0.85	7.64	3.39	5.40	1.70	3.98	2.97	0.48	7.48	3.50	4.96	1.73	4.32	3.06	0.50	8.14	3.82	5.70	937
0.03	1.95	3.50	3.10	1.35	5.66	2.16	4.51	1.73	3.36	2.78	0.90	5.82	2.46	4.27	1.99	4.55	3.38	0.73	8.37	3.82	5.68	991
0.06	1.94	2.93	2.79	1.64	4.22	1.29	3.71	1.77	2.85	2.63	1.41	4.28	1.44	3.58	2.13	4.28	3.48	0.86	7.70	3.42	5.24	1001
0.11	1.91	2.63	2.57	1.66	3.61	0.98	3.24	1.79	2.56	2.43	1.48	3.64	1.08	3.12	2.19	3.85	3.18	0.90	6.79	2.94	4.62	1006
0.15	1.80	2.27	2.26	1.62	2.92	0.65	2.67	1.77	2.24	2.21	1.51	2.98	0.73	2.61	2.09	3.24	2.91	1.49	5.00	1.75	3.96	1109
0.18	1.71	2.07	2.08	1.55	2.60	0.53	2.40	1.70	2.08	2.04	1.46	2.70	0.62	2.42	1.95	2.88	2.56	1.20	4.57	1.68	3.41	1212
0.32	1.64	1.92	1.94	1.49	2.36	0.44	2.19	1.65	1.95	1.94	1.46	2.44	0.49	2.24	1.91	2.58	2.39	1.51	3.65	1.07	3.05	1668


==> data/mlm_plots/tef/imdb/roberta/a/ets_sts_auc.tex <==
name	auc
et_use	0.76
et_tse	0.75
et_ce	1.04


==> data/mlm_plots/tef/imdb/roberta/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.54	1.34	0.97	-0.10	2.79	1.45	1.63	1.81	4.38	3.23	0.37	8.40	4.02	5.53	1.70	4.59	3.16	-0.59	9.76	5.17	5.62	937
0.03	0.45	0.92	0.71	-1.01	2.85	1.93	1.10	2.24	4.06	3.46	1.42	6.71	2.65	5.11	1.98	3.96	3.12	0.68	7.24	3.28	4.86	991
0.06	0.37	0.59	0.53	0.25	0.93	0.34	0.72	2.54	3.87	3.55	1.94	5.79	1.93	4.75	2.13	3.53	3.04	1.29	5.76	2.23	4.21	1001
0.11	0.30	0.44	0.41	0.23	0.66	0.21	0.54	2.65	3.69	3.50	2.14	5.24	1.55	4.43	2.23	3.27	3.00	1.56	4.98	1.71	3.89	1006
0.15	0.22	0.31	0.29	0.18	0.44	0.13	0.37	2.68	3.46	3.36	2.31	4.61	1.15	4.06	2.25	3.01	2.81	1.80	4.22	1.21	3.50	1109
0.18	0.17	0.24	0.22	0.13	0.34	0.10	0.29	2.64	3.30	3.17	2.29	4.31	1.01	3.84	2.16	2.84	2.68	1.78	3.90	1.06	3.28	1212
0.32	0.13	0.18	0.17	0.11	0.26	0.08	0.23	2.56	3.14	3.08	2.25	4.03	0.89	3.62	2.11	2.67	2.61	1.79	3.56	0.89	3.05	1668


==> data/mlm_plots/tef/imdb/roberta/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.12
et_p_h	1.09
et_p_l2	0.97


==> data/mlm_plots/tef/imdb/roberta/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.09	0.13	0.13	0.07	0.19	0.06	0.16	0.02	0.04	0.04	0.02	0.07	0.03	0.06	0.03	0.04	0.04	0.02	0.06	0.02	0.05	937
0.03	0.21	0.29	0.27	0.17	0.40	0.11	0.35	0.05	0.07	0.06	0.04	0.10	0.03	0.09	0.04	0.06	0.06	0.04	0.08	0.02	0.07	991
0.06	0.40	0.53	0.51	0.35	0.70	0.17	0.64	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.06	0.08	0.08	0.06	0.10	0.02	0.09	1001
0.11	0.62	0.81	0.78	0.54	1.07	0.26	0.97	0.09	0.11	0.11	0.08	0.14	0.03	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.11	1006
0.15	1.02	1.33	1.28	0.89	1.77	0.44	1.59	0.11	0.13	0.13	0.10	0.17	0.04	0.15	0.10	0.11	0.11	0.09	0.14	0.02	0.13	1109
0.18	1.39	1.87	1.80	1.21	2.53	0.66	2.24	0.13	0.15	0.15	0.11	0.19	0.04	0.17	0.11	0.12	0.12	0.10	0.15	0.03	0.14	1212
0.32	1.85	2.55	2.38	1.60	3.49	0.95	3.11	0.14	0.16	0.16	0.13	0.20	0.04	0.19	0.12	0.14	0.14	0.11	0.16	0.03	0.15	1668


==> data/mlm_plots/tef/imdb/roberta/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.45
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/roberta/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.02	0.97	0.95	0.96	0.96	0.93	0.98	0.02	0.97	0.94	0.96	0.96	0.92	0.99	0.03	0.98	937
0.03	0.92	0.93	0.94	0.91	0.96	0.02	0.95	0.91	0.93	0.93	0.90	0.96	0.03	0.95	0.92	0.94	0.94	0.90	0.98	0.04	0.96	991
0.06	0.89	0.90	0.90	0.88	0.93	0.03	0.92	0.87	0.89	0.90	0.86	0.93	0.03	0.92	0.89	0.91	0.92	0.87	0.96	0.04	0.95	1001
0.11	0.86	0.87	0.87	0.85	0.90	0.03	0.89	0.84	0.87	0.87	0.83	0.90	0.03	0.89	0.87	0.89	0.90	0.85	0.94	0.05	0.93	1006
0.15	0.82	0.83	0.83	0.81	0.86	0.03	0.85	0.81	0.83	0.83	0.79	0.86	0.04	0.85	0.84	0.87	0.87	0.81	0.92	0.05	0.91	1109
0.18	0.79	0.81	0.81	0.78	0.83	0.03	0.82	0.78	0.80	0.81	0.77	0.84	0.04	0.83	0.81	0.84	0.85	0.78	0.90	0.06	0.88	1212
0.32	0.76	0.78	0.78	0.75	0.81	0.03	0.80	0.76	0.78	0.78	0.75	0.82	0.04	0.81	0.79	0.82	0.83	0.76	0.88	0.06	0.86	1668


==> data/mlm_plots/tef/imdb/roberta/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/imdb/roberta/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	4.94	6.15	6.11	4.39	7.90	1.76	7.04	0.07	0.13	0.11	0.05	0.21	0.08	0.16	3.25	11.32	7.53	-0.78	23.43	12.11	15.30	937
0.03	6.83	8.66	8.68	6.11	11.20	2.55	10.06	0.11	0.18	0.15	0.08	0.28	0.10	0.22	4.93	15.84	10.85	0.33	31.35	15.51	21.81	991
0.06	8.44	10.63	10.58	7.45	13.81	3.18	12.51	0.15	0.23	0.21	0.11	0.36	0.12	0.29	7.04	20.99	15.03	1.87	40.10	19.12	28.73	1001
0.11	10.30	13.06	12.93	8.94	17.19	4.12	15.15	0.18	0.28	0.25	0.14	0.42	0.14	0.36	8.19	24.46	18.62	3.06	45.87	21.40	34.18	1006
0.15	16.47	20.48	20.15	14.49	26.46	5.99	24.17	0.23	0.35	0.32	0.19	0.51	0.16	0.44	10.21	28.40	21.64	4.39	52.40	24.00	40.34	1109
0.18	18.97	23.61	23.42	16.75	30.47	6.86	28.06	0.27	0.40	0.37	0.23	0.57	0.17	0.50	11.42	31.80	24.26	5.60	58.00	26.20	46.70	1212
0.32	22.43	28.24	27.91	19.54	36.94	8.70	33.39	0.29	0.43	0.41	0.25	0.62	0.18	0.56	11.76	32.42	26.80	6.85	58.00	25.58	46.78	1668


==> data/mlm_plots/tef/imdb/roberta/a/time_misc_auc.tex <==
name	auc
attack_time	6.00
l2	0.10
lom	8.43


==> data/mlm_plots/tef/imdb/roberta/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.69	0.75	0.77	0.64	0.87	0.12	0.83	0.88	0.90	0.91	0.85	0.95	0.05	0.93	0.93	0.94	0.95	0.91	0.97	0.03	0.97	937
0.03	0.56	0.65	0.67	0.50	0.79	0.14	0.75	0.81	0.85	0.86	0.78	0.91	0.06	0.89	0.89	0.91	0.92	0.88	0.95	0.04	0.94	991
0.06	0.46	0.56	0.57	0.41	0.72	0.16	0.67	0.76	0.80	0.81	0.72	0.88	0.08	0.86	0.86	0.89	0.89	0.84	0.93	0.05	0.92	1001
0.11	0.40	0.51	0.53	0.35	0.68	0.17	0.64	0.71	0.77	0.77	0.68	0.85	0.09	0.83	0.84	0.86	0.87	0.81	0.92	0.05	0.90	1006
0.15	0.33	0.46	0.47	0.28	0.64	0.18	0.59	0.67	0.73	0.74	0.63	0.82	0.10	0.79	0.80	0.83	0.84	0.77	0.89	0.06	0.88	1109
0.18	0.29	0.43	0.44	0.24	0.62	0.19	0.57	0.65	0.71	0.71	0.60	0.81	0.11	0.78	0.78	0.82	0.83	0.75	0.88	0.06	0.86	1212
0.32	0.25	0.40	0.41	0.20	0.59	0.20	0.55	0.61	0.68	0.69	0.57	0.79	0.11	0.76	0.76	0.80	0.81	0.73	0.87	0.07	0.84	1668


==> data/mlm_plots/tef/imdb/roberta/a/top_intersections_auc.tex <==
name	auc
top10	0.15
top30	0.23
top50	0.26


==> data/mlm_plots/tef/imdb/roberta/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.06	58.80	53.15	34.91	82.69	23.89	71.13	15.00	19.08	19.00	12.45	25.71	6.63	23.00	46.49	64.99	59.70	39.65	90.34	25.34	78.51	15.00	19.54	19.00	12.81	26.28	6.73	24.00	904
0.03	42.06	59.26	53.30	34.42	84.09	24.84	71.83	14.00	18.58	18.00	11.74	25.43	6.84	23.00	52.93	73.25	67.33	44.81	101.69	28.44	88.74	15.00	19.38	19.00	12.32	26.43	7.06	23.50	995
0.06	42.57	59.69	53.17	34.50	84.89	25.20	72.67	14.00	18.48	18.00	11.42	25.54	7.06	23.00	63.29	86.96	79.76	54.29	119.63	32.67	103.63	15.00	19.69	19.00	12.37	27.01	7.32	24.00	1153
0.11	41.68	59.50	52.97	34.04	84.96	25.46	72.78	14.00	18.30	18.00	11.47	25.13	6.83	23.00	75.26	103.04	95.62	65.40	140.68	37.64	122.07	15.00	19.95	19.00	12.70	27.19	7.25	24.00	1226
0.15	42.28	60.05	54.06	34.17	85.92	25.88	73.46	13.00	18.06	18.00	11.22	24.91	6.84	22.50	101.82	132.00	123.08	86.97	177.03	45.03	156.27	15.50	20.28	20.00	12.93	27.62	7.35	25.00	1203
0.18	42.28	59.76	53.36	34.56	84.96	25.20	71.87	14.00	18.58	18.00	11.69	25.48	6.89	23.00	128.87	165.06	153.13	112.61	217.50	52.45	194.88	17.00	21.32	21.00	13.91	28.74	7.42	26.00	1039
0.32	42.96	60.59	55.31	35.94	85.24	24.65	72.42	14.00	18.89	19.00	11.95	25.82	6.94	23.00	160.83	213.75	197.92	140.88	286.63	72.88	250.07	18.00	22.34	22.00	14.96	29.73	7.38	27.00	1353


==> data/mlm_plots/tef/imdb/roberta/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	18.59
orig_ge	5.76
adv_pp	44.15
adv_ge	6.46


==> data/mlm_plots/tef/imdb/roberta/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.16	0.39	0.44	0.06	0.71	0.33	0.63	0.35	0.52	0.57	0.26	0.77	0.26	0.71	0.25	0.39	0.42	0.18	0.61	0.21	0.54	904
0.03	-0.02	0.17	0.18	-0.15	0.49	0.32	0.40	0.16	0.34	0.38	0.08	0.60	0.26	0.52	0.11	0.25	0.27	0.05	0.45	0.20	0.38	995
0.06	-0.13	0.01	0.01	-0.29	0.32	0.31	0.20	0.02	0.20	0.21	-0.07	0.47	0.27	0.39	0.02	0.15	0.15	-0.05	0.35	0.20	0.28	1153
0.11	-0.18	-0.06	-0.05	-0.34	0.22	0.28	0.10	-0.03	0.12	0.12	-0.14	0.38	0.26	0.31	-0.02	0.09	0.09	-0.10	0.28	0.19	0.22	1226
0.15	-0.27	-0.14	-0.12	-0.40	0.11	0.25	0.01	-0.11	0.04	0.03	-0.18	0.26	0.22	0.19	-0.07	0.03	0.03	-0.13	0.19	0.16	0.14	1203
0.18	-0.35	-0.21	-0.19	-0.44	0.02	0.23	-0.06	-0.17	-0.02	-0.03	-0.23	0.19	0.21	0.13	-0.11	-0.01	-0.02	-0.16	0.15	0.15	0.10	1039
0.32	-0.36	-0.23	-0.23	-0.44	-0.03	0.20	-0.10	-0.19	-0.05	-0.07	-0.24	0.14	0.19	0.07	-0.13	-0.03	-0.04	-0.17	0.11	0.14	0.05	1353


==> data/mlm_plots/tef/imdb/roberta/ig/correlations_auc.tex <==
name	auc
pcc	-0.03
spearman	0.02
kendall	0.02


==> data/mlm_plots/tef/imdb/roberta/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	5.82	11.31	9.50	3.63	18.99	7.68	15.11	5.13	10.84	8.41	2.31	19.36	8.52	14.23	4.68	12.22	8.92	1.64	22.80	10.58	15.79	904
0.03	5.46	8.78	7.75	3.60	13.96	5.18	10.92	4.88	8.66	7.43	2.75	14.58	5.91	10.91	5.39	11.93	9.00	1.93	21.93	10.00	15.09	995
0.06	4.58	6.61	5.93	3.43	9.78	3.18	7.93	4.48	6.80	6.03	3.16	10.44	3.64	8.60	5.07	10.59	8.04	2.23	18.94	8.36	12.97	1153
0.11	3.87	5.19	4.81	3.18	7.19	2.01	6.09	3.82	5.35	4.82	2.97	7.73	2.38	6.31	4.51	8.77	6.87	1.69	15.85	7.08	10.34	1226
0.15	3.26	4.11	3.88	2.80	5.42	1.31	4.73	3.22	4.28	3.92	2.69	5.87	1.59	5.00	4.04	7.03	5.74	1.69	12.38	5.34	8.02	1203
0.18	2.90	3.49	3.37	2.58	4.39	0.90	3.90	2.94	3.61	3.47	2.53	4.69	1.08	4.08	3.51	5.51	4.66	2.02	9.01	3.50	6.75	1039
0.32	2.48	2.99	2.85	2.23	3.74	0.76	3.43	2.48	3.07	2.93	2.18	3.96	0.89	3.53	2.87	4.32	3.82	2.01	6.63	2.31	5.07	1353


==> data/mlm_plots/tef/imdb/roberta/ig/ets_sts_auc.tex <==
name	auc
et_use	1.48
et_tse	1.51
et_ce	2.26


==> data/mlm_plots/tef/imdb/roberta/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.48	5.44	2.73	-7.46	18.33	12.89	4.70	4.57	11.24	8.08	-0.84	23.32	12.08	13.06	4.00	11.87	7.38	-2.10	25.85	13.97	13.82	904
0.03	1.13	2.89	1.62	-7.89	13.66	10.78	2.47	5.15	8.82	7.07	2.06	15.58	6.76	10.16	4.19	8.57	6.29	0.41	16.72	8.16	9.53	995
0.06	0.74	1.25	1.04	0.05	2.44	1.19	1.43	4.98	7.52	6.36	2.57	12.46	4.95	8.69	4.07	6.90	5.30	1.81	11.99	5.09	7.88	1153
0.11	0.51	0.80	0.69	0.08	1.51	0.71	0.93	4.58	6.42	5.81	3.00	9.84	3.42	7.34	3.73	5.73	4.86	1.78	9.67	3.94	6.23	1226
0.15	0.34	0.50	0.45	0.26	0.74	0.24	0.61	4.29	5.57	5.28	3.54	7.59	2.03	6.40	3.48	4.79	4.33	2.42	7.16	2.37	5.41	1203
0.18	0.25	0.36	0.33	0.19	0.54	0.18	0.43	4.01	5.12	4.81	3.42	6.83	1.70	5.80	3.26	4.37	3.94	2.48	6.26	1.89	4.95	1039
0.32	0.17	0.27	0.24	0.12	0.42	0.15	0.33	3.74	4.72	4.48	3.23	6.20	1.49	5.42	3.07	3.99	3.71	2.55	5.44	1.45	4.60	1353


==> data/mlm_plots/tef/imdb/roberta/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.28
et_p_h	1.89
et_p_l2	1.69


==> data/mlm_plots/tef/imdb/roberta/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.12	0.11	0.05	0.18	0.06	0.16	0.02	0.04	0.04	0.02	0.07	0.03	0.06	0.02	0.04	0.04	0.02	0.06	0.02	0.05	904
0.03	0.17	0.25	0.25	0.14	0.37	0.12	0.32	0.04	0.07	0.07	0.04	0.10	0.03	0.09	0.04	0.06	0.06	0.04	0.08	0.02	0.07	995
0.06	0.37	0.49	0.47	0.30	0.68	0.19	0.61	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.06	0.07	0.08	0.05	0.10	0.02	0.09	1153
0.11	0.58	0.79	0.76	0.49	1.09	0.30	0.97	0.09	0.11	0.11	0.07	0.14	0.04	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.11	1226
0.15	0.97	1.31	1.27	0.84	1.78	0.47	1.60	0.11	0.13	0.13	0.10	0.17	0.04	0.16	0.09	0.11	0.11	0.08	0.13	0.02	0.13	1203
0.18	1.43	1.94	1.86	1.22	2.65	0.72	2.31	0.13	0.15	0.15	0.11	0.19	0.04	0.17	0.11	0.12	0.13	0.10	0.15	0.03	0.14	1039
0.32	1.95	2.77	2.60	1.59	3.95	1.18	3.38	0.14	0.17	0.17	0.13	0.20	0.04	0.19	0.12	0.14	0.14	0.11	0.16	0.03	0.15	1353


==> data/mlm_plots/tef/imdb/roberta/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.47
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/roberta/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.96	0.96	0.97	0.94	0.99	0.02	0.98	0.95	0.96	0.97	0.93	0.99	0.03	0.98	904
0.03	0.94	0.95	0.95	0.93	0.97	0.02	0.96	0.93	0.94	0.95	0.91	0.97	0.03	0.96	0.94	0.95	0.96	0.91	0.98	0.03	0.97	995
0.06	0.90	0.92	0.92	0.89	0.94	0.03	0.94	0.90	0.92	0.92	0.88	0.95	0.03	0.94	0.92	0.93	0.94	0.89	0.97	0.04	0.96	1153
0.11	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.87	0.89	0.89	0.86	0.93	0.03	0.91	0.90	0.92	0.92	0.87	0.96	0.04	0.95	1226
0.15	0.83	0.85	0.85	0.82	0.89	0.03	0.87	0.84	0.86	0.86	0.82	0.89	0.04	0.88	0.87	0.89	0.90	0.84	0.94	0.05	0.93	1203
0.18	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.80	0.82	0.83	0.79	0.86	0.04	0.85	0.84	0.87	0.87	0.81	0.92	0.05	0.91	1039
0.32	0.76	0.79	0.79	0.75	0.82	0.03	0.81	0.76	0.79	0.79	0.75	0.83	0.04	0.82	0.80	0.83	0.84	0.77	0.90	0.06	0.87	1353


==> data/mlm_plots/tef/imdb/roberta/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.28


==> data/mlm_plots/tef/imdb/roberta/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	13.43	16.08	16.03	10.86	21.30	5.22	18.06	1.13	7.37	1.89	-7.41	22.16	14.78	7.24	3.65	16.47	9.20	-2.05	34.98	18.51	22.07	904
0.03	17.12	20.43	20.50	15.42	25.43	5.01	23.41	1.58	11.64	3.34	-6.75	30.02	18.38	15.11	5.05	19.95	12.55	-0.24	40.15	20.19	27.26	995
0.06	22.99	32.25	28.02	16.40	48.10	15.85	34.40	2.05	20.67	7.12	-13.27	54.61	33.94	26.58	6.72	23.93	16.25	1.65	46.20	22.27	35.57	1153
0.11	29.77	40.31	36.71	23.77	56.85	16.54	46.20	2.47	21.36	10.07	-9.81	52.54	31.18	31.54	7.11	24.82	17.84	2.26	47.38	22.56	36.96	1226
0.15	40.31	50.93	49.79	35.40	66.46	15.53	58.83	3.09	20.45	12.47	-4.88	45.79	25.34	29.14	7.98	26.29	18.67	3.15	49.43	23.14	39.03	1203
0.18	49.30	59.69	60.00	44.22	75.16	15.47	69.08	3.21	18.30	10.84	-3.24	39.83	21.54	26.19	9.21	28.51	22.65	4.63	52.39	23.88	42.21	1039
0.32	57.70	70.59	69.18	50.99	90.19	19.60	80.78	2.67	14.87	7.04	-6.08	35.82	20.95	20.26	8.84	26.52	20.09	4.41	48.64	22.12	39.52	1353


==> data/mlm_plots/tef/imdb/roberta/ig/time_misc_auc.tex <==
name	auc
attack_time	15.58
l2	5.48
lom	7.95


==> data/mlm_plots/tef/imdb/roberta/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.26	0.41	0.41	0.21	0.60	0.20	0.55	0.47	0.58	0.59	0.42	0.73	0.15	0.69	0.63	0.70	0.71	0.59	0.81	0.11	0.78	904
0.03	0.17	0.29	0.29	0.12	0.46	0.17	0.40	0.38	0.48	0.49	0.34	0.62	0.14	0.58	0.56	0.63	0.64	0.53	0.74	0.11	0.71	995
0.06	0.11	0.22	0.19	0.06	0.37	0.16	0.31	0.32	0.41	0.42	0.28	0.55	0.14	0.51	0.53	0.59	0.59	0.48	0.69	0.11	0.66	1153
0.11	0.08	0.18	0.17	0.04	0.32	0.14	0.27	0.28	0.37	0.37	0.24	0.51	0.14	0.46	0.49	0.56	0.56	0.45	0.66	0.10	0.62	1226
0.15	0.06	0.14	0.12	0.02	0.27	0.12	0.22	0.26	0.34	0.33	0.22	0.45	0.12	0.42	0.47	0.53	0.53	0.44	0.62	0.09	0.58	1203
0.18	0.00	0.12	0.09	0.01	0.23	0.11	0.19	0.24	0.32	0.31	0.20	0.43	0.11	0.39	0.45	0.51	0.51	0.43	0.59	0.08	0.56	1039
0.32	0.00	0.11	0.08	0.00	0.21	0.11	0.17	0.23	0.30	0.29	0.20	0.41	0.11	0.37	0.45	0.50	0.50	0.42	0.58	0.08	0.55	1353


==> data/mlm_plots/tef/imdb/roberta/ig/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.11
top50	0.17


==> data/mlm_plots/tef/imdb/roberta/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	41.91	58.94	53.12	34.41	83.47	24.53	71.05	14.00	18.99	19.00	12.50	25.48	6.49	23.00	47.05	66.00	60.50	39.57	92.44	26.44	78.16	15.00	19.36	19.00	12.83	25.88	6.53	23.00	903
0.03	42.18	59.68	53.33	34.76	84.60	24.92	72.63	14.00	18.64	18.00	11.91	25.37	6.73	23.00	53.61	74.91	69.14	45.85	103.97	29.06	89.85	15.00	19.33	19.00	12.52	26.14	6.81	23.00	1010
0.06	42.22	59.24	53.33	34.54	83.95	24.71	71.19	14.00	18.55	18.00	11.89	25.22	6.66	23.00	64.30	87.27	80.73	54.48	120.05	32.78	103.80	15.00	19.72	20.00	12.88	26.57	6.85	24.00	1120
0.11	41.91	58.99	52.78	33.63	84.34	25.36	71.10	14.00	18.56	18.00	11.65	25.46	6.91	23.00	77.57	103.58	98.79	66.12	141.05	37.47	121.59	15.00	20.23	20.00	13.06	27.39	7.17	25.00	1178
0.15	41.38	58.60	52.78	34.26	82.95	24.35	70.92	14.00	18.56	18.00	11.72	25.40	6.84	23.00	98.85	130.20	123.63	85.64	174.75	44.55	149.96	16.00	20.85	21.00	13.74	27.96	7.11	25.00	1198
0.18	42.28	59.22	52.61	34.05	84.39	25.17	71.79	14.00	18.50	18.00	11.56	25.44	6.94	23.00	122.18	160.31	151.56	105.73	214.89	54.58	184.21	16.00	21.25	21.00	13.83	28.67	7.42	25.50	1255
0.32	44.49	63.68	58.22	36.94	90.41	26.73	77.78	14.00	18.21	18.00	11.10	25.31	7.10	23.00	156.61	206.73	195.48	132.67	280.80	74.06	238.81	16.00	21.43	22.00	13.81	29.05	7.62	26.00	1221


==> data/mlm_plots/tef/imdb/roberta/s/comparison_vals_auc.tex <==
name	auc
orig_pp	18.66
orig_ge	5.74
adv_pp	43.29
adv_ge	6.42


==> data/mlm_plots/tef/imdb/roberta/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.56	0.69	0.73	0.48	0.90	0.21	0.86	0.81	0.85	0.89	0.72	0.98	0.13	0.93	0.63	0.70	0.72	0.56	0.83	0.14	0.80	903
0.03	0.34	0.49	0.51	0.27	0.71	0.22	0.66	0.66	0.73	0.78	0.54	0.92	0.19	0.87	0.48	0.57	0.60	0.40	0.74	0.17	0.69	1010
0.06	0.19	0.33	0.32	0.13	0.52	0.20	0.47	0.49	0.60	0.65	0.36	0.84	0.24	0.77	0.34	0.45	0.47	0.26	0.64	0.19	0.58	1120
0.11	0.12	0.24	0.23	0.07	0.42	0.18	0.36	0.36	0.52	0.56	0.28	0.75	0.23	0.69	0.25	0.38	0.40	0.20	0.56	0.18	0.51	1178
0.15	0.06	0.17	0.14	0.01	0.32	0.16	0.26	0.29	0.44	0.46	0.21	0.66	0.22	0.59	0.20	0.31	0.32	0.15	0.48	0.16	0.42	1198
0.18	0.00	0.11	0.10	-0.04	0.26	0.15	0.20	0.18	0.33	0.35	0.09	0.58	0.24	0.51	0.12	0.24	0.24	0.06	0.41	0.17	0.36	1255
0.32	-0.04	0.07	0.05	-0.08	0.22	0.15	0.16	0.08	0.27	0.28	0.01	0.53	0.26	0.46	0.06	0.19	0.19	0.01	0.37	0.18	0.32	1221


==> data/mlm_plots/tef/imdb/roberta/s/correlations_auc.tex <==
name	auc
pcc	0.06
spearman	0.14
kendall	0.10


==> data/mlm_plots/tef/imdb/roberta/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	2.21	5.37	4.20	1.09	9.64	4.28	7.56	2.24	5.52	4.07	0.61	10.42	4.90	7.08	2.26	6.54	4.33	0.14	12.93	6.40	8.47	903
0.03	2.81	4.64	4.04	1.97	7.31	2.67	5.98	2.69	4.78	3.95	1.44	8.12	3.34	5.97	3.30	7.26	5.51	1.11	13.42	6.16	9.08	1010
0.06	2.70	3.90	3.65	2.29	5.50	1.61	4.79	2.66	4.00	3.66	2.09	5.91	1.91	5.07	3.44	6.58	5.13	1.39	11.78	5.20	8.02	1120
0.11	2.50	3.28	3.16	2.15	4.41	1.13	3.86	2.47	3.35	3.15	2.02	4.67	1.33	3.98	3.18	5.48	4.49	1.73	9.24	3.75	6.50	1178
0.15	2.25	2.72	2.64	1.98	3.45	0.73	3.10	2.23	2.77	2.67	1.92	3.63	0.86	3.16	2.84	4.40	3.75	1.91	6.89	2.49	5.21	1198
0.18	2.09	2.48	2.42	1.83	3.13	0.65	2.81	2.08	2.55	2.47	1.81	3.29	0.74	2.91	2.61	3.80	3.43	1.88	5.73	1.93	4.57	1255
0.32	1.98	2.29	2.25	1.79	2.79	0.50	2.55	1.97	2.37	2.31	1.68	3.05	0.68	2.67	2.29	3.30	2.99	1.70	4.90	1.60	3.85	1221


==> data/mlm_plots/tef/imdb/roberta/s/ets_sts_auc.tex <==
name	auc
et_use	0.94
et_tse	0.97
et_ce	1.47


==> data/mlm_plots/tef/imdb/roberta/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.59	1.96	1.15	-2.03	5.96	4.00	2.09	2.09	5.66	4.00	0.03	11.30	5.63	7.34	1.91	6.05	3.68	-0.61	12.70	6.65	7.47	903
0.03	0.63	1.13	0.95	0.24	2.03	0.89	1.38	3.10	5.26	4.52	1.90	8.62	3.36	6.59	2.66	5.18	4.04	0.92	9.44	4.26	6.28	1010
0.06	0.49	0.78	0.68	0.30	1.25	0.48	0.94	3.43	4.92	4.53	2.71	7.13	2.21	6.03	2.82	4.48	3.88	1.94	7.02	2.54	5.27	1120
0.11	0.36	0.52	0.47	0.28	0.77	0.24	0.63	3.35	4.44	4.16	2.81	6.08	1.63	5.21	2.74	3.95	3.53	2.05	5.85	1.90	4.55	1178
0.15	0.26	0.35	0.32	0.21	0.49	0.14	0.41	3.19	3.95	3.80	2.74	5.15	1.20	4.55	2.58	3.41	3.15	2.03	4.78	1.38	3.90	1198
0.18	0.19	0.27	0.25	0.16	0.38	0.11	0.32	3.12	3.74	3.66	2.72	4.76	1.02	4.26	2.54	3.19	3.01	2.06	4.31	1.12	3.64	1255
0.32	0.15	0.22	0.20	0.13	0.31	0.09	0.26	3.00	3.62	3.54	2.68	4.55	0.93	4.12	2.46	3.09	2.94	2.09	4.10	1.00	3.50	1221


==> data/mlm_plots/tef/imdb/roberta/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.15
et_p_h	1.30
et_p_l2	1.15


==> data/mlm_plots/tef/imdb/roberta/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.13	0.12	0.07	0.19	0.06	0.17	0.02	0.04	0.04	0.01	0.07	0.03	0.06	0.02	0.04	0.04	0.02	0.06	0.02	0.05	903
0.03	0.20	0.27	0.27	0.16	0.38	0.11	0.34	0.04	0.06	0.06	0.03	0.10	0.03	0.08	0.04	0.06	0.06	0.04	0.08	0.02	0.07	1010
0.06	0.38	0.51	0.48	0.32	0.69	0.18	0.61	0.07	0.09	0.09	0.06	0.12	0.03	0.11	0.06	0.07	0.07	0.05	0.10	0.02	0.09	1120
0.11	0.63	0.82	0.80	0.53	1.11	0.29	0.97	0.09	0.11	0.11	0.07	0.14	0.03	0.13	0.08	0.09	0.09	0.07	0.11	0.02	0.11	1178
0.15	1.02	1.32	1.28	0.89	1.75	0.43	1.58	0.11	0.13	0.13	0.10	0.17	0.04	0.16	0.10	0.11	0.11	0.09	0.13	0.02	0.13	1198
0.18	1.39	1.86	1.78	1.20	2.51	0.65	2.22	0.13	0.15	0.15	0.11	0.19	0.04	0.17	0.11	0.12	0.12	0.10	0.15	0.03	0.14	1255
0.32	1.77	2.46	2.29	1.45	3.47	1.01	2.97	0.13	0.16	0.16	0.12	0.20	0.04	0.18	0.12	0.13	0.13	0.11	0.16	0.03	0.15	1221


==> data/mlm_plots/tef/imdb/roberta/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.44
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/roberta/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.96	0.97	0.97	0.94	0.99	0.02	0.98	903
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.93	0.94	0.94	0.91	0.96	0.03	0.95	0.93	0.95	0.96	0.92	0.98	0.03	0.97	1010
0.06	0.89	0.91	0.91	0.88	0.93	0.02	0.92	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.91	0.93	0.94	0.89	0.97	0.04	0.96	1120
0.11	0.86	0.88	0.88	0.85	0.90	0.03	0.89	0.86	0.88	0.88	0.84	0.91	0.03	0.90	0.89	0.91	0.92	0.87	0.95	0.04	0.94	1178
0.15	0.82	0.84	0.84	0.82	0.87	0.03	0.86	0.82	0.84	0.85	0.81	0.88	0.03	0.87	0.86	0.89	0.89	0.84	0.93	0.05	0.92	1198
0.18	0.80	0.82	0.81	0.79	0.84	0.03	0.83	0.79	0.82	0.82	0.78	0.85	0.04	0.84	0.84	0.86	0.87	0.81	0.92	0.06	0.90	1255
0.32	0.77	0.79	0.79	0.76	0.82	0.03	0.81	0.77	0.80	0.80	0.76	0.83	0.04	0.82	0.80	0.84	0.85	0.78	0.90	0.06	0.88	1221


==> data/mlm_plots/tef/imdb/roberta/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/imdb/roberta/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	5.47	6.67	6.57	4.87	8.46	1.80	7.65	1.11	44.21	2.30	-165.07	253.49	209.28	7.59	1.97	7.34	4.79	-0.42	15.09	7.75	10.11	903
0.03	7.49	10.06	9.32	4.01	16.11	6.05	10.84	1.95	67.77	4.28	-258.76	394.30	326.53	18.06	3.18	11.00	7.89	0.25	21.75	10.75	15.07	1010
0.06	11.46	16.82	14.74	7.90	25.74	8.92	17.85	3.16	154.75	8.56	-567.18	876.69	721.93	56.43	4.70	14.87	11.55	1.34	28.40	13.53	20.82	1120
0.11	13.88	19.81	17.75	10.03	29.59	9.78	22.36	4.15	126.35	11.08	-270.15	522.84	396.49	52.99	5.29	15.49	12.88	3.16	27.82	12.33	23.01	1178
0.15	20.79	26.62	26.03	17.72	35.52	8.90	31.42	5.12	133.06	11.14	-322.06	588.18	455.12	38.28	6.01	16.43	13.51	3.51	29.34	12.92	24.31	1198
0.18	25.67	31.57	31.85	22.88	40.27	8.70	36.53	5.77	144.54	14.12	-334.82	623.91	479.37	44.97	6.68	17.46	14.61	4.22	30.70	13.24	26.01	1255
0.32	27.06	33.93	33.68	24.07	43.79	9.86	39.55	6.71	214.59	17.35	-453.21	882.39	667.80	66.22	6.15	17.60	14.09	3.88	31.31	13.72	25.50	1221


==> data/mlm_plots/tef/imdb/roberta/s/time_misc_auc.tex <==
name	auc
attack_time	7.88
l2	45.75
lom	4.94


==> data/mlm_plots/tef/imdb/roberta/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.50	0.61	0.62	0.42	0.79	0.18	0.75	0.71	0.77	0.79	0.66	0.89	0.12	0.86	0.82	0.85	0.87	0.78	0.93	0.08	0.91	903
0.03	0.31	0.45	0.44	0.26	0.63	0.19	0.59	0.60	0.67	0.69	0.54	0.81	0.13	0.77	0.74	0.79	0.81	0.70	0.89	0.09	0.86	1010
0.06	0.18	0.32	0.31	0.14	0.49	0.18	0.44	0.49	0.58	0.59	0.44	0.73	0.15	0.68	0.67	0.73	0.74	0.62	0.84	0.11	0.81	1120
0.11	0.12	0.25	0.22	0.09	0.41	0.16	0.36	0.44	0.53	0.54	0.39	0.67	0.14	0.63	0.62	0.69	0.70	0.59	0.80	0.10	0.77	1178
0.15	0.08	0.20	0.18	0.05	0.35	0.15	0.29	0.39	0.48	0.49	0.35	0.62	0.13	0.57	0.60	0.66	0.66	0.56	0.75	0.09	0.73	1198
0.18	0.06	0.15	0.12	0.01	0.29	0.14	0.22	0.33	0.43	0.44	0.30	0.57	0.14	0.52	0.55	0.62	0.62	0.52	0.72	0.10	0.69	1255
0.32	0.00	0.13	0.08	-0.01	0.28	0.14	0.20	0.29	0.40	0.38	0.25	0.54	0.14	0.49	0.52	0.59	0.59	0.49	0.70	0.10	0.67	1221


==> data/mlm_plots/tef/imdb/roberta/s/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.15
top50	0.21


==> data/mlm_plots/tef/imdb/xlnet/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.51	59.12	54.48	35.23	83.00	23.89	71.30	15.00	18.76	18.00	13.31	24.21	5.45	22.00	47.99	66.36	62.09	40.67	92.06	25.69	79.86	15.00	19.13	19.00	13.69	24.58	5.44	22.00	949
0.03	42.38	60.14	54.48	34.73	85.55	25.41	72.78	14.00	17.81	18.00	11.76	23.85	6.05	22.00	54.38	76.03	70.55	46.62	105.44	29.41	91.16	14.00	18.50	18.00	12.41	24.58	6.09	22.00	989
0.06	42.37	60.41	54.69	34.59	86.23	25.82	73.62	13.00	17.57	17.00	11.36	23.79	6.21	21.00	65.83	90.11	85.22	56.90	123.33	33.22	107.32	15.00	18.72	19.00	12.42	25.02	6.30	23.00	997
0.11	42.32	60.43	54.48	34.57	86.29	25.86	73.74	13.00	17.53	17.00	11.30	23.77	6.24	21.00	79.96	105.95	99.32	68.72	143.19	37.24	125.25	15.00	19.09	19.00	12.69	25.48	6.40	23.00	1003
0.15	41.96	59.93	54.29	34.19	85.67	25.74	72.63	13.00	17.50	17.00	11.32	23.68	6.18	21.00	103.01	134.11	126.96	89.83	178.39	44.28	155.56	16.00	19.77	20.00	13.26	26.28	6.51	24.00	1016
0.18	41.91	59.78	54.04	34.18	85.38	25.60	72.65	13.00	17.58	17.00	11.38	23.78	6.20	21.00	129.09	166.88	159.61	113.43	220.34	53.45	194.23	16.00	20.57	21.00	13.93	27.21	6.64	25.00	1082
0.32	42.76	61.28	55.21	35.33	87.24	25.96	74.51	14.00	17.61	17.00	11.42	23.81	6.20	21.00	163.04	216.82	205.32	143.42	290.22	73.40	256.28	17.00	21.46	22.00	14.86	28.07	6.60	26.00	1877


==> data/mlm_plots/tef/imdb/xlnet/a/comparison_vals_auc.tex <==
name	auc
orig_pp	18.72
orig_ge	5.47
adv_pp	44.93
adv_ge	6.21


==> data/mlm_plots/tef/imdb/xlnet/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.50	0.63	0.67	0.42	0.85	0.21	0.81	0.86	0.88	0.93	0.72	1.03	0.15	0.96	0.69	0.74	0.79	0.58	0.90	0.16	0.85	949
0.03	0.34	0.50	0.51	0.28	0.72	0.22	0.67	0.80	0.83	0.89	0.65	1.01	0.18	0.94	0.62	0.68	0.72	0.51	0.85	0.17	0.79	989
0.06	0.20	0.37	0.36	0.16	0.58	0.21	0.52	0.72	0.78	0.84	0.58	0.97	0.20	0.90	0.54	0.62	0.66	0.44	0.79	0.18	0.74	997
0.11	0.13	0.29	0.26	0.09	0.49	0.20	0.42	0.67	0.73	0.79	0.52	0.94	0.21	0.87	0.49	0.57	0.60	0.39	0.75	0.18	0.69	1003
0.15	0.07	0.21	0.17	0.02	0.39	0.19	0.31	0.57	0.67	0.73	0.44	0.89	0.23	0.82	0.41	0.51	0.54	0.32	0.69	0.19	0.64	1016
0.18	0.03	0.16	0.12	-0.02	0.34	0.18	0.26	0.51	0.62	0.68	0.38	0.85	0.24	0.78	0.36	0.46	0.50	0.27	0.65	0.19	0.59	1082
0.32	-0.00	0.11	0.07	-0.06	0.29	0.18	0.21	0.41	0.55	0.62	0.27	0.82	0.27	0.75	0.28	0.40	0.44	0.19	0.61	0.21	0.56	1877


==> data/mlm_plots/tef/imdb/xlnet/a/correlations_auc.tex <==
name	auc
pcc	0.08
spearman	0.21
kendall	0.16


==> data/mlm_plots/tef/imdb/xlnet/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	2.87	6.37	5.23	1.48	11.25	4.89	8.17	2.58	5.86	4.68	1.17	10.55	4.69	7.74	2.79	6.97	5.40	1.22	12.72	5.75	9.57	949
0.03	2.66	4.66	4.10	1.70	7.61	2.96	5.90	2.35	4.41	3.77	1.36	7.47	3.06	5.59	2.95	6.38	4.83	1.16	11.61	5.23	8.00	989
0.06	2.49	3.61	3.38	1.88	5.34	1.73	4.41	2.20	3.43	3.16	1.58	5.28	1.85	4.26	2.78	5.36	4.32	1.35	9.36	4.00	6.73	997
0.11	2.26	3.06	2.94	1.84	4.28	1.22	3.66	2.06	2.91	2.76	1.63	4.19	1.28	3.55	2.60	4.53	3.73	1.28	7.77	3.24	5.46	1003
0.15	2.02	2.51	2.46	1.71	3.31	0.80	2.96	1.89	2.42	2.36	1.59	3.26	0.84	2.86	2.30	3.54	3.15	1.62	5.45	1.92	4.28	1016
0.18	1.86	2.22	2.21	1.60	2.83	0.61	2.55	1.76	2.17	2.14	1.52	2.81	0.65	2.53	2.12	2.95	2.77	1.65	4.24	1.29	3.52	1082
0.32	1.72	2.00	2.00	1.50	2.50	0.50	2.28	1.69	1.99	1.97	1.47	2.52	0.52	2.28	1.88	2.57	2.44	1.54	3.60	1.03	3.03	1877


==> data/mlm_plots/tef/imdb/xlnet/a/ets_sts_auc.tex <==
name	auc
et_use	0.88
et_tse	0.85
et_ce	1.20


==> data/mlm_plots/tef/imdb/xlnet/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.75	2.59	1.30	-3.20	8.37	5.78	2.24	2.66	7.06	4.80	-0.47	14.59	7.53	8.46	2.29	7.04	4.54	-0.94	15.01	7.97	8.80	949
0.03	0.55	1.45	0.86	-3.26	6.16	4.71	1.32	2.78	5.42	4.36	1.02	9.83	4.40	6.78	2.37	5.20	3.74	0.18	10.23	5.02	6.25	989
0.06	0.42	0.73	0.59	0.04	1.41	0.68	0.87	3.01	4.61	4.17	1.93	7.29	2.68	5.51	2.54	4.20	3.53	1.18	7.21	3.01	4.89	997
0.11	0.32	0.51	0.44	0.16	0.87	0.36	0.61	3.04	4.25	3.95	2.00	6.50	2.25	4.92	2.54	3.83	3.28	1.01	6.65	2.82	4.34	1003
0.15	0.22	0.34	0.30	0.12	0.56	0.22	0.40	2.92	3.77	3.59	2.23	5.31	1.54	4.39	2.39	3.32	2.99	1.16	5.48	2.16	3.77	1016
0.18	0.17	0.25	0.22	0.12	0.38	0.13	0.29	2.79	3.45	3.36	2.24	4.67	1.21	4.00	2.26	2.97	2.81	1.54	4.40	1.43	3.43	1082
0.32	0.12	0.19	0.17	0.09	0.28	0.10	0.23	2.72	3.27	3.22	2.14	4.40	1.13	3.72	2.21	2.82	2.69	1.37	4.27	1.45	3.20	1877


==> data/mlm_plots/tef/imdb/xlnet/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.16
et_p_h	1.24
et_p_l2	1.11


==> data/mlm_plots/tef/imdb/xlnet/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.13	0.13	0.06	0.20	0.07	0.17	0.02	0.04	0.04	0.02	0.07	0.03	0.06	0.02	0.04	0.03	0.02	0.05	0.02	0.05	949
0.03	0.20	0.29	0.28	0.16	0.42	0.13	0.36	0.04	0.07	0.06	0.03	0.10	0.03	0.09	0.04	0.06	0.06	0.03	0.08	0.02	0.07	989
0.06	0.38	0.54	0.52	0.33	0.75	0.21	0.66	0.07	0.09	0.09	0.06	0.13	0.03	0.11	0.06	0.08	0.08	0.05	0.10	0.02	0.09	997
0.11	0.61	0.83	0.81	0.51	1.14	0.31	1.01	0.09	0.11	0.11	0.07	0.15	0.04	0.13	0.08	0.09	0.09	0.07	0.12	0.02	0.11	1003
0.15	1.02	1.37	1.31	0.86	1.87	0.51	1.67	0.11	0.13	0.13	0.10	0.17	0.04	0.16	0.10	0.11	0.11	0.09	0.14	0.03	0.13	1016
0.18	1.44	1.98	1.87	1.22	2.74	0.76	2.39	0.13	0.15	0.15	0.11	0.19	0.04	0.18	0.11	0.13	0.13	0.10	0.15	0.03	0.14	1082
0.32	1.97	2.81	2.60	1.60	4.02	1.21	3.43	0.14	0.17	0.17	0.13	0.21	0.04	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.16	1877


==> data/mlm_plots/tef/imdb/xlnet/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.48
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/xlnet/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.95	0.96	0.97	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.93	0.99	0.03	0.98	949
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.92	0.93	0.94	0.90	0.96	0.03	0.95	0.93	0.94	0.95	0.90	0.98	0.04	0.97	989
0.06	0.89	0.91	0.91	0.88	0.93	0.03	0.92	0.87	0.90	0.90	0.86	0.93	0.04	0.92	0.90	0.92	0.93	0.87	0.97	0.05	0.95	997
0.11	0.86	0.88	0.88	0.85	0.91	0.03	0.89	0.85	0.87	0.87	0.83	0.90	0.04	0.89	0.87	0.90	0.91	0.85	0.95	0.05	0.93	1003
0.15	0.81	0.84	0.84	0.81	0.87	0.03	0.85	0.80	0.83	0.83	0.79	0.87	0.04	0.85	0.84	0.87	0.87	0.81	0.92	0.06	0.91	1016
0.18	0.78	0.80	0.80	0.78	0.83	0.03	0.82	0.77	0.80	0.80	0.76	0.84	0.04	0.82	0.81	0.84	0.85	0.78	0.90	0.06	0.88	1082
0.32	0.75	0.77	0.77	0.74	0.81	0.03	0.79	0.75	0.77	0.77	0.74	0.81	0.04	0.80	0.78	0.81	0.82	0.75	0.87	0.06	0.85	1877


==> data/mlm_plots/tef/imdb/xlnet/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/imdb/xlnet/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	10.31	12.31	12.41	9.91	14.71	2.40	14.06	0.08	0.14	0.12	0.05	0.23	0.09	0.18	4.91	15.08	11.12	0.85	29.32	14.24	21.09	949
0.03	12.94	15.83	16.26	11.21	20.45	4.62	18.99	0.10	0.17	0.15	0.08	0.27	0.10	0.22	5.93	17.96	13.48	2.05	33.87	15.91	25.32	989
0.06	14.19	17.30	18.16	12.01	22.60	5.30	21.01	0.14	0.21	0.19	0.11	0.32	0.10	0.26	7.06	21.09	16.72	3.44	38.75	17.66	30.64	997
0.11	17.28	21.31	22.47	14.56	28.07	6.76	25.96	0.16	0.24	0.21	0.12	0.36	0.12	0.30	8.13	23.30	19.21	4.45	42.14	18.84	34.85	1003
0.15	25.01	30.98	32.71	21.28	40.68	9.70	37.72	0.18	0.28	0.24	0.14	0.41	0.13	0.34	8.48	25.83	21.13	5.34	46.31	20.48	38.41	1016
0.18	30.42	38.36	39.78	25.95	50.78	12.41	46.68	0.19	0.30	0.26	0.15	0.45	0.15	0.37	10.66	27.30	22.10	6.05	48.54	21.24	40.62	1082
0.32	38.39	50.93	50.40	31.35	70.50	19.58	61.87	0.20	0.32	0.27	0.15	0.48	0.16	0.39	11.28	29.67	25.41	7.29	52.04	22.38	43.84	1877


==> data/mlm_plots/tef/imdb/xlnet/a/time_misc_auc.tex <==
name	auc
attack_time	10.07
l2	0.08
lom	7.80


==> data/mlm_plots/tef/imdb/xlnet/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.50	0.64	0.67	0.44	0.84	0.20	0.79	0.74	0.80	0.83	0.67	0.93	0.13	0.89	0.84	0.87	0.90	0.78	0.97	0.09	0.94	949
0.03	0.40	0.54	0.57	0.33	0.75	0.21	0.69	0.68	0.75	0.78	0.61	0.89	0.14	0.84	0.81	0.84	0.87	0.74	0.94	0.10	0.91	989
0.06	0.31	0.46	0.46	0.24	0.68	0.22	0.62	0.62	0.69	0.72	0.55	0.84	0.15	0.80	0.77	0.81	0.84	0.71	0.91	0.10	0.88	997
0.11	0.23	0.40	0.40	0.18	0.62	0.22	0.56	0.57	0.65	0.68	0.50	0.81	0.15	0.76	0.74	0.79	0.81	0.68	0.89	0.11	0.86	1003
0.15	0.17	0.34	0.33	0.12	0.56	0.22	0.50	0.50	0.61	0.63	0.45	0.77	0.16	0.72	0.70	0.76	0.78	0.65	0.87	0.11	0.83	1016
0.18	0.12	0.31	0.28	0.09	0.53	0.22	0.46	0.47	0.57	0.60	0.41	0.74	0.16	0.69	0.68	0.74	0.75	0.62	0.85	0.11	0.81	1082
0.32	0.08	0.27	0.24	0.05	0.49	0.22	0.41	0.41	0.53	0.56	0.36	0.71	0.18	0.67	0.64	0.71	0.73	0.58	0.83	0.12	0.79	1877


==> data/mlm_plots/tef/imdb/xlnet/a/top_intersections_auc.tex <==
name	auc
top10	0.11
top30	0.19
top50	0.24


==> data/mlm_plots/tef/imdb/xlnet/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.32	58.90	54.18	34.96	82.84	23.94	71.27	15.00	18.80	18.00	13.25	24.36	5.55	22.00	47.71	65.46	60.71	39.99	90.93	25.47	78.73	15.00	19.12	19.00	13.56	24.67	5.56	23.00	980
0.03	42.32	59.37	53.95	34.47	84.28	24.91	72.08	14.00	17.70	18.00	11.76	23.63	5.93	22.00	53.59	73.70	67.81	44.75	102.65	28.95	88.10	14.00	18.33	18.00	12.28	24.38	6.05	22.00	1148
0.06	41.49	59.54	53.46	33.90	85.19	25.64	71.34	13.00	17.73	18.00	11.58	23.89	6.15	22.00	62.08	85.92	79.53	51.88	119.96	34.04	101.30	15.00	18.79	19.00	12.47	25.10	6.31	23.00	1304
0.11	41.92	60.88	54.29	34.01	87.74	26.87	75.10	13.00	17.37	17.00	10.98	23.76	6.39	21.00	75.83	103.61	96.76	63.73	143.49	39.88	121.59	14.00	18.79	18.00	12.15	25.42	6.64	23.00	1073
0.15	41.36	59.36	54.02	34.08	84.63	25.28	72.62	14.00	17.49	17.00	11.50	23.48	5.99	21.00	95.66	127.20	120.55	83.23	171.17	43.97	148.61	16.00	19.65	19.00	13.43	25.87	6.22	24.00	969
0.18	41.55	59.52	54.02	34.23	84.82	25.30	72.64	14.00	17.75	18.00	11.64	23.86	6.11	22.00	120.63	156.35	146.86	104.46	208.24	51.89	181.54	16.00	20.57	21.00	14.09	27.04	6.48	24.50	943
0.32	43.56	62.49	56.56	36.34	88.64	26.15	76.46	13.00	17.35	17.00	11.21	23.50	6.15	21.00	149.00	200.29	188.83	132.60	267.99	67.69	238.36	16.00	20.84	21.00	14.15	27.53	6.69	25.00	1410


==> data/mlm_plots/tef/imdb/xlnet/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	18.73
orig_ge	5.47
adv_pp	42.31
adv_ge	6.15


==> data/mlm_plots/tef/imdb/xlnet/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.04	0.25	0.29	-0.10	0.60	0.35	0.51	0.27	0.43	0.52	0.11	0.75	0.32	0.67	0.19	0.33	0.39	0.08	0.59	0.25	0.52	980
0.03	-0.18	0.01	0.02	-0.31	0.32	0.32	0.21	0.04	0.22	0.25	-0.09	0.53	0.31	0.45	0.03	0.17	0.19	-0.07	0.40	0.23	0.33	1148
0.06	-0.33	-0.17	-0.14	-0.45	0.11	0.28	0.01	-0.12	0.04	0.06	-0.24	0.32	0.28	0.25	-0.08	0.03	0.05	-0.17	0.24	0.21	0.18	1304
0.11	-0.41	-0.26	-0.25	-0.50	-0.02	0.24	-0.10	-0.20	-0.05	-0.02	-0.30	0.20	0.25	0.13	-0.14	-0.03	-0.01	-0.21	0.15	0.18	0.10	1073
0.15	-0.53	-0.39	-0.40	-0.59	-0.19	0.20	-0.25	-0.35	-0.20	-0.16	-0.43	0.03	0.23	-0.04	-0.24	-0.14	-0.11	-0.30	0.03	0.17	-0.02	969
0.18	-0.59	-0.46	-0.47	-0.64	-0.29	0.17	-0.35	-0.42	-0.29	-0.27	-0.48	-0.09	0.20	-0.15	-0.30	-0.20	-0.19	-0.35	-0.06	0.14	-0.10	943
0.32	-0.60	-0.49	-0.50	-0.64	-0.35	0.15	-0.40	-0.44	-0.33	-0.32	-0.49	-0.17	0.16	-0.21	-0.31	-0.23	-0.22	-0.35	-0.11	0.12	-0.15	1410


==> data/mlm_plots/tef/imdb/xlnet/ig/correlations_auc.tex <==
name	auc
pcc	-0.10
spearman	-0.05
kendall	-0.03


==> data/mlm_plots/tef/imdb/xlnet/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	6.86	12.62	10.23	3.93	21.30	8.69	16.02	5.84	11.98	9.31	2.66	21.30	9.32	14.92	5.98	13.35	10.06	2.77	23.93	10.58	17.78	980
0.03	6.11	9.64	8.26	3.81	15.47	5.83	11.74	5.36	9.65	7.79	2.42	16.89	7.24	11.57	5.94	13.80	10.33	2.13	25.47	11.67	16.20	1148
0.06	4.96	7.04	6.19	3.45	10.64	3.59	8.15	4.59	7.01	6.02	2.99	11.03	4.02	8.22	5.51	10.36	8.26	2.76	17.97	7.61	12.84	1304
0.11	4.11	5.31	4.97	3.47	7.15	1.84	6.09	3.83	5.18	4.76	3.10	7.26	2.08	6.02	4.74	7.69	6.58	2.98	12.40	4.71	9.16	1073
0.15	3.54	4.36	4.23	3.21	5.51	1.15	4.96	3.41	4.27	4.05	2.99	5.56	1.28	4.90	4.16	6.33	5.56	2.86	9.80	3.47	7.48	969
0.18	3.34	3.90	3.79	3.04	4.77	0.87	4.29	3.20	3.88	3.70	2.88	4.89	1.01	4.33	3.81	5.47	5.00	2.93	8.02	2.54	6.55	943
0.32	3.04	3.47	3.40	2.83	4.12	0.64	3.80	3.01	3.49	3.38	2.73	4.24	0.75	3.85	3.36	4.73	4.32	2.56	6.90	2.17	5.53	1410


==> data/mlm_plots/tef/imdb/xlnet/ig/ets_sts_auc.tex <==
name	auc
et_use	1.62
et_tse	1.60
et_ce	2.26


==> data/mlm_plots/tef/imdb/xlnet/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.79	6.03	2.97	-8.03	20.10	14.07	5.55	6.76	15.80	11.14	1.07	30.53	14.73	19.20	5.93	16.92	11.06	-1.44	35.29	18.37	20.90	980
0.03	1.32	2.66	1.95	-0.70	6.02	3.36	2.93	6.91	11.43	9.47	4.29	18.57	7.14	13.91	5.89	11.12	8.55	2.21	20.04	8.92	12.93	1148
0.06	0.95	1.53	1.27	-0.25	3.31	1.78	1.74	6.49	9.41	8.20	3.99	14.84	5.42	10.70	5.34	8.80	7.21	2.78	14.82	6.02	10.27	1304
0.11	0.65	0.99	0.84	0.33	1.65	0.66	1.15	5.93	8.14	7.36	3.94	12.33	4.20	9.15	4.91	7.44	6.28	2.42	12.46	5.02	8.27	1073
0.15	0.45	0.64	0.58	0.32	0.96	0.32	0.77	5.48	6.96	6.58	4.73	9.18	2.22	7.97	4.53	6.17	5.55	3.48	8.85	2.68	7.04	969
0.18	0.33	0.47	0.43	0.25	0.70	0.22	0.56	5.15	6.31	5.99	4.42	8.20	1.89	7.10	4.22	5.50	5.01	3.28	7.73	2.22	6.15	943
0.32	0.25	0.37	0.33	0.19	0.54	0.18	0.43	4.80	5.83	5.48	4.17	7.48	1.65	6.46	3.93	5.05	4.60	3.07	7.03	1.98	5.57	1410


==> data/mlm_plots/tef/imdb/xlnet/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.32
et_p_h	2.38
et_p_l2	2.17


==> data/mlm_plots/tef/imdb/xlnet/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.12	0.12	0.06	0.18	0.06	0.16	0.02	0.04	0.03	0.01	0.06	0.03	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.05	980
0.03	0.17	0.26	0.25	0.14	0.38	0.12	0.32	0.04	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.07	1148
0.06	0.34	0.47	0.46	0.29	0.66	0.19	0.58	0.06	0.08	0.08	0.05	0.12	0.03	0.10	0.06	0.07	0.07	0.05	0.09	0.02	0.08	1304
0.11	0.57	0.76	0.73	0.48	1.04	0.28	0.92	0.08	0.10	0.10	0.07	0.13	0.03	0.12	0.07	0.09	0.09	0.06	0.11	0.02	0.10	1073
0.15	0.94	1.25	1.20	0.81	1.68	0.44	1.48	0.10	0.13	0.13	0.09	0.16	0.04	0.15	0.09	0.11	0.11	0.08	0.13	0.02	0.12	969
0.18	1.33	1.78	1.69	1.14	2.43	0.64	2.16	0.12	0.15	0.15	0.11	0.18	0.04	0.17	0.11	0.12	0.12	0.10	0.15	0.03	0.14	943
0.32	1.75	2.41	2.28	1.46	3.36	0.95	2.95	0.14	0.16	0.16	0.12	0.20	0.04	0.18	0.12	0.13	0.14	0.11	0.16	0.03	0.15	1410


==> data/mlm_plots/tef/imdb/xlnet/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.42
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/xlnet/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.02	0.98	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.93	0.99	0.03	0.98	980
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.92	0.93	0.94	0.91	0.96	0.03	0.95	0.93	0.94	0.95	0.91	0.98	0.04	0.97	1148
0.06	0.89	0.91	0.91	0.88	0.93	0.03	0.93	0.88	0.90	0.91	0.87	0.94	0.03	0.93	0.90	0.92	0.93	0.88	0.97	0.04	0.95	1304
0.11	0.85	0.87	0.87	0.85	0.90	0.03	0.89	0.85	0.87	0.87	0.83	0.90	0.04	0.89	0.87	0.90	0.91	0.85	0.95	0.05	0.93	1073
0.15	0.81	0.83	0.83	0.81	0.86	0.03	0.85	0.80	0.83	0.83	0.79	0.86	0.04	0.85	0.84	0.87	0.88	0.81	0.92	0.06	0.91	969
0.18	0.79	0.81	0.81	0.78	0.84	0.03	0.82	0.78	0.80	0.80	0.77	0.84	0.04	0.83	0.81	0.84	0.85	0.78	0.90	0.06	0.89	943
0.32	0.76	0.78	0.78	0.75	0.81	0.03	0.80	0.76	0.78	0.78	0.74	0.81	0.03	0.80	0.78	0.82	0.83	0.75	0.88	0.06	0.86	1410


==> data/mlm_plots/tef/imdb/xlnet/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/imdb/xlnet/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	12.61	16.96	15.28	4.31	29.62	12.66	16.99	1.02	4.07	1.73	-5.71	13.85	9.78	3.48	2.14	6.74	4.88	0.27	13.21	6.47	9.12	980
0.03	26.91	41.25	33.68	14.44	68.06	26.81	40.98	1.40	9.26	2.60	-18.71	37.24	27.97	5.96	2.70	8.70	6.24	0.38	17.03	8.32	11.63	1148
0.06	36.46	54.09	46.06	24.33	83.86	29.77	59.63	1.78	11.02	3.54	-12.80	34.85	23.83	8.32	2.80	8.90	6.63	0.40	17.41	8.51	11.74	1304
0.11	41.47	53.63	52.23	30.67	76.59	22.96	61.31	1.75	6.25	2.94	-9.46	21.96	15.71	5.84	3.10	8.79	6.62	0.92	16.67	7.88	12.49	1073
0.15	55.37	68.83	71.00	46.29	91.36	22.53	82.28	1.62	4.14	2.63	-0.86	9.14	5.00	4.84	3.48	9.32	6.99	1.06	17.58	8.26	12.71	969
0.18	55.76	75.82	78.79	49.64	102.00	26.18	95.38	1.55	3.88	2.53	-0.54	8.30	4.42	4.70	3.90	9.30	7.29	1.14	17.46	8.16	12.38	943
0.32	47.30	63.25	60.03	35.52	90.97	27.72	72.69	1.69	4.09	2.84	0.50	7.69	3.60	5.22	3.20	9.06	6.81	0.91	17.21	8.15	12.40	1410


==> data/mlm_plots/tef/imdb/xlnet/ig/time_misc_auc.tex <==
name	auc
attack_time	19.12
l2	1.74
lom	2.79


==> data/mlm_plots/tef/imdb/xlnet/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.23	0.38	0.40	0.18	0.58	0.20	0.53	0.44	0.55	0.58	0.37	0.72	0.17	0.67	0.60	0.68	0.71	0.55	0.81	0.13	0.77	980
0.03	0.11	0.24	0.22	0.07	0.41	0.17	0.35	0.32	0.44	0.45	0.28	0.59	0.16	0.55	0.51	0.60	0.61	0.47	0.72	0.12	0.69	1148
0.06	0.06	0.15	0.12	0.02	0.28	0.13	0.23	0.25	0.35	0.35	0.21	0.49	0.14	0.45	0.47	0.53	0.54	0.42	0.64	0.11	0.62	1304
0.11	0.00	0.11	0.09	0.01	0.22	0.10	0.18	0.23	0.31	0.32	0.19	0.43	0.12	0.39	0.44	0.50	0.52	0.40	0.61	0.10	0.58	1073
0.15	0.00	0.07	0.06	-0.02	0.16	0.09	0.12	0.17	0.25	0.26	0.14	0.35	0.10	0.32	0.39	0.45	0.47	0.36	0.55	0.10	0.52	969
0.18	0.00	0.05	0.00	-0.02	0.12	0.07	0.07	0.15	0.21	0.22	0.12	0.31	0.09	0.27	0.37	0.42	0.43	0.34	0.50	0.08	0.48	943
0.32	0.00	0.04	0.00	-0.02	0.10	0.06	0.07	0.13	0.19	0.19	0.11	0.27	0.08	0.24	0.36	0.41	0.41	0.34	0.48	0.07	0.45	1410


==> data/mlm_plots/tef/imdb/xlnet/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.08
top50	0.15


==> data/mlm_plots/tef/imdb/xlnet/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.48	59.06	54.33	35.34	82.78	23.72	71.09	15.00	18.79	18.00	13.30	24.29	5.50	22.00	47.64	65.69	60.79	40.22	91.15	25.47	78.29	15.00	19.10	19.00	13.57	24.62	5.52	23.00	953
0.03	42.08	59.85	54.31	34.57	85.14	25.28	72.65	14.00	17.74	17.00	11.74	23.74	6.00	22.00	52.88	74.11	69.02	45.03	103.18	29.08	89.39	14.00	18.37	18.00	12.30	24.44	6.07	22.00	1035
0.06	42.78	60.20	53.27	34.30	86.09	25.89	72.67	13.00	17.74	17.00	11.58	23.90	6.16	22.00	63.45	86.88	79.29	53.60	120.16	33.28	102.57	14.00	18.70	19.00	12.41	24.98	6.29	23.00	1293
0.11	42.78	61.61	55.68	35.03	88.18	26.57	74.26	14.00	17.92	18.00	11.57	24.28	6.36	22.00	78.35	104.78	98.54	66.71	142.85	38.07	123.26	15.00	19.42	19.00	12.78	26.07	6.64	24.00	1169
0.15	40.80	59.24	53.64	33.85	84.64	25.39	72.75	13.00	17.30	17.00	11.42	23.17	5.87	21.00	98.79	128.92	120.88	85.29	172.54	43.62	150.50	15.00	19.53	20.00	13.23	25.83	6.30	24.00	1027
0.18	41.35	59.03	53.68	33.78	84.28	25.25	71.27	13.00	17.43	17.00	11.36	23.50	6.07	21.00	124.39	159.03	151.56	107.03	211.02	52.00	184.05	16.00	20.26	20.00	13.76	26.75	6.49	24.00	976
0.32	43.26	62.17	57.13	35.91	88.43	26.26	75.69	13.00	17.19	17.00	11.22	23.15	5.96	21.00	158.59	210.56	195.52	135.06	286.05	75.50	246.05	17.00	20.73	21.00	14.26	27.20	6.47	25.00	1472


==> data/mlm_plots/tef/imdb/xlnet/s/comparison_vals_auc.tex <==
name	auc
orig_pp	18.73
orig_ge	5.45
adv_pp	43.40
adv_ge	6.14


==> data/mlm_plots/tef/imdb/xlnet/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.52	0.63	0.66	0.43	0.83	0.20	0.78	0.83	0.85	0.89	0.70	1.00	0.15	0.94	0.65	0.70	0.74	0.55	0.85	0.15	0.80	953
0.03	0.34	0.48	0.50	0.27	0.68	0.20	0.63	0.72	0.76	0.82	0.55	0.96	0.21	0.88	0.54	0.60	0.65	0.42	0.78	0.18	0.72	1035
0.06	0.18	0.31	0.31	0.11	0.51	0.20	0.46	0.44	0.59	0.69	0.31	0.87	0.28	0.81	0.31	0.45	0.51	0.23	0.67	0.22	0.63	1293
0.11	0.16	0.28	0.27	0.11	0.45	0.17	0.40	0.47	0.58	0.64	0.35	0.81	0.23	0.76	0.33	0.43	0.47	0.25	0.62	0.18	0.58	1169
0.15	0.11	0.22	0.21	0.06	0.37	0.15	0.32	0.42	0.53	0.58	0.32	0.75	0.21	0.68	0.29	0.39	0.41	0.23	0.55	0.16	0.50	1027
0.18	0.09	0.18	0.17	0.05	0.32	0.13	0.26	0.40	0.50	0.52	0.31	0.68	0.18	0.63	0.28	0.36	0.37	0.22	0.50	0.14	0.46	976
0.32	0.04	0.14	0.12	0.01	0.27	0.13	0.21	0.29	0.42	0.44	0.22	0.61	0.19	0.56	0.20	0.30	0.30	0.15	0.44	0.14	0.40	1472


==> data/mlm_plots/tef/imdb/xlnet/s/correlations_auc.tex <==
name	auc
pcc	0.08
spearman	0.17
kendall	0.12


==> data/mlm_plots/tef/imdb/xlnet/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.10	6.04	5.14	1.82	10.26	4.22	7.65	2.69	5.75	4.67	1.16	10.35	4.60	7.19	2.77	6.77	5.02	0.78	12.76	5.99	8.77	953
0.03	2.92	4.79	4.08	1.64	7.93	3.14	5.77	2.62	4.52	3.77	1.47	7.56	3.05	5.35	3.05	6.54	5.00	1.30	11.77	5.24	8.07	1035
0.06	2.72	4.13	3.70	2.02	6.23	2.10	4.93	2.52	4.04	3.46	1.62	6.46	2.42	4.86	3.14	6.67	5.02	0.99	12.34	5.68	7.69	1293
0.11	2.34	3.05	2.88	2.00	4.11	1.06	3.59	2.18	2.94	2.77	1.80	4.09	1.15	3.47	2.60	4.48	3.74	1.71	7.25	2.77	5.46	1169
0.15	1.98	2.48	2.42	1.78	3.17	0.70	2.86	1.85	2.43	2.30	1.62	3.24	0.81	2.86	2.29	3.65	3.03	1.39	5.90	2.25	4.35	1027
0.18	1.81	2.17	2.12	1.64	2.71	0.53	2.47	1.76	2.16	2.07	1.55	2.77	0.61	2.47	2.04	3.03	2.67	1.48	4.59	1.55	3.68	976
0.32	1.73	2.00	1.97	1.57	2.43	0.43	2.23	1.71	2.02	1.95	1.53	2.51	0.49	2.27	1.93	2.72	2.48	1.51	3.93	1.21	3.22	1472


==> data/mlm_plots/tef/imdb/xlnet/s/ets_sts_auc.tex <==
name	auc
et_use	0.89
et_tse	0.87
et_ce	1.27


==> data/mlm_plots/tef/imdb/xlnet/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.88	2.91	1.52	-5.13	10.95	8.04	2.62	3.18	7.63	5.62	0.19	15.06	7.43	9.28	2.85	8.26	5.54	-0.75	17.28	9.02	10.36	953
0.03	0.69	1.69	1.02	-4.74	8.12	6.43	1.54	3.52	6.34	4.97	1.07	11.60	5.27	7.47	3.01	6.40	4.55	0.19	12.61	6.21	7.62	1035
0.06	0.52	0.88	0.72	0.11	1.65	0.77	1.08	3.66	5.47	4.80	2.72	8.22	2.75	6.65	3.02	5.16	4.16	1.82	8.49	3.33	6.25	1293
0.11	0.36	0.55	0.48	0.24	0.87	0.32	0.63	3.29	4.42	4.15	2.64	6.20	1.78	5.12	2.78	3.99	3.47	1.81	6.17	2.18	4.60	1169
0.15	0.24	0.35	0.31	0.19	0.51	0.16	0.41	3.02	3.77	3.61	2.56	4.98	1.21	4.30	2.47	3.31	3.02	1.86	4.76	1.45	3.75	1027
0.18	0.18	0.25	0.23	0.13	0.37	0.12	0.30	2.84	3.44	3.28	2.43	4.44	1.00	3.93	2.32	2.98	2.73	1.83	4.13	1.15	3.40	976
0.32	0.13	0.19	0.18	0.09	0.30	0.10	0.23	2.72	3.24	3.16	2.42	4.06	0.82	3.63	2.28	2.78	2.62	1.86	3.71	0.93	3.13	1472


==> data/mlm_plots/tef/imdb/xlnet/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.18
et_p_h	1.30
et_p_l2	1.19


==> data/mlm_plots/tef/imdb/xlnet/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.12	0.12	0.06	0.18	0.06	0.16	0.02	0.04	0.03	0.01	0.06	0.03	0.06	0.02	0.03	0.03	0.02	0.05	0.02	0.05	953
0.03	0.18	0.26	0.24	0.14	0.37	0.12	0.32	0.03	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.07	0.02	0.07	1035
0.06	0.35	0.48	0.45	0.29	0.67	0.19	0.58	0.06	0.08	0.08	0.05	0.12	0.03	0.11	0.06	0.07	0.07	0.05	0.09	0.02	0.09	1293
0.11	0.57	0.77	0.73	0.48	1.06	0.29	0.95	0.08	0.11	0.10	0.07	0.14	0.04	0.13	0.07	0.09	0.09	0.06	0.11	0.03	0.10	1169
0.15	0.96	1.30	1.23	0.80	1.79	0.49	1.57	0.11	0.13	0.13	0.09	0.17	0.04	0.15	0.09	0.11	0.11	0.08	0.13	0.03	0.12	1027
0.18	1.39	1.87	1.77	1.16	2.58	0.71	2.26	0.13	0.15	0.15	0.11	0.19	0.04	0.17	0.11	0.12	0.13	0.10	0.15	0.03	0.14	976
0.32	1.85	2.62	2.40	1.52	3.72	1.10	3.13	0.14	0.16	0.17	0.13	0.20	0.04	0.19	0.12	0.14	0.14	0.11	0.16	0.03	0.15	1472


==> data/mlm_plots/tef/imdb/xlnet/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.45
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/imdb/xlnet/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.93	0.99	0.03	0.98	953
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.92	0.93	0.93	0.90	0.96	0.03	0.95	0.92	0.94	0.95	0.90	0.98	0.04	0.97	1035
0.06	0.89	0.91	0.91	0.88	0.93	0.03	0.93	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.90	0.92	0.93	0.88	0.97	0.04	0.95	1293
0.11	0.86	0.88	0.88	0.85	0.90	0.03	0.89	0.85	0.87	0.87	0.83	0.90	0.04	0.89	0.87	0.90	0.90	0.85	0.95	0.05	0.93	1169
0.15	0.82	0.84	0.84	0.81	0.87	0.03	0.85	0.80	0.83	0.83	0.79	0.87	0.04	0.86	0.84	0.87	0.88	0.81	0.92	0.06	0.91	1027
0.18	0.79	0.81	0.81	0.78	0.84	0.03	0.82	0.78	0.80	0.80	0.76	0.84	0.04	0.83	0.81	0.84	0.85	0.78	0.90	0.06	0.89	976
0.32	0.76	0.78	0.78	0.75	0.81	0.03	0.80	0.75	0.78	0.78	0.74	0.82	0.04	0.81	0.78	0.82	0.83	0.75	0.88	0.07	0.87	1472


==> data/mlm_plots/tef/imdb/xlnet/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/imdb/xlnet/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	11.31	13.52	13.60	9.67	17.38	3.85	15.08	71.65	303.32	126.19	-367.24	973.88	670.56	274.74	2.06	6.73	4.67	0.06	13.41	6.67	9.25	953
0.03	12.66	17.01	15.89	7.24	26.78	9.77	18.20	109.54	729.63	205.01	-1187.64	2646.91	1917.27	453.36	2.91	8.90	6.35	0.83	16.96	8.07	12.59	1035
0.06	18.10	28.91	23.21	11.58	46.24	17.33	35.84	178.43	1695.80	406.17	-1928.20	5319.80	3624.00	1372.87	4.06	12.18	9.67	1.92	22.45	10.26	17.48	1293
0.11	21.93	31.80	27.73	15.00	48.60	16.80	34.64	209.41	1432.03	441.33	-1226.73	4090.80	2658.77	1336.57	3.75	12.05	10.04	2.12	21.98	9.93	17.08	1169
0.15	29.82	37.93	37.92	23.86	52.00	14.07	45.03	225.57	996.35	452.35	-953.36	2946.07	1949.72	949.11	4.31	12.29	10.62	2.64	21.95	9.66	17.72	1027
0.18	35.90	44.60	45.95	29.94	59.25	14.66	53.94	236.22	749.09	407.31	-265.22	1763.40	1014.31	794.07	4.39	12.26	10.07	2.35	22.18	9.92	18.30	976
0.32	40.71	51.85	52.57	33.91	69.79	17.94	63.39	260.75	760.37	470.05	-134.24	1654.98	894.61	909.18	4.75	12.64	10.53	2.86	22.42	9.78	18.20	1472


==> data/mlm_plots/tef/imdb/xlnet/s/time_misc_auc.tex <==
name	auc
attack_time	11.89
l2	304.42
lom	3.68


==> data/mlm_plots/tef/imdb/xlnet/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.53	0.61	0.64	0.43	0.80	0.19	0.73	0.74	0.78	0.81	0.66	0.90	0.12	0.86	0.83	0.86	0.88	0.78	0.94	0.08	0.91	953
0.03	0.38	0.48	0.50	0.28	0.67	0.20	0.62	0.65	0.70	0.74	0.56	0.85	0.14	0.80	0.77	0.81	0.83	0.71	0.90	0.10	0.87	1035
0.06	0.14	0.32	0.33	0.12	0.52	0.20	0.47	0.48	0.59	0.63	0.43	0.76	0.17	0.72	0.65	0.73	0.76	0.61	0.85	0.12	0.83	1293
0.11	0.15	0.28	0.27	0.12	0.45	0.17	0.40	0.49	0.58	0.60	0.44	0.72	0.14	0.69	0.67	0.73	0.74	0.63	0.83	0.10	0.80	1169
0.15	0.12	0.23	0.21	0.08	0.38	0.15	0.33	0.47	0.54	0.56	0.42	0.67	0.13	0.64	0.65	0.71	0.72	0.62	0.80	0.09	0.77	1027
0.18	0.09	0.20	0.20	0.06	0.34	0.14	0.29	0.45	0.52	0.53	0.41	0.63	0.11	0.60	0.65	0.69	0.70	0.61	0.77	0.08	0.74	976
0.32	0.07	0.17	0.14	0.03	0.30	0.13	0.25	0.40	0.47	0.47	0.36	0.58	0.11	0.54	0.61	0.66	0.67	0.58	0.74	0.08	0.71	1472


==> data/mlm_plots/tef/imdb/xlnet/s/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.17
top50	0.22


==> data/mlm_plots/tef/mr/bert/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	99.32	215.17	173.31	27.19	403.16	187.98	257.40	3.00	4.19	4.00	2.18	6.19	2.00	5.00	148.41	304.96	245.50	61.80	548.12	243.16	375.95	3.00	4.39	4.00	2.39	6.38	2.00	5.00	362
0.11	108.19	244.13	184.01	26.11	462.16	218.03	305.52	3.00	4.04	4.00	2.15	5.92	1.89	5.00	183.94	387.10	300.96	80.35	693.86	306.75	483.33	3.00	4.32	4.00	2.36	6.28	1.96	5.00	998
0.15	104.94	248.73	185.44	28.28	469.18	220.45	309.00	2.00	3.95	3.00	1.94	5.96	2.01	5.00	214.52	452.21	363.50	59.37	845.05	392.84	558.30	3.00	4.29	4.00	2.16	6.42	2.13	5.00	803
0.18	99.36	232.31	180.40	28.04	436.58	204.27	292.35	3.00	3.92	4.00	2.11	5.73	1.81	5.00	249.20	510.00	407.39	97.45	922.54	412.55	625.09	3.00	4.40	4.00	2.49	6.30	1.90	5.00	822
0.32	112.78	257.84	194.03	2.80	512.88	255.04	317.87	3.00	3.96	4.00	2.08	5.83	1.87	5.00	363.36	751.30	584.98	62.02	1440.58	689.28	917.75	3.00	4.57	4.00	2.55	6.60	2.03	6.00	2491


==> data/mlm_plots/tef/mr/bert/a/comparison_vals_auc.tex <==
name	auc
orig_pp	62.93
orig_ge	1.03
adv_pp	136.43
adv_ge	1.15


==> data/mlm_plots/tef/mr/bert/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.13	0.51	0.55	0.11	0.90	0.40	0.89	0.44	0.61	0.65	0.34	0.88	0.27	0.83	0.32	0.50	0.52	0.26	0.74	0.24	0.69	362
0.11	0.00	0.41	0.38	-0.01	0.83	0.42	0.81	0.34	0.53	0.59	0.22	0.84	0.31	0.77	0.24	0.43	0.44	0.16	0.69	0.26	0.64	998
0.15	-0.06	0.30	0.15	-0.12	0.72	0.42	0.72	0.18	0.42	0.47	0.09	0.75	0.33	0.68	0.12	0.34	0.36	0.07	0.61	0.27	0.54	803
0.18	-0.11	0.18	0.01	-0.21	0.57	0.39	0.43	0.15	0.37	0.38	0.06	0.68	0.31	0.60	0.11	0.29	0.28	0.04	0.53	0.25	0.47	822
0.32	-0.15	0.08	-0.05	-0.28	0.43	0.35	0.16	0.04	0.27	0.30	-0.06	0.60	0.33	0.52	0.04	0.21	0.21	-0.05	0.46	0.25	0.38	2491


==> data/mlm_plots/tef/mr/bert/a/correlations_auc.tex <==
name	auc
pcc	0.06
spearman	0.10
kendall	0.08


==> data/mlm_plots/tef/mr/bert/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	0.40	2.15	1.89	0.22	4.07	1.92	3.38	0.39	2.29	1.74	-0.07	4.65	2.36	3.46	0.62	8.91	3.40	-3.38	21.20	12.29	11.10	362
0.11	0.60	2.02	1.94	0.36	3.68	1.66	3.09	0.61	2.09	1.89	0.25	3.93	1.84	3.09	0.80	7.44	2.71	-3.51	18.39	10.95	8.39	998
0.15	0.74	1.99	2.12	0.59	3.39	1.40	2.85	0.85	2.06	2.00	0.50	3.62	1.56	2.92	1.21	6.53	2.78	-3.26	16.31	9.78	6.59	803
0.18	1.29	2.02	2.18	0.90	3.15	1.13	2.70	1.25	2.10	2.12	0.82	3.37	1.28	2.74	1.43	6.34	2.76	-3.01	15.69	9.35	7.01	822
0.32	1.51	1.87	1.94	1.01	2.73	0.86	2.32	1.43	1.93	1.94	0.95	2.90	0.97	2.43	1.38	4.19	2.35	-1.71	10.09	5.90	4.35	2491


==> data/mlm_plots/tef/mr/bert/a/ets_sts_auc.tex <==
name	auc
et_use	0.52
et_tse	0.54
et_ce	1.62


==> data/mlm_plots/tef/mr/bert/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.08	2.24	0.40	-11.42	15.90	13.66	1.07	0.94	8.94	4.73	-3.10	20.97	12.04	11.59	0.99	16.07	5.19	-17.54	49.68	33.61	15.22	362
0.11	0.10	1.39	0.40	-4.86	7.64	6.25	1.03	1.51	8.39	5.02	-2.66	19.45	11.05	11.14	1.72	14.14	5.21	-17.64	45.93	31.78	14.56	998
0.15	0.12	1.12	0.35	-3.82	6.05	4.94	0.92	2.31	8.20	4.78	-3.37	19.76	11.56	10.59	2.03	15.53	5.22	-22.02	53.09	37.56	12.78	803
0.18	0.14	1.05	0.30	-2.10	4.20	3.15	0.69	2.95	8.76	5.32	-3.72	21.24	12.48	9.94	2.42	14.79	5.25	-15.46	45.04	30.25	13.52	822
0.32	0.11	0.86	0.23	-4.30	6.01	5.16	0.49	3.10	7.39	4.70	-1.39	16.16	8.77	8.83	2.49	12.87	4.61	-19.93	45.68	32.81	11.05	2491


==> data/mlm_plots/tef/mr/bert/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.30
et_p_h	2.15
et_p_l2	3.75


==> data/mlm_plots/tef/mr/bert/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.21	0.61	0.45	0.03	1.19	0.58	0.80	0.01	0.05	0.03	-0.01	0.11	0.06	0.07	0.02	0.05	0.04	0.01	0.10	0.04	0.07	362
0.11	0.27	0.85	0.63	-0.05	1.76	0.90	1.13	0.02	0.06	0.04	-0.00	0.13	0.06	0.09	0.03	0.06	0.04	0.02	0.10	0.04	0.08	998
0.15	0.37	1.23	0.89	-0.08	2.55	1.31	1.64	0.02	0.08	0.05	0.00	0.16	0.08	0.12	0.03	0.07	0.06	0.02	0.12	0.05	0.10	803
0.18	0.56	1.65	1.32	0.14	3.16	1.51	2.31	0.03	0.09	0.07	0.02	0.17	0.08	0.14	0.04	0.08	0.07	0.03	0.14	0.05	0.13	822
0.32	0.90	2.80	1.88	-0.23	5.83	3.03	3.62	0.04	0.11	0.09	0.03	0.19	0.08	0.17	0.05	0.10	0.09	0.04	0.16	0.06	0.14	2491


==> data/mlm_plots/tef/mr/bert/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.43
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/tef/mr/bert/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.85	0.87	0.88	0.84	0.91	0.04	0.90	0.84	0.87	0.88	0.82	0.92	0.05	0.91	0.90	0.93	0.96	0.86	1.00	0.07	0.98	362
0.11	0.82	0.84	0.85	0.80	0.88	0.04	0.87	0.80	0.84	0.85	0.78	0.90	0.06	0.89	0.84	0.89	0.93	0.79	1.00	0.10	0.98	998
0.15	0.79	0.81	0.81	0.77	0.85	0.04	0.84	0.77	0.81	0.82	0.75	0.87	0.06	0.85	0.81	0.87	0.89	0.76	0.98	0.11	0.96	803
0.18	0.76	0.79	0.79	0.74	0.83	0.05	0.81	0.74	0.78	0.79	0.72	0.85	0.06	0.83	0.76	0.83	0.87	0.70	0.97	0.14	0.94	822
0.32	0.71	0.74	0.74	0.69	0.79	0.05	0.77	0.70	0.74	0.74	0.68	0.81	0.06	0.79	0.71	0.79	0.81	0.64	0.93	0.14	0.89	2491


==> data/mlm_plots/tef/mr/bert/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.22


==> data/mlm_plots/tef/mr/bert/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.19	0.22	0.21	0.16	0.28	0.06	0.22	0.17	0.30	0.32	0.12	0.49	0.19	0.44	0.44	2.97	2.17	-0.18	6.11	3.15	4.22	362
0.11	0.22	0.28	0.27	0.19	0.36	0.09	0.32	0.22	0.34	0.36	0.15	0.53	0.19	0.48	0.75	3.50	2.53	0.04	6.95	3.45	5.39	998
0.15	0.30	0.37	0.34	0.26	0.47	0.10	0.39	0.27	0.38	0.42	0.20	0.57	0.19	0.51	0.98	3.72	2.84	0.39	7.05	3.33	5.89	803
0.18	0.35	0.42	0.38	0.31	0.52	0.10	0.43	0.35	0.43	0.46	0.26	0.60	0.17	0.53	1.60	4.05	3.35	0.69	7.41	3.36	5.83	822
0.32	0.41	0.55	0.56	0.41	0.69	0.14	0.68	0.38	0.46	0.49	0.29	0.62	0.16	0.55	1.62	4.42	3.55	0.85	7.99	3.57	6.54	2491


==> data/mlm_plots/tef/mr/bert/a/time_misc_auc.tex <==
name	auc
attack_time	0.10
l2	0.10
lom	1.02


==> data/mlm_plots/tef/mr/bert/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.46	0.50	0.00	0.91	0.46	1.00	0.43	0.60	0.63	0.34	0.86	0.26	0.80	0.67	0.73	0.75	0.58	0.88	0.15	0.86	362
0.11	0.00	0.40	0.50	-0.02	0.83	0.42	1.00	0.43	0.57	0.57	0.33	0.82	0.24	0.71	0.60	0.70	0.73	0.53	0.87	0.17	0.82	998
0.15	0.00	0.32	0.00	-0.09	0.73	0.41	0.50	0.33	0.50	0.50	0.23	0.76	0.27	0.67	0.55	0.66	0.67	0.49	0.82	0.16	0.79	803
0.18	0.00	0.23	0.00	-0.14	0.59	0.37	0.50	0.29	0.45	0.43	0.21	0.69	0.24	0.67	0.50	0.63	0.62	0.47	0.79	0.16	0.75	822
0.32	0.00	0.16	0.00	-0.17	0.49	0.33	0.00	0.20	0.38	0.33	0.14	0.62	0.24	0.50	0.50	0.59	0.60	0.42	0.76	0.17	0.71	2491


==> data/mlm_plots/tef/mr/bert/a/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.12
top50	0.17


==> data/mlm_plots/tef/mr/bert/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	101.66	208.16	162.40	45.61	370.71	162.55	263.89	3.00	4.10	4.00	2.07	6.13	2.03	5.00	141.10	285.19	213.79	58.62	511.77	226.58	361.24	3.00	4.26	4.00	2.21	6.31	2.05	5.00	375
0.11	106.65	237.95	180.37	34.58	441.32	203.37	294.91	3.00	4.13	4.00	2.24	6.01	1.88	5.00	176.48	361.96	292.58	88.89	635.04	273.08	463.77	3.00	4.35	4.00	2.42	6.29	1.93	6.00	984
0.15	105.59	241.73	184.37	11.98	471.47	229.75	293.95	2.00	3.93	3.00	1.95	5.91	1.98	5.00	205.63	431.26	328.37	93.47	769.04	337.79	558.88	3.00	4.18	4.00	2.11	6.25	2.07	5.00	793
0.18	98.72	223.82	174.62	30.26	417.38	193.56	286.31	3.00	3.92	3.50	2.08	5.77	1.84	5.00	237.92	489.49	365.70	66.47	912.51	423.02	602.73	3.00	4.29	4.00	2.39	6.19	1.90	5.00	838
0.32	114.22	263.83	196.97	-3.46	531.11	267.29	325.20	3.00	3.94	4.00	2.08	5.81	1.86	5.00	334.31	729.76	572.93	132.93	1326.58	596.83	926.18	3.00	4.45	4.00	2.46	6.45	1.99	6.00	2467


==> data/mlm_plots/tef/mr/bert/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	61.89
orig_ge	1.03
adv_pp	130.82
adv_ge	1.12


==> data/mlm_plots/tef/mr/bert/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	-0.16	0.17	0.27	-0.31	0.64	0.47	0.53	0.01	0.25	0.37	-0.19	0.69	0.44	0.58	0.01	0.21	0.28	-0.14	0.55	0.34	0.46	375
0.11	-0.40	-0.03	-0.03	-0.50	0.43	0.47	0.34	-0.25	0.08	0.16	-0.35	0.52	0.44	0.42	-0.16	0.07	0.14	-0.27	0.41	0.34	0.33	984
0.15	-0.56	-0.18	-0.15	-0.62	0.27	0.45	0.15	-0.39	-0.04	0.05	-0.47	0.39	0.43	0.28	-0.27	-0.02	0.04	-0.37	0.32	0.34	0.22	793
0.18	-0.57	-0.28	-0.28	-0.67	0.12	0.39	0.01	-0.44	-0.13	-0.11	-0.52	0.26	0.39	0.19	-0.32	-0.09	-0.07	-0.40	0.21	0.31	0.15	838
0.32	-0.63	-0.37	-0.39	-0.72	-0.02	0.35	-0.13	-0.47	-0.22	-0.22	-0.57	0.12	0.34	0.03	-0.35	-0.16	-0.15	-0.43	0.11	0.27	0.03	2467


==> data/mlm_plots/tef/mr/bert/ig/correlations_auc.tex <==
name	auc
pcc	-0.05
spearman	-0.02
kendall	-0.01


==> data/mlm_plots/tef/mr/bert/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	1.82	3.65	3.25	1.30	6.00	2.35	4.98	1.72	3.81	3.11	1.10	6.52	2.71	4.99	2.91	14.68	7.68	-2.35	31.70	17.03	19.64	375
0.11	2.13	3.65	3.47	1.70	5.61	1.96	4.95	2.12	3.84	3.37	1.40	6.28	2.44	5.08	3.07	14.24	7.37	-2.49	30.96	16.72	18.45	984
0.15	2.18	3.34	3.18	1.76	4.92	1.58	4.37	2.23	3.61	3.22	1.54	5.67	2.07	4.57	2.95	12.94	6.41	-2.79	28.68	15.74	17.04	793
0.18	2.25	3.21	3.06	1.87	4.54	1.34	3.96	2.31	3.41	3.03	1.41	5.42	2.00	4.09	2.93	10.78	4.99	-3.69	25.25	14.47	11.20	838
0.32	2.09	2.76	2.62	1.74	3.79	1.03	3.29	2.04	2.88	2.65	1.66	4.11	1.22	3.43	2.24	6.51	3.44	-2.40	15.42	8.91	6.60	2467


==> data/mlm_plots/tef/mr/bert/ig/ets_sts_auc.tex <==
name	auc
et_use	0.84
et_tse	0.89
et_ce	2.84


==> data/mlm_plots/tef/mr/bert/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.49	4.56	1.14	-15.73	24.86	20.30	2.51	5.41	19.19	11.01	-4.39	42.78	23.59	24.07	5.45	31.94	13.65	-22.74	86.61	54.67	34.14	375
0.11	0.44	4.12	0.89	-21.05	29.29	25.17	2.02	5.36	16.89	9.94	-2.00	35.77	18.89	21.13	5.00	29.57	11.51	-31.59	90.72	61.15	28.48	984
0.15	0.36	2.40	0.71	-7.04	11.85	9.44	1.70	5.61	14.08	9.25	-0.30	28.46	14.38	17.56	4.96	23.71	11.01	-23.54	70.97	47.25	23.13	793
0.18	0.27	1.38	0.52	-3.92	6.69	5.31	1.03	5.07	12.97	8.95	1.07	24.86	11.89	15.87	4.32	25.98	9.10	-33.17	85.13	59.15	22.59	838
0.32	0.19	1.18	0.39	-2.58	4.95	3.76	0.82	4.87	11.53	7.64	-0.90	23.97	12.43	13.52	4.08	20.38	7.77	-25.66	66.42	46.04	18.10	2467


==> data/mlm_plots/tef/mr/bert/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.58
et_p_h	3.64
et_p_l2	6.58


==> data/mlm_plots/tef/mr/bert/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.15	0.49	0.36	0.01	0.97	0.48	0.68	0.01	0.05	0.03	-0.01	0.10	0.05	0.06	0.02	0.04	0.03	0.01	0.08	0.04	0.06	375
0.11	0.27	0.76	0.58	0.04	1.47	0.72	1.05	0.02	0.06	0.04	-0.00	0.13	0.06	0.09	0.02	0.06	0.04	0.01	0.10	0.04	0.08	984
0.15	0.37	1.10	0.79	0.03	2.18	1.07	1.47	0.02	0.08	0.05	0.01	0.15	0.07	0.12	0.03	0.07	0.06	0.02	0.12	0.05	0.10	793
0.18	0.64	1.66	1.27	0.15	3.16	1.50	2.26	0.03	0.09	0.07	0.02	0.16	0.07	0.14	0.04	0.08	0.07	0.03	0.13	0.05	0.12	838
0.32	0.85	2.66	1.77	-0.26	5.58	2.92	3.44	0.04	0.11	0.09	0.02	0.19	0.08	0.17	0.05	0.10	0.09	0.04	0.15	0.06	0.14	2467


==> data/mlm_plots/tef/mr/bert/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/tef/mr/bert/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.85	0.88	0.88	0.84	0.91	0.04	0.90	0.83	0.87	0.88	0.81	0.93	0.06	0.91	0.90	0.93	0.95	0.85	1.00	0.08	0.98	375
0.11	0.82	0.85	0.85	0.81	0.89	0.04	0.87	0.80	0.84	0.85	0.78	0.90	0.06	0.89	0.86	0.90	0.93	0.80	1.00	0.10	0.97	984
0.15	0.78	0.81	0.82	0.77	0.86	0.04	0.84	0.78	0.82	0.82	0.76	0.88	0.06	0.86	0.84	0.88	0.91	0.78	0.99	0.10	0.96	793
0.18	0.76	0.79	0.79	0.74	0.84	0.05	0.82	0.75	0.79	0.79	0.73	0.85	0.06	0.84	0.80	0.86	0.88	0.74	0.97	0.11	0.95	838
0.32	0.71	0.74	0.74	0.69	0.79	0.05	0.77	0.70	0.74	0.74	0.68	0.81	0.06	0.79	0.71	0.79	0.81	0.65	0.93	0.14	0.89	2467


==> data/mlm_plots/tef/mr/bert/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.22


==> data/mlm_plots/tef/mr/bert/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.39	0.43	0.41	0.34	0.53	0.10	0.45	0.47	6.75	5.05	-0.77	14.26	7.51	10.83	1.46	3.92	2.80	0.47	7.36	3.44	5.65	375
0.11	0.42	0.53	0.52	0.38	0.68	0.15	0.58	0.65	7.39	5.51	-0.48	15.26	7.87	11.60	1.59	4.64	3.47	0.63	8.64	4.01	6.69	984
0.15	0.56	0.72	0.68	0.52	0.91	0.20	0.83	0.81	8.01	5.95	-0.41	16.42	8.42	12.30	1.81	4.82	3.82	0.88	8.76	3.94	6.93	793
0.18	0.74	0.86	0.84	0.70	1.03	0.17	0.94	1.14	8.75	6.62	-0.23	17.74	8.99	13.31	2.10	5.14	4.10	1.07	9.21	4.07	7.40	838
0.32	0.61	0.94	0.99	0.65	1.23	0.29	1.18	1.71	10.37	8.70	0.28	20.47	10.09	15.48	1.67	4.97	3.74	0.69	9.25	4.28	7.07	2467


==> data/mlm_plots/tef/mr/bert/ig/time_misc_auc.tex <==
name	auc
attack_time	0.20
l2	2.25
lom	1.26


==> data/mlm_plots/tef/mr/bert/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.20	0.00	-0.16	0.56	0.36	0.50	0.27	0.44	0.43	0.19	0.69	0.25	0.60	0.50	0.60	0.67	0.41	0.79	0.19	0.75	375
0.11	0.00	0.14	0.00	-0.13	0.42	0.27	0.00	0.17	0.36	0.33	0.12	0.61	0.25	0.57	0.42	0.55	0.58	0.36	0.74	0.19	0.67	984
0.15	0.00	0.10	0.00	-0.15	0.34	0.25	0.00	0.14	0.31	0.33	0.08	0.54	0.23	0.50	0.33	0.50	0.50	0.30	0.70	0.20	0.67	793
0.18	0.00	0.05	0.00	-0.12	0.23	0.18	0.00	0.00	0.27	0.29	0.06	0.48	0.21	0.43	0.36	0.47	0.50	0.29	0.64	0.18	0.60	838
0.32	0.00	0.05	0.00	-0.13	0.22	0.17	0.00	0.00	0.23	0.20	0.03	0.42	0.19	0.33	0.33	0.43	0.45	0.27	0.60	0.17	0.55	2467


==> data/mlm_plots/tef/mr/bert/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.08
top50	0.13


==> data/mlm_plots/tef/mr/bert/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	96.27	215.62	163.97	32.20	399.03	183.42	279.87	3.00	4.12	4.00	2.16	6.08	1.96	5.00	137.79	303.40	224.98	10.38	596.43	293.02	361.48	3.00	4.33	4.00	2.37	6.30	1.96	5.00	372
0.11	109.31	251.17	190.58	26.84	475.50	224.33	311.75	3.00	4.15	4.00	2.25	6.05	1.90	5.00	187.86	384.99	281.36	74.23	695.76	310.76	482.32	3.00	4.38	4.00	2.42	6.34	1.96	5.25	1004
0.15	111.39	254.48	192.28	12.61	496.35	241.87	329.89	3.00	4.02	4.00	2.04	6.00	1.98	5.00	222.72	469.38	363.54	27.92	910.83	441.45	580.09	3.00	4.33	4.00	2.29	6.38	2.05	5.00	780
0.18	99.71	234.99	178.07	9.74	460.25	225.26	299.93	2.00	3.90	4.00	2.04	5.76	1.86	5.00	239.06	487.51	377.23	84.84	890.18	402.67	593.70	3.00	4.31	4.00	2.32	6.29	1.99	5.00	826
0.32	112.03	266.51	192.34	-27.62	560.64	294.13	314.15	2.00	3.89	4.00	2.05	5.73	1.84	5.00	335.86	712.81	538.89	104.04	1321.59	608.77	872.42	3.00	4.48	4.00	2.47	6.49	2.01	6.00	2483


==> data/mlm_plots/tef/mr/bert/s/comparison_vals_auc.tex <==
name	auc
orig_pp	64.30
orig_ge	1.03
adv_pp	132.48
adv_ge	1.14


==> data/mlm_plots/tef/mr/bert/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.27	0.46	0.51	0.18	0.74	0.28	0.67	0.51	0.60	0.66	0.34	0.85	0.25	0.78	0.36	0.46	0.50	0.25	0.67	0.21	0.61	372
0.11	0.19	0.36	0.38	0.08	0.64	0.28	0.57	0.37	0.51	0.56	0.25	0.77	0.26	0.71	0.26	0.39	0.42	0.18	0.60	0.21	0.53	1004
0.15	0.07	0.26	0.24	-0.01	0.52	0.26	0.43	0.26	0.42	0.46	0.16	0.69	0.27	0.62	0.19	0.32	0.33	0.11	0.53	0.21	0.46	780
0.18	0.01	0.20	0.18	-0.06	0.46	0.26	0.38	0.16	0.36	0.38	0.06	0.65	0.30	0.58	0.12	0.27	0.28	0.04	0.49	0.22	0.42	826
0.32	-0.08	0.09	0.07	-0.15	0.34	0.24	0.25	0.06	0.26	0.28	-0.03	0.55	0.29	0.47	0.04	0.19	0.19	-0.03	0.40	0.21	0.33	2483


==> data/mlm_plots/tef/mr/bert/s/correlations_auc.tex <==
name	auc
pcc	0.06
spearman	0.10
kendall	0.08


==> data/mlm_plots/tef/mr/bert/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	1.25	2.34	1.98	0.91	3.77	1.43	3.18	1.20	2.51	1.89	0.56	4.46	1.95	3.11	2.24	9.32	5.95	0.07	18.57	9.25	12.40	372
0.11	1.35	2.25	2.01	0.90	3.60	1.35	2.83	1.30	2.44	2.00	0.66	4.21	1.78	2.99	2.21	9.17	4.93	-1.20	19.54	10.37	12.47	1004
0.15	1.43	2.08	1.93	1.08	3.07	1.00	2.58	1.41	2.21	1.90	0.75	3.68	1.46	2.64	1.81	7.69	3.66	-1.61	16.98	9.30	9.98	780
0.18	1.41	2.01	1.88	1.08	2.93	0.92	2.45	1.40	2.08	1.88	0.89	3.26	1.18	2.51	1.76	6.66	3.36	-2.11	15.44	8.77	7.73	826
0.32	1.36	1.83	1.79	1.16	2.50	0.67	2.21	1.38	1.88	1.79	1.11	2.64	0.76	2.27	1.52	4.51	2.38	-2.16	11.18	6.67	4.36	2483


==> data/mlm_plots/tef/mr/bert/s/ets_sts_auc.tex <==
name	auc
et_use	0.53
et_tse	0.56
et_ce	1.80


==> data/mlm_plots/tef/mr/bert/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.29	2.36	0.62	-4.38	9.09	6.74	1.30	3.45	10.70	7.49	-0.64	22.04	11.34	14.30	3.36	18.21	8.79	-9.92	46.34	28.13	20.16	372
0.11	0.26	3.04	0.51	-13.82	19.91	16.86	1.37	3.03	10.30	6.17	-4.38	24.98	14.68	12.52	2.92	17.52	7.14	-15.13	50.17	32.65	16.57	1004
0.15	0.21	1.38	0.40	-2.24	5.01	3.62	0.96	3.52	8.80	6.20	-1.21	18.81	10.01	10.15	3.16	16.61	6.77	-23.05	56.27	39.66	14.77	780
0.18	0.17	1.05	0.32	-3.19	5.30	4.24	0.72	3.28	7.85	5.26	-0.31	16.02	8.17	9.36	2.67	14.88	5.78	-16.78	46.54	31.66	13.20	826
0.32	0.12	1.11	0.23	-7.92	10.14	9.03	0.56	3.08	7.30	4.86	-0.73	15.32	8.03	8.69	2.54	14.55	4.77	-24.23	53.33	38.78	12.25	2483


==> data/mlm_plots/tef/mr/bert/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.41
et_p_h	2.22
et_p_l2	4.11


==> data/mlm_plots/tef/mr/bert/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.17	0.57	0.40	0.01	1.14	0.57	0.78	0.01	0.05	0.03	-0.01	0.11	0.06	0.07	0.02	0.05	0.03	0.01	0.09	0.04	0.07	372
0.11	0.23	0.81	0.54	-0.15	1.78	0.96	1.09	0.02	0.07	0.04	-0.00	0.14	0.07	0.10	0.03	0.06	0.05	0.01	0.11	0.05	0.09	1004
0.15	0.41	1.20	0.86	0.04	2.36	1.16	1.66	0.02	0.08	0.05	0.01	0.15	0.07	0.11	0.03	0.07	0.06	0.02	0.12	0.05	0.10	780
0.18	0.57	1.57	1.18	0.12	3.02	1.45	2.10	0.03	0.09	0.07	0.02	0.17	0.07	0.14	0.04	0.08	0.07	0.03	0.13	0.05	0.12	826
0.32	0.82	2.64	1.86	-0.11	5.39	2.75	3.42	0.04	0.11	0.09	0.03	0.20	0.09	0.18	0.05	0.10	0.09	0.04	0.16	0.06	0.14	2483


==> data/mlm_plots/tef/mr/bert/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/tef/mr/bert/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.85	0.88	0.88	0.84	0.91	0.04	0.90	0.84	0.87	0.87	0.81	0.92	0.05	0.91	0.89	0.93	0.96	0.85	1.01	0.08	0.98	372
0.11	0.82	0.84	0.85	0.80	0.89	0.04	0.87	0.80	0.84	0.85	0.78	0.90	0.06	0.89	0.87	0.91	0.94	0.82	1.00	0.09	0.98	1004
0.15	0.78	0.81	0.81	0.77	0.85	0.04	0.84	0.76	0.81	0.81	0.75	0.87	0.06	0.85	0.82	0.88	0.90	0.77	0.98	0.10	0.96	780
0.18	0.76	0.79	0.79	0.74	0.83	0.05	0.82	0.75	0.79	0.79	0.73	0.85	0.06	0.83	0.79	0.85	0.88	0.73	0.97	0.12	0.94	826
0.32	0.71	0.74	0.74	0.69	0.79	0.05	0.77	0.70	0.74	0.74	0.68	0.80	0.06	0.79	0.72	0.79	0.81	0.65	0.93	0.14	0.90	2483


==> data/mlm_plots/tef/mr/bert/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.22


==> data/mlm_plots/tef/mr/bert/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.21	0.25	0.23	0.16	0.33	0.08	0.25	1.28	59.46	18.70	-22.84	141.75	82.29	93.66	0.45	1.37	1.01	0.12	2.61	1.24	1.70	372
0.11	0.24	0.30	0.30	0.21	0.40	0.09	0.34	1.44	62.88	20.23	-32.36	158.11	95.24	96.80	0.52	1.45	1.10	0.16	2.74	1.29	2.03	1004
0.15	0.32	0.38	0.35	0.27	0.49	0.11	0.38	2.18	79.26	37.44	-28.40	186.92	107.66	121.98	0.60	1.56	1.26	0.32	2.79	1.23	2.29	780
0.18	0.34	0.42	0.36	0.28	0.55	0.13	0.47	2.26	88.48	34.14	-38.23	215.20	126.72	136.69	0.72	1.68	1.34	0.36	2.99	1.31	2.45	826
0.32	0.51	0.63	0.56	0.47	0.78	0.15	0.75	4.12	108.33	72.07	-23.68	240.35	132.01	167.92	0.70	1.83	1.51	0.44	3.22	1.39	2.72	2483


==> data/mlm_plots/tef/mr/bert/s/time_misc_auc.tex <==
name	auc
attack_time	0.11
l2	22.17
lom	0.42


==> data/mlm_plots/tef/mr/bert/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.18	0.00	-0.15	0.51	0.33	0.50	0.43	0.56	0.57	0.35	0.76	0.21	0.71	0.67	0.73	0.75	0.60	0.87	0.14	0.83	372
0.11	0.00	0.18	0.00	-0.11	0.47	0.29	0.50	0.40	0.52	0.50	0.31	0.72	0.20	0.67	0.62	0.70	0.73	0.56	0.83	0.13	0.80	1004
0.15	0.00	0.11	0.00	-0.14	0.36	0.25	0.00	0.33	0.43	0.50	0.23	0.63	0.20	0.57	0.57	0.67	0.67	0.52	0.81	0.14	0.78	780
0.18	0.00	0.08	0.00	-0.14	0.30	0.22	0.00	0.29	0.40	0.40	0.18	0.61	0.21	0.50	0.55	0.64	0.64	0.49	0.78	0.14	0.73	826
0.32	0.00	0.05	0.00	-0.12	0.21	0.16	0.00	0.17	0.32	0.33	0.11	0.52	0.20	0.50	0.50	0.59	0.60	0.45	0.74	0.14	0.69	2483


==> data/mlm_plots/tef/mr/bert/s/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.11
top50	0.17


==> data/mlm_plots/tef/mr/cnn/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	102.34	182.94	150.87	83.34	282.54	99.60	225.43	4.00	4.83	5.00	3.04	6.61	1.78	6.00	104.90	207.16	195.41	104.64	309.68	102.52	296.52	4.00	5.03	5.00	3.18	6.88	1.85	6.00	210
0.06	103.98	202.01	165.72	51.94	352.07	150.07	242.66	3.00	4.52	4.00	2.18	6.86	2.34	6.00	126.97	255.55	198.82	59.68	451.42	195.87	310.46	3.00	4.65	4.00	2.27	7.02	2.38	6.00	762
0.11	96.41	222.88	172.48	18.27	427.50	204.62	271.81	3.00	4.16	4.00	2.09	6.23	2.07	5.00	151.76	333.34	246.93	38.90	627.77	294.43	401.76	3.00	4.43	4.00	2.24	6.62	2.19	6.00	873
0.15	98.16	266.17	169.00	-78.13	610.48	344.31	294.27	2.00	3.95	3.00	1.48	6.43	2.48	5.00	185.48	434.77	288.82	-16.90	886.44	451.67	513.02	3.00	4.23	4.00	1.65	6.81	2.58	5.00	439
0.18	95.61	216.76	165.08	29.51	404.00	187.25	272.17	3.00	4.18	4.00	2.06	6.31	2.13	5.00	224.42	450.09	360.88	67.15	833.03	382.94	565.73	3.00	4.70	4.00	2.31	7.08	2.38	6.00	700
0.32	100.21	234.22	172.71	4.93	463.51	229.29	283.19	3.00	4.06	4.00	2.14	5.98	1.92	5.00	313.61	674.18	512.27	31.53	1316.82	642.64	831.46	3.00	4.71	4.00	2.55	6.88	2.16	6.00	2195


==> data/mlm_plots/tef/mr/cnn/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	65.23
orig_ge	1.22
adv_pp	128.85
adv_ge	1.34


==> data/mlm_plots/tef/mr/cnn/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.00	0.00	0.00	0.00	0.00	0.00	-0.12	0.03	0.03	-0.22	0.28	0.25	0.19	0.00	0.00	0.00	0.00	0.00	0.00	0.00	210
0.06	0.00	0.31	0.25	-0.04	0.65	0.35	0.61	0.03	0.35	0.40	-0.03	0.73	0.38	0.68	0.00	0.31	0.28	0.01	0.61	0.30	0.59	762
0.11	0.00	0.29	0.29	-0.07	0.65	0.36	0.58	0.20	0.39	0.40	0.07	0.71	0.32	0.60	0.12	0.32	0.34	0.05	0.59	0.27	0.51	873
0.15	0.00	0.21	0.20	-0.14	0.55	0.35	0.48	0.11	0.29	0.30	-0.03	0.60	0.32	0.50	0.04	0.24	0.23	0.01	0.48	0.24	0.42	439
0.18	-0.11	0.08	0.04	-0.25	0.41	0.33	0.34	-0.03	0.17	0.17	-0.12	0.47	0.29	0.38	0.00	0.15	0.13	-0.07	0.37	0.22	0.30	700
0.32	-0.33	-0.09	-0.09	-0.43	0.26	0.34	0.14	-0.20	0.00	0.00	-0.30	0.31	0.30	0.21	-0.13	0.01	0.00	-0.21	0.24	0.23	0.16	2195


==> data/mlm_plots/tef/mr/cnn/ig/correlations_auc.tex <==
name	auc
pcc	0.03
spearman	0.06
kendall	0.05


==> data/mlm_plots/tef/mr/cnn/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	5.23	7.45	6.43	3.85	11.05	3.60	8.77	5.07	8.83	7.60	2.87	14.79	5.96	10.72	6.69	22.51	23.85	6.30	38.72	16.21	37.49	210
0.06	1.54	3.34	2.94	0.80	5.87	2.53	4.53	1.39	3.77	2.84	0.25	7.29	3.52	5.05	2.29	11.29	6.52	-0.83	23.41	12.12	15.80	762
0.11	1.30	2.35	2.20	1.00	3.70	1.35	3.31	1.21	2.38	2.09	0.78	3.99	1.60	3.13	1.67	7.91	3.83	-1.99	17.80	9.90	9.65	873
0.15	1.33	2.16	2.09	1.00	3.32	1.16	2.86	1.29	2.27	2.00	0.75	3.79	1.52	2.88	1.73	7.43	3.13	-2.28	17.14	9.71	8.58	439
0.18	1.54	2.19	2.13	1.26	3.12	0.93	2.67	1.41	2.17	2.02	1.05	3.29	1.12	2.72	1.72	5.42	3.07	-1.46	12.31	6.89	6.12	700
0.32	1.58	2.06	2.02	1.30	2.82	0.76	2.50	1.48	2.06	1.94	1.22	2.89	0.84	2.55	1.52	4.07	2.45	-1.18	9.32	5.25	4.37	2195


==> data/mlm_plots/tef/mr/cnn/ig/ets_sts_auc.tex <==
name	auc
et_use	0.75
et_tse	0.80
et_ce	2.15


==> data/mlm_plots/tef/mr/cnn/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.56	6.94	3.82	-0.97	14.86	7.91	7.12	13.29	36.81	25.71	7.15	66.47	29.66	66.18	9.91	55.58	39.74	1.08	110.08	54.50	84.85	210
0.06	0.45	6.18	1.16	-31.38	43.75	37.57	3.07	4.41	18.34	11.50	-3.62	40.30	21.96	24.03	4.52	30.56	13.70	-21.52	82.65	52.09	32.81	762
0.11	0.29	2.47	0.66	-4.19	9.14	6.66	1.68	3.50	11.76	7.13	-1.30	24.82	13.06	15.24	3.47	21.24	8.02	-20.98	63.46	42.22	19.84	873
0.15	0.24	2.42	0.50	-12.03	16.88	14.45	1.09	3.61	11.78	8.45	0.18	23.38	11.60	14.17	3.92	22.49	10.31	-13.97	58.94	36.46	22.63	439
0.18	0.20	1.09	0.38	-1.71	3.90	2.80	0.84	3.35	9.66	6.17	-1.31	20.63	10.97	11.15	2.87	18.07	6.42	-24.57	60.71	42.64	13.47	700
0.32	0.14	1.04	0.27	-5.94	8.01	6.98	0.58	3.57	8.26	5.43	-0.41	16.92	8.67	9.29	2.99	15.58	5.62	-23.74	54.90	39.32	13.13	2195


==> data/mlm_plots/tef/mr/cnn/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.71
et_p_h	3.62
et_p_l2	6.42


==> data/mlm_plots/tef/mr/cnn/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.07	0.21	0.13	-0.01	0.43	0.22	0.32	0.01	0.03	0.01	-0.01	0.08	0.04	0.05	0.01	0.03	0.02	-0.00	0.07	0.04	0.04	210
0.06	0.12	0.38	0.28	0.00	0.76	0.38	0.53	0.01	0.04	0.02	-0.01	0.09	0.05	0.05	0.01	0.04	0.03	0.01	0.07	0.03	0.05	762
0.11	0.20	0.70	0.48	-0.07	1.48	0.77	0.98	0.02	0.06	0.04	-0.00	0.12	0.06	0.08	0.02	0.06	0.04	0.01	0.10	0.04	0.08	873
0.15	0.37	1.02	0.75	0.08	1.95	0.93	1.36	0.02	0.06	0.04	-0.00	0.13	0.07	0.09	0.03	0.06	0.05	0.01	0.11	0.05	0.09	439
0.18	0.52	1.51	1.27	0.12	2.91	1.40	1.98	0.03	0.09	0.07	0.02	0.17	0.08	0.15	0.04	0.08	0.07	0.03	0.14	0.05	0.12	700
0.32	0.89	2.80	1.94	-0.20	5.80	3.00	3.57	0.04	0.11	0.10	0.03	0.20	0.09	0.18	0.06	0.10	0.10	0.05	0.16	0.06	0.15	2195


==> data/mlm_plots/tef/mr/cnn/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/tef/mr/cnn/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.90	0.92	0.92	0.89	0.95	0.03	0.94	0.90	0.92	0.93	0.86	0.97	0.05	0.95	0.93	0.94	0.98	0.87	1.01	0.07	0.99	210
0.06	0.86	0.88	0.88	0.84	0.92	0.04	0.90	0.84	0.88	0.89	0.81	0.94	0.06	0.92	0.90	0.92	0.95	0.84	1.00	0.08	0.98	762
0.11	0.82	0.84	0.84	0.80	0.88	0.04	0.87	0.79	0.83	0.84	0.77	0.89	0.06	0.88	0.84	0.88	0.92	0.77	0.99	0.11	0.97	873
0.15	0.78	0.81	0.81	0.76	0.85	0.04	0.84	0.76	0.80	0.80	0.74	0.87	0.06	0.85	0.79	0.86	0.89	0.73	0.98	0.13	0.96	439
0.18	0.76	0.78	0.78	0.74	0.82	0.04	0.81	0.72	0.77	0.77	0.70	0.84	0.07	0.81	0.75	0.82	0.86	0.69	0.96	0.14	0.92	700
0.32	0.69	0.73	0.73	0.68	0.78	0.05	0.76	0.67	0.72	0.72	0.65	0.79	0.07	0.77	0.67	0.75	0.78	0.59	0.92	0.16	0.88	2195


==> data/mlm_plots/tef/mr/cnn/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.23
sts_tse	0.23
sts_ce	0.24


==> data/mlm_plots/tef/mr/cnn/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.47	0.59	0.59	0.43	0.75	0.16	0.72	0.03	0.06	0.05	0.03	0.08	0.03	0.08	1.94	3.91	3.61	1.56	6.26	2.35	5.63	210
0.06	0.26	0.40	0.34	0.21	0.58	0.18	0.50	0.07	0.86	0.58	-0.13	1.84	0.99	1.32	0.73	2.27	1.75	0.30	4.24	1.97	3.32	762
0.11	0.29	0.40	0.40	0.26	0.54	0.14	0.48	0.37	1.29	1.07	0.17	2.41	1.12	1.75	0.69	2.12	1.66	0.13	4.11	1.99	2.74	873
0.15	0.36	0.45	0.43	0.32	0.58	0.13	0.53	0.54	1.55	1.28	0.29	2.82	1.27	2.15	0.60	1.89	1.38	0.12	3.66	1.77	2.64	439
0.18	0.39	0.51	0.51	0.39	0.63	0.12	0.59	0.72	1.59	1.38	0.36	2.83	1.23	2.18	0.81	2.44	1.82	0.28	4.59	2.16	3.38	700
0.32	0.60	0.66	0.66	0.54	0.78	0.12	0.75	0.52	1.83	1.46	0.25	3.41	1.58	2.62	0.95	2.70	2.04	0.40	4.99	2.30	3.94	2195


==> data/mlm_plots/tef/mr/cnn/ig/time_misc_auc.tex <==
name	auc
attack_time	0.15
l2	0.41
lom	0.70


==> data/mlm_plots/tef/mr/cnn/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.07	0.00	-0.14	0.28	0.21	0.00	0.14	0.25	0.29	0.08	0.41	0.16	0.29	0.38	0.48	0.50	0.35	0.62	0.13	0.62	210
0.06	0.00	0.22	0.00	-0.12	0.56	0.34	0.50	0.29	0.49	0.50	0.24	0.75	0.26	0.71	0.54	0.67	0.68	0.50	0.84	0.17	0.78	762
0.11	0.00	0.24	0.00	-0.10	0.58	0.34	0.50	0.33	0.50	0.50	0.27	0.73	0.23	0.67	0.58	0.67	0.69	0.50	0.84	0.17	0.78	873
0.15	0.00	0.23	0.00	-0.14	0.59	0.36	0.50	0.33	0.45	0.50	0.22	0.67	0.22	0.60	0.55	0.63	0.67	0.47	0.79	0.16	0.71	439
0.18	0.00	0.16	0.00	-0.12	0.44	0.28	0.50	0.29	0.40	0.43	0.21	0.60	0.20	0.50	0.50	0.59	0.60	0.44	0.74	0.15	0.69	700
0.32	0.00	0.10	0.00	-0.14	0.35	0.24	0.00	0.15	0.31	0.29	0.11	0.52	0.21	0.43	0.45	0.53	0.54	0.40	0.67	0.14	0.62	2195


==> data/mlm_plots/tef/mr/cnn/ig/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.12
top50	0.17


==> data/mlm_plots/tef/mr/cnn/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	104.14	200.12	165.34	72.70	327.54	127.42	262.93	3.00	4.96	5.00	2.51	7.40	2.44	6.00	138.94	238.05	193.62	77.78	398.32	160.27	302.59	4.00	5.09	5.00	2.62	7.56	2.47	6.00	732
0.06	98.70	205.88	158.52	26.37	385.38	179.50	257.79	3.00	4.04	4.00	2.24	5.83	1.79	5.00	127.95	272.14	202.03	14.33	529.96	257.81	323.62	3.00	4.16	4.00	2.33	5.99	1.83	5.00	1149
0.11	94.61	256.39	166.94	2.41	510.37	253.98	318.52	3.00	3.84	3.00	2.17	5.50	1.67	5.00	140.77	370.49	247.58	-48.60	789.58	419.09	457.93	3.00	3.97	4.00	2.28	5.67	1.69	5.00	625
0.15	110.47	273.82	174.49	-34.83	582.47	308.65	318.48	2.00	3.61	3.00	1.86	5.36	1.75	4.00	195.80	465.23	355.75	91.24	839.22	373.99	644.18	3.00	4.01	4.00	2.06	5.96	1.95	5.00	250
0.18	103.79	239.97	174.30	11.66	468.29	228.32	289.21	3.00	3.94	3.00	2.05	5.84	1.89	5.00	209.49	499.88	353.84	31.99	967.77	467.89	612.89	3.00	4.33	4.00	2.33	6.33	2.00	5.00	234
0.32	98.25	254.68	172.14	-39.82	549.18	294.50	273.51	3.00	4.00	4.00	2.18	5.82	1.82	5.00	309.89	706.49	500.35	-17.49	1430.47	723.98	870.28	3.00	4.59	4.00	2.66	6.52	1.93	6.00	722


==> data/mlm_plots/tef/mr/cnn/s/comparison_vals_auc.tex <==
name	auc
orig_pp	70.80
orig_ge	1.15
adv_pp	139.24
adv_ge	1.25


==> data/mlm_plots/tef/mr/cnn/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.00	0.00	0.00	0.00	0.00	0.00	-0.27	-0.01	-0.03	-0.38	0.35	0.36	0.27	0.00	0.00	0.00	0.00	0.00	0.00	0.00	732
0.06	0.00	0.09	0.00	-0.15	0.34	0.25	0.00	-0.29	0.02	-0.01	-0.39	0.43	0.41	0.28	0.00	0.08	0.00	-0.13	0.29	0.21	0.00	1149
0.11	0.00	0.23	0.00	-0.11	0.57	0.34	0.54	-0.08	0.29	0.34	-0.13	0.71	0.42	0.64	0.00	0.18	0.00	-0.09	0.45	0.27	0.42	625
0.15	0.00	0.26	0.00	-0.09	0.60	0.34	0.61	-0.09	0.22	0.19	-0.17	0.61	0.39	0.51	0.00	0.20	0.02	-0.07	0.47	0.27	0.39	250
0.18	0.00	0.29	0.30	-0.07	0.64	0.35	0.56	0.03	0.24	0.26	-0.16	0.64	0.40	0.57	0.00	0.22	0.20	-0.05	0.48	0.27	0.42	234
0.32	-0.17	0.13	0.15	-0.27	0.52	0.40	0.46	-0.20	0.11	0.14	-0.30	0.51	0.41	0.44	-0.12	0.09	0.10	-0.20	0.39	0.30	0.31	722


==> data/mlm_plots/tef/mr/cnn/s/correlations_auc.tex <==
name	auc
pcc	0.06
spearman	0.05
kendall	0.04


==> data/mlm_plots/tef/mr/cnn/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	4.66	6.43	5.99	3.79	9.07	2.64	7.45	4.04	7.46	5.95	1.68	13.23	5.77	8.92	7.53	21.61	17.33	5.83	37.39	15.78	37.37	732
0.06	3.15	4.56	4.20	1.97	7.16	2.60	5.63	2.70	4.87	3.91	0.33	9.41	4.54	6.24	3.17	15.73	8.38	0.36	31.11	15.37	26.94	1149
0.11	1.38	2.63	2.74	1.22	4.04	1.41	3.60	1.34	2.72	2.65	1.01	4.43	1.71	3.71	1.93	10.33	3.98	-3.12	23.77	13.44	11.34	625
0.15	1.03	2.03	2.07	0.92	3.14	1.11	2.84	1.01	2.23	2.06	0.77	3.69	1.46	3.23	1.32	6.81	3.15	-1.19	14.81	8.00	10.34	250
0.18	0.95	1.69	1.60	0.72	2.66	0.97	2.29	0.85	1.62	1.48	0.67	2.57	0.95	2.17	1.25	5.98	2.59	-2.88	14.83	8.85	6.39	234
0.32	0.99	1.63	1.59	0.83	2.43	0.80	2.16	0.92	1.63	1.56	0.76	2.50	0.87	2.20	1.14	4.04	2.07	-2.39	10.47	6.43	3.93	722


==> data/mlm_plots/tef/mr/cnn/s/ets_sts_auc.tex <==
name	auc
et_use	0.72
et_tse	0.75
et_ce	2.43


==> data/mlm_plots/tef/mr/cnn/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.50	6.92	2.65	-6.78	20.61	13.69	5.49	14.35	33.79	25.05	-2.42	70.01	36.21	41.88	13.65	58.07	28.49	-26.61	142.74	84.67	56.95	732
0.06	0.72	4.39	1.45	-4.00	12.78	8.39	3.75	7.89	24.10	18.07	1.21	46.99	22.89	32.11	8.12	49.63	21.94	-25.84	125.10	75.47	55.70	1149
0.11	0.31	2.10	0.81	-1.74	5.95	3.84	1.77	3.97	18.17	9.70	-2.93	39.27	21.10	26.07	3.68	42.64	11.86	-32.76	118.04	75.40	42.38	625
0.15	0.21	5.17	0.40	-26.20	36.55	31.37	1.15	3.01	15.05	6.35	-7.87	37.97	22.92	15.83	2.88	36.89	9.15	-43.89	117.67	80.78	26.40	250
0.18	0.14	0.91	0.27	-1.95	3.77	2.86	0.93	2.44	8.17	4.32	-1.22	17.57	9.40	9.77	2.15	18.29	4.39	-21.04	57.61	39.33	14.21	234
0.32	0.11	0.61	0.19	-0.88	2.10	1.49	0.46	2.71	6.37	4.15	-0.66	13.40	7.03	6.99	2.37	12.15	4.21	-22.61	46.90	34.75	9.60	722


==> data/mlm_plots/tef/mr/cnn/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.69
et_p_h	3.96
et_p_l2	8.50


==> data/mlm_plots/tef/mr/cnn/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.09	0.24	0.19	0.03	0.46	0.22	0.33	0.01	0.04	0.02	-0.01	0.09	0.05	0.04	0.01	0.03	0.02	-0.00	0.07	0.03	0.03	732
0.06	0.12	0.42	0.27	-0.03	0.86	0.45	0.60	0.01	0.04	0.02	-0.01	0.09	0.05	0.05	0.01	0.04	0.02	0.00	0.08	0.04	0.05	1149
0.11	0.21	0.71	0.46	-0.05	1.47	0.76	0.93	0.01	0.06	0.03	-0.01	0.13	0.07	0.07	0.02	0.05	0.03	0.00	0.10	0.05	0.07	625
0.15	0.29	1.14	0.68	0.00	2.27	1.14	1.88	0.01	0.06	0.03	-0.01	0.13	0.07	0.09	0.03	0.06	0.05	0.01	0.11	0.05	0.09	250
0.18	0.42	1.54	1.11	0.04	3.03	1.50	2.35	0.02	0.09	0.06	0.01	0.17	0.08	0.13	0.03	0.08	0.07	0.02	0.13	0.05	0.12	234
0.32	0.79	2.83	1.99	0.05	5.61	2.78	3.79	0.04	0.11	0.09	0.03	0.20	0.08	0.18	0.06	0.10	0.10	0.05	0.16	0.06	0.15	722


==> data/mlm_plots/tef/mr/cnn/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.42
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/tef/mr/cnn/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.89	0.91	0.92	0.88	0.94	0.03	0.93	0.88	0.90	0.92	0.85	0.96	0.05	0.94	0.93	0.95	0.97	0.88	1.01	0.06	0.99	732
0.06	0.86	0.88	0.89	0.84	0.92	0.04	0.91	0.83	0.87	0.88	0.81	0.93	0.06	0.92	0.87	0.91	0.95	0.82	1.01	0.09	0.98	1149
0.11	0.82	0.84	0.84	0.80	0.88	0.04	0.87	0.79	0.83	0.84	0.77	0.90	0.06	0.88	0.83	0.89	0.92	0.78	0.99	0.10	0.97	625
0.15	0.77	0.80	0.81	0.76	0.85	0.05	0.83	0.75	0.80	0.81	0.73	0.87	0.07	0.85	0.79	0.86	0.89	0.73	0.98	0.12	0.96	250
0.18	0.75	0.78	0.78	0.74	0.82	0.04	0.80	0.73	0.76	0.76	0.70	0.83	0.07	0.81	0.77	0.85	0.87	0.74	0.96	0.11	0.94	234
0.32	0.69	0.72	0.72	0.67	0.78	0.05	0.76	0.67	0.72	0.71	0.65	0.78	0.06	0.76	0.68	0.76	0.79	0.60	0.93	0.16	0.88	722


==> data/mlm_plots/tef/mr/cnn/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.23
sts_tse	0.23
sts_ce	0.25


==> data/mlm_plots/tef/mr/cnn/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.47	0.51	0.51	0.43	0.59	0.08	0.56	27.52	44.01	44.16	24.10	63.93	19.92	60.55	11.91	12.50	12.55	11.53	13.46	0.97	13.15	732
0.06	0.41	0.45	0.48	0.31	0.59	0.14	0.54	25.59	40.49	37.57	20.58	60.40	19.91	54.10	6.07	7.54	7.87	4.04	11.04	3.50	9.87	1149
0.11	0.17	0.38	0.46	0.21	0.55	0.17	0.52	21.53	35.28	31.95	17.08	53.49	18.21	48.83	0.74	3.64	3.43	0.43	6.85	3.21	5.09	625
0.15	0.23	0.35	0.31	0.20	0.51	0.16	0.50	24.05	36.04	32.04	17.85	54.24	18.20	45.77	0.59	3.22	1.51	-0.79	7.22	4.01	2.83	250
0.18	0.23	0.32	0.25	0.19	0.44	0.12	0.37	24.19	36.33	34.27	20.43	52.23	15.90	47.09	0.44	1.56	0.99	-0.83	3.95	2.39	1.77	234
0.32	0.33	0.40	0.38	0.33	0.48	0.08	0.46	26.83	37.63	35.72	23.93	51.33	13.70	46.97	0.44	1.24	0.99	-0.16	2.65	1.41	1.61	722


==> data/mlm_plots/tef/mr/cnn/s/time_misc_auc.tex <==
name	auc
attack_time	0.11
l2	10.84
lom	0.98


==> data/mlm_plots/tef/mr/cnn/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.14	0.00	-0.12	0.40	0.26	0.50	0.14	0.32	0.29	0.11	0.53	0.21	0.43	0.42	0.52	0.54	0.37	0.68	0.16	0.62	732
0.06	0.00	0.11	0.00	-0.15	0.37	0.26	0.00	0.17	0.33	0.33	0.08	0.58	0.25	0.50	0.46	0.58	0.58	0.40	0.76	0.18	0.70	1149
0.11	0.00	0.19	0.00	-0.16	0.54	0.35	0.50	0.00	0.33	0.33	0.03	0.62	0.29	0.50	0.40	0.55	0.58	0.32	0.77	0.22	0.70	625
0.15	0.00	0.25	0.00	-0.15	0.65	0.40	0.50	0.20	0.41	0.43	0.13	0.68	0.27	0.50	0.46	0.59	0.62	0.41	0.78	0.18	0.69	250
0.18	0.00	0.23	0.00	-0.13	0.58	0.36	0.50	0.17	0.38	0.33	0.11	0.65	0.27	0.57	0.50	0.60	0.60	0.42	0.78	0.18	0.70	234
0.32	0.00	0.14	0.00	-0.16	0.45	0.31	0.00	0.14	0.31	0.29	0.06	0.55	0.25	0.43	0.38	0.52	0.50	0.33	0.70	0.19	0.62	722


==> data/mlm_plots/tef/mr/cnn/s/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.10
top50	0.16


==> data/mlm_plots/tef/mr/lstm/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	106.09	160.38	136.33	75.97	244.79	84.41	204.24	3.00	4.42	4.00	2.51	6.32	1.91	5.25	120.53	202.37	182.77	90.21	314.53	112.16	236.02	3.00	4.54	4.00	2.59	6.49	1.95	6.00	288
0.06	98.76	221.29	177.37	36.28	406.30	185.01	280.39	3.00	4.06	3.00	1.87	6.26	2.19	5.00	142.32	280.74	229.42	85.74	475.75	195.00	353.96	3.00	4.20	4.00	2.02	6.37	2.18	5.00	1068
0.11	96.21	238.19	170.18	-56.32	532.69	294.50	265.40	3.00	4.11	4.00	1.92	6.31	2.19	5.00	155.38	352.95	258.76	-5.10	710.99	358.05	435.33	3.00	4.33	4.00	2.09	6.58	2.25	5.00	943
0.15	105.44	275.04	164.88	-90.12	640.20	365.16	293.95	2.00	3.91	3.00	1.54	6.28	2.37	5.00	189.95	452.00	309.31	-53.00	956.99	504.99	515.55	3.00	4.19	4.00	1.77	6.61	2.42	5.00	473
0.18	101.76	236.65	175.29	32.38	440.91	204.27	312.51	3.00	4.45	4.00	2.18	6.72	2.27	5.00	228.55	468.65	371.56	6.19	931.10	462.46	550.91	3.00	4.87	5.00	2.54	7.21	2.34	6.00	616
0.32	101.27	238.24	174.46	10.21	466.27	228.03	286.30	3.00	4.35	4.00	2.10	6.61	2.26	5.00	307.52	631.92	487.17	78.71	1185.13	553.21	755.77	3.00	4.99	5.00	2.58	7.40	2.41	6.00	1547


==> data/mlm_plots/tef/mr/lstm/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	68.62
orig_ge	1.23
adv_pp	130.02
adv_ge	1.34


==> data/mlm_plots/tef/mr/lstm/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.00	0.00	0.00	0.00	0.00	0.00	-0.30	-0.18	-0.24	-0.38	0.03	0.21	-0.05	0.00	0.00	0.00	0.00	0.00	0.00	0.00	288
0.06	0.00	-0.03	0.00	-0.34	0.29	0.31	0.00	-0.21	0.04	0.03	-0.31	0.40	0.36	0.29	0.00	0.03	0.00	-0.21	0.27	0.24	0.00	1068
0.11	-0.48	-0.16	-0.03	-0.60	0.28	0.44	0.00	-0.40	-0.04	-0.01	-0.50	0.42	0.46	0.31	-0.26	-0.03	0.00	-0.39	0.32	0.35	0.12	943
0.15	-0.65	-0.26	-0.24	-0.69	0.17	0.43	0.00	-0.53	-0.13	-0.15	-0.60	0.33	0.47	0.21	-0.32	-0.09	-0.01	-0.43	0.25	0.34	0.10	473
0.18	-0.72	-0.37	-0.42	-0.78	0.05	0.42	-0.14	-0.49	-0.20	-0.23	-0.60	0.20	0.40	0.10	-0.37	-0.14	-0.16	-0.46	0.19	0.33	0.08	616
0.32	-0.71	-0.40	-0.46	-0.79	-0.01	0.39	-0.18	-0.50	-0.23	-0.27	-0.60	0.14	0.37	0.01	-0.37	-0.16	-0.19	-0.46	0.14	0.30	0.03	1547


==> data/mlm_plots/tef/mr/lstm/ig/correlations_auc.tex <==
name	auc
pcc	-0.08
spearman	-0.04
kendall	-0.03


==> data/mlm_plots/tef/mr/lstm/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	4.75	6.40	5.70	3.32	9.48	3.08	6.80	4.83	7.42	6.54	3.12	11.72	4.30	8.68	8.37	24.59	27.98	8.56	40.62	16.03	39.08	288
0.06	3.34	4.80	4.56	2.60	7.01	2.21	5.70	2.98	5.26	4.30	1.34	9.18	3.92	6.18	4.55	19.22	12.18	1.56	36.87	17.65	32.36	1068
0.11	2.77	4.05	3.65	1.99	6.11	2.06	5.12	2.59	4.21	3.64	1.60	6.81	2.61	5.42	3.28	14.88	7.39	-3.30	33.05	18.17	18.68	943
0.15	2.61	3.52	3.39	2.04	4.99	1.47	4.45	2.42	3.87	3.57	1.76	5.98	2.11	4.91	3.41	13.34	6.61	-2.50	29.18	15.84	14.64	473
0.18	2.49	3.41	3.40	2.03	4.80	1.38	4.23	2.36	3.45	3.25	1.67	5.23	1.78	4.28	2.90	11.78	5.48	-4.38	27.94	16.16	12.47	616
0.32	2.18	2.90	2.83	1.74	4.05	1.15	3.45	2.06	2.94	2.76	1.55	4.32	1.38	3.52	2.31	6.98	3.74	-3.36	17.32	10.34	6.82	1547


==> data/mlm_plots/tef/mr/lstm/ig/ets_sts_auc.tex <==
name	auc
et_use	1.08
et_tse	1.14
et_ce	3.77


==> data/mlm_plots/tef/mr/lstm/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.41	7.16	1.98	-6.42	20.73	13.58	4.65	8.10	24.36	15.10	-6.48	55.20	30.84	24.46	7.69	35.38	18.78	-15.24	85.99	50.61	33.01	288
0.06	0.76	4.27	1.38	-6.32	14.85	10.58	3.18	7.97	25.38	16.80	-2.31	53.07	27.69	34.14	7.65	49.18	21.03	-29.52	127.88	78.70	48.13	1068
0.11	0.53	3.35	1.18	-7.18	13.88	10.53	2.56	6.50	21.71	14.02	-0.75	44.16	22.45	28.50	6.04	41.31	16.31	-30.75	113.37	72.06	40.65	943
0.15	0.40	5.14	0.81	-22.39	32.67	27.53	1.90	5.95	17.63	11.11	0.11	35.15	17.52	23.27	5.62	36.90	13.53	-29.55	103.35	66.45	39.66	473
0.18	0.35	2.72	0.62	-10.20	15.65	12.92	1.39	5.45	14.30	8.99	-1.76	30.37	16.07	17.13	4.66	24.82	9.40	-32.11	81.75	56.93	22.92	616
0.32	0.20	2.59	0.41	-21.57	26.75	24.16	0.87	5.01	11.79	7.49	-2.95	26.54	14.74	13.34	4.14	22.15	7.52	-31.78	76.08	53.93	17.75	1547


==> data/mlm_plots/tef/mr/lstm/ig/ets_time_misc_auc.tex <==
name	auc
et_p	1.03
et_p_h	5.01
et_p_l2	9.31


==> data/mlm_plots/tef/mr/lstm/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.11	0.29	0.25	0.04	0.55	0.26	0.35	0.02	0.05	0.03	-0.00	0.10	0.05	0.07	0.02	0.05	0.03	0.01	0.08	0.04	0.06	288
0.06	0.16	0.44	0.37	0.06	0.83	0.39	0.60	0.01	0.05	0.02	-0.01	0.11	0.06	0.06	0.01	0.05	0.03	0.00	0.09	0.04	0.06	1068
0.11	0.22	0.77	0.49	-0.22	1.77	1.00	0.94	0.01	0.06	0.04	-0.01	0.14	0.07	0.09	0.02	0.06	0.04	0.01	0.11	0.05	0.08	943
0.15	0.33	1.11	0.74	-0.03	2.26	1.14	1.35	0.02	0.07	0.04	0.00	0.14	0.07	0.12	0.03	0.07	0.05	0.02	0.12	0.05	0.11	473
0.18	0.51	1.39	1.08	0.15	2.64	1.24	1.87	0.03	0.09	0.07	0.02	0.16	0.07	0.14	0.04	0.08	0.08	0.03	0.13	0.05	0.11	616
0.32	0.79	2.43	1.70	-0.12	4.98	2.55	3.14	0.04	0.11	0.09	0.03	0.19	0.08	0.17	0.05	0.10	0.09	0.04	0.15	0.05	0.14	1547


==> data/mlm_plots/tef/mr/lstm/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.38
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/tef/mr/lstm/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.90	0.91	0.92	0.87	0.96	0.05	0.94	0.94	0.95	0.98	0.89	1.01	0.06	0.99	288
0.06	0.85	0.88	0.88	0.84	0.92	0.04	0.91	0.84	0.87	0.88	0.81	0.93	0.06	0.92	0.89	0.93	0.96	0.85	1.01	0.08	0.98	1068
0.11	0.82	0.84	0.85	0.80	0.89	0.04	0.87	0.79	0.84	0.84	0.77	0.90	0.06	0.88	0.85	0.89	0.92	0.77	1.01	0.12	0.97	943
0.15	0.78	0.81	0.81	0.77	0.85	0.04	0.84	0.77	0.81	0.82	0.74	0.88	0.07	0.86	0.82	0.88	0.91	0.77	0.99	0.11	0.96	473
0.18	0.76	0.79	0.79	0.74	0.83	0.05	0.82	0.74	0.78	0.78	0.71	0.84	0.07	0.83	0.78	0.85	0.87	0.73	0.97	0.12	0.95	616
0.32	0.71	0.74	0.74	0.69	0.80	0.05	0.78	0.69	0.74	0.73	0.67	0.80	0.07	0.78	0.72	0.79	0.81	0.65	0.93	0.14	0.90	1547


==> data/mlm_plots/tef/mr/lstm/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.23
sts_tse	0.23
sts_ce	0.25


==> data/mlm_plots/tef/mr/lstm/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.39	0.46	0.47	0.34	0.58	0.12	0.56	0.00	0.01	0.01	-0.00	0.03	0.02	0.02	4.23	7.93	8.26	3.20	12.66	4.73	11.90	288
0.06	0.24	0.37	0.36	0.22	0.52	0.15	0.50	0.01	0.44	0.02	-1.88	2.75	2.31	0.05	1.44	4.42	3.53	0.55	8.30	3.87	6.16	1068
0.11	0.25	0.37	0.37	0.24	0.49	0.13	0.46	0.01	0.76	0.03	-2.27	3.78	3.02	0.13	1.53	4.94	3.48	0.05	9.84	4.90	6.16	943
0.15	0.33	0.42	0.42	0.30	0.54	0.12	0.51	0.02	1.02	0.05	-2.59	4.63	3.61	0.24	1.72	5.06	3.09	0.01	10.11	5.05	6.67	473
0.18	0.34	0.41	0.42	0.31	0.51	0.10	0.49	0.03	0.96	0.06	-1.38	3.30	2.34	0.23	1.96	5.81	4.32	0.58	11.04	5.23	8.59	616
0.32	0.44	0.50	0.51	0.40	0.60	0.10	0.57	0.03	1.55	0.08	-2.58	5.69	4.14	1.98	1.94	5.66	4.22	0.62	10.70	5.04	7.82	1547


==> data/mlm_plots/tef/mr/lstm/ig/time_misc_auc.tex <==
name	auc
attack_time	0.12
l2	0.28
lom	1.59


==> data/mlm_plots/tef/mr/lstm/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.17	0.00	-0.09	0.42	0.26	0.50	0.14	0.35	0.29	0.15	0.54	0.20	0.46	0.50	0.58	0.62	0.47	0.69	0.11	0.67	288
0.06	0.00	0.14	0.00	-0.15	0.43	0.29	0.00	0.17	0.33	0.29	0.10	0.56	0.23	0.50	0.38	0.50	0.50	0.32	0.68	0.18	0.62	1068
0.11	0.00	0.11	0.00	-0.15	0.37	0.26	0.00	0.00	0.29	0.29	0.02	0.57	0.27	0.50	0.33	0.48	0.46	0.27	0.69	0.21	0.64	943
0.15	0.00	0.12	0.00	-0.17	0.41	0.29	0.00	0.00	0.28	0.25	0.01	0.55	0.27	0.50	0.31	0.45	0.43	0.23	0.67	0.22	0.64	473
0.18	0.00	0.09	0.00	-0.14	0.32	0.23	0.00	0.00	0.25	0.17	0.02	0.48	0.23	0.43	0.31	0.45	0.45	0.26	0.64	0.19	0.60	616
0.32	0.00	0.08	0.00	-0.14	0.30	0.22	0.00	0.00	0.24	0.20	0.02	0.46	0.22	0.40	0.31	0.44	0.43	0.26	0.62	0.18	0.57	1547


==> data/mlm_plots/tef/mr/lstm/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.08
top50	0.13


==> data/mlm_plots/tef/mr/lstm/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	102.22	181.40	144.76	67.29	295.51	114.11	225.13	3.00	4.69	4.00	2.85	6.52	1.83	6.00	123.31	215.41	174.13	88.59	342.24	126.82	284.99	3.00	4.80	4.00	2.97	6.64	1.84	6.00	516
0.06	102.29	228.66	177.37	38.60	418.71	190.05	293.87	3.00	4.21	4.00	1.95	6.47	2.26	5.00	136.33	292.59	228.36	66.61	518.57	225.98	378.88	3.00	4.35	4.00	2.07	6.63	2.28	5.00	1208
0.11	94.54	257.91	168.83	-139.89	655.71	397.80	279.59	3.00	4.02	4.00	1.93	6.10	2.09	5.00	165.73	409.51	255.16	-402.34	1221.36	811.85	438.84	3.00	4.23	4.00	2.07	6.38	2.16	5.00	898
0.15	104.10	286.83	176.15	-72.36	646.01	359.19	294.27	2.00	3.57	3.00	1.91	5.23	1.66	4.00	193.42	458.47	324.45	-10.51	927.46	468.98	592.53	2.00	3.91	3.00	2.10	5.72	1.81	5.00	351
0.18	101.85	216.60	168.94	53.00	380.19	163.59	279.32	3.00	4.62	4.00	1.67	7.57	2.95	5.00	235.59	453.86	364.06	111.05	796.68	342.81	556.92	3.00	5.11	5.00	2.09	8.13	3.02	6.00	473
0.32	101.85	236.16	173.04	14.35	457.97	221.81	279.59	3.00	4.28	4.00	2.06	6.49	2.22	5.00	320.06	649.22	507.84	49.62	1248.82	599.60	784.74	3.00	5.06	5.00	2.66	7.46	2.40	6.00	1242


==> data/mlm_plots/tef/mr/lstm/s/comparison_vals_auc.tex <==
name	auc
orig_pp	68.73
orig_ge	1.23
adv_pp	133.37
adv_ge	1.36


==> data/mlm_plots/tef/mr/lstm/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.00	0.00	0.00	0.00	0.00	0.00	-0.12	0.14	0.23	-0.23	0.51	0.37	0.45	0.00	0.00	0.00	0.00	0.00	0.00	0.00	516
0.06	0.00	0.12	0.00	-0.12	0.36	0.24	0.00	-0.17	0.13	0.07	-0.30	0.55	0.43	0.46	0.00	0.13	0.00	-0.12	0.38	0.25	0.04	1208
0.11	0.00	0.18	0.00	-0.07	0.44	0.26	0.39	-0.02	0.30	0.40	-0.11	0.72	0.42	0.66	0.00	0.23	0.06	-0.03	0.50	0.27	0.48	898
0.15	0.00	0.16	0.00	-0.08	0.41	0.25	0.39	0.10	0.31	0.36	-0.08	0.69	0.38	0.63	0.00	0.23	0.18	-0.02	0.48	0.25	0.45	351
0.18	0.00	0.16	0.12	-0.06	0.38	0.22	0.32	0.23	0.38	0.42	0.09	0.67	0.29	0.59	0.12	0.28	0.28	0.07	0.48	0.21	0.43	473
0.32	-0.10	0.07	0.04	-0.16	0.29	0.22	0.21	0.10	0.29	0.32	0.01	0.57	0.28	0.49	0.07	0.21	0.22	0.00	0.42	0.21	0.36	1242


==> data/mlm_plots/tef/mr/lstm/s/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.08
kendall	0.06


==> data/mlm_plots/tef/mr/lstm/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.03	4.76	6.47	5.65	3.30	9.64	3.17	7.21	4.27	7.28	5.44	1.59	12.96	5.68	8.63	8.19	24.61	24.62	7.92	41.30	16.69	40.46	516
0.06	3.04	4.58	4.22	2.06	7.10	2.52	5.56	2.52	4.99	3.76	0.69	9.30	4.30	5.82	3.93	17.76	11.14	2.02	33.49	15.74	31.49	1208
0.11	1.95	2.80	2.73	1.54	4.06	1.26	3.45	1.70	2.99	2.70	1.20	4.78	1.79	3.68	2.51	10.76	5.73	-1.10	22.62	11.86	14.68	898
0.15	1.59	2.38	2.34	1.37	3.38	1.00	3.03	1.58	2.43	2.26	1.26	3.60	1.17	2.93	2.14	8.21	4.83	-0.91	17.33	9.12	10.58	351
0.18	1.59	2.05	2.04	1.34	2.75	0.70	2.40	1.48	2.10	1.93	1.11	3.10	0.99	2.51	1.85	6.34	3.01	-2.36	15.05	8.70	6.81	473
0.32	1.46	1.85	1.79	1.24	2.45	0.60	2.15	1.39	1.87	1.73	1.09	2.65	0.78	2.20	1.55	4.10	2.34	-1.92	10.13	6.02	4.13	1242


==> data/mlm_plots/tef/mr/lstm/s/ets_sts_auc.tex <==
name	auc
et_use	0.79
et_tse	0.83
et_ce	2.66


==> data/mlm_plots/tef/mr/lstm/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.03	1.40	5.51	2.30	-3.53	14.55	9.04	4.52	9.02	30.15	19.12	-5.74	66.05	35.90	36.97	7.91	50.51	21.41	-23.26	124.27	73.76	63.06	516
0.06	0.69	3.87	1.23	-4.95	12.70	8.82	2.90	7.15	25.13	15.48	-0.86	51.12	25.99	35.18	7.28	49.28	20.83	-24.89	123.44	74.16	50.22	1208
0.11	0.34	1.73	0.78	-3.96	7.41	5.69	1.52	4.25	16.58	8.72	-3.39	36.56	19.97	21.11	4.23	33.93	9.89	-28.75	96.61	62.68	30.25	898
0.15	0.25	6.13	0.56	-27.45	39.71	33.58	1.27	4.31	14.64	8.28	-4.24	33.51	18.87	14.26	4.13	39.16	10.84	-42.23	120.56	81.39	25.13	351
0.18	0.20	2.86	0.36	-15.28	21.01	18.15	0.74	3.55	9.03	5.39	-3.66	21.72	12.69	9.75	2.96	17.10	5.57	-29.15	63.34	46.24	12.92	473
0.32	0.14	0.94	0.25	-5.33	7.21	6.27	0.49	3.21	6.93	4.74	-2.00	15.85	8.93	7.68	2.69	13.85	4.80	-28.86	56.56	42.71	9.58	1242


==> data/mlm_plots/tef/mr/lstm/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.86
et_p_h	3.96
et_p_l2	8.09


==> data/mlm_plots/tef/mr/lstm/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.11	0.28	0.22	0.03	0.53	0.25	0.36	0.01	0.05	0.02	-0.01	0.11	0.06	0.06	0.01	0.04	0.03	0.00	0.08	0.04	0.06	516
0.06	0.15	0.43	0.33	0.04	0.82	0.39	0.57	0.01	0.04	0.02	-0.01	0.10	0.05	0.05	0.01	0.04	0.03	0.00	0.08	0.04	0.05	1208
0.11	0.27	0.84	0.50	-0.20	1.87	1.03	1.01	0.01	0.06	0.04	-0.01	0.14	0.07	0.09	0.02	0.06	0.04	0.01	0.11	0.05	0.08	898
0.15	0.34	1.15	0.82	-0.04	2.34	1.19	1.42	0.02	0.06	0.04	-0.00	0.12	0.06	0.08	0.03	0.06	0.05	0.02	0.11	0.05	0.08	351
0.18	0.57	1.56	1.21	0.10	3.02	1.46	2.04	0.03	0.09	0.07	0.02	0.17	0.07	0.14	0.04	0.08	0.08	0.03	0.14	0.05	0.12	473
0.32	0.89	2.63	1.84	-0.20	5.45	2.82	3.21	0.05	0.12	0.10	0.03	0.20	0.08	0.18	0.06	0.10	0.10	0.05	0.16	0.06	0.14	1242


==> data/mlm_plots/tef/mr/lstm/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.41
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/tef/mr/lstm/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.88	0.90	0.91	0.85	0.96	0.05	0.94	0.94	0.95	0.98	0.90	1.01	0.05	0.99	516
0.06	0.86	0.89	0.89	0.85	0.93	0.04	0.91	0.84	0.88	0.88	0.82	0.94	0.06	0.92	0.89	0.93	0.97	0.85	1.01	0.08	0.99	1208
0.11	0.82	0.84	0.84	0.80	0.88	0.04	0.87	0.80	0.84	0.84	0.77	0.90	0.06	0.88	0.85	0.89	0.93	0.79	1.00	0.11	0.97	898
0.15	0.79	0.81	0.81	0.77	0.86	0.05	0.84	0.77	0.81	0.80	0.75	0.87	0.06	0.85	0.82	0.87	0.91	0.76	0.99	0.12	0.96	351
0.18	0.75	0.79	0.78	0.74	0.83	0.04	0.81	0.73	0.78	0.78	0.71	0.84	0.06	0.82	0.78	0.85	0.86	0.74	0.96	0.11	0.94	473
0.32	0.71	0.74	0.73	0.69	0.79	0.05	0.77	0.68	0.73	0.73	0.67	0.80	0.07	0.78	0.72	0.79	0.81	0.65	0.92	0.13	0.89	1242


==> data/mlm_plots/tef/mr/lstm/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.23
sts_tse	0.23
sts_ce	0.25


==> data/mlm_plots/tef/mr/lstm/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.03	0.40	0.46	0.46	0.36	0.55	0.09	0.52	1.11	1.90	1.66	0.91	2.90	1.00	2.44	8.66	11.52	11.26	7.83	15.21	3.69	13.78	516
0.06	0.30	0.40	0.41	0.27	0.52	0.12	0.49	1.10	5.58	1.62	-10.57	21.72	16.14	2.49	3.33	6.30	6.15	2.47	10.13	3.83	8.64	1208
0.11	0.29	0.37	0.38	0.25	0.48	0.12	0.45	1.20	13.68	1.83	-32.01	59.38	45.69	3.01	1.62	3.63	3.27	1.00	6.27	2.63	5.11	898
0.15	0.31	0.39	0.40	0.28	0.50	0.11	0.47	1.41	17.28	2.29	-21.70	56.26	38.98	16.82	1.46	3.12	2.24	0.58	5.66	2.54	3.80	351
0.18	0.34	0.42	0.42	0.33	0.50	0.09	0.48	1.94	23.80	2.66	-73.84	121.45	97.64	16.65	1.25	3.26	2.40	0.53	5.98	2.73	4.34	473
0.32	0.42	0.46	0.46	0.39	0.54	0.08	0.52	2.24	29.80	3.22	-28.71	88.31	58.51	40.87	1.22	3.15	2.58	0.71	5.59	2.44	4.58	1242


==> data/mlm_plots/tef/mr/lstm/s/time_misc_auc.tex <==
name	auc
attack_time	0.12
l2	5.58
lom	1.19


==> data/mlm_plots/tef/mr/lstm/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.03	0.00	0.09	0.00	-0.12	0.29	0.20	0.00	0.14	0.25	0.14	0.06	0.43	0.19	0.29	0.31	0.45	0.46	0.29	0.60	0.16	0.54	516
0.06	0.00	0.12	0.00	-0.16	0.39	0.27	0.00	0.20	0.36	0.33	0.12	0.60	0.24	0.50	0.43	0.57	0.57	0.39	0.76	0.18	0.69	1208
0.11	0.00	0.12	0.00	-0.15	0.40	0.27	0.00	0.20	0.40	0.40	0.13	0.67	0.27	0.57	0.46	0.59	0.62	0.38	0.81	0.21	0.75	898
0.15	0.00	0.18	0.00	-0.17	0.53	0.35	0.00	0.20	0.42	0.50	0.14	0.70	0.28	0.60	0.54	0.62	0.67	0.44	0.80	0.18	0.73	351
0.18	0.00	0.10	0.00	-0.13	0.32	0.23	0.00	0.29	0.41	0.43	0.19	0.63	0.22	0.57	0.54	0.64	0.69	0.48	0.80	0.16	0.75	473
0.32	0.00	0.05	0.00	-0.11	0.20	0.16	0.00	0.17	0.34	0.33	0.14	0.55	0.20	0.50	0.54	0.62	0.62	0.48	0.76	0.14	0.71	1242


==> data/mlm_plots/tef/mr/lstm/s/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.11
top50	0.18


==> data/mlm_plots/tef/mr/lstmatt/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	102.04	213.31	173.96	45.31	381.30	168.00	272.18	3.00	4.49	4.00	2.31	6.67	2.18	6.00	139.21	286.55	226.57	61.43	511.68	225.13	345.22	3.00	4.71	4.00	2.52	6.90	2.19	6.00	567
0.11	101.27	225.86	175.78	32.58	419.14	193.28	279.99	3.00	4.35	4.00	2.23	6.47	2.12	5.00	159.85	338.01	267.56	64.68	611.35	273.34	416.58	3.00	4.64	4.00	2.47	6.80	2.16	6.00	933
0.15	102.23	249.32	177.49	19.07	479.58	230.26	305.23	2.00	3.95	3.00	1.82	6.08	2.13	5.00	187.40	434.83	318.83	11.30	858.37	423.54	513.72	3.00	4.29	4.00	2.01	6.57	2.28	5.00	508
0.18	103.03	227.08	177.92	46.20	407.95	180.87	283.77	3.00	4.25	4.00	2.11	6.38	2.14	5.00	226.83	451.24	354.84	97.64	804.85	353.61	542.97	3.00	4.73	4.00	2.46	6.99	2.26	6.00	781
0.32	104.35	239.97	178.60	-0.35	480.29	240.32	290.69	3.00	4.23	4.00	2.13	6.34	2.11	5.00	324.42	669.85	510.15	108.90	1230.81	560.95	834.28	3.00	4.91	5.00	2.58	7.23	2.32	6.00	2697


==> data/mlm_plots/tef/mr/lstmatt/a/comparison_vals_auc.tex <==
name	auc
orig_pp	60.44
orig_ge	1.10
adv_pp	122.62
adv_ge	1.22


==> data/mlm_plots/tef/mr/lstmatt/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.47	0.62	0.66	0.38	0.85	0.23	0.79	0.61	0.73	0.77	0.51	0.94	0.22	0.89	0.50	0.62	0.65	0.41	0.82	0.21	0.77	567
0.11	0.36	0.53	0.56	0.27	0.79	0.26	0.74	0.50	0.65	0.69	0.41	0.89	0.24	0.84	0.40	0.54	0.56	0.32	0.77	0.22	0.71	933
0.15	0.32	0.49	0.51	0.22	0.75	0.27	0.70	0.46	0.61	0.63	0.37	0.86	0.25	0.81	0.37	0.51	0.52	0.29	0.73	0.22	0.66	508
0.18	0.12	0.34	0.35	0.04	0.64	0.30	0.57	0.25	0.45	0.49	0.14	0.76	0.31	0.69	0.20	0.36	0.37	0.11	0.61	0.25	0.55	781
0.32	-0.07	0.18	0.16	-0.15	0.51	0.33	0.42	0.02	0.28	0.31	-0.08	0.65	0.37	0.56	0.03	0.23	0.22	-0.06	0.51	0.28	0.43	2697


==> data/mlm_plots/tef/mr/lstmatt/a/correlations_auc.tex <==
name	auc
pcc	0.10
spearman	0.13
kendall	0.10


==> data/mlm_plots/tef/mr/lstmatt/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	0.82	1.65	1.41	0.48	2.82	1.17	2.14	0.77	1.72	1.34	0.30	3.14	1.42	2.25	1.35	5.79	3.17	-0.89	12.47	6.68	7.70	567
0.11	0.80	1.60	1.44	0.55	2.64	1.04	2.18	0.80	1.63	1.34	0.40	2.85	1.22	2.12	1.21	4.96	2.48	-1.34	11.25	6.29	6.08	933
0.15	0.80	1.44	1.27	0.58	2.31	0.86	1.95	0.75	1.45	1.22	0.48	2.43	0.98	1.92	1.12	4.03	2.19	-1.16	9.21	5.18	4.54	508
0.18	0.98	1.63	1.56	0.76	2.50	0.87	2.13	0.95	1.65	1.48	0.62	2.68	1.03	2.12	1.22	4.42	2.23	-1.78	10.62	6.20	4.70	781
0.32	1.05	1.57	1.55	0.85	2.28	0.72	2.00	1.04	1.58	1.52	0.79	2.38	0.80	1.98	1.18	2.93	1.82	-0.78	6.63	3.71	3.17	2697


==> data/mlm_plots/tef/mr/lstmatt/a/ets_sts_auc.tex <==
name	auc
et_use	0.41
et_tse	0.42
et_ce	1.09


==> data/mlm_plots/tef/mr/lstmatt/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.22	2.13	0.50	-9.71	13.96	11.83	1.21	2.43	7.60	5.08	-0.49	15.69	8.09	9.43	2.50	10.60	5.28	-6.46	27.66	17.06	12.12	567
0.11	0.21	1.46	0.38	-3.91	6.82	5.36	0.91	2.62	7.43	4.83	-0.42	15.27	7.84	9.34	2.52	11.58	5.26	-12.42	35.58	24.00	11.37	933
0.15	0.14	0.82	0.30	-1.16	2.80	1.98	0.67	2.47	8.28	4.59	-4.92	21.48	13.20	8.89	2.39	15.93	5.25	-22.28	54.14	38.21	12.77	508
0.18	0.14	1.02	0.30	-3.07	5.11	4.09	0.64	2.61	6.64	4.43	-0.00	13.29	6.64	8.28	2.42	10.02	4.59	-10.21	30.26	20.23	10.23	781
0.32	0.10	0.86	0.21	-4.24	5.95	5.10	0.44	2.67	6.21	4.21	-0.80	13.22	7.01	7.42	2.33	10.66	4.10	-14.83	36.15	25.49	9.47	2697


==> data/mlm_plots/tef/mr/lstmatt/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.29
et_p_h	1.82
et_p_l2	2.97


==> data/mlm_plots/tef/mr/lstmatt/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.15	0.47	0.32	0.01	0.93	0.46	0.62	0.01	0.05	0.03	-0.00	0.10	0.05	0.06	0.02	0.04	0.03	0.01	0.08	0.04	0.06	567
0.11	0.24	0.71	0.51	0.02	1.40	0.69	0.92	0.02	0.06	0.04	0.00	0.11	0.06	0.07	0.02	0.05	0.04	0.01	0.09	0.04	0.07	933
0.15	0.33	1.06	0.72	0.00	2.11	1.05	1.44	0.02	0.07	0.04	0.00	0.13	0.07	0.09	0.03	0.06	0.05	0.01	0.11	0.05	0.08	508
0.18	0.45	1.41	1.05	0.05	2.77	1.36	1.90	0.03	0.09	0.07	0.02	0.15	0.07	0.13	0.04	0.08	0.07	0.03	0.12	0.05	0.11	781
0.32	0.87	2.64	1.87	-0.05	5.33	2.69	3.45	0.04	0.11	0.09	0.03	0.19	0.08	0.17	0.06	0.10	0.10	0.05	0.16	0.06	0.14	2697


==> data/mlm_plots/tef/mr/lstmatt/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.38
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/tef/mr/lstmatt/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.85	0.87	0.88	0.84	0.91	0.04	0.90	0.83	0.87	0.87	0.81	0.92	0.06	0.91	0.88	0.92	0.95	0.83	1.01	0.09	0.98	567
0.11	0.82	0.84	0.84	0.80	0.88	0.04	0.87	0.79	0.83	0.84	0.77	0.90	0.06	0.88	0.83	0.88	0.91	0.76	1.00	0.12	0.97	933
0.15	0.78	0.81	0.81	0.77	0.86	0.05	0.84	0.76	0.80	0.80	0.74	0.86	0.06	0.85	0.80	0.85	0.88	0.73	0.98	0.12	0.94	508
0.18	0.76	0.79	0.79	0.74	0.83	0.05	0.82	0.73	0.78	0.78	0.71	0.84	0.07	0.83	0.77	0.83	0.86	0.71	0.96	0.13	0.93	781
0.32	0.69	0.73	0.73	0.68	0.78	0.05	0.76	0.68	0.73	0.72	0.66	0.79	0.07	0.77	0.67	0.76	0.78	0.60	0.91	0.16	0.87	2697


==> data/mlm_plots/tef/mr/lstmatt/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.20
sts_ce	0.22


==> data/mlm_plots/tef/mr/lstmatt/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.12	0.13	0.13	0.10	0.17	0.04	0.14	0.10	0.15	0.14	0.08	0.23	0.07	0.19	0.69	1.85	1.44	0.32	3.37	1.53	2.74	567
0.11	0.15	0.21	0.22	0.15	0.26	0.06	0.24	0.12	0.18	0.16	0.10	0.26	0.08	0.23	0.66	2.02	1.66	0.35	3.69	1.67	2.97	933
0.15	0.23	0.27	0.27	0.21	0.33	0.06	0.30	0.14	0.20	0.19	0.12	0.29	0.09	0.25	0.63	1.76	1.36	0.28	3.24	1.48	2.50	508
0.18	0.28	0.31	0.30	0.26	0.36	0.05	0.33	0.14	0.21	0.19	0.12	0.30	0.09	0.27	1.07	2.67	2.33	0.72	4.62	1.95	3.86	781
0.32	0.37	0.43	0.43	0.34	0.53	0.09	0.49	0.17	0.24	0.22	0.14	0.33	0.09	0.29	1.26	3.03	2.68	0.86	5.20	2.17	4.35	2697


==> data/mlm_plots/tef/mr/lstmatt/a/time_misc_auc.tex <==
name	auc
attack_time	0.08
l2	0.05
lom	0.63


==> data/mlm_plots/tef/mr/lstmatt/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.36	0.00	-0.04	0.75	0.40	0.50	0.57	0.65	0.71	0.46	0.85	0.19	0.75	0.75	0.80	0.83	0.67	0.94	0.13	0.89	567
0.11	0.00	0.33	0.00	-0.07	0.72	0.39	0.50	0.50	0.59	0.57	0.38	0.79	0.21	0.71	0.67	0.76	0.77	0.62	0.91	0.14	0.85	933
0.15	0.00	0.26	0.00	-0.13	0.64	0.39	0.50	0.40	0.55	0.50	0.30	0.79	0.24	0.68	0.67	0.75	0.75	0.61	0.90	0.14	0.86	508
0.18	0.00	0.22	0.00	-0.13	0.56	0.34	0.50	0.29	0.47	0.43	0.24	0.70	0.23	0.67	0.55	0.67	0.69	0.51	0.83	0.16	0.77	781
0.32	0.00	0.14	0.00	-0.16	0.44	0.30	0.00	0.17	0.37	0.33	0.14	0.60	0.23	0.50	0.50	0.60	0.60	0.43	0.77	0.17	0.71	2697


==> data/mlm_plots/tef/mr/lstmatt/a/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.13
top50	0.18


==> data/mlm_plots/tef/mr/lstmatt/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	104.46	211.54	175.44	45.83	377.24	165.71	269.18	3.00	4.50	4.00	2.30	6.70	2.20	6.00	142.31	281.78	225.34	76.83	486.72	204.95	359.03	3.00	4.68	4.00	2.41	6.95	2.27	6.00	545
0.11	98.15	235.74	176.60	-55.26	526.73	291.00	278.83	3.00	4.37	4.00	2.22	6.53	2.16	5.00	160.51	355.18	266.25	-20.91	731.26	376.09	446.23	3.00	4.63	4.00	2.37	6.88	2.26	6.00	916
0.15	99.81	255.58	178.21	-21.61	532.78	277.20	301.78	2.00	3.87	3.00	1.89	5.85	1.98	5.00	185.70	423.36	320.99	83.36	763.36	340.00	526.08	3.00	4.14	4.00	2.05	6.24	2.10	5.00	504
0.18	101.60	226.04	177.92	17.46	434.62	208.58	279.50	3.00	4.32	4.00	2.14	6.50	2.18	5.00	225.15	467.61	362.66	52.16	883.05	415.45	561.19	3.00	4.75	4.00	2.46	7.04	2.29	6.00	783
0.32	104.57	242.41	177.42	-18.84	503.66	261.25	289.99	3.00	4.24	4.00	2.10	6.39	2.14	5.00	310.91	663.35	508.17	104.18	1222.53	559.17	831.19	3.00	4.90	5.00	2.54	7.26	2.36	6.00	2682


==> data/mlm_plots/tef/mr/lstmatt/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	61.17
orig_ge	1.11
adv_pp	123.78
adv_ge	1.21


==> data/mlm_plots/tef/mr/lstmatt/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.19	0.45	0.48	0.09	0.81	0.36	0.75	0.44	0.60	0.59	0.35	0.85	0.25	0.79	0.38	0.53	0.54	0.30	0.76	0.23	0.69	545
0.11	0.04	0.31	0.34	-0.07	0.70	0.39	0.63	0.31	0.48	0.48	0.20	0.76	0.28	0.68	0.27	0.42	0.42	0.18	0.67	0.24	0.59	916
0.15	-0.10	0.22	0.24	-0.19	0.63	0.41	0.53	0.15	0.37	0.37	0.07	0.68	0.30	0.59	0.16	0.34	0.33	0.08	0.59	0.25	0.51	504
0.18	-0.17	0.10	0.10	-0.26	0.45	0.35	0.33	0.09	0.27	0.28	-0.02	0.56	0.29	0.46	0.10	0.24	0.26	0.01	0.47	0.23	0.39	783
0.32	-0.33	-0.07	-0.09	-0.42	0.27	0.35	0.16	-0.13	0.08	0.08	-0.23	0.38	0.31	0.29	-0.08	0.08	0.08	-0.16	0.32	0.24	0.24	2682


==> data/mlm_plots/tef/mr/lstmatt/ig/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.08
kendall	0.07


==> data/mlm_plots/tef/mr/lstmatt/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	0.99	2.42	2.07	0.46	4.38	1.96	3.29	1.00	2.65	2.15	0.34	4.95	2.30	3.51	1.86	8.52	4.68	-1.75	18.79	10.27	10.91	545
0.11	1.18	2.35	2.18	0.79	3.92	1.57	3.20	1.18	2.53	2.18	0.68	4.38	1.85	3.53	1.84	8.22	4.42	-1.45	17.89	9.67	10.60	916
0.15	1.26	2.20	2.08	0.82	3.58	1.38	3.03	1.17	2.28	2.03	0.61	3.95	1.67	3.00	1.75	7.00	3.37	-2.99	16.99	9.99	7.73	504
0.18	1.50	2.23	2.13	1.14	3.32	1.09	2.80	1.48	2.34	2.16	1.05	3.63	1.29	2.95	1.82	6.05	3.51	-1.18	13.29	7.23	7.00	783
0.32	1.53	2.07	2.02	1.23	2.90	0.83	2.54	1.52	2.10	2.00	1.16	3.05	0.94	2.55	1.60	4.12	2.47	-1.31	9.56	5.44	4.41	2682


==> data/mlm_plots/tef/mr/lstmatt/ig/ets_sts_auc.tex <==
name	auc
et_use	0.58
et_tse	0.61
et_ce	1.63


==> data/mlm_plots/tef/mr/lstmatt/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.28	2.61	0.63	-5.56	10.78	8.17	1.80	2.75	11.84	6.46	-3.86	27.54	15.70	12.42	2.72	23.77	7.03	-29.53	77.08	53.31	19.61	545
0.11	0.25	1.90	0.56	-6.22	10.03	8.13	1.29	3.35	10.99	6.76	-2.49	24.47	13.48	13.17	3.01	20.96	7.95	-19.17	61.10	40.13	20.01	916
0.15	0.21	2.91	0.46	-15.39	21.22	18.30	1.12	3.16	11.69	6.71	-4.98	28.35	16.67	13.12	3.10	24.52	7.37	-29.80	78.84	54.32	22.43	504
0.18	0.21	1.91	0.40	-13.69	17.50	15.59	0.93	3.56	9.36	6.12	-1.20	19.92	10.56	11.06	3.11	18.89	6.23	-28.96	66.73	47.85	15.28	783
0.32	0.15	0.88	0.28	-2.61	4.38	3.50	0.62	3.47	8.42	5.55	-1.39	18.22	9.81	9.54	2.89	16.01	5.54	-23.29	55.30	39.30	12.83	2682


==> data/mlm_plots/tef/mr/lstmatt/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.48
et_p_h	2.59
et_p_l2	5.14


==> data/mlm_plots/tef/mr/lstmatt/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.15	0.45	0.32	0.02	0.89	0.44	0.64	0.01	0.05	0.03	-0.01	0.10	0.06	0.07	0.02	0.05	0.03	0.01	0.09	0.04	0.06	545
0.11	0.27	0.72	0.55	0.06	1.38	0.66	0.96	0.01	0.06	0.04	-0.00	0.12	0.06	0.09	0.02	0.06	0.04	0.01	0.10	0.04	0.08	916
0.15	0.35	1.08	0.80	0.01	2.16	1.07	1.44	0.02	0.07	0.04	-0.00	0.14	0.07	0.10	0.03	0.06	0.05	0.01	0.12	0.05	0.09	504
0.18	0.51	1.42	1.04	0.11	2.73	1.31	1.93	0.03	0.09	0.07	0.01	0.16	0.07	0.14	0.04	0.08	0.07	0.03	0.13	0.05	0.11	783
0.32	0.86	2.56	1.84	0.01	5.11	2.55	3.38	0.04	0.11	0.09	0.03	0.20	0.08	0.18	0.05	0.10	0.09	0.04	0.16	0.06	0.14	2682


==> data/mlm_plots/tef/mr/lstmatt/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.38
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/tef/mr/lstmatt/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.85	0.87	0.88	0.84	0.91	0.04	0.90	0.84	0.87	0.88	0.82	0.93	0.05	0.91	0.90	0.93	0.95	0.85	1.00	0.08	0.98	545
0.11	0.82	0.84	0.84	0.80	0.88	0.04	0.87	0.81	0.84	0.85	0.78	0.90	0.06	0.89	0.86	0.90	0.93	0.79	1.00	0.10	0.97	916
0.15	0.78	0.81	0.81	0.77	0.86	0.05	0.84	0.76	0.80	0.81	0.74	0.87	0.06	0.85	0.81	0.86	0.90	0.75	0.98	0.12	0.96	504
0.18	0.76	0.79	0.79	0.74	0.83	0.04	0.82	0.74	0.79	0.79	0.72	0.85	0.06	0.83	0.78	0.84	0.87	0.72	0.96	0.12	0.93	783
0.32	0.69	0.73	0.73	0.68	0.78	0.05	0.76	0.68	0.73	0.72	0.66	0.79	0.07	0.77	0.68	0.76	0.79	0.60	0.92	0.16	0.88	2682


==> data/mlm_plots/tef/mr/lstmatt/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.22


==> data/mlm_plots/tef/mr/lstmatt/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.14	0.17	0.16	0.14	0.19	0.03	0.18	1.09	2.85	2.07	-0.04	5.73	2.89	3.53	0.94	3.83	2.48	-0.31	7.96	4.14	5.38	545
0.11	0.18	0.21	0.20	0.16	0.26	0.05	0.23	1.40	3.37	2.37	-0.62	7.36	3.99	3.89	1.10	4.16	2.92	-0.06	8.38	4.22	5.60	916
0.15	0.22	0.27	0.27	0.20	0.35	0.07	0.30	1.59	2.90	2.44	0.88	4.92	2.02	3.59	1.23	3.41	2.48	0.26	6.56	3.15	4.62	504
0.18	0.29	0.33	0.32	0.26	0.40	0.07	0.35	1.83	3.82	2.80	0.43	7.21	3.39	4.81	1.64	5.01	3.61	0.22	9.80	4.79	6.99	783
0.32	0.45	0.50	0.52	0.42	0.59	0.09	0.56	1.93	3.87	2.89	0.49	7.25	3.38	4.59	1.63	5.01	3.65	0.37	9.64	4.64	6.95	2682


==> data/mlm_plots/tef/mr/lstmatt/ig/time_misc_auc.tex <==
name	auc
attack_time	0.09
l2	0.92
lom	1.17


==> data/mlm_plots/tef/mr/lstmatt/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.29	0.00	-0.08	0.65	0.36	0.50	0.50	0.63	0.67	0.42	0.84	0.21	0.75	0.69	0.78	0.78	0.65	0.91	0.13	0.86	545
0.11	0.00	0.23	0.00	-0.11	0.57	0.34	0.50	0.43	0.55	0.57	0.33	0.76	0.22	0.71	0.67	0.73	0.75	0.60	0.87	0.14	0.83	916
0.15	0.00	0.20	0.00	-0.15	0.56	0.35	0.50	0.33	0.49	0.50	0.25	0.73	0.24	0.67	0.58	0.69	0.70	0.54	0.83	0.14	0.78	504
0.18	0.00	0.17	0.00	-0.13	0.46	0.30	0.50	0.29	0.44	0.43	0.23	0.65	0.21	0.57	0.57	0.65	0.67	0.51	0.80	0.14	0.77	783
0.32	0.00	0.12	0.00	-0.15	0.38	0.26	0.00	0.20	0.34	0.33	0.13	0.56	0.21	0.50	0.50	0.57	0.57	0.42	0.72	0.15	0.67	2682


==> data/mlm_plots/tef/mr/lstmatt/ig/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.12
top50	0.17


==> data/mlm_plots/tef/mr/lstmatt/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	102.87	206.98	173.02	58.87	355.08	148.10	265.86	3.00	4.48	4.00	2.21	6.75	2.27	6.00	151.94	294.16	233.22	82.55	505.78	211.61	364.74	3.00	4.77	4.00	2.43	7.11	2.34	6.00	538
0.11	99.67	235.25	174.88	-58.19	528.70	293.44	279.35	3.00	4.40	4.00	2.24	6.57	2.17	5.00	172.51	366.30	272.79	20.86	711.74	345.44	449.72	3.00	4.73	4.00	2.47	7.00	2.27	6.00	896
0.15	98.81	265.10	174.81	-36.28	566.48	301.38	310.32	2.00	3.94	3.00	1.85	6.02	2.09	5.00	199.18	490.54	319.84	-80.78	1061.86	571.32	553.28	3.00	4.28	4.00	2.05	6.51	2.23	5.00	509
0.18	101.27	221.60	177.40	46.10	397.10	175.50	281.74	3.00	4.27	4.00	2.16	6.38	2.11	5.00	237.22	480.07	373.13	92.21	867.92	387.86	593.21	3.00	4.81	4.00	2.55	7.08	2.27	6.00	772
0.32	105.18	241.70	179.25	-9.07	492.46	250.76	292.37	3.00	4.23	4.00	2.13	6.33	2.10	5.00	324.04	674.91	503.19	93.74	1256.09	581.18	824.69	3.00	4.95	5.00	2.66	7.24	2.29	6.00	2694


==> data/mlm_plots/tef/mr/lstmatt/s/comparison_vals_auc.tex <==
name	auc
orig_pp	61.00
orig_ge	1.10
adv_pp	129.09
adv_ge	1.23


==> data/mlm_plots/tef/mr/lstmatt/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.39	0.54	0.56	0.31	0.77	0.23	0.71	0.58	0.69	0.74	0.48	0.90	0.21	0.85	0.44	0.56	0.59	0.37	0.76	0.19	0.71	538
0.11	0.27	0.43	0.45	0.18	0.69	0.25	0.61	0.46	0.59	0.65	0.33	0.85	0.26	0.79	0.33	0.47	0.50	0.25	0.69	0.22	0.64	896
0.15	0.18	0.36	0.38	0.09	0.64	0.28	0.56	0.36	0.52	0.59	0.22	0.82	0.30	0.75	0.28	0.41	0.43	0.17	0.65	0.24	0.58	509
0.18	0.08	0.26	0.26	0.00	0.52	0.26	0.43	0.26	0.43	0.47	0.13	0.72	0.29	0.65	0.19	0.33	0.35	0.10	0.55	0.23	0.49	772
0.32	-0.09	0.09	0.07	-0.17	0.34	0.26	0.25	0.03	0.25	0.26	-0.07	0.57	0.32	0.48	0.02	0.18	0.18	-0.05	0.42	0.24	0.35	2694


==> data/mlm_plots/tef/mr/lstmatt/s/correlations_auc.tex <==
name	auc
pcc	0.07
spearman	0.12
kendall	0.09


==> data/mlm_plots/tef/mr/lstmatt/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	1.13	1.94	1.78	0.82	3.05	1.12	2.40	1.13	2.10	1.77	0.61	3.60	1.49	2.67	1.92	7.25	4.57	-0.01	14.52	7.26	10.42	538
0.11	1.21	1.91	1.78	0.90	2.91	1.01	2.43	1.12	1.99	1.72	0.74	3.25	1.26	2.56	1.84	7.40	3.94	-0.78	15.57	8.17	10.41	896
0.15	1.12	1.70	1.63	0.88	2.51	0.82	2.09	1.07	1.79	1.62	0.73	2.85	1.06	2.25	1.47	6.82	3.04	-2.55	16.18	9.37	8.22	509
0.18	1.29	1.83	1.73	1.03	2.62	0.79	2.28	1.22	1.88	1.73	0.92	2.83	0.96	2.32	1.63	5.02	2.91	-1.20	11.23	6.22	5.56	772
0.32	1.38	1.76	1.70	1.15	2.37	0.61	2.08	1.32	1.79	1.69	1.07	2.51	0.72	2.13	1.39	3.65	2.17	-1.23	8.53	4.88	3.77	2694


==> data/mlm_plots/tef/mr/lstmatt/s/ets_sts_auc.tex <==
name	auc
et_use	0.47
et_tse	0.49
et_ce	1.44


==> data/mlm_plots/tef/mr/lstmatt/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.25	2.17	0.51	-5.81	10.15	7.98	1.28	2.76	8.58	4.93	-2.36	19.52	10.94	9.34	2.67	17.68	5.99	-18.97	54.34	36.65	15.84	538
0.11	0.23	1.46	0.42	-3.15	6.07	4.61	1.00	2.63	7.66	4.78	-0.89	16.21	8.55	8.99	2.35	16.53	5.89	-18.48	51.54	35.01	14.29	896
0.15	0.17	1.73	0.34	-7.42	10.88	9.15	0.84	2.66	8.33	5.09	-2.24	18.89	10.56	8.87	2.31	21.32	6.34	-32.85	75.49	54.17	14.38	509
0.18	0.16	0.88	0.31	-2.41	4.16	3.28	0.68	2.77	6.64	4.57	-0.19	13.48	6.83	8.03	2.31	14.00	4.67	-19.49	47.49	33.49	11.19	772
0.32	0.12	0.99	0.24	-4.97	6.94	5.96	0.51	3.06	6.86	4.57	-1.03	14.75	7.89	7.71	2.52	13.53	4.54	-23.21	50.26	36.74	10.62	2694


==> data/mlm_plots/tef/mr/lstmatt/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.32
et_p_h	1.90
et_p_l2	4.10


==> data/mlm_plots/tef/mr/lstmatt/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.18	0.52	0.40	0.06	0.98	0.46	0.74	0.01	0.06	0.03	-0.00	0.11	0.06	0.08	0.02	0.05	0.04	0.01	0.10	0.04	0.08	538
0.11	0.26	0.82	0.58	-0.03	1.67	0.85	1.07	0.02	0.07	0.04	0.00	0.14	0.07	0.11	0.03	0.07	0.05	0.02	0.11	0.05	0.10	896
0.15	0.39	1.18	0.83	0.04	2.31	1.13	1.54	0.02	0.08	0.05	0.00	0.16	0.08	0.12	0.03	0.07	0.06	0.02	0.13	0.05	0.11	509
0.18	0.56	1.56	1.16	0.11	3.01	1.45	2.09	0.03	0.10	0.08	0.02	0.17	0.08	0.15	0.05	0.09	0.08	0.04	0.14	0.05	0.13	772
0.32	0.87	2.61	1.81	-0.16	5.38	2.77	3.37	0.04	0.12	0.10	0.03	0.20	0.09	0.18	0.06	0.10	0.10	0.05	0.16	0.06	0.15	2694


==> data/mlm_plots/tef/mr/lstmatt/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.40
pp_l2_d	0.02
pp_h_d	0.02


==> data/mlm_plots/tef/mr/lstmatt/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.85	0.87	0.87	0.83	0.91	0.04	0.90	0.83	0.87	0.87	0.81	0.93	0.06	0.91	0.89	0.92	0.95	0.84	1.00	0.08	0.98	538
0.11	0.82	0.84	0.84	0.80	0.88	0.04	0.87	0.80	0.84	0.84	0.78	0.90	0.06	0.88	0.87	0.90	0.93	0.81	1.00	0.10	0.98	896
0.15	0.78	0.80	0.81	0.76	0.85	0.05	0.83	0.76	0.80	0.81	0.74	0.87	0.06	0.85	0.80	0.87	0.91	0.76	0.99	0.12	0.96	509
0.18	0.76	0.79	0.78	0.74	0.83	0.05	0.82	0.74	0.78	0.79	0.71	0.85	0.07	0.83	0.79	0.85	0.87	0.74	0.96	0.11	0.93	772
0.32	0.69	0.73	0.73	0.68	0.78	0.05	0.76	0.68	0.73	0.73	0.66	0.79	0.07	0.77	0.69	0.77	0.79	0.61	0.92	0.15	0.88	2694


==> data/mlm_plots/tef/mr/lstmatt/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.20
sts_ce	0.22


==> data/mlm_plots/tef/mr/lstmatt/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.14	0.16	0.15	0.13	0.18	0.03	0.17	21.58	44.15	33.83	4.34	83.96	39.81	52.47	0.50	1.57	1.19	0.24	2.89	1.33	2.31	538
0.11	0.17	0.21	0.21	0.16	0.26	0.05	0.24	24.75	51.48	39.27	9.34	93.62	42.14	62.89	0.58	1.81	1.39	0.25	3.37	1.56	2.69	896
0.15	0.23	0.27	0.26	0.20	0.35	0.07	0.31	25.61	56.39	40.75	9.27	103.51	47.12	68.96	0.58	1.69	1.39	0.22	3.15	1.47	2.33	509
0.18	0.27	0.32	0.30	0.25	0.38	0.07	0.34	29.82	59.18	47.13	16.54	101.82	42.64	72.16	0.97	2.47	2.11	0.60	4.34	1.87	3.52	772
0.32	0.41	0.47	0.46	0.37	0.58	0.10	0.51	36.36	67.57	53.06	20.07	115.07	47.50	83.10	1.12	2.87	2.57	0.80	4.95	2.07	4.20	2694


==> data/mlm_plots/tef/mr/lstmatt/s/time_misc_auc.tex <==
name	auc
attack_time	0.08
l2	15.16
lom	0.59


==> data/mlm_plots/tef/mr/lstmatt/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.25	0.00	-0.09	0.60	0.34	0.50	0.50	0.62	0.67	0.44	0.81	0.19	0.71	0.69	0.78	0.77	0.65	0.90	0.12	0.85	538
0.11	0.00	0.19	0.00	-0.11	0.48	0.30	0.50	0.43	0.54	0.57	0.34	0.75	0.21	0.67	0.66	0.73	0.75	0.59	0.87	0.14	0.83	896
0.15	0.00	0.15	0.00	-0.15	0.44	0.30	0.00	0.33	0.49	0.50	0.27	0.71	0.22	0.67	0.58	0.70	0.70	0.54	0.86	0.16	0.83	509
0.18	0.00	0.10	0.00	-0.13	0.32	0.23	0.00	0.29	0.43	0.43	0.23	0.63	0.20	0.57	0.54	0.65	0.64	0.50	0.80	0.15	0.77	772
0.32	0.00	0.04	0.00	-0.11	0.19	0.15	0.00	0.14	0.32	0.33	0.11	0.53	0.21	0.43	0.50	0.58	0.60	0.43	0.74	0.16	0.69	2694


==> data/mlm_plots/tef/mr/lstmatt/s/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.12
top50	0.17


==> data/mlm_plots/tef/mr/roberta/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	51.66	123.50	87.75	0.81	246.18	122.69	154.61	1.00	1.83	1.00	0.48	3.18	1.35	2.00	82.72	179.53	125.11	10.21	348.85	169.32	211.15	1.00	2.03	2.00	0.66	3.39	1.36	3.00	380
0.11	50.80	120.99	83.02	-6.39	248.37	127.38	150.18	1.00	1.69	1.00	0.57	2.82	1.13	2.00	95.19	208.55	152.78	30.95	386.14	177.60	265.67	1.00	1.94	2.00	0.76	3.12	1.18	2.00	857
0.15	53.85	124.52	84.94	-7.79	256.83	132.31	142.55	1.00	1.72	1.00	0.68	2.76	1.04	2.00	118.52	245.32	184.45	39.56	451.08	205.76	305.51	1.00	2.05	2.00	0.88	3.21	1.16	3.00	885
0.18	50.80	123.21	83.07	-1.57	247.98	124.77	147.65	1.00	1.71	1.00	0.56	2.87	1.15	2.00	133.89	287.30	213.68	42.79	531.81	244.51	375.94	1.00	2.14	2.00	0.81	3.47	1.33	3.00	807
0.32	61.03	138.57	97.39	-3.99	281.12	142.56	167.31	1.00	1.71	1.00	0.59	2.83	1.12	2.00	205.15	441.52	335.31	30.82	852.23	410.71	533.17	1.00	2.25	2.00	0.92	3.58	1.33	3.00	2358


==> data/mlm_plots/tef/mr/roberta/a/comparison_vals_auc.tex <==
name	auc
orig_pp	33.03
orig_ge	0.45
adv_pp	77.46
adv_ge	0.55


==> data/mlm_plots/tef/mr/roberta/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.58	0.71	0.75	0.48	0.93	0.22	0.88	0.66	0.76	0.81	0.57	0.94	0.19	0.91	0.52	0.63	0.65	0.45	0.81	0.18	0.78	380
0.11	0.44	0.59	0.62	0.34	0.84	0.25	0.78	0.57	0.69	0.75	0.45	0.92	0.23	0.87	0.44	0.56	0.58	0.35	0.76	0.21	0.71	857
0.15	0.25	0.44	0.46	0.16	0.72	0.28	0.64	0.39	0.56	0.61	0.28	0.84	0.28	0.78	0.28	0.44	0.47	0.21	0.68	0.23	0.62	885
0.18	0.13	0.34	0.35	0.04	0.64	0.30	0.56	0.31	0.49	0.55	0.17	0.81	0.32	0.74	0.22	0.38	0.40	0.12	0.64	0.26	0.57	807
0.32	-0.02	0.18	0.18	-0.13	0.50	0.31	0.39	0.11	0.34	0.37	-0.03	0.71	0.37	0.64	0.07	0.26	0.28	-0.02	0.55	0.29	0.48	2358


==> data/mlm_plots/tef/mr/roberta/a/correlations_auc.tex <==
name	auc
pcc	0.10
spearman	0.14
kendall	0.11


==> data/mlm_plots/tef/mr/roberta/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	0.49	1.47	1.07	0.04	2.90	1.43	1.92	0.62	1.77	1.21	-0.18	3.72	1.95	2.25	0.91	5.13	2.78	-1.04	11.30	6.17	6.70	380
0.11	0.75	1.53	1.31	0.48	2.58	1.05	2.06	0.75	1.68	1.32	0.33	3.02	1.35	2.27	1.10	5.78	2.64	-1.75	13.31	7.53	6.93	857
0.15	1.02	1.68	1.52	0.73	2.64	0.95	2.22	1.03	1.82	1.60	0.70	2.95	1.12	2.38	1.46	5.83	2.83	-1.54	13.19	7.37	6.77	885
0.18	1.18	1.78	1.66	0.87	2.70	0.91	2.22	1.19	1.94	1.71	0.80	3.08	1.14	2.40	1.61	5.99	3.01	-1.86	13.83	7.84	7.19	807
0.32	1.25	1.76	1.68	0.97	2.54	0.78	2.17	1.28	1.88	1.76	0.95	2.81	0.93	2.32	1.37	4.46	2.39	-1.73	10.66	6.19	4.66	2358


==> data/mlm_plots/tef/mr/roberta/a/ets_sts_auc.tex <==
name	auc
et_use	0.44
et_tse	0.48
et_ce	1.42


==> data/mlm_plots/tef/mr/roberta/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.11	0.77	0.23	-1.57	3.10	2.33	0.66	1.24	5.40	2.66	-2.45	13.24	7.84	5.73	1.12	8.62	2.96	-11.19	28.43	19.81	8.19	380
0.11	0.11	0.95	0.24	-3.89	5.79	4.84	0.46	1.37	5.23	2.74	-2.18	12.64	7.41	5.72	1.32	9.07	2.90	-13.87	32.00	22.93	7.21	857
0.15	0.13	0.69	0.23	-4.09	5.47	4.78	0.51	1.84	5.75	3.32	-1.90	13.39	7.65	6.55	1.60	10.61	3.30	-14.49	35.72	25.10	9.42	885
0.18	0.12	0.67	0.21	-2.47	3.80	3.14	0.44	2.02	5.35	3.27	-1.51	12.20	6.86	5.77	1.75	9.13	2.80	-13.50	31.76	22.63	6.91	807
0.32	0.09	0.68	0.17	-4.72	6.08	5.40	0.35	2.33	5.33	3.57	-1.65	12.32	6.98	5.89	1.86	9.04	3.24	-15.38	33.45	24.41	6.94	2358


==> data/mlm_plots/tef/mr/roberta/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.19
et_p_h	1.40
et_p_l2	2.41


==> data/mlm_plots/tef/mr/roberta/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.22	0.58	0.47	0.11	1.05	0.47	0.84	0.01	0.07	0.03	-0.01	0.14	0.08	0.10	0.02	0.06	0.04	0.01	0.11	0.05	0.09	380
0.11	0.38	1.05	0.79	-0.07	2.18	1.12	1.37	0.02	0.09	0.06	0.00	0.18	0.09	0.14	0.03	0.08	0.06	0.02	0.14	0.06	0.12	857
0.15	0.54	1.44	1.06	-0.04	2.93	1.48	1.84	0.03	0.10	0.08	0.02	0.19	0.09	0.17	0.04	0.09	0.08	0.03	0.15	0.06	0.14	885
0.18	0.72	1.98	1.43	-0.94	4.90	2.92	2.65	0.05	0.12	0.10	0.03	0.21	0.09	0.19	0.05	0.10	0.10	0.04	0.16	0.06	0.15	807
0.32	1.06	3.12	2.30	-0.03	6.27	3.15	4.02	0.06	0.14	0.12	0.04	0.23	0.09	0.21	0.07	0.12	0.12	0.06	0.18	0.06	0.16	2358


==> data/mlm_plots/tef/mr/roberta/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.50
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/mr/roberta/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.87	0.89	0.89	0.85	0.92	0.04	0.91	0.86	0.89	0.90	0.84	0.95	0.05	0.93	0.90	0.92	0.96	0.84	1.01	0.09	0.99	380
0.11	0.83	0.86	0.86	0.82	0.90	0.04	0.88	0.82	0.85	0.86	0.79	0.92	0.06	0.90	0.86	0.90	0.93	0.79	1.01	0.11	0.98	857
0.15	0.79	0.82	0.83	0.78	0.87	0.05	0.86	0.79	0.83	0.84	0.77	0.89	0.06	0.88	0.83	0.88	0.92	0.78	0.99	0.11	0.96	885
0.18	0.78	0.81	0.80	0.76	0.85	0.05	0.83	0.77	0.81	0.81	0.75	0.88	0.06	0.86	0.82	0.86	0.90	0.74	0.99	0.13	0.96	807
0.32	0.72	0.76	0.76	0.71	0.81	0.05	0.79	0.72	0.77	0.77	0.70	0.83	0.07	0.81	0.73	0.81	0.84	0.67	0.95	0.14	0.91	2358


==> data/mlm_plots/tef/mr/roberta/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.22


==> data/mlm_plots/tef/mr/roberta/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.17	0.18	0.17	0.15	0.22	0.04	0.19	0.06	0.09	0.08	0.04	0.14	0.05	0.10	0.25	0.83	0.55	-0.04	1.70	0.87	1.09	380
0.11	0.18	0.22	0.20	0.15	0.29	0.07	0.24	0.08	0.12	0.11	0.06	0.19	0.07	0.15	0.39	1.30	0.80	-0.10	2.71	1.40	1.74	857
0.15	0.23	0.31	0.30	0.22	0.41	0.10	0.37	0.09	0.14	0.13	0.07	0.22	0.07	0.18	0.43	1.57	0.98	-0.06	3.20	1.63	2.22	885
0.18	0.31	0.38	0.36	0.29	0.46	0.08	0.43	0.10	0.16	0.14	0.08	0.23	0.07	0.19	0.54	1.68	1.18	0.07	3.29	1.61	2.35	807
0.32	0.42	0.47	0.47	0.40	0.54	0.07	0.52	0.13	0.18	0.17	0.10	0.27	0.08	0.23	0.64	2.12	1.47	0.07	4.17	2.05	2.85	2358


==> data/mlm_plots/tef/mr/roberta/a/time_misc_auc.tex <==
name	auc
attack_time	0.09
l2	0.04
lom	0.43


==> data/mlm_plots/tef/mr/roberta/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.39	0.00	-0.09	0.88	0.49	1.00	0.50	0.66	0.71	0.43	0.89	0.23	0.80	0.71	0.80	0.83	0.66	0.93	0.13	0.88	380
0.11	0.00	0.33	0.00	-0.09	0.76	0.42	0.50	0.50	0.60	0.60	0.37	0.84	0.23	0.80	0.67	0.77	0.78	0.62	0.92	0.15	0.89	857
0.15	0.00	0.21	0.00	-0.15	0.56	0.36	0.50	0.33	0.53	0.50	0.27	0.79	0.26	0.71	0.60	0.70	0.71	0.52	0.88	0.18	0.83	885
0.18	0.00	0.13	0.00	-0.16	0.42	0.29	0.00	0.25	0.46	0.50	0.19	0.73	0.27	0.67	0.57	0.67	0.70	0.48	0.85	0.18	0.80	807
0.32	0.00	0.09	0.00	-0.17	0.36	0.26	0.00	0.20	0.38	0.40	0.12	0.65	0.26	0.50	0.50	0.61	0.62	0.42	0.81	0.19	0.75	2358


==> data/mlm_plots/tef/mr/roberta/a/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.13
top50	0.18


==> data/mlm_plots/tef/mr/roberta/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	51.66	123.77	87.20	3.22	244.33	120.55	163.09	1.00	1.85	1.00	0.41	3.29	1.44	2.00	73.94	159.93	123.16	1.16	318.70	158.77	187.47	1.00	1.98	2.00	0.52	3.44	1.46	2.75	378
0.11	53.46	120.53	85.31	7.69	233.37	112.84	151.62	1.00	1.76	1.00	0.51	3.01	1.25	2.00	87.03	179.57	132.25	14.60	344.53	164.97	222.97	1.00	2.01	2.00	0.67	3.34	1.33	2.00	990
0.15	55.07	131.10	89.47	-13.03	275.23	144.13	161.14	1.00	1.75	1.00	0.61	2.90	1.15	2.00	103.48	217.91	171.90	40.81	395.01	177.10	276.72	1.00	2.10	2.00	0.82	3.39	1.28	3.00	1051
0.18	55.35	125.07	84.22	1.27	248.88	123.80	145.78	1.00	1.68	1.00	0.69	2.67	0.99	2.00	117.64	265.05	192.25	34.40	495.70	230.65	315.41	1.00	2.09	2.00	0.90	3.29	1.20	3.00	853
0.32	60.14	137.50	97.97	-4.25	279.24	141.74	169.40	1.00	1.65	1.00	0.60	2.71	1.06	2.00	175.64	362.37	278.70	43.76	680.98	318.61	450.97	1.00	2.17	2.00	0.89	3.45	1.28	3.00	2007


==> data/mlm_plots/tef/mr/roberta/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	33.36
orig_ge	0.45
adv_pp	67.38
adv_ge	0.54


==> data/mlm_plots/tef/mr/roberta/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	-0.07	0.17	0.19	-0.20	0.55	0.37	0.40	0.04	0.26	0.26	-0.06	0.57	0.32	0.48	0.04	0.20	0.21	-0.05	0.45	0.25	0.38	378
0.11	-0.31	-0.05	-0.05	-0.43	0.34	0.38	0.22	-0.16	0.07	0.09	-0.27	0.41	0.34	0.32	-0.11	0.06	0.07	-0.20	0.32	0.26	0.25	990
0.15	-0.45	-0.22	-0.22	-0.55	0.12	0.34	-0.01	-0.29	-0.08	-0.09	-0.40	0.23	0.31	0.12	-0.20	-0.06	-0.05	-0.29	0.18	0.24	0.10	1051
0.18	-0.52	-0.29	-0.30	-0.61	0.02	0.31	-0.10	-0.38	-0.16	-0.15	-0.46	0.14	0.30	0.05	-0.26	-0.11	-0.10	-0.34	0.12	0.23	0.05	853
0.32	-0.60	-0.41	-0.44	-0.69	-0.13	0.28	-0.23	-0.47	-0.28	-0.30	-0.56	-0.00	0.28	-0.10	-0.34	-0.21	-0.21	-0.43	0.01	0.22	-0.07	2007


==> data/mlm_plots/tef/mr/roberta/ig/correlations_auc.tex <==
name	auc
pcc	-0.06
spearman	-0.03
kendall	-0.02


==> data/mlm_plots/tef/mr/roberta/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	2.39	4.19	3.79	1.73	6.64	2.46	5.37	2.29	4.58	3.97	1.46	7.71	3.13	5.85	3.77	16.49	11.41	1.28	31.70	15.21	26.61	378
0.11	2.59	3.97	3.69	1.94	6.01	2.03	4.81	2.58	4.52	3.90	1.68	7.36	2.84	5.55	4.23	17.48	10.32	-0.47	35.43	17.95	24.73	990
0.15	2.70	3.75	3.58	2.11	5.38	1.64	4.47	2.72	4.18	3.50	1.96	6.40	2.22	5.15	3.90	15.13	7.83	-1.57	31.82	16.70	20.19	1051
0.18	2.72	3.56	3.33	2.12	4.99	1.44	4.14	2.64	3.86	3.41	1.98	5.73	1.87	4.52	3.04	11.95	6.14	-2.34	26.25	14.30	13.68	853
0.32	2.56	3.19	3.02	2.11	4.27	1.08	3.63	2.54	3.45	3.13	1.94	4.96	1.51	3.99	2.94	9.29	5.01	-2.80	21.38	12.09	9.95	2007


==> data/mlm_plots/tef/mr/roberta/ig/ets_sts_auc.tex <==
name	auc
et_use	0.94
et_tse	1.03
et_ce	3.41


==> data/mlm_plots/tef/mr/roberta/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.53	3.86	1.10	-9.56	17.27	13.42	3.19	4.54	17.63	9.92	-2.08	37.35	19.72	22.35	4.50	26.51	11.93	-14.81	67.83	41.32	30.54	378
0.11	0.48	3.85	0.96	-11.67	19.36	15.52	2.34	4.69	14.72	8.58	-3.33	32.76	18.04	17.97	4.09	22.29	9.33	-21.76	66.35	44.06	21.39	990
0.15	0.41	2.45	0.82	-5.90	10.80	8.35	1.87	4.51	14.32	9.20	-2.75	31.40	17.07	16.10	3.74	22.91	8.81	-15.99	61.81	38.90	21.19	1051
0.18	0.30	3.03	0.57	-19.10	25.16	22.13	1.17	4.56	11.28	7.72	0.44	22.12	10.84	12.97	3.76	18.29	7.23	-23.14	59.72	41.43	16.61	853
0.32	0.22	1.72	0.40	-9.36	12.81	11.09	0.87	4.50	10.49	6.47	-3.06	24.03	13.55	11.43	3.61	16.23	6.29	-24.06	56.52	40.29	14.21	2007


==> data/mlm_plots/tef/mr/roberta/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.73
et_p_h	3.30
et_p_l2	5.17


==> data/mlm_plots/tef/mr/roberta/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.13	0.42	0.29	0.04	0.80	0.38	0.59	0.01	0.06	0.03	-0.01	0.12	0.07	0.07	0.02	0.05	0.03	0.01	0.10	0.05	0.07	378
0.11	0.22	0.74	0.52	-0.07	1.55	0.81	1.01	0.02	0.08	0.05	0.00	0.16	0.08	0.12	0.03	0.07	0.05	0.02	0.13	0.05	0.10	990
0.15	0.34	1.10	0.72	-0.22	2.42	1.32	1.37	0.03	0.10	0.07	0.01	0.18	0.09	0.15	0.04	0.08	0.07	0.03	0.14	0.06	0.13	1051
0.18	0.53	1.57	1.16	-0.01	3.15	1.58	2.04	0.04	0.11	0.08	0.02	0.19	0.08	0.16	0.05	0.09	0.08	0.04	0.15	0.06	0.14	853
0.32	0.80	2.48	1.68	-0.24	5.20	2.72	3.19	0.05	0.13	0.11	0.04	0.22	0.09	0.20	0.06	0.11	0.10	0.05	0.17	0.06	0.16	2007


==> data/mlm_plots/tef/mr/roberta/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.39
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/tef/mr/roberta/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.87	0.89	0.89	0.85	0.93	0.04	0.91	0.86	0.89	0.90	0.84	0.94	0.05	0.93	0.91	0.93	0.97	0.85	1.01	0.08	0.99	378
0.11	0.83	0.86	0.86	0.82	0.89	0.04	0.88	0.83	0.86	0.87	0.80	0.92	0.06	0.90	0.89	0.92	0.95	0.83	1.01	0.09	0.98	990
0.15	0.80	0.83	0.83	0.78	0.87	0.04	0.86	0.79	0.83	0.84	0.77	0.89	0.06	0.88	0.85	0.89	0.92	0.79	1.00	0.10	0.97	1051
0.18	0.78	0.81	0.80	0.76	0.85	0.04	0.83	0.77	0.81	0.81	0.75	0.87	0.06	0.86	0.80	0.86	0.90	0.74	0.98	0.12	0.95	853
0.32	0.73	0.77	0.77	0.72	0.82	0.05	0.80	0.73	0.78	0.78	0.71	0.84	0.06	0.82	0.77	0.83	0.86	0.71	0.96	0.12	0.93	2007


==> data/mlm_plots/tef/mr/roberta/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.23


==> data/mlm_plots/tef/mr/roberta/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.34	0.40	0.37	0.30	0.49	0.10	0.41	1.66	6.27	3.74	-0.86	13.39	7.13	8.01	1.48	4.39	3.33	0.66	8.11	3.72	6.37	378
0.11	0.37	0.47	0.45	0.33	0.62	0.15	0.54	2.51	9.83	5.22	-4.71	24.37	14.54	11.47	1.71	4.83	3.77	0.86	8.81	3.98	7.12	990
0.15	0.37	0.49	0.45	0.31	0.68	0.18	0.54	2.80	9.81	5.08	-17.38	37.00	27.19	10.37	1.98	5.21	3.99	1.15	9.28	4.07	7.79	1051
0.18	0.35	0.46	0.38	0.25	0.66	0.21	0.44	2.80	9.44	5.38	-6.59	25.48	16.03	11.27	1.83	5.12	4.04	0.96	9.28	4.16	7.27	853
0.32	0.42	0.64	0.46	0.35	0.93	0.29	0.96	3.29	9.73	6.24	-5.08	24.54	14.81	11.48	2.01	5.41	4.46	1.15	9.67	4.26	7.83	2007


==> data/mlm_plots/tef/mr/roberta/ig/time_misc_auc.tex <==
name	auc
attack_time	0.13
l2	2.44
lom	1.32


==> data/mlm_plots/tef/mr/roberta/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.20	0.00	-0.20	0.59	0.40	0.00	0.25	0.42	0.40	0.19	0.65	0.23	0.60	0.50	0.58	0.59	0.42	0.74	0.16	0.67	378
0.11	0.00	0.12	0.00	-0.17	0.42	0.30	0.00	0.17	0.33	0.33	0.11	0.55	0.22	0.50	0.44	0.53	0.50	0.37	0.69	0.16	0.64	990
0.15	0.00	0.06	0.00	-0.15	0.27	0.21	0.00	0.00	0.25	0.25	0.05	0.46	0.21	0.40	0.36	0.48	0.50	0.33	0.63	0.15	0.57	1051
0.18	0.00	0.04	0.00	-0.12	0.19	0.16	0.00	0.00	0.23	0.25	0.04	0.42	0.19	0.33	0.38	0.44	0.45	0.28	0.61	0.16	0.55	853
0.32	0.00	0.03	0.00	-0.12	0.17	0.14	0.00	0.00	0.17	0.17	-0.01	0.35	0.18	0.33	0.33	0.40	0.40	0.25	0.54	0.15	0.50	2007


==> data/mlm_plots/tef/mr/roberta/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.07
top50	0.12


==> data/mlm_plots/tef/mr/roberta/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	52.02	122.78	90.09	18.86	226.70	103.92	153.77	1.00	1.84	1.00	0.50	3.18	1.34	2.00	85.31	181.04	134.52	21.73	340.35	159.31	223.01	1.00	1.98	2.00	0.61	3.34	1.36	3.00	401
0.11	50.86	117.29	82.24	0.58	233.99	116.70	143.72	1.00	1.69	1.00	0.62	2.76	1.07	2.00	92.16	206.45	148.74	10.87	402.02	195.58	245.24	1.00	1.91	2.00	0.74	3.08	1.17	2.00	921
0.15	55.60	126.91	85.65	-14.99	268.81	141.90	155.20	1.00	1.79	1.00	0.66	2.92	1.13	2.00	113.68	253.25	179.69	2.59	503.91	250.66	298.53	1.00	2.06	2.00	0.83	3.29	1.23	3.00	911
0.18	53.47	117.53	85.35	17.44	217.61	100.08	146.59	1.00	1.73	1.00	0.58	2.89	1.15	2.00	127.75	273.15	208.13	73.38	472.93	199.77	356.34	1.00	2.12	2.00	0.81	3.44	1.32	3.00	840
0.32	60.73	134.52	97.64	13.07	255.98	121.45	167.17	1.00	1.69	1.00	0.56	2.82	1.13	2.00	192.91	409.79	311.65	29.23	790.35	380.56	502.99	1.00	2.24	2.00	0.88	3.59	1.36	3.00	2231


==> data/mlm_plots/tef/mr/roberta/s/comparison_vals_auc.tex <==
name	auc
orig_pp	32.19
orig_ge	0.45
adv_pp	74.37
adv_ge	0.54


==> data/mlm_plots/tef/mr/roberta/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.46	0.62	0.65	0.36	0.87	0.26	0.84	0.59	0.69	0.74	0.47	0.91	0.22	0.86	0.43	0.56	0.58	0.36	0.76	0.20	0.71	401
0.11	0.28	0.49	0.52	0.20	0.77	0.28	0.71	0.46	0.60	0.65	0.35	0.85	0.25	0.79	0.33	0.47	0.50	0.26	0.68	0.21	0.63	921
0.15	0.14	0.34	0.35	0.06	0.61	0.28	0.55	0.25	0.45	0.49	0.15	0.74	0.30	0.67	0.18	0.34	0.34	0.10	0.57	0.23	0.51	911
0.18	0.04	0.23	0.23	-0.06	0.52	0.29	0.45	0.15	0.36	0.40	0.02	0.70	0.34	0.60	0.11	0.27	0.31	0.01	0.53	0.26	0.45	840
0.32	-0.10	0.11	0.09	-0.18	0.39	0.28	0.30	0.00	0.24	0.26	-0.11	0.59	0.35	0.50	-0.00	0.18	0.19	-0.08	0.44	0.26	0.35	2231


==> data/mlm_plots/tef/mr/roberta/s/correlations_auc.tex <==
name	auc
pcc	0.08
spearman	0.11
kendall	0.08


==> data/mlm_plots/tef/mr/roberta/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	0.78	1.98	1.60	0.36	3.60	1.62	2.74	0.84	2.50	1.86	0.07	4.94	2.44	3.27	1.52	8.03	4.15	-1.36	17.43	9.40	11.55	401
0.11	0.94	1.93	1.67	0.60	3.26	1.33	2.59	1.02	2.18	1.76	0.31	4.05	1.87	2.85	1.48	7.14	3.61	-1.57	15.85	8.71	8.79	921
0.15	1.27	2.12	1.93	0.86	3.38	1.26	2.60	1.30	2.39	1.98	0.60	4.18	1.79	2.95	1.85	7.28	3.93	-1.13	15.69	8.41	9.24	911
0.18	1.34	2.12	1.89	0.96	3.28	1.16	2.58	1.38	2.35	2.02	0.81	3.89	1.54	2.86	1.70	7.26	3.38	-1.81	16.33	9.07	8.43	840
0.32	1.45	1.99	1.91	1.12	2.86	0.87	2.34	1.49	2.18	1.97	1.07	3.28	1.10	2.58	1.75	5.20	2.86	-1.57	11.97	6.77	5.13	2231


==> data/mlm_plots/tef/mr/roberta/s/ets_sts_auc.tex <==
name	auc
et_use	0.53
et_tse	0.60
et_ce	1.76


==> data/mlm_plots/tef/mr/roberta/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.16	1.06	0.36	-1.74	3.86	2.80	0.77	1.75	6.33	3.66	-2.49	15.16	8.82	7.12	1.64	9.65	3.79	-8.77	28.07	18.42	10.51	401
0.11	0.16	0.96	0.32	-2.18	4.10	3.14	0.68	1.84	6.57	3.73	-2.08	15.23	8.65	7.28	1.55	10.34	3.81	-10.42	31.09	20.75	10.63	921
0.15	0.17	0.87	0.30	-1.54	3.28	2.41	0.61	2.21	7.12	3.94	-1.79	16.03	8.91	7.85	1.73	12.52	3.94	-15.87	40.91	28.39	10.65	911
0.18	0.13	1.29	0.27	-5.68	8.27	6.97	0.55	2.43	6.50	3.95	-1.84	14.85	8.34	6.89	2.07	11.42	3.69	-19.40	42.24	30.82	8.44	840
0.32	0.11	0.73	0.22	-2.54	4.01	3.28	0.45	2.62	5.90	3.92	-1.04	12.84	6.94	6.45	2.18	8.96	3.61	-10.89	28.82	19.86	7.69	2231


==> data/mlm_plots/tef/mr/roberta/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.26
et_p_h	1.67
et_p_l2	2.76


==> data/mlm_plots/tef/mr/roberta/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.21	0.58	0.46	0.10	1.05	0.48	0.82	0.02	0.07	0.03	-0.01	0.14	0.07	0.10	0.02	0.06	0.04	0.01	0.11	0.05	0.09	401
0.11	0.33	1.03	0.68	-0.22	2.29	1.26	1.32	0.02	0.09	0.05	0.00	0.17	0.08	0.14	0.03	0.08	0.06	0.02	0.14	0.06	0.12	921
0.15	0.52	1.34	1.03	0.11	2.58	1.24	1.76	0.03	0.11	0.08	0.02	0.20	0.09	0.18	0.04	0.09	0.08	0.03	0.15	0.06	0.14	911
0.18	0.65	1.98	1.40	-0.30	4.25	2.27	2.37	0.04	0.12	0.09	0.02	0.21	0.09	0.19	0.05	0.10	0.10	0.04	0.17	0.06	0.15	840
0.32	0.99	2.99	2.01	-0.90	6.88	3.89	3.47	0.05	0.14	0.12	0.04	0.23	0.09	0.21	0.06	0.12	0.11	0.06	0.18	0.06	0.16	2231


==> data/mlm_plots/tef/mr/roberta/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.48
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/mr/roberta/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.87	0.89	0.89	0.86	0.93	0.04	0.92	0.87	0.90	0.92	0.86	0.95	0.05	0.94	0.92	0.93	0.97	0.86	1.01	0.08	0.99	401
0.11	0.83	0.86	0.85	0.82	0.89	0.04	0.88	0.82	0.86	0.86	0.80	0.92	0.06	0.90	0.86	0.90	0.94	0.81	1.00	0.10	0.98	921
0.15	0.80	0.83	0.83	0.79	0.87	0.04	0.86	0.80	0.84	0.84	0.78	0.89	0.06	0.88	0.83	0.89	0.92	0.78	0.99	0.11	0.97	911
0.18	0.77	0.80	0.80	0.76	0.85	0.05	0.83	0.77	0.81	0.81	0.75	0.87	0.06	0.85	0.80	0.86	0.89	0.74	0.98	0.12	0.95	840
0.32	0.73	0.76	0.76	0.71	0.81	0.05	0.79	0.73	0.77	0.78	0.71	0.84	0.06	0.82	0.76	0.82	0.84	0.70	0.95	0.12	0.92	2231


==> data/mlm_plots/tef/mr/roberta/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.23


==> data/mlm_plots/tef/mr/roberta/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.12	0.15	0.14	0.10	0.19	0.05	0.15	6.31	63.26	13.35	-140.67	267.19	203.93	34.27	0.32	0.76	0.61	0.17	1.35	0.59	1.06	401
0.11	0.14	0.20	0.18	0.12	0.29	0.09	0.22	7.51	106.69	21.67	-202.43	415.82	309.13	77.17	0.36	1.00	0.74	0.08	1.93	0.93	1.37	921
0.15	0.21	0.32	0.36	0.21	0.42	0.10	0.40	10.30	113.42	26.42	-217.19	444.03	330.61	79.78	0.40	1.19	0.93	0.14	2.23	1.04	1.65	911
0.18	0.38	0.40	0.40	0.36	0.44	0.04	0.43	14.36	122.15	36.69	-147.99	392.29	270.14	105.66	0.48	1.39	1.12	0.23	2.55	1.16	2.06	840
0.32	0.38	0.41	0.41	0.37	0.46	0.05	0.44	16.95	128.47	41.86	-132.57	389.51	261.04	139.35	0.53	1.48	1.24	0.29	2.67	1.19	2.11	2231


==> data/mlm_plots/tef/mr/roberta/s/time_misc_auc.tex <==
name	auc
attack_time	0.09
l2	29.82
lom	0.33


==> data/mlm_plots/tef/mr/roberta/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.33	0.00	-0.14	0.79	0.47	1.00	0.50	0.64	0.67	0.43	0.85	0.21	0.80	0.67	0.77	0.78	0.64	0.90	0.13	0.88	401
0.11	0.00	0.22	0.00	-0.14	0.57	0.35	0.50	0.43	0.57	0.60	0.36	0.79	0.22	0.67	0.64	0.73	0.75	0.59	0.88	0.15	0.82	921
0.15	0.00	0.13	0.00	-0.16	0.42	0.29	0.00	0.33	0.45	0.50	0.20	0.70	0.25	0.67	0.57	0.66	0.67	0.50	0.82	0.16	0.75	911
0.18	0.00	0.09	0.00	-0.15	0.34	0.24	0.00	0.25	0.42	0.40	0.17	0.67	0.25	0.60	0.50	0.62	0.62	0.45	0.80	0.17	0.75	840
0.32	0.00	0.05	0.00	-0.14	0.24	0.19	0.00	0.17	0.33	0.33	0.09	0.58	0.25	0.50	0.50	0.58	0.60	0.41	0.76	0.18	0.70	2231


==> data/mlm_plots/tef/mr/roberta/s/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.12
top50	0.17


==> data/mlm_plots/tef/mr/xlnet/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	55.39	130.46	98.46	5.12	255.81	125.35	155.80	1.00	1.69	1.00	0.73	2.65	0.96	2.00	82.75	173.63	135.08	21.31	325.94	152.32	209.63	1.00	1.84	2.00	0.82	2.86	1.02	2.00	541
0.11	50.72	124.98	86.23	-8.09	258.04	133.06	150.55	1.00	1.57	1.00	0.64	2.51	0.94	2.00	85.84	194.66	145.04	27.35	361.98	167.31	256.48	1.00	1.81	2.00	0.79	2.83	1.02	2.00	948
0.15	50.88	120.79	82.88	8.93	232.65	111.86	149.64	1.00	1.54	1.00	0.69	2.39	0.85	2.00	114.25	245.95	177.81	31.45	460.45	214.50	303.07	1.00	1.87	2.00	0.89	2.85	0.98	2.00	941
0.18	56.74	124.08	92.92	14.24	233.91	109.84	157.38	1.00	1.58	1.00	0.68	2.48	0.90	2.00	134.23	279.64	209.62	38.60	520.68	241.04	339.12	1.00	2.00	2.00	0.95	3.04	1.05	3.00	847
0.32	63.10	149.00	107.22	-5.06	303.06	154.06	175.74	1.00	1.63	1.00	0.68	2.58	0.95	2.00	185.05	421.62	308.44	33.57	809.67	388.05	506.26	1.00	2.11	2.00	0.96	3.26	1.15	3.00	1985


==> data/mlm_plots/tef/mr/xlnet/a/comparison_vals_auc.tex <==
name	auc
orig_pp	33.99
orig_ge	0.41
adv_pp	74.73
adv_ge	0.51


==> data/mlm_plots/tef/mr/xlnet/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.45	0.63	0.71	0.33	0.93	0.30	0.88	0.57	0.70	0.78	0.44	0.95	0.26	0.88	0.43	0.57	0.62	0.34	0.80	0.23	0.73	541
0.11	0.23	0.47	0.51	0.12	0.82	0.35	0.78	0.40	0.58	0.69	0.26	0.90	0.32	0.83	0.29	0.47	0.51	0.20	0.74	0.27	0.67	948
0.15	0.03	0.33	0.33	-0.05	0.70	0.38	0.64	0.19	0.45	0.55	0.08	0.82	0.37	0.75	0.14	0.36	0.41	0.06	0.66	0.30	0.60	941
0.18	-0.03	0.22	0.23	-0.14	0.59	0.36	0.50	0.09	0.36	0.43	-0.03	0.75	0.39	0.67	0.07	0.28	0.31	-0.03	0.58	0.30	0.51	847
0.32	-0.21	0.06	0.02	-0.30	0.43	0.37	0.30	-0.13	0.19	0.21	-0.23	0.61	0.42	0.53	-0.08	0.15	0.15	-0.17	0.46	0.32	0.38	1985


==> data/mlm_plots/tef/mr/xlnet/a/correlations_auc.tex <==
name	auc
pcc	0.07
spearman	0.10
kendall	0.08


==> data/mlm_plots/tef/mr/xlnet/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	0.55	1.70	1.35	0.21	3.19	1.49	2.37	0.53	1.91	1.29	-0.08	3.91	2.00	2.50	1.12	6.20	3.10	-1.52	13.92	7.72	8.35	541
0.11	0.77	1.86	1.55	0.30	3.42	1.56	2.61	0.74	1.96	1.56	0.26	3.66	1.70	2.67	0.99	6.94	2.67	-3.26	17.15	10.20	8.10	948
0.15	1.03	1.97	1.82	0.74	3.21	1.24	2.73	1.02	2.09	1.89	0.66	3.52	1.43	2.88	1.46	7.65	3.64	-2.97	18.27	10.62	8.56	941
0.18	1.21	2.00	1.93	0.92	3.09	1.08	2.65	1.20	2.07	1.86	0.83	3.31	1.24	2.66	1.53	6.54	3.10	-3.00	16.08	9.54	6.66	847
0.32	1.44	2.05	2.00	1.08	3.02	0.97	2.55	1.48	2.15	2.06	1.05	3.25	1.10	2.70	1.59	5.11	2.67	-2.34	12.56	7.45	5.06	1985


==> data/mlm_plots/tef/mr/xlnet/a/ets_sts_auc.tex <==
name	auc
et_use	0.51
et_tse	0.54
et_ce	1.66


==> data/mlm_plots/tef/mr/xlnet/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.14	1.94	0.40	-9.85	13.73	11.79	0.90	1.28	8.45	3.36	-6.31	23.22	14.77	9.45	1.23	13.34	3.54	-19.79	46.46	33.13	11.87	541
0.11	0.14	1.37	0.35	-2.44	5.17	3.81	0.97	1.60	8.01	3.78	-4.52	20.55	12.54	8.43	1.55	16.13	3.62	-28.53	60.79	44.66	10.35	948
0.15	0.13	1.06	0.30	-2.86	4.99	3.93	0.71	2.13	7.23	3.97	-5.22	19.68	12.45	7.62	1.86	10.65	3.80	-12.55	33.85	23.20	10.84	941
0.18	0.15	1.29	0.31	-6.45	9.04	7.75	0.75	2.25	7.22	3.93	-2.48	16.92	9.70	8.25	1.98	10.58	3.80	-8.29	29.44	18.87	10.18	847
0.32	0.12	0.92	0.25	-2.48	4.32	3.40	0.59	2.81	7.41	4.53	-3.49	18.30	10.90	7.93	2.38	12.56	4.26	-17.64	42.76	30.20	10.03	1985


==> data/mlm_plots/tef/mr/xlnet/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.32
et_p_h	1.95
et_p_l2	3.20


==> data/mlm_plots/tef/mr/xlnet/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.15	0.56	0.38	-0.02	1.14	0.58	0.74	0.01	0.07	0.03	-0.02	0.15	0.08	0.08	0.02	0.06	0.03	0.00	0.12	0.06	0.08	541
0.11	0.23	0.91	0.61	-0.19	2.01	1.10	1.17	0.02	0.08	0.05	0.00	0.16	0.08	0.11	0.03	0.07	0.06	0.02	0.13	0.06	0.11	948
0.15	0.41	1.53	0.96	-0.30	3.37	1.83	2.03	0.03	0.10	0.07	0.01	0.19	0.09	0.17	0.04	0.09	0.08	0.03	0.15	0.06	0.14	941
0.18	0.45	1.84	1.22	-0.61	4.28	2.44	2.18	0.03	0.11	0.09	0.02	0.21	0.09	0.18	0.05	0.10	0.09	0.04	0.16	0.06	0.15	847
0.32	0.80	2.80	1.78	-1.24	6.84	4.04	3.44	0.04	0.13	0.10	0.03	0.22	0.10	0.20	0.06	0.11	0.10	0.05	0.17	0.06	0.16	1985


==> data/mlm_plots/tef/mr/xlnet/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.46
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/tef/mr/xlnet/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.85	0.88	0.88	0.84	0.92	0.04	0.91	0.84	0.88	0.89	0.82	0.94	0.06	0.92	0.90	0.93	0.96	0.84	1.01	0.09	0.98	541
0.11	0.81	0.84	0.84	0.80	0.89	0.05	0.88	0.80	0.84	0.85	0.78	0.91	0.06	0.89	0.84	0.89	0.93	0.78	1.00	0.11	0.97	948
0.15	0.79	0.82	0.82	0.78	0.87	0.05	0.85	0.78	0.82	0.82	0.76	0.88	0.06	0.86	0.82	0.88	0.91	0.76	1.00	0.12	0.97	941
0.18	0.77	0.80	0.80	0.75	0.84	0.05	0.83	0.75	0.80	0.80	0.73	0.86	0.06	0.84	0.79	0.85	0.88	0.72	0.98	0.13	0.95	847
0.32	0.73	0.76	0.76	0.71	0.81	0.05	0.79	0.72	0.77	0.77	0.70	0.83	0.06	0.81	0.74	0.81	0.83	0.68	0.94	0.13	0.91	1985


==> data/mlm_plots/tef/mr/xlnet/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.22


==> data/mlm_plots/tef/mr/xlnet/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.20	0.26	0.21	0.14	0.38	0.12	0.27	0.05	0.10	0.09	0.03	0.17	0.07	0.13	0.41	1.60	0.99	-0.09	3.29	1.69	2.16	541
0.11	0.24	0.35	0.32	0.21	0.49	0.14	0.40	0.07	0.13	0.11	0.05	0.21	0.08	0.17	0.58	2.11	1.30	-0.05	4.26	2.16	3.00	948
0.15	0.34	0.43	0.39	0.30	0.56	0.13	0.49	0.09	0.16	0.13	0.06	0.25	0.10	0.20	0.69	2.59	1.72	0.13	5.06	2.46	3.78	941
0.18	0.38	0.49	0.47	0.36	0.62	0.13	0.59	0.10	0.16	0.15	0.07	0.26	0.09	0.21	0.69	2.61	1.76	0.11	5.11	2.50	3.74	847
0.32	0.55	0.62	0.62	0.52	0.73	0.10	0.68	0.12	0.19	0.17	0.10	0.28	0.09	0.23	0.85	2.95	2.24	0.37	5.52	2.58	4.41	1985


==> data/mlm_plots/tef/mr/xlnet/a/time_misc_auc.tex <==
name	auc
attack_time	0.12
l2	0.04
lom	0.66


==> data/mlm_plots/tef/mr/xlnet/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.35	0.00	-0.12	0.83	0.48	1.00	0.50	0.63	0.67	0.37	0.88	0.26	0.80	0.67	0.77	0.78	0.60	0.93	0.16	0.88	541
0.11	0.00	0.26	0.00	-0.15	0.68	0.42	0.50	0.33	0.55	0.50	0.29	0.81	0.26	0.72	0.60	0.72	0.75	0.55	0.89	0.17	0.83	948
0.15	0.00	0.20	0.00	-0.18	0.58	0.38	0.00	0.25	0.47	0.50	0.19	0.75	0.28	0.67	0.56	0.66	0.67	0.48	0.85	0.18	0.80	941
0.18	0.00	0.14	0.00	-0.18	0.45	0.32	0.00	0.25	0.41	0.33	0.14	0.68	0.27	0.60	0.50	0.62	0.60	0.43	0.81	0.19	0.75	847
0.32	0.00	0.08	0.00	-0.18	0.35	0.27	0.00	0.00	0.31	0.25	0.04	0.57	0.27	0.50	0.43	0.55	0.56	0.35	0.75	0.20	0.67	1985


==> data/mlm_plots/tef/mr/xlnet/a/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.11
top50	0.17


==> data/mlm_plots/tef/mr/xlnet/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	57.59	126.58	95.62	10.38	242.78	116.20	148.65	1.00	1.67	1.00	0.72	2.62	0.95	2.00	81.29	164.70	124.01	25.68	303.72	139.02	205.71	1.00	1.80	2.00	0.81	2.78	0.98	2.00	516
0.11	52.15	125.99	86.82	-12.18	264.17	138.18	148.27	1.00	1.55	1.00	0.70	2.39	0.84	2.00	89.35	195.31	138.77	3.25	387.37	192.06	235.30	1.00	1.75	2.00	0.80	2.69	0.94	2.00	916
0.15	57.10	133.51	94.27	-1.00	268.02	134.51	164.14	1.00	1.62	1.00	0.68	2.55	0.94	2.00	116.03	252.70	185.42	36.18	469.21	216.51	303.49	1.00	1.87	2.00	0.79	2.96	1.08	2.00	1004
0.18	53.91	123.76	93.17	13.24	234.28	110.52	154.71	1.00	1.60	1.00	0.72	2.49	0.88	2.00	125.88	267.12	195.89	43.90	490.33	223.22	330.70	1.00	1.93	2.00	0.91	2.95	1.02	2.75	886
0.32	62.33	151.85	106.53	-6.32	310.01	158.16	181.60	1.00	1.63	1.00	0.65	2.60	0.98	2.00	184.31	431.09	304.09	14.48	847.69	416.60	517.04	1.00	2.08	2.00	0.94	3.22	1.14	3.00	1971


==> data/mlm_plots/tef/mr/xlnet/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	34.63
orig_ge	0.42
adv_pp	74.41
adv_ge	0.50


==> data/mlm_plots/tef/mr/xlnet/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.15	0.37	0.39	0.03	0.71	0.34	0.64	0.19	0.38	0.40	0.08	0.67	0.30	0.60	0.13	0.29	0.30	0.06	0.52	0.23	0.45	516
0.11	-0.10	0.16	0.18	-0.23	0.55	0.39	0.44	-0.03	0.20	0.22	-0.15	0.54	0.35	0.45	-0.02	0.15	0.16	-0.12	0.42	0.27	0.33	916
0.15	-0.25	-0.01	-0.03	-0.35	0.34	0.35	0.23	-0.18	0.04	0.02	-0.29	0.36	0.32	0.26	-0.14	0.03	0.02	-0.21	0.27	0.24	0.19	1004
0.18	-0.33	-0.09	-0.14	-0.45	0.26	0.35	0.13	-0.25	-0.04	-0.05	-0.35	0.27	0.31	0.15	-0.18	-0.02	-0.03	-0.26	0.21	0.24	0.12	886
0.32	-0.50	-0.27	-0.31	-0.59	0.05	0.32	-0.09	-0.42	-0.21	-0.23	-0.52	0.11	0.31	-0.02	-0.31	-0.15	-0.16	-0.39	0.09	0.24	-0.01	1971


==> data/mlm_plots/tef/mr/xlnet/ig/correlations_auc.tex <==
name	auc
pcc	-0.01
spearman	0.00
kendall	0.00


==> data/mlm_plots/tef/mr/xlnet/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	1.49	3.01	2.54	0.95	5.07	2.06	4.09	1.54	3.45	2.53	0.63	6.27	2.82	4.58	2.94	12.28	7.84	0.01	24.56	12.27	18.59	516
0.11	1.91	2.95	2.74	1.25	4.65	1.70	3.67	1.69	3.06	2.58	0.82	5.30	2.24	3.89	2.04	10.58	5.07	-1.90	23.06	12.48	14.90	916
0.15	2.05	2.96	2.73	1.51	4.41	1.45	3.62	2.02	3.17	2.83	1.39	4.95	1.78	3.91	2.40	11.01	5.62	-1.73	23.75	12.74	14.28	1004
0.18	2.06	2.84	2.73	1.58	4.09	1.25	3.41	2.08	2.97	2.72	1.41	4.52	1.56	3.46	2.34	8.70	4.28	-2.29	19.69	10.99	9.77	886
0.32	2.15	2.78	2.71	1.80	3.75	0.97	3.23	2.21	2.95	2.76	1.75	4.14	1.19	3.46	2.28	7.04	3.79	-2.07	16.16	9.12	7.37	1971


==> data/mlm_plots/tef/mr/xlnet/ig/ets_sts_auc.tex <==
name	auc
et_use	0.75
et_tse	0.79
et_ce	2.41


==> data/mlm_plots/tef/mr/xlnet/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.39	3.61	0.91	-9.26	16.47	12.86	2.14	3.39	13.55	7.70	-0.84	27.94	14.39	19.56	3.49	20.35	8.17	-13.91	54.62	34.26	26.22	516
0.11	0.31	2.87	0.62	-7.44	13.19	10.32	1.60	4.09	13.07	7.24	-3.94	30.09	17.02	14.99	3.44	22.01	8.27	-28.11	72.13	50.12	18.70	916
0.15	0.27	2.27	0.51	-7.64	12.18	9.91	1.18	4.24	11.82	7.76	-0.37	24.01	12.19	14.78	3.35	18.81	8.10	-22.95	60.56	41.76	18.55	1004
0.18	0.22	1.37	0.44	-2.21	4.95	3.58	1.12	3.78	10.62	6.54	0.02	21.23	10.61	13.83	2.95	17.56	7.04	-21.70	56.82	39.26	17.41	886
0.32	0.18	1.13	0.34	-2.28	4.53	3.41	0.77	4.01	10.00	6.08	-2.58	22.58	12.58	11.37	3.25	15.48	5.81	-18.91	49.88	34.40	13.73	1971


==> data/mlm_plots/tef/mr/xlnet/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.49
et_p_h	2.94
et_p_l2	4.74


==> data/mlm_plots/tef/mr/xlnet/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.15	0.45	0.33	0.04	0.87	0.41	0.63	0.01	0.06	0.03	-0.01	0.12	0.07	0.07	0.02	0.05	0.03	0.00	0.10	0.05	0.07	516
0.11	0.22	0.82	0.57	0.03	1.61	0.79	1.15	0.02	0.07	0.05	-0.00	0.15	0.07	0.10	0.02	0.06	0.05	0.01	0.12	0.05	0.10	916
0.15	0.42	1.39	0.91	-0.37	3.16	1.77	1.75	0.02	0.09	0.06	0.00	0.18	0.09	0.14	0.03	0.08	0.06	0.02	0.14	0.06	0.11	1004
0.18	0.47	1.65	1.21	0.02	3.29	1.64	2.30	0.03	0.11	0.08	0.02	0.20	0.09	0.18	0.04	0.09	0.08	0.03	0.15	0.06	0.13	886
0.32	0.78	2.73	1.83	-0.62	6.09	3.35	3.35	0.05	0.13	0.10	0.03	0.22	0.09	0.20	0.05	0.11	0.10	0.05	0.17	0.06	0.16	1971


==> data/mlm_plots/tef/mr/xlnet/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.43
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/tef/mr/xlnet/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.86	0.88	0.88	0.84	0.92	0.04	0.91	0.85	0.88	0.89	0.82	0.94	0.06	0.93	0.91	0.92	0.97	0.82	1.03	0.10	0.99	516
0.11	0.82	0.85	0.85	0.80	0.89	0.04	0.88	0.80	0.84	0.85	0.77	0.90	0.07	0.89	0.83	0.88	0.92	0.77	1.00	0.12	0.98	916
0.15	0.79	0.82	0.82	0.77	0.86	0.05	0.85	0.78	0.82	0.82	0.75	0.88	0.06	0.87	0.82	0.87	0.91	0.74	1.00	0.13	0.97	1004
0.18	0.77	0.80	0.80	0.75	0.84	0.05	0.83	0.76	0.80	0.80	0.73	0.86	0.07	0.85	0.77	0.84	0.88	0.71	0.98	0.13	0.95	886
0.32	0.73	0.76	0.76	0.71	0.81	0.05	0.79	0.72	0.77	0.77	0.70	0.83	0.06	0.81	0.73	0.81	0.83	0.68	0.94	0.13	0.91	1971


==> data/mlm_plots/tef/mr/xlnet/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.22


==> data/mlm_plots/tef/mr/xlnet/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.39	0.47	0.42	0.29	0.65	0.18	0.47	1.66	4.12	2.54	-0.94	9.18	5.06	4.64	0.54	1.85	1.39	0.16	3.55	1.70	2.55	516
0.11	0.43	0.58	0.55	0.36	0.80	0.22	0.65	1.94	4.62	3.21	-0.16	9.39	4.78	5.59	0.68	2.00	1.57	0.25	3.74	1.74	2.77	916
0.15	0.59	0.76	0.69	0.50	1.03	0.26	0.83	2.23	5.03	3.60	0.26	9.79	4.76	6.33	0.80	2.16	1.74	0.36	3.97	1.81	2.98	1004
0.18	0.68	0.90	0.81	0.60	1.19	0.30	1.04	2.36	5.78	3.79	-0.19	11.74	5.97	7.25	0.85	2.23	1.74	0.41	4.04	1.82	3.01	886
0.32	0.62	0.85	0.70	0.51	1.20	0.34	1.11	2.88	6.70	4.78	0.51	12.89	6.19	8.63	0.84	2.37	1.84	0.39	4.34	1.98	3.35	1971


==> data/mlm_plots/tef/mr/xlnet/ig/time_misc_auc.tex <==
name	auc
attack_time	0.20
l2	1.44
lom	0.57


==> data/mlm_plots/tef/mr/xlnet/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.22	0.00	-0.19	0.64	0.41	0.00	0.33	0.45	0.43	0.22	0.68	0.23	0.60	0.50	0.63	0.62	0.48	0.77	0.15	0.71	516
0.11	0.00	0.16	0.00	-0.18	0.50	0.34	0.00	0.20	0.38	0.40	0.16	0.61	0.23	0.50	0.50	0.58	0.60	0.42	0.73	0.16	0.67	916
0.15	0.00	0.12	0.00	-0.18	0.42	0.30	0.00	0.17	0.29	0.33	0.07	0.51	0.22	0.50	0.40	0.51	0.50	0.35	0.67	0.16	0.67	1004
0.18	0.00	0.09	0.00	-0.17	0.34	0.26	0.00	0.00	0.27	0.25	0.05	0.50	0.23	0.40	0.40	0.48	0.50	0.31	0.64	0.16	0.60	886
0.32	0.00	0.05	0.00	-0.16	0.26	0.21	0.00	0.00	0.20	0.20	-0.01	0.40	0.20	0.33	0.33	0.42	0.43	0.26	0.58	0.16	0.50	1971


==> data/mlm_plots/tef/mr/xlnet/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.08
top50	0.13


==> data/mlm_plots/tef/mr/xlnet/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	57.53	132.90	98.32	8.80	257.01	124.10	157.05	1.00	1.69	1.00	0.72	2.65	0.97	2.00	81.20	178.32	134.27	30.18	326.46	148.14	222.61	1.00	1.81	2.00	0.79	2.83	1.02	2.00	481
0.11	52.72	135.20	88.04	-16.02	286.42	151.22	161.06	1.00	1.57	1.00	0.65	2.49	0.92	2.00	90.69	210.27	151.99	-1.26	421.79	211.53	257.33	1.00	1.75	1.00	0.71	2.80	1.04	2.00	903
0.15	51.64	125.49	83.82	-9.76	260.74	135.25	149.69	1.00	1.59	1.00	0.68	2.49	0.91	2.00	111.61	255.53	183.59	17.03	494.04	238.50	308.72	1.00	1.87	2.00	0.86	2.88	1.01	2.00	907
0.18	57.92	129.54	94.15	5.58	253.51	123.97	160.78	1.00	1.62	1.00	0.67	2.56	0.95	2.00	134.18	296.13	223.54	32.20	560.06	263.93	354.20	1.00	1.94	2.00	0.83	3.06	1.12	3.00	842
0.32	62.64	146.42	105.57	2.50	290.33	143.91	175.69	1.00	1.63	1.00	0.67	2.59	0.96	2.00	197.71	447.38	325.39	26.45	868.30	420.93	556.45	1.00	2.10	2.00	0.95	3.26	1.16	3.00	2197


==> data/mlm_plots/tef/mr/xlnet/s/comparison_vals_auc.tex <==
name	auc
orig_pp	34.99
orig_ge	0.42
adv_pp	79.06
adv_ge	0.50


==> data/mlm_plots/tef/mr/xlnet/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.52	0.66	0.72	0.41	0.90	0.24	0.84	0.63	0.72	0.78	0.49	0.95	0.23	0.88	0.49	0.59	0.62	0.38	0.79	0.21	0.74	481
0.11	0.38	0.53	0.60	0.25	0.81	0.28	0.74	0.50	0.62	0.68	0.34	0.89	0.28	0.81	0.37	0.49	0.53	0.25	0.72	0.24	0.64	903
0.15	0.26	0.43	0.47	0.14	0.72	0.29	0.65	0.39	0.53	0.60	0.24	0.83	0.29	0.75	0.28	0.41	0.45	0.17	0.65	0.24	0.59	907
0.18	0.14	0.34	0.36	0.03	0.65	0.31	0.56	0.25	0.45	0.52	0.14	0.76	0.31	0.70	0.18	0.34	0.38	0.09	0.59	0.25	0.53	842
0.32	-0.02	0.20	0.20	-0.13	0.52	0.32	0.43	0.11	0.31	0.37	-0.03	0.66	0.35	0.57	0.07	0.23	0.26	-0.04	0.50	0.27	0.42	2197


==> data/mlm_plots/tef/mr/xlnet/s/correlations_auc.tex <==
name	auc
pcc	0.10
spearman	0.12
kendall	0.10


==> data/mlm_plots/tef/mr/xlnet/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.06	0.64	1.57	1.29	0.34	2.80	1.23	2.22	0.70	1.81	1.41	0.24	3.39	1.58	2.45	1.20	6.03	3.23	-1.08	13.13	7.10	7.92	481
0.11	0.85	1.64	1.41	0.58	2.70	1.06	2.17	0.84	1.81	1.46	0.45	3.16	1.36	2.33	1.27	6.74	3.07	-2.66	16.15	9.40	8.62	903
0.15	0.92	1.68	1.46	0.54	2.82	1.14	2.13	0.91	1.80	1.52	0.51	3.10	1.30	2.36	1.34	5.69	2.74	-1.68	13.05	7.36	6.40	907
0.18	1.04	1.75	1.58	0.75	2.75	1.00	2.19	1.08	1.88	1.63	0.72	3.03	1.15	2.37	1.39	5.77	2.67	-2.04	13.58	7.81	6.30	842
0.32	1.17	1.71	1.62	0.89	2.54	0.83	2.07	1.19	1.84	1.68	0.88	2.79	0.96	2.27	1.36	4.31	2.35	-1.66	10.27	5.97	4.43	2197


==> data/mlm_plots/tef/mr/xlnet/s/ets_sts_auc.tex <==
name	auc
et_use	0.44
et_tse	0.48
et_ce	1.45


==> data/mlm_plots/tef/mr/xlnet/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.06	0.17	1.90	0.35	-10.84	14.64	12.74	0.89	1.71	6.63	3.64	-2.14	15.41	8.77	7.44	1.56	10.27	4.24	-8.54	29.08	18.81	10.79	481
0.11	0.16	2.04	0.31	-12.16	16.24	14.20	0.79	1.78	6.37	3.39	-1.78	14.53	8.15	7.98	1.49	11.68	3.49	-17.28	40.64	28.96	9.53	903
0.15	0.12	1.78	0.23	-8.05	11.60	9.83	0.67	1.91	6.68	3.47	-4.01	17.36	10.68	6.94	1.70	10.25	3.51	-16.34	36.85	26.60	9.43	907
0.18	0.12	1.34	0.24	-9.16	11.84	10.50	0.53	2.11	6.03	3.47	-1.81	13.88	7.84	6.63	1.75	8.95	3.52	-7.26	25.16	16.21	9.17	842
0.32	0.09	0.98	0.18	-8.02	9.99	9.01	0.41	2.27	6.11	3.48	-3.71	15.94	9.82	5.98	1.82	10.72	3.27	-23.41	44.86	34.13	7.63	2197


==> data/mlm_plots/tef/mr/xlnet/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.39
et_p_h	1.63
et_p_l2	2.65


==> data/mlm_plots/tef/mr/xlnet/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.16	0.53	0.40	0.04	1.03	0.49	0.75	0.01	0.06	0.03	-0.01	0.14	0.07	0.08	0.02	0.06	0.04	0.00	0.11	0.05	0.07	481
0.11	0.24	0.91	0.58	-0.08	1.91	0.99	1.27	0.02	0.09	0.05	0.00	0.18	0.09	0.13	0.03	0.08	0.06	0.02	0.14	0.06	0.11	903
0.15	0.42	1.62	1.07	-0.52	3.75	2.13	2.05	0.03	0.10	0.06	0.01	0.19	0.09	0.17	0.04	0.09	0.07	0.03	0.15	0.06	0.13	907
0.18	0.53	1.78	1.29	0.05	3.52	1.73	2.29	0.03	0.11	0.08	0.02	0.20	0.09	0.18	0.05	0.10	0.08	0.04	0.16	0.06	0.14	842
0.32	0.88	3.06	2.06	-0.49	6.60	3.55	3.98	0.05	0.14	0.12	0.04	0.23	0.10	0.21	0.06	0.12	0.11	0.05	0.18	0.07	0.17	2197


==> data/mlm_plots/tef/mr/xlnet/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.48
pp_l2_d	0.03
pp_h_d	0.02


==> data/mlm_plots/tef/mr/xlnet/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.86	0.88	0.89	0.85	0.92	0.04	0.91	0.87	0.89	0.89	0.84	0.94	0.05	0.92	0.90	0.93	0.96	0.84	1.01	0.08	0.99	481
0.11	0.82	0.85	0.85	0.81	0.89	0.04	0.88	0.82	0.85	0.86	0.79	0.91	0.06	0.89	0.85	0.90	0.93	0.80	1.00	0.10	0.98	903
0.15	0.79	0.82	0.81	0.77	0.86	0.05	0.85	0.78	0.82	0.82	0.76	0.88	0.06	0.86	0.82	0.87	0.90	0.76	0.98	0.11	0.96	907
0.18	0.77	0.80	0.80	0.75	0.85	0.05	0.83	0.76	0.80	0.81	0.74	0.87	0.07	0.85	0.80	0.85	0.89	0.73	0.98	0.13	0.95	842
0.32	0.72	0.76	0.75	0.70	0.81	0.05	0.79	0.71	0.76	0.77	0.70	0.83	0.07	0.81	0.73	0.81	0.83	0.67	0.95	0.14	0.91	2197


==> data/mlm_plots/tef/mr/xlnet/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.21
sts_tse	0.21
sts_ce	0.22


==> data/mlm_plots/tef/mr/xlnet/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.06	0.19	0.22	0.21	0.16	0.29	0.07	0.23	56.68	248.47	109.37	-93.65	590.60	342.13	278.53	0.20	0.54	0.40	0.07	1.01	0.47	0.75	481
0.11	0.22	0.29	0.26	0.18	0.40	0.11	0.33	72.80	341.49	147.89	-208.52	891.50	550.01	334.70	0.20	0.56	0.40	0.07	1.05	0.49	0.79	903
0.15	0.29	0.38	0.37	0.27	0.49	0.11	0.45	86.02	376.04	178.04	-130.92	883.00	506.96	439.01	0.24	0.67	0.52	0.08	1.27	0.60	0.94	907
0.18	0.39	0.45	0.44	0.36	0.54	0.09	0.51	95.25	493.60	201.99	-199.20	1186.40	692.80	602.55	0.25	0.74	0.56	0.11	1.36	0.62	1.07	842
0.32	0.48	0.54	0.53	0.45	0.63	0.09	0.60	124.36	647.68	332.75	-146.37	1441.72	794.05	883.96	0.29	0.84	0.67	0.16	1.53	0.69	1.25	2197


==> data/mlm_plots/tef/mr/xlnet/s/time_misc_auc.tex <==
name	auc
attack_time	0.11
l2	121.67
lom	0.18


==> data/mlm_plots/tef/mr/xlnet/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.06	0.00	0.29	0.00	-0.16	0.75	0.45	1.00	0.50	0.66	0.67	0.44	0.87	0.21	0.80	0.67	0.78	0.83	0.64	0.93	0.15	0.88	481
0.11	0.00	0.22	0.00	-0.16	0.60	0.38	0.50	0.40	0.57	0.60	0.34	0.80	0.23	0.67	0.67	0.75	0.75	0.59	0.90	0.16	0.83	903
0.15	0.00	0.17	0.00	-0.17	0.51	0.34	0.00	0.33	0.51	0.50	0.25	0.77	0.26	0.67	0.67	0.71	0.71	0.54	0.88	0.17	0.83	907
0.18	0.00	0.11	0.00	-0.17	0.39	0.28	0.00	0.33	0.45	0.50	0.21	0.69	0.24	0.67	0.57	0.66	0.64	0.48	0.83	0.17	0.80	842
0.32	0.00	0.06	0.00	-0.16	0.29	0.23	0.00	0.20	0.36	0.33	0.10	0.61	0.25	0.50	0.50	0.61	0.62	0.43	0.78	0.17	0.71	2197


==> data/mlm_plots/tef/mr/xlnet/s/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.12
top50	0.18


==> data/mlm_plots/tef/yelp/bert/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	40.45	57.66	52.26	31.19	84.12	26.46	65.99	22.00	33.04	32.00	19.51	46.57	13.53	43.00	47.67	66.05	59.69	37.31	94.79	28.74	76.27	22.00	33.35	32.00	19.73	46.97	13.62	43.00	802
0.03	42.45	65.43	55.05	23.24	107.61	42.18	74.91	16.00	28.80	27.00	13.97	43.63	14.83	41.00	56.76	84.65	72.25	33.01	136.30	51.65	95.08	16.00	29.32	28.00	14.24	44.39	15.08	41.00	938
0.06	42.61	69.75	54.66	5.38	134.12	64.37	75.56	15.00	28.55	28.00	13.37	43.73	15.18	41.00	69.59	109.67	87.31	18.73	200.62	90.95	117.25	16.00	29.44	28.00	13.87	45.00	15.57	42.00	1003
0.11	42.61	70.45	55.58	12.95	127.96	57.51	77.36	15.00	27.34	25.00	12.13	42.55	15.21	39.00	86.57	134.68	110.02	35.74	233.61	98.93	150.19	15.00	28.51	26.00	12.77	44.26	15.75	41.00	1010
0.15	42.35	71.91	54.96	-17.79	161.61	89.70	75.68	15.00	27.95	26.00	12.93	42.97	15.02	39.00	119.92	175.27	147.39	68.01	282.54	107.26	194.31	16.00	29.76	28.00	13.93	45.58	15.82	43.00	1007
0.18	42.37	68.96	55.21	15.31	122.61	53.65	76.76	15.00	27.68	25.00	12.34	43.01	15.34	39.00	163.66	231.11	202.88	105.34	356.87	125.77	256.89	16.00	30.09	28.00	13.79	46.40	16.30	43.00	1080
0.32	42.95	69.41	56.06	21.23	117.58	48.17	76.50	15.00	27.71	26.00	12.65	42.77	15.06	39.00	212.28	312.43	266.10	140.62	484.25	171.82	361.22	17.00	30.55	29.00	14.33	46.77	16.22	44.00	1816


==> data/mlm_plots/tef/yelp/bert/a/comparison_vals_auc.tex <==
name	auc
orig_pp	21.45
orig_ge	8.71
adv_pp	60.73
adv_ge	9.28


==> data/mlm_plots/tef/yelp/bert/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.14	0.31	0.28	0.10	0.53	0.22	0.45	0.83	0.87	0.89	0.78	0.95	0.09	0.92	0.66	0.71	0.73	0.61	0.82	0.10	0.79	802
0.03	0.04	0.17	0.11	-0.01	0.34	0.18	0.24	0.74	0.79	0.81	0.68	0.90	0.11	0.87	0.56	0.62	0.64	0.51	0.74	0.12	0.70	938
0.06	-0.01	0.07	0.03	-0.06	0.21	0.14	0.11	0.63	0.69	0.71	0.55	0.83	0.14	0.79	0.46	0.52	0.54	0.40	0.65	0.12	0.61	1003
0.11	-0.02	0.02	-0.01	-0.08	0.12	0.10	0.04	0.51	0.60	0.62	0.44	0.76	0.16	0.72	0.37	0.44	0.45	0.31	0.58	0.13	0.53	1010
0.15	-0.05	-0.02	-0.03	-0.12	0.09	0.10	-0.00	0.37	0.49	0.52	0.29	0.68	0.19	0.62	0.25	0.35	0.36	0.20	0.49	0.15	0.45	1007
0.18	-0.08	-0.05	-0.05	-0.12	0.02	0.07	-0.02	0.24	0.38	0.41	0.18	0.59	0.21	0.54	0.16	0.27	0.28	0.12	0.42	0.15	0.38	1080
0.32	-0.12	-0.08	-0.08	-0.15	-0.02	0.06	-0.04	0.14	0.28	0.28	0.06	0.49	0.21	0.43	0.09	0.19	0.19	0.04	0.34	0.15	0.29	1816


==> data/mlm_plots/tef/yelp/bert/a/correlations_auc.tex <==
name	auc
pcc	0.00
spearman	0.15
kendall	0.11


==> data/mlm_plots/tef/yelp/bert/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	7.66	11.30	10.61	6.11	16.50	5.19	14.16	6.69	10.39	9.34	4.89	15.89	5.50	12.82	6.49	13.19	11.15	4.32	22.07	8.88	17.42	802
0.03	5.52	7.43	6.91	4.41	10.46	3.02	8.81	4.92	7.04	6.27	3.50	10.57	3.54	8.40	5.27	10.72	8.19	2.53	18.90	8.19	13.21	938
0.06	3.84	4.87	4.63	3.23	6.51	1.64	5.51	3.53	4.65	4.32	2.80	6.50	1.85	5.32	4.12	7.62	5.74	1.39	13.85	6.23	8.71	1003
0.11	3.14	3.80	3.64	2.78	4.82	1.02	4.25	2.89	3.62	3.43	2.45	4.79	1.17	4.06	3.32	5.95	4.62	0.48	11.42	5.47	6.54	1010
0.15	2.53	2.91	2.80	2.23	3.60	0.68	3.20	2.38	2.81	2.69	2.03	3.60	0.78	3.08	2.59	4.18	3.54	1.29	7.07	2.89	4.83	1007
0.18	2.24	2.50	2.44	2.05	2.94	0.45	2.65	2.12	2.43	2.35	1.92	2.93	0.51	2.60	2.23	3.45	2.86	0.68	6.23	2.77	3.96	1080
0.32	2.03	2.23	2.18	1.90	2.57	0.33	2.37	1.96	2.20	2.14	1.82	2.59	0.39	2.35	1.91	2.81	2.43	0.99	4.63	1.82	3.22	1816


==> data/mlm_plots/tef/yelp/bert/a/ets_sts_auc.tex <==
name	auc
et_use	1.14
et_tse	1.09
et_ce	1.61


==> data/mlm_plots/tef/yelp/bert/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.57	3.60	2.36	-1.76	8.96	5.36	3.54	6.99	12.60	10.30	3.95	21.26	8.65	15.32	6.32	13.98	10.29	2.11	25.85	11.87	17.36	802
0.03	1.00	1.92	1.35	-0.75	4.59	2.67	1.92	6.44	10.34	8.58	3.48	17.20	6.86	12.08	5.65	12.00	8.24	-4.21	28.20	16.20	13.07	938
0.06	0.59	0.97	0.75	-0.00	1.94	0.97	1.04	5.37	7.82	6.63	2.88	12.76	4.94	8.51	4.59	7.99	5.95	1.41	14.57	6.58	8.62	1003
0.11	0.39	0.66	0.49	-0.36	1.69	1.02	0.66	4.82	6.63	5.58	2.82	10.44	3.81	7.16	4.02	7.03	4.94	-1.63	15.69	8.66	7.03	1010
0.15	0.24	0.36	0.30	0.10	0.62	0.26	0.39	4.06	5.42	4.74	2.36	8.48	3.06	5.60	3.41	6.06	4.17	-5.25	17.38	11.31	5.40	1007
0.18	0.16	0.24	0.20	0.07	0.40	0.17	0.27	3.59	4.62	4.16	2.52	6.71	2.10	4.90	3.01	4.45	3.63	1.14	7.76	3.31	4.52	1080
0.32	0.11	0.17	0.15	0.06	0.28	0.11	0.20	3.34	4.16	3.78	2.66	5.66	1.50	4.48	2.78	3.97	3.28	1.22	6.73	2.76	4.10	1816


==> data/mlm_plots/tef/yelp/bert/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.20
et_p_h	1.87
et_p_l2	1.95


==> data/mlm_plots/tef/yelp/bert/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.09	0.16	0.15	0.07	0.24	0.08	0.21	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.04	0.03	0.02	0.05	0.02	0.05	802
0.03	0.22	0.32	0.31	0.17	0.47	0.15	0.41	0.03	0.06	0.05	0.02	0.09	0.03	0.07	0.03	0.05	0.05	0.03	0.07	0.02	0.06	938
0.06	0.45	0.64	0.61	0.35	0.92	0.29	0.79	0.05	0.08	0.08	0.04	0.12	0.04	0.10	0.05	0.07	0.07	0.05	0.10	0.03	0.09	1003
0.11	0.74	1.02	0.98	0.56	1.47	0.45	1.23	0.07	0.10	0.10	0.06	0.14	0.04	0.12	0.07	0.09	0.09	0.06	0.11	0.03	0.10	1010
0.15	1.28	1.77	1.68	1.01	2.52	0.75	2.15	0.09	0.12	0.12	0.08	0.17	0.04	0.15	0.09	0.11	0.11	0.08	0.14	0.03	0.12	1007
0.18	1.99	2.72	2.59	1.58	3.86	1.14	3.30	0.12	0.14	0.15	0.10	0.19	0.05	0.17	0.11	0.12	0.13	0.09	0.15	0.03	0.14	1080
0.32	2.74	3.99	3.73	2.15	5.82	1.83	4.81	0.13	0.16	0.16	0.11	0.21	0.05	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.16	1816


==> data/mlm_plots/tef/yelp/bert/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.65
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/bert/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.94	0.99	0.02	0.98	802
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.91	0.93	0.93	0.90	0.96	0.03	0.95	0.92	0.94	0.95	0.90	0.98	0.04	0.97	938
0.06	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.89	0.91	0.92	0.86	0.96	0.05	0.95	1003
0.11	0.85	0.86	0.86	0.83	0.89	0.03	0.88	0.83	0.85	0.86	0.81	0.89	0.04	0.88	0.85	0.88	0.89	0.82	0.94	0.06	0.92	1010
0.15	0.80	0.82	0.82	0.78	0.85	0.03	0.84	0.79	0.81	0.81	0.76	0.85	0.04	0.83	0.80	0.84	0.85	0.76	0.92	0.08	0.89	1007
0.18	0.77	0.78	0.78	0.75	0.81	0.03	0.80	0.75	0.78	0.78	0.74	0.81	0.04	0.80	0.77	0.81	0.81	0.72	0.89	0.08	0.86	1080
0.32	0.73	0.75	0.75	0.72	0.78	0.03	0.77	0.72	0.75	0.75	0.71	0.79	0.04	0.77	0.72	0.77	0.78	0.67	0.86	0.09	0.83	1816


==> data/mlm_plots/tef/yelp/bert/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/yelp/bert/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	2.77	4.21	3.81	2.25	6.18	1.97	5.18	0.25	0.39	0.36	0.20	0.59	0.19	0.50	5.34	19.34	12.96	-0.36	39.04	19.70	26.48	802
0.03	3.19	4.75	4.41	2.49	7.02	2.26	6.06	0.34	0.50	0.47	0.29	0.70	0.20	0.62	4.81	21.09	13.59	-0.73	42.90	21.82	30.45	938
0.06	4.62	8.52	7.74	3.32	13.73	5.20	10.91	0.40	0.57	0.56	0.37	0.78	0.21	0.72	6.04	23.90	16.38	0.48	47.32	23.42	35.12	1003
0.11	6.00	11.75	10.76	4.35	19.15	7.40	15.33	0.43	0.59	0.57	0.39	0.80	0.21	0.75	6.05	23.40	15.44	0.28	46.52	23.12	34.33	1010
0.15	8.77	16.73	15.05	6.15	27.31	10.58	22.22	0.39	0.55	0.52	0.35	0.76	0.21	0.69	6.63	23.44	17.13	0.52	46.36	22.92	31.79	1007
0.18	10.48	19.73	17.75	7.81	31.65	11.92	26.20	0.35	0.50	0.45	0.30	0.70	0.20	0.60	6.18	22.40	16.29	0.45	44.35	21.95	31.13	1080
0.32	13.16	24.75	22.26	9.54	39.96	15.21	32.61	0.31	0.44	0.40	0.26	0.62	0.18	0.53	6.17	21.64	14.36	0.86	42.42	20.78	31.71	1816


==> data/mlm_plots/tef/yelp/bert/a/time_misc_auc.tex <==
name	auc
attack_time	5.03
l2	0.16
lom	6.98


==> data/mlm_plots/tef/yelp/bert/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.50	0.60	0.61	0.43	0.77	0.17	0.71	0.73	0.78	0.79	0.69	0.87	0.09	0.85	0.83	0.86	0.87	0.80	0.92	0.06	0.91	802
0.03	0.33	0.46	0.48	0.27	0.65	0.19	0.60	0.65	0.71	0.72	0.60	0.82	0.11	0.79	0.78	0.82	0.83	0.75	0.89	0.07	0.87	938
0.06	0.18	0.32	0.33	0.12	0.51	0.20	0.45	0.55	0.63	0.64	0.50	0.75	0.12	0.71	0.73	0.77	0.78	0.70	0.85	0.07	0.82	1003
0.11	0.06	0.22	0.20	0.05	0.40	0.18	0.33	0.48	0.56	0.57	0.42	0.70	0.14	0.66	0.68	0.73	0.74	0.65	0.81	0.08	0.79	1010
0.15	0.00	0.13	0.10	-0.01	0.27	0.14	0.21	0.40	0.49	0.50	0.34	0.63	0.15	0.58	0.63	0.69	0.69	0.60	0.78	0.09	0.74	1007
0.18	0.00	0.08	0.00	-0.04	0.19	0.12	0.12	0.33	0.43	0.43	0.28	0.57	0.14	0.52	0.59	0.65	0.65	0.55	0.74	0.09	0.72	1080
0.32	0.00	0.04	0.00	-0.04	0.13	0.09	0.05	0.26	0.36	0.36	0.22	0.49	0.14	0.45	0.54	0.61	0.61	0.51	0.70	0.09	0.67	1816


==> data/mlm_plots/tef/yelp/bert/a/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.15
top50	0.21


==> data/mlm_plots/tef/yelp/bert/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	40.75	58.64	53.02	31.19	86.10	27.45	68.41	20.00	31.83	30.00	18.14	45.52	13.69	42.00	46.74	66.35	60.11	35.26	97.45	31.09	76.74	20.00	32.09	31.00	18.40	45.79	13.70	43.00	766
0.03	42.46	65.69	55.48	23.15	108.23	42.54	74.51	16.00	28.58	27.00	13.77	43.38	14.81	40.00	55.04	82.87	71.00	33.77	131.97	49.10	94.21	16.00	29.03	28.00	14.04	44.02	14.99	41.00	949
0.06	42.33	70.75	54.70	5.09	136.42	65.67	75.67	15.00	28.08	27.00	12.86	43.30	15.22	40.00	67.34	106.95	85.75	12.49	201.41	94.46	114.25	15.00	28.84	28.00	13.24	44.43	15.60	41.00	1037
0.11	41.85	69.14	55.58	14.93	123.35	54.21	77.28	14.00	26.95	25.00	11.85	42.05	15.10	38.00	81.46	130.11	105.34	29.33	230.88	100.78	141.32	15.00	28.04	26.00	12.49	43.58	15.54	40.00	1288
0.15	42.27	67.47	54.69	19.42	115.52	48.05	76.02	16.00	29.13	27.00	13.56	44.71	15.58	42.00	113.40	164.31	140.62	66.13	262.50	98.19	181.73	17.00	30.89	29.00	14.68	47.09	16.21	44.00	1463
0.18	41.89	68.04	54.72	15.40	120.68	52.64	73.53	16.00	28.63	28.00	13.99	43.28	14.64	40.00	140.24	213.66	177.25	75.61	351.71	138.05	229.95	18.00	30.82	31.00	15.22	46.41	15.60	44.00	1188
0.32	45.89	76.59	58.09	9.84	143.34	66.75	82.25	14.00	26.48	25.00	11.34	41.62	15.14	39.00	185.44	278.22	239.45	121.21	435.23	157.01	311.09	15.00	28.63	27.00	12.53	44.73	16.10	41.00	912


==> data/mlm_plots/tef/yelp/bert/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	21.68
orig_ge	8.70
adv_pp	56.15
adv_ge	9.19


==> data/mlm_plots/tef/yelp/bert/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.32	0.05	0.08	-0.39	0.48	0.44	0.37	-0.18	0.14	0.22	-0.24	0.53	0.38	0.44	-0.13	0.11	0.15	-0.18	0.40	0.29	0.32	766
0.03	-0.45	-0.16	-0.17	-0.55	0.23	0.39	0.10	-0.30	-0.02	0.04	-0.37	0.33	0.35	0.25	-0.21	-0.01	0.03	-0.27	0.25	0.26	0.18	949
0.06	-0.60	-0.35	-0.39	-0.68	-0.03	0.33	-0.15	-0.41	-0.18	-0.17	-0.48	0.13	0.31	0.05	-0.29	-0.13	-0.12	-0.35	0.10	0.23	0.04	1037
0.11	-0.73	-0.52	-0.55	-0.78	-0.26	0.26	-0.33	-0.54	-0.33	-0.34	-0.60	-0.06	0.27	-0.11	-0.40	-0.24	-0.24	-0.44	-0.04	0.20	-0.08	1288
0.15	-0.73	-0.60	-0.63	-0.78	-0.42	0.18	-0.49	-0.54	-0.39	-0.41	-0.59	-0.18	0.20	-0.23	-0.39	-0.28	-0.29	-0.43	-0.13	0.15	-0.15	1463
0.18	-0.72	-0.60	-0.61	-0.76	-0.44	0.16	-0.50	-0.51	-0.37	-0.37	-0.54	-0.20	0.17	-0.25	-0.37	-0.27	-0.26	-0.39	-0.14	0.13	-0.17	1188
0.32	-0.70	-0.60	-0.60	-0.74	-0.46	0.14	-0.49	-0.47	-0.38	-0.36	-0.53	-0.23	0.15	-0.28	-0.33	-0.27	-0.26	-0.38	-0.15	0.12	-0.19	912


==> data/mlm_plots/tef/yelp/bert/ig/correlations_auc.tex <==
name	auc
pcc	-0.16
spearman	-0.09
kendall	-0.07


==> data/mlm_plots/tef/yelp/bert/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	8.50	15.20	12.70	5.54	24.85	9.65	19.30	7.30	14.35	11.52	3.63	25.06	10.72	18.16	7.48	17.98	12.65	2.96	33.01	15.02	23.89	766
0.03	6.54	10.05	8.92	4.91	15.19	5.14	12.27	5.91	9.72	8.35	3.76	15.68	5.96	11.68	6.62	14.85	10.50	1.77	27.92	13.08	17.74	949
0.06	5.33	7.20	6.68	4.33	10.06	2.87	8.61	4.89	7.09	6.41	3.64	10.53	3.45	8.31	5.63	11.92	8.49	0.66	23.17	11.26	14.00	1037
0.11	4.64	6.02	5.67	3.83	8.22	2.19	6.83	4.45	6.02	5.57	3.51	8.53	2.51	6.92	5.26	10.33	7.49	0.80	19.87	9.54	11.78	1288
0.15	3.94	4.67	4.58	3.61	5.74	1.06	5.19	3.87	4.68	4.52	3.43	5.93	1.25	5.34	4.43	7.57	6.16	1.51	13.63	6.06	8.64	1463
0.18	3.46	3.98	3.93	3.18	4.79	0.80	4.34	3.34	3.97	3.91	3.04	4.90	0.93	4.45	3.66	5.78	4.82	1.85	9.71	3.93	6.78	1188
0.32	3.09	3.55	3.43	2.87	4.22	0.67	3.90	3.01	3.55	3.41	2.78	4.32	0.77	3.93	3.25	4.88	4.11	1.67	8.10	3.21	5.41	912


==> data/mlm_plots/tef/yelp/bert/ig/ets_sts_auc.tex <==
name	auc
et_use	1.72
et_tse	1.69
et_ce	2.60


==> data/mlm_plots/tef/yelp/bert/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.12	7.23	3.54	-10.57	25.03	17.80	6.13	9.08	19.44	14.92	3.53	35.35	15.91	24.13	8.59	21.43	15.11	-0.09	42.95	21.52	26.05	766
0.03	1.39	4.34	2.09	-13.37	22.06	17.72	3.23	8.70	15.17	12.65	4.84	25.50	10.33	18.22	7.74	16.68	12.66	0.95	32.42	15.73	20.09	949
0.06	0.88	2.03	1.25	-2.93	6.99	4.96	1.78	7.62	12.15	10.17	3.72	20.59	8.44	13.43	6.60	14.07	9.19	-12.38	40.51	26.44	14.10	1037
0.11	0.62	1.13	0.83	-0.96	3.22	2.09	1.18	7.24	10.49	9.00	3.92	17.06	6.57	11.40	6.12	10.71	7.90	-1.26	22.68	11.97	10.85	1288
0.15	0.40	0.70	0.52	-0.89	2.30	1.59	0.69	6.34	8.41	7.65	4.15	12.67	4.26	9.25	5.31	8.22	6.72	-0.32	16.76	8.54	8.48	1463
0.18	0.28	0.45	0.35	-0.87	1.77	1.32	0.46	5.75	7.33	6.64	4.37	10.29	2.96	7.89	4.79	7.13	5.72	1.25	13.02	5.89	7.23	1188
0.32	0.20	0.38	0.28	-0.32	1.08	0.70	0.37	5.26	6.86	6.24	3.85	9.87	3.01	7.23	4.42	6.79	5.44	0.75	12.83	6.04	6.56	912


==> data/mlm_plots/tef/yelp/bert/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.40
et_p_h	2.93
et_p_l2	3.04


==> data/mlm_plots/tef/yelp/bert/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.14	0.13	0.06	0.22	0.08	0.18	0.02	0.03	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.04	766
0.03	0.19	0.29	0.28	0.14	0.44	0.15	0.39	0.03	0.05	0.05	0.02	0.08	0.03	0.07	0.03	0.05	0.05	0.03	0.07	0.02	0.06	949
0.06	0.40	0.57	0.56	0.31	0.83	0.26	0.71	0.05	0.08	0.08	0.04	0.11	0.04	0.10	0.05	0.07	0.07	0.04	0.09	0.02	0.08	1037
0.11	0.68	0.96	0.91	0.52	1.40	0.44	1.18	0.07	0.10	0.10	0.06	0.14	0.04	0.12	0.07	0.08	0.09	0.06	0.11	0.03	0.10	1288
0.15	1.20	1.60	1.54	0.95	2.26	0.65	1.97	0.10	0.12	0.12	0.08	0.16	0.04	0.15	0.09	0.10	0.10	0.08	0.13	0.03	0.12	1463
0.18	1.77	2.37	2.25	1.38	3.36	0.99	2.89	0.11	0.14	0.14	0.09	0.18	0.04	0.17	0.10	0.12	0.12	0.09	0.15	0.03	0.14	1188
0.32	2.15	3.06	2.92	1.76	4.35	1.30	3.89	0.12	0.15	0.15	0.10	0.19	0.05	0.18	0.11	0.13	0.13	0.10	0.16	0.03	0.15	912


==> data/mlm_plots/tef/yelp/bert/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.55
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/bert/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.93	0.99	0.03	0.98	766
0.03	0.92	0.94	0.94	0.91	0.96	0.02	0.95	0.91	0.93	0.93	0.90	0.96	0.03	0.95	0.92	0.94	0.95	0.90	0.98	0.04	0.97	949
0.06	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.87	0.89	0.89	0.86	0.93	0.04	0.92	0.89	0.91	0.92	0.86	0.97	0.05	0.95	1037
0.11	0.84	0.86	0.87	0.83	0.90	0.03	0.88	0.84	0.86	0.86	0.82	0.90	0.04	0.89	0.86	0.89	0.90	0.83	0.95	0.06	0.93	1288
0.15	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.80	0.82	0.82	0.78	0.86	0.04	0.85	0.82	0.86	0.87	0.78	0.93	0.08	0.91	1463
0.18	0.78	0.79	0.79	0.76	0.82	0.03	0.81	0.77	0.79	0.79	0.75	0.83	0.04	0.81	0.78	0.82	0.84	0.75	0.90	0.08	0.88	1188
0.32	0.75	0.77	0.77	0.74	0.80	0.03	0.79	0.74	0.77	0.77	0.73	0.81	0.04	0.79	0.75	0.80	0.81	0.71	0.88	0.08	0.86	912


==> data/mlm_plots/tef/yelp/bert/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/yelp/bert/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.57	4.60	4.39	3.16	6.04	1.44	5.37	6.55	20.31	15.72	3.05	37.56	17.26	30.33	4.96	15.54	11.13	0.70	30.39	14.85	21.97	766
0.03	4.80	6.98	6.60	3.75	10.21	3.23	8.66	7.34	22.88	18.57	3.47	42.29	19.41	33.22	5.22	16.07	11.81	0.50	31.65	15.57	21.67	949
0.06	7.47	9.82	9.18	6.36	13.28	3.46	11.51	9.73	26.39	20.80	3.95	48.84	22.45	37.16	5.50	17.32	12.11	0.46	34.18	16.86	23.23	1037
0.11	10.28	15.01	13.19	7.96	22.06	7.05	17.91	7.84	25.07	19.12	3.57	46.58	21.50	36.60	5.25	17.18	12.14	-0.05	34.41	17.23	23.71	1288
0.15	15.07	21.59	21.09	12.26	30.91	9.32	26.55	7.36	24.70	18.38	2.72	46.68	21.98	35.68	6.12	18.72	13.09	0.25	37.18	18.47	24.82	1463
0.18	18.05	23.95	23.30	14.80	33.09	9.14	28.84	11.37	29.04	25.18	6.93	51.14	22.11	42.00	5.22	18.65	12.79	0.50	36.81	18.15	27.70	1188
0.32	19.78	23.90	23.56	17.66	30.13	6.24	27.10	16.09	33.82	31.86	11.22	56.42	22.60	46.34	5.61	16.38	11.96	1.22	31.55	15.17	22.39	912


==> data/mlm_plots/tef/yelp/bert/ig/time_misc_auc.tex <==
name	auc
attack_time	5.78
l2	8.64
lom	5.43


==> data/mlm_plots/tef/yelp/bert/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.10	0.27	0.24	0.06	0.48	0.21	0.41	0.27	0.41	0.43	0.22	0.59	0.18	0.53	0.44	0.56	0.58	0.41	0.71	0.15	0.67	766
0.03	0.00	0.18	0.14	0.01	0.36	0.18	0.29	0.20	0.34	0.35	0.17	0.50	0.16	0.44	0.40	0.50	0.51	0.36	0.63	0.13	0.60	949
0.06	0.00	0.10	0.05	-0.02	0.22	0.12	0.18	0.16	0.26	0.26	0.12	0.41	0.14	0.37	0.36	0.45	0.46	0.33	0.57	0.12	0.54	1037
0.11	0.00	0.06	0.00	-0.04	0.15	0.09	0.10	0.10	0.20	0.19	0.08	0.32	0.12	0.29	0.31	0.40	0.39	0.29	0.51	0.11	0.48	1288
0.15	0.00	0.03	0.00	-0.03	0.09	0.06	0.05	0.10	0.17	0.17	0.07	0.27	0.10	0.24	0.31	0.38	0.38	0.29	0.47	0.09	0.44	1463
0.18	0.00	0.03	0.00	-0.02	0.09	0.06	0.05	0.11	0.18	0.18	0.08	0.27	0.09	0.24	0.33	0.39	0.39	0.31	0.47	0.08	0.45	1188
0.32	0.00	0.03	0.00	-0.02	0.07	0.05	0.05	0.11	0.17	0.17	0.08	0.25	0.08	0.23	0.35	0.39	0.40	0.32	0.46	0.07	0.44	912


==> data/mlm_plots/tef/yelp/bert/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.06
top50	0.13


==> data/mlm_plots/tef/yelp/bert/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	41.41	58.91	52.91	31.68	86.13	27.23	69.09	21.00	32.29	31.00	18.59	46.00	13.70	43.00	48.14	68.08	60.39	37.48	98.68	30.60	78.98	21.00	32.61	31.00	18.81	46.41	13.80	43.00	753
0.03	42.25	64.48	54.68	28.15	100.82	36.33	74.91	16.00	28.78	28.00	13.92	43.65	14.86	40.00	57.38	84.74	73.29	41.69	127.78	43.04	96.82	16.00	29.33	28.00	14.25	44.40	15.07	41.00	938
0.06	42.83	71.70	56.58	7.63	135.77	64.07	78.01	14.00	27.24	25.00	11.93	42.55	15.31	39.00	74.51	116.52	93.38	17.66	215.38	98.86	122.75	15.00	28.05	26.00	12.42	43.68	15.63	40.00	1019
0.11	42.53	72.28	55.72	-8.72	153.29	81.00	77.11	14.00	27.59	25.00	12.02	43.16	15.57	39.00	91.66	146.60	115.95	-5.87	299.06	152.47	153.98	15.00	28.82	27.00	12.77	44.87	16.05	41.00	1135
0.15	42.48	67.44	54.68	15.30	119.58	52.14	73.85	16.00	28.86	28.00	13.88	43.85	14.98	41.00	122.52	179.93	154.63	64.94	294.92	114.99	196.70	17.00	30.70	29.00	15.06	46.35	15.64	43.00	1314
0.18	42.45	68.06	55.48	18.27	117.84	49.78	76.83	15.00	27.75	26.00	12.58	42.92	15.17	40.00	158.57	236.56	203.46	98.98	374.15	137.58	268.11	16.00	29.95	28.00	13.95	45.95	16.00	43.00	1215
0.32	43.97	75.27	57.78	10.19	140.35	65.08	81.71	14.00	26.55	24.00	11.48	41.62	15.07	38.00	210.55	322.23	266.89	115.97	528.49	206.26	366.16	15.00	29.16	27.00	13.01	45.31	16.15	43.00	1226


==> data/mlm_plots/tef/yelp/bert/s/comparison_vals_auc.tex <==
name	auc
orig_pp	21.74
orig_ge	8.63
adv_pp	62.86
adv_ge	9.17


==> data/mlm_plots/tef/yelp/bert/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.41	0.55	0.55	0.36	0.73	0.19	0.68	0.71	0.77	0.78	0.66	0.87	0.11	0.84	0.53	0.60	0.60	0.49	0.71	0.11	0.66	753
0.03	0.27	0.41	0.40	0.22	0.60	0.19	0.54	0.61	0.69	0.70	0.55	0.82	0.13	0.78	0.44	0.52	0.52	0.40	0.64	0.12	0.60	938
0.06	0.15	0.28	0.27	0.11	0.46	0.18	0.39	0.49	0.59	0.61	0.43	0.75	0.16	0.71	0.35	0.43	0.44	0.30	0.57	0.13	0.53	1019
0.11	0.08	0.18	0.16	0.03	0.33	0.15	0.27	0.38	0.49	0.50	0.31	0.67	0.18	0.62	0.27	0.35	0.36	0.22	0.49	0.14	0.45	1135
0.15	0.01	0.10	0.08	-0.02	0.22	0.12	0.16	0.26	0.39	0.39	0.21	0.58	0.18	0.52	0.18	0.28	0.27	0.14	0.41	0.13	0.37	1314
0.18	-0.03	0.05	0.04	-0.07	0.17	0.12	0.12	0.17	0.31	0.31	0.11	0.51	0.20	0.45	0.12	0.22	0.22	0.07	0.36	0.14	0.31	1215
0.32	-0.07	0.01	-0.00	-0.12	0.13	0.12	0.08	0.07	0.22	0.23	0.00	0.45	0.22	0.39	0.05	0.16	0.16	0.00	0.31	0.15	0.27	1226


==> data/mlm_plots/tef/yelp/bert/s/correlations_auc.tex <==
name	auc
pcc	0.04
spearman	0.13
kendall	0.09


==> data/mlm_plots/tef/yelp/bert/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	4.46	7.13	6.64	3.32	10.94	3.81	9.05	4.06	6.69	5.93	2.75	10.64	3.94	8.55	4.02	8.81	6.88	2.00	15.63	6.82	11.61	753
0.03	3.48	5.00	4.68	2.65	7.35	2.35	6.13	3.15	4.80	4.31	2.08	7.52	2.72	5.78	3.60	8.00	6.00	1.23	14.78	6.77	9.73	938
0.06	2.84	3.68	3.53	2.34	5.02	1.34	4.35	2.65	3.55	3.36	2.09	5.00	1.46	4.18	3.14	6.68	4.79	0.35	13.02	6.33	7.46	1019
0.11	2.59	3.13	3.04	2.22	4.04	0.91	3.62	2.43	3.05	2.93	2.07	4.03	0.98	3.56	2.90	5.63	4.29	0.50	10.77	5.14	6.39	1135
0.15	2.24	2.61	2.57	2.02	3.19	0.59	2.93	2.15	2.56	2.51	1.91	3.22	0.65	2.92	2.45	4.01	3.35	1.16	6.86	2.85	4.71	1314
0.18	2.04	2.34	2.31	1.88	2.80	0.46	2.61	2.00	2.34	2.29	1.78	2.90	0.56	2.61	2.11	3.59	2.89	0.32	6.86	3.27	4.00	1215
0.32	1.91	2.16	2.12	1.74	2.57	0.42	2.36	1.87	2.16	2.12	1.69	2.64	0.48	2.38	1.87	3.08	2.55	-0.03	6.20	3.11	3.36	1226


==> data/mlm_plots/tef/yelp/bert/s/ets_sts_auc.tex <==
name	auc
et_use	0.93
et_tse	0.91
et_ce	1.47


==> data/mlm_plots/tef/yelp/bert/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.93	2.15	1.42	-0.79	5.09	2.94	2.16	4.29	8.08	6.37	1.95	14.20	6.12	10.27	3.78	8.70	6.05	-0.24	17.64	8.94	11.04	753
0.03	0.62	1.37	0.88	-1.74	4.48	3.11	1.34	4.04	6.86	5.76	1.93	11.79	4.93	7.93	3.48	7.57	5.30	-4.42	19.56	11.99	8.20	938
0.06	0.41	0.75	0.56	-0.52	2.01	1.27	0.76	3.89	5.73	4.87	2.15	9.32	3.58	6.38	3.25	5.91	4.32	0.49	11.33	5.42	6.35	1019
0.11	0.30	0.51	0.39	-0.42	1.45	0.94	0.51	3.75	5.07	4.49	2.37	7.77	2.70	5.48	3.08	5.52	3.89	-1.95	12.99	7.47	5.29	1135
0.15	0.20	0.31	0.25	0.04	0.57	0.27	0.33	3.48	4.39	4.05	2.68	6.09	1.71	4.79	2.88	4.38	3.46	0.19	8.57	4.19	4.49	1314
0.18	0.14	0.30	0.18	-1.60	2.20	1.90	0.24	3.19	3.95	3.71	2.51	5.40	1.45	4.36	2.73	3.83	3.21	0.09	7.57	3.74	3.98	1215
0.32	0.11	0.17	0.14	-0.09	0.44	0.26	0.19	3.10	3.91	3.61	2.17	5.66	1.74	4.21	2.55	3.83	3.09	0.12	7.54	3.71	3.83	1226


==> data/mlm_plots/tef/yelp/bert/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.16
et_p_h	1.47
et_p_l2	1.51


==> data/mlm_plots/tef/yelp/bert/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.10	0.17	0.16	0.08	0.26	0.09	0.22	0.02	0.04	0.04	0.01	0.07	0.03	0.06	0.02	0.04	0.04	0.02	0.06	0.02	0.05	753
0.03	0.23	0.35	0.33	0.17	0.53	0.18	0.46	0.03	0.06	0.06	0.03	0.09	0.03	0.08	0.04	0.05	0.05	0.03	0.08	0.02	0.07	938
0.06	0.49	0.69	0.66	0.37	1.00	0.32	0.84	0.05	0.08	0.09	0.04	0.12	0.04	0.11	0.05	0.07	0.08	0.05	0.10	0.03	0.09	1019
0.11	0.80	1.13	1.07	0.60	1.66	0.53	1.36	0.08	0.11	0.11	0.06	0.15	0.04	0.13	0.07	0.09	0.09	0.06	0.12	0.03	0.11	1135
0.15	1.36	1.86	1.78	1.07	2.65	0.79	2.26	0.10	0.13	0.13	0.08	0.17	0.04	0.16	0.09	0.11	0.11	0.08	0.14	0.03	0.13	1314
0.18	1.97	2.73	2.60	1.61	3.84	1.12	3.31	0.12	0.15	0.15	0.10	0.19	0.04	0.17	0.11	0.13	0.13	0.10	0.16	0.03	0.14	1215
0.32	2.62	3.77	3.52	2.03	5.51	1.74	4.60	0.13	0.16	0.16	0.11	0.21	0.05	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.16	1226


==> data/mlm_plots/tef/yelp/bert/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.65
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/bert/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.96	0.97	0.95	0.98	0.01	0.97	0.95	0.96	0.96	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.94	0.99	0.03	0.98	753
0.03	0.92	0.94	0.94	0.91	0.96	0.02	0.95	0.91	0.93	0.93	0.90	0.96	0.03	0.95	0.92	0.94	0.95	0.90	0.98	0.04	0.97	938
0.06	0.88	0.90	0.90	0.87	0.92	0.03	0.91	0.87	0.89	0.89	0.86	0.92	0.03	0.91	0.89	0.92	0.93	0.86	0.97	0.05	0.95	1019
0.11	0.85	0.86	0.86	0.83	0.89	0.03	0.88	0.84	0.86	0.86	0.82	0.89	0.03	0.88	0.86	0.89	0.90	0.84	0.95	0.06	0.94	1135
0.15	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.79	0.82	0.82	0.78	0.85	0.04	0.84	0.82	0.85	0.86	0.78	0.92	0.07	0.90	1314
0.18	0.78	0.79	0.79	0.76	0.82	0.03	0.81	0.77	0.79	0.79	0.75	0.83	0.04	0.81	0.78	0.83	0.84	0.75	0.90	0.08	0.88	1215
0.32	0.75	0.77	0.76	0.73	0.80	0.03	0.78	0.74	0.76	0.77	0.72	0.80	0.04	0.79	0.74	0.79	0.80	0.70	0.88	0.09	0.85	1226


==> data/mlm_plots/tef/yelp/bert/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/yelp/bert/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	1.77	2.18	2.18	1.59	2.78	0.60	2.47	17.48	130.28	73.22	-25.89	286.45	156.17	198.00	2.23	6.95	5.06	0.55	13.35	6.40	9.82	753
0.03	4.77	6.79	6.26	3.76	9.81	3.02	8.46	25.22	176.62	92.80	-45.76	399.00	222.38	258.59	2.10	7.82	5.55	0.31	15.32	7.50	11.22	938
0.06	4.08	5.38	4.85	2.83	7.93	2.55	5.83	35.84	232.26	129.46	-63.51	528.03	295.77	327.33	2.37	8.77	6.25	0.49	17.06	8.28	12.55	1019
0.11	9.88	14.35	13.43	7.27	21.43	7.08	17.69	43.75	267.00	151.04	-114.44	648.45	381.44	333.46	2.69	9.98	7.15	0.66	19.29	9.32	14.56	1135
0.15	13.44	18.33	17.14	10.46	26.21	7.88	22.08	42.67	309.25	133.95	-191.33	809.83	500.58	353.41	3.90	11.31	9.15	1.87	20.74	9.44	15.97	1314
0.18	12.92	15.38	14.73	11.07	19.68	4.30	17.35	50.56	345.85	166.71	-157.03	848.72	502.87	417.15	3.45	11.31	8.66	1.45	21.17	9.86	16.51	1215
0.32	13.56	16.20	15.98	11.37	21.03	4.83	18.09	84.73	414.00	248.99	-117.34	945.34	531.34	510.81	2.96	11.00	7.83	0.88	21.12	10.12	16.55	1226


==> data/mlm_plots/tef/yelp/bert/s/time_misc_auc.tex <==
name	auc
attack_time	4.17
l2	96.23
lom	3.20


==> data/mlm_plots/tef/yelp/bert/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.40	0.52	0.50	0.35	0.69	0.17	0.63	0.65	0.70	0.70	0.61	0.80	0.09	0.76	0.76	0.80	0.80	0.74	0.87	0.06	0.84	753
0.03	0.29	0.40	0.40	0.22	0.57	0.18	0.50	0.57	0.64	0.64	0.53	0.74	0.10	0.71	0.72	0.77	0.77	0.70	0.83	0.07	0.81	938
0.06	0.14	0.27	0.25	0.09	0.44	0.18	0.38	0.50	0.57	0.56	0.45	0.68	0.12	0.64	0.67	0.72	0.72	0.64	0.80	0.08	0.78	1019
0.11	0.07	0.19	0.18	0.04	0.34	0.15	0.29	0.43	0.50	0.50	0.38	0.63	0.12	0.58	0.63	0.68	0.68	0.60	0.76	0.08	0.74	1135
0.15	0.00	0.13	0.10	0.00	0.25	0.12	0.20	0.36	0.44	0.44	0.33	0.56	0.11	0.52	0.59	0.64	0.64	0.56	0.73	0.08	0.70	1314
0.18	0.00	0.10	0.07	-0.01	0.22	0.12	0.18	0.33	0.40	0.40	0.29	0.52	0.11	0.48	0.56	0.61	0.62	0.53	0.70	0.09	0.67	1215
0.32	0.00	0.08	0.00	-0.03	0.18	0.10	0.12	0.27	0.35	0.35	0.23	0.47	0.12	0.43	0.53	0.58	0.59	0.49	0.68	0.10	0.65	1226


==> data/mlm_plots/tef/yelp/bert/s/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.14
top50	0.20


==> data/mlm_plots/tef/yelp/cnn/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.81	60.32	54.43	34.04	86.61	26.29	70.05	18.00	29.64	28.00	16.12	43.15	13.51	40.00	47.94	67.26	60.73	38.81	95.71	28.45	77.01	18.00	29.87	28.00	16.24	43.49	13.63	40.00	757
0.03	43.69	67.33	57.14	29.18	105.47	38.14	76.39	15.00	26.61	24.00	11.96	41.26	14.65	37.00	56.23	83.27	72.84	38.83	127.70	44.44	95.03	15.00	27.11	24.00	12.19	42.03	14.92	38.00	963
0.06	43.79	72.24	58.26	14.09	130.40	58.16	79.74	13.00	25.01	22.00	10.14	39.89	14.88	36.00	69.71	107.47	87.42	16.08	198.85	91.38	118.58	13.00	25.90	23.00	10.48	41.32	15.42	37.00	1052
0.11	44.59	73.56	58.36	11.82	135.30	61.74	80.28	13.00	25.75	23.00	10.60	40.90	15.15	37.00	84.77	130.61	107.82	22.56	238.66	108.05	141.91	14.00	27.12	24.00	11.20	43.03	15.92	40.00	1119
0.15	44.05	69.61	57.02	21.62	117.60	47.99	77.56	14.00	25.15	22.00	10.68	39.62	14.47	36.00	112.95	162.66	141.16	66.21	259.12	96.46	184.48	15.00	27.29	24.00	11.63	42.95	15.66	39.00	1042
0.18	43.97	70.63	58.06	26.34	114.93	44.30	80.60	13.00	24.79	21.00	9.98	39.59	14.80	35.00	145.70	218.53	182.39	75.42	361.64	143.11	242.22	14.00	27.63	24.00	11.09	44.17	16.54	40.00	1080
0.32	43.72	72.53	57.92	20.85	124.22	51.68	79.87	13.00	24.58	21.00	10.13	39.03	14.45	35.00	197.59	298.57	253.40	119.29	477.85	179.28	336.21	15.00	28.36	25.00	11.75	44.98	16.62	41.00	1746


==> data/mlm_plots/tef/yelp/cnn/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	22.02
orig_ge	7.84
adv_pp	57.93
adv_ge	8.54


==> data/mlm_plots/tef/yelp/cnn/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.21	0.42	0.43	0.12	0.72	0.30	0.64	0.45	0.61	0.66	0.37	0.85	0.24	0.81	0.35	0.55	0.56	0.30	0.79	0.25	0.77	757
0.03	-0.05	0.17	0.15	-0.15	0.49	0.32	0.41	0.24	0.43	0.45	0.18	0.67	0.25	0.62	0.20	0.38	0.37	0.14	0.61	0.23	0.57	963
0.06	-0.25	-0.04	-0.08	-0.34	0.26	0.30	0.14	0.07	0.25	0.24	0.01	0.48	0.24	0.41	0.07	0.22	0.20	0.02	0.43	0.21	0.36	1052
0.11	-0.36	-0.17	-0.21	-0.45	0.11	0.28	-0.02	-0.04	0.11	0.10	-0.10	0.32	0.21	0.25	-0.02	0.11	0.09	-0.07	0.29	0.18	0.23	1119
0.15	-0.47	-0.30	-0.32	-0.54	-0.06	0.24	-0.18	-0.17	-0.05	-0.06	-0.24	0.13	0.19	0.05	-0.12	-0.02	-0.03	-0.17	0.13	0.15	0.07	1042
0.18	-0.52	-0.38	-0.40	-0.60	-0.15	0.23	-0.25	-0.27	-0.15	-0.17	-0.33	0.02	0.17	-0.06	-0.19	-0.10	-0.11	-0.23	0.03	0.13	-0.02	1080
0.32	-0.57	-0.43	-0.45	-0.64	-0.21	0.21	-0.31	-0.37	-0.26	-0.27	-0.42	-0.09	0.17	-0.16	-0.27	-0.18	-0.19	-0.31	-0.06	0.13	-0.11	1746


==> data/mlm_plots/tef/yelp/cnn/ig/correlations_auc.tex <==
name	auc
pcc	-0.07
spearman	-0.00
kendall	0.01


==> data/mlm_plots/tef/yelp/cnn/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	5.38	9.87	8.74	3.49	16.26	6.38	12.82	5.05	9.69	8.35	2.76	16.63	6.93	12.54	4.76	11.30	8.90	2.15	20.44	9.14	14.91	757
0.03	4.70	7.38	6.87	3.32	11.45	4.06	9.08	4.42	7.33	6.54	2.73	11.93	4.60	9.09	4.75	10.64	8.20	1.81	19.46	8.82	13.71	963
0.06	4.16	5.74	5.47	3.03	8.45	2.71	6.82	3.88	5.66	5.16	2.34	8.98	3.32	6.53	4.31	8.52	6.37	0.96	16.09	7.57	9.73	1052
0.11	3.68	4.77	4.53	2.64	6.89	2.13	5.48	3.47	4.72	4.31	1.60	7.85	3.12	5.42	3.83	6.96	5.39	0.88	13.05	6.08	7.79	1119
0.15	3.15	3.82	3.71	2.65	4.99	1.17	4.27	2.96	3.68	3.56	2.46	4.89	1.22	4.17	3.18	5.43	4.29	0.24	10.62	5.19	5.82	1042
0.18	2.80	3.28	3.20	2.49	4.07	0.79	3.66	2.65	3.19	3.10	2.34	4.04	0.85	3.58	2.65	4.27	3.47	0.92	7.62	3.35	4.82	1080
0.32	2.50	2.87	2.83	2.27	3.46	0.60	3.19	2.38	2.79	2.74	2.13	3.44	0.66	3.11	2.24	3.43	2.93	0.81	6.06	2.63	3.87	1746


==> data/mlm_plots/tef/yelp/cnn/ig/ets_sts_auc.tex <==
name	auc
et_use	1.34
et_tse	1.32
et_ce	1.83


==> data/mlm_plots/tef/yelp/cnn/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.39	5.01	2.33	-9.98	20.01	15.00	4.39	5.38	13.73	9.68	0.21	27.25	13.52	16.47	5.26	16.08	10.16	-4.09	36.25	20.17	18.78	757
0.03	1.03	2.81	1.60	-4.17	9.80	6.98	2.60	6.29	12.37	9.38	2.05	22.68	10.31	14.71	5.68	15.10	9.46	-6.83	37.04	21.94	16.13	963
0.06	0.74	1.57	1.02	-1.38	4.53	2.95	1.47	6.19	10.16	8.18	2.41	17.92	7.76	11.43	5.36	12.36	7.74	-13.94	38.67	26.31	12.36	1052
0.11	0.54	0.99	0.73	-0.94	2.91	1.93	1.02	5.78	8.62	7.28	2.65	14.59	5.97	9.56	5.02	9.34	6.70	-1.59	20.27	10.93	9.75	1119
0.15	0.35	0.60	0.45	-0.40	1.60	1.00	0.62	5.29	7.50	6.26	0.68	14.33	6.82	7.95	4.54	8.01	5.61	-6.51	22.53	14.52	7.69	1042
0.18	0.24	0.38	0.32	0.00	0.75	0.38	0.42	4.81	6.16	5.69	3.94	8.39	2.22	6.93	4.22	6.01	5.10	2.54	9.49	3.48	6.68	1080
0.32	0.16	0.28	0.22	-0.25	0.81	0.53	0.30	4.37	5.61	5.10	2.80	8.41	2.81	6.17	3.79	5.71	4.53	-2.84	14.25	8.54	5.78	1746


==> data/mlm_plots/tef/yelp/cnn/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.30
et_p_h	2.42
et_p_l2	2.65


==> data/mlm_plots/tef/yelp/cnn/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.12	0.12	0.05	0.20	0.07	0.17	0.01	0.03	0.02	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.01	0.05	0.02	0.04	757
0.03	0.17	0.26	0.26	0.13	0.40	0.13	0.35	0.02	0.05	0.04	0.02	0.08	0.03	0.07	0.03	0.05	0.04	0.02	0.07	0.02	0.06	963
0.06	0.36	0.54	0.51	0.23	0.84	0.31	0.67	0.04	0.07	0.07	0.03	0.11	0.04	0.09	0.05	0.06	0.06	0.04	0.09	0.03	0.08	1052
0.11	0.61	0.85	0.81	0.46	1.25	0.40	1.05	0.06	0.09	0.09	0.05	0.13	0.04	0.11	0.06	0.08	0.08	0.05	0.11	0.03	0.10	1119
0.15	1.08	1.50	1.42	0.84	2.16	0.66	1.85	0.08	0.11	0.12	0.07	0.15	0.04	0.14	0.08	0.10	0.10	0.07	0.13	0.03	0.12	1042
0.18	1.65	2.28	2.17	1.32	3.24	0.96	2.73	0.11	0.13	0.14	0.09	0.18	0.04	0.16	0.10	0.12	0.12	0.09	0.15	0.03	0.14	1080
0.32	2.42	3.55	3.24	1.84	5.25	1.71	4.34	0.13	0.15	0.16	0.11	0.20	0.05	0.18	0.12	0.14	0.14	0.11	0.17	0.03	0.16	1746


==> data/mlm_plots/tef/yelp/cnn/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.56
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/cnn/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.96	0.96	0.97	0.95	0.98	0.02	0.98	0.95	0.96	0.97	0.94	0.99	0.03	0.98	757
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.92	0.93	0.94	0.91	0.96	0.03	0.95	0.92	0.94	0.95	0.90	0.98	0.04	0.97	963
0.06	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.88	0.90	0.90	0.86	0.93	0.03	0.92	0.88	0.91	0.92	0.86	0.96	0.05	0.95	1052
0.11	0.85	0.87	0.87	0.84	0.90	0.03	0.89	0.84	0.86	0.86	0.82	0.90	0.04	0.89	0.85	0.88	0.89	0.82	0.94	0.06	0.93	1119
0.15	0.80	0.82	0.82	0.79	0.86	0.03	0.84	0.79	0.81	0.81	0.77	0.85	0.04	0.84	0.80	0.84	0.85	0.76	0.91	0.07	0.89	1042
0.18	0.77	0.79	0.78	0.75	0.82	0.03	0.80	0.75	0.78	0.78	0.74	0.82	0.04	0.80	0.75	0.80	0.81	0.72	0.88	0.08	0.86	1080
0.32	0.73	0.75	0.75	0.71	0.78	0.03	0.77	0.71	0.74	0.73	0.70	0.78	0.04	0.76	0.69	0.75	0.76	0.65	0.84	0.09	0.81	1746


==> data/mlm_plots/tef/yelp/cnn/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/yelp/cnn/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.29	3.79	4.02	3.11	4.48	0.69	4.33	18.38	43.66	31.47	5.20	82.13	38.47	53.37	2.24	8.18	5.23	-1.42	17.77	9.60	11.15	757
0.03	4.08	4.83	4.91	3.47	6.19	1.36	5.19	23.36	55.66	42.66	10.17	101.15	45.49	73.82	2.33	9.21	5.69	-2.44	20.86	11.65	12.46	963
0.06	5.36	6.34	6.35	4.56	8.13	1.78	6.83	28.02	64.83	50.71	13.78	115.89	51.06	86.92	2.53	9.92	6.49	-2.32	22.16	12.24	12.92	1052
0.11	7.50	8.81	8.44	6.34	11.28	2.47	9.57	31.83	70.91	56.85	17.00	124.83	53.92	91.78	3.01	11.85	7.14	-4.78	28.47	16.62	14.37	1119
0.15	9.57	11.11	11.04	8.66	13.56	2.45	11.92	37.44	78.43	62.41	21.63	135.23	56.80	103.56	3.09	10.37	7.23	-0.90	21.63	11.26	14.29	1042
0.18	12.19	13.86	14.13	11.43	16.29	2.43	15.18	39.36	82.60	68.61	24.61	140.60	58.00	107.01	3.09	10.13	7.32	-0.57	20.83	10.70	14.29	1080
0.32	14.91	16.76	17.13	14.07	19.44	2.69	18.64	45.40	88.89	76.09	29.70	148.08	59.19	117.13	3.44	10.51	7.75	-0.65	21.67	11.16	14.26	1746


==> data/mlm_plots/tef/yelp/cnn/ig/time_misc_auc.tex <==
name	auc
attack_time	3.55
l2	23.63
lom	3.21


==> data/mlm_plots/tef/yelp/cnn/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.45	0.59	0.60	0.40	0.79	0.20	0.75	0.60	0.72	0.74	0.56	0.88	0.16	0.87	0.68	0.79	0.80	0.66	0.92	0.13	0.91	757
0.03	0.31	0.44	0.45	0.25	0.63	0.19	0.57	0.50	0.62	0.62	0.46	0.78	0.16	0.74	0.61	0.71	0.71	0.58	0.84	0.13	0.82	963
0.06	0.19	0.31	0.30	0.12	0.49	0.19	0.41	0.42	0.53	0.52	0.38	0.67	0.14	0.63	0.56	0.64	0.63	0.53	0.76	0.12	0.73	1052
0.11	0.12	0.23	0.22	0.06	0.40	0.17	0.33	0.36	0.45	0.45	0.32	0.58	0.13	0.54	0.51	0.59	0.58	0.49	0.70	0.11	0.67	1119
0.15	0.07	0.16	0.14	0.03	0.29	0.13	0.23	0.31	0.38	0.37	0.27	0.48	0.11	0.44	0.47	0.53	0.53	0.44	0.63	0.09	0.59	1042
0.18	0.00	0.13	0.11	-0.00	0.26	0.13	0.20	0.25	0.32	0.32	0.22	0.43	0.10	0.38	0.44	0.49	0.49	0.41	0.57	0.08	0.55	1080
0.32	0.00	0.10	0.08	-0.02	0.22	0.12	0.17	0.20	0.26	0.26	0.17	0.36	0.10	0.32	0.39	0.44	0.44	0.36	0.51	0.07	0.49	1746


==> data/mlm_plots/tef/yelp/cnn/ig/top_intersections_auc.tex <==
name	auc
top10	0.06
top30	0.12
top50	0.17


==> data/mlm_plots/tef/yelp/cnn/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	43.16	60.36	54.92	34.57	86.16	25.79	69.32	18.00	29.16	27.00	16.13	42.18	13.03	38.00	48.17	67.22	60.95	39.44	95.00	27.78	77.96	18.00	29.44	27.00	16.27	42.62	13.18	39.00	798
0.03	43.58	66.75	56.40	29.13	104.36	37.62	76.51	14.00	26.05	23.00	11.82	40.28	14.23	36.00	55.98	84.18	71.30	37.94	130.43	46.25	95.03	15.00	26.62	24.00	12.05	41.19	14.57	37.00	955
0.06	43.81	72.01	57.62	14.41	129.61	57.60	79.96	12.00	24.28	21.00	9.39	39.16	14.89	35.00	69.68	107.68	89.13	31.96	183.39	75.71	118.69	13.00	25.30	22.00	9.73	40.86	15.57	37.00	1077
0.11	43.65	73.77	57.77	11.72	135.82	62.05	81.24	13.00	24.79	21.00	9.60	39.98	15.19	36.00	84.97	134.86	108.43	33.00	236.72	101.86	145.46	13.00	26.40	23.00	10.20	42.60	16.20	39.00	1004
0.15	43.88	71.97	57.60	11.73	132.21	60.24	79.78	14.00	25.43	23.00	10.89	39.97	14.54	36.00	113.31	166.98	142.32	63.95	270.00	103.02	184.63	15.00	28.02	25.00	11.98	44.06	16.04	40.00	940
0.18	43.75	71.83	57.65	13.57	130.09	58.26	79.68	13.00	24.84	21.00	10.18	39.50	14.66	35.75	148.68	218.11	182.30	64.68	371.53	153.42	239.58	14.25	28.34	25.00	11.56	45.12	16.78	41.75	962
0.32	44.51	73.00	58.70	13.06	132.95	59.94	81.16	13.00	24.88	21.50	10.46	39.29	14.42	35.75	208.67	311.85	265.48	128.70	494.99	183.15	355.94	16.00	30.00	26.00	12.60	47.40	17.40	44.00	1842


==> data/mlm_plots/tef/yelp/cnn/s/comparison_vals_auc.tex <==
name	auc
orig_pp	22.24
orig_ge	7.79
adv_pp	59.19
adv_ge	8.67


==> data/mlm_plots/tef/yelp/cnn/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.74	0.73	0.83	0.45	1.02	0.29	0.91	0.83	0.79	0.91	0.45	1.13	0.34	0.95	0.67	0.71	0.80	0.42	0.99	0.28	0.89	798
0.03	0.64	0.70	0.75	0.49	0.92	0.21	0.84	0.76	0.79	0.85	0.59	0.99	0.20	0.90	0.61	0.67	0.71	0.48	0.86	0.19	0.78	955
0.06	0.46	0.56	0.62	0.31	0.82	0.25	0.74	0.60	0.66	0.73	0.42	0.91	0.25	0.82	0.46	0.53	0.58	0.32	0.75	0.21	0.67	1077
0.11	0.38	0.49	0.51	0.26	0.72	0.23	0.65	0.51	0.60	0.64	0.39	0.81	0.21	0.75	0.38	0.46	0.48	0.29	0.64	0.17	0.58	1004
0.15	0.24	0.38	0.37	0.16	0.60	0.22	0.52	0.35	0.47	0.49	0.25	0.69	0.22	0.62	0.25	0.35	0.35	0.19	0.51	0.16	0.45	940
0.18	0.12	0.28	0.28	0.06	0.50	0.22	0.43	0.20	0.35	0.36	0.13	0.57	0.22	0.50	0.14	0.25	0.25	0.09	0.41	0.16	0.36	962
0.32	-0.04	0.12	0.11	-0.13	0.37	0.25	0.28	-0.03	0.13	0.14	-0.12	0.39	0.26	0.30	-0.01	0.10	0.10	-0.08	0.28	0.18	0.21	1842


==> data/mlm_plots/tef/yelp/cnn/s/correlations_auc.tex <==
name	auc
pcc	0.12
spearman	0.14
kendall	0.11


==> data/mlm_plots/tef/yelp/cnn/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	1.48	5.09	2.51	-1.68	11.86	6.77	4.88	1.40	4.65	2.42	-1.66	10.96	6.31	4.51	1.45	5.08	2.77	-1.89	12.04	6.97	5.72	798
0.03	1.33	2.80	2.04	0.03	5.57	2.77	3.22	1.23	2.77	1.92	-0.17	5.70	2.93	3.16	1.47	4.24	2.66	-1.22	9.70	5.46	4.77	955
0.06	1.32	2.40	1.98	0.73	4.08	1.67	3.00	1.24	2.28	1.87	0.70	3.86	1.58	2.83	1.42	3.91	2.55	-0.98	8.80	4.89	4.21	1077
0.11	1.31	2.02	1.85	0.93	3.12	1.09	2.51	1.22	1.95	1.75	0.83	3.07	1.12	2.37	1.47	3.21	2.29	-0.61	7.02	3.82	3.75	1004
0.15	1.33	1.83	1.77	1.07	2.59	0.76	2.23	1.24	1.75	1.66	0.97	2.52	0.77	2.10	1.35	2.53	2.01	0.19	4.88	2.35	2.99	940
0.18	1.30	1.72	1.68	1.10	2.34	0.62	2.06	1.22	1.64	1.56	1.00	2.27	0.64	1.96	1.26	2.20	1.79	0.03	4.36	2.17	2.47	962
0.32	1.37	1.69	1.67	1.17	2.21	0.52	1.99	1.29	1.61	1.59	1.10	2.12	0.51	1.89	1.20	1.87	1.61	0.45	3.29	1.42	2.13	1842


==> data/mlm_plots/tef/yelp/cnn/s/ets_sts_auc.tex <==
name	auc
et_use	0.64
et_tse	0.61
et_ce	0.86


==> data/mlm_plots/tef/yelp/cnn/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.41	2.48	0.74	-4.34	9.29	6.81	1.55	1.63	6.84	2.96	-6.73	20.41	13.57	6.17	1.61	7.33	3.18	-6.33	20.98	13.66	6.61	798
0.03	0.30	0.96	0.49	-2.06	3.98	3.02	0.83	1.72	3.88	2.71	-0.25	8.01	4.13	4.54	1.57	4.41	2.64	-1.92	10.75	6.34	5.00	955
0.06	0.24	0.73	0.37	-1.37	2.82	2.10	0.58	2.00	4.21	2.98	-1.87	10.28	6.08	4.67	1.86	4.75	2.90	-3.62	13.11	8.36	4.84	1077
0.11	0.19	0.38	0.28	-0.25	1.01	0.63	0.40	2.13	3.44	2.92	1.10	5.77	2.33	4.05	1.89	3.77	2.71	-0.69	8.22	4.46	4.06	1004
0.15	0.15	0.29	0.21	-0.71	1.30	1.00	0.30	2.22	3.32	2.91	1.12	5.53	2.20	3.79	1.98	3.40	2.69	-0.02	6.82	3.42	3.67	940
0.18	0.12	0.21	0.17	-0.17	0.59	0.38	0.23	2.23	3.16	2.91	1.63	4.69	1.53	3.65	1.98	3.17	2.63	0.77	5.58	2.40	3.49	962
0.32	0.09	0.17	0.12	-0.65	0.99	0.82	0.17	2.37	3.22	2.98	0.91	5.52	2.30	3.64	2.09	3.36	2.67	-5.55	12.27	8.91	3.42	1842


==> data/mlm_plots/tef/yelp/cnn/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.14
et_p_h	1.10
et_p_l2	1.17


==> data/mlm_plots/tef/yelp/cnn/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.12	0.12	0.05	0.20	0.08	0.17	0.01	0.03	0.03	0.01	0.06	0.03	0.05	0.02	0.03	0.03	0.01	0.05	0.02	0.04	798
0.03	0.17	0.28	0.27	0.12	0.44	0.16	0.37	0.03	0.05	0.05	0.02	0.08	0.03	0.07	0.03	0.05	0.05	0.02	0.07	0.02	0.06	955
0.06	0.37	0.57	0.53	0.22	0.92	0.35	0.70	0.04	0.07	0.07	0.03	0.11	0.04	0.10	0.05	0.07	0.07	0.04	0.09	0.03	0.08	1077
0.11	0.64	0.92	0.86	0.45	1.40	0.48	1.12	0.06	0.09	0.09	0.05	0.13	0.04	0.12	0.06	0.08	0.08	0.06	0.11	0.03	0.10	1004
0.15	1.09	1.51	1.46	0.88	2.14	0.63	1.89	0.09	0.12	0.12	0.07	0.16	0.04	0.14	0.09	0.10	0.11	0.08	0.13	0.03	0.12	940
0.18	1.59	2.29	2.15	1.26	3.31	1.03	2.84	0.11	0.14	0.14	0.09	0.18	0.05	0.17	0.10	0.12	0.13	0.09	0.15	0.03	0.14	962
0.32	2.54	3.77	3.46	1.91	5.64	1.86	4.62	0.13	0.16	0.17	0.11	0.21	0.05	0.19	0.13	0.15	0.15	0.11	0.18	0.03	0.17	1842


==> data/mlm_plots/tef/yelp/cnn/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.58
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/cnn/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.96	0.97	0.95	0.98	0.02	0.98	0.95	0.96	0.97	0.93	0.99	0.03	0.98	798
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.92	0.93	0.94	0.91	0.96	0.03	0.95	0.93	0.94	0.95	0.91	0.98	0.04	0.97	955
0.06	0.88	0.90	0.90	0.87	0.93	0.03	0.92	0.88	0.89	0.90	0.86	0.93	0.03	0.92	0.89	0.91	0.92	0.86	0.97	0.05	0.95	1077
0.11	0.85	0.87	0.87	0.84	0.90	0.03	0.89	0.84	0.86	0.86	0.82	0.90	0.04	0.88	0.86	0.89	0.89	0.82	0.95	0.06	0.92	1004
0.15	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.79	0.81	0.81	0.77	0.85	0.04	0.84	0.80	0.84	0.85	0.76	0.91	0.07	0.89	940
0.18	0.76	0.79	0.78	0.75	0.82	0.03	0.80	0.75	0.77	0.77	0.73	0.81	0.04	0.80	0.75	0.79	0.80	0.71	0.88	0.08	0.85	962
0.32	0.71	0.74	0.73	0.70	0.77	0.03	0.76	0.69	0.72	0.72	0.68	0.76	0.04	0.75	0.66	0.72	0.73	0.62	0.82	0.10	0.79	1842


==> data/mlm_plots/tef/yelp/cnn/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/yelp/cnn/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	1.92	2.87	2.24	0.55	5.20	2.32	2.83	407.63	1219.38	673.18	-207.12	2645.89	1426.50	1434.93	1.67	10.22	3.74	-8.61	29.04	18.82	7.49	798
0.03	2.87	3.35	3.21	1.92	4.79	1.44	3.84	568.27	1608.28	972.11	-71.96	3288.53	1680.25	2053.49	1.89	8.14	4.03	-8.99	25.28	17.14	7.92	955
0.06	3.88	4.60	4.31	2.83	6.37	1.77	4.96	694.77	1953.97	1232.92	-16.75	3924.69	1970.72	2520.77	2.17	9.99	5.18	-7.95	27.93	17.94	9.85	1077
0.11	5.21	5.89	5.99	4.49	7.29	1.40	6.68	926.16	2339.00	1530.43	108.79	4569.22	2230.21	2975.43	2.30	8.66	5.30	-6.19	23.51	14.85	10.05	1004
0.15	6.24	7.05	7.11	5.49	8.61	1.56	7.68	1204.00	2844.90	1933.58	311.17	5378.63	2533.73	3527.25	2.81	8.35	6.21	-0.84	17.54	9.19	11.01	940
0.18	9.26	10.16	10.42	8.53	11.79	1.63	11.19	1400.88	3277.69	2231.92	376.93	6178.46	2900.76	4119.09	2.78	8.16	5.95	0.53	15.80	7.63	11.25	962
0.32	10.12	11.76	11.89	9.75	13.78	2.02	13.35	1740.05	4082.07	2882.41	733.02	7431.12	3349.05	5445.44	2.82	9.03	6.64	-0.62	18.68	9.65	12.14	1842


==> data/mlm_plots/tef/yelp/cnn/s/time_misc_auc.tex <==
name	auc
attack_time	2.49
l2	899.58
lom	2.71


==> data/mlm_plots/tef/yelp/cnn/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.45	0.57	0.64	0.32	0.83	0.26	0.76	0.75	0.78	0.83	0.58	0.97	0.20	0.89	0.83	0.86	0.90	0.71	1.00	0.14	0.95	798
0.03	0.32	0.47	0.50	0.21	0.72	0.25	0.64	0.68	0.73	0.76	0.57	0.89	0.16	0.82	0.80	0.84	0.86	0.73	0.95	0.11	0.90	955
0.06	0.11	0.33	0.33	0.07	0.60	0.26	0.50	0.54	0.61	0.64	0.43	0.79	0.18	0.73	0.72	0.77	0.79	0.64	0.90	0.13	0.85	1077
0.11	0.08	0.28	0.25	0.04	0.52	0.24	0.42	0.47	0.55	0.56	0.38	0.71	0.17	0.65	0.68	0.73	0.74	0.61	0.84	0.11	0.80	1004
0.15	0.00	0.21	0.17	-0.01	0.42	0.21	0.33	0.37	0.46	0.46	0.30	0.61	0.15	0.54	0.61	0.67	0.67	0.57	0.76	0.10	0.73	940
0.18	0.00	0.16	0.10	-0.03	0.36	0.20	0.25	0.29	0.39	0.38	0.24	0.54	0.15	0.47	0.54	0.60	0.60	0.50	0.70	0.10	0.67	962
0.32	0.00	0.13	0.05	-0.06	0.31	0.18	0.20	0.21	0.31	0.29	0.16	0.45	0.15	0.39	0.45	0.52	0.51	0.41	0.63	0.11	0.59	1842


==> data/mlm_plots/tef/yelp/cnn/s/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.15
top50	0.20


==> data/mlm_plots/tef/yelp/lstm/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.07	61.20	54.77	32.14	90.26	29.06	70.83	19.00	31.17	29.00	17.30	45.04	13.87	42.00	48.25	68.80	61.44	36.59	101.02	32.21	78.96	19.00	31.48	30.00	17.47	45.50	14.01	43.00	770
0.03	42.09	65.53	54.60	25.04	106.02	40.49	73.38	17.00	28.93	28.00	14.19	43.67	14.74	41.00	56.06	83.90	69.52	26.19	141.62	57.71	92.73	17.00	29.57	28.00	14.51	44.63	15.06	41.25	1200
0.06	41.97	66.56	54.54	22.77	110.35	43.79	74.05	18.00	31.35	32.00	16.00	46.71	15.36	45.00	65.88	101.02	83.39	29.80	172.24	71.22	110.99	19.00	32.50	33.00	16.59	48.40	15.91	47.00	1840
0.11	42.75	71.49	56.65	17.18	125.80	54.31	80.38	15.00	27.09	25.00	12.71	41.46	14.37	38.25	85.89	134.98	112.21	37.59	232.38	97.40	152.45	16.00	28.68	27.00	13.46	43.90	15.22	41.00	2032
0.15	45.55	73.61	57.79	24.94	122.27	48.66	79.74	12.00	21.50	19.00	9.45	33.54	12.05	29.00	116.41	175.74	152.34	78.48	273.01	97.26	201.80	13.00	23.34	21.00	10.35	36.33	12.99	31.00	1090
0.18	55.45	99.66	78.61	18.97	180.35	80.69	118.71	8.00	14.16	13.00	5.98	22.35	8.19	19.00	166.78	282.80	220.17	66.25	499.34	216.55	317.09	9.00	15.51	15.00	6.50	24.53	9.02	20.00	536
0.32	59.22	127.03	92.31	13.24	240.83	113.80	157.52	7.00	11.52	11.00	5.25	17.79	6.27	15.00	210.87	410.22	306.32	83.24	737.20	326.98	491.75	8.00	12.77	12.00	5.70	19.83	7.07	16.00	315


==> data/mlm_plots/tef/yelp/lstm/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	27.99
orig_ge	6.29
adv_pp	71.44
adv_ge	6.69


==> data/mlm_plots/tef/yelp/lstm/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.60	-0.19	-0.16	-0.69	0.30	0.49	0.17	-0.30	0.03	0.08	-0.41	0.47	0.44	0.37	-0.20	0.03	0.07	-0.31	0.38	0.34	0.29	770
0.03	-0.71	-0.35	-0.33	-0.78	0.08	0.43	-0.07	-0.43	-0.12	-0.09	-0.52	0.28	0.40	0.17	-0.31	-0.09	-0.06	-0.41	0.23	0.32	0.14	1200
0.06	-0.81	-0.52	-0.52	-0.85	-0.19	0.33	-0.27	-0.58	-0.29	-0.26	-0.64	0.05	0.34	-0.04	-0.43	-0.22	-0.18	-0.50	0.06	0.28	-0.02	1840
0.11	-0.65	-0.49	-0.48	-0.74	-0.24	0.25	-0.34	-0.41	-0.26	-0.25	-0.49	-0.02	0.24	-0.10	-0.28	-0.18	-0.17	-0.37	0.00	0.18	-0.06	2032
0.15	-0.63	-0.50	-0.51	-0.69	-0.31	0.19	-0.38	-0.36	-0.25	-0.25	-0.42	-0.07	0.18	-0.13	-0.26	-0.17	-0.17	-0.30	-0.04	0.13	-0.09	1090
0.18	-0.64	-0.53	-0.55	-0.71	-0.35	0.18	-0.45	-0.39	-0.29	-0.29	-0.46	-0.11	0.17	-0.19	-0.28	-0.20	-0.20	-0.33	-0.07	0.13	-0.14	536
0.32	-0.71	-0.58	-0.57	-0.74	-0.42	0.16	-0.46	-0.45	-0.34	-0.34	-0.52	-0.16	0.18	-0.22	-0.33	-0.25	-0.25	-0.39	-0.11	0.14	-0.15	315


==> data/mlm_plots/tef/yelp/lstm/ig/correlations_auc.tex <==
name	auc
pcc	-0.16
spearman	-0.08
kendall	-0.06


==> data/mlm_plots/tef/yelp/lstm/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	12.51	21.27	19.56	9.48	33.06	11.79	27.36	11.17	21.23	18.20	7.77	34.70	13.47	27.98	11.69	26.77	22.09	7.92	45.62	18.85	37.12	770
0.03	8.47	13.06	11.95	6.54	19.57	6.51	16.51	8.05	13.43	11.23	4.45	22.41	8.98	16.69	10.57	22.21	17.52	5.65	38.76	16.56	29.19	1200
0.06	6.37	8.87	8.33	5.51	12.22	3.35	10.78	6.29	8.81	8.05	5.13	12.49	3.68	10.67	7.86	15.10	11.81	3.69	26.50	11.40	18.19	1840
0.11	4.61	5.85	5.52	4.07	7.63	1.78	6.80	4.44	5.76	5.42	3.82	7.69	1.93	6.65	5.16	9.69	7.33	1.75	17.62	7.93	11.52	2032
0.15	3.79	4.53	4.35	3.34	5.71	1.19	5.00	3.62	4.45	4.23	3.13	5.76	1.32	4.94	4.07	7.34	5.77	1.00	13.68	6.34	7.41	1090
0.18	3.30	3.87	3.80	3.05	4.70	0.83	4.25	3.17	3.84	3.71	2.87	4.81	0.97	4.24	3.38	5.87	4.42	-0.17	11.92	6.05	6.32	536
0.32	3.02	3.56	3.37	2.72	4.41	0.85	3.94	2.92	3.54	3.37	2.60	4.47	0.93	3.97	2.75	5.06	3.74	-1.37	11.48	6.42	4.81	315


==> data/mlm_plots/tef/yelp/lstm/ig/ets_sts_auc.tex <==
name	auc
et_use	1.89
et_tse	1.89
et_ce	2.97


==> data/mlm_plots/tef/yelp/lstm/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.99	7.14	4.80	-2.98	17.26	10.12	8.06	12.36	22.85	18.70	6.53	39.17	16.32	28.97	11.23	25.18	19.36	3.20	47.15	21.97	32.56	770
0.03	1.74	3.42	2.43	-2.72	9.56	6.14	3.43	9.78	16.41	13.78	5.98	26.83	10.43	19.70	8.71	17.17	13.24	2.77	31.56	14.39	20.39	1200
0.06	1.03	1.86	1.47	-0.68	4.41	2.55	2.11	8.53	12.86	11.20	5.47	20.25	7.39	15.16	7.24	13.70	10.23	0.49	26.91	13.21	15.51	1840
0.11	0.62	1.14	0.80	-3.07	5.34	4.20	1.11	6.74	9.61	8.41	4.04	15.19	5.58	10.53	5.75	10.20	7.66	-1.28	21.68	11.48	10.49	2032
0.15	0.39	0.64	0.51	-0.55	1.82	1.19	0.69	5.94	8.11	7.15	3.91	12.32	4.20	8.71	5.05	8.46	6.38	0.58	16.35	7.88	8.70	1090
0.18	0.29	0.60	0.42	-0.51	1.71	1.11	0.60	5.87	8.16	7.14	4.00	12.32	4.16	8.88	5.08	10.68	6.50	-11.85	33.21	22.53	9.54	536
0.32	0.25	0.53	0.33	-0.38	1.44	0.91	0.50	5.52	8.02	6.74	3.31	12.73	4.71	8.52	4.66	10.73	6.56	-11.67	33.13	22.40	9.78	315


==> data/mlm_plots/tef/yelp/lstm/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.39
et_p_h	3.12
et_p_l2	3.63


==> data/mlm_plots/tef/yelp/lstm/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.13	0.12	0.06	0.21	0.07	0.18	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.05	770
0.03	0.20	0.29	0.29	0.14	0.45	0.15	0.37	0.03	0.06	0.05	0.02	0.09	0.03	0.08	0.03	0.05	0.05	0.03	0.07	0.02	0.07	1200
0.06	0.38	0.54	0.52	0.29	0.79	0.25	0.69	0.05	0.08	0.08	0.04	0.11	0.03	0.10	0.05	0.07	0.07	0.05	0.09	0.02	0.09	1840
0.11	0.68	0.98	0.93	0.51	1.44	0.46	1.19	0.07	0.10	0.10	0.06	0.14	0.04	0.12	0.07	0.09	0.09	0.06	0.12	0.03	0.11	2032
0.15	1.09	1.57	1.49	0.83	2.31	0.74	1.90	0.09	0.12	0.12	0.07	0.16	0.04	0.14	0.09	0.10	0.11	0.07	0.13	0.03	0.12	1090
0.18	1.27	2.09	1.80	0.85	3.33	1.24	2.63	0.08	0.12	0.11	0.06	0.17	0.05	0.15	0.09	0.11	0.11	0.07	0.14	0.03	0.13	536
0.32	1.57	2.62	2.33	1.09	4.16	1.54	3.28	0.08	0.12	0.12	0.06	0.18	0.06	0.17	0.09	0.12	0.12	0.08	0.15	0.04	0.14	315


==> data/mlm_plots/tef/yelp/lstm/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.49
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/lstm/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.96	0.97	0.98	0.94	0.99	0.02	0.98	770
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.96	0.93	0.94	0.94	0.92	0.96	0.02	0.96	0.94	0.95	0.96	0.92	0.99	0.03	0.98	1200
0.06	0.89	0.91	0.91	0.88	0.93	0.02	0.92	0.89	0.90	0.90	0.88	0.93	0.03	0.93	0.91	0.93	0.94	0.88	0.97	0.04	0.96	1840
0.11	0.85	0.87	0.87	0.84	0.90	0.03	0.89	0.84	0.86	0.86	0.83	0.90	0.04	0.89	0.86	0.89	0.90	0.83	0.95	0.06	0.93	2032
0.15	0.81	0.83	0.83	0.80	0.86	0.03	0.85	0.80	0.82	0.82	0.78	0.86	0.04	0.85	0.82	0.86	0.87	0.79	0.93	0.07	0.90	1090
0.18	0.78	0.80	0.80	0.76	0.83	0.03	0.82	0.77	0.79	0.80	0.75	0.83	0.04	0.82	0.77	0.82	0.83	0.73	0.91	0.09	0.88	536
0.32	0.75	0.77	0.77	0.73	0.81	0.04	0.80	0.73	0.77	0.76	0.72	0.81	0.05	0.79	0.71	0.77	0.78	0.66	0.88	0.11	0.85	315


==> data/mlm_plots/tef/yelp/lstm/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.26


==> data/mlm_plots/tef/yelp/lstm/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.07	3.87	3.42	1.94	5.81	1.93	4.07	28.82	760.05	74.16	-7531.43	9051.53	8291.48	292.51	6.48	21.87	15.62	1.01	42.74	20.87	32.33	770
0.03	6.91	9.05	7.52	5.16	12.94	3.89	9.88	36.23	26659.05	115.62	-666181.83	719499.93	692840.88	526.89	4.52	23.16	13.83	-1.61	47.92	24.77	35.27	1200
0.06	10.98	13.58	13.12	9.96	17.20	3.62	16.07	49.98	15943.72	162.02	-197870.20	229757.64	213813.92	685.63	7.76	26.61	21.81	2.82	50.41	23.80	37.61	1840
0.11	13.79	15.73	15.33	12.78	18.68	2.95	17.63	41.22	16220.42	81.85	-202954.05	235394.90	219174.47	183.36	5.64	20.66	16.09	2.23	39.08	18.42	31.93	2032
0.15	13.79	15.83	15.34	12.74	18.92	3.09	17.65	33.01	1641.90	52.16	-18230.50	21514.31	19872.40	82.97	3.51	13.86	9.38	-0.22	27.94	14.08	21.34	1090
0.18	14.45	16.44	16.15	13.22	19.67	3.23	18.05	26.84	70.90	40.31	-193.86	335.65	264.75	60.51	2.12	7.30	4.98	0.45	14.15	6.85	10.54	536
0.32	13.24	14.95	14.69	12.30	17.60	2.65	16.99	25.35	68.95	37.98	-153.09	290.99	222.04	56.67	1.58	5.69	4.26	-0.02	11.40	5.71	7.62	315


==> data/mlm_plots/tef/yelp/lstm/ig/time_misc_auc.tex <==
name	auc
attack_time	4.53
l2	2085.10
lom	4.30


==> data/mlm_plots/tef/yelp/lstm/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.05	0.23	0.18	0.02	0.45	0.22	0.40	0.21	0.38	0.38	0.17	0.59	0.21	0.54	0.42	0.53	0.55	0.36	0.70	0.17	0.67	770
0.03	0.00	0.15	0.09	-0.03	0.32	0.17	0.23	0.15	0.31	0.31	0.12	0.50	0.19	0.44	0.36	0.47	0.47	0.31	0.63	0.16	0.60	1200
0.06	0.00	0.08	0.05	-0.04	0.20	0.12	0.14	0.09	0.23	0.22	0.07	0.38	0.15	0.33	0.31	0.41	0.42	0.26	0.55	0.14	0.50	1840
0.11	0.00	0.08	0.05	-0.03	0.19	0.11	0.13	0.16	0.24	0.23	0.12	0.35	0.12	0.31	0.37	0.43	0.43	0.32	0.53	0.10	0.50	2032
0.15	0.00	0.06	0.00	-0.03	0.16	0.09	0.12	0.18	0.25	0.25	0.14	0.35	0.11	0.31	0.39	0.43	0.43	0.36	0.51	0.08	0.49	1090
0.18	0.00	0.05	0.00	-0.04	0.13	0.09	0.08	0.15	0.22	0.22	0.11	0.33	0.11	0.28	0.37	0.42	0.42	0.33	0.51	0.09	0.47	536
0.32	0.00	0.03	0.00	-0.05	0.12	0.09	0.00	0.13	0.20	0.20	0.08	0.32	0.12	0.28	0.36	0.41	0.41	0.31	0.51	0.10	0.47	315


==> data/mlm_plots/tef/yelp/lstm/ig/top_intersections_auc.tex <==
name	auc
top10	0.02
top30	0.07
top50	0.13


==> data/mlm_plots/tef/yelp/lstm/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.07	61.24	53.71	30.48	92.00	30.76	70.86	18.00	29.59	28.00	16.14	43.04	13.45	41.00	46.43	66.98	59.73	34.06	99.90	32.92	79.12	18.00	29.82	28.00	16.30	43.34	13.52	41.00	1140
0.03	43.33	71.40	57.03	25.37	117.43	46.03	83.10	12.00	24.28	21.00	9.73	38.82	14.55	35.00	56.95	90.24	74.73	32.73	147.75	57.51	103.78	12.00	24.79	21.00	9.92	39.66	14.87	36.00	894
0.06	45.06	82.83	60.94	-7.04	172.69	89.86	88.67	12.00	24.14	21.00	9.34	38.94	14.80	35.00	73.31	124.38	93.45	24.31	224.45	100.07	137.97	12.00	25.01	21.50	9.65	40.37	15.36	36.00	916
0.11	45.54	84.79	62.46	-12.67	182.25	97.46	90.56	11.00	23.91	21.00	9.07	38.75	14.84	35.00	91.51	153.15	118.55	14.48	291.83	138.68	171.23	12.00	25.25	22.00	9.58	40.91	15.67	37.00	1041
0.15	42.78	73.45	56.80	15.47	131.42	57.98	79.65	15.00	26.26	24.00	12.03	40.49	14.23	37.00	120.08	180.97	156.35	77.71	284.23	103.26	206.27	16.00	28.80	26.00	13.15	44.46	15.65	40.00	1191
0.18	43.58	71.35	55.47	20.06	122.64	51.29	78.58	14.00	26.79	24.00	11.91	41.66	14.87	39.00	150.49	226.42	186.41	76.44	376.40	149.98	248.95	15.00	29.94	28.00	13.35	46.54	16.60	44.00	1119
0.32	48.50	84.04	62.26	23.38	144.71	60.67	93.82	11.00	21.86	18.00	7.74	35.98	14.12	31.50	189.83	323.14	253.43	93.23	553.06	229.92	369.13	12.00	24.90	21.00	8.99	40.81	15.91	35.50	807


==> data/mlm_plots/tef/yelp/lstm/s/comparison_vals_auc.tex <==
name	auc
orig_pp	24.03
orig_ge	7.70
adv_pp	62.82
adv_ge	8.38


==> data/mlm_plots/tef/yelp/lstm/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.00	0.27	0.26	-0.01	0.55	0.28	0.53	0.03	0.39	0.55	-0.03	0.81	0.42	0.77	0.00	0.31	0.39	0.01	0.62	0.31	0.60	1140
0.03	0.19	0.31	0.32	0.12	0.51	0.20	0.46	0.47	0.55	0.61	0.29	0.81	0.26	0.72	0.34	0.41	0.45	0.22	0.61	0.20	0.54	894
0.06	0.10	0.21	0.19	0.03	0.38	0.18	0.32	0.33	0.45	0.47	0.22	0.68	0.23	0.60	0.23	0.32	0.33	0.16	0.49	0.17	0.44	916
0.11	0.01	0.11	0.10	-0.05	0.27	0.16	0.20	0.18	0.32	0.34	0.09	0.55	0.23	0.48	0.13	0.23	0.23	0.06	0.39	0.17	0.34	1041
0.15	-0.09	-0.01	-0.02	-0.15	0.14	0.14	0.07	-0.01	0.14	0.14	-0.09	0.36	0.22	0.29	-0.01	0.10	0.10	-0.06	0.25	0.15	0.19	1191
0.18	-0.13	-0.05	-0.07	-0.19	0.08	0.13	0.01	-0.10	0.04	0.03	-0.17	0.25	0.21	0.16	-0.06	0.03	0.02	-0.12	0.18	0.15	0.11	1119
0.32	-0.18	-0.10	-0.11	-0.23	0.04	0.14	-0.03	-0.17	-0.02	-0.06	-0.24	0.19	0.22	0.10	-0.11	-0.01	-0.04	-0.16	0.14	0.15	0.07	807


==> data/mlm_plots/tef/yelp/lstm/s/correlations_auc.tex <==
name	auc
pcc	0.01
spearman	0.06
kendall	0.04


==> data/mlm_plots/tef/yelp/lstm/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	7.09	17.35	12.35	4.59	30.10	12.76	26.78	6.78	15.88	12.29	4.66	27.09	11.22	23.35	7.15	18.54	13.21	4.45	32.62	14.09	27.71	1140
0.03	4.36	6.77	5.71	2.67	10.87	4.10	8.00	4.08	6.93	5.35	1.16	12.71	5.77	7.54	4.54	10.94	7.37	1.43	20.45	9.51	13.87	894
0.06	3.24	4.45	4.17	2.62	6.28	1.83	5.21	3.09	4.37	3.99	2.24	6.50	2.13	4.99	3.59	7.72	5.43	0.47	14.96	7.25	8.65	916
0.11	2.78	3.53	3.40	2.35	4.71	1.18	4.03	2.64	3.46	3.23	2.16	4.77	1.30	3.99	3.06	6.00	4.45	0.47	11.52	5.52	6.51	1041
0.15	2.50	2.91	2.80	2.20	3.63	0.72	3.17	2.34	2.81	2.72	2.03	3.60	0.78	3.07	2.62	4.26	3.56	1.24	7.28	3.02	4.79	1191
0.18	2.30	2.59	2.53	2.07	3.12	0.52	2.81	2.17	2.51	2.44	1.95	3.07	0.56	2.76	2.36	3.52	3.00	0.74	6.29	2.77	3.93	1119
0.32	2.13	2.38	2.34	1.92	2.84	0.46	2.61	2.03	2.32	2.26	1.81	2.83	0.51	2.52	1.97	3.19	2.49	0.00	6.37	3.18	3.30	807


==> data/mlm_plots/tef/yelp/lstm/s/ets_sts_auc.tex <==
name	auc
et_use	1.17
et_tse	1.14
et_ce	1.71


==> data/mlm_plots/tef/yelp/lstm/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.77	10.99	4.15	-19.64	41.61	30.63	8.60	7.18	25.87	13.67	-3.37	55.12	29.25	29.65	7.05	29.99	16.03	-7.50	67.48	37.49	31.11	1140
0.03	0.85	2.40	1.18	-3.45	8.26	5.86	1.84	5.13	10.39	7.22	-1.07	21.85	11.46	11.36	4.47	12.28	7.45	-3.65	28.22	15.93	12.59	894
0.06	0.52	1.06	0.70	-1.28	3.41	2.35	0.97	4.55	7.37	5.90	1.71	13.02	5.66	8.15	3.97	8.44	5.61	-4.03	20.91	12.47	8.67	916
0.11	0.37	1.22	0.49	-7.09	9.52	8.30	0.65	4.21	7.01	5.21	-2.74	16.77	9.75	6.68	3.57	9.74	4.66	-20.24	39.73	29.98	7.06	1041
0.15	0.24	0.36	0.30	0.11	0.62	0.26	0.39	3.86	5.08	4.52	2.20	7.96	2.88	5.44	3.33	5.96	4.04	-14.91	26.82	20.86	5.19	1191
0.18	0.18	0.26	0.23	0.08	0.45	0.18	0.30	3.69	4.65	4.29	2.90	6.41	1.75	5.07	3.18	5.07	3.82	-3.55	13.69	8.62	4.87	1119
0.32	0.14	0.28	0.19	-0.74	1.29	1.01	0.25	3.56	4.66	4.18	1.98	7.34	2.68	4.98	3.05	5.50	3.75	-6.95	17.95	12.45	4.94	807


==> data/mlm_plots/tef/yelp/lstm/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.32
et_p_h	2.03
et_p_l2	2.41


==> data/mlm_plots/tef/yelp/lstm/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.05	0.10	0.08	0.03	0.18	0.07	0.14	0.01	0.03	0.02	0.00	0.06	0.03	0.04	0.01	0.03	0.02	0.01	0.05	0.02	0.04	1140
0.03	0.20	0.29	0.28	0.14	0.44	0.15	0.39	0.02	0.05	0.04	0.02	0.08	0.03	0.07	0.03	0.05	0.05	0.02	0.07	0.02	0.06	894
0.06	0.41	0.60	0.56	0.24	0.96	0.36	0.72	0.04	0.07	0.07	0.03	0.11	0.04	0.10	0.05	0.07	0.07	0.04	0.09	0.03	0.08	916
0.11	0.68	0.96	0.91	0.50	1.43	0.46	1.19	0.06	0.09	0.10	0.05	0.14	0.04	0.12	0.06	0.08	0.09	0.06	0.11	0.03	0.10	1041
0.15	1.25	1.71	1.66	1.03	2.38	0.68	2.07	0.10	0.12	0.13	0.08	0.17	0.04	0.15	0.09	0.11	0.11	0.08	0.14	0.03	0.13	1191
0.18	1.77	2.40	2.28	1.43	3.37	0.97	2.89	0.11	0.14	0.14	0.09	0.18	0.04	0.16	0.11	0.12	0.12	0.09	0.15	0.03	0.14	1119
0.32	2.20	3.20	2.87	1.58	4.81	1.62	3.86	0.11	0.14	0.15	0.09	0.20	0.05	0.18	0.11	0.13	0.13	0.10	0.17	0.03	0.15	807


==> data/mlm_plots/tef/yelp/lstm/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.56
pp_l2_d	0.03
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/lstm/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.99	0.01	0.98	0.96	0.97	0.97	0.95	0.99	0.02	0.98	0.96	0.97	0.98	0.95	0.99	0.02	0.99	1140
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.96	0.92	0.94	0.94	0.91	0.96	0.03	0.95	0.93	0.95	0.96	0.91	0.99	0.04	0.98	894
0.06	0.89	0.90	0.90	0.88	0.93	0.03	0.92	0.88	0.90	0.90	0.86	0.93	0.03	0.92	0.90	0.92	0.93	0.86	0.98	0.06	0.96	916
0.11	0.85	0.87	0.87	0.83	0.90	0.03	0.89	0.84	0.86	0.86	0.82	0.90	0.04	0.89	0.86	0.89	0.90	0.82	0.95	0.07	0.93	1041
0.15	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.79	0.81	0.81	0.78	0.85	0.04	0.84	0.81	0.85	0.86	0.79	0.91	0.06	0.89	1191
0.18	0.77	0.79	0.79	0.76	0.82	0.03	0.81	0.76	0.78	0.78	0.75	0.82	0.04	0.81	0.77	0.82	0.82	0.74	0.89	0.07	0.86	1119
0.32	0.74	0.76	0.76	0.73	0.80	0.03	0.78	0.73	0.76	0.76	0.72	0.80	0.04	0.78	0.72	0.77	0.78	0.68	0.87	0.10	0.84	807


==> data/mlm_plots/tef/yelp/lstm/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.26


==> data/mlm_plots/tef/yelp/lstm/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	4.68	7.62	6.40	3.83	11.42	3.80	10.17	495.66	1905.03	1079.50	-2583.81	6393.86	4488.83	2464.81	7.02	38.29	24.45	-0.02	76.60	38.31	64.26	1140
0.03	4.47	5.90	5.32	3.58	8.22	2.32	6.38	951.24	49931.21	1789.76	-552770.50	652632.92	602701.71	3156.25	3.45	13.51	9.13	-1.22	28.25	14.73	19.34	894
0.06	6.19	7.36	6.92	5.43	9.30	1.94	8.24	1302.46	13286.10	2348.41	-139152.17	165724.37	152438.27	4317.05	3.59	14.53	8.61	-3.17	32.24	17.70	18.76	916
0.11	8.60	10.30	10.23	7.75	12.85	2.55	11.86	1764.60	84469.88	2981.75	-604932.96	773872.71	689402.83	5469.30	3.85	16.40	9.75	-2.78	35.58	19.18	21.83	1041
0.15	11.46	12.87	12.79	10.70	15.03	2.17	14.39	2321.23	9511.33	3734.15	-35151.70	54174.35	44663.02	6337.00	5.10	17.28	12.27	0.93	33.64	16.35	24.54	1191
0.18	12.11	13.80	13.51	11.66	15.95	2.14	14.97	2405.24	28311.87	4096.75	-228276.51	284900.24	256588.37	7058.03	5.23	18.37	12.46	-0.37	37.11	18.74	25.27	1119
0.32	11.80	13.52	13.51	11.46	15.58	2.06	14.76	1889.81	13188.36	3422.48	-220603.30	246980.01	233791.66	5853.96	4.02	14.11	9.78	0.03	28.19	14.08	20.45	807


==> data/mlm_plots/tef/yelp/lstm/s/time_misc_auc.tex <==
name	auc
attack_time	3.57
l2	9256.84
lom	5.22


==> data/mlm_plots/tef/yelp/lstm/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.00	0.28	0.27	0.04	0.51	0.23	0.46	0.27	0.49	0.54	0.26	0.73	0.24	0.71	0.52	0.67	0.69	0.50	0.83	0.16	0.81	1140
0.03	0.14	0.27	0.27	0.09	0.45	0.18	0.40	0.48	0.55	0.58	0.40	0.71	0.15	0.65	0.68	0.71	0.73	0.59	0.83	0.12	0.79	894
0.06	0.00	0.18	0.17	0.01	0.35	0.17	0.27	0.41	0.48	0.49	0.34	0.61	0.14	0.56	0.62	0.67	0.68	0.56	0.77	0.11	0.73	916
0.11	0.00	0.11	0.09	-0.02	0.24	0.13	0.18	0.32	0.40	0.41	0.26	0.54	0.14	0.49	0.56	0.62	0.62	0.52	0.71	0.10	0.68	1041
0.15	0.00	0.06	0.00	-0.04	0.16	0.10	0.09	0.24	0.31	0.31	0.19	0.43	0.12	0.38	0.49	0.55	0.54	0.45	0.64	0.09	0.60	1191
0.18	0.00	0.04	0.00	-0.04	0.11	0.07	0.05	0.20	0.27	0.26	0.16	0.37	0.11	0.32	0.45	0.51	0.50	0.42	0.60	0.09	0.55	1119
0.32	0.00	0.03	0.00	-0.03	0.09	0.06	0.00	0.15	0.23	0.23	0.12	0.34	0.11	0.30	0.42	0.48	0.48	0.38	0.58	0.10	0.53	807


==> data/mlm_plots/tef/yelp/lstm/s/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.11
top50	0.17


==> data/mlm_plots/tef/yelp/lstmatt/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	41.68	60.29	53.71	32.49	88.09	27.80	70.19	19.00	30.14	29.00	16.79	43.50	13.35	41.00	47.83	67.95	60.40	38.04	97.85	29.90	78.93	19.00	30.49	29.00	17.02	43.97	13.48	42.00	754
0.03	43.07	69.77	56.68	22.05	117.49	47.72	78.60	14.00	26.50	24.00	12.10	40.90	14.40	38.00	56.44	89.57	74.24	24.26	154.88	65.31	99.40	15.00	27.11	25.00	12.36	41.86	14.75	39.00	950
0.06	43.57	75.63	57.90	9.49	141.76	66.14	82.70	13.00	25.12	22.00	10.36	39.89	14.77	37.00	69.62	114.96	91.25	15.49	214.42	99.46	126.89	13.00	26.12	23.00	10.74	41.51	15.38	38.00	1020
0.11	43.77	79.02	58.58	-10.69	168.73	89.71	83.30	12.75	25.02	22.00	10.18	39.86	14.84	37.00	87.07	142.58	110.19	21.11	264.05	121.47	152.85	13.00	26.48	23.00	10.79	42.17	15.69	39.00	1024
0.15	43.54	76.77	57.25	-15.88	169.43	92.65	79.78	14.00	26.02	24.00	11.35	40.69	14.67	38.00	116.50	174.81	147.16	58.77	290.85	116.04	196.59	15.00	28.36	26.00	12.39	44.33	15.97	41.00	984
0.18	43.28	72.41	57.02	15.10	129.72	57.31	79.91	13.00	25.50	23.00	10.95	40.06	14.55	37.00	151.07	224.62	193.98	90.77	358.48	133.86	254.95	15.00	28.65	26.00	12.39	44.91	16.26	42.00	1031
0.32	43.57	73.72	57.74	19.37	128.08	54.36	81.32	13.00	25.54	23.00	10.94	40.13	14.59	37.00	210.50	319.97	271.08	142.70	497.23	177.27	371.22	15.00	29.88	27.00	12.84	46.91	17.03	44.00	1952


==> data/mlm_plots/tef/yelp/lstmatt/a/comparison_vals_auc.tex <==
name	auc
orig_pp	22.97
orig_ge	7.98
adv_pp	61.37
adv_ge	8.75


==> data/mlm_plots/tef/yelp/lstmatt/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.34	0.51	0.52	0.26	0.76	0.25	0.70	0.96	0.97	0.97	0.94	0.99	0.02	0.98	0.85	0.87	0.88	0.82	0.92	0.05	0.91	754
0.03	0.17	0.39	0.37	0.13	0.64	0.25	0.56	0.92	0.94	0.94	0.90	0.97	0.03	0.96	0.78	0.82	0.82	0.76	0.87	0.06	0.85	950
0.06	0.09	0.27	0.22	0.05	0.50	0.22	0.41	0.87	0.90	0.91	0.84	0.95	0.05	0.93	0.71	0.75	0.75	0.68	0.82	0.07	0.79	1020
0.11	0.05	0.20	0.14	0.00	0.39	0.20	0.28	0.83	0.85	0.87	0.78	0.92	0.07	0.90	0.65	0.69	0.70	0.61	0.77	0.08	0.74	1024
0.15	0.01	0.13	0.07	-0.04	0.29	0.17	0.19	0.76	0.79	0.81	0.70	0.89	0.09	0.85	0.58	0.62	0.62	0.53	0.71	0.09	0.67	984
0.18	-0.00	0.09	0.04	-0.06	0.24	0.15	0.13	0.69	0.74	0.75	0.64	0.83	0.09	0.80	0.50	0.55	0.56	0.47	0.64	0.09	0.61	1031
0.32	-0.02	0.05	0.01	-0.08	0.17	0.12	0.07	0.58	0.65	0.66	0.53	0.76	0.12	0.73	0.41	0.47	0.48	0.37	0.57	0.10	0.54	1952


==> data/mlm_plots/tef/yelp/lstmatt/a/correlations_auc.tex <==
name	auc
pcc	0.05
spearman	0.24
kendall	0.19


==> data/mlm_plots/tef/yelp/lstmatt/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	4.37	8.02	7.29	3.16	12.88	4.86	10.73	3.84	7.56	6.79	2.79	12.33	4.77	10.20	3.96	9.28	7.12	2.11	16.44	7.17	13.04	754
0.03	3.57	5.50	5.11	2.57	8.43	2.93	7.04	3.22	5.24	4.83	2.27	8.21	2.97	6.80	3.39	7.71	6.02	1.59	13.84	6.12	10.32	950
0.06	2.87	4.02	3.84	2.21	5.84	1.81	5.00	2.64	3.82	3.64	2.03	5.60	1.79	4.72	2.83	6.03	4.67	0.86	11.20	5.17	7.19	1020
0.11	2.52	3.20	3.14	2.02	4.38	1.18	3.82	2.29	3.03	2.97	1.86	4.21	1.18	3.63	2.40	4.46	3.53	0.68	8.24	3.78	5.24	1024
0.15	2.13	2.50	2.51	1.81	3.20	0.70	2.88	1.98	2.38	2.36	1.67	3.09	0.71	2.77	2.00	3.25	2.72	0.63	5.86	2.61	3.76	984
0.18	1.89	2.13	2.14	1.65	2.61	0.48	2.39	1.77	2.03	2.03	1.53	2.52	0.49	2.29	1.70	2.55	2.23	0.47	4.63	2.08	3.01	1031
0.32	1.68	1.84	1.83	1.51	2.18	0.33	2.00	1.59	1.77	1.75	1.42	2.12	0.35	1.93	1.41	2.04	1.79	0.51	3.58	1.53	2.34	1952


==> data/mlm_plots/tef/yelp/lstmatt/a/ets_sts_auc.tex <==
name	auc
et_use	0.92
et_tse	0.88
et_ce	1.20


==> data/mlm_plots/tef/yelp/lstmatt/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.09	3.26	1.86	-5.23	11.74	8.49	3.09	4.56	9.24	7.50	2.09	16.39	7.15	11.47	4.44	10.31	7.70	0.37	20.25	9.94	12.78	754
0.03	0.73	1.60	1.06	-2.07	5.26	3.66	1.51	4.42	7.76	6.25	0.40	15.11	7.36	8.89	3.93	9.63	6.18	-7.23	26.49	16.86	9.65	950
0.06	0.47	1.13	0.67	-3.09	5.36	4.23	0.94	4.20	6.39	5.43	1.88	10.90	4.51	7.33	3.67	7.06	5.06	-2.07	16.19	9.13	7.49	1020
0.11	0.34	0.59	0.46	-0.25	1.44	0.84	0.64	3.88	5.46	4.84	2.06	8.85	3.39	6.00	3.40	5.72	4.31	0.13	11.31	5.59	6.10	1024
0.15	0.22	0.43	0.29	-0.85	1.71	1.28	0.39	3.52	4.59	4.12	2.19	7.00	2.40	4.96	2.97	4.86	3.67	-0.47	10.19	5.33	4.79	984
0.18	0.15	0.24	0.20	-0.06	0.53	0.29	0.27	3.20	3.98	3.66	2.44	5.51	1.53	4.37	2.71	4.03	3.26	0.84	7.22	3.19	4.15	1031
0.32	0.10	0.16	0.13	0.03	0.29	0.13	0.18	2.90	3.58	3.31	2.16	4.99	1.41	3.84	2.48	3.59	2.93	0.14	7.03	3.45	3.56	1952


==> data/mlm_plots/tef/yelp/lstmatt/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.19
et_p_h	1.54
et_p_l2	1.65


==> data/mlm_plots/tef/yelp/lstmatt/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.14	0.13	0.06	0.21	0.08	0.19	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.05	754
0.03	0.20	0.30	0.29	0.14	0.47	0.16	0.40	0.03	0.05	0.05	0.02	0.09	0.03	0.08	0.03	0.05	0.05	0.03	0.07	0.02	0.07	950
0.06	0.40	0.59	0.56	0.25	0.93	0.34	0.73	0.05	0.08	0.07	0.04	0.11	0.04	0.10	0.05	0.07	0.07	0.04	0.09	0.03	0.09	1020
0.11	0.65	0.94	0.90	0.48	1.40	0.46	1.17	0.07	0.10	0.10	0.05	0.14	0.04	0.12	0.07	0.09	0.09	0.06	0.11	0.03	0.10	1024
0.15	1.15	1.58	1.54	0.90	2.25	0.68	1.94	0.09	0.12	0.12	0.07	0.16	0.04	0.15	0.09	0.11	0.11	0.08	0.14	0.03	0.12	984
0.18	1.72	2.42	2.29	1.38	3.45	1.03	2.97	0.11	0.14	0.14	0.09	0.18	0.05	0.17	0.11	0.12	0.13	0.09	0.15	0.03	0.14	1031
0.32	2.59	3.89	3.55	1.94	5.83	1.94	4.74	0.13	0.16	0.17	0.11	0.21	0.05	0.19	0.13	0.14	0.15	0.11	0.18	0.03	0.17	1952


==> data/mlm_plots/tef/yelp/lstmatt/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.60
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/lstmatt/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.95	0.96	0.97	0.94	0.98	0.02	0.97	0.95	0.96	0.97	0.94	0.99	0.03	0.98	754
0.03	0.93	0.94	0.94	0.91	0.96	0.02	0.95	0.92	0.93	0.94	0.90	0.96	0.03	0.95	0.92	0.94	0.95	0.89	0.99	0.05	0.97	950
0.06	0.89	0.90	0.90	0.87	0.93	0.03	0.92	0.87	0.89	0.90	0.86	0.93	0.04	0.92	0.88	0.91	0.92	0.84	0.97	0.06	0.95	1020
0.11	0.85	0.87	0.87	0.83	0.90	0.03	0.89	0.83	0.86	0.86	0.82	0.90	0.04	0.88	0.83	0.87	0.88	0.80	0.94	0.07	0.92	1024
0.15	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.78	0.81	0.81	0.77	0.85	0.04	0.83	0.78	0.83	0.84	0.75	0.91	0.08	0.88	984
0.18	0.76	0.78	0.78	0.75	0.81	0.03	0.80	0.75	0.77	0.77	0.73	0.81	0.04	0.79	0.74	0.78	0.79	0.70	0.87	0.08	0.84	1031
0.32	0.72	0.74	0.74	0.70	0.77	0.03	0.76	0.70	0.73	0.72	0.69	0.76	0.04	0.75	0.66	0.73	0.73	0.63	0.82	0.10	0.80	1952


==> data/mlm_plots/tef/yelp/lstmatt/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/yelp/lstmatt/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	1.92	2.17	2.17	1.84	2.50	0.33	2.39	0.26	0.40	0.35	0.19	0.61	0.21	0.49	5.19	20.14	12.26	-2.34	42.62	22.48	26.81	754
0.03	2.67	2.95	2.89	2.50	3.41	0.46	3.29	0.32	0.47	0.44	0.26	0.68	0.21	0.59	5.03	20.86	12.83	-2.85	44.57	23.71	27.81	950
0.06	3.76	4.50	4.10	2.82	6.18	1.68	4.51	0.40	0.54	0.51	0.34	0.75	0.20	0.67	5.31	22.00	13.11	-2.71	46.72	24.72	30.05	1020
0.11	9.60	11.58	11.56	9.59	13.56	1.98	12.96	0.46	0.60	0.58	0.41	0.80	0.20	0.73	5.53	23.75	14.61	-2.28	49.79	26.03	32.27	1024
0.15	7.49	8.40	8.40	7.03	9.77	1.37	9.10	0.51	0.65	0.63	0.46	0.84	0.19	0.79	6.77	26.37	16.94	-0.89	53.64	27.27	36.33	984
0.18	10.04	11.31	11.22	9.78	12.85	1.54	12.35	0.52	0.67	0.65	0.48	0.85	0.19	0.80	7.10	26.52	17.97	-0.21	53.25	26.73	35.18	1031
0.32	12.61	14.49	14.34	12.03	16.96	2.47	16.10	0.52	0.66	0.63	0.47	0.84	0.18	0.78	7.65	26.31	17.72	-0.14	52.75	26.44	34.98	1952


==> data/mlm_plots/tef/yelp/lstmatt/a/time_misc_auc.tex <==
name	auc
attack_time	3.06
l2	0.19
lom	7.71


==> data/mlm_plots/tef/yelp/lstmatt/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.77	0.82	0.83	0.72	0.92	0.10	0.89	0.88	0.91	0.91	0.87	0.96	0.05	0.94	0.93	0.94	0.94	0.91	0.97	0.03	0.96	754
0.03	0.64	0.72	0.73	0.57	0.86	0.15	0.82	0.83	0.87	0.87	0.81	0.93	0.06	0.91	0.89	0.91	0.92	0.87	0.95	0.04	0.94	950
0.06	0.50	0.58	0.61	0.38	0.78	0.20	0.70	0.78	0.82	0.82	0.74	0.89	0.08	0.86	0.86	0.88	0.89	0.83	0.94	0.05	0.91	1020
0.11	0.40	0.50	0.50	0.30	0.70	0.20	0.64	0.73	0.77	0.78	0.67	0.87	0.10	0.82	0.83	0.86	0.86	0.81	0.91	0.05	0.89	1024
0.15	0.31	0.42	0.43	0.22	0.61	0.20	0.55	0.68	0.72	0.73	0.64	0.80	0.08	0.77	0.79	0.82	0.82	0.76	0.88	0.06	0.86	984
0.18	0.22	0.34	0.33	0.14	0.54	0.20	0.47	0.62	0.67	0.68	0.58	0.77	0.10	0.73	0.76	0.79	0.79	0.73	0.85	0.06	0.83	1031
0.32	0.09	0.26	0.25	0.06	0.45	0.20	0.40	0.55	0.61	0.62	0.50	0.72	0.11	0.68	0.71	0.75	0.75	0.69	0.81	0.06	0.79	1952


==> data/mlm_plots/tef/yelp/lstmatt/a/top_intersections_auc.tex <==
name	auc
top10	0.13
top30	0.22
top50	0.26


==> data/mlm_plots/tef/yelp/lstmatt/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	42.00	60.88	53.84	32.22	89.54	28.66	70.79	19.00	30.30	29.00	16.95	43.65	13.35	41.00	48.03	68.58	60.77	37.02	100.15	31.57	79.88	19.00	30.60	29.00	17.15	44.05	13.45	41.75	730
0.03	43.05	70.10	56.71	21.94	118.26	48.16	78.86	14.00	26.48	24.00	12.09	40.86	14.38	38.00	56.78	89.57	73.89	26.67	152.46	62.90	97.14	14.50	27.06	25.00	12.38	41.75	14.68	39.00	955
0.06	43.62	75.15	57.95	9.89	140.42	65.27	82.21	13.00	25.17	22.00	10.41	39.93	14.76	37.00	69.61	113.68	90.73	18.74	208.63	94.95	122.62	13.00	26.13	23.00	10.83	41.43	15.30	38.00	1021
0.11	43.68	76.94	58.05	-0.49	154.36	77.43	82.92	12.00	25.07	22.00	10.23	39.91	14.84	37.00	84.70	141.03	111.37	6.98	275.07	134.05	147.43	13.00	26.48	24.00	10.84	42.11	15.64	39.00	1028
0.15	43.56	72.80	57.10	18.73	126.87	54.07	79.93	14.00	25.98	24.00	11.38	40.57	14.59	38.00	112.23	169.28	142.27	70.97	267.59	98.31	186.07	15.00	28.25	25.00	12.47	44.02	15.78	41.00	974
0.18	43.06	72.64	56.99	17.48	127.81	55.17	80.31	13.00	25.83	24.00	11.13	40.53	14.70	37.00	145.98	218.28	186.25	84.62	351.95	133.67	246.08	15.00	28.92	26.00	12.55	45.29	16.37	42.00	1059
0.32	43.74	74.23	58.57	19.67	128.78	54.56	81.35	13.00	25.44	23.00	10.87	40.01	14.57	37.00	196.57	299.39	249.94	126.95	471.84	172.45	344.33	15.00	29.36	26.00	12.76	45.96	16.60	43.00	1909


==> data/mlm_plots/tef/yelp/lstmatt/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	22.77
orig_ge	8.00
adv_pp	59.11
adv_ge	8.74


==> data/mlm_plots/tef/yelp/lstmatt/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.25	0.46	0.52	0.13	0.80	0.33	0.72	0.53	0.65	0.67	0.45	0.84	0.19	0.79	0.41	0.53	0.54	0.36	0.70	0.17	0.65	730
0.03	0.04	0.28	0.31	-0.07	0.63	0.35	0.54	0.37	0.50	0.51	0.29	0.71	0.21	0.64	0.28	0.40	0.40	0.22	0.57	0.18	0.51	955
0.06	-0.12	0.10	0.09	-0.23	0.44	0.33	0.32	0.21	0.34	0.34	0.13	0.55	0.21	0.48	0.16	0.27	0.26	0.10	0.43	0.17	0.37	1021
0.11	-0.25	-0.03	-0.05	-0.35	0.29	0.32	0.17	0.08	0.21	0.21	0.00	0.42	0.21	0.34	0.07	0.17	0.17	0.01	0.33	0.16	0.27	1028
0.15	-0.36	-0.18	-0.19	-0.46	0.10	0.28	-0.02	-0.06	0.07	0.06	-0.12	0.25	0.18	0.18	-0.03	0.06	0.05	-0.08	0.19	0.14	0.14	974
0.18	-0.44	-0.26	-0.28	-0.53	0.00	0.26	-0.12	-0.14	-0.03	-0.03	-0.21	0.16	0.18	0.08	-0.10	-0.01	-0.02	-0.14	0.12	0.13	0.07	1059
0.32	-0.49	-0.33	-0.35	-0.57	-0.10	0.24	-0.20	-0.23	-0.11	-0.12	-0.29	0.06	0.18	-0.00	-0.16	-0.08	-0.08	-0.21	0.05	0.13	0.00	1909


==> data/mlm_plots/tef/yelp/lstmatt/ig/correlations_auc.tex <==
name	auc
pcc	-0.04
spearman	0.03
kendall	0.03


==> data/mlm_plots/tef/yelp/lstmatt/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	4.27	9.01	7.32	2.28	15.73	6.73	12.01	3.93	8.63	6.67	1.83	15.43	6.80	11.04	4.00	10.36	7.52	1.06	19.67	9.30	13.30	730
0.03	3.76	6.56	5.74	2.39	10.73	4.17	8.63	3.50	6.32	5.31	1.98	10.67	4.35	8.30	3.76	9.14	6.89	1.04	17.23	8.09	11.49	955
0.06	3.39	5.06	4.69	2.58	7.54	2.48	6.48	3.10	4.88	4.54	2.21	7.55	2.67	6.08	3.43	7.45	5.67	0.78	14.12	6.67	9.12	1021
0.11	3.08	4.16	4.01	2.51	5.81	1.65	5.13	2.81	3.99	3.82	2.22	5.75	1.77	4.85	3.20	6.07	4.70	0.86	11.28	5.21	7.21	1028
0.15	2.82	3.48	3.41	2.35	4.60	1.12	4.11	2.64	3.32	3.23	2.13	4.51	1.19	3.90	2.75	4.47	3.73	1.47	7.48	3.01	5.35	974
0.18	2.52	3.03	2.98	2.18	3.87	0.84	3.49	2.36	2.91	2.86	2.00	3.81	0.91	3.38	2.36	3.61	3.19	1.43	5.79	2.18	4.34	1059
0.32	2.32	2.70	2.67	2.07	3.33	0.63	3.03	2.20	2.61	2.56	1.97	3.25	0.64	2.96	2.08	3.08	2.71	1.09	5.07	1.99	3.53	1909


==> data/mlm_plots/tef/yelp/lstmatt/ig/ets_sts_auc.tex <==
name	auc
et_use	1.21
et_tse	1.17
et_ce	1.58


==> data/mlm_plots/tef/yelp/lstmatt/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.04	4.27	1.88	-9.36	17.91	13.64	3.42	4.45	10.26	7.89	1.66	18.87	8.60	13.22	4.31	11.12	7.89	0.09	22.15	11.03	13.93	730
0.03	0.77	1.75	1.22	-0.75	4.24	2.50	1.88	4.82	9.05	7.38	1.87	16.24	7.18	10.70	4.53	10.59	7.03	-4.46	25.65	15.05	11.87	955
0.06	0.58	1.37	0.82	-4.77	7.50	6.13	1.18	4.91	7.94	6.76	2.50	13.38	5.44	9.51	4.46	8.71	6.34	-0.86	18.28	9.57	9.91	1021
0.11	0.43	0.78	0.59	-0.42	1.97	1.19	0.83	4.90	7.08	6.30	3.35	10.81	3.73	8.55	4.36	7.52	5.72	0.62	14.43	6.90	8.49	1028
0.15	0.31	0.49	0.40	-0.11	1.09	0.60	0.55	4.67	6.22	5.63	3.10	9.34	3.12	7.01	4.08	6.54	5.07	0.11	12.97	6.43	6.84	974
0.18	0.22	0.34	0.29	0.10	0.58	0.24	0.38	4.34	5.64	5.23	3.41	7.87	2.23	6.38	3.74	5.87	4.60	-0.10	11.85	5.98	6.12	1059
0.32	0.15	0.25	0.21	0.02	0.48	0.23	0.28	4.03	5.13	4.77	3.28	6.98	1.85	5.76	3.48	5.13	4.23	1.11	9.15	4.02	5.41	1909


==> data/mlm_plots/tef/yelp/lstmatt/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.24
et_p_h	2.03
et_p_l2	2.15


==> data/mlm_plots/tef/yelp/lstmatt/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.08	0.14	0.13	0.06	0.21	0.08	0.18	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.04	730
0.03	0.20	0.30	0.29	0.16	0.44	0.14	0.38	0.03	0.05	0.05	0.02	0.08	0.03	0.07	0.03	0.05	0.05	0.03	0.07	0.02	0.06	955
0.06	0.40	0.56	0.55	0.31	0.82	0.26	0.71	0.05	0.07	0.07	0.04	0.11	0.04	0.10	0.05	0.07	0.07	0.04	0.09	0.03	0.08	1021
0.11	0.64	0.91	0.88	0.49	1.34	0.42	1.12	0.06	0.09	0.09	0.05	0.13	0.04	0.12	0.06	0.08	0.08	0.05	0.11	0.03	0.10	1028
0.15	1.10	1.51	1.46	0.90	2.12	0.61	1.85	0.09	0.12	0.12	0.07	0.16	0.04	0.14	0.09	0.10	0.11	0.08	0.13	0.03	0.12	974
0.18	1.67	2.28	2.21	1.38	3.17	0.89	2.78	0.11	0.13	0.14	0.09	0.18	0.05	0.17	0.10	0.12	0.12	0.09	0.15	0.03	0.14	1059
0.32	2.37	3.48	3.19	1.87	5.08	1.61	4.26	0.13	0.16	0.16	0.11	0.20	0.05	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.16	1909


==> data/mlm_plots/tef/yelp/lstmatt/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.56
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/lstmatt/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.95	0.96	0.97	0.95	0.98	0.02	0.98	0.95	0.96	0.97	0.94	0.99	0.03	0.98	730
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.92	0.93	0.94	0.91	0.96	0.03	0.95	0.92	0.94	0.95	0.90	0.98	0.04	0.97	955
0.06	0.89	0.90	0.90	0.87	0.93	0.03	0.92	0.88	0.90	0.90	0.86	0.93	0.04	0.92	0.88	0.91	0.92	0.85	0.97	0.06	0.95	1021
0.11	0.85	0.87	0.87	0.84	0.90	0.03	0.89	0.84	0.86	0.86	0.82	0.90	0.04	0.89	0.85	0.88	0.89	0.81	0.95	0.07	0.93	1028
0.15	0.80	0.82	0.82	0.79	0.86	0.03	0.84	0.79	0.81	0.81	0.77	0.86	0.04	0.84	0.79	0.83	0.84	0.75	0.91	0.08	0.89	974
0.18	0.77	0.79	0.78	0.75	0.82	0.03	0.80	0.75	0.77	0.77	0.73	0.82	0.04	0.80	0.75	0.79	0.80	0.70	0.88	0.09	0.85	1059
0.32	0.73	0.75	0.75	0.71	0.78	0.03	0.77	0.71	0.74	0.74	0.70	0.78	0.04	0.76	0.69	0.74	0.75	0.65	0.84	0.10	0.81	1909


==> data/mlm_plots/tef/yelp/lstmatt/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/yelp/lstmatt/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	2.58	2.91	2.89	2.46	3.36	0.45	3.25	1.74	3.35	2.74	0.93	5.76	2.41	4.33	2.43	9.45	6.16	-0.78	19.67	10.23	12.39	730
0.03	3.48	3.86	3.80	3.28	4.45	0.59	4.16	2.24	4.13	3.50	1.47	6.80	2.67	5.40	2.35	10.22	6.69	-1.20	21.64	11.42	13.20	955
0.06	5.25	5.85	5.75	4.93	6.76	0.91	6.57	2.66	4.79	4.13	1.88	7.70	2.91	6.18	2.41	10.85	6.59	-1.57	23.27	12.42	14.57	1021
0.11	6.14	7.11	6.86	5.58	8.63	1.52	7.67	3.04	5.33	4.71	2.23	8.43	3.10	6.86	2.86	11.80	7.48	-1.40	24.99	13.20	16.05	1028
0.15	8.94	10.10	9.93	8.31	11.89	1.79	10.63	3.51	5.86	5.27	2.53	9.19	3.33	7.43	3.32	12.95	8.31	-1.46	27.36	14.41	17.09	974
0.18	13.49	15.05	14.53	13.00	17.11	2.06	16.41	3.74	6.12	5.53	2.48	9.76	3.64	7.60	3.80	13.46	8.98	-1.07	27.98	14.53	17.64	1059
0.32	15.43	17.21	17.19	14.32	20.09	2.88	19.24	3.87	6.24	5.71	3.07	9.40	3.17	7.92	3.64	13.50	9.04	-0.76	27.76	14.26	18.49	1909


==> data/mlm_plots/tef/yelp/lstmatt/ig/time_misc_auc.tex <==
name	auc
attack_time	3.51
l2	1.73
lom	3.87


==> data/mlm_plots/tef/yelp/lstmatt/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.42	0.55	0.55	0.37	0.73	0.18	0.67	0.61	0.69	0.71	0.57	0.81	0.12	0.77	0.72	0.78	0.79	0.69	0.87	0.09	0.84	730
0.03	0.30	0.42	0.41	0.24	0.60	0.18	0.53	0.53	0.60	0.60	0.48	0.73	0.12	0.68	0.66	0.72	0.72	0.63	0.81	0.09	0.78	955
0.06	0.20	0.31	0.29	0.12	0.50	0.19	0.41	0.44	0.52	0.51	0.39	0.64	0.12	0.59	0.60	0.66	0.66	0.56	0.75	0.09	0.71	1021
0.11	0.14	0.24	0.23	0.07	0.42	0.17	0.33	0.38	0.45	0.45	0.33	0.57	0.12	0.52	0.55	0.61	0.61	0.52	0.70	0.09	0.67	1028
0.15	0.08	0.18	0.17	0.03	0.32	0.15	0.25	0.31	0.38	0.38	0.27	0.49	0.11	0.45	0.51	0.56	0.56	0.48	0.64	0.08	0.61	974
0.18	0.00	0.15	0.12	0.00	0.29	0.14	0.22	0.27	0.34	0.33	0.23	0.44	0.10	0.40	0.47	0.52	0.52	0.44	0.60	0.08	0.56	1059
0.32	0.00	0.12	0.09	-0.01	0.24	0.13	0.18	0.24	0.30	0.29	0.19	0.40	0.10	0.36	0.43	0.48	0.48	0.40	0.56	0.08	0.53	1909


==> data/mlm_plots/tef/yelp/lstmatt/ig/top_intersections_auc.tex <==
name	auc
top10	0.07
top30	0.13
top50	0.18


==> data/mlm_plots/tef/yelp/lstmatt/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	41.87	60.70	54.34	32.32	89.08	28.38	70.85	19.00	30.28	29.00	16.90	43.67	13.38	41.00	47.67	68.74	61.05	37.36	100.13	31.38	80.30	19.00	30.59	29.00	17.10	44.09	13.49	42.00	746
0.03	42.96	68.40	56.62	23.61	113.20	44.80	78.14	14.50	26.65	24.00	12.33	40.97	14.32	38.00	56.89	87.47	73.10	33.35	141.58	54.11	99.32	15.00	27.21	25.00	12.58	41.84	14.63	39.00	947
0.06	43.56	74.87	57.84	9.75	139.99	65.12	81.55	13.00	25.22	22.00	10.50	39.95	14.72	37.00	70.52	114.93	91.64	24.99	204.87	89.94	125.18	13.00	26.21	23.00	10.93	41.50	15.29	38.00	1022
0.11	43.77	78.64	58.58	-10.67	167.95	89.31	82.98	13.00	25.15	22.50	10.33	39.97	14.82	37.00	86.18	145.13	112.96	10.47	279.80	134.66	155.86	13.00	26.63	24.00	10.98	42.28	15.65	39.00	1028
0.15	43.68	72.88	57.07	19.47	126.28	53.41	80.49	13.00	25.90	23.00	11.22	40.58	14.68	37.00	116.69	176.54	147.60	72.04	281.03	104.50	200.75	15.00	28.28	26.00	12.30	44.26	15.98	42.00	1024
0.18	42.85	73.57	57.02	11.23	135.90	62.34	79.60	13.00	25.83	23.00	11.02	40.64	14.81	38.00	152.36	225.35	191.56	98.78	351.92	126.57	255.43	15.00	28.86	26.00	12.39	45.33	16.47	43.00	1046
0.32	43.63	74.59	57.81	12.61	136.57	61.98	81.30	13.00	25.49	23.00	10.99	39.99	14.50	37.00	193.46	302.91	249.48	123.14	482.69	179.77	345.46	15.00	29.44	27.00	12.85	46.03	16.59	43.00	1894


==> data/mlm_plots/tef/yelp/lstmatt/s/comparison_vals_auc.tex <==
name	auc
orig_pp	22.90
orig_ge	8.01
adv_pp	60.42
adv_ge	8.75


==> data/mlm_plots/tef/yelp/lstmatt/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.43	0.58	0.62	0.34	0.82	0.24	0.77	0.61	0.72	0.78	0.51	0.93	0.21	0.88	0.46	0.57	0.60	0.39	0.76	0.19	0.71	746
0.03	0.26	0.44	0.44	0.19	0.69	0.25	0.63	0.43	0.58	0.62	0.32	0.84	0.26	0.78	0.32	0.45	0.46	0.24	0.66	0.21	0.59	947
0.06	0.11	0.29	0.28	0.04	0.55	0.25	0.46	0.21	0.41	0.44	0.12	0.71	0.30	0.64	0.16	0.32	0.32	0.09	0.54	0.22	0.47	1022
0.11	0.01	0.19	0.16	-0.05	0.43	0.24	0.33	0.06	0.28	0.28	-0.02	0.59	0.31	0.51	0.06	0.22	0.21	-0.00	0.44	0.22	0.36	1028
0.15	-0.11	0.05	0.01	-0.19	0.29	0.24	0.18	-0.13	0.10	0.07	-0.22	0.42	0.32	0.30	-0.07	0.09	0.06	-0.14	0.31	0.22	0.23	1024
0.18	-0.21	-0.04	-0.08	-0.28	0.20	0.24	0.09	-0.26	-0.04	-0.09	-0.36	0.27	0.31	0.14	-0.16	-0.01	-0.05	-0.23	0.21	0.22	0.11	1046
0.32	-0.29	-0.14	-0.19	-0.36	0.08	0.22	-0.04	-0.41	-0.20	-0.26	-0.49	0.09	0.29	-0.04	-0.26	-0.12	-0.16	-0.32	0.08	0.20	-0.01	1894


==> data/mlm_plots/tef/yelp/lstmatt/s/correlations_auc.tex <==
name	auc
pcc	0.03
spearman	0.04
kendall	0.03


==> data/mlm_plots/tef/yelp/lstmatt/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.38	7.18	5.73	1.65	12.72	5.54	9.29	3.03	6.88	5.44	1.31	12.45	5.57	8.90	3.12	8.48	6.33	1.17	15.79	7.31	11.58	746
0.03	2.97	4.99	4.46	2.01	7.97	2.98	6.37	2.75	4.84	4.31	1.85	7.84	2.99	6.10	3.11	7.66	5.62	0.65	14.66	7.01	9.57	947
0.06	2.67	3.89	3.67	2.03	5.74	1.86	4.81	2.45	3.77	3.54	1.85	5.70	1.92	4.66	2.81	6.28	4.43	0.23	12.33	6.05	7.44	1022
0.11	2.36	3.24	3.15	1.95	4.53	1.29	3.95	2.26	3.12	2.99	1.81	4.43	1.31	3.79	2.45	4.87	3.77	0.70	9.05	4.17	5.73	1028
0.15	2.23	2.74	2.75	1.88	3.60	0.86	3.19	2.11	2.62	2.61	1.73	3.52	0.90	3.11	2.19	3.90	3.00	0.23	7.57	3.67	4.43	1024
0.18	2.10	2.47	2.49	1.79	3.15	0.68	2.85	1.96	2.37	2.38	1.67	3.07	0.70	2.72	1.98	3.17	2.68	0.97	5.37	2.20	3.76	1046
0.32	2.03	2.31	2.34	1.78	2.84	0.53	2.63	1.92	2.23	2.23	1.67	2.79	0.56	2.52	1.79	2.66	2.37	1.07	4.24	1.58	3.09	1894


==> data/mlm_plots/tef/yelp/lstmatt/s/ets_sts_auc.tex <==
name	auc
et_use	0.97
et_tse	0.93
et_ce	1.34


==> data/mlm_plots/tef/yelp/lstmatt/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.82	2.49	1.48	-2.26	7.25	4.75	2.54	3.47	7.92	5.84	0.90	14.94	7.02	10.01	3.34	8.98	6.07	-0.87	18.83	9.85	11.14	746
0.03	0.60	1.34	0.97	-1.33	4.01	2.67	1.41	3.76	6.90	5.67	1.49	12.31	5.41	8.39	3.45	8.08	5.42	-3.43	19.60	11.51	8.96	947
0.06	0.43	0.84	0.63	-0.82	2.50	1.66	0.90	3.86	5.99	5.21	2.12	9.86	3.87	7.05	3.41	6.52	4.93	-0.35	13.38	6.86	7.28	1022
0.11	0.32	0.58	0.45	-0.78	1.94	1.36	0.63	3.68	5.49	4.86	1.82	9.15	3.66	6.27	3.24	5.96	4.42	-2.76	14.69	8.72	6.21	1028
0.15	0.23	0.38	0.31	-0.26	1.01	0.63	0.40	3.63	4.95	4.53	1.99	7.91	2.96	5.50	3.12	5.18	4.00	-0.56	10.92	5.74	5.26	1024
0.18	0.17	0.29	0.22	-0.35	0.92	0.63	0.29	3.50	4.55	4.31	2.73	6.37	1.82	5.16	3.01	4.70	3.81	0.34	9.06	4.36	4.82	1046
0.32	0.13	0.21	0.17	-0.03	0.45	0.24	0.24	3.45	4.39	4.15	2.73	6.06	1.67	4.95	2.99	4.36	3.69	1.04	7.68	3.32	4.65	1894


==> data/mlm_plots/tef/yelp/lstmatt/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.17
et_p_h	1.61
et_p_l2	1.71


==> data/mlm_plots/tef/yelp/lstmatt/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.09	0.14	0.13	0.06	0.22	0.08	0.19	0.02	0.04	0.03	0.01	0.06	0.02	0.05	0.02	0.03	0.03	0.02	0.05	0.02	0.05	746
0.03	0.21	0.30	0.30	0.16	0.45	0.14	0.39	0.03	0.05	0.05	0.02	0.09	0.03	0.08	0.03	0.05	0.05	0.03	0.07	0.02	0.07	947
0.06	0.43	0.59	0.57	0.33	0.85	0.26	0.73	0.05	0.08	0.08	0.04	0.11	0.04	0.10	0.05	0.07	0.07	0.04	0.09	0.03	0.09	1022
0.11	0.68	0.96	0.92	0.53	1.39	0.43	1.15	0.06	0.09	0.10	0.05	0.14	0.04	0.12	0.07	0.09	0.09	0.06	0.11	0.03	0.10	1028
0.15	1.23	1.60	1.56	0.97	2.24	0.64	1.92	0.09	0.12	0.12	0.08	0.16	0.04	0.15	0.09	0.11	0.11	0.08	0.13	0.03	0.12	1024
0.18	1.80	2.42	2.36	1.43	3.42	0.99	2.94	0.11	0.14	0.14	0.09	0.18	0.05	0.17	0.10	0.12	0.13	0.09	0.15	0.03	0.14	1046
0.32	2.50	3.53	3.30	1.91	5.16	1.62	4.34	0.13	0.16	0.16	0.11	0.20	0.05	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.16	1894


==> data/mlm_plots/tef/yelp/lstmatt/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.58
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/lstmatt/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.95	0.96	0.96	0.94	0.98	0.02	0.98	0.95	0.96	0.97	0.94	0.99	0.03	0.98	746
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.95	0.92	0.93	0.94	0.91	0.96	0.03	0.95	0.93	0.94	0.95	0.90	0.98	0.04	0.97	947
0.06	0.89	0.90	0.90	0.88	0.93	0.03	0.92	0.88	0.90	0.90	0.86	0.93	0.03	0.92	0.88	0.91	0.92	0.85	0.97	0.06	0.95	1022
0.11	0.85	0.87	0.87	0.84	0.90	0.03	0.89	0.84	0.86	0.86	0.82	0.90	0.04	0.89	0.84	0.88	0.89	0.82	0.95	0.06	0.93	1028
0.15	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.79	0.81	0.81	0.77	0.85	0.04	0.84	0.79	0.84	0.84	0.76	0.91	0.08	0.89	1024
0.18	0.77	0.79	0.78	0.76	0.82	0.03	0.80	0.75	0.77	0.77	0.74	0.81	0.04	0.80	0.75	0.80	0.81	0.72	0.88	0.08	0.85	1046
0.32	0.73	0.75	0.75	0.72	0.78	0.03	0.77	0.71	0.74	0.74	0.70	0.78	0.04	0.76	0.69	0.75	0.76	0.65	0.84	0.09	0.81	1894


==> data/mlm_plots/tef/yelp/lstmatt/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.25
sts_ce	0.26


==> data/mlm_plots/tef/yelp/lstmatt/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	2.48	2.79	2.83	2.41	3.17	0.38	3.04	36.01	80.15	58.98	4.18	156.13	75.97	96.35	3.74	15.70	9.14	-2.26	33.66	17.96	21.05	746
0.03	3.41	3.83	3.88	3.26	4.41	0.57	4.25	48.79	99.40	77.44	7.00	191.80	92.40	119.21	3.92	17.81	10.14	-2.47	38.09	20.28	24.84	947
0.06	4.60	5.34	5.27	4.34	6.34	1.00	5.91	57.02	118.58	94.48	25.62	211.53	92.95	149.05	4.55	19.89	11.30	-1.56	41.33	21.44	29.08	1022
0.11	7.09	8.54	8.51	7.03	10.06	1.51	9.47	67.80	134.89	103.62	21.86	247.91	113.03	161.40	5.05	21.11	12.61	-0.80	43.02	21.91	30.74	1028
0.15	8.72	10.20	9.94	8.24	12.17	1.96	11.05	78.43	160.19	122.40	21.85	298.52	138.33	189.60	6.28	23.01	15.65	0.64	45.38	22.37	32.58	1024
0.18	10.97	13.00	13.14	10.95	15.04	2.05	14.44	83.70	169.23	129.30	32.74	305.71	136.48	209.84	6.69	23.76	15.90	0.71	46.80	23.05	33.86	1046
0.32	14.49	16.35	16.29	13.82	18.88	2.53	17.82	92.22	181.77	140.21	40.94	322.60	140.83	222.92	7.20	23.16	15.40	1.22	45.09	21.93	33.04	1894


==> data/mlm_plots/tef/yelp/lstmatt/s/time_misc_auc.tex <==
name	auc
attack_time	3.33
l2	46.91
lom	6.81


==> data/mlm_plots/tef/yelp/lstmatt/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.29	0.45	0.45	0.24	0.67	0.21	0.60	0.57	0.66	0.67	0.52	0.81	0.15	0.76	0.71	0.78	0.79	0.67	0.89	0.11	0.86	746
0.03	0.18	0.33	0.30	0.12	0.54	0.21	0.47	0.46	0.57	0.57	0.41	0.74	0.16	0.69	0.64	0.72	0.72	0.59	0.84	0.12	0.80	947
0.06	0.06	0.23	0.18	0.02	0.43	0.21	0.33	0.35	0.47	0.46	0.30	0.64	0.17	0.59	0.56	0.65	0.65	0.51	0.78	0.14	0.74	1022
0.11	0.00	0.16	0.11	-0.02	0.33	0.17	0.25	0.29	0.40	0.40	0.24	0.56	0.16	0.50	0.50	0.59	0.59	0.46	0.73	0.14	0.68	1028
0.15	0.00	0.11	0.05	-0.05	0.26	0.16	0.15	0.21	0.31	0.29	0.15	0.47	0.16	0.40	0.43	0.52	0.52	0.38	0.66	0.14	0.60	1024
0.18	0.00	0.08	0.00	-0.06	0.22	0.14	0.10	0.15	0.26	0.23	0.10	0.42	0.16	0.33	0.38	0.47	0.46	0.33	0.60	0.13	0.54	1046
0.32	0.00	0.05	0.00	-0.06	0.17	0.11	0.06	0.10	0.20	0.17	0.06	0.34	0.14	0.26	0.32	0.41	0.39	0.28	0.53	0.12	0.48	1894


==> data/mlm_plots/tef/yelp/lstmatt/s/top_intersections_auc.tex <==
name	auc
top10	0.04
top30	0.10
top50	0.17


==> data/mlm_plots/tef/yelp/roberta/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	32.31	46.48	42.12	25.63	67.33	20.85	54.15	11.00	16.02	15.00	9.18	22.86	6.84	21.00	38.09	52.68	48.10	29.64	75.72	23.04	60.87	11.00	16.35	16.00	9.45	23.25	6.90	21.00	685
0.03	33.89	51.22	44.38	21.14	81.29	30.08	57.38	8.00	14.05	13.00	6.79	21.31	7.26	19.00	45.49	66.00	57.06	28.04	103.96	37.96	71.81	8.00	14.61	14.00	7.16	22.07	7.46	20.00	918
0.06	35.17	55.79	45.52	17.52	94.06	38.27	60.35	7.00	12.91	12.00	5.34	20.49	7.58	18.00	55.87	83.42	71.02	33.56	133.29	49.86	91.32	7.00	13.75	12.00	5.79	21.71	7.96	19.00	1018
0.11	34.75	54.38	45.15	20.02	88.73	34.35	60.14	7.00	13.01	12.00	5.50	20.53	7.51	18.00	67.19	101.20	86.28	35.29	167.11	65.91	108.34	8.00	14.17	13.00	6.15	22.19	8.02	20.00	1084
0.15	34.08	55.11	44.35	4.93	105.29	50.18	58.36	7.00	13.53	12.00	5.99	21.06	7.54	19.00	87.22	131.57	111.33	29.06	234.08	102.51	142.24	8.00	15.34	14.00	6.99	23.69	8.35	22.00	1314
0.18	33.36	53.48	44.02	11.67	95.30	41.81	58.40	7.00	13.99	13.00	6.26	21.73	7.73	19.00	111.50	159.13	139.15	69.92	248.34	89.21	178.38	9.00	16.37	16.00	7.70	25.04	8.67	23.00	1300
0.32	37.09	62.17	48.99	7.89	116.44	54.27	65.10	7.00	12.25	11.00	5.12	19.38	7.13	17.00	138.08	219.80	177.51	69.73	369.87	150.07	244.25	8.00	14.65	13.00	6.40	22.90	8.25	20.00	1174


==> data/mlm_plots/tef/yelp/roberta/a/comparison_vals_auc.tex <==
name	auc
orig_pp	17.26
orig_ge	4.15
adv_pp	43.51
adv_ge	4.68


==> data/mlm_plots/tef/yelp/roberta/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.26	0.45	0.44	0.22	0.69	0.24	0.64	0.93	0.94	0.95	0.90	0.98	0.04	0.97	0.79	0.82	0.83	0.75	0.88	0.06	0.86	685
0.03	0.12	0.30	0.25	0.07	0.53	0.23	0.44	0.87	0.89	0.91	0.83	0.96	0.07	0.94	0.70	0.74	0.76	0.66	0.82	0.08	0.80	918
0.06	0.05	0.19	0.12	-0.01	0.38	0.19	0.28	0.80	0.83	0.86	0.72	0.94	0.11	0.90	0.61	0.66	0.69	0.56	0.77	0.11	0.74	1018
0.11	0.01	0.11	0.06	-0.04	0.27	0.16	0.16	0.75	0.79	0.82	0.65	0.92	0.13	0.87	0.56	0.61	0.64	0.49	0.73	0.12	0.69	1084
0.15	-0.01	0.06	0.02	-0.07	0.19	0.13	0.10	0.66	0.72	0.77	0.56	0.88	0.16	0.83	0.49	0.55	0.58	0.41	0.68	0.14	0.64	1314
0.18	-0.03	0.03	-0.00	-0.09	0.16	0.12	0.06	0.62	0.68	0.73	0.50	0.86	0.18	0.80	0.44	0.51	0.55	0.36	0.65	0.15	0.61	1300
0.32	-0.06	-0.01	-0.02	-0.11	0.10	0.10	0.02	0.46	0.59	0.65	0.36	0.81	0.23	0.76	0.32	0.43	0.47	0.25	0.61	0.18	0.56	1174


==> data/mlm_plots/tef/yelp/roberta/a/correlations_auc.tex <==
name	auc
pcc	0.03
spearman	0.22
kendall	0.17


==> data/mlm_plots/tef/yelp/roberta/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	5.96	9.94	8.95	4.15	15.72	5.78	13.04	5.13	9.41	8.14	3.44	15.37	5.97	12.41	5.64	11.81	9.17	3.05	20.58	8.77	16.19	685
0.03	4.61	6.90	6.48	3.43	10.37	3.47	8.45	4.33	6.85	6.10	2.73	10.97	4.12	8.52	4.63	10.53	8.04	2.18	18.88	8.35	13.57	918
0.06	3.69	4.96	4.67	2.91	7.01	2.05	5.88	3.45	4.98	4.48	2.57	7.38	2.41	5.96	3.98	8.59	6.35	1.38	15.79	7.20	10.32	1018
0.11	3.06	3.88	3.73	2.59	5.17	1.29	4.52	2.93	3.90	3.70	2.41	5.40	1.49	4.61	3.35	6.42	5.11	1.34	11.50	5.08	7.42	1084
0.15	2.65	3.10	3.00	2.25	3.94	0.85	3.44	2.56	3.16	3.04	2.08	4.24	1.08	3.49	2.90	4.78	3.96	1.40	8.17	3.38	5.52	1314
0.18	2.34	2.67	2.61	2.05	3.30	0.62	2.93	2.29	2.71	2.60	1.98	3.43	0.72	3.01	2.56	4.06	3.37	1.24	6.88	2.82	4.52	1300
0.32	2.19	2.49	2.40	1.96	3.01	0.53	2.67	2.17	2.54	2.41	1.94	3.14	0.60	2.79	2.25	3.48	2.88	0.98	5.99	2.51	3.88	1174


==> data/mlm_plots/tef/yelp/roberta/a/ets_sts_auc.tex <==
name	auc
et_use	1.16
et_tse	1.16
et_ce	1.77


==> data/mlm_plots/tef/yelp/roberta/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.23	3.25	2.01	-2.92	9.42	6.17	3.28	4.79	10.45	7.81	1.24	19.66	9.21	13.29	4.26	11.16	7.55	0.44	21.87	10.72	14.14	685
0.03	0.84	1.72	1.21	-2.71	6.16	4.44	1.68	4.86	8.26	6.75	1.73	14.79	6.53	9.56	4.13	8.83	6.08	-0.67	18.34	9.51	10.29	918
0.06	0.57	1.12	0.75	-1.46	3.71	2.59	1.02	4.48	6.92	5.72	1.86	11.98	5.06	7.59	3.77	7.58	5.06	-2.51	17.66	10.08	7.53	1018
0.11	0.38	0.65	0.49	-0.48	1.78	1.13	0.69	4.06	5.84	4.97	1.66	10.03	4.18	6.27	3.32	6.06	4.26	-0.60	12.71	6.65	6.08	1084
0.15	0.24	0.37	0.31	0.14	0.59	0.22	0.41	3.60	4.65	4.18	2.42	6.89	2.24	5.08	2.96	4.47	3.57	0.14	8.80	4.33	4.64	1314
0.18	0.18	0.40	0.23	-2.62	3.41	3.01	0.29	3.32	4.21	3.80	2.22	6.19	1.99	4.49	2.69	4.07	3.24	-0.69	8.83	4.76	4.03	1300
0.32	0.14	0.24	0.18	-0.21	0.69	0.45	0.25	3.24	4.19	3.70	2.13	6.26	2.06	4.49	2.65	4.31	3.19	-2.75	11.37	7.06	4.05	1174


==> data/mlm_plots/tef/yelp/roberta/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.21
et_p_h	1.67
et_p_l2	1.71


==> data/mlm_plots/tef/yelp/roberta/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.09	0.14	0.13	0.07	0.22	0.07	0.18	0.02	0.04	0.03	0.01	0.07	0.03	0.06	0.02	0.04	0.03	0.02	0.06	0.02	0.05	685
0.03	0.21	0.30	0.29	0.17	0.44	0.14	0.38	0.03	0.06	0.06	0.03	0.10	0.04	0.09	0.04	0.05	0.05	0.03	0.08	0.02	0.07	918
0.06	0.40	0.56	0.55	0.32	0.81	0.24	0.71	0.05	0.08	0.08	0.04	0.12	0.04	0.11	0.05	0.07	0.07	0.04	0.10	0.03	0.09	1018
0.11	0.66	0.92	0.90	0.55	1.29	0.37	1.14	0.07	0.10	0.10	0.06	0.15	0.04	0.13	0.07	0.09	0.09	0.06	0.12	0.03	0.11	1084
0.15	1.12	1.56	1.51	0.94	2.18	0.62	1.96	0.10	0.13	0.13	0.08	0.17	0.04	0.16	0.09	0.11	0.11	0.08	0.14	0.03	0.13	1314
0.18	1.68	2.23	2.17	1.36	3.10	0.87	2.71	0.12	0.15	0.15	0.10	0.19	0.05	0.17	0.11	0.13	0.13	0.10	0.15	0.03	0.14	1300
0.32	1.99	2.91	2.70	1.48	4.34	1.43	3.52	0.13	0.15	0.16	0.10	0.20	0.05	0.19	0.12	0.13	0.13	0.10	0.17	0.03	0.15	1174


==> data/mlm_plots/tef/yelp/roberta/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.52
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/roberta/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.96	0.97	0.97	0.94	0.99	0.02	0.98	685
0.03	0.93	0.94	0.95	0.92	0.96	0.02	0.96	0.93	0.94	0.94	0.91	0.97	0.03	0.96	0.93	0.95	0.96	0.91	0.99	0.04	0.98	918
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.89	0.91	0.91	0.87	0.94	0.04	0.93	0.90	0.93	0.93	0.88	0.97	0.05	0.96	1018
0.11	0.86	0.88	0.88	0.85	0.91	0.03	0.90	0.85	0.88	0.88	0.84	0.91	0.04	0.90	0.87	0.90	0.91	0.84	0.96	0.06	0.94	1084
0.15	0.82	0.84	0.84	0.81	0.87	0.03	0.86	0.82	0.84	0.84	0.80	0.88	0.04	0.87	0.84	0.87	0.88	0.82	0.93	0.06	0.92	1314
0.18	0.79	0.81	0.81	0.78	0.84	0.03	0.83	0.79	0.81	0.81	0.77	0.85	0.04	0.84	0.81	0.85	0.86	0.77	0.92	0.07	0.89	1300
0.32	0.77	0.79	0.79	0.76	0.83	0.03	0.81	0.77	0.79	0.79	0.75	0.83	0.04	0.82	0.78	0.82	0.82	0.74	0.89	0.08	0.87	1174


==> data/mlm_plots/tef/yelp/roberta/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/yelp/roberta/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	1.61	2.24	2.12	1.37	3.11	0.87	2.68	0.21	0.36	0.32	0.17	0.55	0.19	0.46	4.32	18.98	11.10	-3.14	41.11	22.12	24.89	685
0.03	2.63	4.10	3.67	2.03	6.16	2.06	5.36	0.29	0.45	0.42	0.24	0.66	0.21	0.58	3.66	20.17	10.49	-4.39	44.74	24.57	27.14	918
0.06	3.42	4.37	4.24	3.09	5.64	1.27	5.11	0.35	0.53	0.51	0.31	0.75	0.22	0.70	4.22	21.73	10.54	-5.23	48.70	26.96	27.86	1018
0.11	4.62	7.42	6.75	3.47	11.38	3.96	9.77	0.41	0.60	0.58	0.37	0.83	0.23	0.77	5.24	23.76	12.77	-4.17	51.69	27.93	30.70	1084
0.15	7.14	11.22	10.19	5.26	17.17	5.95	14.20	0.48	0.67	0.67	0.44	0.90	0.23	0.89	6.35	26.97	15.67	-1.48	55.41	28.44	37.62	1314
0.18	9.02	14.22	13.06	7.03	21.41	7.19	18.68	0.48	0.68	0.66	0.44	0.91	0.23	0.90	7.21	30.43	17.92	-0.88	61.73	31.30	43.98	1300
0.32	8.36	13.68	12.38	6.56	20.80	7.12	18.47	0.45	0.63	0.59	0.41	0.85	0.22	0.81	6.49	27.67	15.52	-2.51	57.84	30.17	38.30	1174


==> data/mlm_plots/tef/yelp/roberta/a/time_misc_auc.tex <==
name	auc
attack_time	3.21
l2	0.19
lom	8.12


==> data/mlm_plots/tef/yelp/roberta/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.61	0.70	0.71	0.56	0.84	0.14	0.80	0.82	0.85	0.87	0.79	0.92	0.07	0.90	0.89	0.91	0.92	0.87	0.95	0.04	0.94	685
0.03	0.50	0.58	0.60	0.37	0.78	0.20	0.71	0.75	0.80	0.81	0.71	0.88	0.09	0.86	0.85	0.88	0.89	0.83	0.93	0.05	0.92	918
0.06	0.30	0.44	0.50	0.20	0.68	0.24	0.62	0.67	0.73	0.75	0.61	0.85	0.12	0.81	0.81	0.84	0.85	0.77	0.91	0.07	0.89	1018
0.11	0.20	0.38	0.40	0.14	0.62	0.24	0.56	0.64	0.69	0.71	0.56	0.82	0.13	0.77	0.79	0.82	0.83	0.74	0.90	0.08	0.87	1084
0.15	0.12	0.33	0.33	0.09	0.57	0.24	0.50	0.58	0.65	0.67	0.50	0.79	0.14	0.74	0.74	0.79	0.80	0.70	0.87	0.08	0.84	1314
0.18	0.07	0.30	0.29	0.06	0.53	0.24	0.47	0.55	0.62	0.66	0.46	0.78	0.16	0.73	0.73	0.77	0.79	0.68	0.86	0.09	0.83	1300
0.32	0.00	0.20	0.17	-0.01	0.42	0.21	0.35	0.44	0.55	0.58	0.37	0.73	0.18	0.68	0.67	0.73	0.75	0.62	0.84	0.11	0.80	1174


==> data/mlm_plots/tef/yelp/roberta/a/top_intersections_auc.tex <==
name	auc
top10	0.11
top30	0.20
top50	0.25


==> data/mlm_plots/tef/yelp/roberta/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	32.26	45.73	42.13	26.13	65.33	19.60	52.98	11.00	16.08	16.00	9.20	22.96	6.88	21.00	37.47	51.26	47.56	29.72	72.81	21.55	59.12	11.00	16.37	16.00	9.37	23.37	7.00	22.00	711
0.03	33.04	50.75	43.73	20.46	81.04	30.29	57.02	8.00	14.20	13.00	6.90	21.51	7.30	19.00	43.85	63.62	56.06	28.11	99.14	35.51	71.29	8.00	14.76	14.00	7.19	22.32	7.57	20.00	939
0.06	34.76	54.95	44.39	15.77	94.13	39.18	58.74	7.00	13.30	12.00	5.83	20.77	7.47	19.00	53.65	80.40	67.83	28.13	132.66	52.27	86.53	8.00	14.11	13.00	6.25	21.97	7.86	20.00	1199
0.11	33.77	53.08	44.56	20.09	86.08	32.99	58.89	7.00	13.36	12.00	5.82	20.91	7.54	19.00	67.35	97.89	85.83	47.86	147.92	50.03	112.07	8.00	14.70	14.00	6.52	22.88	8.18	21.00	1441
0.15	34.25	55.79	44.29	6.15	105.43	49.64	58.62	7.00	13.60	12.00	6.00	21.20	7.60	19.00	88.64	129.97	109.33	35.58	224.36	94.39	141.67	8.00	15.44	14.00	7.02	23.86	8.42	21.00	1607
0.18	35.20	54.11	45.05	11.01	97.21	43.10	58.40	7.00	13.45	13.00	6.12	20.79	7.34	18.00	109.39	155.64	133.66	68.92	242.36	86.72	167.44	9.00	15.51	15.00	7.32	23.71	8.19	21.00	1026
0.32	39.29	74.57	54.43	-0.62	149.76	75.19	78.61	5.00	9.92	8.00	3.07	16.76	6.85	14.00	144.47	241.41	193.96	67.09	415.72	174.32	274.28	6.00	11.91	10.00	4.08	19.75	7.83	16.00	569


==> data/mlm_plots/tef/yelp/roberta/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	18.06
orig_ge	3.98
adv_pp	44.27
adv_ge	4.47


==> data/mlm_plots/tef/yelp/roberta/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	-0.13	0.10	0.10	-0.32	0.53	0.43	0.39	0.12	0.32	0.32	0.02	0.61	0.29	0.51	0.09	0.24	0.23	0.01	0.47	0.23	0.38	711
0.03	-0.24	-0.03	-0.04	-0.42	0.35	0.38	0.19	0.02	0.20	0.18	-0.07	0.48	0.28	0.38	0.01	0.16	0.13	-0.06	0.37	0.21	0.28	939
0.06	-0.39	-0.19	-0.19	-0.53	0.16	0.35	0.01	-0.11	0.06	0.05	-0.20	0.32	0.26	0.21	-0.08	0.05	0.04	-0.14	0.24	0.19	0.15	1199
0.11	-0.52	-0.34	-0.34	-0.64	-0.04	0.30	-0.17	-0.21	-0.04	-0.06	-0.29	0.20	0.25	0.11	-0.14	-0.03	-0.04	-0.21	0.15	0.18	0.08	1441
0.15	-0.60	-0.45	-0.46	-0.69	-0.20	0.25	-0.30	-0.33	-0.18	-0.21	-0.40	0.05	0.22	-0.04	-0.23	-0.12	-0.14	-0.29	0.04	0.16	-0.03	1607
0.18	-0.60	-0.47	-0.48	-0.69	-0.26	0.22	-0.34	-0.34	-0.21	-0.23	-0.41	-0.00	0.21	-0.09	-0.24	-0.14	-0.16	-0.30	0.01	0.15	-0.06	1026
0.32	-0.61	-0.47	-0.48	-0.68	-0.26	0.21	-0.32	-0.34	-0.21	-0.22	-0.41	-0.00	0.20	-0.09	-0.24	-0.14	-0.15	-0.29	0.01	0.15	-0.05	569


==> data/mlm_plots/tef/yelp/roberta/ig/correlations_auc.tex <==
name	auc
pcc	-0.11
spearman	-0.03
kendall	-0.02


==> data/mlm_plots/tef/yelp/roberta/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	10.29	18.45	15.93	6.46	30.45	11.99	24.16	9.65	17.60	14.47	5.76	29.44	11.84	23.61	9.03	19.97	15.95	5.20	34.74	14.77	28.18	711
0.03	7.50	11.78	10.53	5.05	18.50	6.73	14.46	7.08	11.91	10.45	4.44	19.39	7.47	14.80	7.97	16.48	12.89	4.08	28.89	12.40	21.44	939
0.06	5.78	8.22	7.43	4.39	12.04	3.83	9.94	5.55	8.30	7.46	3.91	12.69	4.39	10.22	7.09	13.59	10.61	2.93	24.25	10.66	16.07	1199
0.11	4.73	6.35	5.93	3.80	8.89	2.55	7.58	4.72	6.61	6.01	3.50	9.71	3.11	7.99	5.76	11.38	8.99	1.68	21.07	9.70	13.54	1441
0.15	3.98	4.96	4.76	3.51	6.42	1.46	5.69	3.96	5.12	4.90	3.41	6.84	1.71	5.92	4.91	8.31	6.72	1.84	14.78	6.47	9.92	1607
0.18	3.56	4.27	4.17	3.26	5.29	1.02	4.86	3.59	4.43	4.28	3.19	5.66	1.23	5.13	4.31	6.86	5.71	2.24	11.48	4.62	8.05	1026
0.32	3.17	3.80	3.69	2.87	4.72	0.93	4.29	3.12	3.93	3.77	2.72	5.13	1.20	4.48	3.36	5.71	4.55	1.24	10.18	4.47	6.62	569


==> data/mlm_plots/tef/yelp/roberta/ig/ets_sts_auc.tex <==
name	auc
et_use	1.90
et_tse	1.94
et_ce	2.94


==> data/mlm_plots/tef/yelp/roberta/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	2.19	6.37	3.71	-4.80	17.53	11.17	6.30	7.77	17.33	12.66	1.84	32.81	15.49	22.19	7.24	20.22	12.50	-3.09	43.54	23.32	24.50	711
0.03	1.34	3.52	2.00	-9.00	16.04	12.52	2.87	6.75	12.07	9.93	2.75	21.40	9.33	14.53	5.80	12.87	9.08	-0.63	26.38	13.50	15.25	939
0.06	0.83	1.98	1.18	-2.73	6.68	4.71	1.67	6.18	10.53	8.50	1.85	19.21	8.68	11.78	5.26	11.82	7.60	-5.24	28.87	17.06	11.69	1199
0.11	0.59	1.00	0.73	-1.11	3.12	2.12	0.99	5.94	8.60	7.22	2.57	14.63	6.03	9.35	4.83	9.14	6.29	-4.33	22.60	13.46	8.94	1441
0.15	0.38	0.60	0.50	0.12	1.09	0.48	0.67	5.44	7.51	6.58	3.11	11.92	4.41	8.51	4.56	7.37	5.62	0.07	14.66	7.29	7.44	1607
0.18	0.29	0.43	0.38	0.16	0.71	0.27	0.50	5.00	6.60	5.99	3.36	9.85	3.24	7.34	4.09	6.16	5.11	0.83	11.49	5.33	6.56	1026
0.32	0.21	0.39	0.29	-0.05	0.83	0.44	0.40	4.63	6.50	5.83	2.67	10.32	3.83	7.19	3.84	6.79	4.95	-1.01	14.58	7.80	6.51	569


==> data/mlm_plots/tef/yelp/roberta/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.36
et_p_h	2.56
et_p_l2	2.66


==> data/mlm_plots/tef/yelp/roberta/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.07	0.13	0.12	0.05	0.21	0.08	0.17	0.02	0.04	0.03	0.01	0.07	0.03	0.06	0.02	0.04	0.03	0.02	0.06	0.02	0.05	711
0.03	0.19	0.28	0.27	0.14	0.42	0.14	0.36	0.03	0.06	0.06	0.03	0.10	0.04	0.09	0.04	0.05	0.05	0.03	0.08	0.02	0.07	939
0.06	0.37	0.52	0.52	0.28	0.77	0.25	0.65	0.05	0.08	0.08	0.04	0.12	0.04	0.11	0.05	0.07	0.07	0.04	0.10	0.03	0.09	1199
0.11	0.67	0.95	0.90	0.49	1.40	0.46	1.14	0.08	0.11	0.11	0.06	0.15	0.04	0.13	0.08	0.09	0.09	0.06	0.12	0.03	0.11	1441
0.15	1.10	1.52	1.45	0.83	2.21	0.69	1.86	0.10	0.13	0.13	0.08	0.17	0.05	0.16	0.09	0.11	0.11	0.08	0.14	0.03	0.13	1607
0.18	1.51	2.13	1.97	0.94	3.32	1.19	2.56	0.11	0.14	0.14	0.10	0.19	0.05	0.17	0.10	0.12	0.12	0.09	0.15	0.03	0.14	1026
0.32	1.81	2.78	2.50	1.20	4.36	1.58	3.46	0.11	0.15	0.15	0.09	0.21	0.06	0.19	0.11	0.13	0.13	0.09	0.17	0.04	0.15	569


==> data/mlm_plots/tef/yelp/roberta/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.50
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/roberta/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.97	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.99	0.02	0.98	711
0.03	0.94	0.95	0.95	0.93	0.97	0.02	0.96	0.94	0.95	0.95	0.92	0.97	0.02	0.96	0.94	0.95	0.96	0.92	0.99	0.03	0.98	939
0.06	0.90	0.92	0.92	0.89	0.95	0.03	0.94	0.90	0.92	0.92	0.89	0.95	0.03	0.94	0.92	0.93	0.94	0.89	0.98	0.04	0.96	1199
0.11	0.86	0.88	0.89	0.85	0.92	0.03	0.91	0.86	0.88	0.89	0.84	0.93	0.04	0.91	0.89	0.91	0.93	0.85	0.97	0.06	0.95	1441
0.15	0.83	0.85	0.85	0.82	0.88	0.03	0.87	0.83	0.85	0.85	0.81	0.89	0.04	0.87	0.86	0.88	0.89	0.82	0.94	0.06	0.92	1607
0.18	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.80	0.82	0.83	0.79	0.86	0.04	0.85	0.83	0.86	0.87	0.79	0.93	0.07	0.91	1026
0.32	0.78	0.80	0.80	0.76	0.84	0.04	0.82	0.77	0.80	0.80	0.76	0.85	0.05	0.83	0.79	0.83	0.84	0.75	0.91	0.08	0.88	569


==> data/mlm_plots/tef/yelp/roberta/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.27


==> data/mlm_plots/tef/yelp/roberta/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	2.92	4.42	3.71	0.88	7.97	3.55	4.70	6.07	23.18	12.10	-27.50	73.85	50.67	20.53	4.60	17.60	12.08	-0.29	35.50	17.89	24.52	711
0.03	3.82	6.45	4.99	0.57	12.33	5.88	6.54	8.80	25.86	15.51	-17.59	69.32	43.45	24.79	4.08	16.88	10.93	-1.21	34.98	18.10	22.97	939
0.06	15.94	22.86	21.45	12.30	33.42	10.56	27.67	11.09	33.24	18.15	-30.33	96.81	63.57	29.56	4.34	18.67	11.70	-0.89	38.23	19.56	26.98	1199
0.11	8.20	13.99	12.72	6.56	21.42	7.43	18.30	11.65	27.00	18.88	-9.14	63.13	36.13	29.16	5.86	17.56	12.83	1.97	33.16	15.59	25.19	1441
0.15	11.34	17.40	15.89	8.90	25.91	8.51	22.43	13.45	26.90	19.95	-6.28	60.08	33.18	28.95	5.48	17.95	13.14	1.13	34.77	16.82	24.93	1607
0.18	12.63	18.47	16.59	10.25	26.70	8.23	23.89	13.39	26.23	20.62	-9.52	61.99	35.76	29.50	4.34	16.13	11.28	0.06	32.21	16.07	21.59	1026
0.32	11.00	16.72	15.61	8.97	24.47	7.75	21.83	13.08	24.52	20.41	4.66	44.39	19.86	30.05	3.91	13.10	8.60	-1.18	27.38	14.28	16.66	569


==> data/mlm_plots/tef/yelp/roberta/ig/time_misc_auc.tex <==
name	auc
attack_time	5.09
l2	8.31
lom	5.07


==> data/mlm_plots/tef/yelp/roberta/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.16	0.31	0.29	0.11	0.50	0.20	0.42	0.38	0.49	0.48	0.33	0.64	0.15	0.58	0.56	0.63	0.62	0.51	0.75	0.12	0.70	711
0.03	0.09	0.24	0.20	0.04	0.43	0.20	0.33	0.33	0.43	0.40	0.28	0.58	0.15	0.51	0.52	0.59	0.58	0.48	0.70	0.11	0.66	939
0.06	0.00	0.17	0.12	-0.02	0.36	0.19	0.25	0.26	0.35	0.34	0.21	0.49	0.14	0.43	0.47	0.54	0.53	0.44	0.64	0.10	0.60	1199
0.11	0.00	0.12	0.07	-0.03	0.26	0.14	0.18	0.22	0.32	0.31	0.18	0.46	0.14	0.39	0.44	0.51	0.50	0.41	0.61	0.10	0.56	1441
0.15	0.00	0.07	0.00	-0.06	0.21	0.13	0.11	0.17	0.26	0.24	0.14	0.38	0.12	0.32	0.40	0.46	0.45	0.36	0.55	0.09	0.51	1607
0.18	0.00	0.06	0.00	-0.04	0.16	0.10	0.08	0.17	0.24	0.24	0.14	0.35	0.11	0.30	0.39	0.45	0.44	0.36	0.54	0.09	0.49	1026
0.32	0.00	0.05	0.00	-0.05	0.14	0.10	0.06	0.17	0.23	0.23	0.11	0.35	0.12	0.31	0.39	0.45	0.45	0.35	0.54	0.09	0.50	569


==> data/mlm_plots/tef/yelp/roberta/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.09
top50	0.15


==> data/mlm_plots/tef/yelp/roberta/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	33.22	45.24	41.76	27.07	63.40	18.16	52.62	11.00	16.31	16.00	9.89	22.73	6.42	20.25	38.23	51.30	47.51	31.48	71.12	19.82	59.75	11.00	16.64	16.00	10.09	23.19	6.55	21.00	740
0.03	32.31	50.04	43.07	16.22	83.86	33.82	54.70	9.00	15.46	16.00	8.16	22.77	7.30	21.00	43.08	63.77	55.48	23.72	103.83	40.05	70.42	10.00	16.01	16.00	8.44	23.57	7.56	22.00	1132
0.06	33.88	50.96	42.85	15.36	86.55	35.59	55.85	8.00	15.13	15.00	7.53	22.73	7.60	21.00	53.44	77.36	65.50	30.37	124.35	46.99	84.42	9.00	16.10	16.00	7.99	24.20	8.11	23.00	1401
0.11	34.09	53.24	44.66	19.97	86.51	33.27	58.25	7.00	13.19	12.00	5.78	20.60	7.41	18.00	70.60	102.33	86.11	46.09	158.57	56.24	116.51	8.00	14.52	13.00	6.43	22.60	8.09	20.00	1387
0.15	34.72	56.22	44.37	5.27	107.17	50.95	60.14	7.00	12.39	11.00	5.27	19.50	7.11	17.00	93.90	139.39	116.63	40.47	238.32	98.92	152.50	8.00	14.06	13.00	6.18	21.95	7.89	19.00	1395
0.18	35.80	59.62	48.33	10.48	108.76	49.14	63.66	6.00	11.51	10.00	4.85	18.17	6.66	16.00	118.14	176.73	153.39	73.66	279.80	103.07	194.02	8.00	13.38	12.00	5.79	20.96	7.59	18.00	930
0.32	41.20	70.94	54.29	13.53	128.34	57.41	78.66	5.00	9.48	8.00	3.38	15.57	6.09	13.00	144.81	245.20	190.80	88.09	402.31	157.11	281.63	6.00	11.30	9.00	4.11	18.48	7.18	16.00	525


==> data/mlm_plots/tef/yelp/roberta/s/comparison_vals_auc.tex <==
name	auc
orig_pp	18.14
orig_ge	3.83
adv_pp	46.79
adv_ge	4.29


==> data/mlm_plots/tef/yelp/roberta/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.51	0.63	0.67	0.40	0.86	0.23	0.80	0.75	0.78	0.83	0.58	0.97	0.20	0.89	0.57	0.62	0.66	0.44	0.79	0.18	0.73	740
0.03	0.17	0.41	0.45	0.13	0.69	0.28	0.63	0.40	0.58	0.70	0.27	0.88	0.31	0.81	0.29	0.44	0.52	0.20	0.69	0.25	0.63	1132
0.06	0.06	0.27	0.27	0.03	0.52	0.25	0.45	0.27	0.47	0.54	0.19	0.76	0.28	0.70	0.19	0.35	0.39	0.13	0.57	0.22	0.52	1401
0.11	0.07	0.22	0.22	0.02	0.42	0.20	0.35	0.29	0.45	0.49	0.20	0.70	0.25	0.63	0.20	0.33	0.35	0.14	0.52	0.19	0.46	1387
0.15	0.05	0.17	0.16	-0.00	0.34	0.17	0.27	0.24	0.39	0.41	0.17	0.62	0.23	0.56	0.17	0.28	0.29	0.11	0.45	0.17	0.40	1395
0.18	0.00	0.12	0.10	-0.04	0.29	0.17	0.22	0.19	0.33	0.34	0.11	0.56	0.23	0.48	0.13	0.23	0.23	0.07	0.40	0.16	0.34	930
0.32	-0.02	0.09	0.07	-0.08	0.26	0.17	0.18	0.14	0.28	0.28	0.05	0.52	0.24	0.45	0.09	0.20	0.19	0.03	0.37	0.17	0.32	525


==> data/mlm_plots/tef/yelp/roberta/s/correlations_auc.tex <==
name	auc
pcc	0.06
spearman	0.12
kendall	0.09


==> data/mlm_plots/tef/yelp/roberta/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	3.52	7.06	5.80	1.86	12.26	5.20	9.07	3.20	7.00	5.55	1.34	12.65	5.66	8.68	3.26	8.72	6.12	1.10	16.35	7.63	11.94	740
0.03	3.47	6.51	5.29	2.29	10.73	4.22	8.68	3.33	6.65	5.27	1.84	11.45	4.80	8.77	4.06	10.21	7.83	1.82	18.60	8.39	13.78	1132
0.06	3.07	4.81	4.26	2.31	7.32	2.50	5.99	2.95	4.98	4.27	1.99	7.96	2.99	6.21	4.07	8.44	6.43	1.81	15.07	6.63	10.98	1401
0.11	2.50	3.38	3.15	1.99	4.77	1.39	4.08	2.41	3.41	3.13	1.85	4.97	1.56	4.09	3.13	5.86	4.56	1.36	10.36	4.50	6.95	1387
0.15	2.28	2.83	2.77	1.98	3.69	0.85	3.27	2.29	2.88	2.79	1.94	3.82	0.94	3.34	2.70	4.72	3.84	1.05	8.38	3.66	5.48	1395
0.18	2.06	2.54	2.52	1.81	3.28	0.73	2.89	2.09	2.60	2.54	1.81	3.40	0.80	3.03	2.42	3.94	3.33	1.43	6.45	2.51	4.70	930
0.32	1.95	2.36	2.34	1.70	3.01	0.66	2.70	2.00	2.43	2.39	1.73	3.14	0.70	2.80	2.14	3.76	2.87	0.06	7.45	3.70	4.27	525


==> data/mlm_plots/tef/yelp/roberta/s/ets_sts_auc.tex <==
name	auc
et_use	1.06
et_tse	1.08
et_ce	1.70


==> data/mlm_plots/tef/yelp/roberta/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.77	1.80	1.19	-0.54	4.14	2.34	2.13	2.67	6.52	4.70	0.29	12.75	6.23	8.32	2.45	7.16	4.58	-1.13	15.46	8.29	8.74	740
0.03	0.61	1.41	0.98	-1.59	4.42	3.00	1.58	3.45	6.47	5.38	1.80	11.14	4.67	8.02	3.08	6.76	5.16	0.30	13.22	6.46	7.72	1132
0.06	0.46	0.84	0.67	-0.02	1.71	0.86	0.98	3.64	5.60	5.05	2.63	8.57	2.97	6.99	3.10	5.63	4.60	1.13	10.14	4.51	6.75	1401
0.11	0.29	0.52	0.41	-0.63	1.67	1.15	0.55	3.19	4.71	4.27	1.97	7.44	2.73	5.43	2.76	4.72	3.73	0.17	9.27	4.55	5.12	1387
0.15	0.20	0.33	0.26	-0.49	1.15	0.82	0.35	3.04	4.15	3.67	1.96	6.33	2.18	4.61	2.54	4.16	3.20	-0.12	8.45	4.28	4.36	1395
0.18	0.15	0.24	0.21	0.10	0.38	0.14	0.28	2.88	3.88	3.58	2.13	5.63	1.75	4.47	2.39	3.80	3.02	0.60	7.00	3.20	4.08	930
0.32	0.12	0.22	0.17	-0.01	0.46	0.24	0.25	2.87	3.81	3.43	1.95	5.68	1.86	4.33	2.33	3.91	3.04	0.80	7.02	3.11	4.14	525


==> data/mlm_plots/tef/yelp/roberta/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.16
et_p_h	1.40
et_p_l2	1.42


==> data/mlm_plots/tef/yelp/roberta/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.09	0.14	0.14	0.07	0.21	0.07	0.18	0.02	0.04	0.04	0.01	0.07	0.03	0.06	0.02	0.04	0.04	0.02	0.06	0.02	0.05	740
0.03	0.21	0.30	0.29	0.17	0.42	0.13	0.37	0.04	0.06	0.06	0.03	0.10	0.03	0.09	0.04	0.06	0.05	0.03	0.08	0.02	0.07	1132
0.06	0.40	0.56	0.54	0.32	0.79	0.23	0.70	0.06	0.08	0.08	0.05	0.12	0.04	0.11	0.06	0.07	0.07	0.05	0.10	0.02	0.09	1401
0.11	0.72	1.01	0.96	0.58	1.43	0.43	1.23	0.08	0.11	0.11	0.06	0.15	0.04	0.14	0.07	0.09	0.09	0.06	0.12	0.03	0.11	1387
0.15	1.21	1.69	1.59	0.78	2.60	0.91	2.03	0.10	0.13	0.13	0.08	0.18	0.05	0.16	0.10	0.11	0.12	0.08	0.14	0.03	0.13	1395
0.18	1.59	2.25	2.10	1.24	3.26	1.01	2.74	0.11	0.14	0.15	0.09	0.20	0.05	0.18	0.10	0.12	0.13	0.09	0.16	0.03	0.15	930
0.32	1.87	2.84	2.56	1.33	4.35	1.51	3.59	0.12	0.15	0.15	0.09	0.21	0.06	0.19	0.11	0.13	0.13	0.10	0.17	0.04	0.16	525


==> data/mlm_plots/tef/yelp/roberta/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.53
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/roberta/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.96	0.97	0.97	0.95	0.99	0.02	0.99	740
0.03	0.94	0.95	0.95	0.93	0.97	0.02	0.96	0.93	0.95	0.95	0.92	0.97	0.02	0.96	0.94	0.96	0.96	0.93	0.99	0.03	0.98	1132
0.06	0.90	0.92	0.92	0.89	0.94	0.03	0.93	0.90	0.91	0.92	0.88	0.95	0.03	0.94	0.92	0.94	0.94	0.90	0.98	0.04	0.97	1401
0.11	0.86	0.88	0.88	0.84	0.91	0.03	0.90	0.85	0.87	0.88	0.83	0.92	0.04	0.90	0.88	0.91	0.92	0.86	0.96	0.05	0.94	1387
0.15	0.83	0.85	0.84	0.81	0.88	0.03	0.87	0.83	0.85	0.85	0.81	0.88	0.04	0.87	0.85	0.88	0.89	0.82	0.94	0.06	0.92	1395
0.18	0.80	0.82	0.82	0.79	0.85	0.03	0.84	0.80	0.82	0.82	0.78	0.86	0.04	0.85	0.82	0.86	0.87	0.79	0.92	0.07	0.91	930
0.32	0.78	0.80	0.80	0.76	0.84	0.04	0.82	0.78	0.80	0.80	0.76	0.85	0.04	0.83	0.79	0.83	0.84	0.75	0.91	0.08	0.89	525


==> data/mlm_plots/tef/yelp/roberta/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.27
sts_tse	0.27
sts_ce	0.27


==> data/mlm_plots/tef/yelp/roberta/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.82	6.09	5.23	2.32	9.87	3.77	7.12	19.76	263.42	72.12	-485.82	1012.66	749.24	265.91	2.38	8.72	5.47	-1.08	18.52	9.80	11.03	740
0.03	4.10	8.63	6.36	1.18	16.09	7.46	10.36	41.88	2119.28	208.42	-4829.17	9067.74	6948.45	659.47	2.83	14.58	8.59	-0.83	29.99	15.41	22.96	1132
0.06	5.29	10.26	8.00	2.28	18.24	7.98	12.74	76.22	2731.99	311.99	-7947.53	13411.51	10679.52	1027.79	3.39	16.25	10.32	0.73	31.77	15.52	26.67	1401
0.11	8.45	13.61	11.78	6.35	20.88	7.26	16.93	57.10	1270.75	214.54	-4116.98	6658.49	5387.74	593.22	2.75	12.50	7.29	-0.95	25.95	13.45	17.82	1387
0.15	8.46	11.75	10.49	6.52	16.98	5.23	13.07	67.88	620.77	223.25	-1216.58	2458.12	1837.35	596.07	3.14	12.08	7.57	-0.35	24.51	12.43	17.88	1395
0.18	9.08	13.33	11.59	6.74	19.92	6.59	16.39	84.78	451.28	235.19	-124.27	1026.82	575.54	614.00	2.90	10.50	6.83	-0.39	21.40	10.90	13.86	930
0.32	9.65	12.78	11.43	7.42	18.14	5.36	14.66	77.80	585.00	235.18	-1447.02	2617.02	2032.02	583.46	2.15	8.77	5.48	-0.65	18.20	9.42	12.21	525


==> data/mlm_plots/tef/yelp/roberta/s/time_misc_auc.tex <==
name	auc
attack_time	3.74
l2	318.52
lom	3.60


==> data/mlm_plots/tef/yelp/roberta/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.40	0.54	0.57	0.33	0.75	0.21	0.69	0.67	0.72	0.75	0.58	0.86	0.14	0.81	0.78	0.81	0.83	0.72	0.91	0.10	0.88	740
0.03	0.19	0.37	0.37	0.14	0.60	0.23	0.50	0.46	0.59	0.62	0.40	0.77	0.19	0.73	0.64	0.73	0.76	0.59	0.86	0.14	0.83	1132
0.06	0.06	0.24	0.20	0.04	0.44	0.20	0.39	0.37	0.51	0.52	0.33	0.68	0.17	0.64	0.59	0.68	0.69	0.55	0.80	0.12	0.78	1401
0.11	0.00	0.19	0.17	0.01	0.38	0.18	0.30	0.37	0.49	0.50	0.33	0.64	0.15	0.60	0.59	0.67	0.67	0.56	0.78	0.11	0.75	1387
0.15	0.00	0.15	0.12	-0.01	0.31	0.16	0.25	0.36	0.46	0.47	0.32	0.61	0.14	0.57	0.58	0.65	0.65	0.54	0.75	0.11	0.72	1395
0.18	0.00	0.12	0.06	-0.03	0.27	0.15	0.20	0.33	0.41	0.40	0.27	0.55	0.14	0.50	0.56	0.62	0.62	0.52	0.72	0.10	0.68	930
0.32	0.00	0.08	0.00	-0.05	0.22	0.13	0.11	0.29	0.38	0.38	0.23	0.52	0.15	0.49	0.53	0.61	0.61	0.50	0.71	0.10	0.67	525


==> data/mlm_plots/tef/yelp/roberta/s/top_intersections_auc.tex <==
name	auc
top10	0.05
top30	0.14
top50	0.20


==> data/mlm_plots/tef/yelp/xlnet/a/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	33.06	46.61	42.16	26.33	66.90	20.28	54.11	11.00	15.50	15.00	9.23	21.77	6.27	20.00	38.41	52.81	47.59	30.16	75.45	22.65	60.15	11.00	15.71	16.00	9.43	21.98	6.28	20.00	722
0.03	34.36	49.76	43.54	22.49	77.04	27.27	57.10	9.00	14.18	13.50	7.71	20.65	6.47	19.00	44.96	63.40	55.69	30.78	96.01	32.62	71.15	9.00	14.52	14.00	7.99	21.06	6.53	19.00	974
0.06	34.36	52.75	43.74	13.01	92.49	39.74	58.22	8.00	13.64	13.00	6.66	20.62	6.98	19.00	53.32	80.90	68.47	19.66	142.15	61.24	88.34	8.00	14.38	14.00	7.13	21.63	7.25	19.00	1213
0.11	34.36	52.94	44.76	21.54	84.33	31.40	58.78	8.00	13.58	13.00	6.65	20.52	6.93	19.00	68.31	100.49	85.39	45.25	155.74	55.25	115.05	8.00	14.68	14.00	7.32	22.05	7.36	21.00	1364
0.15	34.74	52.88	44.83	18.08	87.67	34.80	58.87	7.00	12.84	12.00	5.95	19.74	6.89	18.00	88.79	127.65	109.11	53.83	201.48	73.82	144.22	8.00	14.48	14.00	7.01	21.95	7.47	20.00	1254
0.18	33.85	56.51	44.40	8.65	104.38	47.86	60.75	7.00	11.98	11.00	5.41	18.56	6.58	17.00	111.79	170.96	139.79	38.26	303.66	132.70	191.08	8.00	14.18	13.00	6.59	21.77	7.59	20.00	952
0.32	36.59	60.61	48.42	9.51	111.72	51.11	65.93	6.00	11.24	10.00	4.77	17.70	6.47	16.00	143.32	226.88	181.09	47.50	406.26	179.38	251.49	8.00	13.87	13.00	6.11	21.63	7.76	19.00	1086


==> data/mlm_plots/tef/yelp/xlnet/a/comparison_vals_auc.tex <==
name	auc
orig_pp	17.10
orig_ge	3.93
adv_pp	44.65
adv_ge	4.45


==> data/mlm_plots/tef/yelp/xlnet/a/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.48	0.68	0.75	0.42	0.95	0.27	0.92	0.89	0.91	0.94	0.80	1.01	0.11	0.97	0.73	0.78	0.81	0.65	0.90	0.12	0.86	722
0.03	0.29	0.53	0.54	0.24	0.83	0.30	0.80	0.79	0.84	0.88	0.69	0.98	0.15	0.93	0.61	0.69	0.72	0.54	0.83	0.15	0.79	974
0.06	0.14	0.39	0.35	0.09	0.70	0.30	0.63	0.67	0.74	0.79	0.54	0.94	0.20	0.88	0.49	0.58	0.61	0.40	0.76	0.18	0.70	1213
0.11	0.08	0.32	0.26	0.03	0.61	0.29	0.53	0.58	0.67	0.72	0.44	0.89	0.23	0.84	0.42	0.51	0.54	0.32	0.70	0.19	0.65	1364
0.15	-0.01	0.20	0.13	-0.09	0.48	0.29	0.35	0.42	0.55	0.63	0.27	0.83	0.28	0.77	0.31	0.41	0.45	0.20	0.63	0.22	0.58	1254
0.18	-0.07	0.11	0.04	-0.16	0.38	0.27	0.23	0.25	0.45	0.51	0.13	0.77	0.32	0.71	0.17	0.33	0.37	0.09	0.58	0.24	0.52	952
0.32	-0.11	0.04	-0.01	-0.22	0.30	0.26	0.13	0.09	0.35	0.41	-0.00	0.70	0.35	0.66	0.06	0.26	0.29	-0.00	0.52	0.26	0.48	1086


==> data/mlm_plots/tef/yelp/xlnet/a/correlations_auc.tex <==
name	auc
pcc	0.07
spearman	0.17
kendall	0.13


==> data/mlm_plots/tef/yelp/xlnet/a/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	1.41	5.63	4.17	0.25	11.01	5.38	8.26	1.28	5.43	3.71	0.11	10.75	5.32	8.04	1.37	6.43	4.05	-0.39	13.26	6.83	9.17	722
0.03	1.81	4.53	3.99	0.90	8.15	3.62	6.18	1.76	4.48	3.80	0.71	8.25	3.77	6.07	2.06	6.72	4.52	-0.16	13.61	6.88	8.82	974
0.06	2.04	3.58	3.52	1.34	5.82	2.24	4.76	1.94	3.54	3.33	1.20	5.88	2.34	4.70	2.51	5.84	4.37	0.42	11.27	5.42	7.36	1213
0.11	1.83	2.87	2.82	1.32	4.41	1.55	3.73	1.71	2.81	2.72	1.20	4.41	1.60	3.60	2.18	4.27	3.58	0.74	7.79	3.53	5.32	1364
0.15	1.98	2.55	2.55	1.47	3.64	1.09	3.17	1.92	2.52	2.47	1.40	3.64	1.12	3.10	2.18	3.75	3.17	0.78	6.72	2.97	4.45	1254
0.18	2.02	2.45	2.45	1.54	3.36	0.91	2.93	1.94	2.44	2.41	1.47	3.42	0.97	2.94	2.03	3.40	2.86	0.94	5.86	2.46	4.08	952
0.32	1.95	2.32	2.31	1.50	3.14	0.82	2.65	1.91	2.30	2.27	1.48	3.12	0.82	2.67	1.83	3.02	2.55	0.51	5.52	2.51	3.48	1086


==> data/mlm_plots/tef/yelp/xlnet/a/ets_sts_auc.tex <==
name	auc
et_use	0.90
et_tse	0.89
et_ce	1.29


==> data/mlm_plots/tef/yelp/xlnet/a/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.33	1.90	0.94	-2.17	5.98	4.08	2.09	1.36	5.81	3.73	-0.65	12.28	6.47	7.71	1.35	6.19	3.40	-1.65	14.02	7.83	8.09	722
0.03	0.35	1.19	0.76	-1.22	3.60	2.41	1.31	1.96	5.47	4.34	0.20	10.74	5.27	7.09	1.86	5.62	3.81	-0.49	11.73	6.11	6.84	974
0.06	0.32	0.71	0.54	-0.77	2.20	1.48	0.84	2.63	4.94	4.46	1.11	8.77	3.83	6.16	2.37	5.04	3.98	-0.29	10.36	5.33	5.80	1213
0.11	0.23	0.53	0.36	-2.72	3.77	3.24	0.51	2.69	4.14	3.91	1.59	6.68	2.54	5.16	2.27	4.00	3.43	0.37	7.62	3.62	4.70	1364
0.15	0.19	0.34	0.27	-0.28	0.97	0.62	0.38	2.94	4.00	3.90	1.94	6.06	2.06	4.97	2.42	3.79	3.35	0.97	6.60	2.81	4.64	1254
0.18	0.15	0.26	0.21	-0.17	0.69	0.43	0.29	2.87	4.01	3.63	1.18	6.83	2.83	4.69	2.40	3.86	3.15	0.20	7.52	3.66	4.31	952
0.32	0.12	0.22	0.17	-0.39	0.83	0.61	0.24	2.82	3.82	3.57	1.76	5.88	2.06	4.40	2.38	3.74	3.04	-0.37	7.86	4.12	4.06	1086


==> data/mlm_plots/tef/yelp/xlnet/a/ets_time_misc_auc.tex <==
name	auc
et_p	0.15
et_p_h	1.33
et_p_l2	1.31


==> data/mlm_plots/tef/yelp/xlnet/a/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.09	0.14	0.13	0.06	0.22	0.08	0.18	0.02	0.04	0.03	0.01	0.07	0.03	0.05	0.02	0.04	0.03	0.02	0.05	0.02	0.05	722
0.03	0.20	0.29	0.28	0.15	0.43	0.14	0.37	0.03	0.06	0.05	0.02	0.09	0.03	0.08	0.03	0.05	0.05	0.03	0.08	0.02	0.07	974
0.06	0.40	0.57	0.55	0.31	0.82	0.25	0.71	0.05	0.08	0.08	0.04	0.12	0.04	0.11	0.05	0.07	0.07	0.04	0.10	0.03	0.09	1213
0.11	0.70	0.97	0.93	0.57	1.37	0.40	1.18	0.08	0.10	0.10	0.06	0.14	0.04	0.13	0.07	0.09	0.09	0.06	0.12	0.03	0.11	1364
0.15	1.11	1.55	1.48	0.87	2.24	0.68	1.88	0.10	0.13	0.12	0.08	0.17	0.05	0.16	0.09	0.11	0.11	0.08	0.14	0.03	0.13	1254
0.18	1.65	2.26	2.12	1.29	3.22	0.96	2.77	0.11	0.14	0.15	0.09	0.19	0.05	0.18	0.11	0.13	0.13	0.09	0.16	0.03	0.15	952
0.32	2.06	3.10	2.76	1.45	4.75	1.65	3.76	0.13	0.16	0.16	0.10	0.21	0.05	0.19	0.12	0.14	0.14	0.10	0.17	0.04	0.16	1086


==> data/mlm_plots/tef/yelp/xlnet/a/pp_distances_auc.tex <==
name	auc
pp_r_d	0.54
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/xlnet/a/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.95	0.97	0.97	0.94	0.99	0.02	0.98	722
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.96	0.93	0.94	0.94	0.92	0.96	0.02	0.96	0.93	0.95	0.95	0.91	0.98	0.04	0.97	974
0.06	0.89	0.91	0.91	0.88	0.93	0.03	0.93	0.88	0.90	0.91	0.87	0.94	0.03	0.93	0.90	0.92	0.93	0.88	0.97	0.05	0.96	1213
0.11	0.85	0.87	0.87	0.84	0.91	0.03	0.89	0.85	0.87	0.87	0.83	0.91	0.04	0.89	0.86	0.89	0.91	0.83	0.96	0.06	0.93	1364
0.15	0.81	0.84	0.84	0.81	0.87	0.03	0.86	0.81	0.83	0.83	0.79	0.87	0.04	0.85	0.83	0.86	0.87	0.80	0.93	0.06	0.91	1254
0.18	0.79	0.81	0.81	0.78	0.84	0.03	0.83	0.78	0.81	0.81	0.77	0.85	0.04	0.83	0.80	0.84	0.84	0.77	0.90	0.07	0.89	952
0.32	0.76	0.79	0.78	0.75	0.82	0.04	0.81	0.75	0.78	0.78	0.74	0.82	0.04	0.81	0.75	0.80	0.81	0.71	0.89	0.09	0.86	1086


==> data/mlm_plots/tef/yelp/xlnet/a/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/yelp/xlnet/a/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	3.15	4.67	4.33	2.61	6.73	2.06	5.60	0.06	0.13	0.11	0.03	0.23	0.10	0.18	2.36	14.15	7.02	-3.38	31.68	17.53	19.75	722
0.03	5.40	9.20	8.03	3.83	14.57	5.37	11.54	0.09	0.17	0.15	0.06	0.29	0.11	0.22	3.44	16.36	9.52	-2.38	35.11	18.75	22.05	974
0.06	7.12	15.55	12.00	4.07	27.03	11.48	21.63	0.12	0.21	0.19	0.08	0.35	0.14	0.27	4.37	20.79	12.40	-2.60	44.19	23.40	30.08	1213
0.11	10.01	19.14	17.34	8.09	30.19	11.05	26.49	0.14	0.24	0.20	0.09	0.39	0.15	0.30	5.18	21.81	14.89	-0.50	44.12	22.31	29.85	1364
0.15	12.93	22.26	20.84	10.22	34.29	12.04	30.15	0.16	0.27	0.23	0.11	0.43	0.16	0.33	5.82	22.60	13.28	-1.30	46.50	23.90	31.01	1254
0.18	13.95	25.18	23.69	10.52	39.84	14.66	33.18	0.17	0.28	0.23	0.11	0.45	0.17	0.36	4.66	22.33	13.13	-1.08	45.74	23.41	31.58	952
0.32	13.11	25.54	22.31	9.21	41.88	16.34	32.89	0.18	0.29	0.23	0.12	0.47	0.18	0.36	4.36	21.50	12.60	-1.60	44.60	23.10	30.82	1086


==> data/mlm_plots/tef/yelp/xlnet/a/time_misc_auc.tex <==
name	auc
attack_time	6.48
l2	0.08
lom	6.57


==> data/mlm_plots/tef/yelp/xlnet/a/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.53	0.66	0.70	0.45	0.87	0.21	0.82	0.78	0.82	0.84	0.71	0.93	0.11	0.90	0.86	0.89	0.91	0.82	0.96	0.07	0.94	722
0.03	0.36	0.53	0.53	0.29	0.76	0.24	0.70	0.67	0.75	0.78	0.61	0.88	0.14	0.85	0.80	0.85	0.86	0.76	0.93	0.08	0.91	974
0.06	0.20	0.40	0.39	0.14	0.67	0.26	0.58	0.58	0.67	0.69	0.50	0.83	0.16	0.78	0.75	0.80	0.81	0.69	0.90	0.10	0.86	1213
0.11	0.17	0.35	0.33	0.10	0.60	0.25	0.50	0.50	0.62	0.64	0.45	0.79	0.17	0.74	0.71	0.76	0.78	0.65	0.87	0.11	0.84	1364
0.15	0.00	0.25	0.20	0.01	0.49	0.24	0.40	0.41	0.54	0.56	0.34	0.73	0.19	0.67	0.65	0.71	0.74	0.59	0.84	0.13	0.81	1254
0.18	0.00	0.19	0.10	-0.04	0.42	0.23	0.33	0.33	0.47	0.50	0.28	0.67	0.20	0.63	0.58	0.67	0.70	0.53	0.82	0.14	0.78	952
0.32	0.00	0.16	0.00	-0.07	0.39	0.23	0.29	0.25	0.43	0.43	0.21	0.65	0.22	0.59	0.53	0.63	0.65	0.47	0.78	0.16	0.75	1086


==> data/mlm_plots/tef/yelp/xlnet/a/top_intersections_auc.tex <==
name	auc
top10	0.09
top30	0.17
top50	0.22


==> data/mlm_plots/tef/yelp/xlnet/ig/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	32.96	46.41	42.36	27.40	65.42	19.01	54.72	10.00	15.05	14.00	8.88	21.22	6.17	19.00	37.61	52.92	48.78	31.28	74.56	21.64	61.59	10.00	15.32	15.00	9.08	21.56	6.24	20.00	720
0.03	34.72	51.50	44.36	20.65	82.35	30.85	57.22	8.00	13.44	13.00	6.82	20.06	6.62	18.00	44.27	65.81	57.01	28.38	103.24	37.43	73.99	8.00	13.91	13.00	7.09	20.73	6.82	19.00	994
0.06	34.94	56.14	45.18	12.56	99.73	43.58	60.77	7.00	12.54	12.00	5.67	19.42	6.87	17.00	55.17	83.70	69.94	30.07	137.33	53.63	91.59	7.00	13.32	13.00	6.08	20.56	7.24	18.00	1145
0.11	34.93	53.64	45.68	22.36	84.93	31.28	60.06	7.00	12.48	12.00	5.82	19.14	6.66	17.00	65.45	98.69	82.81	43.05	154.32	55.64	112.87	8.00	13.61	13.00	6.47	20.75	7.14	19.00	1079
0.15	34.28	55.80	44.25	5.93	105.67	49.87	59.29	7.00	13.07	12.00	6.14	20.01	6.93	18.00	86.36	128.09	107.16	51.99	204.18	76.09	141.13	9.00	14.91	14.00	7.11	22.70	7.79	21.00	1197
0.18	34.04	54.35	44.41	7.87	100.84	46.48	58.70	7.00	12.96	12.00	6.01	19.91	6.95	18.00	107.73	155.65	134.17	59.45	251.85	96.20	170.79	8.00	15.37	14.00	7.24	23.50	8.13	22.00	1111
0.32	36.80	60.29	47.83	7.16	113.43	53.13	63.99	7.00	12.12	11.00	5.32	18.93	6.80	16.00	139.91	210.59	178.96	91.73	329.45	118.86	235.22	8.00	14.70	14.00	6.61	22.80	8.10	21.00	1243


==> data/mlm_plots/tef/yelp/xlnet/ig/comparison_vals_auc.tex <==
name	auc
orig_pp	17.22
orig_ge	3.97
adv_pp	42.35
adv_ge	4.52


==> data/mlm_plots/tef/yelp/xlnet/ig/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.02	0.29	0.33	-0.11	0.70	0.41	0.61	0.26	0.45	0.54	0.09	0.80	0.35	0.71	0.19	0.35	0.41	0.07	0.64	0.28	0.56	720
0.03	-0.20	0.11	0.11	-0.31	0.53	0.42	0.41	0.05	0.28	0.34	-0.09	0.64	0.37	0.52	0.04	0.22	0.25	-0.07	0.50	0.28	0.40	994
0.06	-0.34	-0.05	-0.10	-0.45	0.35	0.40	0.23	-0.13	0.11	0.13	-0.24	0.46	0.35	0.35	-0.09	0.09	0.10	-0.17	0.35	0.26	0.26	1145
0.11	-0.48	-0.27	-0.31	-0.58	0.05	0.32	-0.10	-0.28	-0.08	-0.09	-0.38	0.22	0.30	0.11	-0.20	-0.05	-0.05	-0.28	0.17	0.22	0.08	1079
0.15	-0.62	-0.46	-0.48	-0.69	-0.22	0.24	-0.33	-0.46	-0.28	-0.28	-0.52	-0.03	0.24	-0.12	-0.33	-0.20	-0.19	-0.38	-0.01	0.18	-0.08	1197
0.18	-0.64	-0.51	-0.53	-0.70	-0.32	0.19	-0.40	-0.47	-0.33	-0.33	-0.53	-0.13	0.20	-0.20	-0.34	-0.23	-0.23	-0.38	-0.09	0.15	-0.14	1111
0.32	-0.64	-0.54	-0.55	-0.70	-0.38	0.16	-0.45	-0.49	-0.37	-0.38	-0.54	-0.21	0.17	-0.27	-0.35	-0.26	-0.27	-0.39	-0.14	0.13	-0.19	1243


==> data/mlm_plots/tef/yelp/xlnet/ig/correlations_auc.tex <==
name	auc
pcc	-0.11
spearman	-0.05
kendall	-0.04


==> data/mlm_plots/tef/yelp/xlnet/ig/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	6.16	12.92	10.86	3.71	22.13	9.21	17.59	5.47	12.45	9.94	3.07	21.83	9.38	16.98	5.70	15.65	11.79	2.33	28.97	13.32	22.03	720
0.03	5.18	8.83	7.76	3.63	14.03	5.20	11.76	4.73	8.67	7.46	2.84	14.49	5.83	11.36	5.46	13.57	10.01	1.45	25.68	12.11	17.96	994
0.06	4.25	6.42	6.10	3.06	9.78	3.36	8.07	3.84	6.25	5.72	2.29	10.21	3.96	7.83	4.63	11.09	7.86	0.77	21.42	10.33	13.51	1145
0.11	4.18	5.53	5.31	3.40	7.67	2.14	6.56	3.85	5.45	5.07	2.94	7.97	2.52	6.48	4.65	9.11	7.01	1.44	16.78	7.67	10.51	1079
0.15	3.87	4.70	4.53	3.39	6.00	1.31	5.35	3.67	4.67	4.48	3.13	6.21	1.54	5.42	4.43	7.35	5.99	1.26	13.44	6.09	8.36	1197
0.18	3.48	4.16	4.04	3.16	5.16	1.00	4.64	3.38	4.14	3.96	2.98	5.29	1.15	4.77	3.64	6.26	5.16	1.59	10.94	4.68	7.12	1111
0.32	3.19	3.74	3.60	2.83	4.65	0.91	4.11	3.09	3.75	3.58	2.69	4.81	1.06	4.13	3.10	5.07	4.24	1.40	8.75	3.68	5.72	1243


==> data/mlm_plots/tef/yelp/xlnet/ig/ets_sts_auc.tex <==
name	auc
et_use	1.64
et_tse	1.62
et_ce	2.50


==> data/mlm_plots/tef/yelp/xlnet/ig/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	1.40	5.00	2.43	-14.93	24.92	19.92	3.92	5.51	13.66	10.32	0.44	26.89	13.22	17.02	5.30	14.95	9.99	-1.40	31.30	16.35	18.43	720
0.03	0.95	2.29	1.56	-6.08	10.67	8.37	2.36	5.78	10.67	8.65	2.31	19.02	8.36	13.27	4.97	11.32	8.29	0.10	22.53	11.22	14.27	994
0.06	0.68	1.54	1.01	-4.93	8.01	6.47	1.42	5.35	9.00	7.67	2.54	15.46	6.46	10.88	4.63	9.36	6.98	0.53	18.18	8.82	11.01	1145
0.11	0.53	1.44	0.76	-5.96	8.84	7.40	1.00	5.67	8.16	7.28	3.18	13.14	4.98	9.28	4.73	8.31	6.32	-0.75	17.36	9.06	8.99	1079
0.15	0.40	0.64	0.51	-0.31	1.60	0.96	0.69	5.49	7.49	6.78	2.95	12.03	4.54	8.09	4.66	7.49	5.76	-1.87	16.85	9.36	7.54	1197
0.18	0.29	0.49	0.38	-0.85	1.83	1.34	0.50	5.10	6.48	6.05	4.02	8.95	2.46	7.28	4.26	6.21	5.19	0.92	11.49	5.28	6.63	1111
0.32	0.21	0.44	0.28	-2.26	3.14	2.70	0.40	4.84	6.11	5.58	3.68	8.54	2.43	6.64	3.98	5.96	4.88	1.32	10.61	4.64	6.07	1243


==> data/mlm_plots/tef/yelp/xlnet/ig/ets_time_misc_auc.tex <==
name	auc
et_p	0.33
et_p_h	2.38
et_p_l2	2.39


==> data/mlm_plots/tef/yelp/xlnet/ig/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.09	0.14	0.13	0.07	0.22	0.08	0.19	0.02	0.04	0.03	0.01	0.07	0.03	0.06	0.02	0.04	0.03	0.02	0.06	0.02	0.05	720
0.03	0.20	0.30	0.28	0.16	0.44	0.14	0.39	0.03	0.06	0.05	0.02	0.10	0.04	0.08	0.04	0.05	0.05	0.03	0.08	0.02	0.07	994
0.06	0.38	0.55	0.54	0.30	0.81	0.25	0.70	0.05	0.08	0.08	0.04	0.12	0.04	0.11	0.05	0.07	0.07	0.04	0.10	0.03	0.09	1145
0.11	0.65	0.91	0.87	0.49	1.33	0.42	1.10	0.07	0.10	0.10	0.06	0.15	0.04	0.13	0.07	0.09	0.09	0.06	0.12	0.03	0.11	1079
0.15	1.08	1.50	1.42	0.84	2.16	0.66	1.80	0.10	0.13	0.13	0.08	0.17	0.05	0.15	0.09	0.11	0.11	0.08	0.14	0.03	0.13	1197
0.18	1.54	2.12	2.01	1.23	3.01	0.89	2.56	0.12	0.15	0.15	0.10	0.19	0.05	0.18	0.11	0.13	0.13	0.10	0.16	0.03	0.15	1111
0.32	1.97	2.92	2.73	1.42	4.42	1.50	3.65	0.13	0.16	0.16	0.11	0.21	0.05	0.19	0.12	0.14	0.14	0.10	0.17	0.03	0.16	1243


==> data/mlm_plots/tef/yelp/xlnet/ig/pp_distances_auc.tex <==
name	auc
pp_r_d	0.51
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/xlnet/ig/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.96	0.98	0.01	0.98	0.96	0.97	0.97	0.95	0.98	0.02	0.98	0.96	0.97	0.97	0.94	0.99	0.02	0.98	720
0.03	0.93	0.94	0.95	0.92	0.96	0.02	0.96	0.93	0.94	0.94	0.91	0.97	0.03	0.96	0.93	0.95	0.96	0.91	0.99	0.04	0.98	994
0.06	0.89	0.91	0.91	0.88	0.94	0.03	0.93	0.89	0.90	0.91	0.87	0.94	0.04	0.93	0.90	0.92	0.94	0.87	0.98	0.05	0.96	1145
0.11	0.86	0.88	0.88	0.84	0.91	0.03	0.90	0.85	0.87	0.87	0.83	0.91	0.04	0.90	0.87	0.90	0.91	0.84	0.96	0.06	0.94	1079
0.15	0.82	0.84	0.84	0.81	0.87	0.03	0.86	0.81	0.83	0.84	0.79	0.87	0.04	0.86	0.84	0.87	0.88	0.81	0.93	0.06	0.91	1197
0.18	0.79	0.81	0.81	0.78	0.84	0.03	0.83	0.78	0.81	0.81	0.77	0.85	0.04	0.84	0.80	0.84	0.85	0.77	0.91	0.07	0.89	1111
0.32	0.76	0.79	0.79	0.75	0.82	0.04	0.81	0.76	0.78	0.78	0.74	0.83	0.04	0.81	0.76	0.81	0.82	0.72	0.89	0.08	0.86	1243


==> data/mlm_plots/tef/yelp/xlnet/ig/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/yelp/xlnet/ig/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	4.87	6.78	5.86	1.45	12.11	5.33	7.22	1.07	2.29	1.74	0.38	4.20	1.91	2.92	1.10	3.63	2.50	0.03	7.22	3.60	4.96	720
0.03	14.57	20.73	18.91	11.44	30.02	9.29	24.84	1.47	2.91	2.36	0.64	5.18	2.27	3.69	1.16	3.92	2.47	-0.71	8.55	4.63	5.12	994
0.06	8.31	15.12	10.80	1.60	28.63	13.51	15.13	1.85	3.66	2.93	0.69	6.64	2.97	4.70	1.21	4.11	2.79	-0.06	8.27	4.16	5.57	1145
0.11	22.93	33.60	31.45	18.06	49.14	15.54	41.58	2.12	3.94	3.22	1.15	6.74	2.79	5.04	1.28	4.40	3.10	-0.17	8.98	4.57	5.96	1079
0.15	18.81	38.99	34.19	15.57	62.41	23.42	53.18	2.23	4.03	3.56	1.43	6.62	2.60	5.14	1.55	4.83	3.55	0.20	9.47	4.64	6.74	1197
0.18	19.12	33.84	24.66	10.77	56.91	23.07	37.35	2.20	4.17	3.61	1.22	7.11	2.95	5.40	1.69	4.76	3.69	0.49	9.03	4.27	6.64	1111
0.32	27.86	51.24	48.96	23.00	79.47	28.23	66.89	2.47	4.50	3.92	1.21	7.79	3.29	5.75	1.68	4.49	3.43	0.40	8.57	4.09	5.91	1243


==> data/mlm_plots/tef/yelp/xlnet/ig/time_misc_auc.tex <==
name	auc
attack_time	10.57
l2	1.23
lom	1.39


==> data/mlm_plots/tef/yelp/xlnet/ig/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.23	0.41	0.40	0.18	0.63	0.22	0.56	0.43	0.56	0.60	0.37	0.75	0.19	0.71	0.60	0.69	0.72	0.54	0.83	0.14	0.79	720
0.03	0.12	0.30	0.27	0.07	0.52	0.23	0.44	0.35	0.47	0.49	0.28	0.66	0.19	0.60	0.53	0.62	0.64	0.47	0.76	0.15	0.71	994
0.06	0.00	0.20	0.15	-0.01	0.41	0.21	0.29	0.26	0.39	0.39	0.21	0.56	0.17	0.50	0.46	0.56	0.57	0.42	0.69	0.14	0.65	1145
0.11	0.00	0.11	0.06	-0.04	0.26	0.15	0.18	0.20	0.30	0.30	0.15	0.45	0.15	0.39	0.41	0.49	0.50	0.37	0.62	0.12	0.57	1079
0.15	0.00	0.05	0.00	-0.05	0.16	0.11	0.07	0.13	0.22	0.21	0.10	0.34	0.12	0.30	0.34	0.42	0.42	0.32	0.52	0.10	0.49	1197
0.18	0.00	0.04	0.00	-0.05	0.12	0.08	0.06	0.11	0.19	0.18	0.09	0.29	0.10	0.26	0.35	0.40	0.40	0.32	0.49	0.09	0.46	1111
0.32	0.00	0.03	0.00	-0.04	0.09	0.07	0.00	0.11	0.17	0.17	0.07	0.27	0.10	0.23	0.33	0.39	0.39	0.31	0.47	0.08	0.44	1243


==> data/mlm_plots/tef/yelp/xlnet/ig/top_intersections_auc.tex <==
name	auc
top10	0.03
top30	0.08
top50	0.14


==> data/mlm_plots/tef/yelp/xlnet/s/comparison_vals.tex <==
x	orig_pp_lq	orig_pp_mean	orig_pp_median	orig_pp_mms	orig_pp_mps	orig_pp_std	orig_pp_uq	orig_ge_lq	orig_ge_mean	orig_ge_median	orig_ge_mms	orig_ge_mps	orig_ge_std	orig_ge_uq	adv_pp_lq	adv_pp_mean	adv_pp_median	adv_pp_mms	adv_pp_mps	adv_pp_std	adv_pp_uq	adv_ge_lq	adv_ge_mean	adv_ge_median	adv_ge_mms	adv_ge_mps	adv_ge_std	adv_ge_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	33.30	46.76	42.32	26.57	66.96	20.19	54.39	10.00	15.15	15.00	8.93	21.37	6.22	19.00	39.06	53.29	48.44	31.15	75.43	22.14	61.13	10.00	15.38	15.00	9.14	21.63	6.24	20.00	714
0.03	34.16	51.49	44.17	20.48	82.49	31.01	58.20	8.00	13.49	13.00	6.93	20.04	6.55	18.00	45.62	66.76	58.39	28.22	105.31	38.54	74.91	8.00	13.98	13.00	7.26	20.70	6.72	19.00	982
0.06	35.43	56.26	45.70	12.65	99.88	43.62	60.72	7.00	13.06	12.00	6.17	19.94	6.89	18.00	57.05	86.68	72.46	27.38	145.98	59.30	93.19	8.00	13.86	13.00	6.64	21.08	7.22	19.00	1107
0.11	35.79	54.60	45.63	22.16	87.05	32.44	60.75	7.00	12.92	12.00	5.97	19.87	6.95	18.00	69.73	102.35	86.59	47.02	157.67	55.33	117.23	8.00	14.21	14.00	6.67	21.76	7.54	20.00	1080
0.15	33.74	54.41	44.24	3.36	105.46	51.05	58.45	7.00	12.68	12.00	5.71	19.65	6.97	18.00	88.57	129.43	110.46	46.45	212.41	82.98	143.07	8.00	14.60	14.00	6.80	22.39	7.80	20.00	1080
0.18	33.38	53.54	44.08	10.89	96.19	42.65	58.35	7.00	12.85	12.00	6.05	19.64	6.80	18.00	112.37	159.60	138.91	75.25	243.95	84.35	178.21	9.00	15.41	15.00	7.43	23.38	7.98	22.00	1150
0.32	36.07	58.28	47.06	13.99	102.58	44.29	63.70	7.00	12.46	12.00	5.60	19.31	6.86	17.00	144.74	215.92	182.29	91.78	340.05	124.14	246.51	8.00	15.31	14.50	7.14	23.48	8.17	22.00	1406


==> data/mlm_plots/tef/yelp/xlnet/s/comparison_vals_auc.tex <==
name	auc
orig_pp	17.01
orig_ge	4.01
adv_pp	43.41
adv_ge	4.60


==> data/mlm_plots/tef/yelp/xlnet/s/correlations.tex <==
x	pcc_lq	pcc_mean	pcc_median	pcc_mms	pcc_mps	pcc_std	pcc_uq	spearman_lq	spearman_mean	spearman_median	spearman_mms	spearman_mps	spearman_std	spearman_uq	kendall_lq	kendall_mean	kendall_median	kendall_mms	kendall_mps	kendall_std	kendall_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.61	0.71	0.73	0.55	0.86	0.16	0.82	0.87	0.90	0.92	0.83	0.98	0.07	0.95	0.71	0.76	0.78	0.66	0.86	0.10	0.83	714
0.03	0.47	0.58	0.60	0.40	0.76	0.18	0.71	0.80	0.84	0.87	0.73	0.95	0.11	0.91	0.62	0.68	0.70	0.57	0.80	0.12	0.76	982
0.06	0.35	0.47	0.48	0.29	0.66	0.19	0.60	0.71	0.77	0.80	0.63	0.91	0.14	0.87	0.53	0.60	0.62	0.47	0.74	0.13	0.70	1107
0.11	0.28	0.39	0.39	0.22	0.57	0.17	0.51	0.65	0.72	0.75	0.58	0.86	0.14	0.82	0.48	0.55	0.56	0.42	0.68	0.13	0.64	1080
0.15	0.22	0.33	0.31	0.17	0.48	0.16	0.42	0.57	0.65	0.67	0.50	0.80	0.15	0.76	0.41	0.48	0.49	0.35	0.62	0.13	0.57	1080
0.18	0.17	0.28	0.26	0.13	0.42	0.15	0.36	0.50	0.60	0.61	0.44	0.75	0.15	0.71	0.35	0.44	0.44	0.31	0.56	0.13	0.53	1150
0.32	0.13	0.23	0.22	0.08	0.38	0.15	0.32	0.43	0.53	0.55	0.36	0.70	0.17	0.65	0.30	0.38	0.39	0.25	0.52	0.13	0.47	1406


==> data/mlm_plots/tef/yelp/xlnet/s/correlations_auc.tex <==
name	auc
pcc	0.11
spearman	0.20
kendall	0.15


==> data/mlm_plots/tef/yelp/xlnet/s/ets_sts.tex <==
x	et_use_lq	et_use_mean	et_use_median	et_use_mms	et_use_mps	et_use_std	et_use_uq	et_tse_lq	et_tse_mean	et_tse_median	et_tse_mms	et_tse_mps	et_tse_std	et_tse_uq	et_ce_lq	et_ce_mean	et_ce_median	et_ce_mms	et_ce_mps	et_ce_std	et_ce_uq	count
0.01	2.80	5.05	4.39	1.77	8.34	3.28	6.41	2.39	4.75	4.04	1.46	8.04	3.29	6.09	2.44	5.96	4.28	0.91	11.01	5.05	8.02	714
0.03	2.47	4.09	3.51	1.57	6.62	2.53	5.13	2.23	3.94	3.26	1.22	6.66	2.72	4.92	2.49	5.94	4.47	0.74	11.14	5.20	7.38	982
0.06	2.08	3.06	2.82	1.57	4.56	1.50	3.73	1.94	3.03	2.67	1.36	4.69	1.67	3.68	2.35	4.94	3.74	0.72	9.16	4.22	5.98	1107
0.11	1.91	2.66	2.47	1.42	3.91	1.24	3.16	1.78	2.58	2.31	1.23	3.94	1.35	3.01	2.15	4.09	3.16	0.55	7.63	3.54	4.77	1080
0.15	1.73	2.19	2.14	1.44	2.94	0.75	2.52	1.65	2.14	2.06	1.36	2.92	0.78	2.47	1.88	3.10	2.64	0.97	5.22	2.12	3.63	1080
0.18	1.60	1.96	1.91	1.37	2.55	0.59	2.24	1.56	1.93	1.89	1.32	2.54	0.61	2.22	1.74	2.80	2.36	0.75	4.86	2.05	3.11	1150
0.32	1.53	1.81	1.79	1.34	2.27	0.47	2.04	1.49	1.79	1.76	1.30	2.28	0.49	2.04	1.48	2.21	1.96	1.06	3.37	1.16	2.65	1406


==> data/mlm_plots/tef/yelp/xlnet/s/ets_sts_auc.tex <==
name	auc
et_use	0.77
et_tse	0.75
et_ce	1.09


==> data/mlm_plots/tef/yelp/xlnet/s/ets_time_misc.tex <==
x	et_p_lq	et_p_mean	et_p_median	et_p_mms	et_p_mps	et_p_std	et_p_uq	et_p_h_lq	et_p_h_mean	et_p_h_median	et_p_h_mms	et_p_h_mps	et_p_h_std	et_p_h_uq	et_p_l2_lq	et_p_l2_mean	et_p_l2_median	et_p_l2_mms	et_p_l2_mps	et_p_l2_std	et_p_l2_uq	count
0.01	0.63	1.61	0.96	-2.26	5.48	3.87	1.54	2.56	5.18	3.85	0.77	9.59	4.41	6.43	2.23	5.87	3.79	-1.38	13.12	7.25	7.00	714
0.03	0.45	1.04	0.65	-1.90	3.97	2.93	0.99	2.53	4.66	3.69	1.08	8.23	3.58	5.51	2.23	5.06	3.58	-0.44	10.56	5.50	5.77	982
0.06	0.31	0.70	0.44	-1.65	3.04	2.34	0.68	2.59	4.16	3.54	1.43	6.88	2.72	4.90	2.21	4.30	3.22	0.30	8.31	4.01	4.99	1107
0.11	0.23	0.45	0.33	-0.51	1.42	0.97	0.46	2.53	3.69	3.30	1.73	5.65	1.96	4.26	2.13	3.68	2.93	0.89	6.47	2.79	4.19	1080
0.15	0.17	0.29	0.22	-0.41	0.99	0.70	0.30	2.48	3.36	3.06	1.50	5.22	1.86	3.73	2.09	3.27	2.62	0.33	6.22	2.94	3.44	1080
0.18	0.13	0.20	0.16	0.05	0.34	0.15	0.22	2.40	3.01	2.79	1.87	4.14	1.13	3.39	2.01	2.85	2.39	0.91	4.79	1.94	3.01	1150
0.32	0.10	0.16	0.13	0.04	0.27	0.12	0.18	2.31	2.97	2.74	1.72	4.22	1.25	3.32	1.93	2.92	2.37	0.13	5.72	2.79	3.05	1406


==> data/mlm_plots/tef/yelp/xlnet/s/ets_time_misc_auc.tex <==
name	auc
et_p	0.13
et_p_h	1.08
et_p_l2	1.09


==> data/mlm_plots/tef/yelp/xlnet/s/pp_distances.tex <==
x	pp_r_d_lq	pp_r_d_mean	pp_r_d_median	pp_r_d_mms	pp_r_d_mps	pp_r_d_std	pp_r_d_uq	pp_l2_d_lq	pp_l2_d_mean	pp_l2_d_median	pp_l2_d_mms	pp_l2_d_mps	pp_l2_d_std	pp_l2_d_uq	pp_h_d_lq	pp_h_d_mean	pp_h_d_median	pp_h_d_mms	pp_h_d_mps	pp_h_d_std	pp_h_d_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	0.10	0.15	0.14	0.07	0.22	0.08	0.20	0.02	0.04	0.03	0.01	0.07	0.03	0.06	0.02	0.04	0.03	0.02	0.06	0.02	0.05	714
0.03	0.22	0.32	0.31	0.17	0.47	0.15	0.41	0.04	0.06	0.06	0.03	0.10	0.03	0.09	0.04	0.06	0.06	0.03	0.08	0.02	0.07	982
0.06	0.41	0.60	0.58	0.33	0.88	0.27	0.76	0.05	0.08	0.08	0.04	0.12	0.04	0.11	0.06	0.07	0.07	0.05	0.10	0.03	0.09	1107
0.11	0.69	0.97	0.91	0.44	1.50	0.53	1.18	0.07	0.11	0.11	0.06	0.15	0.04	0.13	0.08	0.09	0.09	0.06	0.12	0.03	0.11	1080
0.15	1.11	1.60	1.51	0.87	2.32	0.73	1.94	0.10	0.13	0.13	0.08	0.18	0.05	0.16	0.09	0.11	0.11	0.08	0.14	0.03	0.13	1080
0.18	1.64	2.27	2.18	1.33	3.21	0.94	2.77	0.12	0.15	0.15	0.10	0.19	0.04	0.18	0.11	0.13	0.13	0.10	0.16	0.03	0.15	1150
0.32	2.07	3.08	2.84	1.60	4.56	1.48	3.80	0.13	0.16	0.16	0.11	0.21	0.05	0.19	0.12	0.14	0.14	0.11	0.17	0.03	0.16	1406


==> data/mlm_plots/tef/yelp/xlnet/s/pp_distances_auc.tex <==
name	auc
pp_r_d	0.54
pp_l2_d	0.04
pp_h_d	0.03


==> data/mlm_plots/tef/yelp/xlnet/s/semantic_sims.tex <==
x	sts_use_lq	sts_use_mean	sts_use_median	sts_use_mms	sts_use_mps	sts_use_std	sts_use_uq	sts_tse_lq	sts_tse_mean	sts_tse_median	sts_tse_mms	sts_tse_mps	sts_tse_std	sts_tse_uq	sts_ce_lq	sts_ce_mean	sts_ce_median	sts_ce_mms	sts_ce_mps	sts_ce_std	sts_ce_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.96	0.97	0.97	0.95	0.98	0.01	0.98	0.95	0.96	0.97	0.94	0.98	0.02	0.98	0.95	0.96	0.97	0.94	0.99	0.03	0.98	714
0.03	0.93	0.94	0.94	0.92	0.96	0.02	0.96	0.92	0.94	0.94	0.91	0.96	0.03	0.95	0.93	0.95	0.95	0.91	0.98	0.04	0.97	982
0.06	0.89	0.91	0.91	0.88	0.93	0.03	0.92	0.88	0.90	0.90	0.87	0.94	0.03	0.92	0.90	0.92	0.93	0.88	0.97	0.05	0.96	1107
0.11	0.86	0.88	0.88	0.85	0.91	0.03	0.90	0.84	0.87	0.87	0.83	0.91	0.04	0.89	0.87	0.90	0.90	0.84	0.95	0.05	0.93	1080
0.15	0.82	0.84	0.84	0.81	0.87	0.03	0.86	0.81	0.83	0.83	0.79	0.87	0.04	0.86	0.83	0.86	0.87	0.80	0.92	0.06	0.91	1080
0.18	0.79	0.81	0.81	0.78	0.84	0.03	0.83	0.78	0.80	0.80	0.77	0.84	0.04	0.83	0.80	0.84	0.85	0.76	0.91	0.07	0.88	1150
0.32	0.76	0.78	0.78	0.75	0.82	0.03	0.80	0.75	0.78	0.78	0.74	0.82	0.04	0.80	0.75	0.79	0.81	0.71	0.88	0.08	0.85	1406


==> data/mlm_plots/tef/yelp/xlnet/s/semantic_sims_auc.tex <==
name	auc
sts_use	0.26
sts_tse	0.26
sts_ce	0.27


==> data/mlm_plots/tef/yelp/xlnet/s/time_misc.tex <==
x	attack_time_lq	attack_time_mean	attack_time_median	attack_time_mms	attack_time_mps	attack_time_std	attack_time_uq	l2_lq	l2_mean	l2_median	l2_mms	l2_mps	l2_std	l2_uq	lom_lq	lom_mean	lom_median	lom_mms	lom_mps	lom_std	lom_uq	count
0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0.00	0
0.01	6.14	7.87	7.46	5.42	10.31	2.45	9.56	83.18	224.38	155.60	-13.18	461.94	237.56	278.56	1.73	5.73	3.76	-0.39	11.85	6.12	7.76	714
0.03	5.50	8.09	7.15	3.40	12.79	4.69	9.12	125.90	325.82	225.07	-116.31	767.96	442.13	396.94	1.70	6.62	4.41	-0.49	13.73	7.11	9.23	982
0.06	7.47	11.78	9.74	4.09	19.48	7.69	13.39	158.13	473.32	296.87	-339.91	1286.55	813.23	522.95	1.86	7.95	5.02	-0.43	16.33	8.38	11.58	1107
0.11	9.44	15.04	13.31	6.40	23.68	8.64	17.89	188.00	516.36	361.52	-40.50	1073.21	556.86	631.67	2.16	8.74	5.42	-0.47	17.96	9.21	12.42	1080
0.15	12.82	18.69	17.26	9.46	27.92	9.23	22.50	206.82	551.08	400.24	7.93	1094.22	543.14	678.51	2.40	9.31	5.91	-0.06	18.67	9.36	13.50	1080
0.18	16.33	24.38	22.38	11.92	36.83	12.46	30.38	233.46	602.91	435.45	-36.50	1242.33	639.41	745.04	2.67	10.30	6.43	0.20	20.40	10.10	15.57	1150
0.32	18.34	28.17	25.74	13.50	42.83	14.66	35.06	258.00	662.16	501.28	50.83	1273.49	611.33	838.25	2.32	9.73	6.28	-0.24	19.70	9.97	13.91	1406


==> data/mlm_plots/tef/yelp/xlnet/s/time_misc_auc.tex <==
name	auc
attack_time	6.12
l2	169.50
lom	2.82


==> data/mlm_plots/tef/yelp/xlnet/s/top_intersections.tex <==
x	top10_lq	top10_mean	top10_median	top10_mms	top10_mps	top10_std	top10_uq	top30_lq	top30_mean	top30_median	top30_mms	top30_mps	top30_std	top30_uq	top50_lq	top50_mean	top50_median	top50_mms	top50_mps	top50_std	top50_uq	count
0.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	1.00	1.00	1.00	1.00	1.00	0.00	1.00	0
0.01	0.56	0.65	0.67	0.49	0.81	0.16	0.77	0.76	0.81	0.82	0.73	0.90	0.09	0.88	0.85	0.88	0.89	0.83	0.94	0.05	0.92	714
0.03	0.40	0.52	0.50	0.32	0.72	0.20	0.67	0.69	0.75	0.76	0.64	0.86	0.11	0.82	0.81	0.85	0.85	0.78	0.91	0.07	0.89	982
0.06	0.25	0.39	0.40	0.18	0.59	0.20	0.50	0.61	0.69	0.69	0.57	0.80	0.12	0.76	0.76	0.81	0.82	0.73	0.89	0.08	0.86	1107
0.11	0.17	0.30	0.29	0.11	0.49	0.19	0.43	0.57	0.65	0.66	0.53	0.77	0.12	0.72	0.74	0.78	0.79	0.71	0.86	0.08	0.84	1080
0.15	0.12	0.24	0.22	0.06	0.43	0.19	0.33	0.50	0.59	0.59	0.47	0.71	0.12	0.67	0.71	0.76	0.76	0.67	0.84	0.08	0.81	1080
0.18	0.06	0.20	0.18	0.03	0.37	0.17	0.29	0.47	0.55	0.55	0.43	0.67	0.12	0.62	0.68	0.73	0.74	0.65	0.81	0.08	0.78	1150
0.32	0.00	0.15	0.12	-0.00	0.31	0.16	0.25	0.42	0.49	0.50	0.37	0.62	0.12	0.58	0.65	0.71	0.71	0.62	0.79	0.08	0.76	1406


==> data/mlm_plots/tef/yelp/xlnet/s/top_intersections_auc.tex <==
name	auc
top10	0.08
top30	0.19
top50	0.24


==> data/mlm_plots/timing_data/agnews_bert_a_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.67	0.07	0.60	0.74	0.69	0.72	0.61	505	tef_at
1	1.88	0.30	1.58	2.18	1.84	2.06	1.68	505	mlm_at
2	1.42	0.21	1.20	1.63	1.40	1.53	1.24	505	mlm_d_at
3	0.82	0.08	0.75	0.90	0.82	0.88	0.76	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_a_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.57	0.15	1.42	1.72	1.59	1.69	1.47	505	tef_at
1	4.96	0.55	4.41	5.51	4.89	5.25	4.48	505	mlm_at
2	3.66	0.47	3.19	4.14	3.58	3.88	3.34	505	mlm_d_at
3	1.84	0.25	1.59	2.10	1.79	1.94	1.67	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_a_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.66	0.07	0.59	0.73	0.68	0.72	0.61	512	tef_at
1	1.88	0.31	1.58	2.19	1.82	2.05	1.67	512	mlm_at
2	1.43	0.22	1.21	1.65	1.41	1.54	1.24	512	mlm_d_at
3	0.82	0.07	0.74	0.89	0.82	0.87	0.76	512	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_a_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.49	0.13	1.36	1.62	1.46	1.57	1.39	505	tef_at
1	4.09	0.33	3.76	4.42	4.07	4.26	3.97	505	mlm_at
2	3.09	0.49	2.60	3.59	3.00	3.11	2.80	505	mlm_d_at
3	1.43	0.15	1.29	1.58	1.37	1.55	1.32	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_a_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.19	0.27	0.92	1.46	1.19	1.33	1.03	501	tef_at
1	2.05	0.48	1.56	2.53	2.03	2.28	1.81	501	mlm_at
2	1.70	0.42	1.27	2.12	1.70	1.86	1.49	501	mlm_d_at
3	1.29	0.30	0.98	1.59	1.30	1.42	1.11	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_a_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.95	0.67	2.29	3.62	2.97	3.30	2.54	501	tef_at
1	4.66	1.02	3.64	5.67	4.62	5.14	4.11	501	mlm_at
2	3.99	1.03	2.96	5.02	3.95	4.45	3.41	501	mlm_d_at
3	3.23	0.91	2.32	4.13	3.10	3.56	2.78	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_a_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.76	0.08	0.68	0.84	0.77	0.80	0.70	505	tef_at
1	1.24	0.17	1.08	1.41	1.24	1.32	1.11	505	mlm_at
2	1.02	0.14	0.88	1.16	1.02	1.11	0.93	505	mlm_d_at
3	0.75	0.07	0.67	0.82	0.76	0.80	0.70	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_a_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.67	0.17	1.49	1.84	1.67	1.78	1.53	512	tef_at
1	5.16	0.58	4.58	5.75	5.06	5.41	4.71	512	mlm_at
2	3.86	0.52	3.34	4.38	3.71	4.13	3.55	512	mlm_d_at
3	1.95	0.29	1.66	2.24	1.86	2.08	1.79	512	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_a_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.96	0.13	0.83	1.10	0.96	1.05	0.87	505	tef_at
1	1.86	0.33	1.54	2.19	1.79	2.04	1.61	505	mlm_at
2	1.47	0.24	1.24	1.71	1.44	1.62	1.33	505	mlm_d_at
3	1.02	0.13	0.88	1.15	1.01	1.11	0.94	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_a_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.44	0.34	2.10	2.77	2.36	2.66	2.21	505	tef_at
1	4.03	0.64	3.38	4.67	3.99	4.38	3.59	505	mlm_at
2	3.30	0.54	2.76	3.84	3.25	3.52	2.95	505	mlm_d_at
3	2.43	0.43	2.00	2.86	2.37	2.62	2.14	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_ig_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.10	0.21	1.89	2.31	2.09	2.27	1.90	505	tef_at
1	3.41	0.77	2.64	4.18	3.31	3.82	2.90	505	mlm_at
2	2.99	0.72	2.28	3.71	2.92	3.30	2.50	505	mlm_d_at
3	2.49	0.40	2.08	2.89	2.42	2.65	2.29	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_ig_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	4.76	0.40	4.36	5.16	4.80	5.02	4.52	474	tef_at
1	8.84	1.36	7.48	10.20	8.60	9.56	8.07	474	mlm_at
2	7.56	0.92	6.64	8.48	7.56	8.34	6.85	474	mlm_d_at
3	6.33	0.74	5.59	7.08	6.39	6.79	5.95	474	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_ig_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.11	0.21	1.90	2.31	2.09	2.26	1.94	512	tef_at
1	3.37	0.78	2.59	4.15	3.24	3.79	2.81	512	mlm_at
2	3.00	0.64	2.35	3.64	2.91	3.22	2.53	512	mlm_d_at
3	2.51	0.38	2.12	2.89	2.46	2.67	2.30	512	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_ig_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.33	0.24	2.09	2.58	2.29	2.51	2.17	509	tef_at
1	9.16	2.02	7.15	11.18	8.98	9.83	7.70	509	mlm_at
2	6.49	1.22	5.27	7.71	6.26	7.16	5.39	509	mlm_d_at
3	3.15	0.47	2.69	3.62	3.18	3.49	2.83	509	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_ig_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.59	0.38	1.21	1.97	1.61	1.78	1.33	501	tef_at
1	3.03	1.50	1.53	4.53	2.75	3.40	2.24	501	mlm_at
2	2.47	1.11	1.36	3.59	2.32	2.74	1.91	501	mlm_d_at
3	1.86	0.68	1.19	2.54	1.77	2.11	1.50	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_ig_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	3.71	0.86	2.86	4.57	3.67	4.25	3.23	501	tef_at
1	8.22	2.47	5.74	10.69	7.91	9.43	6.87	501	mlm_at
2	6.68	1.97	4.71	8.65	6.49	7.35	5.51	501	mlm_d_at
3	4.57	1.31	3.26	5.89	4.40	5.17	3.70	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_ig_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.87	0.03	0.84	0.91	0.87	0.90	0.84	517	tef_at
1	2.86	0.60	2.26	3.46	2.84	2.91	2.36	517	mlm_at
2	2.49	1.12	1.38	3.61	2.08	2.15	1.81	517	mlm_d_at
3	1.13	0.19	0.94	1.32	1.08	1.18	0.99	517	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_ig_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.32	0.23	2.09	2.55	2.30	2.50	2.18	509	tef_at
1	9.19	2.04	7.16	11.23	8.92	9.96	7.59	509	mlm_at
2	6.49	1.23	5.26	7.72	6.26	7.08	5.46	509	mlm_d_at
3	3.14	0.46	2.68	3.60	3.15	3.46	2.79	509	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_ig_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.15	0.16	0.99	1.31	1.15	1.25	1.04	505	tef_at
1	2.66	1.22	1.44	3.88	2.32	2.83	2.07	505	mlm_at
2	1.97	0.51	1.46	2.48	1.93	2.21	1.63	505	mlm_d_at
3	1.31	0.24	1.07	1.55	1.31	1.42	1.13	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_ig_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.92	0.39	2.53	3.32	2.94	3.16	2.71	505	tef_at
1	7.85	1.90	5.95	9.74	7.41	9.03	6.33	505	mlm_at
2	5.84	1.30	4.54	7.13	5.70	6.59	5.08	505	mlm_d_at
3	3.37	0.59	2.78	3.96	3.28	3.75	2.97	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_s_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.77	0.10	0.67	0.87	0.77	0.83	0.72	505	tef_at
1	2.69	1.31	1.38	4.00	2.54	2.78	2.06	505	mlm_at
2	1.71	0.49	1.22	2.19	1.55	2.04	1.34	505	mlm_d_at
3	1.08	0.39	0.69	1.48	0.93	1.18	0.85	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.90	0.21	1.68	2.11	1.89	2.05	1.74	505	tef_at
1	10.39	3.47	6.92	13.86	9.44	13.65	7.24	505	mlm_at
2	7.15	2.33	4.82	9.49	6.91	9.65	4.93	505	mlm_d_at
3	2.61	0.48	2.13	3.10	2.52	3.12	2.22	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_s_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.75	0.12	0.63	0.87	0.75	0.83	0.65	509	tef_at
1	2.70	1.28	1.42	3.97	2.51	2.78	2.02	509	mlm_at
2	1.71	0.47	1.25	2.18	1.57	2.04	1.36	509	mlm_d_at
3	1.07	0.39	0.68	1.47	0.93	1.17	0.83	509	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.79	0.32	2.47	3.11	2.75	2.99	2.62	512	tef_at
1	6.57	1.82	4.76	8.39	6.27	8.60	4.89	512	mlm_at
2	4.74	1.21	3.53	5.95	4.30	5.89	3.79	512	mlm_d_at
3	2.88	0.45	2.43	3.33	2.94	3.12	2.52	512	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_s_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.50	0.42	1.08	1.91	1.42	1.65	1.26	501	tef_at
1	2.99	1.66	1.33	4.64	2.62	3.21	2.31	501	mlm_at
2	2.31	0.97	1.34	3.28	2.13	2.44	1.88	501	mlm_d_at
3	1.77	0.70	1.07	2.47	1.68	1.87	1.46	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	3.59	0.86	2.73	4.45	3.51	3.96	3.17	501	tef_at
1	7.82	2.95	4.87	10.76	7.00	8.81	5.68	501	mlm_at
2	6.15	2.18	3.96	8.33	5.60	7.60	4.61	501	mlm_d_at
3	4.09	1.26	2.83	5.36	3.83	4.72	3.44	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_s_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.20	0.27	0.93	1.47	1.16	1.39	1.00	503	tef_at
1	2.00	0.76	1.24	2.76	1.85	2.11	1.56	503	mlm_at
2	1.58	0.61	0.97	2.19	1.43	1.69	1.27	503	mlm_d_at
3	1.26	0.29	0.96	1.55	1.19	1.39	1.05	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_s_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.64	0.32	2.32	2.96	2.61	2.83	2.46	505	tef_at
1	6.20	1.76	4.44	7.96	5.87	8.07	4.56	505	mlm_at
2	4.43	1.14	3.29	5.57	4.12	5.40	3.56	505	mlm_d_at
3	2.75	0.44	2.32	3.19	2.79	2.96	2.36	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_s_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.04	0.19	0.85	1.23	1.02	1.16	0.89	505	tef_at
1	3.03	1.44	1.59	4.48	2.80	3.35	2.24	505	mlm_at
2	2.08	0.72	1.36	2.80	1.88	2.25	1.66	505	mlm_d_at
3	1.36	0.44	0.92	1.80	1.25	1.41	1.10	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_bert_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.62	0.45	2.17	3.07	2.55	2.89	2.29	505	tef_at
1	7.25	2.44	4.82	9.69	6.39	9.55	5.27	505	mlm_at
2	5.33	1.73	3.60	7.06	4.87	6.88	3.95	505	mlm_d_at
3	2.83	0.67	2.16	3.51	2.62	3.10	2.40	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_ig_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.10	0.13	0.97	1.22	1.11	1.20	1.03	507	tef_at
1	2.55	0.37	2.18	2.92	2.46	2.65	2.33	507	mlm_at
2	1.92	0.24	1.68	2.16	1.89	2.11	1.78	507	mlm_d_at
3	1.30	0.13	1.17	1.43	1.32	1.41	1.22	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_ig_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.18	0.25	1.94	2.43	2.21	2.34	2.02	507	tef_at
1	6.14	1.38	4.76	7.52	5.84	6.47	5.55	507	mlm_at
2	4.56	0.63	3.93	5.19	4.51	4.87	4.17	507	mlm_d_at
3	2.50	0.26	2.23	2.76	2.56	2.67	2.33	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_ig_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.12	0.08	1.05	1.20	1.15	1.19	1.07	507	tef_at
1	1.91	0.24	1.67	2.14	1.87	1.96	1.78	507	mlm_at
2	1.50	0.13	1.37	1.63	1.47	1.56	1.38	507	mlm_d_at
3	1.13	0.07	1.07	1.20	1.13	1.19	1.10	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_ig_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.17	0.13	2.04	2.30	2.18	2.25	2.09	507	tef_at
1	4.01	0.75	3.26	4.75	3.80	4.08	3.59	507	mlm_at
2	3.19	0.56	2.62	3.75	3.04	3.20	2.90	507	mlm_d_at
3	2.19	0.15	2.04	2.33	2.21	2.34	2.04	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_ig_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.15	0.24	0.91	1.38	1.18	1.31	0.99	499	tef_at
1	1.73	0.40	1.33	2.13	1.79	1.99	1.47	499	mlm_at
2	1.44	0.31	1.13	1.75	1.49	1.65	1.26	499	mlm_d_at
3	1.18	0.25	0.94	1.43	1.20	1.35	1.04	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_ig_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.38	0.47	1.91	2.86	2.43	2.69	2.09	499	tef_at
1	4.84	1.28	3.56	6.12	4.96	5.51	4.21	499	mlm_at
2	3.73	0.88	2.85	4.61	3.88	4.20	3.31	499	mlm_d_at
3	2.38	0.47	1.91	2.85	2.42	2.71	2.09	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_ig_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.12	0.05	1.07	1.17	1.13	1.14	1.08	507	tef_at
1	2.99	0.43	2.56	3.43	2.94	3.18	2.76	507	mlm_at
2	2.14	0.22	1.92	2.36	2.18	2.31	1.93	507	mlm_d_at
3	1.33	0.05	1.28	1.38	1.34	1.37	1.31	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_ig_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.23	0.09	2.15	2.32	2.21	2.30	2.20	507	tef_at
1	7.16	2.17	4.99	9.33	6.34	6.87	6.00	507	mlm_at
2	5.10	0.71	4.40	5.81	4.93	5.25	4.77	507	mlm_d_at
3	2.59	0.11	2.48	2.70	2.64	2.68	2.49	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_ig_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.11	0.17	0.94	1.28	1.11	1.25	1.00	499	tef_at
1	2.43	0.45	1.99	2.88	2.42	2.60	2.20	499	mlm_at
2	1.86	0.30	1.57	2.16	1.88	2.00	1.67	499	mlm_d_at
3	1.29	0.19	1.10	1.49	1.30	1.43	1.17	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_ig_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.16	0.32	1.84	2.47	2.13	2.37	1.97	499	tef_at
1	5.72	1.28	4.45	7.00	5.66	6.06	5.10	499	mlm_at
2	4.27	0.68	3.59	4.96	4.22	4.65	3.80	499	mlm_d_at
3	2.46	0.33	2.12	2.79	2.45	2.66	2.27	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_s_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.63	0.08	0.55	0.71	0.63	0.68	0.58	507	tef_at
1	1.64	0.27	1.36	1.91	1.64	1.76	1.48	507	mlm_at
2	1.16	0.19	0.97	1.35	1.14	1.23	1.06	507	mlm_d_at
3	0.61	0.08	0.53	0.69	0.62	0.67	0.57	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.24	0.14	1.10	1.38	1.26	1.36	1.15	507	tef_at
1	4.61	1.30	3.31	5.92	4.30	4.57	4.05	507	mlm_at
2	3.28	0.84	2.44	4.12	3.11	3.32	2.90	507	mlm_d_at
3	1.28	0.12	1.16	1.41	1.29	1.35	1.22	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_s_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.58	0.04	0.54	0.62	0.58	0.60	0.56	507	tef_at
1	2.09	0.32	1.77	2.41	2.06	2.18	1.90	507	mlm_at
2	1.45	0.21	1.23	1.66	1.39	1.58	1.27	507	mlm_d_at
3	0.72	0.06	0.66	0.78	0.70	0.74	0.69	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.30	0.08	1.22	1.38	1.33	1.35	1.24	507	tef_at
1	5.15	1.73	3.42	6.88	4.50	5.08	4.36	507	mlm_at
2	3.65	1.05	2.60	4.70	3.30	3.58	3.09	507	mlm_d_at
3	1.35	0.12	1.23	1.47	1.34	1.38	1.29	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_s_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.61	0.15	0.46	0.75	0.61	0.68	0.51	499	tef_at
1	1.04	0.28	0.76	1.32	1.05	1.18	0.91	499	mlm_at
2	0.79	0.21	0.59	1.00	0.81	0.91	0.69	499	mlm_d_at
3	0.55	0.14	0.41	0.69	0.55	0.64	0.46	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.34	0.28	1.07	1.62	1.36	1.55	1.18	499	tef_at
1	4.05	1.22	2.82	5.27	4.09	4.59	3.65	499	mlm_at
2	2.89	0.84	2.05	3.72	2.90	3.26	2.59	499	mlm_d_at
3	1.31	0.26	1.05	1.57	1.33	1.49	1.17	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_s_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.58	0.02	0.56	0.60	0.58	0.59	0.57	507	tef_at
1	2.24	0.32	1.92	2.56	2.11	2.48	2.08	507	mlm_at
2	1.57	0.21	1.36	1.78	1.48	1.69	1.43	507	mlm_d_at
3	0.73	0.07	0.66	0.80	0.70	0.74	0.69	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_s_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.31	0.04	1.27	1.35	1.30	1.33	1.29	507	tef_at
1	5.78	2.22	3.55	8.00	4.89	5.56	4.52	507	mlm_at
2	4.04	1.28	2.75	5.32	3.45	4.15	3.31	507	mlm_d_at
3	1.41	0.15	1.26	1.55	1.35	1.45	1.31	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_s_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.61	0.10	0.51	0.71	0.60	0.70	0.54	499	tef_at
1	1.48	0.28	1.20	1.76	1.46	1.67	1.27	499	mlm_at
2	1.07	0.20	0.86	1.27	1.07	1.16	0.92	499	mlm_d_at
3	0.59	0.10	0.49	0.70	0.60	0.67	0.52	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_cnn_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.26	0.18	1.08	1.45	1.28	1.38	1.18	499	tef_at
1	4.27	1.10	3.16	5.37	4.17	4.50	3.78	499	mlm_at
2	2.99	0.73	2.27	3.72	2.92	3.21	2.60	499	mlm_d_at
3	1.26	0.16	1.10	1.42	1.25	1.36	1.18	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_ig_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.64	0.08	0.56	0.72	0.65	0.71	0.60	499	tef_at
1	2.31	1.72	0.59	4.04	1.90	2.27	1.77	499	mlm_at
2	1.41	0.36	1.05	1.78	1.33	1.49	1.20	499	mlm_d_at
3	0.83	0.40	0.43	1.23	0.77	0.83	0.67	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_ig_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.42	0.17	1.25	1.59	1.43	1.53	1.32	499	tef_at
1	5.40	1.77	3.62	7.17	4.87	5.72	4.33	499	mlm_at
2	3.75	1.16	2.59	4.91	3.41	4.10	3.04	499	mlm_d_at
3	1.62	0.34	1.27	1.96	1.56	1.73	1.35	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_ig_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.61	0.04	0.57	0.65	0.61	0.63	0.58	499	tef_at
1	2.90	2.37	0.53	5.27	2.17	3.16	1.74	499	mlm_at
2	1.51	0.39	1.12	1.90	1.36	1.73	1.21	499	mlm_d_at
3	0.75	0.12	0.64	0.87	0.71	0.73	0.70	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_ig_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.32	0.07	1.26	1.39	1.35	1.37	1.27	499	tef_at
1	6.12	2.16	3.96	8.28	5.59	6.60	4.50	499	mlm_at
2	4.16	1.33	2.83	5.50	3.90	4.41	3.21	499	mlm_d_at
3	1.54	0.26	1.28	1.80	1.46	1.68	1.31	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_ig_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.91	0.23	0.68	1.14	0.89	1.05	0.77	499	tef_at
1	2.08	1.11	0.97	3.18	1.99	2.30	1.74	499	mlm_at
2	1.56	0.42	1.13	1.98	1.55	1.76	1.36	499	mlm_d_at
3	1.05	0.35	0.70	1.40	1.02	1.18	0.85	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_ig_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.88	0.44	1.43	2.32	1.84	2.19	1.57	499	tef_at
1	5.91	1.99	3.92	7.90	5.85	6.70	4.93	499	mlm_at
2	4.27	1.46	2.80	5.73	4.05	4.91	3.50	499	mlm_d_at
3	2.15	0.59	1.56	2.75	2.08	2.50	1.78	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_ig_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.60	0.03	0.57	0.63	0.60	0.61	0.58	499	tef_at
1	3.16	2.41	0.74	5.57	2.58	2.76	1.85	499	mlm_at
2	1.45	0.35	1.10	1.80	1.45	1.64	1.22	499	mlm_d_at
3	0.66	0.11	0.55	0.77	0.60	0.73	0.56	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_ig_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.38	0.11	1.27	1.48	1.35	1.50	1.26	499	tef_at
1	6.17	1.91	4.26	8.08	5.65	6.95	4.78	499	mlm_at
2	3.98	1.32	2.66	5.30	3.34	4.08	3.10	499	mlm_d_at
3	1.37	0.23	1.14	1.59	1.25	1.48	1.19	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_ig_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.82	0.15	0.67	0.96	0.80	0.92	0.72	499	tef_at
1	1.39	0.27	1.12	1.67	1.39	1.52	1.20	499	mlm_at
2	1.10	0.23	0.86	1.33	1.08	1.21	0.94	499	mlm_d_at
3	0.78	0.16	0.62	0.93	0.76	0.85	0.67	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_ig_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.76	0.30	1.45	2.06	1.77	1.99	1.55	499	tef_at
1	4.43	1.32	3.11	5.74	4.03	4.80	3.69	499	mlm_at
2	3.21	0.93	2.28	4.14	3.02	3.48	2.66	499	mlm_d_at
3	1.57	0.33	1.25	1.90	1.53	1.80	1.34	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_s_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.58	0.07	0.52	0.65	0.59	0.62	0.54	499	tef_at
1	1.10	0.18	0.92	1.29	1.11	1.26	1.00	499	mlm_at
2	0.80	0.12	0.68	0.93	0.77	0.88	0.69	499	mlm_d_at
3	0.53	0.06	0.47	0.59	0.53	0.57	0.51	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.57	0.18	1.39	1.75	1.57	1.71	1.48	499	tef_at
1	3.13	0.79	2.34	3.92	2.94	3.29	2.77	499	mlm_at
2	2.14	0.27	1.87	2.42	2.16	2.37	1.93	499	mlm_d_at
3	1.19	0.15	1.04	1.34	1.19	1.28	1.11	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_s_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.55	0.05	0.50	0.61	0.54	0.58	0.52	499	tef_at
1	1.12	0.15	0.97	1.27	1.09	1.25	0.96	499	mlm_at
2	0.79	0.09	0.70	0.88	0.78	0.83	0.71	499	mlm_d_at
3	0.49	0.03	0.46	0.52	0.49	0.50	0.47	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.57	0.08	1.49	1.65	1.58	1.60	1.53	499	tef_at
1	3.41	0.97	2.44	4.38	3.12	3.44	2.85	499	mlm_at
2	2.20	0.25	1.95	2.45	2.20	2.46	1.97	499	mlm_d_at
3	1.15	0.13	1.03	1.28	1.13	1.16	1.08	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_s_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.81	0.19	0.62	1.00	0.81	0.93	0.67	499	tef_at
1	1.86	0.50	1.36	2.35	1.87	2.13	1.62	499	mlm_at
2	1.41	0.36	1.05	1.77	1.38	1.58	1.27	499	mlm_d_at
3	0.92	0.23	0.70	1.15	0.91	1.03	0.79	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.71	0.39	1.32	2.10	1.68	1.95	1.47	499	tef_at
1	4.56	1.32	3.24	5.89	4.61	5.17	4.07	499	mlm_at
2	3.29	0.79	2.50	4.07	3.28	3.79	2.92	499	mlm_d_at
3	1.77	0.44	1.34	2.21	1.72	1.98	1.51	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_s_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.58	0.02	0.56	0.60	0.58	0.59	0.56	499	tef_at
1	1.89	0.21	1.68	2.10	1.92	2.06	1.90	499	mlm_at
2	1.19	0.16	1.03	1.35	1.20	1.21	1.07	499	mlm_d_at
3	0.56	0.04	0.52	0.60	0.55	0.56	0.54	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_s_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.16	0.03	1.13	1.19	1.16	1.17	1.15	499	tef_at
1	5.55	1.59	3.95	7.14	4.79	5.59	4.63	499	mlm_at
2	3.37	0.30	3.07	3.66	3.36	3.49	3.09	499	mlm_d_at
3	1.35	0.27	1.09	1.62	1.24	1.54	1.14	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_s_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.65	0.10	0.55	0.75	0.63	0.73	0.59	499	tef_at
1	1.81	0.37	1.44	2.17	1.77	1.96	1.51	499	mlm_at
2	1.30	0.24	1.05	1.54	1.26	1.38	1.12	499	mlm_d_at
3	0.76	0.13	0.63	0.89	0.76	0.84	0.68	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstm_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.45	0.21	1.24	1.66	1.41	1.56	1.36	499	tef_at
1	3.60	0.86	2.74	4.46	3.42	3.78	3.17	499	mlm_at
2	2.50	0.39	2.11	2.89	2.43	2.76	2.21	499	mlm_d_at
3	1.19	0.19	1.00	1.38	1.18	1.29	1.06	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_a_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.75	0.09	0.66	0.83	0.75	0.81	0.70	503	tef_at
1	2.57	0.55	2.02	3.11	2.56	2.95	2.15	503	mlm_at
2	1.73	0.32	1.41	2.06	1.73	1.88	1.57	503	mlm_d_at
3	0.96	0.13	0.83	1.10	0.94	1.03	0.86	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_a_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.79	0.19	1.60	1.98	1.79	1.91	1.67	503	tef_at
1	5.02	1.09	3.93	6.11	4.78	5.44	4.22	503	mlm_at
2	3.53	0.79	2.74	4.33	3.36	3.78	3.09	503	mlm_d_at
3	1.52	0.16	1.36	1.68	1.53	1.63	1.43	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_a_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.65	0.02	0.62	0.67	0.65	0.66	0.63	503	tef_at
1	2.12	0.30	1.82	2.42	2.15	2.30	1.95	503	mlm_at
2	1.39	0.25	1.14	1.63	1.31	1.43	1.27	503	mlm_d_at
3	0.71	0.09	0.62	0.80	0.69	0.76	0.65	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_a_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.40	0.05	1.35	1.45	1.40	1.44	1.38	503	tef_at
1	6.14	1.38	4.76	7.52	5.75	6.31	5.42	503	mlm_at
2	4.23	1.05	3.18	5.28	4.03	4.42	3.58	503	mlm_d_at
3	1.48	0.15	1.33	1.64	1.44	1.54	1.36	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_a_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.42	0.38	1.04	1.80	1.39	1.61	1.21	499	tef_at
1	2.66	0.80	1.86	3.47	2.59	3.07	2.25	499	mlm_at
2	2.17	0.59	1.58	2.76	2.13	2.46	1.84	499	mlm_d_at
3	1.66	0.46	1.20	2.12	1.62	1.85	1.35	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_a_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	3.03	0.80	2.23	3.83	2.97	3.37	2.57	499	tef_at
1	6.58	1.88	4.70	8.46	6.43	7.49	5.72	499	mlm_at
2	5.16	1.37	3.79	6.52	5.10	5.94	4.36	499	mlm_d_at
3	3.38	0.91	2.47	4.29	3.24	3.80	2.87	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_a_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.57	0.02	0.56	0.59	0.57	0.58	0.56	503	tef_at
1	2.68	0.29	2.38	2.97	2.71	2.77	2.50	503	mlm_at
2	1.72	0.29	1.43	2.02	1.56	1.82	1.50	503	mlm_d_at
3	0.82	0.13	0.68	0.95	0.81	0.85	0.69	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_a_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.29	0.03	1.26	1.32	1.28	1.32	1.27	503	tef_at
1	6.63	1.47	5.16	8.10	6.03	7.17	5.42	503	mlm_at
2	4.56	1.13	3.44	5.69	4.18	4.36	4.02	503	mlm_d_at
3	1.38	0.13	1.24	1.51	1.37	1.40	1.28	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_a_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.87	0.14	0.73	1.01	0.84	0.95	0.80	503	tef_at
1	1.91	0.44	1.47	2.36	1.76	2.22	1.55	503	mlm_at
2	1.44	0.28	1.16	1.72	1.43	1.62	1.23	503	mlm_d_at
3	0.93	0.15	0.78	1.09	0.90	1.04	0.82	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_a_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.91	0.30	1.61	2.20	1.86	2.07	1.73	503	tef_at
1	4.51	0.95	3.56	5.46	4.33	4.96	3.85	503	mlm_at
2	3.31	0.71	2.60	4.03	3.20	3.60	2.79	503	mlm_d_at
3	1.73	0.24	1.49	1.98	1.72	1.86	1.54	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_ig_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.06	0.19	0.87	1.25	1.06	1.15	0.94	503	tef_at
1	2.79	1.86	0.93	4.64	2.19	2.83	1.90	503	mlm_at
2	1.88	0.92	0.95	2.80	1.63	1.97	1.45	503	mlm_d_at
3	1.09	0.18	0.92	1.27	1.06	1.19	0.97	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_ig_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.45	0.35	2.11	2.80	2.42	2.68	2.18	503	tef_at
1	10.07	3.62	6.45	13.69	8.90	12.27	7.17	503	mlm_at
2	6.88	2.40	4.48	9.27	6.36	8.53	4.89	503	mlm_d_at
3	3.02	0.71	2.31	3.73	2.84	3.26	2.47	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_ig_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.96	0.07	0.89	1.03	0.89	1.03	0.89	51	tef_at
1	3.89	1.86	2.03	5.74	5.62	5.62	1.94	51	mlm_at
2	2.28	0.68	1.60	2.97	2.92	2.92	1.57	51	mlm_d_at
3	0.96	0.06	0.90	1.02	0.90	1.02	0.90	51	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_ig_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.13	0.00	2.13	2.13	2.13	2.13	2.13	24	tef_at
1	5.00	0.00	5.00	5.00	5.00	5.00	5.00	24	mlm_at
2	4.14	0.00	4.14	4.14	4.14	4.14	4.14	24	mlm_d_at
3	1.84	0.00	1.84	1.84	1.84	1.84	1.84	24	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_ig_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.70	1.34	1.36	4.04	2.49	3.17	1.49	31	tef_at
1	3.39	1.33	2.06	4.72	3.64	3.82	1.91	31	mlm_at
2	3.15	1.30	1.86	4.45	3.26	3.91	1.77	31	mlm_d_at
3	2.83	1.28	1.55	4.12	2.65	3.20	1.65	31	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_ig_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	5.41	1.64	3.77	7.05	5.08	6.08	4.45	467	tef_at
1	9.27	3.42	5.85	12.69	8.35	10.72	7.26	467	mlm_at
2	7.72	2.76	4.96	10.48	7.03	8.74	6.14	467	mlm_d_at
3	5.98	1.99	4.00	7.97	5.64	6.98	4.79	467	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_ig_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.79	0.06	0.74	0.85	0.79	0.84	0.75	503	tef_at
1	4.27	2.42	1.86	6.69	3.87	4.92	2.74	503	mlm_at
2	1.99	0.51	1.47	2.50	1.83	2.50	1.60	503	mlm_d_at
3	0.88	0.11	0.77	0.99	0.86	0.88	0.85	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_ig_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.78	0.10	1.68	1.88	1.78	1.83	1.72	503	tef_at
1	8.46	1.64	6.82	10.10	8.47	9.53	7.07	503	mlm_at
2	5.50	1.40	4.10	6.89	5.13	6.87	4.33	503	mlm_d_at
3	2.08	0.19	1.89	2.26	2.07	2.25	2.03	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_ig_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.69	0.34	1.35	2.03	1.68	1.86	1.43	503	tef_at
1	3.50	1.95	1.54	5.45	2.89	3.47	2.68	503	mlm_at
2	2.67	1.07	1.60	3.74	2.43	2.83	2.13	503	mlm_d_at
3	1.89	0.31	1.58	2.21	1.88	2.14	1.71	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_ig_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	3.56	0.72	2.84	4.28	3.51	3.97	3.07	503	tef_at
1	7.67	2.52	5.16	10.19	6.64	8.57	6.06	503	mlm_at
2	6.00	1.92	4.08	7.92	5.23	6.87	4.68	503	mlm_d_at
3	3.75	1.02	2.73	4.78	3.55	4.16	3.03	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_s_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.09	0.13	0.96	1.22	1.06	1.19	0.99	503	tef_at
1	2.52	1.59	0.93	4.11	2.08	2.42	1.95	503	mlm_at
2	1.70	0.43	1.28	2.13	1.60	1.74	1.52	503	mlm_d_at
3	1.11	0.14	0.97	1.26	1.08	1.18	0.99	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.39	0.28	2.10	2.67	2.36	2.56	2.16	503	tef_at
1	6.51	2.09	4.42	8.60	5.82	6.29	5.53	503	mlm_at
2	4.55	0.88	3.66	5.43	4.32	4.82	4.03	503	mlm_d_at
3	2.55	0.34	2.21	2.89	2.49	2.68	2.32	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_s_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.84	0.06	0.78	0.90	0.85	0.87	0.80	503	tef_at
1	3.18	2.40	0.77	5.58	2.41	2.74	2.21	503	mlm_at
2	1.85	0.54	1.31	2.38	1.64	1.90	1.57	503	mlm_d_at
3	0.98	0.10	0.88	1.08	0.96	0.99	0.91	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.00	0.12	1.88	2.12	2.01	2.10	1.91	503	tef_at
1	4.19	1.30	2.90	5.49	3.62	4.25	3.38	503	mlm_at
2	2.75	0.49	2.26	3.25	2.61	2.83	2.51	503	mlm_d_at
3	1.69	0.15	1.54	1.85	1.66	1.75	1.61	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_s_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.88	0.87	2.02	3.75	2.82	3.17	2.42	499	tef_at
1	3.80	1.19	2.61	4.99	3.68	4.33	3.10	499	mlm_at
2	3.42	1.03	2.39	4.46	3.28	3.82	2.86	499	mlm_d_at
3	3.13	0.97	2.16	4.10	3.00	3.50	2.65	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	6.06	1.84	4.22	7.89	5.89	6.72	5.08	450	tef_at
1	8.40	2.43	5.97	10.83	8.20	9.35	7.08	450	mlm_at
2	7.32	2.17	5.15	9.50	6.95	8.17	6.26	450	mlm_d_at
3	6.42	2.01	4.41	8.43	6.17	7.16	5.38	450	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_s_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.66	0.02	0.64	0.68	0.66	0.68	0.65	503	tef_at
1	3.91	3.03	0.87	6.94	2.52	4.41	2.18	503	mlm_at
2	1.91	0.64	1.27	2.55	1.65	1.73	1.52	503	mlm_d_at
3	0.82	0.13	0.69	0.95	0.76	0.77	0.76	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_s_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.66	0.08	1.58	1.75	1.67	1.72	1.61	503	tef_at
1	6.51	2.53	3.98	9.04	5.00	8.01	4.54	503	mlm_at
2	3.63	1.05	2.58	4.68	3.28	3.35	3.09	503	mlm_d_at
3	1.48	0.24	1.24	1.71	1.38	1.49	1.31	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_s_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.71	0.29	1.42	2.00	1.66	1.93	1.49	503	tef_at
1	3.32	1.52	1.80	4.84	3.08	3.45	2.73	503	mlm_at
2	2.60	0.55	2.05	3.15	2.55	2.82	2.25	503	mlm_d_at
3	1.96	0.33	1.63	2.30	1.89	2.24	1.71	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_lstmatt_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	3.22	0.58	2.64	3.81	3.10	3.52	2.82	503	tef_at
1	6.09	1.51	4.58	7.59	5.61	6.47	5.33	503	mlm_at
2	4.69	0.85	3.85	5.54	4.50	5.03	4.19	503	mlm_d_at
3	3.21	0.58	2.63	3.80	3.12	3.66	2.79	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_a_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.54	0.06	0.48	0.61	0.55	0.59	0.50	501	tef_at
1	1.31	0.21	1.09	1.52	1.25	1.41	1.18	501	mlm_at
2	1.03	0.16	0.87	1.20	1.00	1.11	0.95	501	mlm_d_at
3	0.64	0.06	0.58	0.70	0.64	0.69	0.61	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_a_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.32	0.19	1.13	1.50	1.35	1.40	1.17	501	tef_at
1	3.81	0.67	3.15	4.48	3.69	3.94	3.43	501	mlm_at
2	2.91	0.49	2.42	3.41	2.82	3.27	2.60	501	mlm_d_at
3	1.47	0.22	1.25	1.68	1.47	1.59	1.34	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_a_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.52	0.04	0.48	0.56	0.51	0.55	0.49	501	tef_at
1	1.41	0.23	1.19	1.64	1.30	1.48	1.27	501	mlm_at
2	1.10	0.16	0.94	1.25	1.05	1.18	0.97	501	mlm_d_at
3	0.63	0.04	0.59	0.68	0.63	0.66	0.59	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_a_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.27	0.15	1.13	1.42	1.26	1.36	1.20	508	tef_at
1	5.17	0.86	4.32	6.03	5.04	5.47	4.59	508	mlm_at
2	3.76	0.69	3.07	4.46	3.76	4.16	3.24	508	mlm_d_at
3	1.75	0.23	1.52	1.98	1.78	1.87	1.60	508	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_a_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.89	0.21	0.68	1.09	0.87	1.01	0.76	499	tef_at
1	1.68	0.41	1.27	2.08	1.65	1.88	1.45	499	mlm_at
2	1.40	0.33	1.07	1.74	1.42	1.60	1.19	499	mlm_d_at
3	1.08	0.23	0.85	1.32	1.10	1.23	0.95	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_a_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.77	0.74	2.03	3.51	2.76	3.17	2.22	501	tef_at
1	4.27	1.11	3.16	5.37	4.24	4.85	3.66	501	mlm_at
2	3.80	0.99	2.81	4.79	3.78	4.24	3.21	501	mlm_d_at
3	3.06	0.78	2.28	3.84	3.07	3.50	2.50	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_a_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.57	0.06	0.51	0.64	0.58	0.62	0.54	501	tef_at
1	0.96	0.13	0.83	1.09	0.94	1.01	0.87	501	mlm_at
2	0.80	0.10	0.70	0.90	0.79	0.84	0.76	501	mlm_d_at
3	0.61	0.06	0.55	0.67	0.61	0.64	0.57	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_a_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.73	0.26	1.48	1.99	1.69	1.94	1.60	501	tef_at
1	3.19	0.45	2.74	3.64	3.22	3.49	2.86	501	mlm_at
2	2.57	0.41	2.17	2.98	2.52	2.93	2.31	501	mlm_d_at
3	1.84	0.30	1.53	2.14	1.77	2.01	1.65	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_a_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.78	0.12	0.67	0.90	0.78	0.87	0.71	501	tef_at
1	1.18	0.20	0.97	1.38	1.16	1.30	1.04	501	mlm_at
2	1.02	0.17	0.85	1.19	1.01	1.13	0.92	501	mlm_d_at
3	0.83	0.11	0.72	0.94	0.84	0.91	0.74	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_a_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.65	0.24	1.42	1.89	1.66	1.80	1.50	501	tef_at
1	2.92	0.57	2.35	3.49	2.80	3.23	2.55	501	mlm_at
2	2.44	0.40	2.04	2.84	2.38	2.75	2.17	501	mlm_d_at
3	1.75	0.26	1.48	2.01	1.73	1.83	1.61	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_ig_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.83	0.15	0.68	0.99	0.83	0.93	0.69	501	tef_at
1	2.58	1.53	1.06	4.11	2.12	2.68	1.84	501	mlm_at
2	2.14	1.09	1.05	3.23	1.68	2.55	1.47	501	mlm_d_at
3	1.26	0.44	0.82	1.70	1.12	1.46	0.93	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_ig_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	4.20	0.50	3.70	4.70	4.30	4.53	3.98	485	tef_at
1	9.29	1.59	7.70	10.89	9.39	10.48	8.45	485	mlm_at
2	8.28	1.26	7.02	9.54	8.26	9.18	7.62	485	mlm_d_at
3	6.49	1.00	5.49	7.49	6.65	7.33	5.91	485	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_ig_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.76	0.25	1.51	2.01	1.74	1.90	1.62	508	tef_at
1	2.94	0.70	2.24	3.65	2.80	3.15	2.44	508	mlm_at
2	2.71	0.82	1.89	3.53	2.52	2.80	2.21	508	mlm_d_at
3	2.23	0.45	1.79	2.68	2.15	2.47	1.96	508	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_ig_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	4.23	0.69	3.54	4.92	4.16	4.87	3.65	477	tef_at
1	8.74	1.98	6.76	10.73	9.14	10.22	7.36	477	mlm_at
2	7.88	1.77	6.12	9.65	7.88	8.97	6.70	477	mlm_d_at
3	6.61	1.42	5.19	8.03	6.52	7.55	5.60	477	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_ig_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.22	0.63	1.59	2.84	2.18	2.49	1.90	499	tef_at
1	3.28	1.48	1.80	4.76	3.09	3.74	2.59	499	mlm_at
2	3.07	1.58	1.49	4.65	2.90	3.33	2.27	499	mlm_d_at
3	2.79	1.30	1.49	4.10	2.55	3.02	2.16	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_ig_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	5.34	1.21	4.13	6.56	5.42	6.13	4.80	409	tef_at
1	10.24	3.49	6.75	13.73	10.03	12.32	7.65	409	mlm_at
2	9.44	3.47	5.97	12.91	8.93	11.72	7.26	409	mlm_d_at
3	8.18	2.89	5.30	11.07	7.67	9.97	6.11	409	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_ig_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.75	0.04	0.71	0.79	0.75	0.76	0.71	515	tef_at
1	5.18	2.46	2.72	7.63	4.76	8.21	2.91	515	mlm_at
2	2.65	1.34	1.32	3.99	2.18	3.53	2.01	515	mlm_d_at
3	1.42	0.45	0.97	1.88	1.26	1.70	1.09	515	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_ig_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.80	0.07	1.73	1.87	1.80	1.85	1.78	515	tef_at
1	9.23	0.78	8.45	10.01	9.24	9.65	8.78	515	mlm_at
2	6.62	0.39	6.23	7.01	6.58	6.98	6.36	515	mlm_d_at
3	2.87	0.25	2.62	3.12	2.84	3.02	2.75	515	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_ig_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.97	0.19	0.77	1.16	0.95	1.07	0.85	501	tef_at
1	2.69	1.63	1.06	4.33	2.26	2.74	1.94	501	mlm_at
2	2.20	1.16	1.04	3.37	1.91	2.42	1.57	501	mlm_d_at
3	1.41	0.56	0.86	1.97	1.28	1.58	1.07	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_ig_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.40	0.36	2.04	2.76	2.40	2.64	2.21	501	tef_at
1	8.04	2.22	5.82	10.26	8.66	9.89	6.06	501	mlm_at
2	6.50	1.41	5.09	7.90	6.77	7.54	5.08	501	mlm_d_at
3	3.48	0.74	2.74	4.21	3.53	4.04	2.96	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_s_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.57	0.05	0.51	0.62	0.56	0.61	0.53	501	tef_at
1	1.44	0.67	0.77	2.11	1.26	1.43	1.11	501	mlm_at
2	0.99	0.19	0.80	1.18	0.96	1.07	0.86	501	mlm_d_at
3	0.73	0.27	0.46	1.01	0.67	0.71	0.63	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.34	0.14	1.20	1.48	1.34	1.47	1.23	501	tef_at
1	5.95	2.44	3.51	8.39	4.91	7.30	4.01	501	mlm_at
2	3.99	1.46	2.53	5.45	3.40	4.05	3.09	501	mlm_d_at
3	1.93	0.39	1.54	2.31	1.93	2.33	1.63	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_s_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.53	0.05	0.47	0.58	0.53	0.58	0.48	507	tef_at
1	1.77	0.79	0.98	2.56	1.55	1.78	1.38	507	mlm_at
2	1.17	0.25	0.92	1.42	1.15	1.31	1.00	507	mlm_d_at
3	0.82	0.31	0.51	1.13	0.75	0.80	0.68	507	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.39	0.15	1.24	1.54	1.40	1.50	1.27	508	tef_at
1	6.25	2.51	3.74	8.76	5.08	7.77	4.41	508	mlm_at
2	4.18	1.51	2.67	5.69	3.62	4.19	3.24	508	mlm_d_at
3	2.04	0.42	1.62	2.46	2.07	2.40	1.67	508	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_s_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.11	0.29	0.82	1.41	1.07	1.22	0.96	499	tef_at
1	1.80	0.60	1.19	2.40	1.73	2.01	1.44	499	mlm_at
2	1.49	0.36	1.12	1.85	1.45	1.70	1.27	499	mlm_d_at
3	1.26	0.36	0.90	1.61	1.20	1.42	1.04	499	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.54	0.63	1.91	3.17	2.42	2.87	2.15	501	tef_at
1	5.98	2.57	3.41	8.55	5.52	6.46	4.60	501	mlm_at
2	4.59	1.65	2.94	6.25	4.28	5.22	3.61	501	mlm_d_at
3	3.29	1.10	2.19	4.39	3.06	3.75	2.67	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_s_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.73	0.07	0.66	0.81	0.72	0.79	0.68	508	tef_at
1	1.45	0.98	0.47	2.42	1.14	1.27	1.02	508	mlm_at
2	0.98	0.14	0.83	1.12	0.95	1.06	0.86	508	mlm_d_at
3	0.80	0.09	0.71	0.88	0.79	0.85	0.73	508	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_s_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.92	0.20	1.72	2.12	1.92	2.08	1.78	501	tef_at
1	4.26	1.31	2.95	5.57	3.75	5.18	3.28	501	mlm_at
2	3.06	0.68	2.38	3.73	2.84	3.37	2.67	501	mlm_d_at
3	2.17	0.35	1.82	2.52	2.22	2.42	1.91	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_s_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.73	0.10	0.63	0.83	0.72	0.80	0.65	501	tef_at
1	1.69	0.63	1.06	2.32	1.58	1.73	1.41	501	mlm_at
2	1.27	0.23	1.04	1.50	1.22	1.41	1.10	501	mlm_d_at
3	0.97	0.29	0.67	1.26	0.93	1.03	0.85	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_roberta_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.83	0.28	1.55	2.11	1.82	1.99	1.60	501	tef_at
1	4.95	1.92	3.03	6.87	4.34	5.51	3.57	501	mlm_at
2	3.55	1.19	2.36	4.75	3.27	3.78	2.77	501	mlm_d_at
3	2.10	0.49	1.61	2.59	2.02	2.28	1.80	501	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_a_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.65	0.07	0.58	0.72	0.65	0.71	0.61	503	tef_at
1	2.33	1.57	0.76	3.90	2.05	2.29	1.52	503	mlm_at
2	1.51	1.01	0.49	2.52	1.20	1.40	0.99	503	mlm_d_at
3	0.87	0.43	0.44	1.31	0.74	0.88	0.67	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_a_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.56	0.16	1.40	1.72	1.54	1.69	1.43	503	tef_at
1	6.58	1.55	5.03	8.13	6.96	7.60	5.53	503	mlm_at
2	4.54	1.16	3.38	5.69	4.87	5.29	3.59	503	mlm_d_at
3	2.20	0.40	1.81	2.60	2.20	2.44	1.92	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_a_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.50	0.05	0.45	0.55	0.47	0.53	0.46	520	tef_at
1	2.52	1.89	0.63	4.41	1.95	2.57	1.14	520	mlm_at
2	1.85	1.06	0.79	2.90	1.42	1.92	1.21	520	mlm_d_at
3	0.87	0.38	0.49	1.26	0.70	0.93	0.65	520	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_a_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.86	0.20	1.66	2.07	1.82	1.98	1.76	503	tef_at
1	9.41	2.24	7.17	11.65	9.27	11.09	8.19	503	mlm_at
2	6.27	1.68	4.59	7.95	6.49	7.34	4.85	503	mlm_d_at
3	3.06	0.58	2.48	3.65	3.11	3.52	2.83	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_a_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.26	0.37	0.89	1.64	1.19	1.42	1.03	500	tef_at
1	2.47	1.58	0.89	4.05	2.04	2.53	1.74	500	mlm_at
2	2.13	1.66	0.48	3.79	1.69	2.10	1.46	500	mlm_d_at
3	1.68	0.84	0.84	2.51	1.50	1.76	1.24	500	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_a_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	3.83	1.04	2.79	4.87	3.79	4.34	3.06	490	tef_at
1	10.89	4.55	6.35	15.44	10.26	14.15	7.06	490	mlm_at
2	8.41	3.59	4.82	11.99	7.66	10.94	5.70	490	mlm_d_at
3	5.85	2.34	3.51	8.19	5.30	6.97	4.22	490	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_a_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.52	0.04	0.48	0.56	0.51	0.56	0.49	520	tef_at
1	2.65	2.00	0.65	4.64	2.06	2.76	1.19	520	mlm_at
2	1.95	1.14	0.82	3.09	1.55	1.99	1.21	520	mlm_d_at
3	0.94	0.43	0.51	1.37	0.73	0.99	0.66	520	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_a_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.55	0.16	1.39	1.71	1.54	1.67	1.45	503	tef_at
1	7.92	1.85	6.07	9.76	8.46	9.08	6.62	503	mlm_at
2	5.36	1.34	4.02	6.70	5.74	6.08	4.12	503	mlm_d_at
3	2.54	0.46	2.09	3.00	2.56	2.87	2.30	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_a_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.87	0.17	0.69	1.04	0.84	0.99	0.74	503	tef_at
1	2.48	2.02	0.46	4.50	1.84	2.36	1.49	503	mlm_at
2	1.92	1.48	0.44	3.40	1.34	1.80	1.19	503	mlm_d_at
3	1.13	0.39	0.74	1.52	1.02	1.24	0.94	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_a_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.03	0.30	1.73	2.32	1.98	2.25	1.84	503	tef_at
1	7.19	2.27	4.92	9.46	7.19	8.60	5.34	503	mlm_at
2	5.35	1.39	3.95	6.74	5.37	6.32	3.96	503	mlm_d_at
3	3.02	0.60	2.42	3.62	2.96	3.49	2.54	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_ig_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.85	0.12	0.73	0.98	0.83	0.93	0.78	503	tef_at
1	4.63	2.60	2.04	7.23	3.82	7.47	2.13	503	mlm_at
2	3.29	2.00	1.29	5.29	1.92	5.58	1.51	503	mlm_d_at
3	1.87	0.80	1.07	2.67	1.60	2.60	1.11	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_ig_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.95	0.22	1.73	2.17	1.90	2.11	1.76	503	tef_at
1	9.81	1.55	8.26	11.35	10.04	10.69	9.29	503	mlm_at
2	6.87	1.23	5.65	8.10	6.90	7.81	6.54	503	mlm_d_at
3	3.51	0.46	3.05	3.96	3.55	3.79	3.16	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_ig_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.86	0.12	0.74	0.98	0.82	0.94	0.77	503	tef_at
1	4.70	2.72	1.98	7.42	3.64	7.28	2.04	503	mlm_at
2	3.34	2.03	1.30	5.37	1.93	5.46	1.52	503	mlm_d_at
3	1.89	0.80	1.09	2.69	1.61	2.57	1.14	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_ig_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.99	0.23	1.77	2.22	1.96	2.17	1.78	503	tef_at
1	9.75	1.49	8.25	11.24	9.79	10.72	9.28	503	mlm_at
2	6.81	1.19	5.62	8.01	6.95	7.48	6.41	503	mlm_d_at
3	3.55	0.46	3.09	4.01	3.50	3.81	3.26	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_ig_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.46	0.43	1.03	1.89	1.38	1.61	1.18	500	tef_at
1	3.13	2.02	1.11	5.15	2.37	3.38	2.00	500	mlm_at
2	2.63	1.62	1.01	4.26	2.05	2.59	1.72	500	mlm_d_at
3	2.17	1.02	1.15	3.19	1.80	2.45	1.57	500	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_ig_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	3.32	0.85	2.47	4.16	3.15	3.75	2.76	500	tef_at
1	8.93	3.29	5.63	12.22	8.82	11.26	6.00	500	mlm_at
2	7.23	2.11	5.13	9.34	7.31	8.62	5.68	500	mlm_d_at
3	5.24	1.44	3.79	6.68	4.99	6.05	4.05	500	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_ig_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.86	0.14	0.72	0.99	0.82	0.93	0.76	512	tef_at
1	5.15	2.81	2.34	7.95	4.03	7.89	2.30	512	mlm_at
2	3.68	2.20	1.48	5.89	3.37	5.85	1.61	512	mlm_d_at
3	2.04	0.88	1.16	2.92	1.95	2.71	1.19	512	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_ig_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.05	0.21	1.84	2.26	2.04	2.22	1.91	503	tef_at
1	9.76	1.52	8.23	11.28	9.87	10.81	9.38	503	mlm_at
2	6.77	1.18	5.59	7.95	7.03	7.55	6.30	503	mlm_d_at
3	3.56	0.47	3.09	4.03	3.56	3.78	3.25	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_ig_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.03	0.20	0.83	1.23	1.00	1.13	0.89	503	tef_at
1	3.57	2.41	1.16	5.98	2.16	5.39	1.80	503	mlm_at
2	2.91	1.89	1.02	4.79	1.87	4.70	1.40	503	mlm_d_at
3	1.91	0.85	1.05	2.76	1.51	2.77	1.19	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_ig_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.32	0.38	1.93	2.70	2.22	2.50	2.06	503	tef_at
1	7.80	1.80	6.00	9.59	7.92	8.98	6.86	503	mlm_at
2	5.64	1.27	4.38	6.91	5.80	6.43	4.89	503	mlm_d_at
3	3.57	0.57	3.00	4.14	3.55	3.90	3.11	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_s_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.67	0.09	0.57	0.76	0.65	0.76	0.60	503	tef_at
1	2.12	0.87	1.25	2.99	1.82	2.50	1.53	503	mlm_at
2	1.70	0.98	0.71	2.68	1.37	1.87	1.15	503	mlm_d_at
3	1.19	0.62	0.57	1.81	0.91	1.40	0.76	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.53	0.17	1.35	1.70	1.52	1.67	1.39	503	tef_at
1	8.75	1.68	7.07	10.44	9.14	9.86	8.14	503	mlm_at
2	5.58	1.21	4.37	6.79	5.75	6.57	4.77	503	mlm_d_at
3	2.77	0.51	2.26	3.28	2.71	3.07	2.41	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_s_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.74	0.10	0.63	0.84	0.70	0.82	0.67	512	tef_at
1	2.55	1.05	1.50	3.60	2.16	2.85	1.83	512	mlm_at
2	2.01	1.12	0.90	3.13	1.68	2.17	1.37	512	mlm_d_at
3	1.39	0.71	0.68	2.10	1.11	1.54	0.91	512	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.62	0.20	1.42	1.83	1.58	1.79	1.45	503	tef_at
1	9.09	1.75	7.34	10.85	9.42	10.24	8.49	503	mlm_at
2	5.79	1.28	4.50	7.07	5.94	6.81	4.99	503	mlm_d_at
3	2.92	0.53	2.39	3.45	2.82	3.24	2.57	503	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_s_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.27	0.37	0.90	1.65	1.22	1.40	1.05	500	tef_at
1	2.02	0.85	1.16	2.87	1.77	2.29	1.48	500	mlm_at
2	1.78	0.70	1.08	2.49	1.62	1.92	1.37	500	mlm_d_at
3	1.52	0.58	0.94	2.10	1.43	1.62	1.19	500	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	3.17	0.78	2.39	3.94	3.02	3.70	2.62	500	tef_at
1	9.41	3.68	5.74	13.09	8.91	12.26	6.52	500	mlm_at
2	6.64	2.79	3.86	9.43	6.03	8.50	4.60	500	mlm_d_at
3	4.92	1.86	3.06	6.77	4.70	5.95	3.49	500	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_s_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	0.82	0.11	0.71	0.93	0.81	0.89	0.73	505	tef_at
1	1.51	0.41	1.10	1.92	1.33	1.87	1.18	505	mlm_at
2	1.21	0.32	0.89	1.54	1.21	1.38	0.96	505	mlm_d_at
3	0.99	0.26	0.73	1.25	0.88	1.14	0.79	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_s_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.19	0.26	1.93	2.45	2.20	2.36	2.03	505	tef_at
1	6.42	0.99	5.43	7.42	6.59	7.06	5.70	505	mlm_at
2	4.60	0.96	3.64	5.56	4.62	5.51	4.03	505	mlm_d_at
3	3.08	0.58	2.50	3.65	3.03	3.41	2.66	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_s_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	1.28	0.27	1.02	1.55	1.21	1.38	1.12	505	tef_at
1	1.97	0.62	1.35	2.59	1.75	2.27	1.52	505	mlm_at
2	1.66	0.46	1.20	2.12	1.53	1.93	1.32	505	mlm_d_at
3	1.51	0.59	0.92	2.09	1.31	1.74	1.15	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/agnews_xlnet_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	2.59	0.39	2.20	2.98	2.56	2.82	2.32	505	tef_at
1	6.57	1.79	4.78	8.36	6.72	7.55	5.46	505	mlm_at
2	5.03	1.40	3.62	6.43	5.08	6.23	3.84	505	mlm_d_at
3	3.73	0.97	2.76	4.70	3.70	4.48	3.01	505	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_bert_a_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	82.26	35.77	46.48	118.03	94.09	100.43	66.82	28	tef_at
1	161.47	102.08	59.39	263.55	156.12	182.62	89.05	28	mlm_at
2	130.23	78.48	51.75	208.71	133.53	147.16	82.84	28	mlm_d_at
3	93.83	45.19	48.65	139.02	100.68	119.08	61.53	28	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_bert_a_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	73.43	30.75	42.68	104.18	80.49	90.91	66.72	31	tef_at
1	143.59	82.39	61.19	225.98	134.65	172.59	109.88	31	mlm_at
2	119.04	68.75	50.29	187.78	120.28	147.70	91.11	31	mlm_d_at
3	84.71	38.88	45.83	123.59	86.82	110.13	71.22	31	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_bert_a_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	51.80	20.92	30.88	72.73	50.00	60.31	35.56	38	tef_at
1	154.37	57.35	97.02	211.72	130.09	200.49	108.04	38	mlm_at
2	112.39	53.45	58.94	165.84	92.94	126.11	84.05	38	mlm_d_at
3	47.69	15.41	32.28	63.11	46.25	55.26	33.53	38	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_bert_a_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	62.51	30.06	32.45	92.57	67.10	72.69	43.71	32	tef_at
1	167.70	96.59	71.10	264.29	162.24	196.91	124.94	32	mlm_at
2	124.69	72.22	52.47	196.92	124.53	154.09	95.67	32	mlm_d_at
3	69.84	35.01	34.83	104.85	73.79	82.04	57.21	32	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_bert_a_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	65.00	27.94	37.06	92.93	72.35	77.64	51.39	35	tef_at
1	131.70	78.46	53.24	210.17	123.87	150.05	94.82	35	mlm_at
2	106.05	61.07	44.97	167.12	107.44	118.84	77.88	35	mlm_d_at
3	74.52	34.13	40.39	108.65	79.31	91.14	58.71	35	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_cnn_ig_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	78.67	10.53	68.15	89.20	68.68	89.38	68.68	29	tef_at
1	201.11	10.96	190.14	212.07	190.70	212.26	190.70	29	mlm_at
2	139.41	13.82	125.59	153.22	126.29	153.46	126.29	29	mlm_d_at
3	71.23	13.71	57.51	84.94	58.21	85.17	58.21	29	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_cnn_ig_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	89.70	13.06	76.64	102.77	97.38	100.74	72.91	22	tef_at
1	225.02	15.60	209.43	240.62	227.82	241.73	206.22	22	mlm_at
2	158.69	13.20	145.49	171.88	166.09	169.98	141.85	22	mlm_d_at
3	80.97	14.30	66.66	95.27	90.38	92.37	62.51	22	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_cnn_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	65.00	11.19	53.80	76.19	54.37	76.38	54.37	29	tef_at
1	163.18	9.94	153.24	173.12	153.74	173.29	153.74	29	mlm_at
2	116.33	6.41	109.93	122.74	110.25	122.85	110.25	29	mlm_d_at
3	48.12	7.24	40.88	55.37	41.25	55.49	41.25	29	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_cnn_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	59.43	0.00	59.43	59.43	59.43	59.43	59.43	29	tef_at
1	184.47	0.00	184.47	184.47	184.47	184.47	184.47	29	mlm_at
2	110.08	0.00	110.08	110.08	110.08	110.08	110.08	29	mlm_d_at
3	44.45	0.00	44.45	44.45	44.45	44.45	44.45	29	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_cnn_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	60.22	11.74	48.47	71.96	56.93	71.43	48.56	37	tef_at
1	149.20	14.31	134.89	163.50	149.35	162.33	134.30	37	mlm_at
2	103.51	12.15	91.37	115.66	102.08	116.05	91.14	37	mlm_d_at
3	47.08	11.49	35.59	58.57	45.77	60.35	34.45	37	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_cnn_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	72.74	13.35	59.39	86.08	68.98	89.82	55.35	29	tef_at
1	224.28	10.00	214.28	234.28	230.11	231.25	208.40	29	mlm_at
2	155.60	2.93	152.67	158.54	157.05	158.53	155.24	29	mlm_d_at
3	43.94	5.95	37.99	49.88	41.01	51.00	36.52	29	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_lstm_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	91.96	15.77	76.19	107.73	101.34	104.79	70.93	23	tef_at
1	212.87	23.37	189.50	236.25	218.01	237.73	183.52	23	mlm_at
2	152.27	16.24	136.03	168.51	161.46	165.84	130.66	23	mlm_d_at
3	70.98	13.62	57.36	84.60	78.84	82.24	52.84	23	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_lstmatt_a_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	70.72	10.26	60.46	80.97	70.72	80.81	60.62	32	tef_at
1	198.66	10.27	188.40	208.93	198.67	208.77	188.56	32	mlm_at
2	131.56	0.15	131.42	131.71	131.56	131.71	131.42	32	mlm_d_at
3	48.95	8.52	40.43	57.46	48.95	57.33	40.56	32	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_lstmatt_a_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	65.47	0.00	65.47	65.47	65.47	65.47	65.47	32	tef_at
1	180.68	0.00	180.68	180.68	180.68	180.68	180.68	32	mlm_at
2	135.10	0.00	135.10	135.10	135.10	135.10	135.10	32	mlm_d_at
3	49.34	0.00	49.34	49.34	49.34	49.34	49.34	32	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_lstmatt_a_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	98.89	20.33	78.56	119.22	102.27	110.20	87.16	20	tef_at
1	354.49	32.48	322.01	386.97	343.09	372.82	325.66	20	mlm_at
2	232.82	16.66	216.16	249.48	230.93	249.05	219.31	20	mlm_d_at
3	79.17	14.34	64.83	93.51	77.04	87.23	74.45	20	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_lstmatt_a_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	79.71	7.45	72.26	87.16	84.44	85.29	69.41	24	tef_at
1	198.83	3.42	195.41	202.24	199.46	202.57	194.45	24	mlm_at
2	142.37	3.66	138.71	146.03	143.68	145.95	137.47	24	mlm_d_at
3	59.11	10.79	48.32	69.91	64.81	68.23	44.30	24	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_roberta_a_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	61.52	23.78	37.75	85.30	70.33	78.13	53.07	41	tef_at
1	99.28	40.38	58.90	139.66	113.42	121.51	83.99	41	mlm_at
2	88.72	31.60	57.12	120.32	98.29	106.92	80.74	41	mlm_d_at
3	64.46	24.60	39.86	89.05	71.34	80.03	60.12	41	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_roberta_a_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	57.43	23.47	33.97	80.90	67.29	73.91	42.98	43	tef_at
1	91.58	38.86	52.72	130.43	107.78	117.53	69.23	43	mlm_at
2	82.23	31.17	51.06	113.40	93.92	98.78	72.44	43	mlm_d_at
3	59.94	23.83	36.11	83.77	68.25	76.09	54.60	43	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_roberta_a_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	115.90	51.33	64.57	167.23	133.81	151.75	98.27	20	tef_at
1	209.28	98.11	111.17	307.39	247.71	271.51	154.67	20	mlm_at
2	185.89	77.34	108.55	263.23	219.87	230.07	160.81	20	mlm_d_at
3	134.25	57.65	76.60	191.91	147.75	174.96	118.97	20	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_roberta_a_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	55.36	22.59	32.77	77.95	66.62	71.34	38.19	46	tef_at
1	89.42	38.52	50.90	127.95	103.16	114.38	64.47	46	mlm_at
2	79.59	30.74	48.85	110.33	90.91	97.59	69.83	46	mlm_d_at
3	57.89	22.86	35.03	80.75	66.45	71.98	51.96	46	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_roberta_a_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	96.15	47.39	48.75	143.54	111.71	128.62	59.81	24	tef_at
1	177.40	90.83	86.57	268.23	220.28	235.39	99.44	24	mlm_at
2	164.31	65.09	99.23	229.40	193.80	202.06	140.03	24	mlm_d_at
3	109.68	47.53	62.15	157.21	119.78	148.23	95.22	24	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_roberta_a_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	50.12	19.81	30.30	69.93	58.22	64.73	38.92	50	tef_at
1	80.88	33.78	47.10	114.66	92.90	102.53	57.65	50	mlm_at
2	72.10	26.96	45.14	99.06	81.31	88.87	60.46	50	mlm_d_at
3	52.09	20.20	31.89	72.30	59.18	64.24	45.35	50	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_roberta_a_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	101.87	48.05	53.83	149.92	118.96	135.61	72.59	22	tef_at
1	187.20	92.02	95.17	279.22	224.89	241.06	115.51	22	mlm_at
2	170.04	68.12	101.92	238.16	194.66	208.99	152.31	22	mlm_d_at
3	118.62	48.95	69.68	167.57	131.22	157.31	104.12	22	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_roberta_a_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	56.82	23.15	33.67	79.97	67.28	72.19	45.75	44	tef_at
1	91.65	38.57	53.09	130.22	105.16	117.63	72.29	44	mlm_at
2	81.66	30.84	50.83	112.50	92.11	99.97	70.93	44	mlm_d_at
3	58.86	23.15	35.71	82.01	66.75	74.44	53.40	44	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_roberta_a_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	108.88	51.90	56.98	160.78	122.16	144.50	80.21	22	tef_at
1	198.91	97.85	101.06	296.76	234.42	261.53	128.68	22	mlm_at
2	179.18	73.33	105.85	252.51	211.35	223.88	155.84	22	mlm_d_at
3	127.35	53.16	74.20	180.51	139.18	167.08	111.67	22	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_xlnet_a_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	67.89	23.10	44.78	90.99	74.94	83.72	62.55	38	tef_at
1	91.45	33.45	58.00	124.90	102.56	116.57	78.76	38	mlm_at
2	83.16	29.03	54.13	112.19	91.31	103.27	78.01	38	mlm_d_at
3	74.53	26.30	48.23	100.83	83.37	88.68	68.44	38	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_xlnet_a_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	74.58	27.79	46.79	102.37	83.50	91.89	67.38	34	tef_at
1	101.69	40.78	60.91	142.48	112.61	130.06	85.24	34	mlm_at
2	92.29	35.52	56.77	127.80	104.06	113.36	84.42	34	mlm_d_at
3	83.47	32.94	50.53	116.41	94.23	102.63	71.13	34	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_xlnet_a_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	83.03	34.63	48.40	117.66	86.66	112.83	61.41	32	tef_at
1	113.79	49.61	64.18	163.40	123.75	151.20	81.87	32	mlm_at
2	101.73	42.53	59.19	144.26	115.86	133.83	75.91	32	mlm_d_at
3	92.92	38.90	54.02	131.82	108.44	121.04	66.55	32	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_xlnet_a_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	72.92	26.65	46.27	99.57	79.24	91.42	66.56	34	tef_at
1	99.08	39.68	59.40	138.76	109.23	127.82	84.34	34	mlm_at
2	90.11	34.36	55.75	124.46	98.27	113.12	81.71	34	mlm_d_at
3	81.60	31.46	50.14	113.06	92.44	99.40	69.43	34	mlm_d_fast_at


==> data/mlm_plots/timing_data/fakenews_xlnet_a_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	77.52	30.37	47.15	107.88	81.74	98.48	67.45	33	tef_at
1	106.95	44.16	62.79	151.11	115.21	139.79	83.90	33	mlm_at
2	96.84	38.76	58.08	135.60	107.30	119.30	83.64	33	mlm_d_at
3	87.20	35.31	51.89	122.50	96.49	108.23	71.05	33	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_a_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	16.79	4.80	11.99	21.59	16.30	20.05	12.72	147	tef_at
1	35.70	17.08	18.62	52.78	31.07	38.50	26.79	147	mlm_at
2	24.77	8.44	16.33	33.22	22.85	27.73	20.09	147	mlm_d_at
3	15.26	4.15	11.12	19.41	14.76	17.91	12.76	147	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_a_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	24.15	1.99	22.17	26.14	24.91	26.21	21.59	23	tef_at
1	166.25	2.98	163.27	169.23	167.62	168.97	162.33	23	mlm_at
2	112.40	5.68	106.73	118.08	113.09	119.35	105.63	23	mlm_d_at
3	30.79	3.10	27.69	33.89	31.91	34.05	26.81	23	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_a_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	17.73	4.90	12.83	22.64	16.89	21.90	13.40	136	tef_at
1	38.65	19.08	19.58	57.73	33.38	41.89	27.94	136	mlm_at
2	26.26	8.45	17.81	34.72	25.08	30.80	21.38	136	mlm_d_at
3	16.09	4.17	11.92	20.26	15.89	18.40	13.89	136	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_a_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	31.57	5.42	26.15	36.99	32.18	35.30	29.64	50	tef_at
1	115.25	35.67	79.58	150.93	119.39	140.68	81.19	50	mlm_at
2	88.84	23.77	65.07	112.61	93.81	100.55	71.23	50	mlm_d_at
3	47.49	12.59	34.90	60.08	44.59	59.53	39.14	50	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_a_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	15.19	4.46	10.73	19.64	14.27	17.35	12.07	139	tef_at
1	51.80	28.60	23.20	80.40	45.35	60.61	33.12	139	mlm_at
2	28.87	9.59	19.28	38.46	25.92	32.47	23.46	139	mlm_d_at
3	12.74	3.77	8.97	16.51	13.00	14.27	10.12	139	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_a_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	25.36	3.84	21.51	29.20	27.19	27.75	22.81	48	tef_at
1	169.51	47.11	122.40	216.61	189.74	207.54	131.53	48	mlm_at
2	118.89	30.70	88.19	149.59	126.53	143.94	101.66	48	mlm_d_at
3	40.83	9.90	30.93	50.73	38.94	50.36	32.38	48	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_a_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	14.05	3.98	10.06	18.03	13.57	15.85	10.81	126	tef_at
1	61.21	33.74	27.46	94.95	57.63	68.51	38.50	126	mlm_at
2	32.91	10.54	22.36	43.45	31.89	37.37	26.89	126	mlm_d_at
3	13.97	4.05	9.92	18.02	14.13	15.53	11.14	126	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_a_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	24.41	3.55	20.86	27.96	22.67	26.06	21.53	50	tef_at
1	158.56	21.70	136.86	180.26	166.01	172.78	155.06	50	mlm_at
2	106.91	22.10	84.80	129.01	106.76	123.12	103.13	50	mlm_d_at
3	30.35	6.53	23.82	36.88	32.38	33.61	23.52	50	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_a_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	19.69	9.03	10.66	28.72	17.79	23.86	13.99	131	tef_at
1	34.59	17.96	16.63	52.54	31.03	41.09	24.16	131	mlm_at
2	26.55	11.82	14.73	38.37	24.66	31.92	19.48	131	mlm_d_at
3	19.24	7.99	11.25	27.23	18.31	22.80	14.21	131	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_a_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	24.41	2.55	21.86	26.97	23.39	26.75	21.73	50	tef_at
1	161.04	20.05	140.99	181.10	168.73	178.22	159.25	50	mlm_at
2	108.41	21.25	87.16	129.65	108.78	128.00	105.82	50	mlm_d_at
3	31.29	5.50	25.79	36.79	34.30	35.43	24.80	50	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_ig_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	20.59	4.78	15.80	25.37	20.53	21.87	17.33	94	tef_at
1	65.59	35.87	29.72	101.45	55.71	68.67	50.87	94	mlm_at
2	44.93	15.16	29.78	60.09	42.41	47.47	35.10	94	mlm_d_at
3	23.76	4.94	18.82	28.70	24.06	26.19	20.77	94	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_ig_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	82.13	11.88	70.25	94.01	87.67	88.52	72.31	23	tef_at
1	184.86	53.86	131.00	238.73	221.03	229.79	126.33	23	mlm_at
2	149.10	26.66	122.44	175.75	160.23	175.03	125.63	23	mlm_d_at
3	127.40	31.30	96.11	158.70	142.67	154.74	97.29	23	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_ig_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	17.09	2.79	14.30	19.88	16.69	19.66	15.25	115	tef_at
1	51.74	12.19	39.54	63.93	47.92	53.94	46.53	115	mlm_at
2	41.87	21.84	20.03	63.71	35.10	36.84	31.49	115	mlm_d_at
3	17.50	2.50	15.00	19.99	17.81	18.71	15.81	115	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_ig_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	35.08	2.78	32.31	37.86	35.24	36.37	33.09	44	tef_at
1	147.12	32.42	114.71	179.54	170.22	178.78	113.93	44	mlm_at
2	104.52	21.08	83.44	125.60	105.11	112.54	86.51	44	mlm_d_at
3	43.12	4.95	38.17	48.07	40.08	48.96	38.37	44	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_ig_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	19.70	4.42	15.28	24.13	19.31	21.24	16.76	97	tef_at
1	63.74	34.73	29.02	98.47	54.95	67.77	50.00	97	mlm_at
2	44.13	15.57	28.57	59.70	40.95	47.51	34.27	97	mlm_d_at
3	22.94	4.99	17.95	27.93	24.21	25.44	19.67	97	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_ig_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	82.83	11.98	70.85	94.81	89.17	89.57	72.35	23	tef_at
1	190.76	56.65	134.12	247.41	230.64	231.21	127.11	23	mlm_at
2	152.35	26.99	125.36	179.35	166.48	176.05	128.84	23	mlm_d_at
3	127.56	31.45	96.11	159.01	143.03	156.34	97.05	23	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_ig_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	47.06	7.82	39.24	54.88	47.42	52.78	41.96	50	tef_at
1	76.24	17.94	58.31	94.18	77.05	83.86	67.67	50	mlm_at
2	68.60	18.38	50.22	86.98	66.73	67.98	60.48	50	mlm_d_at
3	58.29	10.37	47.92	68.67	58.77	67.40	55.08	50	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_ig_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	36.93	2.15	34.77	39.08	36.43	38.07	36.31	44	tef_at
1	156.30	31.05	125.24	187.35	181.38	185.18	129.78	44	mlm_at
2	109.99	21.32	88.67	131.31	113.42	123.08	89.19	44	mlm_d_at
3	44.56	5.72	38.84	50.27	40.21	50.11	39.07	44	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_ig_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	18.09	3.10	14.99	21.19	18.32	19.86	15.49	107	tef_at
1	55.18	13.94	41.24	69.12	51.07	60.79	46.59	107	mlm_at
2	44.12	22.77	21.35	66.89	37.05	43.11	29.32	107	mlm_d_at
3	18.19	2.77	15.43	20.96	18.40	19.55	16.11	107	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_ig_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	82.36	12.12	70.24	94.48	88.49	89.32	71.76	23	tef_at
1	186.06	55.05	131.01	241.11	224.03	225.00	124.36	23	mlm_at
2	150.60	26.64	123.97	177.24	164.02	175.20	125.75	23	mlm_d_at
3	127.23	31.37	95.86	158.60	142.37	155.47	96.36	23	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_s_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	33.17	9.18	24.00	42.35	31.61	40.92	26.34	56	tef_at
1	79.21	40.29	38.92	119.50	66.08	106.62	44.23	56	mlm_at
2	77.31	40.54	36.77	117.85	63.63	105.30	40.68	56	mlm_d_at
3	46.05	22.52	23.53	68.57	42.98	54.08	28.27	56	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	29.52	1.72	27.81	31.24	28.46	29.80	28.29	37	tef_at
1	179.10	9.24	169.86	188.34	177.11	189.37	171.79	37	mlm_at
2	126.90	11.19	115.71	138.09	126.73	132.43	122.89	37	mlm_d_at
3	42.33	5.35	36.98	47.67	45.09	45.87	42.21	37	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_s_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	17.22	2.36	14.86	19.58	18.34	18.97	15.01	65	tef_at
1	119.52	28.69	90.83	148.22	114.82	145.36	95.50	65	mlm_at
2	91.99	12.42	79.57	104.41	95.08	101.05	86.79	65	mlm_d_at
3	21.54	5.60	15.94	27.13	22.24	24.62	18.41	65	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	40.31	5.75	34.56	46.05	41.42	44.13	36.33	35	tef_at
1	155.88	15.80	140.09	171.68	150.93	169.14	149.07	35	mlm_at
2	122.87	14.69	108.18	137.57	128.03	129.66	112.06	35	mlm_d_at
3	83.86	16.12	67.74	99.98	93.02	94.08	73.91	35	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_s_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	20.48	5.02	15.46	25.50	19.48	23.91	17.24	58	tef_at
1	116.10	58.07	58.03	174.16	102.06	180.71	72.04	58	mlm_at
2	108.32	37.94	70.38	146.26	112.37	140.99	92.34	58	mlm_d_at
3	31.50	13.50	17.99	45.00	27.61	46.02	19.12	58	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	30.61	4.65	25.96	35.26	31.56	33.18	28.73	35	tef_at
1	224.49	17.24	207.25	241.73	230.78	234.46	208.20	35	mlm_at
2	164.13	12.71	151.42	176.84	170.90	171.69	153.35	35	mlm_d_at
3	62.05	10.83	51.22	72.89	64.90	71.10	57.25	35	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_s_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	29.01	7.54	21.47	36.55	29.18	34.26	23.43	65	tef_at
1	82.89	33.14	49.75	116.03	81.21	111.92	52.82	65	mlm_at
2	64.58	32.36	32.22	96.95	54.28	86.23	37.24	65	mlm_d_at
3	42.04	19.56	22.48	61.60	37.91	51.00	24.19	65	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_s_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	38.03	5.45	32.58	43.49	39.53	42.07	31.72	37	tef_at
1	147.95	14.17	133.78	162.12	144.46	161.79	142.62	37	mlm_at
2	116.00	20.45	95.56	136.45	121.30	126.67	112.40	37	mlm_d_at
3	80.27	14.78	65.50	95.05	89.34	89.94	69.20	37	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_s_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	35.82	9.03	26.79	44.85	37.24	42.07	28.72	23	tef_at
1	77.89	40.70	37.19	118.59	61.18	105.08	48.61	23	mlm_at
2	89.17	56.02	33.14	145.19	67.89	142.63	43.55	23	mlm_d_at
3	52.47	24.62	27.84	77.09	48.86	55.43	36.09	23	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_bert_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	47.60	10.73	36.87	58.33	49.70	52.47	39.59	29	tef_at
1	177.10	37.89	139.20	214.99	183.47	202.95	173.81	29	mlm_at
2	142.23	30.67	111.57	172.90	150.24	165.46	116.41	29	mlm_d_at
3	99.07	22.00	77.07	121.07	107.69	116.08	77.53	29	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_ig_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	11.63	1.43	10.20	13.06	11.33	13.32	10.52	212	tef_at
1	22.63	2.46	20.17	25.09	22.71	24.22	20.89	212	mlm_at
2	17.33	1.78	15.55	19.12	16.92	18.80	16.13	212	mlm_d_at
3	11.08	1.29	9.80	12.37	10.77	12.27	10.43	212	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_ig_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	23.87	3.52	20.35	27.39	25.17	27.05	21.41	90	tef_at
1	51.28	6.30	44.99	57.58	54.03	55.77	46.73	90	mlm_at
2	39.22	3.92	35.31	43.14	40.71	42.22	34.95	90	mlm_d_at
3	23.01	3.15	19.85	26.16	22.39	25.58	21.45	90	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_ig_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	12.19	1.14	11.05	13.33	12.72	12.84	10.80	184	tef_at
1	24.55	2.61	21.94	27.16	25.15	27.03	21.92	184	mlm_at
2	18.33	1.50	16.83	19.84	18.25	19.78	17.49	184	mlm_d_at
3	11.33	1.02	10.31	12.35	11.63	11.90	10.18	184	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_ig_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	24.35	2.92	21.43	27.27	25.26	27.29	20.34	77	tef_at
1	53.49	3.39	50.10	56.88	55.30	56.32	48.67	77	mlm_at
2	41.42	4.74	36.67	46.16	43.72	45.57	34.71	77	mlm_d_at
3	22.59	2.76	19.82	25.35	23.56	25.29	18.76	77	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_ig_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	12.05	2.67	9.38	14.72	12.16	13.85	10.23	216	tef_at
1	21.28	4.32	16.96	25.60	21.52	24.03	19.49	216	mlm_at
2	16.87	3.38	13.49	20.24	17.37	19.40	14.91	216	mlm_d_at
3	11.70	2.56	9.14	14.26	11.72	13.39	10.05	216	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_ig_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	25.76	6.53	19.23	32.28	26.15	29.90	20.20	97	tef_at
1	51.58	12.94	38.64	64.53	51.81	61.25	45.13	97	mlm_at
2	40.09	9.17	30.92	49.26	41.61	45.64	35.06	97	mlm_d_at
3	24.92	6.79	18.12	31.71	26.26	28.75	19.73	97	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_ig_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	12.23	0.80	11.43	13.03	12.65	12.93	11.11	159	tef_at
1	26.56	2.27	24.29	28.82	27.73	28.56	23.40	159	mlm_at
2	19.30	1.57	17.73	20.87	19.96	20.79	17.14	159	mlm_d_at
3	11.37	0.73	10.64	12.10	11.69	12.07	10.36	159	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_ig_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	26.10	0.00	26.10	26.10	26.10	26.10	26.10	52	tef_at
1	61.66	0.00	61.66	61.66	61.66	61.66	61.66	52	mlm_at
2	48.55	0.00	48.55	48.55	48.55	48.55	48.55	52	mlm_d_at
3	24.66	0.00	24.66	24.66	24.66	24.66	24.66	52	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_ig_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	11.69	1.84	9.85	13.54	11.46	13.27	10.47	220	tef_at
1	21.91	2.87	19.04	24.77	21.31	24.79	19.69	220	mlm_at
2	16.97	2.27	14.70	19.25	16.74	18.40	15.82	220	mlm_d_at
3	11.32	1.72	9.59	13.04	11.23	12.70	10.11	220	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_ig_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	24.44	4.46	19.97	28.90	24.07	29.80	20.89	97	tef_at
1	50.83	6.84	43.99	57.67	50.46	54.99	45.31	97	mlm_at
2	39.26	5.27	34.00	44.53	38.04	43.30	35.82	97	mlm_d_at
3	23.64	4.67	18.97	28.30	23.18	27.30	20.26	97	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_s_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	7.67	0.97	6.71	8.64	7.50	8.57	7.12	321	tef_at
1	16.21	1.37	14.84	17.58	16.06	17.18	15.47	321	mlm_at
2	12.06	0.96	11.10	13.02	12.06	12.82	11.53	321	mlm_d_at
3	6.35	0.81	5.54	7.15	6.25	6.88	5.84	321	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	17.06	2.83	14.23	19.88	17.09	19.41	14.72	146	tef_at
1	37.78	4.76	33.02	42.54	37.77	42.64	33.36	146	mlm_at
2	26.87	3.03	23.83	29.90	27.60	29.67	23.96	146	mlm_d_at
3	12.65	2.31	10.34	14.96	12.99	14.59	10.40	146	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_s_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	7.50	0.63	6.88	8.13	7.77	7.86	7.15	321	tef_at
1	15.95	1.24	14.71	17.19	16.05	17.20	14.80	321	mlm_at
2	11.79	0.75	11.04	12.53	11.55	12.63	11.11	321	mlm_d_at
3	6.23	0.46	5.77	6.70	6.12	6.57	6.05	321	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	16.71	1.56	15.15	18.27	17.05	17.13	16.48	134	tef_at
1	39.88	2.51	37.36	42.39	39.02	41.78	38.38	134	mlm_at
2	28.44	1.72	26.72	30.16	28.86	30.09	27.52	134	mlm_d_at
3	12.43	1.28	11.15	13.71	12.45	13.42	12.24	134	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_s_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	7.03	1.53	5.50	8.56	7.01	8.29	5.90	363	tef_at
1	14.16	2.49	11.68	16.65	14.44	15.66	13.08	363	mlm_at
2	10.72	1.86	8.85	12.58	10.79	12.09	9.75	363	mlm_d_at
3	6.01	1.36	4.65	7.37	5.84	7.14	5.04	363	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	16.35	3.78	12.58	20.13	16.41	19.12	13.72	155	tef_at
1	36.73	7.18	29.55	43.91	38.98	40.85	34.62	155	mlm_at
2	26.19	5.44	20.76	31.63	27.08	29.96	23.62	155	mlm_d_at
3	12.29	3.12	9.16	15.41	12.13	14.39	10.05	155	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_s_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	7.73	0.56	7.17	8.29	7.86	8.11	7.31	265	tef_at
1	17.55	1.12	16.44	18.67	17.80	18.15	16.85	265	mlm_at
2	12.88	0.81	12.07	13.69	13.45	13.50	12.17	265	mlm_d_at
3	6.40	0.41	5.99	6.81	6.38	6.84	6.09	265	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_s_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	15.66	1.29	14.37	16.94	14.39	16.95	14.39	105	tef_at
1	38.08	3.04	35.04	41.12	35.08	41.13	35.08	105	mlm_at
2	27.04	1.85	25.19	28.89	25.22	28.90	25.22	105	mlm_d_at
3	11.95	1.03	10.92	12.99	10.93	12.99	10.93	105	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_s_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	7.38	1.15	6.23	8.53	7.24	8.21	6.63	348	tef_at
1	15.32	1.60	13.72	16.93	15.01	16.24	14.00	348	mlm_at
2	11.44	1.15	10.29	12.59	11.28	12.19	10.64	348	mlm_d_at
3	6.11	0.93	5.18	7.04	5.98	6.70	5.42	348	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_cnn_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	16.35	3.20	13.15	19.56	15.92	18.78	14.57	152	tef_at
1	38.17	5.49	32.68	43.66	37.04	42.10	34.26	152	mlm_at
2	27.03	4.19	22.83	31.22	26.34	29.74	23.73	152	mlm_d_at
3	12.11	2.45	9.66	14.55	12.02	13.85	10.02	152	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_ig_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	9.71	1.30	8.41	11.01	9.34	10.50	8.90	254	tef_at
1	20.97	2.44	18.53	23.41	20.80	23.12	19.08	254	mlm_at
2	15.36	1.47	13.89	16.83	15.68	16.74	13.97	254	mlm_d_at
3	8.82	0.99	7.82	9.81	8.98	9.81	8.08	254	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_ig_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	20.76	2.68	18.08	23.44	20.68	22.93	19.84	113	tef_at
1	47.55	4.43	43.12	51.98	47.14	52.07	42.26	113	mlm_at
2	34.72	2.75	31.97	37.47	34.43	37.12	33.91	113	mlm_d_at
3	17.97	1.94	16.04	19.91	17.61	19.10	16.96	113	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_ig_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	8.77	0.96	7.81	9.73	8.51	9.56	8.09	254	tef_at
1	20.04	1.66	18.38	21.71	19.95	20.63	18.68	254	mlm_at
2	14.79	1.15	13.64	15.95	14.77	15.63	14.46	254	mlm_d_at
3	8.01	0.83	7.19	8.84	7.92	8.59	7.35	254	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_ig_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	18.38	2.09	16.29	20.48	17.67	20.68	17.67	113	tef_at
1	45.65	4.07	41.57	49.72	45.93	49.36	45.93	113	mlm_at
2	33.06	2.53	30.53	35.59	33.09	34.77	33.09	113	mlm_d_at
3	15.02	1.04	13.98	16.06	14.70	15.92	14.70	113	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_ig_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	16.32	3.85	12.47	20.17	15.89	18.39	14.24	162	tef_at
1	26.16	5.26	20.89	31.42	25.63	28.65	22.11	162	mlm_at
2	22.02	4.80	17.22	26.83	21.74	25.39	17.91	162	mlm_d_at
3	16.67	4.25	12.42	20.92	16.32	18.86	13.45	162	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_ig_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	33.71	7.23	26.48	40.93	35.11	37.77	27.31	76	tef_at
1	60.48	11.31	49.17	71.79	63.34	66.69	53.84	76	mlm_at
2	49.19	9.40	39.79	58.59	51.78	55.51	43.88	76	mlm_d_at
3	34.34	7.84	26.50	42.18	35.03	37.04	26.75	76	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_ig_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	7.67	0.41	7.26	8.08	7.42	7.58	7.33	224	tef_at
1	19.87	0.15	19.72	20.02	19.81	19.97	19.67	224	mlm_at
2	15.14	1.13	14.00	16.27	15.48	16.78	13.89	224	mlm_d_at
3	7.00	0.40	6.60	7.41	7.36	7.43	6.51	224	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_ig_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	16.82	0.81	16.02	17.63	16.04	17.65	16.04	113	tef_at
1	47.43	0.63	46.80	48.06	46.82	48.07	46.82	113	mlm_at
2	33.46	0.52	32.93	33.98	32.95	33.99	32.95	113	mlm_d_at
3	13.90	0.64	13.26	14.54	13.28	14.55	13.28	113	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_ig_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	11.31	1.62	9.68	12.93	11.24	12.56	10.44	224	tef_at
1	20.81	2.27	18.55	23.08	20.61	22.00	19.42	224	mlm_at
2	16.55	2.15	14.41	18.70	16.33	17.58	15.27	224	mlm_d_at
3	10.94	1.65	9.29	12.60	10.59	11.82	10.13	224	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_ig_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	24.59	3.96	20.63	28.55	23.43	28.35	22.40	97	tef_at
1	48.33	4.86	43.47	53.18	48.13	51.53	45.59	97	mlm_at
2	37.67	4.52	33.15	42.18	37.68	42.03	35.78	97	mlm_d_at
3	23.12	3.70	19.43	26.82	21.59	26.94	20.93	97	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_s_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	9.12	1.45	7.68	10.57	9.12	10.01	8.40	181	tef_at
1	43.43	39.39	4.03	82.82	19.31	99.56	16.84	181	mlm_at
2	24.83	21.75	3.08	46.59	14.15	15.95	12.47	181	mlm_d_at
3	9.50	3.71	5.79	13.22	8.17	9.36	7.43	181	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	18.80	2.33	16.47	21.14	18.66	19.36	17.75	113	tef_at
1	56.75	29.51	27.24	86.26	41.29	42.61	40.72	113	mlm_at
2	39.80	18.84	20.96	58.63	30.59	69.93	27.61	113	mlm_d_at
3	16.16	3.63	12.54	19.79	15.04	17.78	13.36	113	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_s_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	8.02	0.79	7.23	8.82	7.89	8.75	7.32	166	tef_at
1	57.28	40.60	16.68	97.88	18.89	98.32	16.77	166	mlm_at
2	29.26	23.48	5.78	52.74	13.71	62.13	12.26	166	mlm_d_at
3	8.10	2.41	5.69	10.50	6.67	10.74	6.35	166	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	18.47	1.65	16.82	20.11	19.55	19.73	16.18	83	tef_at
1	88.40	34.93	53.47	123.32	111.58	114.56	39.77	83	mlm_at
2	45.01	20.52	24.49	65.53	32.54	72.72	27.88	83	mlm_d_at
3	14.82	2.34	12.48	17.17	15.19	17.40	11.81	83	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_s_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	16.43	4.18	12.25	20.60	16.05	18.45	12.92	149	tef_at
1	32.92	27.87	5.05	60.79	25.21	28.52	23.13	149	mlm_at
2	24.72	15.58	9.14	40.30	21.22	23.85	18.98	149	mlm_d_at
3	17.00	6.75	10.25	23.74	15.61	17.64	13.25	149	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	30.71	6.56	24.15	37.26	32.04	33.95	24.55	79	tef_at
1	61.22	30.10	31.12	91.31	54.11	57.72	46.81	79	mlm_at
2	48.49	17.92	30.57	66.41	45.39	48.16	39.59	79	mlm_d_at
3	30.80	8.68	22.12	39.48	30.22	31.84	24.68	79	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_s_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	7.72	0.78	6.95	8.50	6.97	8.52	6.97	113	tef_at
1	62.01	45.69	16.32	107.70	17.71	108.72	17.71	113	mlm_at
2	38.96	27.40	11.55	66.36	12.39	66.97	12.39	113	mlm_d_at
3	7.72	1.84	5.87	9.56	5.93	9.60	5.93	113	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_s_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	16.35	0.00	16.35	16.35	16.35	16.35	16.35	55	tef_at
1	109.28	0.00	109.28	109.28	109.28	109.28	109.28	55	mlm_at
2	66.17	0.00	66.17	66.17	66.17	66.17	66.17	55	mlm_d_at
3	14.40	0.00	14.40	14.40	14.40	14.40	14.40	55	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_s_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	11.25	1.92	9.32	13.17	10.90	12.48	10.09	181	tef_at
1	35.67	33.42	2.25	69.09	19.66	23.28	18.67	181	mlm_at
2	24.12	20.19	3.93	44.31	16.42	18.06	14.33	181	mlm_d_at
3	12.14	4.94	7.20	17.07	10.47	12.56	9.28	181	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstm_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	23.58	4.73	18.85	28.32	22.58	26.75	20.59	97	tef_at
1	59.11	32.98	26.13	92.09	44.95	53.33	41.46	97	mlm_at
2	43.20	17.21	26.00	60.41	36.27	46.36	32.39	97	mlm_d_at
3	22.18	5.55	16.63	27.73	21.69	25.38	18.54	97	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_a_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	8.81	0.97	7.84	9.77	8.73	9.30	8.25	286	tef_at
1	18.16	1.55	16.61	19.71	18.09	19.75	17.15	286	mlm_at
2	13.18	1.01	12.17	14.19	13.33	13.90	12.34	286	mlm_d_at
3	7.61	0.85	6.76	8.46	7.64	8.30	6.96	286	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_a_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	18.14	2.34	15.80	20.47	18.28	19.57	17.23	134	tef_at
1	42.14	4.20	37.94	46.34	41.63	46.07	39.17	134	mlm_at
2	29.61	3.04	26.57	32.66	29.98	31.59	27.35	134	mlm_d_at
3	14.51	1.98	12.53	16.49	14.91	16.30	13.33	134	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_a_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	7.94	0.72	7.22	8.66	7.90	8.55	7.39	299	tef_at
1	17.44	1.10	16.34	18.54	17.76	18.49	16.30	299	mlm_at
2	12.55	0.62	11.93	13.17	12.35	12.84	11.90	299	mlm_d_at
3	6.64	0.42	6.22	7.06	6.53	6.78	6.41	299	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_a_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	17.00	1.37	15.62	18.37	17.26	18.19	16.29	134	tef_at
1	42.23	2.26	39.97	44.49	41.22	41.89	40.85	134	mlm_at
2	28.64	1.50	27.14	30.15	28.57	28.69	28.14	134	mlm_d_at
3	12.68	1.11	11.58	13.79	13.15	13.58	11.92	134	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_a_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	14.52	3.66	10.86	18.18	14.55	15.94	12.14	184	tef_at
1	23.13	4.36	18.77	27.48	23.01	25.39	20.59	184	mlm_at
2	19.27	3.99	15.28	23.26	18.98	21.27	16.79	184	mlm_d_at
3	14.44	3.90	10.54	18.34	14.04	16.21	12.03	184	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_a_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	28.37	6.13	22.24	34.50	29.58	31.51	24.30	91	tef_at
1	50.19	8.85	41.34	59.04	50.99	53.50	47.04	91	mlm_at
2	40.29	7.62	32.67	47.91	40.32	44.35	35.34	91	mlm_d_at
3	26.76	6.21	20.56	32.97	26.70	29.40	23.39	91	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_a_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	7.56	0.56	7.00	8.11	7.25	8.16	7.12	272	tef_at
1	18.72	1.32	17.40	20.04	18.80	19.64	17.49	272	mlm_at
2	12.97	0.43	12.55	13.40	13.23	13.27	12.69	272	mlm_d_at
3	6.17	0.38	5.78	6.55	5.92	6.55	5.91	272	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_a_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	14.96	0.80	14.16	15.76	14.91	15.94	14.03	158	tef_at
1	39.66	2.38	37.29	42.04	38.06	42.90	37.79	158	mlm_at
2	27.03	1.04	25.99	28.07	26.71	28.39	25.96	158	mlm_d_at
3	11.46	0.50	10.96	11.95	11.38	12.08	10.90	158	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_a_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	10.49	1.45	9.04	11.95	10.26	11.53	9.65	249	tef_at
1	19.49	2.10	17.39	21.59	19.26	20.82	18.55	249	mlm_at
2	14.91	1.65	13.26	16.56	14.93	16.05	14.12	249	mlm_d_at
3	9.63	1.37	8.26	11.00	9.46	10.89	8.64	249	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_a_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	22.03	3.23	18.81	25.26	22.00	24.80	19.55	118	tef_at
1	44.60	4.16	40.44	48.76	44.61	48.18	41.65	118	mlm_at
2	32.72	3.11	29.61	35.83	32.77	35.36	31.08	118	mlm_d_at
3	18.25	2.89	15.36	21.15	17.09	20.76	16.76	118	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_ig_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	14.09	2.22	11.87	16.31	13.81	15.43	12.91	158	tef_at
1	34.36	11.42	22.94	45.77	31.70	37.42	25.77	158	mlm_at
2	25.40	7.81	17.59	33.21	23.51	27.99	18.82	158	mlm_d_at
3	14.21	3.66	10.55	17.86	13.22	15.24	12.17	158	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_ig_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	27.68	3.77	23.91	31.45	28.57	31.34	26.39	69	tef_at
1	76.66	22.23	54.43	98.90	73.95	83.00	57.75	69	mlm_at
2	56.97	15.11	41.87	72.08	58.77	62.37	42.69	69	mlm_d_at
3	28.14	5.72	22.42	33.86	27.29	31.11	26.22	69	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_ig_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	11.50	1.41	10.09	12.91	11.47	12.15	10.90	158	tef_at
1	37.00	13.04	23.96	50.04	31.01	51.86	27.33	158	mlm_at
2	25.75	7.23	18.52	32.98	23.25	33.64	20.80	158	mlm_d_at
3	11.36	1.95	9.41	13.31	11.20	12.88	9.98	158	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_ig_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	22.43	1.21	21.23	23.64	22.47	23.75	20.89	82	tef_at
1	84.08	12.01	72.08	96.09	82.14	101.49	72.30	82	mlm_at
2	59.15	9.61	49.55	68.76	54.16	73.93	52.06	82	mlm_d_at
3	22.43	2.88	19.55	25.31	23.98	24.98	18.38	82	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_ig_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	29.04	7.22	21.82	36.26	29.38	32.64	24.19	88	tef_at
1	45.78	14.45	31.33	60.23	42.48	52.93	38.15	88	mlm_at
2	41.16	13.90	27.26	55.05	38.28	47.52	33.18	88	mlm_d_at
3	32.47	9.06	23.41	41.53	31.45	34.82	26.68	88	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_ig_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	56.72	7.51	49.21	64.24	59.08	62.08	54.30	39	tef_at
1	105.35	28.11	77.23	133.46	99.56	112.25	86.63	39	mlm_at
2	90.50	24.86	65.63	115.36	82.17	107.92	79.67	39	mlm_d_at
3	69.34	15.71	53.64	85.05	65.29	77.93	62.98	39	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_ig_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	9.62	0.71	8.91	10.32	10.01	10.26	8.66	158	tef_at
1	42.63	11.80	30.83	54.43	44.97	56.81	27.92	158	mlm_at
2	28.70	6.08	22.62	34.78	31.43	34.44	20.58	158	mlm_d_at
3	9.74	1.47	8.27	11.20	10.14	11.42	7.86	158	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_ig_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	21.42	0.00	21.42	21.42	21.42	21.42	21.42	55	tef_at
1	107.88	0.00	107.88	107.88	107.88	107.88	107.88	55	mlm_at
2	69.02	0.00	69.02	69.02	69.02	69.02	69.02	55	mlm_d_at
3	20.41	0.00	20.41	20.41	20.41	20.41	20.41	55	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_ig_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	19.38	3.76	15.62	23.14	18.49	21.53	17.18	129	tef_at
1	34.97	9.33	25.63	44.30	34.80	37.32	27.83	129	mlm_at
2	29.11	8.51	20.60	37.62	28.07	32.77	23.32	129	mlm_d_at
3	20.14	4.52	15.62	24.66	19.16	21.40	17.83	129	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_ig_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	41.72	5.78	35.94	47.49	39.50	46.37	37.07	55	tef_at
1	89.16	23.99	65.18	113.15	88.34	93.00	78.03	55	mlm_at
2	70.93	19.49	51.44	90.43	64.80	78.75	62.04	55	mlm_d_at
3	45.69	9.36	36.33	55.04	43.61	49.70	41.31	55	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_s_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	11.58	1.18	10.40	12.76	11.95	12.45	10.62	217	tef_at
1	20.56	1.69	18.86	22.25	20.10	22.32	19.21	217	mlm_at
2	16.24	1.32	14.92	17.56	16.27	17.45	15.00	217	mlm_d_at
3	10.27	1.12	9.14	11.39	10.39	11.15	9.32	217	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	23.87	3.37	20.50	27.24	23.74	26.09	21.88	110	tef_at
1	45.94	4.09	41.85	50.03	46.07	48.43	42.43	110	mlm_at
2	35.56	2.54	33.02	38.09	35.48	37.90	32.91	110	mlm_d_at
3	20.13	2.41	17.72	22.54	19.76	22.48	18.57	110	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_s_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	9.48	0.61	8.87	10.08	9.59	9.89	9.04	272	tef_at
1	18.51	0.91	17.60	19.43	18.35	19.42	17.95	272	mlm_at
2	14.00	0.65	13.35	14.65	14.00	14.25	13.49	272	mlm_d_at
3	7.93	0.52	7.41	8.44	7.89	8.45	7.58	272	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	19.75	1.96	17.79	21.71	20.42	20.93	20.42	110	tef_at
1	42.68	2.14	40.54	44.81	42.77	45.33	42.33	110	mlm_at
2	31.18	1.60	29.58	32.78	31.97	32.74	31.19	110	mlm_d_at
3	15.67	1.25	14.42	16.92	15.96	16.36	15.96	110	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_s_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	24.03	5.97	18.05	30.00	23.64	26.03	20.37	114	tef_at
1	33.19	7.13	26.07	40.32	33.07	35.73	29.63	114	mlm_at
2	29.27	6.06	23.21	35.32	29.36	31.16	25.95	114	mlm_d_at
3	24.13	6.09	18.04	30.22	23.47	26.18	20.91	114	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	53.09	9.45	43.64	62.55	56.06	59.53	45.43	51	tef_at
1	79.70	10.54	69.16	90.24	83.32	85.50	74.12	51	mlm_at
2	67.59	8.96	58.63	76.54	71.04	71.93	67.35	51	mlm_d_at
3	52.62	9.49	43.13	62.12	53.45	57.48	52.72	51	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_s_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	8.20	0.52	7.68	8.73	8.42	8.59	7.63	272	tef_at
1	18.43	0.88	17.55	19.32	18.64	18.85	18.15	272	mlm_at
2	13.42	0.46	12.95	13.88	13.41	13.42	13.18	272	mlm_d_at
3	6.59	0.37	6.23	6.96	6.49	6.95	6.29	272	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_s_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	17.44	1.12	16.32	18.57	17.45	18.56	16.33	110	tef_at
1	42.41	2.59	39.82	45.00	42.41	44.99	39.83	110	mlm_at
2	30.84	1.25	29.59	32.09	30.84	32.08	29.60	110	mlm_d_at
3	13.38	0.55	12.83	13.93	13.38	13.93	12.83	110	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_s_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	16.05	2.55	13.50	18.60	15.62	17.83	14.20	166	tef_at
1	25.14	3.22	21.92	28.35	24.39	27.85	23.05	166	mlm_at
2	20.90	2.45	18.46	23.35	20.60	22.52	19.04	166	mlm_d_at
3	15.17	2.49	12.68	17.66	14.50	16.50	13.32	166	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_lstmatt_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	34.85	5.98	28.86	40.83	34.37	38.78	30.40	75	tef_at
1	59.45	7.30	52.15	66.75	60.83	64.41	52.29	75	mlm_at
2	47.79	5.43	42.37	53.22	47.38	50.82	43.28	75	mlm_d_at
3	31.87	6.03	25.84	37.91	30.31	35.02	27.56	75	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_a_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	11.42	3.69	7.73	15.12	11.21	13.99	9.17	223	tef_at
1	18.43	6.00	12.43	24.43	18.20	22.07	14.50	223	mlm_at
2	15.50	4.92	10.59	20.42	15.88	18.51	12.42	223	mlm_d_at
3	11.90	3.86	8.04	15.76	11.78	14.23	9.41	223	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_a_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	20.35	3.90	16.45	24.25	20.12	23.48	16.95	110	tef_at
1	45.39	7.94	37.45	53.34	44.91	51.02	40.94	110	mlm_at
2	34.35	4.88	29.47	39.23	34.86	36.98	33.72	110	mlm_d_at
3	23.03	5.24	17.79	28.27	23.32	26.75	18.09	110	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_a_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	8.40	1.81	6.59	10.20	8.41	9.40	7.32	236	tef_at
1	25.86	5.05	20.80	30.91	25.73	28.73	22.79	236	mlm_at
2	18.72	3.31	15.41	22.03	18.87	20.72	16.86	236	mlm_d_at
3	8.98	1.91	7.07	10.88	8.95	10.15	7.65	236	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_a_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	17.37	3.53	13.84	20.90	17.58	20.32	14.79	99	tef_at
1	68.95	12.71	56.24	81.66	69.75	79.84	61.59	99	mlm_at
2	47.97	7.66	40.31	55.63	47.00	54.03	45.12	99	mlm_d_at
3	20.41	4.65	15.76	25.06	21.41	24.15	15.91	99	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_a_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	7.94	1.59	6.35	9.53	7.83	8.81	6.82	284	tef_at
1	20.53	3.88	16.65	24.41	20.07	22.81	18.01	284	mlm_at
2	15.18	2.75	12.42	17.93	15.42	16.89	13.43	284	mlm_d_at
3	7.35	1.52	5.83	8.87	7.32	8.53	6.40	284	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_a_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	17.47	3.46	14.00	20.93	17.60	20.44	14.57	99	tef_at
1	68.67	12.22	56.45	80.88	69.64	78.27	60.22	99	mlm_at
2	47.92	7.21	40.71	55.13	48.08	52.13	45.23	99	mlm_d_at
3	20.51	4.52	15.99	25.03	21.61	24.03	15.69	99	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_a_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	11.70	3.82	7.88	15.52	11.79	13.89	9.43	216	tef_at
1	19.09	6.09	12.99	25.18	19.19	23.02	15.14	216	mlm_at
2	15.96	5.09	10.87	21.05	16.21	19.48	12.98	216	mlm_d_at
3	12.16	3.89	8.27	16.06	12.45	14.67	9.51	216	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_a_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	24.57	6.99	17.58	31.57	24.82	28.53	19.31	93	tef_at
1	48.73	13.38	35.35	62.10	52.99	57.47	39.21	93	mlm_at
2	39.73	10.18	29.55	49.90	40.74	47.45	31.71	93	mlm_d_at
3	29.32	9.38	19.94	38.71	29.42	34.11	23.33	93	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_a_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	9.30	1.92	7.38	11.23	9.27	10.95	8.05	274	tef_at
1	16.67	3.23	13.44	19.90	16.31	18.84	14.60	274	mlm_at
2	13.39	2.46	10.93	15.84	13.35	14.89	11.85	274	mlm_d_at
3	9.25	2.02	7.23	11.26	9.12	10.72	7.89	274	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_a_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	20.60	4.33	16.27	24.93	20.86	24.33	17.53	110	tef_at
1	45.90	7.89	38.01	53.78	45.71	50.88	41.60	110	mlm_at
2	35.67	5.47	30.20	41.14	35.63	38.04	32.61	110	mlm_d_at
3	23.45	5.71	17.73	29.16	24.43	26.82	18.51	110	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_ig_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	33.38	8.58	24.80	41.96	32.07	35.64	26.34	76	tef_at
1	47.19	16.81	30.38	63.99	43.36	51.95	40.07	76	mlm_at
2	45.88	19.50	26.38	65.38	41.94	48.55	35.06	76	mlm_d_at
3	35.72	10.52	25.20	46.24	34.08	39.52	29.97	76	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_ig_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	62.18	9.85	52.34	72.03	64.35	70.43	51.92	31	tef_at
1	136.31	40.23	96.09	176.54	124.29	133.83	113.78	31	mlm_at
2	124.36	27.39	96.97	151.75	120.04	154.68	102.44	31	mlm_d_at
3	86.71	16.11	70.60	102.83	77.45	92.37	73.79	31	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_ig_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	33.17	8.59	24.58	41.76	32.43	35.23	26.58	76	tef_at
1	47.08	17.25	29.83	64.33	44.21	49.36	40.22	76	mlm_at
2	45.52	19.24	26.28	64.77	41.27	48.83	35.11	76	mlm_d_at
3	35.46	10.52	24.95	45.98	34.51	39.04	29.69	76	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_ig_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	62.90	11.15	51.74	74.05	68.46	73.48	50.20	27	tef_at
1	140.01	43.08	96.94	183.09	126.70	164.08	114.70	27	mlm_at
2	127.28	31.51	95.77	158.79	133.59	158.12	88.60	27	mlm_d_at
3	88.42	17.57	70.86	105.99	80.64	103.92	73.64	27	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_ig_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	32.88	8.43	24.45	41.31	32.07	34.21	27.07	80	tef_at
1	46.33	16.65	29.68	62.97	43.28	49.08	38.42	80	mlm_at
2	44.97	18.82	26.14	63.79	41.17	46.78	35.77	80	mlm_d_at
3	35.27	10.41	24.86	45.68	34.68	38.50	29.88	80	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_ig_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	61.92	10.06	51.86	71.98	64.41	70.54	54.14	34	tef_at
1	131.76	39.41	92.35	171.16	120.79	141.55	108.06	34	mlm_at
2	121.91	27.28	94.63	149.19	120.29	150.82	109.84	34	mlm_d_at
3	86.99	15.36	71.63	102.34	89.62	92.61	75.91	34	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_ig_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	33.07	8.34	24.73	41.42	32.29	35.32	26.69	76	tef_at
1	46.71	16.75	29.95	63.46	43.34	49.40	39.97	76	mlm_at
2	45.57	19.10	26.47	64.67	41.38	47.80	35.72	76	mlm_d_at
3	35.55	10.56	24.99	46.12	34.13	38.68	29.73	76	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_ig_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	61.60	10.43	51.17	72.03	64.51	70.23	51.01	31	tef_at
1	133.24	40.04	93.20	173.27	120.11	135.60	109.11	31	mlm_at
2	122.40	27.46	94.94	149.85	119.95	152.42	99.51	31	mlm_d_at
3	86.13	15.81	70.32	101.95	77.32	91.36	73.28	31	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_ig_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	33.30	8.39	24.91	41.68	32.73	35.55	26.67	76	tef_at
1	46.74	17.26	29.48	63.99	43.20	49.57	40.08	76	mlm_at
2	45.54	19.39	26.15	64.93	40.98	48.65	34.74	76	mlm_d_at
3	35.73	10.67	25.06	46.40	34.47	38.99	29.76	76	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_ig_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	62.77	10.75	52.02	73.52	65.07	71.44	52.09	31	tef_at
1	133.99	40.54	93.45	174.53	120.21	135.35	110.44	31	mlm_at
2	123.38	28.54	94.83	151.92	119.59	153.29	100.37	31	mlm_d_at
3	87.62	15.94	71.69	103.56	78.60	94.21	74.25	31	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_s_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	15.49	5.37	10.12	20.86	14.55	18.56	11.45	158	tef_at
1	25.57	14.19	11.38	39.77	22.94	27.85	18.42	158	mlm_at
2	22.54	12.75	9.80	35.29	20.42	24.04	16.37	158	mlm_d_at
3	17.00	7.93	9.06	24.93	15.84	18.82	12.99	158	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	31.99	7.86	24.13	39.85	32.46	38.11	26.68	58	tef_at
1	75.52	32.20	43.32	107.72	68.76	89.37	54.71	58	mlm_at
2	73.71	39.57	34.14	113.28	54.04	104.94	47.85	58	mlm_d_at
3	49.56	22.62	26.94	72.18	40.45	68.70	36.28	58	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_s_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	16.52	5.79	10.73	22.31	15.53	20.23	12.35	148	tef_at
1	27.95	17.21	10.74	45.17	24.91	31.19	19.58	148	mlm_at
2	23.96	13.11	10.85	37.06	21.36	26.60	18.27	148	mlm_d_at
3	18.25	8.86	9.40	27.11	17.01	19.45	13.96	148	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	33.30	7.97	25.33	41.27	33.38	37.24	28.70	56	tef_at
1	78.80	32.30	46.50	111.10	71.69	89.28	55.60	56	mlm_at
2	77.05	43.19	33.85	120.24	56.00	107.06	47.92	56	mlm_d_at
3	51.16	22.33	28.82	73.49	44.05	68.52	36.75	56	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_s_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	13.33	3.42	9.91	16.75	12.99	14.84	11.25	186	tef_at
1	25.21	11.92	13.29	37.14	21.09	27.01	18.52	186	mlm_at
2	20.81	8.86	11.95	29.66	17.81	19.93	16.25	186	mlm_d_at
3	14.18	3.79	10.39	17.96	13.42	15.91	11.66	186	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	27.52	4.41	23.11	31.94	28.21	31.11	23.72	65	tef_at
1	87.67	29.92	57.75	117.59	85.48	113.07	69.75	65	mlm_at
2	68.15	27.52	40.64	95.67	55.92	92.32	45.73	65	mlm_d_at
3	41.89	12.40	29.49	54.30	42.21	50.54	33.07	65	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_s_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	16.32	5.96	10.36	22.28	15.53	19.91	11.83	148	tef_at
1	27.06	15.63	11.43	42.68	25.02	28.98	18.94	148	mlm_at
2	23.58	13.31	10.27	36.90	21.11	25.71	17.42	148	mlm_d_at
3	18.14	8.92	9.22	27.06	16.88	19.36	14.07	148	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_s_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	32.21	7.74	24.47	39.95	31.64	37.79	27.44	56	tef_at
1	78.17	34.85	43.32	113.02	70.62	88.57	54.03	56	mlm_at
2	75.72	40.65	35.07	116.37	57.00	106.30	48.49	56	mlm_d_at
3	49.92	22.07	27.85	71.98	40.97	68.96	35.79	56	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_s_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	14.88	5.11	9.77	19.99	14.46	17.41	10.98	168	tef_at
1	24.51	13.59	10.92	38.10	22.45	26.29	17.84	168	mlm_at
2	21.38	11.69	9.69	33.07	19.57	22.91	15.72	168	mlm_d_at
3	16.40	7.59	8.82	23.99	15.64	18.21	12.70	168	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_roberta_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	29.85	6.90	22.95	36.75	29.74	35.79	26.05	64	tef_at
1	71.52	30.36	41.16	101.88	65.16	84.71	49.50	64	mlm_at
2	66.96	35.50	31.46	102.46	49.94	94.80	45.02	64	mlm_d_at
3	45.39	20.19	25.20	65.58	38.86	60.11	33.95	64	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_a_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	25.30	8.67	16.63	33.97	21.86	30.87	19.27	67	tef_at
1	79.20	44.79	34.42	123.99	87.86	119.40	30.59	67	mlm_at
2	52.90	31.89	21.00	84.79	42.64	79.21	30.34	67	mlm_d_at
3	42.97	23.34	19.63	66.32	34.54	64.99	22.23	67	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_a_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	35.50	8.69	26.81	44.19	37.79	42.33	28.75	45	tef_at
1	114.79	38.43	76.37	153.22	112.71	140.78	91.66	45	mlm_at
2	89.03	35.96	53.08	124.99	96.36	112.34	50.88	45	mlm_d_at
3	66.61	25.18	41.43	91.79	70.56	83.28	42.90	45	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_a_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	27.20	9.23	17.97	36.43	27.62	31.55	20.23	63	tef_at
1	83.08	48.14	34.94	131.21	105.12	127.13	31.12	63	mlm_at
2	54.45	35.84	18.61	90.29	40.86	70.87	30.63	63	mlm_d_at
3	45.95	27.38	18.57	73.33	35.40	68.64	24.53	63	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_a_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	33.69	8.14	25.55	41.83	36.71	39.98	28.31	45	tef_at
1	110.71	37.45	73.26	148.16	113.48	137.41	83.66	45	mlm_at
2	85.97	35.71	50.25	121.68	92.29	108.75	49.94	45	mlm_d_at
3	63.54	24.48	39.06	88.02	63.68	76.91	43.38	45	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_a_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	25.67	8.94	16.73	34.61	22.24	31.20	19.27	69	tef_at
1	80.33	45.19	35.14	125.52	87.99	122.31	30.62	69	mlm_at
2	54.25	33.01	21.24	87.27	42.93	78.61	31.51	69	mlm_d_at
3	44.37	24.76	19.61	69.13	35.09	66.33	22.02	69	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_a_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	35.92	8.66	27.26	44.58	37.34	43.15	28.74	44	tef_at
1	120.64	39.07	81.58	159.71	122.72	149.69	100.14	44	mlm_at
2	94.45	38.89	55.56	133.34	102.16	118.88	53.92	44	mlm_d_at
3	68.85	26.07	42.77	94.92	71.12	83.54	44.94	44	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_a_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	27.29	9.48	17.81	36.77	27.52	32.71	19.93	63	tef_at
1	84.94	49.69	35.25	134.64	107.74	130.55	30.85	63	mlm_at
2	55.70	35.67	20.03	91.37	40.35	78.69	32.31	63	mlm_d_at
3	45.42	25.58	19.84	71.00	35.56	69.59	23.62	63	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_a_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	33.33	8.02	25.32	41.35	35.20	39.17	28.09	47	tef_at
1	109.46	35.64	73.82	145.11	113.59	136.06	82.98	47	mlm_at
2	85.08	33.54	51.54	118.62	93.98	108.63	50.32	47	mlm_d_at
3	62.83	23.07	39.76	85.90	65.29	77.90	40.89	47	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_a_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	28.31	10.21	18.11	38.52	27.58	35.42	19.81	63	tef_at
1	86.31	50.02	36.29	136.33	109.22	128.64	32.09	63	mlm_at
2	56.16	35.07	21.09	91.23	42.04	82.25	31.15	63	mlm_d_at
3	47.28	26.40	20.88	73.68	36.86	70.71	24.74	63	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_a_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	37.00	8.78	28.21	45.78	39.66	43.75	31.02	42	tef_at
1	125.28	41.35	83.93	166.63	129.82	158.15	95.50	42	mlm_at
2	97.48	40.36	57.12	137.83	103.73	125.73	57.16	42	mlm_d_at
3	71.42	28.23	43.18	99.65	74.90	88.15	46.16	42	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_ig_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	47.13	13.58	33.54	60.71	43.95	51.14	37.52	40	tef_at
1	95.38	62.10	33.29	157.48	68.43	117.94	59.51	40	mlm_at
2	80.60	53.83	26.77	134.42	60.65	79.28	52.16	40	mlm_d_at
3	69.68	38.21	31.47	107.89	57.50	74.08	49.50	40	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_ig_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	50.46	13.92	36.54	64.38	47.89	59.91	40.11	38	tef_at
1	104.87	67.32	37.55	172.18	73.35	131.95	62.84	38	mlm_at
2	87.80	57.73	30.08	145.53	66.31	87.32	55.20	38	mlm_d_at
3	74.91	40.34	34.57	115.25	62.01	77.37	53.21	38	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_ig_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	48.65	13.89	34.76	62.53	45.76	52.77	38.79	40	tef_at
1	100.49	66.56	33.93	167.05	71.30	122.82	62.67	40	mlm_at
2	84.29	56.93	27.37	141.22	63.14	83.08	54.69	40	mlm_d_at
3	71.97	39.53	32.44	111.50	59.16	76.44	50.66	40	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_ig_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	48.23	13.99	34.24	62.22	44.70	52.46	38.17	40	tef_at
1	97.11	63.21	33.91	160.32	70.33	117.35	60.09	40	mlm_at
2	82.29	54.82	27.47	137.11	61.65	82.36	53.62	40	mlm_d_at
3	71.29	39.08	32.20	110.37	58.76	76.33	50.64	40	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_ig_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	47.59	13.31	34.29	60.90	45.77	53.65	37.88	42	tef_at
1	102.94	69.82	33.12	172.75	68.92	125.16	59.95	42	mlm_at
2	80.06	52.62	27.44	132.68	62.50	77.93	52.84	42	mlm_d_at
3	69.69	37.39	32.30	107.08	59.91	74.08	50.15	42	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_s_16_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	20.91	7.21	13.70	28.12	19.84	23.68	16.91	87	tef_at
1	53.20	40.12	13.08	93.32	33.95	68.18	25.50	87	mlm_at
2	39.23	28.18	11.06	67.41	29.63	43.24	22.13	87	mlm_d_at
3	34.77	19.08	15.69	53.85	27.80	45.82	19.56	87	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_s_16_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	39.22	8.73	30.49	47.95	41.02	45.89	31.20	40	tef_at
1	124.66	50.07	74.59	174.73	136.12	165.65	78.63	40	mlm_at
2	87.53	31.80	55.73	119.33	83.17	117.65	63.83	40	mlm_d_at
3	77.84	35.50	42.34	113.34	74.64	105.34	44.68	40	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_s_32_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	21.95	7.77	14.18	29.72	20.35	24.41	17.45	79	tef_at
1	56.55	43.93	12.62	100.49	35.47	68.48	24.45	79	mlm_at
2	40.96	30.11	10.85	71.07	29.62	46.40	23.56	79	mlm_d_at
3	35.95	19.70	16.25	55.66	29.01	49.11	19.87	79	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_s_32_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	40.97	8.58	32.39	49.54	42.97	45.91	40.30	38	tef_at
1	133.04	53.56	79.48	186.60	145.96	176.63	77.60	38	mlm_at
2	90.85	34.04	56.81	124.88	83.52	124.64	64.74	38	mlm_d_at
3	81.85	36.72	45.13	118.57	78.45	110.46	47.61	38	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_s_4_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	22.33	7.72	14.61	30.05	20.05	25.38	17.67	81	tef_at
1	58.89	45.13	13.75	104.02	41.62	90.10	24.87	81	mlm_at
2	43.81	33.09	10.72	76.89	31.53	49.05	22.59	81	mlm_d_at
3	38.28	21.88	16.40	60.16	30.62	55.07	20.74	81	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_s_4_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	40.10	9.27	30.83	49.37	43.48	48.29	31.08	40	tef_at
1	127.85	51.87	75.98	179.72	138.66	169.71	79.08	40	mlm_at
2	88.60	32.15	56.46	120.75	85.31	117.10	63.25	40	mlm_d_at
3	79.14	35.83	43.31	114.97	79.02	105.65	45.38	40	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_s_64_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	21.18	7.43	13.75	28.61	19.29	24.05	16.74	81	tef_at
1	55.94	43.24	12.70	99.19	39.00	84.18	23.12	81	mlm_at
2	40.76	30.08	10.68	70.84	28.36	47.28	21.79	81	mlm_d_at
3	35.81	20.13	15.68	55.94	28.14	48.91	19.27	81	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_s_64_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	43.13	8.96	34.17	52.08	44.21	50.39	41.00	35	tef_at
1	137.86	56.04	81.81	193.90	146.49	183.26	87.14	35	mlm_at
2	90.78	35.00	55.78	125.78	83.38	121.65	65.35	35	mlm_d_at
3	82.20	37.15	45.05	119.35	79.93	109.36	48.91	35	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_s_8_0.1.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	21.99	7.61	14.38	29.60	20.41	26.22	17.26	83	tef_at
1	58.02	43.15	14.87	101.18	41.74	79.97	25.72	83	mlm_at
2	42.53	31.35	11.18	73.88	31.52	48.91	23.50	83	mlm_d_at
3	37.05	20.93	16.12	57.98	29.32	50.59	19.66	83	mlm_d_fast_at


==> data/mlm_plots/timing_data/imdb_xlnet_s_8_0.25.tex <==
x	mean	std	mms	mps	median	lq	uq	count	attack_name
0	42.33	8.66	33.67	50.99	43.25	47.84	41.23	38	tef_at
1	137.01	55.49	81.52	192.50	142.55	182.98	80.88	38	mlm_at
2	93.07	35.54	57.53	128.61	85.49	128.56	65.27	38	mlm_d_at
3	84.78	38.48	46.30	123.26	85.84	112.12	49.00	38	mlm_d_fast_at


==> figures/accuracies.tex <==
% Modify separation space of tabs
%\addtolength{\tabcolsep}{-2pt}
\begin{table*}[h!]
\centering\small
\begin{tabular}{c|cccccc}
\hline
\textsc{\textbf{Dataset}}   & \textsc{CNN}     & \textsc{LSTM}    & \textsc{LSTMAtt}   & \textsc{BERT}      & \textsc{RoBERTa}   & \textsc{XLNet} \\\hline\hline
\textsc{AG's News}          & 89.7\%  & 90.8\%  & 91.4\%    & 94.2\%    & 94.0\%    & 93.8\%    \\
\textsc{MR}                 & 73.0\%  & 76.4\%  & 78.0\%    & 82.2\%    & 87.7\%    & 86.3\%    \\
\textsc{IMDB}               & 82.0\%  & 87.2\%  & 87.3\%    & 89.4\%    & 93.3\%    & 93.7\%    \\
\textsc{Yelp}               & 49.0\%  & 54.8\%  & 60.0\%    & 62.6\%    & 67.6\%    & -         \\
\textsc{Fake News}          & 98.9\%  & 99.6\%  & 99.6\%    & 99.8\%    & 100.0\%   & 100.0\%   \\\hline
\end{tabular}
\caption{Classifier accuracies}\label{tbl:accuracies}
\end{table*}
%\addtolength{\tabcolsep}{2pt}

==> figures/architecture_specs.tex <==
\begin{table*}[h]
\scriptsize\centering
\begin{tabular}{c|c|c|c|c|c|c}
\hline
                                  &                 & \textbf{AG's News} & \textbf{MR}       & \textbf{IMDB}     & \textbf{Yelp}       & \textbf{Fake News} \\\hline\hline
\multirow{6}{*}{\textbf{CNN}}     & Input shape     & (64, 300)          & (32,300)          & (256, 300)        & (256, 300)          & (512, 300)         \\
                                  & Num. classes    & 4                  & 2                 & 2                 & 5                   & 2                  \\
                                  & Filter sizes    & {[}3, 5, 7{]}      & {[}3, 5{]}        & {[}3, 5, 7{]}     & {[}3, 5, 7{]}       & {[}3, 5, 7{]}      \\
                                  & Feature sizes   & {[}8, 8, 8{]}      & {[}8, 8{]}        & {[}16, 16, 16{]}  & {[}128, 128, 128{]} & {[}32, 32, 32{]}   \\
                                  & Pooling sizes   & {[}2, 2, 2{]}      & {[}2, 2{]}        & {[}2, 2, 2{]}     & {[}2, 2, 2{]}       & {[}2, 2, 2{]}      \\
                                  & Lin. layer dim. & 8                  & 8                 & 16                & 64                  & 32                 \\
                                  & Num. params     & 67748              & 27946             & 567458            & 16428293            & 4091714            \\\hline
\multirow{6}{*}{\textbf{LSTM}}    & Input shape     & (64, 300)          & (32,300)          & (256, 300)        & (256, 300)          & (512, 300)         \\
                                  & Num. classes    & 4                  & 2                 & 2                 & 5                   & 2                  \\
                                  & Hidden dim.     & 8                  & 8                 & 16                & 256                 & 16                 \\
                                  & Num. layers     & 1                  & 1                 & 2                 & 2                   & 1                  \\
                                  & Pooling sizes   & 2                  & 2                 & 1                 & 2                   & 2                  \\
                                  & Lin. layer dim. & 8                  & 8                 & 16                & 32                  & 16                 \\
                                  & Num. params     & 10988              & 10458             & 18162             & 2146693             & 85986              \\\hline
\multirow{5}{*}{\textbf{LSTMAtt}} & Input shape     & (64, 300)          & (32,300)          & (256, 300)        & (256, 300)          & (512, 300)         \\
                                  & Num. classes    & 4                  & 2                 & 2                 & 5                   & 2                  \\
                                  & Hidden dim.     & 8                  & 8                 & 16                & 256                 & 16                 \\
                                  & Num. layers     & 4                  & 1                 & 2                 & 2                   & 1                  \\
                                  & Lin. layer dim. & 8                  & 8                 & 16                & 32                  & 16                 \\
                                  & Num. params     & 25004              & 19994             & 47666             & 2752901             & 41826              \\\hline
\multirow{3}{*}{\textbf{BERT}}    & Input shape     & (64,)              & (32,)             & (256,)            & (256,)              & (512,)             \\
                                  & Num. classes    & 4                  & 2                 & 2                 & 5                   & 2                  \\
                                  & Model ID        & bert-base-uncased  & bert-base-uncased & bert-base-uncased & bert-base-uncased   & bert-base-uncased  \\
                                  & Num. params     & 109485316          & 109483778         & 109483778         & 109486085           & 109483778          \\\hline
\multirow{3}{*}{\textbf{RoBERTa}} & Input shape     & (64,)              & (32,)             & (256,)            & (256,)              & (512,)             \\
                                  & Num. classes    & 4                  & 2                 & 2                 & 5                   & 2                  \\
                                  & Model ID        & roberta-base       & roberta-base      & roberta-base      & roberta-base        & roberta-base       \\
                                  & Num. params     & 124648708          & 124647170         & 124647170         & 124649477           & 124647170          \\\hline
\multirow{3}{*}{\textbf{XLNet}}   & Input shape     & (64,)              & (32,)             & (256,)            & (256,)              & (512,)             \\
                                  & Num. classes    & 4                  & 2                 & 2                 & 5                   & 2                  \\
                                  & Model ID        & xlnet-base-cased   & xlnet-base-cased  & xlnet-base-cased  & xlnet-base-cased    & xlnet-base-cased   \\
                                  & Num. params     & 117312004          & 117310466         & 117310466         & 117312773           & 117310466          \\\hline\hline
\end{tabular}
\caption{Model specifications}\label{tbl:archspecs}
\end{table*}
